Compact Proofs of Model Performance via Mechanistic Interpretability

We propose using mechanistic interpretability -- techniques for reverse engineering model weights into human-interpretable algorithms -- to derive and compactly prove formal guarantees on model performance. We prototype this approach by formally proving accuracy lower bounds for a small transformer trained on Max-of-K, validating proof transferability across 151 random seeds and four values of K. We create 102 different computer-assisted proof strategies and assess their length and tightness of bound on each of our models. Using quantitative metrics, we find that shorter proofs seem to require and provide more mechanistic understanding. Moreover, we find that more faithful mechanistic understanding leads to tighter performance bounds. We confirm these connections by qualitatively examining a subset of our proofs. Finally, we identify compounding structureless errors as a key challenge for using mechanistic interpretability to generate compact proofs on model performance.

==> advice-tikz.code.tex <==
%%
%% This is file `advice-tikz.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% advice.dtx  (with options: `tikz')
%% 
%% This file is a part of Advice, a TeX package implementing a generic
%% framework for extending the functionality of selected commands and
%% environments, available at https://ctan.org/pkg/advice and
%% https://github.com/sasozivanovic/advice.
%%
%% Copyright (c) 2023- Saso Zivanovic <saso.zivanovic@guest.arnes.si>
%%                     (Sa\v{s}o \v{Z}ivanovi\'{c})
%%
%% This work may be distributed and/or modified under the conditions of the
%% LaTeX Project Public License, either version 1.3c of this license or (at
%% your option) any later version.
% The latest version of this license is in
%% https://www.latex-project.org/lppl.txt and version 1.3c or later is part of
%% all distributions of LaTeX version 2008 or later.
%%
%% This work has the LPPL maintenance status `maintained'.
%% The Current Maintainer of this work is Saso Zivanovic.
%%
%% The files belonging to this work and covered by LPPL are listed in
%% (<texmf>/doc/generic/advice/)FILES.
\edef\adviceresetatcatcode{\catcode`\noexpand\@\the\catcode`\@\relax}%
\catcode`\@=11
\def\AdviceCollectTikZArguments{%
  \toks0={}%
  \advice@tikz@anim
}
\def\advice@tikz@anim{%
  \pgfutil@ifnextchar[{\advice@tikz@opt}{%
      \pgfutil@ifnextchar:{\advice@tikz@anim@a}{%
        \advice@tikz@code}}%]
}
\def\advice@tikz@anim@a#1=#2{%
  \toksapp0{#1={#2}}%
  \advice@tikz@anim
}
\def\advice@tikz@opt[#1]{%
  \toksapp0{[#1]}%
  \advice@tikz@code
}
\def\advice@tikz@code{%
  \pgfutil@ifnextchar\bgroup\advice@tikz@braced\advice@tikz@single
}
\long\def\advice@tikz@braced#1{\toksapp0{{#1}}\advice@tikz@done}
\def\advice@tikz@single#1;{\toksapp0{#1;}\advice@tikz@done}
\def\advice@tikz@done{%
  \expandafter\AdviceInnerHandler\expandafter{\the\toks0}%
}
\adviceresetatcatcode
\endinput
%%
%% End of file `advice-tikz.code.tex'.


==> generated/max-of-10-all-models/adjusted-figures/NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-mmzstorehash.tex <==
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-000.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-001.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-002.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-003.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-004.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-005.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-006.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-007.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-008.dat.md5}


==> generated/max-of-10-all-models/adjusted-figures/NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables.tex <==
% This file was created with tikzplotlib v0.10.1.post9.
\begin{tikzpicture}

\definecolor{crimson2272628}{RGB}{227,26,28}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange2551270}{RGB}{255,127,0}
\definecolor{darkslateblue10661154}{RGB}{106,61,154}
\definecolor{forestgreen5116044}{RGB}{51,160,44}
\definecolor{khaki255255153}{RGB}{255,255,153}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightsalmon251154153}{RGB}{251,154,153}
\definecolor{sandybrown253191111}{RGB}{253,191,111}
\definecolor{sienna1778940}{RGB}{177,89,40}
\definecolor{thistle202178214}{RGB}{202,178,214}

\begin{axis}[legend pos=outer north east,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
%
  legend pos=outer north east,
  draw=lightgray204,
  mark options={mark size=3}
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={EPQKE Singular Ratio: \(\displaystyle \sigma_1 / \sigma_2\)},
xmin=357.824690246582, xmax=1804.304246521,
xtick style={color=black},
xtick={200,400,600,800,1000,1200,1400,1600,1800,2000},
xticklabels={
  \(\displaystyle {200}\),
  \(\displaystyle {400}\),
  \(\displaystyle {600}\),
  \(\displaystyle {800}\),
  \(\displaystyle {1000}\),
  \(\displaystyle {1200}\),
  \(\displaystyle {1400}\),
  \(\displaystyle {1600}\),
  \(\displaystyle {1800}\),
  \(\displaystyle {2000}\)
},
y grid style={darkgray176},
ylabel={Normalized Accuracy Bound},
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={
  \(\displaystyle {0.0}\),
  \(\displaystyle {0.2}\),
  \(\displaystyle {0.4}\),
  \(\displaystyle {0.6}\),
  \(\displaystyle {0.8}\),
  \(\displaystyle {1.0}\)
}
]
\addplot [draw=sienna1778940, fill=sienna1778940, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-000.dat};
\addlegendentry{max-diff-exact}
\addplot [draw=khaki255255153, fill=khaki255255153, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-001.dat};
\addlegendentry{max-diff-subproduct}
\addplot [
  draw=darkslateblue10661154,
  fill=darkslateblue10661154,
  mark size=3pt,
  mark=*,
  only marks
]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-002.dat};
\addlegendentry{mean+max-diff-subproduct}
\addplot [draw=thistle202178214, fill=thistle202178214, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-003.dat};
\addlegendentry{max-diff}
\addplot [draw=darkorange2551270, fill=darkorange2551270, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-004.dat};
\addlegendentry{mean+max-diff}
\addplot [draw=sandybrown253191111, fill=sandybrown253191111, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-005.dat};
\addlegendentry{svd}
\addplot [draw=crimson2272628, fill=crimson2272628, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-006.dat};
\addlegendentry{max-diff-subproduct-recursive}
\addplot [draw=lightsalmon251154153, fill=lightsalmon251154153, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-007.dat};
\addlegendentry{mean+max-diff-subproduct-recursive}
\addplot [draw=forestgreen5116044, fill=forestgreen5116044, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-008.dat};
\addlegendentry{mean-recursive+max-diff-subproduct-recursive}
\end{axis}

\end{tikzpicture}


==> generated/max-of-10-all-models/adjusted-figures/NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-mmzstorehash.tex <==
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-000-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-001-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-002-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-003-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-004-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-005-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-006-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-007-adjusted-2.dat.md5}


==> generated/max-of-10-all-models/adjusted-figures/NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables.tex <==
% This file was created with tikzplotlib v0.10.1.post9.
\begin{tikzpicture}

\definecolor{crimson2272628}{RGB}{227,26,28}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange2551270}{RGB}{255,127,0}
\definecolor{forestgreen5116044}{RGB}{51,160,44}
\definecolor{lightblue166206227}{RGB}{166,206,227}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightgreen178223138}{RGB}{178,223,138}
\definecolor{lightsalmon251154153}{RGB}{251,154,153}
\definecolor{sandybrown253191111}{RGB}{253,191,111}
\definecolor{steelblue31120180}{RGB}{31,120,180}

\begin{axis}[legend pos=outer north east,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  draw=lightgray204,
  mark options={mark size=3}
},
log basis x={2},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={FLOPs to Verify Proof (approximate)},
xmin=609977.773318622, xmax=5.63211318585811e+26,
xmode=log,
xtick style={color=black},
xtick={32,524288,8589934592,140737488355328,2.30584300921369e+18,3.77789318629572e+22,6.1897001964269e+26,1.01412048018258e+31},
xticklabels={
  \(\displaystyle {2^{5}}\),
  \(\displaystyle {2^{19}}\),
  \(\displaystyle {2^{33}}\),
  \(\displaystyle {2^{47}}\),
  \(\displaystyle {2^{61}}\),
  \(\displaystyle {2^{75}}\),
  \(\displaystyle {2^{89}}\),
  \(\displaystyle {2^{103}}\)
},
y grid style={darkgray176},
ylabel={Normalized Accuracy Bound},
ymin=-0.05, ymax=1.05,
ytick style={color=black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
yticklabels={
  \(\displaystyle {\ensuremath{-}0.2}\),
  \(\displaystyle {0.0}\),
  \(\displaystyle {0.2}\),
  \(\displaystyle {0.4}\),
  \(\displaystyle {0.6}\),
  \(\displaystyle {0.8}\),
  \(\displaystyle {1.0}\),
  \(\displaystyle {1.2}\)
}
]
\addplot [draw=lightblue166206227, fill=lightblue166206227, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-000-adjusted-2.dat};
\addlegendentry{brute force (estimated) (acc: 0.9988 ± 0.0013)}
\addplot [draw=steelblue31120180, fill=steelblue31120180, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-001-adjusted-2.dat};
\addlegendentry{cubic (rel acc: 0.915 ± 0.021)}
\addplot [draw=lightgreen178223138, fill=lightgreen178223138, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-002-adjusted-2.dat};
\addlegendentry{subcubic (rel acc: 0.673 ± 0.030)}
\addplot [draw=forestgreen5116044, fill=forestgreen5116044, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-003-adjusted-2.dat};
\addlegendentry{direct-quadratic (rel acc: 0.640 ± 0.032)}
\addplot [draw=lightsalmon251154153, fill=lightsalmon251154153, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-004-adjusted-2.dat};
\addlegendentry{attention-\(\displaystyle \dvocab \dmodel ^2\) (rel acc: 0.658 ± 0.028)}
\addplot [draw=crimson2272628, fill=crimson2272628, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-005-adjusted-2.dat};
\addlegendentry{attention-\(\displaystyle \dvocab \dmodel ^2\), direct-quadratic (rel acc: 0.626 ± 0.031)}
\addplot [draw=sandybrown253191111, fill=sandybrown253191111, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-006-adjusted-2.dat};
\addlegendentry{attention-quadratic (rel acc: 0.393 ± 0.030)}
\addplot [draw=darkorange2551270, fill=darkorange2551270, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-007-adjusted-2.dat};
\addlegendentry{attention-quadratic, direct-quadratic (rel acc: 0.391 ± 0.028)}
\end{axis}

\end{tikzpicture}


==> generated/max-of-10-all-models/adjusted-figures/NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-mmzstorehash.tex <==
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-000-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-001-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-002-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-003-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-004-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-005-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-006-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-007-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-008-adjusted-2.dat.md5}


==> generated/max-of-10-all-models/adjusted-figures/NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables.tex <==
% This file was created with tikzplotlib v0.10.1.post13.
\begin{tikzpicture}

\definecolor{crimson2272628}{RGB}{227,26,28}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange2551270}{RGB}{255,127,0}
\definecolor{forestgreen5116044}{RGB}{51,160,44}
\definecolor{lightblue166206227}{RGB}{166,206,227}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightgreen178223138}{RGB}{178,223,138}
\definecolor{lightsalmon251154153}{RGB}{251,154,153}
\definecolor{orange}{RGB}{255,165,0}
\definecolor{sandybrown253191111}{RGB}{253,191,111}
\definecolor{steelblue31120180}{RGB}{31,120,180}

\begin{axis}[legend pos=outer north east,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
%
  legend pos=outer north east,
  draw=lightgray204,
  mark options={mark size=3}
},
log basis x={2},
tick align=outside,
tick pos=left,
unbounded coords=jump,
x grid style={darkgray176},
xlabel={FLOPs to Verify Proof (approximate)},
xmin=609977.773318622, xmax=5.63211318585811e+26,
xmode=log,
xtick style={color=black},
xtick={0.0625,524288,4398046511104,3.68934881474191e+19,3.09485009821345e+26,2.59614842926741e+33,2.17780714829401e+40},
xticklabels={
  \(\displaystyle {2^{-4}}\),
  \(\displaystyle {2^{19}}\),
  \(\displaystyle {2^{42}}\),
  \(\displaystyle {2^{65}}\),
  \(\displaystyle {2^{88}}\),
  \(\displaystyle {2^{111}}\),
  \(\displaystyle {2^{134}}\)
},
y grid style={darkgray176},
ylabel={Normalized Accuracy Bound},
ymin=-0.05, ymax=1.05,
ytick style={color=black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
yticklabels={
  \(\displaystyle {\ensuremath{-}0.2}\),
  \(\displaystyle {0.0}\),
  \(\displaystyle {0.2}\),
  \(\displaystyle {0.4}\),
  \(\displaystyle {0.6}\),
  \(\displaystyle {0.8}\),
  \(\displaystyle {1.0}\),
  \(\displaystyle {1.2}\)
}
]
\addplot [draw=lightblue166206227, fill=lightblue166206227, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-000-adjusted-2.dat};
\addlegendentry{brute force (estimated) (acc: 0.9988 ± 0.0013)}
\addplot [draw=steelblue31120180, fill=steelblue31120180, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-001-adjusted-2.dat};
\addlegendentry{cubic (rel acc: 0.915 ± 0.021)}
\addplot [draw=lightgreen178223138, fill=lightgreen178223138, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-002-adjusted-2.dat};
\addlegendentry{subcubic (rel acc: 0.673 ± 0.030)}
\addplot [draw=forestgreen5116044, fill=forestgreen5116044, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-003-adjusted-2.dat};
\addlegendentry{direct-quadratic (rel acc: 0.640 ± 0.032)}
\addplot [draw=lightsalmon251154153, fill=lightsalmon251154153, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-004-adjusted-2.dat};
\addlegendentry{attention-\(\displaystyle \dvocab \dmodel ^2\) (rel acc: 0.658 ± 0.028)}
\addplot [draw=crimson2272628, fill=crimson2272628, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-005-adjusted-2.dat};
\addlegendentry{attention-\(\displaystyle \dvocab \dmodel ^2\), direct-quadratic (rel acc: 0.626 ± 0.031)}
\addplot [draw=sandybrown253191111, fill=sandybrown253191111, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-006-adjusted-2.dat};
\addlegendentry{attention-quadratic (rel acc: 0.393 ± 0.030)}
\addplot [draw=darkorange2551270, fill=darkorange2551270, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-007-adjusted-2.dat};
\addlegendentry{attention-quadratic, direct-quadratic (rel acc: 0.391 ± 0.028)}
\addplot [thick, orange, dashed]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-008-adjusted-2.dat};
\addlegendentry{brute-force linear baseline}
\end{axis}

\end{tikzpicture}


==> generated/max-of-10-dvocab-128-all-models/adjusted-figures/NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-mmzstorehash.tex <==
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-000.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-001.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-002.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-003.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-004.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-005.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-006.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-007.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-008.dat.md5}


==> generated/max-of-10-dvocab-128-all-models/adjusted-figures/NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables.tex <==
% This file was created with tikzplotlib v0.10.1.post9.
\begin{tikzpicture}

\definecolor{crimson2272628}{RGB}{227,26,28}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange2551270}{RGB}{255,127,0}
\definecolor{darkslateblue10661154}{RGB}{106,61,154}
\definecolor{forestgreen5116044}{RGB}{51,160,44}
\definecolor{khaki255255153}{RGB}{255,255,153}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightsalmon251154153}{RGB}{251,154,153}
\definecolor{sandybrown253191111}{RGB}{253,191,111}
\definecolor{sienna1778940}{RGB}{177,89,40}
\definecolor{thistle202178214}{RGB}{202,178,214}

\begin{axis}[legend pos=outer north east,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
%
  legend pos=outer north east,
  draw=lightgray204,
  mark options={mark size=3}
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={EPQKE Singular Ratio: \(\displaystyle \sigma_1 / \sigma_2\)},
xmin=657.487899780273, xmax=2139.86848449707,
xtick style={color=black},
xtick={600,800,1000,1200,1400,1600,1800,2000,2200},
xticklabels={
  \(\displaystyle {600}\),
  \(\displaystyle {800}\),
  \(\displaystyle {1000}\),
  \(\displaystyle {1200}\),
  \(\displaystyle {1400}\),
  \(\displaystyle {1600}\),
  \(\displaystyle {1800}\),
  \(\displaystyle {2000}\),
  \(\displaystyle {2200}\)
},
y grid style={darkgray176},
ylabel={Normalized Accuracy Bound},
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={
  \(\displaystyle {0.0}\),
  \(\displaystyle {0.2}\),
  \(\displaystyle {0.4}\),
  \(\displaystyle {0.6}\),
  \(\displaystyle {0.8}\),
  \(\displaystyle {1.0}\)
}
]
\addplot [draw=sienna1778940, fill=sienna1778940, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-000.dat};
\addlegendentry{max-diff-exact}
\addplot [draw=khaki255255153, fill=khaki255255153, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-001.dat};
\addlegendentry{max-diff-subproduct}
\addplot [
  draw=darkslateblue10661154,
  fill=darkslateblue10661154,
  mark size=3pt,
  mark=*,
  only marks
]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-002.dat};
\addlegendentry{mean+max-diff-subproduct}
\addplot [draw=thistle202178214, fill=thistle202178214, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-003.dat};
\addlegendentry{max-diff}
\addplot [draw=darkorange2551270, fill=darkorange2551270, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-004.dat};
\addlegendentry{mean+max-diff}
\addplot [draw=sandybrown253191111, fill=sandybrown253191111, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-005.dat};
\addlegendentry{svd}
\addplot [draw=crimson2272628, fill=crimson2272628, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-006.dat};
\addlegendentry{max-diff-subproduct-recursive}
\addplot [draw=lightsalmon251154153, fill=lightsalmon251154153, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-007.dat};
\addlegendentry{mean-recursive+max-diff-subproduct-recursive}
\addplot [draw=forestgreen5116044, fill=forestgreen5116044, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-008.dat};
\addlegendentry{mean+max-diff-subproduct-recursive}
\end{axis}

\end{tikzpicture}


==> generated/max-of-10-dvocab-128-all-models/adjusted-figures/NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-mmzstorehash.tex <==
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-000-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-001-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-002-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-003-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-004-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-005-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-006-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-007-adjusted-2.dat.md5}


==> generated/max-of-10-dvocab-128-all-models/adjusted-figures/NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables.tex <==
% This file was created with tikzplotlib v0.10.1.post9.
\begin{tikzpicture}

\definecolor{crimson2272628}{RGB}{227,26,28}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange2551270}{RGB}{255,127,0}
\definecolor{forestgreen5116044}{RGB}{51,160,44}
\definecolor{lightblue166206227}{RGB}{166,206,227}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightgreen178223138}{RGB}{178,223,138}
\definecolor{lightsalmon251154153}{RGB}{251,154,153}
\definecolor{sandybrown253191111}{RGB}{253,191,111}
\definecolor{steelblue31120180}{RGB}{31,120,180}

\begin{axis}[legend pos=outer north east,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  draw=lightgray204,
  mark options={mark size=3}
},
log basis x={2},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={FLOPs to Verify Proof (approximate)},
xmin=1722224.47948847, xmax=7.64185592528163e+29,
xmode=log,
xtick style={color=black},
xtick={16,1048576,68719476736,4.5035996273705e+15,2.95147905179353e+20,1.93428131138341e+25,1.26765060022823e+30,8.30767497365572e+34},
xticklabels={
  \(\displaystyle {2^{4}}\),
  \(\displaystyle {2^{20}}\),
  \(\displaystyle {2^{36}}\),
  \(\displaystyle {2^{52}}\),
  \(\displaystyle {2^{68}}\),
  \(\displaystyle {2^{84}}\),
  \(\displaystyle {2^{100}}\),
  \(\displaystyle {2^{116}}\)
},
y grid style={darkgray176},
ylabel={Normalized Accuracy Bound},
ymin=-0.05, ymax=1.05,
ytick style={color=black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
yticklabels={
  \(\displaystyle {\ensuremath{-}0.2}\),
  \(\displaystyle {0.0}\),
  \(\displaystyle {0.2}\),
  \(\displaystyle {0.4}\),
  \(\displaystyle {0.6}\),
  \(\displaystyle {0.8}\),
  \(\displaystyle {1.0}\),
  \(\displaystyle {1.2}\)
}
]
\addplot [draw=lightblue166206227, fill=lightblue166206227, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-000-adjusted-2.dat};
\addlegendentry{brute force (estimated) (acc: 0.9972 ± 0.0031)}
\addplot [draw=steelblue31120180, fill=steelblue31120180, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-001-adjusted-2.dat};
\addlegendentry{cubic (rel acc: 0.885 ± 0.012)}
\addplot [draw=lightgreen178223138, fill=lightgreen178223138, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-002-adjusted-2.dat};
\addlegendentry{subcubic (rel acc: 0.760 ± 0.015)}
\addplot [draw=forestgreen5116044, fill=forestgreen5116044, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-003-adjusted-2.dat};
\addlegendentry{attention-\(\displaystyle \dvocab \dmodel ^2\) (rel acc: 0.742 ± 0.015)}
\addplot [draw=lightsalmon251154153, fill=lightsalmon251154153, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-004-adjusted-2.dat};
\addlegendentry{direct-quadratic (rel acc: 0.626 ± 0.029)}
\addplot [draw=crimson2272628, fill=crimson2272628, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-005-adjusted-2.dat};
\addlegendentry{attention-\(\displaystyle \dvocab \dmodel ^2\), direct-quadratic (rel acc: 0.612 ± 0.028)}
\addplot [draw=sandybrown253191111, fill=sandybrown253191111, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-006-adjusted-2.dat};
\addlegendentry{attention-quadratic (rel acc: 0.451 ± 0.025)}
\addplot [draw=darkorange2551270, fill=darkorange2551270, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-007-adjusted-2.dat};
\addlegendentry{attention-quadratic, direct-quadratic (rel acc: 0.392 ± 0.024)}
\end{axis}

\end{tikzpicture}


==> generated/max-of-10-dvocab-128-all-models/adjusted-figures/NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-mmzstorehash.tex <==
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-000-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-001-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-002-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-003-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-004-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-005-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-006-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-007-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-008-adjusted-2.dat.md5}


==> generated/max-of-10-dvocab-128-all-models/adjusted-figures/NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables.tex <==
% This file was created with tikzplotlib v0.10.1.post13.
\begin{tikzpicture}

\definecolor{crimson2272628}{RGB}{227,26,28}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange2551270}{RGB}{255,127,0}
\definecolor{forestgreen5116044}{RGB}{51,160,44}
\definecolor{lightblue166206227}{RGB}{166,206,227}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightgreen178223138}{RGB}{178,223,138}
\definecolor{lightsalmon251154153}{RGB}{251,154,153}
\definecolor{orange}{RGB}{255,165,0}
\definecolor{sandybrown253191111}{RGB}{253,191,111}
\definecolor{steelblue31120180}{RGB}{31,120,180}

\begin{axis}[legend pos=outer north east,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
%
  legend pos=outer north east,
  draw=lightgray204,
  mark options={mark size=3}
},
log basis x={2},
tick align=outside,
tick pos=left,
unbounded coords=jump,
x grid style={darkgray176},
xlabel={FLOPs to Verify Proof (approximate)},
xmin=1722196.20006751, xmax=7.64186190064118e+29,
xmode=log,
xtick style={color=black},
xtick={0.0078125,1048576,140737488355328,1.88894659314786e+22,2.53530120045646e+30,3.40282366920938e+38},
xticklabels={
  \(\displaystyle {2^{-7}}\),
  \(\displaystyle {2^{20}}\),
  \(\displaystyle {2^{47}}\),
  \(\displaystyle {2^{74}}\),
  \(\displaystyle {2^{101}}\),
  \(\displaystyle {2^{128}}\)
},
y grid style={darkgray176},
ylabel={Normalized Accuracy Bound},
ymin=-0.05, ymax=1.05,
ytick style={color=black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
yticklabels={
  \(\displaystyle {\ensuremath{-}0.2}\),
  \(\displaystyle {0.0}\),
  \(\displaystyle {0.2}\),
  \(\displaystyle {0.4}\),
  \(\displaystyle {0.6}\),
  \(\displaystyle {0.8}\),
  \(\displaystyle {1.0}\),
  \(\displaystyle {1.2}\)
}
]
\addplot [draw=lightblue166206227, fill=lightblue166206227, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-000-adjusted-2.dat};
\addlegendentry{brute force (estimated) (acc: 0.9972 ± 0.0031)}
\addplot [draw=steelblue31120180, fill=steelblue31120180, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-001-adjusted-2.dat};
\addlegendentry{cubic (rel acc: 0.885 ± 0.012)}
\addplot [draw=lightgreen178223138, fill=lightgreen178223138, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-002-adjusted-2.dat};
\addlegendentry{direct-quadratic (rel acc: 0.609 ± 0.030)}
\addplot [draw=forestgreen5116044, fill=forestgreen5116044, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-003-adjusted-2.dat};
\addlegendentry{subcubic (rel acc: 0.613 ± 0.037)}
\addplot [draw=lightsalmon251154153, fill=lightsalmon251154153, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-004-adjusted-2.dat};
\addlegendentry{attention-\(\displaystyle \dvocab \dmodel ^2\), direct-quadratic (rel acc: 0.596 ± 0.030)}
\addplot [draw=crimson2272628, fill=crimson2272628, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-005-adjusted-2.dat};
\addlegendentry{attention-\(\displaystyle \dvocab \dmodel ^2\) (rel acc: 0.595 ± 0.035)}
\addplot [draw=sandybrown253191111, fill=sandybrown253191111, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-006-adjusted-2.dat};
\addlegendentry{attention-quadratic, direct-quadratic (rel acc: 0.385 ± 0.025)}
\addplot [draw=darkorange2551270, fill=darkorange2551270, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-007-adjusted-2.dat};
\addlegendentry{attention-quadratic (rel acc: 0.351 ± 0.029)}
\addplot [thick, orange, dashed]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-008-adjusted-2.dat};
\addlegendentry{brute-force linear baseline}
\end{axis}

\end{tikzpicture}


==> generated/max-of-20-all-models/adjusted-figures/NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-mmzstorehash.tex <==
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-000.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-001.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-002.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-003.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-004.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-005.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-006.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-007.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-008.dat.md5}


==> generated/max-of-20-all-models/adjusted-figures/NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables.tex <==
% This file was created with tikzplotlib v0.10.1.post9.
\begin{tikzpicture}

\definecolor{crimson2272628}{RGB}{227,26,28}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange2551270}{RGB}{255,127,0}
\definecolor{darkslateblue10661154}{RGB}{106,61,154}
\definecolor{forestgreen5116044}{RGB}{51,160,44}
\definecolor{khaki255255153}{RGB}{255,255,153}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightsalmon251154153}{RGB}{251,154,153}
\definecolor{sandybrown253191111}{RGB}{253,191,111}
\definecolor{sienna1778940}{RGB}{177,89,40}
\definecolor{thistle202178214}{RGB}{202,178,214}

\begin{axis}[legend pos=outer north east,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
%
  legend pos=outer north east,
  draw=lightgray204,
  mark options={mark size=3}
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={EPQKE Singular Ratio: \(\displaystyle \sigma_1 / \sigma_2\)},
xmin=281.214195251465, xmax=1468.51343536377,
xtick style={color=black},
xtick={200,400,600,800,1000,1200,1400,1600},
xticklabels={
  \(\displaystyle {200}\),
  \(\displaystyle {400}\),
  \(\displaystyle {600}\),
  \(\displaystyle {800}\),
  \(\displaystyle {1000}\),
  \(\displaystyle {1200}\),
  \(\displaystyle {1400}\),
  \(\displaystyle {1600}\)
},
y grid style={darkgray176},
ylabel={Normalized Accuracy Bound},
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={
  \(\displaystyle {0.0}\),
  \(\displaystyle {0.2}\),
  \(\displaystyle {0.4}\),
  \(\displaystyle {0.6}\),
  \(\displaystyle {0.8}\),
  \(\displaystyle {1.0}\)
}
]
\addplot [draw=sienna1778940, fill=sienna1778940, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-000.dat};
\addlegendentry{max-diff-exact}
\addplot [draw=khaki255255153, fill=khaki255255153, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-001.dat};
\addlegendentry{max-diff-subproduct}
\addplot [
  draw=darkslateblue10661154,
  fill=darkslateblue10661154,
  mark size=3pt,
  mark=*,
  only marks
]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-002.dat};
\addlegendentry{mean+max-diff-subproduct}
\addplot [draw=thistle202178214, fill=thistle202178214, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-003.dat};
\addlegendentry{mean+max-diff}
\addplot [draw=darkorange2551270, fill=darkorange2551270, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-004.dat};
\addlegendentry{max-diff}
\addplot [draw=sandybrown253191111, fill=sandybrown253191111, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-005.dat};
\addlegendentry{svd}
\addplot [draw=crimson2272628, fill=crimson2272628, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-006.dat};
\addlegendentry{mean-recursive+max-diff-subproduct-recursive}
\addplot [draw=lightsalmon251154153, fill=lightsalmon251154153, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-007.dat};
\addlegendentry{mean+max-diff-subproduct-recursive}
\addplot [draw=forestgreen5116044, fill=forestgreen5116044, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-008.dat};
\addlegendentry{max-diff-subproduct-recursive}
\end{axis}

\end{tikzpicture}


==> generated/max-of-20-all-models/adjusted-figures/NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-mmzstorehash.tex <==
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-000-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-001-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-002-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-003-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-004-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-005-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-006-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-007-adjusted-2.dat.md5}


==> generated/max-of-20-all-models/adjusted-figures/NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables.tex <==
% This file was created with tikzplotlib v0.10.1.post9.
\begin{tikzpicture}

\definecolor{crimson2272628}{RGB}{227,26,28}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange2551270}{RGB}{255,127,0}
\definecolor{forestgreen5116044}{RGB}{51,160,44}
\definecolor{lightblue166206227}{RGB}{166,206,227}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightgreen178223138}{RGB}{178,223,138}
\definecolor{lightsalmon251154153}{RGB}{251,154,153}
\definecolor{sandybrown253191111}{RGB}{253,191,111}
\definecolor{steelblue31120180}{RGB}{31,120,180}

\begin{axis}[legend pos=outer north east,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  draw=lightgray204,
  mark options={mark size=3}
},
log basis x={2},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={FLOPs to Verify Proof (approximate)},
xmin=238972.548369894, xmax=2.12780616212076e+46,
xmode=log,
xtick style={color=black},
xtick={0.00048828125,131072,35184372088832,9.44473296573929e+21,2.53530120045646e+30,6.80564733841877e+38,1.82687704666363e+47,4.90398573077084e+55},
xticklabels={
  \(\displaystyle {2^{-11}}\),
  \(\displaystyle {2^{17}}\),
  \(\displaystyle {2^{45}}\),
  \(\displaystyle {2^{73}}\),
  \(\displaystyle {2^{101}}\),
  \(\displaystyle {2^{129}}\),
  \(\displaystyle {2^{157}}\),
  \(\displaystyle {2^{185}}\)
},
y grid style={darkgray176},
ylabel={Normalized Accuracy Bound},
ymin=-0.05, ymax=1.05,
ytick style={color=black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
yticklabels={
  \(\displaystyle {\ensuremath{-}0.2}\),
  \(\displaystyle {0.0}\),
  \(\displaystyle {0.2}\),
  \(\displaystyle {0.4}\),
  \(\displaystyle {0.6}\),
  \(\displaystyle {0.8}\),
  \(\displaystyle {1.0}\),
  \(\displaystyle {1.2}\)
}
]
\addplot [draw=lightblue166206227, fill=lightblue166206227, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-000-adjusted-2.dat};
\addlegendentry{brute force (estimated) (acc: 0.995 ± 0.015)}
\addplot [draw=steelblue31120180, fill=steelblue31120180, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-001-adjusted-2.dat};
\addlegendentry{cubic (rel acc: 0.888 ± 0.036)}
\addplot [draw=lightgreen178223138, fill=lightgreen178223138, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-002-adjusted-2.dat};
\addlegendentry{subcubic (rel acc: 0.563 ± 0.041)}
\addplot [draw=forestgreen5116044, fill=forestgreen5116044, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-003-adjusted-2.dat};
\addlegendentry{attention-\(\displaystyle \dvocab \dmodel ^2\) (rel acc: 0.549 ± 0.041)}
\addplot [draw=lightsalmon251154153, fill=lightsalmon251154153, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-004-adjusted-2.dat};
\addlegendentry{direct-quadratic (rel acc: 0.540 ± 0.040)}
\addplot [draw=crimson2272628, fill=crimson2272628, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-005-adjusted-2.dat};
\addlegendentry{attention-\(\displaystyle \dvocab \dmodel ^2\), direct-quadratic (rel acc: 0.528 ± 0.039)}
\addplot [draw=sandybrown253191111, fill=sandybrown253191111, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-006-adjusted-2.dat};
\addlegendentry{attention-quadratic, direct-quadratic (rel acc: 0.322 ± 0.034)}
\addplot [draw=darkorange2551270, fill=darkorange2551270, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-007-adjusted-2.dat};
\addlegendentry{attention-quadratic (rel acc: 0.323 ± 0.035)}
\end{axis}

\end{tikzpicture}


==> generated/max-of-20-all-models/adjusted-figures/NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-mmzstorehash.tex <==
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-000-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-001-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-002-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-003-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-004-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-005-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-006-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-007-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-008-adjusted-2.dat.md5}


==> generated/max-of-20-all-models/adjusted-figures/NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables.tex <==
% This file was created with tikzplotlib v0.10.1.post13.
\begin{tikzpicture}

\definecolor{crimson2272628}{RGB}{227,26,28}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange2551270}{RGB}{255,127,0}
\definecolor{forestgreen5116044}{RGB}{51,160,44}
\definecolor{lightblue166206227}{RGB}{166,206,227}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightgreen178223138}{RGB}{178,223,138}
\definecolor{lightsalmon251154153}{RGB}{251,154,153}
\definecolor{orange}{RGB}{255,165,0}
\definecolor{sandybrown253191111}{RGB}{253,191,111}
\definecolor{steelblue31120180}{RGB}{31,120,180}

\begin{axis}[legend pos=outer north east,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
%
  legend pos=outer north east,
  draw=lightgray204,
  mark options={mark size=3}
},
log basis x={2},
tick align=outside,
tick pos=left,
unbounded coords=jump,
x grid style={darkgray176},
xlabel={FLOPs to Verify Proof (approximate)},
xmin=238972.548369894, xmax=2.12780616212076e+46,
xmode=log,
xtick style={color=black},
xtick={1.86264514923096e-09,131072,9.22337203685478e+18,6.49037107316853e+32,4.56719261665907e+46,3.21387608851798e+60},
xticklabels={
  \(\displaystyle {2^{-29}}\),
  \(\displaystyle {2^{17}}\),
  \(\displaystyle {2^{63}}\),
  \(\displaystyle {2^{109}}\),
  \(\displaystyle {2^{155}}\),
  \(\displaystyle {2^{201}}\)
},
y grid style={darkgray176},
ylabel={Normalized Accuracy Bound},
ymin=-0.05, ymax=1.05,
ytick style={color=black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
yticklabels={
  \(\displaystyle {\ensuremath{-}0.2}\),
  \(\displaystyle {0.0}\),
  \(\displaystyle {0.2}\),
  \(\displaystyle {0.4}\),
  \(\displaystyle {0.6}\),
  \(\displaystyle {0.8}\),
  \(\displaystyle {1.0}\),
  \(\displaystyle {1.2}\)
}
]
\addplot [draw=lightblue166206227, fill=lightblue166206227, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-000-adjusted-2.dat};
\addlegendentry{brute force (estimated) (acc: 0.995 ± 0.015)}
\addplot [draw=steelblue31120180, fill=steelblue31120180, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-001-adjusted-2.dat};
\addlegendentry{cubic (rel acc: 0.888 ± 0.036)}
\addplot [draw=lightgreen178223138, fill=lightgreen178223138, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-002-adjusted-2.dat};
\addlegendentry{subcubic (rel acc: 0.563 ± 0.041)}
\addplot [draw=forestgreen5116044, fill=forestgreen5116044, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-003-adjusted-2.dat};
\addlegendentry{attention-\(\displaystyle \dvocab \dmodel ^2\) (rel acc: 0.549 ± 0.041)}
\addplot [draw=lightsalmon251154153, fill=lightsalmon251154153, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-004-adjusted-2.dat};
\addlegendentry{direct-quadratic (rel acc: 0.540 ± 0.040)}
\addplot [draw=crimson2272628, fill=crimson2272628, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-005-adjusted-2.dat};
\addlegendentry{attention-\(\displaystyle \dvocab \dmodel ^2\), direct-quadratic (rel acc: 0.528 ± 0.039)}
\addplot [draw=sandybrown253191111, fill=sandybrown253191111, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-006-adjusted-2.dat};
\addlegendentry{attention-quadratic, direct-quadratic (rel acc: 0.322 ± 0.034)}
\addplot [draw=darkorange2551270, fill=darkorange2551270, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-007-adjusted-2.dat};
\addlegendentry{attention-quadratic (rel acc: 0.323 ± 0.035)}
\addplot [thick, orange, dashed]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-008-adjusted-2.dat};
\addlegendentry{brute-force linear baseline}
\end{axis}

\end{tikzpicture}


==> generated/max-of-4/adjusted-figures/EffectiveDimensionVsFLOPExternalTables-mmzstorehash.tex <==
\mmzstorehash{EffectiveDimensionVsFLOPExternalTables-000.dat.md5}
\mmzstorehash{EffectiveDimensionVsFLOPExternalTables-001.dat.md5}
\mmzstorehash{EffectiveDimensionVsFLOPExternalTables-002.dat.md5}
\mmzstorehash{EffectiveDimensionVsFLOPExternalTables-003.dat.md5}
\mmzstorehash{EffectiveDimensionVsFLOPExternalTables-004.dat.md5}
\mmzstorehash{EffectiveDimensionVsFLOPExternalTables-005.dat.md5}
\mmzstorehash{EffectiveDimensionVsFLOPExternalTables-006.dat.md5}
\mmzstorehash{EffectiveDimensionVsFLOPExternalTables-007.dat.md5}


==> generated/max-of-5-all-models/adjusted-figures/NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-mmzstorehash.tex <==
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-000.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-001.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-002.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-003.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-004.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-005.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-006.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-007.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-008.dat.md5}


==> generated/max-of-5-all-models/adjusted-figures/NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables.tex <==
% This file was created with tikzplotlib v0.10.1.post9.
\begin{tikzpicture}

\definecolor{crimson2272628}{RGB}{227,26,28}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange2551270}{RGB}{255,127,0}
\definecolor{darkslateblue10661154}{RGB}{106,61,154}
\definecolor{forestgreen5116044}{RGB}{51,160,44}
\definecolor{khaki255255153}{RGB}{255,255,153}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightsalmon251154153}{RGB}{251,154,153}
\definecolor{sandybrown253191111}{RGB}{253,191,111}
\definecolor{sienna1778940}{RGB}{177,89,40}
\definecolor{thistle202178214}{RGB}{202,178,214}

\begin{axis}[legend pos=outer north east,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
%
  legend pos=outer north east,
  draw=lightgray204,
  mark options={mark size=3}
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={EPQKE Singular Ratio: \(\displaystyle \sigma_1 / \sigma_2\)},
xmin=252.412817382813, xmax=1273.79665527344,
xtick style={color=black},
xtick={200,400,600,800,1000,1200,1400},
xticklabels={
  \(\displaystyle {200}\),
  \(\displaystyle {400}\),
  \(\displaystyle {600}\),
  \(\displaystyle {800}\),
  \(\displaystyle {1000}\),
  \(\displaystyle {1200}\),
  \(\displaystyle {1400}\)
},
y grid style={darkgray176},
ylabel={Normalized Accuracy Bound},
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={
  \(\displaystyle {0.0}\),
  \(\displaystyle {0.2}\),
  \(\displaystyle {0.4}\),
  \(\displaystyle {0.6}\),
  \(\displaystyle {0.8}\),
  \(\displaystyle {1.0}\)
}
]
\addplot [draw=sienna1778940, fill=sienna1778940, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-000.dat};
\addlegendentry{max-diff-exact}
\addplot [draw=khaki255255153, fill=khaki255255153, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-001.dat};
\addlegendentry{max-diff-subproduct}
\addplot [
  draw=darkslateblue10661154,
  fill=darkslateblue10661154,
  mark size=3pt,
  mark=*,
  only marks
]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-002.dat};
\addlegendentry{mean+max-diff-subproduct}
\addplot [draw=thistle202178214, fill=thistle202178214, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-003.dat};
\addlegendentry{max-diff}
\addplot [draw=darkorange2551270, fill=darkorange2551270, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-004.dat};
\addlegendentry{mean+max-diff}
\addplot [draw=sandybrown253191111, fill=sandybrown253191111, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-005.dat};
\addlegendentry{svd}
\addplot [draw=crimson2272628, fill=crimson2272628, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-006.dat};
\addlegendentry{mean+max-diff-subproduct-recursive}
\addplot [draw=lightsalmon251154153, fill=lightsalmon251154153, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-007.dat};
\addlegendentry{max-diff-subproduct-recursive}
\addplot [draw=forestgreen5116044, fill=forestgreen5116044, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsEPQKESingularRatioExternalTables-008.dat};
\addlegendentry{mean-recursive+max-diff-subproduct-recursive}
\end{axis}

\end{tikzpicture}


==> generated/max-of-5-all-models/adjusted-figures/NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-mmzstorehash.tex <==
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-000-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-001-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-002-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-003-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-004-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-005-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-006-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-007-adjusted-2.dat.md5}


==> generated/max-of-5-all-models/adjusted-figures/NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables.tex <==
% This file was created with tikzplotlib v0.10.1.post9.
\begin{tikzpicture}

\definecolor{crimson2272628}{RGB}{227,26,28}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange2551270}{RGB}{255,127,0}
\definecolor{forestgreen5116044}{RGB}{51,160,44}
\definecolor{lightblue166206227}{RGB}{166,206,227}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightgreen178223138}{RGB}{178,223,138}
\definecolor{lightsalmon251154153}{RGB}{251,154,153}
\definecolor{sandybrown253191111}{RGB}{253,191,111}
\definecolor{steelblue31120180}{RGB}{31,120,180}

\begin{axis}[legend pos=outer north east,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  draw=lightgray204,
  mark options={mark size=3}
},
log basis x={2},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={FLOPs to Verify Proof (approximate)},
xmin=756590.541610363, xmax=4.40382634648473e+16,
xmode=log,
xtick style={color=black},
xtick={2048,524288,134217728,34359738368,8796093022208,2.25179981368525e+15,5.76460752303423e+17,1.47573952589676e+20},
xticklabels={
  \(\displaystyle {2^{11}}\),
  \(\displaystyle {2^{19}}\),
  \(\displaystyle {2^{27}}\),
  \(\displaystyle {2^{35}}\),
  \(\displaystyle {2^{43}}\),
  \(\displaystyle {2^{51}}\),
  \(\displaystyle {2^{59}}\),
  \(\displaystyle {2^{67}}\)
},
y grid style={darkgray176},
ylabel={Normalized Accuracy Bound},
ymin=-0.0499999537305331, ymax=1.04999999779669,
ytick style={color=black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
yticklabels={
  \(\displaystyle {\ensuremath{-}0.2}\),
  \(\displaystyle {0.0}\),
  \(\displaystyle {0.2}\),
  \(\displaystyle {0.4}\),
  \(\displaystyle {0.6}\),
  \(\displaystyle {0.8}\),
  \(\displaystyle {1.0}\),
  \(\displaystyle {1.2}\)
}
]
\addplot [draw=lightblue166206227, fill=lightblue166206227, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-000-adjusted-2.dat};
\addlegendentry{brute force (estimated) (acc: 0.9990 ± 0.0018)}
\addplot [draw=steelblue31120180, fill=steelblue31120180, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-001-adjusted-2.dat};
\addlegendentry{cubic (rel acc: 0.942 ± 0.010)}
\addplot [draw=lightgreen178223138, fill=lightgreen178223138, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-002-adjusted-2.dat};
\addlegendentry{subcubic (rel acc: 0.702 ± 0.033)}
\addplot [draw=forestgreen5116044, fill=forestgreen5116044, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-003-adjusted-2.dat};
\addlegendentry{direct-quadratic (rel acc: 0.649 ± 0.055)}
\addplot [draw=lightsalmon251154153, fill=lightsalmon251154153, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-004-adjusted-2.dat};
\addlegendentry{attention-\(\displaystyle \dvocab \dmodel ^2\) (rel acc: 0.682 ± 0.033)}
\addplot [draw=crimson2272628, fill=crimson2272628, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-005-adjusted-2.dat};
\addlegendentry{attention-\(\displaystyle \dvocab \dmodel ^2\), direct-quadratic (rel acc: 0.629 ± 0.053)}
\addplot [draw=sandybrown253191111, fill=sandybrown253191111, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-006-adjusted-2.dat};
\addlegendentry{attention-quadratic (rel acc: 0.354 ± 0.034)}
\addplot [draw=darkorange2551270, fill=darkorange2551270, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyExternalTables-007-adjusted-2.dat};
\addlegendentry{attention-quadratic, direct-quadratic (rel acc: 0.336 ± 0.033)}
\end{axis}

\end{tikzpicture}


==> generated/max-of-5-all-models/adjusted-figures/NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-mmzstorehash.tex <==
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-000-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-001-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-002-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-003-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-004-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-005-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-006-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-007-adjusted-2.dat.md5}
\mmzstorehash{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-008-adjusted-2.dat.md5}


==> generated/max-of-5-all-models/adjusted-figures/NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables.tex <==
% This file was created with tikzplotlib v0.10.1.post13.
\begin{tikzpicture}

\definecolor{crimson2272628}{RGB}{227,26,28}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange2551270}{RGB}{255,127,0}
\definecolor{forestgreen5116044}{RGB}{51,160,44}
\definecolor{lightblue166206227}{RGB}{166,206,227}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightgreen178223138}{RGB}{178,223,138}
\definecolor{lightsalmon251154153}{RGB}{251,154,153}
\definecolor{orange}{RGB}{255,165,0}
\definecolor{sandybrown253191111}{RGB}{253,191,111}
\definecolor{steelblue31120180}{RGB}{31,120,180}

\begin{axis}[legend pos=outer north east,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
%
  legend pos=outer north east,
  draw=lightgray204,
  mark options={mark size=3}
},
log basis x={2},
tick align=outside,
tick pos=left,
unbounded coords=jump,
x grid style={darkgray176},
xlabel={FLOPs to Verify Proof (approximate)},
xmin=756590.541610363, xmax=4.40382634648473e+16,
xmode=log,
xtick style={color=black},
xtick={128,524288,2147483648,8796093022208,3.6028797018964e+16,1.47573952589676e+20,6.04462909807315e+23},
xticklabels={
  \(\displaystyle {2^{7}}\),
  \(\displaystyle {2^{19}}\),
  \(\displaystyle {2^{31}}\),
  \(\displaystyle {2^{43}}\),
  \(\displaystyle {2^{55}}\),
  \(\displaystyle {2^{67}}\),
  \(\displaystyle {2^{79}}\)
},
y grid style={darkgray176},
ylabel={Normalized Accuracy Bound},
ymin=-0.0499999537305331, ymax=1.04999999779669,
ytick style={color=black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
yticklabels={
  \(\displaystyle {\ensuremath{-}0.2}\),
  \(\displaystyle {0.0}\),
  \(\displaystyle {0.2}\),
  \(\displaystyle {0.4}\),
  \(\displaystyle {0.6}\),
  \(\displaystyle {0.8}\),
  \(\displaystyle {1.0}\),
  \(\displaystyle {1.2}\)
}
]
\addplot [draw=lightblue166206227, fill=lightblue166206227, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-000-adjusted-2.dat};
\addlegendentry{brute force (estimated) (acc: 0.9990 ± 0.0018)}
\addplot [draw=steelblue31120180, fill=steelblue31120180, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-001-adjusted-2.dat};
\addlegendentry{cubic (rel acc: 0.942 ± 0.010)}
\addplot [draw=lightgreen178223138, fill=lightgreen178223138, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-002-adjusted-2.dat};
\addlegendentry{subcubic (rel acc: 0.702 ± 0.033)}
\addplot [draw=forestgreen5116044, fill=forestgreen5116044, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-003-adjusted-2.dat};
\addlegendentry{direct-quadratic (rel acc: 0.649 ± 0.055)}
\addplot [draw=lightsalmon251154153, fill=lightsalmon251154153, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-004-adjusted-2.dat};
\addlegendentry{attention-\(\displaystyle \dvocab \dmodel ^2\) (rel acc: 0.682 ± 0.033)}
\addplot [draw=crimson2272628, fill=crimson2272628, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-005-adjusted-2.dat};
\addlegendentry{attention-\(\displaystyle \dvocab \dmodel ^2\), direct-quadratic (rel acc: 0.629 ± 0.053)}
\addplot [draw=sandybrown253191111, fill=sandybrown253191111, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-006-adjusted-2.dat};
\addlegendentry{attention-quadratic (rel acc: 0.354 ± 0.034)}
\addplot [draw=darkorange2551270, fill=darkorange2551270, mark size=3pt, mark=*, only marks]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-007-adjusted-2.dat};
\addlegendentry{attention-quadratic, direct-quadratic (rel acc: 0.336 ± 0.033)}
\addplot [thick, orange, dashed]
table{NormalizedAccuracyBoundVsFLOPsFrontierOnlyWithBaselineExternalTables-008-adjusted-2.dat};
\addlegendentry{brute-force linear baseline}
\end{axis}

\end{tikzpicture}


==> generated/values-10-dvocab-128.tex <==
\def\AllModelsHEADSHASHORT{9b6f505}
\def\AllModelsHEADSHA{9b6f505d441963664b8e05d1b3dc4adf129f3922}
\def\AlmostQuadraticAccuracyLen{2718}
\def\AlmostQuadraticAccuracyMaxFloat{0.451928798694893607557077075398410670459270477294921875}
\def\AlmostQuadraticAccuracyMeanFloat{0.09537265827728653999617591807691496796905994415283203125}
\def\AlmostQuadraticAccuracyMedianFloat{0.0000000000000000000482808779934951193268943825387395918369293212890625}
\def\AlmostQuadraticAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\AlmostQuadraticAccuracyStdDevFloat{0.14340227370849423227383567791548557579517364501953125}
\def\AlmostQuadraticDroppedSequencesFracLen{2718}
\def\AlmostQuadraticDroppedSequencesFracMaxFloat{0.364304421671816702765767104210681281983852386474609375}
\def\AlmostQuadraticDroppedSequencesFracMeanFloat{0.1982036894965367446186377264893963001668453216552734375}
\def\AlmostQuadraticDroppedSequencesFracMedianFloat{0}
\def\AlmostQuadraticDroppedSequencesFracMinFloat{0}
\def\AlmostQuadraticDroppedSequencesFracStdDevFloat{0.1433547128132553194479470448641222901642322540283203125}
\def\AlmostQuadraticDroppedSequencesLen{2718}
\def\AlmostQuadraticDroppedSequencesMaxFloat{430094747616049389880}
\def\AlmostQuadraticDroppedSequencesMeanFloat{233997615014886670336}
\def\AlmostQuadraticDroppedSequencesMedianFloat{0}
\def\AlmostQuadraticDroppedSequencesMinFloat{0}
\def\AlmostQuadraticDroppedSequencesStdDevFloat{169243372737680539648}
\def\AlmostQuadraticEffectiveDimensionalityEstimateLen{2718}
\def\AlmostQuadraticEffectiveDimensionalityEstimateMaxFloat{21186}
\def\AlmostQuadraticEffectiveDimensionalityEstimateMeanFloat{21100.66666666666787932626903057098388671875}
\def\AlmostQuadraticEffectiveDimensionalityEstimateMedianFloat{20930}
\def\AlmostQuadraticEffectiveDimensionalityEstimateMinFloat{20930}
\def\AlmostQuadraticEffectiveDimensionalityEstimateStdDevFloat{85.333333333333342807236476801335811614990234375}
\def\AlmostQuadraticErrUpperBoundLen{2718}
\def\AlmostQuadraticErrUpperBoundMaxFloat{187.469207763671875}
\def\AlmostQuadraticErrUpperBoundMeanFloat{102.81546069349411709481501020491123199462890625}
\def\AlmostQuadraticErrUpperBoundMedianFloat{83.86852264404296875}
\def\AlmostQuadraticErrUpperBoundMinFloat{81.919342041015625}
\def\AlmostQuadraticErrUpperBoundStdDevFloat{9.6921242410523884558415375067852437496185302734375}
\def\AlmostQuadraticGapMostBelowValueLen{2718}
\def\AlmostQuadraticGapMostBelowValueMaxFloat{76}
\def\AlmostQuadraticGapMostBelowValueMeanFloat{30.7534952170713751229413901455700397491455078125}
\def\AlmostQuadraticGapMostBelowValueMedianFloat{1}
\def\AlmostQuadraticGapMostBelowValueMinFloat{1}
\def\AlmostQuadraticGapMostBelowValueNumStdLen{2718}
\def\AlmostQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\AlmostQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\AlmostQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\AlmostQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\AlmostQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\AlmostQuadraticGapMostBelowValueSequenceFracLen{2718}
\def\AlmostQuadraticGapMostBelowValueSequenceFracMaxFloat{1}
\def\AlmostQuadraticGapMostBelowValueSequenceFracMeanFloat{0.999662958869520057447743965894915163516998291015625}
\def\AlmostQuadraticGapMostBelowValueSequenceFracMedianFloat{0.99736704736948011973396432949812151491641998291015625}
\def\AlmostQuadraticGapMostBelowValueSequenceFracMinFloat{0.9940254688262939453125}
\def\AlmostQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.000551504564547116598628717643038044116110540926456451416015625}
\def\AlmostQuadraticGapMostBelowValueStdDevFloat{22.0715176586696770755224861204624176025390625}
\def\AlmostQuadraticInstructionCountBranchLen{2718}
\def\AlmostQuadraticInstructionCountBranchMaxFloat{0}
\def\AlmostQuadraticInstructionCountBranchMeanFloat{0}
\def\AlmostQuadraticInstructionCountBranchMedianFloat{0}
\def\AlmostQuadraticInstructionCountBranchMinFloat{0}
\def\AlmostQuadraticInstructionCountBranchStdDevFloat{0}
\def\AlmostQuadraticInstructionCountIntLen{2718}
\def\AlmostQuadraticInstructionCountIntMaxFloat{0}
\def\AlmostQuadraticInstructionCountIntMeanFloat{0}
\def\AlmostQuadraticInstructionCountIntMedianFloat{0}
\def\AlmostQuadraticInstructionCountIntMinFloat{0}
\def\AlmostQuadraticInstructionCountIntStdDevFloat{0}
\def\AlmostQuadraticInstructionCountLen{2718}
\def\AlmostQuadraticInstructionCountMaxFloat{20948465}
\def\AlmostQuadraticInstructionCountMeanFloat{20705629.3333333320915699005126953125}
\def\AlmostQuadraticInstructionCountMedianFloat{20462164}
\def\AlmostQuadraticInstructionCountMinFloat{20462164}
\def\AlmostQuadraticInstructionCountStdDevFloat{220175.6468150927103124558925628662109375}
\def\AlmostQuadraticMaxGapLen{2718}
\def\AlmostQuadraticMaxGapMaxFloat{98}
\def\AlmostQuadraticMaxGapMeanFloat{52.11662987490802123602406936697661876678466796875}
\def\AlmostQuadraticMaxGapMedianFloat{1}
\def\AlmostQuadraticMaxGapMinFloat{1}
\def\AlmostQuadraticMaxGapStdDevFloat{38.340099356474439673547749407589435577392578125}
\def\AlmostQuadraticNormalizedAccuracyLen{2718}
\def\AlmostQuadraticNormalizedAccuracyMaxFloat{0.45284483628465832527609791213762946426868438720703125}
\def\AlmostQuadraticNormalizedAccuracyMeanFloat{0.09562998254307138179530767274627578444778919219970703125}
\def\AlmostQuadraticNormalizedAccuracyMedianFloat{0.000000000000000000048395942402973877046403457273086360814637485857644968556372233603468657747725956141948699951171875}
\def\AlmostQuadraticNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\AlmostQuadraticNormalizedAccuracyStdDevFloat{0.1437880917737918984311562553557450883090496063232421875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.451928798694893607557077075398410670459270477294921875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.383662939919712175917965168991941027343273162841796875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{32382}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.31131020585100532827027564053423702716827392578125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{15043}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.299347341418428614101543416836648248136043548583984375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{8893}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0252514343739989842452242641002158052287995815277099609375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.361191106294214303584766412313911132514476776123046875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24173}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.3217549413456755047491242294199764728546142578125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{22545}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.22805696152062904236146323455614037811756134033203125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1316400142569892073307613600263721309602260589599609375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0233944905114797409295679386787014664150774478912353515625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{426419193568601303974}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24173}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{379861187677126787072}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{22545}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{269242137817527746560}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{155413097782922049324}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{27619339468805967872}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21122.42384105960445594973862171173095703125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{104}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{104}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{63.99859653739444098619060241617262363433837890625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{179.824432373046875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.2996650847378106163887423463165760040283203125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.85131072998046875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{82.67822265625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.5066345135820657930025845416821539402008056640625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{75}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{12561}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{50.17218543046357837056348216719925403594970703125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{22.75}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{13}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99999940395355224609375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12141}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.999015660475421451991451249341480433940887451171875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{24173}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99676690995693217889339621251565404236316680908203125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20013}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99628353118896484375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{6549}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00065818497769662052086780956727807279094122350215911865234375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{8.4585170755832503886040285578928887844085693359375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20948465}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{5781}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20917470.1324503310024738311767578125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20905172}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{104}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{20905172}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{104}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{13645.16560373371976311318576335906982421875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{96}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{8721}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{84.4238410596026511711897910572588443756103515625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{77}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{11598}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{77}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{11598}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.71044183672842020627058445825241506099700927734375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.45284483628465832527609791213762946426868438720703125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.384717017723093357428609806447639130055904388427734375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{32382}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.3126635989519497282884685773751698434352874755859375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15043}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.300958397943729194512485491941333748400211334228515625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8893}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.02515111962896716957249765300730359740555286407470703125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{682.4775712490081787109375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{23696}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{660.9983980308305717699113301932811737060546875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29195}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{637.450467586517333984375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{519}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{637.3421027660369873046875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{13293}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.6690240432014800120441577746532857418060302734375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7661190032958984375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{11611}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.125046921092152985011125565506517887115478515625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{16284}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{16.882906973361968994140625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{16.85701274871826171875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.26885273590923841613431477526319213211536407470703125}
\def\AlmostQuadraticProofSearchTimeLen{2718}
\def\AlmostQuadraticProofSearchTimeMaxFloat{1046.6073901653289794921875}
\def\AlmostQuadraticProofSearchTimeMeanFloat{658.210672109595407164306379854679107666015625}
\def\AlmostQuadraticProofSearchTimeMedianFloat{631.3133363056182361106039024889469146728515625}
\def\AlmostQuadraticProofSearchTimeMinFloat{624.76801586151123046875}
\def\AlmostQuadraticProofSearchTimeStdDevFloat{14.6822847114774059917863269220106303691864013671875}
\def\AlmostQuadraticProofTimeLen{2718}
\def\AlmostQuadraticProofTimeMaxFloat{19.9767801761627197265625}
\def\AlmostQuadraticProofTimeMeanFloat{18.073890649281150189153777319006621837615966796875}
\def\AlmostQuadraticProofTimeMedianFloat{16.93083802700042639344246708787977695465087890625}
\def\AlmostQuadraticProofTimeMinFloat{16.7781083583831787109375}
\def\AlmostQuadraticProofTimeStdDevFloat{0.243980881048622533224801145479432307183742523193359375}
\def\AnySubcubicAccuracyLen{15100}
\def\AnySubcubicAccuracyLowerWhiskerBottomEndFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\AnySubcubicAccuracyLowerWhiskerCrosshatchFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\AnySubcubicAccuracyMaxFloat{0.68942794737815604744213260346441529691219329833984375}
\def\AnySubcubicAccuracyMeanFloat{0.235299944994164900169408838337403722107410430908203125}
\def\AnySubcubicAccuracyMedianFloat{0.000000000000000000049127910940749419665962705039419233798980712890625}
\def\AnySubcubicAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\AnySubcubicAccuracyQuartileOneFloat{0.0000000000000000000482808779934951193268943825387395918369293212890625}
\def\AnySubcubicAccuracyQuartileThreeFloat{0.0000000000000000000499749438880037200050310275400988757610321044921875}
\def\AnySubcubicAccuracySqrMeanFloat{0.10427768816282968755704274599338532425463199615478515625}
\def\AnySubcubicAccuracyStdDevFloat{0.2211597251955532972278462011672672815620899200439453125}
\def\AnySubcubicAccuracyUpperWhiskerCrosshatchFloat{0.0000000000000000000499749438880037200050310275400988757610321044921875}
\def\AnySubcubicAccuracyUpperWhiskerTopEndFloat{0.00000000000000000005082197683525802034409935004077851772308349609375}
\def\AnySubcubicDroppedSequencesFracLen{15100}
\def\AnySubcubicDroppedSequencesFracMaxFloat{0.425962157820276188235908421120257116854190826416015625}
\def\AnySubcubicDroppedSequencesFracMeanFloat{0.1632154750729473413617398591668461449444293975830078125}
\def\AnySubcubicDroppedSequencesFracMedianFloat{0}
\def\AnySubcubicDroppedSequencesFracMinFloat{0}
\def\AnySubcubicDroppedSequencesFracStdDevFloat{0.11725158517066762431380055886620539240539073944091796875}
\def\AnySubcubicDroppedSequencesLen{15100}
\def\AnySubcubicDroppedSequencesMaxFloat{502887354265325599101}
\def\AnySubcubicDroppedSequencesMeanFloat{192690822242533310464}
\def\AnySubcubicDroppedSequencesMedianFloat{0}
\def\AnySubcubicDroppedSequencesMinFloat{0}
\def\AnySubcubicDroppedSequencesStdDevFloat{138426238968326275072}
\def\AnySubcubicEffectiveDimensionalityEstimateLen{15100}
\def\AnySubcubicEffectiveDimensionalityEstimateMaxFloat{37122}
\def\AnySubcubicEffectiveDimensionalityEstimateMeanFloat{21064}
\def\AnySubcubicEffectiveDimensionalityEstimateMedianFloat{16770}
\def\AnySubcubicEffectiveDimensionalityEstimateMinFloat{16770}
\def\AnySubcubicEffectiveDimensionalityEstimateStdDevFloat{5194.1589964112572488375008106231689453125}
\def\AnySubcubicErrUpperBoundLen{15100}
\def\AnySubcubicErrUpperBoundMaxFloat{187.469207763671875}
\def\AnySubcubicErrUpperBoundMeanFloat{36.02944345300560513578602694906294345855712890625}
\def\AnySubcubicErrUpperBoundMedianFloat{0}
\def\AnySubcubicErrUpperBoundMinFloat{0}
\def\AnySubcubicErrUpperBoundStdDevFloat{44.3671866260445852958582690916955471038818359375}
\def\AnySubcubicGapMostBelowValueLen{15100}
\def\AnySubcubicGapMostBelowValueMaxFloat{78}
\def\AnySubcubicGapMostBelowValueMeanFloat{17.785761589403971782985536265186965465545654296875}
\def\AnySubcubicGapMostBelowValueMedianFloat{1}
\def\AnySubcubicGapMostBelowValueMinFloat{1}
\def\AnySubcubicGapMostBelowValueNumStdLen{15100}
\def\AnySubcubicGapMostBelowValueNumStdMaxFloat{1.5}
\def\AnySubcubicGapMostBelowValueNumStdMeanFloat{1.5}
\def\AnySubcubicGapMostBelowValueNumStdMedianFloat{1.5}
\def\AnySubcubicGapMostBelowValueNumStdMinFloat{1.5}
\def\AnySubcubicGapMostBelowValueNumStdStdDevFloat{0}
\def\AnySubcubicGapMostBelowValueSequenceFracLen{15100}
\def\AnySubcubicGapMostBelowValueSequenceFracMaxFloat{1}
\def\AnySubcubicGapMostBelowValueSequenceFracMeanFloat{0.99677328000794973572595836230902932584285736083984375}
\def\AnySubcubicGapMostBelowValueSequenceFracMedianFloat{0.98013208150863651013651178800500929355621337890625}
\def\AnySubcubicGapMostBelowValueSequenceFracMinFloat{0.930698871612548828125}
\def\AnySubcubicGapMostBelowValueSequenceFracStdDevFloat{0.00412217591972200390892933086206539883278310298919677734375}
\def\AnySubcubicGapMostBelowValueStdDevFloat{17.88057501398032655970382620580494403839111328125}
\def\AnySubcubicInstructionCountBranchLen{15100}
\def\AnySubcubicInstructionCountBranchMaxFloat{0}
\def\AnySubcubicInstructionCountBranchMeanFloat{0}
\def\AnySubcubicInstructionCountBranchMedianFloat{0}
\def\AnySubcubicInstructionCountBranchMinFloat{0}
\def\AnySubcubicInstructionCountBranchStdDevFloat{0}
\def\AnySubcubicInstructionCountIntLen{15100}
\def\AnySubcubicInstructionCountIntMaxFloat{0}
\def\AnySubcubicInstructionCountIntMeanFloat{0}
\def\AnySubcubicInstructionCountIntMedianFloat{0}
\def\AnySubcubicInstructionCountIntMinFloat{0}
\def\AnySubcubicInstructionCountIntStdDevFloat{0}
\def\AnySubcubicInstructionCountLen{15100}
\def\AnySubcubicInstructionCountMaxFloat{26044438}
\def\AnySubcubicInstructionCountMeanFloat{22570093.600000001490116119384765625}
\def\AnySubcubicInstructionCountMedianFloat{20462164}
\def\AnySubcubicInstructionCountMinFloat{20462164}
\def\AnySubcubicInstructionCountStdDevFloat{1415834.36178064276464283466339111328125}
\def\AnySubcubicMaxGapLen{15100}
\def\AnySubcubicMaxGapMaxFloat{100}
\def\AnySubcubicMaxGapMeanFloat{54.1389403973509928391649737022817134857177734375}
\def\AnySubcubicMaxGapMedianFloat{1}
\def\AnySubcubicMaxGapMinFloat{1}
\def\AnySubcubicMaxGapStdDevFloat{31.9062892169000775766107835806906223297119140625}
\def\AnySubcubicNormalizedAccuracyLen{15100}
\def\AnySubcubicNormalizedAccuracyLowerWhiskerBottomEndFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\AnySubcubicNormalizedAccuracyLowerWhiskerCrosshatchFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\AnySubcubicNormalizedAccuracyMaxFloat{0.6908253841360181279895869010942988097667694091796875}
\def\AnySubcubicNormalizedAccuracyMeanFloat{0.2359190620693003281882482724540750496089458465576171875}
\def\AnySubcubicNormalizedAccuracyMedianFloat{0.000000000000000000049250470923809783004091991959694806305698541288337787198182982084659897736855782568454742431640625}
\def\AnySubcubicNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\AnySubcubicNormalizedAccuracyQuartileOneFloat{0.000000000000000000048395942402973877046403457273086360814637485857644968556372233603468657747725956141948699951171875}
\def\AnySubcubicNormalizedAccuracyQuartileThreeFloat{0.000000000000000000050179974537678873881577384758151724298133072356022026474543784591020312291220761835575103759765625}
\def\AnySubcubicNormalizedAccuracySqrMeanFloat{0.10482242176100624309054154537079739384353160858154296875}
\def\AnySubcubicNormalizedAccuracyStdDevFloat{0.2217309584008238243502120212724548764526844024658203125}
\def\AnySubcubicNormalizedAccuracyUpperWhiskerCrosshatchFloat{0.000000000000000000050179974537678873881577384758151724298133072356022026474543784591020312291220761835575103759765625}
\def\AnySubcubicNormalizedAccuracyUpperWhiskerTopEndFloat{0.00000000000000000005094124737744649016959864435895087147072236868368451541931596349144228952354751527309417724609375}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLowerWhiskerBottomEndFloat{0.439408106677848742105396695478702895343303680419921875}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLowerWhiskerBottomEndKey{20013}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLowerWhiskerCrosshatchFloat{0.4494226235681570980062815579003654420375823974609375}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLowerWhiskerCrosshatchKey{20013}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.68942794737815604744213260346441529691219329833984375}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.62155727626461210189035000439616851508617401123046875}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMeanKey{10248}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.51075811320631547829407281824387609958648681640625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMedianKey{8893}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMinFloat{0.43620027112436698946140722910058684647083282470703125}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyQuartileOneFloat{0.473479192165341233877740023672231473028659820556640625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyQuartileOneKey{20013}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyQuartileThreeFloat{0.53637543067787596395845639563049189746379852294921875}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyQuartileThreeKey{8893}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracySqrMeanFloat{0.387288872789979088384626493279938586056232452392578125}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.030909951674108204766611152081168256700038909912109375}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyUpperWhiskerCrosshatchFloat{0.53785584966661870165438585900119505822658538818359375}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyUpperWhiskerCrosshatchKey{8893}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyUpperWhiskerTopEndFloat{0.538472133776615624611849852954037487506866455078125}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyUpperWhiskerTopEndKey{8893}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.16661087469430480023646623521926812827587127685546875}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{21598}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1289420651501977932440468066488392651081085205078125}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{5358}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08450994778538080398622156508281477726995944976806640625}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.035672195017851703047195854878737009130418300628662109375}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01374540397603360615541578937381927971728146076202392578125}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{196699402584494945925}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{21598}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{152227921674322051072}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{5358}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{99771736222686543872}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{42114294530673152936}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{16227708757481060352}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{37122}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{31502.1324503311261651106178760528564453125}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{1185}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17010}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{27671}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16962}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{104}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{7154.5454811650715782889164984226226806640625}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{9.74072265625}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{2306}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0.71863545960937902368215191017952747642993927001953125}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6435823340775674861191646414226852357387542724609375}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{104}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.76158940397350960438416223041713237762451171875}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1895}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9997761249542236328125}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99371826411872510309564177077845670282840728759765625}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{22286}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9738725125789642333984375}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8048}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96438848972320556640625}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0044495893543308288886617418711466598324477672576904296875}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.4725236672516339719862799029215238988399505615234375}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMaxFloat{25098133}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMaxKey{27671}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22888486.6158940382301807403564453125}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMeanKey{519}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21929781}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMinFloat{21929781}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{1001967.88267164281569421291351318359375}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMaxFloat{79}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMaxKey{20976}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMeanFloat{70.14569536423840645511518232524394989013671875}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMedianFloat{45.75}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMinFloat{18}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMinKey{8048}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapStdDevFloat{5.2995031017766276448810458532534539699554443359375}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLowerWhiskerBottomEndFloat{0.454301782115135888151513654520385898649692535400390625}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLowerWhiskerBottomEndKey{20013}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLowerWhiskerCrosshatchFloat{0.46306596819267209497184012434445321559906005859375}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLowerWhiskerCrosshatchKey{20013}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6908253841360181279895869010942988097667694091796875}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.623237723346502292542936629615724086761474609375}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{31308}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5167436093843142952408697965438477694988250732421875}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8893}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.451494450717646544912753370226710103452205657958984375}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyQuartileOneFloat{0.48411903005098044783238719901419244706630706787109375}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyQuartileOneKey{20013}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyQuartileThreeFloat{0.5391699273930548041988686236436478793621063232421875}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyQuartileThreeKey{8893}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracySqrMeanFloat{0.389341541490923870316720467599225230515003204345703125}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0302701451729692101733082409964481485076248645782470703125}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyUpperWhiskerCrosshatchFloat{0.54047978052028666784423194258124567568302154541015625}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyUpperWhiskerCrosshatchKey{8893}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyUpperWhiskerTopEndFloat{0.54102505971143532992329028274980373680591583251953125}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyUpperWhiskerTopEndKey{8893}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{681.8326740264892578125}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{23696}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{661.228598987819395915721543133258819580078125}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7884}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{633.805510103702545166015625}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{1681}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{629.673713207244873046875}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.6341281903399220709616201929748058319091796875}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.6453669071197509765625}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMaxKey{9504}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.108592317593807052844567806459963321685791015625}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMeanKey{519}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.047219097614288330078125}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8648827075958251953125}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2365804177105277628090362895818543620407581329345703125}
\def\AnySubcubicProofSearchTimeLen{15100}
\def\AnySubcubicProofSearchTimeMaxFloat{1046.6073901653289794921875}
\def\AnySubcubicProofSearchTimeMeanFloat{658.191769480626362565089948475360870361328125}
\def\AnySubcubicProofSearchTimeMedianFloat{629.7350604009628796120523475110530853271484375}
\def\AnySubcubicProofSearchTimeMinFloat{619.2171604633331298828125}
\def\AnySubcubicProofSearchTimeStdDevFloat{13.0151182849710362887662995490245521068572998046875}
\def\AnySubcubicProofTimeLen{15100}
\def\AnySubcubicProofTimeMaxFloat{20.580661296844478869161321199499070644378662109375}
\def\AnySubcubicProofTimeMeanFloat{18.089487481954080294599407352507114410400390625}
\def\AnySubcubicProofTimeMedianFloat{17.073483976125718442062861868180334568023681640625}
\def\AnySubcubicProofTimeMinFloat{16.755332469940185546875}
\def\AnySubcubicProofTimeStdDevFloat{0.252180099482248232245495955794467590749263763427734375}
\def\AxisLimitsOVCenteredZmaxFloat{24.6488323211669921875}
\def\AxisLimitsOVCenteredZminFloat{-102.1092071533203125}
\def\AxisLimitsOVZmaxFloat{53.503307342529296875}
\def\AxisLimitsOVZminFloat{-53.503307342529296875}
\def\AxisLimitsQKWithAttnScaleZmaxFloat{185.531953872395973803577362559735774993896484375}
\def\AxisLimitsQKWithAttnScaleZminFloat{-185.531953872395973803577362559735774993896484375}
\def\AxisLimitsQKZmaxFloat{1049.5272216796875}
\def\AxisLimitsQKZminFloat{-1049.5272216796875}
\def\BruteForceEffectiveDimensionalityEstimate{151115727451828646838272}
\def\BruteForceInstructionCountBranch{0}
\def\BruteForceInstructionCountInt{0}
\def\BruteForceInstructionCount{64317662231252189192011120640}
\def\CubicAccuracyLen{151}
\def\CubicAccuracyLowerWhiskerBottomEndFloat{0.84236039357317105125133593901409767568111419677734375}
\def\CubicAccuracyLowerWhiskerBottomEndKey{21598}
\def\CubicAccuracyLowerWhiskerCrosshatchFloat{0.84294190816232494878335046450956724584102630615234375}
\def\CubicAccuracyLowerWhiskerCrosshatchKey{21598}
\def\CubicAccuracyMaxFloat{0.90523176546833361566513076468254439532756805419921875}
\def\CubicAccuracyMaxKey{742}
\def\CubicAccuracyMeanFloat{0.88228300285911342992761774439713917672634124755859375}
\def\CubicAccuracyMeanKey{31308}
\def\CubicAccuracyMedianFloat{0.846503486064500432206614277674816548824310302734375}
\def\CubicAccuracyMedianKey{20976}
\def\CubicAccuracyMinFloat{0.84217412366176258586847325204871594905853271484375}
\def\CubicAccuracyMinKey{21598}
\def\CubicAccuracyQuartileOneFloat{0.8443388048631315090375437648617662489414215087890625}
\def\CubicAccuracyQuartileOneKey{21598}
\def\CubicAccuracyQuartileThreeFloat{0.84798098680389799586265553443809039890766143798828125}
\def\CubicAccuracyQuartileThreeKey{20976}
\def\CubicAccuracySqrMeanFloat{0.77857074780645640910137217360897921025753021240234375}
\def\CubicAccuracyStdDevFloat{0.0121429268449609988056447917870173114351928234100341796875}
\def\CubicAccuracyUpperWhiskerCrosshatchFloat{0.8480475442571802080493625908275134861469268798828125}
\def\CubicAccuracyUpperWhiskerCrosshatchKey{20976}
\def\CubicAccuracyUpperWhiskerTopEndFloat{0.84807525148139950577075296678231097757816314697265625}
\def\CubicAccuracyUpperWhiskerTopEndKey{20976}
\def\CubicCorrectCountLen{151}
\def\CubicCorrectCountMaxFloat{1068709037119143384028}
\def\CubicCorrectCountMaxKey{742}
\def\CubicCorrectCountMeanFloat{1041615920276864892928}
\def\CubicCorrectCountMeanKey{31308}
\def\CubicCorrectCountMedianFloat{999374922555827159040}
\def\CubicCorrectCountMedianKey{20976}
\def\CubicCorrectCountMinFloat{994263713580105814398}
\def\CubicCorrectCountMinKey{21598}
\def\CubicCorrectCountStdDevFloat{14335837684145469440}
\def\CubicEffectiveDimensionalityEstimate{51712}
\def\CubicInstructionCountBranch{0}
\def\CubicInstructionCountInt{0}
\def\CubicInstructionCount{1540696512}
\def\CubicNormalizedAccuracyLen{151}
\def\CubicNormalizedAccuracyLowerWhiskerBottomEndFloat{0.85016893493633094447403664162266068160533905029296875}
\def\CubicNormalizedAccuracyLowerWhiskerBottomEndKey{21598}
\def\CubicNormalizedAccuracyLowerWhiskerCrosshatchFloat{0.85031531282353045586575035486021079123020172119140625}
\def\CubicNormalizedAccuracyLowerWhiskerCrosshatchKey{21598}
\def\CubicNormalizedAccuracyMaxFloat{0.91364379899192738054836127048474736511707305908203125}
\def\CubicNormalizedAccuracyMaxKey{20013}
\def\CubicNormalizedAccuracyMeanFloat{0.88473028765522732097537073059356771409511566162109375}
\def\CubicNormalizedAccuracyMeanKey{25516}
\def\CubicNormalizedAccuracyMedianFloat{0.85121182730165456664650491802603937685489654541015625}
\def\CubicNormalizedAccuracyMedianKey{20976}
\def\CubicNormalizedAccuracyMinFloat{0.850122047383397028141871487605385482311248779296875}
\def\CubicNormalizedAccuracyMinKey{21598}
\def\CubicNormalizedAccuracyQuartileOneFloat{0.85066693734252585290533943407353945076465606689453125}
\def\CubicNormalizedAccuracyQuartileOneKey{21598}
\def\CubicNormalizedAccuracyQuartileThreeFloat{0.85167102947889217201549172386876307427883148193359375}
\def\CubicNormalizedAccuracyQuartileThreeKey{20976}
\def\CubicNormalizedAccuracySqrMeanFloat{0.7828874320596426183982430302421562373638153076171875}
\def\CubicNormalizedAccuracyStdDevFloat{0.01182159740226445925059817199098688433878123760223388671875}
\def\CubicNormalizedAccuracyUpperWhiskerCrosshatchFloat{0.85185676770514262567957075589220039546489715576171875}
\def\CubicNormalizedAccuracyUpperWhiskerCrosshatchKey{20976}
\def\CubicNormalizedAccuracyUpperWhiskerTopEndFloat{0.85193408873272169490320493423496372997760772705078125}
\def\CubicNormalizedAccuracyUpperWhiskerTopEndKey{20976}
\def\CubicProofTimeLen{151}
\def\CubicProofTimeMaxFloat{1008.4877998828887939453125}
\def\CubicProofTimeMaxKey{17197}
\def\CubicProofTimeMeanFloat{971.7858797272309629988740198314189910888671875}
\def\CubicProofTimeMeanKey{22401}
\def\CubicProofTimeMedianFloat{938.556623995304107666015625}
\def\CubicProofTimeMedianKey{24202}
\def\CubicProofTimeMinFloat{937.9930119514464195162872783839702606201171875}
\def\CubicProofTimeMinKey{24262}
\def\CubicProofTimeStdDevFloat{20.74525750832614079399718320928514003753662109375}
\def\EPVOUAbsLenLen{151}
\def\EPVOUAbsLenMaxFloat{16384}
\def\EPVOUAbsLenMaxKey{50}
\def\EPVOUAbsLenMeanFloat{16384}
\def\EPVOUAbsLenMeanKey{50}
\def\EPVOUAbsLenMedianFloat{16384}
\def\EPVOUAbsLenMedianKey{50}
\def\EPVOUAbsLenMinFloat{16384}
\def\EPVOUAbsLenMinKey{50}
\def\EPVOUAbsLenStdDevFloat{0}
\def\EPVOUAbsMaxLen{151}
\def\EPVOUAbsMaxMaxFloat{53.5033111572265625}
\def\EPVOUAbsMaxMaxKey{13716}
\def\EPVOUAbsMaxMeanFloat{43.5574798583984375}
\def\EPVOUAbsMaxMeanKey{7098}
\def\EPVOUAbsMaxMedianFloat{36.784481048583984375}
\def\EPVOUAbsMaxMedianKey{2306}
\def\EPVOUAbsMaxMinFloat{35.368297576904296875}
\def\EPVOUAbsMaxMinKey{20013}
\def\EPVOUAbsMaxStdDevFloat{3.341346263885498046875}
\def\EPVOUAbsMeanLen{151}
\def\EPVOUAbsMeanMaxFloat{9.95603084564208984375}
\def\EPVOUAbsMeanMaxKey{123}
\def\EPVOUAbsMeanMeanFloat{7.643365383148193359375}
\def\EPVOUAbsMeanMeanKey{31308}
\def\EPVOUAbsMeanMedianFloat{6.14350092411041259765625}
\def\EPVOUAbsMeanMedianKey{20338}
\def\EPVOUAbsMeanMinFloat{5.5318603515625}
\def\EPVOUAbsMeanMinKey{20013}
\def\EPVOUAbsMeanStdDevFloat{0.71167278289794921875}
\def\EPVOUAbsMedianLen{151}
\def\EPVOUAbsMedianMaxFloat{0.12387387633323669600127203693773481063544750213623046875}
\def\EPVOUAbsMedianMaxKey{7238}
\def\EPVOUAbsMedianMeanFloat{0.08569017126736853950941252833217731676995754241943359375}
\def\EPVOUAbsMedianMeanKey{16149}
\def\EPVOUAbsMedianMedianFloat{0.052111857198178783423525572970902430824935436248779296875}
\def\EPVOUAbsMedianMedianKey{8893}
\def\EPVOUAbsMedianMinFloat{0.048326245397329332942337742906602215953171253204345703125}
\def\EPVOUAbsMedianMinKey{20013}
\def\EPVOUAbsMedianStdDevFloat{0.0133160860093593236275211211250280030071735382080078125}
\def\EPVOUAbsMinLen{151}
\def\EPVOUAbsMinMaxFloat{0.004761219024658203125}
\def\EPVOUAbsMinMaxKey{26278}
\def\EPVOUAbsMinMeanFloat{0.001140141277574002742767333984375}
\def\EPVOUAbsMinMeanKey{6082}
\def\EPVOUAbsMinMedianFloat{0.00000946223735809326171875}
\def\EPVOUAbsMinMedianKey{12457}
\def\EPVOUAbsMinMinFloat{0.000003516674041748046875}
\def\EPVOUAbsMinMinKey{4729}
\def\EPVOUAbsMinStdDevFloat{0.0010903165675699710845947265625}
\def\EPVOUAbsStdDevLen{151}
\def\EPVOUAbsStdDevMaxFloat{6.121235370635986328125}
\def\EPVOUAbsStdDevMaxKey{123}
\def\EPVOUAbsStdDevMeanFloat{5.127142429351806640625}
\def\EPVOUAbsStdDevMeanKey{8299}
\def\EPVOUAbsStdDevMedianFloat{4.51260554790496826171875}
\def\EPVOUAbsStdDevMedianKey{20338}
\def\EPVOUAbsStdDevMinFloat{4.442618846893310546875}
\def\EPVOUAbsStdDevMinKey{20013}
\def\EPVOUAbsStdDevStdDevFloat{0.310099780559539794921875}
\def\EPVOUCenteredLenLen{151}
\def\EPVOUCenteredLenMaxFloat{16384}
\def\EPVOUCenteredLenMaxKey{50}
\def\EPVOUCenteredLenMeanFloat{16384}
\def\EPVOUCenteredLenMeanKey{50}
\def\EPVOUCenteredLenMedianFloat{16384}
\def\EPVOUCenteredLenMedianKey{50}
\def\EPVOUCenteredLenMinFloat{16384}
\def\EPVOUCenteredLenMinKey{50}
\def\EPVOUCenteredLenStdDevFloat{0}
\def\EPVOUCenteredMaxLen{151}
\def\EPVOUCenteredMaxMaxFloat{24.648834228515625}
\def\EPVOUCenteredMaxMaxKey{20013}
\def\EPVOUCenteredMaxMeanFloat{14.24061870574951171875}
\def\EPVOUCenteredMaxMeanKey{26278}
\def\EPVOUCenteredMaxMedianFloat{10.8770964145660400390625}
\def\EPVOUCenteredMaxMedianKey{30899}
\def\EPVOUCenteredMaxMinFloat{10.699138641357421875}
\def\EPVOUCenteredMaxMinKey{15662}
\def\EPVOUCenteredMaxStdDevFloat{1.6976606845855712890625}
\def\EPVOUCenteredMeanLen{151}
\def\EPVOUCenteredMeanMaxFloat{-10.1656970977783203125}
\def\EPVOUCenteredMeanMaxKey{20013}
\def\EPVOUCenteredMeanMeanFloat{-13.928394317626953125}
\def\EPVOUCenteredMeanMeanKey{11130}
\def\EPVOUCenteredMeanMedianFloat{-15.4082705974578857421875}
\def\EPVOUCenteredMeanMedianKey{17080}
\def\EPVOUCenteredMeanMinFloat{-15.5325412750244140625}
\def\EPVOUCenteredMeanMinKey{123}
\def\EPVOUCenteredMeanStdDevFloat{0.637372553348541259765625}
\def\EPVOUCenteredMedianLen{151}
\def\EPVOUCenteredMedianMaxFloat{-53.81951416015625255795384873636066913604736328125}
\def\EPVOUCenteredMedianMaxKey{20013}
\def\EPVOUCenteredMedianMeanFloat{-64.4132705966368348526884801685810089111328125}
\def\EPVOUCenteredMedianMeanKey{13293}
\def\EPVOUCenteredMedianMedianFloat{-74.62749940872191700691473670303821563720703125}
\def\EPVOUCenteredMedianMedianKey{19917}
\def\EPVOUCenteredMedianMinFloat{-75.285913200378416831881622783839702606201171875}
\def\EPVOUCenteredMedianMinKey{123}
\def\EPVOUCenteredMedianStdDevFloat{3.62283200126034188315315986983478069305419921875}
\def\EPVOUCenteredMinLen{151}
\def\EPVOUCenteredMinMaxFloat{-69.5697174072265625}
\def\EPVOUCenteredMinMaxKey{20013}
\def\EPVOUCenteredMinMeanFloat{-82.52490997314453125}
\def\EPVOUCenteredMinMeanKey{30463}
\def\EPVOUCenteredMinMedianFloat{-100.81427001953125}
\def\EPVOUCenteredMinMedianKey{20751}
\def\EPVOUCenteredMinMinFloat{-102.10921478271484375}
\def\EPVOUCenteredMinMinKey{4810}
\def\EPVOUCenteredMinStdDevFloat{5.925937175750732421875}
\def\EPVOUCenteredOffDiagonalLenLen{151}
\def\EPVOUCenteredOffDiagonalLenMaxFloat{16256}
\def\EPVOUCenteredOffDiagonalLenMaxKey{50}
\def\EPVOUCenteredOffDiagonalLenMeanFloat{16256}
\def\EPVOUCenteredOffDiagonalLenMeanKey{50}
\def\EPVOUCenteredOffDiagonalLenMedianFloat{16256}
\def\EPVOUCenteredOffDiagonalLenMedianKey{50}
\def\EPVOUCenteredOffDiagonalLenMinFloat{16256}
\def\EPVOUCenteredOffDiagonalLenMinKey{50}
\def\EPVOUCenteredOffDiagonalLenStdDevFloat{0}
\def\EPVOUCenteredOffDiagonalMaxLen{151}
\def\EPVOUCenteredOffDiagonalMaxMaxFloat{24.648834228515625}
\def\EPVOUCenteredOffDiagonalMaxMaxKey{20013}
\def\EPVOUCenteredOffDiagonalMaxMeanFloat{14.24061870574951171875}
\def\EPVOUCenteredOffDiagonalMaxMeanKey{26278}
\def\EPVOUCenteredOffDiagonalMaxMedianFloat{10.8770964145660400390625}
\def\EPVOUCenteredOffDiagonalMaxMedianKey{30899}
\def\EPVOUCenteredOffDiagonalMaxMinFloat{10.699138641357421875}
\def\EPVOUCenteredOffDiagonalMaxMinKey{15662}
\def\EPVOUCenteredOffDiagonalMaxStdDevFloat{1.6976606845855712890625}
\def\EPVOUCenteredOffDiagonalMeanLen{151}
\def\EPVOUCenteredOffDiagonalMeanMaxFloat{-10.2457408905029296875}
\def\EPVOUCenteredOffDiagonalMeanMaxKey{20013}
\def\EPVOUCenteredOffDiagonalMeanMeanFloat{-14.038066864013671875}
\def\EPVOUCenteredOffDiagonalMeanMeanKey{11130}
\def\EPVOUCenteredOffDiagonalMeanMedianFloat{-15.529595851898193359375}
\def\EPVOUCenteredOffDiagonalMeanMedianKey{17080}
\def\EPVOUCenteredOffDiagonalMeanMinFloat{-15.6548442840576171875}
\def\EPVOUCenteredOffDiagonalMeanMinKey{123}
\def\EPVOUCenteredOffDiagonalMeanStdDevFloat{0.642391264438629150390625}
\def\EPVOUCenteredOffDiagonalMedianLen{151}
\def\EPVOUCenteredOffDiagonalMedianMaxFloat{-53.8752563476562471578290569595992565155029296875}
\def\EPVOUCenteredOffDiagonalMedianMaxKey{20013}
\def\EPVOUCenteredOffDiagonalMedianMeanFloat{-64.4591674173115052326465956866741180419921875}
\def\EPVOUCenteredOffDiagonalMedianMeanKey{13293}
\def\EPVOUCenteredOffDiagonalMedianMedianFloat{-74.7104413032531766702959430404007434844970703125}
\def\EPVOUCenteredOffDiagonalMedianMedianKey{19917}
\def\EPVOUCenteredOffDiagonalMedianMinFloat{-75.2867872238159208109209430404007434844970703125}
\def\EPVOUCenteredOffDiagonalMedianMinKey{123}
\def\EPVOUCenteredOffDiagonalMedianStdDevFloat{3.62674214931524030447462791926227509975433349609375}
\def\EPVOUCenteredOffDiagonalMinLen{151}
\def\EPVOUCenteredOffDiagonalMinMaxFloat{-69.5697174072265625}
\def\EPVOUCenteredOffDiagonalMinMaxKey{20013}
\def\EPVOUCenteredOffDiagonalMinMeanFloat{-82.52490997314453125}
\def\EPVOUCenteredOffDiagonalMinMeanKey{30463}
\def\EPVOUCenteredOffDiagonalMinMedianFloat{-100.81427001953125}
\def\EPVOUCenteredOffDiagonalMinMedianKey{20751}
\def\EPVOUCenteredOffDiagonalMinMinFloat{-102.10921478271484375}
\def\EPVOUCenteredOffDiagonalMinMinKey{4810}
\def\EPVOUCenteredOffDiagonalMinStdDevFloat{5.925937175750732421875}
\def\EPVOUCenteredOffDiagonalStdDevLen{151}
\def\EPVOUCenteredOffDiagonalStdDevMaxFloat{17.71691131591796875}
\def\EPVOUCenteredOffDiagonalStdDevMaxKey{123}
\def\EPVOUCenteredOffDiagonalStdDevMeanFloat{15.4712123870849609375}
\def\EPVOUCenteredOffDiagonalStdDevMeanKey{24438}
\def\EPVOUCenteredOffDiagonalStdDevMedianFloat{13.746812343597412109375}
\def\EPVOUCenteredOffDiagonalStdDevMedianKey{6532}
\def\EPVOUCenteredOffDiagonalStdDevMinFloat{12.83209323883056640625}
\def\EPVOUCenteredOffDiagonalStdDevMinKey{20013}
\def\EPVOUCenteredOffDiagonalStdDevStdDevFloat{0.746597766876220703125}
\def\EPVOUCenteredStdDevLen{151}
\def\EPVOUCenteredStdDevMaxFloat{17.7013092041015625}
\def\EPVOUCenteredStdDevMaxKey{123}
\def\EPVOUCenteredStdDevMeanFloat{15.460174560546875}
\def\EPVOUCenteredStdDevMeanKey{24438}
\def\EPVOUCenteredStdDevMedianFloat{13.7369153499603271484375}
\def\EPVOUCenteredStdDevMedianKey{6532}
\def\EPVOUCenteredStdDevMinFloat{12.81366252899169921875}
\def\EPVOUCenteredStdDevMinKey{20013}
\def\EPVOUCenteredStdDevStdDevFloat{0.74515306949615478515625}
\def\EPVOUDiagonalLenLen{151}
\def\EPVOUDiagonalLenMaxFloat{128}
\def\EPVOUDiagonalLenMaxKey{50}
\def\EPVOUDiagonalLenMeanFloat{128}
\def\EPVOUDiagonalLenMeanKey{50}
\def\EPVOUDiagonalLenMedianFloat{128}
\def\EPVOUDiagonalLenMedianKey{50}
\def\EPVOUDiagonalLenMinFloat{128}
\def\EPVOUDiagonalLenMinKey{50}
\def\EPVOUDiagonalLenStdDevFloat{0}
\def\EPVOUDiagonalMaxLen{151}
\def\EPVOUDiagonalMaxMaxFloat{53.5033111572265625}
\def\EPVOUDiagonalMaxMaxKey{13716}
\def\EPVOUDiagonalMaxMeanFloat{43.164043426513671875}
\def\EPVOUDiagonalMaxMeanKey{31308}
\def\EPVOUDiagonalMaxMedianFloat{36.49276256561279296875}
\def\EPVOUDiagonalMaxMedianKey{2306}
\def\EPVOUDiagonalMaxMinFloat{34.20142364501953125}
\def\EPVOUDiagonalMaxMinKey{20013}
\def\EPVOUDiagonalMaxStdDevFloat{3.4093606472015380859375}
\def\EPVOUDiagonalMeanLen{151}
\def\EPVOUDiagonalMeanMaxFloat{17.648639678955078125}
\def\EPVOUDiagonalMeanMaxKey{123}
\def\EPVOUDiagonalMeanMeanFloat{15.33030414581298828125}
\def\EPVOUDiagonalMeanMeanKey{9504}
\def\EPVOUDiagonalMeanMedianFloat{12.583904266357421875}
\def\EPVOUDiagonalMeanMedianKey{8048}
\def\EPVOUDiagonalMeanMinFloat{10.033222198486328125}
\def\EPVOUDiagonalMeanMinKey{20013}
\def\EPVOUDiagonalMeanStdDevFloat{0.886132895946502685546875}
\def\EPVOUDiagonalMedianLen{151}
\def\EPVOUDiagonalMedianMaxFloat{5.013033647537231018986858543939888477325439453125}
\def\EPVOUDiagonalMedianMaxKey{123}
\def\EPVOUDiagonalMedianMeanFloat{2.766333271584763497941139576141722500324249267578125}
\def\EPVOUDiagonalMedianMeanKey{29195}
\def\EPVOUDiagonalMedianMedianFloat{-0.41666549369692795767861070999060757458209991455078125}
\def\EPVOUDiagonalMedianMedianKey{27484}
\def\EPVOUDiagonalMedianMinFloat{-1.219049083590507454033513567992486059665679931640625}
\def\EPVOUDiagonalMedianMinKey{27714}
\def\EPVOUDiagonalMedianStdDevFloat{1.134637292030537647491428288049064576625823974609375}
\def\EPVOUDiagonalMinLen{151}
\def\EPVOUDiagonalMinMaxFloat{4.8162784576416015625}
\def\EPVOUDiagonalMinMaxKey{123}
\def\EPVOUDiagonalMinMeanFloat{2.2666947841644287109375}
\def\EPVOUDiagonalMinMeanKey{2743}
\def\EPVOUDiagonalMinMedianFloat{-1.8034813106060028076171875}
\def\EPVOUDiagonalMinMedianKey{27714}
\def\EPVOUDiagonalMinMinFloat{-2.1436822414398193359375}
\def\EPVOUDiagonalMinMinKey{27484}
\def\EPVOUDiagonalMinStdDevFloat{1.34630024433135986328125}
\def\EPVOUDiagonalStdDevLen{151}
\def\EPVOUDiagonalStdDevMaxFloat{11.44049835205078125}
\def\EPVOUDiagonalStdDevMaxKey{4810}
\def\EPVOUDiagonalStdDevMeanFloat{9.18296337127685546875}
\def\EPVOUDiagonalStdDevMeanKey{22401}
\def\EPVOUDiagonalStdDevMedianFloat{7.96256351470947265625}
\def\EPVOUDiagonalStdDevMedianKey{11611}
\def\EPVOUDiagonalStdDevMinFloat{7.93267154693603515625}
\def\EPVOUDiagonalStdDevMinKey{20013}
\def\EPVOUDiagonalStdDevStdDevFloat{0.533301293849945068359375}
\def\EPVOUInputsWithCopyingFailureLenLen{151}
\def\EPVOUInputsWithCopyingFailureLenMaxFloat{70}
\def\EPVOUInputsWithCopyingFailureLenMaxKey{14095}
\def\EPVOUInputsWithCopyingFailureLenMeanFloat{63.3841059602649039561583776958286762237548828125}
\def\EPVOUInputsWithCopyingFailureLenMeanKey{519}
\def\EPVOUInputsWithCopyingFailureLenMedianFloat{60}
\def\EPVOUInputsWithCopyingFailureLenMedianKey{4647}
\def\EPVOUInputsWithCopyingFailureLenMinFloat{60}
\def\EPVOUInputsWithCopyingFailureLenMinKey{4647}
\def\EPVOUInputsWithCopyingFailureLenStdDevFloat{1.7142214928417989217024341996875591576099395751953125}
\def\EPVOUInputsWithCopyingFailureMaxLen{151}
\def\EPVOUInputsWithCopyingFailureMaxMaxFloat{115}
\def\EPVOUInputsWithCopyingFailureMaxMaxKey{20013}
\def\EPVOUInputsWithCopyingFailureMaxMeanFloat{66.5761589403973488288102089427411556243896484375}
\def\EPVOUInputsWithCopyingFailureMaxMeanKey{4729}
\def\EPVOUInputsWithCopyingFailureMaxMedianFloat{59.75}
\def\EPVOUInputsWithCopyingFailureMaxMedianKey{24566}
\def\EPVOUInputsWithCopyingFailureMaxMinFloat{59}
\def\EPVOUInputsWithCopyingFailureMaxMinKey{8745}
\def\EPVOUInputsWithCopyingFailureMaxStdDevFloat{6.44429732614177996907756096334196627140045166015625}
\def\EPVOUInputsWithCopyingFailureMeanLen{151}
\def\EPVOUInputsWithCopyingFailureMeanMaxFloat{34.51428571428571245860439375974237918853759765625}
\def\EPVOUInputsWithCopyingFailureMeanMaxKey{14095}
\def\EPVOUInputsWithCopyingFailureMeanMeanFloat{31.332761383888509953976608812808990478515625}
\def\EPVOUInputsWithCopyingFailureMeanMeanKey{8893}
\def\EPVOUInputsWithCopyingFailureMeanMedianFloat{29.525000000000002131628207280300557613372802734375}
\def\EPVOUInputsWithCopyingFailureMeanMedianKey{24566}
\def\EPVOUInputsWithCopyingFailureMeanMinFloat{29.5}
\def\EPVOUInputsWithCopyingFailureMeanMinKey{8745}
\def\EPVOUInputsWithCopyingFailureMeanStdDevFloat{0.88687352842084410387002435527392663061618804931640625}
\def\EPVOUInputsWithCopyingFailureMedianLen{151}
\def\EPVOUInputsWithCopyingFailureMedianMaxFloat{0.345000000000000028865798640254070051014423370361328125}
\def\EPVOUInputsWithCopyingFailureMedianMaxKey{14095}
\def\EPVOUInputsWithCopyingFailureMedianMeanFloat{0.31192052980132445316741041096975095570087432861328125}
\def\EPVOUInputsWithCopyingFailureMedianMeanKey{519}
\def\EPVOUInputsWithCopyingFailureMedianMedianFloat{0.294999999999999984456877655247808434069156646728515625}
\def\EPVOUInputsWithCopyingFailureMedianMedianKey{4647}
\def\EPVOUInputsWithCopyingFailureMedianMinFloat{0.294999999999999984456877655247808434069156646728515625}
\def\EPVOUInputsWithCopyingFailureMedianMinKey{4647}
\def\EPVOUInputsWithCopyingFailureMedianStdDevFloat{0.00857110746420900425357469742948524071834981441497802734375}
\def\EPVOUInputsWithCopyingFailureMinLen{151}
\def\EPVOUInputsWithCopyingFailureMinMaxFloat{0}
\def\EPVOUInputsWithCopyingFailureMinMaxKey{50}
\def\EPVOUInputsWithCopyingFailureMinMeanFloat{0}
\def\EPVOUInputsWithCopyingFailureMinMeanKey{50}
\def\EPVOUInputsWithCopyingFailureMinMedianFloat{0}
\def\EPVOUInputsWithCopyingFailureMinMedianKey{50}
\def\EPVOUInputsWithCopyingFailureMinMinFloat{0}
\def\EPVOUInputsWithCopyingFailureMinMinKey{50}
\def\EPVOUInputsWithCopyingFailureMinStdDevFloat{0}
\def\EPVOUInputsWithCopyingFailureStdDevLen{151}
\def\EPVOUInputsWithCopyingFailureStdDevMaxFloat{21.371012051527173980502993799746036529541015625}
\def\EPVOUInputsWithCopyingFailureStdDevMaxKey{20013}
\def\EPVOUInputsWithCopyingFailureStdDevMeanFloat{18.544351961119563299007495515979826450347900390625}
\def\EPVOUInputsWithCopyingFailureStdDevMeanKey{12457}
\def\EPVOUInputsWithCopyingFailureStdDevMedianFloat{17.36059421444360850728116929531097412109375}
\def\EPVOUInputsWithCopyingFailureStdDevMedianKey{24566}
\def\EPVOUInputsWithCopyingFailureStdDevMinFloat{17.318102282486574239328547264449298381805419921875}
\def\EPVOUInputsWithCopyingFailureStdDevMinKey{8745}
\def\EPVOUInputsWithCopyingFailureStdDevStdDevFloat{0.61069779520820122176161248717107810080051422119140625}
\def\EPVOULenLen{151}
\def\EPVOULenMaxFloat{16384}
\def\EPVOULenMaxKey{50}
\def\EPVOULenMeanFloat{16384}
\def\EPVOULenMeanKey{50}
\def\EPVOULenMedianFloat{16384}
\def\EPVOULenMedianKey{50}
\def\EPVOULenMinFloat{16384}
\def\EPVOULenMinKey{50}
\def\EPVOULenStdDevFloat{0}
\def\EPVOUMaxAboveDiagLenLen{151}
\def\EPVOUMaxAboveDiagLenMaxFloat{128}
\def\EPVOUMaxAboveDiagLenMaxKey{50}
\def\EPVOUMaxAboveDiagLenMeanFloat{128}
\def\EPVOUMaxAboveDiagLenMeanKey{50}
\def\EPVOUMaxAboveDiagLenMedianFloat{128}
\def\EPVOUMaxAboveDiagLenMedianKey{50}
\def\EPVOUMaxAboveDiagLenMinFloat{128}
\def\EPVOUMaxAboveDiagLenMinKey{50}
\def\EPVOUMaxAboveDiagLenStdDevFloat{0}
\def\EPVOUMaxAboveDiagMaxLen{151}
\def\EPVOUMaxAboveDiagMaxMaxFloat{24.648834228515625}
\def\EPVOUMaxAboveDiagMaxMaxKey{20013}
\def\EPVOUMaxAboveDiagMaxMeanFloat{14.24061870574951171875}
\def\EPVOUMaxAboveDiagMaxMeanKey{26278}
\def\EPVOUMaxAboveDiagMaxMedianFloat{10.8770964145660400390625}
\def\EPVOUMaxAboveDiagMaxMedianKey{30899}
\def\EPVOUMaxAboveDiagMaxMinFloat{10.699138641357421875}
\def\EPVOUMaxAboveDiagMaxMinKey{15662}
\def\EPVOUMaxAboveDiagMaxStdDevFloat{1.6976606845855712890625}
\def\EPVOUMaxAboveDiagMeanLen{151}
\def\EPVOUMaxAboveDiagMeanMaxFloat{1.3100740909576416015625}
\def\EPVOUMaxAboveDiagMeanMaxKey{30371}
\def\EPVOUMaxAboveDiagMeanMeanFloat{0.34076917171478271484375}
\def\EPVOUMaxAboveDiagMeanMeanKey{28778}
\def\EPVOUMaxAboveDiagMeanMedianFloat{-0.413186371326446533203125}
\def\EPVOUMaxAboveDiagMeanMedianKey{1951}
\def\EPVOUMaxAboveDiagMeanMinFloat{-0.443675220012664794921875}
\def\EPVOUMaxAboveDiagMeanMinKey{15662}
\def\EPVOUMaxAboveDiagMeanStdDevFloat{0.388650476932525634765625}
\def\EPVOUMaxAboveDiagMedianLen{151}
\def\EPVOUMaxAboveDiagMedianMaxFloat{-10.6433435249328613991792735760100185871124267578125}
\def\EPVOUMaxAboveDiagMedianMaxKey{8048}
\def\EPVOUMaxAboveDiagMedianMeanFloat{-11.9315489991295411442706608795560896396636962890625}
\def\EPVOUMaxAboveDiagMedianMeanKey{11598}
\def\EPVOUMaxAboveDiagMedianMedianFloat{-14.742823202610015442814983543939888477325439453125}
\def\EPVOUMaxAboveDiagMedianMedianKey{1490}
\def\EPVOUMaxAboveDiagMedianMinFloat{-15.1979126834869386897253207280300557613372802734375}
\def\EPVOUMaxAboveDiagMedianMinKey{17080}
\def\EPVOUMaxAboveDiagMedianStdDevFloat{0.7193842122443989683944209900801070034503936767578125}
\def\EPVOUMaxAboveDiagMinLen{151}
\def\EPVOUMaxAboveDiagMinMaxFloat{-10.766490936279296875}
\def\EPVOUMaxAboveDiagMinMaxKey{27671}
\def\EPVOUMaxAboveDiagMinMeanFloat{-12.38766956329345703125}
\def\EPVOUMaxAboveDiagMinMeanKey{24262}
\def\EPVOUMaxAboveDiagMinMedianFloat{-16.641069889068603515625}
\def\EPVOUMaxAboveDiagMinMedianKey{17080}
\def\EPVOUMaxAboveDiagMinMinFloat{-16.7182102203369140625}
\def\EPVOUMaxAboveDiagMinMinKey{12493}
\def\EPVOUMaxAboveDiagMinStdDevFloat{1.006795406341552734375}
\def\EPVOUMaxAboveDiagStdDevLen{151}
\def\EPVOUMaxAboveDiagStdDevMaxFloat{8.54772853851318359375}
\def\EPVOUMaxAboveDiagStdDevMaxKey{742}
\def\EPVOUMaxAboveDiagStdDevMeanFloat{7.79304790496826171875}
\def\EPVOUMaxAboveDiagStdDevMeanKey{7790}
\def\EPVOUMaxAboveDiagStdDevMedianFloat{6.9068124294281005859375}
\def\EPVOUMaxAboveDiagStdDevMedianKey{24144}
\def\EPVOUMaxAboveDiagStdDevMinFloat{6.86700344085693359375}
\def\EPVOUMaxAboveDiagStdDevMinKey{20013}
\def\EPVOUMaxAboveDiagStdDevStdDevFloat{0.35720264911651611328125}
\def\EPVOUMaxLen{151}
\def\EPVOUMaxMaxFloat{53.5033111572265625}
\def\EPVOUMaxMaxKey{13716}
\def\EPVOUMaxMeanFloat{43.164043426513671875}
\def\EPVOUMaxMeanKey{31308}
\def\EPVOUMaxMedianFloat{36.49276256561279296875}
\def\EPVOUMaxMedianKey{2306}
\def\EPVOUMaxMinFloat{34.20142364501953125}
\def\EPVOUMaxMinKey{20013}
\def\EPVOUMaxRowDiffLenLen{151}
\def\EPVOUMaxRowDiffLenMaxFloat{128}
\def\EPVOUMaxRowDiffLenMaxKey{50}
\def\EPVOUMaxRowDiffLenMeanFloat{128}
\def\EPVOUMaxRowDiffLenMeanKey{50}
\def\EPVOUMaxRowDiffLenMedianFloat{128}
\def\EPVOUMaxRowDiffLenMedianKey{50}
\def\EPVOUMaxRowDiffLenMinFloat{128}
\def\EPVOUMaxRowDiffLenMinKey{50}
\def\EPVOUMaxRowDiffLenStdDevFloat{0}
\def\EPVOUMaxRowDiffMaxLen{151}
\def\EPVOUMaxRowDiffMaxMaxFloat{102.10921478271484375}
\def\EPVOUMaxRowDiffMaxMaxKey{4810}
\def\EPVOUMaxRowDiffMaxMeanFloat{82.52490997314453125}
\def\EPVOUMaxRowDiffMaxMeanKey{30463}
\def\EPVOUMaxRowDiffMaxMedianFloat{70.8506145477294921875}
\def\EPVOUMaxRowDiffMaxMedianKey{26829}
\def\EPVOUMaxRowDiffMaxMinFloat{69.5697174072265625}
\def\EPVOUMaxRowDiffMaxMinKey{20013}
\def\EPVOUMaxRowDiffMaxStdDevFloat{5.925937175750732421875}
\def\EPVOUMaxRowDiffMeanLen{151}
\def\EPVOUMaxRowDiffMeanMaxFloat{42.704620361328125}
\def\EPVOUMaxRowDiffMeanMaxKey{17080}
\def\EPVOUMaxRowDiffMeanMeanFloat{35.83936309814453125}
\def\EPVOUMaxRowDiffMeanMeanKey{25516}
\def\EPVOUMaxRowDiffMeanMedianFloat{30.506530284881591796875}
\def\EPVOUMaxRowDiffMeanMedianKey{20338}
\def\EPVOUMaxRowDiffMeanMinFloat{27.245391845703125}
\def\EPVOUMaxRowDiffMeanMinKey{20013}
\def\EPVOUMaxRowDiffMeanStdDevFloat{2.37909603118896484375}
\def\EPVOUMaxRowDiffMedianLen{151}
\def\EPVOUMaxRowDiffMedianMaxFloat{30.052285203933717383506518672220408916473388671875}
\def\EPVOUMaxRowDiffMedianMaxKey{123}
\def\EPVOUMaxRowDiffMedianMeanFloat{22.287954277960668747482486651279032230377197265625}
\def\EPVOUMaxRowDiffMedianMeanKey{6155}
\def\EPVOUMaxRowDiffMedianMedianFloat{15.5336175990104674582426014239899814128875732421875}
\def\EPVOUMaxRowDiffMedianMedianKey{19451}
\def\EPVOUMaxRowDiffMedianMinFloat{15.1097103929519658294111650320701301097869873046875}
\def\EPVOUMaxRowDiffMedianMinKey{20013}
\def\EPVOUMaxRowDiffMedianStdDevFloat{2.8278912213086666582739781006239354610443115234375}
\def\EPVOUMaxRowDiffMinLen{151}
\def\EPVOUMaxRowDiffMinMaxFloat{29.7081165313720703125}
\def\EPVOUMaxRowDiffMinMaxKey{123}
\def\EPVOUMaxRowDiffMinMeanFloat{21.5023021697998046875}
\def\EPVOUMaxRowDiffMinMeanKey{9134}
\def\EPVOUMaxRowDiffMinMedianFloat{14.0318048000335693359375}
\def\EPVOUMaxRowDiffMinMedianKey{6549}
\def\EPVOUMaxRowDiffMinMinFloat{13.76057338714599609375}
\def\EPVOUMaxRowDiffMinMinKey{20013}
\def\EPVOUMaxRowDiffMinStdDevFloat{3.04404449462890625}
\def\EPVOUMaxRowDiffStdDevLen{151}
\def\EPVOUMaxRowDiffStdDevMaxFloat{17.1300792694091796875}
\def\EPVOUMaxRowDiffStdDevMaxKey{4810}
\def\EPVOUMaxRowDiffStdDevMeanFloat{12.09691715240478515625}
\def\EPVOUMaxRowDiffStdDevMeanKey{1185}
\def\EPVOUMaxRowDiffStdDevMedianFloat{9.9937345981597900390625}
\def\EPVOUMaxRowDiffStdDevMedianKey{18668}
\def\EPVOUMaxRowDiffStdDevMinFloat{9.959606170654296875}
\def\EPVOUMaxRowDiffStdDevMinKey{23447}
\def\EPVOUMaxRowDiffStdDevStdDevFloat{1.04810273647308349609375}
\def\EPVOUMaxStdDevFloat{3.4093606472015380859375}
\def\EPVOUMeanLen{151}
\def\EPVOUMeanMaxFloat{2.2481362819671630859375}
\def\EPVOUMeanMaxKey{4157}
\def\EPVOUMeanMeanFloat{1.40190923213958740234375}
\def\EPVOUMeanMeanKey{22261}
\def\EPVOUMeanMedianFloat{0.3261250555515289306640625}
\def\EPVOUMeanMedianKey{19451}
\def\EPVOUMeanMinFloat{-0.13247501850128173828125}
\def\EPVOUMeanMinKey{20013}
\def\EPVOUMeanStdDevFloat{0.34874284267425537109375}
\def\EPVOUMedianLen{151}
\def\EPVOUMedianMaxFloat{-21.605980587005614523832264239899814128875732421875}
\def\EPVOUMedianMaxKey{1283}
\def\EPVOUMedianMeanFloat{-26.4919223099512777253039530478417873382568359375}
\def\EPVOUMedianMeanKey{13293}
\def\EPVOUMedianMedianFloat{-30.618123772144318905930049368180334568023681640625}
\def\EPVOUMedianMedianKey{29726}
\def\EPVOUMedianMinFloat{-31.368831138610840270075641456060111522674560546875}
\def\EPVOUMedianMinKey{123}
\def\EPVOUMedianStdDevFloat{1.8123534487012780136439005218562670052051544189453125}
\def\EPVOUMinLen{151}
\def\EPVOUMinMaxFloat{-32.28704071044921875}
\def\EPVOUMinMaxKey{28778}
\def\EPVOUMinMeanFloat{-40.44071197509765625}
\def\EPVOUMinMeanKey{6159}
\def\EPVOUMinMedianFloat{-50.62209606170654296875}
\def\EPVOUMinMedianKey{4800}
\def\EPVOUMinMinFloat{-52.301570892333984375}
\def\EPVOUMinMinKey{4810}
\def\EPVOUMinStdDevFloat{3.3324086666107177734375}
\def\EPVOUOffDiagonalAbsLenLen{151}
\def\EPVOUOffDiagonalAbsLenMaxFloat{16256}
\def\EPVOUOffDiagonalAbsLenMaxKey{50}
\def\EPVOUOffDiagonalAbsLenMeanFloat{16256}
\def\EPVOUOffDiagonalAbsLenMeanKey{50}
\def\EPVOUOffDiagonalAbsLenMedianFloat{16256}
\def\EPVOUOffDiagonalAbsLenMedianKey{50}
\def\EPVOUOffDiagonalAbsLenMinFloat{16256}
\def\EPVOUOffDiagonalAbsLenMinKey{50}
\def\EPVOUOffDiagonalAbsLenStdDevFloat{0}
\def\EPVOUOffDiagonalAbsMaxLen{151}
\def\EPVOUOffDiagonalAbsMaxMaxFloat{52.301570892333984375}
\def\EPVOUOffDiagonalAbsMaxMaxKey{4810}
\def\EPVOUOffDiagonalAbsMaxMeanFloat{40.451282501220703125}
\def\EPVOUOffDiagonalAbsMaxMeanKey{6159}
\def\EPVOUOffDiagonalAbsMaxMedianFloat{32.4975948333740234375}
\def\EPVOUOffDiagonalAbsMaxMedianKey{12561}
\def\EPVOUOffDiagonalAbsMaxMinFloat{32.28704071044921875}
\def\EPVOUOffDiagonalAbsMaxMinKey{28778}
\def\EPVOUOffDiagonalAbsMaxStdDevFloat{3.319903850555419921875}
\def\EPVOUOffDiagonalAbsMeanLen{151}
\def\EPVOUOffDiagonalAbsMeanMaxFloat{9.89545917510986328125}
\def\EPVOUOffDiagonalAbsMeanMaxKey{123}
\def\EPVOUOffDiagonalAbsMeanMeanFloat{7.582829952239990234375}
\def\EPVOUOffDiagonalAbsMeanMeanKey{31308}
\def\EPVOUOffDiagonalAbsMeanMedianFloat{6.08774769306182861328125}
\def\EPVOUOffDiagonalAbsMeanMedianKey{5615}
\def\EPVOUOffDiagonalAbsMeanMinFloat{5.49636173248291015625}
\def\EPVOUOffDiagonalAbsMeanMinKey{20013}
\def\EPVOUOffDiagonalAbsMeanStdDevFloat{0.711129605770111083984375}
\def\EPVOUOffDiagonalAbsMedianLen{151}
\def\EPVOUOffDiagonalAbsMedianMaxFloat{0.12374465167522430419921875}
\def\EPVOUOffDiagonalAbsMedianMaxKey{16069}
\def\EPVOUOffDiagonalAbsMedianMeanFloat{0.085090697244648516583964692472363822162151336669921875}
\def\EPVOUOffDiagonalAbsMedianMeanKey{19451}
\def\EPVOUOffDiagonalAbsMedianMedianFloat{0.051020353101193911815602888282228377647697925567626953125}
\def\EPVOUOffDiagonalAbsMedianMedianKey{8893}
\def\EPVOUOffDiagonalAbsMedianMinFloat{0.04827053174376487454377837593710864894092082977294921875}
\def\EPVOUOffDiagonalAbsMedianMinKey{20013}
\def\EPVOUOffDiagonalAbsMedianStdDevFloat{0.0132944622708354269480235387845823424868285655975341796875}
\def\EPVOUOffDiagonalAbsMinLen{151}
\def\EPVOUOffDiagonalAbsMinMaxFloat{0.004761219024658203125}
\def\EPVOUOffDiagonalAbsMinMaxKey{26278}
\def\EPVOUOffDiagonalAbsMinMeanFloat{0.001140141277574002742767333984375}
\def\EPVOUOffDiagonalAbsMinMeanKey{6082}
\def\EPVOUOffDiagonalAbsMinMedianFloat{0.00000946223735809326171875}
\def\EPVOUOffDiagonalAbsMinMedianKey{12457}
\def\EPVOUOffDiagonalAbsMinMinFloat{0.000003516674041748046875}
\def\EPVOUOffDiagonalAbsMinMinKey{4729}
\def\EPVOUOffDiagonalAbsMinStdDevFloat{0.0010903165675699710845947265625}
\def\EPVOUOffDiagonalAbsStdDevLen{151}
\def\EPVOUOffDiagonalAbsStdDevMaxFloat{6.05219745635986328125}
\def\EPVOUOffDiagonalAbsStdDevMaxKey{123}
\def\EPVOUOffDiagonalAbsStdDevMeanFloat{5.035372257232666015625}
\def\EPVOUOffDiagonalAbsStdDevMeanKey{12493}
\def\EPVOUOffDiagonalAbsStdDevMedianFloat{4.4207856655120849609375}
\def\EPVOUOffDiagonalAbsStdDevMedianKey{20338}
\def\EPVOUOffDiagonalAbsStdDevMinFloat{4.385951995849609375}
\def\EPVOUOffDiagonalAbsStdDevMinKey{20013}
\def\EPVOUOffDiagonalAbsStdDevStdDevFloat{0.3163462579250335693359375}
\def\EPVOUOffDiagonalLenLen{151}
\def\EPVOUOffDiagonalLenMaxFloat{16256}
\def\EPVOUOffDiagonalLenMaxKey{50}
\def\EPVOUOffDiagonalLenMeanFloat{16256}
\def\EPVOUOffDiagonalLenMeanKey{50}
\def\EPVOUOffDiagonalLenMedianFloat{16256}
\def\EPVOUOffDiagonalLenMedianKey{50}
\def\EPVOUOffDiagonalLenMinFloat{16256}
\def\EPVOUOffDiagonalLenMinKey{50}
\def\EPVOUOffDiagonalLenStdDevFloat{0}
\def\EPVOUOffDiagonalMaxLen{151}
\def\EPVOUOffDiagonalMaxMaxFloat{42.1108245849609375}
\def\EPVOUOffDiagonalMaxMaxKey{13716}
\def\EPVOUOffDiagonalMaxMeanFloat{31.9938201904296875}
\def\EPVOUOffDiagonalMaxMeanKey{6155}
\def\EPVOUOffDiagonalMaxMedianFloat{25.884349822998046875}
\def\EPVOUOffDiagonalMaxMedianKey{20013}
\def\EPVOUOffDiagonalMaxMinFloat{25.0863704681396484375}
\def\EPVOUOffDiagonalMaxMinKey{2306}
\def\EPVOUOffDiagonalMaxStdDevFloat{3.1851155757904052734375}
\def\EPVOUOffDiagonalMeanLen{151}
\def\EPVOUOffDiagonalMeanMaxFloat{2.1340811252593994140625}
\def\EPVOUOffDiagonalMeanMaxKey{4157}
\def\EPVOUOffDiagonalMeanMeanFloat{1.29223668575286865234375}
\def\EPVOUOffDiagonalMeanMeanKey{22261}
\def\EPVOUOffDiagonalMeanMedianFloat{0.2231521308422088623046875}
\def\EPVOUOffDiagonalMeanMedianKey{19451}
\def\EPVOUOffDiagonalMeanMinFloat{-0.2125198543071746826171875}
\def\EPVOUOffDiagonalMeanMinKey{20013}
\def\EPVOUOffDiagonalMeanStdDevFloat{0.345861613750457763671875}
\def\EPVOUOffDiagonalMedianLen{151}
\def\EPVOUOffDiagonalMedianMaxFloat{-21.619298458099365234375}
\def\EPVOUOffDiagonalMedianMaxKey{1283}
\def\EPVOUOffDiagonalMedianMeanFloat{-26.5274879562933705301475129090249538421630859375}
\def\EPVOUOffDiagonalMedianMeanKey{17096}
\def\EPVOUOffDiagonalMedianMedianFloat{-30.630469048023226008581332280300557613372802734375}
\def\EPVOUOffDiagonalMedianMedianKey{29726}
\def\EPVOUOffDiagonalMedianMinFloat{-31.405017662048340554292735760100185871124267578125}
\def\EPVOUOffDiagonalMedianMinKey{123}
\def\EPVOUOffDiagonalMedianStdDevFloat{1.81643330523833679279732677969150245189666748046875}
\def\EPVOUOffDiagonalMinLen{151}
\def\EPVOUOffDiagonalMinMaxFloat{-32.28704071044921875}
\def\EPVOUOffDiagonalMinMaxKey{28778}
\def\EPVOUOffDiagonalMinMeanFloat{-40.44071197509765625}
\def\EPVOUOffDiagonalMinMeanKey{6159}
\def\EPVOUOffDiagonalMinMedianFloat{-50.62209606170654296875}
\def\EPVOUOffDiagonalMinMedianKey{4800}
\def\EPVOUOffDiagonalMinMinFloat{-52.301570892333984375}
\def\EPVOUOffDiagonalMinMinKey{4810}
\def\EPVOUOffDiagonalMinStdDevFloat{3.3324086666107177734375}
\def\EPVOUOffDiagonalStdDevLen{151}
\def\EPVOUOffDiagonalStdDevMaxFloat{11.42689800262451171875}
\def\EPVOUOffDiagonalStdDevMaxKey{123}
\def\EPVOUOffDiagonalStdDevMeanFloat{9.00793361663818359375}
\def\EPVOUOffDiagonalStdDevMeanKey{12552}
\def\EPVOUOffDiagonalStdDevMedianFloat{7.48386347293853759765625}
\def\EPVOUOffDiagonalStdDevMedianKey{5615}
\def\EPVOUOffDiagonalStdDevMinFloat{7.028613567352294921875}
\def\EPVOUOffDiagonalStdDevMinKey{20013}
\def\EPVOUOffDiagonalStdDevStdDevFloat{0.726432979106903076171875}
\def\EPVOUStdDevLen{151}
\def\EPVOUStdDevMaxFloat{11.4940948486328125}
\def\EPVOUStdDevMaxKey{123}
\def\EPVOUStdDevMeanFloat{9.094280242919921875}
\def\EPVOUStdDevMeanKey{12552}
\def\EPVOUStdDevMedianFloat{7.58029067516326904296875}
\def\EPVOUStdDevMedianKey{5615}
\def\EPVOUStdDevMinFloat{7.09371471405029296875}
\def\EPVOUStdDevMinKey{20013}
\def\EPVOUStdDevStdDevFloat{0.71998500823974609375}
\def\EQKEErrBoundMaxDiffExactLen{151}
\def\EQKEErrBoundMaxDiffExactMaxFloat{3.0429756641387939453125}
\def\EQKEErrBoundMaxDiffExactMaxKey{20013}
\def\EQKEErrBoundMaxDiffExactMeanFloat{1.7272548186068503728307632627547718584537506103515625}
\def\EQKEErrBoundMaxDiffExactMeanKey{17197}
\def\EQKEErrBoundMaxDiffExactMedianFloat{1.1247864663600921630859375}
\def\EQKEErrBoundMaxDiffExactMedianKey{12552}
\def\EQKEErrBoundMaxDiffExactMinFloat{1.1242678165435791015625}
\def\EQKEErrBoundMaxDiffExactMinKey{2549}
\def\EQKEErrBoundMaxDiffExactStdDevFloat{0.3105125741965866215110736447968520224094390869140625}
\def\EQKEErrBoundMaxDiffLen{151}
\def\EQKEErrBoundMaxDiffMaxFloat{8.7125339508056640625}
\def\EQKEErrBoundMaxDiffMaxKey{20013}
\def\EQKEErrBoundMaxDiffMeanFloat{5.21119032790329317350597193581052124500274658203125}
\def\EQKEErrBoundMaxDiffMeanKey{123}
\def\EQKEErrBoundMaxDiffMedianFloat{4.18486309051513671875}
\def\EQKEErrBoundMaxDiffMedianKey{17080}
\def\EQKEErrBoundMaxDiffMinFloat{4.0385189056396484375}
\def\EQKEErrBoundMaxDiffMinKey{2549}
\def\EQKEErrBoundMaxDiffStdDevFloat{0.5706513486772113452616395079530775547027587890625}
\def\EQKEErrBoundMaxDiffSubproductLen{151}
\def\EQKEErrBoundMaxDiffSubproductMaxFloat{8.7125339508056640625}
\def\EQKEErrBoundMaxDiffSubproductMaxKey{20013}
\def\EQKEErrBoundMaxDiffSubproductMeanFloat{5.21119032790329317350597193581052124500274658203125}
\def\EQKEErrBoundMaxDiffSubproductMeanKey{123}
\def\EQKEErrBoundMaxDiffSubproductMedianFloat{4.18486309051513671875}
\def\EQKEErrBoundMaxDiffSubproductMedianKey{17080}
\def\EQKEErrBoundMaxDiffSubproductMinFloat{4.0385189056396484375}
\def\EQKEErrBoundMaxDiffSubproductMinKey{2549}
\def\EQKEErrBoundMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMaxFloat{179.824432373046875}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMaxKey{20013}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMeanFloat{102.302513274135975507306284271180629730224609375}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMeanKey{2306}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMedianFloat{86.872837066650390625}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMedianKey{26932}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMinFloat{82.67822265625}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMinKey{2549}
\def\EQKEErrBoundMaxDiffSubproductRecursiveStdDevFloat{9.4818832522856180133885573013685643672943115234375}
\def\EQKEErrBoundMaxDiffSubproductStdDevFloat{0.5706513486772113452616395079530775547027587890625}
\def\EQKEErrBoundMeanMaxDiffLen{151}
\def\EQKEErrBoundMeanMaxDiffMaxFloat{8.80197429656982421875}
\def\EQKEErrBoundMeanMaxDiffMaxKey{20013}
\def\EQKEErrBoundMeanMaxDiffMeanFloat{5.2154952990298237835986583377234637737274169921875}
\def\EQKEErrBoundMeanMaxDiffMeanKey{29052}
\def\EQKEErrBoundMeanMaxDiffMedianFloat{4.17984616756439208984375}
\def\EQKEErrBoundMeanMaxDiffMedianKey{17080}
\def\EQKEErrBoundMeanMaxDiffMinFloat{4.0430088043212890625}
\def\EQKEErrBoundMeanMaxDiffMinKey{2549}
\def\EQKEErrBoundMeanMaxDiffStdDevFloat{0.57185251083535393323842299651005305349826812744140625}
\def\EQKEErrBoundMeanMaxDiffSubproductLen{151}
\def\EQKEErrBoundMeanMaxDiffSubproductMaxFloat{8.80197429656982421875}
\def\EQKEErrBoundMeanMaxDiffSubproductMaxKey{20013}
\def\EQKEErrBoundMeanMaxDiffSubproductMeanFloat{5.2154952990298237835986583377234637737274169921875}
\def\EQKEErrBoundMeanMaxDiffSubproductMeanKey{29052}
\def\EQKEErrBoundMeanMaxDiffSubproductMedianFloat{4.17984616756439208984375}
\def\EQKEErrBoundMeanMaxDiffSubproductMedianKey{17080}
\def\EQKEErrBoundMeanMaxDiffSubproductMinFloat{4.0430088043212890625}
\def\EQKEErrBoundMeanMaxDiffSubproductMinKey{2549}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMaxFloat{181.3256988525390625}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMaxKey{20013}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMeanFloat{102.10632122115583797494764439761638641357421875}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMeanKey{2306}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMedianFloat{86.661590576171875}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMedianKey{26932}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMinFloat{81.919342041015625}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMinKey{2549}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveStdDevFloat{9.5543243092486846990141202695667743682861328125}
\def\EQKEErrBoundMeanMaxDiffSubproductStdDevFloat{0.57185251083535393323842299651005305349826812744140625}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMaxFloat{187.469207763671875}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMaxKey{20013}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMeanFloat{104.0375475851905235913363867439329624176025390625}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMeanKey{1681}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMedianFloat{87.287982940673828125}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMedianKey{26932}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMinFloat{83.86852264404296875}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMinKey{2549}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveStdDevFloat{9.91771665649914524465202703140676021575927734375}
\def\EQKEErrBoundSvdLen{151}
\def\EQKEErrBoundSvdMaxFloat{17.6198482513427734375}
\def\EQKEErrBoundSvdMaxKey{4800}
\def\EQKEErrBoundSvdMeanFloat{12.3571284275181252354514072067104279994964599609375}
\def\EQKEErrBoundSvdMeanKey{18668}
\def\EQKEErrBoundSvdMedianFloat{8.531565189361572265625}
\def\EQKEErrBoundSvdMedianKey{1696}
\def\EQKEErrBoundSvdMinFloat{8.23297023773193359375}
\def\EQKEErrBoundSvdMinKey{2549}
\def\EQKEErrBoundSvdStdDevFloat{1.78860979247000440039983004680834710597991943359375}
\def\EQKEErrFirstSingularLen{151}
\def\EQKEErrFirstSingularMaxFloat{12.4591217041015625}
\def\EQKEErrFirstSingularMaxKey{4800}
\def\EQKEErrFirstSingularMeanFloat{8.7378095254203334008025194634683430194854736328125}
\def\EQKEErrFirstSingularMeanKey{18668}
\def\EQKEErrFirstSingularMedianFloat{6.03272759914398193359375}
\def\EQKEErrFirstSingularMedianKey{1696}
\def\EQKEErrFirstSingularMinFloat{5.821588039398193359375}
\def\EQKEErrFirstSingularMinKey{2549}
\def\EQKEErrFirstSingularSqrtTwoLen{151}
\def\EQKEErrFirstSingularSqrtTwoMaxFloat{17.6198577880859375}
\def\EQKEErrFirstSingularSqrtTwoMaxKey{4800}
\def\EQKEErrFirstSingularSqrtTwoMeanFloat{12.35712854120115622436060220934450626373291015625}
\def\EQKEErrFirstSingularSqrtTwoMeanKey{18668}
\def\EQKEErrFirstSingularSqrtTwoMedianFloat{8.5315647125244140625}
\def\EQKEErrFirstSingularSqrtTwoMedianKey{1696}
\def\EQKEErrFirstSingularSqrtTwoMinFloat{8.23296833038330078125}
\def\EQKEErrFirstSingularSqrtTwoMinKey{2549}
\def\EQKEErrFirstSingularSqrtTwoStdDevFloat{1.7886095120454783558017197719891555607318878173828125}
\def\EQKEErrFirstSingularStdDevFloat{1.2647379871635118231409933287068270146846771240234375}
\def\EQKEErrFroNormLen{151}
\def\EQKEErrFroNormMaxFloat{18.4571437835693359375}
\def\EQKEErrFroNormMaxKey{4800}
\def\EQKEErrFroNormMeanFloat{15.3931930554623637164013416622765362262725830078125}
\def\EQKEErrFroNormMeanKey{19917}
\def\EQKEErrFroNormMedianFloat{12.5707643032073974609375}
\def\EQKEErrFroNormMedianKey{7884}
\def\EQKEErrFroNormMinFloat{12.23170375823974609375}
\def\EQKEErrFroNormMinKey{2549}
\def\EQKEErrFroNormSqrtTwoLen{151}
\def\EQKEErrFroNormSqrtTwoMaxFloat{26.1023426055908203125}
\def\EQKEErrFroNormSqrtTwoMaxKey{4800}
\def\EQKEErrFroNormSqrtTwoMeanFloat{21.769261998056574469728730036877095699310302734375}
\def\EQKEErrFroNormSqrtTwoMeanKey{19917}
\def\EQKEErrFroNormSqrtTwoMedianFloat{17.77774524688720703125}
\def\EQKEErrFroNormSqrtTwoMedianKey{7884}
\def\EQKEErrFroNormSqrtTwoMinFloat{17.29824066162109375}
\def\EQKEErrFroNormSqrtTwoMinKey{2549}
\def\EQKEErrFroNormSqrtTwoStdDevFloat{1.74785684379334771421099503641016781330108642578125}
\def\EQKEErrFroNormStdDevFloat{1.23592144396627379165920501691289246082305908203125}
\def\EQKEErrLen{16384}
\def\EQKEErrMaxAbsLen{151}
\def\EQKEErrMaxAbsMaxFloat{2.1047303676605224609375}
\def\EQKEErrMaxAbsMaxKey{20013}
\def\EQKEErrMaxAbsMeanFloat{0.97003772914014907424729017293429933488368988037109375}
\def\EQKEErrMaxAbsMeanKey{50}
\def\EQKEErrMaxAbsMedianFloat{0.6215162575244903564453125}
\def\EQKEErrMaxAbsMedianKey{24566}
\def\EQKEErrMaxAbsMinFloat{0.600776612758636474609375}
\def\EQKEErrMaxAbsMinKey{12552}
\def\EQKEErrMaxAbsStdDevFloat{0.182169802801432856309560293084359727799892425537109375}
\def\EQKEErrMaxLen{151}
\def\EQKEErrMaxMaxFloat{2.1047303676605224609375}
\def\EQKEErrMaxMaxKey{20013}
\def\EQKEErrMaxMeanFloat{0.9169232845306396484375}
\def\EQKEErrMaxMeanKey{22401}
\def\EQKEErrMaxMedianFloat{0.5802666246891021728515625}
\def\EQKEErrMaxMedianKey{12552}
\def\EQKEErrMaxMinFloat{0.5309312343597412109375}
\def\EQKEErrMaxMinKey{2549}
\def\EQKEErrMaxRowDiffLen{151}
\def\EQKEErrMaxRowDiffMaxFloat{3.0429756641387939453125}
\def\EQKEErrMaxRowDiffMaxKey{20013}
\def\EQKEErrMaxRowDiffMeanFloat{1.7272548186068503728307632627547718584537506103515625}
\def\EQKEErrMaxRowDiffMeanKey{17197}
\def\EQKEErrMaxRowDiffMedianFloat{1.1247864663600921630859375}
\def\EQKEErrMaxRowDiffMedianKey{12552}
\def\EQKEErrMaxRowDiffMinFloat{1.1242678165435791015625}
\def\EQKEErrMaxRowDiffMinKey{2549}
\def\EQKEErrMaxRowDiffStdDevFloat{0.3105125741965866215110736447968520224094390869140625}
\def\EQKEErrMaxStdDevFloat{0.181504666805267333984375}
\def\EQKEErrMeanDimZeroNormLen{151}
\def\EQKEErrMeanDimZeroNormMaxFloat{0.0621106438338756561279296875}
\def\EQKEErrMeanDimZeroNormMaxKey{29052}
\def\EQKEErrMeanDimZeroNormMeanFloat{0.0211055911984911435952394498372086673043668270111083984375}
\def\EQKEErrMeanDimZeroNormMeanKey{913}
\def\EQKEErrMeanDimZeroNormMedianFloat{0.007380969240330159664154052734375}
\def\EQKEErrMeanDimZeroNormMedianKey{8299}
\def\EQKEErrMeanDimZeroNormMinFloat{0.006125806830823421478271484375}
\def\EQKEErrMeanDimZeroNormMinKey{4157}
\def\EQKEErrMeanDimZeroNormStdDevFloat{0.0085982254848646320899430151030173874460160732269287109375}
\def\EQKEErrMeanLen{151}
\def\EQKEErrMeanMaxFloat{0.0004821250331588089466094970703125}
\def\EQKEErrMeanMaxKey{22286}
\def\EQKEErrMeanMeanFloat{0.00003417634798097424209117889404296875}
\def\EQKEErrMeanMeanKey{5781}
\def\EQKEErrMeanMedianFloat{-0.000284809721051715314388275146484375}
\def\EQKEErrMeanMedianKey{4800}
\def\EQKEErrMeanMinFloat{-0.000291974633000791072845458984375}
\def\EQKEErrMeanMinKey{2306}
\def\EQKEErrMeanStdDevFloat{0.000153981571202166378498077392578125}
\def\EQKEErrMedianLen{151}
\def\EQKEErrMedianMaxFloat{-0.2968424765765667050487763845012523233890533447265625}
\def\EQKEErrMedianMaxKey{2549}
\def\EQKEErrMedianMeanFloat{-0.403767551520210210558303742800489999353885650634765625}
\def\EQKEErrMedianMeanKey{9132}
\def\EQKEErrMedianMedianFloat{-0.50645832151174541291283048849436454474925994873046875}
\def\EQKEErrMedianMedianKey{4800}
\def\EQKEErrMedianMinFloat{-0.5100303918123245683347022350062616169452667236328125}
\def\EQKEErrMedianMinKey{2306}
\def\EQKEErrMedianStdDevFloat{0.0401531719774988193893960897185024805366992950439453125}
\def\EQKEErrMinLen{151}
\def\EQKEErrMinMaxFloat{-0.565237939357757568359375}
\def\EQKEErrMinMaxKey{1696}
\def\EQKEErrMinMeanFloat{-0.9081857204437255859375}
\def\EQKEErrMinMeanKey{19093}
\def\EQKEErrMinMedianFloat{-1.398045122623443603515625}
\def\EQKEErrMinMedianKey{15622}
\def\EQKEErrMinMinFloat{-1.45683968067169189453125}
\def\EQKEErrMinMinKey{2306}
\def\EQKEErrMinStdDevFloat{0.1620748341083526611328125}
\def\EQKEErrProdFirstSingularLen{151}
\def\EQKEErrProdFirstSingularMaxFloat{43.80983837992433649333179346285760402679443359375}
\def\EQKEErrProdFirstSingularMaxKey{19093}
\def\EQKEErrProdFirstSingularMeanFloat{37.35113610678779849649799871258437633514404296875}
\def\EQKEErrProdFirstSingularMeanKey{17194}
\def\EQKEErrProdFirstSingularMedianFloat{30.59429568821036582448869012296199798583984375}
\def\EQKEErrProdFirstSingularMedianKey{26932}
\def\EQKEErrProdFirstSingularMinFloat{29.62505945735365031623587128706276416778564453125}
\def\EQKEErrProdFirstSingularMinKey{24202}
\def\EQKEErrProdFirstSingularSqrtTwoLen{151}
\def\EQKEErrProdFirstSingularSqrtTwoMaxFloat{61.95646760226234306401238427497446537017822265625}
\def\EQKEErrProdFirstSingularSqrtTwoMaxKey{19093}
\def\EQKEErrProdFirstSingularSqrtTwoMeanFloat{52.82248325226270679877416114322841167449951171875}
\def\EQKEErrProdFirstSingularSqrtTwoMeanKey{17194}
\def\EQKEErrProdFirstSingularSqrtTwoMedianFloat{43.26686789351980877427195082418620586395263671875}
\def\EQKEErrProdFirstSingularSqrtTwoMedianKey{26932}
\def\EQKEErrProdFirstSingularSqrtTwoMinFloat{41.89616087069885708160654758103191852569580078125}
\def\EQKEErrProdFirstSingularSqrtTwoMinKey{24202}
\def\EQKEErrProdFirstSingularSqrtTwoStdDevFloat{4.18633834412836325356011002440936863422393798828125}
\def\EQKEErrProdFirstSingularStdDevFloat{2.9601882314744276669671307899989187717437744140625}
\def\EQKEErrProdFroNormLen{151}
\def\EQKEErrProdFroNormMaxFloat{2843.05012356951601759647019207477569580078125}
\def\EQKEErrProdFroNormMaxKey{19004}
\def\EQKEErrProdFroNormMeanFloat{2503.5649435196601189090870320796966552734375}
\def\EQKEErrProdFroNormMeanKey{11598}
\def\EQKEErrProdFroNormMedianFloat{2258.350695347902728826738893985748291015625}
\def\EQKEErrProdFroNormMedianKey{4157}
\def\EQKEErrProdFroNormMinFloat{2239.17769463566582999192178249359130859375}
\def\EQKEErrProdFroNormMinKey{7884}
\def\EQKEErrProdFroNormSqrtTwoLen{151}
\def\EQKEErrProdFroNormSqrtTwoMaxFloat{4020.68004325851370595046319067478179931640625}
\def\EQKEErrProdFroNormSqrtTwoMaxKey{19004}
\def\EQKEErrProdFroNormSqrtTwoMeanFloat{3540.575497407335205934941768646240234375}
\def\EQKEErrProdFroNormSqrtTwoMeanKey{11598}
\def\EQKEErrProdFroNormSqrtTwoMedianFloat{3193.79018195571416072198189795017242431640625}
\def\EQKEErrProdFroNormSqrtTwoMedianKey{4157}
\def\EQKEErrProdFroNormSqrtTwoMinFloat{3166.6754643170797862694598734378814697265625}
\def\EQKEErrProdFroNormSqrtTwoMinKey{7884}
\def\EQKEErrProdFroNormSqrtTwoStdDevFloat{165.211521066418953296306426636874675750732421875}
\def\EQKEErrProdFroNormStdDevFloat{116.822186876208974126711837016046047210693359375}
\def\EQKEErrSimpleFirstSingularLen{151}
\def\EQKEErrSimpleFirstSingularMaxFloat{22.9927005767822265625}
\def\EQKEErrSimpleFirstSingularMaxKey{29052}
\def\EQKEErrSimpleFirstSingularMeanFloat{14.5339764538190223674973822198808193206787109375}
\def\EQKEErrSimpleFirstSingularMeanKey{913}
\def\EQKEErrSimpleFirstSingularMedianFloat{9.3953397274017333984375}
\def\EQKEErrSimpleFirstSingularMedianKey{10248}
\def\EQKEErrSimpleFirstSingularMinFloat{8.2086639404296875}
\def\EQKEErrSimpleFirstSingularMinKey{12552}
\def\EQKEErrSimpleFirstSingularSqrtTwoLen{151}
\def\EQKEErrSimpleFirstSingularSqrtTwoMaxFloat{32.516590118408203125}
\def\EQKEErrSimpleFirstSingularSqrtTwoMaxKey{29052}
\def\EQKEErrSimpleFirstSingularSqrtTwoMeanFloat{20.55414626772040520563678001053631305694580078125}
\def\EQKEErrSimpleFirstSingularSqrtTwoMeanKey{913}
\def\EQKEErrSimpleFirstSingularSqrtTwoMedianFloat{13.28701686859130859375}
\def\EQKEErrSimpleFirstSingularSqrtTwoMedianKey{10248}
\def\EQKEErrSimpleFirstSingularSqrtTwoMinFloat{11.60880374908447265625}
\def\EQKEErrSimpleFirstSingularSqrtTwoMinKey{12552}
\def\EQKEErrSimpleFirstSingularSqrtTwoStdDevFloat{3.81918685568273108543735361308790743350982666015625}
\def\EQKEErrSimpleFirstSingularStdDevFloat{2.700572941709574958935036192997358739376068115234375}
\def\EQKEErrSimpleFroNormLen{151}
\def\EQKEErrSimpleFroNormMaxFloat{28.2850666046142578125}
\def\EQKEErrSimpleFroNormMaxKey{29052}
\def\EQKEErrSimpleFroNormMeanFloat{21.6783301751345192087683244608342647552490234375}
\def\EQKEErrSimpleFroNormMeanKey{29565}
\def\EQKEErrSimpleFroNormMedianFloat{16.484009265899658203125}
\def\EQKEErrSimpleFroNormMedianKey{1696}
\def\EQKEErrSimpleFroNormMinFloat{16.1788196563720703125}
\def\EQKEErrSimpleFroNormMinKey{12552}
\def\EQKEErrSimpleFroNormSqrtTwoLen{151}
\def\EQKEErrSimpleFroNormSqrtTwoMaxFloat{40.001125335693359375}
\def\EQKEErrSimpleFroNormSqrtTwoMaxKey{29052}
\def\EQKEErrSimpleFroNormSqrtTwoMeanFloat{30.657788106147815909707787795923650264739990234375}
\def\EQKEErrSimpleFroNormSqrtTwoMeanKey{29565}
\def\EQKEErrSimpleFroNormSqrtTwoMedianFloat{23.311908721923828125}
\def\EQKEErrSimpleFroNormSqrtTwoMedianKey{1696}
\def\EQKEErrSimpleFroNormSqrtTwoMinFloat{22.880306243896484375}
\def\EQKEErrSimpleFroNormSqrtTwoMinKey{12552}
\def\EQKEErrSimpleFroNormSqrtTwoStdDevFloat{3.091501296500562379065968343638814985752105712890625}
\def\EQKEErrSimpleFroNormStdDevFloat{2.186021478000699236332593500264920294284820556640625}
\def\EQKEErrSimpleLen{16384}
\def\EQKEErrSimpleMaxAbsLen{151}
\def\EQKEErrSimpleMaxAbsMaxFloat{3.6522147655487060546875}
\def\EQKEErrSimpleMaxAbsMaxKey{20013}
\def\EQKEErrSimpleMaxAbsMeanFloat{1.510619542456620667536526525509543716907501220703125}
\def\EQKEErrSimpleMaxAbsMeanKey{5358}
\def\EQKEErrSimpleMaxAbsMedianFloat{0.96014416217803955078125}
\def\EQKEErrSimpleMaxAbsMedianKey{1696}
\def\EQKEErrSimpleMaxAbsMinFloat{0.90133297443389892578125}
\def\EQKEErrSimpleMaxAbsMinKey{12552}
\def\EQKEErrSimpleMaxAbsStdDevFloat{0.324299577892585288996230019620270468294620513916015625}
\def\EQKEErrSimpleMaxLen{151}
\def\EQKEErrSimpleMaxMaxFloat{3.6522147655487060546875}
\def\EQKEErrSimpleMaxMaxKey{20013}
\def\EQKEErrSimpleMaxMeanFloat{1.343785762786865234375}
\def\EQKEErrSimpleMaxMeanKey{1895}
\def\EQKEErrSimpleMaxMedianFloat{0.77354888617992401123046875}
\def\EQKEErrSimpleMaxMedianKey{4157}
\def\EQKEErrSimpleMaxMinFloat{0.74744451045989990234375}
\def\EQKEErrSimpleMaxMinKey{4729}
\def\EQKEErrSimpleMaxRowDiffLen{151}
\def\EQKEErrSimpleMaxRowDiffMaxFloat{4.45621013641357421875}
\def\EQKEErrSimpleMaxRowDiffMaxKey{20013}
\def\EQKEErrSimpleMaxRowDiffMeanFloat{2.453070016886224724572684863233007490634918212890625}
\def\EQKEErrSimpleMaxRowDiffMeanKey{6204}
\def\EQKEErrSimpleMaxRowDiffMedianFloat{1.531414806842803955078125}
\def\EQKEErrSimpleMaxRowDiffMedianKey{27484}
\def\EQKEErrSimpleMaxRowDiffMinFloat{1.4557473659515380859375}
\def\EQKEErrSimpleMaxRowDiffMinKey{12552}
\def\EQKEErrSimpleMaxRowDiffStdDevFloat{0.485868564729872332019766645316849462687969207763671875}
\def\EQKEErrSimpleMaxStdDevFloat{0.3469623625278472900390625}
\def\EQKEErrSimpleMeanDimZeroNormLen{151}
\def\EQKEErrSimpleMeanDimZeroNormMaxFloat{0.233670771121978759765625}
\def\EQKEErrSimpleMeanDimZeroNormMaxKey{19451}
\def\EQKEErrSimpleMeanDimZeroNormMeanFloat{0.056360964518385812949130553306531510315835475921630859375}
\def\EQKEErrSimpleMeanDimZeroNormMeanKey{1895}
\def\EQKEErrSimpleMeanDimZeroNormMedianFloat{0.010559146874584257602691650390625}
\def\EQKEErrSimpleMeanDimZeroNormMedianKey{13654}
\def\EQKEErrSimpleMeanDimZeroNormMinFloat{0.0066243200562894344329833984375}
\def\EQKEErrSimpleMeanDimZeroNormMinKey{4157}
\def\EQKEErrSimpleMeanDimZeroNormStdDevFloat{0.037179366683184507380577343838012893684208393096923828125}
\def\EQKEErrSimpleMeanLen{151}
\def\EQKEErrSimpleMeanMaxFloat{0.0136914961040019989013671875}
\def\EQKEErrSimpleMeanMaxKey{19451}
\def\EQKEErrSimpleMeanMeanFloat{0.0002781334333121776580810546875}
\def\EQKEErrSimpleMeanMeanKey{9816}
\def\EQKEErrSimpleMeanMedianFloat{-0.00782429776154458522796630859375}
\def\EQKEErrSimpleMeanMedianKey{27671}
\def\EQKEErrSimpleMeanMinFloat{-0.007905679754912853240966796875}
\def\EQKEErrSimpleMeanMinKey{4810}
\def\EQKEErrSimpleMeanStdDevFloat{0.00244754576124250888824462890625}
\def\EQKEErrSimpleMedianLen{151}
\def\EQKEErrSimpleMedianMaxFloat{-0.403708663284778557223120287744677625596523284912109375}
\def\EQKEErrSimpleMedianMaxKey{12493}
\def\EQKEErrSimpleMedianMeanFloat{-0.59660878135865880178556608370854519307613372802734375}
\def\EQKEErrSimpleMedianMeanKey{17096}
\def\EQKEErrSimpleMedianMedianFloat{-0.939138272404670626514189279987476766109466552734375}
\def\EQKEErrSimpleMedianMedianKey{29052}
\def\EQKEErrSimpleMedianMinFloat{-0.9669608175754547119140625}
\def\EQKEErrSimpleMedianMinKey{27671}
\def\EQKEErrSimpleMedianStdDevFloat{0.1074648672741953803200232187009532935917377471923828125}
\def\EQKEErrSimpleMinLen{151}
\def\EQKEErrSimpleMinMaxFloat{-0.72641575336456298828125}
\def\EQKEErrSimpleMinMaxKey{12493}
\def\EQKEErrSimpleMinMeanFloat{-1.33956682682037353515625}
\def\EQKEErrSimpleMinMeanKey{15662}
\def\EQKEErrSimpleMinMedianFloat{-2.22488117218017578125}
\def\EQKEErrSimpleMinMedianKey{123}
\def\EQKEErrSimpleMinMinFloat{-2.3396904468536376953125}
\def\EQKEErrSimpleMinMinKey{29052}
\def\EQKEErrSimpleMinStdDevFloat{0.298028528690338134765625}
\def\EQKEErrSimpleStdDevLen{151}
\def\EQKEErrSimpleStdDevMaxFloat{0.22097329795360565185546875}
\def\EQKEErrSimpleStdDevMaxKey{29052}
\def\EQKEErrSimpleStdDevMeanFloat{0.1693451702594757080078125}
\def\EQKEErrSimpleStdDevMeanKey{29565}
\def\EQKEErrSimpleStdDevMedianFloat{0.128780804574489593505859375}
\def\EQKEErrSimpleStdDevMedianKey{1696}
\def\EQKEErrSimpleStdDevMinFloat{0.1263960301876068115234375}
\def\EQKEErrSimpleStdDevMinKey{12552}
\def\EQKEErrSimpleStdDevStdDevFloat{0.0170671679079532623291015625}
\def\EQKEErrSimpleWithAttnScaleFirstSingularLen{151}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMaxFloat{4.064573764801025390625}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMaxKey{29052}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMeanFloat{2.569268355306410622773682916886173188686370849609375}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMeanKey{913}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMedianFloat{1.66087710857391357421875}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMedianKey{10248}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMinFloat{1.45110046863555908203125}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMinKey{12552}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoLen{151}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMaxFloat{5.748175144195556640625}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMaxKey{29052}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMeanFloat{3.63349409608651452430194694898091256618499755859375}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMeanKey{913}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMedianFloat{2.348834931850433349609375}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMedianKey{10248}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMinFloat{2.052165985107421875}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMinKey{12552}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoStdDevFloat{0.67514325104647709974159397461335174739360809326171875}
\def\EQKEErrSimpleWithAttnScaleFirstSingularStdDevFloat{0.47739837242058003052846970604150556027889251708984375}
\def\EQKEErrSimpleWithAttnScaleFroNormLen{151}
\def\EQKEErrSimpleWithAttnScaleFroNormMaxFloat{5.000140666961669921875}
\def\EQKEErrSimpleWithAttnScaleFroNormMaxKey{29052}
\def\EQKEErrSimpleWithAttnScaleFroNormMeanFloat{3.832223631688301157538489860598929226398468017578125}
\def\EQKEErrSimpleWithAttnScaleFroNormMeanKey{29565}
\def\EQKEErrSimpleWithAttnScaleFroNormMedianFloat{2.913988769054412841796875}
\def\EQKEErrSimpleWithAttnScaleFroNormMedianKey{1696}
\def\EQKEErrSimpleWithAttnScaleFroNormMinFloat{2.860038280487060546875}
\def\EQKEErrSimpleWithAttnScaleFroNormMinKey{12552}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoLen{151}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMaxFloat{7.071266651153564453125}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMaxKey{29052}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMeanFloat{5.41958252483645797070721528143621981143951416015625}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMeanKey{29565}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMedianFloat{4.12100231647491455078125}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMedianKey{1696}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMinFloat{4.044704914093017578125}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMinKey{12552}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoStdDevFloat{0.54650534724981458811754464477417059242725372314453125}
\def\EQKEErrSimpleWithAttnScaleFroNormStdDevFloat{0.386437651058684827898304092741454951465129852294921875}
\def\EQKEErrSimpleWithAttnScaleLen{16384}
\def\EQKEErrSimpleWithAttnScaleMaxAbsLen{151}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMaxFloat{0.645626485347747802734375}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMaxKey{20013}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMeanFloat{0.2670423358876183872467890978441573679447174072265625}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMeanKey{5358}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMedianFloat{0.169731117784976959228515625}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMedianKey{1696}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMinFloat{0.15933467447757720947265625}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMinKey{12552}
\def\EQKEErrSimpleWithAttnScaleMaxAbsStdDevFloat{0.057328608741157936756760449270586832426488399505615234375}
\def\EQKEErrSimpleWithAttnScaleMaxLen{151}
\def\EQKEErrSimpleWithAttnScaleMaxMaxFloat{0.645626485347747802734375}
\def\EQKEErrSimpleWithAttnScaleMaxMaxKey{20013}
\def\EQKEErrSimpleWithAttnScaleMaxMeanFloat{0.2375499904155731201171875}
\def\EQKEErrSimpleWithAttnScaleMaxMeanKey{1895}
\def\EQKEErrSimpleWithAttnScaleMaxMedianFloat{0.1367454230785369873046875}
\def\EQKEErrSimpleWithAttnScaleMaxMedianKey{4157}
\def\EQKEErrSimpleWithAttnScaleMaxMinFloat{0.1321307718753814697265625}
\def\EQKEErrSimpleWithAttnScaleMaxMinKey{4729}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffLen{151}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMaxFloat{0.787754118442535400390625}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMaxKey{20013}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMeanFloat{0.433645619659234371479072933652787469327449798583984375}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMeanKey{6204}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMedianFloat{0.27071844041347503662109375}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMedianKey{27484}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMinFloat{0.25734221935272216796875}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMinKey{12552}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffStdDevFloat{0.085890239717642036243461234334972687065601348876953125}
\def\EQKEErrSimpleWithAttnScaleMaxStdDevFloat{0.0613348670303821563720703125}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormLen{151}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMaxFloat{0.041307546198368072509765625}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMaxKey{19451}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMeanFloat{0.00996330510038537058015162273250098223797976970672607421875}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMeanKey{1895}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMedianFloat{0.00186661214684136211872100830078125}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMedianKey{13654}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMinFloat{0.001171027426607906818389892578125}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMinKey{4157}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormStdDevFloat{0.00657244541888004317475857618546797311864793300628662109375}
\def\EQKEErrSimpleWithAttnScaleMeanLen{151}
\def\EQKEErrSimpleWithAttnScaleMeanMaxFloat{0.0024203383363783359527587890625}
\def\EQKEErrSimpleWithAttnScaleMeanMaxKey{19451}
\def\EQKEErrSimpleWithAttnScaleMeanMeanFloat{0.00004916750549455173313617706298828125}
\def\EQKEErrSimpleWithAttnScaleMeanMeanKey{9816}
\def\EQKEErrSimpleWithAttnScaleMeanMedianFloat{-0.0013831544783897697925567626953125}
\def\EQKEErrSimpleWithAttnScaleMeanMedianKey{27671}
\def\EQKEErrSimpleWithAttnScaleMeanMinFloat{-0.00139754009433090686798095703125}
\def\EQKEErrSimpleWithAttnScaleMeanMinKey{4810}
\def\EQKEErrSimpleWithAttnScaleMeanStdDevFloat{0.00043266909779049456119537353515625}
\def\EQKEErrSimpleWithAttnScaleMedianLen{151}
\def\EQKEErrSimpleWithAttnScaleMedianMaxFloat{-0.07136628095060586207676323056148248724639415740966796875}
\def\EQKEErrSimpleWithAttnScaleMedianMaxKey{12493}
\def\EQKEErrSimpleWithAttnScaleMedianMeanFloat{-0.10546653060082171460276612151574227027595043182373046875}
\def\EQKEErrSimpleWithAttnScaleMedianMeanKey{17096}
\def\EQKEErrSimpleWithAttnScaleMedianMedianFloat{-0.16601776830852033040031301425187848508358001708984375}
\def\EQKEErrSimpleWithAttnScaleMedianMedianKey{29052}
\def\EQKEErrSimpleWithAttnScaleMedianMinFloat{-0.1709361421316862028607630463739042170345783233642578125}
\def\EQKEErrSimpleWithAttnScaleMedianMinKey{27671}
\def\EQKEErrSimpleWithAttnScaleMedianStdDevFloat{0.0189972848240554277599034804779876139946281909942626953125}
\def\EQKEErrSimpleWithAttnScaleMinLen{151}
\def\EQKEErrSimpleWithAttnScaleMinMaxFloat{-0.128413379192352294921875}
\def\EQKEErrSimpleWithAttnScaleMinMaxKey{12493}
\def\EQKEErrSimpleWithAttnScaleMinMeanFloat{-0.23680417239665985107421875}
\def\EQKEErrSimpleWithAttnScaleMinMeanKey{15662}
\def\EQKEErrSimpleWithAttnScaleMinMedianFloat{-0.39330713450908660888671875}
\def\EQKEErrSimpleWithAttnScaleMinMedianKey{123}
\def\EQKEErrSimpleWithAttnScaleMinMinFloat{-0.4136027395725250244140625}
\def\EQKEErrSimpleWithAttnScaleMinMinKey{29052}
\def\EQKEErrSimpleWithAttnScaleMinStdDevFloat{0.05268450081348419189453125}
\def\EQKEErrSimpleWithAttnScaleStdDevLen{151}
\def\EQKEErrSimpleWithAttnScaleStdDevMaxFloat{0.0390629284083843231201171875}
\def\EQKEErrSimpleWithAttnScaleStdDevMaxKey{29052}
\def\EQKEErrSimpleWithAttnScaleStdDevMeanFloat{0.02993627823889255523681640625}
\def\EQKEErrSimpleWithAttnScaleStdDevMeanKey{29565}
\def\EQKEErrSimpleWithAttnScaleStdDevMedianFloat{0.0227654441259801387786865234375}
\def\EQKEErrSimpleWithAttnScaleStdDevMedianKey{1696}
\def\EQKEErrSimpleWithAttnScaleStdDevMinFloat{0.02234387211501598358154296875}
\def\EQKEErrSimpleWithAttnScaleStdDevMinKey{12552}
\def\EQKEErrSimpleWithAttnScaleStdDevStdDevFloat{0.00301707745529711246490478515625}
\def\EQKEErrStdDevLen{151}
\def\EQKEErrStdDevMaxFloat{0.1441961824893951416015625}
\def\EQKEErrStdDevMaxKey{4800}
\def\EQKEErrStdDevMeanFloat{0.120259217917919158935546875}
\def\EQKEErrStdDevMeanKey{19917}
\def\EQKEErrStdDevMedianFloat{0.09820903278887271881103515625}
\def\EQKEErrStdDevMedianKey{7884}
\def\EQKEErrStdDevMinFloat{0.095560200512409210205078125}
\def\EQKEErrStdDevMinKey{2549}
\def\EQKEErrStdDevStdDevFloat{0.009655636735260486602783203125}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactLen{151}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMaxFloat{0.537927210330963134765625}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMaxKey{20013}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMeanFloat{0.3053384064049120549810822922154329717159271240234375}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMeanKey{17197}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMedianFloat{0.1988360323011875152587890625}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMedianKey{12552}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMinFloat{0.19874431192874908447265625}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMinKey{2549}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactStdDevFloat{0.054891388580060616886324709184918901883065700531005859375}
\def\EQKEErrWithAttnScaleBoundMaxDiffLen{151}
\def\EQKEErrWithAttnScaleBoundMaxDiffMaxFloat{1.540173053741455078125}
\def\EQKEErrWithAttnScaleBoundMaxDiffMaxKey{20013}
\def\EQKEErrWithAttnScaleBoundMaxDiffMeanFloat{0.92121702945785022276226072790450416505336761474609375}
\def\EQKEErrWithAttnScaleBoundMaxDiffMeanKey{123}
\def\EQKEErrWithAttnScaleBoundMaxDiffMedianFloat{0.73978631198406219482421875}
\def\EQKEErrWithAttnScaleBoundMaxDiffMedianKey{17080}
\def\EQKEErrWithAttnScaleBoundMaxDiffMinFloat{0.71391618251800537109375}
\def\EQKEErrWithAttnScaleBoundMaxDiffMinKey{2549}
\def\EQKEErrWithAttnScaleBoundMaxDiffStdDevFloat{0.10087786259742685668339134963389369659125804901123046875}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductLen{151}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMaxFloat{1.540173053741455078125}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMaxKey{20013}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMeanFloat{0.92121702945785022276226072790450416505336761474609375}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMeanKey{123}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMedianFloat{0.73978631198406219482421875}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMedianKey{17080}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMinFloat{0.71391618251800537109375}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMinKey{2549}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMaxFloat{31.7887706756591796875}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMaxKey{20013}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMeanFloat{18.084700521254379879110274487175047397613525390625}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMeanKey{2306}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMedianFloat{15.35709381103515625}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMedianKey{26932}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMinFloat{14.61558246612548828125}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMinKey{2549}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveStdDevFloat{1.676176088795545471299419659771956503391265869140625}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductStdDevFloat{0.10087786259742685668339134963389369659125804901123046875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffLen{151}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMaxFloat{1.555984020233154296875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMaxKey{20013}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMeanFloat{0.921978034325782846991614860598929226398468017578125}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMeanKey{29052}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMedianFloat{0.7388994395732879638671875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMedianKey{17080}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMinFloat{0.714709758758544921875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMinKey{2549}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffStdDevFloat{0.101090199198665076085745795353432185947895050048828125}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductLen{151}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMaxFloat{1.555984020233154296875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMaxKey{20013}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMeanFloat{0.921978034325782846991614860598929226398468017578125}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMeanKey{29052}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMedianFloat{0.7388994395732879638671875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMedianKey{17080}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMinFloat{0.714709758758544921875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMinKey{2549}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMaxFloat{32.054157257080078125}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMaxKey{20013}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMeanFloat{18.050018424229907765266034402884542942047119140625}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMeanKey{2306}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMedianFloat{15.31974887847900390625}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMedianKey{26932}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMinFloat{14.48142910003662109375}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMinKey{2549}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveStdDevFloat{1.68898191898502236796275610686279833316802978515625}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductStdDevFloat{0.101090199198665076085745795353432185947895050048828125}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMaxFloat{33.140186309814453125}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMaxKey{20013}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMeanFloat{18.391414036024485767484293319284915924072265625}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMeanKey{1681}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMedianFloat{15.430480480194091796875}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMedianKey{26932}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMinFloat{14.82599925994873046875}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMinKey{2549}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveStdDevFloat{1.7532211410927229788825343348435126245021820068359375}
\def\EQKEErrWithAttnScaleBoundSvdLen{151}
\def\EQKEErrWithAttnScaleBoundSvdMaxFloat{3.1147792339324951171875}
\def\EQKEErrWithAttnScaleBoundSvdMaxKey{4800}
\def\EQKEErrWithAttnScaleBoundSvdMeanFloat{2.1844521816203137376533049973659217357635498046875}
\def\EQKEErrWithAttnScaleBoundSvdMeanKey{18668}
\def\EQKEErrWithAttnScaleBoundSvdMedianFloat{1.5081827342510223388671875}
\def\EQKEErrWithAttnScaleBoundSvdMedianKey{1696}
\def\EQKEErrWithAttnScaleBoundSvdMinFloat{1.45539820194244384765625}
\def\EQKEErrWithAttnScaleBoundSvdMinKey{2549}
\def\EQKEErrWithAttnScaleBoundSvdStdDevFloat{0.316184376157668867168837323333718813955783843994140625}
\def\EQKEErrWithAttnScaleFirstSingularLen{151}
\def\EQKEErrWithAttnScaleFirstSingularMaxFloat{2.2024822235107421875}
\def\EQKEErrWithAttnScaleFirstSingularMaxKey{4800}
\def\EQKEErrWithAttnScaleFirstSingularMeanFloat{1.54464113712310791015625}
\def\EQKEErrWithAttnScaleFirstSingularMeanKey{18668}
\def\EQKEErrWithAttnScaleFirstSingularMedianFloat{1.066445410251617431640625}
\def\EQKEErrWithAttnScaleFirstSingularMedianKey{1696}
\def\EQKEErrWithAttnScaleFirstSingularMinFloat{1.02912104129791259765625}
\def\EQKEErrWithAttnScaleFirstSingularMinKey{2549}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoLen{151}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMaxFloat{3.1147801876068115234375}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMaxKey{4800}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMeanFloat{2.18445240819691033351546138874255120754241943359375}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMeanKey{18668}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMedianFloat{1.508181512355804443359375}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMedianKey{1696}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMinFloat{1.4553968906402587890625}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMinKey{2549}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoStdDevFloat{0.316184494763609935663595251753577031195163726806640625}
\def\EQKEErrWithAttnScaleFirstSingularStdDevFloat{0.2235762031250150549954724965573404915630817413330078125}
\def\EQKEErrWithAttnScaleFroNormLen{151}
\def\EQKEErrWithAttnScaleFroNormMaxFloat{3.262793064117431640625}
\def\EQKEErrWithAttnScaleFroNormMaxKey{4800}
\def\EQKEErrWithAttnScaleFroNormMeanFloat{2.72115783975613823031380889005959033966064453125}
\def\EQKEErrWithAttnScaleFroNormMeanKey{19917}
\def\EQKEErrWithAttnScaleFroNormMedianFloat{2.22221815586090087890625}
\def\EQKEErrWithAttnScaleFroNormMedianKey{7884}
\def\EQKEErrWithAttnScaleFroNormMinFloat{2.16228008270263671875}
\def\EQKEErrWithAttnScaleFroNormMinKey{2549}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoLen{151}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMaxFloat{4.614285945892333984375}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMaxKey{4800}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMeanFloat{3.84829826860238366492694694898091256618499755859375}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMeanKey{19917}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMedianFloat{3.14269101619720458984375}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMedianKey{7884}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMinFloat{3.057925701141357421875}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMinKey{2549}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoStdDevFloat{0.30898036944293194583366357619524933397769927978515625}
\def\EQKEErrWithAttnScaleFroNormStdDevFloat{0.21848211278108331523384322281344793736934661865234375}
\def\EQKEErrWithAttnScaleLen{16384}
\def\EQKEErrWithAttnScaleMaxAbsLen{151}
\def\EQKEErrWithAttnScaleMaxAbsMaxFloat{0.372067272663116455078125}
\def\EQKEErrWithAttnScaleMaxAbsMaxKey{20013}
\def\EQKEErrWithAttnScaleMaxAbsMeanFloat{0.171480067024957272270313524131779558956623077392578125}
\def\EQKEErrWithAttnScaleMaxAbsMeanKey{50}
\def\EQKEErrWithAttnScaleMaxAbsMedianFloat{0.109869591891765594482421875}
\def\EQKEErrWithAttnScaleMaxAbsMedianKey{24566}
\def\EQKEErrWithAttnScaleMaxAbsMinFloat{0.10620330274105072021484375}
\def\EQKEErrWithAttnScaleMaxAbsMinKey{12552}
\def\EQKEErrWithAttnScaleMaxAbsStdDevFloat{0.032203375927384460253311004862553090788424015045166015625}
\def\EQKEErrWithAttnScaleMaxLen{151}
\def\EQKEErrWithAttnScaleMaxMaxFloat{0.372067272663116455078125}
\def\EQKEErrWithAttnScaleMaxMaxKey{20013}
\def\EQKEErrWithAttnScaleMaxMeanFloat{0.16209065914154052734375}
\def\EQKEErrWithAttnScaleMaxMeanKey{22401}
\def\EQKEErrWithAttnScaleMaxMedianFloat{0.1025776155292987823486328125}
\def\EQKEErrWithAttnScaleMaxMedianKey{12552}
\def\EQKEErrWithAttnScaleMaxMinFloat{0.093856267631053924560546875}
\def\EQKEErrWithAttnScaleMaxMinKey{2549}
\def\EQKEErrWithAttnScaleMaxRowDiffLen{151}
\def\EQKEErrWithAttnScaleMaxRowDiffMaxFloat{0.537927210330963134765625}
\def\EQKEErrWithAttnScaleMaxRowDiffMaxKey{20013}
\def\EQKEErrWithAttnScaleMaxRowDiffMeanFloat{0.30533840295100056483335038137738592922687530517578125}
\def\EQKEErrWithAttnScaleMaxRowDiffMeanKey{17197}
\def\EQKEErrWithAttnScaleMaxRowDiffMedianFloat{0.1988360397517681121826171875}
\def\EQKEErrWithAttnScaleMaxRowDiffMedianKey{12552}
\def\EQKEErrWithAttnScaleMaxRowDiffMinFloat{0.19874434173107147216796875}
\def\EQKEErrWithAttnScaleMaxRowDiffMinKey{2549}
\def\EQKEErrWithAttnScaleMaxRowDiffStdDevFloat{0.0548913879411465910340695018021506257355213165283203125}
\def\EQKEErrWithAttnScaleMaxStdDevFloat{0.0320857949554920196533203125}
\def\EQKEErrWithAttnScaleMeanDimZeroNormLen{151}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMaxFloat{0.01097971387207508087158203125}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMaxKey{29052}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMeanFloat{0.0037309766873495271190253053106289371498860418796539306640625}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMeanKey{913}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMedianFloat{0.00130478336359374225139617919921875}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMedianKey{8299}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMinFloat{0.001082900329492986202239990234375}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMinKey{4157}
\def\EQKEErrWithAttnScaleMeanDimZeroNormStdDevFloat{0.00151996585361660542685957597797141716000624001026153564453125}
\def\EQKEErrWithAttnScaleMeanLen{151}
\def\EQKEErrWithAttnScaleMeanMaxFloat{0.0000852284501888789236545562744140625}
\def\EQKEErrWithAttnScaleMeanMaxKey{22286}
\def\EQKEErrWithAttnScaleMeanMeanFloat{0.0000060415850384742952883243560791015625}
\def\EQKEErrWithAttnScaleMeanMeanKey{5781}
\def\EQKEErrWithAttnScaleMeanMedianFloat{-0.0000503477249367279000580310821533203125}
\def\EQKEErrWithAttnScaleMeanMedianKey{4800}
\def\EQKEErrWithAttnScaleMeanMinFloat{-0.00005161430090083740651607513427734375}
\def\EQKEErrWithAttnScaleMeanMinKey{2306}
\def\EQKEErrWithAttnScaleMeanStdDevFloat{0.000027220356059842742979526519775390625}
\def\EQKEErrWithAttnScaleMedianLen{151}
\def\EQKEErrWithAttnScaleMedianMaxFloat{-0.0524748316965997219085693359375}
\def\EQKEErrWithAttnScaleMedianMaxKey{2549}
\def\EQKEErrWithAttnScaleMedianMeanFloat{-0.0713766944303565742391270987354801036417484283447265625}
\def\EQKEErrWithAttnScaleMedianMeanKey{9132}
\def\EQKEErrWithAttnScaleMedianMedianFloat{-0.0895300279185175795770845752485911361873149871826171875}
\def\EQKEErrWithAttnScaleMedianMedianKey{4800}
\def\EQKEErrWithAttnScaleMedianMinFloat{-0.0901614856347441595563196869989042170345783233642578125}
\def\EQKEErrWithAttnScaleMedianMinKey{2306}
\def\EQKEErrWithAttnScaleMedianStdDevFloat{0.0070981450714151898828685460784981842152774333953857421875}
\def\EQKEErrWithAttnScaleMinLen{151}
\def\EQKEErrWithAttnScaleMinMaxFloat{-0.0999208986759185791015625}
\def\EQKEErrWithAttnScaleMinMaxKey{1696}
\def\EQKEErrWithAttnScaleMinMeanFloat{-0.16054607927799224853515625}
\def\EQKEErrWithAttnScaleMinMeanKey{19093}
\def\EQKEErrWithAttnScaleMinMedianFloat{-0.2471418045461177825927734375}
\def\EQKEErrWithAttnScaleMinMedianKey{15622}
\def\EQKEErrWithAttnScaleMinMinFloat{-0.2575353085994720458984375}
\def\EQKEErrWithAttnScaleMinMinKey{2306}
\def\EQKEErrWithAttnScaleMinStdDevFloat{0.02865105308592319488525390625}
\def\EQKEErrWithAttnScaleStdDevLen{151}
\def\EQKEErrWithAttnScaleStdDevMaxFloat{0.0254905261099338531494140625}
\def\EQKEErrWithAttnScaleStdDevMaxKey{4800}
\def\EQKEErrWithAttnScaleStdDevMeanFloat{0.0212590284645557403564453125}
\def\EQKEErrWithAttnScaleStdDevMeanKey{19917}
\def\EQKEErrWithAttnScaleStdDevMedianFloat{0.01736106909811496734619140625}
\def\EQKEErrWithAttnScaleStdDevMedianKey{7884}
\def\EQKEErrWithAttnScaleStdDevMinFloat{0.0168928168714046478271484375}
\def\EQKEErrWithAttnScaleStdDevMinKey{2549}
\def\EQKEErrWithAttnScaleStdDevStdDevFloat{0.001706891576759517192840576171875}
\def\EQKEFirstSingularLen{151}
\def\EQKEFirstSingularMaxFloat{24501.234375}
\def\EQKEFirstSingularMaxKey{20013}
\def\EQKEFirstSingularMeanFloat{17366.80640133485212572850286960601806640625}
\def\EQKEFirstSingularMeanKey{3284}
\def\EQKEFirstSingularMedianFloat{15383.89111328125}
\def\EQKEFirstSingularMedianKey{15662}
\def\EQKEFirstSingularMinFloat{14305.0439453125}
\def\EQKEFirstSingularMinKey{4729}
\def\EQKEFirstSingularSqrtTwoLen{151}
\def\EQKEFirstSingularSqrtTwoMaxFloat{34649.9779480068827979266643524169921875}
\def\EQKEFirstSingularSqrtTwoMaxKey{20013}
\def\EQKEFirstSingularSqrtTwoMeanFloat{24560.3731478756308206357061862945556640625}
\def\EQKEFirstSingularSqrtTwoMeanKey{3284}
\def\EQKEFirstSingularSqrtTwoMedianFloat{21756.1074544732764479704201221466064453125}
\def\EQKEFirstSingularSqrtTwoMedianKey{15662}
\def\EQKEFirstSingularSqrtTwoMinFloat{20230.38715780406710109673440456390380859375}
\def\EQKEFirstSingularSqrtTwoMinKey{4729}
\def\EQKEFirstSingularSqrtTwoStdDevFloat{1551.45295756673885989584960043430328369140625}
\def\EQKEFirstSingularStdDevFloat{1097.042906987365995519212447106838226318359375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMaxFloat{-7753838229084479488}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMaxKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMeanFloat{-7753838229084480512}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMeanKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMedianFloat{-7753838229084479488}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMedianKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMinFloat{-7753838229084479488}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMinKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenStdDevFloat{1024}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMaxFloat{221.2199554443359375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMaxKey{20013}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMeanFloat{11.1724071502685546875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMeanKey{13716}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMedianFloat{5.251806735992431640625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMedianKey{8840}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMinFloat{4.48918819427490234375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMinKey{24566}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxStdDevFloat{18.2333087921142578125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMaxFloat{1.01047030335830978486910680658183991909027099609375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMaxKey{20013}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMeanFloat{0.64079599666218090003866336701321415603160858154296875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMeanKey{18146}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMedianFloat{0.55533370919588520564502687193453311920166015625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMedianKey{28090}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMinFloat{0.55522384726965301471324210069724358618259429931640625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMinKey{24173}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanStdDevFloat{0.04556944455215317102414473993121646344661712646484375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMaxFloat{5.51127810262571671273690299130976200103759765625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMaxKey{27714}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMeanFloat{-0.6129817777768746811517530659330077469348907470703125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMeanKey{12457}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMedianFloat{-49.29761505126953125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMedianKey{6910}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMinFloat{-49.9106292724609375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMinKey{8048}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianStdDevFloat{7.15188344711134593723045327351428568363189697265625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMaxFloat{-3.002312183380126953125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMaxKey{8745}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMeanFloat{-9.11452007293701171875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMeanKey{30899}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMedianFloat{-93.00946044921875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMedianKey{8048}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMinFloat{-216.306915283203125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMinKey{20013}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinStdDevFloat{18.0939083099365234375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMaxFloat{2.94117392511545450162202541832812130451202392578125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMaxKey{20013}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMeanFloat{0.5285140312469358558900012212689034640789031982421875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMeanKey{29725}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMedianFloat{0.245557431643346812943917711891117505729198455810546875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMedianKey{8893}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMinFloat{0.23933172705302518945558176710619591176509857177734375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMinKey{4800}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevStdDevFloat{0.301658649014983237801601489991298876702785491943359375}
\def\EQKEHistAttentionDifferenceOverGapLenLen{151}
\def\EQKEHistAttentionDifferenceOverGapLenMaxFloat{2080768}
\def\EQKEHistAttentionDifferenceOverGapLenMaxKey{50}
\def\EQKEHistAttentionDifferenceOverGapLenMeanFloat{2080768}
\def\EQKEHistAttentionDifferenceOverGapLenMeanKey{50}
\def\EQKEHistAttentionDifferenceOverGapLenMedianFloat{2080768}
\def\EQKEHistAttentionDifferenceOverGapLenMedianKey{50}
\def\EQKEHistAttentionDifferenceOverGapLenMinFloat{2080768}
\def\EQKEHistAttentionDifferenceOverGapLenMinKey{50}
\def\EQKEHistAttentionDifferenceOverGapLenStdDevFloat{0}
\def\EQKEHistAttentionDifferenceOverGapMaxLen{151}
\def\EQKEHistAttentionDifferenceOverGapMaxMaxFloat{221.2199554443359375}
\def\EQKEHistAttentionDifferenceOverGapMaxMaxKey{20013}
\def\EQKEHistAttentionDifferenceOverGapMaxMeanFloat{11.1724071502685546875}
\def\EQKEHistAttentionDifferenceOverGapMaxMeanKey{13716}
\def\EQKEHistAttentionDifferenceOverGapMaxMedianFloat{5.251806735992431640625}
\def\EQKEHistAttentionDifferenceOverGapMaxMedianKey{8840}
\def\EQKEHistAttentionDifferenceOverGapMaxMinFloat{4.48918819427490234375}
\def\EQKEHistAttentionDifferenceOverGapMaxMinKey{24566}
\def\EQKEHistAttentionDifferenceOverGapMaxStdDevFloat{18.2333087921142578125}
\def\EQKEHistAttentionDifferenceOverGapMeanLen{151}
\def\EQKEHistAttentionDifferenceOverGapMeanMaxFloat{0.74481356143951416015625}
\def\EQKEHistAttentionDifferenceOverGapMeanMaxKey{20013}
\def\EQKEHistAttentionDifferenceOverGapMeanMeanFloat{0.524846971035003662109375}
\def\EQKEHistAttentionDifferenceOverGapMeanMeanKey{18146}
\def\EQKEHistAttentionDifferenceOverGapMeanMedianFloat{0.4808127582073211669921875}
\def\EQKEHistAttentionDifferenceOverGapMeanMedianKey{22261}
\def\EQKEHistAttentionDifferenceOverGapMeanMinFloat{0.4692261517047882080078125}
\def\EQKEHistAttentionDifferenceOverGapMeanMinKey{4729}
\def\EQKEHistAttentionDifferenceOverGapMeanStdDevFloat{0.02625206299126148223876953125}
\def\EQKEHistAttentionDifferenceOverGapMedianLen{151}
\def\EQKEHistAttentionDifferenceOverGapMedianMaxFloat{0.597636044025421142578125}
\def\EQKEHistAttentionDifferenceOverGapMedianMaxKey{20013}
\def\EQKEHistAttentionDifferenceOverGapMedianMeanFloat{0.46206344259495768511669666622765362262725830078125}
\def\EQKEHistAttentionDifferenceOverGapMedianMeanKey{13036}
\def\EQKEHistAttentionDifferenceOverGapMedianMedianFloat{0.421966604888439178466796875}
\def\EQKEHistAttentionDifferenceOverGapMedianMedianKey{24438}
\def\EQKEHistAttentionDifferenceOverGapMedianMinFloat{0.41472721099853515625}
\def\EQKEHistAttentionDifferenceOverGapMedianMinKey{4729}
\def\EQKEHistAttentionDifferenceOverGapMedianStdDevFloat{0.0204187793013592445989790036264821537770330905914306640625}
\def\EQKEHistAttentionDifferenceOverGapMinLen{151}
\def\EQKEHistAttentionDifferenceOverGapMinMaxFloat{-3.002312183380126953125}
\def\EQKEHistAttentionDifferenceOverGapMinMaxKey{8745}
\def\EQKEHistAttentionDifferenceOverGapMinMeanFloat{-9.11452007293701171875}
\def\EQKEHistAttentionDifferenceOverGapMinMeanKey{30899}
\def\EQKEHistAttentionDifferenceOverGapMinMedianFloat{-93.00946044921875}
\def\EQKEHistAttentionDifferenceOverGapMinMedianKey{8048}
\def\EQKEHistAttentionDifferenceOverGapMinMinFloat{-216.306915283203125}
\def\EQKEHistAttentionDifferenceOverGapMinMinKey{20013}
\def\EQKEHistAttentionDifferenceOverGapMinStdDevFloat{18.0939083099365234375}
\def\EQKEHistAttentionDifferenceOverGapStdDevLen{151}
\def\EQKEHistAttentionDifferenceOverGapStdDevMaxFloat{2.324749469757080078125}
\def\EQKEHistAttentionDifferenceOverGapStdDevMaxKey{20013}
\def\EQKEHistAttentionDifferenceOverGapStdDevMeanFloat{0.58557760715484619140625}
\def\EQKEHistAttentionDifferenceOverGapStdDevMeanKey{2549}
\def\EQKEHistAttentionDifferenceOverGapStdDevMedianFloat{0.498812817037105560302734375}
\def\EQKEHistAttentionDifferenceOverGapStdDevMedianKey{15043}
\def\EQKEHistAttentionDifferenceOverGapStdDevMinFloat{0.4899122416973114013671875}
\def\EQKEHistAttentionDifferenceOverGapStdDevMinKey{22261}
\def\EQKEHistAttentionDifferenceOverGapStdDevStdDevFloat{0.1576455533504486083984375}
\def\EQKEQueryDirectionLen{128}
\def\EQKEQueryDirectionMaxLen{151}
\def\EQKEQueryDirectionMaxMaxFloat{0.17632989585399627685546875}
\def\EQKEQueryDirectionMaxMaxKey{20013}
\def\EQKEQueryDirectionMaxMeanFloat{0.11547164618968963623046875}
\def\EQKEQueryDirectionMaxMeanKey{22261}
\def\EQKEQueryDirectionMaxMedianFloat{0.10131415165960788726806640625}
\def\EQKEQueryDirectionMaxMedianKey{1490}
\def\EQKEQueryDirectionMaxMinFloat{0.100972868502140045166015625}
\def\EQKEQueryDirectionMaxMinKey{6910}
\def\EQKEQueryDirectionMaxStdDevFloat{0.010078734718263149261474609375}
\def\EQKEQueryDirectionMeanLen{151}
\def\EQKEQueryDirectionMeanMaxFloat{0.088208027184009552001953125}
\def\EQKEQueryDirectionMeanMaxKey{13654}
\def\EQKEQueryDirectionMeanMeanFloat{0.087958015501499176025390625}
\def\EQKEQueryDirectionMeanMeanKey{6082}
\def\EQKEQueryDirectionMeanMedianFloat{0.08713379688560962677001953125}
\def\EQKEQueryDirectionMeanMedianKey{4810}
\def\EQKEQueryDirectionMeanMinFloat{0.08665178716182708740234375}
\def\EQKEQueryDirectionMeanMinKey{19451}
\def\EQKEQueryDirectionMeanStdDevFloat{0.000205554999411106109619140625}
\def\EQKEQueryDirectionMedianLen{151}
\def\EQKEQueryDirectionMedianMaxFloat{0.07501677807420492616330420787562616169452667236328125}
\def\EQKEQueryDirectionMedianMaxKey{11124}
\def\EQKEQueryDirectionMedianMeanFloat{0.06859955412415874587139796858537010848522186279296875}
\def\EQKEQueryDirectionMedianMeanKey{17197}
\def\EQKEQueryDirectionMedianMedianFloat{0.04932305110152811200574518579742289148271083831787109375}
\def\EQKEQueryDirectionMedianMedianKey{27671}
\def\EQKEQueryDirectionMedianMinFloat{0.0474040309526026215625194026870303787291049957275390625}
\def\EQKEQueryDirectionMedianMinKey{17080}
\def\EQKEQueryDirectionMedianStdDevFloat{0.005040831012448875221576560790026633185334503650665283203125}
\def\EQKEQueryDirectionMinLen{151}
\def\EQKEQueryDirectionMinMaxFloat{0.074993647634983062744140625}
\def\EQKEQueryDirectionMinMaxKey{11124}
\def\EQKEQueryDirectionMinMeanFloat{0.066273100674152374267578125}
\def\EQKEQueryDirectionMinMeanKey{18146}
\def\EQKEQueryDirectionMinMedianFloat{0.042596898972988128662109375}
\def\EQKEQueryDirectionMinMedianKey{17080}
\def\EQKEQueryDirectionMinMinFloat{0.0374932922422885894775390625}
\def\EQKEQueryDirectionMinMinKey{6910}
\def\EQKEQueryDirectionMinStdDevFloat{0.0063949408940970897674560546875}
\def\EQKEQueryDirectionStdDevLen{151}
\def\EQKEQueryDirectionStdDevMaxFloat{0.017434664070606231689453125}
\def\EQKEQueryDirectionStdDevMaxKey{19451}
\def\EQKEQueryDirectionStdDevMeanFloat{0.00852438621222972869873046875}
\def\EQKEQueryDirectionStdDevMeanKey{9134}
\def\EQKEQueryDirectionStdDevMedianFloat{0.005848156404681503772735595703125}
\def\EQKEQueryDirectionStdDevMedianKey{10248}
\def\EQKEQueryDirectionStdDevMinFloat{0.0056429845280945301055908203125}
\def\EQKEQueryDirectionStdDevMinKey{13654}
\def\EQKEQueryDirectionStdDevStdDevFloat{0.001783398096449673175811767578125}
\def\EQKERatioFirstTwoSingularLen{151}
\def\EQKERatioFirstTwoSingularLowerWhiskerBottomEndFloat{728.089510466134242960833944380283355712890625}
\def\EQKERatioFirstTwoSingularLowerWhiskerBottomEndKey{29052}
\def\EQKERatioFirstTwoSingularLowerWhiskerCrosshatchFloat{738.1441107775771115484531037509441375732421875}
\def\EQKERatioFirstTwoSingularLowerWhiskerCrosshatchKey{29052}
\def\EQKERatioFirstTwoSingularMaxFloat{2072.487548828125}
\def\EQKERatioFirstTwoSingularMaxKey{12552}
\def\EQKERatioFirstTwoSingularMeanFloat{1235.222211623033899741130881011486053466796875}
\def\EQKERatioFirstTwoSingularMeanKey{1895}
\def\EQKERatioFirstTwoSingularMedianFloat{799.72509765625}
\def\EQKERatioFirstTwoSingularMedianKey{19004}
\def\EQKERatioFirstTwoSingularMinFloat{724.86883544921875}
\def\EQKERatioFirstTwoSingularMinKey{29052}
\def\EQKERatioFirstTwoSingularQuartileOneFloat{762.296966552734375}
\def\EQKERatioFirstTwoSingularQuartileOneKey{29052}
\def\EQKERatioFirstTwoSingularQuartileThreeFloat{826.70304107666015625}
\def\EQKERatioFirstTwoSingularQuartileThreeKey{19004}
\def\EQKERatioFirstTwoSingularSqrMeanFloat{1581047.1528976089321076869964599609375}
\def\EQKERatioFirstTwoSingularStdDevFloat{235.10261761773250555052072741091251373291015625}
\def\EQKERatioFirstTwoSingularUpperWhiskerCrosshatchFloat{830.6249741347334065721952356398105621337890625}
\def\EQKERatioFirstTwoSingularUpperWhiskerCrosshatchKey{19004}
\def\EQKERatioFirstTwoSingularUpperWhiskerTopEndFloat{832.257636943398892981349490582942962646484375}
\def\EQKERatioFirstTwoSingularUpperWhiskerTopEndKey{19004}
\def\EQKESecondSingularLen{151}
\def\EQKESecondSingularMaxFloat{22.9926910400390625}
\def\EQKESecondSingularMaxKey{29052}
\def\EQKESecondSingularMeanFloat{14.5339775464392655379697316675446927547454833984375}
\def\EQKESecondSingularMeanKey{913}
\def\EQKESecondSingularMedianFloat{9.3953802585601806640625}
\def\EQKESecondSingularMedianKey{10248}
\def\EQKESecondSingularMinFloat{8.2086658477783203125}
\def\EQKESecondSingularMinKey{12552}
\def\EQKESecondSingularStdDevFloat{2.700573009189512152516954301972873508930206298828125}
\def\EQKESingularLen{32}
\def\EQKESingularMaxLen{151}
\def\EQKESingularMaxMaxFloat{24501.234375}
\def\EQKESingularMaxMaxKey{20013}
\def\EQKESingularMaxMeanFloat{17366.80859375}
\def\EQKESingularMaxMeanKey{3284}
\def\EQKESingularMaxMedianFloat{15383.89111328125}
\def\EQKESingularMaxMedianKey{15662}
\def\EQKESingularMaxMinFloat{14305.0439453125}
\def\EQKESingularMaxMinKey{4729}
\def\EQKESingularMaxStdDevFloat{1097.0428466796875}
\def\EQKESingularMeanLen{151}
\def\EQKESingularMeanMaxFloat{768.0621337890625}
\def\EQKESingularMeanMaxKey{20013}
\def\EQKESingularMeanMeanFloat{544.88348388671875}
\def\EQKESingularMeanMeanKey{3284}
\def\EQKESingularMeanMedianFloat{482.893341064453125}
\def\EQKESingularMeanMedianKey{15662}
\def\EQKESingularMeanMinFloat{449.237274169921875}
\def\EQKESingularMeanMinKey{4729}
\def\EQKESingularMeanStdDevFloat{34.286090850830078125}
\def\EQKESingularMedianLen{151}
\def\EQKESingularMedianMaxFloat{0.024973019091412425318754486625039135105907917022705078125}
\def\EQKESingularMedianMaxKey{11611}
\def\EQKESingularMedianMeanFloat{0.005171862158015376985387145936101660481654107570648193359375}
\def\EQKESingularMedianMeanKey{12552}
\def\EQKESingularMedianMedianFloat{0.00135105011038831428205053697411130997352302074432373046875}
\def\EQKESingularMedianMedianKey{4729}
\def\EQKESingularMedianMinFloat{0.0013447517034364865097517682812622297205962240695953369140625}
\def\EQKESingularMedianMinKey{23696}
\def\EQKESingularMedianStdDevFloat{0.003760145718541062047346468233399718883447349071502685546875}
\def\EQKESingularMinLen{151}
\def\EQKESingularMinMaxFloat{0.02200733311474323272705078125}
\def\EQKESingularMinMaxKey{11611}
\def\EQKESingularMinMeanFloat{0.0033492553047835826873779296875}
\def\EQKESingularMinMeanKey{8048}
\def\EQKESingularMinMedianFloat{0.000947146865655668079853057861328125}
\def\EQKESingularMinMedianKey{20338}
\def\EQKESingularMinMinFloat{0.0009223925299011170864105224609375}
\def\EQKESingularMinMinKey{4729}
\def\EQKESingularMinStdDevFloat{0.00359809584915637969970703125}
\def\EQKESingularStdDevLen{151}
\def\EQKESingularStdDevMaxFloat{4262.60498046875}
\def\EQKESingularStdDevMaxKey{20013}
\def\EQKESingularStdDevMeanFloat{3021.307861328125}
\def\EQKESingularStdDevMeanKey{3284}
\def\EQKESingularStdDevMedianFloat{2676.3001708984375}
\def\EQKESingularStdDevMedianKey{15662}
\def\EQKESingularStdDevMinFloat{2488.57861328125}
\def\EQKESingularStdDevMinKey{4729}
\def\EQKESingularStdDevStdDevFloat{190.876739501953125}
\def\EQKESizeDirectionDiffsLen{127}
\def\EQKESizeDirectionDiffsMaxLen{151}
\def\EQKESizeDirectionDiffsMaxMaxFloat{0.2897014915943145751953125}
\def\EQKESizeDirectionDiffsMaxMaxKey{20013}
\def\EQKESizeDirectionDiffsMaxMeanFloat{0.0294598527252674102783203125}
\def\EQKESizeDirectionDiffsMaxMeanKey{23696}
\def\EQKESizeDirectionDiffsMaxMedianFloat{0.01528818719089031219482421875}
\def\EQKESizeDirectionDiffsMaxMedianKey{8840}
\def\EQKESizeDirectionDiffsMaxMinFloat{0.013193778693675994873046875}
\def\EQKESizeDirectionDiffsMaxMinKey{24566}
\def\EQKESizeDirectionDiffsMaxStdDevFloat{0.0269232131540775299072265625}
\def\EQKESizeDirectionDiffsMeanLen{151}
\def\EQKESizeDirectionDiffsMeanMaxFloat{0.00271021132357418537139892578125}
\def\EQKESizeDirectionDiffsMeanMaxKey{15662}
\def\EQKESizeDirectionDiffsMeanMeanFloat{0.00245289341546595096588134765625}
\def\EQKESizeDirectionDiffsMeanMeanKey{19488}
\def\EQKESizeDirectionDiffsMeanMedianFloat{0.0021979566081427037715911865234375}
\def\EQKESizeDirectionDiffsMeanMedianKey{6204}
\def\EQKESizeDirectionDiffsMeanMinFloat{0.00217912229709327220916748046875}
\def\EQKESizeDirectionDiffsMeanMinKey{27671}
\def\EQKESizeDirectionDiffsMeanStdDevFloat{0.0001061917864717543125152587890625}
\def\EQKESizeDirectionDiffsMedianLen{151}
\def\EQKESizeDirectionDiffsMedianMaxFloat{-0.0086960943043231965499106905781445675529539585113525390625}
\def\EQKESizeDirectionDiffsMedianMaxKey{8745}
\def\EQKESizeDirectionDiffsMedianMeanFloat{-0.0186885603273053042816531643666166928596794605255126953125}
\def\EQKESizeDirectionDiffsMedianMeanKey{519}
\def\EQKESizeDirectionDiffsMedianMedianFloat{-0.07938981665298343315395612762586097232997417449951171875}
\def\EQKESizeDirectionDiffsMedianMedianKey{6910}
\def\EQKESizeDirectionDiffsMedianMinFloat{-0.1161082845926284801141292746251565404236316680908203125}
\def\EQKESizeDirectionDiffsMedianMinKey{20013}
\def\EQKESizeDirectionDiffsMedianStdDevFloat{0.0108464652260859793775349402267238474451005458831787109375}
\def\EQKESizeDirectionDiffsMinLen{151}
\def\EQKESizeDirectionDiffsMinMaxFloat{-0.009233288466930389404296875}
\def\EQKESizeDirectionDiffsMinMaxKey{8745}
\def\EQKESizeDirectionDiffsMinMeanFloat{-0.02359181083738803863525390625}
\def\EQKESizeDirectionDiffsMinMeanKey{11498}
\def\EQKESizeDirectionDiffsMinMedianFloat{-0.1759995184838771820068359375}
\def\EQKESizeDirectionDiffsMinMedianKey{6910}
\def\EQKESizeDirectionDiffsMinMinFloat{-0.283534586429595947265625}
\def\EQKESizeDirectionDiffsMinMinKey{20013}
\def\EQKESizeDirectionDiffsMinStdDevFloat{0.02731262706220149993896484375}
\def\EQKESizeDirectionDiffsStdDevLen{151}
\def\EQKESizeDirectionDiffsStdDevMaxFloat{0.0364087261259555816650390625}
\def\EQKESizeDirectionDiffsStdDevMaxKey{20013}
\def\EQKESizeDirectionDiffsStdDevMeanFloat{0.007568043656647205352783203125}
\def\EQKESizeDirectionDiffsStdDevMeanKey{32374}
\def\EQKESizeDirectionDiffsStdDevMedianFloat{0.0054492219351232051849365234375}
\def\EQKESizeDirectionDiffsStdDevMedianKey{4430}
\def\EQKESizeDirectionDiffsStdDevMinFloat{0.0053632655180990695953369140625}
\def\EQKESizeDirectionDiffsStdDevMinKey{8745}
\def\EQKESizeDirectionDiffsStdDevStdDevFloat{0.00291984342038631439208984375}
\def\EQKESizeDirectionLen{128}
\def\EQKESizeDirectionMaxLen{151}
\def\EQKESizeDirectionMaxMaxFloat{0.2571065425872802734375}
\def\EQKESizeDirectionMaxMaxKey{4810}
\def\EQKESizeDirectionMaxMeanFloat{0.216273128986358642578125}
\def\EQKESizeDirectionMaxMeanKey{2306}
\def\EQKESizeDirectionMaxMedianFloat{0.1867662407457828521728515625}
\def\EQKESizeDirectionMaxMedianKey{5781}
\def\EQKESizeDirectionMaxMinFloat{0.1842738091945648193359375}
\def\EQKESizeDirectionMaxMinKey{27671}
\def\EQKESizeDirectionMaxStdDevFloat{0.015768505632877349853515625}
\def\EQKESizeDirectionMeanLen{151}
\def\EQKESizeDirectionMeanMaxFloat{-0.0117781572043895721435546875}
\def\EQKESizeDirectionMeanMaxKey{19451}
\def\EQKESizeDirectionMeanMeanFloat{-0.03663526475429534912109375}
\def\EQKESizeDirectionMeanMeanKey{29195}
\def\EQKESizeDirectionMeanMedianFloat{-0.04909861087799072265625}
\def\EQKESizeDirectionMeanMedianKey{17080}
\def\EQKESizeDirectionMeanMinFloat{-0.049588739871978759765625}
\def\EQKESizeDirectionMeanMinKey{5781}
\def\EQKESizeDirectionMeanStdDevFloat{0.00650803744792938232421875}
\def\EQKESizeDirectionMedianLen{151}
\def\EQKESizeDirectionMedianMaxFloat{-0.08749681424349546599028570881273481063544750213623046875}
\def\EQKESizeDirectionMedianMaxKey{19451}
\def\EQKESizeDirectionMedianMeanFloat{-0.104040360953535471200126494295545853674411773681640625}
\def\EQKESizeDirectionMedianMeanKey{8721}
\def\EQKESizeDirectionMedianMedianFloat{-0.116179601224139339432639417282189242541790008544921875}
\def\EQKESizeDirectionMedianMedianKey{20013}
\def\EQKESizeDirectionMedianMinFloat{-0.116344289444386961296373783625313080847263336181640625}
\def\EQKESizeDirectionMedianMinKey{6910}
\def\EQKESizeDirectionMedianStdDevFloat{0.004348425083496580689779165140862460248172283172607421875}
\def\EQKESizeDirectionMinLen{151}
\def\EQKESizeDirectionMinMaxFloat{-0.088001392781734466552734375}
\def\EQKESizeDirectionMinMaxKey{19451}
\def\EQKESizeDirectionMinMeanFloat{-0.10548768937587738037109375}
\def\EQKESizeDirectionMinMeanKey{6159}
\def\EQKESizeDirectionMinMedianFloat{-0.1471867859363555908203125}
\def\EQKESizeDirectionMinMedianKey{6910}
\def\EQKESizeDirectionMinMinFloat{-0.16357056796550750732421875}
\def\EQKESizeDirectionMinMinKey{20013}
\def\EQKESizeDirectionMinStdDevFloat{0.0073344097472727298736572265625}
\def\EQKESizeDirectionStdDevLen{151}
\def\EQKESizeDirectionStdDevMaxFloat{0.08760009706020355224609375}
\def\EQKESizeDirectionStdDevMaxKey{19451}
\def\EQKESizeDirectionStdDevMeanFloat{0.080126218497753143310546875}
\def\EQKESizeDirectionStdDevMeanKey{10248}
\def\EQKESizeDirectionStdDevMedianFloat{0.07349633239209651947021484375}
\def\EQKESizeDirectionStdDevMedianKey{17080}
\def\EQKESizeDirectionStdDevMinFloat{0.073167331516742706298828125}
\def\EQKESizeDirectionStdDevMinKey{5781}
\def\EQKESizeDirectionStdDevStdDevFloat{0.002791485749185085296630859375}
\def\EQKEThirdSingularLen{151}
\def\EQKEThirdSingularMaxFloat{14.81468296051025390625}
\def\EQKEThirdSingularMaxKey{20013}
\def\EQKEThirdSingularMeanFloat{9.2536813660173233841987894265912473201751708984375}
\def\EQKEThirdSingularMeanKey{16197}
\def\EQKEThirdSingularMedianFloat{6.5133597850799560546875}
\def\EQKEThirdSingularMedianKey{1696}
\def\EQKEThirdSingularMinFloat{6.40264892578125}
\def\EQKEThirdSingularMinKey{2549}
\def\EQKEThirdSingularStdDevFloat{1.44007893367400097162089878111146390438079833984375}
\def\EQKEWithAttnScaleFirstSingularLen{151}
\def\EQKEWithAttnScaleFirstSingularMaxFloat{4331.24755859375}
\def\EQKEWithAttnScaleFirstSingularMaxKey{20013}
\def\EQKEWithAttnScaleFirstSingularMeanFloat{3070.04670361651506027556024491786956787109375}
\def\EQKEWithAttnScaleFirstSingularMeanKey{3284}
\def\EQKEWithAttnScaleFirstSingularMedianFloat{2719.51348876953125}
\def\EQKEWithAttnScaleFirstSingularMedianKey{15662}
\def\EQKEWithAttnScaleFirstSingularMinFloat{2528.79833984375}
\def\EQKEWithAttnScaleFirstSingularMinKey{4729}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoLen{151}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMaxFloat{6125.3090393586380741908214986324310302734375}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMaxKey{20013}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMeanFloat{4341.70168537328936508856713771820068359375}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMeanKey{3284}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMedianFloat{3845.9728588744428634527139365673065185546875}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMedianKey{15662}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMinFloat{3576.26090871359838274656794965267181396484375}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMinKey{4729}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoStdDevFloat{274.2607492028654405658016912639141082763671875}
\def\EQKEWithAttnScaleFirstSingularStdDevFloat{193.93163557464913537842221558094024658203125}
\def\EQKEWithAttnScaleRatioFirstTwoSingularLen{151}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMaxFloat{2072.487548828125}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMaxKey{12552}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMeanFloat{1235.222216069303613039664924144744873046875}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMeanKey{1895}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMedianFloat{799.72515869140625}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMedianKey{19004}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMinFloat{724.868896484375}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMinKey{29052}
\def\EQKEWithAttnScaleRatioFirstTwoSingularStdDevFloat{235.102617922873406541839358396828174591064453125}
\def\EQKEWithAttnScaleSecondSingularLen{151}
\def\EQKEWithAttnScaleSecondSingularMaxFloat{4.064571857452392578125}
\def\EQKEWithAttnScaleSecondSingularMaxKey{29052}
\def\EQKEWithAttnScaleSecondSingularMeanFloat{2.569268555830646061366451249341480433940887451171875}
\def\EQKEWithAttnScaleSecondSingularMeanKey{913}
\def\EQKEWithAttnScaleSecondSingularMedianFloat{1.66088426113128662109375}
\def\EQKEWithAttnScaleSecondSingularMedianKey{10248}
\def\EQKEWithAttnScaleSecondSingularMinFloat{1.451100826263427734375}
\def\EQKEWithAttnScaleSecondSingularMinKey{12552}
\def\EQKEWithAttnScaleSecondSingularStdDevFloat{0.477398370383780357162351037914049811661243438720703125}
\def\EQKEWithAttnScaleSingularLen{32}
\def\EQKEWithAttnScaleSingularMaxLen{151}
\def\EQKEWithAttnScaleSingularMaxMaxFloat{24501.234375}
\def\EQKEWithAttnScaleSingularMaxMaxKey{20013}
\def\EQKEWithAttnScaleSingularMaxMeanFloat{17366.80859375}
\def\EQKEWithAttnScaleSingularMaxMeanKey{3284}
\def\EQKEWithAttnScaleSingularMaxMedianFloat{15383.89111328125}
\def\EQKEWithAttnScaleSingularMaxMedianKey{15662}
\def\EQKEWithAttnScaleSingularMaxMinFloat{14305.0439453125}
\def\EQKEWithAttnScaleSingularMaxMinKey{4729}
\def\EQKEWithAttnScaleSingularMaxStdDevFloat{1097.0428466796875}
\def\EQKEWithAttnScaleSingularMeanLen{151}
\def\EQKEWithAttnScaleSingularMeanMaxFloat{768.0621337890625}
\def\EQKEWithAttnScaleSingularMeanMaxKey{20013}
\def\EQKEWithAttnScaleSingularMeanMeanFloat{544.88348388671875}
\def\EQKEWithAttnScaleSingularMeanMeanKey{3284}
\def\EQKEWithAttnScaleSingularMeanMedianFloat{482.893341064453125}
\def\EQKEWithAttnScaleSingularMeanMedianKey{15662}
\def\EQKEWithAttnScaleSingularMeanMinFloat{449.237274169921875}
\def\EQKEWithAttnScaleSingularMeanMinKey{4729}
\def\EQKEWithAttnScaleSingularMeanStdDevFloat{34.286090850830078125}
\def\EQKEWithAttnScaleSingularMedianLen{151}
\def\EQKEWithAttnScaleSingularMedianMaxFloat{0.024973019091412425318754486625039135105907917022705078125}
\def\EQKEWithAttnScaleSingularMedianMaxKey{11611}
\def\EQKEWithAttnScaleSingularMedianMeanFloat{0.005171862158015376985387145936101660481654107570648193359375}
\def\EQKEWithAttnScaleSingularMedianMeanKey{12552}
\def\EQKEWithAttnScaleSingularMedianMedianFloat{0.00135105011038831428205053697411130997352302074432373046875}
\def\EQKEWithAttnScaleSingularMedianMedianKey{4729}
\def\EQKEWithAttnScaleSingularMedianMinFloat{0.0013447517034364865097517682812622297205962240695953369140625}
\def\EQKEWithAttnScaleSingularMedianMinKey{23696}
\def\EQKEWithAttnScaleSingularMedianStdDevFloat{0.003760145718541062047346468233399718883447349071502685546875}
\def\EQKEWithAttnScaleSingularMinLen{151}
\def\EQKEWithAttnScaleSingularMinMaxFloat{0.02200733311474323272705078125}
\def\EQKEWithAttnScaleSingularMinMaxKey{11611}
\def\EQKEWithAttnScaleSingularMinMeanFloat{0.0033492553047835826873779296875}
\def\EQKEWithAttnScaleSingularMinMeanKey{8048}
\def\EQKEWithAttnScaleSingularMinMedianFloat{0.000947146865655668079853057861328125}
\def\EQKEWithAttnScaleSingularMinMedianKey{20338}
\def\EQKEWithAttnScaleSingularMinMinFloat{0.0009223925299011170864105224609375}
\def\EQKEWithAttnScaleSingularMinMinKey{4729}
\def\EQKEWithAttnScaleSingularMinStdDevFloat{0.00359809584915637969970703125}
\def\EQKEWithAttnScaleSingularStdDevLen{151}
\def\EQKEWithAttnScaleSingularStdDevMaxFloat{4262.60498046875}
\def\EQKEWithAttnScaleSingularStdDevMaxKey{20013}
\def\EQKEWithAttnScaleSingularStdDevMeanFloat{3021.307861328125}
\def\EQKEWithAttnScaleSingularStdDevMeanKey{3284}
\def\EQKEWithAttnScaleSingularStdDevMedianFloat{2676.3001708984375}
\def\EQKEWithAttnScaleSingularStdDevMedianKey{15662}
\def\EQKEWithAttnScaleSingularStdDevMinFloat{2488.57861328125}
\def\EQKEWithAttnScaleSingularStdDevMinKey{4729}
\def\EQKEWithAttnScaleSingularStdDevStdDevFloat{190.876739501953125}
\def\EQKEWithAttnScaleThirdSingularLen{151}
\def\EQKEWithAttnScaleThirdSingularMaxFloat{2.6188907623291015625}
\def\EQKEWithAttnScaleThirdSingularMaxKey{20013}
\def\EQKEWithAttnScaleThirdSingularMeanFloat{1.6358352386398820055291025710175745189189910888671875}
\def\EQKEWithAttnScaleThirdSingularMeanKey{16197}
\def\EQKEWithAttnScaleThirdSingularMedianFloat{1.1514102518558502197265625}
\def\EQKEWithAttnScaleThirdSingularMedianKey{1696}
\def\EQKEWithAttnScaleThirdSingularMinFloat{1.13183915615081787109375}
\def\EQKEWithAttnScaleThirdSingularMinKey{2549}
\def\EQKEWithAttnScaleThirdSingularStdDevFloat{0.25457239870163095307731282446184195578098297119140625}
\def\EQKPAbsLen{1280}
\def\EQKPAbsMaxLen{151}
\def\EQKPAbsMaxMaxFloat{12.5981922149658203125}
\def\EQKPAbsMaxMaxKey{20013}
\def\EQKPAbsMaxMeanFloat{4.046356678009033203125}
\def\EQKPAbsMaxMeanKey{8048}
\def\EQKPAbsMaxMedianFloat{1.41667568683624267578125}
\def\EQKPAbsMaxMedianKey{13293}
\def\EQKPAbsMaxMinFloat{1.395332813262939453125}
\def\EQKPAbsMaxMinKey{9816}
\def\EQKPAbsMaxStdDevFloat{1.892322540283203125}
\def\EQKPAbsMeanLen{151}
\def\EQKPAbsMeanMaxFloat{3.00025177001953125}
\def\EQKPAbsMeanMaxKey{26278}
\def\EQKPAbsMeanMeanFloat{1.28037369251251220703125}
\def\EQKPAbsMeanMeanKey{23447}
\def\EQKPAbsMeanMedianFloat{0.4902148544788360595703125}
\def\EQKPAbsMeanMedianKey{27714}
\def\EQKPAbsMeanMinFloat{0.4856204092502593994140625}
\def\EQKPAbsMeanMinKey{5615}
\def\EQKPAbsMeanStdDevFloat{0.5373287200927734375}
\def\EQKPAbsMedianLen{151}
\def\EQKPAbsMedianMaxFloat{0.6340886324644088301027977649937383830547332763671875}
\def\EQKPAbsMedianMaxKey{3284}
\def\EQKPAbsMedianMeanFloat{0.06692322367291884954720870837263646535575389862060546875}
\def\EQKPAbsMedianMeanKey{27300}
\def\EQKPAbsMedianMedianFloat{0.001077268138760700995348873476586959441192448139190673828125}
\def\EQKPAbsMedianMedianKey{20338}
\def\EQKPAbsMedianMinFloat{0.000974008599296212322117549664568514344864524900913238525390625}
\def\EQKPAbsMedianMinKey{24202}
\def\EQKPAbsMedianStdDevFloat{0.10930859010522257779296495527887600474059581756591796875}
\def\EQKPAbsMinLen{151}
\def\EQKPAbsMinMaxFloat{0.4928896725177764892578125}
\def\EQKPAbsMinMaxKey{3284}
\def\EQKPAbsMinMeanFloat{0.02885270304977893829345703125}
\def\EQKPAbsMinMeanKey{6549}
\def\EQKPAbsMinMedianFloat{0.00000976701267063617706298828125}
\def\EQKPAbsMinMedianKey{17197}
\def\EQKPAbsMinMinFloat{0.00000970065593719482421875}
\def\EQKPAbsMinMinKey{4647}
\def\EQKPAbsMinStdDevFloat{0.075796492397785186767578125}
\def\EQKPAbsStdDevLen{151}
\def\EQKPAbsStdDevMaxFloat{2.3026502132415771484375}
\def\EQKPAbsStdDevMaxKey{30463}
\def\EQKPAbsStdDevMeanFloat{0.917698442935943603515625}
\def\EQKPAbsStdDevMeanKey{2549}
\def\EQKPAbsStdDevMedianFloat{0.320303522050380706787109375}
\def\EQKPAbsStdDevMedianKey{9816}
\def\EQKPAbsStdDevMinFloat{0.2689040601253509521484375}
\def\EQKPAbsStdDevMinKey{27714}
\def\EQKPAbsStdDevStdDevFloat{0.41750633716583251953125}
\def\EQKPLen{1280}
\def\EQKPMaxLen{151}
\def\EQKPMaxMaxFloat{10.03693103790283203125}
\def\EQKPMaxMaxKey{29195}
\def\EQKPMaxMeanFloat{3.5235106945037841796875}
\def\EQKPMaxMeanKey{50}
\def\EQKPMaxMedianFloat{1.3917225897312164306640625}
\def\EQKPMaxMedianKey{13293}
\def\EQKPMaxMinFloat{1.39130961894989013671875}
\def\EQKPMaxMinKey{27714}
\def\EQKPMaxRowDiffLen{128}
\def\EQKPMaxRowDiffMaxLen{151}
\def\EQKPMaxRowDiffMaxMaxFloat{18.7245731353759765625}
\def\EQKPMaxRowDiffMaxMaxKey{20013}
\def\EQKPMaxRowDiffMaxMeanFloat{7.031847476959228515625}
\def\EQKPMaxRowDiffMaxMeanKey{12552}
\def\EQKPMaxRowDiffMaxMedianFloat{2.7596404552459716796875}
\def\EQKPMaxRowDiffMaxMedianKey{27714}
\def\EQKPMaxRowDiffMaxMinFloat{2.701297760009765625}
\def\EQKPMaxRowDiffMaxMinKey{9816}
\def\EQKPMaxRowDiffMaxStdDevFloat{3.0512287616729736328125}
\def\EQKPMaxRowDiffMeanLen{151}
\def\EQKPMaxRowDiffMeanMaxFloat{11.5913982391357421875}
\def\EQKPMaxRowDiffMeanMaxKey{16284}
\def\EQKPMaxRowDiffMeanMeanFloat{5.300899982452392578125}
\def\EQKPMaxRowDiffMeanMeanKey{15622}
\def\EQKPMaxRowDiffMeanMedianFloat{2.0362335741519927978515625}
\def\EQKPMaxRowDiffMeanMedianKey{9816}
\def\EQKPMaxRowDiffMeanMinFloat{1.71822130680084228515625}
\def\EQKPMaxRowDiffMeanMinKey{27714}
\def\EQKPMaxRowDiffMeanStdDevFloat{2.226818084716796875}
\def\EQKPMaxRowDiffMedianLen{151}
\def\EQKPMaxRowDiffMedianMaxFloat{9.5434973144531252131628207280300557613372802734375}
\def\EQKPMaxRowDiffMedianMaxKey{29195}
\def\EQKPMaxRowDiffMedianMeanFloat{4.0759266383521595145111859892494976520538330078125}
\def\EQKPMaxRowDiffMedianMeanKey{6155}
\def\EQKPMaxRowDiffMedianMedianFloat{1.328457093387842125054021380492486059665679931640625}
\def\EQKPMaxRowDiffMedianMedianKey{17080}
\def\EQKPMaxRowDiffMedianMinFloat{1.2982807922363281960542735760100185871124267578125}
\def\EQKPMaxRowDiffMedianMinKey{27714}
\def\EQKPMaxRowDiffMedianStdDevFloat{1.801735204256714961701391075621359050273895263671875}
\def\EQKPMaxRowDiffMinLen{151}
\def\EQKPMaxRowDiffMinMaxFloat{9.5227718353271484375}
\def\EQKPMaxRowDiffMinMaxKey{29195}
\def\EQKPMaxRowDiffMinMeanFloat{3.9343626499176025390625}
\def\EQKPMaxRowDiffMinMeanKey{26374}
\def\EQKPMaxRowDiffMinMedianFloat{1.2704080045223236083984375}
\def\EQKPMaxRowDiffMinMedianKey{27714}
\def\EQKPMaxRowDiffMinMinFloat{1.21605384349822998046875}
\def\EQKPMaxRowDiffMinMinKey{17080}
\def\EQKPMaxRowDiffMinStdDevFloat{1.7644417285919189453125}
\def\EQKPMaxRowDiffStdDevLen{151}
\def\EQKPMaxRowDiffStdDevMaxFloat{1.7066209316253662109375}
\def\EQKPMaxRowDiffStdDevMaxKey{19917}
\def\EQKPMaxRowDiffStdDevMeanFloat{0.536258637905120849609375}
\def\EQKPMaxRowDiffStdDevMeanKey{22261}
\def\EQKPMaxRowDiffStdDevMedianFloat{0.185079276561737060546875}
\def\EQKPMaxRowDiffStdDevMedianKey{13654}
\def\EQKPMaxRowDiffStdDevMinFloat{0.17680282890796661376953125}
\def\EQKPMaxRowDiffStdDevMinKey{9816}
\def\EQKPMaxRowDiffStdDevStdDevFloat{0.23931793868541717529296875}
\def\EQKPMaxStdDevFloat{1.59253561496734619140625}
\def\EQKPMeanLen{151}
\def\EQKPMeanMaxFloat{0.000002186000301662716083228588104248046875}
\def\EQKPMeanMaxKey{32382}
\def\EQKPMeanMeanFloat{0.00000011654703513386266422457993030548095703125}
\def\EQKPMeanMeanKey{23367}
\def\EQKPMeanMedianFloat{-0.000001796474634829792194068431854248046875}
\def\EQKPMeanMedianKey{30684}
\def\EQKPMeanMinFloat{-0.000001812539949241909198462963104248046875}
\def\EQKPMeanMinKey{12141}
\def\EQKPMeanStdDevFloat{0.00000083755099922200315631926059722900390625}
\def\EQKPMedianLen{151}
\def\EQKPMedianMaxFloat{-1.117745237946510261650701067992486059665679931640625}
\def\EQKPMedianMaxKey{19488}
\def\EQKPMedianMeanFloat{-3.179271859767421215536842282745055854320526123046875}
\def\EQKPMedianMeanKey{50}
\def\EQKPMedianMedianFloat{-8.372101573944092933743377216160297393798828125}
\def\EQKPMedianMedianKey{30463}
\def\EQKPMedianMinFloat{-8.5562315893173224168322121840901672840118408203125}
\def\EQKPMedianMinKey{20976}
\def\EQKPMedianStdDevFloat{1.454743011781640671387094698729924857616424560546875}
\def\EQKPMinLen{151}
\def\EQKPMinMaxFloat{-1.290637969970703125}
\def\EQKPMinMaxKey{19488}
\def\EQKPMinMeanFloat{-3.58376979827880859375}
\def\EQKPMinMeanKey{104}
\def\EQKPMinMedianFloat{-10.949700832366943359375}
\def\EQKPMinMedianKey{20976}
\def\EQKPMinMinFloat{-12.5981922149658203125}
\def\EQKPMinMinKey{20013}
\def\EQKPMinStdDevFloat{1.76785671710968017578125}
\def\EQKPStdDevLen{151}
\def\EQKPStdDevMaxFloat{3.6989548206329345703125}
\def\EQKPStdDevMaxKey{13468}
\def\EQKPStdDevMeanFloat{1.58232915401458740234375}
\def\EQKPStdDevMeanKey{4810}
\def\EQKPStdDevMedianFloat{0.623739421367645263671875}
\def\EQKPStdDevMedianKey{5615}
\def\EQKPStdDevMinFloat{0.560467541217803955078125}
\def\EQKPStdDevMinKey{27714}
\def\EQKPStdDevStdDevFloat{0.66392409801483154296875}
\def\EQKPWithAttnScaleAbsLen{1280}
\def\EQKPWithAttnScaleAbsMaxLen{151}
\def\EQKPWithAttnScaleAbsMaxMaxFloat{2.2270667552947998046875}
\def\EQKPWithAttnScaleAbsMaxMaxKey{20013}
\def\EQKPWithAttnScaleAbsMaxMeanFloat{0.715301513671875}
\def\EQKPWithAttnScaleAbsMaxMeanKey{8048}
\def\EQKPWithAttnScaleAbsMaxMedianFloat{0.2504352517426013946533203125}
\def\EQKPWithAttnScaleAbsMaxMedianKey{13293}
\def\EQKPWithAttnScaleAbsMaxMinFloat{0.24666233360767364501953125}
\def\EQKPWithAttnScaleAbsMaxMinKey{9816}
\def\EQKPWithAttnScaleAbsMaxStdDevFloat{0.33451855182647705078125}
\def\EQKPWithAttnScaleAbsMeanLen{151}
\def\EQKPWithAttnScaleAbsMeanMaxFloat{0.53037464618682861328125}
\def\EQKPWithAttnScaleAbsMeanMaxKey{26278}
\def\EQKPWithAttnScaleAbsMeanMeanFloat{0.226340234279632568359375}
\def\EQKPWithAttnScaleAbsMeanMeanKey{23447}
\def\EQKPWithAttnScaleAbsMeanMedianFloat{0.0866585671901702880859375}
\def\EQKPWithAttnScaleAbsMeanMedianKey{27714}
\def\EQKPWithAttnScaleAbsMeanMinFloat{0.085846371948719024658203125}
\def\EQKPWithAttnScaleAbsMeanMinKey{5615}
\def\EQKPWithAttnScaleAbsMeanStdDevFloat{0.094987206161022186279296875}
\def\EQKPWithAttnScaleAbsMedianLen{151}
\def\EQKPWithAttnScaleAbsMedianMaxFloat{0.112092094905674455329602778874686919152736663818359375}
\def\EQKPWithAttnScaleAbsMedianMaxKey{3284}
\def\EQKPWithAttnScaleAbsMedianMeanFloat{0.01183046652659730003931404240802294225431978702545166015625}
\def\EQKPWithAttnScaleAbsMedianMeanKey{27300}
\def\EQKPWithAttnScaleAbsMedianMedianFloat{0.00019043590185901851092979686352890666967141442000865936279296875}
\def\EQKPWithAttnScaleAbsMedianMedianKey{20338}
\def\EQKPWithAttnScaleAbsMedianMinFloat{0.00017218202832737007114405347607544172205962240695953369140625}
\def\EQKPWithAttnScaleAbsMedianMinKey{24202}
\def\EQKPWithAttnScaleAbsMedianStdDevFloat{0.0193232117081454622675718013624646118842065334320068359375}
\def\EQKPWithAttnScaleAbsMinLen{151}
\def\EQKPWithAttnScaleAbsMinMaxFloat{0.0871314108371734619140625}
\def\EQKPWithAttnScaleAbsMinMaxKey{3284}
\def\EQKPWithAttnScaleAbsMinMeanFloat{0.0051004854030907154083251953125}
\def\EQKPWithAttnScaleAbsMinMeanKey{6549}
\def\EQKPWithAttnScaleAbsMinMedianFloat{0.000001726580222793927532620728015899658203125}
\def\EQKPWithAttnScaleAbsMinMedianKey{17197}
\def\EQKPWithAttnScaleAbsMinMinFloat{0.0000017148498727692640386521816253662109375}
\def\EQKPWithAttnScaleAbsMinMinKey{4647}
\def\EQKPWithAttnScaleAbsMinStdDevFloat{0.013399052433669567108154296875}
\def\EQKPWithAttnScaleAbsStdDevLen{151}
\def\EQKPWithAttnScaleAbsStdDevMaxFloat{0.4070548713207244873046875}
\def\EQKPWithAttnScaleAbsStdDevMaxKey{30463}
\def\EQKPWithAttnScaleAbsStdDevMeanFloat{0.16222767531871795654296875}
\def\EQKPWithAttnScaleAbsStdDevMeanKey{2549}
\def\EQKPWithAttnScaleAbsStdDevMedianFloat{0.056622199714183807373046875}
\def\EQKPWithAttnScaleAbsStdDevMedianKey{9816}
\def\EQKPWithAttnScaleAbsStdDevMinFloat{0.04753597080707550048828125}
\def\EQKPWithAttnScaleAbsStdDevMinKey{27714}
\def\EQKPWithAttnScaleAbsStdDevStdDevFloat{0.073805391788482666015625}
\def\EQKPWithAttnScaleLen{1280}
\def\EQKPWithAttnScaleMaxLen{151}
\def\EQKPWithAttnScaleMaxMaxFloat{1.7742955684661865234375}
\def\EQKPWithAttnScaleMaxMaxKey{29195}
\def\EQKPWithAttnScaleMaxMeanFloat{0.62287461757659912109375}
\def\EQKPWithAttnScaleMaxMeanKey{50}
\def\EQKPWithAttnScaleMaxMedianFloat{0.2460241280496120452880859375}
\def\EQKPWithAttnScaleMaxMedianKey{13293}
\def\EQKPWithAttnScaleMaxMinFloat{0.245951116085052490234375}
\def\EQKPWithAttnScaleMaxMinKey{27714}
\def\EQKPWithAttnScaleMaxRowDiffLen{128}
\def\EQKPWithAttnScaleMaxRowDiffMaxLen{151}
\def\EQKPWithAttnScaleMaxRowDiffMaxMaxFloat{3.3100681304931640625}
\def\EQKPWithAttnScaleMaxRowDiffMaxMaxKey{20013}
\def\EQKPWithAttnScaleMaxRowDiffMaxMeanFloat{1.24306690692901611328125}
\def\EQKPWithAttnScaleMaxRowDiffMaxMeanKey{12552}
\def\EQKPWithAttnScaleMaxRowDiffMaxMedianFloat{0.487840168178081512451171875}
\def\EQKPWithAttnScaleMaxRowDiffMaxMedianKey{27714}
\def\EQKPWithAttnScaleMaxRowDiffMaxMinFloat{0.4775265157222747802734375}
\def\EQKPWithAttnScaleMaxRowDiffMaxMinKey{9816}
\def\EQKPWithAttnScaleMaxRowDiffMaxStdDevFloat{0.53938615322113037109375}
\def\EQKPWithAttnScaleMaxRowDiffMeanLen{151}
\def\EQKPWithAttnScaleMaxRowDiffMeanMaxFloat{2.0490894317626953125}
\def\EQKPWithAttnScaleMaxRowDiffMeanMaxKey{16284}
\def\EQKPWithAttnScaleMaxRowDiffMeanMeanFloat{0.937075555324554443359375}
\def\EQKPWithAttnScaleMaxRowDiffMeanMeanKey{15622}
\def\EQKPWithAttnScaleMaxRowDiffMeanMedianFloat{0.359958648681640625}
\def\EQKPWithAttnScaleMaxRowDiffMeanMedianKey{9816}
\def\EQKPWithAttnScaleMaxRowDiffMeanMinFloat{0.303741514682769775390625}
\def\EQKPWithAttnScaleMaxRowDiffMeanMinKey{27714}
\def\EQKPWithAttnScaleMaxRowDiffMeanStdDevFloat{0.3936495482921600341796875}
\def\EQKPWithAttnScaleMaxRowDiffMedianLen{151}
\def\EQKPWithAttnScaleMaxRowDiffMedianMaxFloat{1.687067834138870292548517682007513940334320068359375}
\def\EQKPWithAttnScaleMaxRowDiffMedianMaxKey{29195}
\def\EQKPWithAttnScaleMaxRowDiffMedianMeanFloat{0.72052885138879929627364617772400379180908203125}
\def\EQKPWithAttnScaleMaxRowDiffMedianMeanKey{6155}
\def\EQKPWithAttnScaleMaxRowDiffMedianMedianFloat{0.2348402667231857809948536441879696212708950042724609375}
\def\EQKPWithAttnScaleMaxRowDiffMedianMedianKey{17080}
\def\EQKPWithAttnScaleMaxRowDiffMedianMinFloat{0.2295057833194732721526776231257827021181583404541015625}
\def\EQKPWithAttnScaleMaxRowDiffMedianMinKey{27714}
\def\EQKPWithAttnScaleMaxRowDiffMedianStdDevFloat{0.3185047978553010583624427454196847975254058837890625}
\def\EQKPWithAttnScaleMaxRowDiffMinLen{151}
\def\EQKPWithAttnScaleMaxRowDiffMinMaxFloat{1.6834042072296142578125}
\def\EQKPWithAttnScaleMaxRowDiffMinMaxKey{29195}
\def\EQKPWithAttnScaleMaxRowDiffMinMeanFloat{0.695503711700439453125}
\def\EQKPWithAttnScaleMaxRowDiffMinMeanKey{26374}
\def\EQKPWithAttnScaleMaxRowDiffMinMedianFloat{0.224578537046909332275390625}
\def\EQKPWithAttnScaleMaxRowDiffMinMedianKey{27714}
\def\EQKPWithAttnScaleMaxRowDiffMinMinFloat{0.21496999263763427734375}
\def\EQKPWithAttnScaleMaxRowDiffMinMinKey{17080}
\def\EQKPWithAttnScaleMaxRowDiffMinStdDevFloat{0.31191217899322509765625}
\def\EQKPWithAttnScaleMaxRowDiffStdDevLen{151}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMaxFloat{0.3016908168792724609375}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMaxKey{19917}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMeanFloat{0.094798028469085693359375}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMeanKey{22261}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMedianFloat{0.032717703841626644134521484375}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMedianKey{13654}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMinFloat{0.0312546230852603912353515625}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMinKey{9816}
\def\EQKPWithAttnScaleMaxRowDiffStdDevStdDevFloat{0.0423058383166790008544921875}
\def\EQKPWithAttnScaleMaxStdDevFloat{0.2815231978893280029296875}
\def\EQKPWithAttnScaleMeanLen{151}
\def\EQKPWithAttnScaleMeanMaxFloat{0.000000389199698247466585598886013031005859375}
\def\EQKPWithAttnScaleMeanMaxKey{32382}
\def\EQKPWithAttnScaleMeanMeanFloat{0.00000002059361037254348048008978366851806640625}
\def\EQKPWithAttnScaleMeanMeanKey{4810}
\def\EQKPWithAttnScaleMeanMedianFloat{-0.00000031730741056890110485255718231201171875}
\def\EQKPWithAttnScaleMeanMedianKey{30684}
\def\EQKPWithAttnScaleMeanMinFloat{-0.00000032053793574959854595363140106201171875}
\def\EQKPWithAttnScaleMeanMinKey{12141}
\def\EQKPWithAttnScaleMeanStdDevFloat{0.0000001481218561139030498452484607696533203125}
\def\EQKPWithAttnScaleMedianLen{151}
\def\EQKPWithAttnScaleMedianMaxFloat{-0.1975913164019584555841646533735911361873149871826171875}
\def\EQKPWithAttnScaleMedianMaxKey{19488}
\def\EQKPWithAttnScaleMedianMeanFloat{-0.56202118254704591659987045204616151750087738037109375}
\def\EQKPWithAttnScaleMedianMeanKey{50}
\def\EQKPWithAttnScaleMedianMedianFloat{-1.4799924899637699748922159415087662637233734130859375}
\def\EQKPWithAttnScaleMedianMedianKey{30463}
\def\EQKPWithAttnScaleMedianMinFloat{-1.5125423556566237603959734769887290894985198974609375}
\def\EQKPWithAttnScaleMedianMinKey{20976}
\def\EQKPWithAttnScaleMedianStdDevFloat{0.257164667554734382992620567165431566536426544189453125}
\def\EQKPWithAttnScaleMinLen{151}
\def\EQKPWithAttnScaleMinMaxFloat{-0.228154718875885009765625}
\def\EQKPWithAttnScaleMinMaxKey{19488}
\def\EQKPWithAttnScaleMinMeanFloat{-0.633526861667633056640625}
\def\EQKPWithAttnScaleMinMeanKey{104}
\def\EQKPWithAttnScaleMinMedianFloat{-1.9356519877910614013671875}
\def\EQKPWithAttnScaleMinMedianKey{20976}
\def\EQKPWithAttnScaleMinMinFloat{-2.2270667552947998046875}
\def\EQKPWithAttnScaleMinMinKey{20013}
\def\EQKPWithAttnScaleMinStdDevFloat{0.31251585483551025390625}
\def\EQKPWithAttnScaleStdDevLen{151}
\def\EQKPWithAttnScaleStdDevMaxFloat{0.65388906002044677734375}
\def\EQKPWithAttnScaleStdDevMaxKey{13468}
\def\EQKPWithAttnScaleStdDevMeanFloat{0.2797189056873321533203125}
\def\EQKPWithAttnScaleStdDevMeanKey{4810}
\def\EQKPWithAttnScaleStdDevMedianFloat{0.11026259325444698333740234375}
\def\EQKPWithAttnScaleStdDevMedianKey{5615}
\def\EQKPWithAttnScaleStdDevMinFloat{0.09907759726047515869140625}
\def\EQKPWithAttnScaleStdDevMinKey{27714}
\def\EQKPWithAttnScaleStdDevStdDevFloat{0.117366306483745574951171875}
\def\EUPUAbsLenLen{151}
\def\EUPUAbsLenMaxFloat{16384}
\def\EUPUAbsLenMaxKey{50}
\def\EUPUAbsLenMeanFloat{16384}
\def\EUPUAbsLenMeanKey{50}
\def\EUPUAbsLenMedianFloat{16384}
\def\EUPUAbsLenMedianKey{50}
\def\EUPUAbsLenMinFloat{16384}
\def\EUPUAbsLenMinKey{50}
\def\EUPUAbsLenStdDevFloat{0}
\def\EUPUAbsMaxLen{151}
\def\EUPUAbsMaxMaxFloat{7.949287891387939453125}
\def\EUPUAbsMaxMaxKey{20013}
\def\EUPUAbsMaxMeanFloat{2.6908891201019287109375}
\def\EUPUAbsMaxMeanKey{8721}
\def\EUPUAbsMaxMedianFloat{2.2588036060333251953125}
\def\EUPUAbsMaxMedianKey{8745}
\def\EUPUAbsMaxMinFloat{2.242000102996826171875}
\def\EUPUAbsMaxMinKey{6082}
\def\EUPUAbsMaxStdDevFloat{0.472648680210113525390625}
\def\EUPUAbsMeanLen{151}
\def\EUPUAbsMeanMaxFloat{1.2186725139617919921875}
\def\EUPUAbsMeanMaxKey{20013}
\def\EUPUAbsMeanMeanFloat{0.940766513347625732421875}
\def\EUPUAbsMeanMeanKey{22401}
\def\EUPUAbsMeanMedianFloat{0.73910032212734222412109375}
\def\EUPUAbsMeanMedianKey{4810}
\def\EUPUAbsMeanMinFloat{0.735749661922454833984375}
\def\EUPUAbsMeanMinKey{20338}
\def\EUPUAbsMeanStdDevFloat{0.078182280063629150390625}
\def\EUPUAbsMedianLen{151}
\def\EUPUAbsMedianMaxFloat{0.0164846247434616115234984334847467835061252117156982421875}
\def\EUPUAbsMedianMaxKey{17080}
\def\EUPUAbsMedianMeanFloat{0.00965058149470768809885523609182200743816792964935302734375}
\def\EUPUAbsMedianMeanKey{18668}
\def\EUPUAbsMedianMedianFloat{0.006321123851230367983455860070307608111761510372161865234375}
\def\EUPUAbsMedianMedianKey{4810}
\def\EUPUAbsMedianMinFloat{0.006125224339775741690117261128989412100054323673248291015625}
\def\EUPUAbsMedianMinKey{2773}
\def\EUPUAbsMedianStdDevFloat{0.00193672384703915258057083104148432539659552276134490966796875}
\def\EUPUAbsMinLen{151}
\def\EUPUAbsMinMaxFloat{0.00063370284624397754669189453125}
\def\EUPUAbsMinMaxKey{24144}
\def\EUPUAbsMinMeanFloat{0.00013029304682277143001556396484375}
\def\EUPUAbsMinMeanKey{8745}
\def\EUPUAbsMinMedianFloat{0.00000249118278361493139527738094329833984375}
\def\EUPUAbsMinMedianKey{27300}
\def\EUPUAbsMinMinFloat{0.00000058767545851878821849822998046875}
\def\EUPUAbsMinMinKey{22286}
\def\EUPUAbsMinStdDevFloat{0.000132284942083060741424560546875}
\def\EUPUAbsStdDevLen{151}
\def\EUPUAbsStdDevMaxFloat{0.724738895893096923828125}
\def\EUPUAbsStdDevMaxKey{20013}
\def\EUPUAbsStdDevMeanFloat{0.519364833831787109375}
\def\EUPUAbsStdDevMeanKey{26932}
\def\EUPUAbsStdDevMedianFloat{0.4353931844234466552734375}
\def\EUPUAbsStdDevMedianKey{13293}
\def\EUPUAbsStdDevMinFloat{0.4331655204296112060546875}
\def\EUPUAbsStdDevMinKey{6082}
\def\EUPUAbsStdDevStdDevFloat{0.0471253357827663421630859375}
\def\EUPULenLen{151}
\def\EUPULenMaxFloat{16384}
\def\EUPULenMaxKey{50}
\def\EUPULenMeanFloat{16384}
\def\EUPULenMeanKey{50}
\def\EUPULenMedianFloat{16384}
\def\EUPULenMedianKey{50}
\def\EUPULenMinFloat{16384}
\def\EUPULenMinKey{50}
\def\EUPULenStdDevFloat{0}
\def\EUPUMaxLen{151}
\def\EUPUMaxMaxFloat{7.949287891387939453125}
\def\EUPUMaxMaxKey{20013}
\def\EUPUMaxMeanFloat{2.2092511653900146484375}
\def\EUPUMaxMeanKey{24438}
\def\EUPUMaxMedianFloat{1.7414084970951080322265625}
\def\EUPUMaxMedianKey{19488}
\def\EUPUMaxMinFloat{1.70965945720672607421875}
\def\EUPUMaxMinKey{12561}
\def\EUPUMaxRowDiffLenLen{151}
\def\EUPUMaxRowDiffLenMaxFloat{128}
\def\EUPUMaxRowDiffLenMaxKey{50}
\def\EUPUMaxRowDiffLenMeanFloat{128}
\def\EUPUMaxRowDiffLenMeanKey{50}
\def\EUPUMaxRowDiffLenMedianFloat{128}
\def\EUPUMaxRowDiffLenMedianKey{50}
\def\EUPUMaxRowDiffLenMinFloat{128}
\def\EUPUMaxRowDiffLenMinKey{50}
\def\EUPUMaxRowDiffLenStdDevFloat{0}
\def\EUPUMaxRowDiffMaxLen{151}
\def\EUPUMaxRowDiffMaxMaxFloat{13.09485626220703125}
\def\EUPUMaxRowDiffMaxMaxKey{20013}
\def\EUPUMaxRowDiffMaxMeanFloat{4.639370441436767578125}
\def\EUPUMaxRowDiffMaxMeanKey{3254}
\def\EUPUMaxRowDiffMaxMedianFloat{3.937569558620452880859375}
\def\EUPUMaxRowDiffMaxMedianKey{19488}
\def\EUPUMaxRowDiffMaxMinFloat{3.90132236480712890625}
\def\EUPUMaxRowDiffMaxMinKey{3175}
\def\EUPUMaxRowDiffMaxStdDevFloat{0.76212394237518310546875}
\def\EUPUMaxRowDiffMeanLen{151}
\def\EUPUMaxRowDiffMeanMaxFloat{4.904124736785888671875}
\def\EUPUMaxRowDiffMeanMaxKey{20013}
\def\EUPUMaxRowDiffMeanMeanFloat{3.4314563274383544921875}
\def\EUPUMaxRowDiffMeanMeanKey{12552}
\def\EUPUMaxRowDiffMeanMedianFloat{2.975428640842437744140625}
\def\EUPUMaxRowDiffMeanMedianKey{32382}
\def\EUPUMaxRowDiffMeanMinFloat{2.965168476104736328125}
\def\EUPUMaxRowDiffMeanMinKey{22545}
\def\EUPUMaxRowDiffMeanStdDevFloat{0.2588199675083160400390625}
\def\EUPUMaxRowDiffMedianLen{151}
\def\EUPUMaxRowDiffMedianMaxFloat{3.770801358222961585653365546022541821002960205078125}
\def\EUPUMaxRowDiffMedianMaxKey{20013}
\def\EUPUMaxRowDiffMedianMeanFloat{2.745064192718228213152542593888938426971435546875}
\def\EUPUMaxRowDiffMedianMeanKey{28090}
\def\EUPUMaxRowDiffMedianMedianFloat{2.205518285334110206719060442992486059665679931640625}
\def\EUPUMaxRowDiffMedianMedianKey{32382}
\def\EUPUMaxRowDiffMedianMinFloat{2.1863294339179990544153042719699442386627197265625}
\def\EUPUMaxRowDiffMedianMinKey{913}
\def\EUPUMaxRowDiffMedianStdDevFloat{0.244996160822353703512277434128918685019016265869140625}
\def\EUPUMaxRowDiffMinLen{151}
\def\EUPUMaxRowDiffMinMaxFloat{3.6710660457611083984375}
\def\EUPUMaxRowDiffMinMaxKey{20013}
\def\EUPUMaxRowDiffMinMeanFloat{2.685910701751708984375}
\def\EUPUMaxRowDiffMinMeanKey{30371}
\def\EUPUMaxRowDiffMinMedianFloat{2.10103380680084228515625}
\def\EUPUMaxRowDiffMinMedianKey{104}
\def\EUPUMaxRowDiffMinMinFloat{2.061328887939453125}
\def\EUPUMaxRowDiffMinMinKey{913}
\def\EUPUMaxRowDiffMinStdDevFloat{0.253579795360565185546875}
\def\EUPUMaxRowDiffStdDevLen{151}
\def\EUPUMaxRowDiffStdDevMaxFloat{0.810237824916839599609375}
\def\EUPUMaxRowDiffStdDevMaxKey{20013}
\def\EUPUMaxRowDiffStdDevMeanFloat{0.3516359031200408935546875}
\def\EUPUMaxRowDiffStdDevMeanKey{32382}
\def\EUPUMaxRowDiffStdDevMedianFloat{0.2485837824642658233642578125}
\def\EUPUMaxRowDiffStdDevMedianKey{8299}
\def\EUPUMaxRowDiffStdDevMinFloat{0.24621678888797760009765625}
\def\EUPUMaxRowDiffStdDevMinKey{12457}
\def\EUPUMaxRowDiffStdDevStdDevFloat{0.07434903085231781005859375}
\def\EUPUMaxStdDevFloat{0.5154416561126708984375}
\def\EUPUMeanLen{151}
\def\EUPUMeanMaxFloat{-0.46974790096282958984375}
\def\EUPUMeanMaxKey{19451}
\def\EUPUMeanMeanFloat{-0.652157604694366455078125}
\def\EUPUMeanMeanKey{3284}
\def\EUPUMeanMedianFloat{-0.84934477508068084716796875}
\def\EUPUMeanMedianKey{519}
\def\EUPUMeanMinFloat{-0.95542430877685546875}
\def\EUPUMeanMinKey{20013}
\def\EUPUMeanStdDevFloat{0.071444235742092132568359375}
\def\EUPUMedianLen{151}
\def\EUPUMedianMaxFloat{-1.769431335330009513739923932007513940334320068359375}
\def\EUPUMedianMaxKey{32382}
\def\EUPUMedianMeanFloat{-2.08901971312942880132368372869677841663360595703125}
\def\EUPUMedianMeanKey{8840}
\def\EUPUMedianMedianFloat{-2.53752841532230366539124588598497211933135986328125}
\def\EUPUMedianMedianKey{2345}
\def\EUPUMedianMinFloat{-2.87063584566116336560526178800500929355621337890625}
\def\EUPUMedianMinKey{20013}
\def\EUPUMedianStdDevFloat{0.132577626836272777222092145166243426501750946044921875}
\def\EUPUMinLen{151}
\def\EUPUMinMaxFloat{-2.242000102996826171875}
\def\EUPUMinMaxKey{6082}
\def\EUPUMinMeanFloat{-2.665431499481201171875}
\def\EUPUMinMeanKey{104}
\def\EUPUMinMedianFloat{-3.6639382839202880859375}
\def\EUPUMinMedianKey{23696}
\def\EUPUMinMinFloat{-5.145568370819091796875}
\def\EUPUMinMinKey{20013}
\def\EUPUMinStdDevFloat{0.283378779888153076171875}
\def\EUPUStdDevLen{151}
\def\EUPUStdDevMaxFloat{1.0476515293121337890625}
\def\EUPUStdDevMaxKey{20013}
\def\EUPUStdDevMeanFloat{0.853788852691650390625}
\def\EUPUStdDevMeanKey{6589}
\def\EUPUStdDevMedianFloat{0.7076859176158905029296875}
\def\EUPUStdDevMedianKey{20338}
\def\EUPUStdDevMinFloat{0.7066462039947509765625}
\def\EUPUStdDevMinKey{32382}
\def\EUPUStdDevStdDevFloat{0.0612009726464748382568359375}
\def\EVOUHistMinAboveDiagDupBySeqCountLenLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMaxFloat{1180591620717411303424}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMaxKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMeanFloat{1180591620717411303424}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMeanKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMedianFloat{1180591620717411303424}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMedianKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMinFloat{1180591620717411303424}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMinKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountLenStdDevFloat{0}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMaxFloat{32.37884521484375}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMaxKey{20013}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMeanFloat{13.98551654815673828125}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMeanKey{10248}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMedianFloat{10.9779918193817138671875}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMedianKey{30684}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMinFloat{10.621227264404296875}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMinKey{19538}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxStdDevFloat{2.0306780338287353515625}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMaxFloat{-7.13879853053825996767045580781996250152587890625}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMaxKey{20013}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMeanFloat{-9.17762135537744683233540854416787624359130859375}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMeanKey{14095}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMedianFloat{-10.1146459975619134041835422976873815059661865234375}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMedianKey{4305}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMinFloat{-10.318915638709373894243981339968740940093994140625}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMinKey{17080}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanStdDevFloat{0.4194109039878999301009798728046007454395294189453125}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMaxFloat{-7.76761424334522931900437470176257193088531494140625}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMaxKey{29726}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMeanFloat{-9.3312624588333079600488417781889438629150390625}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMeanKey{29565}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMedianFloat{-10.850057982386704935606758226640522480010986328125}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMedianKey{519}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMinFloat{-10.8509219577971887105150017305277287960052490234375}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMinKey{18668}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianStdDevFloat{0.5981229398575249600611414280137978494167327880859375}
\def\EVOUHistMinAboveDiagDupBySeqCountMinLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMaxFloat{-11.3302402496337890625}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMaxKey{32374}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMeanFloat{-13.460628509521484375}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMeanKey{7098}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMedianFloat{-17.17393207550048828125}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMedianKey{12493}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMinFloat{-17.28411865234375}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMinKey{17080}
\def\EVOUHistMinAboveDiagDupBySeqCountMinStdDevFloat{1.0479488372802734375}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMaxFloat{54}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMaxKey{20013}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMeanFloat{-1.5562913907284767756067367372452281415462493896484375}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMeanKey{104}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMedianFloat{-5}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMedianKey{1283}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMinFloat{-5}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMinKey{1283}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMaxFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMaxKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMeanFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMeanKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMedianFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMedianKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMinFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMinKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdStdDevFloat{0}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMaxFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMaxKey{20013}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMeanFloat{0.99247788231235223310733317703125067055225372314453125}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMeanKey{7884}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMedianFloat{0.94941915900917750459342414615093730390071868896484375}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMedianKey{8745}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMinFloat{0.9480770383580512383758787109400145709514617919921875}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMinKey{30899}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracStdDevFloat{0.00851120900510418144924162930919919745065271854400634765625}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueStdDevFloat{4.818061715726397409298442653380334377288818359375}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMaxFloat{12.09824711625945070636589662171900272369384765625}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMaxKey{20539}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMeanFloat{10.3173318916122358501752387383021414279937744140625}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMeanKey{9504}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMedianFloat{9.301860381323511006712578819133341312408447265625}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMedianKey{20338}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMinFloat{9.285280171418552441764404647983610630035400390625}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMinKey{24144}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevStdDevFloat{0.51872185575196549933707501622848212718963623046875}
\def\EVOUHistMinAboveDiagLenLen{151}
\def\EVOUHistMinAboveDiagLenMaxFloat{128}
\def\EVOUHistMinAboveDiagLenMaxKey{50}
\def\EVOUHistMinAboveDiagLenMeanFloat{128}
\def\EVOUHistMinAboveDiagLenMeanKey{50}
\def\EVOUHistMinAboveDiagLenMedianFloat{128}
\def\EVOUHistMinAboveDiagLenMedianKey{50}
\def\EVOUHistMinAboveDiagLenMinFloat{128}
\def\EVOUHistMinAboveDiagLenMinKey{50}
\def\EVOUHistMinAboveDiagLenStdDevFloat{0}
\def\EVOUHistMinAboveDiagMaxLen{151}
\def\EVOUHistMinAboveDiagMaxMaxFloat{32.37884521484375}
\def\EVOUHistMinAboveDiagMaxMaxKey{20013}
\def\EVOUHistMinAboveDiagMaxMeanFloat{13.98551654815673828125}
\def\EVOUHistMinAboveDiagMaxMeanKey{10248}
\def\EVOUHistMinAboveDiagMaxMedianFloat{10.9779918193817138671875}
\def\EVOUHistMinAboveDiagMaxMedianKey{30684}
\def\EVOUHistMinAboveDiagMaxMinFloat{10.621227264404296875}
\def\EVOUHistMinAboveDiagMaxMinKey{19538}
\def\EVOUHistMinAboveDiagMaxStdDevFloat{2.0306780338287353515625}
\def\EVOUHistMinAboveDiagMeanLen{151}
\def\EVOUHistMinAboveDiagMeanMaxFloat{1.79043686389923095703125}
\def\EVOUHistMinAboveDiagMeanMaxKey{13716}
\def\EVOUHistMinAboveDiagMeanMeanFloat{0.78453457355499267578125}
\def\EVOUHistMinAboveDiagMeanMeanKey{31308}
\def\EVOUHistMinAboveDiagMeanMedianFloat{0.0016394220292568206787109375}
\def\EVOUHistMinAboveDiagMeanMedianKey{27584}
\def\EVOUHistMinAboveDiagMeanMinFloat{-0.11464436352252960205078125}
\def\EVOUHistMinAboveDiagMeanMinKey{29565}
\def\EVOUHistMinAboveDiagMeanStdDevFloat{0.388307631015777587890625}
\def\EVOUHistMinAboveDiagMedianLen{151}
\def\EVOUHistMinAboveDiagMedianMaxFloat{1.616853237152099609375}
\def\EVOUHistMinAboveDiagMedianMaxKey{14095}
\def\EVOUHistMinAboveDiagMedianMeanFloat{-0.286206182265123787455962656167685054242610931396484375}
\def\EVOUHistMinAboveDiagMedianMeanKey{1283}
\def\EVOUHistMinAboveDiagMedianMedianFloat{-1.5716953277587890625}
\def\EVOUHistMinAboveDiagMedianMedianKey{30463}
\def\EVOUHistMinAboveDiagMedianMinFloat{-1.60052585601806640625}
\def\EVOUHistMinAboveDiagMedianMinKey{7467}
\def\EVOUHistMinAboveDiagMedianStdDevFloat{0.60401548394965576260773332251119427382946014404296875}
\def\EVOUHistMinAboveDiagMinLen{151}
\def\EVOUHistMinAboveDiagMinMaxFloat{-11.3302402496337890625}
\def\EVOUHistMinAboveDiagMinMaxKey{32374}
\def\EVOUHistMinAboveDiagMinMeanFloat{-13.460628509521484375}
\def\EVOUHistMinAboveDiagMinMeanKey{7098}
\def\EVOUHistMinAboveDiagMinMedianFloat{-17.17393207550048828125}
\def\EVOUHistMinAboveDiagMinMedianKey{12493}
\def\EVOUHistMinAboveDiagMinMinFloat{-17.28411865234375}
\def\EVOUHistMinAboveDiagMinMinKey{17080}
\def\EVOUHistMinAboveDiagMinStdDevFloat{1.0479488372802734375}
\def\EVOUHistMinAboveDiagMostBelowValueLen{151}
\def\EVOUHistMinAboveDiagMostBelowValueMaxFloat{72}
\def\EVOUHistMinAboveDiagMostBelowValueMaxKey{20539}
\def\EVOUHistMinAboveDiagMostBelowValueMeanFloat{57.913907284768214367431937716901302337646484375}
\def\EVOUHistMinAboveDiagMostBelowValueMeanKey{1412}
\def\EVOUHistMinAboveDiagMostBelowValueMedianFloat{46.75}
\def\EVOUHistMinAboveDiagMostBelowValueMedianKey{2743}
\def\EVOUHistMinAboveDiagMostBelowValueMinFloat{46}
\def\EVOUHistMinAboveDiagMostBelowValueMinKey{20013}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdLen{151}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMaxFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMaxKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMeanFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMeanKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMedianFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMedianKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMinFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMinKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdStdDevFloat{0}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracLen{151}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMaxFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMaxKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMeanFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMeanKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMedianFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMedianKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMinFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMinKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracStdDevFloat{0}
\def\EVOUHistMinAboveDiagMostBelowValueStdDevFloat{5.698774583451541531076145474798977375030517578125}
\def\EVOUHistMinAboveDiagStdDevLen{151}
\def\EVOUHistMinAboveDiagStdDevMaxFloat{8.410259246826171875}
\def\EVOUHistMinAboveDiagStdDevMaxKey{20539}
\def\EVOUHistMinAboveDiagStdDevMeanFloat{7.585827350616455078125}
\def\EVOUHistMinAboveDiagStdDevMeanKey{29022}
\def\EVOUHistMinAboveDiagStdDevMedianFloat{6.83585560321807861328125}
\def\EVOUHistMinAboveDiagStdDevMedianKey{2743}
\def\EVOUHistMinAboveDiagStdDevMinFloat{6.74063968658447265625}
\def\EVOUHistMinAboveDiagStdDevMinKey{20013}
\def\EVOUHistMinAboveDiagStdDevStdDevFloat{0.357729613780975341796875}
\def\EVOUMaxRowDiffLenLen{151}
\def\EVOUMaxRowDiffLenMaxFloat{128}
\def\EVOUMaxRowDiffLenMaxKey{50}
\def\EVOUMaxRowDiffLenMeanFloat{128}
\def\EVOUMaxRowDiffLenMeanKey{50}
\def\EVOUMaxRowDiffLenMedianFloat{128}
\def\EVOUMaxRowDiffLenMedianKey{50}
\def\EVOUMaxRowDiffLenMinFloat{128}
\def\EVOUMaxRowDiffLenMinKey{50}
\def\EVOUMaxRowDiffLenStdDevFloat{0}
\def\EVOUMaxRowDiffMaxLen{151}
\def\EVOUMaxRowDiffMaxMaxFloat{99.111328125}
\def\EVOUMaxRowDiffMaxMaxKey{11124}
\def\EVOUMaxRowDiffMaxMeanFloat{80.4996490478515625}
\def\EVOUMaxRowDiffMaxMeanKey{19538}
\def\EVOUMaxRowDiffMaxMedianFloat{68.8199310302734375}
\def\EVOUMaxRowDiffMaxMedianKey{20338}
\def\EVOUMaxRowDiffMaxMinFloat{67.29866790771484375}
\def\EVOUMaxRowDiffMaxMinKey{20013}
\def\EVOUMaxRowDiffMaxStdDevFloat{5.99790096282958984375}
\def\EVOUMaxRowDiffMeanLen{151}
\def\EVOUMaxRowDiffMeanMaxFloat{44.1446380615234375}
\def\EVOUMaxRowDiffMeanMaxKey{123}
\def\EVOUMaxRowDiffMeanMeanFloat{37.849552154541015625}
\def\EVOUMaxRowDiffMeanMeanKey{1412}
\def\EVOUMaxRowDiffMeanMedianFloat{32.0808277130126953125}
\def\EVOUMaxRowDiffMeanMedianKey{20338}
\def\EVOUMaxRowDiffMeanMinFloat{28.35857391357421875}
\def\EVOUMaxRowDiffMeanMinKey{20013}
\def\EVOUMaxRowDiffMeanStdDevFloat{2.2263057231903076171875}
\def\EVOUMaxRowDiffMedianLen{151}
\def\EVOUMaxRowDiffMedianMaxFloat{30.276912021636963601167735760100185871124267578125}
\def\EVOUMaxRowDiffMedianMaxKey{20976}
\def\EVOUMaxRowDiffMedianMeanFloat{24.429066270487201251171427429653704166412353515625}
\def\EVOUMaxRowDiffMedianMeanKey{28716}
\def\EVOUMaxRowDiffMedianMedianFloat{19.618532333374023579608547152020037174224853515625}
\def\EVOUMaxRowDiffMedianMedianKey{6910}
\def\EVOUMaxRowDiffMedianMinFloat{18.27992395401000891297371708787977695465087890625}
\def\EVOUMaxRowDiffMedianMinKey{20013}
\def\EVOUMaxRowDiffMedianStdDevFloat{2.176112656454615379431061228387989103794097900390625}
\def\EVOUMaxRowDiffMinLen{151}
\def\EVOUMaxRowDiffMinMaxFloat{29.330539703369140625}
\def\EVOUMaxRowDiffMinMaxKey{8840}
\def\EVOUMaxRowDiffMinMeanFloat{23.105083465576171875}
\def\EVOUMaxRowDiffMinMeanKey{2773}
\def\EVOUMaxRowDiffMinMedianFloat{14.945095539093017578125}
\def\EVOUMaxRowDiffMinMedianKey{6910}
\def\EVOUMaxRowDiffMinMinFloat{13.6133365631103515625}
\def\EVOUMaxRowDiffMinMinKey{6082}
\def\EVOUMaxRowDiffMinStdDevFloat{2.7938079833984375}
\def\EVOUMaxRowDiffStdDevLen{151}
\def\EVOUMaxRowDiffStdDevMaxFloat{13.58303070068359375}
\def\EVOUMaxRowDiffStdDevMaxKey{4810}
\def\EVOUMaxRowDiffStdDevMeanFloat{10.10936450958251953125}
\def\EVOUMaxRowDiffStdDevMeanKey{20539}
\def\EVOUMaxRowDiffStdDevMedianFloat{8.580819606781005859375}
\def\EVOUMaxRowDiffStdDevMedianKey{12561}
\def\EVOUMaxRowDiffStdDevMinFloat{8.55801296234130859375}
\def\EVOUMaxRowDiffStdDevMinKey{16149}
\def\EVOUMaxRowDiffStdDevStdDevFloat{0.826801002025604248046875}
\def\ImportanceSamplingAccuracyLen{151}
\def\ImportanceSamplingAccuracyMaxFloat{0.99885328179059162945208072414970956742763519287109375}
\def\ImportanceSamplingAccuracyMaxKey{25516}
\def\ImportanceSamplingAccuracyMeanFloat{0.99723292088841564151380225666798651218414306640625}
\def\ImportanceSamplingAccuracyMeanKey{3284}
\def\ImportanceSamplingAccuracyMedianFloat{0.98230771243874581699628834030590951442718505859375}
\def\ImportanceSamplingAccuracyMedianKey{16284}
\def\ImportanceSamplingAccuracyMinFloat{0.96612543173239540106322920109960250556468963623046875}
\def\ImportanceSamplingAccuracyMinKey{20013}
\def\ImportanceSamplingAccuracyStdDevFloat{0.0030678799605512903359016974036421743221580982208251953125}
\def\ImportanceSamplingBatchSize{4096}
\def\ImportanceSamplingInstructionCountBranch{0}
\def\ImportanceSamplingInstructionCountInt{0}
\def\ImportanceSamplingInstructionCount{0}
\def\ImportanceSamplingLossLen{151}
\def\ImportanceSamplingLossMaxFloat{nan}
\def\ImportanceSamplingLossMaxKey{50}
\def\ImportanceSamplingLossMeanFloat{nan}
\def\ImportanceSamplingLossMeanKey{50}
\def\ImportanceSamplingLossMedianFloat{nan}
\def\ImportanceSamplingLossMedianKey{50}
\def\ImportanceSamplingLossMinFloat{nan}
\def\ImportanceSamplingLossMinKey{50}
\def\ImportanceSamplingLossStdDevFloat{nan}
\def\ImportanceSamplingNSamplesPerKey{10}
\def\ImportanceSamplingNumCorrectLen{151}
\def\ImportanceSamplingNumCorrectMaxFloat{49458931}
\def\ImportanceSamplingNumCorrectMaxKey{8745}
\def\ImportanceSamplingNumCorrectMeanFloat{48341351.77483443915843963623046875}
\def\ImportanceSamplingNumCorrectMeanKey{16284}
\def\ImportanceSamplingNumCorrectMedianFloat{46316719.25}
\def\ImportanceSamplingNumCorrectMedianKey{14095}
\def\ImportanceSamplingNumCorrectMinFloat{45661445}
\def\ImportanceSamplingNumCorrectMinKey{6910}
\def\ImportanceSamplingNumCorrectStdDevFloat{553380.549414356239140033721923828125}
\def\ImportanceSamplingNumIncorrectLen{151}
\def\ImportanceSamplingNumIncorrectMaxFloat{9640325}
\def\ImportanceSamplingNumIncorrectMaxKey{6910}
\def\ImportanceSamplingNumIncorrectMeanFloat{6960418.22516556270420551300048828125}
\def\ImportanceSamplingNumIncorrectMeanKey{16284}
\def\ImportanceSamplingNumIncorrectMedianFloat{6058531.5}
\def\ImportanceSamplingNumIncorrectMedianKey{4800}
\def\ImportanceSamplingNumIncorrectMinFloat{5842839}
\def\ImportanceSamplingNumIncorrectMinKey{8745}
\def\ImportanceSamplingNumIncorrectStdDevFloat{553380.549414356239140033721923828125}
\def\ImportanceSamplingTimeLen{151}
\def\ImportanceSamplingTimeMaxFloat{2209.615185260772705078125}
\def\ImportanceSamplingTimeMaxKey{6532}
\def\ImportanceSamplingTimeMeanFloat{2078.8228050225616243551485240459442138671875}
\def\ImportanceSamplingTimeMeanKey{7884}
\def\ImportanceSamplingTimeMedianFloat{1964.228701055049896240234375}
\def\ImportanceSamplingTimeMedianKey{4800}
\def\ImportanceSamplingTimeMinFloat{1957.24325656890869140625}
\def\ImportanceSamplingTimeMinKey{4729}
\def\ImportanceSamplingTimeStdDevFloat{49.88222432502293912648383411578834056854248046875}
\def\ImportanceSamplingTotalSequences{55301770}
\def\LowerWhiskerBottomEndPercentileFloat{0.02151239536919476169618548055950668640434741973876953125}
\def\LowerWhiskerCrosshatchPercentileFloat{0.08867177532617598334496733514242805540561676025390625}
\def\MedianPercentileFloat{0.5}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffExactLinearFitIntercept{0.263425192948974984386012465620297007262706756591796875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffExactLinearFitRSquared{0.0001060210104697478783464248408563435077667236328125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffExactLinearFitSlope{0.000010858929813682752558057394154378272332905908115208148956298828125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffLinearFitIntercept{0.252411984969431346659263226683833636343479156494140625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffLinearFitRSquared{0.00018855075857204806055733570246957242488861083984375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffLinearFitSlope{0.000014102370067550120598409181538190892979400814510881900787353515625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductLinearFitIntercept{0.258205174216684429921997434576041996479034423828125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductLinearFitRSquared{0.0001208342275951235222919422085396945476531982421875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductLinearFitSlope{0.000011390342563536991305297475796098893852104083634912967681884765625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitIntercept{0.144439066678077543404157268014387227594852447509765625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitRSquared{0.0006482436569454907981935321004129946231842041015625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitSlope{0.0000161201650745332339073091765246914519593701697885990142822265625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffLinearFitIntercept{0.25205476867617537806154359714128077030181884765625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffLinearFitRSquared{0.00019539130201728927005433433805592358112335205078125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffLinearFitSlope{0.000014354988895344450019011563191018154839184717275202274322509765625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitIntercept{0.258042392446049095866555944667197763919830322265625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitRSquared{0.000122458664791214033584765275008976459503173828125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitSlope{0.000011463753222518391125376614747555237272536032833158969879150390625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitIntercept{0.1446341110925697670541723027781699784100055694580078125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitRSquared{0.000636339302210853219321506912820041179656982421875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitSlope{0.000015973583683640216342690398843018328989273868501186370849609375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitIntercept{0.1421637532502334211326200374969630502164363861083984375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitRSquared{0.00069160947351687429573985355091281235218048095703125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitSlope{0.000016450120067399050249878911245104973204433917999267578125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioSvdLinearFitIntercept{0.167626885261384417358243581475107930600643157958984375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioSvdLinearFitRSquared{0.00311522891058835238453639249200932681560516357421875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioSvdLinearFitSlope{0.0000488017448673560164736258404349911188546684570610523223876953125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffExactLinearFitIntercept{0.60966458885110930143724772278801538050174713134765625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffExactLinearFitRSquared{0.00200273405041617724720026672002859413623809814453125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffExactLinearFitSlope{0.0000058089787442975116048098083165740490585449151694774627685546875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffLinearFitIntercept{0.59582209293344490230737164893071167171001434326171875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffLinearFitRSquared{0.00152267744213274713871442145318724215030670166015625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffLinearFitSlope{0.0000046332688642094101472731874913346672428815509192645549774169921875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductLinearFitIntercept{0.60224652779812226643940675785415805876255035400390625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductLinearFitRSquared{0.00080532248847464682484087461489252746105194091796875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductLinearFitSlope{0.00000350531570029305933455647005525523951519062393344938755035400390625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitIntercept{0.35235256091795197352922741629299707710742950439453125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitRSquared{0.058886240823644353525878614163957536220550537109375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitSlope{0.0000258344173026203193020526593937091774932923726737499237060546875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffLinearFitIntercept{0.594785528193720214318318539881147444248199462890625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffLinearFitRSquared{0.0021618915696972607065617921762168407440185546875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffLinearFitSlope{0.0000055234632186219296160292237252154023963157669641077518463134765625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitIntercept{0.6017756009557080343341795014566741883754730224609375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitRSquared{0.00095722657793728682662504070322029292583465576171875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitSlope{0.0000038241935190175577758005774631211437508682138286530971527099609375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitIntercept{0.350710135658523380897122478927485644817352294921875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitRSquared{0.0639496358239954876268029693164862692356109619140625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitSlope{0.0000270264964182806498131650396743452802184037864208221435546875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitIntercept{0.3473542476947788504304526213672943413257598876953125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitRSquared{0.06461070547383351847514632027014158666133880615234375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitSlope{0.00002662740409527945261987207092868601421287166886031627655029296875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioSvdLinearFitIntercept{0.404533925392203619342268439140752889215946197509765625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioSvdLinearFitRSquared{0.41690570766939016866814426975906826555728912353515625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioSvdLinearFitSlope{0.00008538503993890225241859825988655074979760684072971343994140625}
\def\NumSeeds{151}
\def\PVOUAbsLenLen{151}
\def\PVOUAbsLenMaxFloat{1280}
\def\PVOUAbsLenMaxKey{50}
\def\PVOUAbsLenMeanFloat{1280}
\def\PVOUAbsLenMeanKey{50}
\def\PVOUAbsLenMedianFloat{1280}
\def\PVOUAbsLenMedianKey{50}
\def\PVOUAbsLenMinFloat{1280}
\def\PVOUAbsLenMinKey{50}
\def\PVOUAbsLenStdDevFloat{0}
\def\PVOUAbsMaxLen{151}
\def\PVOUAbsMaxMaxFloat{2.539762973785400390625}
\def\PVOUAbsMaxMaxKey{2345}
\def\PVOUAbsMaxMeanFloat{1.588750362396240234375}
\def\PVOUAbsMaxMeanKey{15622}
\def\PVOUAbsMaxMedianFloat{1.052676260471343994140625}
\def\PVOUAbsMaxMedianKey{20013}
\def\PVOUAbsMaxMinFloat{1.0094063282012939453125}
\def\PVOUAbsMaxMinKey{23447}
\def\PVOUAbsMaxStdDevFloat{0.2649752199649810791015625}
\def\PVOUAbsMeanLen{151}
\def\PVOUAbsMeanMaxFloat{0.487210094928741455078125}
\def\PVOUAbsMeanMaxKey{7884}
\def\PVOUAbsMeanMeanFloat{0.31770813465118408203125}
\def\PVOUAbsMeanMeanKey{2743}
\def\PVOUAbsMeanMedianFloat{0.2143751718103885650634765625}
\def\PVOUAbsMeanMedianKey{17080}
\def\PVOUAbsMeanMinFloat{0.1856017410755157470703125}
\def\PVOUAbsMeanMinKey{20013}
\def\PVOUAbsMeanStdDevFloat{0.043979100883007049560546875}
\def\PVOUAbsMedianLen{151}
\def\PVOUAbsMedianMaxFloat{0.006876935213804245827784455968867405317723751068115234375}
\def\PVOUAbsMedianMaxKey{8893}
\def\PVOUAbsMedianMeanFloat{0.0028299773471824681177200222492729153600521385669708251953125}
\def\PVOUAbsMedianMeanKey{2743}
\def\PVOUAbsMedianMedianFloat{0.000933602675795555214492693618666407928685657680034637451171875}
\def\PVOUAbsMedianMedianKey{7098}
\def\PVOUAbsMedianMinFloat{0.000875337719917297445680615108898336984566412866115570068359375}
\def\PVOUAbsMedianMinKey{8745}
\def\PVOUAbsMedianStdDevFloat{0.0011459795962775638777930709011343424208462238311767578125}
\def\PVOUAbsMinLen{151}
\def\PVOUAbsMinMaxFloat{0.0014455318450927734375}
\def\PVOUAbsMinMaxKey{15043}
\def\PVOUAbsMinMeanFloat{0.00035896679037250578403472900390625}
\def\PVOUAbsMinMeanKey{7467}
\def\PVOUAbsMinMedianFloat{0.000001609325408935546875}
\def\PVOUAbsMinMedianKey{26278}
\def\PVOUAbsMinMinFloat{0.00000035762786865234375}
\def\PVOUAbsMinMinKey{29110}
\def\PVOUAbsMinStdDevFloat{0.0003280073287896811962127685546875}
\def\PVOUAbsStdDevLen{151}
\def\PVOUAbsStdDevMaxFloat{0.39886677265167236328125}
\def\PVOUAbsStdDevMaxKey{7884}
\def\PVOUAbsStdDevMeanFloat{0.2491745054721832275390625}
\def\PVOUAbsStdDevMeanKey{2236}
\def\PVOUAbsStdDevMedianFloat{0.178475625813007354736328125}
\def\PVOUAbsStdDevMedianKey{17080}
\def\PVOUAbsStdDevMinFloat{0.14823512732982635498046875}
\def\PVOUAbsStdDevMinKey{20013}
\def\PVOUAbsStdDevStdDevFloat{0.0335726775228977203369140625}
\def\PVOULenLen{151}
\def\PVOULenMaxFloat{1280}
\def\PVOULenMaxKey{50}
\def\PVOULenMeanFloat{1280}
\def\PVOULenMeanKey{50}
\def\PVOULenMedianFloat{1280}
\def\PVOULenMedianKey{50}
\def\PVOULenMinFloat{1280}
\def\PVOULenMinKey{50}
\def\PVOULenStdDevFloat{0}
\def\PVOUMaxLen{151}
\def\PVOUMaxMaxFloat{2.539762973785400390625}
\def\PVOUMaxMaxKey{2345}
\def\PVOUMaxMeanFloat{1.48358154296875}
\def\PVOUMaxMeanKey{4800}
\def\PVOUMaxMedianFloat{0.95996446907520294189453125}
\def\PVOUMaxMedianKey{23447}
\def\PVOUMaxMinFloat{0.8795769214630126953125}
\def\PVOUMaxMinKey{17080}
\def\PVOUMaxRowDiffLenLen{151}
\def\PVOUMaxRowDiffLenMaxFloat{10}
\def\PVOUMaxRowDiffLenMaxKey{50}
\def\PVOUMaxRowDiffLenMeanFloat{10}
\def\PVOUMaxRowDiffLenMeanKey{50}
\def\PVOUMaxRowDiffLenMedianFloat{10}
\def\PVOUMaxRowDiffLenMedianKey{50}
\def\PVOUMaxRowDiffLenMinFloat{10}
\def\PVOUMaxRowDiffLenMinKey{50}
\def\PVOUMaxRowDiffLenStdDevFloat{0}
\def\PVOUMaxRowDiffMaxLen{151}
\def\PVOUMaxRowDiffMaxMaxFloat{4.33597564697265625}
\def\PVOUMaxRowDiffMaxMaxKey{9132}
\def\PVOUMaxRowDiffMaxMeanFloat{2.907640933990478515625}
\def\PVOUMaxRowDiffMaxMeanKey{29565}
\def\PVOUMaxRowDiffMaxMedianFloat{1.9386626183986663818359375}
\def\PVOUMaxRowDiffMaxMedianKey{23447}
\def\PVOUMaxRowDiffMaxMinFloat{1.87894189357757568359375}
\def\PVOUMaxRowDiffMaxMinKey{17080}
\def\PVOUMaxRowDiffMaxStdDevFloat{0.477721869945526123046875}
\def\PVOUMaxRowDiffMeanLen{151}
\def\PVOUMaxRowDiffMeanMaxFloat{2.419245243072509765625}
\def\PVOUMaxRowDiffMeanMaxKey{7884}
\def\PVOUMaxRowDiffMeanMeanFloat{1.8585774898529052734375}
\def\PVOUMaxRowDiffMeanMeanKey{13654}
\def\PVOUMaxRowDiffMeanMedianFloat{1.36928308010101318359375}
\def\PVOUMaxRowDiffMeanMedianKey{17080}
\def\PVOUMaxRowDiffMeanMinFloat{1.05514705181121826171875}
\def\PVOUMaxRowDiffMeanMinKey{20013}
\def\PVOUMaxRowDiffMeanStdDevFloat{0.20626346766948699951171875}
\def\PVOUMaxRowDiffMedianLen{151}
\def\PVOUMaxRowDiffMedianMaxFloat{1.791634323596954292412419817992486059665679931640625}
\def\PVOUMaxRowDiffMedianMaxKey{9504}
\def\PVOUMaxRowDiffMedianMeanFloat{1.1577234104255966773422414917149581015110015869140625}
\def\PVOUMaxRowDiffMedianMeanKey{2236}
\def\PVOUMaxRowDiffMedianMedianFloat{0.59454119607806210634493027100688777863979339599609375}
\def\PVOUMaxRowDiffMedianMedianKey{1490}
\def\PVOUMaxRowDiffMedianMinFloat{0.45774932801723478004163325749686919152736663818359375}
\def\PVOUMaxRowDiffMedianMinKey{20013}
\def\PVOUMaxRowDiffMedianStdDevFloat{0.212784879323588971278269355025258846580982208251953125}
\def\PVOUMaxRowDiffMinLen{151}
\def\PVOUMaxRowDiffMinMaxFloat{1.7906818389892578125}
\def\PVOUMaxRowDiffMinMaxKey{9504}
\def\PVOUMaxRowDiffMinMeanFloat{1.1486937999725341796875}
\def\PVOUMaxRowDiffMinMeanKey{23633}
\def\PVOUMaxRowDiffMinMedianFloat{0.56986688077449798583984375}
\def\PVOUMaxRowDiffMinMedianKey{1490}
\def\PVOUMaxRowDiffMinMinFloat{0.441278874874114990234375}
\def\PVOUMaxRowDiffMinMinKey{20013}
\def\PVOUMaxRowDiffMinStdDevFloat{0.216122686862945556640625}
\def\PVOUMaxRowDiffStdDevLen{151}
\def\PVOUMaxRowDiffStdDevMaxFloat{0.94805490970611572265625}
\def\PVOUMaxRowDiffStdDevMaxKey{2345}
\def\PVOUMaxRowDiffStdDevMeanFloat{0.517883121967315673828125}
\def\PVOUMaxRowDiffStdDevMeanKey{1681}
\def\PVOUMaxRowDiffStdDevMedianFloat{0.2151661179959774017333984375}
\def\PVOUMaxRowDiffStdDevMedianKey{24202}
\def\PVOUMaxRowDiffStdDevMinFloat{0.16992528736591339111328125}
\def\PVOUMaxRowDiffStdDevMinKey{3284}
\def\PVOUMaxRowDiffStdDevStdDevFloat{0.1257471144199371337890625}
\def\PVOUMaxStdDevFloat{0.276747643947601318359375}
\def\PVOUMeanLen{151}
\def\PVOUMeanMaxFloat{0.000000047683716530855235760100185871124267578125}
\def\PVOUMeanMaxKey{742}
\def\PVOUMeanMeanFloat{-0.000000000926388299404834469896741211414337158203125}
\def\PVOUMeanMeanKey{30899}
\def\PVOUMeanMedianFloat{-0.00000003296881967429499127320013940334320068359375}
\def\PVOUMeanMedianKey{23367}
\def\PVOUMeanMinFloat{-0.0000000335276126861572265625}
\def\PVOUMeanMinKey{2549}
\def\PVOUMeanStdDevFloat{0.0000000141023246413851666147820651531219482421875}
\def\PVOUMedianLen{151}
\def\PVOUMedianMaxFloat{-0.5715789806842803688624599089962430298328399658203125}
\def\PVOUMedianMaxKey{20013}
\def\PVOUMedianMeanFloat{-1.06951230076764591814253435586579144001007080078125}
\def\PVOUMedianMeanKey{29725}
\def\PVOUMedianMedianFloat{-1.5181706568598747342235810720012523233890533447265625}
\def\PVOUMedianMedianKey{13468}
\def\PVOUMedianMinFloat{-1.5894959688186645063723290149937383830547332763671875}
\def\PVOUMedianMinKey{7884}
\def\PVOUMedianStdDevFloat{0.1561197060520655155446689832388074137270450592041015625}
\def\PVOUMinLen{151}
\def\PVOUMinMaxFloat{-0.934693515300750732421875}
\def\PVOUMinMaxKey{17096}
\def\PVOUMinMeanFloat{-1.49651634693145751953125}
\def\PVOUMinMeanKey{20754}
\def\PVOUMinMedianFloat{-2.066871464252471923828125}
\def\PVOUMinMedianKey{15043}
\def\PVOUMinMinFloat{-2.14122104644775390625}
\def\PVOUMinMinKey{9132}
\def\PVOUMinStdDevFloat{0.250365316867828369140625}
\def\PVOUStdDevLen{151}
\def\PVOUStdDevMaxFloat{0.629657268524169921875}
\def\PVOUStdDevMaxKey{7884}
\def\PVOUStdDevMeanFloat{0.40400660037994384765625}
\def\PVOUStdDevMeanKey{104}
\def\PVOUStdDevMedianFloat{0.2789604961872100830078125}
\def\PVOUStdDevMedianKey{17080}
\def\PVOUStdDevMinFloat{0.237532436847686767578125}
\def\PVOUStdDevMinKey{20013}
\def\PVOUStdDevStdDevFloat{0.053538382053375244140625}
\def\ProofFlopEstimateAllSubcubicMean{22570093.600000001490116119384765625}
\def\ProofFlopEstimateAllSubcubicStdDev{1415881.2460418534465134143829345703125}
\def\ProofFlopEstimateAlmostQuadraticMean{20705629.3333333320915699005126953125}
\def\ProofFlopEstimateAlmostQuadraticStdDev{220216.16124119973392225801944732666015625}
\def\ProofFlopEstimateMainlySubcubicMean{23108652.73076923191547393798828125}
\def\ProofFlopEstimateMainlySubcubicStdDev{1275243.43163708201609551906585693359375}
\def\QuartileOnePercentileFloat{0.25}
\def\QuartileThreePercentileFloat{0.75}
\def\RealSubcubicAccuracyLen{15100}
\def\RealSubcubicAccuracyMaxFloat{0.68942794737815604744213260346441529691219329833984375}
\def\RealSubcubicAccuracyMeanFloat{0.235299944994164900169408838337403722107410430908203125}
\def\RealSubcubicAccuracyMedianFloat{0.000000000000000000049127910940749419665962705039419233798980712890625}
\def\RealSubcubicAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\RealSubcubicAccuracyStdDevFloat{0.2211597251955532972278462011672672815620899200439453125}
\def\RealSubcubicDroppedSequencesFracLen{15100}
\def\RealSubcubicDroppedSequencesFracMaxFloat{0.425962157820276188235908421120257116854190826416015625}
\def\RealSubcubicDroppedSequencesFracMeanFloat{0.1632154750729473413617398591668461449444293975830078125}
\def\RealSubcubicDroppedSequencesFracMedianFloat{0}
\def\RealSubcubicDroppedSequencesFracMinFloat{0}
\def\RealSubcubicDroppedSequencesFracStdDevFloat{0.11725158517066762431380055886620539240539073944091796875}
\def\RealSubcubicDroppedSequencesLen{15100}
\def\RealSubcubicDroppedSequencesMaxFloat{502887354265325599101}
\def\RealSubcubicDroppedSequencesMeanFloat{192690822242533310464}
\def\RealSubcubicDroppedSequencesMedianFloat{0}
\def\RealSubcubicDroppedSequencesMinFloat{0}
\def\RealSubcubicDroppedSequencesStdDevFloat{138426238968326275072}
\def\RealSubcubicEffectiveDimensionalityEstimateLen{15100}
\def\RealSubcubicEffectiveDimensionalityEstimateMaxFloat{37122}
\def\RealSubcubicEffectiveDimensionalityEstimateMeanFloat{21064}
\def\RealSubcubicEffectiveDimensionalityEstimateMedianFloat{16770}
\def\RealSubcubicEffectiveDimensionalityEstimateMinFloat{16770}
\def\RealSubcubicEffectiveDimensionalityEstimateStdDevFloat{5194.1589964112572488375008106231689453125}
\def\RealSubcubicErrUpperBoundLen{15100}
\def\RealSubcubicErrUpperBoundMaxFloat{187.469207763671875}
\def\RealSubcubicErrUpperBoundMeanFloat{36.02944345300560513578602694906294345855712890625}
\def\RealSubcubicErrUpperBoundMedianFloat{0}
\def\RealSubcubicErrUpperBoundMinFloat{0}
\def\RealSubcubicErrUpperBoundStdDevFloat{44.3671866260445852958582690916955471038818359375}
\def\RealSubcubicGapMostBelowValueLen{15100}
\def\RealSubcubicGapMostBelowValueMaxFloat{78}
\def\RealSubcubicGapMostBelowValueMeanFloat{17.785761589403971782985536265186965465545654296875}
\def\RealSubcubicGapMostBelowValueMedianFloat{1}
\def\RealSubcubicGapMostBelowValueMinFloat{1}
\def\RealSubcubicGapMostBelowValueNumStdLen{15100}
\def\RealSubcubicGapMostBelowValueNumStdMaxFloat{1.5}
\def\RealSubcubicGapMostBelowValueNumStdMeanFloat{1.5}
\def\RealSubcubicGapMostBelowValueNumStdMedianFloat{1.5}
\def\RealSubcubicGapMostBelowValueNumStdMinFloat{1.5}
\def\RealSubcubicGapMostBelowValueNumStdStdDevFloat{0}
\def\RealSubcubicGapMostBelowValueSequenceFracLen{15100}
\def\RealSubcubicGapMostBelowValueSequenceFracMaxFloat{1}
\def\RealSubcubicGapMostBelowValueSequenceFracMeanFloat{0.99677328000794973572595836230902932584285736083984375}
\def\RealSubcubicGapMostBelowValueSequenceFracMedianFloat{0.98013208150863651013651178800500929355621337890625}
\def\RealSubcubicGapMostBelowValueSequenceFracMinFloat{0.930698871612548828125}
\def\RealSubcubicGapMostBelowValueSequenceFracStdDevFloat{0.00412217591972200390892933086206539883278310298919677734375}
\def\RealSubcubicGapMostBelowValueStdDevFloat{17.88057501398032655970382620580494403839111328125}
\def\RealSubcubicInstructionCountBranchLen{15100}
\def\RealSubcubicInstructionCountBranchMaxFloat{0}
\def\RealSubcubicInstructionCountBranchMeanFloat{0}
\def\RealSubcubicInstructionCountBranchMedianFloat{0}
\def\RealSubcubicInstructionCountBranchMinFloat{0}
\def\RealSubcubicInstructionCountBranchStdDevFloat{0}
\def\RealSubcubicInstructionCountIntLen{15100}
\def\RealSubcubicInstructionCountIntMaxFloat{0}
\def\RealSubcubicInstructionCountIntMeanFloat{0}
\def\RealSubcubicInstructionCountIntMedianFloat{0}
\def\RealSubcubicInstructionCountIntMinFloat{0}
\def\RealSubcubicInstructionCountIntStdDevFloat{0}
\def\RealSubcubicInstructionCountLen{15100}
\def\RealSubcubicInstructionCountMaxFloat{26044438}
\def\RealSubcubicInstructionCountMeanFloat{22570093.600000001490116119384765625}
\def\RealSubcubicInstructionCountMedianFloat{20462164}
\def\RealSubcubicInstructionCountMinFloat{20462164}
\def\RealSubcubicInstructionCountStdDevFloat{1415834.36178064276464283466339111328125}
\def\RealSubcubicMaxGapLen{15100}
\def\RealSubcubicMaxGapMaxFloat{100}
\def\RealSubcubicMaxGapMeanFloat{54.1389403973509928391649737022817134857177734375}
\def\RealSubcubicMaxGapMedianFloat{1}
\def\RealSubcubicMaxGapMinFloat{1}
\def\RealSubcubicMaxGapStdDevFloat{31.9062892169000775766107835806906223297119140625}
\def\RealSubcubicNormalizedAccuracyLen{15100}
\def\RealSubcubicNormalizedAccuracyMaxFloat{0.6908253841360181279895869010942988097667694091796875}
\def\RealSubcubicNormalizedAccuracyMeanFloat{0.2359190620693003281882482724540750496089458465576171875}
\def\RealSubcubicNormalizedAccuracyMedianFloat{0.000000000000000000049250470923809783004091991959694806305698541288337787198182982084659897736855782568454742431640625}
\def\RealSubcubicNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\RealSubcubicNormalizedAccuracyStdDevFloat{0.2217309584008238243502120212724548764526844024658203125}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.68942794737815604744213260346441529691219329833984375}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.62155727626461210189035000439616851508617401123046875}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMeanKey{10248}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.51075811320631547829407281824387609958648681640625}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMedianKey{8893}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMinFloat{0.43620027112436698946140722910058684647083282470703125}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.030909951674108204766611152081168256700038909912109375}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.16661087469430480023646623521926812827587127685546875}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{21598}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1289420651501977932440468066488392651081085205078125}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{5358}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08450994778538080398622156508281477726995944976806640625}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.035672195017851703047195854878737009130418300628662109375}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01374540397603360615541578937381927971728146076202392578125}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{196699402584494945925}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{21598}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{152227921674322051072}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{5358}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{99771736222686543872}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{42114294530673152936}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{16227708757481060352}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{37122}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{31502.1324503311261651106178760528564453125}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{1185}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17010}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{27671}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16962}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{104}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{7154.5454811650715782889164984226226806640625}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{9.74072265625}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{2306}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0.71863545960937902368215191017952747642993927001953125}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6435823340775674861191646414226852357387542724609375}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{104}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.76158940397350960438416223041713237762451171875}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1895}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9997761249542236328125}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99371826411872510309564177077845670282840728759765625}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{22286}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9738725125789642333984375}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8048}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96438848972320556640625}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0044495893543308288886617418711466598324477672576904296875}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.4725236672516339719862799029215238988399505615234375}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMaxFloat{25098133}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMaxKey{27671}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22888486.6158940382301807403564453125}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMeanKey{519}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21929781}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMinFloat{21929781}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{1001967.88267164281569421291351318359375}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMaxFloat{79}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMaxKey{20976}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMeanFloat{70.14569536423840645511518232524394989013671875}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMedianFloat{45.75}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMinFloat{18}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMinKey{8048}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapStdDevFloat{5.2995031017766276448810458532534539699554443359375}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6908253841360181279895869010942988097667694091796875}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.623237723346502292542936629615724086761474609375}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{31308}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5167436093843142952408697965438477694988250732421875}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8893}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.451494450717646544912753370226710103452205657958984375}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0302701451729692101733082409964481485076248645782470703125}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{681.8326740264892578125}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{23696}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{661.228598987819395915721543133258819580078125}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7884}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{633.805510103702545166015625}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{1681}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{629.673713207244873046875}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.6341281903399220709616201929748058319091796875}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.6453669071197509765625}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMaxKey{9504}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.108592317593807052844567806459963321685791015625}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMeanKey{519}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.047219097614288330078125}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8648827075958251953125}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2365804177105277628090362895818543620407581329345703125}
\def\RealSubcubicProofSearchTimeLen{15100}
\def\RealSubcubicProofSearchTimeMaxFloat{1046.6073901653289794921875}
\def\RealSubcubicProofSearchTimeMeanFloat{658.191769480626362565089948475360870361328125}
\def\RealSubcubicProofSearchTimeMedianFloat{629.7350604009628796120523475110530853271484375}
\def\RealSubcubicProofSearchTimeMinFloat{619.2171604633331298828125}
\def\RealSubcubicProofSearchTimeStdDevFloat{13.0151182849710362887662995490245521068572998046875}
\def\RealSubcubicProofTimeLen{15100}
\def\RealSubcubicProofTimeMaxFloat{20.580661296844478869161321199499070644378662109375}
\def\RealSubcubicProofTimeMeanFloat{18.089487481954080294599407352507114410400390625}
\def\RealSubcubicProofTimeMedianFloat{17.073483976125718442062861868180334568023681640625}
\def\RealSubcubicProofTimeMinFloat{16.755332469940185546875}
\def\RealSubcubicProofTimeStdDevFloat{0.252180099482248232245495955794467590749263763427734375}
\def\ResampleEQKEErrLen{100}
\def\ResampleEQKEErrMaxLen{151}
\def\ResampleEQKEErrMaxMaxFloat{1.95557403564453125}
\def\ResampleEQKEErrMaxMaxKey{25516}
\def\ResampleEQKEErrMaxMeanFloat{1.44911513265394997773682916886173188686370849609375}
\def\ResampleEQKEErrMaxMeanKey{22286}
\def\ResampleEQKEErrMaxMedianFloat{1.1711443364620208740234375}
\def\ResampleEQKEErrMaxMedianKey{21598}
\def\ResampleEQKEErrMaxMinFloat{1.1349952220916748046875}
\def\ResampleEQKEErrMaxMinKey{4157}
\def\ResampleEQKEErrMaxStdDevFloat{0.1268460800262559418083441187263815663754940032958984375}
\def\ResampleEQKEErrMeanLen{151}
\def\ResampleEQKEErrMeanMaxFloat{1.1791959780454634998392293709912337362766265869140625}
\def\ResampleEQKEErrMeanMaxKey{7790}
\def\ResampleEQKEErrMeanMeanFloat{1.0396538064100886433749337811605073511600494384765625}
\def\ResampleEQKEErrMeanMeanKey{9504}
\def\ResampleEQKEErrMeanMedianFloat{0.9091054482758045285351045095012523233890533447265625}
\def\ResampleEQKEErrMeanMedianKey{4157}
\def\ResampleEQKEErrMeanMinFloat{0.90620566964149473765388620449812151491641998291015625}
\def\ResampleEQKEErrMeanMinKey{7884}
\def\ResampleEQKEErrMeanStdDevFloat{0.052554151995034846522880656038978486321866512298583984375}
\def\ResampleEQKEErrMedianLen{151}
\def\ResampleEQKEErrMedianMaxFloat{0.965726595818996447206927769002504646778106689453125}
\def\ResampleEQKEErrMedianMaxKey{7790}
\def\ResampleEQKEErrMedianMeanFloat{0.836976078442785098587819447857327759265899658203125}
\def\ResampleEQKEErrMedianMeanKey{15662}
\def\ResampleEQKEErrMedianMedianFloat{0.7399323691427708293844034415087662637233734130859375}
\def\ResampleEQKEErrMedianMedianKey{4157}
\def\ResampleEQKEErrMedianMinFloat{0.7397874945402145296924345529987476766109466552734375}
\def\ResampleEQKEErrMedianMinKey{4647}
\def\ResampleEQKEErrMedianStdDevFloat{0.043734406301632451630201359193961252458393573760986328125}
\def\ResampleEQKEErrMinLen{151}
\def\ResampleEQKEErrMinMaxFloat{0.93295204639434814453125}
\def\ResampleEQKEErrMinMaxKey{26829}
\def\ResampleEQKEErrMinMeanFloat{0.82583139353240564428659808982047252357006072998046875}
\def\ResampleEQKEErrMinMeanKey{30899}
\def\ResampleEQKEErrMinMedianFloat{0.7306676208972930908203125}
\def\ResampleEQKEErrMinMedianKey{4157}
\def\ResampleEQKEErrMinMinFloat{0.728726863861083984375}
\def\ResampleEQKEErrMinMinKey{4647}
\def\ResampleEQKEErrMinStdDevFloat{0.0445956558157425131394546724550309590995311737060546875}
\def\ResampleEQKEErrNumSamples{100}
\def\ResampleEQKEErrSeed{1234}
\def\ResampleEQKEErrStdDevLen{151}
\def\ResampleEQKEErrStdDevMaxFloat{0.152845508150457443097280929578118957579135894775390625}
\def\ResampleEQKEErrStdDevMaxKey{25516}
\def\ResampleEQKEErrStdDevMeanFloat{0.115672034763182107752754745888523757457733154296875}
\def\ResampleEQKEErrStdDevMeanKey{16149}
\def\ResampleEQKEErrStdDevMedianFloat{0.0880247584036102370674825579044409096240997314453125}
\def\ResampleEQKEErrStdDevMedianKey{7884}
\def\ResampleEQKEErrStdDevMinFloat{0.08183227683809758679078782961369142867624759674072265625}
\def\ResampleEQKEErrStdDevMinKey{4157}
\def\ResampleEQKEErrStdDevStdDevFloat{0.01217930332437487141172827165291892015375196933746337890625}
\def\ResampleNormalEQKEErrLen{100}
\def\ResampleNormalEQKEErrMaxLen{151}
\def\ResampleNormalEQKEErrMaxMaxFloat{1.41143977642059326171875}
\def\ResampleNormalEQKEErrMaxMaxKey{19004}
\def\ResampleNormalEQKEErrMaxMeanFloat{1.2521687414472466581827347908983938395977020263671875}
\def\ResampleNormalEQKEErrMaxMeanKey{12561}
\def\ResampleNormalEQKEErrMaxMedianFloat{1.129352033138275146484375}
\def\ResampleNormalEQKEErrMaxMedianKey{26932}
\def\ResampleNormalEQKEErrMaxMinFloat{1.11769068241119384765625}
\def\ResampleNormalEQKEErrMaxMinKey{7884}
\def\ResampleNormalEQKEErrMaxStdDevFloat{0.05844145855778277998116010394369368441402912139892578125}
\def\ResampleNormalEQKEErrMeanLen{151}
\def\ResampleNormalEQKEErrMeanMaxFloat{1.1182270938158034301324050829862244427204132080078125}
\def\ResampleNormalEQKEErrMeanMaxKey{19004}
\def\ResampleNormalEQKEErrMeanMeanFloat{0.9848547485095775488872504865867085754871368408203125}
\def\ResampleNormalEQKEErrMeanMeanKey{11598}
\def\ResampleNormalEQKEErrMeanMedianFloat{0.8885330855846405029296875}
\def\ResampleNormalEQKEErrMeanMedianKey{26932}
\def\ResampleNormalEQKEErrMeanMinFloat{0.880765932202339119072576067992486059665679931640625}
\def\ResampleNormalEQKEErrMeanMinKey{7884}
\def\ResampleNormalEQKEErrMeanStdDevFloat{0.045919274033033898041455955763012752868235111236572265625}
\def\ResampleNormalEQKEErrMedianLen{151}
\def\ResampleNormalEQKEErrMedianMaxFloat{0.88778042823076253053926620850688777863979339599609375}
\def\ResampleNormalEQKEErrMedianMaxKey{19004}
\def\ResampleNormalEQKEErrMedianMeanFloat{0.78164753974668232938682876920211128890514373779296875}
\def\ResampleNormalEQKEErrMedianMeanKey{8299}
\def\ResampleNormalEQKEErrMedianMedianFloat{0.70522695928812029197985111750313080847263336181640625}
\def\ResampleNormalEQKEErrMedianMedianKey{26932}
\def\ResampleNormalEQKEErrMedianMinFloat{0.69871414721012115034426415149937383830547332763671875}
\def\ResampleNormalEQKEErrMedianMinKey{7884}
\def\ResampleNormalEQKEErrMedianStdDevFloat{0.036530730250896308042296567464291001670062541961669921875}
\def\ResampleNormalEQKEErrMinLen{151}
\def\ResampleNormalEQKEErrMinMaxFloat{0.8861429691314697265625}
\def\ResampleNormalEQKEErrMinMaxKey{19004}
\def\ResampleNormalEQKEErrMinMeanFloat{0.7796269892067309026373322922154329717159271240234375}
\def\ResampleNormalEQKEErrMinMeanKey{8299}
\def\ResampleNormalEQKEErrMinMedianFloat{0.70344357192516326904296875}
\def\ResampleNormalEQKEErrMinMedianKey{26932}
\def\ResampleNormalEQKEErrMinMinFloat{0.697505474090576171875}
\def\ResampleNormalEQKEErrMinMinKey{7884}
\def\ResampleNormalEQKEErrMinStdDevFloat{0.036449215035867683909476255621484597213566303253173828125}
\def\ResampleNormalEQKEErrStdDevLen{151}
\def\ResampleNormalEQKEErrStdDevMaxFloat{0.12543349968504668989766059894463978707790374755859375}
\def\ResampleNormalEQKEErrStdDevMaxKey{19004}
\def\ResampleNormalEQKEErrStdDevMeanFloat{0.109788277194604211306483421140001155436038970947265625}
\def\ResampleNormalEQKEErrStdDevMeanKey{8745}
\def\ResampleNormalEQKEErrStdDevMedianFloat{0.09900013523550448002463753027768689207732677459716796875}
\def\ResampleNormalEQKEErrStdDevMedianKey{26932}
\def\ResampleNormalEQKEErrStdDevMinFloat{0.09841502315642902676273706674692220985889434814453125}
\def\ResampleNormalEQKEErrStdDevMinKey{7884}
\def\ResampleNormalEQKEErrStdDevStdDevFloat{0.00519624620817798511807072969759246916510164737701416015625}
\def\SubcubicAccuracyLen{7852}
\def\SubcubicAccuracyMaxFloat{0.68942794737815604744213260346441529691219329833984375}
\def\SubcubicAccuracyMeanFloat{0.336668652541607549277813404842163436114788055419921875}
\def\SubcubicAccuracyMedianFloat{0.00000000000000000005082197683525802034409935004077851772308349609375}
\def\SubcubicAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicAccuracyStdDevFloat{0.1959502713810888085976813499655690975487232208251953125}
\def\SubcubicAttentionQuadraticAccuracyLen{1812}
\def\SubcubicAttentionQuadraticAccuracyMaxFloat{0.435405177351559424803184583652182482182979583740234375}
\def\SubcubicAttentionQuadraticAccuracyMeanFloat{0.265184867725060058329944467914174310863018035888671875}
\def\SubcubicAttentionQuadraticAccuracyMedianFloat{0.07974025984969557168113851730595342814922332763671875}
\def\SubcubicAttentionQuadraticAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicAttentionQuadraticAccuracyStdDevFloat{0.0807277309626490968685885718514327891170978546142578125}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyMaxFloat{0.451928798694893607557077075398410670459270477294921875}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyMeanFloat{0.09537265827728653999617591807691496796905994415283203125}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyMedianFloat{0.0000000000000000000482808779934951193268943825387395918369293212890625}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyStdDevFloat{0.14340227370849423227383567791548557579517364501953125}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracMaxFloat{0.364304421671816702765767104210681281983852386474609375}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracMeanFloat{0.1982036894965367446186377264893963001668453216552734375}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracStdDevFloat{0.1433547128132553194479470448641222901642322540283203125}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesMaxFloat{430094747616049389880}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesMeanFloat{233997615014886670336}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesStdDevFloat{169243372737680539648}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateMeanFloat{21100.66666666666787932626903057098388671875}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateMedianFloat{20930}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateMinFloat{20930}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateStdDevFloat{85.333333333333342807236476801335811614990234375}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundMaxFloat{187.469207763671875}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundMeanFloat{102.81546069349411709481501020491123199462890625}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundMedianFloat{83.86852264404296875}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundMinFloat{81.919342041015625}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundStdDevFloat{9.6921242410523884558415375067852437496185302734375}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueMaxFloat{76}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueMeanFloat{30.7534952170713751229413901455700397491455078125}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueMedianFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueMinFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracMeanFloat{0.999662958869520057447743965894915163516998291015625}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracMedianFloat{0.99736704736948011973396432949812151491641998291015625}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracMinFloat{0.9940254688262939453125}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.000551504564547116598628717643038044116110540926456451416015625}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueStdDevFloat{22.0715176586696770755224861204624176025390625}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountMaxFloat{20948465}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountMeanFloat{20705629.3333333320915699005126953125}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountMedianFloat{20462164}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountMinFloat{20462164}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountStdDevFloat{220175.6468150927103124558925628662109375}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapMaxFloat{98}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapMeanFloat{52.11662987490802123602406936697661876678466796875}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapMedianFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapMinFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapStdDevFloat{38.340099356474439673547749407589435577392578125}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyMaxFloat{0.45284483628465832527609791213762946426868438720703125}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyMeanFloat{0.09562998254307138179530767274627578444778919219970703125}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyMedianFloat{0.000000000000000000048395942402973877046403457273086360814637485857644968556372233603468657747725956141948699951171875}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyStdDevFloat{0.1437880917737918984311562553557450883090496063232421875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.451928798694893607557077075398410670459270477294921875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.383662939919712175917965168991941027343273162841796875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{32382}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.31131020585100532827027564053423702716827392578125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{15043}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.299347341418428614101543416836648248136043548583984375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{8893}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0252514343739989842452242641002158052287995815277099609375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.361191106294214303584766412313911132514476776123046875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24173}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.3217549413456755047491242294199764728546142578125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{22545}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.22805696152062904236146323455614037811756134033203125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1316400142569892073307613600263721309602260589599609375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0233944905114797409295679386787014664150774478912353515625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{426419193568601303974}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24173}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{379861187677126787072}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{22545}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{269242137817527746560}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{155413097782922049324}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{27619339468805967872}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21122.42384105960445594973862171173095703125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{104}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{104}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{63.99859653739444098619060241617262363433837890625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{179.824432373046875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.2996650847378106163887423463165760040283203125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.85131072998046875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{82.67822265625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.5066345135820657930025845416821539402008056640625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{75}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{12561}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{50.17218543046357837056348216719925403594970703125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{22.75}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{13}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99999940395355224609375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12141}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.999015660475421451991451249341480433940887451171875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{24173}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99676690995693217889339621251565404236316680908203125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20013}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99628353118896484375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{6549}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00065818497769662052086780956727807279094122350215911865234375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{8.4585170755832503886040285578928887844085693359375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20948465}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{5781}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20917470.1324503310024738311767578125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20905172}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{104}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{20905172}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{104}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{13645.16560373371976311318576335906982421875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{96}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{8721}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{84.4238410596026511711897910572588443756103515625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{77}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{11598}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{77}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{11598}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.71044183672842020627058445825241506099700927734375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.45284483628465832527609791213762946426868438720703125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.384717017723093357428609806447639130055904388427734375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{32382}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.3126635989519497282884685773751698434352874755859375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15043}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.300958397943729194512485491941333748400211334228515625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8893}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.02515111962896716957249765300730359740555286407470703125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{682.4775712490081787109375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{23696}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{660.9983980308305717699113301932811737060546875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29195}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{637.450467586517333984375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{519}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{637.3421027660369873046875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{13293}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.6690240432014800120441577746532857418060302734375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7661190032958984375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{11611}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.125046921092152985011125565506517887115478515625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{16284}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{16.882906973361968994140625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{16.85701274871826171875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.26885273590923841613431477526319213211536407470703125}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeMaxFloat{1046.6073901653289794921875}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeMeanFloat{658.210672109595407164306379854679107666015625}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeMedianFloat{631.3133363056182361106039024889469146728515625}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeMinFloat{624.76801586151123046875}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeStdDevFloat{14.6822847114774059917863269220106303691864013671875}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeMaxFloat{19.9767801761627197265625}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeMeanFloat{18.073890649281150189153777319006621837615966796875}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeMedianFloat{16.93083802700042639344246708787977695465087890625}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeMinFloat{16.7781083583831787109375}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeStdDevFloat{0.243980881048622533224801145479432307183742523193359375}
\def\SubcubicAttentionQuadraticDroppedSequencesFracLen{1812}
\def\SubcubicAttentionQuadraticDroppedSequencesFracMaxFloat{0.425962157820276188235908421120257116854190826416015625}
\def\SubcubicAttentionQuadraticDroppedSequencesFracMeanFloat{0.369068819034200024109537707772688008844852447509765625}
\def\SubcubicAttentionQuadraticDroppedSequencesFracMedianFloat{0.271288647927526438419221221920452080667018890380859375}
\def\SubcubicAttentionQuadraticDroppedSequencesFracMinFloat{0.01188737860194520080947544471428045653738081455230712890625}
\def\SubcubicAttentionQuadraticDroppedSequencesFracStdDevFloat{0.0271624042148115411865472168528867769055068492889404296875}
\def\SubcubicAttentionQuadraticDroppedSequencesLen{1812}
\def\SubcubicAttentionQuadraticDroppedSequencesMaxFloat{502887354265325599101}
\def\SubcubicAttentionQuadraticDroppedSequencesMeanFloat{435719555219846987776}
\def\SubcubicAttentionQuadraticDroppedSequencesMedianFloat{320281104538993623040}
\def\SubcubicAttentionQuadraticDroppedSequencesMinFloat{14034139569751991424}
\def\SubcubicAttentionQuadraticDroppedSequencesStdDevFloat{32067706814545817600}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateLen{1812}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateMaxFloat{17216}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateMeanFloat{17046.33333333333212067373096942901611328125}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateMedianFloat{16834}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateMinFloat{16834}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateStdDevFloat{140.605436910842428233081591315567493438720703125}
\def\SubcubicAttentionQuadraticErrUpperBoundLen{1812}
\def\SubcubicAttentionQuadraticErrUpperBoundMaxFloat{187.469207763671875}
\def\SubcubicAttentionQuadraticErrUpperBoundMeanFloat{102.81546069349411709481501020491123199462890625}
\def\SubcubicAttentionQuadraticErrUpperBoundMedianFloat{83.86852264404296875}
\def\SubcubicAttentionQuadraticErrUpperBoundMinFloat{81.919342041015625}
\def\SubcubicAttentionQuadraticErrUpperBoundStdDevFloat{9.6921242410523884558415375067852437496185302734375}
\def\SubcubicAttentionQuadraticGapMostBelowValueLen{1812}
\def\SubcubicAttentionQuadraticGapMostBelowValueMaxFloat{78}
\def\SubcubicAttentionQuadraticGapMostBelowValueMeanFloat{49.18874172185430637682657106779515743255615234375}
\def\SubcubicAttentionQuadraticGapMostBelowValueMedianFloat{28}
\def\SubcubicAttentionQuadraticGapMostBelowValueMinFloat{3}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdLen{1812}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracLen{1812}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracMeanFloat{0.99865791504219936225439369081868790090084075927734375}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracMedianFloat{0.99566833734512327769294870449812151491641998291015625}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracMinFloat{0.97134721279144276007144753748434595763683319091796875}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.001301148576327105198247036099701290368102490901947021484375}
\def\SubcubicAttentionQuadraticGapMostBelowValueStdDevFloat{8.4098731242751210146479934337548911571502685546875}
\def\SubcubicAttentionQuadraticInstructionCountBranchLen{1812}
\def\SubcubicAttentionQuadraticInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntLen{1812}
\def\SubcubicAttentionQuadraticInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntMinFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountLen{1812}
\def\SubcubicAttentionQuadraticInstructionCountMaxFloat{22042384}
\def\SubcubicAttentionQuadraticInstructionCountMeanFloat{21784466.1666666679084300994873046875}
\def\SubcubicAttentionQuadraticInstructionCountMedianFloat{21527284}
\def\SubcubicAttentionQuadraticInstructionCountMinFloat{21527284}
\def\SubcubicAttentionQuadraticInstructionCountStdDevFloat{220780.67722622878500260412693023681640625}
\def\SubcubicAttentionQuadraticMaxGapLen{1812}
\def\SubcubicAttentionQuadraticMaxGapMaxFloat{100}
\def\SubcubicAttentionQuadraticMaxGapMeanFloat{83.0612582781457007286007865332067012786865234375}
\def\SubcubicAttentionQuadraticMaxGapMedianFloat{75.05500000000000682121026329696178436279296875}
\def\SubcubicAttentionQuadraticMaxGapMinFloat{7}
\def\SubcubicAttentionQuadraticMaxGapStdDevFloat{5.17733003773237054900846487726084887981414794921875}
\def\SubcubicAttentionQuadraticNormalizedAccuracyLen{1812}
\def\SubcubicAttentionQuadraticNormalizedAccuracyMaxFloat{0.43638657279267578648074277225532568991184234619140625}
\def\SubcubicAttentionQuadraticNormalizedAccuracyMeanFloat{0.265887856212345285999987254399457015097141265869140625}
\def\SubcubicAttentionQuadraticNormalizedAccuracyMedianFloat{0.08000380987397122389825909749561105854809284210205078125}
\def\SubcubicAttentionQuadraticNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicAttentionQuadraticNormalizedAccuracyStdDevFloat{0.08094901888518378496595317983519635163247585296630859375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.435405177351559424803184583652182482182979583740234375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{26932}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.349579643461583822183769143521203659474849700927734375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{15622}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.27188607686553478703928021786850877106189727783203125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{8893}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.266777089725750704563012050130055285990238189697265625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{15043}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.029303248187992958495584616684936918318271636962890625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.4228219674668822758434316710918210446834564208984375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24173}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.366887884840814082476612156824558041989803314208984375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{2236}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.308050448339645732698244273706222884356975555419921875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.274353133795015080576007449053577147424221038818359375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0198657610698998177145568888590787537395954132080078125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{499180071846651093540}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24173}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{433144762585799589888}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{2236}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{363681778068027539456}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{323899010875957643163}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{23453351058297872384}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17216}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17117.19205298013184801675379276275634765625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{742}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16834}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{1185}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16834}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{1185}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{116.42925346609712278223014436662197113037109375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{187.469207763671875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.4435140344480856811060220934450626373291015625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{20294}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{87.1704120635986328125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{83.86852264404296875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.831408385968639862539930618368089199066162109375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{70}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{21317}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{47.75496688741721840187892667017877101898193359375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{2743}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{31.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{30}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99997800588607799188167746251565404236316680908203125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{6204}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99862506729088085233314586730557493865489959716796875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{18668}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99610291421413421630859375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{14095}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.995666921138763427734375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{24144}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00074333977326390926303190109791785289417020976543426513671875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{7.79366943596206507294255061424337327480316162109375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22042384}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{1951}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21988306.463576160371303558349609375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{104}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21966196}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{742}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{21966196}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{742}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{20380.9432590709111536853015422821044921875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{98}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{82.6092715231788048413363867439329624176025390625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{76.75}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{7467}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{76}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{2743}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.98777533560950470103989573544822633266448974609375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.43638657279267578648074277225532568991184234619140625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26932}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.35054806189050446985078224315657280385494232177734375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{15622}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.27325851067242423741987522589624859392642974853515625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8893}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.267849540418154952181595263027702458202838897705078125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15043}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0293538357705619527837637150469163316302001476287841796875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{686.50016880035400390625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{19093}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{662.6373894561994575269636698067188262939453125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22545}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.0834367275238037109375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{624.885946750640869140625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{16197}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{12.173649816031314685460529290139675140380859375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.797145128250118517598821199499070644378662109375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.12974110502280922219142667017877101898193359375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{5358}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.116713464260101318359375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{1951}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{17.06854724884033203125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.24574152507875368645073876905371434986591339111328125}
\def\SubcubicAttentionQuadraticProofSearchTimeLen{1812}
\def\SubcubicAttentionQuadraticProofSearchTimeMaxFloat{696.9877679347991943359375}
\def\SubcubicAttentionQuadraticProofSearchTimeMeanFloat{659.27159523582349720527417957782745361328125}
\def\SubcubicAttentionQuadraticProofSearchTimeMedianFloat{627.2015078210830552052357234060764312744140625}
\def\SubcubicAttentionQuadraticProofSearchTimeMinFloat{620.335491657257080078125}
\def\SubcubicAttentionQuadraticProofSearchTimeStdDevFloat{11.534468856226038013801371562294661998748779296875}
\def\SubcubicAttentionQuadraticProofTimeLen{1812}
\def\SubcubicAttentionQuadraticProofTimeMaxFloat{20.3301813602447509765625}
\def\SubcubicAttentionQuadraticProofTimeMeanFloat{18.112827170500427342858529300428926944732666015625}
\def\SubcubicAttentionQuadraticProofTimeMedianFloat{17.15965195655822839171378291212022304534912109375}
\def\SubcubicAttentionQuadraticProofTimeMinFloat{17.0136129856109619140625}
\def\SubcubicAttentionQuadraticProofTimeStdDevFloat{0.25837178901233148753391333229956217110157012939453125}
\def\SubcubicAttentionVocabModelSquaredAccuracyLen{3020}
\def\SubcubicAttentionVocabModelSquaredAccuracyMaxFloat{0.66766676502150790195599938670056872069835662841796875}
\def\SubcubicAttentionVocabModelSquaredAccuracyMeanFloat{0.438959947920017634626077551729395054280757904052734375}
\def\SubcubicAttentionVocabModelSquaredAccuracyMedianFloat{0.09875850242360743880265516736471909098327159881591796875}
\def\SubcubicAttentionVocabModelSquaredAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicAttentionVocabModelSquaredAccuracyStdDevFloat{0.1310519360582141634719022249555564485490322113037109375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyMaxFloat{0.6796071498866778082259543225518427789211273193359375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyMeanFloat{0.1435505572753912606476234259389457292854785919189453125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyMedianFloat{0.0000000000000000000482808779934951193268943825387395918369293212890625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyStdDevFloat{0.2148708161267245675407622229613480158150196075439453125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracMaxFloat{0.287210202143366177818251117059844546020030975341796875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracMeanFloat{0.09799990621079497643552969066149671562016010284423828125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracStdDevFloat{0.07551148007521389649010501443626708351075649261474609375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesMaxFloat{339077958035012023165}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesMeanFloat{115697868103557021696}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesStdDevFloat{89148220644767121408}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateMeanFloat{21053.73333333333357586525380611419677734375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateMedianFloat{20866}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateMinFloat{20866}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateStdDevFloat{97.66846414728189529341761954128742218017578125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundMaxFloat{32.51659393310546875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundMeanFloat{9.8789973498969683163295485428534448146820068359375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundMedianFloat{4.2336444854736328125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundStdDevFloat{5.94281420694294837403504061512649059295654296875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueMaxFloat{35}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueMeanFloat{8.4479028697571738604210622725076973438262939453125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueMedianFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueMinFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracMeanFloat{0.99681271205411581259880904326564632356166839599609375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracMedianFloat{0.98255943834781633849928539348184131085872650146484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracMinFloat{0.972655713558197021484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.003761865165272049171818480317597277462482452392578125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueStdDevFloat{6.5474698123937997706889291293919086456298828125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountMaxFloat{24950519}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountMeanFloat{22755269.6666666679084300994873046875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountMedianFloat{21528980}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountMinFloat{21528980}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountStdDevFloat{1100740.811203174293041229248046875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapMaxFloat{89}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapMeanFloat{37.611479028697573312456370331346988677978515625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapMedianFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapMinFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapStdDevFloat{32.0125810088094340244424529373645782470703125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyMaxFloat{0.6809846803679546756171703236759640276432037353515625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyMeanFloat{0.143930430846074208783846870574052445590496063232421875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyMedianFloat{0.000000000000000000048395942402973877046403457273086360814637485857644968556372233603468657747725956141948699951171875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyStdDevFloat{0.2154289274349310556733172461463254876434803009033203125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6796071498866778082259543225518427789211273193359375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.59455275346375746625682268131640739738941192626953125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{28778}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.484250002205975083047206908304360695183277130126953125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{8893}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.429902799932262824622597463530837558209896087646484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0302314729461720388403733750237734057009220123291015625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.17099584457808558735081305712810717523097991943359375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1408756907135202129932594061756390146911144256591796875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{6204}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0904955427191748984494523710964131169021129608154296875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6910}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0398087857448077009347997545773978345096111297607421875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.012794253492768005442403733695755363442003726959228515625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{201876261286384720189}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{166316660019159760896}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{6204}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{106838279446532456448}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6910}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{46997918881254736532}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{15104788466896386048}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{104}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21116.49006622516390052624046802520751953125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{63.76237628725061057366474415175616741180419921875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{10.785564422607421875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.6170718148844134276487238821573555469512939453125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22261}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.17872369289398193359375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.3341311894246901115224090972333215177059173583984375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{15}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10.5165562913907280062630889005959033966064453125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6.25}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999437987804412841796875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99485807071458420836052027880214154720306396484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19917}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97918491065502155645816628748434595763683319091796875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8048}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97576397657394398077457253748434595763683319091796875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.003335920797967724914234732835893737501464784145355224609375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.5218249093697668872238182302680797874927520751953125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22976341}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{1696}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22103573.1192052997648715972900390625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{104}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21971988}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{21971988}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{309661.810038024443201720714569091796875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{84}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{71.1324503311258240501047112047672271728515625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{32.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{32103}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{22}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{24566}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{6.4177686872486834346318573807366192340850830078125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6809846803679546756171703236759640276432037353515625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.59615438711854584763472075792378745973110198974609375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{28778}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.490046106611645548856159848583047278225421905517578125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8893}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.444976175776046145582398594342521391808986663818359375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0294902716131977583879919535547742270864546298980712890625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{686.929138660430908203125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{13468}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{661.0921927145774361633812077343463897705078125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5928}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{639.058513820171356201171875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{23241}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{637.7066695690155029296875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{519}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.293473198988952077570502297021448612213134765625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.69706630706787109375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{30899}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.116891039917799588465641136281192302703857421875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{7238}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{16.95589458942413330078125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8429481983184814453125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.27346456453601419855914400613983161747455596923828125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeMaxFloat{958.2426109313963706881622783839702606201171875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeMeanFloat{657.81840790118076256476342678070068359375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeMedianFloat{630.6859942018985520917340181767940521240234375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeMinFloat{621.452413082122802734375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeStdDevFloat{13.926395273736460467262077145278453826904296875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeMaxFloat{20.391441822051998400411321199499070644378662109375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeMeanFloat{18.0774516937748472855673753656446933746337890625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeMedianFloat{16.975498992204666848238048260100185871124267578125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeMinFloat{16.755332469940185546875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeStdDevFloat{0.25703631624856948523216715329908765852451324462890625}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracLen{3020}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracMaxFloat{0.311808437349295919371883201165474019944667816162109375}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracMeanFloat{0.16683316119721969261746608026442117989063262939453125}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracMedianFloat{0.09020502805537121415735413165748468600213527679443359375}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracMinFloat{0.00110505560391070006311109441554663135320879518985748291015625}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracStdDevFloat{0.0422556519896295779137318504581344313919544219970703125}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesLen{3020}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesMaxFloat{368118428403568686965}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesMeanFloat{196961832167234502656}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesMedianFloat{106495300268750340096}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesMinFloat{1304619386403811018}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesStdDevFloat{49886668666907664384}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateLen{3020}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateMaxFloat{17216}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateMeanFloat{16999.4000000000014551915228366851806640625}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateMedianFloat{16770}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateMinFloat{16770}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateStdDevFloat{148.41576735643690199140110053122043609619140625}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundLen{3020}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundMaxFloat{32.51659393310546875}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundMeanFloat{9.8789973498969683163295485428534448146820068359375}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundMedianFloat{4.23380393981933611513568394002504646778106689453125}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundStdDevFloat{5.94281420694294837403504061512649059295654296875}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueLen{3020}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueMaxFloat{34}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueMeanFloat{11.72516556291390799060536664910614490509033203125}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueMedianFloat{6}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueMinFloat{2}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdLen{3020}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracLen{3020}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracMeanFloat{0.99548601081829202197326367240748368203639984130859375}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracMedianFloat{0.9794743469357489740190203519887290894985198974609375}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracMinFloat{0.930698871612548828125}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracStdDevFloat{0.00428786256066768060868366063687062705866992473602294921875}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueStdDevFloat{4.68575011195238300132359654526226222515106201171875}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchLen{3020}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntLen{3020}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountLen{3020}
\def\SubcubicAttentionVocabModelSquaredInstructionCountMaxFloat{26044438}
\def\SubcubicAttentionVocabModelSquaredInstructionCountMeanFloat{23834106.5}
\def\SubcubicAttentionVocabModelSquaredInstructionCountMedianFloat{22594100}
\def\SubcubicAttentionVocabModelSquaredInstructionCountMinFloat{22594100}
\def\SubcubicAttentionVocabModelSquaredInstructionCountStdDevFloat{1100861.9920018357224762439727783203125}
\def\SubcubicAttentionVocabModelSquaredMaxGapLen{3020}
\def\SubcubicAttentionVocabModelSquaredMaxGapMaxFloat{84}
\def\SubcubicAttentionVocabModelSquaredMaxGapMeanFloat{69.7847682119205359185798442922532558441162109375}
\def\SubcubicAttentionVocabModelSquaredMaxGapMedianFloat{13}
\def\SubcubicAttentionVocabModelSquaredMaxGapMinFloat{2}
\def\SubcubicAttentionVocabModelSquaredMaxGapStdDevFloat{11.374482003164541055184599827043712139129638671875}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyLen{3020}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyMaxFloat{0.67257837986194790591554237835225649178028106689453125}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyMeanFloat{0.440105980437106858449425317303393967449665069580078125}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyMedianFloat{0.09890108632898846063863373956337454728782176971435546875}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyStdDevFloat{0.1313661260063075097992424389303778298199176788330078125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.66766676502150790195599938670056872069835662841796875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMaxKey{8048}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5938845847968290403429136858903802931308746337890625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMeanKey{24262}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.471718997847543786150481537333689630031585693359375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMedianKey{15043}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMinFloat{0.42956721272854958559861415778868831694126129150390625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.035288096422365057558412360094735049642622470855712890625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.169564419042871505904912510231952182948589324951171875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24438}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.141244248498969271476966014233767054975032806396484375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{16197}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1112533276490832723215618216272559948265552520751953125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.11007086010888060545465094719475018791854381561279296875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{742}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01140887368999919139478382845709347748197615146636962890625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{200186332293830011405}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24438}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{166751776252410953728}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{16197}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{131344746399436439552}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{129948735129702830230}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinKey{742}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{13469220680236376064}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17216}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{123}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17110.7284768211902701295912265777587890625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16834}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{1185}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16834}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{1185}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{107.00386412375502231952850706875324249267578125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{21.775320053100582384786321199499070644378662109375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{6.37678693303998755936845554970204830169677734375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{4800}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.18783485889434814453125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{24202}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0430088043212890625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.259982482344167209475926938466727733612060546875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.350993377483444390918521094135940074920654296875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{7}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{7}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1696}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999718189239501953125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9955183757061989435754867372452281415462493896484375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{2773}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.983900368213653564453125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{27671}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98008680343627918585269753748434595763683319091796875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{3175}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0033139289364750991288832704384503813344053924083709716796875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.433740421409200660463056919979862868785858154296875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMaxFloat{26011543}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMaxKey{20013}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMeanFloat{23348902.4900662265717983245849609375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMeanKey{104}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMedianFloat{23033012}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMinFloat{23033012}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{490604.409552066703327000141143798828125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMaxFloat{76}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMaxKey{11124}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMeanFloat{70.88079470198675835490575991570949554443359375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMedianFloat{66}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMedianKey{12552}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMinFloat{66}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMinKey{12552}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.278395951139881692171229587984271347522735595703125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.67257837986194790591554237835225649178028106689453125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8048}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.59549863600120522821868007667944766581058502197265625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24262}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.47694900479240853741202954552136361598968505859375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15043}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.444628822117099919974947397349751554429531097412109375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.034918736906791529583937716552100027911365032196044921875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{686.9306805133819580078125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{15622}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{663.3678374322045101507683284580707550048828125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7238}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{635.054930627346038818359375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13716}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{633.0231206417083740234375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.92488859322330796430833288468420505523681640625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.380094528198238634786321199499070644378662109375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.159057222454752178464332246221601963043212890625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMeanKey{28778}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.604564249515533447265625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMinFloat{17.1956870555877685546875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.290119888194244890389228430649382062256336212158203125}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeLen{3020}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeMaxFloat{701.895977020263671875}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeMeanFloat{658.8556017900144752275082282721996307373046875}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeMedianFloat{628.5478151702881177698145620524883270263671875}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeMinFloat{619.2171604633331298828125}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeStdDevFloat{11.625435564708606506201249430887401103973388671875}
\def\SubcubicAttentionVocabModelSquaredProofTimeLen{3020}
\def\SubcubicAttentionVocabModelSquaredProofTimeMaxFloat{20.580661296844478869161321199499070644378662109375}
\def\SubcubicAttentionVocabModelSquaredProofTimeMeanFloat{18.1143024884312353606219403445720672607421875}
\def\SubcubicAttentionVocabModelSquaredProofTimeMedianFloat{17.225174950361253678465800476260483264923095703125}
\def\SubcubicAttentionVocabModelSquaredProofTimeMinFloat{16.827945232391357421875}
\def\SubcubicAttentionVocabModelSquaredProofTimeStdDevFloat{0.24994469817930642374648186887498013675212860107421875}
\def\SubcubicDirectQuadraticAccuracyLen{1812}
\def\SubcubicDirectQuadraticAccuracyMaxFloat{0.68942794737815604744213260346441529691219329833984375}
\def\SubcubicDirectQuadraticAccuracyMeanFloat{0.151253741475367797786333312615170143544673919677734375}
\def\SubcubicDirectQuadraticAccuracyMedianFloat{0.000000000000000000048327464805594105604801897227872490512844905004032522682737293973076475595007650554180145263671875}
\def\SubcubicDirectQuadraticAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicDirectQuadraticAccuracyStdDevFloat{0.225239357765291303703492076238035224378108978271484375}
\def\SubcubicDirectQuadraticDroppedSequencesFracLen{1812}
\def\SubcubicDirectQuadraticDroppedSequencesFracMaxFloat{0.1632589985555787104321012748187058605253696441650390625}
\def\SubcubicDirectQuadraticDroppedSequencesFracMeanFloat{0.08135557961305243945826504159413161687552928924560546875}
\def\SubcubicDirectQuadraticDroppedSequencesFracMedianFloat{0}
\def\SubcubicDirectQuadraticDroppedSequencesFracMinFloat{0}
\def\SubcubicDirectQuadraticDroppedSequencesFracStdDevFloat{0.05904410235463374012621073916307068429887294769287109375}
\def\SubcubicDirectQuadraticDroppedSequencesLen{1812}
\def\SubcubicDirectQuadraticDroppedSequencesMaxFloat{192742205701432245703}
\def\SubcubicDirectQuadraticDroppedSequencesMeanFloat{96047715589778096128}
\def\SubcubicDirectQuadraticDroppedSequencesMedianFloat{0}
\def\SubcubicDirectQuadraticDroppedSequencesMinFloat{0}
\def\SubcubicDirectQuadraticDroppedSequencesStdDevFloat{69706972492661989376}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateLen{1812}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateMaxFloat{37122}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateMeanFloat{29143.33333333333212067373096942901611328125}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateMedianFloat{21122}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateMinFloat{21122}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateStdDevFloat{7936.229387365821821731515228748321533203125}
\def\SubcubicDirectQuadraticErrUpperBoundLen{1812}
\def\SubcubicDirectQuadraticErrUpperBoundMaxFloat{4.456815242767333984375}
\def\SubcubicDirectQuadraticErrUpperBoundMeanFloat{1.2265328500444525605672652091016061604022979736328125}
\def\SubcubicDirectQuadraticErrUpperBoundMedianFloat{0}
\def\SubcubicDirectQuadraticErrUpperBoundMinFloat{0}
\def\SubcubicDirectQuadraticErrUpperBoundStdDevFloat{1.2737433661555055408598491339944303035736083984375}
\def\SubcubicDirectQuadraticGapMostBelowValueLen{1812}
\def\SubcubicDirectQuadraticGapMostBelowValueMaxFloat{15}
\def\SubcubicDirectQuadraticGapMostBelowValueMeanFloat{6.41225165562913890227036972646601498126983642578125}
\def\SubcubicDirectQuadraticGapMostBelowValueMedianFloat{1}
\def\SubcubicDirectQuadraticGapMostBelowValueMinFloat{1}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdLen{1812}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracLen{1812}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracMeanFloat{0.9948494445211839565246236816165037453174591064453125}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracMedianFloat{0.97817940175533291125020696199499070644378662109375}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracMinFloat{0.9467487335205078125}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.005158068911486944109479058084843927645124495029449462890625}
\def\SubcubicDirectQuadraticGapMostBelowValueStdDevFloat{3.986943925065193905510341210174374282360076904296875}
\def\SubcubicDirectQuadraticInstructionCountBranchLen{1812}
\def\SubcubicDirectQuadraticInstructionCountBranchMaxFloat{0}
\def\SubcubicDirectQuadraticInstructionCountBranchMeanFloat{0}
\def\SubcubicDirectQuadraticInstructionCountBranchMedianFloat{0}
\def\SubcubicDirectQuadraticInstructionCountBranchMinFloat{0}
\def\SubcubicDirectQuadraticInstructionCountBranchStdDevFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntLen{1812}
\def\SubcubicDirectQuadraticInstructionCountIntMaxFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntMeanFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntMedianFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntMinFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntStdDevFloat{0}
\def\SubcubicDirectQuadraticInstructionCountLen{1812}
\def\SubcubicDirectQuadraticInstructionCountMaxFloat{24004214}
\def\SubcubicDirectQuadraticInstructionCountMeanFloat{22746176.1666666679084300994873046875}
\def\SubcubicDirectQuadraticInstructionCountMedianFloat{21486773}
\def\SubcubicDirectQuadraticInstructionCountMinFloat{21486773}
\def\SubcubicDirectQuadraticInstructionCountStdDevFloat{1060180.51862806477583944797515869140625}
\def\SubcubicDirectQuadraticMaxGapLen{1812}
\def\SubcubicDirectQuadraticMaxGapMaxFloat{83}
\def\SubcubicDirectQuadraticMaxGapMeanFloat{34.849337748344368037578533403575420379638671875}
\def\SubcubicDirectQuadraticMaxGapMedianFloat{1}
\def\SubcubicDirectQuadraticMaxGapMinFloat{1}
\def\SubcubicDirectQuadraticMaxGapStdDevFloat{30.559931611363662540270524914376437664031982421875}
\def\SubcubicDirectQuadraticNormalizedAccuracyLen{1812}
\def\SubcubicDirectQuadraticNormalizedAccuracyMaxFloat{0.6908253841360181279895869010942988097667694091796875}
\def\SubcubicDirectQuadraticNormalizedAccuracyMeanFloat{0.1516531719863946914284014155782642774283885955810546875}
\def\SubcubicDirectQuadraticNormalizedAccuracyMedianFloat{0.000000000000000000048442941471619852776855988112366631436635504493017754146406972370897392465849407017230987548828125}
\def\SubcubicDirectQuadraticNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicDirectQuadraticNormalizedAccuracyStdDevFloat{0.225823025960354362151605300823575817048549652099609375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.68942794737815604744213260346441529691219329833984375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.60688500124927269308017230287077836692333221435546875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{11498}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.493586528321392881135665220426744781434535980224609375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.43620027112436698946140722910058684647083282470703125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.030813498185284622643553831267126952297985553741455078125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1590030484385898945642878743456094525754451751708984375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.12997421362961514290645936853252351284027099609375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{20338}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08090877889909052489425533849498606286942958831787109375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6910}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.035672195017851703047195854878737009130418300628662109375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0122431259011626901445080051189506775699555873870849609375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{187717666655123905064}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{153446467520458457088}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{20338}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{95520226410744004608}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6910}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{42114294530673152936}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{14454131850300973056}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{37122}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{35650.423841059600817970931529998779296875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21250}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{1696}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21250}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{1696}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{4603.403132807316069374792277812957763671875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{3.013769626617431640625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4430}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0.219405715039234283647573420239496044814586639404296875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.69605078847275769771130171648110263049602508544921875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.4503311258278142048538938979618251323699951171875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9991238117218017578125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{8893}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9931498639630955693746727774851024150848388671875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{23447}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97377805411815643310546875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12141}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96438848972320556640625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004359459248868200777204950924215154373086988925933837890625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.454332380101825084040001456742174923419952392578125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{24004214}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{1696}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22122112.536423839628696441650390625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21929781}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{21929781}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{601653.942225231789052486419677734375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{83}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{29726}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{71.0794701986754944300628267228603363037109375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{55.75}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{27714}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{55}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.3680404305310940316076084855012595653533935546875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6908253841360181279895869010942988097667694091796875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6085190164105096499724822933785617351531982421875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29052}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.498681007045377377995265533172641880810260772705078125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.451494450717646544912753370226710103452205657958984375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0300462466768390036586655611472451710142195224761962890625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{682.8454401493072509765625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7790}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{657.3037853635700002996600233018398284912109375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5781}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{634.61968994140625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{29052}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{634.5520074367523193359375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{519}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.405919903599343712130576022900640964508056640625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.626359224319454455098821199499070644378662109375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{12561}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.0934467315673828125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{519}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{16.92033255100250244140625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8648827075958251953125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.262628648454287405566986990379518829286098480224609375}
\def\SubcubicDirectQuadraticProofSearchTimeLen{1812}
\def\SubcubicDirectQuadraticProofSearchTimeMaxFloat{797.13279056549072265625}
\def\SubcubicDirectQuadraticProofSearchTimeMeanFloat{656.6600033989542453127796761691570281982421875}
\def\SubcubicDirectQuadraticProofSearchTimeMedianFloat{630.4526846790313356905244290828704833984375}
\def\SubcubicDirectQuadraticProofSearchTimeMinFloat{624.99960613250732421875}
\def\SubcubicDirectQuadraticProofSearchTimeStdDevFloat{12.376547078496475506881324690766632556915283203125}
\def\SubcubicDirectQuadraticProofTimeLen{1812}
\def\SubcubicDirectQuadraticProofTimeMaxFloat{18.8142101764678955078125}
\def\SubcubicDirectQuadraticProofTimeMeanFloat{18.065095411362765531748664216138422489166259765625}
\def\SubcubicDirectQuadraticProofTimeMedianFloat{16.96406684041023282816240680404007434844970703125}
\def\SubcubicDirectQuadraticProofTimeMinFloat{16.8237488269805908203125}
\def\SubcubicDirectQuadraticProofTimeStdDevFloat{0.2402923030274002058614968291294644586741924285888671875}
\def\SubcubicDroppedSequencesFracLen{7852}
\def\SubcubicDroppedSequencesFracMaxFloat{0.425962157820276188235908421120257116854190826416015625}
\def\SubcubicDroppedSequencesFracMeanFloat{0.1887285367314081307998918646262609399855136871337890625}
\def\SubcubicDroppedSequencesFracMedianFloat{0}
\def\SubcubicDroppedSequencesFracMinFloat{0}
\def\SubcubicDroppedSequencesFracStdDevFloat{0.111833381708006551757961233306559734046459197998046875}
\def\SubcubicDroppedSequencesLen{7852}
\def\SubcubicDroppedSequencesMaxFloat{502887354265325599101}
\def\SubcubicDroppedSequencesMeanFloat{222811329055358877696}
\def\SubcubicDroppedSequencesMedianFloat{0}
\def\SubcubicDroppedSequencesMinFloat{0}
\def\SubcubicDroppedSequencesStdDevFloat{132029553360965369856}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.50170407765978808356521767564117908477783203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.312343629492336460895529626213829033076763153076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.11854436160014812651208870875052525661885738372802734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0737141078040008113081427154611446894705295562744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1730421669114597105210151539722573943436145782470703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.13882911067416825456888318512937985360622406005859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0814024144161113738515922477745334617793560028076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.00059480387568049998547881074273391277529299259185791015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.016173955563010773694987420867619221098721027374267578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{204292132286453083952}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{163900484773573165056}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{96103008365827325952}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{702220471598645146}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19094836411546271744}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{32898}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{32898}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{32898}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{32898}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{8893}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.7814569536423849882567083113826811313629150390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99143650950185513437418194371275603771209716796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{23696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97075916826725006103515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.970259964466094970703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{30371}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00546328459628205032050374256868963129818439483642578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.57754961188177400543963813106529414653778076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22584788}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22584788}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22584788}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{22584788}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{79}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{56.966887417218543987473822198808193206787109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{7790}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{22.61524341418171246687052189372479915618896484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.50277849276357289287631147089996375143527984619140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.313139390688194685363754388163215480744838714599609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1189361633002723739327421981215593405067920684814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.073862632287974905320737661895691417157649993896484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{676.314327239990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{654.9829988605928292599855922162532806396484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{623.039620935916900634765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{619.8850858211517333984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8721}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.7489748399163520531374160782434046268463134765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.23934078216552734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.08262773854843175058704218827188014984130859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.47669446468353271484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{17.1007363796234130859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.286725994034933429066569487986271269619464874267578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.5001465047251993922827750793658196926116943359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.309475828057556412442608007040689699351787567138671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{17080}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.113932449659277901243825681376620195806026458740234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0718521469025761583271361132574384100735187530517578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.177818069393813893430689176966552622616291046142578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{26278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1431826778503526298447212639075587503612041473388671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{28716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0844949799838675963403744617608026601374149322509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.000753761178994699957388314626172132193460129201412200927734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.016509702424480694749053810710393008776009082794189453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{209930522738483897340}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{26278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{169040269702006800384}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{28716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{99754065361639555072}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{889884131943329443}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19491216342879830016}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17026}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17026}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17026}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17026}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.456815242767333984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.453065700088905121134530418203212320804595947265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{6204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.5314728319644927978515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27484}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.4557187557220458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.485879266046599533890315569806261919438838958740234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{8893}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.152317880794701210334096685983240604400634765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9922332372886455420513129865867085754871368408203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{2743}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9695019423961639404296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96855843067169200555355246251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005160261161733401165385703990295951371081173419952392578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.63467535052095502834390572388656437397003173828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{24659221}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{24659221}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{24659221}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{24659221}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{79}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{59.28476821192052881315248669125139713287353515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{6155}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{21.74182574062441375417620292864739894866943359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.50121758423742601706862842547707259654998779296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.31026306455724306232468734378926455974578857421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{17080}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.11430900850082274800012527293802122585475444793701171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07199211624641109474875833029727800749242305755615234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{673.68984127044677734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{654.8979095275827830846537835896015167236328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{622.36742818355560302734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{619.4910361766815185546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8721}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.5477523331060805134029578766785562038421630859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.1743738651275634765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.09059954321147500877486891113221645355224609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{4647}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.420273482799530029296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{16.994822025299072265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.282659919339402432303387513456982560455799102783203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.482631184970026883007676588022150099277496337890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.301690724997894788028673929147771559655666351318359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1050634286714047516131387283166986890137195587158203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07076494998331574193262127892012358643114566802978515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1908092443118711012406407689923071302473545074462890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{8893}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.156801875755687103453084318971377797424793243408203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09456801480465161502397819504039944149553775787353515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.00189900900774260007752847201345502980984747409820556640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0173592666303428073970582801166528952307999134063720703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{225267794990016383769}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{8893}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{185118980629936898048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{111646205866251878400}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{2241954122207834713}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20494204725582082048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.5789470672607421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.1628587988038727729644961073063313961029052734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.62857162952423095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.099677562713623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.2070768017832402829725424453499726951122283935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{15}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10.119205298013245197807918884791433811187744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9938767473429244159177642359281890094280242919921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97822944819927215576171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.976913154125213623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00420129218470389857731372984517292934469878673553466796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.74889616016640037088336612214334309101104736328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{23614709}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{23614709}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{23614709}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{23614709}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{62.19205298013245197807918884791433811187744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{7310}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{9.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{19.72584119922546364023219211958348751068115234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.4836647548726438206045941115007735788822174072265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3024564420781672424709540791809558868408203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1051890079515551967848097092428361065685749053955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07089673290135052596827591742112417705357074737548828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{679.7437050342559814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7310}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{654.2203062654331233716220594942569732666015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{2773}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{628.803052365779876708984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{619.2665402889251708984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.7973992725143741466808933182619512081146240234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.6208221912384033203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.076083165920334039356021094135940074920654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{27484}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.099197566509246826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{16.827945232391357421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2494383778494901060529542746735387481749057769775390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.491873180870987081192424739128910005092620849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.304348538389454414954116145963780581951141357421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.108127877225521584758638482526293955743312835693359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0709229401487740940268622580333612859249114990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1860266386215976008866590518664452247321605682373046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{26278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.151991833944971233005816202421556226909160614013671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09017999100803238132773032020850223489105701446533203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.00110505560391070006311109441554663135320879518985748291015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.017091539799736009397346236937664798460900783538818359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{219621490786884115800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{26278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{179440285572905172992}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{106465741740454608896}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{1304619386403811018}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20178128672726474752}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.7125339508056640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.21119032790329317350597193581052124500274658203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.18486309051513671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5706513486772113452616395079530775547027587890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.77483443708609200939463335089385509490966796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1185}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9932664849900252335146433324553072452545166015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4430}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9801904261112213134765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8840}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97926104068756103515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004495036183450244575421361759026694926433265209197998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.7498237770514541988831069829757325351238250732421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22626995}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22626995}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22626995}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{22626995}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{60.72847682119205359185798442922532558441162109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{6159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{9.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{20.884714704202995250170715735293924808502197265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.492926542799276667938812579450313933193683624267578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.305121684204151810693161905874148942530155181884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1084852513389415185063313629143522121012210845947265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07105468023189250026394603310109232552349567413330078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{677.4972207546234130859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7310}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{654.2104931446100408720667473971843719482421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{621.563103258609771728515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8721}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{619.2171604633331298828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.1779293852461503178119528456591069698333740234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.589344024658203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{11598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.082611723451424978748036664910614490509033203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{27484}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.5170590877532958984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{17.06819820404052734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.22846880653996393117921570592443458735942840576171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.297234766475018286069342821065220050513744354248046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.1752296065678015379862841882641077972948551177978515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.05985570555174495044337135141176986508071422576904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04338832366395330153441278753234655596315860748291015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.420772632212148611774438222710159607231616973876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.36853069809922167632265654901857487857341766357421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{20754}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.24180498200347955162214930169284343719482421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.01191731251484600025147830848482044530101120471954345703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.035253870672569596889101006809141836129128932952880859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{496760643816871793046}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{435084254153079128064}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{20754}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{285472935601032462336}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{14069479296497962608}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{41620424313890955264}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{179.824432373046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.302513274135975507306284271180629730224609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.872837066650390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{82.67822265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.48188325228561978974539670161902904510498046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{73}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{30899}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{49.78145695364238321189986891113221645355224609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{4430}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{25.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30371}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99875548304311489999918194371275603771209716796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99095796048641204833984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97290700674056995733707253748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0022064572064680976030970338541692399303428828716278076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{8.62991412152147319147843518294394016265869140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21560179}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21560179}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21560179}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{21560179}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{100}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{83.6622516556291344613782712258398532867431640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{57.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.13343718384585923075746904942207038402557373046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.297871304100864098263201640293118543922901153564453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.17568221993964783234076776352594606578350067138671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.060053535013060134473139584088130504824221134185791015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.043509843700604212968219286494786501862108707427978515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{674.24658107757568359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{654.44703948418828076682984828948974609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{623.567256867885589599609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8721}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{620.335491657257080078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.8354028138475992903977385140024125576019287109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.73194980621337890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.0694854338437522756066755391657352447509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.532316505908966064453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{13293}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{17.135767459869384765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2148753334100011735952051594722433947026729583740234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.487922540717506014740223463377333246171474456787109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.301462149775250765060263802297413349151611328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{24144}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1046523203296225446035094819308142177760601043701171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07073953526663261104356905661916243843734264373779296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.190841654559235907040459778727381490170955657958984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{8893}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1568283185785640243548044736598967574536800384521484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09447331791600320494151077355127199552953243255615234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.00189900900774260007752847201345502980984747409820556640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.017348706156774230946471249126261682249605655670166015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{225306058256480738944}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{8893}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{185150198805053472768}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{111534407513005522944}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{2241954122207834713}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20481737118976221184}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.6250514984130859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.251300483349933045928992214612662792205810546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.6317813396453857421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.075281620025634765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.219462901648069586002520736656151711940765380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{15}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10.112582781456953995302683324553072452545166015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9938392437846454985361788203590549528598785400390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97840508818626414910823996251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97710520029068004266292746251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004264753981658374847041326205498990020714700222015380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.7550043729596505048817789429449476301670074462890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{23631348}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{23631348}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{23631348}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{23631348}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{62.27814569536423761064725113101303577423095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{7310}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{9.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{19.63344859789850005427069845609366893768310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.4889674422253216246048168613924644887447357177734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3022271764108135361226459281169809401035308837890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24144}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.104777408223852341873083560130908153951168060302734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07087060707714716578653479928107117302715778350830078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{674.381141185760498046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{654.62410695821245099068619310855865478515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{626.718101084232330322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{625.06046390533447265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.656156416355830884867827990092337131500244140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{19.31887054443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.08266311765506628717048442922532558441162109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.4968624114990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{17.132220745086669921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2489990738051721386181469597431714646518230438232421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.491438364427183194127479737289831973612308502197265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.304082598777105472809267894263030029833316802978515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1080433236252852646774869072032743133604526519775390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07088176635232400213393333388012251816689968109130859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.186078226758513098904046501047560013830661773681640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{26278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1520404818242185041032854542208951897919178009033203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09019408808950014899696867587408632971346378326416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.00110505560391070006311109441554663135320879518985748291015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.017093967158016067087178413430592627264559268951416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{219682395309054960867}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{26278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{179497718851510239232}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{106482384636711993344}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{1304619386403811018}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20180994391572389888}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.80197429656982421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.2154952990298237835986583377234637737274169921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29052}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.17984616756439208984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0430088043212890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.57185251083535393323842299651005305349826812744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.77483443708609200939463335089385509490966796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1185}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99322471555495106532163163137738592922687530517578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98021240532398223876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8840}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97925865650177001953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004573952373163210453899107932329570758156478404998779296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.7648975560028825615432879203581251204013824462890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22676912}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22676912}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22676912}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{22676912}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{60.71523178807947118684751330874860286712646484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{6159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{9.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{20.878195312713469178333980380557477474212646484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.492490795182346230429715205900720320641994476318359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.304855052703019158144570610602386295795440673828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1084004182800799298558303007666836492717266082763671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0710133553974724718305111537119955755770206451416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{675.29382991790771484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{655.03129230587683196063153445720672607421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{19093}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{627.722712099552154541015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{624.9937312602996826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.650642000520459617973756394349038600921630859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.1298191547393798828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.078989193139488378392343292944133281707763671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.40903759002685546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{13293}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{16.9971768856048583984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2755380419475030873144305587629787623882293701171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.294266101589366113611134778693667612969875335693359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.1751660097873324328787703052512370049953460693359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.059802255113148898579833456778942490927875041961669921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.043465253617399633723206164859220734797418117523193359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.420726722008594011814608393251546658575534820556640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.368517669496955857511011345195583999156951904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{20754}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.24158595614270605977935701957903802394866943359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.01188737860194520080947544471428045653738081455230712890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.03525939439293730714997110453623463399708271026611328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{496706442615249791888}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{435068872694414442496}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{20754}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{285214355505082826752}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{14034139569751991424}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{41626945571872260096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{181.325698852539034078290569595992565155029296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.10632122115583797494764439761638641357421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.661590576171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{81.919342041015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.5543243092486829226572808693163096904754638671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{74}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{30899}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{49.80132450331125681941557559184730052947998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{4430}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{25.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30371}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99874381553258329002886739544919691979885101318359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99097564816474903448551003748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9729073047637939453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0022058405197048999192566132165893577621318399906158447265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{8.6827986054713033325924698146991431713104248046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21580722}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21580722}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21580722}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{21580722}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{100}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{83.6092715231788048413363867439329624176025390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{57.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.1177173864817664394877283484674990177154541015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.2948962817257410051752231083810329437255859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1756181575829755814321941898015211336314678192138671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.05999990791509006438086970547374221496284008026123046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.043585867074411109578502276917788549326360225677490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{677.2333891391754150390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{655.0042229772403743481845594942569732666015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{626.94411027431488037109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8721}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{626.775405406951904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.63791027565076774408225901424884796142578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{19.7917287349700927734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.083547112168066206550065544433891773223876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.486132442951202392578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{13293}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{17.12304592132568359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.261137988920298325101754244315088726580142974853515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.29131926068545410668519934915821067988872528076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.173534047412542580257621693817782215774059295654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.062304037386950394949991505200159735977649688720703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.042599408735652898039258928974959417246282100677490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.424899708669230602442468125445884652435779571533203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.371690508416201825792057888975250534713268280029296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{15399}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.24424084744895679932596976868808269500732421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.01238063818612470008695414236399301444180309772491455078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0353453102336404312300288665937841869890689849853515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{501633035700162894058}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{438814699736361992192}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{15399}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{288348697935157919744}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{14616477701672934517}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{41728377093493252096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{187.469207763671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{104.0375475851905235913363867439329624176025390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{87.287982940673828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{83.86852264404296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.91771665649914524465202703140676021575927734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{77}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{30899}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{51.03973509933774721503141336143016815185546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{25.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30371}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9987208918230423559947439571260474622249603271484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99055804312229145391910378748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97134721279144276007144753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0023297505283135476472633484945617965422570705413818359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{8.9493651369060085443152274820022284984588623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21603472}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21603472}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21603472}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{21603472}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{100}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{83.96026490066225278496858663856983184814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{58.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{6.973821241707060636372261797077953815460205078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.291943130069103273793729158569476567208766937255859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.173981368922410284394430846077739261090755462646484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.06250995884490340159800325636751949787139892578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.042715285703249138149484309678882709704339504241943359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{680.831829071044921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{654.9136286129224799879011698067188262939453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{623.0230081081390380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{621.7965734004974365234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8721}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.664030519386159312489326111972332000732421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.307086944580081677713678800500929355621337890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.092668020172624210317735560238361358642578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{15662}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.4937188625335693359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{17.156928539276123046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.289697329235035050398749945088638924062252044677734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.42875347524414397781811203458346426486968994140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.252848532251204793919185931372339837253093719482421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0722046294577507463685606126091443002223968505859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0635673939134366872139025872456841170787811279296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.308281542072244396646141240125871263444423675537109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.246618444638801559420926423626951873302459716796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1518270683435070100841812745784409344196319580078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.005185276521526899738689930785540127544663846492767333984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0308899280040505173905440727821769542060792446136474609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{363954605392333863412}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{291155669254930006016}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{179245764684434210816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{6121694012417488037}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{36468390166146134016}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{16770}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{16770}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16770}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16770}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{32.51659393310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{29052}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{20.5541418403979179174712044186890125274658203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{913}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{13.2870109081268310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{11.60878849029541015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.819185726656505242004868705407716333866119384765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{32}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29052}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{20.092715231788080387786976643837988376617431640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{8.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30371}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.998758423012613416602789584430865943431854248046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9930743277072906494140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99062860012054443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0013086473051410578427589115335649694316089153289794921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{4.05647384371388231016908321180380880832672119140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{25605526}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{25605526}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{25605526}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{25605526}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{83}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{74.3443708609271567411269643343985080718994140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{20.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{32103}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{9.1817890288193257930515756015665829181671142578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.429671664332323788304535128190764226019382476806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.253493470313803814786268731040763668715953826904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{7310}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.072290933564760184726338820837554521858692169189453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0637084950655793236240498345068772323429584503173828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{678.141414165496826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7310}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{654.2883308628537406548275612294673919677734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{629.883291423320770263671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{621.464503765106201171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.4858635057855398287074422114528715610504150390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.6527798175811767578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{9504}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.070449709102806679084096685983240604400634765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.03667581081390380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{16.91466999053955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2445894504893264265188435047093662433326244354248046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6733616289693087342271837769658304750919342041015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{1185}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5641506316835680490129334430093877017498016357421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.31948756156468050004804126729140989482402801513671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{15043}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06550319225883403928545334338195971213281154632568359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1672577859339718087117176992251188494265079498291015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.133967747960462124634517522281385026872158050537109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{27671}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08479437855204696727895452568191103637218475341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0246351218470362010037888467195443809032440185546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01452613499971106870989334680643878527916967868804931640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{197463140573393667786}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{158161200688503652352}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{27671}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{100107532802486878208}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{29084018427963489558}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17149433262068797440}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{32898}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{32898}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{32898}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{32898}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.8410596026490058108038283535279333591461181640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99940335750579845086605246251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99276451914515717600551170107792131602764129638671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{23633}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96238006651401519775390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95770251750946044921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.006170640990258218112896049234450401854701340198516845703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.64816862134750774515623561455868184566497802734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{23023700}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{23023700}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{23023700}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{23023700}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{30371}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{68.947019867549670379958115518093109130859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{14}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{30684}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{11.0386365888784983013692908571101725101470947265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.67572902718173633029863367482903413474559783935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.56559558706242574199762884745723567903041839599609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.320771909695799328776644188110367394983768463134765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15043}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06565117393453258343161138554933131672441959381103515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{680.870671749114990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7310}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{658.8854562809925710098468698561191558837890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1412}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{633.6287124156951904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{19488}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{625.5548269748687744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.3881877634046393410471864626742899417877197265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.74901580810546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{9504}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.1262503680803916950026177801191806793212890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.205847263336181640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{17.086485385894775390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.232345650868604369776448947959579527378082275390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6645599115710874027485033366247080266475677490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{1185}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5595146974127620520533810122287832200527191162109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{27484}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.3258186161674128111798154350253753364086151123046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.064788068959288291903675371941062621772289276123046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.173101017255082201273808095720596611499786376953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.138525233803149683264877012334181927144527435302734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0879785921918481428338765226726536639034748077392578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0266632838625916988861686007794560282491147518157958984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0147982545065651789617522382513925549574196338653564453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{204361610509010115189}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{163541730285918781440}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{103866788744210219008}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{31478449508985570824}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17470695271694524416}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17026}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17026}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17026}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17026}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.456815242767333984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.453065700088905121134530418203212320804595947265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{6204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.5314728319644927978515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27484}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.4557187557220458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.485879266046599533890315569806261919438838958740234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{15}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.1655629139072853917014072067104279994964599609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9993984699249267578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99313260032641181851431610994040966033935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7310}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96640421450138103143245871251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{30684}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94749915599822998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.006172685764482884786252814279805534170009195804595947265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.69701905992550639012961255502887070178985595703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{25098133}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{25098133}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{25098133}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{25098133}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{30371}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{69.1324503311258240501047112047672271728515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{14.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.8802485221231091117033429327420890331268310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6655521711592200517770834267139434814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1185}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.56094776875051899356350304515217430889606475830078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.32689548128375722768623745650984346866607666015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06493168466341540934205767143794219009578227996826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{680.0743629932403564453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{657.7057766567003227464738301932811737060546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.66511666774749755859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{29022}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{621.9629611968994140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.0681215661795544491496912087313830852508544921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7476749420166015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{9504}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.12660181127636604969666223041713237762451171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.066380083560943603515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{17.0258824825286865234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2419234409756362003118823622571653686463832855224609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.63691284420419502776411491140606813132762908935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.54408265655445420261315803145407699048519134521484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{19093}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.307676205474838315723218329367227852344512939453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0632191100699835140108717723705922253429889678955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1869902700955710928010233828899799846112728118896484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.152456164415162465086694965066271834075450897216796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{5928}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0997838224194380618570221486152149736881256103515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.030648756739593101261487362307889270596206188201904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01546551469110020969599528228854978806339204311370849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{220759146030516831702}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{179988470235256815616}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{5928}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{117803944631542792192}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{36183665392170010753}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18258457054394931200}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.5789470672607421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.1628587988038727729644961073063313961029052734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.62857162952423095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.099677562713623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.2070768017832402829725424453499726951122283935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{16}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10.1589403973509941891961716464720666408538818359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999333560466766357421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9944876633732524506825711796409450471401214599609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9751243889331817626953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{30684}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9634597301483154296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004950520717616128767157857026859346660785377025604248046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.83812716100483175551971726235933601856231689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{24053621}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{24053621}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{24053621}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{24053621}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{30371}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{70.3642384105960303486426710151135921478271484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{14.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{13654}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.588829526303459971359188784845173358917236328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.63834843430326670965513358169118873775005340576171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.5454734424560989669572563798283226788043975830078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{19093}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.308693107997789428775803344251471571624279022216796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06333084439826287825869854941629455424845218658447265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{680.5563776493072509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7310}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{659.12586735100148871424607932567596435546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{630.073925018310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{628.538938999176025390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.3398911579359236156960832886397838592529296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.75499820709228515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{23447}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.13280728479094960903239552862942218780517578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{16069}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.52474689483642578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{13293}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{17.1956870555877685546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.234155052015501630169325153474346734583377838134765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.64246390572948908204153894985211081802845001220703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.548787241208529952274375318665988743305206298828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{6204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.3155244962167673694608538426109589636325836181640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06385885132512879314159448540522134862840175628662109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1816439205732688078054337665889761410653591156005859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1475595838868450637715312723230454139411449432373046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{23241}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09460959467382092091813916567843989469110965728759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0293721520867428996515169359327046549879014492034912109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01520511220731396960503811754961134283803403377532958984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{214447290583060231738}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{174207608293357125632}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{23241}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{111695294711383687168}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{34676516636046135160}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17951028064022902784}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.7125339508056640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.21119032790329317350597193581052124500274658203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.18486309051513671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5706513486772113452616395079530775547027587890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{16}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.8211920529801322032881216728128492832183837890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99945729970931995733707253748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99407336648726307704038163137738592922687530517578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9674010574817657470703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.93096709251403797491519753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.006643688472444379648773615798518221708945930004119873046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.801714020994114040519207264878787100315093994140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{23065907}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{23065907}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{23065907}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{23065907}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{30371}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{69.754966887417225507306284271180629730224609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{14.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{13654}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.02048688683512267516562133096158504486083984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.64719011859366604166865499792038463056087493896484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.55019065995202820484877292983583174645900726318359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.31656733817381932372114761164993979036808013916015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0639807409915459091021006088340072892606258392333984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{682.082708835601806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{659.639219173532410422922112047672271728515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{2773}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{636.5368869304656982421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{19488}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{634.950856685638427734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.7911893829989384840928323683328926563262939453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.870635509490966796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{11498}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.13949251017033503785569337196648120880126953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.721875607967376708984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{29726}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{17.7149295806884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2281922906001947193299628224849584512412548065185546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.435405177351559424803184583652182482182979583740234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.324020453789777729269871997530572116374969482421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.171127126812958885171411793635343201458454132080078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.044377569620532610061847123006373294629156589508056640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.42287338011308051033410038144211284816265106201171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.36934367630419340233771663406514562666416168212890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.256517272009890884287841572586330585181713104248046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07826361240210570613395901773401419632136821746826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0300847283754349208162448547909662011079490184783935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{499240769185951692009}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{436044049409694629888}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{302842141904166125568}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{92397365009001372030}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{35517778231597809664}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{179.824432373046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.302513274135975507306284271180629730224609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.872837066650390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{82.67822265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.48188325228561978974539670161902904510498046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{77}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{49.5099337748344368037578533403575420379638671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{2743}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{27.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{13}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{32103}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9986600954801041485353607640718109905719757080078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{23696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99624253809452056884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24144}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.995275199413299560546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000773906002378485740993141472898741994868032634258270263671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{8.7328773238394976630161181674338877201080322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21999091}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21999091}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21999091}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{21999091}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{98}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{82.89403973509934075991623103618621826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{62}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{14}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{6.3268086363979652020361754694022238254547119140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.43638657279267578648074277225532568991184234619140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3248545704998402339214180756243877112865447998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.171692720134460297121137273279600776731967926025390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.04451716620236913224406549716150038875639438629150390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{680.419544696807861328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7310}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{659.5571879456374517758376896381378173828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{634.4521160125732421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{19488}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{628.72657680511474609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.4034117196590774057085582171566784381866455078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{19.023383855819705701151178800500929355621337890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.13938325761959191595451557077467441558837890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.548369586467742919921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{17.06854724884033203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2497779960565330303889908236669725738465785980224609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6347456743105410748029271417181007564067840576171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5438410774778656975314561350387521088123321533203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.30613281796239266707715387383359484374523162841796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06320714471503525999640515919963945634663105010986328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.187049439789156390911983862679335288703441619873046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1524636167665628649903197810999699868261814117431640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{5928}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.099827942079391995822135186244850046932697296142578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.030664143849361398530550815166861866600811481475830078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01544383451462832089473575791771509102545678615570068359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{220829001274963981243}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{179997268418874966016}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{5928}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{117856031932393340928}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{36201831285029442964}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18232861619716544512}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.6250514984130859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.251300483349933045928992214612662792205810546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.6317813396453857421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.075281620025634765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.219462901648069586002520736656151711940765380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{16}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10.152317880794701210334096685983240604400634765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99933171272277843133480246251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{26278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99447471574442281028183288071886636316776275634765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9752657711505889892578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96346843242645263671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004933257175629042479148012034784187562763690948486328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.8332771812945012346318662821431644260883331298828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{24070260}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{24070260}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{24070260}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{24070260}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{30371}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{70.4304635761589423736950266174972057342529296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{14.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{13654}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.5082818506439839012500669923610985279083251953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.63617637964763840141557693641516380012035369873046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.54523120246544720668424588438938371837139129638671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{23633}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.3071446194257643202973895313334651291370391845703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.063318504661312946524276412674225866794586181640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{682.6196460723876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{659.5902178034876897072535939514636993408203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{19093}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{635.26681315898895263671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{632.7912719249725341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.801178542816639804868827923201024532318115234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.712631702423095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{11498}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.135121304467812564098494476638734340667724609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.650311887264251708984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{5928}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{17.4472506046295166015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2192212868522676327831533171774935908615589141845703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6420972668366624613867088555707596242427825927734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5487328660101378208224787158542312681674957275390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{30371}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.315409459707343742262963814937393181025981903076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.063883719840133690315298053974402137100696563720703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1817230441482007019526889735061558894813060760498046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.147618264043330615908899972055223770439624786376953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0946278330467884287724444902778486721217632293701171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0293883221204590990016658480499245342798531055450439453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01521051036344057971749776925207697786390781402587890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{214540703212625967899}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{174276885594406551552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{111716826781684563968}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{34695606842358218581}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17957401081913290752}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.80197429656982421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.2154952990298237835986583377234637737274169921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29052}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.17984616756439208984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0430088043212890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.57185251083535393323842299651005305349826812744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{16}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.8211920529801322032881216728128492832183837890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99945729970931995733707253748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99410431432408208340945066083804704248905181884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96727485954761494024722878748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.930698871612548828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.006627956367368012698115808944976379279978573322296142578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.7980345881918389228104615540360100567340850830078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{23115824}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{23115824}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{23115824}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{23115824}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{30371}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{69.768211920529807912316755391657352447509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{14.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{13654}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.026087633100605245317638036794960498809814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.64682078256340280741909509742981754243373870849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.550136055689451008987589375465176999568939208984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.31645192145651945825335360495955683290958404541015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06400477370455437409191290498711168766021728515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{682.089663982391357421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{15043}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{659.6232537828533395440899766981601715087890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1412}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{633.12270319461822509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{626.2125942707061767578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.075650812756276053505644085817039012908935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.712992191314697265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{9504}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.13811032819432256246727774851024150848388671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{26278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.626975595951080322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{17.38460063934326171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2247681843551756486476733698509633541107177734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.43116640114242887893425404399749822914600372314453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.3241552959789846255489464965648949146270751953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1702107765032373765112794217202463187277317047119140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04470935096651214302188037663654540665447711944580078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.4228219674668822758434316710918210446834564208984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.36931910773713549911434483874472789466381072998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4647}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2566090154826745628469097937340848147869110107421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.078221367557798793246348623142694123089313507080078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.03007437919942541892925902402566862292587757110595703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{499180071846651093540}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{436015043965293035520}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4647}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{302950453479390052352}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{92347491099794037771}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{35505560081119674368}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{181.325698852539034078290569595992565155029296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.10632122115583797494764439761638641357421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.661590576171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{81.919342041015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.5543243092486829226572808693163096904754638671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{77}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{49.4701986754966895887264399789273738861083984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1185}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{27.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{13}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99998623132705677374332253748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{32103}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.998662110985509610117105694371275603771209716796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9962555468082427978515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24144}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99527609348297119140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0007707339030363041625093512010380436549894511699676513671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{8.7168922913390520790244408999569714069366455078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22019634}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22019634}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22019634}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{22019634}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{98}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{82.8675496688741759498952887952327728271484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{61.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{14}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{6.3524261378576429848408224643208086490631103515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.432138242458183496896850783741683699190616607666015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.324989640621889230853724939152016304433345794677734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1707733411896825981290959362013381905853748321533203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.04484988745172426016782907254309975542128086090087890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{682.106627941131591796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7310}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{659.46397914160161235486157238483428955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{632.889982998371124267578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{624.885946750640869140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.02854120727972286886142683215439319610595703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.69989681243896484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{11598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.12063971418418617531642667017877101898193359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{32103}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.071256160736083984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{17.0136129856109619140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2456654287521386759163277702100458554923534393310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.4314683048911531759728177348733879625797271728515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.320045252993090112436647132199141196906566619873046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.16757250604737727872617369939689524471759796142578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{8893}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04409791955371267224705889020697213709354400634765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.425962157820276188235908421120257116854190826416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.37254001672039904757838257864932529628276824951171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{22545}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.25974774700840741470386774381040595471858978271484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07978799653044900408449535689214826561510562896728515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0301300336441980565194143082408118061721324920654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{502887354265325599101}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{439817622122027352064}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{22545}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{306656013618351833088}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{94197040137677986967}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{35571265252273909760}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16962}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{187.469207763671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{104.0375475851905235913363867439329624176025390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{87.287982940673828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{83.86852264404296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.91771665649914524465202703140676021575927734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{78}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{50.64900662251655916179515770636498928070068359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{28}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{13}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99998420476913441046207253748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{32103}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99865443382831597940452184047899208962917327880859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99622094631195068359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.995227634906768798828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000784981909541081364876935477781216832227073609828948974609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{8.888714979123168546948363655246794223785400390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22042384}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22042384}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22042384}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{22042384}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{98}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{83.2913907284768271210850798524916172027587890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{62}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{14}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{6.33249728834793135234804140054620802402496337890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.43244082669252914552515676405164413154125213623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.320868881778327563747410522410064004361629486083984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.168474363996238218899037519804551266133785247802734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8893}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.044235247847665214171453129665678716264665126800537109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{681.2812786102294921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7310}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{659.306562370022447794326581060886383056640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{26829}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{633.60486352443695068359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{626.0639355182647705078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.0290058989686503565508246538229286670684814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.6579072475433349609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.1248233602536430453255889005959033966064453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{15662}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.120593607425689697265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{17.084067821502685546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.245626073831217095477796874547493644058704376220703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.57546566368248475153990284525207243859767913818359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{12141}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.460614551367845626028696415232843719422817230224609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{20976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.2458536992752751171309455457958392798900604248046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.058786098647888744561651463982343557290732860565185546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.311808437349295919371883201165474019944667816162109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.244805268101960127324900895473547279834747314453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1628295805166272980368802336670341901481151580810546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.045959832493008202780604420922827557660639286041259765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.02860970652351967069559890433083637617528438568115234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{368118428403568686965}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{289015048228653662208}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{192235238362861240320}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{54259793130821351603}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{33776379792851582976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{16770}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{16770}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{16770}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16770}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{32.51659393310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{29052}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{20.5541418403979179174712044186890125274658203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{913}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{13.2870109081268310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{11.60878849029541015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.819185726656505242004868705407716333866119384765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{34}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{20.430463576158938820981347816996276378631591796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{10.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99983596801757801397769753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12141}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99855345527067884692229426946141757071018218994140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98966801166534423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97515940666198719366519753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0021139568270939755080528588138122358941473066806793212890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{4.2822750866271395153717094217427074909210205078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{26044438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{26044438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{26044438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{26044438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{84}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{75.5033112582781456012526177801191806793212890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{1185}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{45.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{6.32547061012397104917681645019911229610443115234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.57867476778349857813310563869890756905078887939453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12141}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.46179104991519992484683143629808910191059112548828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.2461475610972976568735504088181187398731708526611328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.058897621949200111568512028270561131648719310760498046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{683.7836930751800537109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{11598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{659.81567037184504442848265171051025390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{26374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.723063528537750244140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13654}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{630.75046825408935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.1836966661812891032923289458267390727996826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.6835911273956298828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{11598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.14482569062946737403763108886778354644775390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.59169185161590576171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{17.3828547000885009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2271638253662705275726096942889853380620479583740234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.06097333043518800288484982274894719012081623077392578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0034615186873378851924176746734929110971279442310333251953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000000004870439446712226949642854378907941281795501708984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.009960480747666151934982536886309389956295490264892578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.137414163603343186803584785593557171523571014404296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10564329383101288273305584652916877530515193939208984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{25516}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.056960660469952302531471133306695264764130115509033203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.026389242234915101514847179942080401815474033355712890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01509369313841059379033282539239735342562198638916015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{162230010117998455656}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{124721587481881264128}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{25516}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{67247278461355212800}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{31154918259622891995}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17819487644887437312}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{36994}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{36994}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{36994}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{36994}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{11}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{5781}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.403973509933774010960405576042830944061279296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{742}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.998637974262237548828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.990637029638353538985029445029795169830322265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{8721}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9680902659893035888671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6204}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9467487335205078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00607154835646922692860005810189250041730701923370361328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.240480615825444221655970977735705673694610595703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21490869}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21490869}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21490869}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{21490869}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{28.74172185430463599686845554970204830169677734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{12.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{12}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{19.49612411002154743755454546771943569183349609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.061103331896286812441321245614744839258491992950439453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.003469637399078968897914165836482425220310688018798828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000489003933974870045007379824636481726159810746288486051069899218646241934038698673248291015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00998175054707286894817297451254489715211093425750732421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{678.8510887622833251953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{656.7658873330677806734456680715084075927734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27714}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{630.00113403797149658203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{18146}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{628.7638113498687744140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{1185}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.8776507681326695120560543728061020374298095703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.671835422515869140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.053866443255088825026177801191806793212890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{27300}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.486805021762847900390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{6549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{17.082576274871826171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2198817940680239946260599026572890579700469970703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.05616134569542639842776310388217098079621791839599609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.003302681377586327675366373313181611592881381511688232421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{29022}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000000004870439446712226949642854378907941281795501708984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0095896634668472084672696809093395131640136241912841796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.140457124666742594332191629291628487408161163330078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10826808123850080456396227646109764464199542999267578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.058167831642398047653497172859715647064149379730224609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0274659975004233995743430085667569073848426342010498046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01553070945722729613580614937973223277367651462554931640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{165822504451617119804}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{127820389501326032896}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{68672454632316305408}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{32426126503645240719}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18335425448999194624}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21122}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21122}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21122}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21122}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.456815242767333984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.453065700088905121134530418203212320804595947265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{6204}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.5314728319644927978515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27484}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.4557187557220458984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.485879266046599533890315569806261919438838958740234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{12}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{16284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.635761589403973204071007785387337207794189453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1895}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{742}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99862748384475719110042746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99161356016500101784316711928113363683223724365234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{21598}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97852002084255207403629128748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8840}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.978179514408111572265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{7310}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004630235878872746187184805677361509879119694232940673828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.2205928627260898000628230875008739531040191650390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{23565302}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{23565302}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{23565302}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{23565302}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{29.70860927152317998434227774851024150848388671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{8893}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{12.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{12}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{19.64303607586655431305189267732203006744384765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.056281087506240577711391637194537906907498836517333984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0033105232921624163332230406098233288503251969814300537109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29022}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000489003933974870045007379824636481726159810746288486051069899218646241934038698673248291015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0096101441708249489559445777331347926519811153411865234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{691.7115037441253662109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{656.860216044432263515773229300975799560546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.83393037319183349609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{18146}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{630.0294764041900634765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{1185}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.9073455325645678470891652978025376796722412109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.6438848972320556640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.05621133576955372745942440815269947052001953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{4647}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.452186107635498046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{17.1549293994903564453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2178256531288726705053448995386133901774883270263671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.050106858055422802411538185651806998066604137420654296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{8721}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.002833588287892817823843127911231931648217141628265380859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{12141}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000000004870439446712226949642854378907941281795501708984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.008515110493839551930594922168893390335142612457275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.150279131989795811108479028916917741298675537109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.116652402865955406863207599599263630807399749755859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8893}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.062909849959082497772300257565802894532680511474609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.032014733114494299537344801365179591812193393707275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0167396426548088485264376146233189501799643039703369140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{177418283995838874912}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{137718849360098689024}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8893}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{74270841722282475520}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{37796325654476295555}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19762681852071084032}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{20930}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{20930}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{20930}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{20930}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.5789470672607421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.1628587988038727729644961073063313961029052734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11611}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.62857162952423095703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.099677562713623046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.2070768017832402829725424453499726951122283935546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{15662}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.5496688741721857951461061020381748676300048828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1895}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99908232688903797491519753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{15662}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9936874777275994663483515978441573679447174072265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98135666549205791131527121251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8840}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.980889737606048583984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{9504}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0038302243947684485279869814888797918683849275112152099609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.3504413883378345584418411817750893533229827880859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22520790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22520790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22520790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{22520790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{31.086092715231789185281741083599627017974853515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{17096}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{12.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{12}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{20.283729295597968445008518756367266178131103515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0501999287438758268198313317043357528746128082275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8721}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0028407083876553526451125275542608505929820239543914794921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{12141}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000489003933974870045007379824636481726159810746288486051069899218646241934038698673248291015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0085344541343251277554227129940045415423810482025146484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{700.720372676849365234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{655.8509508789769597569829784333705902099609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{30463}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{630.468314230442047119140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{19488}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{629.780283451080322265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{1185}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.4973734313542781393380209919996559619903564453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.8238832950592041015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{14095}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.071076628388158979987565544433891773223876953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{15662}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.53952276706695556640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{17080}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{17.3500869274139404296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2254953698777216464232964199254638515412807464599609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.050370674383315598710009197702675010077655315399169921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{8721}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0029397403396158351684963605521261342801153659820556640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{6589}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000000004870439446712226949642854378907941281795501708984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.008773789653566226032221919695075484924018383026123046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1475151301909607137741176074996474198997020721435546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.11388018550327104472241757093797787092626094818115234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{30899}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.06156442703612947930924548245457117445766925811767578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0304242633478968016458310330563108436763286590576171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0163380778433330521581812178055770345963537693023681640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{174155126632486245966}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{134445992770906243072}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{30899}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{72682446693122981888}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{35918630375026828767}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19288597800467800064}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{20930}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{20930}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{20930}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{20930}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.7125339508056640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.21119032790329317350597193581052124500274658203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{123}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.18486309051513671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5706513486772113452616395079530775547027587890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{12}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{5781}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.23841059602649039561583776958286762237548828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999147474765777587890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99315548574687628757828861125744879245758056640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19004}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.980823576450347900390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{17197}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97902488708496082647769753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.003949588194147133669853477755395942949689924716949462890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.3056606724856971712966924314969219267368316650390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21533076}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21533076}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21533076}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{21533076}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{1895}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{29.72185430463576238935274886898696422576904296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{5781}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{12.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{12}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{19.49024512005172482531634159386157989501953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.050464235095853453294534318729347432963550090789794921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8721}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00294703299624332094863721209776485920883715152740478515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6589}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000489003933974870045007379824636481726159810746288486051069899218646241934038698673248291015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00879353465731359633383856788668708759360015392303466796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{708.8345077037811279296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{656.0598905575985781979397870600223541259765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{20294}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.8820278644561767578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{19488}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{631.0006797313690185546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{18146}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.5789766033631362773803630261681973934173583984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7462978363037109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.066101236848641775623036664910614490509033203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{2773}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.55148220062255859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{17.3282501697540283203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.219410062137855355057780570859904401004314422607421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.02921635116566349832378790551956626586616039276123046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.001488459430417202015994870833992536063306033611297607421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{22286}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.004240396493432448121740918622890603728592395782470703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.322602214737226111740397982430295087397098541259765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.257740438907239910459878728943294845521450042724609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1499638013429341609761280551538220606744289398193359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.10984476387849269329866075395329971797764301300048828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.034104749240071174920529983864980749785900115966796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{380861471543648116569}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{304286202493915496448}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{177046007276398575616}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{129681807814631055954}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{40263781179496521728}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{20930}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{20930}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{20930}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{20930}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{179.824432373046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.302513274135975507306284271180629730224609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.872837066650390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{82.67822265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.48188325228561978974539670161902904510498046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{61}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{40.21854304635761678810013108886778354644775390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{22.25}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{742}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{11}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99984793315660080992302027880214154720306396484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{17197}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99880288541316986083984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12561}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99870628118515003546207253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0002501432015891516015548834417359103099443018436431884765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{6.6838681346600861132856152835302054882049560546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20466260}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20466260}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20466260}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20466260}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{97}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{8721}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{65.0264900662251648100209422409534454345703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{27714}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{18.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{22.839186442367843454803733038716018199920654296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0292786434549710226915575361772425821982324123382568359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00149169611493440014242384261677898393827490508556365966796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0042490039597667776660738780947212944738566875457763671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{740.6296675205230712890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{656.9688941532413082313723862171173095703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29726}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.515073478221893310546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{19488}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{631.4959495067596435546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{18146}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{12.8670299383559143535649127443321049213409423828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.673077106475830078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.070471766768701371574934455566108226776123046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{18146}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.559372246265411376953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{17.3339917659759521484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.207294463010239182754190778723568655550479888916015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.050099536079389099529901585583502310328185558319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{8721}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0028363134785209138943873341531798359937965869903564453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{6549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000000004870439446712226949642854378907941281795501708984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0085036337979590391478179611794985248707234859466552734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.150176445999839203171433155148406513035297393798828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.116626821822569171072103699771105311810970306396484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8893}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.06294531244503272227053258802698110230267047882080078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0320152816044567967157519206011784262955188751220703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0167184737014052821335585718998117954470217227935791015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{177297053776530992193}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{137688648594627739648}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8893}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{74312708436045119488}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{37796973197130053538}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19737689963063480320}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.6250514984130859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.251300483349933045928992214612662792205810546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{9134}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.6317813396453857421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.075281620025634765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.219462901648069586002520736656151711940765380859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{15662}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.5496688741721857951461061020381748676300048828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1895}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999212741851806640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{15662}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99369542172412994585073420239496044814586639404296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98131890594959270135433371251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8840}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98073834180831920281917746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{9504}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0038357064126308790426300721065899779205210506916046142578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.3504413883378345584418411817750893533229827880859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22537429}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22537429}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22537429}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{22537429}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{31.01324503311258240501047112047672271728515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{17096}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{12.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{12}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{20.181621288046482476374876569025218486785888671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.050192593167680855936740869083223515190184116363525390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8721}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0028434263828346095261123682718107374967075884342193603515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000489003933974870045007379824636481726159810746288486051069899218646241934038698673248291015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00852290230106278468014124882756732404232025146484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{759.4250662326812744140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{657.443341635710339687648229300975799560546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{23633}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{633.265080273151397705078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{18146}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{632.55203914642333984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{27300}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{13.5283333985152349754343958920799195766448974609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{19.839447498321533203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.080829400889921743100785533897578716278076171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{20751}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.51489365100860595703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{17080}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{17.0580251216888427734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.269851474783717015792916527061606757342815399169921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.050370674383315598710009197702675010077655315399169921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{8721}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00294577892106982590358921214601650717668235301971435546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{6589}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000000004870439446712226949642854378907941281795501708984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00878374847845882385233284850301060942001640796661376953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1475939749889982888220174572779797017574310302734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.11391808564677434467693473152394290082156658172607421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{30899}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.06159081601589562471321670500401523895561695098876953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.030463254241206501327088318475944106467068195343017578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0163458735700791647771357162355343461968004703521728515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{174248210140386545118}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{134490737362750226432}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{30899}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{72713601301514149888}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{35964662696952610887}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19297801370141650944}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.80197429656982421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.2154952990298237835986583377234637737274169921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29052}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.17984616756439208984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0430088043212890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.57185251083535393323842299651005305349826812744140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{12}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{5781}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.24503311258278159812107332982122898101806640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999147474765777587890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9931591386037157409560904852696694433689117431640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19004}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.980823576450347900390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{17197}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97902488708496082647769753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00395943756393656205727626939960828167386353015899658203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.30697004337046518429588104481808841228485107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21582993}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21582993}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21582993}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{21582993}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{1895}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{29.72185430463576238935274886898696422576904296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{5781}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{12.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{12}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{19.49024512005172482531634159386157989501953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.050464235095853453294534318729347432963550090789794921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8721}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0029531042494006488029201218381558646797202527523040771484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6589}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000489003933974870045007379824636481726159810746288486051069899218646241934038698673248291015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00880362210397386650562179255530281807295978069305419921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{742.548011302947998046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{657.4495183947859686668380163609981536865234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.701404631137847900390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{18146}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{629.87304019927978515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{1185}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{12.8819921960948082784170765080489218235015869140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7273006439208984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.066721864094006377854384481906890869140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{2306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.529174268245697021484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{2743}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{17.24230861663818359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2259865437051112035948818856923026032745838165283203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0292202753293310003857019552242491045035421848297119140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00150280120508911214927127986129562486894428730010986328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{22286}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.004253370341997368166142567957876963191665709018707275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.322361760655513418516449064554763026535511016845703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.2577254981252252719059470109641551971435546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1498784831274729556493952031814842484891414642333984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.10980032109138200546727404116609250195324420928955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.034111988738645702967655637394273071549832820892333984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{380577593469610809267}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{304268563531861917696}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{176945281306130513920}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{129629339032566885507}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{40272328070851813376}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{181.325698852539034078290569595992565155029296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.10632122115583797494764439761638641357421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.661590576171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{81.919342041015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.5543243092486829226572808693163096904754638671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{61}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{40.17218543046357837056348216719925403594970703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{22.25}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{742}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{11}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99985134798959396373874142227577976882457733154296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{14929}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9988344013690948486328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12561}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99870628118515003546207253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0002476659191630442287228308639868146201479248702526092529296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{6.74390732086158717351054292521439492702484130859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20486803}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20486803}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20486803}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20486803}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{97}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{8721}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{65.099337748344368037578533403575420379638671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{27714}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{18.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{22.64255940149356405299840844236314296722412109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0292825759853622517858706686411096598021686077117919921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0015060997247586631331284223733746330253779888153076171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.004262042147376418101123451975809075520373880863189697265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{735.330974578857421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{26278}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{657.4135451301044668070971965789794921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{632.793164730072021484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{7467}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{632.7340095043182373046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{27300}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{12.5390905045677225615463612484745681285858154296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7121655941009521484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.06651733095282708063678001053631305694580078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{20539}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.52286994457244873046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{13293}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{17.2253797054290771484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2247511715773288509812033453272306360304355621337890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0285768838463385001225081083475743071176111698150634765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.001494645720908685353200961998254570062272250652313232421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{17096}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0042155188211468359871236799563121167011559009552001953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.325815042030742407774823732324875891208648681640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.26005030374349191735205977238365449011325836181640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8893}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1516661383060850798454310961460578255355358123779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.112836876057987200994148224708624184131622314453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.034109861104272443110829726720112375915050506591796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{384654508525185752034}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{307013209564584148992}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8893}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{179055772030732075008}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{133214270381988876720}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{40269816203538800640}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{187.469207763671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{104.0375475851905235913363867439329624176025390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1681}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{87.287982940673828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{83.86852264404296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.91771665649914524465202703140676021575927734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{62}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{41.112582781456950442589004524052143096923828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{4800}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{22.25}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{11}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.999840466786694026524173750658519566059112548828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{30899}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99879483878612518310546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99870628118515003546207253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000253406779965420340429427259465455790632404386997222900390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{6.77602224282065179750134120695292949676513671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20509553}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20509553}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20509553}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20509553}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{97}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{8721}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{65.6887417218542992713992134667932987213134765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{18289}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{18.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{18}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{22.089578445506372617046508821658790111541748046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.028637812725032830984961407239097752608358860015869140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00149794158056325787085893974648342918953858315944671630859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{17096}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.004224113883421140754059752708826636080630123615264892578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{675.396580219268798828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{656.858235127089074012474156916141510009765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24202}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{630.730818808078765869140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{18146}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{629.0287520885467529296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{1185}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.8770011345810164726799484924413263797760009765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7255680561065673828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.062060589821921752218258916400372982025146484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{2306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.5524833202362060546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{13293}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{17.2471535205841064453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.21710147366989029915629316747072152793407440185546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0306528878161367000776404978523714817129075527191162109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00180909950881644383292867761525712921866215765476226806640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{16284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000000004870439446712226949642854378907941281795501708984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00526709515489646139252410961262285127304494380950927734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.237693800380067987720877908941474743187427520751953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{15662}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.179167183861139889256008927986840717494487762451171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12561}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0903508533028255234054171296520507894456386566162109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0652425835371920059824191184816299937665462493896484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0272450378496800101058017418154122424311935901641845703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{280619309025185351181}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{15662}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{211523275973997461504}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12561}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{106667460333983924224}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{77024847437964641862}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{32165263391460950016}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{20866}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{20866}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{20866}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{20866}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{32.51659393310546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{29052}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{20.5541418403979179174712044186890125274658203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{913}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{13.2870109081268310546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{11.60878849029541015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.819185726656505242004868705407716333866119384765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{29}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29052}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{18.609271523178808394050065544433891773223876953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1951}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9993904276399423469712246514973230659961700439453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1696}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9957933723926544189453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{3175}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99490654468536376953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000812565928494906404740139027609302502241916954517364501953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{3.642962025193735353667534582200460135936737060546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{24511607}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{24511607}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{24511607}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{24511607}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{89}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{15662}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{46.72185430463576238935274886898696422576904296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{17080}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{15.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{15}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{24.356121370554536298413950135000050067901611328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0307969220286714757961465949165358324535191059112548828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00181341894659774356679537987702133250422775745391845703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{16284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000489003933974870045007379824636481726159810746288486051069899218646241934038698673248291015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00528022093118353692819955114146068808622658252716064453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{725.7835071086883544921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{655.8396139271211495724855922162532806396484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15399}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.630636155605316162109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{19488}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{630.66480255126953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{1185}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{12.2443268798473265945858656778000295162200927734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.648274898529052734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{14095}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.06658491235695151999607332982122898101806640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{14929}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.293848693370819091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{16.9448316097259521484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.23342876112230381835388470790348947048187255859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.139351239401332593903504175614216364920139312744140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.040748210513038569946520084386065718717873096466064453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{6082}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000136885213605954826688909826970519389988112379796802997589111328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000648731722773529976777096203491650196486413559870953804420423693954944610595703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0341965555695179779238657147288904525339603424072265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.148644293062446697373246706774807535111904144287109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1264838735596477692357808564338483847677707672119140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{16069}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0783113816238552029602715265355072915554046630859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0282067606208411987556150535283450153656303882598876953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01341417701254602433402762784453443600796163082122802734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{175488206856987817453}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{149325801280400752640}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{16069}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{92453760951926931456}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{33300665236546994935}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{15836664979831949312}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{36994}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{36994}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{36994}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{36994}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{16284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.0662251655629138014091950026340782642364501953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99883186817169200555355246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99203059807518456647557059113751165568828582763671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{17194}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97751007974147796630859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{27484}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97550213336944580078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0038586772899529726832401621550161507911980152130126953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.232393214600431274874381415429525077342987060546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21929781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21929781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21929781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{21929781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{51.64900662251655916179515770636498928070068359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{11130}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{13.25}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{30371}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{21.440877797680190752771522966213524341583251953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.13963369755367993629846523617743514478206634521484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.040846988064711486909885707063949666917324066162109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{16069}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000001370893036914455728164760790754872488150795106776058673858642578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000651339640814724176840036096506761779706580484106126505139400251209735870361328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0342747435651661047639748858273378573358058929443359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{780.6146526336669921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{660.9286049359681101122987456619739532470703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29565}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{633.450076758861541748046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{19488}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{633.4379966259002685546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{18146}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{15.217239780007677296680412837304174900054931640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7141325473785400390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.089674160180504003392343292944133281707763671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{1283}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.285851776599884033203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{17.08359050750732421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.235568674924320209385086855036206543445587158203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.13907437376533360318120458032353781163692474365234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.040296387115873237572127862904380890540778636932373046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{20415}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000013688518119183754983940459748481544011156074702739715576171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000519075253666131955859153387692143989955335936503644234107923693954944610595703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03423418887748551353578108091824105940759181976318359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1520063574539194106716166743353824131190776824951171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.129780510936628068474618658001418225467205047607421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12552}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08016296219870054640121992406420758925378322601318359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.029248360968963001138565260816903901286423206329345703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01371285102375070785729604949665372259914875030517578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{179457431905872931332}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{153217783744207486976}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12552}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{94639721463672471552}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{34530369879675945874}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{16189277014786263040}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21122}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21122}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21122}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21122}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.456815242767333984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.453065700088905121134530418203212320804595947265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{6204}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.5314728319644927978515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27484}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.4557187557220458984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.485879266046599533890315569806261919438838958740234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{16284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.390728476821191605949934455566108226776123046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99871051311492919921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9928914450651762368948993753292597830295562744140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{9504}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.980971157550811767578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8840}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98077803850173961297542746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0035893437412123688733112114590539931668899953365325927734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.2553119447344729397997298292466439306735992431640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{24004214}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{24004214}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{24004214}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{24004214}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{53.23841059602649039561583776958286762237548828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{6204}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{13.25}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{30371}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{21.02401925306541130566984065808355808258056640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.139356270724566855268022891323198564350605010986328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.040394276588851939224777964909662841819226741790771484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20415}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000137089271147022732594839412693932256814832726377062499523162841796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000521161949400673504359505029474320468682764506684890193355386145412921905517578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.034313265674867345078613567466163658536970615386962890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{752.171185970306396484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{659.38820232460830084164626896381378173828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29110}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{633.653469026088714599609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{18146}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{633.44536876678466796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{13.528129110980732008329141535796225070953369140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.696732044219970703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.10494619489505652154548442922532558441162109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{123}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.366152942180633544921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{16.9774434566497802734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2332322788898751053654478937460226006805896759033203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.1375616653617852958024769804978859610855579376220703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.039162844522316185569277280364985927008092403411865234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{20415}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000001754969311736445063295288142378273998911453190885367803275585174560546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000131019965994680527565652283783492748625576496124267578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03361600768810847628120797025985666550695896148681640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.163877956248932310501231768284924328327178955078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1404155560679425096548555984554695896804332733154296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.086205934776560189103378206709749065339565277099609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.03287080436427759766448986056275316514074802398681640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01464640612632706236084789708229436655528843402862548828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{193472941967784025830}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{165773428912188882944}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{101774004253318709248}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{38806996198707473791}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17291424346365882368}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{20930}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{20930}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{20930}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{20930}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.5789470672607421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.1628587988038727729644961073063313961029052734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11611}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.62857162952423095703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.099677562713623046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.2070768017832402829725424453499726951122283935546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{16284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10.377483443708609200939463335089385509490966796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1412}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999390661716461181640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99450029561061736860239079760503955185413360595703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6155}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.982523381710052490234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12141}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98241913318634044305355246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{27484}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0029758842906757823100483140166261364356614649295806884765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.42234635853338264865897144773043692111968994140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22959702}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22959702}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22959702}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{22959702}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{55.4701986754966895887264399789273738861083984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{14}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{30371}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{20.693860607628177916694767191074788570404052734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.137854961092239547415516653927625156939029693603515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.039259086789361574698631329738418571650981903076171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20415}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000001757585974611265939841365577695452004913789778584032319486141204833984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000013154666959353237424396244541559598353907580003951949265683651901781558990478515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.033695018358024748927892488836732809431850910186767578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{788.6509425640106201171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{660.403959133767102684942074120044708251953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{13468}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{634.02910900115966796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{629.5899829864501953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19488}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{15.8816467625376223082866999902762472629547119140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{19.41299343109130859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{2236}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.08849855448236354504842893220484256744384765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{32103}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.3971350193023681640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{16.93804168701171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.25174860301297508069495734162046574056148529052734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.137044187230735692306637929505086503922939300537109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0396769886006985983417649777038604952394962310791015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{20415}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000001755034024917878262043691332881627242823441292784991674125194549560546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000003898726917274755211784142971964683965779840946197509765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03407954699543140619777403799162129871547222137451171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1602809018407846952669615347986109554767608642578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1368001673134138507226253977933083660900592803955078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12457}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08448987649388146892182049896291573531925678253173828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.031398386826338199606656331752674304880201816558837890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01438849056680072992231433914867011480964720249176025390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{189226289674260354802}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{161505131242956357632}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12457}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{99748040224125501440}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{37068672391218938521}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{16986931397936451584}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{20930}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{20930}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{20930}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{20930}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.7125339508056640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.21119032790329317350597193581052124500274658203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{123}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.18486309051513671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5706513486772113452616395079530775547027587890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{16284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999166429042816162109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9939166074557019836532845147303305566310882568359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{24202}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.984259426593780517578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12141}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98299252986907958984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{16149}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0031390800339772596296017415085088941850699484348297119140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.3617285470172053596371597450342960655689239501953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21971988}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21971988}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21971988}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{21971988}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{54.21854304635761678810013108886778354644775390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{7310}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{14}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{30371}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{21.126517043294132491837444831617176532745361328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.13732196910107596909966787279699929058551788330078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.03977411184360142570870522149562020786106586456298828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20415}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000001757650947941335967484443938437486953940691591924405656754970550537109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000000003914399898737385943644416507947746524114125687976439849080634303390979766845703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.034158968978531711879753629546030424535274505615234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{784.167726993560791015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{662.5702354781675467165769077837467193603515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{635.94926869869232177734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{25516}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{628.778150081634521484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19488}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{15.291387472057412111325902515091001987457275390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{19.8672397136688232421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{2236}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.104317811940678240034685586579144001007080078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{19451}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.46715915203094482421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{16.9722197055816650390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.27851244194490598626856581176980398595333099365234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.100856837906966700924016322460374794900417327880859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0199163673888338339790227138337286305613815784454345703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{5358}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000187040546005187846494524119000946171809118823148310184478759765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{17194}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000533630756770209213613043175428174436092376708984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.017516335434457859510093413746290025301277637481689453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.354957249884903902614752269073505885899066925048828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.31004932896993186997036673346883617341518402099609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2006096076406851391737973244744352996349334716796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1172206527621340033107344424934126436710357666015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.028631326288479620745253129143748083151876926422119140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{419059554927013948075}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{366041639790957821952}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{236838021816000479232}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{138389720426000753247}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{33801903906205171712}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{20930}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{20930}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{20930}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{20930}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{179.824432373046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.302513274135975507306284271180629730224609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.872837066650390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{82.67822265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.48188325228561978974539670161902904510498046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{63}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{26278}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{46.79470198675496561691034003160893917083740234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{24}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{12}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{3175}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9995334760242740035351971528143621981143951416015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{16069}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99705474078655242919921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{2345}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99423247575759876593082253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0006110186939828851117317842778220438049174845218658447265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{7.29993003758064862296350838732905685901641845703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20905172}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20905172}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20905172}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20905172}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{94}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{12561}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{80.781456953642390317327226512134075164794921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{23.25}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{18}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{11.0044506587619874693473320803605020046234130859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.1010612697886577870942659274078323505818843841552734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0199686943073143531590663002361907274462282657623291015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000001873194885872688614678548656156120699733946821652352809906005859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{17194}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005344263761436997529279012658514590476591514624012750601066146227680064839660190045833587646484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0175547366062119535035090933661194867454469203948974609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{784.6767780780792236328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{662.2082252234023371784132905304431915283203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{32382}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{634.81941068172454833984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{25516}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{631.178431034088134765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19488}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{15.3806435158122667417046613991260528564453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{19.170210123062137341776178800500929355621337890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{2236}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.10175158014360619063154445029795169830322265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{26374}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.505578100681304931640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{16.9834988117218017578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2353374871126442113844490222618333064019680023193359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.13796103983449270469208158829133026301860809326171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.039167248323213423033539726247909129597246646881103515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{20415}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000001754969311736445063295288142378273998911453190885367803275585174560546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000131019965994680527565652283783492748625576496124267578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.033589817201248949041225699829738005064427852630615234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1639529697074205982776362588992924429476261138916015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1403966501208600281547234089885023422539234161376953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0862010170418282262172482433015829883515834808349609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.03284857946169329745433884681915515102446079254150390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0146276338901141327031307781680879998020827770233154296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{193561502228316401082}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{165751108709481414656}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{101768198416901242880}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{38780757664945213663}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17269262001590771712}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.6250514984130859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.251300483349933045928992214612662792205810546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{9134}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.6317813396453857421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.075281620025634765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.219462901648069586002520736656151711940765380859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{16284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10.364238410596026795928992214612662792205810546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1412}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999390661716461181640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99444573604507946473773927209549583494663238525390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{24566}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98251344263553608282535378748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12141}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98237329721450794561832253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{27484}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0029811211274613550435697018059499896480701863765716552734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.41647563619308325399970271973870694637298583984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22976341}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22976341}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22976341}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{22976341}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{54.89403973509934075991623103618621826171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{14}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{30371}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{20.7355318802300558900242322124540805816650390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.1382551870727226905888329611116205342113971710205078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.03926357954086144574912253801812767051160335540771484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20415}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000001757585974611265939841365577695452004913789778584032319486141204833984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000013154666959353237424396244541559598353907580003951949265683651901781558990478515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0336688434085077592516910272024688310921192169189453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{796.67212677001953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{662.1664063946300302632153034210205078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24144}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{635.19404828548431396484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{631.657144069671630859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19488}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{16.132520678780213785330488462932407855987548828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7758071422576904296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.096110118145976031200916622765362262725830078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{2345}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.44157505035400390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{16.858488559722900390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.23656661143626001031492478432483039796352386474609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.137044187230735692306637929505086503922939300537109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.039701534113782847856821689447315293364226818084716796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000001755034024917878262043691332881627242823441292784991674125194549560546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000003898726917274755211784142971964683965779840946197509765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.034066858018901115257026646077065379358828067779541015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1603697674222356039930303950313827954232692718505859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.136849879588164469179645266194711439311504364013671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12457}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08453292397641894162507725241084699518978595733642578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.03141726163182249897953823847274179570376873016357421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0143876970152147752590732210364876664243638515472412109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{189331203635091448807}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{161563821137973837824}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12457}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{99798861721302237184}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{37090955828416380250}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{16985994537583470592}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.80197429656982421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.2154952990298237835986583377234637737274169921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29052}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.17984616756439208984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0430088043212890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.57185251083535393323842299651005305349826812744140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{16284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999166429042816162109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9939067411106943250587164584430865943431854248046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{12552}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98423142731189727783203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12141}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.982880532741546630859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{16149}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0031536986689235367055383907342047677957452833652496337890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.3617285470172053596371597450342960655689239501953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22021905}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22021905}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22021905}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{22021905}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{54.27814569536423761064725113101303577423095703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{7310}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{14}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{30371}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{21.120016224029665607986316899769008159637451171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.13732196910107596909966787279699929058551788330078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.039798716918060424163616772830209811218082904815673828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000001757650947941335967484443938437486953940691591924405656754970550537109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000000003914399898737385943644416507947746524114125687976439849080634303390979766845703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.034146246905317596820328418516510282643139362335205078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{792.7619025707244873046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{662.2143998177635921820183284580707550048828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29726}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{634.472433507442474365234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{18146}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{632.18463993072509765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19488}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{15.7128509045096773633076736587099730968475341796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.77601146697998046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.1041661887768867700287955813109874725341796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.496837139129638671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{17.3820765018463134765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.230814349563272458443208279277314431965351104736328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.100812220387155593304129297393956221640110015869140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0199540988039031107204035464519620290957391262054443359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{9504}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000187040546005187846494524119000946171809118823148310184478759765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{17194}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000533630756770209213613043175428174436092376708984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0176184544391382903738563214801615686155855655670166015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.354860030235562506906177304699667729437351226806640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.310011593574422594787876050759223289787769317626953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.200453156247775654552611968028941191732883453369140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.11702431905780209808742853283547447063028812408447265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.02863697920306358668529611577469040639698505401611328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{418944778223632303648}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{365997089699215179776}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{236653316612482007040}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{138157930499802064776}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{33808577689795645440}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{181.325698852539034078290569595992565155029296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.10632122115583797494764439761638641357421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.661590576171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{81.919342041015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.5543243092486829226572808693163096904754638671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{62}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{46.64900662251655916179515770636498928070068359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{24}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{12}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{3175}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99954295671538806455913572790450416505336761474609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99703395366668701171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{2345}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99423372745513916015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000611977401887890790251056660764561456744559109210968017578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{7.2743754885419900091392264585010707378387451171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20925715}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20925715}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20925715}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20925715}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{94}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{12561}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{80.754966887417225507306284271180629730224609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{23.25}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{18}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.9634956523653244175875443033874034881591796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.101016561831314410913051915485993959009647369384765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0200066322399416740562827499161357991397380828857421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000001873194885872688614678548656156120699733946821652352809906005859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{17194}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005344263761436997529279012658514590476591514624012750601066146227680064839660190045833587646484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.017657390183765171720597919602369074709713459014892578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{752.81760120391845703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{661.75480697960256293299607932567596435546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29565}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{635.490290701389312744140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{18146}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{632.9736850261688232421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19488}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{13.6574015768991952057831440470181405544281005859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.73948192596435546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.101531112430901515608638874255120754241943359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{23241}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.47921526432037353515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{16.9763543605804443359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2331107304606203356467375442662159912288188934326171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.10188734729641009402190121591047500260174274444580078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0198046564382910218748978792291381978429853916168212890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000018704054600541082791788881356520590770742273889482021331787109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{17194}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000000000000000094528876913579917840024791075848042964935302734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0175186383111476072504952838926328695379197597503662109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.355984989885878400084351369514479301869869232177734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.312705213434710860287424338821438141167163848876953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2025084096510781639377540841451263986527919769287109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.11994612649562709505435265100459218956530094146728515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.028519016048116886674623771114056580699980258941650390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{420272896160440491669}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{369177154735669248000}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{239079731558871859200}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{141607391878248033795}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{33669311377512173568}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{187.469207763671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{104.0375475851905235913363867439329624176025390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1681}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{87.287982940673828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{83.86852264404296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.91771665649914524465202703140676021575927734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{64}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{47.953642384105961582463351078331470489501953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{11130}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{25.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{12}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99952304284304183124021392359281890094280242919921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{16069}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99698466062545765264957253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{2345}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9940254688262939453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000627411909087625843488289500982091340119950473308563232421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{7.4880370360707910748487847740761935710906982421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20948465}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20948465}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20948465}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20948465}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{94}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{12561}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{81.14569536423840645511518232524394989013671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{23.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{19}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{11.174946761058645705588787677697837352752685546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.10209386797027387994152292094440781511366367340087890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.019856303818331207111658187614011694677174091339111328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000001873194885874921605285747805424989564926363527774810791015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{17194}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000000000000009466981520259823850806760925933729369966050443799851325799021850571079994551837444305419921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.01755701227072996306599605986775713972747325897216796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{779.036859035491943359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{662.1324333876174250690382905304431915283203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29565}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{634.21438491344451904296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{25516}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{628.3896694183349609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19488}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{14.92210795938914458247381844557821750640869140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7862262725830078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.1007343270131286772084422409534454345703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{15662}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.28553402423858642578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{16.999635219573974609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.240941633713150527018598268114146776497364044189453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.12247251675556160288582674411372863687574863433837890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.028867135891292521054918296385949361138045787811279296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{26829}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000002136005334738532265231531143536057728998685288225698082620329643077639047987759113311767578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{12457}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000542101086242752217003726400434970855712890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{17194}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0251100414196918954312653937677168869413435459136962890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.268575512738986110772287929648882709443569183349609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{29052}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.2162773072658783213295663472308660857379436492919921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4305}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1323343506233651545311857944398070685565471649169921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0678287546396220963895729028081404976546764373779296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0260283980058033936888506332252291031181812286376953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{317077999869529422315}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{29052}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{255335176709420941312}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4305}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{156232825479024836608}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{80078059371235152446}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{30728908586349264896}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{20866}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{20866}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{20866}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{20866}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{32.51659393310546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{29052}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{20.5541418403979179174712044186890125274658203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{913}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{13.2870109081268310546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{11.60878849029541015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.819185726656505242004868705407716333866119384765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{34}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29052}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{20.5496688741721840187892667017877101898193359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{10.25}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{14095}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99930860388357911627821295041940174996852874755859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{2345}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99439324438571929931640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99042558670043956414730246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00100802820254239085089043026499666666495613753795623779296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{4.0308228692090235512068829848431050777435302734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{24950519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{24950519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{24950519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{24950519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{87}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{69.6821192052980080688939779065549373626708984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{18.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{15}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.0950063498172095677318793605081737041473388671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.12272076256194784649178330937502323649823665618896484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0289386116878821049447356728023805771954357624053955078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{26829}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000002143577083097822707746744324391545771713120513416090708036509937528535374440252780914306640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12457}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000000005429095477232981377592459938814332407252295885837921514405213230247682076878845691680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17194}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0251740852604009253401518009241044637747108936309814453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{786.0553302764892578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{655.38345502228139594080857932567596435546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{6532}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{627.9288542270660400390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{19488}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{625.7197854518890380859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{15.7804174311630713845033824327401816844940185546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.5986340045928955078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{9816}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.08963492532439687465739552862942218780517578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{20751}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.47345077991485595703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{17.0148355960845947265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2297023263314471874796396377860219217836856842041015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.51964274614739702773391627488308586180210113525390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.38955445210794403809728692067437805235385894775390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{8299}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.14341431613405586364962118750554509460926055908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0279024373481712995026526868969085626304149627685546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06963865698527742231771497927184100262820720672607421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1627698823941876871135292503822711296379566192626953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1304397629020544180367124909025733359158039093017578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09823438720163236992366506683538318611681461334228515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07979498280770259965866131324219168163836002349853515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01198815864061388014594200512874522246420383453369140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{192164759259736501104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{153996091090531385344}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{115974694396556951552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{94205288078063618209}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{14153119638939777024}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{33152}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{33152}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{33152}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{33152}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.5298013245033104112735600210726261138916015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{913}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99922949075698841436832253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{24144}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99389402558471984239218954826355911791324615478515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97873948514461517333984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{28778}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.978678286075592041015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004085034189272830455752494316357115167193114757537841796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.3944447351790045797059747201274149119853973388671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22551893}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22551893}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22551893}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{22551893}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{78}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{71}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{63.25}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{61}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{7790}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.66694259058138616325095426873303949832916259765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.5207267918467237688417981189559213817119598388671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3905584325115964983154981382540427148342132568359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1438922904165245986174426207071519456803798675537109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.028880760646304903804804098399472422897815704345703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0697582308546664808801551771466620266437530517578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{681.20822429656982421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{11598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{658.10931040277546344441361725330352783203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{630.21872711181640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{627.768654346466064453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.0437993266756535604145028628408908843994140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.6160867214202880859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{9816}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.07825277814801978593095554970204830169677734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{23241}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.568316996097564697265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{17.296329021453857421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.218076149395388718676969119769637472927570343017578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.51907427358312452359001554214046336710453033447265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.386755721138959784877187075835536234080791473388671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.135055154466115989730923274692031554877758026123046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.022678887213608500683648117046686820685863494873046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06893592028232252422181858264593756757676601409912109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1693897604022681913082948312876396812498569488525390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1350263276260359746050454532451112754642963409423828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{17096}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.10188278973601468113674428650483605451881885528564453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08483897611865330590230627194614498876035213470458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01210435263263198550631738470428899745456874370574951171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{199980131766247815319}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{159410950971541946368}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{17096}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{120281967857652842496}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{100160184315926721366}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{14290297292294062080}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17280}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17280}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17280}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17280}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.456815242767333984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.453065700088905121134530418203212320804595947265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.5314728319644927978515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27484}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.4557187557220458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.485879266046599533890315569806261919438838958740234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.75496688741721840187892667017877101898193359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{913}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{9816}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{9816}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99954187870025634765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9940559942990738750978607640718109905719757080078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98253071308135986328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12141}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.981816351413726806640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{30684}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0038037521186260283591329400820768569246865808963775634765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.441884746233246250568527102586813271045684814453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{24626326}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{24626326}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{24626326}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{24626326}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{76}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{12141}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{71.192052980132444872651831246912479400634765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{64.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{8299}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{64}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.52068326642667184245283351629041135311126708984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.5201571333710861555488236263045109808444976806640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3877529190446449280926799474400468170642852783203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1354752759401780248804669781748089008033275604248046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0234740608918058875353995773593851481564342975616455078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0690685317660602871026043203528388403356075286865234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{682.7972066402435302734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{658.1102995083032283218926750123500823974609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{9816}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{628.517288148403167724609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{628.0473678112030029296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.2208195662913094992063633981160819530487060546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7324793338775634765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.078507349191124120579843292944133281707763671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{26374}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.4959456920623779296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{17.2436707019805908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.22387076095809821385529403414693661034107208251953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.508877498332698241512161985156126320362091064453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.376215934674731133924296955228783190250396728515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{6159}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.181921064205671723090773639341932721436023712158203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0121155986045065992839919744028520653955638408660888671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0641783501064826233939442090559168718755245208740234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.185960612979202688510582675007754005491733551025390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1491451419807580947018976758045027963817119598388671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1140704651170702244034060868216329254209995269775390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.09211248577998409903244692031876184046268463134765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01239729359138443988419542307610754505731165409088134765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{219543541466720215193}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{176079504893191618560}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{134670635288550916096}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{108747228875300989500}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{14636140933562128384}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.5789470672607421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.1628587988038727729644961073063313961029052734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.62857162952423095703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.099677562713623046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.2070768017832402829725424453499726951122283935546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{15}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.8079470198675497982776505523361265659332275390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{913}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99966651201248157843082253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99544361648180623713955128550878725945949554443359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98250775039196014404296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8745}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98191636800766002313167746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.003325601494959806725404405369772575795650482177734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.5725932174776418026596047639031894505023956298828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{23581814}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{23581814}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{23581814}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{23581814}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{79}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{29726}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{71.5960264900662224363259156234562397003173828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{62.25}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{57}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{13293}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.6121945505951895682983376900665462017059326171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.50963088012770685342189835864701308310031890869140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3771831289949127974381326566799543797969818115234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6159}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1823313167491538155928765263524837791919708251953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.01254039921377669321300718507927740574814379215240478515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0643033254832701961500873721888638101518154144287109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{701.895977020263671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{658.6397947554556822069571353495121002197265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{627.50271093845367431640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{626.57549381256103515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.374554542505705967414542101323604583740234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{19.613144874572750353536321199499070644378662109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.08454474550209312155857332982122898101806640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.512328565120697021484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{2743}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{16.9913461208343505859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.25537503258655736004811842576600611209869384765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.49896401224910580385341063447413034737110137939453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.380235533436785566596682883755420334637165069580078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.157412588466392999730913970779511146247386932373046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0112372670130452996517522734620797564275562763214111328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06542823519886782623888876742057618685066699981689453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.180951771726883203772473507342510856688022613525390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.14416660540370174192759122888674028217792510986328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.108588696735633150058930596060235984623432159423828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0897312954051767974750219991619815118610858917236328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01238184714564041603857003082111987168900668621063232421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{213630145454728070232}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{170201886326883844096}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{128198905470712676352}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{105936015471470476084}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{14617904989146871808}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.7125339508056640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.21119032790329317350597193581052124500274658203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.18486309051513671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5706513486772113452616395079530775547027587890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.4701986754966895887264399789273738861083984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{9816}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9996178150177001953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12493}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99498137575111644803627086730557493865489959716796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98326486349105823858707253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.981899797916412353515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{9816}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.003673362781168954503685508683474836288951337337493896484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.55605183445842332190522938617505133152008056640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22594100}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22594100}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22594100}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{22594100}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{78}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{29726}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{71.4437086092715247787054977379739284515380859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{62.25}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{60}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{13293}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.620944073348618008623134301160462200641632080078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.499702717348907976546712461640709079802036285400390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.38121327810822414061675544871832244098186492919921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8299}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1577755554897531109492803125249338336288928985595703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0116312713069723662473453629218056448735296726226806640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0655617055455517683260069361494970507919788360595703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{681.4738533496856689453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{11598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{659.0167422626192319512483663856983184814453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7310}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{630.006680309772491455078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{626.772342681884765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.241017566746478451022994704544544219970703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.1405866146087646484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.092187985679171191577552235685288906097412109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.540303766727447509765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{17.13799762725830078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.271784416137703044302753596639377065002918243408203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.308551361814407176797914189592120237648487091064453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.2199361842395977928443784321643761359155178070068359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{28778}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0987295156740346235846317313189501874148845672607421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0479751517156739026859213481657207012176513671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.038957887212757037753707578531248145736753940582275390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.41886796257298020140780181463924236595630645751953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24173}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.368865974093988080451111954971565864980220794677734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{24262}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.30755724717754795438651171934907324612140655517578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.271110291607196407515090186279849149286746978759765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0198776371229890495839764952279438148252665996551513671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{494512006800634757674}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24173}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{435480078183127842816}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{24262}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{363099508908726812672}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{320070538561710004697}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{23467371827062218752}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{179.824432373046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.302513274135975507306284271180629730224609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.872837066650390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{82.67822265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.48188325228561978974539670161902904510498046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{72}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{48.78145695364238321189986891113221645355224609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{2743}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{31}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{28}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999981582164764404296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{28778}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9986324515563762549419379865867085754871368408203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99631531536579132080078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24144}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.995577752590179443359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0007279845028552432185942056008798317634500563144683837890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{8.0271839797962769580408348701894283294677734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21527284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21527284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21527284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{21527284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{98}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{83.0264900662251648100209422409534454345703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{913}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{77}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{7467}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{77}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{7467}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.835318919580146701520106944371946156024932861328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.30934926711540045030091050648479722440242767333984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.2205150524836787251370395779304089955985546112060546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{32103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.099283364870893731080059296800754964351654052734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.04965727030872986447196382187030394561588764190673828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0390299029273804831685623639714322052896022796630859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{682.97449207305908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{658.5832338001554262518766336143016815185546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{628.954491198062896728515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{627.0692188739776611328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.15856379527809849605546332895755767822265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.1551911830902099609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.090014418229362291867801104672253131866455078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.527098834514617919921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{13293}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{17.1117045879364013671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2782893384387092883258674191893078386783599853515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.510965817105864861247255248599685728549957275390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.3761555114834973512216720337164588272571563720703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.18224425780521558149160910033970139920711517333984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.011867025872923299412153852472329162992537021636962890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0643949229704894043901930444917525164783000946044921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1860487978698892874707127020883490331470966339111328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1491677256185719446790471920394338667392730712890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.11413213878014967506135945995993097312748432159423828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.09213859760284670574748133731191046535968780517578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01238147448068043464386445151603766134940087795257568359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{219647651809738648049}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{176106166946760065024}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{134743446698401464320}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{108778056274574200054}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{14617465024017778688}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.6250514984130859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.251300483349933045928992214612662792205810546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{9134}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.6317813396453857421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.075281620025634765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.219462901648069586002520736656151711940765380859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{15}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.8079470198675497982776505523361265659332275390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{913}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99966651201248157843082253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99546768531104590227442940886248834431171417236328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98244546353816986083984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8745}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98187714815139759405582253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0032437881393160045324919327214274744619615375995635986328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.5599084358765846758387851878069341182708740234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{23598453}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{23598453}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{23598453}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{23598453}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{79}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{29726}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{71.6026490066225136388311511836946010589599609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{62.25}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{57}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{13293}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.617008732239580748313301228336058557033538818359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.51172229061027518781656908686272799968719482421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.377122281421495786357667157062678597867488861083984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{28090}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1826529864005644043789544639366795308887958526611328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.01228311095345466057160432882255918229930102825164794921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06451945423655232325632624679201398976147174835205078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{683.085255146026611328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{658.2274134048562928001047112047672271728515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{628.783144295215606689453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{628.3475801944732666015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.10789569555615940998904989100992679595947265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{19.1226253509521484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.079596435786871921891361125744879245758056640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.522834241390228271484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{17.20862293243408203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2352197231263667143164042272474034689366817474365234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.498790295918692783150305558592663146555423736572265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.380189337169404673044681430837954394519329071044921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.157220334144946238819073869308340363204479217529296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.01123726701293419928673333885171814472414553165435791015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06546807247078882674440336586485500447452068328857421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.180963589091474197356745889919693581759929656982421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1442292993889058294598726206459105014801025390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1086882833952010629641193872885196469724178314208984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0900047976864891963177939260276616550981998443603515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01238166308290343693709889549836589139886200428009033203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{213644096936343185607}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{170275902320485105664}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{128316476646533824512}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{106258909973035077869}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{14617687686221905920}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.80197429656982421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.2154952990298237835986583377234637737274169921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29052}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.17984616756439208984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0430088043212890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.57185251083535393323842299651005305349826812744140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.4701986754966895887264399789273738861083984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{9816}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99961817264556884765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12493}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9949729584700224283011493753292597830295562744140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9832576811313629150390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.981780588626861572265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{9816}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0036788329416188891331229715575545924366451799869537353515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.55605183445842332190522938617505133152008056640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22644017}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22644017}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22644017}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{22644017}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{78}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{29726}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{71.4437086092715247787054977379739284515380859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{62.25}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{60}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{13293}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.620944073348618008623134301160462200641632080078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.499528743835339350543023329009884037077426910400390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3811668336266933465594775043427944183349609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8299}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.15758297229608186906801847726455889642238616943359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.01163127130685736969339938440270998398773372173309326171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06560076690903891838413386494721635244786739349365234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{681.0834596157073974609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{19093}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{658.2113600124586128004011698067188262939453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{630.570782244205474853515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{627.1015317440032958984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.377271019109929994783669826574623584747314453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.643939971923828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{11598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.082131808956727780923756654374301433563232421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.5153615474700927734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{17.1542510986328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.225029855994581973188672918695374391973018646240234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.3079562246930704905167885954142548143863677978515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.2199816469863092593950426589799462817609310150146484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.09805795600285165114495811167216743342578411102294921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.046660543670478997480000060704696807079017162322998046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0390811566311729807754460352953174151480197906494140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.419049796119869200072827197800506837666034698486328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24173}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.368808915533745340642468590885982848703861236572265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8721}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.307620827678796004978067912816186435520648956298828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.27106370375391819482757682635565288364887237548828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01986387039205529669860794683700078167021274566650390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{494726677962457137856}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24173}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{435412715325015326720}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8721}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{363174571515741339648}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{320015537332502498471}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{23451118939877171200}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{181.325698852539034078290569595992565155029296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.10632122115583797494764439761638641357421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.661590576171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{81.919342041015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.5543243092486829226572808693163096904754638671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{72}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{48.69536423841059757933180662803351879119873046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{2743}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{31}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{28}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{28778}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9986343083792175168156290965271182358264923095703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{13716}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99627822637557972296207253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24144}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.995532929897308349609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000729195831080830104801993041263585837441496551036834716796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{7.95017045715335424205250092200003564357757568359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21547827}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21547827}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21547827}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{21547827}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{98}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{83.006622516556291202505235560238361358642578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{77}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{2743}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{77}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{2743}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.794262543524142383688513291417621076107025146484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.308752590985902741760327216979931108653545379638671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.220560437698301026188119067228399217128753662109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0985997548324924200091601278472808189690113067626953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.048296569097462056785463602182062459178268909454345703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.039153682610227190374896366620305343531072139739990234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{682.419497013092041015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{658.4193582708472831654944457113742828369140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{629.52395498752593994140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{628.8319633007049560546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.3316159620083194425887995748780667781829833984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.6654179096221923828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{11598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.08159810975687520340215996839106082916259765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.501714408397674560546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{17.206445217132568359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2248958550230225894583924173275590874254703521728515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.301223708812563495396119606084539555013179779052734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.21691324511490617243936185332131572067737579345703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{29052}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.09588103913782462794923588944584480486810207366943359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.04772358944407530112474802308497601188719272613525390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.038345361846411012141100371763968723826110363006591796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.42212692218527170240349732921458780765533447265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24173}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.372094848158686819505902576565858907997608184814453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7467}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.311587412274643427156917141473968513309955596923828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.27577414903795627321159145139972679316997528076171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01971213827396522955126556553295813500881195068359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{498359507211162560119}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24173}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{439292059848263532544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7467}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{367857488052465500160}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{325576649564685789205}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{23271985272666333184}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{187.469207763671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{104.0375475851905235913363867439329624176025390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{87.287982940673828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{83.86852264404296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.91771665649914524465202703140676021575927734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{49.927152317880796772442408837378025054931640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{32.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{28}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99999839067459117547542746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{32103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99863009144928283067343954826355911791324615478515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{27484}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.996274471282958984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24144}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.995470702648162841796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000735848522752487015086142463360374676994979381561279296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{8.21974632449511233289740630425512790679931640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21570577}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21570577}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21570577}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{21570577}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{98}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{83.14569536423840645511518232524394989013671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{78}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{78}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.810569810939400614557825974770821630954742431640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.302002665005247472596039415293489582836627960205078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.2174846238478379822911534802187816239893436431884765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29052}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.096428401585535949980254599722684361040592193603515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.049396887688279107753164254290823009796440601348876953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03841770797723763342101932494188076816499233245849609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{681.2555217742919921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{658.085988126843176360125653445720672607421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{629.831108987331390380859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{629.1987326145172119140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.0945049180755024309519285452552139759063720703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.2577378749847412109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.088182335657787547233965597115457057952880859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.509420096874237060546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{17.331598758697509765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.27712624297957966224004167088423855602741241455078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.427951300109888410627689836474019102752208709716796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{8745}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.3200118060092094207647051007370464503765106201171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.14494691887978861100094718494801782071590423583984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.06846373641098850437725076290007564239203929901123046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.053492472191800581604592679241250152699649333953857421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.30873380857318777348297089702100493013858795166015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.2427165847552593402891574214663705788552761077880859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1871000936731276043101246386868297122418880462646484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1626555186369174899052580940406187437474727630615234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.024260219144782817213279457746466505341231822967529296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{364488547433678776533}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{286549166171206549504}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{220888802825937223680}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{192029742366189625381}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{28641411439098707968}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17024}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17024}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17024}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17024}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{32.51659393310546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{29052}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{20.5541418403979179174712044186890125274658203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{913}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{13.2870109081268310546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{11.60878849029541015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.819185726656505242004868705407716333866119384765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{31}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{19.880794701986754802192081115208566188812255859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{12}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{12}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999854266643524169921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.998742197523053931718095554970204830169677734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9958427846431732177734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99471044540405284539730246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000800172248977597147349960504669752481277100741863250732421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{3.968296801009103536017619262565858662128448486328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{25572631}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{25572631}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{25572631}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{25572631}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{82}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{19451}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{75.754966887417225507306284271180629730224609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{69.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{69}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.563025135769385176587320529506541788578033447265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.4301356374158056272705152878188528120517730712890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12141}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.32084368118427841753970142235630191862583160400390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1457435288428090558454641723074018955230712890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0708642316642298097928431843683938495814800262451171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.05353437950664975686354551953627378679811954498291015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{681.593090057373046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{658.9193665507613104637130163609981536865234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{629.26385021209716796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{628.0225331783294677734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.8675803152799996809108051820658147335052490234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{19.627625465393062853536321199499070644378662109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.09035527311413460438416223041713237762451171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.539674282073974609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{17.05085849761962890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2479795858066794755902861879803822375833988189697265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.680767187184961652945958121563307940959930419921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.60759627067880994655268978021922521293163299560546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.455491427068714871406740485326736234128475189208984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.423659542949948619838806962434318847954273223876953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03865002500465190837797280209997552447021007537841796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.155265769210378212772383221818017773330211639404296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1237560565241763443911082731574424542486667633056640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{15662}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0943357552755732797766796693395008333027362823486328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07497542497862159927013436799825285561382770538330078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0113950841549956306819613160996595979668200016021728515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{183305466114015978092}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{146105363345473028096}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{15662}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{111372002212390158336}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{88515358489487607977}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{13452940870757582848}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{33152}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{33152}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{33152}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{33152}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{12}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.1854304635761589992171138874255120754241943359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9997761249542236328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99468359134055128745188767425133846700191497802734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98252689838409423828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98046857118606556280582253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0037747067255092512684522265686837272369302809238433837890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.304114596546743332083906352636404335498809814453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22990805}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22990805}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22990805}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{22990805}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{76}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{12493}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{70.0794701986754944300628267228603363037109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{63.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{31308}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{63}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.245003809220936563662007756647653877735137939453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6825276323316076254599238382070325314998626708984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.60924168728638161685040586235118098556995391845703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.46061035190664423311091013601981103420257568359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.438514015918480659639300256458227522671222686767578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.038251416105634129805057597195627749897539615631103515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{686.4096052646636962890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{663.67792002886335467337630689144134521484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15662}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{632.55606555938720703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{632.43523883819580078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{4157}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.411990586775470291058809380047023296356201171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.2153475284576416015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.14607735659112819348592893220484256744384765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.56362831592559814453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{2743}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{17.107997894287109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.27627130381748699061716934011201374232769012451171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.68038816921901246193016277175047434866428375244140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.60091643278617146162190465474850498139858245849609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{10248}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.444868866995615730441926416460773907601833343505859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.401798419961026997970776619695243425667285919189453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03926536326169381696526983205330907367169857025146484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.160219550770174190557071369767072610557079315185546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1284009849813992631961667711948393844068050384521484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09751985967621712436681491453782655298709869384765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.080242451670031800237126162755885161459445953369140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01152306618200052250322595881470988388173282146453857421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{189153859114375575160}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{151589126960902144000}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{115131129187279781888}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{94733566067461473522}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{13604035379441985536}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17280}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17280}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17280}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17280}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.456815242767333984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.453065700088905121134530418203212320804595947265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.5314728319644927978515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27484}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.4557187557220458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.485879266046599533890315569806261919438838958740234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{12}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.4503311258278142048538938979618251323699951171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999747216701507568359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99500437090728455213906045173644088208675384521484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98161974549293506964176003748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98119032382965076788394753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0034257539969047255679068797462605289183557033538818359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.300477455479329247367559219128452241420745849609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{25065238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{25065238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{25065238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{25065238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{76}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{12493}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{70.22516556291390088517800904810428619384765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{65.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{2743}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{65}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.196240573049347943879183731041848659515380859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.68214763423566504574324653731309808790683746337890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6025427987444957889096031067310832440853118896484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{7790}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.449775434191029166441921915975399315357208251953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.41588639193623888612449945867410860955715179443359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.038906116117155449540820910669935983605682849884033203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{682.5902297496795654296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{14929}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{662.1717223710571715855621732771396636962890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.49178421497344970703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{629.673713207244873046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.0903402709498788425435122917406260967254638671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.037389039993289685526178800500929355621337890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.145127999072041546924083377234637737274169921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.552028238773345947265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{17.0904674530029296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.264398377777001869493034291735966689884662628173828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.64832059939999464592830236142617650330066680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5829069329997829118639174339477904140949249267578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.4638852247966311903581981823663227260112762451171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.400045334271777408563508515726425684988498687744140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.035713819688643004546246828567745978944003582000732421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.176898499669420006252806842894642613828182220458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.142652837533394138969100595204508863389492034912109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1089240563290739538526707974597229622304439544677734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0896609235613747002080486936392844654619693756103515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01186826045661442015355380164010057342238724231719970703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{208844886427199051515}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{168414744663487447040}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{128594828196656087040}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{105852935062343310475}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{14011568847570774016}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.5789470672607421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.1628587988038727729644961073063313961029052734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.62857162952423095703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.099677562713623046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.2070768017832402829725424453499726951122283935546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.3377483443708602095512105734087526798248291015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999593198299407958984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99573564608365494610353607640718109905719757080078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{32103}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9865696728229522705078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.986216247081756591796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.002889998381292800677666576802948839031159877777099609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.413686258450472355008287195232696831226348876953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{24020726}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{24020726}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{24020726}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{24020726}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{76}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{12493}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{70.821192052980137532358639873564243316650390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{65.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{9132}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{64}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.1838846630245374313972206437028944492340087890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.64965905079484487227858835467486642301082611083984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.5844867654729120065582037568674422800540924072265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.46885463329791232656162947023403830826282501220703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.41407183905141720092757395832450129091739654541015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.035333853699749846744015968624808010645210742950439453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{686.9816267490386962890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{22401}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{662.134542457315319552435539662837982177734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{635.744015276432037353515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{634.80264949798583984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{12.7601070743713886912473753909580409526824951171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.716468334198001599588678800500929355621337890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.139070360865815700890379957854747772216796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{2306}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.546968996524810791015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{17.073853969573974609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2241086316523614729856461735835182480514049530029296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.66766676502150790195599938670056872069835662841796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.58941054675433968146336383142624981701374053955078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.463159220035124163938888841585139743983745574951171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.41881128232465669736228619512985460460186004638671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.035947849663756352434074159418742056004703044891357421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1693206277507260104631114927542512305080890655517578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1376931651827416891453736980110988952219486236572265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.104363437926291879875861923210322856903076171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08724117137852570313949485125704086385667324066162109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01170364328867043619830656808744606678374111652374267578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{199898514337119104657}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{162559397044803338240}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{123210600325041897472}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{102996195911059103471}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{13817223198469892096}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.7125339508056640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.21119032790329317350597193581052124500274658203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.18486309051513671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5706513486772113452616395079530775547027587890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.099337748344371590292212204076349735260009765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999718189239501953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9956416160065606479889765978441573679447174072265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{30371}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.983900368213653564453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98008680343627918585269753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0030195619119790443989070904962090935441665351390838623046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.3894349077042968954032176043256185948848724365234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{23033012}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{23033012}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{23033012}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{23033012}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{76}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{12493}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{70.6158940397350960438416223041713237762451171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{66}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{66}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.1618637015938606538156818714924156665802001953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.67257837986194790591554237835225649178028106689453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.59101317208097725597326643764972686767578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.46827134435101702703008186290389858186244964599609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.433495764182162790500996152331936173141002655029296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03562081316475747272409790866731782443821430206298828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{684.1159942150115966796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{22401}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{664.2095631384692069332231767475605010986328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{635.614442288875579833984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13716}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{635.2611672878265380859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.89605179848656035801468533463776111602783203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.380094528198238634786321199499070644378662109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.162060734452001753425065544433891773223876953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.555310785770416259765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{17.114662647247314453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.286557054910298647509847569381236098706722259521484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.423896870746865495060973216823185794055461883544921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.345934407044196368108401884455815888941287994384765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.2711868865810895812273884075693786144256591796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.263980328587969881315444808933534659445285797119140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0284669202556614951704627713979789405129849910736083984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.41754231270147201815490234366734512150287628173828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.365258444886783661953444379832944832742214202880859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8721}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.3062947511356364227452786508365534245967864990234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.26903052088608780945122589400853030383586883544921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.019754492657641564701265224357484839856624603271484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{492946955670327021371}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{431221059429609046016}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8721}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{361609016660457226240}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{317615178675355869464}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{23321988503135252480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17088}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{179.824432373046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.302513274135975507306284271180629730224609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.872837066650390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{82.67822265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.48188325228561978974539670161902904510498046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{70}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{47.10596026490065924008376896381378173828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{31}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{28}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99997800588607799188167746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9986099553424001573631585415569134056568145751953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29022}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99610291421413421630859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.995666921138763427734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{24144}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0007528122066445155739777828074466015095822513103485107421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{7.563551776025587258800442214123904705047607421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21966196}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21966196}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21966196}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{21966196}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{98}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{82.3443708609271567411269643343985080718994140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{75.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{2743}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.9138771822647395737249098601751029491424560546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.42485232667181549448542909885873086750507354736328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3468913608443877638620733705465681850910186767578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.272556509625235310334545602017897181212902069091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.26504153622939929935142799877212382853031158447265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.02849973288381917047029645573275047354400157928466796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{684.9872226715087890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{22401}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{664.61399189999565351172350347042083740234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{634.52175152301788330078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4157}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{633.2736628055572509765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.16311932334567558200433268211781978607177734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.0717351436614990234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.157263267908664516880890005268156528472900390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{23367}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.567543923854827880859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{17.1381928920745849609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.278810004460354587951798066569608636200428009033203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6532556548037333765677203700761310756206512451171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.58305246778202590718365172506310045719146728515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.46440357154471201273082670013536699116230010986328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.4003055075172226029422972715110518038272857666015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0358422979091169435772457063649198971688747406005859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.176895371452436389603235511458478868007659912109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1426727771831809155056447480092174373567104339599609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.10902467276513187754982681099136243574321269989013671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08968427206172180365939539115061052143573760986328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0118380527094636978091557466541416943073272705078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{208841193280440444130}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{168438285246945722368}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{128713615117972537344}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{105880500106209491077}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{13975905834403895296}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.6250514984130859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.251300483349933045928992214612662792205810546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{9134}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.6317813396453857421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.075281620025634765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.219462901648069586002520736656151711940765380859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.344370860927153188413285533897578716278076171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999593198299407958984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9957788286619628781437540965271182358264923095703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98666520416736602783203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98634105920791637078792746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0028868083398743637178751608729498911998234689235687255859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.409740747458536613834212403162382543087005615234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{24037365}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{24037365}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{24037365}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{24037365}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{76}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{12493}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{70.794701986754972722337697632610797882080078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{65.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{9132}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{64}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.214694695281341108028527742135338485240936279296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.65422278524166410651474734549992717802524566650390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.58463314941132582536198469824739731848239898681640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24566}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.4693770829046737258494204070302657783031463623046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.414341134566160784746813305901014246046543121337890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.035471370251374235993413464029799797572195529937744140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{685.7139434814453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{664.4505743648832094550016336143016815185546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{635.612303435802459716796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4157}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{632.25999546051025390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.04679262377704418440771405585110187530517578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.319389820098876953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.165872180698723781233638874255120754241943359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.5385303497314453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{17.0731213092803955078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.287165418829357588226258712893468327820301055908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6676387557210168299803854097262956202030181884765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.58915229920609946123732925116200931370258331298828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.463082841819539681171846723373164422810077667236328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.418571789662090687489381934938137419521808624267578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03601371407861224394064691978201153688132762908935546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1694009048774031966910769142486969940364360809326171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.137756792411470152526220545041724108159542083740234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1043945842152555758541865316146868281066417694091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08724817168272240575088716241225483827292919158935546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01171055935796987655661549609931171289645135402679443359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{199993288840209575513}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{162634514817889566720}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{123247371372808896512}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{103004460411536192636}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{13825388251933104128}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.80197429656982421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.2154952990298237835986583377234637737274169921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29052}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.17984616756439208984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0430088043212890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.57185251083535393323842299651005305349826812744140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.105960264900662792797447764314711093902587890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999718189239501953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99566024265541930304834750131703913211822509765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{30371}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98390035331249237060546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98008674383163441046207253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00302546010525681606517789390409234329126775264739990234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.3865595034830879850318297030753456056118011474609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{23082929}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{23082929}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{23082929}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{23082929}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{76}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{12493}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{70.6158940397350960438416223041713237762451171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{66}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{66}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.1618637015938606538156818714924156665802001953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6725501645142142326250223050010390579700469970703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.5907543094126468385951511663733981549739837646484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.4681928004945259402802548720501363277435302734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.43324787435885425690429428868810646235942840576171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0356897667152713260474428125235135667026042938232421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{686.9306805133819580078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{664.2953297302423152359551750123500823974609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{19488}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{634.239748477935791015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{633.0231206417083740234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.2292827405612687385882964008487761020660400390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.580661296844478869161321199499070644378662109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.1715337424878242700287955813109874725341796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.73142802715301513671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{17.7286517620086669921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.284636265659082010603952994642895646393299102783203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.4224561132699247156807587089133448898792266845703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.346057998934033494986550749672460369765758514404296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{2306}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.27106130825781205029301190734258852899074554443359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.266777089725750704563012050130055285990238189697265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.028393026967351797651417655288241803646087646484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.41739003806011998332081702756113372743129730224609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.365252071392213106815205492239329032599925994873046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8721}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.306388079339856622684834519532159902155399322509765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.269086732324232913438066816524951718747615814208984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.019740869154307734423259290679197874851524829864501953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{492767181504699100168}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{431213534935324491776}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8721}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{361719199156336197632}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{317681541428218439115}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{23305904709254508544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{181.325698852539034078290569595992565155029296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.10632122115583797494764439761638641357421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.661590576171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{81.919342041015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.5543243092486829226572808693163096904754638671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{70}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{47.10596026490065924008376896381378173828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{30.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{27}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99996185302734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99860367238126845901291517293429933488368988037109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99613805115222930908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.995692670345306396484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{24144}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0007567330224106487424062805757785099558532238006591796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{7.60459282439968564659693583962507545948028564453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21986739}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21986739}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21986739}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{21986739}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{90}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{82.3046357615894095260955509729683399200439453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{76}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{2743}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{76}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{2743}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.64448289236149758352212302270345389842987060546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.42340832175342668630690923237125389277935028076171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.34701596467293616132820943676051683723926544189453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.27242930324509806450095084073836915194988250732421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.267849540418154952181595263027702458202838897705078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.02843225411963749837962467381657916121184825897216796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{684.9339663982391357421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{19093}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{664.277556261479503518785350024700164794921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{634.366406500339508056640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{633.149266719818115234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.1576394028796102020351099781692028045654296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.3301813602447509765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.15624924684991725598592893220484256744384765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.627543985843658447265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{6549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{17.4027864933013916015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.278612048870455153437575290809036232531070709228515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.423203634524063010413641450213617645204067230224609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.3412442638521486770741830696351826190948486328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{9132}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.261006460603845524826027713061193935573101043701171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2594714868449690126084306029952131211757659912109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0275920151210239279759850461459791404195129871368408203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.422376572821110796152055399943492375314235687255859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.3686038975708758602678472016123123466968536376953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{23241}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.31028434581463937291800903039984405040740966796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.274353133795015080576007449053577147424221038818359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0196060905201408015863240308362946962006390094757080078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{498654242659940935544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{435170672835954933760}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{23241}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{366319098708546879488}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{323899010875957643163}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{23146786183105298432}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17216}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{187.469207763671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{104.0375475851905235913363867439329624176025390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{87.287982940673828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{83.86852264404296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.91771665649914524465202703140676021575927734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{71}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{48.3973509933774863611688488163053989410400390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{32.25}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{30}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99997413158416759149105246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{32103}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99858767070517640007665249868296086788177490234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{10248}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99600887298583984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24144}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99592250585556041375667746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0007544419539759835043046809488487269845791161060333251953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{7.78015770469443879164828103967010974884033203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22009489}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22009489}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22009489}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{22009489}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{98}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{82.6225165562913872463468578644096851348876953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{76.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{7467}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{76}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{2743}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.980603347638034250621785758994519710540771484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.424157527907031262071058108631405048072338104248046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3421919956559114073257887866930104792118072509765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.262144054921473579344848303662729449570178985595703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.260867935632622394148683042658376507461071014404296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0276635187256388768994863625039215548895299434661865234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{696.9877679347991943359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{14929}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{664.58639393894873137469403445720672607421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{634.789174854755401611328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{633.3740022182464599609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.4266740829465955897603635094128549098968505859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7868483066558837890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.150071769360675233428992214612662792205810546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.680631816387176513671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{2743}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{17.533187389373779296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2193756411866649991271316366692190058529376983642578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.5646017998401247073303466095239855349063873291015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.49137765207473271811267068187589757144451141357421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.404699364479737422328753382316790521144866943359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.39812355784724140495001165618305094540119171142578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.035338854554594574530757000729863648302853107452392578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.300533684025837077857801205027499236166477203369140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.2372784425303066935253326619204017333686351776123046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1819346509335495742920585371393826790153980255126953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1595912858577701876061638586179469712078571319580078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0241133093386178450068246803539295797236263751983642578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{354807549104237390712}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{280128941028158111744}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{214790524410295877632}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{188412134823200673959}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{28467970952939130880}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{17024}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{17024}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17024}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17024}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{32.51659393310546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{29052}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{20.5541418403979179174712044186890125274658203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{913}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{13.2870109081268310546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{11.60878849029541015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.819185726656505242004868705407716333866119384765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{32}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{18.920529801324502017223494476638734340667724609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{11.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{8745}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{11}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99978941679000843389957253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99863691953633793030320475736516527831554412841796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.995248734951019287109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.995136439800262451171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000901216432548787083935126762668232913711108267307281494140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{3.71059549460845605750591857940889894962310791015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{26011543}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{26011543}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{26011543}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{26011543}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{82}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{74.927152317880796772442408837378025054931640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{67.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{67}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.519064626541626328304346316144801676273345947265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.565774882383446087175116190337575972080230712890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.492726772840490656601986074747401289641857147216796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.405642735667783693731536232007783837616443634033203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.399724024685359446973365038502379320561885833740234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.035219429827171765123861035817753872834146022796630859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{679.154917240142822265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{658.8385911035221624842961318790912628173828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{913}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{633.7017824649810791015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{632.733926296234130859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.6431025178057101499007330858148634433746337890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.8329589366912841796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.137542473559346234424083377234637737274169921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.668922960758209228515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{17.462230682373046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2339537882086889231114668064037687145173549652099609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.398383403768505617303929966510622762143611907958984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.259574623466292175866243496784591116011142730712890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0629465252839907785098461090456112287938594818115234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00057078808106089998740395596854568793787620961666107177734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.071062764105729925301346838750760070979595184326171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.140541282124082400617481880544801242649555206298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.12012895573148096861615385932964272797107696533203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{6204}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08051439678637882513267953754620975814759731292724609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.03167815003466430134881903768473421223461627960205078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01124241361380243046930171857411551172845065593719482421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{165921860040573462258}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{141823238542119305216}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{6204}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{95054622193115758592}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{37398958490753692851}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{13272699309094500352}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{37122}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{37122}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{37122}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{37122}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{12}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{16284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99875295162200916632144753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9919664026885632868157927077845670282840728759765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9787164628505706787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97702139616012562139957253748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0036873680942152557184210426299841856234706938266754150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.196019889533171731699212614330463111400604248046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21490869}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21490869}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21490869}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{21490869}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{54.66887417218543276931086438708007335662841796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{13}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{13}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{20.274840656172219865993611165322363376617431640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.399413612249276628318739312817342579364776611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.2602378942940430928132400367758236825466156005859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.06305026429033254442568789954748353920876979827880859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000590801217226420293145150441915802730363793671131134033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0712208136873342112505014256385038606822490692138671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{797.13279056549072265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{655.206388890348534914664924144744873046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1412}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.4730570316314697265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{631.4582920074462890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{13293}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{15.6692410112564690649605836370028555393218994140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.539545536041259765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.017608018900386213090314413420855998992919921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{20754}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.119296729564666748046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{16.84192180633544921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2333441326763732448501542648955364711582660675048828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.398033986747971690878244999112212099134922027587890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.258094796066517695454223257911507971584796905517578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.058043911233499424773274455446880892850458621978759765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000462306709809299988707398387788316540536470711231231689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0708512154896593637776192053934209980070590972900390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1439895180345328873361410160214290954172611236572265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.12318828516429325414804907268262468278408050537109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0830139840616308244403143135059508495032787322998046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.032691997041097299592227187758908257819712162017822265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01146943880598853306163054099897635751403868198394775390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{169992818462708093160}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{145435057235511721984}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{98005613985530150912}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{38595897771237877779}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{13540723348681175040}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21250}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21250}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21250}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21250}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.456815242767333984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.453065700088905121134530418203212320804595947265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{6204}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.5314728319644927978515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.4557187557220458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.485879266046599533890315569806261919438838958740234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.27152317880794640814201557077467441558837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99844670295715320929019753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9923959733634595270501677077845670282840728759765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97714480757713306768863503748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97507029771804798468082253748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004075124912268920408797701071534902439452707767486572265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.2498146873732924877486993864295072853565216064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{23565302}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{23565302}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{23565302}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{23565302}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{80}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{54.099337748344368037578533403575420379638671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{32382}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{13}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{13}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{20.808414932708206634970338200218975543975830078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.39906329164597675873693560788524337112903594970703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.25875507200799408025204684236086905002593994140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.058161433565543992074697854377518524415791034698486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0004785162408780820855920545842110414014314301311969757080078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.071010678399016480266681128341588191688060760498046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{679.2566711902618408203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{653.9366795006177426330395974218845367431640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{9816}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{629.484053194522857666015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13293}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{626.6978046894073486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.8906430104666380742628462030552327632904052734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.504243373870849609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{9816}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.030054384509458742513743345625698566436767578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{26829}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.198074758052825927734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{16.857151508331298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2352572506701394450256970003465539775788784027099609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.404082111554126710561973823132575489580631256103515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.2541990750977216606543152010999619960784912109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.061970961504083599269421256394707597792148590087890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00080449092765860004579370201582833033171482384204864501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07074357029222799742029792469111271202564239501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.155832165876540307269948471002862788736820220947265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.13299184488550308547161193928332068026065826416015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.091253440084651249453173704750952310860157012939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.03589546554351440155183894376023090444505214691162109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01227381171420331706922723924435558728873729705810546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{183974149272089199111}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{157009057695574720512}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{107733046725577654272}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{42377885842423693395}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{14490359264051638272}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.5789470672607421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.1628587988038727729644961073063313961029052734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11611}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.62857162952423095703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.099677562713623046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.2070768017832402829725424453499726951122283935546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10.25827814569536400313154445029795169830322265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99892097711563121453792746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{15043}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99427625596128554885666517293429933488368988037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98113346099853515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8840}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97290587425231922491519753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0032747101359900314225537254486653182539157569408416748046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.33453157274807931997884224983863532543182373046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22520790}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22520790}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22520790}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{22520790}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{81}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{57.072847682119203227557591162621974945068359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{13.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{13}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{19.96788790833536353375166072510182857513427734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.4045923638913182518450639690854586660861968994140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.25484935094987049009063184712431393563747406005859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.062075123484654264049975580519458162598311901092529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000832698220370865749805078248613199320971034467220306396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07090112960549550813471597621173714287579059600830078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{680.3722589015960693359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{654.596481583765807954478077590465545654296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.441181182861328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13293}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{630.5875542163848876953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.755916472783436432791859260760247707366943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.5271823406219482421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.020395195247321140641361125744879245758056640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{23367}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.0187556743621826171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{16.952646732330322265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.258572519120451982388431133585982024669647216796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.401740432965557781042065244037075899541378021240234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.256016030006405548302694796802825294435024261474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{30371}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.06058745750775862415338224309380166232585906982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00085375599557729994933119588296221991186030209064483642578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07108059415740421160823103718939819373190402984619140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1519976385713475985905773768536164425313472747802734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.129692105278827740644231880651204846799373626708984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{17194}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0881951025000244914764380155247636139392852783203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.034432898597619797376179207049062824808061122894287109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.012019980012019863824246357353331404738128185272216796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{179447138466166594356}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{153113412765384343552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{17194}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{104122398999842144256}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{40651191561362288580}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{14190687683381417984}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.7125339508056640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.21119032790329317350597193581052124500274658203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.18486309051513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5706513486772113452616395079530775547027587890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{16284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.9403973509933774010960405576042830944061279296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999019086360931396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99411511381730333081208073053858242928981781005859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98269011080265045166015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97393202781677234991519753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0030325136905347328288018449171659085550345480442047119140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.2246463908041123058723087524413131177425384521484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21533076}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21533076}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21533076}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{21533076}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{81}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{56.63576158940397675678468658588826656341552734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{4157}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{13.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{13}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{20.123619098264470039794105105102062225341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.402779322631127867371247930350364185869693756103515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.25667051830183551519581897082389332354068756103515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{30371}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.060713201719383692867015867022928432561457157135009765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000883690634296209758143103574212773310136981308460235595703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07123684280499571752631737808769685216248035430908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{689.2448160648345947265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{24262}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{654.95137073188425347325392067432403564453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{632.532400190830230712890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{632.2713348865509033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{13293}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.84045354236946678838648949749767780303955078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.5954115390777587890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.02681289129699138129581115208566188812255859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{22401}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.122203350067138671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{17.0476043224334716796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.247275690194209418759641039287089370191097259521484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.28048577108590200257509650327847339212894439697265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.1695562098578521081915226886849268339574337005615234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{9134}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.044390752912956077391726239511626772582530975341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.02332544233881660156182391574475332163274288177490234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.048067422643187064645875494761639856733381748199462890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.34124911092065290940666955066262744367122650146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.296377792901700243266560619304073043167591094970703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.20515698199908849463923843359225429594516754150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.12309580981564240131920229259776533581316471099853515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.024318746965951966443331144773765117861330509185791015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{402875840930189262416}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{349901138866467569664}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{242206613879796727808}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{145325881613771506188}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{28710508894349873152}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{179.824432373046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.302513274135975507306284271180629730224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.872837066650390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{82.67822265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.48188325228561978974539670161902904510498046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{59}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{44.046357615894038417536648921668529510498046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{23.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{12}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.999580395537496446678460415569134056568145751953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{27584}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99706031382083892822265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12561}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9948346614837646484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00054073508107739249976819717602438686299137771129608154296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{6.424639808332671009338810108602046966552734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20466260}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20466260}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20466260}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20466260}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{93}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{1412}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{80.072847682119203227557591162621974945068359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{22.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{21}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.91150394678812318716154550202190876007080078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.281211099544303844144366166801773943006992340087890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1699969880588465820370203118727658875286579132080078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{9134}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.044655834098513348673353817730458104051649570465087890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0241432857191129779383942377535277046263217926025390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.048175536176805110188947622873456566594541072845458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{680.22106075286865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{23696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{654.702591813952722077374346554279327392578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.687671482563018798828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13293}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{631.0650737285614013671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.6029012984180521783628137200139462947845458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.570300579071044921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.03731281867879943092702887952327728271484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{3175}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.03210961818695068359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{16.7808163166046142578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.25297444700038440590361688009579665958881378173828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.40486208186312211410040617920458316802978515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.2541673566928268623854592078714631497859954833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.06160533805074326629824810197533224709331989288330078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00080449092765860004579370201582833033171482384204864501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07071045325293438821301350571957300417125225067138671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.15570557672889850930886268542963080108165740966796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.132969383321212664128552205511368811130523681640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{1696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0912863754240879343715420191074372269213199615478515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.035915007056130099361013208181248046457767486572265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01223576067958762579601650344329755171202123165130615234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{183824699185109597154}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{156982539760985374720}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{1696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{107771929911342104576}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{42400956388473925257}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{14445436531424727040}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.6250514984130859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.251300483349933045928992214612662792205810546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{9134}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.6317813396453857421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.075281620025634765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.219462901648069586002520736656151711940765380859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10.23841059602649039561583776958286762237548828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99892097711563121453792746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{15043}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99422522333284091278216010323376394808292388916015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4800}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.981195151805877685546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8840}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.972655713558197021484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0032661595283135663216056432389677866012789309024810791015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.3307798304898963426268210241687484085559844970703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22537429}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22537429}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22537429}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{22537429}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{81}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{57.006622516556291202505235560238361358642578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{13.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{13}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{20.07584845633210335336116258986294269561767578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.405373319103286944287134474507183767855167388916015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.25481759191489239402272914958302862942218780517578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.061708925224064868630957647610557614825665950775146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000832698220370865749805078248613199320971034467220306396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07086804728137814646249381667075795121490955352783203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{770.0991647243499755859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{655.2774262823016897527850233018398284912109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1412}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.577586829662322998046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{630.361099720001220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{14.2764626836054286940225210855714976787567138671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.61765956878662109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{9816}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.028370219350652092771269963122904300689697265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{20754}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{16.986416757106781005859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{16.755332469940185546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.260946038330846175057331493007950484752655029296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.40113699366754318464955986200948245823383331298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.255984282628264614434243640062049962580204010009765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.06009541195494870480242610710774897597730159759521484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00085375599557729994933119588296221991186030209064483642578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0710207190376810626464276765545946545898914337158203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1520095488124287019804370402198401279747486114501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.12973572492949425605246460690977983176708221435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{17194}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08821862073792792469095758178809774108231067657470703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.034454124344002100277517541826455271802842617034912109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0120236144663347817307386122820389573462307453155517578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{179461199596987733328}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{153164909759459983360}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{17194}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{104150164434445008896}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{40676250499684681605}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{14194978489691492352}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.80197429656982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.2154952990298237835986583377234637737274169921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29052}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.17984616756439208984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0430088043212890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.57185251083535393323842299651005305349826812744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{16284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.9403973509933774010960405576042830944061279296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999019086360931396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9941120787172128547837246514973230659961700439453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9828036129474639892578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97393202781677234991519753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0030306544033469880010389641000756455468945205211639404296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.2246463908041123058723087524413131177425384521484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21582993}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21582993}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21582993}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{21582993}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{81}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{56.76158940397350960438416223041713237762451171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{4157}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{13.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{13}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{19.96543656112843478922513895668089389801025390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.402174322855752552907659946868079714477062225341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.256638656378443685834866982986568473279476165771484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{30371}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0602201923483603185349721798047539778053760528564453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000883690634296209758143103574212773310136981308460235595703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0711767010219000739734696026062010787427425384521484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{958.2426109313963706881622783839702606201171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{656.2545055616770923734293319284915924072265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27671}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.324820995330810546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{630.79305553436279296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{26.86177807963839114790971507318317890167236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.571672916412353515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{9816}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.019372995326062181220549973659217357635498046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{16.914998590946197509765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{16.76795291900634765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.26251447030294527973381946139852516353130340576171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.282026682642950110579960210088756866753101348876953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.1695898255403663623663845783084980212152004241943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{9134}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.043589982559524349803314891005356912501156330108642578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0233114288393398982890403203782625496387481689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0481719419099879420098631044311332516372203826904296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.341175269473538100850618093318189494311809539794921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.296375294894897223230145755223929882049560546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{30371}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2049409427075001843832069425843656063079833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1229331650456094993106859192266711033880710601806640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.02433604632358384034507281512560439296066761016845703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{402788664336463884640}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{349898189740567232512}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{30371}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{241951559702401875968}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{145133864561117208903}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{28730932371013832704}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{181.325698852539034078290569595992565155029296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.10632122115583797494764439761638641357421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.661590576171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{81.919342041015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.5543243092486829226572808693163096904754638671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{59}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{44.046357615894038417536648921668529510498046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{23.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{12}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99957930765404601203272250131703913211822509765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9970798790454864501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12561}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99480938911437999383480246251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000538987072649686174870276023085580163751728832721710205078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{6.40399063120498279744197134277783334255218505859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20486803}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20486803}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20486803}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20486803}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{93}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{29110}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{79.821192052980137532358639873564243316650390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{22.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{21}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{11.615293693472938940658423234708607196807861328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.282616329103480168338791145288269035518169403076171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1700305013936581344236032009575865231454372406005859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{9134}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.043853687502172049306192747053501079790294170379638671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0241287808742797586780692853380969609133899211883544921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.048279997958988761508347664630491635762155055999755859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{1046.6073901653289794921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{656.9246547932656312696053646504878997802734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.523334085941314697265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{23241}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{630.286437511444091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{33.573967663583260900850291363894939422607421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.6005985736846923828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{9816}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.028543912811784366567735560238361358642578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.1094734668731689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{16.7781083583831787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2411692770467143975832158275807159952819347381591796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.27945076377185140703574006693088449537754058837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.1683229698315593936275291753190685994923114776611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.04450039675079960066472750668253866024315357208251953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0225136866007694010083373115094218519516289234161376953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.047589658916143140476862072318908758461475372314453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.34288210895413240297813217694056220352649688720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.298988016553862145929798543875222094357013702392578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7790}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.207027796819203524503194557837559841573238372802734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.126064177035681901362096368757192976772785186767578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0242155678895951652351836713705779402516782283782958984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{404803744725163245987}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{352982747038408245248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7790}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{244415282180338450432}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{148830311080962413424}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{28588696541369655296}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{187.469207763671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{104.0375475851905235913363867439329624176025390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{87.287982940673828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{83.86852264404296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.91771665649914524465202703140676021575927734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{61}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{45.0264900662251648100209422409534454345703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{24.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{13}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99959888047729894555715191017952747642993927001953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.997950494289398193359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12561}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99782675504684437139957253748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000393089256145395479248583203712996692047454416751861572265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{6.4704596394124553881965766777284443378448486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20509553}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20509553}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20509553}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20509553}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{93}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{1412}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{80.6357615894039696513573289848864078521728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{22.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{21}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.538785787600733812041653436608612537384033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.2798036385991882202262104328838177025318145751953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.16876055135501599746561396386823616921901702880859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.04475885385341416000670733410515822470188140869140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.023303067967478378885726186808824422769248485565185546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.047698518662224902164847861740781809203326702117919921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{740.1135828495025634765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{654.7408008685964659889577887952327728271484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{30899}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.820179760456085205078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{631.7942841053009033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{12.551700998370538542303620488382875919342041015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.560001373291015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{9816}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.026848600400203537219567806459963321685791015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{32103}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.367010414600372314453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8000316619873046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.229151791791914638540816895329044200479984283447265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.3502220652548124757430514364386908710002899169921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.2148159412810098090051980079806526191532611846923828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{28778}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0494849497078310995856753606858546845614910125732421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{1696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.003470056872063300053288248392391324159689247608184814453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06326379577118890207287904559052549302577972412109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.261449570766861982828999089178978465497493743896484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{29052}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.207866507596377925182196122477762401103973388671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1398196496709535885383246522906119935214519500732421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07325683156882729918368823973651160486042499542236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0230525534358469140483460790846947929821908473968505859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{308665172487521103637}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{29052}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{245405457096076001280}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{165069906813171826688}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{86486401510464249072}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{27215651422501236736}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{20994}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{20994}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{20994}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{20994}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{32.51659393310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{29052}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{20.5541418403979179174712044186890125274658203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{913}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{13.2870109081268310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{11.60878849029541015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.819185726656505242004868705407716333866119384765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{35}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29052}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{20.907284768211919612213023356162011623382568359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{12}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{6}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999999463558197021484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99934056973615226215912343832314945757389068603515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7098}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99316944181919097900390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98739540576934803350894753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0011639647030542098725403032943859216175042092800140380859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{4.0203966615569246556560756289400160312652587890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{24511607}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{24511607}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{24511607}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{24511607}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{85}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{71.2980132450331183235903154127299785614013671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{17.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{14.4533021511581321050243786885403096675872802734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.3506643061316605525234990636818110942840576171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.215364890817856202698266088191303424537181854248046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{28778}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.049598532227492185542327973735154955647885799407958984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0035917250059767208934802251718565457849763333797454833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06340585533166091802836916713204118423163890838623046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{714.6636641025543212890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{654.566855943755626867641694843769073486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{26829}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{630.371035873889923095703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{630.1529781818389892578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{13293}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.572099406848071367903685313649475574493408203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.5622208118438720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{7310}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.024686363359162299957461073063313961029052734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{16.952344119548797607421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{16.846088409423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.267207005921072215937073224267805926501750946044921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.68942794737815604744213260346441529691219329833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.60677246273333829140739226204459555447101593017578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{11498}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.493586528321392881135665220426744781434535980224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.43620027112436698946140722910058684647083282470703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0308237029352933129822122992891308967955410480499267578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1590030484385898945642878743456094525754451751708984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.129610558792541852302093730031629092991352081298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08090877889909052489425533849498606286942958831787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.035672195017851703047195854878737009130418300628662109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01220272911964798666362153056752504198811948299407958984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{187717666655123905064}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{153017139666976407552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{95520226410744004608}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{42114294530673152936}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{14406439748540762112}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{37122}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{37122}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{37122}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{37122}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.4105960264900669898224805365316569805145263671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9991238117218017578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9930714747763627059384816675446927547454833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{23447}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97377805411815643310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96438848972320556640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00432364202240125179710350522555017960257828235626220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.456983744421120885448317494592629373073577880859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21929781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21929781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21929781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{21929781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{83}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{29726}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{71.1324503311258240501047112047672271728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{55.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{27714}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{55}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.3667550452271139960203072405420243740081787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6908253841360181279895869010942988097667694091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.60840625268289105775920688756741583347320556640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.498681007045377377995265533172641880810260772705078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.451494450717646544912753370226710103452205657958984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0300583285534850620790425779205179424025118350982666015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{682.8454401493072509765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7790}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{657.3315430982223688261001370847225189208984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{634.61968994140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{29052}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{634.5520074367523193359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.430308197834580852259023231454193592071533203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.626359224319454455098821199499070644378662109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{12561}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.09120882741662938997251330874860286712646484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{16.92033255100250244140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8648827075958251953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2634221528689180136240111096412874758243560791015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.68653376015249667485562667934573255479335784912109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.60279421774442931702964187934412620961666107177734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{13716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.4881881015119569067195470779552124440670013427734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.43453682948569027910679096748935990035533905029296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0306655788306931555153855839535026461817324161529541015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1632589985555787104321012748187058605253696441650390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1331633961025236179143149684023228473961353302001953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{23367}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08386237166767528117272689769379212521016597747802734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.036667900638075200114851526222992106340825557708740234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.012411446495726237426726612511629355140030384063720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{192742205701432245703}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{157211589624913002496}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{23367}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{99007213284346757120}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{43289816242610281214}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{14652849733836869632}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21250}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21250}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21250}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21250}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.456815242767333984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.453065700088905121134530418203212320804595947265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{6204}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.5314728319644927978515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.4557187557220458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.485879266046599533890315569806261919438838958740234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{15}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.76821192052980080688939779065549373626708984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.998985767364501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.993586850482107042381585415569134056568145751953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9768750667572021484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96321922540664683953792746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004370426450259917196261572058801903040148317813873291015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.545956951369293452813735711970366537570953369140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{24004214}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{24004214}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{24004214}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{24004214}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{83}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{29726}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{70.953642384105961582463351078331470489501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{45}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{42}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{5.0524897126022860760485855280421674251556396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6879253305342876156913689555949531495571136474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.60441741950700345054059425820014439523220062255859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20751}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.4932515313075154228528163002920337021350860595703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.44977268500892908509314338516560383141040802001953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0299066048751779299530451083910520537756383419036865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{682.8255341053009033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{23696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{657.0547424215354794796439819037914276123046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{635.26934051513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{29052}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{633.752150058746337890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.5915359082923661304675988503731787204742431640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.73790836334228515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.101477815615421462780432193540036678314208984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{8048}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.0052306652069091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{16.9323804378509521484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.260214906466087192438152442264254204928874969482421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.67120679118131487683740488137118518352508544921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.59017607982812514411108395506744273006916046142578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.4795444092400484858984555103234015405178070068359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.429759404081381413131879298816784285008907318115234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.029719107629869567777092242977232672274112701416015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1750782387550006979903827186717535369098186492919921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1441644975369113790275577002830686978995800018310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09291666371197172813456433004830614663660526275634765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0397842687002211981006638552571530453860759735107421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01307025628349333702671319912269609631039202213287353515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{206695901644116149274}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{170199397797013520384}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{109696634603371429888}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{46968974263851176000}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{15430635048921333760}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.5789470672607421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.1628587988038727729644961073063313961029052734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11611}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.62857162952423095703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.099677562713623046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.2070768017832402829725424453499726951122283935546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{16}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10.8410596026490058108038283535279333591461181640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99942493438720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.995279330686228203006749026826582849025726318359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98449146747589111328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97576105594634998663394753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00306131213498717254239966933937466819770634174346923828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.6238810318859713266448352442239411175251007080078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22959702}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22959702}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22959702}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{22959702}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{84}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{71.940397350993379177452879957854747772216796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{58.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{27714}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{56}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.1705873108722801845260619302280247211456298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6725672945460108298476598065462894737720489501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.59176653200499218510088894618093036115169525146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.48531412461833856042403567698784172534942626953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.4448277521385228805428369014407508075237274169921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0289790979413139526688070191084989346563816070556640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{685.904563426971435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{23696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{661.3398171023817440072889439761638641357421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29195}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{633.356704175472259521484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{13293}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{621.452413082122802734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{29110}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.10418381968886336608193232677876949310302734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.9855327606201171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.164603215969162164356021094135940074920654296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.14246237277984619140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{16.9472858905792236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.25683294530997680116257697591208852827548980712890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.67950559649257835648228365243994630873203277587890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.59421722814258559619560173814534209668636322021484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{13716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.483447164324070255414511620983830653131008148193359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.426691448404643625114118776764371432363986968994140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03039004179693594043243365376838482916355133056640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.17099584457808558735081305712810717523097991943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1404970845601842821537275085574947297573089599609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0902194772065133265837033604839234612882137298583984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.03870452369416139959401590431298245675861835479736328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01282764666626091953904875708758481778204441070556640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{201876261286384720189}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{165869680766979309568}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{106512358815515148288}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{45694236357185499941}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{15144212167711277056}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.7125339508056640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.21119032790329317350597193581052124500274658203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.18486309051513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5706513486772113452616395079530775547027587890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{15}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10.4635761589403966098643650184385478496551513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999437987804412841796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.994763788403264737070230694371275603771209716796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97959220409393310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8048}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97723025083541881219417746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0033507353200151941165219060536628603585995733737945556640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.543088991253677821902101641171611845493316650390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21971988}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21971988}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21971988}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{21971988}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{84}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{71.06622516556291202505235560238361358642578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{32.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{32103}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{22}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{6.48040231987537662661225112969987094402313232421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.680882921130088192285256809554994106292724609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.5958173260045438457410682531190104782581329345703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.489215119396595010670125702745281159877777099609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.441652226915843992838262010991456918418407440185546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0296487143585505881493435964557647821493446826934814453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{686.929138660430908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{661.3239663878813416886259801685810089111328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{637.302913367748260498046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{636.091644763946533203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{13293}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.6024104906281539939527647220529615879058837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.8012397289276123046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{11611}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.14580199892157708063678001053631305694580078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.042808353900909423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8429481983184814453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.257819505072727606087568119619390927255153656005859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.451928798694893607557077075398410670459270477294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.38305750872573707255241970415227115154266357421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.311124441940290097363686072640120983123779296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{15043}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.299347341418428614101543416836648248136043548583984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0252367417856979893431290662419996806420385837554931640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.361191106294214303584766412313911132514476776123046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.321655935279945126570311231262166984379291534423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{22545}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.22805696152062904236146323455614037811756134033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1316400142569892073307613600263721309602260589599609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.02337629195085098865458661521188332699239253997802734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{426419193568601303974}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{379744301945525370880}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{22545}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{269242137817527746560}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{155413097782922049324}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{27597854400618549248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{179.824432373046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.302513274135975507306284271180629730224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.872837066650390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{82.67822265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.48188325228561978974539670161902904510498046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{12561}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{50.14569536423841356054253992624580860137939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{22.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{13}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99999940395355224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99901234748347700342918642490985803306102752685546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99676693975925456658870871251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99628365039825439453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000657216948672864511964142320010751063819043338298797607421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{8.444910964907226258446826250292360782623291015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20905172}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20905172}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20905172}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20905172}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{96}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{30371}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{84.2913907284768271210850798524916172027587890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{77}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{11598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{77}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{11598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.70714256711205702998768174438737332820892333984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.45284483628465832527609791213762946426868438720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.384109944083058596486779379119980148971080780029296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.31247708826558417971597236828529275953769683837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15043}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.300958397943729194512485491941333748400211334228515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.025137010863723767417621246522685396485030651092529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{682.4775712490081787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{23696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{661.15826080650685980799607932567596435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29195}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{637.409310877323150634765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{636.77678680419921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.4790008224897004396325428388081490993499755859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7661190032958984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{11611}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.130508042329193330033376696519553661346435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{16197}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.004198968410491943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{16.85701274871826171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.254096833543042299741188116968260146677494049072265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.66822926722377362640514775193878449499607086181640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.590134955513218262268537728232331573963165283203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.480237268841943787389681119748274795711040496826171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.429902799932262824622597463530837558209896087646484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0296922372165305779867505719948894693516194820404052734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1750407268175578068269970799519796855747699737548828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.144134757132646507127304857931449078023433685302734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0929999123833521179616212748442194424569606781005859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0398087857448077009347997545773978345096111297607421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01303155037293808778120496327801447478123009204864501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{206651615365094271603}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{170164286524941664256}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{109794917287239024640}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{46997918881254736532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{15384939175247564800}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.6250514984130859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.251300483349933045928992214612662792205810546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{9134}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.6317813396453857421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.075281620025634765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.219462901648069586002520736656151711940765380859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{16}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10.8278145695364234057933572330512106418609619140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99942493438720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9952279881925771842787753485026769340038299560546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.984491884708404541015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97576397657394398077457253748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0031177962434883305618826820904132546274922788143157958984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.6143462351490918127439044837956316769123077392578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22976341}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22976341}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22976341}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{22976341}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{84}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{71.847682119205302342379582114517688751220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{54.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.556849650075026403328593005426228046417236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6695837352929154828728997017606161534786224365234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.59172529052539790672682329386589117348194122314453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.486011777130408884062262586667202413082122802734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.444976175776046145582398594342521391808986663818359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0289511020471684664412403975575216463766992092132568359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{685.92855358123779296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{23696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{660.79228748548894145642407238483428955078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{30899}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{637.983963668346405029296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{29052}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{637.1339271068572998046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.5181757345798541081194343860261142253875732421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.8263695240020751953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{9816}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.130253333919096547788285533897578716278076171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.1388032436370849609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{16.909327030181884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.251765146567650643927294140667072497308254241943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6796071498866778082259543225518427789211273193359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5941241671260557577483041313826106488704681396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{13716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.4829390565879443375507662494783289730548858642578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.4267126495239395023162387587944976985454559326171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0303764965152098671830049880782098625786602497100830078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.171052973288023213438435732314246706664562225341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.140544585704908853163175308509380556643009185791015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0902325405282829728914606448597623966634273529052734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.03870707990574639989489469371619634330272674560546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01282673263974003219356490035352180711925029754638671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{201943706962639377226}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{165925760220415492096}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{106527781263735177216}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{45697254199163569856}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{15143133075659603968}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.80197429656982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.2154952990298237835986583377234637737274169921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29052}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.17984616756439208984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0430088043212890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.57185251083535393323842299651005305349826812744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{15}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10.4701986754966895887264399789273738861083984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999437987804412841796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9947715326650252709583810428739525377750396728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.979551494121551513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8048}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97723031044006358758480246251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.003344375057368884941733089277704493724741041660308837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.543231094873245279330831181141547858715057373046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22021905}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22021905}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22021905}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{22021905}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{84}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{71.09271523178807683507329784333705902099609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{32.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{32103}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{22}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{6.4616556152249398081721665221266448497772216796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6809846803679546756171703236759640276432037353515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.59572402157297477121034035008051432669162750244140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{28778}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.48870443439140409669363407374476082623004913330078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.4416741713948935110778393209329806268215179443359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0296349331398296118866841908356946078129112720489501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{688.65967273712158203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{660.7990751992787181734456680715084075927734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{8048}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{639.260184109210968017578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{29052}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{638.245685577392578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.5107897853216769590289914049208164215087890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.66867351531982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{9816}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.124053058245323200026177801191806793212890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{16.976657688617706298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{16.9260005950927734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.271874816358621540501872004824690520763397216796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.451590701690002316315286634562653489410877227783203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.382871059522703560684675494485418312251567840576171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{30684}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.31114629630658452441593908588401973247528076171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{15043}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.298691703240745398684197198235779069364070892333984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0253891753508156022001163165668913279660046100616455078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.3614330860079884022439955515437759459018707275390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.321644106536284668518277385373949073255062103271484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.22797917281804658262700513660092838108539581298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1314899519429121033109453264842159114778041839599609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.023379270649282642147159805290357326157391071319580078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{426704872791066580114}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{379730337029876023296}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{269150301127072415744}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{155235935472337125996}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{27601371027027603456}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{181.325698852539034078290569595992565155029296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.10632122115583797494764439761638641357421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.661590576171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{81.919342041015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.5543243092486829226572808693163096904754638671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{12561}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{50.072847682119203227557591162621974945068359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{22.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{13}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99999940395355224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9990120656442957880472022225148975849151611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9967111647129058837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99628353118896484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000662535873529482809141111232520415796898305416107177734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{8.389601998428236839799865265376865863800048828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20925715}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20925715}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20925715}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20925715}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{96}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{8721}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{84.3576158940397391461374354548752307891845703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{77}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{11598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{77}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{11598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.676206601687454611493421907653100788593292236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.452506053973660449241123160390998236835002899169921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.383922930643753990143096643805620260536670684814453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{28716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.31249880726326184632313243128010071814060211181640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15043}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.300299231188977666651140907561057247221469879150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0252901692022981829099936845750562497414648532867431640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{691.0052568912506103515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{660.6688375883544495081878267228603363037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5928}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{637.41803681850433349609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{637.3421027660369873046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{13293}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.0529499007640463759116755682043731212615966796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.667628765106201171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.119611575903480371607656707055866718292236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{7790}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{16.91580164432525634765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8915383815765380859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2603913948454994464754008731688372790813446044921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.44600255386874920748851991447736509144306182861328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.379149246525496363968699142787954770028591156005859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.309608941308744445297662650773418135941028594970703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.298760172896312792278905590137583203613758087158203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.024772679821564856650351060807224712334573268890380859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.364304421671816702765767104210681281983852386474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.32434288801594923778992551888222806155681610107421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.22997909429524654445486930853803642094135284423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1346142852179524063149784751658444292843341827392578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0232315707048969082026967925003191339783370494842529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{430094747616049389880}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{382916495830915284992}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{271511391665147510784}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{158924497157178292236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{27426997710305382400}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21186}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{187.469207763671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{104.0375475851905235913363867439329624176025390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{87.287982940673828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{83.86852264404296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.91771665649914524465202703140676021575927734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{76}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{12561}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{51.32450331125827602818390005268156528472900390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{23.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{14}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99999940395355224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99901103933915391674958073053858242928981781005859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99687507748603831903011496251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{2345}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99659121036529541015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0006430217535119170553514766908165256609208881855010986328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{8.478683570249931022999589913524687290191650390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20948465}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20948465}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20948465}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20948465}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{98}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{30371}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{84.4238410596026511711897910572588443756103515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{74.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{4800}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{67}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{7790}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.04025618178761636301032922347076237201690673828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.446906579249859436941960666445083916187286376953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.380191402455108018454410512276808731257915496826171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29110}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.31033857135022924200740135347587056457996368408203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.300368069341171273212154346765601076185703277587890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.024677568095700978811901649123683455400168895721435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{689.549524784088134765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{660.6186599699866519586066715419292449951171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{13716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{637.759378373622894287109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{29052}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{637.484978199005126953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.8206296358282667569028490106575191020965576171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.663522720336910509786321199499070644378662109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.108719186277578927501963335089385509490966796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{22401}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{16.916987895965576171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8654651641845703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.26888339328690180618508520637988112866878509521484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.5895029291439424223852938666823320090770721435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.50274132995830578263252164106233976781368255615234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.409657365719020116756610150332562625408172607421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.409514887579278175078201229553087614476680755615234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.033419734307959421404365940588832017965614795684814453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.287210202143366177818251117059844546020030975341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.2264164553218135089718288099902565591037273406982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1580713157208079311377701969831832684576511383056640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{11611}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07880929657630940388113316430462873540818691253662109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0242392716833698361467153148396391770802438259124755859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{339077958035012023165}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{267305369945471320064}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{186617670815762284544}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{11611}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{93041595172624319875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{28616681041679237120}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{20994}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{20994}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{20994}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{20994}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{32.51659393310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{29052}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{20.5541418403979179174712044186890125274658203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{913}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{13.2870109081268310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{11.60878849029541015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.819185726656505242004868705407716333866119384765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{35}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29052}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{22.066225165562915577766034402884542942047119140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{12.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{8}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99994063377380359991519753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{16197}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9991035445636471390429278471856378018856048583984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99490988254547119140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98869574069976795538394753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.001010702776999700298887763239008563687093555927276611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{4.188709001783049501455025165341794490814208984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{24950519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{24950519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{24950519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{24950519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{86}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{76.8145695364238463298534043133258819580078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{58.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{7790}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{53}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{9816}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.81076198861939019479905255138874053955078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.590697822773053271561138899414800107479095458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.50410694916892062611424307760898955166339874267578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{27714}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.417538493718209557936660303312237374484539031982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.4119098477349851794571122809429652988910675048828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.033080605729875998954891969106029137037694454193115234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{685.1681640148162841796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{23696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{661.8091903885468809676240198314189910888671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{16284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{634.09680473804473876953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{623.6064260005950927734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{29110}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.9872484070813722922821398242376744747161865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.391441822051998400411321199499070644378662109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.172174000582156594418847816996276378631591796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{7310}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.123950660228729248046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{16.9772243499755859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.332338518565463925114045196096412837505340576171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{37122}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{37122}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{37122}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{37122}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21486773}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21486773}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21486773}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{21486773}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{678.7728121280670166015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{9132}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{653.4638736895377633118187077343463897705078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27484}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{626.43980896472930908203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{19488}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{624.99960613250732421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.4473852269511979784510913304984569549560546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.678240299224857068338678800500929355621337890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{9816}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.04448828634047430341524886898696422576904296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{16.909754574298858642578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{16.827679157257080078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.255619319561842084365110849830671213567256927490234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21250}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21250}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21250}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21250}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.456815242767333984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.453065700088905121134530418203212320804595947265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{6204}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.5314728319644927978515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27484}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.4557187557220458984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.485879266046599533890315569806261919438838958740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{23561206}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{23561206}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{23561206}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{23561206}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{682.1974461078643798828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{9132}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{653.692868270621374904294498264789581298828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{32374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{626.930445730686187744140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{19488}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{625.82231235504150390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.58139521273428584891007631085813045501708984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7214996814727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.04112703910726622780202887952327728271484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{6589}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.382730185985565185546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{16.96328830718994140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2370002995331836614933962437135051004588603973388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.5789470672607421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.1628587988038727729644961073063313961029052734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11611}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.62857162952423095703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.099677562713623046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.2070768017832402829725424453499726951122283935546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22516694}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22516694}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22516694}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{22516694}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{683.7362043857574462890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{9132}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{653.8289822916320872536743991076946258544921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{20539}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{629.57616722583770751953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{625.2390806674957275390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.40447318536096332763918326236307621002197265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.030808925628665662088678800500929355621337890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.068030707883519170309227774851024150848388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{20976}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.407443225383758544921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{16.852074146270751953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.289227915642486899105989550662343390285968780517578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.7125339508056640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.21119032790329317350597193581052124500274658203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.18486309051513671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5706513486772113452616395079530775547027587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21528980}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21528980}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21528980}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{21528980}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{681.8838374614715576171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{9132}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{653.505047417634386874851770699024200439453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29195}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{629.019084990024566650390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{625.7820436954498291015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.4306577019944786144378667813725769519805908203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.0084283351898193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.064871797498486927224803366698324680328369140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{104}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.4364521503448486328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8245866298675537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.278967278513896410618855270513449795544147491455078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{179.824432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.302513274135975507306284271180629730224609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.872837066650390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{82.67822265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.48188325228561978974539670161902904510498046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20462164}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20462164}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20462164}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20462164}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{681.1930387020111083984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{9132}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{653.90170933237141071003861725330352783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{3175}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{629.630512416362762451171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20751}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{626.55223751068115234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.44835024238222587200652924366295337677001953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{19.9767801761627197265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.065618099755798908745418884791433811187744140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{19093}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.384281337261199951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8492183685302734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.287225493202949599957918280779267661273479461669921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.6250514984130859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.251300483349933045928992214612662792205810546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{9134}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.6317813396453857421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.075281620025634765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.219462901648069586002520736656151711940765380859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22533333}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22533333}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22533333}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{22533333}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{681.6680152416229248046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{9132}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{653.76756073623300835606642067432403564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29022}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{627.9681289196014404296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{627.508643627166748046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.6109029340179983336156510631553828716278076171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7537033557891845703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.051291715230373569056609994731843471527099609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{19451}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.34059107303619384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8251616954803466796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.24343454112775020359293876026640646159648895263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.80197429656982421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.2154952990298237835986583377234637737274169921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29052}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.17984616756439208984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0430088043212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.57185251083535393323842299651005305349826812744140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21578897}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21578897}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21578897}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{21578897}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{687.9943206310272216796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{1185}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{653.81553657481208574608899652957916259765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{11611}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{628.867734611034393310546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{628.3525178432464599609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.9503030601059929693974481779150664806365966796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.749863624572750353536321199499070644378662109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.043737343604991707479712204076349735260009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{25516}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{16.9450399875640869140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{16.82100963592529296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.259271010590493677927526050552842207252979278564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{181.325698852539034078290569595992565155029296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.10632122115583797494764439761638641357421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.661590576171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{81.919342041015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.5543243092486829226572808693163096904754638671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20482707}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20482707}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20482707}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20482707}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{709.552583217620849609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{1185}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{653.712454058476623686146922409534454345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29022}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{628.469978392124176025390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{19488}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{627.9193704128265380859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{12.366880618038866401775521808303892612457275390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.68349742889404296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.0476764780006675437107332982122898101806640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{20751}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.132227122783660888671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{16.86089038848876953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2410470054956747321117660476375021971762180328369140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{187.469207763671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{104.0375475851905235913363867439329624176025390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1681}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{87.287982940673828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{83.86852264404296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.91771665649914524465202703140676021575927734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20505457}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20505457}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20505457}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20505457}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{680.936485767364501953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{9132}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{653.3689143168215878176852129399776458740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{23241}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{626.993317902088165283203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{19488}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{624.76801586151123046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.363800490983617663687255117110908031463623046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7349898815155029296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.038352393156646513716623303480446338653564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{20754}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{16.892018496990203857421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8132536411285400390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.249266473117703724060589820510358549654483795166015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{20994}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{20994}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{20994}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{20994}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{32.51659393310546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{29052}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{20.5541418403979179174712044186890125274658203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{913}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{13.2870109081268310546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{11.60878849029541015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.819185726656505242004868705407716333866119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{24507511}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{24507511}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{24507511}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{24507511}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{683.9183804988861083984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{9132}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{653.9206116925801097750081680715084075927734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27714}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{627.79631221294403076171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{624.3426544666290283203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.6305465289214868818135073524899780750274658203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{19.8014085292816162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.0593382143816398865965311415493488311767578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{17194}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.382410466670989990234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{16.84928798675537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.270804701434084360567311478007468394935131072998046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{37122}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{37122}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{37122}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{37122}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21925685}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21925685}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21925685}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{21925685}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{688.35439205169677734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{658.4017157854623292223550379276275634765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{2345}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{632.020674169063568115234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{629.8585703372955322265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.794973524764369443573741591535508632659912109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.72806644439697265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.072819627673421649660667753778398036956787109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{20754}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.386778533458709716796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{16.9378187656402587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2319316981102834684946856214082799851894378662109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21250}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21250}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21250}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21250}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.456815242767333984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.453065700088905121134530418203212320804595947265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{6204}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.5314728319644927978515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27484}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.4557187557220458984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.485879266046599533890315569806261919438838958740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{24000118}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{24000118}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{24000118}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{24000118}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{689.1367647647857666015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{656.8893184930283268840867094695568084716796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{3175}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{632.65503084659576416015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{631.172809600830078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.7866903028205687320451033883728086948394775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.8142101764678955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.077662802689911103470876696519553661346435546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{20415}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.44411265850067138671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8237488269805908203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.23642150208266243804899886526982299983501434326171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.5789470672607421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.1628587988038727729644961073063313961029052734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11611}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.62857162952423095703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.099677562713623046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.2070768017832402829725424453499726951122283935546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22955606}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22955606}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22955606}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{22955606}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{698.627169132232666015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{660.9399111902476988689159043133258819580078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27714}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{637.130983650684356689453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{634.9583852291107177734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{12.4827780681021156539145522401668131351470947265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.591652393341064453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.071934587908106806253272225148975849151611328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.284303009510040283203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{16.9181766510009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.23366273037238283194483301485888659954071044921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.7125339508056640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.21119032790329317350597193581052124500274658203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.18486309051513671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5706513486772113452616395079530775547027587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{21967892}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{21967892}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21967892}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{21967892}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{811.9468135833740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28716}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{662.219250060075182773289270699024200439453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{638.013772308826446533203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{637.6327979564666748046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{19.428280196676492863616658723913133144378662109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.585767269134521484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.07211733022273136839430662803351879119873046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{4800}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.118317306041717529296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{16.9723641872406005859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2383721136785276473180061884704628027975559234619140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{179.824432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.302513274135975507306284271180629730224609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.872837066650390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{82.67822265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.48188325228561978974539670161902904510498046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20901076}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20901076}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20901076}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20901076}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{746.894912242889404296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{1185}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{660.5605209757950433413498103618621826171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{2549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{638.27348482608795166015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{634.84160518646240234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{13.623766141004484353516090777702629566192626953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.697875499725345349588678800500929355621337890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.070343795991103519327225512824952602386474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.2022559642791748046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{16.898882389068603515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2419166456821602306792584613504004664719104766845703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.6250514984130859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{22401}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{9.251300483349933045928992214612662792205810546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{9134}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.6317813396453857421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.075281620025634765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.219462901648069586002520736656151711940765380859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22972245}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22972245}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22972245}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{22972245}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{689.4099094867706298828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{9132}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{659.909265273454138878150843083858489990234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{23241}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{638.54987776279449462890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{637.2226717472076416015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.548743285754166976175838499329984188079833984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.71437549591064453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.07768972662110940063939779065549373626708984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{20013}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.329461753368377685546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{16.9263184070587158203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2355112611670164557420292794631677679717540740966796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{8.80197429656982421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.2154952990298237835986583377234637737274169921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29052}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.17984616756439208984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0430088043212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.57185251083535393323842299651005305349826812744140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22017809}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22017809}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22017809}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{22017809}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{687.1638462543487548828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{9132}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{659.7283722059615911348373629152774810791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5781}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{635.4398822784423828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{633.145431995391845703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.4141416118259737544349263771437108516693115234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.644696712493896484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.074208038532180609081478905864059925079345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{1895}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.216705322265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{16.95386028289794921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2347439753886131630356004507120815105736255645751953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{181.325698852539034078290569595992565155029296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{102.10632122115583797494764439761638641357421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{2306}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{86.661590576171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{81.919342041015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.5543243092486829226572808693163096904754638671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20921619}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20921619}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20921619}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20921619}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{688.4544150829315185546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{659.9071551853458004188723862171173095703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{3175}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{636.996083915233612060546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{631.320918560028076171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.8505629579552884678150803665630519390106201171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.682313442230224609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.072681466475227551882198895327746868133544921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{17194}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.227971732616424560546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{16.92615222930908203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2308204534779494665475141346178133971989154815673828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21186}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{187.469207763671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{104.0375475851905235913363867439329624176025390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1681}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{87.287982940673828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{26932}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{83.86852264404296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.91771665649914524465202703140676021575927734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20944369}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20944369}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20944369}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{20944369}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{687.3847596645355224609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{660.19139826218815869651734828948974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{3175}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{635.17659318447113037109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{634.2646424770355224609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.7874967116104354403205434209667146205902099609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.7311904430389404296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.080748610149157684645615518093109130859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{20751}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.403787910938262939453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{13036}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{16.922702789306640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2292357045298019091461583229829557240009307861328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000567512074660381227175776075455360114574432373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000000053632331183432882748824220558830881631630339131425495445733286903333691952866502106189727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.000000000000000000048069119756681544242127301913569681346416473388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000000016088188625428085707471888046448442635331117497103663570453234432644507023724145255982875823974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{20994}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{20994}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{20994}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{20994}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{32.51659393310546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{29052}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{20.5541418403979179174712044186890125274658203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{913}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{13.2870109081268310546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{10248}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{11.60878849029541015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.819185726656505242004868705407716333866119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{24946423}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{24946423}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{24946423}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{24946423}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000000005684661491997768345862978491497677261842301593215804017371339806885544021497480571269989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000053780384151751401254850923942423230404924026419395376445893586225821536572766490280628204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000000000000000004825949700686007804173711955374785889765081834477792634141568584027481847442686557769775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000157948991958693665718698287945026857471953322965906740086585412219388757648630416952073574066162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{687.6373424530029296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{6910}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{655.824951685027599523891694843769073486328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{2345}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{634.331499993801116943359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{633.39380168914794921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{29022}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{12.8891102165949060776029000408016145229339599609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.55406951904296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{12493}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.04976643789682810847807559184730052947998046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{10248}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.119303047657012939453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8307476043701171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.2356905391159523632804706494425772689282894134521484375}
\def\SubcubicEffectiveDimensionalityEstimateLen{7852}
\def\SubcubicEffectiveDimensionalityEstimateMaxFloat{37122}
\def\SubcubicEffectiveDimensionalityEstimateMeanFloat{21057.23076923076951061375439167022705078125}
\def\SubcubicEffectiveDimensionalityEstimateMedianFloat{16770}
\def\SubcubicEffectiveDimensionalityEstimateMinFloat{16770}
\def\SubcubicEffectiveDimensionalityEstimateStdDevFloat{7202.4058176508069664123468101024627685546875}
\def\SubcubicErrUpperBoundLen{7852}
\def\SubcubicErrUpperBoundMaxFloat{187.469207763671875}
\def\SubcubicErrUpperBoundMeanFloat{27.9980025446299549685136298649013042449951171875}
\def\SubcubicErrUpperBoundMedianFloat{0}
\def\SubcubicErrUpperBoundMinFloat{0}
\def\SubcubicErrUpperBoundStdDevFloat{41.58819632564287616105502820573747158050537109375}
\def\SubcubicGapMostBelowValueLen{7852}
\def\SubcubicGapMostBelowValueMaxFloat{78}
\def\SubcubicGapMostBelowValueMeanFloat{18.684156902699950109081328264437615871429443359375}
\def\SubcubicGapMostBelowValueMedianFloat{1}
\def\SubcubicGapMostBelowValueMinFloat{1}
\def\SubcubicGapMostBelowValueNumStdLen{7852}
\def\SubcubicGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicGapMostBelowValueSequenceFracLen{7852}
\def\SubcubicGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicGapMostBelowValueSequenceFracMeanFloat{0.9957502572984642252862386158085428178310394287109375}
\def\SubcubicGapMostBelowValueSequenceFracMedianFloat{0.97864236891269673623838798448559828102588653564453125}
\def\SubcubicGapMostBelowValueSequenceFracMinFloat{0.930698871612548828125}
\def\SubcubicGapMostBelowValueSequenceFracStdDevFloat{0.004524371510118242907527719154359147069044411182403564453125}
\def\SubcubicGapMostBelowValueStdDevFloat{17.66783541329773044026296702213585376739501953125}
\def\SubcubicGroupAccuracyLen{1208}
\def\SubcubicGroupAccuracyMaxFloat{0.680767187184961652945958121563307940959930419921875}
\def\SubcubicGroupAccuracyMeanFloat{0.466288457919763532633083968903520144522190093994140625}
\def\SubcubicGroupAccuracyMedianFloat{0.15212515543627780356672474226797930896282196044921875}
\def\SubcubicGroupAccuracyMinFloat{0.0000000000000000000516690097825123206831676725414581596851348876953125}
\def\SubcubicGroupAccuracyStdDevFloat{0.1362834642000913809578577229331131093204021453857421875}
\def\SubcubicGroupDroppedSequencesFracLen{1208}
\def\SubcubicGroupDroppedSequencesFracMaxFloat{0.177818069393813893430689176966552622616291046142578125}
\def\SubcubicGroupDroppedSequencesFracMeanFloat{0.1340159877902248608538826601943583227694034576416015625}
\def\SubcubicGroupDroppedSequencesFracMedianFloat{0.0804033300257335492577936975067132152616977691650390625}
\def\SubcubicGroupDroppedSequencesFracMinFloat{0.00059480387568049998547881074273391277529299259185791015625}
\def\SubcubicGroupDroppedSequencesFracStdDevFloat{0.01497981536499314904331559006323004723526537418365478515625}
\def\SubcubicGroupDroppedSequencesLen{1208}
\def\SubcubicGroupDroppedSequencesMaxFloat{209930522738483897340}
\def\SubcubicGroupDroppedSequencesMeanFloat{158218152227306373120}
\def\SubcubicGroupDroppedSequencesMedianFloat{94923497706157752320}
\def\SubcubicGroupDroppedSequencesMinFloat{702220471598645146}
\def\SubcubicGroupDroppedSequencesStdDevFloat{17685044499804841984}
\def\SubcubicGroupEffectiveDimensionalityEstimateLen{1208}
\def\SubcubicGroupEffectiveDimensionalityEstimateMaxFloat{33152}
\def\SubcubicGroupEffectiveDimensionalityEstimateMeanFloat{25089}
\def\SubcubicGroupEffectiveDimensionalityEstimateMedianFloat{17026}
\def\SubcubicGroupEffectiveDimensionalityEstimateMinFloat{17026}
\def\SubcubicGroupEffectiveDimensionalityEstimateStdDevFloat{7937.0161269837417421513237059116363525390625}
\def\SubcubicGroupErrUpperBoundLen{1208}
\def\SubcubicGroupErrUpperBoundMaxFloat{4.456815242767333984375}
\def\SubcubicGroupErrUpperBoundMeanFloat{1.2265328500444525605672652091016061604022979736328125}
\def\SubcubicGroupErrUpperBoundMedianFloat{0}
\def\SubcubicGroupErrUpperBoundMinFloat{0}
\def\SubcubicGroupErrUpperBoundStdDevFloat{1.2737433661555057629044540590257383882999420166015625}
\def\SubcubicGroupGapMostBelowValueLen{1208}
\def\SubcubicGroupGapMostBelowValueMaxFloat{15}
\def\SubcubicGroupGapMostBelowValueMeanFloat{8.732615894039735593423756654374301433563232421875}
\def\SubcubicGroupGapMostBelowValueMedianFloat{6}
\def\SubcubicGroupGapMostBelowValueMinFloat{2}
\def\SubcubicGroupGapMostBelowValueNumStdLen{1208}
\def\SubcubicGroupGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicGroupGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicGroupGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicGroupGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicGroupGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicGroupGapMostBelowValueSequenceFracLen{1208}
\def\SubcubicGroupGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicGroupGapMostBelowValueSequenceFracMeanFloat{0.993400606049212431258865763084031641483306884765625}
\def\SubcubicGroupGapMostBelowValueSequenceFracMedianFloat{0.97097460687160486170199646949185989797115325927734375}
\def\SubcubicGroupGapMostBelowValueSequenceFracMinFloat{0.94749915599822998046875}
\def\SubcubicGroupGapMostBelowValueSequenceFracStdDevFloat{0.005004783183299173210389909627338056452572345733642578125}
\def\SubcubicGroupGapMostBelowValueStdDevFloat{1.5399306914864110407137332003912888467311859130859375}
\def\SubcubicGroupInstructionCountBranchLen{1208}
\def\SubcubicGroupInstructionCountBranchMaxFloat{0}
\def\SubcubicGroupInstructionCountBranchMeanFloat{0}
\def\SubcubicGroupInstructionCountBranchMedianFloat{0}
\def\SubcubicGroupInstructionCountBranchMinFloat{0}
\def\SubcubicGroupInstructionCountBranchStdDevFloat{0}
\def\SubcubicGroupInstructionCountIntLen{1208}
\def\SubcubicGroupInstructionCountIntMaxFloat{0}
\def\SubcubicGroupInstructionCountIntMeanFloat{0}
\def\SubcubicGroupInstructionCountIntMedianFloat{0}
\def\SubcubicGroupInstructionCountIntMinFloat{0}
\def\SubcubicGroupInstructionCountIntStdDevFloat{0}
\def\SubcubicGroupInstructionCountLen{1208}
\def\SubcubicGroupInstructionCountMaxFloat{25098133}
\def\SubcubicGroupInstructionCountMeanFloat{23825013}
\def\SubcubicGroupInstructionCountMedianFloat{22551893}
\def\SubcubicGroupInstructionCountMinFloat{22551893}
\def\SubcubicGroupInstructionCountStdDevFloat{1060306.335011019371449947357177734375}
\def\SubcubicGroupMaxGapLen{1208}
\def\SubcubicGroupMaxGapMaxFloat{80}
\def\SubcubicGroupMaxGapMeanFloat{67.1034768211920464864306268282234668731689453125}
\def\SubcubicGroupMaxGapMedianFloat{13}
\def\SubcubicGroupMaxGapMinFloat{2}
\def\SubcubicGroupMaxGapStdDevFloat{13.55367259792883061209067818708717823028564453125}
\def\SubcubicGroupNormalizedAccuracyLen{1208}
\def\SubcubicGroupNormalizedAccuracyMaxFloat{0.6825276323316076254599238382070325314998626708984375}
\def\SubcubicGroupNormalizedAccuracyMeanFloat{0.467505206080687685243901796638965606689453125}
\def\SubcubicGroupNormalizedAccuracyMedianFloat{0.1526279452250713097871681611650274135172367095947265625}
\def\SubcubicGroupNormalizedAccuracyMinFloat{0.00000000000000000005348064349145917742309062037520150949918531287392768993650682407547947150305844843387603759765625}
\def\SubcubicGroupNormalizedAccuracyStdDevFloat{0.13660665672806449055798339031753130257129669189453125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.680767187184961652945958121563307940959930419921875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMaxKey{20539}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.611536797242929086593221654766239225864410400390625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMeanKey{19004}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.455491427068714871406740485326736234128475189208984375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMedianKey{15043}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMinFloat{0.423659542949948619838806962434318847954273223876953125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0376388457021663846990833235395257361233234405517578125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.16661087469430480023646623521926812827587127685546875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{21598}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1264689933521866149757073571890941821038722991943359375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{32382}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0943357552755732797766796693395008333027362823486328125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07497542497862159927013436799825285561382770538330078125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0120868507283927832662850931910725194029510021209716796875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{196699402584494945925}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{21598}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{149308233832157511680}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{32382}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{111372002212390158336}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{88515358489487607977}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{14269634690802659328}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{33152}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{123}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{29227.50993377483609947375953197479248046875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{104}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17026}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{5615}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{17026}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{5615}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{6834.46898470403903047554194927215576171875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{3.277657032012939453125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19004}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0.6175665397517728916199075683834962546825408935546875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{104}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{104}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMinKey{104}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.1008094471074751918848733112099580466747283935546875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{12}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.344370860927153188413285533897578716278076171875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.75}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9997761249542236328125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9945253350876814835146433324553072452545166015625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{31308}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98166821897029876708984375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4800}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9770338535308837890625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{8048}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.003979935204912711348146370227141233044676482677459716796875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.361953980103265404721923914621584117412567138671875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMaxFloat{25098133}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMaxKey{5615}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMeanFloat{23503684.576158940792083740234375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMeanKey{104}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMedianFloat{22990805}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMedianKey{123}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMinFloat{22990805}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMinKey{123}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{893239.034812845173291862010955810546875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMaxFloat{75}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMaxKey{104}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMeanFloat{69.90728476821192316492670215666294097900390625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMedianFloat{53.25}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMedianKey{7310}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMinFloat{18}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMinKey{8048}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.80114637714797254375298507511615753173828125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6825276323316076254599238382070325314998626708984375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20539}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.61319167775718252944017194749903865158557891845703125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{19093}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.46061035190664423311091013601981103420257568359375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15043}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.438514015918480659639300256458227522671222686767578125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.037204636552178003972013442535171634517610073089599609375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{681.13336849212646484375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{6204}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{662.540686034208874843898229300975799560546875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{9504}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{631.74485743045806884765625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4157}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{629.673713207244873046875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{11.5075733176545345060048930463381111621856689453125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMaxFloat{20.037389039993289685526178800500929355621337890625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMaxKey{1951}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.141582253752954301262434455566108226776123046875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMeanKey{11130}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.556410849094390869140625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMedianKey{5928}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMinFloat{17.107997894287109375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMinKey{2236}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.270387021170584274099013555314741097390651702880859375}
\def\SubcubicGroupProofSearchTimeLen{1208}
\def\SubcubicGroupProofSearchTimeMaxFloat{686.4096052646636962890625}
\def\SubcubicGroupProofSearchTimeMeanFloat{658.56767420460846551577560603618621826171875}
\def\SubcubicGroupProofSearchTimeMedianFloat{626.9316808247566541467676870524883270263671875}
\def\SubcubicGroupProofSearchTimeMinFloat{619.4910361766815185546875}
\def\SubcubicGroupProofSearchTimeStdDevFloat{11.4388326229623800145418499596416950225830078125}
\def\SubcubicGroupProofTimeLen{1208}
\def\SubcubicGroupProofTimeMaxFloat{20.23934078216552734375}
\def\SubcubicGroupProofTimeMeanFloat{18.109255618014874045229589683003723621368408203125}
\def\SubcubicGroupProofTimeMedianFloat{17.112746442556382220345767564140260219573974609375}
\def\SubcubicGroupProofTimeMinFloat{16.994822025299072265625}
\def\SubcubicGroupProofTimeStdDevFloat{0.2561063362577369328931808922789059579372406005859375}
\def\SubcubicInstructionCountBranchLen{7852}
\def\SubcubicInstructionCountBranchMaxFloat{0}
\def\SubcubicInstructionCountBranchMeanFloat{0}
\def\SubcubicInstructionCountBranchMedianFloat{0}
\def\SubcubicInstructionCountBranchMinFloat{0}
\def\SubcubicInstructionCountBranchStdDevFloat{0}
\def\SubcubicInstructionCountIntLen{7852}
\def\SubcubicInstructionCountIntMaxFloat{0}
\def\SubcubicInstructionCountIntMeanFloat{0}
\def\SubcubicInstructionCountIntMedianFloat{0}
\def\SubcubicInstructionCountIntMinFloat{0}
\def\SubcubicInstructionCountIntStdDevFloat{0}
\def\SubcubicInstructionCountLen{7852}
\def\SubcubicInstructionCountMaxFloat{26044438}
\def\SubcubicInstructionCountMeanFloat{23108652.73076923191547393798828125}
\def\SubcubicInstructionCountMedianFloat{21486773}
\def\SubcubicInstructionCountMinFloat{21486773}
\def\SubcubicInstructionCountStdDevFloat{1275162.2240443206392228603363037109375}
\def\SubcubicMaxGapLen{7852}
\def\SubcubicMaxGapMaxFloat{100}
\def\SubcubicMaxGapMeanFloat{64.37404482934283578288159333169460296630859375}
\def\SubcubicMaxGapMedianFloat{1}
\def\SubcubicMaxGapMinFloat{1}
\def\SubcubicMaxGapStdDevFloat{24.36971772338574737659655511379241943359375}
\def\SubcubicNormalizedAccuracyLen{7852}
\def\SubcubicNormalizedAccuracyMaxFloat{0.6908253841360181279895869010942988097667694091796875}
\def\SubcubicNormalizedAccuracyMeanFloat{0.337551030687933073526352245607995428144931793212890625}
\def\SubcubicNormalizedAccuracyMedianFloat{0.000000000000000000050964114366684052336036402036975125661073931295965628901663280192479987817932851612567901611328125}
\def\SubcubicNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicNormalizedAccuracyStdDevFloat{0.1964490613371009108956144473268068395555019378662109375}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.68942794737815604744213260346441529691219329833984375}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.6215540411111633023466538361390121281147003173828125}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMeanKey{10248}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.51075811320631547829407281824387609958648681640625}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMedianKey{8893}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMinFloat{0.43620027112436698946140722910058684647083282470703125}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0309164882979499518189658857636459288187325000762939453125}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.16661087469430480023646623521926812827587127685546875}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{21598}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1288859268529858326246539945714175701141357421875}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{5358}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08450994778538080398622156508281477726995944976806640625}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{742}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.035672195017851703047195854878737009130418300628662109375}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.013745702360534566011107671101854066364467144012451171875}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{196699402584494945925}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{21598}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{152161645271032266752}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{5358}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{99771736222686543872}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{742}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{42114294530673152936}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{16228061027722649600}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{37122}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{31502.5562913907269830815494060516357421875}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{1185}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{17010}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{27671}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{16962}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{104}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{7153.9362023454350492102093994617462158203125}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{9.74072265625}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{2306}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0.70201981304497118596685822922154329717159271240234375}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6156005135075786061094049728126265108585357666015625}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{104}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.75496688741721840187892667017877101898193359375}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1895}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.25}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1696}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9997761249542236328125}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13468}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99369900866060068000962246514973230659961700439453125}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4430}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9738725125789642333984375}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8048}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96438848972320556640625}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0044530000237323168199576883807822014205157756805419921875}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.46918406610458784911088514490984380245208740234375}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMaxFloat{25098133}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMaxKey{27671}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22901614.4900662265717983245849609375}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMeanKey{519}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21929781}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMinFloat{21929781}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{1003512.8554835920222103595733642578125}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMaxFloat{79}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMaxKey{20976}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMeanFloat{70.14569536423840645511518232524394989013671875}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMedianFloat{45.75}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMinFloat{18}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMinKey{8048}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapStdDevFloat{5.2995031017766276448810458532534539699554443359375}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6908253841360181279895869010942988097667694091796875}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6232344809258016926634127230499871075153350830078125}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{31308}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5167436093843142952408697965438477694988250732421875}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8893}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.451494450717646544912753370226710103452205657958984375}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0302768803838888538038087716586233000271022319793701171875}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{681.8326740264892578125}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{23696}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{661.221284338970008320757187902927398681640625}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7884}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{633.805510103702545166015625}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{1681}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{629.673713207244873046875}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.638154569704614260672315140254795551300048828125}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.6453669071197509765625}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMaxKey{9504}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.108917710007421675300065544433891773223876953125}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMeanKey{519}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMedianFloat{17.047219097614288330078125}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8648827075958251953125}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.236865488828590431413800843074568547308444976806640625}
\def\SubcubicProofSearchTimeLen{7852}
\def\SubcubicProofSearchTimeMaxFloat{797.13279056549072265625}
\def\SubcubicProofSearchTimeMeanFloat{658.400627174124792873044498264789581298828125}
\def\SubcubicProofSearchTimeMedianFloat{628.396376689672479187720455229282379150390625}
\def\SubcubicProofSearchTimeMinFloat{619.2171604633331298828125}
\def\SubcubicProofSearchTimeStdDevFloat{11.7949536159866372742044404731132090091705322265625}
\def\SubcubicProofTimeLen{7852}
\def\SubcubicProofTimeMaxFloat{20.580661296844478869161321199499070644378662109375}
\def\SubcubicProofTimeMeanFloat{18.101830109521191758403801941312849521636962890625}
\def\SubcubicProofTimeMedianFloat{17.136336152553557354849544935859739780426025390625}
\def\SubcubicProofTimeMinFloat{16.8237488269805908203125}
\def\SubcubicProofTimeStdDevFloat{0.251507911813992068861267625834443606436252593994140625}
\def\SubcubicVocabModelSquaredAccuracyLen{7248}
\def\SubcubicVocabModelSquaredAccuracyMaxFloat{0.6796071498866778082259543225518427789211273193359375}
\def\SubcubicVocabModelSquaredAccuracyMeanFloat{0.12548384515110200254639494232833385467529296875}
\def\SubcubicVocabModelSquaredAccuracyMedianFloat{0.0000000000000000000482808779934951193268943825387395918369293212890625}
\def\SubcubicVocabModelSquaredAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicVocabModelSquaredAccuracyStdDevFloat{0.1926434710770391911527354977806680835783481597900390625}
\def\SubcubicVocabModelSquaredDroppedSequencesFracLen{7248}
\def\SubcubicVocabModelSquaredDroppedSequencesFracMaxFloat{0.364304421671816702765767104210681281983852386474609375}
\def\SubcubicVocabModelSquaredDroppedSequencesFracMeanFloat{0.13557632494294813430002477616653777658939361572265625}
\def\SubcubicVocabModelSquaredDroppedSequencesFracMedianFloat{0}
\def\SubcubicVocabModelSquaredDroppedSequencesFracMinFloat{0}
\def\SubcubicVocabModelSquaredDroppedSequencesFracStdDevFloat{0.11671982252894892717609565124803339131176471710205078125}
\def\SubcubicVocabModelSquaredDroppedSequencesLen{7248}
\def\SubcubicVocabModelSquaredDroppedSequencesMaxFloat{430094747616049389880}
\def\SubcubicVocabModelSquaredDroppedSequencesMeanFloat{160060273195305926656}
\def\SubcubicVocabModelSquaredDroppedSequencesMedianFloat{0}
\def\SubcubicVocabModelSquaredDroppedSequencesMinFloat{0}
\def\SubcubicVocabModelSquaredDroppedSequencesStdDevFloat{137798444449298235392}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateLen{7248}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateMeanFloat{21071.33333333333212067373096942901611328125}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateMedianFloat{20866}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateMinFloat{20866}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateStdDevFloat{95.962955815715105245544691570103168487548828125}
\def\SubcubicVocabModelSquaredErrUpperBoundLen{7248}
\def\SubcubicVocabModelSquaredErrUpperBoundMaxFloat{187.469207763671875}
\def\SubcubicVocabModelSquaredErrUpperBoundMeanFloat{44.73017110374589577759252279065549373626708984375}
\def\SubcubicVocabModelSquaredErrUpperBoundMedianFloat{4.249743938446044921875}
\def\SubcubicVocabModelSquaredErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicVocabModelSquaredErrUpperBoundStdDevFloat{45.62499476805830767034422024153172969818115234375}
\def\SubcubicVocabModelSquaredGapMostBelowValueLen{7248}
\def\SubcubicVocabModelSquaredGapMostBelowValueMaxFloat{76}
\def\SubcubicVocabModelSquaredGapMostBelowValueMeanFloat{16.8125}
\def\SubcubicVocabModelSquaredGapMostBelowValueMedianFloat{1}
\def\SubcubicVocabModelSquaredGapMostBelowValueMinFloat{1}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdLen{7248}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracLen{7248}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracMeanFloat{0.99788155460989236278379621580825187265872955322265625}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracMedianFloat{0.983848989009857177734375}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracMinFloat{0.972655713558197021484375}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracStdDevFloat{0.0032958865445513944696098729281175110372714698314666748046875}
\def\SubcubicVocabModelSquaredGapMostBelowValueStdDevFloat{18.057854761417178934834737447090446949005126953125}
\def\SubcubicVocabModelSquaredInstructionCountBranchLen{7248}
\def\SubcubicVocabModelSquaredInstructionCountBranchMaxFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountBranchMeanFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountBranchMedianFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountBranchMinFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountBranchStdDevFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntLen{7248}
\def\SubcubicVocabModelSquaredInstructionCountIntMaxFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntMeanFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntMedianFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntMinFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntStdDevFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountLen{7248}
\def\SubcubicVocabModelSquaredInstructionCountMaxFloat{24950519}
\def\SubcubicVocabModelSquaredInstructionCountMeanFloat{21986654.5416666679084300994873046875}
\def\SubcubicVocabModelSquaredInstructionCountMedianFloat{20462164}
\def\SubcubicVocabModelSquaredInstructionCountMinFloat{20462164}
\def\SubcubicVocabModelSquaredInstructionCountStdDevFloat{1326673.773891054093837738037109375}
\def\SubcubicVocabModelSquaredMaxGapLen{7248}
\def\SubcubicVocabModelSquaredMaxGapMaxFloat{98}
\def\SubcubicVocabModelSquaredMaxGapMeanFloat{43.05091059602649039561583776958286762237548828125}
\def\SubcubicVocabModelSquaredMaxGapMedianFloat{1}
\def\SubcubicVocabModelSquaredMaxGapMinFloat{1}
\def\SubcubicVocabModelSquaredMaxGapStdDevFloat{35.22856661721715454405057244002819061279296875}
\def\SubcubicVocabModelSquaredNormalizedAccuracyLen{7248}
\def\SubcubicVocabModelSquaredNormalizedAccuracyMaxFloat{0.6809846803679546756171703236759640276432037353515625}
\def\SubcubicVocabModelSquaredNormalizedAccuracyMeanFloat{0.1258177627324481573367620512726716697216033935546875}
\def\SubcubicVocabModelSquaredNormalizedAccuracyMedianFloat{0.000000000000000000048395942402973877046403457273086360814637485857644968556372233603468657747725956141948699951171875}
\def\SubcubicVocabModelSquaredNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicVocabModelSquaredNormalizedAccuracyStdDevFloat{0.1931474209755101034691193717662827111780643463134765625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6796071498866778082259543225518427789211273193359375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.59455275346375746625682268131640739738941192626953125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMeanKey{28778}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.484250002205975083047206908304360695183277130126953125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMedianKey{8893}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMinFloat{0.429902799932262824622597463530837558209896087646484375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0302314729461720388403733750237734057009220123291015625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.17099584457808558735081305712810717523097991943359375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1408756907135202129932594061756390146911144256591796875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{6204}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0904955427191748984494523710964131169021129608154296875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6910}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0398087857448077009347997545773978345096111297607421875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.012794253492768005442403733695755363442003726959228515625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{201876261286384720189}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{166316660019159760896}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{6204}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{106838279446532456448}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6910}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{46997918881254736532}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{15104788466896386048}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{104}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21116.49006622516390052624046802520751953125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{63.76237628725061057366474415175616741180419921875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{10.785564422607421875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.6170718148844134276487238821573555469512939453125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22261}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.17872369289398193359375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.3341311894246901115224090972333215177059173583984375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{15}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10.5165562913907280062630889005959033966064453125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6.25}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999437987804412841796875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99485807071458420836052027880214154720306396484375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19917}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97918491065502155645816628748434595763683319091796875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8048}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97576397657394398077457253748434595763683319091796875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.003335920797967724914234732835893737501464784145355224609375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.5218249093697668872238182302680797874927520751953125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22976341}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMaxKey{1696}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22103573.1192052997648715972900390625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMeanKey{104}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21971988}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMinFloat{21971988}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{309661.810038024443201720714569091796875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMaxFloat{84}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMeanFloat{71.1324503311258240501047112047672271728515625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMedianFloat{32.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMedianKey{32103}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMinFloat{22}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMinKey{24566}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapStdDevFloat{6.4177686872486834346318573807366192340850830078125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6809846803679546756171703236759640276432037353515625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.59615438711854584763472075792378745973110198974609375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{28778}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.490046106611645548856159848583047278225421905517578125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8893}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.444976175776046145582398594342521391808986663818359375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0294902716131977583879919535547742270864546298980712890625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{686.929138660430908203125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{13468}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{661.0921927145774361633812077343463897705078125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5928}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{639.058513820171356201171875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{23241}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{637.7066695690155029296875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinKey{519}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.293473198988952077570502297021448612213134765625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.69706630706787109375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMaxKey{30899}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.116891039917799588465641136281192302703857421875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMeanKey{7238}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMedianFloat{16.95589458942413330078125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8429481983184814453125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.27346456453601419855914400613983161747455596923828125}
\def\SubcubicVocabModelSquaredProofSearchTimeLen{7248}
\def\SubcubicVocabModelSquaredProofSearchTimeMaxFloat{1046.6073901653289794921875}
\def\SubcubicVocabModelSquaredProofSearchTimeMeanFloat{657.9655069793362827113014645874500274658203125}
\def\SubcubicVocabModelSquaredProofSearchTimeMedianFloat{631.0056577396393322487710975110530853271484375}
\def\SubcubicVocabModelSquaredProofSearchTimeMinFloat{621.452413082122802734375}
\def\SubcubicVocabModelSquaredProofSearchTimeStdDevFloat{14.2158335499789263423053853330202400684356689453125}
\def\SubcubicVocabModelSquaredProofTimeLen{7248}
\def\SubcubicVocabModelSquaredProofTimeMaxFloat{20.391441822051998400411321199499070644378662109375}
\def\SubcubicVocabModelSquaredProofTimeMeanFloat{18.076116302089712206679905648343265056610107421875}
\def\SubcubicVocabModelSquaredProofTimeMedianFloat{16.97225365877151403992684208787977695465087890625}
\def\SubcubicVocabModelSquaredProofTimeMinFloat{16.755332469940185546875}
\def\SubcubicVocabModelSquaredProofTimeStdDevFloat{0.25222562499947243086495518582523800432682037353515625}
\def\SubcubicWithoutVocabSquaredAccuracyLen{4530}
\def\SubcubicWithoutVocabSquaredAccuracyMaxFloat{0.6796071498866778082259543225518427789211273193359375}
\def\SubcubicWithoutVocabSquaredAccuracyMeanFloat{0.1435505572753912606476234259389457292854785919189453125}
\def\SubcubicWithoutVocabSquaredAccuracyMedianFloat{0.0000000000000000000482808779934951193268943825387395918369293212890625}
\def\SubcubicWithoutVocabSquaredAccuracyMinFloat{0.0000000000000000000474338450462408189878260600380599498748779296875}
\def\SubcubicWithoutVocabSquaredAccuracyStdDevFloat{0.2148708161267245675407622229613480158150196075439453125}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracLen{4530}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracMaxFloat{0.287210202143366177818251117059844546020030975341796875}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracMeanFloat{0.09799990621079497643552969066149671562016010284423828125}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracMedianFloat{0}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracMinFloat{0}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracStdDevFloat{0.07551148007521389649010501443626708351075649261474609375}
\def\SubcubicWithoutVocabSquaredDroppedSequencesLen{4530}
\def\SubcubicWithoutVocabSquaredDroppedSequencesMaxFloat{339077958035012023165}
\def\SubcubicWithoutVocabSquaredDroppedSequencesMeanFloat{115697868103557021696}
\def\SubcubicWithoutVocabSquaredDroppedSequencesMedianFloat{0}
\def\SubcubicWithoutVocabSquaredDroppedSequencesMinFloat{0}
\def\SubcubicWithoutVocabSquaredDroppedSequencesStdDevFloat{89148220644767121408}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateLen{4530}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateMeanFloat{21053.73333333333357586525380611419677734375}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateMedianFloat{20866}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateMinFloat{20866}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateStdDevFloat{97.66846414728189529341761954128742218017578125}
\def\SubcubicWithoutVocabSquaredErrUpperBoundLen{4530}
\def\SubcubicWithoutVocabSquaredErrUpperBoundMaxFloat{32.51659393310546875}
\def\SubcubicWithoutVocabSquaredErrUpperBoundMeanFloat{9.8789973498969683163295485428534448146820068359375}
\def\SubcubicWithoutVocabSquaredErrUpperBoundMedianFloat{4.2336444854736328125}
\def\SubcubicWithoutVocabSquaredErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicWithoutVocabSquaredErrUpperBoundStdDevFloat{5.94281420694294837403504061512649059295654296875}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueLen{4530}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueMaxFloat{35}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueMeanFloat{8.4479028697571738604210622725076973438262939453125}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueMedianFloat{1}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueMinFloat{1}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdLen{4530}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracLen{4530}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracMeanFloat{0.99681271205411581259880904326564632356166839599609375}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracMedianFloat{0.98255943834781633849928539348184131085872650146484375}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracMinFloat{0.972655713558197021484375}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracStdDevFloat{0.003761865165272049171818480317597277462482452392578125}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueStdDevFloat{6.5474698123937997706889291293919086456298828125}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchLen{4530}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchMaxFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchMeanFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchMedianFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchMinFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntLen{4530}
\def\SubcubicWithoutVocabSquaredInstructionCountIntMaxFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntMeanFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntMedianFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntMinFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountLen{4530}
\def\SubcubicWithoutVocabSquaredInstructionCountMaxFloat{24950519}
\def\SubcubicWithoutVocabSquaredInstructionCountMeanFloat{22755269.6666666679084300994873046875}
\def\SubcubicWithoutVocabSquaredInstructionCountMedianFloat{21528980}
\def\SubcubicWithoutVocabSquaredInstructionCountMinFloat{21528980}
\def\SubcubicWithoutVocabSquaredInstructionCountStdDevFloat{1100740.811203174293041229248046875}
\def\SubcubicWithoutVocabSquaredMaxGapLen{4530}
\def\SubcubicWithoutVocabSquaredMaxGapMaxFloat{89}
\def\SubcubicWithoutVocabSquaredMaxGapMeanFloat{37.611479028697573312456370331346988677978515625}
\def\SubcubicWithoutVocabSquaredMaxGapMedianFloat{1}
\def\SubcubicWithoutVocabSquaredMaxGapMinFloat{1}
\def\SubcubicWithoutVocabSquaredMaxGapStdDevFloat{32.0125810088094340244424529373645782470703125}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyLen{4530}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyMaxFloat{0.6809846803679546756171703236759640276432037353515625}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyMeanFloat{0.143930430846074208783846870574052445590496063232421875}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyMedianFloat{0.000000000000000000048395942402973877046403457273086360814637485857644968556372233603468657747725956141948699951171875}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyMinFloat{0.000000000000000000047850160818518668990675953975508271546828674650381058833410741204517080404912121593952178955078125}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyStdDevFloat{0.2154289274349310556733172461463254876434803009033203125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6796071498866778082259543225518427789211273193359375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMaxKey{17080}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.59455275346375746625682268131640739738941192626953125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMeanKey{28778}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.484250002205975083047206908304360695183277130126953125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMedianKey{8893}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMinFloat{0.429902799932262824622597463530837558209896087646484375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMinKey{20013}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0302314729461720388403733750237734057009220123291015625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.17099584457808558735081305712810717523097991943359375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{13468}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1408756907135202129932594061756390146911144256591796875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{6204}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0904955427191748984494523710964131169021129608154296875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6910}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0398087857448077009347997545773978345096111297607421875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20013}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.012794253492768005442403733695755363442003726959228515625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{201876261286384720189}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{13468}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{166316660019159760896}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{6204}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{106838279446532456448}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6910}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{46997918881254736532}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20013}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{15104788466896386048}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{21186}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{104}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{21116.49006622516390052624046802520751953125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{21058}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{21058}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{63.76237628725061057366474415175616741180419921875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{10.785564422607421875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20013}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.6170718148844134276487238821573555469512939453125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22261}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{4.17872369289398193359375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{17080}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{4.0385189056396484375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinKey{2549}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.3341311894246901115224090972333215177059173583984375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{15}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{10.5165562913907280062630889005959033966064453125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6.25}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6910}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20013}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999437987804412841796875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99485807071458420836052027880214154720306396484375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19917}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97918491065502155645816628748434595763683319091796875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8048}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97576397657394398077457253748434595763683319091796875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20013}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.003335920797967724914234732835893737501464784145355224609375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.5218249093697668872238182302680797874927520751953125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMaxFloat{22976341}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMaxKey{1696}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMeanFloat{22103573.1192052997648715972900390625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMeanKey{104}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMedianFloat{21971988}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMinFloat{21971988}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{309661.810038024443201720714569091796875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMaxFloat{84}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMaxKey{4729}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMeanFloat{71.1324503311258240501047112047672271728515625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMedianFloat{32.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMedianKey{32103}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMinFloat{22}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMinKey{24566}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapStdDevFloat{6.4177686872486834346318573807366192340850830078125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6809846803679546756171703236759640276432037353515625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{17080}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.59615438711854584763472075792378745973110198974609375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{28778}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.490046106611645548856159848583047278225421905517578125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8893}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.444976175776046145582398594342521391808986663818359375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20013}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0294902716131977583879919535547742270864546298980712890625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{686.929138660430908203125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{13468}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{661.0921927145774361633812077343463897705078125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5928}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{639.058513820171356201171875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{23241}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{637.7066695690155029296875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinKey{519}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.293473198988952077570502297021448612213134765625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMaxFloat{18.69706630706787109375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMaxKey{30899}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMeanFloat{18.116891039917799588465641136281192302703857421875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMeanKey{7238}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMedianFloat{16.95589458942413330078125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMedianKey{2236}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMinFloat{16.8429481983184814453125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMinKey{1951}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.27346456453601419855914400613983161747455596923828125}
\def\SubcubicWithoutVocabSquaredProofSearchTimeLen{4530}
\def\SubcubicWithoutVocabSquaredProofSearchTimeMaxFloat{958.2426109313963706881622783839702606201171875}
\def\SubcubicWithoutVocabSquaredProofSearchTimeMeanFloat{657.81840790118076256476342678070068359375}
\def\SubcubicWithoutVocabSquaredProofSearchTimeMedianFloat{630.6859942018985520917340181767940521240234375}
\def\SubcubicWithoutVocabSquaredProofSearchTimeMinFloat{621.452413082122802734375}
\def\SubcubicWithoutVocabSquaredProofSearchTimeStdDevFloat{13.926395273736460467262077145278453826904296875}
\def\SubcubicWithoutVocabSquaredProofTimeLen{4530}
\def\SubcubicWithoutVocabSquaredProofTimeMaxFloat{20.391441822051998400411321199499070644378662109375}
\def\SubcubicWithoutVocabSquaredProofTimeMeanFloat{18.0774516937748472855673753656446933746337890625}
\def\SubcubicWithoutVocabSquaredProofTimeMedianFloat{16.975498992204666848238048260100185871124267578125}
\def\SubcubicWithoutVocabSquaredProofTimeMinFloat{16.755332469940185546875}
\def\SubcubicWithoutVocabSquaredProofTimeStdDevFloat{0.25703631624856948523216715329908765852451324462890625}
\def\TrainAccuracyLen{151}
\def\TrainAccuracyMaxFloat{0.9988749999999999573674358543939888477325439453125}
\def\TrainAccuracyMaxKey{4647}
\def\TrainAccuracyMeanFloat{0.99684407767660065946557779170689173042774200439453125}
\def\TrainAccuracyMeanKey{19538}
\def\TrainAccuracyMedianFloat{0.9818404947916665737039920713868923485279083251953125}
\def\TrainAccuracyMedianKey{16284}
\def\TrainAccuracyMinFloat{0.9690026041666666145601993775926530361175537109375}
\def\TrainAccuracyMinKey{20013}
\def\TrainAccuracyStdDevFloat{0.0032198409026528685382417815930011784075759351253509521484375}
\def\TrainLossLen{151}
\def\TrainLossMaxFloat{0.1226821899283677408387660534572205506265163421630859375}
\def\TrainLossMaxKey{20013}
\def\TrainLossMeanFloat{0.0141150320832335272880353471691705635748803615570068359375}
\def\TrainLossMeanKey{3284}
\def\TrainLossMedianFloat{0.006095861948138918233464078610950309666804969310760498046875}
\def\TrainLossMedianKey{1283}
\def\TrainLossMinFloat{0.005824383022394613758365711220221783150918781757354736328125}
\def\TrainLossMinKey{1951}
\def\TrainLossStdDevFloat{0.0141694236639412531053583421680741594173014163970947265625}
\def\UpperWhiskerCrosshatchPercentileFloat{0.91132822467382401665503266485757194459438323974609375}
\def\UpperWhiskerTopEndPercentileFloat{0.97848760463080519667045109599712304770946502685546875}
\def\WEkkPerpFirstSingularLen{151}
\def\WEkkPerpFirstSingularMaxFloat{4.433342456817626953125}
\def\WEkkPerpFirstSingularMaxKey{16069}
\def\WEkkPerpFirstSingularMeanFloat{4.12576253524679259498952887952327728271484375}
\def\WEkkPerpFirstSingularMeanKey{12552}
\def\WEkkPerpFirstSingularMedianFloat{3.86108863353729248046875}
\def\WEkkPerpFirstSingularMedianKey{24144}
\def\WEkkPerpFirstSingularMinFloat{3.8040287494659423828125}
\def\WEkkPerpFirstSingularMinKey{24202}
\def\WEkkPerpFirstSingularStdDevFloat{0.1286399096369405803397256704556639306247234344482421875}
\def\WEkkPerpFroNormLen{151}
\def\WEkkPerpFroNormMaxFloat{12.22583293914794921875}
\def\WEkkPerpFroNormMaxKey{19004}
\def\WEkkPerpFroNormMeanFloat{11.5730722882100280912709422409534454345703125}
\def\WEkkPerpFroNormMeanKey{7310}
\def\WEkkPerpFroNormMedianFloat{11.046955585479736328125}
\def\WEkkPerpFroNormMedianKey{7884}
\def\WEkkPerpFroNormMinFloat{11.02140522003173828125}
\def\WEkkPerpFroNormMinKey{14095}
\def\WEkkPerpFroNormStdDevFloat{0.200682437823346770944255013091606087982654571533203125}
\def\WEqqPerpFirstSingularLen{151}
\def\WEqqPerpFirstSingularMaxFloat{4.512805938720703125}
\def\WEqqPerpFirstSingularMaxKey{9504}
\def\WEqqPerpFirstSingularMeanFloat{4.17197101479334531148879250395111739635467529296875}
\def\WEqqPerpFirstSingularMeanKey{8893}
\def\WEqqPerpFirstSingularMedianFloat{3.88133966922760009765625}
\def\WEqqPerpFirstSingularMedianKey{14095}
\def\WEqqPerpFirstSingularMinFloat{3.835529327392578125}
\def\WEqqPerpFirstSingularMinKey{24202}
\def\WEqqPerpFirstSingularStdDevFloat{0.1370753263211284267431011585358646698296070098876953125}
\def\WEqqPerpFroNormLen{151}
\def\WEqqPerpFroNormMaxFloat{12.3804111480712890625}
\def\WEqqPerpFroNormMaxKey{19004}
\def\WEqqPerpFroNormMeanFloat{11.7504198503810055598250983166508376598358154296875}
\def\WEqqPerpFroNormMeanKey{7310}
\def\WEqqPerpFroNormMedianFloat{11.2052037715911865234375}
\def\WEqqPerpFroNormMedianKey{14095}
\def\WEqqPerpFroNormMinFloat{11.13461017608642578125}
\def\WEqqPerpFroNormMinKey{7884}
\def\WEqqPerpFroNormStdDevFloat{0.2022367902498510561226652271216153167188167572021484375}
\def\WKkPerpFirstSingularLen{151}
\def\WKkPerpFirstSingularMaxFloat{1.686556339263916015625}
\def\WKkPerpFirstSingularMaxKey{20751}
\def\WKkPerpFirstSingularMeanFloat{1.4677139789063409214264765978441573679447174072265625}
\def\WKkPerpFirstSingularMeanKey{27584}
\def\WKkPerpFirstSingularMedianFloat{1.346714496612548828125}
\def\WKkPerpFirstSingularMedianKey{20338}
\def\WKkPerpFirstSingularMinFloat{1.32256925106048583984375}
\def\WKkPerpFirstSingularMinKey{4647}
\def\WKkPerpFirstSingularStdDevFloat{0.055983738871950412818723208374649402685463428497314453125}
\def\WKkPerpFroNormLen{151}
\def\WKkPerpFroNormMaxFloat{4.541313648223876953125}
\def\WKkPerpFroNormMaxKey{21317}
\def\WKkPerpFroNormMeanFloat{4.26324977780020031303820360335521399974822998046875}
\def\WKkPerpFroNormMeanKey{14095}
\def\WKkPerpFroNormMedianFloat{3.994552910327911376953125}
\def\WKkPerpFroNormMedianKey{50}
\def\WKkPerpFroNormMinFloat{3.9625318050384521484375}
\def\WKkPerpFroNormMinKey{27671}
\def\WKkPerpFroNormStdDevFloat{0.0980326422163107225049571979980100877583026885986328125}
\def\WQqPerpFirstSingularLen{151}
\def\WQqPerpFirstSingularMaxFloat{1.641561985015869140625}
\def\WQqPerpFirstSingularMaxKey{1895}
\def\WQqPerpFirstSingularMeanFloat{1.4775189208668588758399664584430865943431854248046875}
\def\WQqPerpFirstSingularMeanKey{23696}
\def\WQqPerpFirstSingularMedianFloat{1.365040302276611328125}
\def\WQqPerpFirstSingularMedianKey{519}
\def\WQqPerpFirstSingularMinFloat{1.34823858737945556640625}
\def\WQqPerpFirstSingularMinKey{5358}
\def\WQqPerpFirstSingularStdDevFloat{0.058925648333852033433633010872654267586767673492431640625}
\def\WQqPerpFroNormLen{151}
\def\WQqPerpFroNormMaxFloat{4.513673305511474609375}
\def\WQqPerpFroNormMaxKey{1185}
\def\WQqPerpFroNormMeanFloat{4.31707857460375610259006862179376184940338134765625}
\def\WQqPerpFroNormMeanKey{24144}
\def\WQqPerpFroNormMedianFloat{4.07626211643218994140625}
\def\WQqPerpFroNormMedianKey{4305}
\def\WQqPerpFroNormMinFloat{4.027872562408447265625}
\def\WQqPerpFroNormMinKey{6532}
\def\WQqPerpFroNormStdDevFloat{0.093595007769946170217423286885605193674564361572265625}


==> generated/values-10.tex <==
\def\AllModelsHEADSHASHORT{8830e1d}
\def\AllModelsHEADSHA{8830e1dfd45370596a2540de380db3492fe35914}
\def\AlmostQuadraticAccuracyLen{2718}
\def\AlmostQuadraticAccuracyMaxFloat{0.452543729453746712554362829905585385859012603759765625}
\def\AlmostQuadraticAccuracyMeanFloat{0.126723408827566885737070379036595113575458526611328125}
\def\AlmostQuadraticAccuracyMedianFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\AlmostQuadraticAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\AlmostQuadraticAccuracyStdDevFloat{0.150288814804498738197935381322167813777923583984375}
\def\AlmostQuadraticDroppedSequencesFracLen{2718}
\def\AlmostQuadraticDroppedSequencesFracMaxFloat{0.46377977035578010767125078928074799478054046630859375}
\def\AlmostQuadraticDroppedSequencesFracMeanFloat{0.225632850369890614050660815337323583662509918212890625}
\def\AlmostQuadraticDroppedSequencesFracMedianFloat{0}
\def\AlmostQuadraticDroppedSequencesFracMinFloat{0}
\def\AlmostQuadraticDroppedSequencesFracStdDevFloat{0.1621320873651361516021296438339049927890300750732421875}
\def\AlmostQuadraticDroppedSequencesLen{2718}
\def\AlmostQuadraticDroppedSequencesMaxFloat{534701670644804012}
\def\AlmostQuadraticDroppedSequencesMeanFloat{260136965337185856}
\def\AlmostQuadraticDroppedSequencesMedianFloat{0}
\def\AlmostQuadraticDroppedSequencesMinFloat{0}
\def\AlmostQuadraticDroppedSequencesStdDevFloat{186925570110061536}
\def\AlmostQuadraticEffectiveDimensionalityEstimateLen{2718}
\def\AlmostQuadraticEffectiveDimensionalityEstimateMaxFloat{6530}
\def\AlmostQuadraticEffectiveDimensionalityEstimateMeanFloat{6487.3333333333330301684327423572540283203125}
\def\AlmostQuadraticEffectiveDimensionalityEstimateMedianFloat{6402}
\def\AlmostQuadraticEffectiveDimensionalityEstimateMinFloat{6402}
\def\AlmostQuadraticEffectiveDimensionalityEstimateStdDevFloat{42.66666666666666429819088079966604709625244140625}
\def\AlmostQuadraticErrUpperBoundLen{2718}
\def\AlmostQuadraticErrUpperBoundMaxFloat{156.4159393310546875}
\def\AlmostQuadraticErrUpperBoundMeanFloat{91.8609873116937478698673658072948455810546875}
\def\AlmostQuadraticErrUpperBoundMedianFloat{78.9598388671875}
\def\AlmostQuadraticErrUpperBoundMinFloat{78.61283111572265625}
\def\AlmostQuadraticErrUpperBoundStdDevFloat{7.64323512735036647569586421013809740543365478515625}
\def\AlmostQuadraticGapMostBelowValueLen{2718}
\def\AlmostQuadraticGapMostBelowValueMaxFloat{23}
\def\AlmostQuadraticGapMostBelowValueMeanFloat{9.1795437821927894361806465894915163516998291015625}
\def\AlmostQuadraticGapMostBelowValueMedianFloat{1}
\def\AlmostQuadraticGapMostBelowValueMinFloat{1}
\def\AlmostQuadraticGapMostBelowValueNumStdLen{2718}
\def\AlmostQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\AlmostQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\AlmostQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\AlmostQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\AlmostQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\AlmostQuadraticGapMostBelowValueSequenceFracLen{2718}
\def\AlmostQuadraticGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\AlmostQuadraticGapMostBelowValueSequenceFracMeanFloat{0.99895022817180822993776700968737713992595672607421875}
\def\AlmostQuadraticGapMostBelowValueSequenceFracMedianFloat{0.990021169185638427734375}
\def\AlmostQuadraticGapMostBelowValueSequenceFracMinFloat{0.98604261875152598992855246251565404236316680908203125}
\def\AlmostQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.001612141786953481641109231503605769830755889415740966796875}
\def\AlmostQuadraticGapMostBelowValueStdDevFloat{6.018318327787913091242444352246820926666259765625}
\def\AlmostQuadraticInstructionCountBranchLen{2718}
\def\AlmostQuadraticInstructionCountBranchMaxFloat{0}
\def\AlmostQuadraticInstructionCountBranchMeanFloat{0}
\def\AlmostQuadraticInstructionCountBranchMedianFloat{0}
\def\AlmostQuadraticInstructionCountBranchMinFloat{0}
\def\AlmostQuadraticInstructionCountBranchStdDevFloat{0}
\def\AlmostQuadraticInstructionCountIntLen{2718}
\def\AlmostQuadraticInstructionCountIntMaxFloat{0}
\def\AlmostQuadraticInstructionCountIntMeanFloat{0}
\def\AlmostQuadraticInstructionCountIntMedianFloat{0}
\def\AlmostQuadraticInstructionCountIntMinFloat{0}
\def\AlmostQuadraticInstructionCountIntStdDevFloat{0}
\def\AlmostQuadraticInstructionCountLen{2718}
\def\AlmostQuadraticInstructionCountMaxFloat{5611377}
\def\AlmostQuadraticInstructionCountMeanFloat{5542546.666666666977107524871826171875}
\def\AlmostQuadraticInstructionCountMedianFloat{5473748}
\def\AlmostQuadraticInstructionCountMinFloat{5473748}
\def\AlmostQuadraticInstructionCountStdDevFloat{55524.7348105128548922948539257049560546875}
\def\AlmostQuadraticMaxGapLen{2718}
\def\AlmostQuadraticMaxGapMaxFloat{47}
\def\AlmostQuadraticMaxGapMeanFloat{24.037159676232523253247563843615353107452392578125}
\def\AlmostQuadraticMaxGapMedianFloat{1}
\def\AlmostQuadraticMaxGapMinFloat{1}
\def\AlmostQuadraticMaxGapStdDevFloat{17.518740589558962739147318643517792224884033203125}
\def\AlmostQuadraticNormalizedAccuracyLen{2718}
\def\AlmostQuadraticNormalizedAccuracyMaxFloat{0.45286923071017870512378067360259592533111572265625}
\def\AlmostQuadraticNormalizedAccuracyMeanFloat{0.12687312556441232569426347254193387925624847412109375}
\def\AlmostQuadraticNormalizedAccuracyMedianFloat{0.000000000000000026054821497037114438219634609030939328582006345885226095138165192111046053469181060791015625}
\def\AlmostQuadraticNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\AlmostQuadraticNormalizedAccuracyStdDevFloat{0.1504676457476110951194669951291871257126331329345703125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.452543729453746712554362829905585385859012603759765625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{7238}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.390423493111564379187683471172931604087352752685546875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{31308}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.325130980910436073738623008466674946248531341552734375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{9816}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.318141293842261585478325969233992509543895721435546875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{11124}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0279359164293897233033447946581873111426830291748046875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.456757311611598215694840519063291139900684356689453125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.3493432199636561374944676572340540587902069091796875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29725}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.268695947037915328081680854666046798229217529296875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4810}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.268159626117558114177796824151300825178623199462890625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.028945140281470826959520081800292246043682098388671875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{526605326943422293}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{402765310784699136}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29725}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{309785335540715008}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4810}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{309166999618264736}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{33371474684369596}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6502.0264900662250511231832206249237060546875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{104}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{104}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{31.745667070430105383138652541674673557281494140625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.4159393310546875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.4848378667768287186845554970204830169677734375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29726}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.8730869293212890625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.61283111572265625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.66115263186247030802178414887748658657073974609375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{23}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29565}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{13.6887417218543046004697316675446927547454833984375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{10}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4810}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{10}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4810}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99999964237213123663394753748434595763683319091796875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13654}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99807756902366284723626677077845670282840728759765625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29195}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9917971193790435791015625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24438}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.991044223308563232421875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{29022}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00160033295619864597038317644006610862561501562595367431640625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.065758140461221525896462480886839330196380615234375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5611377}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{3284}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5593392.218543046154081821441650390625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5584660}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{104}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{5584660}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{104}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{8919.140182845294475555419921875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{45}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{3254}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{38.66225165562914156680562882684171199798583984375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{14}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{7098}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.73437125964751448492506824550218880176544189453125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.45286923071017870512378067360259592533111572265625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7238}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.390894573938078193631184831247082911431789398193359375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{31308}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.325522332758098886795750104283797554671764373779296875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{9816}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.318423535380195465993580228314385749399662017822265625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11124}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0279968896252014466663471381480121635831892490386962890625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.1968085765838623046875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.6048799982134056563154445029795169830322265625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.071754515171051025390625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{79.3047096729278564453125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.4051890214643290022422661422751843929290771484375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.777535915374755859375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{913}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.62063053112156385537900860072113573551177978515625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{32374}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.50573670864105224609375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{24173}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{4.5055332183837890625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.058966118215369713040363564005019725300371646881103515625}
\def\AlmostQuadraticProofSearchTimeLen{2718}
\def\AlmostQuadraticProofSearchTimeMaxFloat{101.354745388031005859375}
\def\AlmostQuadraticProofSearchTimeMeanFloat{84.1996096230500512547223479487001895904541015625}
\def\AlmostQuadraticProofSearchTimeMedianFloat{81.1775342977046960868392488919198513031005859375}
\def\AlmostQuadraticProofSearchTimeMinFloat{79.2337474822998046875}
\def\AlmostQuadraticProofSearchTimeStdDevFloat{1.4334570284820162822114752998459152877330780029296875}
\def\AlmostQuadraticProofTimeLen{2718}
\def\AlmostQuadraticProofTimeMaxFloat{4.8339951038360595703125}
\def\AlmostQuadraticProofTimeMeanFloat{4.5956573026683766869382452568970620632171630859375}
\def\AlmostQuadraticProofTimeMedianFloat{4.46842619061470003316571819595992565155029296875}
\def\AlmostQuadraticProofTimeMinFloat{4.4427516460418701171875}
\def\AlmostQuadraticProofTimeStdDevFloat{0.059335069010919845589047127987214480526745319366455078125}
\def\AnySubcubicAccuracyLen{15100}
\def\AnySubcubicAccuracyLowerWhiskerBottomEndFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\AnySubcubicAccuracyLowerWhiskerCrosshatchFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\AnySubcubicAccuracyMaxFloat{0.73561759633376000433457875260501168668270111083984375}
\def\AnySubcubicAccuracyMeanFloat{0.303314539339781863436229514263686724007129669189453125}
\def\AnySubcubicAccuracyMedianFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\AnySubcubicAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\AnySubcubicAccuracyQuartileOneFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\AnySubcubicAccuracyQuartileThreeFloat{0.000000000000000026888213877640509963384829461574554443359375}
\def\AnySubcubicAccuracySqrMeanFloat{0.1511759064311366251853741005106712691485881805419921875}
\def\AnySubcubicAccuracyStdDevFloat{0.2432615807237808180918392508829128928482532501220703125}
\def\AnySubcubicAccuracyUpperWhiskerCrosshatchFloat{0.000000000000000026888213877640509963384829461574554443359375}
\def\AnySubcubicAccuracyUpperWhiskerTopEndFloat{0.000000000000000026888213877640509963384829461574554443359375}
\def\AnySubcubicDroppedSequencesFracLen{15100}
\def\AnySubcubicDroppedSequencesFracMaxFloat{0.46377977035578010767125078928074799478054046630859375}
\def\AnySubcubicDroppedSequencesFracMeanFloat{0.1621743713089575378294426855063647963106632232666015625}
\def\AnySubcubicDroppedSequencesFracMedianFloat{0}
\def\AnySubcubicDroppedSequencesFracMinFloat{0}
\def\AnySubcubicDroppedSequencesFracStdDevFloat{0.12409221244347089230242175972307450138032436370849609375}
\def\AnySubcubicDroppedSequencesLen{15100}
\def\AnySubcubicDroppedSequencesMaxFloat{534701670644804012}
\def\AnySubcubicDroppedSequencesMeanFloat{186974320178192832}
\def\AnySubcubicDroppedSequencesMedianFloat{0}
\def\AnySubcubicDroppedSequencesMinFloat{0}
\def\AnySubcubicDroppedSequencesStdDevFloat{143068580280318976}
\def\AnySubcubicEffectiveDimensionalityEstimateLen{15100}
\def\AnySubcubicEffectiveDimensionalityEstimateMaxFloat{10370}
\def\AnySubcubicEffectiveDimensionalityEstimateMeanFloat{6049.600000000000363797880709171295166015625}
\def\AnySubcubicEffectiveDimensionalityEstimateMedianFloat{4290}
\def\AnySubcubicEffectiveDimensionalityEstimateMinFloat{4290}
\def\AnySubcubicEffectiveDimensionalityEstimateStdDevFloat{1530.49032666005450664670206606388092041015625}
\def\AnySubcubicErrUpperBoundLen{15100}
\def\AnySubcubicErrUpperBoundMaxFloat{156.4159393310546875}
\def\AnySubcubicErrUpperBoundMeanFloat{31.734276126946834750697234994731843471527099609375}
\def\AnySubcubicErrUpperBoundMedianFloat{0}
\def\AnySubcubicErrUpperBoundMinFloat{0}
\def\AnySubcubicErrUpperBoundStdDevFloat{39.7595860426961138500701053999364376068115234375}
\def\AnySubcubicGapMostBelowValueLen{15100}
\def\AnySubcubicGapMostBelowValueMaxFloat{23}
\def\AnySubcubicGapMostBelowValueMeanFloat{5.47019867549668870054802027880214154720306396484375}
\def\AnySubcubicGapMostBelowValueMedianFloat{1}
\def\AnySubcubicGapMostBelowValueMinFloat{1}
\def\AnySubcubicGapMostBelowValueNumStdLen{15100}
\def\AnySubcubicGapMostBelowValueNumStdMaxFloat{1.5}
\def\AnySubcubicGapMostBelowValueNumStdMeanFloat{1.5}
\def\AnySubcubicGapMostBelowValueNumStdMedianFloat{1.5}
\def\AnySubcubicGapMostBelowValueNumStdMinFloat{1.5}
\def\AnySubcubicGapMostBelowValueNumStdStdDevFloat{0}
\def\AnySubcubicGapMostBelowValueSequenceFracLen{15100}
\def\AnySubcubicGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\AnySubcubicGapMostBelowValueSequenceFracMeanFloat{0.99053359043124500349364325302303768694400787353515625}
\def\AnySubcubicGapMostBelowValueSequenceFracMedianFloat{0.9522950348258019115377237540087662637233734130859375}
\def\AnySubcubicGapMostBelowValueSequenceFracMinFloat{0.92754381895065318719417746251565404236316680908203125}
\def\AnySubcubicGapMostBelowValueSequenceFracStdDevFloat{0.0110176616847880888550026412531224195845425128936767578125}
\def\AnySubcubicGapMostBelowValueStdDevFloat{4.52716297434603465177360703819431364536285400390625}
\def\AnySubcubicInstructionCountBranchLen{15100}
\def\AnySubcubicInstructionCountBranchMaxFloat{0}
\def\AnySubcubicInstructionCountBranchMeanFloat{0}
\def\AnySubcubicInstructionCountBranchMedianFloat{0}
\def\AnySubcubicInstructionCountBranchMinFloat{0}
\def\AnySubcubicInstructionCountBranchStdDevFloat{0}
\def\AnySubcubicInstructionCountIntLen{15100}
\def\AnySubcubicInstructionCountIntMaxFloat{0}
\def\AnySubcubicInstructionCountIntMeanFloat{0}
\def\AnySubcubicInstructionCountIntMedianFloat{0}
\def\AnySubcubicInstructionCountIntMinFloat{0}
\def\AnySubcubicInstructionCountIntStdDevFloat{0}
\def\AnySubcubicInstructionCountLen{15100}
\def\AnySubcubicInstructionCountMaxFloat{8343894}
\def\AnySubcubicInstructionCountMeanFloat{6440064.799999999813735485076904296875}
\def\AnySubcubicInstructionCountMedianFloat{5473748}
\def\AnySubcubicInstructionCountMinFloat{5473748}
\def\AnySubcubicInstructionCountStdDevFloat{795875.490351449348963797092437744140625}
\def\AnySubcubicMaxGapLen{15100}
\def\AnySubcubicMaxGapMaxFloat{47}
\def\AnySubcubicMaxGapMeanFloat{23.63258278145695356897704186849296092987060546875}
\def\AnySubcubicMaxGapMedianFloat{1}
\def\AnySubcubicMaxGapMinFloat{1}
\def\AnySubcubicMaxGapStdDevFloat{14.672164864329364064587934990413486957550048828125}
\def\AnySubcubicNormalizedAccuracyLen{15100}
\def\AnySubcubicNormalizedAccuracyLowerWhiskerBottomEndFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\AnySubcubicNormalizedAccuracyLowerWhiskerCrosshatchFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\AnySubcubicNormalizedAccuracyMaxFloat{0.7362903356393937226442858445807360112667083740234375}
\def\AnySubcubicNormalizedAccuracyMeanFloat{0.30367035045883528088239700082340277731418609619140625}
\def\AnySubcubicNormalizedAccuracyMedianFloat{0.000000000000000026065848841239090779005246038169553657235825929079642282459872149047441780567169189453125}
\def\AnySubcubicNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\AnySubcubicNormalizedAccuracyQuartileOneFloat{0.000000000000000026054821497037114438219634609030939328582006345885226095138165192111046053469181060791015625}
\def\AnySubcubicNormalizedAccuracyQuartileThreeFloat{0.0000000000000000269144096360585379536958041473409656342735118690449869216507750024902634322643280029296875}
\def\AnySubcubicNormalizedAccuracySqrMeanFloat{0.151527348144924578488001998266554437577724456787109375}
\def\AnySubcubicNormalizedAccuracyStdDevFloat{0.2435398661351622084936252576881088316440582275390625}
\def\AnySubcubicNormalizedAccuracyUpperWhiskerCrosshatchFloat{0.000000000000000026914835868756612251468723734188020622569434818515711482778129948201240040361881256103515625}
\def\AnySubcubicNormalizedAccuracyUpperWhiskerTopEndFloat{0.000000000000000026914835868756612251468723734188020622569434818515711482778129948201240040361881256103515625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLowerWhiskerBottomEndFloat{0.58915540868639360017056105789379216730594635009765625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLowerWhiskerBottomEndKey{11498}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLowerWhiskerCrosshatchFloat{0.59065578389890582844401478723739273846149444580078125}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLowerWhiskerCrosshatchKey{11498}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.73561759633376000433457875260501168668270111083984375}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMaxKey{13293}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.6744402969050644625070844995207153260707855224609375}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMeanKey{2773}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.59984506874493315198293430512421764433383941650390625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMinFloat{0.5886748106702359706332572386600077152252197265625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMinKey{11498}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyQuartileOneFloat{0.5942599397075845057969445406342856585979461669921875}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyQuartileOneKey{11498}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyQuartileThreeFloat{0.60426387473841192132795185898430645465850830078125}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyQuartileThreeKey{2549}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracySqrMeanFloat{0.45564032884127281253228147761547006666660308837890625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0277599487009831287498418106451936182565987110137939453125}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyUpperWhiskerCrosshatchFloat{0.6056101006343264092635081397020258009433746337890625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyUpperWhiskerCrosshatchKey{2549}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyUpperWhiskerTopEndFloat{0.60617052145736860513380861448240466415882110595703125}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyUpperWhiskerTopEndKey{2549}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.166309213880606099333903102888143621385097503662109375}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10834467436685824015540902109933085739612579345703125}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{23367}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.069256780745197199511409280603402294218540191650390625}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{14095}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0641773134406526946094118102337233722209930419921875}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0192612986811899582206830672248543123714625835418701171875}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{191741469097210324}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{124912904987177120}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{23367}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{79847631860979296}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{14095}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{73991404773622603}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{22206765456199400}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{3284}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{7230.609271523178904317319393157958984375}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{7238}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{10248}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{10248}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{2008.985681842410258468589745461940765380859375}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.4831371307373046875}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{30371}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{1.36984169483184814453125}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{21317}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.4478428364381130677429609932005405426025390625}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{11498}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.172185430463576150117432916886173188686370849609375}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99907410144805919305355246251565404236316680908203125}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{18146}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.988061948722561478319903471856378018856048583984375}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29110}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95318606495857227667301003748434595763683319091796875}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{3284}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94793224334716796875}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{19093}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.009528229840375206094460480699126492254436016082763671875}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.39469309737089641743068568757735192775726318359375}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7393557}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMaxKey{10248}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6458010.072847682051360607147216796875}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMeanKey{24202}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5896885}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMedianKey{3284}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMinFloat{5896885}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMinKey{3284}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{527408.75618842965923249721527099609375}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMaxFloat{36}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMeanFloat{30.576158940397352381523887743242084980010986328125}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMedianKey{8048}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMinKey{8048}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.8219106516352869817865212098695337772369384765625}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLowerWhiskerBottomEndFloat{0.59136690932082702776284577339538373053073883056640625}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLowerWhiskerBottomEndKey{11498}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLowerWhiskerCrosshatchFloat{0.5926875934421442781996347548556514084339141845703125}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLowerWhiskerCrosshatchKey{11498}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7362903356393937226442858445807360112667083740234375}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{13293}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6752443192679418171309180252137593924999237060546875}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{19093}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.6007763318331817981032827447052113711833953857421875}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.5909438696948836611255728712421841919422149658203125}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11498}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyQuartileOneFloat{0.59586010076403272961442780797369778156280517578125}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyQuartileOneKey{11498}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyQuartileThreeFloat{0.604844588930247173408361049951054155826568603515625}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyQuartileThreeKey{2549}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracySqrMeanFloat{0.456718987106024820743499503805651329457759857177734375}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0276422937253531335322076500915500218980014324188232421875}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyUpperWhiskerCrosshatchFloat{0.6063754706263051463821511788410134613513946533203125}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyUpperWhiskerCrosshatchKey{2549}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyUpperWhiskerTopEndFloat{0.6070127618734046937021275880397297441959381103515625}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyUpperWhiskerTopEndKey{2549}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{92.9854123592376851092922152020037174224853515625}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.6036648987144843658825266174972057342529296875}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{19451}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.923117816448211669921875}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.9165172576904296875}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5493088914244939058306727019953541457653045654296875}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7482655048370361328125}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61012741745702481210855694371275603771209716796875}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMeanKey{8721}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.49540579319000244140625}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMedianKey{28778}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMinFloat{4.49149227142333984375}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0570625438540881269045001999984378926455974578857421875}
\def\AnySubcubicProofSearchTimeLen{15100}
\def\AnySubcubicProofSearchTimeMaxFloat{101.354745388031005859375}
\def\AnySubcubicProofSearchTimeMeanFloat{84.2111817345240325494160060770809650421142578125}
\def\AnySubcubicProofSearchTimeMedianFloat{81.12614621996880259757745079696178436279296875}
\def\AnySubcubicProofSearchTimeMinFloat{78.8330733776092529296875}
\def\AnySubcubicProofSearchTimeStdDevFloat{1.4637204285312879203928559945779852569103240966796875}
\def\AnySubcubicProofTimeLen{15100}
\def\AnySubcubicProofTimeMaxFloat{5.38143634796142578125}
\def\AnySubcubicProofTimeMeanFloat{4.596908784623177979256070102564990520477294921875}
\def\AnySubcubicProofTimeMedianFloat{4.46908013820648175595806605997495353221893310546875}
\def\AnySubcubicProofTimeMinFloat{4.4427516460418701171875}
\def\AnySubcubicProofTimeStdDevFloat{0.0596223763155452335382733508595265448093414306640625}
\def\AxisLimitsOVCenteredZmaxFloat{16.0412654876708984375}
\def\AxisLimitsOVCenteredZminFloat{-83.0191192626953125}
\def\AxisLimitsOVZmaxFloat{44.590057373046875}
\def\AxisLimitsOVZminFloat{-44.590057373046875}
\def\AxisLimitsQKWithAttnScaleZmaxFloat{90.04020739613196155914920382201671600341796875}
\def\AxisLimitsQKWithAttnScaleZminFloat{-90.04020739613196155914920382201671600341796875}
\def\AxisLimitsQKZmaxFloat{509.344329833984375}
\def\AxisLimitsQKZminFloat{-509.344329833984375}
\def\BruteForceEffectiveDimensionalityEstimate{73786976294838206464}
\def\BruteForceInstructionCountBranch{0}
\def\BruteForceInstructionCountInt{0}
\def\BruteForceInstructionCount{62762550636020750526447616}
\def\CubicAccuracyLen{151}
\def\CubicAccuracyLowerWhiskerBottomEndFloat{0.84248002825541890015159651738940738141536712646484375}
\def\CubicAccuracyLowerWhiskerBottomEndKey{19538}
\def\CubicAccuracyLowerWhiskerCrosshatchFloat{0.844445839697866684758764677098952233791351318359375}
\def\CubicAccuracyLowerWhiskerCrosshatchKey{19538}
\def\CubicAccuracyMaxFloat{0.95311130376731256763633837181259877979755401611328125}
\def\CubicAccuracyMaxKey{1681}
\def\CubicAccuracyMeanFloat{0.913839618762660510498108124011196196079254150390625}
\def\CubicAccuracyMeanKey{6549}
\def\CubicAccuracyMedianFloat{0.8564857622103054790585474620456807315349578857421875}
\def\CubicAccuracyMedianKey{20415}
\def\CubicAccuracyMinFloat{0.841850342379844907014785349019803106784820556640625}
\def\CubicAccuracyMinKey{19538}
\def\CubicAccuracyQuartileOneFloat{0.84916805229507519303666640553274191915988922119140625}
\def\CubicAccuracyQuartileOneKey{19538}
\def\CubicAccuracyQuartileThreeFloat{0.8615505482466210285252827816293574869632720947265625}
\def\CubicAccuracyQuartileThreeKey{20415}
\def\CubicAccuracySqrMeanFloat{0.83553253883828659809296368621289730072021484375}
\def\CubicAccuracyStdDevFloat{0.02072896567611644258466441215205122716724872589111328125}
\def\CubicAccuracyUpperWhiskerCrosshatchFloat{0.861911238327302431372345381532795727252960205078125}
\def\CubicAccuracyUpperWhiskerCrosshatchKey{20415}
\def\CubicAccuracyUpperWhiskerTopEndFloat{0.86206139012017179990010617984808050096035003662109375}
\def\CubicAccuracyUpperWhiskerTopEndKey{20415}
\def\CubicCorrectCountLen{151}
\def\CubicCorrectCountMaxFloat{1098862518397203584}
\def\CubicCorrectCountMaxKey{1681}
\def\CubicCorrectCountMeanFloat{1053585348233193984}
\def\CubicCorrectCountMeanKey{6549}
\def\CubicCorrectCountMedianFloat{987460853641847552}
\def\CubicCorrectCountMedianKey{20415}
\def\CubicCorrectCountMinFloat{970587363390360064}
\def\CubicCorrectCountMinKey{19538}
\def\CubicCorrectCountStdDevFloat{23898870296251860}
\def\CubicEffectiveDimensionalityEstimate{13568}
\def\CubicInstructionCountBranch{0}
\def\CubicInstructionCountInt{0}
\def\CubicInstructionCount{193981664}
\def\CubicNormalizedAccuracyLen{151}
\def\CubicNormalizedAccuracyLowerWhiskerBottomEndFloat{0.8441807869318898038812903905636630952358245849609375}
\def\CubicNormalizedAccuracyLowerWhiskerBottomEndKey{19538}
\def\CubicNormalizedAccuracyLowerWhiskerCrosshatchFloat{0.84606984110109484387152178896940313279628753662109375}
\def\CubicNormalizedAccuracyLowerWhiskerCrosshatchKey{19538}
\def\CubicNormalizedAccuracyMaxFloat{0.9540954713295974887188322099973447620868682861328125}
\def\CubicNormalizedAccuracyMaxKey{1681}
\def\CubicNormalizedAccuracyMeanFloat{0.9149356480770542976443948646192438900470733642578125}
\def\CubicNormalizedAccuracyMeanKey{3175}
\def\CubicNormalizedAccuracyMedianFloat{0.85763965157625843271915755394729785621166229248046875}
\def\CubicNormalizedAccuracyMedianKey{20415}
\def\CubicNormalizedAccuracyMinFloat{0.843575687834968501732646473101340234279632568359375}
\def\CubicNormalizedAccuracyMinKey{19538}
\def\CubicNormalizedAccuracyQuartileOneFloat{0.8506076697056135227370532447821460664272308349609375}
\def\CubicNormalizedAccuracyQuartileOneKey{19538}
\def\CubicNormalizedAccuracyQuartileThreeFloat{0.8625276037102460602312703485949896275997161865234375}
\def\CubicNormalizedAccuracyQuartileThreeKey{20415}
\def\CubicNormalizedAccuracySqrMeanFloat{0.8375339189188235611283062098664231598377227783203125}
\def\CubicNormalizedAccuracyStdDevFloat{0.0206562047976873199017777693597963661886751651763916015625}
\def\CubicNormalizedAccuracyUpperWhiskerCrosshatchFloat{0.86291472218201070720766665544942952692508697509765625}
\def\CubicNormalizedAccuracyUpperWhiskerCrosshatchKey{20415}
\def\CubicNormalizedAccuracyUpperWhiskerTopEndFloat{0.8630758758585368450866326384129934012889862060546875}
\def\CubicNormalizedAccuracyUpperWhiskerTopEndKey{20415}
\def\CubicProofTimeLen{151}
\def\CubicProofTimeMaxFloat{127.6399190425872802734375}
\def\CubicProofTimeMaxKey{6532}
\def\CubicProofTimeMeanFloat{123.470259546444111720120417885482311248779296875}
\def\CubicProofTimeMeanKey{27714}
\def\CubicProofTimeMedianFloat{119.4399235248565673828125}
\def\CubicProofTimeMedianKey{7790}
\def\CubicProofTimeMinFloat{119.355511188507080078125}
\def\CubicProofTimeMinKey{2345}
\def\CubicProofTimeStdDevFloat{2.025646974305817860084744097548536956310272216796875}
\def\EPVOUAbsLenLen{151}
\def\EPVOUAbsLenMaxFloat{4096}
\def\EPVOUAbsLenMaxKey{50}
\def\EPVOUAbsLenMeanFloat{4096}
\def\EPVOUAbsLenMeanKey{50}
\def\EPVOUAbsLenMedianFloat{4096}
\def\EPVOUAbsLenMedianKey{50}
\def\EPVOUAbsLenMinFloat{4096}
\def\EPVOUAbsLenMinKey{50}
\def\EPVOUAbsLenStdDevFloat{0}
\def\EPVOUAbsMaxLen{151}
\def\EPVOUAbsMaxMaxFloat{44.590057373046875}
\def\EPVOUAbsMaxMaxKey{6589}
\def\EPVOUAbsMaxMeanFloat{35.6483612060546875}
\def\EPVOUAbsMaxMeanKey{104}
\def\EPVOUAbsMaxMedianFloat{29.71045398712158203125}
\def\EPVOUAbsMaxMedianKey{11124}
\def\EPVOUAbsMaxMinFloat{29.3502197265625}
\def\EPVOUAbsMaxMinKey{16149}
\def\EPVOUAbsMaxStdDevFloat{3.0287301540374755859375}
\def\EPVOUAbsMeanLen{151}
\def\EPVOUAbsMeanMaxFloat{9.6216888427734375}
\def\EPVOUAbsMeanMaxKey{742}
\def\EPVOUAbsMeanMeanFloat{7.20910167694091796875}
\def\EPVOUAbsMeanMeanKey{1696}
\def\EPVOUAbsMeanMedianFloat{5.422875881195068359375}
\def\EPVOUAbsMeanMedianKey{3284}
\def\EPVOUAbsMeanMinFloat{5.33421421051025390625}
\def\EPVOUAbsMeanMinKey{4810}
\def\EPVOUAbsMeanStdDevFloat{0.840044558048248291015625}
\def\EPVOUAbsMedianLen{151}
\def\EPVOUAbsMedianMaxFloat{0.1563824206590652410309161268742172978818416595458984375}
\def\EPVOUAbsMedianMaxKey{20415}
\def\EPVOUAbsMedianMeanFloat{0.08475280025579183529327309543077717535197734832763671875}
\def\EPVOUAbsMedianMeanKey{1283}
\def\EPVOUAbsMedianMedianFloat{0.04460592530667782662501252843867405317723751068115234375}
\def\EPVOUAbsMedianMedianKey{11611}
\def\EPVOUAbsMedianMinFloat{0.04092256277799606600797943656289135105907917022705078125}
\def\EPVOUAbsMedianMinKey{11124}
\def\EPVOUAbsMedianStdDevFloat{0.022267099344363473767405281478204415179789066314697265625}
\def\EPVOUAbsMinLen{151}
\def\EPVOUAbsMinMaxFloat{0.0221908092498779296875}
\def\EPVOUAbsMinMaxKey{26932}
\def\EPVOUAbsMinMeanFloat{0.0039086225442588329315185546875}
\def\EPVOUAbsMinMeanKey{7098}
\def\EPVOUAbsMinMedianFloat{0.0000567324459552764892578125}
\def\EPVOUAbsMinMedianKey{15622}
\def\EPVOUAbsMinMinFloat{0.00005276501178741455078125}
\def\EPVOUAbsMinMinKey{19488}
\def\EPVOUAbsMinStdDevFloat{0.00350805954076349735260009765625}
\def\EPVOUAbsStdDevLen{151}
\def\EPVOUAbsStdDevMaxFloat{5.976147174835205078125}
\def\EPVOUAbsStdDevMaxKey{742}
\def\EPVOUAbsStdDevMeanFloat{4.7679576873779296875}
\def\EPVOUAbsStdDevMeanKey{1696}
\def\EPVOUAbsStdDevMedianFloat{3.8485424518585205078125}
\def\EPVOUAbsStdDevMedianKey{9132}
\def\EPVOUAbsStdDevMinFloat{3.7562744617462158203125}
\def\EPVOUAbsStdDevMinKey{3284}
\def\EPVOUAbsStdDevStdDevFloat{0.3851605355739593505859375}
\def\EPVOUCenteredLenLen{151}
\def\EPVOUCenteredLenMaxFloat{4096}
\def\EPVOUCenteredLenMaxKey{50}
\def\EPVOUCenteredLenMeanFloat{4096}
\def\EPVOUCenteredLenMeanKey{50}
\def\EPVOUCenteredLenMedianFloat{4096}
\def\EPVOUCenteredLenMedianKey{50}
\def\EPVOUCenteredLenMinFloat{4096}
\def\EPVOUCenteredLenMinKey{50}
\def\EPVOUCenteredLenStdDevFloat{0}
\def\EPVOUCenteredMaxLen{151}
\def\EPVOUCenteredMaxMaxFloat{16.0412616729736328125}
\def\EPVOUCenteredMaxMaxKey{20415}
\def\EPVOUCenteredMaxMeanFloat{12.173976898193359375}
\def\EPVOUCenteredMaxMeanKey{13654}
\def\EPVOUCenteredMaxMedianFloat{8.7478287220001220703125}
\def\EPVOUCenteredMaxMedianKey{17197}
\def\EPVOUCenteredMaxMinFloat{8.664562225341796875}
\def\EPVOUCenteredMaxMinKey{3284}
\def\EPVOUCenteredMaxStdDevFloat{1.47744667530059814453125}
\def\EPVOUCenteredMeanLen{151}
\def\EPVOUCenteredMeanMaxFloat{-10.2688159942626953125}
\def\EPVOUCenteredMeanMaxKey{4810}
\def\EPVOUCenteredMeanMeanFloat{-13.16547870635986328125}
\def\EPVOUCenteredMeanMeanKey{6082}
\def\EPVOUCenteredMeanMedianFloat{-14.8008162975311279296875}
\def\EPVOUCenteredMeanMedianKey{24262}
\def\EPVOUCenteredMeanMinFloat{-14.81822490692138671875}
\def\EPVOUCenteredMeanMinKey{15662}
\def\EPVOUCenteredMeanStdDevFloat{0.72372949123382568359375}
\def\EPVOUCenteredMedianLen{151}
\def\EPVOUCenteredMedianMaxFloat{-46.2265060424804659078290569595992565155029296875}
\def\EPVOUCenteredMedianMaxKey{11124}
\def\EPVOUCenteredMedianMeanFloat{-55.0379058629471700214708107523620128631591796875}
\def\EPVOUCenteredMedianMeanKey{29565}
\def\EPVOUCenteredMedianMedianFloat{-64.733989715576171875}
\def\EPVOUCenteredMedianMedianKey{19093}
\def\EPVOUCenteredMedianMinFloat{-65.5280540466308565328290569595992565155029296875}
\def\EPVOUCenteredMedianMinKey{742}
\def\EPVOUCenteredMedianStdDevFloat{3.74705415476573033828344705398194491863250732421875}
\def\EPVOUCenteredMinLen{151}
\def\EPVOUCenteredMinMaxFloat{-54.162384033203125}
\def\EPVOUCenteredMinMaxKey{11124}
\def\EPVOUCenteredMinMeanFloat{-66.5613861083984375}
\def\EPVOUCenteredMinMeanKey{27714}
\def\EPVOUCenteredMinMedianFloat{-82.39397430419921875}
\def\EPVOUCenteredMinMedianKey{27671}
\def\EPVOUCenteredMinMinFloat{-83.0191192626953125}
\def\EPVOUCenteredMinMinKey{6589}
\def\EPVOUCenteredMinStdDevFloat{5.750451564788818359375}
\def\EPVOUCenteredOffDiagonalLenLen{151}
\def\EPVOUCenteredOffDiagonalLenMaxFloat{4032}
\def\EPVOUCenteredOffDiagonalLenMaxKey{50}
\def\EPVOUCenteredOffDiagonalLenMeanFloat{4032}
\def\EPVOUCenteredOffDiagonalLenMeanKey{50}
\def\EPVOUCenteredOffDiagonalLenMedianFloat{4032}
\def\EPVOUCenteredOffDiagonalLenMedianKey{50}
\def\EPVOUCenteredOffDiagonalLenMinFloat{4032}
\def\EPVOUCenteredOffDiagonalLenMinKey{50}
\def\EPVOUCenteredOffDiagonalLenStdDevFloat{0}
\def\EPVOUCenteredOffDiagonalMaxLen{151}
\def\EPVOUCenteredOffDiagonalMaxMaxFloat{16.0412616729736328125}
\def\EPVOUCenteredOffDiagonalMaxMaxKey{20415}
\def\EPVOUCenteredOffDiagonalMaxMeanFloat{12.173976898193359375}
\def\EPVOUCenteredOffDiagonalMaxMeanKey{13654}
\def\EPVOUCenteredOffDiagonalMaxMedianFloat{8.7478287220001220703125}
\def\EPVOUCenteredOffDiagonalMaxMedianKey{17197}
\def\EPVOUCenteredOffDiagonalMaxMinFloat{8.664562225341796875}
\def\EPVOUCenteredOffDiagonalMaxMinKey{3284}
\def\EPVOUCenteredOffDiagonalMaxStdDevFloat{1.47744667530059814453125}
\def\EPVOUCenteredOffDiagonalMeanLen{151}
\def\EPVOUCenteredOffDiagonalMeanMaxFloat{-10.43181324005126953125}
\def\EPVOUCenteredOffDiagonalMeanMaxKey{4810}
\def\EPVOUCenteredOffDiagonalMeanMeanFloat{-13.3744564056396484375}
\def\EPVOUCenteredOffDiagonalMeanMeanKey{6082}
\def\EPVOUCenteredOffDiagonalMeanMedianFloat{-15.03575038909912109375}
\def\EPVOUCenteredOffDiagonalMeanMedianKey{24262}
\def\EPVOUCenteredOffDiagonalMeanMinFloat{-15.0534343719482421875}
\def\EPVOUCenteredOffDiagonalMeanMinKey{15662}
\def\EPVOUCenteredOffDiagonalMeanStdDevFloat{0.735217273235321044921875}
\def\EPVOUCenteredOffDiagonalMedianLen{151}
\def\EPVOUCenteredOffDiagonalMedianMaxFloat{-46.24238494873046789734871708787977695465087890625}
\def\EPVOUCenteredOffDiagonalMedianMaxKey{11124}
\def\EPVOUCenteredOffDiagonalMedianMeanFloat{-55.11651315385933713741906103678047657012939453125}
\def\EPVOUCenteredOffDiagonalMedianMeanKey{5615}
\def\EPVOUCenteredOffDiagonalMedianMedianFloat{-64.76787643432618324368377216160297393798828125}
\def\EPVOUCenteredOffDiagonalMedianMedianKey{19093}
\def\EPVOUCenteredOffDiagonalMedianMinFloat{-65.546325531005862785605131648480892181396484375}
\def\EPVOUCenteredOffDiagonalMedianMinKey{742}
\def\EPVOUCenteredOffDiagonalMedianStdDevFloat{3.75828659435262490973173044039867818355560302734375}
\def\EPVOUCenteredOffDiagonalMinLen{151}
\def\EPVOUCenteredOffDiagonalMinMaxFloat{-54.162384033203125}
\def\EPVOUCenteredOffDiagonalMinMaxKey{11124}
\def\EPVOUCenteredOffDiagonalMinMeanFloat{-66.5613861083984375}
\def\EPVOUCenteredOffDiagonalMinMeanKey{27714}
\def\EPVOUCenteredOffDiagonalMinMedianFloat{-82.39397430419921875}
\def\EPVOUCenteredOffDiagonalMinMedianKey{27671}
\def\EPVOUCenteredOffDiagonalMinMinFloat{-83.0191192626953125}
\def\EPVOUCenteredOffDiagonalMinMinKey{6589}
\def\EPVOUCenteredOffDiagonalMinStdDevFloat{5.750451564788818359375}
\def\EPVOUCenteredOffDiagonalStdDevLen{151}
\def\EPVOUCenteredOffDiagonalStdDevMaxFloat{16.1934719085693359375}
\def\EPVOUCenteredOffDiagonalStdDevMaxKey{742}
\def\EPVOUCenteredOffDiagonalStdDevMeanFloat{13.9622249603271484375}
\def\EPVOUCenteredOffDiagonalStdDevMeanKey{913}
\def\EPVOUCenteredOffDiagonalStdDevMedianFloat{11.8624246120452880859375}
\def\EPVOUCenteredOffDiagonalStdDevMedianKey{9132}
\def\EPVOUCenteredOffDiagonalStdDevMinFloat{11.8513431549072265625}
\def\EPVOUCenteredOffDiagonalStdDevMinKey{8721}
\def\EPVOUCenteredOffDiagonalStdDevStdDevFloat{0.8458144664764404296875}
\def\EPVOUCenteredStdDevLen{151}
\def\EPVOUCenteredStdDevMaxFloat{16.1730365753173828125}
\def\EPVOUCenteredStdDevMaxKey{742}
\def\EPVOUCenteredStdDevMeanFloat{13.9517650604248046875}
\def\EPVOUCenteredStdDevMeanKey{913}
\def\EPVOUCenteredStdDevMedianFloat{11.864238739013671875}
\def\EPVOUCenteredStdDevMedianKey{9132}
\def\EPVOUCenteredStdDevMinFloat{11.85459423065185546875}
\def\EPVOUCenteredStdDevMinKey{8721}
\def\EPVOUCenteredStdDevStdDevFloat{0.842473804950714111328125}
\def\EPVOUDiagonalLenLen{151}
\def\EPVOUDiagonalLenMaxFloat{64}
\def\EPVOUDiagonalLenMaxKey{50}
\def\EPVOUDiagonalLenMeanFloat{64}
\def\EPVOUDiagonalLenMeanKey{50}
\def\EPVOUDiagonalLenMedianFloat{64}
\def\EPVOUDiagonalLenMedianKey{50}
\def\EPVOUDiagonalLenMinFloat{64}
\def\EPVOUDiagonalLenMinKey{50}
\def\EPVOUDiagonalLenStdDevFloat{0}
\def\EPVOUDiagonalMaxLen{151}
\def\EPVOUDiagonalMaxMaxFloat{42.374660491943359375}
\def\EPVOUDiagonalMaxMaxKey{20013}
\def\EPVOUDiagonalMaxMeanFloat{35.318450927734375}
\def\EPVOUDiagonalMaxMeanKey{6549}
\def\EPVOUDiagonalMaxMedianFloat{29.71045398712158203125}
\def\EPVOUDiagonalMaxMedianKey{11124}
\def\EPVOUDiagonalMaxMinFloat{29.3502197265625}
\def\EPVOUDiagonalMaxMinKey{16149}
\def\EPVOUDiagonalMaxStdDevFloat{2.8467028141021728515625}
\def\EPVOUDiagonalMeanLen{151}
\def\EPVOUDiagonalMeanMaxFloat{17.058948516845703125}
\def\EPVOUDiagonalMeanMaxKey{742}
\def\EPVOUDiagonalMeanMeanFloat{14.3908252716064453125}
\def\EPVOUDiagonalMeanMeanKey{23696}
\def\EPVOUDiagonalMeanMedianFloat{11.7988603115081787109375}
\def\EPVOUDiagonalMeanMedianKey{7098}
\def\EPVOUDiagonalMeanMinFloat{10.960205078125}
\def\EPVOUDiagonalMeanMinKey{4810}
\def\EPVOUDiagonalMeanStdDevFloat{1.00385248661041259765625}
\def\EPVOUDiagonalMedianLen{151}
\def\EPVOUDiagonalMedianMaxFloat{6.07841091632842989156415569595992565155029296875}
\def\EPVOUDiagonalMedianMaxKey{6159}
\def\EPVOUDiagonalMedianMeanFloat{2.75541484229217292778457704116590321063995361328125}
\def\EPVOUDiagonalMedianMeanKey{12561}
\def\EPVOUDiagonalMedianMedianFloat{-0.66395353004336354896253169499686919152736663818359375}
\def\EPVOUDiagonalMedianMedianKey{5615}
\def\EPVOUDiagonalMedianMinFloat{-1.6813383668661117109621727649937383830547332763671875}
\def\EPVOUDiagonalMedianMinKey{6589}
\def\EPVOUDiagonalMedianStdDevFloat{1.3246648346373692817223854945041239261627197265625}
\def\EPVOUDiagonalMinLen{151}
\def\EPVOUDiagonalMinMaxFloat{5.8455810546875}
\def\EPVOUDiagonalMinMaxKey{6159}
\def\EPVOUDiagonalMinMeanFloat{2.5319182872772216796875}
\def\EPVOUDiagonalMinMeanKey{24202}
\def\EPVOUDiagonalMinMedianFloat{-0.84708559513092041015625}
\def\EPVOUDiagonalMinMedianKey{5615}
\def\EPVOUDiagonalMinMinFloat{-1.8642990589141845703125}
\def\EPVOUDiagonalMinMinKey{6589}
\def\EPVOUDiagonalMinStdDevFloat{1.369691371917724609375}
\def\EPVOUDiagonalStdDevLen{151}
\def\EPVOUDiagonalStdDevMaxFloat{11.086559295654296875}
\def\EPVOUDiagonalStdDevMaxKey{6589}
\def\EPVOUDiagonalStdDevMeanFloat{8.31965732574462890625}
\def\EPVOUDiagonalStdDevMeanKey{4430}
\def\EPVOUDiagonalStdDevMedianFloat{7.13535594940185546875}
\def\EPVOUDiagonalStdDevMedianKey{26932}
\def\EPVOUDiagonalStdDevMinFloat{7.12699031829833984375}
\def\EPVOUDiagonalStdDevMinKey{20976}
\def\EPVOUDiagonalStdDevStdDevFloat{0.709415912628173828125}
\def\EPVOUInputsWithCopyingFailureLenLen{151}
\def\EPVOUInputsWithCopyingFailureLenMaxFloat{34}
\def\EPVOUInputsWithCopyingFailureLenMaxKey{7884}
\def\EPVOUInputsWithCopyingFailureLenMeanFloat{30.5165562913907280062630889005959033966064453125}
\def\EPVOUInputsWithCopyingFailureLenMeanKey{123}
\def\EPVOUInputsWithCopyingFailureLenMedianFloat{27.75}
\def\EPVOUInputsWithCopyingFailureLenMedianKey{1696}
\def\EPVOUInputsWithCopyingFailureLenMinFloat{27}
\def\EPVOUInputsWithCopyingFailureLenMinKey{519}
\def\EPVOUInputsWithCopyingFailureLenStdDevFloat{1.3063994533064882119788308045826852321624755859375}
\def\EPVOUInputsWithCopyingFailureMaxLen{151}
\def\EPVOUInputsWithCopyingFailureMaxMaxFloat{48}
\def\EPVOUInputsWithCopyingFailureMaxMaxKey{4810}
\def\EPVOUInputsWithCopyingFailureMaxMeanFloat{30.874172185430463599686845554970204830169677734375}
\def\EPVOUInputsWithCopyingFailureMaxMeanKey{104}
\def\EPVOUInputsWithCopyingFailureMaxMedianFloat{26.75}
\def\EPVOUInputsWithCopyingFailureMaxMedianKey{1696}
\def\EPVOUInputsWithCopyingFailureMaxMinFloat{26}
\def\EPVOUInputsWithCopyingFailureMaxMinKey{519}
\def\EPVOUInputsWithCopyingFailureMaxStdDevFloat{2.750808757081141919798028538934886455535888671875}
\def\EPVOUInputsWithCopyingFailureMeanLen{151}
\def\EPVOUInputsWithCopyingFailureMeanMaxFloat{16.676470588235293490697586094029247760772705078125}
\def\EPVOUInputsWithCopyingFailureMeanMaxKey{7884}
\def\EPVOUInputsWithCopyingFailureMeanMeanFloat{14.8255099864356321148761708172969520092010498046875}
\def\EPVOUInputsWithCopyingFailureMeanMeanKey{29726}
\def\EPVOUInputsWithCopyingFailureMeanMedianFloat{13.375}
\def\EPVOUInputsWithCopyingFailureMeanMedianKey{1696}
\def\EPVOUInputsWithCopyingFailureMeanMinFloat{13}
\def\EPVOUInputsWithCopyingFailureMeanMinKey{519}
\def\EPVOUInputsWithCopyingFailureMeanStdDevFloat{0.66597369225369629219812850351445376873016357421875}
\def\EPVOUInputsWithCopyingFailureMedianLen{151}
\def\EPVOUInputsWithCopyingFailureMedianMaxFloat{0.1650000000000000077715611723760957829654216766357421875}
\def\EPVOUInputsWithCopyingFailureMedianMaxKey{7884}
\def\EPVOUInputsWithCopyingFailureMedianMeanFloat{0.1475827814569536655664450108815799467265605926513671875}
\def\EPVOUInputsWithCopyingFailureMedianMeanKey{123}
\def\EPVOUInputsWithCopyingFailureMedianMedianFloat{0.1337500000000000077715611723760957829654216766357421875}
\def\EPVOUInputsWithCopyingFailureMedianMedianKey{1696}
\def\EPVOUInputsWithCopyingFailureMedianMinFloat{0.13000000000000000444089209850062616169452667236328125}
\def\EPVOUInputsWithCopyingFailureMedianMinKey{519}
\def\EPVOUInputsWithCopyingFailureMedianStdDevFloat{0.006531997266532438804753635253064203425310552120208740234375}
\def\EPVOUInputsWithCopyingFailureMinLen{151}
\def\EPVOUInputsWithCopyingFailureMinMaxFloat{0}
\def\EPVOUInputsWithCopyingFailureMinMaxKey{50}
\def\EPVOUInputsWithCopyingFailureMinMeanFloat{0}
\def\EPVOUInputsWithCopyingFailureMinMeanKey{50}
\def\EPVOUInputsWithCopyingFailureMinMedianFloat{0}
\def\EPVOUInputsWithCopyingFailureMinMedianKey{50}
\def\EPVOUInputsWithCopyingFailureMinMinFloat{0}
\def\EPVOUInputsWithCopyingFailureMinMinKey{50}
\def\EPVOUInputsWithCopyingFailureMinStdDevFloat{0}
\def\EPVOUInputsWithCopyingFailureStdDevLen{151}
\def\EPVOUInputsWithCopyingFailureStdDevMaxFloat{10.4589778909017923069768585264682769775390625}
\def\EPVOUInputsWithCopyingFailureStdDevMaxKey{4810}
\def\EPVOUInputsWithCopyingFailureStdDevMeanFloat{8.9237493212836032085988335893489420413970947265625}
\def\EPVOUInputsWithCopyingFailureStdDevMeanKey{18146}
\def\EPVOUInputsWithCopyingFailureStdDevMedianFloat{8.005530648950969663246723939664661884307861328125}
\def\EPVOUInputsWithCopyingFailureStdDevMedianKey{1696}
\def\EPVOUInputsWithCopyingFailureStdDevMinFloat{7.7888809636986149342874341527931392192840576171875}
\def\EPVOUInputsWithCopyingFailureStdDevMinKey{519}
\def\EPVOUInputsWithCopyingFailureStdDevStdDevFloat{0.43390130557822337298290449325577355921268463134765625}
\def\EPVOULenLen{151}
\def\EPVOULenMaxFloat{4096}
\def\EPVOULenMaxKey{50}
\def\EPVOULenMeanFloat{4096}
\def\EPVOULenMeanKey{50}
\def\EPVOULenMedianFloat{4096}
\def\EPVOULenMedianKey{50}
\def\EPVOULenMinFloat{4096}
\def\EPVOULenMinKey{50}
\def\EPVOULenStdDevFloat{0}
\def\EPVOUMaxAboveDiagLenLen{151}
\def\EPVOUMaxAboveDiagLenMaxFloat{64}
\def\EPVOUMaxAboveDiagLenMaxKey{50}
\def\EPVOUMaxAboveDiagLenMeanFloat{64}
\def\EPVOUMaxAboveDiagLenMeanKey{50}
\def\EPVOUMaxAboveDiagLenMedianFloat{64}
\def\EPVOUMaxAboveDiagLenMedianKey{50}
\def\EPVOUMaxAboveDiagLenMinFloat{64}
\def\EPVOUMaxAboveDiagLenMinKey{50}
\def\EPVOUMaxAboveDiagLenStdDevFloat{0}
\def\EPVOUMaxAboveDiagMaxLen{151}
\def\EPVOUMaxAboveDiagMaxMaxFloat{16.0412616729736328125}
\def\EPVOUMaxAboveDiagMaxMaxKey{20415}
\def\EPVOUMaxAboveDiagMaxMeanFloat{12.173976898193359375}
\def\EPVOUMaxAboveDiagMaxMeanKey{13654}
\def\EPVOUMaxAboveDiagMaxMedianFloat{8.7478287220001220703125}
\def\EPVOUMaxAboveDiagMaxMedianKey{17197}
\def\EPVOUMaxAboveDiagMaxMinFloat{8.664562225341796875}
\def\EPVOUMaxAboveDiagMaxMinKey{3284}
\def\EPVOUMaxAboveDiagMaxStdDevFloat{1.47744667530059814453125}
\def\EPVOUMaxAboveDiagMeanLen{151}
\def\EPVOUMaxAboveDiagMeanMaxFloat{0.806737422943115234375}
\def\EPVOUMaxAboveDiagMeanMaxKey{1412}
\def\EPVOUMaxAboveDiagMeanMeanFloat{-0.4321459829807281494140625}
\def\EPVOUMaxAboveDiagMeanMeanKey{28090}
\def\EPVOUMaxAboveDiagMeanMedianFloat{-1.644882857799530029296875}
\def\EPVOUMaxAboveDiagMeanMedianKey{26829}
\def\EPVOUMaxAboveDiagMeanMinFloat{-1.6515109539031982421875}
\def\EPVOUMaxAboveDiagMeanMinKey{3284}
\def\EPVOUMaxAboveDiagMeanStdDevFloat{0.4701806604862213134765625}
\def\EPVOUMaxAboveDiagMedianLen{151}
\def\EPVOUMaxAboveDiagMedianMaxFloat{-10.8870730304718019709753207280300557613372802734375}
\def\EPVOUMaxAboveDiagMedianMaxKey{20338}
\def\EPVOUMaxAboveDiagMedianMeanFloat{-12.134409499357868611468802555464208126068115234375}
\def\EPVOUMaxAboveDiagMedianMeanKey{6589}
\def\EPVOUMaxAboveDiagMedianMedianFloat{-14.5466645312309257320748656638897955417633056640625}
\def\EPVOUMaxAboveDiagMedianMedianKey{16284}
\def\EPVOUMaxAboveDiagMedianMinFloat{-15.6915497207641596588700849679298698902130126953125}
\def\EPVOUMaxAboveDiagMedianMinKey{2306}
\def\EPVOUMaxAboveDiagMedianStdDevFloat{0.676813038713518277944558576564304530620574951171875}
\def\EPVOUMaxAboveDiagMinLen{151}
\def\EPVOUMaxAboveDiagMinMaxFloat{-10.9172801971435546875}
\def\EPVOUMaxAboveDiagMinMaxKey{20338}
\def\EPVOUMaxAboveDiagMinMeanFloat{-12.35158824920654296875}
\def\EPVOUMaxAboveDiagMinMeanKey{17080}
\def\EPVOUMaxAboveDiagMinMedianFloat{-15.832014560699462890625}
\def\EPVOUMaxAboveDiagMinMedianKey{16284}
\def\EPVOUMaxAboveDiagMinMinFloat{-16.812076568603515625}
\def\EPVOUMaxAboveDiagMinMinKey{2306}
\def\EPVOUMaxAboveDiagMinStdDevFloat{0.84118878841400146484375}
\def\EPVOUMaxAboveDiagStdDevLen{151}
\def\EPVOUMaxAboveDiagStdDevMaxFloat{8.89408779144287109375}
\def\EPVOUMaxAboveDiagStdDevMaxKey{20539}
\def\EPVOUMaxAboveDiagStdDevMeanFloat{7.821030139923095703125}
\def\EPVOUMaxAboveDiagStdDevMeanKey{23447}
\def\EPVOUMaxAboveDiagStdDevMedianFloat{6.7523357868194580078125}
\def\EPVOUMaxAboveDiagStdDevMedianKey{26829}
\def\EPVOUMaxAboveDiagStdDevMinFloat{6.675055980682373046875}
\def\EPVOUMaxAboveDiagStdDevMinKey{4810}
\def\EPVOUMaxAboveDiagStdDevStdDevFloat{0.4455790817737579345703125}
\def\EPVOUMaxLen{151}
\def\EPVOUMaxMaxFloat{42.374660491943359375}
\def\EPVOUMaxMaxKey{20013}
\def\EPVOUMaxMeanFloat{35.318450927734375}
\def\EPVOUMaxMeanKey{6549}
\def\EPVOUMaxMedianFloat{29.71045398712158203125}
\def\EPVOUMaxMedianKey{11124}
\def\EPVOUMaxMinFloat{29.3502197265625}
\def\EPVOUMaxMinKey{16149}
\def\EPVOUMaxRowDiffLenLen{151}
\def\EPVOUMaxRowDiffLenMaxFloat{64}
\def\EPVOUMaxRowDiffLenMaxKey{50}
\def\EPVOUMaxRowDiffLenMeanFloat{64}
\def\EPVOUMaxRowDiffLenMeanKey{50}
\def\EPVOUMaxRowDiffLenMedianFloat{64}
\def\EPVOUMaxRowDiffLenMedianKey{50}
\def\EPVOUMaxRowDiffLenMinFloat{64}
\def\EPVOUMaxRowDiffLenMinKey{50}
\def\EPVOUMaxRowDiffLenStdDevFloat{0}
\def\EPVOUMaxRowDiffMaxLen{151}
\def\EPVOUMaxRowDiffMaxMaxFloat{83.0191192626953125}
\def\EPVOUMaxRowDiffMaxMaxKey{6589}
\def\EPVOUMaxRowDiffMaxMeanFloat{66.5613861083984375}
\def\EPVOUMaxRowDiffMaxMeanKey{27714}
\def\EPVOUMaxRowDiffMaxMedianFloat{54.67501068115234375}
\def\EPVOUMaxRowDiffMaxMedianKey{3284}
\def\EPVOUMaxRowDiffMaxMinFloat{54.162384033203125}
\def\EPVOUMaxRowDiffMaxMinKey{11124}
\def\EPVOUMaxRowDiffMaxStdDevFloat{5.750451564788818359375}
\def\EPVOUMaxRowDiffMeanLen{151}
\def\EPVOUMaxRowDiffMeanMaxFloat{41.493408203125}
\def\EPVOUMaxRowDiffMeanMaxKey{742}
\def\EPVOUMaxRowDiffMeanMeanFloat{33.502140045166015625}
\def\EPVOUMaxRowDiffMeanMeanKey{6589}
\def\EPVOUMaxRowDiffMeanMedianFloat{26.2496795654296875}
\def\EPVOUMaxRowDiffMeanMedianKey{3284}
\def\EPVOUMaxRowDiffMeanMinFloat{26.150562286376953125}
\def\EPVOUMaxRowDiffMeanMinKey{4810}
\def\EPVOUMaxRowDiffMeanStdDevFloat{2.8419148921966552734375}
\def\EPVOUMaxRowDiffMedianLen{151}
\def\EPVOUMaxRowDiffMedianMaxFloat{28.676967391967775000694018672220408916473388671875}
\def\EPVOUMaxRowDiffMedianMaxKey{29565}
\def\EPVOUMaxRowDiffMedianMeanFloat{21.24692602107067074257429339922964572906494140625}
\def\EPVOUMaxRowDiffMedianMeanKey{32103}
\def\EPVOUMaxRowDiffMedianMedianFloat{13.496902852058411781399627216160297393798828125}
\def\EPVOUMaxRowDiffMedianMedianKey{3284}
\def\EPVOUMaxRowDiffMedianMinFloat{13.456567506790161559138141456060111522674560546875}
\def\EPVOUMaxRowDiffMedianMinKey{17096}
\def\EPVOUMaxRowDiffMedianStdDevFloat{3.41519952927979542067760121426545083522796630859375}
\def\EPVOUMaxRowDiffMinLen{151}
\def\EPVOUMaxRowDiffMinMaxFloat{28.3949069976806640625}
\def\EPVOUMaxRowDiffMinMaxKey{20539}
\def\EPVOUMaxRowDiffMinMeanFloat{20.787029266357421875}
\def\EPVOUMaxRowDiffMinMeanKey{519}
\def\EPVOUMaxRowDiffMinMedianFloat{13.10850811004638671875}
\def\EPVOUMaxRowDiffMinMedianKey{17096}
\def\EPVOUMaxRowDiffMinMinFloat{12.93810272216796875}
\def\EPVOUMaxRowDiffMinMinKey{4800}
\def\EPVOUMaxRowDiffMinStdDevFloat{3.5155165195465087890625}
\def\EPVOUMaxRowDiffStdDevLen{151}
\def\EPVOUMaxRowDiffStdDevMaxFloat{14.48293304443359375}
\def\EPVOUMaxRowDiffStdDevMaxKey{6589}
\def\EPVOUMaxRowDiffStdDevMeanFloat{9.94670772552490234375}
\def\EPVOUMaxRowDiffStdDevMeanKey{123}
\def\EPVOUMaxRowDiffStdDevMedianFloat{7.19509220123291015625}
\def\EPVOUMaxRowDiffStdDevMedianKey{13654}
\def\EPVOUMaxRowDiffStdDevMinFloat{6.71072673797607421875}
\def\EPVOUMaxRowDiffStdDevMinKey{1681}
\def\EPVOUMaxRowDiffStdDevStdDevFloat{1.20370352268218994140625}
\def\EPVOUMaxStdDevFloat{2.8467028141021728515625}
\def\EPVOUMeanLen{151}
\def\EPVOUMeanMaxFloat{2.34634876251220703125}
\def\EPVOUMeanMaxKey{742}
\def\EPVOUMeanMeanFloat{1.2253463268280029296875}
\def\EPVOUMeanMeanKey{32103}
\def\EPVOUMeanMedianFloat{0.56866867840290069580078125}
\def\EPVOUMeanMedianKey{11130}
\def\EPVOUMeanMinFloat{0.56523621082305908203125}
\def\EPVOUMeanMinKey{5358}
\def\EPVOUMeanStdDevFloat{0.393566548824310302734375}
\def\EPVOUMedianLen{151}
\def\EPVOUMedianMaxFloat{-18.189110279083251953125}
\def\EPVOUMedianMaxKey{3284}
\def\EPVOUMedianMeanFloat{-23.10987852393396480010778759606182575225830078125}
\def\EPVOUMedianMeanKey{12493}
\def\EPVOUMedianMedianFloat{-28.25610443353652811993015347979962825775146484375}
\def\EPVOUMedianMedianKey{742}
\def\EPVOUMedianMinFloat{-28.28837337493896342266452847979962825775146484375}
\def\EPVOUMedianMinKey{6159}
\def\EPVOUMedianStdDevFloat{2.016771222940575203352864264161325991153717041015625}
\def\EPVOUMinLen{151}
\def\EPVOUMinMaxFloat{-24.396045684814453125}
\def\EPVOUMinMaxKey{11124}
\def\EPVOUMinMeanFloat{-32.27516937255859375}
\def\EPVOUMinMeanKey{29565}
\def\EPVOUMinMedianFloat{-44.29390430450439453125}
\def\EPVOUMinMedianKey{27671}
\def\EPVOUMinMinFloat{-44.590057373046875}
\def\EPVOUMinMinKey{6589}
\def\EPVOUMinStdDevFloat{3.508446216583251953125}
\def\EPVOUOffDiagonalAbsLenLen{151}
\def\EPVOUOffDiagonalAbsLenMaxFloat{4032}
\def\EPVOUOffDiagonalAbsLenMaxKey{50}
\def\EPVOUOffDiagonalAbsLenMeanFloat{4032}
\def\EPVOUOffDiagonalAbsLenMeanKey{50}
\def\EPVOUOffDiagonalAbsLenMedianFloat{4032}
\def\EPVOUOffDiagonalAbsLenMedianKey{50}
\def\EPVOUOffDiagonalAbsLenMinFloat{4032}
\def\EPVOUOffDiagonalAbsLenMinKey{50}
\def\EPVOUOffDiagonalAbsLenStdDevFloat{0}
\def\EPVOUOffDiagonalAbsMaxLen{151}
\def\EPVOUOffDiagonalAbsMaxMaxFloat{44.590057373046875}
\def\EPVOUOffDiagonalAbsMaxMaxKey{6589}
\def\EPVOUOffDiagonalAbsMaxMeanFloat{32.27516937255859375}
\def\EPVOUOffDiagonalAbsMaxMeanKey{29565}
\def\EPVOUOffDiagonalAbsMaxMedianFloat{25.530743122100830078125}
\def\EPVOUOffDiagonalAbsMaxMedianKey{1951}
\def\EPVOUOffDiagonalAbsMaxMinFloat{24.396045684814453125}
\def\EPVOUOffDiagonalAbsMaxMinKey{11124}
\def\EPVOUOffDiagonalAbsMaxStdDevFloat{3.508446216583251953125}
\def\EPVOUOffDiagonalAbsMeanLen{151}
\def\EPVOUOffDiagonalAbsMeanMaxFloat{9.50363826751708984375}
\def\EPVOUOffDiagonalAbsMeanMaxKey{742}
\def\EPVOUOffDiagonalAbsMeanMeanFloat{7.09508609771728515625}
\def\EPVOUOffDiagonalAbsMeanMeanKey{1696}
\def\EPVOUOffDiagonalAbsMeanMedianFloat{5.31716954708099365234375}
\def\EPVOUOffDiagonalAbsMeanMedianKey{3284}
\def\EPVOUOffDiagonalAbsMeanMinFloat{5.244912624359130859375}
\def\EPVOUOffDiagonalAbsMeanMinKey{4810}
\def\EPVOUOffDiagonalAbsMeanStdDevFloat{0.838552772998809814453125}
\def\EPVOUOffDiagonalAbsMedianLen{151}
\def\EPVOUOffDiagonalAbsMedianMaxFloat{0.15617234528064727339113915149937383830547332763671875}
\def\EPVOUOffDiagonalAbsMedianMaxKey{20415}
\def\EPVOUOffDiagonalAbsMedianMeanFloat{0.08372503260545284542448740694453590549528598785400390625}
\def\EPVOUOffDiagonalAbsMedianMeanKey{1283}
\def\EPVOUOffDiagonalAbsMedianMedianFloat{0.0434831597656011592523128683751565404236316680908203125}
\def\EPVOUOffDiagonalAbsMedianMedianKey{11611}
\def\EPVOUOffDiagonalAbsMedianMinFloat{0.040111691653728485940089143468867405317723751068115234375}
\def\EPVOUOffDiagonalAbsMedianMinKey{11124}
\def\EPVOUOffDiagonalAbsMedianStdDevFloat{0.022151520027394601408676777509754174388945102691650390625}
\def\EPVOUOffDiagonalAbsMinLen{151}
\def\EPVOUOffDiagonalAbsMinMaxFloat{0.0221908092498779296875}
\def\EPVOUOffDiagonalAbsMinMaxKey{26932}
\def\EPVOUOffDiagonalAbsMinMeanFloat{0.0039086225442588329315185546875}
\def\EPVOUOffDiagonalAbsMinMeanKey{7098}
\def\EPVOUOffDiagonalAbsMinMedianFloat{0.0000567324459552764892578125}
\def\EPVOUOffDiagonalAbsMinMedianKey{15622}
\def\EPVOUOffDiagonalAbsMinMinFloat{0.00005276501178741455078125}
\def\EPVOUOffDiagonalAbsMinMinKey{19488}
\def\EPVOUOffDiagonalAbsMinStdDevFloat{0.00350805954076349735260009765625}
\def\EPVOUOffDiagonalAbsStdDevLen{151}
\def\EPVOUOffDiagonalAbsStdDevMaxFloat{5.860240936279296875}
\def\EPVOUOffDiagonalAbsStdDevMaxKey{742}
\def\EPVOUOffDiagonalAbsStdDevMeanFloat{4.5982990264892578125}
\def\EPVOUOffDiagonalAbsStdDevMeanKey{3254}
\def\EPVOUOffDiagonalAbsStdDevMedianFloat{3.652351081371307373046875}
\def\EPVOUOffDiagonalAbsStdDevMedianKey{9132}
\def\EPVOUOffDiagonalAbsStdDevMinFloat{3.53973102569580078125}
\def\EPVOUOffDiagonalAbsStdDevMinKey{3284}
\def\EPVOUOffDiagonalAbsStdDevStdDevFloat{0.4003148376941680908203125}
\def\EPVOUOffDiagonalLenLen{151}
\def\EPVOUOffDiagonalLenMaxFloat{4032}
\def\EPVOUOffDiagonalLenMaxKey{50}
\def\EPVOUOffDiagonalLenMeanFloat{4032}
\def\EPVOUOffDiagonalLenMeanKey{50}
\def\EPVOUOffDiagonalLenMedianFloat{4032}
\def\EPVOUOffDiagonalLenMedianKey{50}
\def\EPVOUOffDiagonalLenMinFloat{4032}
\def\EPVOUOffDiagonalLenMinKey{50}
\def\EPVOUOffDiagonalLenStdDevFloat{0}
\def\EPVOUOffDiagonalMaxLen{151}
\def\EPVOUOffDiagonalMaxMaxFloat{30.27228546142578125}
\def\EPVOUOffDiagonalMaxMaxKey{19093}
\def\EPVOUOffDiagonalMaxMeanFloat{23.7827053070068359375}
\def\EPVOUOffDiagonalMaxMeanKey{30684}
\def\EPVOUOffDiagonalMaxMedianFloat{18.4834766387939453125}
\def\EPVOUOffDiagonalMaxMedianKey{11124}
\def\EPVOUOffDiagonalMaxMinFloat{18.2821407318115234375}
\def\EPVOUOffDiagonalMaxMinKey{17197}
\def\EPVOUOffDiagonalMaxStdDevFloat{2.7955169677734375}
\def\EPVOUOffDiagonalMeanLen{151}
\def\EPVOUOffDiagonalMeanMaxFloat{2.1128151416778564453125}
\def\EPVOUOffDiagonalMeanMaxKey{742}
\def\EPVOUOffDiagonalMeanMeanFloat{1.0163705348968505859375}
\def\EPVOUOffDiagonalMeanMeanKey{32103}
\def\EPVOUOffDiagonalMeanMedianFloat{0.3762396275997161865234375}
\def\EPVOUOffDiagonalMeanMedianKey{11130}
\def\EPVOUOffDiagonalMeanMinFloat{0.3602350652217864990234375}
\def\EPVOUOffDiagonalMeanMinKey{5358}
\def\EPVOUOffDiagonalMeanStdDevFloat{0.3870448768138885498046875}
\def\EPVOUOffDiagonalMedianLen{151}
\def\EPVOUOffDiagonalMedianMaxFloat{-18.28663406372070454608547152020037174224853515625}
\def\EPVOUOffDiagonalMedianMaxKey{8721}
\def\EPVOUOffDiagonalMedianMeanFloat{-23.1686727966535954692517407238483428955078125}
\def\EPVOUOffDiagonalMedianMeanKey{15043}
\def\EPVOUOffDiagonalMedianMedianFloat{-28.31390732049941760806177626363933086395263671875}
\def\EPVOUOffDiagonalMedianMedianKey{742}
\def\EPVOUOffDiagonalMedianMinFloat{-28.37518245697021512796709430404007434844970703125}
\def\EPVOUOffDiagonalMedianMinKey{6159}
\def\EPVOUOffDiagonalMedianStdDevFloat{2.023275371825525414948288016603328287601470947265625}
\def\EPVOUOffDiagonalMinLen{151}
\def\EPVOUOffDiagonalMinMaxFloat{-24.396045684814453125}
\def\EPVOUOffDiagonalMinMaxKey{11124}
\def\EPVOUOffDiagonalMinMeanFloat{-32.27516937255859375}
\def\EPVOUOffDiagonalMinMeanKey{29565}
\def\EPVOUOffDiagonalMinMedianFloat{-44.29390430450439453125}
\def\EPVOUOffDiagonalMinMedianKey{27671}
\def\EPVOUOffDiagonalMinMinFloat{-44.590057373046875}
\def\EPVOUOffDiagonalMinMinKey{6589}
\def\EPVOUOffDiagonalMinStdDevFloat{3.508446216583251953125}
\def\EPVOUOffDiagonalStdDevLen{151}
\def\EPVOUOffDiagonalStdDevMaxFloat{10.96346569061279296875}
\def\EPVOUOffDiagonalStdDevMaxKey{742}
\def\EPVOUOffDiagonalStdDevMeanFloat{8.390468597412109375}
\def\EPVOUOffDiagonalStdDevMeanKey{29052}
\def\EPVOUOffDiagonalStdDevMedianFloat{6.41249370574951171875}
\def\EPVOUOffDiagonalStdDevMedianKey{4810}
\def\EPVOUOffDiagonalStdDevMinFloat{6.393895626068115234375}
\def\EPVOUOffDiagonalStdDevMinKey{3284}
\def\EPVOUOffDiagonalStdDevStdDevFloat{0.8747894763946533203125}
\def\EPVOUStdDevLen{151}
\def\EPVOUStdDevMaxFloat{11.08087921142578125}
\def\EPVOUStdDevMaxKey{742}
\def\EPVOUStdDevMeanFloat{8.5536289215087890625}
\def\EPVOUStdDevMeanKey{20751}
\def\EPVOUStdDevMedianFloat{6.58859336376190185546875}
\def\EPVOUStdDevMedianKey{3284}
\def\EPVOUStdDevMinFloat{6.57523345947265625}
\def\EPVOUStdDevMinKey{4810}
\def\EPVOUStdDevStdDevFloat{0.858868420124053955078125}
\def\EQKEErrBoundMaxDiffExactLen{151}
\def\EQKEErrBoundMaxDiffExactMaxFloat{3.240688323974609375}
\def\EQKEErrBoundMaxDiffExactMaxKey{8299}
\def\EQKEErrBoundMaxDiffExactMeanFloat{1.5684236390701193908370214558090083301067352294921875}
\def\EQKEErrBoundMaxDiffExactMeanKey{1283}
\def\EQKEErrBoundMaxDiffExactMedianFloat{0.986862957477569580078125}
\def\EQKEErrBoundMaxDiffExactMedianKey{14929}
\def\EQKEErrBoundMaxDiffExactMinFloat{0.972379207611083984375}
\def\EQKEErrBoundMaxDiffExactMinKey{18289}
\def\EQKEErrBoundMaxDiffExactStdDevFloat{0.297939111957562563492984963886556215584278106689453125}
\def\EQKEErrBoundMaxDiffLen{151}
\def\EQKEErrBoundMaxDiffMaxFloat{5.9180507659912109375}
\def\EQKEErrBoundMaxDiffMaxKey{24438}
\def\EQKEErrBoundMaxDiffMeanFloat{4.6426645604190444061032394529320299625396728515625}
\def\EQKEErrBoundMaxDiffMeanKey{13716}
\def\EQKEErrBoundMaxDiffMedianFloat{3.75143182277679443359375}
\def\EQKEErrBoundMaxDiffMedianKey{27300}
\def\EQKEErrBoundMaxDiffMinFloat{3.7459304332733154296875}
\def\EQKEErrBoundMaxDiffMinKey{18289}
\def\EQKEErrBoundMaxDiffStdDevFloat{0.44003606333357636604119988987804390490055084228515625}
\def\EQKEErrBoundMaxDiffSubproductLen{151}
\def\EQKEErrBoundMaxDiffSubproductMaxFloat{5.9180507659912109375}
\def\EQKEErrBoundMaxDiffSubproductMaxKey{24438}
\def\EQKEErrBoundMaxDiffSubproductMeanFloat{4.6426645604190444061032394529320299625396728515625}
\def\EQKEErrBoundMaxDiffSubproductMeanKey{13716}
\def\EQKEErrBoundMaxDiffSubproductMedianFloat{3.75143182277679443359375}
\def\EQKEErrBoundMaxDiffSubproductMedianKey{27300}
\def\EQKEErrBoundMaxDiffSubproductMinFloat{3.7459304332733154296875}
\def\EQKEErrBoundMaxDiffSubproductMinKey{18289}
\def\EQKEErrBoundMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMaxFloat{155.63616943359375}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMaxKey{4810}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMeanFloat{91.4297275164269507286007865332067012786865234375}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMeanKey{4729}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMedianFloat{78.906459808349609375}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMedianKey{29022}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMinFloat{78.7463226318359375}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMinKey{7238}
\def\EQKEErrBoundMaxDiffSubproductRecursiveStdDevFloat{7.59340187814654488107635188498534262180328369140625}
\def\EQKEErrBoundMaxDiffSubproductStdDevFloat{0.44003606333357636604119988987804390490055084228515625}
\def\EQKEErrBoundMeanMaxDiffLen{151}
\def\EQKEErrBoundMeanMaxDiffMaxFloat{5.87827014923095703125}
\def\EQKEErrBoundMeanMaxDiffMaxKey{24438}
\def\EQKEErrBoundMeanMaxDiffMeanFloat{4.65154951139791084102625973173417150974273681640625}
\def\EQKEErrBoundMeanMaxDiffMeanKey{17080}
\def\EQKEErrBoundMeanMaxDiffMedianFloat{3.79167711734771728515625}
\def\EQKEErrBoundMeanMaxDiffMedianKey{18289}
\def\EQKEErrBoundMeanMaxDiffMinFloat{3.74662494659423828125}
\def\EQKEErrBoundMeanMaxDiffMinKey{27300}
\def\EQKEErrBoundMeanMaxDiffStdDevFloat{0.4412442825297662185590752415009774267673492431640625}
\def\EQKEErrBoundMeanMaxDiffSubproductLen{151}
\def\EQKEErrBoundMeanMaxDiffSubproductMaxFloat{5.87827014923095703125}
\def\EQKEErrBoundMeanMaxDiffSubproductMaxKey{24438}
\def\EQKEErrBoundMeanMaxDiffSubproductMeanFloat{4.65154951139791084102625973173417150974273681640625}
\def\EQKEErrBoundMeanMaxDiffSubproductMeanKey{17080}
\def\EQKEErrBoundMeanMaxDiffSubproductMedianFloat{3.79167711734771728515625}
\def\EQKEErrBoundMeanMaxDiffSubproductMedianKey{18289}
\def\EQKEErrBoundMeanMaxDiffSubproductMinFloat{3.74662494659423828125}
\def\EQKEErrBoundMeanMaxDiffSubproductMinKey{27300}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMaxFloat{156.4159393310546875}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMaxKey{4810}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMeanFloat{91.266749906224134747390053234994411468505859375}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMeanKey{15622}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMedianFloat{79.3579044342041015625}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMedianKey{29022}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMinFloat{78.61283111572265625}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMinKey{7238}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveStdDevFloat{7.59797218712847044486125014373101294040679931640625}
\def\EQKEErrBoundMeanMaxDiffSubproductStdDevFloat{0.4412442825297662185590752415009774267673492431640625}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMaxFloat{156.3029937744140625}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMaxKey{4810}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMeanFloat{92.8864845124301581336112576536834239959716796875}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMeanKey{19004}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMedianFloat{81.2790679931640625}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMedianKey{29022}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMinFloat{80.37683868408203125}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMinKey{7238}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveStdDevFloat{7.6339667658878003209110829629935324192047119140625}
\def\EQKEErrBoundSvdLen{151}
\def\EQKEErrBoundSvdMaxFloat{10.73470783233642578125}
\def\EQKEErrBoundSvdMaxKey{8299}
\def\EQKEErrBoundSvdMeanFloat{7.61620194390909599491124026826582849025726318359375}
\def\EQKEErrBoundSvdMeanKey{12141}
\def\EQKEErrBoundSvdMedianFloat{5.3824913501739501953125}
\def\EQKEErrBoundSvdMedianKey{18289}
\def\EQKEErrBoundSvdMinFloat{5.3243618011474609375}
\def\EQKEErrBoundSvdMinKey{29726}
\def\EQKEErrBoundSvdStdDevFloat{1.16211599614242633293770268210209906101226806640625}
\def\EQKEErrFirstSingularLen{151}
\def\EQKEErrFirstSingularMaxFloat{7.59058666229248046875}
\def\EQKEErrFirstSingularMaxKey{8299}
\def\EQKEErrFirstSingularMeanFloat{5.3854682066582686417177683324553072452545166015625}
\def\EQKEErrFirstSingularMeanKey{12141}
\def\EQKEErrFirstSingularMedianFloat{3.805996119976043701171875}
\def\EQKEErrFirstSingularMedianKey{18289}
\def\EQKEErrFirstSingularMinFloat{3.764893054962158203125}
\def\EQKEErrFirstSingularMinKey{29726}
\def\EQKEErrFirstSingularSqrtTwoLen{151}
\def\EQKEErrFirstSingularSqrtTwoMaxFloat{10.734710693359375}
\def\EQKEErrFirstSingularSqrtTwoMaxKey{8299}
\def\EQKEErrFirstSingularSqrtTwoMeanFloat{7.6162020639078509276487238821573555469512939453125}
\def\EQKEErrFirstSingularSqrtTwoMeanKey{12141}
\def\EQKEErrFirstSingularSqrtTwoMedianFloat{5.38249123096466064453125}
\def\EQKEErrFirstSingularSqrtTwoMedianKey{18289}
\def\EQKEErrFirstSingularSqrtTwoMinFloat{5.32436275482177734375}
\def\EQKEErrFirstSingularSqrtTwoMinKey{29726}
\def\EQKEErrFirstSingularSqrtTwoStdDevFloat{1.162116310488143344770151088596321642398834228515625}
\def\EQKEErrFirstSingularStdDevFloat{0.821740341425333031821764961932785809040069580078125}
\def\EQKEErrFroNormLen{151}
\def\EQKEErrFroNormMaxFloat{11.0111179351806640625}
\def\EQKEErrFroNormMaxKey{6159}
\def\EQKEErrFroNormMeanFloat{8.69618556673163567438678001053631305694580078125}
\def\EQKEErrFroNormMeanKey{5781}
\def\EQKEErrFroNormMedianFloat{6.91580760478973388671875}
\def\EQKEErrFroNormMedianKey{18289}
\def\EQKEErrFroNormMinFloat{6.534504413604736328125}
\def\EQKEErrFroNormMinKey{14929}
\def\EQKEErrFroNormSqrtTwoLen{151}
\def\EQKEErrFroNormSqrtTwoMaxFloat{15.57207202911376953125}
\def\EQKEErrFroNormSqrtTwoMaxKey{6159}
\def\EQKEErrFroNormSqrtTwoMeanFloat{12.298263379280140128457787795923650264739990234375}
\def\EQKEErrFroNormSqrtTwoMeanKey{5781}
\def\EQKEErrFroNormSqrtTwoMedianFloat{9.780428409576416015625}
\def\EQKEErrFroNormSqrtTwoMedianKey{18289}
\def\EQKEErrFroNormSqrtTwoMinFloat{9.241184234619140625}
\def\EQKEErrFroNormSqrtTwoMinKey{14929}
\def\EQKEErrFroNormSqrtTwoStdDevFloat{1.1628471420020485282975641894154250621795654296875}
\def\EQKEErrFroNormStdDevFloat{0.82225710704672450024332874818355776369571685791015625}
\def\EQKEErrLen{4096}
\def\EQKEErrMaxAbsLen{151}
\def\EQKEErrMaxAbsMaxFloat{1.77985727787017822265625}
\def\EQKEErrMaxAbsMaxKey{8299}
\def\EQKEErrMaxAbsMeanFloat{0.88729998054883341129794871449121274054050445556640625}
\def\EQKEErrMaxAbsMeanKey{3284}
\def\EQKEErrMaxAbsMedianFloat{0.58157543838024139404296875}
\def\EQKEErrMaxAbsMedianKey{14929}
\def\EQKEErrMaxAbsMinFloat{0.554614365100860595703125}
\def\EQKEErrMaxAbsMinKey{18289}
\def\EQKEErrMaxAbsStdDevFloat{0.172811105646697160675984150657313875854015350341796875}
\def\EQKEErrMaxLen{151}
\def\EQKEErrMaxMaxFloat{1.77985727787017822265625}
\def\EQKEErrMaxMaxKey{8299}
\def\EQKEErrMaxMeanFloat{0.827064573764801025390625}
\def\EQKEErrMaxMeanKey{24262}
\def\EQKEErrMaxMedianFloat{0.505340285599231719970703125}
\def\EQKEErrMaxMedianKey{13654}
\def\EQKEErrMaxMinFloat{0.4919857680797576904296875}
\def\EQKEErrMaxMinKey{18289}
\def\EQKEErrMaxRowDiffLen{151}
\def\EQKEErrMaxRowDiffMaxFloat{3.240688323974609375}
\def\EQKEErrMaxRowDiffMaxKey{8299}
\def\EQKEErrMaxRowDiffMeanFloat{1.5684236390701193908370214558090083301067352294921875}
\def\EQKEErrMaxRowDiffMeanKey{1283}
\def\EQKEErrMaxRowDiffMedianFloat{0.986862957477569580078125}
\def\EQKEErrMaxRowDiffMedianKey{14929}
\def\EQKEErrMaxRowDiffMinFloat{0.972379207611083984375}
\def\EQKEErrMaxRowDiffMinKey{18289}
\def\EQKEErrMaxRowDiffStdDevFloat{0.297939111957562563492984963886556215584278106689453125}
\def\EQKEErrMaxStdDevFloat{0.16746841371059417724609375}
\def\EQKEErrMeanDimZeroNormLen{151}
\def\EQKEErrMeanDimZeroNormMaxFloat{0.0486762113869190216064453125}
\def\EQKEErrMeanDimZeroNormMaxKey{20294}
\def\EQKEErrMeanDimZeroNormMeanFloat{0.0215833500206519847408603851590669364668428897857666015625}
\def\EQKEErrMeanDimZeroNormMeanKey{3284}
\def\EQKEErrMeanDimZeroNormMedianFloat{0.006765477475710213184356689453125}
\def\EQKEErrMeanDimZeroNormMedianKey{6082}
\def\EQKEErrMeanDimZeroNormMinFloat{0.005994598381221294403076171875}
\def\EQKEErrMeanDimZeroNormMinKey{2549}
\def\EQKEErrMeanDimZeroNormStdDevFloat{0.0086078126710742962346412099350345670245587825775146484375}
\def\EQKEErrMeanLen{151}
\def\EQKEErrMeanMaxFloat{0.0012601171620190143585205078125}
\def\EQKEErrMeanMaxKey{4157}
\def\EQKEErrMeanMeanFloat{0.000028468470191000960767269134521484375}
\def\EQKEErrMeanMeanKey{6532}
\def\EQKEErrMeanMedianFloat{-0.000759111091610975563526153564453125}
\def\EQKEErrMeanMedianKey{20338}
\def\EQKEErrMeanMinFloat{-0.0009170623379759490489959716796875}
\def\EQKEErrMeanMinKey{20013}
\def\EQKEErrMeanStdDevFloat{0.0002926471061073243618011474609375}
\def\EQKEErrMedianLen{151}
\def\EQKEErrMedianMaxFloat{-0.32634242102503774329846919499686919152736663818359375}
\def\EQKEErrMedianMaxKey{14929}
\def\EQKEErrMedianMeanFloat{-0.456898849783156923987093023242778144776821136474609375}
\def\EQKEErrMedianMeanKey{11124}
\def\EQKEErrMedianMedianFloat{-0.6299867220222949981689453125}
\def\EQKEErrMedianMedianKey{23633}
\def\EQKEErrMedianMinFloat{-0.646804630756378173828125}
\def\EQKEErrMedianMinKey{6159}
\def\EQKEErrMedianStdDevFloat{0.05779195452570300151062809845825540833175182342529296875}
\def\EQKEErrMinLen{151}
\def\EQKEErrMinMaxFloat{-0.529239714145660400390625}
\def\EQKEErrMinMaxKey{27300}
\def\EQKEErrMinMeanFloat{-0.8331415653228759765625}
\def\EQKEErrMinMeanKey{15662}
\def\EQKEErrMinMedianFloat{-1.3697610199451446533203125}
\def\EQKEErrMinMedianKey{11124}
\def\EQKEErrMinMinFloat{-1.46083104610443115234375}
\def\EQKEErrMinMinKey{8299}
\def\EQKEErrMinStdDevFloat{0.16684980690479278564453125}
\def\EQKEErrProdFirstSingularLen{151}
\def\EQKEErrProdFirstSingularMaxFloat{32.86769476839349835017856094054877758026123046875}
\def\EQKEErrProdFirstSingularMaxKey{742}
\def\EQKEErrProdFirstSingularMeanFloat{25.517768509257809483870005351491272449493408203125}
\def\EQKEErrProdFirstSingularMeanKey{29195}
\def\EQKEErrProdFirstSingularMedianFloat{20.884199896924958039789999020285904407501220703125}
\def\EQKEErrProdFirstSingularMedianKey{9132}
\def\EQKEErrProdFirstSingularMinFloat{20.73661735625258728532571694813668727874755859375}
\def\EQKEErrProdFirstSingularMinKey{19488}
\def\EQKEErrProdFirstSingularSqrtTwoLen{151}
\def\EQKEErrProdFirstSingularSqrtTwoMaxFloat{46.48193970540130948165824520401656627655029296875}
\def\EQKEErrProdFirstSingularSqrtTwoMaxKey{742}
\def\EQKEErrProdFirstSingularSqrtTwoMeanFloat{36.08757430728946502540566143579781055450439453125}
\def\EQKEErrProdFirstSingularSqrtTwoMeanKey{29195}
\def\EQKEErrProdFirstSingularSqrtTwoMedianFloat{29.53471873354207133388626971282064914703369140625}
\def\EQKEErrProdFirstSingularSqrtTwoMedianKey{9132}
\def\EQKEErrProdFirstSingularSqrtTwoMinFloat{29.32600550295372698883511475287377834320068359375}
\def\EQKEErrProdFirstSingularSqrtTwoMinKey{19488}
\def\EQKEErrProdFirstSingularSqrtTwoStdDevFloat{3.361571628422932445090509645524434745311737060546875}
\def\EQKEErrProdFirstSingularStdDevFloat{2.376990093902160428029901595436967909336090087890625}
\def\EQKEErrProdFroNormLen{151}
\def\EQKEErrProdFroNormMaxFloat{1518.61230702579041462740860879421234130859375}
\def\EQKEErrProdFroNormMaxKey{7310}
\def\EQKEErrProdFroNormMeanFloat{1368.115963972122017366928048431873321533203125}
\def\EQKEErrProdFroNormMeanKey{32374}
\def\EQKEErrProdFroNormMedianFloat{1213.7964073054872642387636005878448486328125}
\def\EQKEErrProdFroNormMedianKey{6532}
\def\EQKEErrProdFroNormMinFloat{1210.2936076854502971400506794452667236328125}
\def\EQKEErrProdFroNormMinKey{16069}
\def\EQKEErrProdFroNormSqrtTwoLen{151}
\def\EQKEErrProdFroNormSqrtTwoMaxFloat{2147.64212058256771342712454497814178466796875}
\def\EQKEErrProdFroNormSqrtTwoMaxKey{7310}
\def\EQKEErrProdFroNormSqrtTwoMeanFloat{1934.808151148516344619565643370151519775390625}
\def\EQKEErrProdFroNormSqrtTwoMeanKey{32374}
\def\EQKEErrProdFroNormSqrtTwoMedianFloat{1716.567341171157522694556973874568939208984375}
\def\EQKEErrProdFroNormSqrtTwoMedianKey{6532}
\def\EQKEErrProdFroNormSqrtTwoMinFloat{1711.613634442225929888081736862659454345703125}
\def\EQKEErrProdFroNormSqrtTwoMinKey{16069}
\def\EQKEErrProdFroNormSqrtTwoStdDevFloat{87.0263579653084349274649866856634616851806640625}
\def\EQKEErrProdFroNormStdDevFloat{61.5369278592375081871068687178194522857666015625}
\def\EQKEErrSimpleFirstSingularLen{151}
\def\EQKEErrSimpleFirstSingularMaxFloat{23.7548885345458984375}
\def\EQKEErrSimpleFirstSingularMaxKey{19917}
\def\EQKEErrSimpleFirstSingularMeanFloat{9.5989841530654604895289594423957169055938720703125}
\def\EQKEErrSimpleFirstSingularMeanKey{25516}
\def\EQKEErrSimpleFirstSingularMedianFloat{5.66811668872833251953125}
\def\EQKEErrSimpleFirstSingularMedianKey{22545}
\def\EQKEErrSimpleFirstSingularMinFloat{5.471868038177490234375}
\def\EQKEErrSimpleFirstSingularMinKey{15622}
\def\EQKEErrSimpleFirstSingularSqrtTwoLen{151}
\def\EQKEErrSimpleFirstSingularSqrtTwoMaxFloat{33.594486236572265625}
\def\EQKEErrSimpleFirstSingularSqrtTwoMaxKey{19917}
\def\EQKEErrSimpleFirstSingularSqrtTwoMeanFloat{13.5750133691244574407619438716210424900054931640625}
\def\EQKEErrSimpleFirstSingularSqrtTwoMeanKey{25516}
\def\EQKEErrSimpleFirstSingularSqrtTwoMedianFloat{8.0159270763397216796875}
\def\EQKEErrSimpleFirstSingularSqrtTwoMedianKey{22545}
\def\EQKEErrSimpleFirstSingularSqrtTwoMinFloat{7.7383899688720703125}
\def\EQKEErrSimpleFirstSingularSqrtTwoMinKey{15622}
\def\EQKEErrSimpleFirstSingularSqrtTwoStdDevFloat{3.608553754130089163965067200479097664356231689453125}
\def\EQKEErrSimpleFirstSingularStdDevFloat{2.551632859475447379082879706402309238910675048828125}
\def\EQKEErrSimpleFroNormLen{151}
\def\EQKEErrSimpleFroNormMaxFloat{25.280361175537109375}
\def\EQKEErrSimpleFroNormMaxKey{19917}
\def\EQKEErrSimpleFroNormMeanFloat{13.2143544013926526048408049973659217357635498046875}
\def\EQKEErrSimpleFroNormMeanKey{6549}
\def\EQKEErrSimpleFroNormMedianFloat{9.8413565158843994140625}
\def\EQKEErrSimpleFroNormMedianKey{5358}
\def\EQKEErrSimpleFroNormMinFloat{9.52376079559326171875}
\def\EQKEErrSimpleFroNormMinKey{15622}
\def\EQKEErrSimpleFroNormSqrtTwoLen{151}
\def\EQKEErrSimpleFroNormSqrtTwoMaxFloat{35.751827239990234375}
\def\EQKEErrSimpleFroNormSqrtTwoMaxKey{19917}
\def\EQKEErrSimpleFroNormSqrtTwoMeanFloat{18.687918865128068546255235560238361358642578125}
\def\EQKEErrSimpleFroNormSqrtTwoMeanKey{6549}
\def\EQKEErrSimpleFroNormSqrtTwoMedianFloat{13.917779445648193359375}
\def\EQKEErrSimpleFroNormSqrtTwoMedianKey{5358}
\def\EQKEErrSimpleFroNormSqrtTwoMinFloat{13.468631744384765625}
\def\EQKEErrSimpleFroNormSqrtTwoMinKey{15622}
\def\EQKEErrSimpleFroNormSqrtTwoStdDevFloat{2.94731708773177647486818386823870241641998291015625}
\def\EQKEErrSimpleFroNormStdDevFloat{2.08406796663087146015413964050821959972381591796875}
\def\EQKEErrSimpleLen{4096}
\def\EQKEErrSimpleMaxAbsLen{151}
\def\EQKEErrSimpleMaxAbsMaxFloat{3.7656028270721435546875}
\def\EQKEErrSimpleMaxAbsMaxKey{19917}
\def\EQKEErrSimpleMaxAbsMeanFloat{1.489641731937989543865796804311685264110565185546875}
\def\EQKEErrSimpleMaxAbsMeanKey{1283}
\def\EQKEErrSimpleMaxAbsMedianFloat{0.933683335781097412109375}
\def\EQKEErrSimpleMaxAbsMedianKey{19538}
\def\EQKEErrSimpleMaxAbsMinFloat{0.91521203517913818359375}
\def\EQKEErrSimpleMaxAbsMinKey{20415}
\def\EQKEErrSimpleMaxAbsStdDevFloat{0.355872264943901284173222165918559767305850982666015625}
\def\EQKEErrSimpleMaxLen{151}
\def\EQKEErrSimpleMaxMaxFloat{2.025590419769287109375}
\def\EQKEErrSimpleMaxMaxKey{30463}
\def\EQKEErrSimpleMaxMeanFloat{1.23733150959014892578125}
\def\EQKEErrSimpleMaxMeanKey{21598}
\def\EQKEErrSimpleMaxMedianFloat{0.78809629380702972412109375}
\def\EQKEErrSimpleMaxMedianKey{12552}
\def\EQKEErrSimpleMaxMinFloat{0.765118658542633056640625}
\def\EQKEErrSimpleMaxMinKey{26932}
\def\EQKEErrSimpleMaxRowDiffLen{151}
\def\EQKEErrSimpleMaxRowDiffMaxFloat{5.1106624603271484375}
\def\EQKEErrSimpleMaxRowDiffMaxKey{19917}
\def\EQKEErrSimpleMaxRowDiffMeanFloat{2.297073252943178101048715689103119075298309326171875}
\def\EQKEErrSimpleMaxRowDiffMeanKey{29110}
\def\EQKEErrSimpleMaxRowDiffMedianFloat{1.4803087711334228515625}
\def\EQKEErrSimpleMaxRowDiffMedianKey{14929}
\def\EQKEErrSimpleMaxRowDiffMinFloat{1.44828641414642333984375}
\def\EQKEErrSimpleMaxRowDiffMinKey{19538}
\def\EQKEErrSimpleMaxRowDiffStdDevFloat{0.512261280027975995920996865606866776943206787109375}
\def\EQKEErrSimpleMaxStdDevFloat{0.29541289806365966796875}
\def\EQKEErrSimpleMeanDimZeroNormLen{151}
\def\EQKEErrSimpleMeanDimZeroNormMaxFloat{0.3890773355960845947265625}
\def\EQKEErrSimpleMeanDimZeroNormMaxKey{19917}
\def\EQKEErrSimpleMeanDimZeroNormMeanFloat{0.049022107742825483944759668020196841098368167877197265625}
\def\EQKEErrSimpleMeanDimZeroNormMeanKey{19488}
\def\EQKEErrSimpleMeanDimZeroNormMedianFloat{0.009335805661976337432861328125}
\def\EQKEErrSimpleMeanDimZeroNormMedianKey{5358}
\def\EQKEErrSimpleMeanDimZeroNormMinFloat{0.008067115209996700286865234375}
\def\EQKEErrSimpleMeanDimZeroNormMinKey{21598}
\def\EQKEErrSimpleMeanDimZeroNormStdDevFloat{0.038403768624441329826435520544691826216876506805419921875}
\def\EQKEErrSimpleMeanLen{151}
\def\EQKEErrSimpleMeanMaxFloat{0.008168168365955352783203125}
\def\EQKEErrSimpleMeanMaxKey{22401}
\def\EQKEErrSimpleMeanMeanFloat{-0.00020042792311869561672210693359375}
\def\EQKEErrSimpleMeanMeanKey{7310}
\def\EQKEErrSimpleMeanMedianFloat{-0.013560487888753414154052734375}
\def\EQKEErrSimpleMeanMedianKey{1681}
\def\EQKEErrSimpleMeanMinFloat{-0.0236646234989166259765625}
\def\EQKEErrSimpleMeanMinKey{19917}
\def\EQKEErrSimpleMeanStdDevFloat{0.0032648146152496337890625}
\def\EQKEErrSimpleMedianLen{151}
\def\EQKEErrSimpleMedianMaxFloat{-0.40928204581141469642346919499686919152736663818359375}
\def\EQKEErrSimpleMedianMaxKey{14929}
\def\EQKEErrSimpleMedianMeanFloat{-0.72675228960664062238805627202964387834072113037109375}
\def\EQKEErrSimpleMedianMeanKey{23241}
\def\EQKEErrSimpleMedianMedianFloat{-1.7430720262229442152346337024937383830547332763671875}
\def\EQKEErrSimpleMedianMedianKey{1681}
\def\EQKEErrSimpleMedianMinFloat{-1.9225207298994064775143897350062616169452667236328125}
\def\EQKEErrSimpleMedianMinKey{19917}
\def\EQKEErrSimpleMedianStdDevFloat{0.2083085076028131366054907402940443716943264007568359375}
\def\EQKEErrSimpleMinLen{151}
\def\EQKEErrSimpleMinMaxFloat{-0.665629446506500244140625}
\def\EQKEErrSimpleMinMaxKey{14929}
\def\EQKEErrSimpleMinMeanFloat{-1.31499016284942626953125}
\def\EQKEErrSimpleMinMeanKey{6155}
\def\EQKEErrSimpleMinMedianFloat{-2.9003143310546875}
\def\EQKEErrSimpleMinMedianKey{1681}
\def\EQKEErrSimpleMinMinFloat{-3.7656028270721435546875}
\def\EQKEErrSimpleMinMinKey{19917}
\def\EQKEErrSimpleMinStdDevFloat{0.416278302669525146484375}
\def\EQKEErrSimpleStdDevLen{151}
\def\EQKEErrSimpleStdDevMaxFloat{0.3942961394786834716796875}
\def\EQKEErrSimpleStdDevMaxKey{19917}
\def\EQKEErrSimpleStdDevMeanFloat{0.20645381510257720947265625}
\def\EQKEErrSimpleStdDevMeanKey{6549}
\def\EQKEErrSimpleStdDevMedianFloat{0.1537708081305027008056640625}
\def\EQKEErrSimpleStdDevMedianKey{5358}
\def\EQKEErrSimpleStdDevMinFloat{0.14880730211734771728515625}
\def\EQKEErrSimpleStdDevMinKey{15622}
\def\EQKEErrSimpleStdDevStdDevFloat{0.0325289778411388397216796875}
\def\EQKEErrSimpleWithAttnScaleFirstSingularLen{151}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMaxFloat{4.199310779571533203125}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMaxKey{19917}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMeanFloat{1.696876720876883126720713335089385509490966796875}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMeanKey{25516}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMedianFloat{1.0019908845424652099609375}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMedianKey{22545}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMinFloat{0.9672987461090087890625}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMinKey{15622}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoLen{151}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMaxFloat{5.938722133636474609375}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMaxKey{19917}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMeanFloat{2.399746025634917234725662638084031641483306884765625}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMeanKey{25516}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMedianFloat{1.417029082775115966796875}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMedianKey{22545}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMinFloat{1.36796700954437255859375}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMinKey{15622}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoStdDevFloat{0.6379082306544086033994744866504333913326263427734375}
\def\EQKEErrSimpleWithAttnScaleFirstSingularStdDevFloat{0.451069243835855615554208952744374983012676239013671875}
\def\EQKEErrSimpleWithAttnScaleFroNormLen{151}
\def\EQKEErrSimpleWithAttnScaleFroNormMaxFloat{4.4689788818359375}
\def\EQKEErrSimpleWithAttnScaleFroNormMaxKey{19917}
\def\EQKEErrSimpleWithAttnScaleFroNormMeanFloat{2.335989948929540371835855694371275603771209716796875}
\def\EQKEErrSimpleWithAttnScaleFroNormMeanKey{6549}
\def\EQKEErrSimpleWithAttnScaleFroNormMedianFloat{1.7397225797176361083984375}
\def\EQKEErrSimpleWithAttnScaleFroNormMedianKey{5358}
\def\EQKEErrSimpleWithAttnScaleFroNormMinFloat{1.68357884883880615234375}
\def\EQKEErrSimpleWithAttnScaleFroNormMinKey{15622}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoLen{151}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMaxFloat{6.32009029388427734375}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMaxKey{19917}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMeanFloat{3.3035886161374730107809227774851024150848388671875}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMeanKey{6549}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMedianFloat{2.460339248180389404296875}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMedianKey{5358}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMinFloat{2.380939960479736328125}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMinKey{15622}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoStdDevFloat{0.52101700221837699000815291583421640098094940185546875}
\def\EQKEErrSimpleWithAttnScaleFroNormStdDevFloat{0.368414663966862010457958831466385163366794586181640625}
\def\EQKEErrSimpleWithAttnScaleLen{4096}
\def\EQKEErrSimpleWithAttnScaleMaxAbsLen{151}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMaxFloat{0.665670812129974365234375}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMaxKey{19917}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMeanFloat{0.263333946959861842085359739940031431615352630615234375}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMeanKey{1283}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMedianFloat{0.1650534532964229583740234375}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMedianKey{19538}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMinFloat{0.161788165569305419921875}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMinKey{20415}
\def\EQKEErrSimpleWithAttnScaleMaxAbsStdDevFloat{0.06290992315934486323047991618295782245695590972900390625}
\def\EQKEErrSimpleWithAttnScaleMaxLen{151}
\def\EQKEErrSimpleWithAttnScaleMaxMaxFloat{0.3580771982669830322265625}
\def\EQKEErrSimpleWithAttnScaleMaxMaxKey{30463}
\def\EQKEErrSimpleWithAttnScaleMaxMeanFloat{0.218731403350830078125}
\def\EQKEErrSimpleWithAttnScaleMaxMeanKey{21598}
\def\EQKEErrSimpleWithAttnScaleMaxMedianFloat{0.139317058026790618896484375}
\def\EQKEErrSimpleWithAttnScaleMaxMedianKey{12552}
\def\EQKEErrSimpleWithAttnScaleMaxMinFloat{0.13525514304637908935546875}
\def\EQKEErrSimpleWithAttnScaleMaxMinKey{26932}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffLen{151}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMaxFloat{0.903446018695831298828125}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMaxKey{19917}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMeanFloat{0.40606902529861754747031454826355911791324615478515625}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMeanKey{29110}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMedianFloat{0.2616840898990631103515625}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMedianKey{14929}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMinFloat{0.25602328777313232421875}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMinKey{19538}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffStdDevFloat{0.0905558569775993527084523293524398468434810638427734375}
\def\EQKEErrSimpleWithAttnScaleMaxStdDevFloat{0.05222211778163909912109375}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormLen{151}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMaxFloat{0.068779803812503814697265625}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMaxKey{19917}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMeanFloat{0.008665966278632843133866714424584642983973026275634765625}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMeanKey{19488}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMedianFloat{0.0016503530205227434635162353515625}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMedianKey{5358}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMinFloat{0.001426077564246952533721923828125}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMinKey{21598}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormStdDevFloat{0.006788891341171782688179714426723876385949552059173583984375}
\def\EQKEErrSimpleWithAttnScaleMeanLen{151}
\def\EQKEErrSimpleWithAttnScaleMeanMaxFloat{0.0014439411461353302001953125}
\def\EQKEErrSimpleWithAttnScaleMeanMaxKey{22401}
\def\EQKEErrSimpleWithAttnScaleMeanMeanFloat{-0.00003543100319802761077880859375}
\def\EQKEErrSimpleWithAttnScaleMeanMeanKey{7310}
\def\EQKEErrSimpleWithAttnScaleMeanMedianFloat{-0.00239717774093151092529296875}
\def\EQKEErrSimpleWithAttnScaleMeanMedianKey{1681}
\def\EQKEErrSimpleWithAttnScaleMeanMinFloat{-0.004183352924883365631103515625}
\def\EQKEErrSimpleWithAttnScaleMeanMinKey{19917}
\def\EQKEErrSimpleWithAttnScaleMeanStdDevFloat{0.00057714316062629222869873046875}
\def\EQKEErrSimpleWithAttnScaleMedianLen{151}
\def\EQKEErrSimpleWithAttnScaleMedianMaxFloat{-0.07235152572393417635954193656289135105907917022705078125}
\def\EQKEErrSimpleWithAttnScaleMedianMaxKey{14929}
\def\EQKEErrSimpleWithAttnScaleMedianMeanFloat{-0.1284728700837848014426612053284770809113979339599609375}
\def\EQKEErrSimpleWithAttnScaleMedianMeanKey{23241}
\def\EQKEErrSimpleWithAttnScaleMedianMedianFloat{-0.30813451986759898826306880437186919152736663818359375}
\def\EQKEErrSimpleWithAttnScaleMedianMedianKey{1681}
\def\EQKEErrSimpleWithAttnScaleMedianMinFloat{-0.33985685780644414588635981999686919152736663818359375}
\def\EQKEErrSimpleWithAttnScaleMedianMinKey{19917}
\def\EQKEErrSimpleWithAttnScaleMedianStdDevFloat{0.036824090118112128011684802686431794427335262298583984375}
\def\EQKEErrSimpleWithAttnScaleMinLen{151}
\def\EQKEErrSimpleWithAttnScaleMinMaxFloat{-0.11766777932643890380859375}
\def\EQKEErrSimpleWithAttnScaleMinMaxKey{14929}
\def\EQKEErrSimpleWithAttnScaleMinMeanFloat{-0.23245961964130401611328125}
\def\EQKEErrSimpleWithAttnScaleMinMeanKey{6155}
\def\EQKEErrSimpleWithAttnScaleMinMedianFloat{-0.512707985937595367431640625}
\def\EQKEErrSimpleWithAttnScaleMinMedianKey{1681}
\def\EQKEErrSimpleWithAttnScaleMinMinFloat{-0.665670812129974365234375}
\def\EQKEErrSimpleWithAttnScaleMinMinKey{19917}
\def\EQKEErrSimpleWithAttnScaleMinStdDevFloat{0.073588304221630096435546875}
\def\EQKEErrSimpleWithAttnScaleStdDevLen{151}
\def\EQKEErrSimpleWithAttnScaleStdDevMaxFloat{0.069702364504337310791015625}
\def\EQKEErrSimpleWithAttnScaleStdDevMaxKey{19917}
\def\EQKEErrSimpleWithAttnScaleStdDevMeanFloat{0.0364962257444858551025390625}
\def\EQKEErrSimpleWithAttnScaleStdDevMeanKey{6549}
\def\EQKEErrSimpleWithAttnScaleStdDevMedianFloat{0.0271830954588949680328369140625}
\def\EQKEErrSimpleWithAttnScaleStdDevMedianKey{5358}
\def\EQKEErrSimpleWithAttnScaleStdDevMinFloat{0.02630566246807575225830078125}
\def\EQKEErrSimpleWithAttnScaleStdDevMinKey{15622}
\def\EQKEErrSimpleWithAttnScaleStdDevStdDevFloat{0.005750364623963832855224609375}
\def\EQKEErrStdDevLen{151}
\def\EQKEErrStdDevMaxFloat{0.172048509120941162109375}
\def\EQKEErrStdDevMaxKey{6159}
\def\EQKEErrStdDevMeanFloat{0.13587756454944610595703125}
\def\EQKEErrStdDevMeanKey{5781}
\def\EQKEErrStdDevMedianFloat{0.10805855877697467803955078125}
\def\EQKEErrStdDevMedianKey{18289}
\def\EQKEErrStdDevMinFloat{0.102101556956768035888671875}
\def\EQKEErrStdDevMinKey{14929}
\def\EQKEErrStdDevStdDevFloat{0.01284774951636791229248046875}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactLen{151}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMaxFloat{0.57287824153900146484375}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMaxKey{8299}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMeanFloat{0.277260753887378641469041440359433181583881378173828125}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMeanKey{1283}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMedianFloat{0.17445437610149383544921875}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMedianKey{14929}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMinFloat{0.17189393937587738037109375}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMinKey{18289}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactStdDevFloat{0.0526686978444150799560929954168386757373809814453125}
\def\EQKEErrWithAttnScaleBoundMaxDiffLen{151}
\def\EQKEErrWithAttnScaleBoundMaxDiffMaxFloat{1.04617345333099365234375}
\def\EQKEErrWithAttnScaleBoundMaxDiffMaxKey{24438}
\def\EQKEErrWithAttnScaleBoundMaxDiffMeanFloat{0.82071491345664526750880440886248834431171417236328125}
\def\EQKEErrWithAttnScaleBoundMaxDiffMeanKey{13716}
\def\EQKEErrWithAttnScaleBoundMaxDiffMedianFloat{0.6631657779216766357421875}
\def\EQKEErrWithAttnScaleBoundMaxDiffMedianKey{27300}
\def\EQKEErrWithAttnScaleBoundMaxDiffMinFloat{0.66219329833984375}
\def\EQKEErrWithAttnScaleBoundMaxDiffMinKey{18289}
\def\EQKEErrWithAttnScaleBoundMaxDiffStdDevFloat{0.077788121937353238433132673890213482081890106201171875}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductLen{151}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMaxFloat{1.04617345333099365234375}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMaxKey{24438}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMeanFloat{0.82071491345664526750880440886248834431171417236328125}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMeanKey{13716}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMedianFloat{0.6631657779216766357421875}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMedianKey{27300}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMinFloat{0.66219329833984375}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMinKey{18289}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMaxFloat{27.512847900390625}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMaxKey{4810}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMeanFloat{16.16264534628154336814986891113221645355224609375}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMeanKey{4729}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMedianFloat{13.9488251209259033203125}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMedianKey{29022}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMinFloat{13.92051601409912109375}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMinKey{7238}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveStdDevFloat{1.34233638541398736521159662515856325626373291015625}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductStdDevFloat{0.077788121937353238433132673890213482081890106201171875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffLen{151}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMaxFloat{1.039141178131103515625}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMaxKey{24438}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMeanFloat{0.8222855657141729945891484021558426320552825927734375}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMeanKey{17080}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMedianFloat{0.67028020322322845458984375}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMedianKey{18289}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMinFloat{0.66231596469879150390625}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMinKey{27300}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffStdDevFloat{0.07800171714907293274432475982393953017890453338623046875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductLen{151}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMaxFloat{1.039141178131103515625}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMaxKey{24438}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMeanFloat{0.8222855657141729945891484021558426320552825927734375}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMeanKey{17080}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMedianFloat{0.67028020322322845458984375}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMedianKey{18289}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMinFloat{0.66231596469879150390625}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMinKey{27300}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMaxFloat{27.650691986083984375}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMaxKey{4810}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMeanFloat{16.13383478834139594937369110994040966033935546875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMeanKey{15622}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMedianFloat{14.028628826141357421875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMedianKey{29022}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMinFloat{13.8969173431396484375}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMinKey{7238}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveStdDevFloat{1.3431443131834868154328432865440845489501953125}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductStdDevFloat{0.07800171714907293274432475982393953017890453338623046875}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMaxFloat{27.63072967529296875}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMaxKey{4810}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMeanFloat{16.42016602194072305564986891113221645355224609375}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMeanKey{19004}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMedianFloat{14.368244171142578125}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMedianKey{29022}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMinFloat{14.2087535858154296875}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMinKey{7238}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveStdDevFloat{1.3495076369472822630513064723345451056957244873046875}
\def\EQKEErrWithAttnScaleBoundSvdLen{151}
\def\EQKEErrWithAttnScaleBoundSvdMaxFloat{1.89764630794525146484375}
\def\EQKEErrWithAttnScaleBoundSvdMaxKey{8299}
\def\EQKEErrWithAttnScaleBoundSvdMeanFloat{1.3463670232438094132021433324553072452545166015625}
\def\EQKEErrWithAttnScaleBoundSvdMeanKey{12141}
\def\EQKEErrWithAttnScaleBoundSvdMedianFloat{0.951499044895172119140625}
\def\EQKEErrWithAttnScaleBoundSvdMedianKey{18289}
\def\EQKEErrWithAttnScaleBoundSvdMinFloat{0.94122350215911865234375}
\def\EQKEErrWithAttnScaleBoundSvdMinKey{29726}
\def\EQKEErrWithAttnScaleBoundSvdStdDevFloat{0.2054349694000939530180716019458486698567867279052734375}
\def\EQKEErrWithAttnScaleFirstSingularLen{151}
\def\EQKEErrWithAttnScaleFirstSingularMaxFloat{1.34183871746063232421875}
\def\EQKEErrWithAttnScaleFirstSingularMaxKey{8299}
\def\EQKEErrWithAttnScaleFirstSingularMeanFloat{0.95202529154076476203272250131703913211822509765625}
\def\EQKEErrWithAttnScaleFirstSingularMeanKey{12141}
\def\EQKEErrWithAttnScaleFirstSingularMedianFloat{0.67281137406826019287109375}
\def\EQKEErrWithAttnScaleFirstSingularMedianKey{18289}
\def\EQKEErrWithAttnScaleFirstSingularMinFloat{0.665545403957366943359375}
\def\EQKEErrWithAttnScaleFirstSingularMinKey{29726}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoLen{151}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMaxFloat{1.897646427154541015625}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMaxKey{8299}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMeanFloat{1.346367057980291104257730694371275603771209716796875}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMeanKey{12141}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMedianFloat{0.9514989554882049560546875}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMedianKey{18289}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMinFloat{0.941223323345184326171875}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMinKey{29726}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoStdDevFloat{0.2054350807031087022824777932328288443386554718017578125}
\def\EQKEErrWithAttnScaleFirstSingularStdDevFloat{0.145264541312669248629418916607392020523548126220703125}
\def\EQKEErrWithAttnScaleFroNormLen{151}
\def\EQKEErrWithAttnScaleFroNormMaxFloat{1.9465091228485107421875}
\def\EQKEErrWithAttnScaleFroNormMaxKey{6159}
\def\EQKEErrWithAttnScaleFroNormMeanFloat{1.5372829674095507268560822922154329717159271240234375}
\def\EQKEErrWithAttnScaleFroNormMeanKey{5781}
\def\EQKEErrWithAttnScaleFroNormMedianFloat{1.222553670406341552734375}
\def\EQKEErrWithAttnScaleFroNormMedianKey{18289}
\def\EQKEErrWithAttnScaleFroNormMinFloat{1.15514814853668212890625}
\def\EQKEErrWithAttnScaleFroNormMinKey{14929}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoLen{151}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMaxFloat{2.752779483795166015625}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMaxKey{6159}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMeanFloat{2.174046374314668295113506246707402169704437255859375}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMeanKey{5781}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMedianFloat{1.7289519011974334716796875}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMedianKey{18289}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMinFloat{1.63362610340118408203125}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMinKey{14929}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoStdDevFloat{0.2055642644461633528063515541361994110047817230224609375}
\def\EQKEErrWithAttnScaleFroNormStdDevFloat{0.1453558888602594911798604471186990849673748016357421875}
\def\EQKEErrWithAttnScaleLen{4096}
\def\EQKEErrWithAttnScaleMaxAbsLen{151}
\def\EQKEErrWithAttnScaleMaxAbsMaxFloat{0.31463730335235595703125}
\def\EQKEErrWithAttnScaleMaxAbsMaxKey{8299}
\def\EQKEErrWithAttnScaleMaxAbsMeanFloat{0.1568539610366947723019137583833071403205394744873046875}
\def\EQKEErrWithAttnScaleMaxAbsMeanKey{3284}
\def\EQKEErrWithAttnScaleMaxAbsMedianFloat{0.10280898772180080413818359375}
\def\EQKEErrWithAttnScaleMaxAbsMedianKey{14929}
\def\EQKEErrWithAttnScaleMaxAbsMinFloat{0.098042897880077362060546875}
\def\EQKEErrWithAttnScaleMaxAbsMinKey{18289}
\def\EQKEErrWithAttnScaleMaxAbsStdDevFloat{0.0305489770137687514928170884331848355941474437713623046875}
\def\EQKEErrWithAttnScaleMaxLen{151}
\def\EQKEErrWithAttnScaleMaxMaxFloat{0.31463730335235595703125}
\def\EQKEErrWithAttnScaleMaxMaxKey{8299}
\def\EQKEErrWithAttnScaleMaxMeanFloat{0.14620576798915863037109375}
\def\EQKEErrWithAttnScaleMaxMeanKey{24262}
\def\EQKEErrWithAttnScaleMaxMedianFloat{0.08933238685131072998046875}
\def\EQKEErrWithAttnScaleMaxMedianKey{13654}
\def\EQKEErrWithAttnScaleMaxMinFloat{0.086971618235111236572265625}
\def\EQKEErrWithAttnScaleMaxMinKey{18289}
\def\EQKEErrWithAttnScaleMaxRowDiffLen{151}
\def\EQKEErrWithAttnScaleMaxRowDiffMaxFloat{0.572878181934356689453125}
\def\EQKEErrWithAttnScaleMaxRowDiffMaxKey{8299}
\def\EQKEErrWithAttnScaleMaxRowDiffMeanFloat{0.277260751913714909022701249341480433940887451171875}
\def\EQKEErrWithAttnScaleMaxRowDiffMeanKey{1283}
\def\EQKEErrWithAttnScaleMaxRowDiffMedianFloat{0.17445437610149383544921875}
\def\EQKEErrWithAttnScaleMaxRowDiffMedianKey{14929}
\def\EQKEErrWithAttnScaleMaxRowDiffMinFloat{0.1718939840793609619140625}
\def\EQKEErrWithAttnScaleMaxRowDiffMinKey{18289}
\def\EQKEErrWithAttnScaleMaxRowDiffStdDevFloat{0.052668692881789651305535215897180023603141307830810546875}
\def\EQKEErrWithAttnScaleMaxStdDevFloat{0.0296045131981372833251953125}
\def\EQKEErrWithAttnScaleMeanDimZeroNormLen{151}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMaxFloat{0.00860481895506381988525390625}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMaxKey{20294}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMeanFloat{0.0038154333496824006759229330754124021041207015514373779296875}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMeanKey{3284}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMedianFloat{0.0011959786643274128437042236328125}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMedianKey{6082}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMinFloat{0.00105970515869557857513427734375}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMinKey{2549}
\def\EQKEErrWithAttnScaleMeanDimZeroNormStdDevFloat{0.00152166075440297540212475357890298255369998514652252197265625}
\def\EQKEErrWithAttnScaleMeanLen{151}
\def\EQKEErrWithAttnScaleMeanMaxFloat{0.0002227593795396387577056884765625}
\def\EQKEErrWithAttnScaleMeanMaxKey{4157}
\def\EQKEErrWithAttnScaleMeanMeanFloat{0.00000503256205774960108101367950439453125}
\def\EQKEErrWithAttnScaleMeanMeanKey{6532}
\def\EQKEErrWithAttnScaleMeanMedianFloat{-0.0001341931274509988725185394287109375}
\def\EQKEErrWithAttnScaleMeanMedianKey{20338}
\def\EQKEErrWithAttnScaleMeanMinFloat{-0.000162115276907570660114288330078125}
\def\EQKEErrWithAttnScaleMeanMinKey{20013}
\def\EQKEErrWithAttnScaleMeanStdDevFloat{0.00005173319004825316369533538818359375}
\def\EQKEErrWithAttnScaleMedianLen{151}
\def\EQKEErrWithAttnScaleMedianMaxFloat{-0.057689735759049655394736788593945675529539585113525390625}
\def\EQKEErrWithAttnScaleMedianMaxKey{14929}
\def\EQKEErrWithAttnScaleMedianMeanFloat{-0.0807690703118873754018380850538960658013820648193359375}
\def\EQKEErrWithAttnScaleMedianMeanKey{11124}
\def\EQKEErrWithAttnScaleMedianMedianFloat{-0.11136697190813719948732085640585864894092082977294921875}
\def\EQKEErrWithAttnScaleMedianMedianKey{23633}
\def\EQKEErrWithAttnScaleMedianMinFloat{-0.1143399864435195867340411268742172978818416595458984375}
\def\EQKEErrWithAttnScaleMedianMinKey{6159}
\def\EQKEErrWithAttnScaleMedianStdDevFloat{0.01021627073960418123632631903774381498806178569793701171875}
\def\EQKEErrWithAttnScaleMinLen{151}
\def\EQKEErrWithAttnScaleMinMaxFloat{-0.093557246029376983642578125}
\def\EQKEErrWithAttnScaleMinMaxKey{27300}
\def\EQKEErrWithAttnScaleMinMeanFloat{-0.14728002250194549560546875}
\def\EQKEErrWithAttnScaleMinMeanKey{15662}
\def\EQKEErrWithAttnScaleMinMedianFloat{-0.2421418242156505584716796875}
\def\EQKEErrWithAttnScaleMinMedianKey{11124}
\def\EQKEErrWithAttnScaleMinMinFloat{-0.258240878582000732421875}
\def\EQKEErrWithAttnScaleMinMinKey{8299}
\def\EQKEErrWithAttnScaleMinStdDevFloat{0.029495157301425933837890625}
\def\EQKEErrWithAttnScaleStdDevLen{151}
\def\EQKEErrWithAttnScaleStdDevMaxFloat{0.0304141677916049957275390625}
\def\EQKEErrWithAttnScaleStdDevMaxKey{6159}
\def\EQKEErrWithAttnScaleStdDevMeanFloat{0.0240199901163578033447265625}
\def\EQKEErrWithAttnScaleStdDevMeanKey{5781}
\def\EQKEErrWithAttnScaleStdDevMedianFloat{0.0191022357903420925140380859375}
\def\EQKEErrWithAttnScaleStdDevMedianKey{18289}
\def\EQKEErrWithAttnScaleStdDevMinFloat{0.0180491767823696136474609375}
\def\EQKEErrWithAttnScaleStdDevMinKey{14929}
\def\EQKEErrWithAttnScaleStdDevStdDevFloat{0.002271182835102081298828125}
\def\EQKEFirstSingularLen{151}
\def\EQKEFirstSingularMaxFloat{10488.7802734375}
\def\EQKEFirstSingularMaxKey{1681}
\def\EQKEFirstSingularMeanFloat{8855.322744205297567532397806644439697265625}
\def\EQKEFirstSingularMeanKey{4157}
\def\EQKEFirstSingularMedianFloat{7335.0709228515625}
\def\EQKEFirstSingularMedianKey{30684}
\def\EQKEFirstSingularMinFloat{7290.59130859375}
\def\EQKEFirstSingularMinKey{3284}
\def\EQKEFirstSingularSqrtTwoLen{151}
\def\EQKEFirstSingularSqrtTwoMaxFloat{14833.37531544669400318525731563568115234375}
\def\EQKEFirstSingularSqrtTwoMaxKey{1681}
\def\EQKEFirstSingularSqrtTwoMeanFloat{12523.31752404606595518998801708221435546875}
\def\EQKEFirstSingularSqrtTwoMeanKey{4157}
\def\EQKEFirstSingularSqrtTwoMedianFloat{10373.356780065214479691348969936370849609375}
\def\EQKEFirstSingularSqrtTwoMedianKey{30684}
\def\EQKEFirstSingularSqrtTwoMinFloat{10310.453106332692186697386205196380615234375}
\def\EQKEFirstSingularSqrtTwoMinKey{3284}
\def\EQKEFirstSingularSqrtTwoStdDevFloat{927.4499237294943441156647168099880218505859375}
\def\EQKEFirstSingularStdDevFloat{655.8061302800716703131911344826221466064453125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMaxFloat{-5991416716160870400}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMaxKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMeanFloat{-5991416716160868352}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMeanKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMedianFloat{-5991416716160870400}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMedianKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMinFloat{-5991416716160870400}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMinKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenStdDevFloat{2048}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMaxFloat{64.22934722900390625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMaxKey{4810}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMeanFloat{10.27843379974365234375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMeanKey{12457}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMedianFloat{6.17380130290985107421875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMedianKey{26829}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMinFloat{5.912799835205078125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMinKey{11124}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxStdDevFloat{5.739755153656005859375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMaxFloat{2.50152351674751916021932629519142210483551025390625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMaxKey{4810}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMeanFloat{1.9685811655114304752345333326957188546657562255859375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMeanKey{11498}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMedianFloat{1.7398775221740780949630789109505712985992431640625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMedianKey{12287}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMinFloat{1.7278012677588776568882167339324951171875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMinKey{3284}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanStdDevFloat{0.1075356098384828429370685398680507205426692962646484375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMaxFloat{3.715731143951416015625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMaxKey{8299}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMeanFloat{1.328772723726111326669752088491804897785186767578125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMeanKey{20338}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMedianFloat{-0.288834981620311737060546875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMedianKey{27584}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMinFloat{-2.2676165103912353515625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMinKey{4810}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianStdDevFloat{0.76365752882936333012509066975326277315616607666015625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMaxFloat{-2.0331747531890869140625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMaxKey{8721}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMeanFloat{-7.1209888458251953125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMeanKey{29052}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMedianFloat{-44.41776180267333984375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMedianKey{5781}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMinFloat{-62.16867828369140625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMinKey{4810}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinStdDevFloat{5.834512233734130859375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMaxFloat{2.2431915615060038504680051119066774845123291015625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMaxKey{4810}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMeanFloat{1.2616857463633925906520971693680621683597564697265625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMeanKey{8840}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMedianFloat{1.0059118096666554986740038657444529235363006591796875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMedianKey{11124}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMinFloat{1.0015202592597292063913982929079793393611907958984375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMinKey{12287}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevStdDevFloat{0.1309772738829743932154059393724310211837291717529296875}
\def\EQKEHistAttentionDifferenceOverGapLenLen{151}
\def\EQKEHistAttentionDifferenceOverGapLenMaxFloat{258048}
\def\EQKEHistAttentionDifferenceOverGapLenMaxKey{50}
\def\EQKEHistAttentionDifferenceOverGapLenMeanFloat{258048}
\def\EQKEHistAttentionDifferenceOverGapLenMeanKey{50}
\def\EQKEHistAttentionDifferenceOverGapLenMedianFloat{258048}
\def\EQKEHistAttentionDifferenceOverGapLenMedianKey{50}
\def\EQKEHistAttentionDifferenceOverGapLenMinFloat{258048}
\def\EQKEHistAttentionDifferenceOverGapLenMinKey{50}
\def\EQKEHistAttentionDifferenceOverGapLenStdDevFloat{0}
\def\EQKEHistAttentionDifferenceOverGapMaxLen{151}
\def\EQKEHistAttentionDifferenceOverGapMaxMaxFloat{64.22934722900390625}
\def\EQKEHistAttentionDifferenceOverGapMaxMaxKey{4810}
\def\EQKEHistAttentionDifferenceOverGapMaxMeanFloat{10.27843379974365234375}
\def\EQKEHistAttentionDifferenceOverGapMaxMeanKey{12457}
\def\EQKEHistAttentionDifferenceOverGapMaxMedianFloat{6.17380130290985107421875}
\def\EQKEHistAttentionDifferenceOverGapMaxMedianKey{26829}
\def\EQKEHistAttentionDifferenceOverGapMaxMinFloat{5.912799835205078125}
\def\EQKEHistAttentionDifferenceOverGapMaxMinKey{11124}
\def\EQKEHistAttentionDifferenceOverGapMaxStdDevFloat{5.739755153656005859375}
\def\EQKEHistAttentionDifferenceOverGapMeanLen{151}
\def\EQKEHistAttentionDifferenceOverGapMeanMaxFloat{1.298802852630615234375}
\def\EQKEHistAttentionDifferenceOverGapMeanMaxKey{4810}
\def\EQKEHistAttentionDifferenceOverGapMeanMeanFloat{1.08498537540435791015625}
\def\EQKEHistAttentionDifferenceOverGapMeanMeanKey{30899}
\def\EQKEHistAttentionDifferenceOverGapMeanMedianFloat{0.97350703179836273193359375}
\def\EQKEHistAttentionDifferenceOverGapMeanMedianKey{30684}
\def\EQKEHistAttentionDifferenceOverGapMeanMinFloat{0.972909390926361083984375}
\def\EQKEHistAttentionDifferenceOverGapMeanMinKey{3284}
\def\EQKEHistAttentionDifferenceOverGapMeanStdDevFloat{0.0539906919002532958984375}
\def\EQKEHistAttentionDifferenceOverGapMedianLen{151}
\def\EQKEHistAttentionDifferenceOverGapMedianMaxFloat{1.171818244548244347669196940842084586620330810546875}
\def\EQKEHistAttentionDifferenceOverGapMedianMaxKey{13036}
\def\EQKEHistAttentionDifferenceOverGapMedianMeanFloat{1.0261415515514398233420934047899208962917327880859375}
\def\EQKEHistAttentionDifferenceOverGapMedianMeanKey{1895}
\def\EQKEHistAttentionDifferenceOverGapMedianMedianFloat{0.89087165766999920624158448845264501869678497314453125}
\def\EQKEHistAttentionDifferenceOverGapMedianMedianKey{3175}
\def\EQKEHistAttentionDifferenceOverGapMedianMinFloat{0.88624087772296589182730031097889877855777740478515625}
\def\EQKEHistAttentionDifferenceOverGapMedianMinKey{19538}
\def\EQKEHistAttentionDifferenceOverGapMedianStdDevFloat{0.0551112218595460057191104397134040482342243194580078125}
\def\EQKEHistAttentionDifferenceOverGapMinLen{151}
\def\EQKEHistAttentionDifferenceOverGapMinMaxFloat{-2.0331747531890869140625}
\def\EQKEHistAttentionDifferenceOverGapMinMaxKey{8721}
\def\EQKEHistAttentionDifferenceOverGapMinMeanFloat{-7.1209888458251953125}
\def\EQKEHistAttentionDifferenceOverGapMinMeanKey{29052}
\def\EQKEHistAttentionDifferenceOverGapMinMedianFloat{-44.41776180267333984375}
\def\EQKEHistAttentionDifferenceOverGapMinMedianKey{5781}
\def\EQKEHistAttentionDifferenceOverGapMinMinFloat{-62.16867828369140625}
\def\EQKEHistAttentionDifferenceOverGapMinMinKey{4810}
\def\EQKEHistAttentionDifferenceOverGapMinStdDevFloat{5.834512233734130859375}
\def\EQKEHistAttentionDifferenceOverGapStdDevLen{151}
\def\EQKEHistAttentionDifferenceOverGapStdDevMaxFloat{2.285614013671875}
\def\EQKEHistAttentionDifferenceOverGapStdDevMaxKey{4810}
\def\EQKEHistAttentionDifferenceOverGapStdDevMeanFloat{1.01473462581634521484375}
\def\EQKEHistAttentionDifferenceOverGapStdDevMeanKey{27300}
\def\EQKEHistAttentionDifferenceOverGapStdDevMedianFloat{0.85120414197444915771484375}
\def\EQKEHistAttentionDifferenceOverGapStdDevMedianKey{32382}
\def\EQKEHistAttentionDifferenceOverGapStdDevMinFloat{0.8496496677398681640625}
\def\EQKEHistAttentionDifferenceOverGapStdDevMinKey{11124}
\def\EQKEHistAttentionDifferenceOverGapStdDevStdDevFloat{0.13885580003261566162109375}
\def\EQKEQueryDirectionLen{64}
\def\EQKEQueryDirectionMaxLen{151}
\def\EQKEQueryDirectionMaxMaxFloat{0.19259800016880035400390625}
\def\EQKEQueryDirectionMaxMaxKey{29022}
\def\EQKEQueryDirectionMaxMeanFloat{0.1579657495021820068359375}
\def\EQKEQueryDirectionMaxMeanKey{5358}
\def\EQKEQueryDirectionMaxMedianFloat{0.1418088972568511962890625}
\def\EQKEQueryDirectionMaxMedianKey{31308}
\def\EQKEQueryDirectionMaxMinFloat{0.14144639670848846435546875}
\def\EQKEQueryDirectionMaxMinKey{14929}
\def\EQKEQueryDirectionMaxStdDevFloat{0.0099591948091983795166015625}
\def\EQKEQueryDirectionMeanLen{151}
\def\EQKEQueryDirectionMeanMaxFloat{0.1247732937335968017578125}
\def\EQKEQueryDirectionMeanMaxKey{6082}
\def\EQKEQueryDirectionMeanMeanFloat{0.124376475811004638671875}
\def\EQKEQueryDirectionMeanMeanKey{22286}
\def\EQKEQueryDirectionMeanMedianFloat{0.12336383201181888580322265625}
\def\EQKEQueryDirectionMeanMedianKey{28716}
\def\EQKEQueryDirectionMeanMinFloat{0.12331725656986236572265625}
\def\EQKEQueryDirectionMeanMinKey{1951}
\def\EQKEQueryDirectionMeanStdDevFloat{0.000255489605478942394256591796875}
\def\EQKEQueryDirectionMedianLen{151}
\def\EQKEQueryDirectionMedianMaxFloat{0.111224692948162562355918225875939242541790008544921875}
\def\EQKEQueryDirectionMedianMaxKey{30684}
\def\EQKEQueryDirectionMedianMeanFloat{0.0962650931910272456004662444684072397649288177490234375}
\def\EQKEQueryDirectionMedianMeanKey{7884}
\def\EQKEQueryDirectionMedianMedianFloat{0.06542699687182902679172258331163902767002582550048828125}
\def\EQKEQueryDirectionMedianMedianKey{29565}
\def\EQKEQueryDirectionMedianMinFloat{0.06348112888634205308591162975062616169452667236328125}
\def\EQKEQueryDirectionMedianMinKey{19917}
\def\EQKEQueryDirectionMedianStdDevFloat{0.00848102048500555365240227700951436418108642101287841796875}
\def\EQKEQueryDirectionMinLen{151}
\def\EQKEQueryDirectionMinMaxFloat{0.111088432371616363525390625}
\def\EQKEQueryDirectionMinMaxKey{30684}
\def\EQKEQueryDirectionMinMeanFloat{0.094514973461627960205078125}
\def\EQKEQueryDirectionMinMeanKey{7238}
\def\EQKEQueryDirectionMinMedianFloat{0.063680939376354217529296875}
\def\EQKEQueryDirectionMinMedianKey{1681}
\def\EQKEQueryDirectionMinMinFloat{0.0632666051387786865234375}
\def\EQKEQueryDirectionMinMinKey{19917}
\def\EQKEQueryDirectionMinStdDevFloat{0.009428567253053188323974609375}
\def\EQKEQueryDirectionStdDevLen{151}
\def\EQKEQueryDirectionStdDevMaxFloat{0.02044148556888103485107421875}
\def\EQKEQueryDirectionStdDevMaxKey{1951}
\def\EQKEQueryDirectionStdDevMeanFloat{0.01224371977150440216064453125}
\def\EQKEQueryDirectionStdDevMeanKey{6910}
\def\EQKEQueryDirectionStdDevMedianFloat{0.00813629548065364360809326171875}
\def\EQKEQueryDirectionStdDevMedianKey{13293}
\def\EQKEQueryDirectionStdDevMinFloat{0.00752504169940948486328125}
\def\EQKEQueryDirectionStdDevMinKey{6082}
\def\EQKEQueryDirectionStdDevStdDevFloat{0.0023494991473853588104248046875}
\def\EQKERatioFirstTwoSingularLen{151}
\def\EQKERatioFirstTwoSingularLowerWhiskerBottomEndFloat{426.31100091730041867776890285313129425048828125}
\def\EQKERatioFirstTwoSingularLowerWhiskerBottomEndKey{19917}
\def\EQKERatioFirstTwoSingularLowerWhiskerCrosshatchFloat{434.85636899011069544940255582332611083984375}
\def\EQKERatioFirstTwoSingularLowerWhiskerCrosshatchKey{19917}
\def\EQKERatioFirstTwoSingularMaxFloat{1738.55517578125}
\def\EQKERatioFirstTwoSingularMaxKey{15622}
\def\EQKERatioFirstTwoSingularMeanFloat{973.814385824645569300628267228603363037109375}
\def\EQKERatioFirstTwoSingularMeanKey{31308}
\def\EQKERatioFirstTwoSingularMedianFloat{487.19382476806640625}
\def\EQKERatioFirstTwoSingularMedianKey{1681}
\def\EQKERatioFirstTwoSingularMinFloat{423.573760986328125}
\def\EQKERatioFirstTwoSingularMinKey{19917}
\def\EQKERatioFirstTwoSingularQuartileOneFloat{455.383792877197265625}
\def\EQKERatioFirstTwoSingularQuartileOneKey{19917}
\def\EQKERatioFirstTwoSingularQuartileThreeFloat{511.6292724609375}
\def\EQKERatioFirstTwoSingularQuartileThreeKey{1681}
\def\EQKERatioFirstTwoSingularSqrMeanFloat{997835.30997051228769123554229736328125}
\def\EQKERatioFirstTwoSingularStdDevFloat{222.532810909943947308420320041477680206298828125}
\def\EQKERatioFirstTwoSingularUpperWhiskerCrosshatchFloat{517.8799534315761547986767254769802093505859375}
\def\EQKERatioFirstTwoSingularUpperWhiskerCrosshatchKey{1681}
\def\EQKERatioFirstTwoSingularUpperWhiskerTopEndFloat{520.4820514782492182348505593836307525634765625}
\def\EQKERatioFirstTwoSingularUpperWhiskerTopEndKey{1681}
\def\EQKESecondSingularLen{151}
\def\EQKESecondSingularMaxFloat{23.75489044189453125}
\def\EQKESecondSingularMaxKey{19917}
\def\EQKESecondSingularMeanFloat{9.598985024635364737832787795923650264739990234375}
\def\EQKESecondSingularMeanKey{25516}
\def\EQKESecondSingularMedianFloat{5.6681287288665771484375}
\def\EQKESecondSingularMedianKey{22545}
\def\EQKESecondSingularMinFloat{5.471874713897705078125}
\def\EQKESecondSingularMinKey{15622}
\def\EQKESecondSingularStdDevFloat{2.55163002786475345828876015730202198028564453125}
\def\EQKESingularLen{32}
\def\EQKESingularMaxLen{151}
\def\EQKESingularMaxMaxFloat{10488.7802734375}
\def\EQKESingularMaxMaxKey{1681}
\def\EQKESingularMaxMeanFloat{8855.322265625}
\def\EQKESingularMaxMeanKey{4157}
\def\EQKESingularMaxMedianFloat{7335.0709228515625}
\def\EQKESingularMaxMedianKey{30684}
\def\EQKESingularMaxMinFloat{7290.59130859375}
\def\EQKESingularMaxMinKey{3284}
\def\EQKESingularMaxStdDevFloat{655.80615234375}
\def\EQKESingularMeanLen{151}
\def\EQKESingularMeanMaxFloat{329.191680908203125}
\def\EQKESingularMeanMaxKey{1681}
\def\EQKESingularMeanMeanFloat{277.913970947265625}
\def\EQKESingularMeanMeanKey{4157}
\def\EQKESingularMeanMedianFloat{230.36562347412109375}
\def\EQKESingularMeanMedianKey{30684}
\def\EQKESingularMeanMinFloat{228.9756011962890625}
\def\EQKESingularMeanMinKey{3284}
\def\EQKESingularMeanStdDevFloat{20.5115489959716796875}
\def\EQKESingularMedianLen{151}
\def\EQKESingularMedianMaxFloat{0.00351753218099474899982492814842771622352302074432373046875}
\def\EQKESingularMedianMaxKey{20976}
\def\EQKESingularMedianMeanFloat{0.00158211926246194507610087764959416745114140212535858154296875}
\def\EQKESingularMedianMeanKey{18289}
\def\EQKESingularMedianMedianFloat{0.000499655241874279502055367085944226346327923238277435302734375}
\def\EQKESingularMedianMedianKey{7790}
\def\EQKESingularMedianMinFloat{0.0004861070736660621821774441730923399518360383808612823486328125}
\def\EQKESingularMedianMinKey{9816}
\def\EQKESingularMedianStdDevFloat{0.000658629037516132221675990709996995065012015402317047119140625}
\def\EQKESingularMinLen{151}
\def\EQKESingularMinMaxFloat{0.002745185978710651397705078125}
\def\EQKESingularMinMaxKey{20338}
\def\EQKESingularMinMeanFloat{0.001012226217426359653472900390625}
\def\EQKESingularMinMeanKey{21598}
\def\EQKESingularMinMedianFloat{0.0004707291009253822267055511474609375}
\def\EQKESingularMinMedianKey{2743}
\def\EQKESingularMinMinFloat{0.0004603552515618503093719482421875}
\def\EQKESingularMinMinKey{9816}
\def\EQKESingularMinStdDevFloat{0.00045875317300669848918914794921875}
\def\EQKESingularStdDevLen{151}
\def\EQKESingularStdDevMaxFloat{1824.7196044921875}
\def\EQKESingularStdDevMaxKey{1681}
\def\EQKESingularStdDevMeanFloat{1540.5494384765625}
\def\EQKESingularStdDevMeanKey{4157}
\def\EQKESingularStdDevMedianFloat{1276.0438232421875}
\def\EQKESingularStdDevMedianKey{30684}
\def\EQKESingularStdDevMinFloat{1268.3046875}
\def\EQKESingularStdDevMinKey{3284}
\def\EQKESingularStdDevStdDevFloat{114.102386474609375}
\def\EQKESizeDirectionDiffsLen{63}
\def\EQKESizeDirectionDiffsMaxLen{151}
\def\EQKESizeDirectionDiffsMaxMaxFloat{0.2134025990962982177734375}
\def\EQKESizeDirectionDiffsMaxMaxKey{4810}
\def\EQKESizeDirectionDiffsMaxMeanFloat{0.0414469502866268157958984375}
\def\EQKESizeDirectionDiffsMaxMeanKey{18146}
\def\EQKESizeDirectionDiffsMaxMedianFloat{0.0249995253980159759521484375}
\def\EQKESizeDirectionDiffsMaxMedianKey{26374}
\def\EQKESizeDirectionDiffsMaxMinFloat{0.024478852748870849609375}
\def\EQKESizeDirectionDiffsMaxMinKey{15622}
\def\EQKESizeDirectionDiffsMaxStdDevFloat{0.02020668424665927886962890625}
\def\EQKESizeDirectionDiffsMeanLen{151}
\def\EQKESizeDirectionDiffsMeanMaxFloat{0.0074008437804877758026123046875}
\def\EQKESizeDirectionDiffsMeanMaxKey{28778}
\def\EQKESizeDirectionDiffsMeanMeanFloat{0.00637655518949031829833984375}
\def\EQKESizeDirectionDiffsMeanMeanKey{24173}
\def\EQKESizeDirectionDiffsMeanMedianFloat{0.00559147330932319164276123046875}
\def\EQKESizeDirectionDiffsMeanMedianKey{15622}
\def\EQKESizeDirectionDiffsMeanMinFloat{0.0053919623605906963348388671875}
\def\EQKESizeDirectionDiffsMeanMinKey{2345}
\def\EQKESizeDirectionDiffsMeanStdDevFloat{0.00033067981712520122528076171875}
\def\EQKESizeDirectionDiffsMedianLen{151}
\def\EQKESizeDirectionDiffsMedianMaxFloat{-0.00894455179572105352203692518742172978818416595458984375}
\def\EQKESizeDirectionDiffsMedianMaxKey{8721}
\def\EQKESizeDirectionDiffsMedianMeanFloat{-0.0259257347383443914612399794350494630634784698486328125}
\def\EQKESizeDirectionDiffsMedianMeanKey{6204}
\def\EQKESizeDirectionDiffsMedianMedianFloat{-0.11837354600429535189665131156289135105907917022705078125}
\def\EQKESizeDirectionDiffsMedianMedianKey{5781}
\def\EQKESizeDirectionDiffsMedianMinFloat{-0.148360285162925709112613503748434595763683319091796875}
\def\EQKESizeDirectionDiffsMedianMinKey{4810}
\def\EQKESizeDirectionDiffsMedianStdDevFloat{0.01477348524709438427893193335194155224598944187164306640625}
\def\EQKESizeDirectionDiffsMinLen{151}
\def\EQKESizeDirectionDiffsMinMaxFloat{-0.0089757740497589111328125}
\def\EQKESizeDirectionDiffsMinMaxKey{8721}
\def\EQKESizeDirectionDiffsMinMeanFloat{-0.02856989018619060516357421875}
\def\EQKESizeDirectionDiffsMinMeanKey{28090}
\def\EQKESizeDirectionDiffsMinMedianFloat{-0.163775525987148284912109375}
\def\EQKESizeDirectionDiffsMinMedianKey{5781}
\def\EQKESizeDirectionDiffsMinMinFloat{-0.206407070159912109375}
\def\EQKESizeDirectionDiffsMinMinKey{4810}
\def\EQKESizeDirectionDiffsMinStdDevFloat{0.02075720392167568206787109375}
\def\EQKESizeDirectionDiffsStdDevLen{151}
\def\EQKESizeDirectionDiffsStdDevMaxFloat{0.039338998496532440185546875}
\def\EQKESizeDirectionDiffsStdDevMaxKey{4810}
\def\EQKESizeDirectionDiffsStdDevMeanFloat{0.01247579418122768402099609375}
\def\EQKESizeDirectionDiffsStdDevMeanKey{1412}
\def\EQKESizeDirectionDiffsStdDevMedianFloat{0.00915886578150093555450439453125}
\def\EQKESizeDirectionDiffsStdDevMedianKey{29022}
\def\EQKESizeDirectionDiffsStdDevMinFloat{0.00913411192595958709716796875}
\def\EQKESizeDirectionDiffsStdDevMinKey{32382}
\def\EQKESizeDirectionDiffsStdDevStdDevFloat{0.003279286436736583709716796875}
\def\EQKESizeDirectionLen{64}
\def\EQKESizeDirectionMaxLen{151}
\def\EQKESizeDirectionMaxMaxFloat{0.326307952404022216796875}
\def\EQKESizeDirectionMaxMaxKey{28778}
\def\EQKESizeDirectionMaxMeanFloat{0.2644797861576080322265625}
\def\EQKESizeDirectionMaxMeanKey{27484}
\def\EQKESizeDirectionMaxMedianFloat{0.21249423921108245849609375}
\def\EQKESizeDirectionMaxMedianKey{1696}
\def\EQKESizeDirectionMaxMinFloat{0.200592517852783203125}
\def\EQKESizeDirectionMaxMinKey{2345}
\def\EQKESizeDirectionMaxStdDevFloat{0.025460161268711090087890625}
\def\EQKESizeDirectionMeanLen{151}
\def\EQKESizeDirectionMeanMaxFloat{-0.0191762745380401611328125}
\def\EQKESizeDirectionMeanMaxKey{3284}
\def\EQKESizeDirectionMeanMeanFloat{-0.049380145967006683349609375}
\def\EQKESizeDirectionMeanMeanKey{8048}
\def\EQKESizeDirectionMeanMedianFloat{-0.07314396835863590240478515625}
\def\EQKESizeDirectionMeanMedianKey{2345}
\def\EQKESizeDirectionMeanMinFloat{-0.07365359365940093994140625}
\def\EQKESizeDirectionMeanMinKey{19917}
\def\EQKESizeDirectionMeanStdDevFloat{0.011679609306156635284423828125}
\def\EQKESizeDirectionMedianLen{151}
\def\EQKESizeDirectionMedianMaxFloat{-0.123025978393852708503430903874686919152736663818359375}
\def\EQKESizeDirectionMedianMaxKey{3284}
\def\EQKESizeDirectionMedianMeanFloat{-0.148644603975117195471256081873434595763683319091796875}
\def\EQKESizeDirectionMedianMeanKey{50}
\def\EQKESizeDirectionMedianMedianFloat{-0.163247167188674213722521244562813080847263336181640625}
\def\EQKESizeDirectionMedianMedianKey{23696}
\def\EQKESizeDirectionMedianMinFloat{-0.167806982249021519049136941248434595763683319091796875}
\def\EQKESizeDirectionMedianMinKey{2345}
\def\EQKESizeDirectionMedianStdDevFloat{0.007424501745249056060271808377137858769856393337249755859375}
\def\EQKESizeDirectionMinLen{151}
\def\EQKESizeDirectionMinMaxFloat{-0.123348571360111236572265625}
\def\EQKESizeDirectionMinMaxKey{3284}
\def\EQKESizeDirectionMinMeanFloat{-0.149314582347869873046875}
\def\EQKESizeDirectionMinMeanKey{6589}
\def\EQKESizeDirectionMinMedianFloat{-0.1648471914231777191162109375}
\def\EQKESizeDirectionMinMedianKey{5781}
\def\EQKESizeDirectionMinMinFloat{-0.17044807970523834228515625}
\def\EQKESizeDirectionMinMinKey{2345}
\def\EQKESizeDirectionMinStdDevFloat{0.007597322575747966766357421875}
\def\EQKESizeDirectionStdDevLen{151}
\def\EQKESizeDirectionStdDevMaxFloat{0.12352032959461212158203125}
\def\EQKESizeDirectionStdDevMaxKey{3284}
\def\EQKESizeDirectionStdDevMeanFloat{0.114129073917865753173828125}
\def\EQKESizeDirectionStdDevMeanKey{23633}
\def\EQKESizeDirectionStdDevMedianFloat{0.10136482305824756622314453125}
\def\EQKESizeDirectionStdDevMedianKey{2345}
\def\EQKESizeDirectionStdDevMinFloat{0.100995801389217376708984375}
\def\EQKESizeDirectionStdDevMinKey{19917}
\def\EQKESizeDirectionStdDevStdDevFloat{0.004974323324859142303466796875}
\def\EQKEThirdSingularLen{151}
\def\EQKEThirdSingularMaxFloat{8.2380084991455078125}
\def\EQKEThirdSingularMaxKey{6159}
\def\EQKEThirdSingularMeanFloat{5.5607376840730378120269961073063313961029052734375}
\def\EQKEThirdSingularMeanKey{22261}
\def\EQKEThirdSingularMedianFloat{3.908039629459381103515625}
\def\EQKEThirdSingularMedianKey{32382}
\def\EQKEThirdSingularMinFloat{3.5774071216583251953125}
\def\EQKEThirdSingularMinKey{27300}
\def\EQKEThirdSingularStdDevFloat{0.86317961142677657182531447688234038650989532470703125}
\def\EQKEWithAttnScaleFirstSingularLen{151}
\def\EQKEWithAttnScaleFirstSingularMaxFloat{1854.1719970703125}
\def\EQKEWithAttnScaleFirstSingularMaxKey{1681}
\def\EQKEWithAttnScaleFirstSingularMeanFloat{1565.41471488902107012108899652957916259765625}
\def\EQKEWithAttnScaleFirstSingularMeanKey{4157}
\def\EQKEWithAttnScaleFirstSingularMedianFloat{1296.669647216796875}
\def\EQKEWithAttnScaleFirstSingularMedianKey{30684}
\def\EQKEWithAttnScaleFirstSingularMinFloat{1288.806640625}
\def\EQKEWithAttnScaleFirstSingularMinKey{3284}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoLen{151}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMaxFloat{2622.19518522924272474483586847782135009765625}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMaxKey{1681}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMeanFloat{2213.83072053446585414349101483821868896484375}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMeanKey{4157}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMedianFloat{1833.767801011530764299095608294010162353515625}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMedianKey{30684}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMinFloat{1822.6478304483825922943651676177978515625}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMinKey{3284}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoStdDevFloat{163.951530801194536479670205153524875640869140625}
\def\EQKEWithAttnScaleFirstSingularStdDevFloat{115.9312392154397599597359658218920230865478515625}
\def\EQKEWithAttnScaleRatioFirstTwoSingularLen{151}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMaxFloat{1738.55517578125}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMaxKey{15622}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMeanFloat{973.8143817825822452505235560238361358642578125}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMeanKey{31308}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMedianFloat{487.19382476806640625}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMedianKey{1681}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMinFloat{423.573760986328125}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMinKey{19917}
\def\EQKEWithAttnScaleRatioFirstTwoSingularStdDevFloat{222.53280785180919565391377545893192291259765625}
\def\EQKEWithAttnScaleSecondSingularLen{151}
\def\EQKEWithAttnScaleSecondSingularMaxFloat{4.19931125640869140625}
\def\EQKEWithAttnScaleSecondSingularMaxKey{19917}
\def\EQKEWithAttnScaleSecondSingularMeanFloat{1.6968768827173092983429114610771648585796356201171875}
\def\EQKEWithAttnScaleSecondSingularMeanKey{25516}
\def\EQKEWithAttnScaleSecondSingularMedianFloat{1.00199306011199951171875}
\def\EQKEWithAttnScaleSecondSingularMedianKey{22545}
\def\EQKEWithAttnScaleSecondSingularMinFloat{0.967299938201904296875}
\def\EQKEWithAttnScaleSecondSingularMinKey{15622}
\def\EQKEWithAttnScaleSecondSingularStdDevFloat{0.45106873676301528774956750567071139812469482421875}
\def\EQKEWithAttnScaleSingularLen{32}
\def\EQKEWithAttnScaleSingularMaxLen{151}
\def\EQKEWithAttnScaleSingularMaxMaxFloat{10488.7802734375}
\def\EQKEWithAttnScaleSingularMaxMaxKey{1681}
\def\EQKEWithAttnScaleSingularMaxMeanFloat{8855.322265625}
\def\EQKEWithAttnScaleSingularMaxMeanKey{4157}
\def\EQKEWithAttnScaleSingularMaxMedianFloat{7335.0709228515625}
\def\EQKEWithAttnScaleSingularMaxMedianKey{30684}
\def\EQKEWithAttnScaleSingularMaxMinFloat{7290.59130859375}
\def\EQKEWithAttnScaleSingularMaxMinKey{3284}
\def\EQKEWithAttnScaleSingularMaxStdDevFloat{655.80615234375}
\def\EQKEWithAttnScaleSingularMeanLen{151}
\def\EQKEWithAttnScaleSingularMeanMaxFloat{329.191680908203125}
\def\EQKEWithAttnScaleSingularMeanMaxKey{1681}
\def\EQKEWithAttnScaleSingularMeanMeanFloat{277.913970947265625}
\def\EQKEWithAttnScaleSingularMeanMeanKey{4157}
\def\EQKEWithAttnScaleSingularMeanMedianFloat{230.36562347412109375}
\def\EQKEWithAttnScaleSingularMeanMedianKey{30684}
\def\EQKEWithAttnScaleSingularMeanMinFloat{228.9756011962890625}
\def\EQKEWithAttnScaleSingularMeanMinKey{3284}
\def\EQKEWithAttnScaleSingularMeanStdDevFloat{20.5115489959716796875}
\def\EQKEWithAttnScaleSingularMedianLen{151}
\def\EQKEWithAttnScaleSingularMedianMaxFloat{0.00351753218099474899982492814842771622352302074432373046875}
\def\EQKEWithAttnScaleSingularMedianMaxKey{20976}
\def\EQKEWithAttnScaleSingularMedianMeanFloat{0.00158211926246194507610087764959416745114140212535858154296875}
\def\EQKEWithAttnScaleSingularMedianMeanKey{18289}
\def\EQKEWithAttnScaleSingularMedianMedianFloat{0.000499655241874279502055367085944226346327923238277435302734375}
\def\EQKEWithAttnScaleSingularMedianMedianKey{7790}
\def\EQKEWithAttnScaleSingularMedianMinFloat{0.0004861070736660621821774441730923399518360383808612823486328125}
\def\EQKEWithAttnScaleSingularMedianMinKey{9816}
\def\EQKEWithAttnScaleSingularMedianStdDevFloat{0.000658629037516132221675990709996995065012015402317047119140625}
\def\EQKEWithAttnScaleSingularMinLen{151}
\def\EQKEWithAttnScaleSingularMinMaxFloat{0.002745185978710651397705078125}
\def\EQKEWithAttnScaleSingularMinMaxKey{20338}
\def\EQKEWithAttnScaleSingularMinMeanFloat{0.001012226217426359653472900390625}
\def\EQKEWithAttnScaleSingularMinMeanKey{21598}
\def\EQKEWithAttnScaleSingularMinMedianFloat{0.0004707291009253822267055511474609375}
\def\EQKEWithAttnScaleSingularMinMedianKey{2743}
\def\EQKEWithAttnScaleSingularMinMinFloat{0.0004603552515618503093719482421875}
\def\EQKEWithAttnScaleSingularMinMinKey{9816}
\def\EQKEWithAttnScaleSingularMinStdDevFloat{0.00045875317300669848918914794921875}
\def\EQKEWithAttnScaleSingularStdDevLen{151}
\def\EQKEWithAttnScaleSingularStdDevMaxFloat{1824.7196044921875}
\def\EQKEWithAttnScaleSingularStdDevMaxKey{1681}
\def\EQKEWithAttnScaleSingularStdDevMeanFloat{1540.5494384765625}
\def\EQKEWithAttnScaleSingularStdDevMeanKey{4157}
\def\EQKEWithAttnScaleSingularStdDevMedianFloat{1276.0438232421875}
\def\EQKEWithAttnScaleSingularStdDevMedianKey{30684}
\def\EQKEWithAttnScaleSingularStdDevMinFloat{1268.3046875}
\def\EQKEWithAttnScaleSingularStdDevMinKey{3284}
\def\EQKEWithAttnScaleSingularStdDevStdDevFloat{114.102386474609375}
\def\EQKEWithAttnScaleThirdSingularLen{151}
\def\EQKEWithAttnScaleThirdSingularMaxFloat{1.45628798007965087890625}
\def\EQKEWithAttnScaleThirdSingularMaxKey{6159}
\def\EQKEWithAttnScaleThirdSingularMeanFloat{0.983008852068162131132567083113826811313629150390625}
\def\EQKEWithAttnScaleThirdSingularMeanKey{22261}
\def\EQKEWithAttnScaleThirdSingularMedianFloat{0.6908503472805023193359375}
\def\EQKEWithAttnScaleThirdSingularMedianKey{32382}
\def\EQKEWithAttnScaleThirdSingularMinFloat{0.632402241230010986328125}
\def\EQKEWithAttnScaleThirdSingularMinKey{27300}
\def\EQKEWithAttnScaleThirdSingularStdDevFloat{0.152590042951222748524031658234889619052410125732421875}
\def\EQKPAbsLen{640}
\def\EQKPAbsMaxLen{151}
\def\EQKPAbsMaxMaxFloat{13.5455780029296875}
\def\EQKPAbsMaxMaxKey{2306}
\def\EQKPAbsMaxMeanFloat{3.964107990264892578125}
\def\EQKPAbsMaxMeanKey{19093}
\def\EQKPAbsMaxMedianFloat{0.83582402765750885009765625}
\def\EQKPAbsMaxMedianKey{24202}
\def\EQKPAbsMaxMinFloat{0.7649059295654296875}
\def\EQKPAbsMaxMinKey{26278}
\def\EQKPAbsMaxStdDevFloat{2.287724018096923828125}
\def\EQKPAbsMeanLen{151}
\def\EQKPAbsMeanMaxFloat{5.04351711273193359375}
\def\EQKPAbsMeanMaxKey{26374}
\def\EQKPAbsMeanMeanFloat{1.2520809173583984375}
\def\EQKPAbsMeanMeanKey{32382}
\def\EQKPAbsMeanMedianFloat{0.316237308084964752197265625}
\def\EQKPAbsMeanMedianKey{24202}
\def\EQKPAbsMeanMinFloat{0.2936584055423736572265625}
\def\EQKPAbsMeanMinKey{26278}
\def\EQKPAbsMeanStdDevFloat{0.704301059246063232421875}
\def\EQKPAbsMedianLen{151}
\def\EQKPAbsMedianMaxFloat{2.10192644596099853515625}
\def\EQKPAbsMedianMaxKey{26374}
\def\EQKPAbsMedianMeanFloat{0.06615350094946126358053106741863302886486053466796875}
\def\EQKPAbsMedianMeanKey{16284}
\def\EQKPAbsMedianMedianFloat{0.00134281818958697889143660830768567393533885478973388671875}
\def\EQKPAbsMedianMedianKey{32382}
\def\EQKPAbsMedianMinFloat{0.00115186748909763998771627058204103377647697925567626953125}
\def\EQKPAbsMedianMinKey{2773}
\def\EQKPAbsMedianStdDevFloat{0.1902878800842557893702178262174129486083984375}
\def\EQKPAbsMinLen{151}
\def\EQKPAbsMinMaxFloat{1.937100887298583984375}
\def\EQKPAbsMinMaxKey{26374}
\def\EQKPAbsMinMeanFloat{0.04216359555721282958984375}
\def\EQKPAbsMinMeanKey{3254}
\def\EQKPAbsMinMedianFloat{0.0000071545500759384594857692718505859375}
\def\EQKPAbsMinMedianKey{50}
\def\EQKPAbsMinMinFloat{0.000000931322574615478515625}
\def\EQKPAbsMinMinKey{16149}
\def\EQKPAbsMinStdDevFloat{0.17159569263458251953125}
\def\EQKPAbsStdDevLen{151}
\def\EQKPAbsStdDevMaxFloat{3.0929393768310546875}
\def\EQKPAbsStdDevMaxKey{2306}
\def\EQKPAbsStdDevMeanFloat{0.923752963542938232421875}
\def\EQKPAbsStdDevMeanKey{24566}
\def\EQKPAbsStdDevMedianFloat{0.2053572498261928558349609375}
\def\EQKPAbsStdDevMedianKey{8893}
\def\EQKPAbsStdDevMinFloat{0.1751504242420196533203125}
\def\EQKPAbsStdDevMinKey{26278}
\def\EQKPAbsStdDevStdDevFloat{0.526749193668365478515625}
\def\EQKPLen{640}
\def\EQKPMaxLen{151}
\def\EQKPMaxMaxFloat{13.5455780029296875}
\def\EQKPMaxMaxKey{2306}
\def\EQKPMaxMeanFloat{3.5019791126251220703125}
\def\EQKPMaxMeanKey{19093}
\def\EQKPMaxMedianFloat{0.83582402765750885009765625}
\def\EQKPMaxMedianKey{24202}
\def\EQKPMaxMinFloat{0.7649059295654296875}
\def\EQKPMaxMinKey{26278}
\def\EQKPMaxRowDiffLen{64}
\def\EQKPMaxRowDiffMaxLen{151}
\def\EQKPMaxRowDiffMaxMaxFloat{20.8915233612060546875}
\def\EQKPMaxRowDiffMaxMaxKey{2306}
\def\EQKPMaxRowDiffMaxMeanFloat{6.789508819580078125}
\def\EQKPMaxRowDiffMaxMeanKey{30684}
\def\EQKPMaxRowDiffMaxMedianFloat{1.56544387340545654296875}
\def\EQKPMaxRowDiffMaxMedianKey{24202}
\def\EQKPMaxRowDiffMaxMinFloat{1.52803814411163330078125}
\def\EQKPMaxRowDiffMaxMinKey{26278}
\def\EQKPMaxRowDiffMaxStdDevFloat{3.757100582122802734375}
\def\EQKPMaxRowDiffMeanLen{151}
\def\EQKPMaxRowDiffMeanMaxFloat{15.580738067626953125}
\def\EQKPMaxRowDiffMeanMaxKey{2306}
\def\EQKPMaxRowDiffMeanMeanFloat{5.2899074554443359375}
\def\EQKPMaxRowDiffMeanMeanKey{7098}
\def\EQKPMaxRowDiffMeanMedianFloat{1.2161662876605987548828125}
\def\EQKPMaxRowDiffMeanMedianKey{24202}
\def\EQKPMaxRowDiffMeanMinFloat{0.99162971973419189453125}
\def\EQKPMaxRowDiffMeanMinKey{26278}
\def\EQKPMaxRowDiffMeanStdDevFloat{2.94843959808349609375}
\def\EQKPMaxRowDiffMedianLen{151}
\def\EQKPMaxRowDiffMedianMaxFloat{13.2231940937042242723009621840901672840118408203125}
\def\EQKPMaxRowDiffMedianMaxKey{2306}
\def\EQKPMaxRowDiffMedianMeanFloat{4.0418647788909094487053152988664805889129638671875}
\def\EQKPMaxRowDiffMedianMeanKey{6082}
\def\EQKPMaxRowDiffMedianMedianFloat{0.7536535673588513617460193927399814128875732421875}
\def\EQKPMaxRowDiffMedianMedianKey{24202}
\def\EQKPMaxRowDiffMedianMinFloat{0.718098590672016090508122942992486059665679931640625}
\def\EQKPMaxRowDiffMedianMinKey{26278}
\def\EQKPMaxRowDiffMedianStdDevFloat{2.368855586864234030741727110580541193485260009765625}
\def\EQKPMaxRowDiffMinLen{151}
\def\EQKPMaxRowDiffMinMaxFloat{13.095088958740234375}
\def\EQKPMaxRowDiffMinMaxKey{2306}
\def\EQKPMaxRowDiffMinMeanFloat{3.969257354736328125}
\def\EQKPMaxRowDiffMinMeanKey{2743}
\def\EQKPMaxRowDiffMinMedianFloat{0.70975758135318756103515625}
\def\EQKPMaxRowDiffMinMedianKey{24202}
\def\EQKPMaxRowDiffMinMinFloat{0.702721655368804931640625}
\def\EQKPMaxRowDiffMinMinKey{26278}
\def\EQKPMaxRowDiffMinStdDevFloat{2.3514559268951416015625}
\def\EQKPMaxRowDiffStdDevLen{151}
\def\EQKPMaxRowDiffStdDevMaxFloat{1.66561067104339599609375}
\def\EQKPMaxRowDiffStdDevMaxKey{11498}
\def\EQKPMaxRowDiffStdDevMeanFloat{0.557626903057098388671875}
\def\EQKPMaxRowDiffStdDevMeanKey{519}
\def\EQKPMaxRowDiffStdDevMedianFloat{0.143349163234233856201171875}
\def\EQKPMaxRowDiffStdDevMedianKey{16149}
\def\EQKPMaxRowDiffStdDevMinFloat{0.127683162689208984375}
\def\EQKPMaxRowDiffStdDevMinKey{26278}
\def\EQKPMaxRowDiffStdDevStdDevFloat{0.306068360805511474609375}
\def\EQKPMaxStdDevFloat{2.188551425933837890625}
\def\EQKPMeanLen{151}
\def\EQKPMeanMaxFloat{0.00000246465197051293216645717620849609375}
\def\EQKPMeanMaxKey{13036}
\def\EQKPMeanMeanFloat{0.00000001108705927066466756514273583889007568359375}
\def\EQKPMeanMeanKey{20754}
\def\EQKPMeanMedianFloat{-0.00000249177679734202683903276920318603515625}
\def\EQKPMeanMedianKey{2306}
\def\EQKPMeanMinFloat{-0.0000024926848709583282470703125}
\def\EQKPMeanMinKey{742}
\def\EQKPMeanStdDevFloat{0.0000008280347856270964257419109344482421875}
\def\EQKPMedianLen{151}
\def\EQKPMedianMaxFloat{-0.6493447592854499905712373220012523233890533447265625}
\def\EQKPMedianMaxKey{26278}
\def\EQKPMedianMeanFloat{-3.0766349237742804945128227700479328632354736328125}
\def\EQKPMedianMeanKey{30684}
\def\EQKPMedianMedianFloat{-7.9271465563774103912919599679298698902130126953125}
\def\EQKPMedianMedianKey{26374}
\def\EQKPMedianMinFloat{-8.98257958889007568359375}
\def\EQKPMedianMinKey{19538}
\def\EQKPMedianStdDevFloat{1.662315696902322503802906794589944183826446533203125}
\def\EQKPMinLen{151}
\def\EQKPMinMaxFloat{-0.76313221454620361328125}
\def\EQKPMinMaxKey{26278}
\def\EQKPMinMeanFloat{-3.3573055267333984375}
\def\EQKPMinMeanKey{519}
\def\EQKPMinMedianFloat{-8.8664486408233642578125}
\def\EQKPMinMedianKey{26374}
\def\EQKPMinMinFloat{-9.1999301910400390625}
\def\EQKPMinMinKey{19538}
\def\EQKPMinStdDevFloat{1.82369935512542724609375}
\def\EQKPStdDevLen{151}
\def\EQKPStdDevMaxFloat{5.3096370697021484375}
\def\EQKPStdDevMaxKey{26374}
\def\EQKPStdDevMeanFloat{1.56748485565185546875}
\def\EQKPStdDevMeanKey{32382}
\def\EQKPStdDevMedianFloat{0.389459155499935150146484375}
\def\EQKPStdDevMedianKey{24202}
\def\EQKPStdDevMinFloat{0.3419252932071685791015625}
\def\EQKPStdDevMinKey{26278}
\def\EQKPStdDevStdDevFloat{0.85879075527191162109375}
\def\EQKPWithAttnScaleAbsLen{640}
\def\EQKPWithAttnScaleAbsMaxLen{151}
\def\EQKPWithAttnScaleAbsMaxMaxFloat{2.3945424556732177734375}
\def\EQKPWithAttnScaleAbsMaxMaxKey{2306}
\def\EQKPWithAttnScaleAbsMaxMeanFloat{0.7007620334625244140625}
\def\EQKPWithAttnScaleAbsMaxMeanKey{19093}
\def\EQKPWithAttnScaleAbsMaxMedianFloat{0.147754214704036712646484375}
\def\EQKPWithAttnScaleAbsMaxMedianKey{24202}
\def\EQKPWithAttnScaleAbsMaxMinFloat{0.13521754741668701171875}
\def\EQKPWithAttnScaleAbsMaxMinKey{26278}
\def\EQKPWithAttnScaleAbsMaxStdDevFloat{0.4044162929058074951171875}
\def\EQKPWithAttnScaleAbsMeanLen{151}
\def\EQKPWithAttnScaleAbsMeanMaxFloat{0.89157640933990478515625}
\def\EQKPWithAttnScaleAbsMeanMaxKey{26374}
\def\EQKPWithAttnScaleAbsMeanMeanFloat{0.22133873403072357177734375}
\def\EQKPWithAttnScaleAbsMeanMeanKey{32382}
\def\EQKPWithAttnScaleAbsMeanMedianFloat{0.05590338446199893951416015625}
\def\EQKPWithAttnScaleAbsMeanMedianKey{24202}
\def\EQKPWithAttnScaleAbsMeanMinFloat{0.0519119612872600555419921875}
\def\EQKPWithAttnScaleAbsMeanMinKey{26278}
\def\EQKPWithAttnScaleAbsMeanStdDevFloat{0.124504029750823974609375}
\def\EQKPWithAttnScaleAbsMedianLen{151}
\def\EQKPWithAttnScaleAbsMedianMaxFloat{0.37157162174582480940188133899937383830547332763671875}
\def\EQKPWithAttnScaleAbsMedianMaxKey{26374}
\def\EQKPWithAttnScaleAbsMedianMeanFloat{0.01169439752100575984072872159913458744995296001434326171875}
\def\EQKPWithAttnScaleAbsMedianMeanKey{16284}
\def\EQKPWithAttnScaleAbsMedianMedianFloat{0.00023737896022794308732890844471086211342480964958667755126953125}
\def\EQKPWithAttnScaleAbsMedianMedianKey{32382}
\def\EQKPWithAttnScaleAbsMedianMinFloat{0.000203623330307891605393810774415896958089433610439300537109375}
\def\EQKPWithAttnScaleAbsMedianMinKey{2773}
\def\EQKPWithAttnScaleAbsMedianStdDevFloat{0.03363846352626308211508643353226943872869014739990234375}
\def\EQKPWithAttnScaleAbsMinLen{151}
\def\EQKPWithAttnScaleAbsMinMaxFloat{0.34243428707122802734375}
\def\EQKPWithAttnScaleAbsMinMaxKey{26374}
\def\EQKPWithAttnScaleAbsMinMeanFloat{0.007453541271388530731201171875}
\def\EQKPWithAttnScaleAbsMinMeanKey{3254}
\def\EQKPWithAttnScaleAbsMinMedianFloat{0.00000126475771367040579207241535186767578125}
\def\EQKPWithAttnScaleAbsMinMedianKey{50}
\def\EQKPWithAttnScaleAbsMinMinFloat{0.000000164636134059037431143224239349365234375}
\def\EQKPWithAttnScaleAbsMinMinKey{16149}
\def\EQKPWithAttnScaleAbsMinStdDevFloat{0.03033412061631679534912109375}
\def\EQKPWithAttnScaleAbsStdDevLen{151}
\def\EQKPWithAttnScaleAbsStdDevMaxFloat{0.546759665012359619140625}
\def\EQKPWithAttnScaleAbsStdDevMaxKey{2306}
\def\EQKPWithAttnScaleAbsStdDevMeanFloat{0.16329796612262725830078125}
\def\EQKPWithAttnScaleAbsStdDevMeanKey{24566}
\def\EQKPWithAttnScaleAbsStdDevMedianFloat{0.036302377469837665557861328125}
\def\EQKPWithAttnScaleAbsStdDevMedianKey{8893}
\def\EQKPWithAttnScaleAbsStdDevMinFloat{0.0309625156223773956298828125}
\def\EQKPWithAttnScaleAbsStdDevMinKey{26278}
\def\EQKPWithAttnScaleAbsStdDevStdDevFloat{0.09311698377132415771484375}
\def\EQKPWithAttnScaleLen{640}
\def\EQKPWithAttnScaleMaxLen{151}
\def\EQKPWithAttnScaleMaxMaxFloat{2.3945424556732177734375}
\def\EQKPWithAttnScaleMaxMaxKey{2306}
\def\EQKPWithAttnScaleMaxMeanFloat{0.619068324565887451171875}
\def\EQKPWithAttnScaleMaxMeanKey{19093}
\def\EQKPWithAttnScaleMaxMedianFloat{0.147754214704036712646484375}
\def\EQKPWithAttnScaleMaxMedianKey{24202}
\def\EQKPWithAttnScaleMaxMinFloat{0.13521754741668701171875}
\def\EQKPWithAttnScaleMaxMinKey{26278}
\def\EQKPWithAttnScaleMaxRowDiffLen{64}
\def\EQKPWithAttnScaleMaxRowDiffMaxLen{151}
\def\EQKPWithAttnScaleMaxRowDiffMaxMaxFloat{3.693134307861328125}
\def\EQKPWithAttnScaleMaxRowDiffMaxMaxKey{2306}
\def\EQKPWithAttnScaleMaxRowDiffMaxMeanFloat{1.20022690296173095703125}
\def\EQKPWithAttnScaleMaxRowDiffMaxMeanKey{30684}
\def\EQKPWithAttnScaleMaxRowDiffMaxMedianFloat{0.27673399448394775390625}
\def\EQKPWithAttnScaleMaxRowDiffMaxMedianKey{24202}
\def\EQKPWithAttnScaleMaxRowDiffMaxMinFloat{0.2701215445995330810546875}
\def\EQKPWithAttnScaleMaxRowDiffMaxMinKey{26278}
\def\EQKPWithAttnScaleMaxRowDiffMaxStdDevFloat{0.664167881011962890625}
\def\EQKPWithAttnScaleMaxRowDiffMeanLen{151}
\def\EQKPWithAttnScaleMaxRowDiffMeanMaxFloat{2.75431156158447265625}
\def\EQKPWithAttnScaleMaxRowDiffMeanMaxKey{2306}
\def\EQKPWithAttnScaleMaxRowDiffMeanMeanFloat{0.9351322650909423828125}
\def\EQKPWithAttnScaleMaxRowDiffMeanMeanKey{7098}
\def\EQKPWithAttnScaleMaxRowDiffMeanMedianFloat{0.214989848434925079345703125}
\def\EQKPWithAttnScaleMaxRowDiffMeanMedianKey{24202}
\def\EQKPWithAttnScaleMaxRowDiffMeanMinFloat{0.1752970218658447265625}
\def\EQKPWithAttnScaleMaxRowDiffMeanMinKey{26278}
\def\EQKPWithAttnScaleMaxRowDiffMeanStdDevFloat{0.5212154388427734375}
\def\EQKPWithAttnScaleMaxRowDiffMedianLen{151}
\def\EQKPWithAttnScaleMaxRowDiffMedianMaxFloat{2.337552584409713585245071953977458178997039794921875}
\def\EQKPWithAttnScaleMaxRowDiffMedianMaxKey{2306}
\def\EQKPWithAttnScaleMaxRowDiffMedianMeanFloat{0.71450751051800132085389805070008151233196258544921875}
\def\EQKPWithAttnScaleMaxRowDiffMedianMeanKey{6082}
\def\EQKPWithAttnScaleMaxRowDiffMedianMedianFloat{0.133228384237736474648983175939065404236316680908203125}
\def\EQKPWithAttnScaleMaxRowDiffMedianMedianKey{24202}
\def\EQKPWithAttnScaleMaxRowDiffMedianMinFloat{0.126943095177412035301500736750313080847263336181640625}
\def\EQKPWithAttnScaleMaxRowDiffMedianMinKey{26278}
\def\EQKPWithAttnScaleMaxRowDiffMedianStdDevFloat{0.418758468905816971794564551601069979369640350341796875}
\def\EQKPWithAttnScaleMaxRowDiffMinLen{151}
\def\EQKPWithAttnScaleMaxRowDiffMinMaxFloat{2.314906597137451171875}
\def\EQKPWithAttnScaleMaxRowDiffMinMaxKey{2306}
\def\EQKPWithAttnScaleMaxRowDiffMinMeanFloat{0.70167219638824462890625}
\def\EQKPWithAttnScaleMaxRowDiffMinMeanKey{2743}
\def\EQKPWithAttnScaleMaxRowDiffMinMedianFloat{0.12546859681606292724609375}
\def\EQKPWithAttnScaleMaxRowDiffMinMedianKey{24202}
\def\EQKPWithAttnScaleMaxRowDiffMinMinFloat{0.1242248117923736572265625}
\def\EQKPWithAttnScaleMaxRowDiffMinMinKey{26278}
\def\EQKPWithAttnScaleMaxRowDiffMinStdDevFloat{0.415682613849639892578125}
\def\EQKPWithAttnScaleMaxRowDiffStdDevLen{151}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMaxFloat{0.294441163539886474609375}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMaxKey{11498}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMeanFloat{0.09857542812824249267578125}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMeanKey{519}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMedianFloat{0.02534079365432262420654296875}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMedianKey{16149}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMinFloat{0.022571407258510589599609375}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMinKey{26278}
\def\EQKPWithAttnScaleMaxRowDiffStdDevStdDevFloat{0.054105751216411590576171875}
\def\EQKPWithAttnScaleMaxStdDevFloat{0.3868848979473114013671875}
\def\EQKPWithAttnScaleMeanLen{151}
\def\EQKPWithAttnScaleMeanMaxFloat{0.000000436417764149155118502676486968994140625}
\def\EQKPWithAttnScaleMeanMaxKey{13036}
\def\EQKPWithAttnScaleMeanMeanFloat{0.00000000183940029874207766624749638140201568603515625}
\def\EQKPWithAttnScaleMeanMeanKey{20754}
\def\EQKPWithAttnScaleMeanMedianFloat{-0.00000043888576328754425048828125}
\def\EQKPWithAttnScaleMeanMedianKey{2306}
\def\EQKPWithAttnScaleMeanMinFloat{-0.0000004409812390804290771484375}
\def\EQKPWithAttnScaleMeanMinKey{742}
\def\EQKPWithAttnScaleMeanStdDevFloat{0.0000001463077836660886532627046108245849609375}
\def\EQKPWithAttnScaleMedianLen{151}
\def\EQKPWithAttnScaleMedianMaxFloat{-0.1147890245541930143158282362492172978818416595458984375}
\def\EQKPWithAttnScaleMedianMaxKey{26278}
\def\EQKPWithAttnScaleMedianMeanFloat{-0.5438773633857929556967292228364385664463043212890625}
\def\EQKPWithAttnScaleMedianMeanKey{30684}
\def\EQKPWithAttnScaleMedianMedianFloat{-1.40133480817079547620096491300500929355621337890625}
\def\EQKPWithAttnScaleMedianMedianKey{26374}
\def\EQKPWithAttnScaleMedianMinFloat{-1.5879108041524887529050147350062616169452667236328125}
\def\EQKPWithAttnScaleMedianMinKey{19538}
\def\EQKPWithAttnScaleMedianStdDevFloat{0.29385867963290823734467949179816059768199920654296875}
\def\EQKPWithAttnScaleMinLen{151}
\def\EQKPWithAttnScaleMinMaxFloat{-0.1349039971828460693359375}
\def\EQKPWithAttnScaleMinMaxKey{26278}
\def\EQKPWithAttnScaleMinMeanFloat{-0.59349334239959716796875}
\def\EQKPWithAttnScaleMinMeanKey{519}
\def\EQKPWithAttnScaleMinMedianFloat{-1.56738150119781494140625}
\def\EQKPWithAttnScaleMinMedianKey{26374}
\def\EQKPWithAttnScaleMinMinFloat{-1.6263332366943359375}
\def\EQKPWithAttnScaleMinMinKey{19538}
\def\EQKPWithAttnScaleMinStdDevFloat{0.3223875463008880615234375}
\def\EQKPWithAttnScaleStdDevLen{151}
\def\EQKPWithAttnScaleStdDevMaxFloat{0.938620090484619140625}
\def\EQKPWithAttnScaleStdDevMaxKey{26374}
\def\EQKPWithAttnScaleStdDevMeanFloat{0.2770948112010955810546875}
\def\EQKPWithAttnScaleStdDevMeanKey{32382}
\def\EQKPWithAttnScaleStdDevMedianFloat{0.068847303278744220733642578125}
\def\EQKPWithAttnScaleStdDevMedianKey{24202}
\def\EQKPWithAttnScaleStdDevMinFloat{0.0604444257915019989013671875}
\def\EQKPWithAttnScaleStdDevMinKey{26278}
\def\EQKPWithAttnScaleStdDevStdDevFloat{0.1518141925334930419921875}
\def\EUPUAbsLenLen{151}
\def\EUPUAbsLenMaxFloat{4096}
\def\EUPUAbsLenMaxKey{50}
\def\EUPUAbsLenMeanFloat{4096}
\def\EUPUAbsLenMeanKey{50}
\def\EUPUAbsLenMedianFloat{4096}
\def\EUPUAbsLenMedianKey{50}
\def\EUPUAbsLenMinFloat{4096}
\def\EUPUAbsLenMinKey{50}
\def\EUPUAbsLenStdDevFloat{0}
\def\EUPUAbsMaxLen{151}
\def\EUPUAbsMaxMaxFloat{4.1362667083740234375}
\def\EUPUAbsMaxMaxKey{4810}
\def\EUPUAbsMaxMeanFloat{2.399017810821533203125}
\def\EUPUAbsMaxMeanKey{9132}
\def\EUPUAbsMaxMedianFloat{1.9738380014896392822265625}
\def\EUPUAbsMaxMedianKey{13468}
\def\EUPUAbsMaxMinFloat{1.909387111663818359375}
\def\EUPUAbsMaxMinKey{15399}
\def\EUPUAbsMaxStdDevFloat{0.2455985844135284423828125}
\def\EUPUAbsMeanLen{151}
\def\EUPUAbsMeanMaxFloat{1.04710865020751953125}
\def\EUPUAbsMeanMaxKey{28090}
\def\EUPUAbsMeanMeanFloat{0.84350109100341796875}
\def\EUPUAbsMeanMeanKey{1185}
\def\EUPUAbsMeanMedianFloat{0.64969213306903839111328125}
\def\EUPUAbsMeanMedianKey{30463}
\def\EUPUAbsMeanMinFloat{0.64810931682586669921875}
\def\EUPUAbsMeanMinKey{29726}
\def\EUPUAbsMeanStdDevFloat{0.0854190289974212646484375}
\def\EUPUAbsMedianLen{151}
\def\EUPUAbsMedianMaxFloat{0.0174738285131752525691783972661141888238489627838134765625}
\def\EUPUAbsMedianMaxKey{20539}
\def\EUPUAbsMedianMeanFloat{0.00990716090606254089212523439300639438442885875701904296875}
\def\EUPUAbsMedianMeanKey{8840}
\def\EUPUAbsMedianMedianFloat{0.005047069629654289159292890332153547205962240695953369140625}
\def\EUPUAbsMedianMedianKey{9134}
\def\EUPUAbsMedianMinFloat{0.004673839895986021432394696972778547205962240695953369140625}
\def\EUPUAbsMedianMinKey{29726}
\def\EUPUAbsMedianStdDevFloat{0.0026326126208305673966070248326332148280926048755645751953125}
\def\EUPUAbsMinLen{151}
\def\EUPUAbsMinMaxFloat{0.0040166391991078853607177734375}
\def\EUPUAbsMinMaxKey{20539}
\def\EUPUAbsMinMeanFloat{0.0004261823487468063831329345703125}
\def\EUPUAbsMinMeanKey{6155}
\def\EUPUAbsMinMedianFloat{0.000002620530864305692375637590885162353515625}
\def\EUPUAbsMinMedianKey{17197}
\def\EUPUAbsMinMinFloat{0.0000016808475038487813435494899749755859375}
\def\EUPUAbsMinMinKey{6159}
\def\EUPUAbsMinStdDevFloat{0.000526564544998109340667724609375}
\def\EUPUAbsStdDevLen{151}
\def\EUPUAbsStdDevMaxFloat{0.5831315517425537109375}
\def\EUPUAbsStdDevMaxKey{11611}
\def\EUPUAbsStdDevMeanFloat{0.46208488941192626953125}
\def\EUPUAbsStdDevMeanKey{24262}
\def\EUPUAbsStdDevMedianFloat{0.37492416799068450927734375}
\def\EUPUAbsStdDevMedianKey{19004}
\def\EUPUAbsStdDevMinFloat{0.361901819705963134765625}
\def\EUPUAbsStdDevMinKey{30463}
\def\EUPUAbsStdDevStdDevFloat{0.0418598316609859466552734375}
\def\EUPULenLen{151}
\def\EUPULenMaxFloat{4096}
\def\EUPULenMaxKey{50}
\def\EUPULenMeanFloat{4096}
\def\EUPULenMeanKey{50}
\def\EUPULenMedianFloat{4096}
\def\EUPULenMedianKey{50}
\def\EUPULenMinFloat{4096}
\def\EUPULenMinKey{50}
\def\EUPULenStdDevFloat{0}
\def\EUPUMaxLen{151}
\def\EUPUMaxMaxFloat{4.1362667083740234375}
\def\EUPUMaxMaxKey{4810}
\def\EUPUMaxMeanFloat{2.059669017791748046875}
\def\EUPUMaxMeanKey{2549}
\def\EUPUMaxMedianFloat{1.5914775431156158447265625}
\def\EUPUMaxMedianKey{19538}
\def\EUPUMaxMinFloat{1.52948033809661865234375}
\def\EUPUMaxMinKey{1412}
\def\EUPUMaxRowDiffLenLen{151}
\def\EUPUMaxRowDiffLenMaxFloat{64}
\def\EUPUMaxRowDiffLenMaxKey{50}
\def\EUPUMaxRowDiffLenMeanFloat{64}
\def\EUPUMaxRowDiffLenMeanKey{50}
\def\EUPUMaxRowDiffLenMedianFloat{64}
\def\EUPUMaxRowDiffLenMedianKey{50}
\def\EUPUMaxRowDiffLenMinFloat{64}
\def\EUPUMaxRowDiffLenMinKey{50}
\def\EUPUMaxRowDiffLenStdDevFloat{0}
\def\EUPUMaxRowDiffMaxLen{151}
\def\EUPUMaxRowDiffMaxMaxFloat{7.470183849334716796875}
\def\EUPUMaxRowDiffMaxMaxKey{4810}
\def\EUPUMaxRowDiffMaxMeanFloat{4.217689990997314453125}
\def\EUPUMaxRowDiffMaxMeanKey{24438}
\def\EUPUMaxRowDiffMaxMedianFloat{3.4847991466522216796875}
\def\EUPUMaxRowDiffMaxMedianKey{15399}
\def\EUPUMaxRowDiffMaxMinFloat{3.448888301849365234375}
\def\EUPUMaxRowDiffMaxMinKey{12561}
\def\EUPUMaxRowDiffMaxStdDevFloat{0.416750371456146240234375}
\def\EUPUMaxRowDiffMeanLen{151}
\def\EUPUMaxRowDiffMeanMaxFloat{3.76753520965576171875}
\def\EUPUMaxRowDiffMeanMaxKey{13716}
\def\EUPUMaxRowDiffMeanMeanFloat{3.1331183910369873046875}
\def\EUPUMaxRowDiffMeanMeanKey{29052}
\def\EUPUMaxRowDiffMeanMedianFloat{2.677449405193328857421875}
\def\EUPUMaxRowDiffMeanMedianKey{23633}
\def\EUPUMaxRowDiffMeanMinFloat{2.669384002685546875}
\def\EUPUMaxRowDiffMeanMinKey{29726}
\def\EUPUMaxRowDiffMeanStdDevFloat{0.21097107231616973876953125}
\def\EUPUMaxRowDiffMedianLen{151}
\def\EUPUMaxRowDiffMedianMaxFloat{3.022554600238799960010283029987476766109466552734375}
\def\EUPUMaxRowDiffMedianMaxKey{28090}
\def\EUPUMaxRowDiffMedianMeanFloat{2.468851190390965566479053450166247785091400146484375}
\def\EUPUMaxRowDiffMedianMeanKey{3254}
\def\EUPUMaxRowDiffMedianMedianFloat{2.03203177720308314491148848901502788066864013671875}
\def\EUPUMaxRowDiffMedianMedianKey{23633}
\def\EUPUMaxRowDiffMedianMinFloat{2.004540019035339515340865546022541821002960205078125}
\def\EUPUMaxRowDiffMedianMinKey{12552}
\def\EUPUMaxRowDiffMedianStdDevFloat{0.2279226955396611853377208944948506541550159454345703125}
\def\EUPUMaxRowDiffMinLen{151}
\def\EUPUMaxRowDiffMinMaxFloat{3.006002902984619140625}
\def\EUPUMaxRowDiffMinMaxKey{28090}
\def\EUPUMaxRowDiffMinMeanFloat{2.4370734691619873046875}
\def\EUPUMaxRowDiffMinMeanKey{11598}
\def\EUPUMaxRowDiffMinMedianFloat{1.9196160137653350830078125}
\def\EUPUMaxRowDiffMinMedianKey{7310}
\def\EUPUMaxRowDiffMinMinFloat{1.89183628559112548828125}
\def\EUPUMaxRowDiffMinMinKey{15622}
\def\EUPUMaxRowDiffMinStdDevFloat{0.238520145416259765625}
\def\EUPUMaxRowDiffStdDevLen{151}
\def\EUPUMaxRowDiffStdDevMaxFloat{0.692953288555145263671875}
\def\EUPUMaxRowDiffStdDevMaxKey{4810}
\def\EUPUMaxRowDiffStdDevMeanFloat{0.370445191860198974609375}
\def\EUPUMaxRowDiffStdDevMeanKey{15622}
\def\EUPUMaxRowDiffStdDevMedianFloat{0.2333082258701324462890625}
\def\EUPUMaxRowDiffStdDevMedianKey{15043}
\def\EUPUMaxRowDiffStdDevMinFloat{0.232532083988189697265625}
\def\EUPUMaxRowDiffStdDevMinKey{32382}
\def\EUPUMaxRowDiffStdDevStdDevFloat{0.082355819642543792724609375}
\def\EUPUMaxStdDevFloat{0.2637060582637786865234375}
\def\EUPUMeanLen{151}
\def\EUPUMeanMaxFloat{-0.30664670467376708984375}
\def\EUPUMeanMaxKey{19004}
\def\EUPUMeanMeanFloat{-0.5036513805389404296875}
\def\EUPUMeanMeanKey{15662}
\def\EUPUMeanMedianFloat{-0.677304208278656005859375}
\def\EUPUMeanMedianKey{24202}
\def\EUPUMeanMinFloat{-0.67830002307891845703125}
\def\EUPUMeanMinKey{11611}
\def\EUPUMeanStdDevFloat{0.072672091424465179443359375}
\def\EUPUMedianLen{151}
\def\EUPUMedianMaxFloat{-1.576497069001197903759248220012523233890533447265625}
\def\EUPUMedianMaxKey{19004}
\def\EUPUMedianMeanFloat{-1.9360142411577780929832215406349860131740570068359375}
\def\EUPUMedianMeanKey{7884}
\def\EUPUMedianMedianFloat{-2.212952874600887298583984375}
\def\EUPUMedianMedianKey{13716}
\def\EUPUMedianMinFloat{-2.236316645145416170947783029987476766109466552734375}
\def\EUPUMedianMinKey{4810}
\def\EUPUMedianStdDevFloat{0.1341368125361127316974574341656989417970180511474609375}
\def\EUPUMinLen{151}
\def\EUPUMinMaxFloat{-1.909387111663818359375}
\def\EUPUMinMaxKey{15399}
\def\EUPUMinMeanFloat{-2.3705823421478271484375}
\def\EUPUMinMeanKey{19093}
\def\EUPUMinMedianFloat{-3.066869437694549560546875}
\def\EUPUMinMedianKey{22261}
\def\EUPUMinMinFloat{-3.333917140960693359375}
\def\EUPUMinMinKey{4810}
\def\EUPUMinStdDevFloat{0.2246848642826080322265625}
\def\EUPUStdDevLen{151}
\def\EUPUStdDevMaxFloat{1.01130211353302001953125}
\def\EUPUStdDevMaxKey{30899}
\def\EUPUStdDevMeanFloat{0.81846141815185546875}
\def\EUPUStdDevMeanKey{14929}
\def\EUPUStdDevMedianFloat{0.64477603137493133544921875}
\def\EUPUStdDevMedianKey{30463}
\def\EUPUStdDevMinFloat{0.6321370601654052734375}
\def\EUPUStdDevMinKey{29726}
\def\EUPUStdDevStdDevFloat{0.072389371693134307861328125}
\def\EVOUHistMinAboveDiagDupBySeqCountLenLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMaxFloat{1152921504606846976}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMaxKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMeanFloat{1152921504606846976}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMeanKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMedianFloat{1152921504606846976}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMedianKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMinFloat{1152921504606846976}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMinKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountLenStdDevFloat{0}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMaxFloat{14.91612911224365234375}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMaxKey{742}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMeanFloat{11.78066349029541015625}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMeanKey{24438}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMedianFloat{8.55142688751220703125}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMedianKey{26829}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMinFloat{8.4827022552490234375}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMinKey{3284}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxStdDevFloat{1.2828505039215087890625}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMaxFloat{-8.81506749328383421016042120754718780517578125}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMaxKey{2549}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMeanFloat{-10.203741985816034087974912836216390132904052734375}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMeanKey{20294}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMedianFloat{-11.0814547059882233526195705053396522998809814453125}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMedianKey{24173}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMinFloat{-11.2407209841531976479700460913591086864471435546875}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMinKey{3175}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanStdDevFloat{0.43552439325024827621035683478112332522869110107421875}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMaxFloat{-8.316859849120874059735797345638275146484375}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMaxKey{8721}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMeanFloat{-10.4654229004566676763943178229965269565582275390625}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMeanKey{22545}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMedianFloat{-12.4552761531938482875148110906593501567840576171875}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMedianKey{5615}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMinFloat{-12.5176291175019098744769507902674376964569091796875}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMinKey{24173}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianStdDevFloat{0.7367895461838991355563166507636196911334991455078125}
\def\EVOUHistMinAboveDiagDupBySeqCountMinLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMaxFloat{-11.873058319091796875}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMaxKey{24566}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMeanFloat{-13.7037811279296875}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMeanKey{7238}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMedianFloat{-17.067573070526123046875}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMedianKey{6159}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMinFloat{-19.05162811279296875}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMinKey{2306}
\def\EVOUHistMinAboveDiagDupBySeqCountMinStdDevFloat{1.071216106414794921875}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMaxFloat{13}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMaxKey{2306}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMeanFloat{-3.079470198675496650508875973173417150974273681640625}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMeanKey{1185}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMedianFloat{-6}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMedianKey{1895}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMinFloat{-6}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMinKey{1895}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMaxFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMaxKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMeanFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMeanKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMedianFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMedianKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMinFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMinKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdStdDevFloat{0}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMaxFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMaxKey{2306}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMeanFloat{0.98906411398325533301800760455080308020114898681640625}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMeanKey{24262}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMedianFloat{0.9429553449153900146484375}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMedianKey{26829}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMinFloat{0.939621269702911376953125}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMinKey{25516}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracStdDevFloat{0.01244573615258662106775044975393029744736850261688232421875}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueStdDevFloat{2.351618236147627438725749016157351434230804443359375}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMaxFloat{11.6516310054191887246588521520607173442840576171875}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMaxKey{24173}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMeanFloat{10.3611648845346966396618881844915449619293212890625}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMeanKey{4157}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMedianFloat{8.791562358726093151517488877288997173309326171875}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMedianKey{26829}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMinFloat{8.7376256487958432472851200145669281482696533203125}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMinKey{9132}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevStdDevFloat{0.53452869051782891940405306741013191640377044677734375}
\def\EVOUHistMinAboveDiagLenLen{151}
\def\EVOUHistMinAboveDiagLenMaxFloat{64}
\def\EVOUHistMinAboveDiagLenMaxKey{50}
\def\EVOUHistMinAboveDiagLenMeanFloat{64}
\def\EVOUHistMinAboveDiagLenMeanKey{50}
\def\EVOUHistMinAboveDiagLenMedianFloat{64}
\def\EVOUHistMinAboveDiagLenMedianKey{50}
\def\EVOUHistMinAboveDiagLenMinFloat{64}
\def\EVOUHistMinAboveDiagLenMinKey{50}
\def\EVOUHistMinAboveDiagLenStdDevFloat{0}
\def\EVOUHistMinAboveDiagMaxLen{151}
\def\EVOUHistMinAboveDiagMaxMaxFloat{14.91612911224365234375}
\def\EVOUHistMinAboveDiagMaxMaxKey{742}
\def\EVOUHistMinAboveDiagMaxMeanFloat{11.78066349029541015625}
\def\EVOUHistMinAboveDiagMaxMeanKey{24438}
\def\EVOUHistMinAboveDiagMaxMedianFloat{8.55142688751220703125}
\def\EVOUHistMinAboveDiagMaxMedianKey{26829}
\def\EVOUHistMinAboveDiagMaxMinFloat{8.4827022552490234375}
\def\EVOUHistMinAboveDiagMaxMinKey{3284}
\def\EVOUHistMinAboveDiagMaxStdDevFloat{1.2828505039215087890625}
\def\EVOUHistMinAboveDiagMeanLen{151}
\def\EVOUHistMinAboveDiagMeanMaxFloat{0.891056954860687255859375}
\def\EVOUHistMinAboveDiagMeanMaxKey{1412}
\def\EVOUHistMinAboveDiagMeanMeanFloat{-0.1685074865818023681640625}
\def\EVOUHistMinAboveDiagMeanMeanKey{26932}
\def\EVOUHistMinAboveDiagMeanMedianFloat{-1.4760489165782928466796875}
\def\EVOUHistMinAboveDiagMeanMedianKey{3284}
\def\EVOUHistMinAboveDiagMeanMinFloat{-1.47888123989105224609375}
\def\EVOUHistMinAboveDiagMeanMinKey{26829}
\def\EVOUHistMinAboveDiagMeanStdDevFloat{0.4688076078891754150390625}
\def\EVOUHistMinAboveDiagMedianLen{151}
\def\EVOUHistMinAboveDiagMedianMaxFloat{0.802640438079833984375}
\def\EVOUHistMinAboveDiagMedianMaxKey{5781}
\def\EVOUHistMinAboveDiagMedianMeanFloat{-1.2123439390927750469728607640718109905719757080078125}
\def\EVOUHistMinAboveDiagMedianMeanKey{5358}
\def\EVOUHistMinAboveDiagMedianMedianFloat{-2.94434583187103271484375}
\def\EVOUHistMinAboveDiagMedianMedianKey{30371}
\def\EVOUHistMinAboveDiagMedianMinFloat{-3.10355281829833984375}
\def\EVOUHistMinAboveDiagMedianMinKey{27714}
\def\EVOUHistMinAboveDiagMedianStdDevFloat{0.916071035835220204290862966445274651050567626953125}
\def\EVOUHistMinAboveDiagMinLen{151}
\def\EVOUHistMinAboveDiagMinMaxFloat{-11.873058319091796875}
\def\EVOUHistMinAboveDiagMinMaxKey{24566}
\def\EVOUHistMinAboveDiagMinMeanFloat{-13.7037811279296875}
\def\EVOUHistMinAboveDiagMinMeanKey{7238}
\def\EVOUHistMinAboveDiagMinMedianFloat{-17.067573070526123046875}
\def\EVOUHistMinAboveDiagMinMedianKey{6159}
\def\EVOUHistMinAboveDiagMinMinFloat{-19.05162811279296875}
\def\EVOUHistMinAboveDiagMinMinKey{2306}
\def\EVOUHistMinAboveDiagMinStdDevFloat{1.071216106414794921875}
\def\EVOUHistMinAboveDiagMostBelowValueLen{151}
\def\EVOUHistMinAboveDiagMostBelowValueMaxFloat{75}
\def\EVOUHistMinAboveDiagMostBelowValueMaxKey{18289}
\def\EVOUHistMinAboveDiagMostBelowValueMeanFloat{56.76158940397350960438416223041713237762451171875}
\def\EVOUHistMinAboveDiagMostBelowValueMeanKey{1895}
\def\EVOUHistMinAboveDiagMostBelowValueMedianFloat{41}
\def\EVOUHistMinAboveDiagMostBelowValueMedianKey{19538}
\def\EVOUHistMinAboveDiagMostBelowValueMinFloat{41}
\def\EVOUHistMinAboveDiagMostBelowValueMinKey{19538}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdLen{151}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMaxFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMaxKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMeanFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMeanKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMedianFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMedianKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMinFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMinKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdStdDevFloat{0}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracLen{151}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMaxFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMaxKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMeanFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMeanKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMedianFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMedianKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMinFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMinKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracStdDevFloat{0}
\def\EVOUHistMinAboveDiagMostBelowValueStdDevFloat{6.54551927958033896715051014325581490993499755859375}
\def\EVOUHistMinAboveDiagStdDevLen{151}
\def\EVOUHistMinAboveDiagStdDevMaxFloat{8.63927555084228515625}
\def\EVOUHistMinAboveDiagStdDevMaxKey{18289}
\def\EVOUHistMinAboveDiagStdDevMeanFloat{7.56669712066650390625}
\def\EVOUHistMinAboveDiagStdDevMeanKey{27671}
\def\EVOUHistMinAboveDiagStdDevMedianFloat{6.485137462615966796875}
\def\EVOUHistMinAboveDiagStdDevMedianKey{4810}
\def\EVOUHistMinAboveDiagStdDevMinFloat{6.42694568634033203125}
\def\EVOUHistMinAboveDiagStdDevMinKey{19538}
\def\EVOUHistMinAboveDiagStdDevStdDevFloat{0.4137505590915679931640625}
\def\EVOUMaxRowDiffLenLen{151}
\def\EVOUMaxRowDiffLenMaxFloat{64}
\def\EVOUMaxRowDiffLenMaxKey{50}
\def\EVOUMaxRowDiffLenMeanFloat{64}
\def\EVOUMaxRowDiffLenMeanKey{50}
\def\EVOUMaxRowDiffLenMedianFloat{64}
\def\EVOUMaxRowDiffLenMedianKey{50}
\def\EVOUMaxRowDiffLenMinFloat{64}
\def\EVOUMaxRowDiffLenMinKey{50}
\def\EVOUMaxRowDiffLenStdDevFloat{0}
\def\EVOUMaxRowDiffMaxLen{151}
\def\EVOUMaxRowDiffMaxMaxFloat{83.601715087890625}
\def\EVOUMaxRowDiffMaxMaxKey{6589}
\def\EVOUMaxRowDiffMaxMeanFloat{65.87128448486328125}
\def\EVOUMaxRowDiffMaxMeanKey{15662}
\def\EVOUMaxRowDiffMaxMedianFloat{53.589984893798828125}
\def\EVOUMaxRowDiffMaxMedianKey{29726}
\def\EVOUMaxRowDiffMaxMinFloat{51.893421173095703125}
\def\EVOUMaxRowDiffMaxMinKey{11124}
\def\EVOUMaxRowDiffMaxStdDevFloat{5.896025180816650390625}
\def\EVOUMaxRowDiffMeanLen{151}
\def\EVOUMaxRowDiffMeanMaxFloat{41.444854736328125}
\def\EVOUMaxRowDiffMeanMaxKey{742}
\def\EVOUMaxRowDiffMeanMeanFloat{34.20511627197265625}
\def\EVOUMaxRowDiffMeanMeanKey{28716}
\def\EVOUMaxRowDiffMeanMedianFloat{27.107979297637939453125}
\def\EVOUMaxRowDiffMeanMedianKey{3284}
\def\EVOUMaxRowDiffMeanMinFloat{26.8407154083251953125}
\def\EVOUMaxRowDiffMeanMinKey{4810}
\def\EVOUMaxRowDiffMeanStdDevFloat{2.5496234893798828125}
\def\EVOUMaxRowDiffMedianLen{151}
\def\EVOUMaxRowDiffMedianMaxFloat{29.121360073089601172569018672220408916473388671875}
\def\EVOUMaxRowDiffMedianMaxKey{26932}
\def\EVOUMaxRowDiffMedianMeanFloat{22.1070556920095810937709757126867771148681640625}
\def\EVOUMaxRowDiffMedianMeanKey{6082}
\def\EVOUMaxRowDiffMedianMedianFloat{14.268889118432998230900921043939888477325439453125}
\def\EVOUMaxRowDiffMedianMedianKey{3284}
\def\EVOUMaxRowDiffMedianMinFloat{13.54591596126556396484375}
\def\EVOUMaxRowDiffMedianMinKey{4810}
\def\EVOUMaxRowDiffMedianStdDevFloat{2.68050750359481337881106810527853667736053466796875}
\def\EVOUMaxRowDiffMinLen{151}
\def\EVOUMaxRowDiffMinMaxFloat{29.0986480712890625}
\def\EVOUMaxRowDiffMinMaxKey{26932}
\def\EVOUMaxRowDiffMinMeanFloat{21.489070892333984375}
\def\EVOUMaxRowDiffMinMeanKey{30899}
\def\EVOUMaxRowDiffMinMedianFloat{13.5225489139556884765625}
\def\EVOUMaxRowDiffMinMedianKey{3284}
\def\EVOUMaxRowDiffMinMinFloat{12.37885570526123046875}
\def\EVOUMaxRowDiffMinMinKey{4810}
\def\EVOUMaxRowDiffMinStdDevFloat{2.8791592121124267578125}
\def\EVOUMaxRowDiffStdDevLen{151}
\def\EVOUMaxRowDiffStdDevMaxFloat{13.90869903564453125}
\def\EVOUMaxRowDiffStdDevMaxKey{6589}
\def\EVOUMaxRowDiffStdDevMeanFloat{8.9337062835693359375}
\def\EVOUMaxRowDiffStdDevMeanKey{13468}
\def\EVOUMaxRowDiffStdDevMedianFloat{6.677680492401123046875}
\def\EVOUMaxRowDiffStdDevMedianKey{13654}
\def\EVOUMaxRowDiffStdDevMinFloat{6.526166439056396484375}
\def\EVOUMaxRowDiffStdDevMinKey{22261}
\def\EVOUMaxRowDiffStdDevStdDevFloat{1.02128326892852783203125}
\def\ImportanceSamplingAccuracyLen{151}
\def\ImportanceSamplingAccuracyMaxFloat{0.999574198846924222294774153851903975009918212890625}
\def\ImportanceSamplingAccuracyMaxKey{32374}
\def\ImportanceSamplingAccuracyMeanFloat{0.99880046824179224973505597517942078411579132080078125}
\def\ImportanceSamplingAccuracyMeanKey{20976}
\def\ImportanceSamplingAccuracyMedianFloat{0.9909756464333592251847449006163515150547027587890625}
\def\ImportanceSamplingAccuracyMedianKey{5781}
\def\ImportanceSamplingAccuracyMinFloat{0.9861113271708623617683997508720494806766510009765625}
\def\ImportanceSamplingAccuracyMinKey{4810}
\def\ImportanceSamplingAccuracyStdDevFloat{0.0013393070473378099714822919708012705086730420589447021484375}
\def\ImportanceSamplingBatchSize{4096}
\def\ImportanceSamplingInstructionCountBranch{0}
\def\ImportanceSamplingInstructionCountInt{0}
\def\ImportanceSamplingInstructionCount{0}
\def\ImportanceSamplingLossLen{151}
\def\ImportanceSamplingLossMaxFloat{0.041087809933881801194299754342864616774022579193115234375}
\def\ImportanceSamplingLossMaxKey{4810}
\def\ImportanceSamplingLossMeanFloat{0.004573984575460143635339260725913845817558467388153076171875}
\def\ImportanceSamplingLossMeanKey{13468}
\def\ImportanceSamplingLossMedianFloat{0.0021796727269319999577279478586433469899930059909820556640625}
\def\ImportanceSamplingLossMedianKey{8048}
\def\ImportanceSamplingLossMinFloat{0.002041580203265999822470622149239716236479580402374267578125}
\def\ImportanceSamplingLossMinKey{7310}
\def\ImportanceSamplingLossStdDevFloat{0.00391093786991324188218044355380698107182979583740234375}
\def\ImportanceSamplingNSamplesPerKey{10}
\def\ImportanceSamplingNumCorrectLen{151}
\def\ImportanceSamplingNumCorrectMaxFloat{6348815}
\def\ImportanceSamplingNumCorrectMaxKey{519}
\def\ImportanceSamplingNumCorrectMeanFloat{6156698.821192053146660327911376953125}
\def\ImportanceSamplingNumCorrectMeanKey{8893}
\def\ImportanceSamplingNumCorrectMedianFloat{5923417}
\def\ImportanceSamplingNumCorrectMedianKey{5781}
\def\ImportanceSamplingNumCorrectMinFloat{5892595}
\def\ImportanceSamplingNumCorrectMinKey{7884}
\def\ImportanceSamplingNumCorrectStdDevFloat{90906.129735046546556986868381500244140625}
\def\ImportanceSamplingNumIncorrectLen{151}
\def\ImportanceSamplingNumIncorrectMaxFloat{1028439}
\def\ImportanceSamplingNumIncorrectMaxKey{7884}
\def\ImportanceSamplingNumIncorrectMeanFloat{764335.178807946969754993915557861328125}
\def\ImportanceSamplingNumIncorrectMeanKey{8893}
\def\ImportanceSamplingNumIncorrectMedianFloat{592871}
\def\ImportanceSamplingNumIncorrectMedianKey{32374}
\def\ImportanceSamplingNumIncorrectMinFloat{572219}
\def\ImportanceSamplingNumIncorrectMinKey{519}
\def\ImportanceSamplingNumIncorrectStdDevFloat{90906.129735046546556986868381500244140625}
\def\ImportanceSamplingTimeLen{151}
\def\ImportanceSamplingTimeMaxFloat{302.907425403594970703125}
\def\ImportanceSamplingTimeMaxKey{29726}
\def\ImportanceSamplingTimeMeanFloat{251.994913243300089789045159704983234405517578125}
\def\ImportanceSamplingTimeMeanKey{3284}
\def\ImportanceSamplingTimeMedianFloat{198.984722256660489847490680404007434844970703125}
\def\ImportanceSamplingTimeMedianKey{18668}
\def\ImportanceSamplingTimeMinFloat{87.3364048004150390625}
\def\ImportanceSamplingTimeMinKey{123}
\def\ImportanceSamplingTimeStdDevFloat{18.147854262937475056105540716089308261871337890625}
\def\ImportanceSamplingTotalSequences{6921034}
\def\LowerWhiskerBottomEndPercentileFloat{0.02151239536919476169618548055950668640434741973876953125}
\def\LowerWhiskerCrosshatchPercentileFloat{0.08867177532617598334496733514242805540561676025390625}
\def\MedianPercentileFloat{0.5}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffExactLinearFitIntercept{0.35405332832977276513730657825362868607044219970703125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffExactLinearFitRSquared{0.00000037662278462580189852815237827599048614501953125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffExactLinearFitSlope{-0.0000007404302114799278533653127155889084320961046614684164524078369140625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffLinearFitIntercept{0.34965295462309498031316934429924003779888153076171875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffLinearFitRSquared{0.0000270814856511147894480018294416368007659912109375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffLinearFitSlope{-0.00000611474378612610657891292265109228765140869654715061187744140625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductLinearFitIntercept{0.352875413822907935124106870716786943376064300537109375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductLinearFitRSquared{0.0000189352166286571588216247619129717350006103515625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductLinearFitSlope{-0.0000051724954513404171853254050195136670708961901254951953887939453125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitIntercept{0.2116687922460222803788809642355772666633129119873046875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitRSquared{0.00000000920381892921540156748960725963115692138671875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitSlope{-0.0000000693062211580625878647201579436931684341516302083618938922882080078125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffLinearFitIntercept{0.349388590903735696269194477281416766345500946044921875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffLinearFitRSquared{0.000025204970394820946921754512004554271697998046875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffLinearFitSlope{-0.0000058982184581756241908956882313841418863376020453870296478271484375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitIntercept{0.352829869643027593806294817113666795194149017333984375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitRSquared{0.0000187792000332365205395035445690155029296875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitSlope{-0.000005151234913858714198060632927234081535061704926192760467529296875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitIntercept{0.2114813270010537926690830090592498891055583953857421875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitRSquared{0.0000000064097844809651860487065277993679046630859375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitSlope{0.00000005781118074429962827218064890487381202177630257210694253444671630859375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitIntercept{0.2092372471455429538966797053944901563227176666259765625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitRSquared{0.00000036241287471039385081894579343497753143310546875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitSlope{0.0000004306882956170298951231972632569533487867374788038432598114013671875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioSvdLinearFitIntercept{0.278398604217542755545622412682860158383846282958984375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioSvdLinearFitRSquared{0.0010089606187089206201790148043073713779449462890625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioSvdLinearFitSlope{0.00003377585277548224968434398274297336683957837522029876708984375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffExactLinearFitIntercept{0.66286381919569858922614002949558198451995849609375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffExactLinearFitRSquared{0.001008528840198863463228917680680751800537109375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffExactLinearFitSlope{0.000004091450860325805891624419141638924202197813428938388824462890625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffLinearFitIntercept{0.64576617024854610082940098436665721237659454345703125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffLinearFitRSquared{0.00142497126275664687256039542262442409992218017578125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffLinearFitSlope{0.0000045347580982770301910177342119556698207816225476562976837158203125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductLinearFitIntercept{0.6527080951987824786186820347211323678493499755859375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductLinearFitRSquared{0.0012717006673568231889248636434786021709442138671875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductLinearFitSlope{0.000004367551549412935143622445377520335796361905522644519805908203125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitIntercept{0.393308095092535670023181637589004822075366973876953125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitRSquared{0.00025212981419941993266320423572324216365814208984375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitSlope{0.00000207110584273470766956200435349177979560408857651054859161376953125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffLinearFitIntercept{0.64562222440872840678594002383761107921600341796875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffLinearFitRSquared{0.0013229667900116481860095518641173839569091796875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffLinearFitSlope{0.00000433433744210281733677016247074931243332684971392154693603515625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitIntercept{0.6525160887683674193482374903396703302860260009765625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitRSquared{0.00148654297692629722149604276637546718120574951171875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitSlope{0.0000047400661974662923077157399009973204329071450047194957733154296875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitIntercept{0.393839296656614379354977018010686151683330535888671875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitRSquared{0.00016241537190431198922624389524571597576141357421875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitSlope{0.000001642992965911702409685765831348636112352323834784328937530517578125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitIntercept{0.39044131973568585447509349251049570739269256591796875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitRSquared{0.00005683281383295213373685328406281769275665283203125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitSlope{0.000000954720251532834571485896212050814568783607683144509792327880859375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioSvdLinearFitIntercept{0.51353410378286301618544484881567768752574920654296875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioSvdLinearFitRSquared{0.234165186982087991651724223629571497440338134765625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioSvdLinearFitSlope{0.000074331704732941250948242972729218536187545396387577056884765625}
\def\NumSeeds{151}
\def\PVOUAbsLenLen{151}
\def\PVOUAbsLenMaxFloat{640}
\def\PVOUAbsLenMaxKey{50}
\def\PVOUAbsLenMeanFloat{640}
\def\PVOUAbsLenMeanKey{50}
\def\PVOUAbsLenMedianFloat{640}
\def\PVOUAbsLenMedianKey{50}
\def\PVOUAbsLenMinFloat{640}
\def\PVOUAbsLenMinKey{50}
\def\PVOUAbsLenStdDevFloat{0}
\def\PVOUAbsMaxLen{151}
\def\PVOUAbsMaxMaxFloat{2.505237102508544921875}
\def\PVOUAbsMaxMaxKey{1951}
\def\PVOUAbsMaxMeanFloat{1.50908434391021728515625}
\def\PVOUAbsMaxMeanKey{12457}
\def\PVOUAbsMaxMedianFloat{0.98432330787181854248046875}
\def\PVOUAbsMaxMedianKey{19451}
\def\PVOUAbsMaxMinFloat{0.920002996921539306640625}
\def\PVOUAbsMaxMinKey{17194}
\def\PVOUAbsMaxStdDevFloat{0.3310389220714569091796875}
\def\PVOUAbsMeanLen{151}
\def\PVOUAbsMeanMaxFloat{0.398436844348907470703125}
\def\PVOUAbsMeanMaxKey{19093}
\def\PVOUAbsMeanMeanFloat{0.2919519245624542236328125}
\def\PVOUAbsMeanMeanKey{4729}
\def\PVOUAbsMeanMedianFloat{0.2053053863346576690673828125}
\def\PVOUAbsMeanMedianKey{19488}
\def\PVOUAbsMeanMinFloat{0.18469803035259246826171875}
\def\PVOUAbsMeanMinKey{16197}
\def\PVOUAbsMeanStdDevFloat{0.0397930145263671875}
\def\PVOUAbsMedianLen{151}
\def\PVOUAbsMedianMaxFloat{0.00900987528264522545551340471092771622352302074432373046875}
\def\PVOUAbsMedianMaxKey{32382}
\def\PVOUAbsMedianMeanFloat{0.0028871116867375296206887913541550005902536213397979736328125}
\def\PVOUAbsMedianMeanKey{26278}
\def\PVOUAbsMedianMedianFloat{0.000666736811399459903919317849130266040447168052196502685546875}
\def\PVOUAbsMedianMedianKey{28716}
\def\PVOUAbsMedianMinFloat{0.00052343130111694342876393903907228377647697925567626953125}
\def\PVOUAbsMedianMinKey{7790}
\def\PVOUAbsMedianStdDevFloat{0.001533534166034335177730696386788622476160526275634765625}
\def\PVOUAbsMinLen{151}
\def\PVOUAbsMinMaxFloat{0.0039626061916351318359375}
\def\PVOUAbsMinMaxKey{13036}
\def\PVOUAbsMinMeanFloat{0.000704278587363660335540771484375}
\def\PVOUAbsMinMeanKey{2345}
\def\PVOUAbsMinMedianFloat{0.0000018179416656494140625}
\def\PVOUAbsMinMedianKey{4810}
\def\PVOUAbsMinMinFloat{0.00000011920928955078125}
\def\PVOUAbsMinMinKey{5615}
\def\PVOUAbsMinStdDevFloat{0.00072550238110125064849853515625}
\def\PVOUAbsStdDevLen{151}
\def\PVOUAbsStdDevMaxFloat{0.340394675731658935546875}
\def\PVOUAbsStdDevMaxKey{1951}
\def\PVOUAbsStdDevMeanFloat{0.23625850677490234375}
\def\PVOUAbsStdDevMeanKey{13468}
\def\PVOUAbsStdDevMedianFloat{0.1666869409382343292236328125}
\def\PVOUAbsStdDevMedianKey{7467}
\def\PVOUAbsStdDevMinFloat{0.161654770374298095703125}
\def\PVOUAbsStdDevMinKey{17194}
\def\PVOUAbsStdDevStdDevFloat{0.032588958740234375}
\def\PVOULenLen{151}
\def\PVOULenMaxFloat{640}
\def\PVOULenMaxKey{50}
\def\PVOULenMeanFloat{640}
\def\PVOULenMeanKey{50}
\def\PVOULenMedianFloat{640}
\def\PVOULenMedianKey{50}
\def\PVOULenMinFloat{640}
\def\PVOULenMinKey{50}
\def\PVOULenStdDevFloat{0}
\def\PVOUMaxLen{151}
\def\PVOUMaxMaxFloat{2.505237102508544921875}
\def\PVOUMaxMaxKey{1951}
\def\PVOUMaxMeanFloat{1.382044315338134765625}
\def\PVOUMaxMeanKey{13654}
\def\PVOUMaxMedianFloat{0.78875462710857391357421875}
\def\PVOUMaxMedianKey{17194}
\def\PVOUMaxMinFloat{0.7590711116790771484375}
\def\PVOUMaxMinKey{20294}
\def\PVOUMaxRowDiffLenLen{151}
\def\PVOUMaxRowDiffLenMaxFloat{10}
\def\PVOUMaxRowDiffLenMaxKey{50}
\def\PVOUMaxRowDiffLenMeanFloat{10}
\def\PVOUMaxRowDiffLenMeanKey{50}
\def\PVOUMaxRowDiffLenMedianFloat{10}
\def\PVOUMaxRowDiffLenMedianKey{50}
\def\PVOUMaxRowDiffLenMinFloat{10}
\def\PVOUMaxRowDiffLenMinKey{50}
\def\PVOUMaxRowDiffLenStdDevFloat{0}
\def\PVOUMaxRowDiffMaxLen{151}
\def\PVOUMaxRowDiffMaxMaxFloat{4.970876216888427734375}
\def\PVOUMaxRowDiffMaxMaxKey{1951}
\def\PVOUMaxRowDiffMaxMeanFloat{2.72969913482666015625}
\def\PVOUMaxRowDiffMaxMeanKey{28778}
\def\PVOUMaxRowDiffMaxMedianFloat{1.770168602466583251953125}
\def\PVOUMaxRowDiffMaxMedianKey{7467}
\def\PVOUMaxRowDiffMaxMinFloat{1.66566562652587890625}
\def\PVOUMaxRowDiffMaxMinKey{17194}
\def\PVOUMaxRowDiffMaxStdDevFloat{0.6015903949737548828125}
\def\PVOUMaxRowDiffMeanLen{151}
\def\PVOUMaxRowDiffMeanMaxFloat{2.1749210357666015625}
\def\PVOUMaxRowDiffMeanMaxKey{28090}
\def\PVOUMaxRowDiffMeanMeanFloat{1.60400593280792236328125}
\def\PVOUMaxRowDiffMeanMeanKey{27300}
\def\PVOUMaxRowDiffMeanMedianFloat{1.1662960946559906005859375}
\def\PVOUMaxRowDiffMeanMedianKey{17194}
\def\PVOUMaxRowDiffMeanMinFloat{1.12469422817230224609375}
\def\PVOUMaxRowDiffMeanMinKey{7467}
\def\PVOUMaxRowDiffMeanStdDevFloat{0.191579163074493408203125}
\def\PVOUMaxRowDiffMedianLen{151}
\def\PVOUMaxRowDiffMedianMaxFloat{1.6024084532260893798394363329862244427204132080078125}
\def\PVOUMaxRowDiffMedianMaxKey{2549}
\def\PVOUMaxRowDiffMedianMeanFloat{0.92760563143041740996608268687850795686244964599609375}
\def\PVOUMaxRowDiffMedianMeanKey{12493}
\def\PVOUMaxRowDiffMedianMedianFloat{0.4549935555458068936474091970012523233890533447265625}
\def\PVOUMaxRowDiffMedianMedianKey{23447}
\def\PVOUMaxRowDiffMedianMinFloat{0.44858604073524477318102299250313080847263336181640625}
\def\PVOUMaxRowDiffMedianMinKey{20751}
\def\PVOUMaxRowDiffMedianStdDevFloat{0.19186240471755500180961462319828569889068603515625}
\def\PVOUMaxRowDiffMinLen{151}
\def\PVOUMaxRowDiffMinMaxFloat{1.59651947021484375}
\def\PVOUMaxRowDiffMinMaxKey{2549}
\def\PVOUMaxRowDiffMinMeanFloat{0.919437825679779052734375}
\def\PVOUMaxRowDiffMinMeanKey{15043}
\def\PVOUMaxRowDiffMinMedianFloat{0.4266707897186279296875}
\def\PVOUMaxRowDiffMinMedianKey{20751}
\def\PVOUMaxRowDiffMinMinFloat{0.422105312347412109375}
\def\PVOUMaxRowDiffMinMinKey{23447}
\def\PVOUMaxRowDiffMinStdDevFloat{0.1949186027050018310546875}
\def\PVOUMaxRowDiffStdDevLen{151}
\def\PVOUMaxRowDiffStdDevMaxFloat{1.0294682979583740234375}
\def\PVOUMaxRowDiffStdDevMaxKey{1951}
\def\PVOUMaxRowDiffStdDevMeanFloat{0.525887012481689453125}
\def\PVOUMaxRowDiffStdDevMeanKey{12493}
\def\PVOUMaxRowDiffStdDevMedianFloat{0.272195778787136077880859375}
\def\PVOUMaxRowDiffStdDevMedianKey{16149}
\def\PVOUMaxRowDiffStdDevMinFloat{0.2593893706798553466796875}
\def\PVOUMaxRowDiffStdDevMinKey{24262}
\def\PVOUMaxRowDiffStdDevStdDevFloat{0.1558911502361297607421875}
\def\PVOUMaxStdDevFloat{0.337821304798126220703125}
\def\PVOUMeanLen{151}
\def\PVOUMeanMaxFloat{0.000000034272670035306873614899814128875732421875}
\def\PVOUMeanMaxKey{7884}
\def\PVOUMeanMeanFloat{0.000000000595799798386309475972666405141353607177734375}
\def\PVOUMeanMeanKey{3175}
\def\PVOUMeanMedianFloat{-0.0000000257045034146585749113000929355621337890625}
\def\PVOUMeanMedianKey{24566}
\def\PVOUMeanMinFloat{-0.000000026822089438383045489899814128875732421875}
\def\PVOUMeanMinKey{24438}
\def\PVOUMeanStdDevFloat{0.0000000128231594231920098536647856235504150390625}
\def\PVOUMedianLen{151}
\def\PVOUMedianMaxFloat{-0.66008410334587097612057959850062616169452667236328125}
\def\PVOUMedianMaxKey{7467}
\def\PVOUMedianMeanFloat{-1.0207504598115451077688931036391295492649078369140625}
\def\PVOUMedianMeanKey{13293}
\def\PVOUMedianMedianFloat{-1.4690441016852855415919520964962430298328399658203125}
\def\PVOUMedianMedianKey{1951}
\def\PVOUMedianMinFloat{-1.4835610193014143742828991889837197959423065185546875}
\def\PVOUMedianMinKey{29725}
\def\PVOUMedianStdDevFloat{0.1623978880471395047635496666771359741687774658203125}
\def\PVOUMinLen{151}
\def\PVOUMinMaxFloat{-0.711409270763397216796875}
\def\PVOUMinMaxKey{7467}
\def\PVOUMinMeanFloat{-1.40715515613555908203125}
\def\PVOUMinMeanKey{742}
\def\PVOUMinMedianFloat{-2.28925669193267822265625}
\def\PVOUMinMedianKey{29565}
\def\PVOUMinMinFloat{-2.4656391143798828125}
\def\PVOUMinMinKey{1951}
\def\PVOUMinStdDevFloat{0.3066748678684234619140625}
\def\PVOUStdDevLen{151}
\def\PVOUStdDevMaxFloat{0.5196750164031982421875}
\def\PVOUStdDevMaxKey{1951}
\def\PVOUStdDevMeanFloat{0.375869095325469970703125}
\def\PVOUStdDevMeanKey{4729}
\def\PVOUStdDevMedianFloat{0.263714961707592010498046875}
\def\PVOUStdDevMedianKey{17194}
\def\PVOUStdDevMinFloat{0.2535533905029296875}
\def\PVOUStdDevMinKey{16197}
\def\PVOUStdDevStdDevFloat{0.049213491380214691162109375}
\def\ProofFlopEstimateAllSubcubicMean{6440064.799999999813735485076904296875}
\def\ProofFlopEstimateAllSubcubicStdDev{795901.845153527916409075260162353515625}
\def\ProofFlopEstimateAlmostQuadraticMean{5542546.666666666977107524871826171875}
\def\ProofFlopEstimateAlmostQuadraticStdDev{55534.9518930927515611983835697174072265625}
\def\ProofFlopEstimateMainlySubcubicMean{6564605.96153846196830272674560546875}
\def\ProofFlopEstimateMainlySubcubicStdDev{752640.100030499626882374286651611328125}
\def\QuartileOnePercentileFloat{0.25}
\def\QuartileThreePercentileFloat{0.75}
\def\RealSubcubicAccuracyLen{15100}
\def\RealSubcubicAccuracyMaxFloat{0.73561759633376000433457875260501168668270111083984375}
\def\RealSubcubicAccuracyMeanFloat{0.303314539339781863436229514263686724007129669189453125}
\def\RealSubcubicAccuracyMedianFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\RealSubcubicAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\RealSubcubicAccuracyStdDevFloat{0.2432615807237808180918392508829128928482532501220703125}
\def\RealSubcubicDroppedSequencesFracLen{15100}
\def\RealSubcubicDroppedSequencesFracMaxFloat{0.46377977035578010767125078928074799478054046630859375}
\def\RealSubcubicDroppedSequencesFracMeanFloat{0.1621743713089575378294426855063647963106632232666015625}
\def\RealSubcubicDroppedSequencesFracMedianFloat{0}
\def\RealSubcubicDroppedSequencesFracMinFloat{0}
\def\RealSubcubicDroppedSequencesFracStdDevFloat{0.12409221244347089230242175972307450138032436370849609375}
\def\RealSubcubicDroppedSequencesLen{15100}
\def\RealSubcubicDroppedSequencesMaxFloat{534701670644804012}
\def\RealSubcubicDroppedSequencesMeanFloat{186974320178192832}
\def\RealSubcubicDroppedSequencesMedianFloat{0}
\def\RealSubcubicDroppedSequencesMinFloat{0}
\def\RealSubcubicDroppedSequencesStdDevFloat{143068580280318976}
\def\RealSubcubicEffectiveDimensionalityEstimateLen{15100}
\def\RealSubcubicEffectiveDimensionalityEstimateMaxFloat{10370}
\def\RealSubcubicEffectiveDimensionalityEstimateMeanFloat{6049.600000000000363797880709171295166015625}
\def\RealSubcubicEffectiveDimensionalityEstimateMedianFloat{4290}
\def\RealSubcubicEffectiveDimensionalityEstimateMinFloat{4290}
\def\RealSubcubicEffectiveDimensionalityEstimateStdDevFloat{1530.49032666005450664670206606388092041015625}
\def\RealSubcubicErrUpperBoundLen{15100}
\def\RealSubcubicErrUpperBoundMaxFloat{156.4159393310546875}
\def\RealSubcubicErrUpperBoundMeanFloat{31.734276126946834750697234994731843471527099609375}
\def\RealSubcubicErrUpperBoundMedianFloat{0}
\def\RealSubcubicErrUpperBoundMinFloat{0}
\def\RealSubcubicErrUpperBoundStdDevFloat{39.7595860426961138500701053999364376068115234375}
\def\RealSubcubicGapMostBelowValueLen{15100}
\def\RealSubcubicGapMostBelowValueMaxFloat{23}
\def\RealSubcubicGapMostBelowValueMeanFloat{5.47019867549668870054802027880214154720306396484375}
\def\RealSubcubicGapMostBelowValueMedianFloat{1}
\def\RealSubcubicGapMostBelowValueMinFloat{1}
\def\RealSubcubicGapMostBelowValueNumStdLen{15100}
\def\RealSubcubicGapMostBelowValueNumStdMaxFloat{1.5}
\def\RealSubcubicGapMostBelowValueNumStdMeanFloat{1.5}
\def\RealSubcubicGapMostBelowValueNumStdMedianFloat{1.5}
\def\RealSubcubicGapMostBelowValueNumStdMinFloat{1.5}
\def\RealSubcubicGapMostBelowValueNumStdStdDevFloat{0}
\def\RealSubcubicGapMostBelowValueSequenceFracLen{15100}
\def\RealSubcubicGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\RealSubcubicGapMostBelowValueSequenceFracMeanFloat{0.99053359043124500349364325302303768694400787353515625}
\def\RealSubcubicGapMostBelowValueSequenceFracMedianFloat{0.9522950348258019115377237540087662637233734130859375}
\def\RealSubcubicGapMostBelowValueSequenceFracMinFloat{0.92754381895065318719417746251565404236316680908203125}
\def\RealSubcubicGapMostBelowValueSequenceFracStdDevFloat{0.0110176616847880888550026412531224195845425128936767578125}
\def\RealSubcubicGapMostBelowValueStdDevFloat{4.52716297434603465177360703819431364536285400390625}
\def\RealSubcubicInstructionCountBranchLen{15100}
\def\RealSubcubicInstructionCountBranchMaxFloat{0}
\def\RealSubcubicInstructionCountBranchMeanFloat{0}
\def\RealSubcubicInstructionCountBranchMedianFloat{0}
\def\RealSubcubicInstructionCountBranchMinFloat{0}
\def\RealSubcubicInstructionCountBranchStdDevFloat{0}
\def\RealSubcubicInstructionCountIntLen{15100}
\def\RealSubcubicInstructionCountIntMaxFloat{0}
\def\RealSubcubicInstructionCountIntMeanFloat{0}
\def\RealSubcubicInstructionCountIntMedianFloat{0}
\def\RealSubcubicInstructionCountIntMinFloat{0}
\def\RealSubcubicInstructionCountIntStdDevFloat{0}
\def\RealSubcubicInstructionCountLen{15100}
\def\RealSubcubicInstructionCountMaxFloat{8343894}
\def\RealSubcubicInstructionCountMeanFloat{6440064.799999999813735485076904296875}
\def\RealSubcubicInstructionCountMedianFloat{5473748}
\def\RealSubcubicInstructionCountMinFloat{5473748}
\def\RealSubcubicInstructionCountStdDevFloat{795875.490351449348963797092437744140625}
\def\RealSubcubicMaxGapLen{15100}
\def\RealSubcubicMaxGapMaxFloat{47}
\def\RealSubcubicMaxGapMeanFloat{23.63258278145695356897704186849296092987060546875}
\def\RealSubcubicMaxGapMedianFloat{1}
\def\RealSubcubicMaxGapMinFloat{1}
\def\RealSubcubicMaxGapStdDevFloat{14.672164864329364064587934990413486957550048828125}
\def\RealSubcubicNormalizedAccuracyLen{15100}
\def\RealSubcubicNormalizedAccuracyMaxFloat{0.7362903356393937226442858445807360112667083740234375}
\def\RealSubcubicNormalizedAccuracyMeanFloat{0.30367035045883528088239700082340277731418609619140625}
\def\RealSubcubicNormalizedAccuracyMedianFloat{0.000000000000000026065848841239090779005246038169553657235825929079642282459872149047441780567169189453125}
\def\RealSubcubicNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\RealSubcubicNormalizedAccuracyStdDevFloat{0.2435398661351622084936252576881088316440582275390625}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.73561759633376000433457875260501168668270111083984375}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMaxKey{13293}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.6744402969050644625070844995207153260707855224609375}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMeanKey{2773}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.59984506874493315198293430512421764433383941650390625}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMinFloat{0.5886748106702359706332572386600077152252197265625}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMinKey{11498}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0277599487009831287498418106451936182565987110137939453125}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.166309213880606099333903102888143621385097503662109375}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10834467436685824015540902109933085739612579345703125}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{23367}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.069256780745197199511409280603402294218540191650390625}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{14095}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0641773134406526946094118102337233722209930419921875}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0192612986811899582206830672248543123714625835418701171875}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{191741469097210324}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{124912904987177120}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{23367}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{79847631860979296}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{14095}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{73991404773622603}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{22206765456199400}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{3284}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{7230.609271523178904317319393157958984375}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{7238}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{10248}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{10248}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{2008.985681842410258468589745461940765380859375}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.4831371307373046875}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{30371}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{1.36984169483184814453125}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{21317}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.4478428364381130677429609932005405426025390625}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{11498}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.172185430463576150117432916886173188686370849609375}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99907410144805919305355246251565404236316680908203125}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{18146}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.988061948722561478319903471856378018856048583984375}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29110}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95318606495857227667301003748434595763683319091796875}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{3284}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94793224334716796875}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{19093}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.009528229840375206094460480699126492254436016082763671875}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.39469309737089641743068568757735192775726318359375}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7393557}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMaxKey{10248}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6458010.072847682051360607147216796875}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMeanKey{24202}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5896885}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMedianKey{3284}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMinFloat{5896885}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMinKey{3284}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{527408.75618842965923249721527099609375}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMaxFloat{36}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMeanFloat{30.576158940397352381523887743242084980010986328125}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMedianKey{8048}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMinKey{8048}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.8219106516352869817865212098695337772369384765625}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7362903356393937226442858445807360112667083740234375}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{13293}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6752443192679418171309180252137593924999237060546875}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{19093}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.6007763318331817981032827447052113711833953857421875}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.5909438696948836611255728712421841919422149658203125}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11498}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0276422937253531335322076500915500218980014324188232421875}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{92.9854123592376851092922152020037174224853515625}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.6036648987144843658825266174972057342529296875}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{19451}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.923117816448211669921875}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.9165172576904296875}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5493088914244939058306727019953541457653045654296875}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7482655048370361328125}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61012741745702481210855694371275603771209716796875}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMeanKey{8721}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.49540579319000244140625}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMedianKey{28778}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMinFloat{4.49149227142333984375}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0570625438540881269045001999984378926455974578857421875}
\def\RealSubcubicProofSearchTimeLen{15100}
\def\RealSubcubicProofSearchTimeMaxFloat{101.354745388031005859375}
\def\RealSubcubicProofSearchTimeMeanFloat{84.2111817345240325494160060770809650421142578125}
\def\RealSubcubicProofSearchTimeMedianFloat{81.12614621996880259757745079696178436279296875}
\def\RealSubcubicProofSearchTimeMinFloat{78.8330733776092529296875}
\def\RealSubcubicProofSearchTimeStdDevFloat{1.4637204285312879203928559945779852569103240966796875}
\def\RealSubcubicProofTimeLen{15100}
\def\RealSubcubicProofTimeMaxFloat{5.38143634796142578125}
\def\RealSubcubicProofTimeMeanFloat{4.596908784623177979256070102564990520477294921875}
\def\RealSubcubicProofTimeMedianFloat{4.46908013820648175595806605997495353221893310546875}
\def\RealSubcubicProofTimeMinFloat{4.4427516460418701171875}
\def\RealSubcubicProofTimeStdDevFloat{0.0596223763155452335382733508595265448093414306640625}
\def\ResampleEQKEErrLen{100}
\def\ResampleEQKEErrMaxLen{151}
\def\ResampleEQKEErrMaxMaxFloat{1.89808976650238037109375}
\def\ResampleEQKEErrMaxMaxKey{519}
\def\ResampleEQKEErrMaxMeanFloat{1.396057392587724876875654445029795169830322265625}
\def\ResampleEQKEErrMaxMeanKey{20751}
\def\ResampleEQKEErrMaxMedianFloat{1.0984767377376556396484375}
\def\ResampleEQKEErrMaxMedianKey{15399}
\def\ResampleEQKEErrMaxMinFloat{1.0839126110076904296875}
\def\ResampleEQKEErrMaxMinKey{20976}
\def\ResampleEQKEErrMaxStdDevFloat{0.1415627695057965762526208663985016755759716033935546875}
\def\ResampleEQKEErrMeanLen{151}
\def\ResampleEQKEErrMeanMaxFloat{1.0918330991268156981988113329862244427204132080078125}
\def\ResampleEQKEErrMeanMaxKey{7310}
\def\ResampleEQKEErrMeanMeanFloat{0.9720000295410093915648985785082913935184478759765625}
\def\ResampleEQKEErrMeanMeanKey{26932}
\def\ResampleEQKEErrMeanMedianFloat{0.875349613279104321605927907512523233890533447265625}
\def\ResampleEQKEErrMeanMedianKey{6532}
\def\ResampleEQKEErrMeanMinFloat{0.87160788476467132568359375}
\def\ResampleEQKEErrMeanMinKey{16069}
\def\ResampleEQKEErrMeanStdDevFloat{0.049075188704820769947101410934919840656220912933349609375}
\def\ResampleEQKEErrMedianLen{151}
\def\ResampleEQKEErrMedianMaxFloat{0.874287066459655815009455182007513940334320068359375}
\def\ResampleEQKEErrMedianMaxKey{19451}
\def\ResampleEQKEErrMedianMeanFloat{0.76263041837128586752925230030086822807788848876953125}
\def\ResampleEQKEErrMedianMeanKey{7467}
\def\ResampleEQKEErrMedianMedianFloat{0.6813107521831989199512236154987476766109466552734375}
\def\ResampleEQKEErrMedianMedianKey{29110}
\def\ResampleEQKEErrMedianMinFloat{0.68004884660243991589823053800500929355621337890625}
\def\ResampleEQKEErrMedianMinKey{7098}
\def\ResampleEQKEErrMedianStdDevFloat{0.04228828006187958232775514488821499980986118316650390625}
\def\ResampleEQKEErrMinLen{151}
\def\ResampleEQKEErrMinMaxFloat{0.85718023777008056640625}
\def\ResampleEQKEErrMinMaxKey{19451}
\def\ResampleEQKEErrMinMeanFloat{0.7510484504383920789649664584430865943431854248046875}
\def\ResampleEQKEErrMinMeanKey{6159}
\def\ResampleEQKEErrMinMedianFloat{0.6611323654651641845703125}
\def\ResampleEQKEErrMinMedianKey{29110}
\def\ResampleEQKEErrMinMinFloat{0.65490829944610595703125}
\def\ResampleEQKEErrMinMinKey{2549}
\def\ResampleEQKEErrMinStdDevFloat{0.04395538709875825011952343857046798802912235260009765625}
\def\ResampleEQKEErrNumSamples{100}
\def\ResampleEQKEErrSeed{1234}
\def\ResampleEQKEErrStdDevLen{151}
\def\ResampleEQKEErrStdDevMaxFloat{0.1606937649438355542041989565404946915805339813232421875}
\def\ResampleEQKEErrStdDevMaxKey{519}
\def\ResampleEQKEErrStdDevMeanFloat{0.11928265618240761758439560935585177503526210784912109375}
\def\ResampleEQKEErrStdDevMeanKey{7238}
\def\ResampleEQKEErrStdDevMedianFloat{0.09123422531014900582757576330550364218652248382568359375}
\def\ResampleEQKEErrStdDevMedianKey{15399}
\def\ResampleEQKEErrStdDevMinFloat{0.08622003282275610136498045221742358990013599395751953125}
\def\ResampleEQKEErrStdDevMinKey{20976}
\def\ResampleEQKEErrStdDevStdDevFloat{0.01350638960448406929171216717122661066241562366485595703125}
\def\ResampleNormalEQKEErrLen{100}
\def\ResampleNormalEQKEErrMaxLen{151}
\def\ResampleNormalEQKEErrMaxMaxFloat{1.50558054447174072265625}
\def\ResampleNormalEQKEErrMaxMaxKey{7310}
\def\ResampleNormalEQKEErrMaxMeanFloat{1.3410637615532274846685822922154329717159271240234375}
\def\ResampleNormalEQKEErrMaxMeanKey{9504}
\def\ResampleNormalEQKEErrMaxMedianFloat{1.19834804534912109375}
\def\ResampleNormalEQKEErrMaxMedianKey{6532}
\def\ResampleNormalEQKEErrMaxMinFloat{1.192976474761962890625}
\def\ResampleNormalEQKEErrMaxMinKey{16069}
\def\ResampleNormalEQKEErrMaxStdDevFloat{0.06262636046380838650282640855948557145893573760986328125}
\def\ResampleNormalEQKEErrMeanLen{151}
\def\ResampleNormalEQKEErrMeanMaxFloat{1.03069824457168568443421463598497211933135986328125}
\def\ResampleNormalEQKEErrMeanMaxKey{7310}
\def\ResampleNormalEQKEErrMeanMeanFloat{0.92890340213744071462542706285603344440460205078125}
\def\ResampleNormalEQKEErrMeanMeanKey{32374}
\def\ResampleNormalEQKEErrMeanMedianFloat{0.8240527676045894533984892404987476766109466552734375}
\def\ResampleNormalEQKEErrMeanMedianKey{6532}
\def\ResampleNormalEQKEErrMeanMinFloat{0.8213244026899337857372529470012523233890533447265625}
\def\ResampleNormalEQKEErrMeanMinKey{16069}
\def\ResampleNormalEQKEErrMeanStdDevFloat{0.041786030855978935349970271317943115718662738800048828125}
\def\ResampleNormalEQKEErrMedianLen{151}
\def\ResampleNormalEQKEErrMedianMaxFloat{0.827339304089546256903986432007513940334320068359375}
\def\ResampleNormalEQKEErrMedianMaxKey{24144}
\def\ResampleNormalEQKEErrMedianMeanFloat{0.75187872785803488984157638697070069611072540283203125}
\def\ResampleNormalEQKEErrMedianMeanKey{12561}
\def\ResampleNormalEQKEErrMedianMedianFloat{0.660124757885932833545439279987476766109466552734375}
\def\ResampleNormalEQKEErrMedianMedianKey{6532}
\def\ResampleNormalEQKEErrMedianMinFloat{0.65966561377048493763908254550187848508358001708984375}
\def\ResampleNormalEQKEErrMedianMinKey{16069}
\def\ResampleNormalEQKEErrMedianStdDevFloat{0.03580725936045635326987479629679000936448574066162109375}
\def\ResampleNormalEQKEErrMinLen{151}
\def\ResampleNormalEQKEErrMinMaxFloat{0.8230388164520263671875}
\def\ResampleNormalEQKEErrMinMaxKey{24144}
\def\ResampleNormalEQKEErrMinMeanFloat{0.745669060984984088946703195688314735889434814453125}
\def\ResampleNormalEQKEErrMinMeanKey{12561}
\def\ResampleNormalEQKEErrMinMedianFloat{0.6532876491546630859375}
\def\ResampleNormalEQKEErrMinMedianKey{16069}
\def\ResampleNormalEQKEErrMinMinFloat{0.6508386135101318359375}
\def\ResampleNormalEQKEErrMinMinKey{6532}
\def\ResampleNormalEQKEErrMinStdDevFloat{0.03769990416182704418002202828574809245765209197998046875}
\def\ResampleNormalEQKEErrStdDevLen{151}
\def\ResampleNormalEQKEErrStdDevMaxFloat{0.11432600503308094908039294068657909519970417022705078125}
\def\ResampleNormalEQKEErrStdDevMaxKey{7310}
\def\ResampleNormalEQKEErrStdDevMeanFloat{0.10182410903638912380575476390731637366116046905517578125}
\def\ResampleNormalEQKEErrStdDevMeanKey{6082}
\def\ResampleNormalEQKEErrStdDevMedianFloat{0.09109403608579447197968192995176650583744049072265625}
\def\ResampleNormalEQKEErrStdDevMedianKey{16069}
\def\ResampleNormalEQKEErrStdDevMinFloat{0.09098392677842261078158259124393225647509098052978515625}
\def\ResampleNormalEQKEErrStdDevMinKey{6532}
\def\ResampleNormalEQKEErrStdDevStdDevFloat{0.004764517782177755955697051604147418402135372161865234375}
\def\SubcubicAccuracyLen{7852}
\def\SubcubicAccuracyMaxFloat{0.73561759633376000433457875260501168668270111083984375}
\def\SubcubicAccuracyMeanFloat{0.426576906411640865979251202588784508407115936279296875}
\def\SubcubicAccuracyMedianFloat{0.000000000000000026888213877640509963384829461574554443359375}
\def\SubcubicAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicAccuracyStdDevFloat{0.20572442246982214353323570321663282811641693115234375}
\def\SubcubicAttentionQuadraticAccuracyLen{1812}
\def\SubcubicAttentionQuadraticAccuracyMaxFloat{0.466887709092356606443985356236225925385951995849609375}
\def\SubcubicAttentionQuadraticAccuracyMeanFloat{0.336621976878664408427965781811508350074291229248046875}
\def\SubcubicAttentionQuadraticAccuracyMedianFloat{0.11999926163030394388187005461077205836772918701171875}
\def\SubcubicAttentionQuadraticAccuracyMinFloat{0.044735253986640501067117980937837273813784122467041015625}
\def\SubcubicAttentionQuadraticAccuracyStdDevFloat{0.060923275199585034955784834664882509969174861907958984375}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyMaxFloat{0.452543729453746712554362829905585385859012603759765625}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyMeanFloat{0.126723408827566885737070379036595113575458526611328125}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyMedianFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyStdDevFloat{0.150288814804498738197935381322167813777923583984375}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracMaxFloat{0.46377977035578010767125078928074799478054046630859375}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracMeanFloat{0.225632850369890614050660815337323583662509918212890625}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracStdDevFloat{0.1621320873651361516021296438339049927890300750732421875}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesMaxFloat{534701670644804012}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesMeanFloat{260136965337185856}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesStdDevFloat{186925570110061536}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateMeanFloat{6487.3333333333330301684327423572540283203125}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateStdDevFloat{42.66666666666666429819088079966604709625244140625}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundMaxFloat{156.4159393310546875}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundMeanFloat{91.8609873116937478698673658072948455810546875}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundMedianFloat{78.9598388671875}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundMinFloat{78.61283111572265625}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundStdDevFloat{7.64323512735036647569586421013809740543365478515625}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueMaxFloat{23}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueMeanFloat{9.1795437821927894361806465894915163516998291015625}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueMedianFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueMinFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracMeanFloat{0.99895022817180822993776700968737713992595672607421875}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracMedianFloat{0.990021169185638427734375}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracMinFloat{0.98604261875152598992855246251565404236316680908203125}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.001612141786953481641109231503605769830755889415740966796875}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueStdDevFloat{6.018318327787913091242444352246820926666259765625}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountMaxFloat{5611377}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountMeanFloat{5542546.666666666977107524871826171875}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountMedianFloat{5473748}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountMinFloat{5473748}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountStdDevFloat{55524.7348105128548922948539257049560546875}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapMaxFloat{47}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapMeanFloat{24.037159676232523253247563843615353107452392578125}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapMedianFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapMinFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapStdDevFloat{17.518740589558962739147318643517792224884033203125}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyMaxFloat{0.45286923071017870512378067360259592533111572265625}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyMeanFloat{0.12687312556441232569426347254193387925624847412109375}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyMedianFloat{0.000000000000000026054821497037114438219634609030939328582006345885226095138165192111046053469181060791015625}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyStdDevFloat{0.1504676457476110951194669951291871257126331329345703125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.452543729453746712554362829905585385859012603759765625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{7238}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.390423493111564379187683471172931604087352752685546875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{31308}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.325130980910436073738623008466674946248531341552734375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{9816}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.318141293842261585478325969233992509543895721435546875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{11124}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0279359164293897233033447946581873111426830291748046875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.456757311611598215694840519063291139900684356689453125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.3493432199636561374944676572340540587902069091796875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29725}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.268695947037915328081680854666046798229217529296875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4810}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.268159626117558114177796824151300825178623199462890625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.028945140281470826959520081800292246043682098388671875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{526605326943422293}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{402765310784699136}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29725}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{309785335540715008}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4810}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{309166999618264736}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{33371474684369596}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6502.0264900662250511231832206249237060546875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{104}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{104}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{31.745667070430105383138652541674673557281494140625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.4159393310546875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.4848378667768287186845554970204830169677734375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29726}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.8730869293212890625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.61283111572265625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.66115263186247030802178414887748658657073974609375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{23}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29565}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{13.6887417218543046004697316675446927547454833984375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{10}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4810}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{10}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4810}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99999964237213123663394753748434595763683319091796875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13654}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99807756902366284723626677077845670282840728759765625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29195}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9917971193790435791015625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24438}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.991044223308563232421875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{29022}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00160033295619864597038317644006610862561501562595367431640625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.065758140461221525896462480886839330196380615234375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5611377}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{3284}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5593392.218543046154081821441650390625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5584660}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{104}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{5584660}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{104}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{8919.140182845294475555419921875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{45}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{3254}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{38.66225165562914156680562882684171199798583984375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{14}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{7098}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.73437125964751448492506824550218880176544189453125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.45286923071017870512378067360259592533111572265625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7238}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.390894573938078193631184831247082911431789398193359375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{31308}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.325522332758098886795750104283797554671764373779296875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{9816}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.318423535380195465993580228314385749399662017822265625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11124}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0279968896252014466663471381480121635831892490386962890625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.1968085765838623046875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.6048799982134056563154445029795169830322265625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.071754515171051025390625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{79.3047096729278564453125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.4051890214643290022422661422751843929290771484375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.777535915374755859375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{913}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.62063053112156385537900860072113573551177978515625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{32374}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.50573670864105224609375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{24173}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{4.5055332183837890625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.058966118215369713040363564005019725300371646881103515625}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeMaxFloat{101.354745388031005859375}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeMeanFloat{84.1996096230500512547223479487001895904541015625}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeMedianFloat{81.1775342977046960868392488919198513031005859375}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeMinFloat{79.2337474822998046875}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeStdDevFloat{1.4334570284820162822114752998459152877330780029296875}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeMaxFloat{4.8339951038360595703125}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeMeanFloat{4.5956573026683766869382452568970620632171630859375}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeMedianFloat{4.46842619061470003316571819595992565155029296875}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeMinFloat{4.4427516460418701171875}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeStdDevFloat{0.059335069010919845589047127987214480526745319366455078125}
\def\SubcubicAttentionQuadraticDroppedSequencesFracLen{1812}
\def\SubcubicAttentionQuadraticDroppedSequencesFracMaxFloat{0.45416146537232560120855850982479751110076904296875}
\def\SubcubicAttentionQuadraticDroppedSequencesFracMeanFloat{0.3722685428609882052342072711326181888580322265625}
\def\SubcubicAttentionQuadraticDroppedSequencesFracMedianFloat{0.31220047324589661474902868576464243233203887939453125}
\def\SubcubicAttentionQuadraticDroppedSequencesFracMinFloat{0.3086802924016363025572218248271383345127105712890625}
\def\SubcubicAttentionQuadraticDroppedSequencesFracStdDevFloat{0.024525890060721249052999581863332423381507396697998046875}
\def\SubcubicAttentionQuadraticDroppedSequencesLen{1812}
\def\SubcubicAttentionQuadraticDroppedSequencesMaxFloat{523612519991512137}
\def\SubcubicAttentionQuadraticDroppedSequencesMeanFloat{429196408553089024}
\def\SubcubicAttentionQuadraticDroppedSequencesMedianFloat{359942639353628864}
\def\SubcubicAttentionQuadraticDroppedSequencesMinFloat{355884147158175998}
\def\SubcubicAttentionQuadraticDroppedSequencesStdDevFloat{28276426070628856}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateLen{1812}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateMeanFloat{4459.6666666666669698315672576427459716796875}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateStdDevFloat{69.8514296362087492298087454400956630706787109375}
\def\SubcubicAttentionQuadraticErrUpperBoundLen{1812}
\def\SubcubicAttentionQuadraticErrUpperBoundMaxFloat{156.4159393310546875}
\def\SubcubicAttentionQuadraticErrUpperBoundMeanFloat{91.8609873116937478698673658072948455810546875}
\def\SubcubicAttentionQuadraticErrUpperBoundMedianFloat{78.9598388671875}
\def\SubcubicAttentionQuadraticErrUpperBoundMinFloat{78.61283111572265625}
\def\SubcubicAttentionQuadraticErrUpperBoundStdDevFloat{7.64323512735036647569586421013809740543365478515625}
\def\SubcubicAttentionQuadraticGapMostBelowValueLen{1812}
\def\SubcubicAttentionQuadraticGapMostBelowValueMaxFloat{22}
\def\SubcubicAttentionQuadraticGapMostBelowValueMeanFloat{12.7488962472406175407968476065434515476226806640625}
\def\SubcubicAttentionQuadraticGapMostBelowValueMedianFloat{9}
\def\SubcubicAttentionQuadraticGapMostBelowValueMinFloat{9}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdLen{1812}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracLen{1812}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracMeanFloat{0.998192975128986415001008936087600886821746826171875}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracMedianFloat{0.99032340943813312872379128748434595763683319091796875}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracMinFloat{0.98490077257156360968082253748434595763683319091796875}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.00158842564051119429328895460429293962079100310802459716796875}
\def\SubcubicAttentionQuadraticGapMostBelowValueStdDevFloat{2.01959875592423809820274982484988868236541748046875}
\def\SubcubicAttentionQuadraticInstructionCountBranchLen{1812}
\def\SubcubicAttentionQuadraticInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntLen{1812}
\def\SubcubicAttentionQuadraticInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntMinFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountLen{1812}
\def\SubcubicAttentionQuadraticInstructionCountMaxFloat{5875728}
\def\SubcubicAttentionQuadraticInstructionCountMeanFloat{5803452.833333333022892475128173828125}
\def\SubcubicAttentionQuadraticInstructionCountMedianFloat{5731892}
\def\SubcubicAttentionQuadraticInstructionCountMinFloat{5731892}
\def\SubcubicAttentionQuadraticInstructionCountStdDevFloat{55669.5640765420612297020852565765380859375}
\def\SubcubicAttentionQuadraticMaxGapLen{1812}
\def\SubcubicAttentionQuadraticMaxGapMaxFloat{45}
\def\SubcubicAttentionQuadraticMaxGapMeanFloat{38.08774834437085843319437117315828800201416015625}
\def\SubcubicAttentionQuadraticMaxGapMedianFloat{11}
\def\SubcubicAttentionQuadraticMaxGapMinFloat{10}
\def\SubcubicAttentionQuadraticMaxGapStdDevFloat{3.525924801052038759507922804914414882659912109375}
\def\SubcubicAttentionQuadraticNormalizedAccuracyLen{1812}
\def\SubcubicAttentionQuadraticNormalizedAccuracyMaxFloat{0.467223527547085126787607123333145864307880401611328125}
\def\SubcubicAttentionQuadraticNormalizedAccuracyMeanFloat{0.337019963999195371062711501508601941168308258056640625}
\def\SubcubicAttentionQuadraticNormalizedAccuracyMedianFloat{0.1201792735170924275589499075067578814923763275146484375}
\def\SubcubicAttentionQuadraticNormalizedAccuracyMinFloat{0.045365318046782031335961704598958021961152553558349609375}
\def\SubcubicAttentionQuadraticNormalizedAccuracyStdDevFloat{0.060992974364862902192374605192526360042393207550048828125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.466887709092356606443985356236225925385951995849609375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{7238}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.3922578845997801710865360291791148483753204345703125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{4647}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.320946827591013617020365700227557681500911712646484375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{12287}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.312498058804795808551801883368170820176601409912109375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{11124}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0299977552759169256713089879440303775481879711151123046875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.437731908416957582463879816714324988424777984619140625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.3680353010889969578300906505319289863109588623046875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{13716}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.31028766990496936539756234196829609572887420654296875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1412}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.30898509158054132672788227864657528698444366455078125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.023631780581428611653915794477143208496272563934326171875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{504670530466505312}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{424315813079960320}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{13716}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{357737327247789952}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1412}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{356235556686122123}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{27245588024479548}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{104}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4503.5496688741723119164817035198211669921875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{9132}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{9132}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{52.3286467253097953289397992193698883056640625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.4159393310546875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.594581401900740047494764439761638641357421875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{14929}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.906459808349609375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.7463226318359375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.6995004144125953615684920805506408214569091796875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{21}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{27584}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{12.403973509933774010960405576042830944061279296875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{6532}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999834835529327392578125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{3175}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99804457607648233707919871449121274054050445556640625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6204}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99079622328281402587890625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{2773}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99066841602325439453125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{4157}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0016663760551162017618798127926993402070365846157073974609375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.912589202168599289421990761184133589267730712890625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5875728}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{1490}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5851342.735099337995052337646484375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{104}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5840756}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{5840756}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{9617.7159655192444915883243083953857421875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{43}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{6082}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{38.086092715231785632568062283098697662353515625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{32.25}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{29052}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{30}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{2345}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.966407951014865762573435858939774334430694580078125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.467223527547085126787607123333145864307880401611328125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7238}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.392731675846423156084341599125764332711696624755859375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{17080}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.321272908155751546477318925099098123610019683837890625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12287}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.31277529390261415986884685480617918074131011962890625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11124}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0300639007178607996217944986483416869305074214935302734375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{92.4560732841491557110202847979962825775146484375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.5437334910133841958668199367821216583251953125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1951}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.57914769649505615234375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.1144449710845947265625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.646587558162117215232456146623007953166961669921875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.757457256317138671875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.6167012003083893745269961073063313961029052734375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{10248}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.499331891536712646484375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{27584}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{4.488025665283203125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{28778}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.057737022243197620718913043447173549793660640716552734375}
\def\SubcubicAttentionQuadraticProofSearchTimeLen{1812}
\def\SubcubicAttentionQuadraticProofSearchTimeMaxFloat{92.5717060565948344219577847979962825775146484375}
\def\SubcubicAttentionQuadraticProofSearchTimeMeanFloat{84.2336343107107694549995358102023601531982421875}
\def\SubcubicAttentionQuadraticProofSearchTimeMedianFloat{81.0178870213031814273563213646411895751953125}
\def\SubcubicAttentionQuadraticProofSearchTimeMinFloat{80.2824556827545166015625}
\def\SubcubicAttentionQuadraticProofSearchTimeStdDevFloat{1.5376680242278288890389603693620301783084869384765625}
\def\SubcubicAttentionQuadraticProofTimeLen{1812}
\def\SubcubicAttentionQuadraticProofTimeMaxFloat{4.92527079582214444286591970012523233890533447265625}
\def\SubcubicAttentionQuadraticProofTimeMeanFloat{4.60028835269262703633330602315254509449005126953125}
\def\SubcubicAttentionQuadraticProofTimeMedianFloat{4.4755256903171538596097889239899814128875732421875}
\def\SubcubicAttentionQuadraticProofTimeMinFloat{4.4480721950531005859375}
\def\SubcubicAttentionQuadraticProofTimeStdDevFloat{0.059666635137547975598071303693359368480741977691650390625}
\def\SubcubicAttentionVocabModelSquaredAccuracyLen{3020}
\def\SubcubicAttentionVocabModelSquaredAccuracyMaxFloat{0.71161430067189834769436629358096979558467864990234375}
\def\SubcubicAttentionVocabModelSquaredAccuracyMeanFloat{0.55272976521586991704992897211923263967037200927734375}
\def\SubcubicAttentionVocabModelSquaredAccuracyMedianFloat{0.2026966779395435735988684200492571108043193817138671875}
\def\SubcubicAttentionVocabModelSquaredAccuracyMinFloat{0.08779767939409789667681849323344067670404911041259765625}
\def\SubcubicAttentionVocabModelSquaredAccuracyStdDevFloat{0.09679406007460532312958179090855992399156093597412109375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyMaxFloat{0.70495421337041774823006790029467083513736724853515625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyMeanFloat{0.195614448055888623390075053976033814251422882080078125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyMedianFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyStdDevFloat{0.2317268382155659722787532928123255260288715362548828125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracMaxFloat{0.302663733530732004251007083439617417752742767333984375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracMeanFloat{0.09874242723707594981963353575338260270655155181884765625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracStdDevFloat{0.07403403175116836376634665839446824975311756134033203125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesMaxFloat{348947527052177429}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesMeanFloat{113842267778701744}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesStdDevFloat{85355427278668128}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateMeanFloat{6457.4666666666662422358058393001556396484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateMedianFloat{6338}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateMinFloat{6338}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateStdDevFloat{56.60372975539882389739432255737483501434326171875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundMaxFloat{33.5944671630859375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundMeanFloat{7.89254473882005669338468578644096851348876953125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundMedianFloat{3.806694507598876953125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundMinFloat{3.745930433273314985598290149937383830547332763671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundStdDevFloat{3.77648699916363828066323549137450754642486572265625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueMaxFloat{9}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueMeanFloat{3.17086092715231782079854383482597768306732177734375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueMedianFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueMinFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracMeanFloat{0.98907907038071829486369779260712675750255584716796875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracMedianFloat{0.9518301597237586175737078519887290894985198974609375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracMinFloat{0.941314160823822021484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.01106941254663927100276854531557546579279005527496337890625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueStdDevFloat{1.6520609673434847319839491319726221263408660888671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountMaxFloat{8079543}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountMeanFloat{6762704.333333333022892475128173828125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountMedianFloat{6004052}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountMinFloat{6004052}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountStdDevFloat{716580.174071789137087762355804443359375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapMaxFloat{41}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapMeanFloat{15.7333333333333325043668082798831164836883544921875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapMedianFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapMinFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapStdDevFloat{13.8512426954759977348885513492859899997711181640625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyMaxFloat{0.70586535370262193378465553905698470771312713623046875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyMeanFloat{0.195844039139030756668802268904983066022396087646484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyMedianFloat{0.000000000000000026054821497037114438219634609030939328582006345885226095138165192111046053469181060791015625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyStdDevFloat{0.231996551928451755220095265030977316200733184814453125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.70495421337041774823006790029467083513736724853515625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{18289}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.62487745964228846862198452072334475815296173095703125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{24202}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.5237321854485148531210825240123085677623748779296875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.521449397118541657647483589244075119495391845703125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{2306}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0309035344591167028538425398664912790991365909576416015625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.198309672249317003878132936733891256153583526611328125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1355118421907518799773839646150008775293827056884765625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{23633}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08819241261316472513254183240860584191977977752685546875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07640795145471369897993696440607891418039798736572265625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0167626782758810120854686687152934609912335872650146484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{228635485707773261}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{156234516990607328}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{23633}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{101678929044877776}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{88092370355095476}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19326052259069240}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{742}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6492.2781456953644010354764759540557861328125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{31.4842878800922107984661124646663665771484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{11.43377780914306640625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{23633}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.044434572687212181563154445029795169830322265625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{6155}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.817322850227355512942040149937383830547332763671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{15662}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.806694507598876953125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{18289}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.2242014892683481530610833942773751914501190185546875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.887417218543046448786526525509543716907501220703125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1185}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1185}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99766051769256602899105246251565404236316680908203125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{24144}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98323778956141694163051170107792131602764129638671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{17194}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95128062367439281121761496251565404236316680908203125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{10248}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.941314160823822021484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{19004}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01126216006376259438914733124192935065366327762603759765625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.50877135938195550135532130298088304698467254638671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6881493}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{9134}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6209911.523178808391094207763671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{742}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6114964}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{6114964}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{237574.8963797009200789034366607666015625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{41}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{29.642384105960264406576243345625698566436767578125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{1951}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{742}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.6982361193426225298708232003264129161834716796875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.70586535370262193378465553905698470771312713623046875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18289}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.62562329264245575277669786373735405504703521728515625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{2773}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.525400740304266644642439132439903914928436279296875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.522058608420906011815532110631465911865234375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2306}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0308397769129801595233697497633329476229846477508544921875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.3213505744933939922702847979962825775146484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.6141748775709601204653154127299785614013671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27671}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.276223599910736083984375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{79.694097042083740234375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3390074957860347293348013408831320703029632568359375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.74157428741455078125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.620685501603890799060536664910614490509033203125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{19538}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.507993161678314208984375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{4.5032379627227783203125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05704269111738767550345841073067276738584041595458984375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeMaxFloat{100.6354253292083598125827847979962825775146484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeMeanFloat{84.2033788139456902399615501053631305694580078125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeMedianFloat{81.1768663084506982841048738919198513031005859375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeMinFloat{78.8330733776092529296875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeStdDevFloat{1.421929963451891154591066879220306873321533203125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeMaxFloat{5.38143634796142578125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeMeanFloat{4.59503990945963369796345432405360043048858642578125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeMedianFloat{4.4664830994606017355863514239899814128875732421875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeMinFloat{4.447611331939697265625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeStdDevFloat{0.060364283353939028609058681240639998577535152435302734375}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracLen{3020}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracMaxFloat{0.295947151523005713702474395176977850496768951416015625}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracMeanFloat{0.141858614677438321649560748483054339885711669921875}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracMedianFloat{0.091523656399694619523188521270640194416046142578125}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracMinFloat{0.0716376994440456049684229355989373289048671722412109375}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracStdDevFloat{0.0331443307570566669806311210777494125068187713623046875}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesLen{3020}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesMaxFloat{341203835218014245}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesMeanFloat{163551847475355168}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesMedianFloat{105519591643456048}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesMinFloat{82592644229602166}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesStdDevFloat{38212811685612768}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateLen{3020}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateMeanFloat{4429.8000000000001818989403545856475830078125}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateMedianFloat{4290}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateMinFloat{4290}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateStdDevFloat{79.13760168213337919951300136744976043701171875}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundLen{3020}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundMaxFloat{33.5944671630859375}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundMeanFloat{7.89254473882005669338468578644096851348876953125}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundMedianFloat{3.807494904994964457500827847979962825775146484375}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundMinFloat{3.745930433273314985598290149937383830547332763671875}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundStdDevFloat{3.776486999163638724752445341437123715877532958984375}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueLen{3020}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueMaxFloat{8}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueMeanFloat{3.74072847682119213885698627564124763011932373046875}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueMedianFloat{3}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueMinFloat{3}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdLen{3020}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracLen{3020}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracMaxFloat{0.9997780323028564453125}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracMeanFloat{0.98504513985668584741262066017952747642993927001953125}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracMedianFloat{0.95065081119537364617855246251565404236316680908203125}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracMinFloat{0.93418014049530040399105246251565404236316680908203125}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracStdDevFloat{0.01068017517889430743893708353198235272429883480072021484375}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueStdDevFloat{0.83189530618182272458938086856505833566188812255859375}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchLen{3020}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntLen{3020}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountLen{3020}
\def\SubcubicAttentionVocabModelSquaredInstructionCountMaxFloat{8343894}
\def\SubcubicAttentionVocabModelSquaredInstructionCountMeanFloat{7023610.5}
\def\SubcubicAttentionVocabModelSquaredInstructionCountMedianFloat{6262196}
\def\SubcubicAttentionVocabModelSquaredInstructionCountMinFloat{6262196}
\def\SubcubicAttentionVocabModelSquaredInstructionCountStdDevFloat{716591.41082031535916030406951904296875}
\def\SubcubicAttentionVocabModelSquaredMaxGapLen{3020}
\def\SubcubicAttentionVocabModelSquaredMaxGapMaxFloat{39}
\def\SubcubicAttentionVocabModelSquaredMaxGapMeanFloat{29.965894039735101017640772624872624874114990234375}
\def\SubcubicAttentionVocabModelSquaredMaxGapMedianFloat{6}
\def\SubcubicAttentionVocabModelSquaredMaxGapMinFloat{5}
\def\SubcubicAttentionVocabModelSquaredMaxGapStdDevFloat{7.39879816368294473960531831835396587848663330078125}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyLen{3020}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyMaxFloat{0.712132372911521205338658546679653227329254150390625}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyMeanFloat{0.55337646726230083071840226693893782794475555419921875}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyMedianFloat{0.2030060651318115194641222842619754374027252197265625}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyMinFloat{0.08903424692016066732680457107562688179314136505126953125}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyStdDevFloat{0.096858371204732229831080303483759053051471710205078125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.71161430067189834769436629358096979558467864990234375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMaxKey{8893}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.656939700032864504208873768220655620098114013671875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMeanKey{22261}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.5843479571640834979717737951432354748249053955078125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMinFloat{0.57136739664562596896502100207726471126079559326171875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.02761322717826554529185756337028578855097293853759765625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1834952129293707934198920384005759842693805694580078125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{31308}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.12191828545485546009263799760447000153362751007080078125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{27484}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0823619425247599512562857171360519714653491973876953125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07536675377881170423410850389700499363243579864501953125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.019471327218404714531896360085738706402480602264404296875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{211555576978684046}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{31308}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{140562213105699040}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{27484}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{94956854697988960}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{86891951164001400}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{22448911873335412}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4500.5033112582777903298847377300262451171875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{104}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{1490}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{1490}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{44.674670093644408552790991961956024169921875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.95111083984375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.79649324764479079163947972119785845279693603515625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{13293}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.746451318264007568359375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27300}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.745930433273314985598290149937383830547332763671875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinKey{18289}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.221566824109622917404749387060292065143585205078125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{11498}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.291390728476821347925351801677606999874114990234375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99935060739517200811832253748434595763683319091796875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{18146}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98613212716500486809678704958059825003147125244140625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{27484}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.954102337360382080078125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11124}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95224982500076282843082253748434595763683319091796875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{19917}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.009224668728170105913566345634535537101328372955322265625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.496202852845806396953065586785669438540935516357421875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMaxFloat{8335639}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMaxKey{8840}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6612188.10596026480197906494140625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMeanKey{5358}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6371060}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMedianKey{123}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMinFloat{6371060}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMinKey{123}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{406288.639873901498503983020782470703125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMaxFloat{36}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMeanFloat{31.642384105960264406576243345625698566436767578125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMeanKey{1283}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMedianFloat{14.75}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMedianKey{12457}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMinKey{26829}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.352066419826162491091281481203623116016387939453125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.712132372911521205338658546679653227329254150390625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8893}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.657722346745189145877930059214122593402862548828125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29110}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5862273182949244709760705518419854342937469482421875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.57207766409504667848295866861008107662200927734375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.027486216270285114549043470333344885148108005523681640625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.7872295379638813983547152020037174224853515625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.5525372659923277751659043133258819580078125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{9134}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.633276283740997314453125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{9132}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.3909714221954345703125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5444024579267552343964098326978273689746856689453125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.76941967010498046875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61714983460129513304082138347439467906951904296875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMeanKey{6910}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.497490704059600830078125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMedianKey{27584}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMinFloat{4.48071384429931640625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMinKey{23696}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.056815546022368011713776780879925354383885860443115234375}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeLen{3020}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeMaxFloat{92.6686336994171142578125}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeMeanFloat{84.2341102856673984433655277825891971588134765625}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeMedianFloat{81.189638884067534263522247783839702606201171875}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeMinFloat{80.3132793903350830078125}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeStdDevFloat{1.5212317925819454078606440816656686365604400634765625}
\def\SubcubicAttentionVocabModelSquaredProofTimeLen{3020}
\def\SubcubicAttentionVocabModelSquaredProofTimeMaxFloat{4.8384621143341064453125}
\def\SubcubicAttentionVocabModelSquaredProofTimeMeanFloat{4.60088589925639634969911639927886426448822021484375}
\def\SubcubicAttentionVocabModelSquaredProofTimeMedianFloat{4.4723829686641689562520696199499070644378662109375}
\def\SubcubicAttentionVocabModelSquaredProofTimeMinFloat{4.44962310791015625}
\def\SubcubicAttentionVocabModelSquaredProofTimeStdDevFloat{0.058570643333253402662563757985481061041355133056640625}
\def\SubcubicDirectQuadraticAccuracyLen{1812}
\def\SubcubicDirectQuadraticAccuracyMaxFloat{0.71584725760343437261923327241674996912479400634765625}
\def\SubcubicDirectQuadraticAccuracyMeanFloat{0.204368597005113061815251285224803723394870758056640625}
\def\SubcubicDirectQuadraticAccuracyMedianFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\SubcubicDirectQuadraticAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicDirectQuadraticAccuracyStdDevFloat{0.241350061913419400294600336565054021775722503662109375}
\def\SubcubicDirectQuadraticDroppedSequencesFracLen{1812}
\def\SubcubicDirectQuadraticDroppedSequencesFracMaxFloat{0.1901377455241186897882954554006573744118213653564453125}
\def\SubcubicDirectQuadraticDroppedSequencesFracMeanFloat{0.0824919166218024690895305184312746860086917877197265625}
\def\SubcubicDirectQuadraticDroppedSequencesFracMedianFloat{0}
\def\SubcubicDirectQuadraticDroppedSequencesFracMinFloat{0}
\def\SubcubicDirectQuadraticDroppedSequencesFracStdDevFloat{0.05996000207523698166678371990201412700116634368896484375}
\def\SubcubicDirectQuadraticDroppedSequencesLen{1812}
\def\SubcubicDirectQuadraticDroppedSequencesMaxFloat{219213895652220809}
\def\SubcubicDirectQuadraticDroppedSequencesMeanFloat{95106704629511088}
\def\SubcubicDirectQuadraticDroppedSequencesMedianFloat{0}
\def\SubcubicDirectQuadraticDroppedSequencesMinFloat{0}
\def\SubcubicDirectQuadraticDroppedSequencesStdDevFloat{69129175808811912}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateLen{1812}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateMeanFloat{8428.666666666666060336865484714508056640625}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateStdDevFloat{1920.237022406927508200169540941715240478515625}
\def\SubcubicDirectQuadraticErrUpperBoundLen{1812}
\def\SubcubicDirectQuadraticErrUpperBoundMaxFloat{5.11057758331298828125}
\def\SubcubicDirectQuadraticErrUpperBoundMeanFloat{1.1485378201434155442939299973659217357635498046875}
\def\SubcubicDirectQuadraticErrUpperBoundMedianFloat{0}
\def\SubcubicDirectQuadraticErrUpperBoundMinFloat{0}
\def\SubcubicDirectQuadraticErrUpperBoundStdDevFloat{1.2042997573343117156952075674780644476413726806640625}
\def\SubcubicDirectQuadraticGapMostBelowValueLen{1812}
\def\SubcubicDirectQuadraticGapMostBelowValueMaxFloat{5}
\def\SubcubicDirectQuadraticGapMostBelowValueMeanFloat{2.762693156732891619498104773811064660549163818359375}
\def\SubcubicDirectQuadraticGapMostBelowValueMedianFloat{1}
\def\SubcubicDirectQuadraticGapMostBelowValueMinFloat{1}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdLen{1812}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracLen{1812}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracMeanFloat{0.98624696771698550090690105207613669335842132568359375}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracMedianFloat{0.951090533733367937685443394002504646778106689453125}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracMinFloat{0.92754381895065318719417746251565404236316680908203125}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.01378822510794682799917243443132974789477884769439697265625}
\def\SubcubicDirectQuadraticGapMostBelowValueStdDevFloat{1.317641811485505076717572592315264046192169189453125}
\def\SubcubicDirectQuadraticInstructionCountBranchLen{1812}
\def\SubcubicDirectQuadraticInstructionCountBranchMaxFloat{0}
\def\SubcubicDirectQuadraticInstructionCountBranchMeanFloat{0}
\def\SubcubicDirectQuadraticInstructionCountBranchMedianFloat{0}
\def\SubcubicDirectQuadraticInstructionCountBranchMinFloat{0}
\def\SubcubicDirectQuadraticInstructionCountBranchStdDevFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntLen{1812}
\def\SubcubicDirectQuadraticInstructionCountIntMaxFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntMeanFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntMedianFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntMinFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntStdDevFloat{0}
\def\SubcubicDirectQuadraticInstructionCountLen{1812}
\def\SubcubicDirectQuadraticInstructionCountMaxFloat{7129206}
\def\SubcubicDirectQuadraticInstructionCountMeanFloat{6457930.833333333022892475128173828125}
\def\SubcubicDirectQuadraticInstructionCountMedianFloat{5785973}
\def\SubcubicDirectQuadraticInstructionCountMinFloat{5785973}
\def\SubcubicDirectQuadraticInstructionCountStdDevFloat{618560.8591333641670644283294677734375}
\def\SubcubicDirectQuadraticMaxGapLen{1812}
\def\SubcubicDirectQuadraticMaxGapMaxFloat{41}
\def\SubcubicDirectQuadraticMaxGapMeanFloat{14.57064017660044186186496517620980739593505859375}
\def\SubcubicDirectQuadraticMaxGapMedianFloat{1}
\def\SubcubicDirectQuadraticMaxGapMinFloat{1}
\def\SubcubicDirectQuadraticMaxGapStdDevFloat{13.223832047756051366604879149235785007476806640625}
\def\SubcubicDirectQuadraticNormalizedAccuracyLen{1812}
\def\SubcubicDirectQuadraticNormalizedAccuracyMaxFloat{0.71677247699460855390185543001280166208744049072265625}
\def\SubcubicDirectQuadraticNormalizedAccuracyMeanFloat{0.204608177722058914849156963100540451705455780029296875}
\def\SubcubicDirectQuadraticNormalizedAccuracyMedianFloat{0.000000000000000026054853499066030575439223184788958386114296621768708639432787776968325488269329071044921875}
\def\SubcubicDirectQuadraticNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicDirectQuadraticNormalizedAccuracyStdDevFloat{0.2416303682069002312093886075672344304621219635009765625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.71584725760343437261923327241674996912479400634765625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{18289}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.63934881943063093245882555493153631687164306640625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{13716}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.5311258290272553583832859658286906778812408447265625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{2306}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.53062165354070811584819011841318570077419281005859375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{11498}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03152804225039114449646859839049284346401691436767578125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.188722722522415897739023193935281597077846527099609375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.12218274615083686562844178524755989201366901397705078125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{1185}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0781542788153279655016802962563815526664257049560546875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.06464661360273170342960469270110479556024074554443359375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0162273033292714696784742045565508306026458740234375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{217582485204044212}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{140867115529219312}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{1185}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{90105748723230976}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{74532471022598964}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18708806970095360}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{9835.9602649006628780625760555267333984375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{104}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{104}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{1328.72651215985251837992109358310699462890625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{3.282664775848388671875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4305}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0.3000293922740102647850335415569134056568145751953125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.76525547692727846627036569771007634699344635009765625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{17096}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.476821192052980347142465689103119075298309326171875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99750804901123035772769753748434595763683319091796875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{25516}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.97852695027724012621916926946141757071018218994140625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{913}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94610036909580230712890625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4729}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.92754381895065318719417746251565404236316680908203125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11124}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01220980854305843237017636937480347114615142345428466796875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.5377711801499811539173379060230217874050140380859375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7129206}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{104}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6068267.390728476457297801971435546875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5896885}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{5896885}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{426410.8292164950980804860591888427734375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{41}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{28.68874172185430637682657106779515743255615234375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{2773}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{742}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.3183236900689667692176954005844891071319580078125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.71677247699460855390185543001280166208744049072265625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18289}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6401113188647589158364326067385263741016387939453125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8893}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5324788591634213030800992783042602241039276123046875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.5319146001804988532768447839771397411823272705078125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2306}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.031452061853096631438564401150870253331959247589111328125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.6798899173736572265625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.5662014658087883844928001053631305694580078125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{18668}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.2748432159423828125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27484}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{79.3032329082489013671875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.34157246311157241080991298076696693897247314453125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7543885707855224609375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{5781}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.612954078131163981879581115208566188812255859375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{13036}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.502824306488037109375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{24144}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{4.493517398834228515625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0599426957144254257681126318857423029839992523193359375}
\def\SubcubicDirectQuadraticProofSearchTimeLen{1812}
\def\SubcubicDirectQuadraticProofSearchTimeMaxFloat{92.4898955821990966796875}
\def\SubcubicDirectQuadraticProofSearchTimeMeanFloat{84.165868630209246248341514728963375091552734375}
\def\SubcubicDirectQuadraticProofSearchTimeMedianFloat{81.17865376949310984855401329696178436279296875}
\def\SubcubicDirectQuadraticProofSearchTimeMinFloat{79.22819805145263671875}
\def\SubcubicDirectQuadraticProofSearchTimeStdDevFloat{1.3980504769743919979418933507986366748809814453125}
\def\SubcubicDirectQuadraticProofTimeLen{1812}
\def\SubcubicDirectQuadraticProofTimeMaxFloat{4.7962067127227783203125}
\def\SubcubicDirectQuadraticProofTimeMeanFloat{4.592442951060288436337941675446927547454833984375}
\def\SubcubicDirectQuadraticProofTimeMedianFloat{4.46751432895660371968915569595992565155029296875}
\def\SubcubicDirectQuadraticProofTimeMinFloat{4.44956684112548828125}
\def\SubcubicDirectQuadraticProofTimeStdDevFloat{0.05957373844575723775829345640886458568274974822998046875}
\def\SubcubicDroppedSequencesFracLen{7852}
\def\SubcubicDroppedSequencesFracMaxFloat{0.45416146537232560120855850982479751110076904296875}
\def\SubcubicDroppedSequencesFracMeanFloat{0.1768033270601046813563783643985516391694545745849609375}
\def\SubcubicDroppedSequencesFracMedianFloat{0}
\def\SubcubicDroppedSequencesFracMinFloat{0}
\def\SubcubicDroppedSequencesFracStdDevFloat{0.115855650039206448109752045638742856681346893310546875}
\def\SubcubicDroppedSequencesLen{7852}
\def\SubcubicDroppedSequencesMaxFloat{523612519991512137}
\def\SubcubicDroppedSequencesMeanFloat{203840357853632416}
\def\SubcubicDroppedSequencesMedianFloat{0}
\def\SubcubicDroppedSequencesMinFloat{0}
\def\SubcubicDroppedSequencesStdDevFloat{133572470360406208}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6160115752259158750092638001660816371440887451171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.473386473749898062379770635743625462055206298828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1775705394483161614349597812179126776754856109619140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.090097537833757901371001253210124559700489044189453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.08145821186826486537402303156341076828539371490478515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.17293503544937760540989302171510644257068634033203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.11805571224286005860282244839254417456686496734619140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0837302573098448466026866299216635525226593017578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.082887050027262099138880557802622206509113311767578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0180308432850439133432463023609670926816761493682861328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{199380521269534832}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{136108969386471200}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{96534414238784848}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{95562262429854096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20788146969523088}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{17096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.28476821192052970133090639137662947177886962890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99920666217803955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{23447}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98149662815182414643544461796409450471401214599609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{17096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94802320003509510382144753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94792503118515003546207253748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{19093}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0109897986257447045910229377341238432563841342926025390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.47975550400728028677121983491815626621246337890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6052372}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6052372}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6052372}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{6052372}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{24.397350993377482808455170015804469585418701171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{11.0484061181229122894364991225302219390869140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6179135379654658866144245621399022638797760009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.473910296128787933422898959179292432963848114013671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.17798798395469095368071066332049667835235595703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0913664972212075710000789285913924686610698699951171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.08146238548218674713208287130328244529664516448974609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.3886256217956400860202847979962825775146484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9452643173419943423141376115381717681884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{6910}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.085705816745758056640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.4812791347503662109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.4059015745889842374793943235999904572963714599609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.73463344573974609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58302573968243098789798750658519566059112548828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.44960558414459228515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.446563243865966796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{23696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0609386227519898293625288943076157011091709136962890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6070823425929503525111385897616855800151824951171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.469329773210667322569378256957861594855785369873046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{27714}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.161303166536871100955607971627614460885524749755859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.08810089005800769701437502590124495327472686767578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.08071852404040147366259816408273763954639434814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.175609399482327510622070576573605649173259735107421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.12377362211725566332187753459947998635470867156982421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09145618384722058180624770784561405889689922332763671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08948303859269719773283924268980626948177814483642578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01788442765097857101164180448904517106711864471435546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{202463853074269919}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{142701270642065760}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{105441801086737984}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{103166919491085054}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20619341236398508}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.11057758331298828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.297075640286831088587859994731843471527099609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.480218231678009033203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{14929}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.448263645172119140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.51224755971247670771617777063511312007904052734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{11498}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.34437086092715230023486583377234637737274169921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99914473295211803094417746251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{23447}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98087493473330866766701774395187385380268096923828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94384522736072540283203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{19093}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94122815132141124383480246251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01111269301205830735412849463727980037219822406768798828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.5152811566603154869170566598768346011638641357421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7284693}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7284693}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7284693}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{7284693}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{24.79470198675496561691034003160893917083740234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{27714}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.87394229052546279490343295037746429443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6084665593469982258767458915826864540576934814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.469850756988938134117717027038452215492725372314453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{27714}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.161703389879376879800787492058589123189449310302734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.089341728089431582393586950274766422808170318603515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.08072668255743674359248274186029448173940181732177734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.2870800495147562969577847979962825775146484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9818328863737662004496087320148944854736328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{20976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{80.761123239994049072265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.2805917263031005859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.42489401747214206039870987297035753726959228515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7016022205352783203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58891206387652506037966304575093090534210205078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{2743}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4780347347259521484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4721610546112060546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{23696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.055499701323369766969850758187021710909903049468994140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.60344371438468413781919252869556657969951629638671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{29726}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.4542201082424426328287836440722458064556121826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{22401}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1578681351699084134398987089298316277563571929931640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0901582942619799931893709299401962198317050933837890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.08045033215053869202204595012517529539763927459716796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.190271981777587806394791414277278818190097808837890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{17096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1398893769914318074842896066911634989082813262939453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.10823470778335765596356310425107949413359165191650390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.10528382300084980494059294642283930443227291107177734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0178207773485035518568064816236073966138064861297607421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{219368659515543149}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{17096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{161281470999476032}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{124786122148271168}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{121383983624900737}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20545957433900336}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.95111083984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.271134603891940884068390005268156528472900390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{7310}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64434564113616943359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6082}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.634481906890869140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.46292293381569304955291954684071242809295654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.74834437086092719937369110994040966033935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99854719638824462890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12493}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98409666920339822215879621580825187265872955322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95206375420093536376953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95064401626586925164730246251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0114020273840471815518515796838983078487217426300048828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.56637037756888208850369892388698644936084747314453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7028661}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7028661}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7028661}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{7028661}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{26.317880794701988378392343292944133281707763671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{5.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.319640414783155080158394412137567996978759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6044561077310592889233475943910889327526092529296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29726}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.454725510872600990897041128846467472612857818603515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22401}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.15827305033582472759690062957815825939178466796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.09142810936027141732740375346111250109970569610595703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.08046027489566588697389448725516558624804019927978515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.0221202373504638671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9926218181256416528412955813109874725341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.079146862030029296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{24262}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.6291315555572509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.4500022063128643612373025462147779762744903564453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.8384621143341064453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58724950323041724686845554970204830169677734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{5358}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.473269522190093994140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24144}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.468800067901611328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05881494924003473345752723844270803965628147125244140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.60625882992351598499425335830892436206340789794921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{15399}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.461899764507573917793337159309885464608669281005859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.162985982503980386670860980302677489817142486572265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.09129687677057850281325812602517544291913509368896484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0797358891258702351390041940248920582234859466552734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1833958004852170031728775256851804442703723907470703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1334452073029378793567190086832852102816104888916015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{20539}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1003470522092643479883378176964470185339450836181640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.09740898852673519903166976519059971906244754791259765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0178849023601586505638483259872373309917747974395751953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{211440962233993550}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{153851849186275776}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{20539}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{115692274415966928}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{112304917614474671}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20619888538820660}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.9180507659912109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.6426645604190444061032394529320299625396728515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.75143182277679443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.745930433273314985598290149937383830547332763671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.44003606333357636604119988987804390490055084228515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.549668874172185351056896251975558698177337646484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99873387813568115234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12493}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98169150691948192655189586730557493865489959716796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{32103}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95448003709316253662109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{5928}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95294559001922596319644753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01159536121588620148636916695750187500379979610443115234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.5833080101683389973032944908482022583484649658203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6270451}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6270451}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6270451}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6270451}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{25.900662251655628409707787795923650264739990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{5.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.541469648150570748157406342215836048126220703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.60723123029801140404515535919927060604095458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{15399}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.46241302023959907074868169729597866535186767578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.163398030346182332461779651566757820546627044677734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0925827279892502408298327054581022821366786956787109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0797383474943161030257243737651151604950428009033203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{89.8407781124114990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9325436440524725867362576536834239959716796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{80.914862811565399169921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.666733264923095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.468466625099761113659724287572316825389862060546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7827155590057373046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5902048009910334513961061020381748676300048828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{1412}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.466132640838623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{28778}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4613654613494873046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.058370995610024296873508120597762172110378742218017578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.37600663789785648827290742701734416186809539794921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.2732999145462124968020134474500082433223724365234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.089561035636802899251307508166064508259296417236328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.044735253986640501067117980937837273813784122467041015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.050468815836575843525313445070423767901957035064697265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.447500816358302577757655171808437444269657135009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.375589574676921611473545681292307563126087188720703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.315563101309467353150495227964711375534534454345703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.309279266565292976221002163583762012422084808349609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0250244335959945128633474809021208784542977809906005859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{515933314508606502}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{433025297551162176}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{363819485560113984}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{356574717352159758}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{28851207633428124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{155.63616943359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.4297275164269507286007865332067012786865234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.906459808349609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.7463226318359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59340187814654488107635188498534262180328369140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{22}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{13.0662251655629138014091950026340782642364501953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{913}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{29022}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99830752413793899524563357772422023117542266845703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.988555908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98670303821563720703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{29022}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00159832861794918790199204750024364329874515533447265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.12730241196438196737972248229198157787322998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5740147}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5740147}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5740147}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5740147}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{45}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{38.15894039735099596555301104672253131866455078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{10.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{10}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.5223400073571298207752988673746585845947265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.376177219312338440015963669793563894927501678466796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.273602187428533483171122497878968715667724609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.08976920600607617151123207577256835065782070159912109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.045365318046782031335961704598958021961152553558349609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.050478511677920660793983387293337727896869182586669921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.27426624298095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9472475383455360997686511836946010589599609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{14929}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{80.745534956455230712890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.657550811767578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3739331158273595523411358954035677015781402587890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7563436031341552734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5881835419610634829723494476638734340667724609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{22286}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.47997188568115234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.479328155517578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{28778}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0620149568924732441654867898250813595950603485107421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.60332225551732421298112285512615926563739776611328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{29726}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.454064344367994088269568919713492505252361297607421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.157856206252155184532881548875593580305576324462890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.090236002460756303822364543520961888134479522705078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0807900003362082841373847941213170997798442840576171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.190541277704504297130227996603935025632381439208984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{17096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.13998292116256172423760517631308175623416900634765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1085301494932228993928191584927844814956188201904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1059100694950426968521384196719736792147159576416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.017762051691715706469576474546556710265576839447021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{219679136580788189}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{17096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{161389320086002368}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{125126743248932640}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{122105996675240383}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20478251361317460}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.51984310150146484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.3223633639859837529684227774851024150848388671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{23447}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64782559871673583984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.627370357513427734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6082}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.4404406740468065351024051778949797153472900390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.74834437086092719937369110994040966033935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99854719638824462890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12493}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98408723430128286491225253485026769340038299560546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95159031450748443603515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95052838325500477179019753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0114447188944052750947388830127238179557025432586669921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.56637037756888208850369892388698644936084747314453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7036980}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7036980}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7036980}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{7036980}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{26.23178807947019919311060220934450626373291015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{5.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.3081294406095427262926023104228079319000244140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.60433444509299760749598817710648290812969207763671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29726}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.45456964920507247907011105780838988721370697021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1582613747691493377711680068387067876756191253662109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.09150691202345474783985679323450312949717044830322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.080801206677723058646733989007771015167236328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.1391112804412841796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.949780086807862744535668753087520599365234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{26374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{80.443201839923858642578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.3132793903350830078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.382870107307653473327491155941970646381378173828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.721947193145751953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58632100970539813289406083640642464160919189453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{1412}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.471485078334808349609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{27584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4690730571746826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24144}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.056248029664033527552646773983724415302276611328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.606724859353612533396926664863713085651397705078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{15399}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.461800280971488896764043374787434004247188568115234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1629859612766577370290832504906575195491313934326171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.09129679178855709675843854711274616420269012451171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.079724072164482351343650634589721448719501495361328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.183429388051791597558093371844734065234661102294921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1335239386724149657226234921836294233798980712890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8840}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.10018514957047119917632471697288565337657928466796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.09634080776981350513477053709721076302230358123779296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.017899760195160645259715437305203522555530071258544921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{211479686061784808}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{153942620275233088}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8840}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{115505613382049696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{111073389049012393}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20637018456306356}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.87827014923095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.65154951139791084102625973173417150974273681640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17080}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.79167711734771728515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.74662494659423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.4412442825297662185590752415009774267673492431640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.543046357615894148551660691737197339534759521484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99873387813568115234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12493}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98134106200262405383938357772422023117542266845703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9508850872516632080078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94561123847961436883480246251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{29195}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0119507811483053512369156834438399528153240680694580078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.58383408849097195858490749742486514151096343994140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6295408}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6295408}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6295408}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6295408}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{25.834437086092716384655432193540036678314208984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{5.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.5217721064128202357323971227742731571197509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.60769800720949707084628244047053158283233642578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{15399}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.46231347964396152239174853093572892248630523681640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1633980088196436974978809075764729641377925872802734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.09258264181031783390807277100975625216960906982421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.079726753533921890237934348988346755504608154296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.1097221374511576641452847979962825775146484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9802401507927100965389399789273738861083984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{80.96417105197906494140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.4172875881195068359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.414767287114880645049197482876479625701904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.73500347137451171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{6159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58845692280902017756716304575093090534210205078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{8745}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4830443859100341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4824993610382080078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24144}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.056300404553734494095262874679974629543721675872802734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.377146260341494621304292422792059369385242462158203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.273798302543121041541240856531658209860324859619140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{5615}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.08842960479096963199996395132984616793692111968994140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0456107557761721016387213012421852909028530120849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.050760975068059648040996734152940916828811168670654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.446956503193125687101172616166877560317516326904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.3754983647381961997524513208190910518169403076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.31524700807104399924440940594649873673915863037109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.3086802924016363025572218248271383345127105712890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.025020966638300508322334536615016986615955829620361328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{515305764155233530}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{432920139651371904}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{363455054868074944}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{355884147158175998}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{28847210503347144}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.4159393310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.266749906224134747390053234994411468505859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.3579044342041015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.61283111572265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59797218712847044486125014373101294040679931640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{22}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{13.019867549668873607515706680715084075927734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{913}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{29022}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9982686780935881021292743753292597830295562744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{22545}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98860338330268848761051003748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4157}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.986570894718170166015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{29022}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00175021570304948934602984333963604512973688542842864990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.126683824271293321572784407180733978748321533203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5752434}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5752434}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5752434}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5752434}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{45}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{38.086092715231785632568062283098697662353515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{10.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{10}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.49567915789612726484847371466457843780517578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.377317358763892940487494342960417270660400390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.274100974818711151659300639948924072086811065673828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.08863998517598208060075393177612568251788616180419921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.046253150652907144835257469139833119697868824005126953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.050769164802911874445623396923110703937709331512451171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.6886188983917236328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.979990673380967791672446765005588531494140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{80.9497392177581787109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.62659740447998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.442723620705475440217924187891185283660888671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.72400569915771484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58605424142041773194478082587011158466339111328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.471990168094635009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{28778}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.46855926513671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24144}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.06033923062659062030999024273114628158509731292724609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.37427456144393811410253647409263066947460174560546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.270901698993869566312042707068030722439289093017578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{16284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0890910657564952523923551552798016928136348724365234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.046345249773301198936703571007456048391759395599365234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.050532643969846073594975877085744286887347698211669921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.45416146537232560120855850982479751110076904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.378801684148758421866176604453357867896556854248046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.316078824369940114547006260181660763919353485107421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.309578046761052882995812751687481068074703216552734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0250343333614663730857241574767613201402127742767333984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{523612519991512137}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{436728607636394240}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{364414073766954688}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{356919187465001997}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{28862621285931196}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.3029937744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{92.8864845124301581336112576536834239959716796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{81.2790679931640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{80.37683868408203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.6339667658878003209110829629935324192047119140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{22}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{13.350993377483444390918521094135940074920654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9983517701262669685746686809579841792583465576171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{23447}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99053774774074554443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98490077257156360968082253748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{29022}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0015559783784153606404909719884699370595626533031463623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.211345446119928670469789722119458019733428955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5766864}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5766864}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5766864}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5766864}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{45}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{38.33112582781456723068913561291992664337158203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{11}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.51300087283473683186230118735693395137786865234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.374444357074282974107148902476183138787746429443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.27120045504061440766463420004583895206451416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{16284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.08930434116838363578505521900297026149928569793701171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.046997989472714989112045458341526682488620281219482421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0505402750584041104975341340832528658211231231689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.8196580410003662109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.99779003661200249553075991570949554443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{32382}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{80.991009414196014404296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.371208667755126953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.43516035670530062162697504390962421894073486328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.73589038848876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58749788170618710836379250395111739635467529296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{29195}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.46659862995147705078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.451401233673095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24144}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.058875920734622687324755219151484197936952114105224609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.56686235252430294817571621024399064481258392333984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.41165576436815598526663961820304393768310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{29052}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.138759842866603866351482565733022056519985198974609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.08779767939409789667681849323344067670404911041259765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07617266506263499492579427396776736713945865631103515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.295947151523005713702474395176977850496768951416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.2016802096970452817803476364133530296385288238525390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{30899}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.149470893762314371855381978093646466732025146484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22545}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1465570256708186025473850122580188326537609100341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20751}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.024847973683692743673834257833732408471405506134033203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{341203835218014245}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{232521450813341920}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{30899}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{172328207731377728}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22545}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{168968746547104466}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20751}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{28647763205834372}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{33.5944671630859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{13.575011654405404470935536664910614490509033203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{8.01591932773590087890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{22545}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{7.73836469650268465869658029987476766109466552734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.60855280594514926661986464750953018665313720703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{5.0728476821192050039144305628724396228790283203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{913}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{913}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99936711788177479132144753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{23447}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98667701230143867174859906299388967454433441162109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{22401}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95886051654815684930355246251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{22261}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.955898284912109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{12493}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00915364405730975834452056716372680966742336750030517578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.7728791767361673503700103537994436919689178466796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{8235030}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{8235030}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{8235030}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{8235030}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{39}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{9504}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{30.73509933774834479436321998946368694305419921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.8425752517611204694958360050804913043975830078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.56711951868086540873292733522248454391956329345703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.412111682040763371848157703425385989248752593994140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29052}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.13914447806600793722253683881717734038829803466796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.08903424692016066732680457107562688179314136505126953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0761761832556604734367766695868340320885181427001953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.401337146759033203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9898743803137932673053001053631305694580078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.048664033412933349609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.51245021820068359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.474748480819587204138088054605759680271148681640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7258255481719970703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58417536565010141913489860598929226398468017578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4670994281768798828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{27584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{4.46478557586669921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05765119615083059978477564300192170776426792144775390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.7272280932522534602213681864668615162372589111328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{13293}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.64509377796271605287614647750160656869411468505859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{6155}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.55603959535268032698951401471276767551898956298828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.5302661982607419499657908090739510953426361083984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0350687207264081257651611167602823115885257720947265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1594002234673694007316413490116246975958347320556640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.110693763814015799784584714871016331017017364501953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8840}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.07818066742335937069352524986243224702775478363037109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0702618070916976034112622073735110461711883544921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0175385359768064803820397656863860902376472949981689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{183775945474667193}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{127621220727050112}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8840}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{90136172716907008}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{81006348348556030}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20220555286981044}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.198675496688741848316794857964850962162017822265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9993808269500732421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{18146}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9853124914579833859562540965271182358264923095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6910}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95311392843723297119140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.951040089130401611328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{30684}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00907503839054670836949956225225832895375788211822509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.4152692822937982253250766007113270461559295654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6161236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6161236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6161236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{6161236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{27.582781456953643584029123303480446338653564453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{11498}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.853747375807774488976065185852348804473876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7278931601632818715330586201162077486515045166015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{13293}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.64585527726730751485462178607122041285037994384765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{4647}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.55823963837229639839421224678517319262027740478515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.53773461844522885133557110748370178043842315673828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.034886473642951554285929205434513278305530548095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.25670337677001953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.4992156060326209399136132560670375823974609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.653380095958709716796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.5980319976806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8745}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.49539125222222413214012703974731266498565673828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.813351154327392578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.6097862341546065323427683324553072452545166015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.493856847286224365234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4934060573577880859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{27584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.06227701956413887740549029103931388817727565765380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.71568685958703659455437673386768437922000885009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{13293}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.63981971575138663066439903559512458741664886474609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{19451}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.5512409515489145039879304022178985178470611572265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.526910607047787582501996439532376825809478759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0341686403667478544310398547168006189167499542236328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.16493197282667348968487885940703563392162322998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1164187819481792285358778826775960624217987060546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{26278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08301422380630586739247434024946414865553379058837890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0760654705112893958496300683691515587270259857177734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.017442463172553601680192514322698116302490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{190153618269104040}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{134221717248191264}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{26278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{95708883814535792}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{87697516710503563}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20109790884950016}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.11057758331298828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.297075640286831088587859994731843471527099609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.480218231678009033203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{14929}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.448263645172119140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.51224755971247670771617777063511312007904052734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{11498}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.25165562913907280062630889005959033966064453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99917298555374156610042746251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98407909846463736958099843832314945757389068603515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29726}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95039625465869892462222878748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95038396120071400030582253748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0095035714525852181544518515465824748389422893524169921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.47755646032635612474592790022143162786960601806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7393557}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7393557}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7393557}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{7393557}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{13654}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{28.21192052980132558559489552862942218780517578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.4865372711496203095293822116218507289886474609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7163413717729458785044016622123308479785919189453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{13293}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.64057530325524980607809766297577880322933197021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{17194}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5534335731371389233146373953786678612232208251953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.53433176612977939523574377744807861745357513427734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03398828485707239277502367258421145379543304443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.8867824077606201171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.57396780891923526723985560238361358642578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.02673590183258056640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.713016510009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.468124038268110442828628947609104216098785400390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.797620296478271484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61135531892839622969404445029795169830322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.501071453094482421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.486188411712646484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{27584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.059122251169258573100240283793027629144489765167236328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.70629906425320643226228867206373251974582672119140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{20751}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.621712063702317241364880828768946230411529541015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{23367}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.52871452793826112515063186947372741997241973876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.463980632746680610178913184427074156701564788818359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0337145155934381046680670124260359443724155426025390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1778672185866154997757604405705933459103107452392578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1329605442918657398632120703041437081992626190185546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.10324534963670585485662201108425506390631198883056640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.09991843451896069427942137508580344729125499725341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0170671897307164942281243469324181205593049526214599609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{205066941273115681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{153293070778323200}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{119033783846810928}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{115198111863560950}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19677130063748180}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.95111083984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.271134603891940884068390005268156528472900390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{7310}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64434564113616943359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6082}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.634481906890869140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.46292293381569304955291954684071242809295654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.5695364238410594026618127827532589435577392578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99970901012420643194644753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.984475948163215708319739860598929226398468017578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95492327213287353515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95234334468841563836605246251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0114542465639567610236060346551312250085175037384033203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.56976739502615725285750158946029841899871826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7137525}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7137525}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7137525}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{7137525}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{28.9735099337748351899790577590465545654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.82164344772959108098575597978197038173675537109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.70685347139818366368757551754242740571498870849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20751}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6224426660991440041215128076146356761455535888671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6155}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5308612886976475930822516602347604930400848388671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.47051546814479217051285786510561592876911163330078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.033505087705223597638326538117325981147587299346923828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.8712635040283203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.4751506657000419409087044186890125274658203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.787262380123138427734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8745}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.6612627506256103515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.4808686017108285692955860213260166347026824951171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7509796619415283203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.60990477239848761570328861125744879245758056640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{29195}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.486469745635986328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.47908687591552734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.057224728537499859604142926627901033498346805572509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.706510910515920631524977579829283058643341064453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{20751}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.63064822636265083222184557598666287958621978759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.53563993933864839647185362991876900196075439453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.482873423746763286157346328764106146991252899169921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03390506054097321142482002187534817494451999664306640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.17458839986451069048456474774866364896297454833984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.126476477041986001825790708608110435307025909423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12141}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09223638983653292822140201678848825395107269287109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08989582113857770562237448075393331237137317657470703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0172997738980899228022902747170519432984292507171630859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{201286720658693607}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{145817450208619872}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12141}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{106341317349839312}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{103642825364957067}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19945281351944092}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.9180507659912109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.6426645604190444061032394529320299625396728515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.75143182277679443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.745930433273314985598290149937383830547332763671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.44003606333357636604119988987804390490055084228515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.40397350993377489913882527616806328296661376953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99921888113021839483707253748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9827433714014015553317449302994646131992340087890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94368542730808258056640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.937711656093597412109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.011559311941416815228134140625115833245217800140380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.554079487770910983357453005737625062465667724609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6379315}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6379315}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6379315}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6379315}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{13654}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{28.5165562913907280062630889005959033966064453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.143460631376459701868952834047377109527587890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.70706548394893020681450934716849587857723236083984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20751}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6313900258901019579838020945317111909389495849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5381905396163733090730829644598998129367828369140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.4896743505949976427160663661197759211063385009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.033695054650443208299481767653560382314026355743408203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.9430687427520751953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.4863461484972191328779445029795169830322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{23633}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.70212018489837646484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8745}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.699162960052490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.4438809296253569680601458458113484084606170654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.74775218963623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61505038848775939186452887952327728271484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.48490893840789794921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{27584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4790942668914794921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05925659207367157954582381762520526535809040069580078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.452765236172162299776999816458555869758129119873046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.375667607524545754671407848945818841457366943359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{19488}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.299101269076867459784097036390448920428752899169921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.298704890241176912457632397490669973194599151611328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03204206882851969029335492678001173771917819976806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.442430165688019183534152034553699195384979248046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.3718297144393403197426550832460634410381317138671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.313764000711625357098455424420535564422607421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.312067782318491915294345062648062594234943389892578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.024318709116649857293612768671664525754749774932861328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{510087252308487706}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{428690473828938496}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{361745263791910912}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{359789657129957705}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{28037562704864196}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{155.63616943359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.4297275164269507286007865332067012786865234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.906459808349609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.7463226318359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59340187814654488107635188498534262180328369140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{21}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{27584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{12.6953642384105958029749672277830541133880615234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99825517428631815874950916622765362262725830078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99062334001064311639339621251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{15399}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98981308937072765008480246251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{29022}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0014688915238626515553932438962192463804967701435089111328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.9291880647528081293984314470435492694377899169921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5849011}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5849011}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5849011}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5849011}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{45}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{27584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{37.85430463576158643945746007375419139862060546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{10.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{10}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.3021592468599703096288067172281444072723388671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.4530908967517943697345117470831610262393951416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.37611486662771642652813852691906504333019256591796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.29935243822459423057580352178774774074554443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.29891316508851006883418222059844993054866790771484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.032035098261232901328821043307470972649753093719482421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.3435821533203267108547152020037174224853515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.451053707804902614952879957854747772216796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.53683817386627197265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8745}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.093149662017822265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5080456505612114259662348558777011930942535400390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.8899013996124267578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61202436093463052912966304575093090534210205078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{31308}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.490885436534881591796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{28778}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4786121845245361328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.060596704415427658785286979536977014504373073577880859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.706158060369256102006829678430221974849700927734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{20751}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.6216492273318630079614877104177139699459075927734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{8840}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.52781533219656850963730221337755210697650909423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.462276212696232813303964803708367981016635894775390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.033967988585604784457228078053958597593009471893310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.177740454994085694817584908378194086253643035888671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1330725354148796502062879199002054519951343536376953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.10328599376536252985037123153233551420271396636962890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.10008101103210780002950031075670267455279827117919921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0170520336731758807846670578101111459545791149139404296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{204920792801286922}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{153422187752371008}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{119080643336775200}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{115385549821712224}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19659656319084560}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.51984310150146484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.3223633639859837529684227774851024150848388671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{23447}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64782559871673583984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.627370357513427734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6082}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.4404406740468065351024051778949797153472900390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.5695364238410594026618127827532589435577392578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99970901012420643194644753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.984483216772016334061845554970204830169677734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95537306368350982666015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.953155457973480224609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.011424997901232018804318357751981238834559917449951171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.56976739502615725285750158946029841899871826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7145844}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7145844}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7145844}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{7145844}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{28.827814569536425182150196633301675319671630859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.002285757400755983326234854757785797119140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7067123568336948213897130699479021131992340087890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20751}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.62237959406511766946579200521227903664112091064453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8840}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.52977452804772529049159857095219194889068603515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.468787042556843835949820231689955107867717742919921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03375922217260483859657682614852092228829860687255859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.98644351959228515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.47421572539980161309358663856983184814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.35150563716888427734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.2977759838104248046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.4902323435688760167039390580612234771251678466796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7737987041473388671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61237361099546294695983306155540049076080322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{23241}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.505397260189056396484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4936010837554931640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{28778}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.057145723144231198864506637846716330386698246002197265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.7071478801984605322417110073729418218135833740234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{20751}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.63067786305818029912728661656728945672512054443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{23241}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.5366942916768453475384603734710253775119781494140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.483181906375472980386120980256237089633941650390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.034003318294972488533556287393366801552474498748779296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1747725338514987958316027061300701461732387542724609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.12658201644568556343273257880355231463909149169921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09249158911242059966095752088222070597112178802490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.090062040307330504251837055562646128237247467041015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0172872693556330413178212523916954523883759975433349609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{201499012692021156}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{145939128856728512}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{106635542082970272}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{103834463019090060}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19930864596040276}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.87827014923095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.65154951139791084102625973173417150974273681640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17080}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.79167711734771728515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.74662494659423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.4412442825297662185590752415009774267673492431640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.41059602649006610164406083640642464160919189453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99921882152557361944644753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98280589233171067320427027880214154720306396484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{22401}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94364525377750407830745871251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9376981258392333984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01164253674513581436611442398998406133614480495452880859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.5551865407982699007760629683616571128368377685546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6404272}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6404272}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6404272}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6404272}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{13654}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{28.5165562913907280062630889005959033966064453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.143460631376459701868952834047377109527587890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.70770295361874324679973824459011666476726531982421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20751}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.63141972899586018552753330368432216346263885498046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{23241}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5392479809490693387630244615138508379459381103515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.489987177980922450348799657149356789886951446533203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.033794475152848148236106595732053392566740512847900390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{89.9318244457244873046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7790}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.4651534904707403939028154127299785614013671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{17096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.58737623691558837890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.5710837841033935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.4294813574512257314808039154740981757640838623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7890017032623291015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61624582713802933398028471856378018856048583984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.499858558177947998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{27584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.490185260772705078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24144}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.060186186094211731323344594102309201844036579132080078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.44944535441514588125500040405313484370708465576171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1412}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.375080974721800686211281572468578815460205078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.3009378162643143728161021499545313417911529541015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2984694378137648929083525217720307409763336181640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.031522938286836311994054682372734532691538333892822265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.442518480528161284315302737013553269207477569580078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.371796828144926261305869275020086206495761871337890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.313757244112318367523783990691299550235271453857421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.31216960451281938748735456101712770760059356689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0243378004916488359377080286094496841542422771453857421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{510189072386863500}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{428652558512901760}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{361737473963271936}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{359907050127444185}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{28059573561653036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.4159393310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.266749906224134747390053234994411468505859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.3579044342041015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.61283111572265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59797218712847044486125014373101294040679931640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{21}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{27584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{12.6821192052980133979644961073063313961029052734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9982602548915029405662835415569134056568145751953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4647}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9906609058380126953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{15399}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.989690840244293212890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{29022}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00145108976164106426125222082390564537490718066692352294921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.899358068370156527038261629058979451656341552734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5861298}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5861298}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5861298}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5861298}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{45}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{27584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{38.01324503311258240501047112047672271728515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{10.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{10}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.3184292505046784071964793838560581207275390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.449888419526173588547379722513142041862010955810546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1412}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.375528042250566407300738092089886777102947235107421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{27484}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.301161817745985216365767200841219164431095123291015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.298734227310712696645822461505304090678691864013671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03151992114612645057292183992103673517704010009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{89.6066195964813232421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7790}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.4779211416939261880543199367821216583251953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.392186701297760009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8745}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.7109158039093017578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.4936237521449611254098499557585455477237701416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7771575450897216796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61147139246100579157428001053631305694580078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.490291595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{27584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.488025665283203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{28778}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0580198659442092701254978237557224929332733154296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.44722978542810032376308981838519684970378875732421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.37185186019559679504453697518329136073589324951171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.295602792269287151238899014060734771192073822021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.28871100852736741870785408536903560161590576171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03217800792714786695114526082761585712432861328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.449019502187882280086483888226212002336978912353515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.375168050804586761248771153987036086618900299072265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.315918989249970028065916949344682507216930389404296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.31315265063477681906078942120075225830078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0242517706668881095899426014739219681359827518463134765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{517684240060270752}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{432539313614042176}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{364229796419949824}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{361040425141469186}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{27960387926648836}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.3029937744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{92.8864845124301581336112576536834239959716796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{81.2790679931640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{80.37683868408203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.6339667658878003209110829629935324192047119140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{22}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{27584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{13}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{10}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{10}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99841449829126827086867024263483472168445587158203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{27484}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99317924678325653076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9910409450531005859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2773}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00113879932174759147811560211493997485376894474029541015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.94969856729476465062589340959675610065460205078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5875728}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5875728}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5875728}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5875728}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{45}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{27584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{38}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{10.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{10}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.33986602167540613805840621353127062320709228515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.447691587786299416418245300519629381597042083740234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3722951007892201236160190092050470411777496337890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.295877329708175207390041805410874076187610626220703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.28901630519327847768096262370818294584751129150390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.032177588166553257320590120116321486420929431915283203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.69683170318603515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.4937166046622536441645934246480464935302734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22261}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.442661285400390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.0155842304229736328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5625734027202435871828356539481319487094879150390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7988169193267822265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.6100508929877879182868127827532589435577392578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{29195}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.504387378692626953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4995372295379638671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{27584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.053910585943680124076937687505051144398748874664306640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.66095228150124218924332808455801568925380706787109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{15399}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.561675751211015761299449877697043120861053466796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{4305}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.477662253277391590788880648688063956797122955322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.465980721156154686912742590720881707966327667236328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{1696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.037476812389583412377103144308421178720891475677490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.29388371351424869004631545976735651493072509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1953914767248114137121461908463970758020877838134765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.145554166984522115324551805315422825515270233154296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{22545}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.14481931843510731372504096725606359541416168212890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{20751}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0245519580844160527355324319387364084832370281219482421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{338824853164295172}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{225271035332923360}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{167812529201591488}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{22545}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{166965306506342046}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{20751}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{28306480455729204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{33.5944671630859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{13.575011654405404470935536664910614490509033203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{8.01591932773590087890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{22545}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{7.73836469650268465869658029987476766109466552734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.60855280594514926661986464750953018665313720703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.9470198675496686036012761178426444530487060546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99947369098663318975894753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{23447}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98804100341354772485402691017952747642993927001953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96388305723667144775390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12141}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96157193183898914679019753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{12493}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00874174120298574532095248201812864863313734531402587890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.79558449894999772045167674150434322655200958251953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{8343894}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{8343894}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{8343894}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{8343894}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{39}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{13654}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{32.5629139072847664237997378222644329071044921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{5.33956388692202299495193074108101427555084228515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.66201240667275762508126035754685290157794952392578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{15399}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.56234242529490263695635121621307916939258575439453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{4305}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.47800458572059600914627708334592171013355255126953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.46634274211755410988189396448433399200439453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0373996541687392769492959132549003697931766510009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.97549533843994140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.4949708127028173976214020512998104095458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.70245778560638427734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.6616342067718505859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.451475357841811142378674048813991248607635498046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.74783420562744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61015065932115941649271917412988841533660888671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{29726}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.49000322818756103515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{4.489861965179443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.055129027389446909335202207103066029958426952362060546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.1915228280621887879675568910897709429264068603515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.028385347704761094977943258754748967476189136505126953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002667137344314340907658333890140056610107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04281651636621632006640680856435210444033145904541015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1782419365093134977495736848140950314700603485107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.118968000930316952779008943252847529947757720947265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{24202}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0735332660287725536907288415022776462137699127197265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.071739921126955097374633396611898206174373626708984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0173873982842286146921484402128044166602194309234619140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{205498961624355912}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{137160766632649840}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{24202}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{84778083708548016}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{82710497806065609}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20046305391051368}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.6887417218543046004697316675446927547454833984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99681425094604481085269753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.979217225352659870196703195688314735889434814453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{30684}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94767718017101287841796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{19004}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.942640125751495361328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{19488}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01251722639864144386023792065998350153677165508270263671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.504094893615498307326561189256608486175537109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5788021}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5788021}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5788021}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{5788021}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{3284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{13.139072847682118805323625565506517887115478515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{5.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.7670664104376641034832573495805263519287109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.1917729220310550319883446945823379792273044586181640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.028414001062487363735709067213974776677787303924560546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000026699832275826737798156451452898750299072577700358090135868138759178691543638706207275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2345}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000026054821497037114438219634609030939328582006345885226095138165192111046053469181060791015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.04286069620567158067192536918810219503939151763916015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{92.4898955821990966796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.95646531692403868873952887952327728271484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15043}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{80.836852848529815673828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.1151092052459716796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.535412247392867524098392095766030251979827880859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7503879070281982421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{13293}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5751048523858681704723494476638734340667724609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{5358}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.458415508270263671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4545810222625732421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.06016387574730701348624251068031298927962779998779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.190687213244917497245722870502504520118236541748046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0282689494500146069888568689520980115048587322235107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002667137344314340907658333890140056610107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04316909029291675359285562763034249655902385711669921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1813609935356338132006470686974353156983852386474609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.12290681166104379384851341683315695263445377349853515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{24202}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.078098552549267619138362306330236606299877166748046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07790547852922920235574366643049870617687702178955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.017711238529401686359054934882806264795362949371337890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{209094989544095622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{141701906226681024}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{24202}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{90041500712718608}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{89818901523035359}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20419667773768556}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.11057758331298828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.297075640286831088587859994731843471527099609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29110}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.480218231678009033203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{14929}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.448263645172119140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{19538}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.51224755971247670771617777063511312007904052734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.84768211920529790148748361389152705669403076171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1681}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1681}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99755263328552234991519753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13654}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9817657048339085701371686809579841792583465576171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1185}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95011062920093536376953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24202}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94496440887451160772769753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01106522428193369884941166247926958021707832813262939453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.45671363310110379973849603629787452518939971923828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7020342}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7020342}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7020342}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{7020342}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{3284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{13.5695364238410594026618127827532589435577392578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{16069}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{5.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.89639404126273092288101906888186931610107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.190936216052859430991617273321026004850864410400390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.02829746738215045687159232556950883008539676666259765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000026699832275826737798156451452898750299072577700358090135868138759178691543638706207275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2345}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000026054821497037114438219634609030939328582006345885226095138165192111046053469181060791015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.04321338433098607934024215637691668234765529632568359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{92.1987555027008056640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9389438613361136276580509729683399200439453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{23633}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.133028686046600341796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.9580290317535400390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5316024309261908609158808758365921676158905029296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.68649578094482421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{18146}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5777703468373278639091950026340782642364501953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{1951}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4701092243194580078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.46013927459716796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{27584}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05472165047547254690396556497944402508437633514404296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.188217795055852288310660469505819492042064666748046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.02775791697087028053747559397379518486559391021728515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{20751}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002667137344314340907658333890140056610107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.043235218974038973349660608391786809079349040985107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1907180067200645867675490308101871050894260406494140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1350030945604213938882054435453028418123722076416015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29565}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0892883018288179730603815187350846827030181884765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0889852407853302940221595918046659789979457855224609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.018574279370263131749840823658814770169556140899658203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{219882891263315674}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{155647970907181504}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29565}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{102942403288271168}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{102592997694025669}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{21414686118551692}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.95111083984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.271134603891940884068390005268156528472900390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{7310}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64434564113616943359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6082}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.634481906890869140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.46292293381569304955291954684071242809295654296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.0662251655629138014091950026340782642364501953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.997880160808563232421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{6082}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98234707353920336370123322922154329717159271240234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{20539}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94714675843715678826839621251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{21598}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.944597899913787841796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00912665620930452892167750178487040102481842041015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.393134359725982263089605339700938202440738677978515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6764310}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6764310}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6764310}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{6764310}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{123}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.3112582781456953995302683324553072452545166015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{29726}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{6}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{9.2837431295898280581013750634156167507171630859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.1884635732529113261168873805218026973307132720947265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0277858042058684064079532305413522408343851566314697265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20751}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000026699832275826737798156451452898750299072577700358090135868138759178691543638706207275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2345}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000026054821497037114438219634609030939328582006345885226095138165192111046053469181060791015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.04327889679140527190437381932497373782098293304443359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.5552415847778462421047152020037174224853515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9706997366140939220713335089385509490966796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{17096}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.195648491382598876953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.002455234527587890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{24262}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.502730649760085857025160294142551720142364501953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.6966373920440673828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{18289}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5788344484291325642288938979618251323699951171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{32374}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.463824748992919921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.454077243804931640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.056244105600983453074892537415507831610739231109619140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.186702124896788002050840304946177639067173004150390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0279095223026066541205381099644000642001628875732421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002667137344314340907658333890140056610107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.042958628409511402657106060587466345168650150299072265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1876685410055217995139997810838394798338413238525390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.13018346707896044645025313002406619489192962646484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{10248}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0864806289878475575871874525546445511281490325927734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08289307135516339741787561479213763959705829620361328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.018313921859880455400571008794941008090972900390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{216367096663458052}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{150091318739611040}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{10248}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{99705376892015744}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{95569204548277771}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{21114514345945600}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.9180507659912109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.6426645604190444061032394529320299625396728515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{13716}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.75143182277679443359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27300}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.745930433273314985598290149937383830547332763671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{18289}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.44003606333357636604119988987804390490055084228515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.97350993377483430180063805892132222652435302734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1681}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1681}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99728471040725719110042746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13654}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98193719805471157968668194371275603771209716796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{9134}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95008398592472076416015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{1681}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94800353050231922491519753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{14095}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.010577893877540545108928426998318172991275787353515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.444942437940154367215228603527066297829151153564453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6006100}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6006100}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6006100}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6006100}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{3284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.0596026490066225989039594423957169055938720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{20415}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{5.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{9.1196838187897153460426125093363225460052490234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.1869459239043717857509108171143452636897563934326171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.02793757406318612968032510934790479950606822967529296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000026699832275826737798156451452898750299072577700358090135868138759178691543638706207275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2345}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000026054821497037114438219634609030939328582006345885226095138165192111046053469181060791015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.04300242099550809216079727548276423476636409759521484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.4279124736786030780422152020037174224853515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.021571868302800112360273487865924835205078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{9134}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.07873547077178955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.005058765411376953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{24262}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5480026161721405220106362321530468761920928955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.6829464435577392578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58157371843098015773421138874255120754241943359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{21598}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.450608789920806884765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4489467144012451171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.055457870739419982963891442295789602212607860565185546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.09304381099645879504844714347200351767241954803466796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0165448009673827833854176105887745507061481475830078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{6532}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002667137344314340907658333890140056610107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.02173481936088929311612361061634146608412265777587890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.409953339499774915832830401996034197509288787841796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.318616350054406416436592053287313319742679595947265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.20893895829248887441309534551692195236682891845703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1929158140843532931452131151672801934182643890380859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{19538}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.03809936012507410263427942709313356317579746246337890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{472644020994682019}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{367339641697068160}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{240890218165563520}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{222416790636587430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{19538}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{43925571599958544}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{155.63616943359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.4297275164269507286007865332067012786865234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{4729}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.906459808349609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.7463226318359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59340187814654488107635188498534262180328369140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{22}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29565}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{12.9072847682119213885698627564124763011932373046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{17194}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99877579954286288543841010323376394808292388916015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{12141}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98887051641941081658870871251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20976}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98604261875152598992855246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00192290346737250734433788412758303820737637579441070556640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.072688989545679039139258748036809265613555908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5475796}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5475796}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5475796}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5475796}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{45}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{8840}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{30.5430463576158928162840311415493488311767578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{23633}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{10}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{10}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.647721579082801923732404247857630252838134765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0931653092857540610083333376678638160228729248046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0165612432032007962645625553932404727675020694732666015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6532}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000026699832275826737798156451452898750299072577700358090135868138759178691543638706207275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2345}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000026054821497037114438219634609030939328582006345885226095138165192111046053469181060791015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0217556806492133041064374054940344649367034435272216796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.5081684589385986328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9852694975619300521429977379739284515380859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{11124}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{80.86650943756103515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{24262}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.42235565185546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5240570133745368064381864314782433211803436279296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.6961882114410400390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{18289}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5803921222686767578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{29195}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.46347320079803466796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.459115505218505859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.058018962776232300970757904678976046852767467498779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.1858470025911174994259766890536411665380001068115234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.02771664708206074412277786223057773895561695098876953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{20751}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002667137344314340907658333890140056610107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.043169869368388770480837735021850676275789737701416015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1919158859089453994517526780327898450195789337158203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1350731314932046844834445664673694409430027008056640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29565}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0899933706972938785018101270907209254801273345947265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08948314567866079427549408364939154125750064849853515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0185935160818056464948622164001790224574506282806396484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{221263951940097392}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{155728717993104096}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29565}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{103755292348965856}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{103167042952795326}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{21436864536966972}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.51984310150146484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.3223633639859837529684227774851024150848388671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64782559871673583984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8048}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.627370357513427734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6082}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.4404406740468065351024051778949797153472900390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.0662251655629138014091950026340782642364501953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.997880160808563232421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{6082}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98230435911393321202211836862261407077312469482421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{20539}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.946804583072662353515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{21598}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94322919845581043585269753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0091693937017722493276750128643470816314220428466796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.393134359725982263089605339700938202440738677978515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6772629}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6772629}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6772629}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{6772629}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{38}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{13654}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.4635761589403966098643650184385478496551513671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{29726}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{6}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{9.367249438630548041828660643659532070159912109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.186089684964546198120416420351830311119556427001953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0277445010924112674122188337832994875498116016387939453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20751}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000026699832275826737798156451452898750299072577700358090135868138759178691543638706207275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2345}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000026054821497037114438219634609030939328582006345885226095138165192111046053469181060791015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.043213444072651728544709470725138089619576930999755859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.7003498077392578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.987839378268517975811846554279327392578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{16284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.028825819492340087890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.914773464202880859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.524677205946520341939276477205567061901092529296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.6906368732452392578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{18146}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5742942402694399817164594423957169055938720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{13036}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.453177988529205322265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.447611331939697265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05884445353808775980297696150955744087696075439453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.1867022867578652933762128895978094078600406646728515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.02794149126599189403297174294493743218481540679931640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002667137344314340907658333890140056610107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.043006055859491264248273267867261893115937709808349609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1876699644574079950398726168714347295463085174560546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1302598746965742126935339229021337814629077911376953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{10248}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0864806396173844749153403199670719914138317108154296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08289307135441879859083513792938902042806148529052734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01831838258557545728866244871824164874851703643798828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{216368737791748408}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{150179410725073696}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{10248}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{99705389147037488}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{95569204547419348}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{21119657212525524}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.87827014923095703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.65154951139791084102625973173417150974273681640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17080}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.79167711734771728515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18289}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.74662494659423828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27300}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.4412442825297662185590752415009774267673492431640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.97350993377483430180063805892132222652435302734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1681}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1681}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99728471040725719110042746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13654}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.981916248798370361328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{9134}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95008312165737152099609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{1681}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94800025224685680047542746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{14095}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.010572413070050544481315313305458403192460536956787109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.444942437940154367215228603527066297829151153564453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6031057}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6031057}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6031057}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6031057}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{3284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.01324503311258240501047112047672271728515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{20415}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{5.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{9.06122424587309893695419305004179477691650390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.1869460859768102001243761378646013326942920684814453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0279695730176489250340399195238205720670521259307861328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000026699832275826737798156451452898750299072577700358090135868138759178691543638706207275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2345}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000026054821497037114438219634609030939328582006345885226095138165192111046053469181060791015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.043049857810733206664455252621337422169744968414306640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.920928955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9896405816867712701423442922532558441162109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{17080}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.114953577518463134765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{24262}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.110162258148193359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.530425991983071387636528015718795359134674072265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.727324008941650390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{18146}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5802433143388352476677027880214154720306396484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{19488}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.47142326831817626953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4667737483978271484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.055271520445505116503337461608680314384400844573974609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0976729519497460951793499361883732490241527557373046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0165690000740006844470730840157557395286858081817626953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{6532}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002667137344314340907658333890140056610107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0220238658819472236938263876027122023515403270721435546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.409105971847572413846449990160181187093257904052734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.318518313434045630128110815348918549716472625732421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{10248}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.209252172277774761699475902787526138126850128173828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1926987934164862970032316979995812289416790008544921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{19538}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0380767530671492215876838827171013690531253814697265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{471667072606149610}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{367226613169215232}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{10248}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{241251329304743296}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{222166582841659443}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{19538}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{43899507436721056}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.4159393310546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.266749906224134747390053234994411468505859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.3579044342041015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.61283111572265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59797218712847044486125014373101294040679931640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{22}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29565}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{12.887417218543046004697316675446927547454833984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1185}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{17194}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99878758547321855321143857509014196693897247314453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6589}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98887056112289439813167746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20976}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.986042797565460205078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0019258785131006585407409392729505270835943520069122314453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.095542561546577697839666143408976495265960693359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5488083}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5488083}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5488083}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5488083}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{45}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{8840}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{30.635761589403973204071007785387337207794189453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{23633}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{10}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{10}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.6512962514991631479688294348306953907012939453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.097800495054926550597684808963094837963581085205078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0165854814441312725659116722454200498759746551513671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6532}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000026699832275826737798156451452898750299072577700358090135868138759178691543638706207275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2345}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000026054821497037114438219634609030939328582006345885226095138165192111046053469181060791015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.022045084827788809234139222326120943762362003326416015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.1842095851898193359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.956098011787361201641033403575420379638671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{80.8924357891082763671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.7157418727874755859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5386633095317570063542689240421168506145477294921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7047092914581298828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{18146}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.57926557553525004351513416622765362262725830078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.46238076686859130859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.46107578277587890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{27584}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.056111363031700937920032146166704478673636913299560546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.09254309004274409444779081468368531204760074615478515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0165304327792854290068991218731753178872168064117431640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{29052}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002667137344314340907658333890140056610107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0217852982011353425717548049078686744906008243560791015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.41412840355286562044057063758373260498046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.32128860286401239587661393670714460313320159912109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.212121690239700289026814061799086630344390869140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.193619639100624796324012777404277585446834564208984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{19538}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.038406462481139824749476474607945419847965240478515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{477457542124601316}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{370420539427008896}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{244559658270902784}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{223228245633327036}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{19538}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{44279636510382136}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.3029937744140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{92.8864845124301581336112576536834239959716796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{19004}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{81.2790679931640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{80.37683868408203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.6339667658878003209110829629935324192047119140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{23}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29565}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{13.1920529801324502017223494476638734340667724609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99890715791689643765494110994040966033935546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{742}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9917552471160888671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98981314897537242547542746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20976}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00163225666406920620621345818790359771810472011566162109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.139862073255503815971678704954683780670166015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5502513}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5502513}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5502513}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5502513}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{45}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{8840}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{30.78807947019867441440510447137057781219482421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{23633}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{10.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{10}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.670631399184429710658150725066661834716796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0926639344815721466286362328901304863393306732177734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0165468537578327724857363278943012119270861148834228515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29052}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000026699832275826737798156451452898750299072577700358090135868138759178691543638706207275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2345}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000026054821497037114438219634609030939328582006345885226095138165192111046053469181060791015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0218060102786540623009958750344594591297209262847900390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{92.0529692173004150390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.936784718999803089900524355471134185791015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22401}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{80.871922194957733154296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.4099490642547607421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.547390700124666285120156317134387791156768798828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7034170627593994140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58523486150021586382763416622765362262725830078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{8840}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.479226887226104736328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24144}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.47785091400146484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.059348485107922288595005966271855868399143218994140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.1526713006414731899074155307971523143351078033447265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{24173}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0243656910448724998985436940301951835863292217254638671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002667137344314340907658333890140056610107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.036009101172852310546179666062016622163355350494384765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.28578366015559197865769647250999696552753448486328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1856947884292781403292593722653691656887531280517578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1145271709580508445736057865360635332763195037841796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1141347970446127957355741955325356684625148773193359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{19538}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0259799874199087600656898899842417449690401554107666015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{329486127458636993}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{214091514873533536}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{132040838259321648}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6155}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{131588461936672173}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{19538}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{29952886185828156}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{33.5944671630859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{13.575011654405404470935536664910614490509033203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{8.01591932773590087890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{22545}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{7.73836469650268465869658029987476766109466552734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.60855280594514926661986464750953018665313720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{5.39735099337748369663358971592970192432403564453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99989891052246082647769753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{17197}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98736564489389888610304524263483472168445587158203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{11598}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95721587538719188348323996251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24202}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95035737752914439813167746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{14095}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00803122518572950590265424608560351771302521228790283203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.7465547375386465400737279196619056165218353271484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7970679}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7970679}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7970679}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{7970679}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{38}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{18.165562913907283615344567806459963321685791015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{6532}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{13716}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.38110258634859661697191768325865268707275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.1529286305309615345837670474793412722647190093994140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24173}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0243904359332911789548514747139051905833184719085693359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000026699832275826737798156451452898750299072577700358090135868138759178691543638706207275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2345}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000026054821497037114438219634609030939328582006345885226095138165192111046053469181060791015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0360471095601906099670230787523905746638774871826171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.2270514965057373046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9121695006920020887264399789273738861083984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{3175}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.188188135623931884765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8840}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.0699508190155029296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{24262}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.4646171661674778352590919894282706081867218017578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7018988132476806640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.57622572759918799789602417149581015110015869140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{4800}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.461473882198333740234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{27584}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4596426486968994140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0571939557543482968160475365948514081537723541259765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.316027251226199401568095481707132421433925628662109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{20539}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.17350072285281126216460734212887473404407501220703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{4430}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0366648308360966457275509355895337648689746856689453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{1696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.03437937617870889805971046371269039809703826904296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06837443958188671455644680463592521846294403076171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1846504094344358914980830377317033708095550537109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.128434100554310759445542089451919309794902801513671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08689318646557851744116618419866426847875118255615234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0742029432305930936042415169140440411865711212158203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0158806296431117481560146842411995748989284038543701171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{212887427871420196}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{148074436453903104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{100181023279978128}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{85550168955671923}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18309119422240484}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{17096}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.64900662251655649725989860598929226398468017578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.996698796749114990234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{6155}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.979209143594400810428624026826582849025726318359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7467}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95161910355091094970703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.945552170276641845703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{29195}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0114158301731732587935841394255476188845932483673095703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.490960344181473995472941851403447799384593963623046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5896885}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5896885}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5896885}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{5896885}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{38}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{19004}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{21.165562913907283615344567806459963321685791015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{913}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.68168604369684970833986881189048290252685546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.316292792310344406114808180063846521079540252685546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20539}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.173698081915087787496787541385856457054615020751953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{4430}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.036693549579447364006323795138087007217109203338623046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.034407020731252409284639526276805554516613483428955078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0684270717338676670582486849525594152510166168212890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.849534511566162109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.464546893606126332088024355471134185791015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{16284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.7341289520263671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.5480701923370361328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{24262}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.4427097275253200070466164106619544327259063720703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.770748615264892578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.59772947608240389882894305628724396228790283203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{23241}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.475460529327392578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.47414302825927734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.056644423200939895968186732488902634941041469573974609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.3252321431322953149134491468430496752262115478515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{20539}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.170596492233743124433686944030341692268848419189453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{4430}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.032040663163631626086935710873149218969047069549560546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{1696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0263946159369027009977681785812819725833833217620849609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06815426154309368877992625357364886440336704254150390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1901377455241186897882954554006573744118213653564453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1333062213439471233034083752500009723007678985595703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8745}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0927572431065823710394369072673725895583629608154296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0814891701707121940412292815381078980863094329833984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0160921760297967064712310047980281524360179901123046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{219213895652220809}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{153691609285316960}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8745}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{106941820285624048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{93950616682380944}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18553015800671452}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.11057758331298828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.297075640286831088587859994731843471527099609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29110}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.480218231678009033203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{14929}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.448263645172119140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{19538}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.51224755971247670771617777063511312007904052734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{9816}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.761589403973510048473372080479748547077178955078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99609392881393443719417746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{6155}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.97999681226465085170929114610771648585796356201171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{2773}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94944663345813762322933371251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29052}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94711869955062877313167746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01161810884388156557556204262482424383051693439483642578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.470431804905378669889870479892124421894550323486328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7129206}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7129206}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7129206}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{7129206}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{38}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{19004}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{21.5430463576158928162840311415493488311767578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{913}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.7344436027875769212869272450916469097137451171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.32550541860316395403884826009743846952915191650390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20539}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1707910361262010290328561268324847333133220672607421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{4430}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.03206573508612413359042392357878270559012889862060546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0264158399214026139156796801898963167332112789154052734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06820713942969149068407119784751557745039463043212890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.111195087432861328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.4931962790078614489175379276275634765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.66703402996063232421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{24262}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.3161678314208984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.438347056071325180681697020190767943859100341796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.720851898193359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5984190884015418987473822198808193206787109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{6549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.48032963275909423828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{27584}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4717540740966796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.056769496049388516734079956904679420404136180877685546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.325696530142330298307484781616949476301670074462890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.16437630956872961718318038037978112697601318359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.017602001213746699959106223332128138281404972076416015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0165619996458068012568087823410678538493812084197998046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0673285541827492173272418085616664029657840728759765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2040156732747707979402917999323108233511447906494140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1475813865367727739652536911307834088802337646484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{16149}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1061394986741026336130033769222791306674480438232421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.102430020428285306621773997903801500797271728515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0167026914190019949713050806394676328636705875396728515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{235214056995327750}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{170149754217940800}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{16149}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{122370510509562880}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{118093773269088828}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19256892121779656}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.95111083984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.271134603891940884068390005268156528472900390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{7310}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64434564113616943359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6082}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.634481906890869140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.46292293381569304955291954684071242809295654296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.0728476821192050039144305628724396228790283203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.998348712921142578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9824230118303109993149746514973230659961700439453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95154148340225208624332253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95025634765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{27484}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00860198548741508521586762725519292871467769145965576171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.3471613886644016044868976678117178380489349365234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6873174}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6873174}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6873174}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{6873174}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{38}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{22.344370860927153188413285533897578716278076171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{913}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.79615234233409637454315088689327239990234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.3260106316971260742576532720704562962055206298828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1645634233600892226689893504953943192958831787109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0176199135892210791143330794739085831679403781890869140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0165753171960454741273860435057940776459872722625732421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06737967260307942130026503946282900869846343994140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.6559071540832377422702847979962825775146484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.357736944362812891995417885482311248779296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1412}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.922154128551483154296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.7826855182647705078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3262216504896511271027748080086894333362579345703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7360992431640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.59970924396388536337099139927886426448822021484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{11498}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4998581409454345703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4848763942718505859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05530729328499565944365912173452670685946941375732421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.3153246772389806107383947164635173976421356201171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{27714}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.166670458966603707295917047304101288318634033203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.02232048928207865101658313733423710800707340240478515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0181461175308121995530807879504209267906844615936279296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0678562313535088501570413654917501844465732574462890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.199764666629571596700998270534910261631011962890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1418609602751353115923649284013663418591022491455078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{30371}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0987558334554210770495075166763854213058948516845703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.09323238226903500514008982236191513948142528533935546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0167020821650856153561814920749384327791631221771240234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{230312980017850981}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{163554551765381184}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{30371}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{113857724096127280}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{107489618443696621}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19256189699837688}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.9180507659912109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.6426645604190444061032394529320299625396728515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{13716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.75143182277679443359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27300}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.745930433273314985598290149937383830547332763671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{18289}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.44003606333357636604119988987804390490055084228515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{1895}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99868261814117442742855246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2236}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9829688711671640266587246514973230659961700439453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95194323360919952392578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12141}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95178967714309681280582253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{27484}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.009186443423334474112085246133574401028454303741455078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.3817006212182665336740683414973318576812744140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6114964}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6114964}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6114964}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6114964}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{38}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{21.22516556291390799060536664910614490509033203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{2236}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{11.004016235764094489013587008230388164520263671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.315498016075541343194998944454709999263286590576171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27714}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1668600729951726646671517073627910576760768890380859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0223434026714516183187431153100988012738525867462158203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0181607088746729393446965872271903208456933498382568359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06790673494708375501627273251870064996182918548583984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{95.1485407352447651874172152020037174224853515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{16284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.46718865830376898884424008429050445556640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.7589581012725830078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.2942535877227783203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5877929863780517738547359840595163404941558837890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7604694366455078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.60455947838082213507959750131703913211822509765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{31308}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4909946918487548828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.484261989593505859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{28778}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.057007849184896784711096273667862988077104091644287109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.2382795500936377985912173471660935319960117340087890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0993469055458043037720727852502022869884967803955078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0224065973979900752433014332609673147089779376983642578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.016503652934575500921265955867056618444621562957763671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.039399999325771449532052059794295928440988063812255859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.453221690785535480383572348728193901479244232177734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.3574201364241884615324806873104535043239593505859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4305}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.272944512343557377231917371318559162318706512451171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{2306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.265082436243615104931592441062093712389469146728515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{11498}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0296270311848977029034468699819626635871827602386474609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{522529033660918715}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{412077361462959872}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4305}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{314683597845316352}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{2306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{305619241238837339}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{11498}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{34157641370726236}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{155.63616943359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.4297275164269507286007865332067012786865234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{4729}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.906459808349609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.7463226318359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59340187814654488107635188498534262180328369140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{22}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{27584}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{13.4172185430463581923277160967700183391571044921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{10}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{5781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{10}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99834827792565550286241204958059825003147125244140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{26278}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9893803894519805908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29022}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98929876089096080438167746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20976}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00195091538451497487939578778792792945750989019870758056640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.0077914982844475844103726558387279510498046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5584660}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5584660}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5584660}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5584660}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{47}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{36.11920529801324164509424008429050445556640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{4157}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{11.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{5781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.12418430541036595826653865515254437923431396484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.2385093467608842832117233001554268412292003631591796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0994600489100368190253931288680178113281726837158203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0224236606783210501436798267604899592697620391845703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0165131078588308145838059459720170707441866397857666015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03942543217616141515424743602125090546905994415283203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{101.354745388031005859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{16284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.53096698767302541455137543380260467529296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.94923388957977294921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{19004}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.9434320926666259765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8840}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.9272444180790262446834049114841036498546600341796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7203881740570068359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.601134336547346492807264439761638641357421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{11498}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.49119126796722412109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{28778}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4897439479827880859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.055283777119707618041832830613202531822025775909423828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.325918680039876507148477458031265996396541595458984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.1643922135856570321266190148890018463134765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.017550276219374348618540437882984406314790248870849609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.016561932734699198743744119610710185952484607696533203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06737281622413275605776306065308745019137859344482421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2040227096334865930504776088127982802689075469970703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1476904383544190568766651949772494845092296600341796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{16149}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.106487725156996670961007112055085599422454833984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.10246374498474790371016496237643877975642681121826171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0166828333006350214284818633814211352728307247161865234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{235222169364605322}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{170275482403621632}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{16149}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{122771988310164992}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{118132655035467825}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19233997270073340}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.51984310150146484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.3223633639859837529684227774851024150848388671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{23447}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64782559871673583984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.627370357513427734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6082}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.4404406740468065351024051778949797153472900390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.07947019867549709459808582323603332042694091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.998348712921142578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9825542557318478475991696541314013302326202392578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.951983749866485595703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95025622844696044921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{27484}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00858083463234242220518677157770071062259376049041748046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.355154640471309124283294522683718241751194000244140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6881493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6881493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6881493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{6881493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{38}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{22.25827814569536400313154445029795169830322265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{913}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.7410603988699069333279112470336258411407470703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.32623299583591147676742139083216898143291473388671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.16457929695305673067906582218711264431476593017578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0175681325652812560245141781933853053487837314605712890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0165752502311344619700950175911202677525579929351806640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06742378658108579003727101053300430066883563995361328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{100.6354253292083598125827847979962825775146484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{16284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.5317111189002190485553001053631305694580078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1412}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.687497913837432861328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{19004}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.6145813465118408203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.929245843462179976768311462365090847015380859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.75756359100341796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.60215499858982557412900860072113573551177978515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4879190921783447265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.472749233245849609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0589392088361171406774019487784244120121002197265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.314321230393479200682094187868642620742321014404296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{27714}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.1666323984061961194225176541294786147773265838623046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.022089487274823127460621208228985778987407684326171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0181461175308121995530807879504209267906844615936279296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06789948921801979009327254743766388855874538421630859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.199947205930880389512793726680683903396129608154296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.14193926509746368491704515690798871219158172607421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{30371}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09875580191237752492039447815841413103044033050537109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.09323238226959600083443291396179120056331157684326171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0167161354561871609847312214469639002345502376556396484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{230523433503765796}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{163644831078957984}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{30371}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{113857687729474064}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{107489618444343445}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19272392041359164}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.87827014923095703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.65154951139791084102625973173417150974273681640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17080}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.79167711734771728515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18289}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.74662494659423828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27300}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.4412442825297662185590752415009774267673492431640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{1895}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.006622516556291202505235560238361358642578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99868261814117442742855246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2236}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98307795674595610524448829892207868397235870361328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{123}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95183674991130828857421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12141}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95178967714309681280582253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{27484}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0091728794613972798599466074165320605970919132232666015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.372865914179052959642746145618730224668979644775390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6139921}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6139921}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6139921}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6139921}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{38}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{21.23178807947019919311060220934450626373291015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{2236}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.996353223682401534233576967380940914154052734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.31449401761983841740999423564062453806400299072265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27714}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1668219869010663380937131705650244839489459991455078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{21317}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0221121504172582215852482789841815247200429439544677734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0181607088746729393446965872271903208456933498382568359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.067950077433779731972407489593024365603923797607421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.5077717304229594219577847979962825775146484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.4765544648202109101475798524916172027587890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5358}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.436423122882843017578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.97689723968505859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.4889248864990116683060250579728744924068450927734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7515552043914794921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.60357007127723960593357332982122898101806640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{29195}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.479700982570648193359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{28778}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4764664173126220703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.057000147888811636409656102841836400330066680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.246135846016452497497795093295280821621417999267578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.09931241411268849905713551606822875328361988067626953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{4729}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0226050634141156496503821671240075374953448772430419921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0153303705803484006942039030718660796992480754852294921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.039691720227990258396122413842022069729864597320556640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.453035853363410290217672127255355007946491241455078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.357371846332119658118386951173306442797183990478515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.27294760686943331240428278761100955307483673095703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{2306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.26468704153818578550527718107332475483417510986328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{11498}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.02958729726466462206513341470781597308814525604248046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{522314777700589868}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{412021686777354368}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{314687165590745216}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{2306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{305163382180140140}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{11498}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{34111831279627180}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.4159393310546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.266749906224134747390053234994411468505859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.3579044342041015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.61283111572265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59797218712847044486125014373101294040679931640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{22}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29565}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{13.403973509933774010960405576042830944061279296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{10}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{5781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{10}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9983574949352946870106961796409450471401214599609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{12493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98913323879241954461605246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29022}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.988796532154083251953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20976}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0019815100282996648238531545160867608501575887203216552734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.98397156018330012017258923151530325412750244140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5596947}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5596947}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5596947}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5596947}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{47}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{36.06622516556291202505235560238361358642578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{11.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{5781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.17212122295194376420113258063793182373046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.246373219291172229628017475988599471747875213623046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.099425653559058913000257007297477684915065765380859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{4729}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0226223540983947722649016753848627558909356594085693359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.01533915333245895913638623397901028511114418506622314453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03971775800292343117092741522355936467647552490234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{92.1596868038177632342922152020037174224853515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.5046941602466858967090956866741180419921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.688271939754486083984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{24262}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.6264908313751220703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.4347166805568580816299117941525764763355255126953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.780879974365234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.60293205842277064476775194634683430194854736328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.484358966350555419921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.482809543609619140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05927473313676349941925280973009648732841014862060546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.2357132921901168021161510068850475363433361053466796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0986081854926766643298918779692030511796474456787109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{4729}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.02296273302527307436093906289897859096527099609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0164380464748558989540594410527774016372859477996826171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0392263945201375141547117664231336675584316253662109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.458136734167779113846563632250763475894927978515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.360417144547158507794648585331742651760578155517578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.274744395506919147909030698428978212177753448486328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{2306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.2700396324043656814950509215123020112514495849609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{11498}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0298215860971582820415637371525008347816765308380126953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{528195692872382967}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{415532676577413440}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{316758721850135936}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{2306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{311334499295121123}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{11498}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{34381947912898356}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.3029937744140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{92.8864845124301581336112576536834239959716796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{19004}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{81.2790679931640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{80.37683868408203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.6339667658878003209110829629935324192047119140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{23}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29565}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{13.75496688741721840187892667017877101898193359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{10}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{16069}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{10}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{16069}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2236}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9984561311488120427526382627547718584537506103515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7790}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98884727060794819220035378748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29022}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.988796532154083251953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20976}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.001977743045027162242799345648336384329013526439666748046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.109476842388280370954589670873247087001800537109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5611377}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5611377}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5611377}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5611377}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{47}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{20013}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{36.4370860927152335762002621777355670928955078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{5928}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{11.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{5781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{6.8807978889525980292773965629749000072479248046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.2359406139596505191935449374796007759869098663330078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0987208161502056980030062049991101957857608795166015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{4729}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.02298024728793508775215315154127893038094043731689453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.01644746381324402317858357491786591708660125732421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.039252865870300170103579517899561324156820774078369140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.4437625408172607421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.51873385353593448598985560238361358642578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{13468}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.764286518096923828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.6036193370819091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{24262}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3755639690948819886529008726938627660274505615234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.768011569976806640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.60321638915712494366516693844459950923919677734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{11598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.492232739925384521484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4750306606292724609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05612148374723523180929163345354027114808559417724609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.312242976347418821347901030094362795352935791015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.152609320453917896021067690526251681149005889892578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{123}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.01502184279963775064004050108223964343778789043426513671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{24566}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00992879958526000049034987426921361475251615047454833984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{24202}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06217496482227492793359857614632346667349338531494140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.302663733530732004251007083439617417752742767333984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.20391833455134922292728560933028347790241241455078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.146922938423748761227471959500689990818500518798828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{2306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1442081462314482032116558229972724802792072296142578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{11498}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0237192015833732096352637341851732344366610050201416015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{348947527052177429}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{235101833087863968}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{169390615228767552}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{2306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{166260672929725525}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{11498}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{27346377577575744}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{33.5944671630859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{13.575011654405404470935536664910614490509033203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{8.01591932773590087890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{22545}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{7.73836469650268465869658029987476766109466552734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.60855280594514926661986464750953018665313720703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19917}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{5.377483443708609200939463335089385509490966796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{913}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{913}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99962973594665516241519753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98511791505560974968602749868296086788177490234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9517808854579925537109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{5928}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94579571485519398077457253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{14095}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0098863068477850028770159696023256401531398296356201171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.76115737818249573631845805721241049468517303466796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{8079543}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{8079543}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{8079543}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{8079543}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{40}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{13654}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{26.119205298013245197807918884791433811187744140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{1412}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{8.25}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{1696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.0653014563988012497475210693664848804473876953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.312544103302323517112881745561026036739349365234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1527840388165775109552413368874113075435161590576171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{123}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0150369053880024146352401004378407378681004047393798828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{24566}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00993594182011610198290707529622522997669875621795654296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{24202}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.062217145228426730396709132264732033945620059967041015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.2520935535430766094577847979962825775146484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.37375857498471987128141336143016815185546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1412}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.717167794704437255859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.2143971920013427734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3351947418505585307713090514880605041980743408203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7610924243927001953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{6082}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.6024436208586028129730038926936686038970947265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{1895}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.49823629856109619140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4861724376678466796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.059150563681992174291934816210414282977581024169921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6853792067548403199594986290321685373783111572265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{13293}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5393719471566680301322094237548299133777618408203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.3434846181464037417896406623185612261295318603515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.286298199687039900407370396351325325667858123779296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.061253106274518943907825274663991876877844333648681640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.160299982821053899062491154836607165634632110595703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.108081094144104994381194728703121654689311981201171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{24173}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0729573783802793529584818088551401160657405853271484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.06683067794005000117341097620737855322659015655517578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.018013412089531284643317832205866579897701740264892578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{184813297382501254}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{124609017680175856}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{24173}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{84114130454362736}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{77050525764538120}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20768050169365572}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.15894039735099330101775194634683430194854736328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999562203884124755859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98761316601014292881899336862261407077312469482421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6910}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95835866034030925408870871251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.951836109161376953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00842364903213732064968244372948902309872210025787353515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.38330585770828562441892017886857502162456512451171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6044117}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6044117}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6044117}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{6044117}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{36}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{29.602649006622517191544829984195530414581298828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.110368765130356649706300231628119945526123046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.686006001891261707470448527601547539234161376953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{13293}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.54000366251078479873370952191180549561977386474609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.34561720201589529732899563896353356540203094482421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.28671677732157829776582502745441161096096038818359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0611993556385193315794168711363454349339008331298828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.4622571468353129375827847979962825775146484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9179224857431336204172112047672271728515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{19488}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{80.98274219036102294921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{24262}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.652270793914794921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.47431047033683793046066057286225259304046630859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7158701419830322265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5855918925329550717151505523361265659332275390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.471005260944366455078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{28090}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4655029773712158203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.056815296073144005983834858852787874639034271240234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.64736233486711058926488249198882840573787689208984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.535338186960725437302244245074689388275146484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.33266409605672098148687609864282421767711639404296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.283241222075901688537413747326354496181011199951171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06132251208131274389234732780096237547695636749267578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1652072410704664984226752721951925195753574371337890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1137607562729408827717492158626555465161800384521484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.07924994553134145913730890242732129991054534912109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.06955880684344080411296573629442718811333179473876953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0180632989471183717788971279105680878274142742156982421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{190470980946908342}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{131157222287411872}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{91368966442004928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{80195844244596894}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20825565800274988}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.11057758331298828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.297075640286831088587859994731843471527099609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.480218231678009033203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{14929}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.448263645172119140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.51224755971247670771617777063511312007904052734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{17096}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.205298013245033050822030418203212320804595947265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99955928325653076171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.986405548275701260507730694371275603771209716796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6910}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95538233220577228888004128748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{30684}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.954569399356842041015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.008604848168897567817214877550213714130222797393798828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.435477674775459455691617449701880104839801788330078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7276438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7276438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7276438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{7276438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{36}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{29.860927152317881194676374434493482112884521484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{6.63428755224093702480558931711129844188690185546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.64776427439016170950480955070815980434417724609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.53596855585588076831271564515191130340099334716796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.33293685639786285701546830750885419547557830810546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.283655330305956521197430220126989297568798065185546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.061293109186055454162822542230060207657516002655029296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.3245375156402587890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9490345329638358862212044186890125274658203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.063386380672454833984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.8696956634521484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.49403338213126968270216821110807359218597412109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7211124897003173828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5855695096072768279782394529320299625396728515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{20976}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4664180278778076171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.450253963470458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05766021554821583461336587106416118331253528594970703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.64264056087525867067000717725022695958614349365234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.519671031286042417463022502488456666469573974609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.30597279340054484020328118276665918529033660888671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.293137145456404402121819430249161086976528167724609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.059906604013452192936117768340409384109079837799072265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1778020357580822885523730292334221303462982177734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1303869305557179558707758815216948278248310089111328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09489068132618884432449846144663752056658267974853515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08047594137231260658094100790549418888986110687255859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.017698485469447584883528890031811897642910480499267578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{204991790588368626}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{150325896157366880}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{109401507087758576}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{92782443411619086}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20404964496697920}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.95111083984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.271134603891940884068390005268156528472900390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{7310}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64434564113616943359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.634481906890869140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.46292293381569304955291954684071242809295654296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{8721}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.476821192052980347142465689103119075298309326171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9997780323028564453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98483165210445988702048225604812614619731903076171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9466208517551422119140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9362618923187255859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01127338311424808114935558478464372456073760986328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.5499480660139521859264277736656367778778076171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7020406}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7020406}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7020406}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{7020406}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{30.9735099337748351899790577590465545654296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{4157}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{5.915460739438231030362658202648162841796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.64303956870537060108716786999139003455638885498046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.5202870275656164000821490844828076660633087158203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.30623032157671203901116996348719112575054168701171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.293565721860568284995451904251240193843841552734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.059904582476339555963118499448682996444404125213623046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.313985347747802734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9544132308454749136217287741601467132568359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.313335239887237548828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.2742273807525634765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5505604899751481706715594555134885013103485107421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7257854938507080078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58797031206800465241713027353398501873016357421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.472574651241302490234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.47046661376953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.055722264497980601716253801214406848885118961334228515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.64988009748401942555773302956367842853069305419921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.526727709388797205036780724185518920421600341796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.314194222396460165480647219737875275313854217529296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.287985675110652594721472041783272288739681243896484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.060993756700605687715022185102498042397201061248779296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1756258980430077942802569168634363450109958648681640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.12382453441356451595556364964068052358925342559814453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0857454718554509220940218483519856818020343780517578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0739761369445721961302098179658059962093830108642578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0179591044447667096128906649710188503377139568328857421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{202482874619673320}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{142759968523329152}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{98857798424810592}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{85288679111138393}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20705437717851948}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.9180507659912109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.6426645604190444061032394529320299625396728515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{13716}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.75143182277679443359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.745930433273314985598290149937383830547332763671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.44003606333357636604119988987804390490055084228515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.34437086092715230023486583377234637737274169921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99953562021255482061832253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98469993570782488045978197988006286323070526123046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{8721}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.953603684902191162109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.948362290859222412109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01017834577562867250100087090913802967406809329986572265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.5152811566603154869170566598768346011638641357421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6262196}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6262196}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6262196}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6262196}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{30.052980132450329620041884481906890869140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{6.7321390669551544050364100257866084575653076171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.65028360025573495040163152225431986153125762939453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.52734991050148727342872234657988883554935455322265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.31445601342266094047062097160960547626018524169921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2884067198912363405582937048166058957576751708984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06097923973174608491820691824614186771214008331298828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.118791103363037109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9524603426851143694875645451247692108154296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.25404298305511474609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.124378204345703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5414686319864852048766579173388890922069549560546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7500150203704833984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.59202312002118873124345554970204830169677734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.473985493183135986328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4694344997406005859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.057951786529075378917585936733303242363035678863525390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.38691240228254908384286636646720580756664276123046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.312301609838236959859614216838963329792022705078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1708923928674770664759563487677951343357563018798828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.165785018960877106319884433105471543967723846435546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0396997708314082708991321624125703237950801849365234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.44205715240007659172505327660473994910717010498046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.370558774141282964986743309054872952401638031005859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.3137817195216829890824783433345146477222442626953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.313585027368136703973533485623192973434925079345703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.024099801658955789795957258547787205316126346588134765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{509657197267314574}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{427225179428236736}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{361765692189062464}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{361538921575451490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{27785179589369900}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{155.63616943359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.4297275164269507286007865332067012786865234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.906459808349609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.7463226318359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59340187814654488107635188498534262180328369140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{21}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{12.5827814569536418076722839032299816608428955078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999968051910400390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99806968857910460801718954826355911791324615478515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99033418297767628057926003748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29022}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99032622575759876593082253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{4157}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0017548442044068627253261549725493750884197652339935302734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.9644442649563085279140750571968965232372283935546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5731892}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5731892}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5731892}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5731892}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{45}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{38.19205298013245197807918884791433811187744140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{28.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{28}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.2573360370020392196011016494594514369964599609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.38708793127116203347526379729970358312129974365234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.312678117336528671454942696072976104915142059326171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.171036648335729069003718905150890350341796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.166027402256176903616591289392090402543544769287109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0397557004515341760875202226088731549680233001708984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.3847510814666748046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9237928469449485646691755391657352447509765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{19488}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{80.803187429904937744140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{9132}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.2824556827545166015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.51372169215601193315023920149542391300201416015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.716167449951171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.59031715772009807352560528670437633991241455078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.484134018421173095703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.473488330841064453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0562471398626651353236383101830142550170421600341796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.63931062551660844395229332803864963352680206298828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.519795184566365975342705496586859226226806640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{22401}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.305893200690677158348762532114051282405853271484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.29291508327639770303818522734218277037143707275390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.059939236896361346162986905028446926735341548919677734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1778141542233004079864855384585098363459110260009765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1305445533464194285411252849371521733701229095458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09499559572667180817884258203775971196591854095458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0805359854042591027933895020396448671817779541015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0176206153565949541484059182039345614612102508544921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{205005762227521503}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{150507622862382752}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{109522465156218256}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{92851669467273477}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20315186369023964}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.51984310150146484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.3223633639859837529684227774851024150848388671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64782559871673583984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.627370357513427734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.4404406740468065351024051778949797153472900390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{8721}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.476821192052980347142465689103119075298309326171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9997780323028564453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9848270617573466889638211796409450471401214599609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9461005032062530517578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.93418014049530040399105246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01128732204910666558905774081722483970224857330322265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.5499480660139521859264277736656367778778076171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7028725}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7028725}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7028725}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{7028725}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{31.052980132450329620041884481906890869140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{4157}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{5.91864052704225240830737675423733890056610107421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.63981245030526368022805172586231492459774017333984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.5204113995932069247629669916932471096515655517578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22401}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.306150632140430867256242208895855583250522613525390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.293343335018156736726524513869662769138813018798828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.059937716141394696556243815166453714482486248016357421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.7217080593109130859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9448808992145814045215956866741180419921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.304103434085845947265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.0527698993682861328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5166261842922545977074832990183494985103607177734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7361476421356201171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58816059693595423851775194634683430194854736328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4659354686737060546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4621975421905517578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0587640838843478674480280687930644489824771881103515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.65010437508097862480127560047549195587635040283203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.52660011150652585865117316643591038882732391357421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.31402598220110966575902011754806153476238250732421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.28820564980539220556465807021595537662506103515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06101317893321060725764226617684471420943737030029296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1756313344299079981514211112880730070173740386962890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.12391405680871432626322103942584362812340259552001953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.085638199319486185689953572364174760878086090087890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.074117724572485499390239738204400055110454559326171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0179659568579166421808945841576132806949317455291748046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{202489142347037918}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{142863180817841248}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{98734121611243120}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{85451918532145922}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20713338012330952}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.87827014923095703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.65154951139791084102625973173417150974273681640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.79167711734771728515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.74662494659423828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.4412442825297662185590752415009774267673492431640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.34437086092715230023486583377234637737274169921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99953562021255482061832253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9846592213933831327921097908983938395977020263671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{8721}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95332412421703327520816628748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94778692722320556640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01022754842613953808749815976852914900518953800201416015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.5152811566603154869170566598768346011638641357421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6287153}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6287153}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6287153}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6287153}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{30.066225165562915577766034402884542942047119140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{6.7359555870830067902943483204580843448638916015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.65050801710396888299925421961233951151371002197265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.527222450850693302726313049788586795330047607421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.3142877093562737034204701558337546885013580322265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.288627016196406904757765232716337777674198150634765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.061000802446916073396021573671532678417861461639404296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.2740449905395649921047152020037174224853515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9826576851851172023089020512998104095458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.2615811824798583984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.0855338573455810546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5065226179421002949965213701943866908550262451171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7205562591552734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58888266576046977007763416622765362262725830078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4565088748931884765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.44962310791015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0585104894506347505966914468444883823394775390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.389673581198206608888767732423730194568634033203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.311861298967744338117569213864044286310672760009765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.17272046132932050710451221675612032413482666015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.166237978109243400570704807250876910984516143798828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.039159916669349238704800342247835942544043064117431640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.4415989101218948942317865657969377934932708740234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.37043764361174769117468486001598648726940155029296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12561}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.31378909561567691621775111343595199286937713623046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.3127308542051328021926792644080705940723419189453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0239969353789523977271702648295104154385626316070556640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{509128879890478819}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{427085525435871104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12561}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{361774196246448000}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{360554126967166215}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{27666582843055076}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.4159393310546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.266749906224134747390053234994411468505859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.3579044342041015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.61283111572265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59797218712847044486125014373101294040679931640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{21}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{12.5629139072847682001565772225148975849151611328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99989998340606678350894753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{6155}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99805303322558369671924083377234637737274169921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.990444362163543701171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29022}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99037086963653564453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{4157}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00170173691864576007333476059812937819515354931354522705078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.9985960600209065063381785876117646694183349609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5744179}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5744179}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5744179}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5744179}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{45}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{38.059602649006620822547120042145252227783203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{24.25}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{13}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.968335739207281331886179032153449952602386474609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.389850362839718689311752086723572574555873870849609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.312237435001444352256072534146369434893131256103515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1728659906332616902346899223630316555500030517578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.1664810236461118642115053489760612137615680694580078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03921770792617705614357959120752639137208461761474609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.5356478691101216327297152020037174224853515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9249190794711097396429977379739284515380859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.25100672245025634765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.9644763469696044921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.495204242045236942004748925683088600635528564453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.92527079582214444286591970012523233890533447265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5880691010430947329723494476638734340667724609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.46774137020111083984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4662382602691650390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.06362480207120792263797426357996300794184207916259765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.38673920336654499241291205180459655821323394775390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.309759100752564631164887032355181872844696044921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.168460177202848837563209372092387638986110687255859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.163972752510135710846128631601459346711635589599609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03972041937201377381772005037419148720800876617431640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.447775261461593909739775654088589362800121307373046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.37387446338114715960188050303258933126926422119140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.31593796678270547051425864992779679596424102783203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.31305629612451391086125340734724886715412139892578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0239773966305870632476082704442887916229665279388427734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{516249728170025170}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{431047908855469760}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{364251676025544896}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{360929335954521282}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{27644056199891576}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.3029937744140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{92.8864845124301581336112576536834239959716796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{81.2790679931640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{80.37683868408203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.6339667658878003209110829629935324192047119140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{22}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{12.887417218543046004697316675446927547454833984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{7098}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{7098}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999968051910400390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99824801028169540817458482706570066511631011962890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7790}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99028635025024425164730246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4157}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.989761173725128173828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{29022}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00145038757877115321269501091450138119398616254329681396484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.0248229302278186736430143355391919612884521484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5758609}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5758609}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5758609}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5758609}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{45}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{38.4503311258278159812107332982122898101806640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{31}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{31}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.121129093685139022085195392719469964504241943359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.387128605290947336303730708095827139914035797119140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.310132724117742342162529212146182544529438018798828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.168602491169706658613591798712150193750858306884765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.164212486210695007837756520530092529952526092529296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03977913520383839773852940879805828444659709930419921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.1562995910644389141452847979962825775146484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7790}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.93873771452746268550981767475605010986328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.052029550075531005859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.5438859462738037109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{9132}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.4796033993493278302366888965480029582977294921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.715634822845458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5856818142316200237473822198808193206787109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.452420771121978759765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4480721950531005859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.056897380699332110454147226619170396588742733001708984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.579895583275190862337922226288355886936187744140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.4685772334425666318935554954805411398410797119140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{20976}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.246032437774628132132193059078417718410491943359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2340378863005899978677604167387471534311771392822265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.05921953051840554704821073528364649973809719085693359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.29154352366065749979640031597227789461612701416015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1933543225494465944702682236311375163495540618896484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7467}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.142684928337893313088358127060928381979465484619140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1420448658371712136183617758433683775365352630615234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0246867943612423708377168196648199227638542652130126953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{336126797957227220}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{222922356475945600}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7467}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{164504522264044160}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{163766580442669202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{28461936098883380}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{33.5944671630859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{13.575011654405404470935536664910614490509033203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{8.01591932773590087890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{7.73836469650268465869658029987476766109466552734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.60855280594514926661986464750953018665313720703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.8211920529801322032881216728128492832183837890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99947363138198841436832253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9880313608820074922078902091016061604022979736328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{30899}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95296226441860198974609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.950302898883819580078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{4157}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00944912151112466645874743420563390827737748622894287109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.7641477329794543749130752985365688800811767578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{8226775}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{8226775}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{8226775}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{8226775}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{38}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{33.5364238410596016137787955813109874725341796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{22.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.83725180537676724412676776410080492496490478515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.58025563349993702910722959131817333400249481201171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.4691348134701727179418639934738166630268096923828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20976}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.246239174670283611501275800037547014653682708740234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2343800575924358808865832770607084967195987701416015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.05923793395899130953541344979385030455887317657470703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.8018367290496826171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9407715402691536610291223041713237762451171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.145259797573089599609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.0204160213470458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5283119727605358750821551439003087580204010009765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7349522113800048828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.589525688562961391880890005268156528472900390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4812166690826416015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4721157550811767578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.054652121989720379990895793298477656207978725433349609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.7341594371867916635210349340923130512237548828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{13293}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.668885782043378895878049661405384540557861328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.5933400560268358159277113372809253633022308349609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.57546861148124861529140616767108440399169921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.030976479007805306220557639562684926204383373260498046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1539212874643121897744180159861571155488491058349609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10133517098319951010854111927983467467129230499267578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.069256780745197199511409280603402294218540191650390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0641773134406526946094118102337233722209930419921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0172968462237613473941877373363240621984004974365234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{177459162334377912}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{116831497799542544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{79847631860979296}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{73991404773622603}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19941905973252192}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.112582781456953551213473474490456283092498779296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9993798732757568359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{913}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99028749892253753461801579760503955185413360595703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29022}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95766504108905792236328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94793224334716796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{19093}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00832757695641525748364575321147640352137386798858642578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.316082107649846955066408327184035442769527435302734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6152981}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6152981}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6152981}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{6152981}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{36}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{31.337748344370861985908049973659217357635498046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{20.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{16149}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.73773584902808853058786553447134792804718017578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.73483084297216028080157457225141115486621856689453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{13293}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6696843914413939113927654034341685473918914794921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.594256017310780482176824079942889511585235595703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.577686766942659080115163305890746414661407470703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0309046542492546760794169813379994593560695648193359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{92.9854123592376851092922152020037174224853515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.5453926553789330000654445029795169830322265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{19488}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.857090175151824951171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.848140716552734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5730675735238452972453160327859222888946533203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7482655048370361328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61042990747666525663817083113826811313629150390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4904348850250244140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.487262725830078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0555870369800154084938270671045756898820400238037109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.73561759633376000433457875260501168668270111083984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{13293}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.66429128564715522742289977031759917736053466796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{29726}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.5827551055544055724766394632752053439617156982421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.56949832679841339011517220569658093154430389404296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0300927792852791579913951380831349524669349193572998046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.15572651502734180528619845063076354563236236572265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10735629826063330938268336467444896697998046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0765172944962608514440915996601688675582408905029296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.06827238695354130582071405797250918112695217132568359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.017305899932951014641435705243566189892590045928955078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{179540448012503691}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{123773384919670832}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{88218434299074336}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{78712703089577803}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19952344189273412}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.11057758331298828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.297075640286831088587859994731843471527099609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.480218231678009033203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{14929}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.448263645172119140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.51224755971247670771617777063511312007904052734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.15231788079470209851251638610847294330596923828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999212741851806640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9896313473088851342396310428739525377750396728515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9609626233577728271484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95930850505828857421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.007484060626396585487463131158847318147309124469757080078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.359328740827828785331377048350987024605274200439453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7385302}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7385302}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7385302}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{7385302}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{36}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{31.582781456953643584029123303480446338653564453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{913}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{22.25}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{12493}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.548490309874397841127802166738547384738922119140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7362903356393937226442858445807360112667083740234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{13293}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.66508232220377594412497046505450271070003509521484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.583951544068183725499920910806395113468170166015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.57169346967614653731715179674210958182811737060546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.02997670467080841560925108524315874092280864715576171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.6413471698760986328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.5349645219891243641541223041713237762451171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15399}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.8389937877655029296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.6545865535736083984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5687455196580331051592338553746230900287628173828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7486369609832763671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61268543407617048757174416095949709415435791015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.498536288738250732421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4961836338043212890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.054038109808210950391060833908341010101139545440673828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.7039112448525648435548873749212361872196197509765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.64690758115582569498513976213871501386165618896484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{19488}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.57023515833889337756090753828175365924835205078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.55813887451567978370547962185810320079326629638671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0286109936709710820090801774995270534418523311614990234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1706179090860446001531869342215941287577152252197265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1243834359131776035045646722210221923887729644775390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0892094389826951772448637711931951344013214111328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07536640081707800253862927775116986595094203948974609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0171764572582346793094831838288882863707840442657470703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{196709056456356769}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{143404338081190112}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{102851480617061664}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{86891544226828269}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19803106945979116}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.95111083984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.271134603891940884068390005268156528472900390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{7310}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64434564113616943359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.634481906890869140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.46292293381569304955291954684071242809295654296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.324503311258278248629949302994646131992340087890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99946641921997081414730246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98563858136436011125880440886248834431171417236328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{24566}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95021580159664142950504128748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94411373138427723272769753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00992424132185491282565070747523350291885435581207275390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.50885755529267673313853492800262756645679473876953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7129270}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7129270}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7129270}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{7129270}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{36}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{32.03973509933774721503141336143016815185546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{23}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.281166178761567575605795354931615293025970458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.70446377768649781625498462744872085750102996826171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.64767950462656553867191178142093122005462646484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{19488}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5711944884133062227959953816025517880916595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.55883269757445452885491476990864612162113189697265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.02851975220112602793509637422175728715956211090087890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{92.24398136138916015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.4996682539680961099293199367821216583251953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.565169155597686767578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.865510463714599609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5454573323671147999647246251697652041912078857421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7475969791412353515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.610661944016715807492801104672253131866455078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.48266422748565673828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{23696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4765226840972900390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0547776377793098567803298237777198664844036102294921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.71161430067189834769436629358096979558467864990234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.65362658425288966412836089148186147212982177734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.57577880104049172782509913304238580167293548583984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.57125914708815572762290457831113599240779876708984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.029178292428728568042028967965961783193051815032958984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1643766842603195110772418274791561998426914215087890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.117820658546517353926219584536738693714141845703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0813778143119303909447381784048047848045825958251953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0716376994440456049684229355989373289048671722412109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0174628607593150519949887211623718030750751495361328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{189513414139692226}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{135837970925220416}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{93822232118127456}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{82592644229602166}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20133307701369376}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.9180507659912109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.6426645604190444061032394529320299625396728515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{13716}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.75143182277679443359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.745930433273314985598290149937383830547332763671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.44003606333357636604119988987804390490055084228515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.238410596026489951526627919520251452922821044921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99935060739517200811832253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98687308789878491754876677077845670282840728759765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95479498803615570068359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{30684}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95471984148025523797542746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00845645346388862288733445637944896589033305644989013671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.441379674250374443023048343093250878155231475830078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6371060}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6371060}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6371060}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6371060}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{36}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{31.79470198675496561691034003160893917083740234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{21.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.453050218557350614645429232041351497173309326171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.712132372911521205338658546679653227329254150390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.65440463793211922638448641009745188057422637939453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{17194}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.57762520285609897374712318196543492376804351806640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.5719692799724305221076292582438327372074127197265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0290504744421008209709356151506653986871242523193359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.566142559051513671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.539584000379051076379255391657352447509765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.622814595699310302734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.3909714221954345703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5438545242696279924388136350899003446102142333984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7581255435943603515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61540159326515464499607332982122898101806640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.490842044353485107421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.48071384429931640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{23696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.056591691486692873025443617507335147820413112640380859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.466887709092356606443985356236225925385951995849609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.389815056069120757786805597788770683109760284423828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.317014627620137823260648701761965639889240264892578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.30710089047030331155241356100304983556270599365234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03003078111337019462379060996681801043450832366943359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.438270590125455383745389781324774958193302154541015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.3667976017568197466545143470284529030323028564453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.310034719673494441050110026480979286134243011474609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.30898509158054132672788227864657528698444366455078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0237209428216763433538982752679658005945384502410888671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{505291588192370743}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{422888842903655680}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{357445695486327296}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{356235556686122123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{27348385088660072}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{155.63616943359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.4297275164269507286007865332067012786865234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.906459808349609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.7463226318359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59340187814654488107635188498534262180328369140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{20}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{12.2913907284768217920145616517402231693267822265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999882876873016357421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99797368128568131329103607640718109905719757080078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99078525602817535400390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99062454700469959600894753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{4157}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00173144055143632509367879190875783024239353835582733154296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.8649411118430834211068258809973485767841339111328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5840756}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5840756}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5840756}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5840756}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{43}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{37.89403973509934075991623103618621826171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{30}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{30}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.08479934677222988881339915678836405277252197265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.467223527547085126787607123333145864307880401611328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.390285689371118904578139563454897142946720123291015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.31733677986096975320862156877410598099231719970703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.30737333742800687641505419378518126904964447021484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.030093230132056884851277089865106972865760326385498046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{92.1637389659881591796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.550938994679228244422120042145252227783203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.674093544483184814453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.494228363037109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.6243248908567042843031913434970192611217498779296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7590630054473876953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.6170093365852409306171466596424579620361328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.496950566768646240234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4878709316253662109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.055963484607059639508452875134025816805660724639892578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.704336612303127385104062341270036995410919189453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.64649614613160200082830897372332401573657989501953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.5715317795285483892797628868720494210720062255859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.56078043777497954547328617991297505795955657958984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0283186435334116977380336521719073061831295490264892578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1713989500014133915417602338493452407419681549072265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.12450355554302812433054015173183870501816272735595703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0897322180786922218853618460343568585813045501708984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07536675377881170423410850389700499363243579864501953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01716370111532039555157780341687612235546112060546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{197609535323663285}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{143542826585570192}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{103454203878995584}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{86891951164001400}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19788400114497412}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.51984310150146484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.3223633639859837529684227774851024150848388671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64782559871673583984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.627370357513427734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.4404406740468065351024051778949797153472900390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.331125827814569451135184863233007490634918212890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99946641921997081414730246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98593584078037188600518447856302373111248016357421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{24566}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.954392015933990478515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.945151627063751220703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0095472108221392910920588548151499708183109760284423828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.51109354653178107330546708908514119684696197509765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7137589}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7137589}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7137589}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{7137589}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{36}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{32.0264900662251648100209422409534454345703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{23}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.2929405622664429387214113376103341579437255859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.70488947902785226151678443784476257860660552978515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.64726763332431735964433983099297620356082916259765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{26829}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.572493091428477374194017102126963436603546142578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.5614775445639945683495852790656499564647674560546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0282270457469195705513254068819151143543422222137451171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{92.212519168853759765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.5350098073087821148874354548752307891845703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{9134}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.55961477756500244140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.0812427997589111328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5968229579783315141838784256833605468273162841796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7457535266876220703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61596390427343106210855694371275603771209716796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{22401}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.50706946849822998046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.5066106319427490234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.057029170658235282809211952326222672127187252044677734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.71109423157826545658366512725478969514369964599609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.65372868355233626491695986260310746729373931884765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.57581721015741116342923078263993375003337860107421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.57136739664562596896502100207726471126079559326171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.029323200574443382404599134360978496260941028594970703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1644647717913889917173975163677823729813098907470703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.117896702236690187337586621652008034288883209228515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7310}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0814296805459929495807358534875675104558467864990234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07163770586374369753190904930306714959442615509033203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0174471672969169801226119176362772122956812381744384765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{189614972148549970}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{135925643330910336}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7310}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{93882029814741168}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{82592651631010208}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20115214371088896}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.87827014923095703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.65154951139791084102625973173417150974273681640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.79167711734771728515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.74662494659423828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.4412442825297662185590752415009774267673492431640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.238410596026489951526627919520251452922821044921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99935060739517200811832253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98685919883235395655418642490985803306102752685546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95471327006816875115902121251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9546935558319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{30684}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0084662084234712921271270857914714724756777286529541015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.441379674250374443023048343093250878155231475830078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6396017}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6396017}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6396017}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6396017}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{36}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{31.80132450331125681941557559184730052947998046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{21.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.452245538168193572658992707147262990474700927734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.71161192519514304688499350959318690001964569091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.65450684364563105344103632887708954513072967529296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{17194}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.57766368935049694499639372224919497966766357421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.57207766409504667848295866861008107662200927734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0291956561930747475475111940568240243010222911834716796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.9657807350158833514797152020037174224853515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.5457137025744742686583776958286762237548828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22401}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.9488074779510498046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.8687045574188232421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.551966234638555430791484468500129878520965576171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.76941967010498046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61959253241684297819347193581052124500274658203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.5127885341644287109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.495399951934814453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.057091522566042447739409482210248825140297412872314453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.4633675384606428249156806487007997930049896240234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.389945826071633694365203837151057086884975433349609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.320946827591013617020365700227557681500911712646484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.312498058804795808551801883368170820176601409912109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0297289474514793490567132749902157229371368885040283203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.437731908416957582463879816714324988424777984619140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.36672177667631700170858266574214212596416473388671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4157}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.31025238827439582944833773581194691359996795654296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.30884396505824718293098385402117855846881866455078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0237352351645055796580674467577409814111888408660888671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{504670530466505312}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{422801422537755584}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4157}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{357696650297184192}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{356072848883698855}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{27364863038059116}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.4159393310546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.266749906224134747390053234994411468505859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.3579044342041015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.61283111572265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59797218712847044486125014373101294040679931640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{20}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{12.3178807947019866020355038926936686038970947265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999834835529327392578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9980462963217930916215436809579841792583465576171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9910742342472076416015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{15399}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99066841602325439453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{4157}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0016530495893029273878072071823908117949031293392181396484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.8747922125117579827957570159924216568470001220703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5853043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5853043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5853043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5853043}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{43}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{37.966887417218543987473822198808193206787109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{30}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{30}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.08246294114262742169785269652493298053741455078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.4637008249612442067899564790423028171062469482421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.390417238350745154917831314378418028354644775390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.321272908155751546477318925099098123610019683837890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.31277529390261415986884685480617918074131011962890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0298012123865056162419495677795566734857857227325439453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{92.5717060565948344219577847979962825775146484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.55550161576428536136518232524394989013671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24173}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.679595530033111572265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.1144449710845947265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.6259875847845552954140657675452530384063720703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7545759677886962890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61362399012837176570656083640642464160919189453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.502237260341644287109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.50151824951171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.057244968222027292625853078789077699184417724609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.456192331901186187703700625206693075597286224365234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.385180472319526068236683613577042706310749053955078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.306283922051853896295625645507243461906909942626953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.304535216409694109440664533394738100469112396240234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0292602481800916906784504334382290835492312908172607421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.44547722418133639532555889672948978841304779052734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.370148037811814656361519837446394376456737518310546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.31353294373465667721490035546594299376010894775390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.312034624953820005632820766550139524042606353759765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.02372211122293164942131937777958228252828121185302734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{513600271571228112}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{426751632681269440}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{361478873234374336}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{359751429291191431}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{27349732163593332}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.3029937744140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{92.8864845124301581336112576536834239959716796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{81.2790679931640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{80.37683868408203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.6339667658878003209110829629935324192047119140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{21}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{12.5298013245033104112735600210726261138916015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{7098}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{7098}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999934971332550048828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9980670920270957591213800697005353868007659912109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29195}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99055941402912128790347878748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4157}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99032324552535999639957253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{15399}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00162595723812415117980056944446687339222989976406097412109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.9490461141876640471792825337615795433521270751953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5867473}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5867473}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5867473}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5867473}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{43}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{38.046357615894038417536648921668529510498046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{30.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{29}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.178576448580482605166253051720559597015380859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.45666338884222301697235479878145270049571990966796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.385646736857403471532279581879265606403350830078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.30659483636424667007958078102092258632183074951171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.304805387209581224450261061065248213708400726318359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0293408609993081638533940491697649122215807437896728515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{92.4948673248291015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.5620017746426384519509156234562397003173828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.71232950687408447265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.66510009765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.559510537742517133352748714969493448734283447265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.757457256317138671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61347652113200812351578861125744879245758056640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.5096724033355712890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24144}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.5031006336212158203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05478389908627780136018969869837746955454349517822265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6621551572052073453278353554196655750274658203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5824616449107635762771906229318119585514068603515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.49782164341601042867324622420710511505603790283203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.49051629023424980768908199024735949933528900146484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03554178971837144984657896884527872316539287567138671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.28941094044583437483453280947287566959857940673828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.18753883988987019026950520128593780100345611572265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7098}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1390173984349327984677557878967490978538990020751953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1357324545199357912483861809960217215120792388916015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0244423818601612642675835473937695496715605258941650390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{333668096908493929}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{216217561458051744}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7098}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{160276148170132288}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{156488865689104868}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{28180147670392224}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{33.5944671630859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{13.575011654405404470935536664910614490509033203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{8.01591932773590087890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{7.73836469650268465869658029987476766109466552734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.60855280594514926661986464750953018665313720703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.65562913907284769976513416622765362262725830078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99940294027328480108707253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98810393960270659352573829892207868397235870361328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{17096}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95967742800712596551448996251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.957381546497344970703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{4157}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0095583461319999930838609003558303811587393283843994140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.709876937529092089107507490552961826324462890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{8335639}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{8335639}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{8335639}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{8335639}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{38}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{33.5562913907284752212945022620260715484619140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{27}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{27}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.8328704429901225836374578648246824741363525390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.66268573318054790899367390011320821940898895263671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.58315734138908215111740673819440416991710662841796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.49819514210465409842498729631188325583934783935546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.49084433481925737741136117620044387876987457275390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{19917}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03550668941778091503014280760908150114119052886962890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{92.6686336994171142578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.5461493280549660767064779065549373626708984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.652634143829345703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.10903263092041015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.54140209010584161575252437614835798740386962890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.749848842620849609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.6094027670803452423342605470679700374603271484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{23367}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.485122025012969970703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{4.483571529388427734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05489566354758089461451930901603191159665584564208984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.5262864214512970040260597670567221939563751220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.39110203858047232206018861688789911568164825439453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{23241}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1814938116835701220619370133135817013680934906005859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.1721580099632449012414525668646092526614665985107421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07469415660008808799386059718017349950969219207763671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1701476788002432016799758685010601766407489776611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.11718246138337605477541814025244093500077724456787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{19093}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0769828372145550943184133529939572326838970184326171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0603247131780288992075611531618051230907440185546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.015044749380677090166980036656241281889379024505615234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{196166917847738901}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{135102179691655712}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{19093}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{88755168510308928}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{69549659082189669}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17345415092403160}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.47019867549668870054802027880214154720306396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.995876729488372802734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{6082}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.97632468101994096532081357509014196693897247314453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9498957693576812744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29195}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.945259749889373779296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0119654818605877157067229887843495816923677921295166015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.52497804457235541786275234699132852256298065185546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5788021}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5788021}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5788021}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{5788021}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{36}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{21.980132450331126392484293319284915924072265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{913}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.655639428869864815396795165725052356719970703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.5265251796889061086659467036952264606952667236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.39155720215207789891564971185289323329925537109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1816808573153142203349119654376409016549587249755859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.1723177367218544642213373663253150880336761474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07472170796426648442523088533562258817255496978759765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{87.597664356231689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4800}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.8236981354012442579914932139217853546142578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.211779177188873291015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.9657886028289794921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.189241566289711560244768406846560537815093994140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7462863922119140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58619113157916569178951249341480433940887451171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{11498}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.470986068248748779296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{23696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4674932956695556640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.057661354676853127099178664138889871537685394287109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.53054662987978773447395042239804752171039581298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.387761590833687053159195556872873567044734954833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.181083856078374350051518604232114739716053009033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.169719251312953012256201645868713967502117156982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07379627587282540368551764231597189791500568389892578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.173717281903376707941077938812668435275554656982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.12126927384342524318672218441861332394182682037353515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0801746850862353477307209459468140266835689544677734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.06340663004847919836937109039354254491627216339111328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0152959572798831745787939695446766563691198825836181640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{200282390028252879}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{139813953662141632}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{92435118561002656}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{73102867317542355}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17635038081524966}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.11057758331298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.297075640286831088587859994731843471527099609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29110}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.480218231678009033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{14929}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.448263645172119140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.51224755971247670771617777063511312007904052734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.642384105960264850665453195688314735889434814453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99641281366348277703792746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{27584}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.97912407316119465239268038203590549528598785400390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{11498}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95144067704677581787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29052}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.951070129871368408203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01253311993857313295930300256486589205451309680938720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.5190971640335211301220397217548452317714691162109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7020342}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7020342}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7020342}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{7020342}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{36}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{2743}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{22.23841059602649039561583776958286762237548828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{913}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.8192302484584939037404183181934058666229248046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.530787320828967512653662197408266365528106689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.388214096178541800963301966476137749850749969482421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5928}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1812705482715956384343058971353457309305667877197265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.1698767154117285793635261370582156814634799957275390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07382507256118518712550979898878722451627254486083984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{88.3772742748260498046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.8385770462996191554339020512998104095458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{9134}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.166368067264556884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.903672695159912109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.20928875198105512112078940845094621181488037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.72804737091064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58673467541372570366320360335521399974822998046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.453691899776458740234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24202}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.44956684112548828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.056594625053719489760073457773614791221916675567626953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.521848885154867048186133615672588348388671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.379622239632713576185096826520748436450958251953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{22545}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1737697654880362707618957074373611249029636383056640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.1635670553837058893709155427131918258965015411376953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07258488349707760411977375269998447038233280181884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1858239047325661863485635194592759944498538970947265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1336718448463214137245103074747021310031414031982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0918888941225383948374627607336151413619518280029296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0793517482834387999357517173848464153707027435302734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.015733383420464118473969250544541864655911922454833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{214240375836189658}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{154113144483793952}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{105940682068416320}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{91486337024126104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18139356085677904}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.95111083984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.271134603891940884068390005268156528472900390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{7310}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64434564113616943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6082}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.634481906890869140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{8048}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.46292293381569304955291954684071242809295654296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99722492694854736328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9834000168257202023625040965271182358264923095703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95266561210155487060546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{14929}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.948092043399810791015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20976}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00908258465398343282914961349661098211072385311126708984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.36393726262341952182310933494591154158115386962890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6764310}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6764310}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6764310}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{6764310}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.642384105960264406576243345625698566436767578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.4920937568309735610228017321787774562835693359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.522085630233287023571620011352933943271636962890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.380065153634901786716682181577198207378387451171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22545}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.173893582144618363827248685993254184722900390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.16371881152666623027158721015439368784427642822265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07261031145237735462405481712266919203102588653564453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.1778752803802348125827847979962825775146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.928052772749339283109293319284915924072265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{32103}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{80.75560891628265380859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{78.8330733776092529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.348952706601405981956531832111068069934844970703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7217986583709716796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{19093}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5874291208406159370269961073063313961029052734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.45963561534881591796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{27584}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4500758647918701171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0578075427459331658841534817838692106306552886962890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.5302119900116679662716023813118226826190948486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.382527848440148421360618158360011875629425048828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{26932}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1721907628094417053166154119026032276451587677001953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.1646089154752408967308241471982910297811031341552734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07312097826004933243115857521843281574547290802001953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.18261587226937259220704845574800856411457061767578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1289988942897635215700802291394211351871490478515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29726}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08672662668289950194111526116103050298988819122314453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07275765660371820431340239565543015487492084503173828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01579613295784036697266827786734211258590221405029296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{210541766221896871}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{148725599297173792}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29726}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{99988992924724832}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{83883866923227094}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18211701376723120}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.9180507659912109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.6426645604190444061032394529320299625396728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{13716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.75143182277679443359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.745930433273314985598290149937383830547332763671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.44003606333357636604119988987804390490055084228515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.854304635761589548081929024192504584789276123046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99624240398406982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98140878393160591031119110994040966033935546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9501501619815826416015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{13293}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94897919893264759405582253748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20976}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01150261993786940058204226744464904186315834522247314453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.4515954204299952312595678449724800884723663330078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6006100}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6006100}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6006100}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6006100}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{22.76821192052980080688939779065549373626708984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{6532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.8282459358755289713371894322335720062255859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.5304525291461288372119042833219282329082489013671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.382974046094407327700537280179560184478759765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{26932}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.17231363229513163570771894228528253734111785888671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.164761638247261255063591534053557552397251129150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0731460622675019489502545866344007663428783416748046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.2571122646331787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.97304187547291576265706680715084075927734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27671}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.258380413055419921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.1210005283355712890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.29674043820233197976676819962449371814727783203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.720051288604736328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.584183841351642030303992214612662792205810546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{8840}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.465468108654022216796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.465061664581298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{27584}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05737965134657400934070636822070810012519359588623046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.367198589207115511090506743130390532314777374267578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.257162202967756992055825548959546722471714019775390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{23241}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.11406325799048915026201456157650682143867015838623046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{29110}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.11141008093914529786250255938284681178629398345947265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.049538431506045955965422677991227828897535800933837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.405903848903757913380019317628466524183750152587890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.3249851956211295966880925334407947957515716552734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.247621278750981776983763893440482206642627716064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.24513353824894490440300387490424327552318572998046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0274161512380699072533030147269528242759406566619873046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{467975276203830907}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{374682420710463232}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{285487897270253408}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{282619727747573650}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{31608670335924432}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{155.63616943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.4297275164269507286007865332067012786865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.906459808349609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.7463226318359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59340187814654488107635188498534262180328369140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{18}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{12.74172185430463599686845554970204830169677734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99838989341495842921858638874255120754241943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99268817901611339227230246251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.992678165435791015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00144977096171728238142850653247251102584414184093475341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.750926249326907768733008197159506380558013916015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5475796}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5475796}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5475796}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5475796}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{44}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{36.74172185430463599686845554970204830169677734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{11.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{5.9772898864126648987848966498859226703643798828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.3673651747096824404792414497933350503444671630859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.25746328391531825285909462763811461627483367919921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.114215142334727459694221352037857286632061004638671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{29110}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.1115134462783975155542037782652187161147594451904296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.049567209268534584420962119111209176480770111083984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{89.87618541717529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9609383115705298905595554970204830169677734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.50990164279937744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.4626958370208740234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.2585761073790939779115660712704993784427642822265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7670114040374755859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58539306722729378407166223041713237762451171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{6532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.46989500522613525390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4606549739837646484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.058481667417801315445036181017712806351482868194580078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.52134823100151750363551172995357774198055267333984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.37962084660731587604232117882929742336273193359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1737061391716470115653692118939943611621856689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.1635693608542863886068374768001376651227474212646484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07258146186779070030414828806897276081144809722900390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1860293170777269911031481797181186266243457794189453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.133779386831283597647512806361191906034946441650390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.092492968606514625040659893784322775900363922119140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.079351751065790399053412329521961510181427001953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0156948568850411203368100387933736783452332019805908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{214477200146237203}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{154237131950904960}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{106637132531376720}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{91486340231959114}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18094938014490740}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.51984310150146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.3223633639859837529684227774851024150848388671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{23447}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64782559871673583984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8048}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.627370357513427734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6082}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.4404406740468065351024051778949797153472900390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.006622516556291202505235560238361358642578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.997250616550445556640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98356079147351493929818389005959033966064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29565}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95254163444042205810546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{14929}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.948091447353363037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20976}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0088133033652413282632576141395475133322179317474365234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.354660340105851290548599763496895320713520050048828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6772629}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6772629}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6772629}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{6772629}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.609271523178808394050065544433891773223876953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.5667061224048683953924410161562263965606689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.521584748950187471194794852635823190212249755859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.380063824419225648743037027088575996458530426025390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.17382991486947518833261483450769446790218353271484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.1637211191362430151574614001219742931425571441650390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07260708045637133400962426321711973287165164947509765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{89.8906590938568115234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.91845456338086250980268232524394989013671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{18668}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.232249319553375244140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.22672557830810546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.2655944129253249297306638254667632281780242919921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.748263835906982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5846661021377865807835405576042830944061279296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{6532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.462316930294036865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{27584}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4564473628997802734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.059663074229783584490061087990397936664521694183349609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.530121480665301181289805754204280674457550048828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.38240246389215404310135681953397579491138458251953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{30371}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.172262018064911204273670364273129962384700775146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.1646089159909961130434652432086295448243618011474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0732313791840137617850103879391099326312541961669921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.182762735299915213271759739654953591525554656982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.12906661316895695623685469399788416922092437744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29726}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08673426586137676641552474166019237600266933441162109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0727576567243665983664158147803391329944133758544921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0157984454434342662387802391776858712546527385711669921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{210711087768041206}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{148803673849263776}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29726}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{99997800297868864}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{83883867062325298}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18214367491093416}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.87827014923095703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.65154951139791084102625973173417150974273681640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.79167711734771728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.74662494659423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.4412442825297662185590752415009774267673492431640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.860927152317880750587164584430865943431854248046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99624240398406982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98159165808696624555551579760503955185413360595703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9501501619815826416015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{13293}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94897919893264759405582253748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20976}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01146361657448779526602411493740873993374407291412353515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.446320276701834328658691219970933161675930023193359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6031057}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6031057}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6031057}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6031057}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{37}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{22.78807947019867441440510447137057781219482421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{6532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.8338501112067771003921734518371522426605224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.53036197873875201569404680412844754755496978759765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.382848603646726293181501432627555914223194122314453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{30371}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.17238493360214135474706154127488844096660614013671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.164761638763494977499846072532818652689456939697265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07325713232669568697463802209313143976032733917236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{89.900264739990234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.933253356163078251483966596424579620361328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{30371}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.397212088108062744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.3364498615264892578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.2486424497163113311870574761996977031230926513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.713474273681640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5895995099023476626598494476638734340667724609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.477419674396514892578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{28778}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.46851062774658203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05595019769201493853305606762660318054258823394775390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.367872457797292773395980702844099141657352447509765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.25699249316324734859762202177080325782299041748046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.11377285174409978996123982142307795584201812744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{29110}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.10896699850676140608474185000886791385710239410400390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0496684790345237880959672338576638139784336090087890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.406047124285208782534795091123669408261775970458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.324882340659903123825102966293343342840671539306640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2477259720847650725783495317955384962260723114013671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.2451274528510392070046464141341857612133026123046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.027473079210847510533977100521951797418296337127685546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{468140461472186275}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{374563837013809728}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{285608600466161216}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{282612711761464108}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{31674303819953400}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.4159393310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.266749906224134747390053234994411468505859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.3579044342041015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.61283111572265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59797218712847044486125014373101294040679931640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{18}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{12.74834437086092719937369110994040966033935546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1412}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99842912235007386101415249868296086788177490234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99268728494644176141292746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.992674767971038818359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0013984522374233220032291313827954581938683986663818359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.7575515142143967040055940742604434490203857421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5488083}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5488083}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5488083}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5488083}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{44}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{36.66887417218543276931086438708007335662841796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{11.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{6.1003982654751638392554013989865779876708984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.368039349011104410802630582111305557191371917724609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.257293440847765231271893071607337333261966705322265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1139246378040010554411054499723832122981548309326171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{29110}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.10906809717461087017031928780852467752993106842041015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.049698360507539750263727995616136468015611171722412109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{88.3321521282196044921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.893336239240028362473822198808193206787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{23447}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.393484771251678466796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.2078721523284912109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.1876896952866307088925168500281870365142822265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.726370334625244140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58789856070714296976120749604888260364532470703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{7790}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.478738963603973388671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4628751277923583984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.055821270334427137982391542436744202859699726104736328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.36311881296637249505465661059133708477020263671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.255365302668355609316819254672736860811710357666015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.114750747652371420937100765513605438172817230224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{29110}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.11251817399200879366016891935942112468183040618896484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.049660332784572568110004198160822852514684200286865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.4087456470736168245849739832920022308826446533203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.327700331860620475143974772436195053160190582275390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.24910699471378017211264932484482415020465850830078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.246135102254131987731256003826274536550045013427734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.02750336317589267831618116133540752343833446502685546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{471251646425613595}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{377812759668909696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{287200811153501312}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{283774452427393987}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{31709218854498736}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.3029937744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{92.8864845124301581336112576536834239959716796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{81.2790679931640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{80.37683868408203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.6339667658878003209110829629935324192047119140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{19}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{13.006622516556291202505235560238361358642578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1412}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1412}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99845002897527834750945885389228351414203643798828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9937088787555694580078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99269151687622081414730246251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00134199137442285909745109950819141886313445866107940673828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.8752366340452046866715818396187387406826019287109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5502513}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5502513}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5502513}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5502513}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{44}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{36.87417218543046004697316675446927547454833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{11.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{5.9859710557507668227117392234504222869873046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.363283547613311441626393616388668306171894073486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.255664173482683942939530652438406832516193389892578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.114903489132205216538551439953153021633625030517578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{29110}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.1126225674107073915219956461442052386701107025146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.04968887466128989183200559409669949673116207122802734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{87.340034008026123046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4800}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.856133415209541226431610994040966033935546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7790}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.221376597881317138671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.9273684024810791015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.18238036495460807628887778264470398426055908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.737315654754638671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58909326199664224787966304575093090534210205078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{2743}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4583957195281982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{23696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4427516460418701171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0591437368078770731028015461561153642833232879638671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.50602796872916300241485032529453746974468231201171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.347241824583108094071093319143983535468578338623046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1491470719354753560192961003849632106721401214599609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.145394723423100391546114451557514257729053497314453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06761211881086211239466621236715582199394702911376953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.26585690555168761672888422253890894353389739990234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.188285150104643694835004907872644253075122833251953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{1412}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.135277666356530879010477974588866345584392547607421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.130274506733676798120313833351247012615203857421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0223126718650250334408102759198300191201269626617431640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{306512143558772170}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{217077998553771904}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{1412}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{155964530635474656}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{150196280315305568}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{25724759218423528}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{33.5944671630859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{13.575011654405404470935536664910614490509033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{8.01591932773590087890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{22545}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{7.73836469650268465869658029987476766109466552734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.60855280594514926661986464750953018665313720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{5.3178807947019866020355038926936686038970947265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99938166141509998663394753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98674248622742710690403100670664571225643157958984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9625551998615264892578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{7098}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95680391788482677117855246251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.008361937172525736594597134399009519256651401519775390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.749135138669100530961486583692021667957305908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7970679}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7970679}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7970679}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{7970679}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{39}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{28.344370860927153188413285533897578716278076171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{1412}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{8.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{9.7056318446995657467368801007978618144989013671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.50625753639625481472563706120126880705356597900390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.34764784917924396179245150051428936421871185302734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{12493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1492752170980577997028149184188805520534515380859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.145488690466375081289385207128361798822879791259765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06765787240339361796603867560406797565519809722900390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{89.5447294712066650390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.9611849548011406341174733825027942657470703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{18668}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{80.837035596370697021484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{79.11759853363037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3121013614916663403420216127415187656879425048828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.752509593963623046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{28716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.58964491522075324070328861125744879245758056640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.470319569110870361328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{24202}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4644296169281005859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0617496818643770151169292148551903665065765380859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.71584725760343437261923327241674996912479400634765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.63902079873878048221769176961970515549182891845703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{7098}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.52979208835776869790379350888542830944061279296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.52730339280895066611520860533346422016620635986328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0317321236846111187634988937134039588272571563720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.18263435082102519313451693960814736783504486083984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.12159151304679087501892098543976317159831523895263671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{28716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0781542788153279655016802962563815526664257049560546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.06464661360273170342960469270110479556024074554443359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.016269550284457846844876627301346161402761936187744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{210563070541471196}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{140185470169329264}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{28716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{90105748723230976}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{74532471022598964}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18757514393233892}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{17096}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.47019867549668870054802027880214154720306396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99750804901123035772769753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.97852400320255206178643447856302373111248016357421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{913}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94610036909580230712890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.92754381895065318719417746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0122870413718872140140803139729541726410388946533203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.53744486265625113219357444904744625091552734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5896885}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5896885}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5896885}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{5896885}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{41}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{28.4834437086092719937369110994040966033935546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.4043936039121991399269973044283688068389892578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.71677247699460855390185543001280166208744049072265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.63978291844806312038684836807078681886196136474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5314800699574504516675688137183897197246551513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.52791944335661533660442046311800368130207061767578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.031657561132913382417886083430857979692518711090087890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.6798899173736572265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.5750448103772072272477089427411556243896484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{18668}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.3839404582977294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{79.3032329082489013671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3522030440289347641424910761998035013675689697265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7543885707855224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61295981912423425086444694898091256618499755859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.5005047321319580078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{28778}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.493517398834228515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.059907597311307674015079527407579007558524608612060546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.71253189621949319931815125528373755514621734619140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.63378722365749562417391871349536813795566558837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{11611}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.5295823929833247678544694281299598515033721923828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.52444790936498575373292396761826239526271820068359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{11498}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0313588208922854771998345313477329909801483154296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.188722722522415897739023193935281597077846527099609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.126244616698418854472407701905467547476291656494140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{11498}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0822426810429009169656211497567710466682910919189453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.06857470977105099840809288025411660782992839813232421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.016240226248072815729006634910547290928661823272705078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{217582485204044212}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{145550133432455776}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{11498}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{94819355570882368}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{79061257567218004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18723706081083716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.11057758331298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.297075640286831088587859994731843471527099609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29110}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.480218231678009033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{14929}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.448263645172119140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.51224755971247670771617777063511312007904052734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{11498}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.622516556291390799060536664910614490509033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9977920055389404296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98080196917451767379958482706570066511631011962890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{16069}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95792391896247874871761496251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24262}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.957883775234222412109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{9132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01151430506600963250829483541792797041125595569610595703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.56076723523222649081532154013984836637973785400390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7129206}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7129206}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7129206}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{7129206}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{41}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{28.72847682119205359185798442922532558441162109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.5062764321134647360622693668119609355926513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.713452830567163243102868364076130092144012451171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6345433293905007321455968849477358162403106689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.530553301258601894829780576401390135288238525390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.5264694044929110194885879536741413176059722900390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11498}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.031288245246457214998603291178369545377790927886962890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.8731882572173930157077847979962825775146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.581827488956065508318715728819370269775390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7467}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{80.9808099269866943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{79.22819805145263671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.35626873942433423536613190663047134876251220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.791477680206298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61846142730965514289209750131703913211822509765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.501349031925201416015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.500324249267578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.060444744520330363768412240688121528364717960357666015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6854556380094558587501296642585657536983489990234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.6186953744994181381144926490378566086292266845703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.51988800734750795218275243314565159380435943603515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.51740608996243875328246986100566573441028594970703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0302755087929055845263892621233026147820055484771728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.203814040549097297283509533372125588357448577880859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1403756566997508559158092111829319037497043609619140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0935126592308048731894132288289256393909454345703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08279153718015440366340129685340798459947109222412109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.016578039345494781364731551320801372639834880828857421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{234981590289866279}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{161842113332451008}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{107812755780166928}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{95452143614457388}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19113178065639352}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.95111083984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.271134603891940884068390005268156528472900390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{7310}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64434564113616943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6082}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.634481906890869140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{8048}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.46292293381569304955291954684071242809295654296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.006622516556291202505235560238361358642578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99797385931015003546207253748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{26932}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9849183575207034468945721528143621981143951416015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{8840}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.961849987506866455078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95701932907104481085269753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00888312837794834331273108318782760761678218841552734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.40684033254060059103807134306407533586025238037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6873174}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6873174}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6873174}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{6873174}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{41}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{29.887417218543046004697316675446927547454833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.60667452325586790351508170715533196926116943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.68634157679226159842755805584602057933807373046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.61943420122054793086618929010001011192798614501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{7098}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.52083952130345345654660604850505478680133819580078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.5180105774537639984345105403917841613292694091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03021787810160812826065779290729551576077938079833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.656856536865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.6420298175306555776842287741601467132568359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.289232075214385986328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{79.4946441650390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.4281047918466793777980683444184251129627227783203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7870121002197265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{19093}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.6195129969262129776552683324553072452545166015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{23241}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.494820177555084228515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.49272251129150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0584024373258581197543293228591210208833217620849609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.704816415929176098842390274512581527233123779296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.62430918708305416231496565160341560840606689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.52370316592798149546439390178420580923557281494140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.521449397118541657647483589244075119495391845703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0309024266836278420356176610539478133432567119598388671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.19827230620907199121205621850094757974147796630859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1349182281508599923203206571997725404798984527587890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.088177135513167248515031815259135328233242034912109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0763468430547238063876847036226536147296428680419921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0166611152681694942023771233152729109860956668853759765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{228592405596432848}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{155550126598579424}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{101661315747762672}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{88021917166635051}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19208958083406080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.9180507659912109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.6426645604190444061032394529320299625396728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{13716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.75143182277679443359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.745930433273314985598290149937383830547332763671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.44003606333357636604119988987804390490055084228515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.860927152317880750587164584430865943431854248046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99766051769256602899105246251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98283625162200427549663572790450416505336761474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95133471488952625616519753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.941314160823822021484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01122187191775352900491302676755367428995668888092041015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.515196035464283941252006115973927080631256103515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6114964}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6114964}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6114964}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6114964}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{41}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{29.589403973509934786534358863718807697296142578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.69473159679655083209581789560616016387939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.70572737816072639294162627265905030071735382080078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.62505434570172635488916057511232793331146240234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{11611}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5253716089274014233723164579714648425579071044921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.522058608420906011815532110631465911865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0308388453773975786120775666176996310241520404815673828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.6937975883484028827297152020037174224853515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.63601038787538755059358663856983184814453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{17197}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.3759014606475830078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8840}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{79.694097042083740234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3635143062812147274343033132026903331279754638671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.73076152801513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.621443672685433767810536664910614490509033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.506965160369873046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.5032379627227783203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.054071052880519776540069187831250019371509552001953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.4505775185013429773306370407226495444774627685546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.38937781002413307529508301740861497819423675537109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{28716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.323703563655007686694631274804123677313327789306640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{9816}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.318141293842261585478325969233992509543895721435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.028273159990963296628319056935652042739093303680419921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.456757311611598215694840519063291139900684356689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.349072646178722578724773484282195568084716796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.269256164562843292031857345136813819408416748046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.26846168491917821175007929923594929277896881103515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.028865630308298299844249612533531035296618938446044921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{526605326943422293}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{402453360449466368}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{310431222372462080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{309515249706308201}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{33279805926468280}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{155.63616943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.4297275164269507286007865332067012786865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.906459808349609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.7463226318359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59340187814654488107635188498534262180328369140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{23}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29565}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{13.629139072847682001565772225148975849151611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99999970197677601202457253748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13654}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99800028706228494090879621580825187265872955322265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99171392619609832763671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.991044223308563232421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0016901568220495798329505721113719118875451385974884033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.047825187980237160445540212094783782958984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5584660}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5584660}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5584660}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5584660}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{45}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{38.5960264900662224363259156234562397003173828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{14}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{7098}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.71889538528788055060658734873868525028228759765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.450901605520666493021053611300885677337646484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3898475717158611519863598005031235516071319580078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{18668}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.324093051042709412445930183821474201977252960205078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{9816}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.318423535380195465993580228314385749399662017822265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.02833341071498966801112118218952673487365245819091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.8073475360870361328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.6152283861147651577994110994040966033935546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{26374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.30133903026580810546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{79.2999744415283203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.386740792879260997239043717854656279087066650390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.749933719635009765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61862631507267185071441417676396667957305908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.50518953800201416015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.500221729278564453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05459567475115763290904880022935685701668262481689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6836620649648905700956902364850975573062896728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.61869340864737143448337519657798111438751220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{30899}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.520065897855285452777707178029231727123260498046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.51811774438739444104129461265983991324901580810546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0301952599379473433927056902348340372554957866668701171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2038608843317439023312687140787602402269840240478515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1404890607024087412213475545286200940608978271484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09416126054999139627366133709074347279965877532958984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.082931042124690101946526965548400767147541046142578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0165601038316263195204758318368476466275751590728759765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{235035597494236580}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{161972859245823808}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{108560542188973472}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{95612981865011542}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19092499826004228}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.51984310150146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.3223633639859837529684227774851024150848388671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{23447}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64782559871673583984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8048}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.627370357513427734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6082}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.4404406740468065351024051778949797153472900390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{1696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.01324503311258240501047112047672271728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99799925088882435186832253748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{26932}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98499297543077279915024746514973230659961700439453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96066041290760040283203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95689535140991199835269753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00884654451305662455073974825836558011360466480255126953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.414740882433143720486867778163286857306957244873046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6881493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6881493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6881493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{6881493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{41}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{29.894039735099337207202552235685288906097412109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.609816175413612882039160467684268951416015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6844480158527523894207433841074816882610321044921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6194323105318695343868284908239729702472686767578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{30899}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.52101761962103021463832419613027013838291168212890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.5187230633072752450374309773906134068965911865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0301388641048121151688743424301719642244279384613037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{89.8289673328399658203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.6238423104317831757725798524916172027587890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.20114338397979736328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{79.35091304779052734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3619504708491565470040995933231897652149200439453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.773114681243896484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.6193005154464419348414594423957169055938720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.498317062854766845703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4959132671356201171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.056147466197973637525020507155204541049897670745849609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.70495421337041774823006790029467083513736724853515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.62428730789605768602967827973770909011363983154296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.5237043707133761660799109449726529419422149658203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.52133813817798702050509973560110665857791900634765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0308944171849114719574647125455157947726547718048095703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.198309672249317003878132936733891256153583526611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.13499207717037264853132683128933422267436981201171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08819258013537910334544989154892391525208950042724609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07640795145471369897993696440607891418039798736572265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01665280925969238323691712366780848242342472076416015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{228635485707773261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{155635268721269664}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{101679122184841280}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{88092370355095476}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19199381907615368}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.87827014923095703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.65154951139791084102625973173417150974273681640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.79167711734771728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.74662494659423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.4412442825297662185590752415009774267673492431640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.874172185430463599686845554970204830169677734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99760144948959361688167746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98336176524888596617302027880214154720306396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{15662}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95513828098773967401058371251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24262}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95460277795791637078792746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0105962191913363083795029950806565466336905956268310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.50565852102837283155167824588716030120849609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6139921}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6139921}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6139921}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6139921}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{41}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{29.582781456953643584029123303480446338653564453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.69308420475026455420675119967199862003326416015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.70586535370262193378465553905698470771312713623046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.62503256308990984280171687714755535125732421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{11611}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5253728930730676704996540138381533324718475341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.52194721949611044831129902377142570912837982177734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.030833204398046716587789006780440104193985462188720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.3213505744933939922702847979962825775146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.6196209673849892851649201475083827972412109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.121362030506134033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{79.07465076446533203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3720377121324804914337391892331652343273162841796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7524166107177734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{22545}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.6210097492925381601480694371275603771209716796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{29195}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.495258867740631103515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.49457454681396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0582166009762373481972730360212153755128383636474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.452543729453746712554362829905585385859012603759765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.38931799743817696590753030250198207795619964599609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.3229943258779461867646887185401283204555511474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{9816}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.316419199392763694778096805748646147549152374267578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.028090176688460623266596627445323974825441837310791015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.456945816312070374198839317614329047501087188720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.349015187124841641530537117432686500251293182373046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{24202}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.268695947037915328081680854666046798229217529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.268159626117558114177796824151300825178623199462890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.02889673186872643295686202691285870969295501708984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{526822658066316132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{402387114670612672}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{24202}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{309785335540715008}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{309166999618264736}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{33315663584312704}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.4159393310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.266749906224134747390053234994411468505859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.3579044342041015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.61283111572265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59797218712847044486125014373101294040679931640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{22}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29565}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{13.602649006622517191544829984195530414581298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{9.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99999964237213123663394753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13654}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99804503001914124382665249868296086788177490234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29195}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99176202714443206787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9909038543701171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0016387366829487570209222813133465024293400347232818603515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.000263129044006493728602436021901667118072509765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5596947}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5596947}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5596947}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5596947}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{45}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{38.6225165562913872463468578644096851348876953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{14}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{7098}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.705627940735058967192117052036337554454803466796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.45286923071017870512378067360259592533111572265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.389787977332818391662527801599935628473758697509765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.323383067273152580156647672993130981922149658203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{9816}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.31669991316113321744296627002768218517303466796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0281545734941912352555792864450268098153173923492431640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.1968085765838623046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.6064406893900695649790577590465545654296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.19818270206451416015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{79.2337474822998046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.39992466185484776275416152202524244785308837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.777535915374755859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{913}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61991708483917040695132527616806328296661376953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.50573670864105224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.5055332183837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05952121101420933257930556692372192628681659698486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.446602701762030374066370086438837461173534393310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.3858938136626959281016979730338789522647857666015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{24262}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.318482585411221041926665975552168674767017364501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.310328900439339305794561596485436893999576568603515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0279518529880168620227465225980267859995365142822265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.46377977035578010767125078928074799478054046630859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.352103211556883011201790623090346343815326690673828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.271269311887213204759206064409227110445499420166015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.270443671009432284879636654295609332621097564697265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.029043437415367460985304859377720276825129985809326171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{534701670644804012}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{405947364445064512}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{312752223214669888}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{311800324091593886}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{33484803563880252}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.3029937744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{92.8864845124301581336112576536834239959716796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{81.2790679931640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{80.37683868408203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.6339667658878003209110829629935324192047119140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{23}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29565}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{13.9403973509933774010960405576042830944061279296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99815729832807120747162343832314945757389068603515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{24202}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.990974724292755126953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.98966938257217396124332253748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.001688738303658919581717867686165845952928066253662109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.09771805402088507008784290519542992115020751953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5611377}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5611377}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5611377}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5611377}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{46}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{20013}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{38.5761589403973488288102089427411556243896484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{14}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{7098}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.9724833110860462426217054598964750766754150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.44692392981379225336269200852257199585437774658203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.38635971584050832206003178725950419902801513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24262}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.3188061525159999742840000180876813828945159912109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.310604211151342457508661709653097204864025115966796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.028016879092474571144588679771914030425250530242919921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.7496116161346435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.5764554146899314446272910572588443756103515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.071754515171051025390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{79.3047096729278564453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.377104182399366383293681792565621435642242431640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7933237552642822265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{26374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61786281825690902991254915832541882991790771484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{20754}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.508054196834564208984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24202}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.5017240047454833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.059236075661843919093474397641330142505466938018798828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.63292568333308174555185132703627459704875946044921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.56066097074780796294390938783180899918079376220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{9134}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.47195993937772329207547272744704969227313995361328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.468246267810927097041684419309603981673717498779296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03319894427291809890778750968820531852543354034423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.27981297906428237443066109335632063448429107666015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.19849116407433797792947416382958181202411651611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.139249282234366111854484415744082070887088775634765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.13811879499097379220273751343484036624431610107421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0229317424443315764914785859218682162463665008544921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{322602400831316596}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{228844731535750272}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{160543491989068896}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{159240128935478172}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{26438499002175456}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{33.5944671630859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{13.575011654405404470935536664910614490509033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{8.01591932773590087890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{22545}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{7.73836469650268465869658029987476766109466552734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.60855280594514926661986464750953018665313720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{5.3178807947019866020355038926936686038970947265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{3175}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{3175}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.998670876026153564453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30684}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98754649012294037913051170107792131602764129638671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7790}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96741829812526713983089621251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96237051486969005242855246251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00782314333319032717550811639739549718797206878662109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.7921039209293729843608389273867942392826080322265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{8079543}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{8079543}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{8079543}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{8079543}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{41}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{33.70198675496688878183704218827188014984130859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{1696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{9.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{7098}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.217269293181939104897537617944180965423583984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.63374372811731749521868550800718367099761962890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.56133156931399275091365552725619636476039886474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{9134}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.47233404968463832407365998733439482748508453369140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.468793321696149012378640463793999515473842620849609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.033182604401771030599999079413464642129838466644287109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{91.4699509143829203594577847979962825775146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.682915289670432912316755391657352447509765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{13654}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.525080263614654541015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.3173239231109619140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.4290307863393036935661939423880539834499359130859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{5.38143634796142578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.62465720460904350375130889005959033966064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{23241}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.509857833385467529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{4.5042121410369873046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{27671}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0838797204610251256884367876409669406712055206298828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000312250225675825276994146406650543212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000028576984413856343341489327501425956055673845666864618664249064750038087368011474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000011759879384116084681148352151476625810555362015003932722734258931041040341369807720184326171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5785973}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5785973}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5785973}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{5785973}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000003133222701478914311511061339435390439149730075854040356464480510112480260431766510009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000002861098874597717785940125592838820276873548555953384597838606850928044877946376800537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13654}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.000000000000000001169184552510181958950408267230599793489497532919464857503744070754692074842751026153564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.143490314483642578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.75456530053094184040674008429050445556640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4430}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.124690115451812744140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.9650180339813232421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.321717540481376573779925820417702198028564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.71823024749755859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5765407827516266792144961073063313961029052734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4758546352386474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{27671}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4731509685516357421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{27714}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05707630397729886173596725029710796661674976348876953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000312250225675825276994146406650543212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000028576984413856343341489327501425956055673845666864618664249064750038087368011474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000011759879384116084681148352151476625810555362015003932722734258931041040341369807720184326171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.11057758331298828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.297075640286831088587859994731843471527099609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29110}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.480218231678009033203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{14929}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.448263645172119140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{19538}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.51224755971247670771617777063511312007904052734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7018294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7018294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7018294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{7018294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000003133222701478914311511061339435390439149730075854040356464480510112480260431766510009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000002861098874597717785940125592838820276873548555953384597838606850928044877946376800537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13654}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.000000000000000001169184552510181958950408267230599793489497532919464857503744070754692074842751026153564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.1036674976348734844577847979962825775146484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.7500222692426490311845554970204830169677734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{13036}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.11802875995635986328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.4960548877716064453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3116682338384386685703475450281985104084014892578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.748447895050048828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5810908387038882239039594423957169055938720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{15622}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4714076519012451171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.462373256683349609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0570557769930979119532565846384386532008647918701171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000312250225675825276994146406650543212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000028576984413856343341489327501425956055673845666864618664249064750038087368011474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000011759879384116084681148352151476625810555362015003932722734258931041040341369807720184326171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.95111083984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.271134603891940884068390005268156528472900390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{7310}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64434564113616943359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6082}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.634481906890869140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{8048}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.46292293381569304955291954684071242809295654296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6762262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6762262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6762262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{6762262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000003133222701478914311511061339435390439149730075854040356464480510112480260431766510009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000002861098874597717785940125592838820276873548555953384597838606850928044877946376800537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13654}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.000000000000000001169184552510181958950408267230599793489497532919464857503744070754692074842751026153564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{89.615163326263427734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.7881292065247862410615198314189910888671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4430}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.138509571552276611328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{24262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.0925252437591552734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3297527605230252678580882275127805769443511962890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7064568996429443359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.57848831675700029819608971592970192432403564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{15622}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.480757057666778564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{27671}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4805605411529541015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05445976927987121463115016695155645720660686492919921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000312250225675825276994146406650543212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000028576984413856343341489327501425956055673845666864618664249064750038087368011474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000011759879384116084681148352151476625810555362015003932722734258931041040341369807720184326171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.9180507659912109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.6426645604190444061032394529320299625396728515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{13716}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.75143182277679443359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27300}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.745930433273314985598290149937383830547332763671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{18289}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.44003606333357636604119988987804390490055084228515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6004052}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6004052}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6004052}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6004052}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000003133222701478914311511061339435390439149730075854040356464480510112480260431766510009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000002861098874597717785940125592838820276873548555953384597838606850928044877946376800537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13654}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.000000000000000001169184552510181958950408267230599793489497532919464857503744070754692074842751026153564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{89.17316150665283203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.8030188304698953061233623884618282318115234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{32103}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.349636971950531005859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.2958481311798095703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{24262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.269903062657281367364703328348696231842041015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.75932788848876953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{27714}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.585720651197117803121727774851024150848388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{4647}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4672372341156005859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4607684612274169921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.06017466980855019909046887960357707925140857696533203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000312250225675825276994146406650543212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000028576984413856343341489327501425956055673845666864618664249064750038087368011474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000011759879384116084681148352151476625810555362015003932722734258931041040341369807720184326171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{155.63616943359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.4297275164269507286007865332067012786865234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{4729}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.906459808349609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.7463226318359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59340187814654488107635188498534262180328369140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5473748}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5473748}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5473748}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5473748}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000003133222701478914311511061339435390439149730075854040356464480510112480260431766510009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000002861098874597717785940125592838820276873548555953384597838606850928044877946376800537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13654}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.000000000000000001169184552510181958950408267230599793489497532919464857503744070754692074842751026153564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{89.174670696258544921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.7718872518728829845713335089385509490966796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1412}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.179927647113800048828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.169048786163330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{24262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.2600167169181812898415273593855090439319610595703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7611739635467529296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{1185}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.583641792764726830000654445029795169830322265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{12141}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4689548015594482421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4611971378326416015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.059510789511747132218832945227404707111418247222900390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000312250225675825276994146406650543212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000028576984413856343341489327501425956055673845666864618664249064750038087368011474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000011759879384116084681148352151476625810555362015003932722734258931041040341369807720184326171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.51984310150146484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.3223633639859837529684227774851024150848388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64782559871673583984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8048}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.627370357513427734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6082}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.4404406740468065351024051778949797153472900390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6770581}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6770581}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6770581}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{6770581}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000003133222701478914311511061339435390439149730075854040356464480510112480260431766510009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000002861098874597717785940125592838820276873548555953384597838606850928044877946376800537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13654}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.000000000000000001169184552510181958950408267230599793489497532919464857503744070754692074842751026153564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{88.3962841033935546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.7838239448749533266891376115381717681884765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.258931934833526611328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.24252986907958984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.268500261773251480690305470488965511322021484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.720701694488525390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.582209612360063744063154445029795169830322265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{3175}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4771747589111328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{27671}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4747486114501953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{28778}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.055832873329136993578725167708398657850921154022216796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000312250225675825276994146406650543212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000028576984413856343341489327501425956055673845666864618664249064750038087368011474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000011759879384116084681148352151476625810555362015003932722734258931041040341369807720184326171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.87827014923095703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.65154951139791084102625973173417150974273681640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17080}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.79167711734771728515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18289}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.74662494659423828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27300}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.4412442825297662185590752415009774267673492431640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6029009}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6029009}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6029009}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6029009}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000003133222701478914311511061339435390439149730075854040356464480510112480260431766510009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000002861098874597717785940125592838820276873548555953384597838606850928044877946376800537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13654}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.000000000000000001169184552510181958950408267230599793489497532919464857503744070754692074842751026153564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.1595213413238383282077847979962825775146484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.7917885606652106389446998946368694305419921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{23633}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.258927881717681884765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.1810810565948486328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3104104837217398493720565966214053332805633544921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7140829563140869140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5822606465674393660947316675446927547454833984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{31308}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.468237817287445068359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4656162261962890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05694301569239872129468693628950859420001506805419921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000312250225675825276994146406650543212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000028576984413856343341489327501425956055673845666864618664249064750038087368011474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000011759879384116084681148352151476625810555362015003932722734258931041040341369807720184326171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.4159393310546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.266749906224134747390053234994411468505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{15622}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.3579044342041015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.61283111572265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59797218712847044486125014373101294040679931640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5486035}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5486035}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5486035}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5486035}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000003133222701478914311511061339435390439149730075854040356464480510112480260431766510009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000002861098874597717785940125592838820276873548555953384597838606850928044877946376800537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13654}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.000000000000000001169184552510181958950408267230599793489497532919464857503744070754692074842751026153564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.767185211181640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.7839098734571479099031421355903148651123046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{32103}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.4038383960723876953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27484}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.3206913471221923828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.349250020212923839579843843239359557628631591796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.722593784332275390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5801778218604081160947316675446927547454833984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.462818562984466552734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4619286060333251953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{27714}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05606581390181679391826463643155875615775585174560546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000312250225675825276994146406650543212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000028576984413856343341489327501425956055673845666864618664249064750038087368011474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000011759879384116084681148352151476625810555362015003932722734258931041040341369807720184326171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.3029937744140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{92.8864845124301581336112576536834239959716796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{81.2790679931640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{80.37683868408203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.6339667658878003209110829629935324192047119140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5500465}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5500465}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5500465}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5500465}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000003133222701478914311511061339435390439149730075854040356464480510112480260431766510009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000002861098874597717785940125592838820276873548555953384597838606850928044877946376800537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13654}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.000000000000000001169184552510181958950408267230599793489497532919464857503744070754692074842751026153564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{89.3889315128326416015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.7771862200553840693828533403575420379638671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1412}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.11452901363372802734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{80.95798778533935546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3062967057814962590356344662723131477832794189453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.726410388946533203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{18668}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.5800924206411597339183572330512106418609619140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{4729}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.476884543895721435546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.46184825897216796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.055575214388424776235098079268936999142169952392578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000312250225675825276994146406650543212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000028576984413856343341489327501425956055673845666864618664249064750038087368011474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000011759879384116084681148352151476625810555362015003932722734258931041040341369807720184326171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{33.5944671630859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{13.575011654405404470935536664910614490509033203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{8.01591932773590087890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{22545}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{7.73836469650268465869658029987476766109466552734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{15622}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.60855280594514926661986464750953018665313720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7968631}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7968631}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7968631}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{7968631}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000003133222701478914311511061339435390439149730075854040356464480510112480260431766510009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000002861098874597717785940125592838820276873548555953384597838606850928044877946376800537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13654}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.000000000000000001169184552510181958950408267230599793489497532919464857503744070754692074842751026153564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{89.3375174999237060546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{83.799466698374970974327879957854747772216796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27671}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.246200621128082275390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.169208526611328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.2838423222211172713969062897376716136932373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7354485988616943359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{7098}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.57892207752000413023552027880214154720306396484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{4800}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4697949886322021484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{23696}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{4.467715740203857421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{27671}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0577134686700177812479495287334430031478404998779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.000000001432319241510826568486436372040770947933197021484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{19451}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0000000000094855862667404788444832299904325837759666573134609279804863035678863525390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.000000000116173881473569517343137211796391845830545008766421233303844928741455078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5894837}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5894837}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5894837}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{5894837}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000014331657476996512631137739717814526263506280656656599603593349456787109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{19451}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000949119230187648768000631435951374294084093019563397319871000945568084716796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000011624254068360836964958947577328425559972657765683834441006183624267578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{89.0987355709075927734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.413675324016850254338351078331470489501953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22401}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.9044678211212158203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.8420352935791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{27300}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.2768727920573328393771816990920342504978179931640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.766941547393798828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.59848787610894049748821998946368694305419921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.485096514225006103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4823758602142333984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.06109950216990282789719657330351765267550945281982421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000000001595221697792137405258472426794469356536865234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{19451}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000000000010567219698613931766924710899332949510208423671286936951219104230403900146484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00000000000129386496331569837130586638953792037970251527223553011936019174754619598388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.11057758331298828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.297075640286831088587859994731843471527099609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29110}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.480218231678009033203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{14929}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.448263645172119140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{19538}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.51224755971247670771617777063511312007904052734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7127158}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{7127158}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{7127158}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{7127158}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.000000000015961644799601016394015902216563132336168973068879495258443057537078857421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{19451}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000105734666776816791854217364785661077738044937024408653769569355063140392303466796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000129462964109534467293504835551740743643071851476378242296050302684307098388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.0061495304107666015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.3998608368122091860641376115381717681884765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{11598}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.89240372180938720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.844693660736083984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{27300}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.2821779819039431647098581379395909607410430908203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7962067127227783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{20751}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.59982509802508854335201249341480433940887451171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{6204}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.485114634037017822265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{4.478858470916748046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.057484297943287417098634506373855401761829853057861328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000000000011335550553770448482789617230893191898830237029915934954260592348873615264892578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{19451}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000779074652472630477471410103164079498924289688029098943644612518255598843097686767578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00000000000000919182716516098583271618387482485010701893125839578857494416297413408756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.95111083984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.271134603891940884068390005268156528472900390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{7310}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64434564113616943359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6082}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.634481906890869140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{8048}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.46292293381569304955291954684071242809295654296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6871126}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6871126}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6871126}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{6871126}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000011342249907810669195371606231832325444746668863249539072057814337313175201416015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{19451}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000077955220381738530087653661111407443974724812245369331975552995572797954082489013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000919725817203474149105900978044382955328196228850234916762929060496389865875244140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{89.5918819904327392578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.4165718634396995412316755391657352447509765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.79967844486236572265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.697741985321044921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{27300}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.2419108328951000697060180755215696990489959716796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7738263607025146484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.59664326471998219147963027353398501873016357421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4880278110504150390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24202}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.48113918304443359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.057489037755205980861905601386752096004784107208251953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000000000011335550553770448482789617230893191898830237029915934954260592348873615264892578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{19451}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000779074652472630477471410103164079498924289688029098943644612518255598843097686767578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00000000000000919182716516098583271618387482485010701893125839578857494416297413408756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.9180507659912109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.6426645604190444061032394529320299625396728515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{13716}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.75143182277679443359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{27300}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.745930433273314985598290149937383830547332763671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{18289}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.44003606333357636604119988987804390490055084228515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6112916}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6112916}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6112916}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6112916}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000011342249907810669195371606231832325444746668863249539072057814337313175201416015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{19451}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000077955220381738530087653661111407443974724812245369331975552995572797954082489013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000919725817203474149105900978044382955328196228850234916762929060496389865875244140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{89.73089504241943359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.4327107170559685300759156234562397003173828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.8359901905059814453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.8091166019439697265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{27300}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.2645750454607924684324871122953481972217559814453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.793606281280517578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.60325048932966041093095554970204830169677734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.501492559909820556640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{14929}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.5008389949798583984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{28716}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05867930429701630201666517905323416925966739654541015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000312250225675825276994146406650543212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000028576984413856343341489327501425956055673845666864618664249064750038087368011474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000011759879384116084681148352151476625810555362015003932722734258931041040341369807720184326171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{155.63616943359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.4297275164269507286007865332067012786865234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{4729}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.906459808349609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.7463226318359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59340187814654488107635188498534262180328369140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5582612}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5582612}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5582612}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5582612}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000003133222701478914311511061339435390439149730075854040356464480510112480260431766510009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000002861098874597717785940125592838820276873548555953384597838606850928044877946376800537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13654}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.000000000000000001169184552510181958950408267230599793489497532919464857503744070754692074842751026153564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{88.9624779224395751953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.434038250651582302452879957854747772216796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{18668}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.951232373714447021484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.7778513431549072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.24200995776137990134202482295222580432891845703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7838866710662841796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.60309257886267619852560528670437633991241455078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{23633}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.486116826534271240234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.484857082366943359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24202}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05827737743684165139246289299990166909992694854736328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000000000011335550553770448482789617230893191898830237029915934954260592348873615264892578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{19451}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000779074652472630477471410103164079498924289688029098943644612518255598843097686767578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00000000000000919182716516098583271618387482485010701893125839578857494416297413408756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{15.51984310150146484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.3223633639859837529684227774851024150848388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.64782559871673583984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8048}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.627370357513427734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6082}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.4404406740468065351024051778949797153472900390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6879445}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6879445}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6879445}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{6879445}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000011342249907810669195371606231832325444746668863249539072057814337313175201416015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{19451}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000077955220381738530087653661111407443974724812245369331975552995572797954082489013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000919725817203474149105900978044382955328196228850234916762929060496389865875244140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{88.7277839183807373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.429046626122584484619437716901302337646484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{26829}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.861556947231292724609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.6156718730926513671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{27300}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.22890280717930266973780817352235317230224609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.774942874908447265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.59861918948344072788358971592970192432403564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{4729}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4813497066497802734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{4.480580806732177734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0584420419352937592361030283427680842578411102294921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000000000011335550553770448482789617230893191898830237029915934954260592348873615264892578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{19451}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000779074652472630477471410103164079498924289688029098943644612518255598843097686767578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00000000000000919182716516098583271618387482485010701893125839578857494416297413408756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.87827014923095703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24438}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.65154951139791084102625973173417150974273681640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17080}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.79167711734771728515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18289}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.74662494659423828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27300}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.4412442825297662185590752415009774267673492431640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6137873}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6137873}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6137873}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{6137873}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000011342249907810669195371606231832325444746668863249539072057814337313175201416015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{19451}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000077955220381738530087653661111407443974724812245369331975552995572797954082489013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000919725817203474149105900978044382955328196228850234916762929060496389865875244140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.051361560821533203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.4399360978840149982715956866741180419921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.73710191249847412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.06766510009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3014942494765067149131709811626933515071868896484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.790956020355224609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.6032063313667350712421466596424579620361328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{29726}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.50347244739532470703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{4.502208232879638671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05514601465846809269510941931002889759838581085205078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000312250225675825276994146406650543212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000028576984413856343341489327501425956055673845666864618664249064750038087368011474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000011759879384116084681148352151476625810555362015003932722734258931041040341369807720184326171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.4159393310546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{91.266749906224134747390053234994411468505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{15622}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.3579044342041015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.61283111572265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.59797218712847044486125014373101294040679931640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5594899}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5594899}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5594899}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5594899}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000003133222701478914311511061339435390439149730075854040356464480510112480260431766510009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000002861098874597717785940125592838820276873548555953384597838606850928044877946376800537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13654}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.000000000000000001169184552510181958950408267230599793489497532919464857503744070754692074842751026153564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.3823804855346821796047152020037174224853515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.4392254352569580078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7098}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.832821905612945556640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.7772274017333984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{27300}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.318863437754470790963523540995083749294281005859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7859237194061279296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.60171845890828290492891028407029807567596435546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{4800}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.490040957927703857421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4768579006195068359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.059729151155932934391667998852426535449922084808349609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000312250225675825276994146406650543212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000028576984413856343341489327501425956055673845666864618664249064750038087368011474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000000000000011759879384116084681148352151476625810555362015003932722734258931041040341369807720184326171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{156.3029937744140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4810}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{92.8864845124301581336112576536834239959716796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{81.2790679931640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{29022}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{80.37683868408203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{7238}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.6339667658878003209110829629935324192047119140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5609329}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5609329}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5609329}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{5609329}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000003133222701478914311511061339435390439149730075854040356464480510112480260431766510009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000002861098874597717785940125592838820276873548555953384597838606850928044877946376800537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13654}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.000000000000000001169184552510181958950408267230599793489497532919464857503744070754692074842751026153564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.3969378471374369610202847979962825775146484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.445646497587489420766360126435756683349609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15662}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.776119053363800048828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.4443643093109130859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3165543594149931028169930868898518383502960205078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.8339951038360595703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.60214192346231865116124026826582849025726318359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.488752424716949462890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{15622}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4687583446502685546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{15399}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.059016883278992036954146982452584779821336269378662109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000312250225675825276994146406650543212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{19451}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000000000000000028582728531326465056027755806618519196419693083506541331217931656283326447010040283203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000000000000002580401170515500552937737666070461273193359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.000000000000000001186740785990232810326814045997203286872469965614463986713911225479023414663970470428466796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{33.5944671630859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{13.575011654405404470935536664910614490509033203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{8.01591932773590087890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{22545}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{7.73836469650268465869658029987476766109466552734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{15622}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{3.60855280594514926661986464750953018665313720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{8077495}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{8077495}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{8077495}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{8077495}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00000000000000003133222701478914311511061339435390439149730075854040356464480510112480260431766510009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000000000000002861673625824285619278074494006762027769085450046131213763800360538880340754985809326171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13654}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000025841459233503520464618591873892085419911191952204408683879677255390561185777187347412109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{23447}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0000000000000000011799287600459837767291381339236708927457499600992101018714919291596743278205394744873046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{88.22135162353515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.4095947505622490325549733825027942657470703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.88648927211761474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.81387042999267578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.211051623711310032405208403361029922962188720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7576076984405517578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{19004}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.596820213936812393740183324553072452545166015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.4556481838226318359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{15399}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{4.4516727924346923828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{24202}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.060068092087843145965297964039564249105751514434814453125}
\def\SubcubicEffectiveDimensionalityEstimateLen{7852}
\def\SubcubicEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicEffectiveDimensionalityEstimateMeanFloat{5662.76923076923048938624560832977294921875}
\def\SubcubicEffectiveDimensionalityEstimateMedianFloat{4290}
\def\SubcubicEffectiveDimensionalityEstimateMinFloat{4290}
\def\SubcubicEffectiveDimensionalityEstimateStdDevFloat{2046.997581970168312182067893445491790771484375}
\def\SubcubicErrUpperBoundLen{7852}
\def\SubcubicErrUpperBoundMaxFloat{156.4159393310546875}
\def\SubcubicErrUpperBoundMeanFloat{24.676028825376814523906432441435754299163818359375}
\def\SubcubicErrUpperBoundMedianFloat{0}
\def\SubcubicErrUpperBoundMinFloat{0}
\def\SubcubicErrUpperBoundStdDevFloat{37.18086241115832990544731728732585906982421875}
\def\SubcubicGapMostBelowValueLen{7852}
\def\SubcubicGapMostBelowValueMaxFloat{22}
\def\SubcubicGapMostBelowValueMeanFloat{5.51273560876209867132047293125651776790618896484375}
\def\SubcubicGapMostBelowValueMedianFloat{1}
\def\SubcubicGapMostBelowValueMinFloat{1}
\def\SubcubicGapMostBelowValueNumStdLen{7852}
\def\SubcubicGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicGapMostBelowValueSequenceFracLen{7852}
\def\SubcubicGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicGapMostBelowValueSequenceFracMeanFloat{0.9884592850886615433836368538322858512401580810546875}
\def\SubcubicGapMostBelowValueSequenceFracMedianFloat{0.9518244817852974382077491100062616169452667236328125}
\def\SubcubicGapMostBelowValueSequenceFracMinFloat{0.92754381895065318719417746251565404236316680908203125}
\def\SubcubicGapMostBelowValueSequenceFracStdDevFloat{0.0114806026584997299122559155648559681139886379241943359375}
\def\SubcubicGapMostBelowValueStdDevFloat{4.181712583050693154973487253300845623016357421875}
\def\SubcubicGroupAccuracyLen{1208}
\def\SubcubicGroupAccuracyMaxFloat{0.73561759633376000433457875260501168668270111083984375}
\def\SubcubicGroupAccuracyMeanFloat{0.5794396178103244920976067078299820423126220703125}
\def\SubcubicGroupAccuracyMedianFloat{0.272868636165373157353997157770209014415740966796875}
\def\SubcubicGroupAccuracyMinFloat{0.08810089005800769701437502590124495327472686767578125}
\def\SubcubicGroupAccuracyStdDevFloat{0.09682728900976815544776599153919960372149944305419921875}
\def\SubcubicGroupDroppedSequencesFracLen{1208}
\def\SubcubicGroupDroppedSequencesFracMaxFloat{0.175609399482327510622070576573605649173259735107421875}
\def\SubcubicGroupDroppedSequencesFracMeanFloat{0.11243439997289865484031423648048075847327709197998046875}
\def\SubcubicGroupDroppedSequencesFracMedianFloat{0.0735562510601221186679055108470492996275424957275390625}
\def\SubcubicGroupDroppedSequencesFracMinFloat{0.0641773134406526946094118102337233722209930419921875}
\def\SubcubicGroupDroppedSequencesFracStdDevFloat{0.018891193026527371146006117896831710822880268096923828125}
\def\SubcubicGroupDroppedSequencesLen{1208}
\def\SubcubicGroupDroppedSequencesMaxFloat{202463853074269919}
\def\SubcubicGroupDroppedSequencesMeanFloat{129628037586322416}
\def\SubcubicGroupDroppedSequencesMedianFloat{84804583645474992}
\def\SubcubicGroupDroppedSequencesMinFloat{73991404773622603}
\def\SubcubicGroupDroppedSequencesStdDevFloat{21780062687962312}
\def\SubcubicGroupEffectiveDimensionalityEstimateLen{1208}
\def\SubcubicGroupEffectiveDimensionalityEstimateMaxFloat{8384}
\def\SubcubicGroupEffectiveDimensionalityEstimateMeanFloat{6401}
\def\SubcubicGroupEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicGroupEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicGroupEffectiveDimensionalityEstimateStdDevFloat{1921.033315692364567439653910696506500244140625}
\def\SubcubicGroupErrUpperBoundLen{1208}
\def\SubcubicGroupErrUpperBoundMaxFloat{5.11057758331298828125}
\def\SubcubicGroupErrUpperBoundMeanFloat{1.1485378201434155442939299973659217357635498046875}
\def\SubcubicGroupErrUpperBoundMedianFloat{0}
\def\SubcubicGroupErrUpperBoundMinFloat{0}
\def\SubcubicGroupErrUpperBoundStdDevFloat{1.204299757334311937739812492509372532367706298828125}
\def\SubcubicGroupGapMostBelowValueLen{1208}
\def\SubcubicGroupGapMostBelowValueMaxFloat{5}
\def\SubcubicGroupGapMostBelowValueMeanFloat{3.21357615894039749804278471856378018856048583984375}
\def\SubcubicGroupGapMostBelowValueMedianFloat{3}
\def\SubcubicGroupGapMostBelowValueMinFloat{3}
\def\SubcubicGroupGapMostBelowValueNumStdLen{1208}
\def\SubcubicGroupGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicGroupGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicGroupGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicGroupGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicGroupGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicGroupGapMostBelowValueSequenceFracLen{1208}
\def\SubcubicGroupGapMostBelowValueSequenceFracMaxFloat{0.999562203884124755859375}
\def\SubcubicGroupGapMostBelowValueSequenceFracMeanFloat{0.9857125891656275396002229172154329717159271240234375}
\def\SubcubicGroupGapMostBelowValueSequenceFracMedianFloat{0.9504227432608602921249030259787105023860931396484375}
\def\SubcubicGroupGapMostBelowValueSequenceFracMinFloat{0.94122815132141124383480246251565404236316680908203125}
\def\SubcubicGroupGapMostBelowValueSequenceFracStdDevFloat{0.009821451238689556106908895571905304677784442901611328125}
\def\SubcubicGroupGapMostBelowValueStdDevFloat{0.4333923545028657287048190482892096042633056640625}
\def\SubcubicGroupInstructionCountBranchLen{1208}
\def\SubcubicGroupInstructionCountBranchMaxFloat{0}
\def\SubcubicGroupInstructionCountBranchMeanFloat{0}
\def\SubcubicGroupInstructionCountBranchMedianFloat{0}
\def\SubcubicGroupInstructionCountBranchMinFloat{0}
\def\SubcubicGroupInstructionCountBranchStdDevFloat{0}
\def\SubcubicGroupInstructionCountIntLen{1208}
\def\SubcubicGroupInstructionCountIntMaxFloat{0}
\def\SubcubicGroupInstructionCountIntMeanFloat{0}
\def\SubcubicGroupInstructionCountIntMedianFloat{0}
\def\SubcubicGroupInstructionCountIntMinFloat{0}
\def\SubcubicGroupInstructionCountIntStdDevFloat{0}
\def\SubcubicGroupInstructionCountLen{1208}
\def\SubcubicGroupInstructionCountMaxFloat{7393557}
\def\SubcubicGroupInstructionCountMeanFloat{6718837}
\def\SubcubicGroupInstructionCountMedianFloat{6044117}
\def\SubcubicGroupInstructionCountMinFloat{6044117}
\def\SubcubicGroupInstructionCountStdDevFloat{618573.87646141345612704753875732421875}
\def\SubcubicGroupMaxGapLen{1208}
\def\SubcubicGroupMaxGapMaxFloat{37}
\def\SubcubicGroupMaxGapMeanFloat{28.421357615894038417536648921668529510498046875}
\def\SubcubicGroupMaxGapMedianFloat{5}
\def\SubcubicGroupMaxGapMinFloat{5}
\def\SubcubicGroupMaxGapStdDevFloat{8.3016658831239880100838490761816501617431640625}
\def\SubcubicGroupNormalizedAccuracyLen{1208}
\def\SubcubicGroupNormalizedAccuracyMaxFloat{0.7362903356393937226442858445807360112667083740234375}
\def\SubcubicGroupNormalizedAccuracyMeanFloat{0.5801163207065147542351724041509442031383514404296875}
\def\SubcubicGroupNormalizedAccuracyMedianFloat{0.2732675793246059914309853411396034061908721923828125}
\def\SubcubicGroupNormalizedAccuracyMinFloat{0.089341728089431582393586950274766422808170318603515625}
\def\SubcubicGroupNormalizedAccuracyStdDevFloat{0.0968864788624545780759689250771771185100078582763671875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.73561759633376000433457875260501168668270111083984375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMaxKey{13293}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.6719485003074250339949458066257648169994354248046875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMeanKey{20754}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.59654351894768631314747153737698681652545928955078125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMinFloat{0.57546861148124861529140616767108440399169921875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMinKey{11498}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.02986885106555713098597237831199890933930873870849609375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.16493197282667348968487885940703563392162322998046875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10427451405117170446512631087898625992238521575927734375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29022}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.069256780745197199511409280603402294218540191650390625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{14095}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0641773134406526946094118102337233722209930419921875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0176540967684821990812960024186395457945764064788818359375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{190153618269104040}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{120220329632024752}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29022}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{79847631860979296}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{14095}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{73991404773622603}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20353787808793372}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{8384}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{7226.2781456953644010354764759540557861328125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{4729}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{1895}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{1895}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{1760.8537068534706122591160237789154052734375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{3.352389812469482421875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{23633}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0.67823263904116803946209302011993713676929473876953125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.069749581839877894395840485231019556522369384765625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{4}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{519}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.132450331125827602818390005268156528472900390625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9993798732757568359375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{913}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98965070184492909266538163137738592922687530517578125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{5781}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95811855792999267578125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11124}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94793224334716796875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{19093}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.008059231314733648898762652379446080885827541351318359375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.33897970575019142902561952723772265017032623291015625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7393557}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMaxKey{1895}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6521103.68211920559406280517578125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMeanKey{4729}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6152981}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMinFloat{6152981}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{563917.976413863711059093475341796875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMaxFloat{36}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMeanFloat{30.68874172185430637682657106779515743255615234375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMedianFloat{7.75}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMedianKey{26829}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMinKey{4729}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.48866922337440232837479925365187227725982666015625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7362903356393937226442858445807360112667083740234375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{13293}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.672749991036507566377622424624860286712646484375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20754}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.59746205614512570836183158462517894804477691650390625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.577686766942659080115163305890746414661407470703125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11498}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.029774664870804400107484610771280131302773952484130859375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{92.9854123592376851092922152020037174224853515625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.5942312913225151760343578644096851348876953125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5358}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.857090175151824951171875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3254}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.848140716552734375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMinKey{3284}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5729946795281559701606965973041951656341552734375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7482655048370361328125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61091648032333711881847193581052124500274658203125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMeanKey{20415}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.49016630649566650390625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMedianKey{15043}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMinFloat{4.486188411712646484375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMinKey{27584}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0568896977651920099372517825031536631286144256591796875}
\def\SubcubicGroupProofSearchTimeLen{1208}
\def\SubcubicGroupProofSearchTimeMaxFloat{92.9854123592376851092922152020037174224853515625}
\def\SubcubicGroupProofSearchTimeMeanFloat{84.243449351842826899883220903575420379638671875}
\def\SubcubicGroupProofSearchTimeMedianFloat{81.092922512292858527871430851519107818603515625}
\def\SubcubicGroupProofSearchTimeMinFloat{80.2805917263031005859375}
\def\SubcubicGroupProofSearchTimeStdDevFloat{1.518243705312535052343037023092620074748992919921875}
\def\SubcubicGroupProofTimeLen{1208}
\def\SubcubicGroupProofTimeMaxFloat{4.813351154327392578125}
\def\SubcubicGroupProofTimeMeanFloat{4.59841951254187808473261611652560532093048095703125}
\def\SubcubicGroupProofTimeMedianFloat{4.47218479514121991513775355997495353221893310546875}
\def\SubcubicGroupProofTimeMinFloat{4.446563243865966796875}
\def\SubcubicGroupProofTimeStdDevFloat{0.059194223155749382814239112349241622723639011383056640625}
\def\SubcubicInstructionCountBranchLen{7852}
\def\SubcubicInstructionCountBranchMaxFloat{0}
\def\SubcubicInstructionCountBranchMeanFloat{0}
\def\SubcubicInstructionCountBranchMedianFloat{0}
\def\SubcubicInstructionCountBranchMinFloat{0}
\def\SubcubicInstructionCountBranchStdDevFloat{0}
\def\SubcubicInstructionCountIntLen{7852}
\def\SubcubicInstructionCountIntMaxFloat{0}
\def\SubcubicInstructionCountIntMeanFloat{0}
\def\SubcubicInstructionCountIntMedianFloat{0}
\def\SubcubicInstructionCountIntMinFloat{0}
\def\SubcubicInstructionCountIntStdDevFloat{0}
\def\SubcubicInstructionCountLen{7852}
\def\SubcubicInstructionCountMaxFloat{8343894}
\def\SubcubicInstructionCountMeanFloat{6564605.96153846196830272674560546875}
\def\SubcubicInstructionCountMedianFloat{5731892}
\def\SubcubicInstructionCountMinFloat{5731892}
\def\SubcubicInstructionCountStdDevFloat{752592.171855201595462858676910400390625}
\def\SubcubicMaxGapLen{7852}
\def\SubcubicMaxGapMaxFloat{45}
\def\SubcubicMaxGapMeanFloat{28.049796230259804730167161324061453342437744140625}
\def\SubcubicMaxGapMedianFloat{1}
\def\SubcubicMaxGapMinFloat{1}
\def\SubcubicMaxGapStdDevFloat{11.89514990008266437371275969780981540679931640625}
\def\SubcubicNormalizedAccuracyLen{7852}
\def\SubcubicNormalizedAccuracyMaxFloat{0.7362903356393937226442858445807360112667083740234375}
\def\SubcubicNormalizedAccuracyMeanFloat{0.427076877145253608336616935048368759453296661376953125}
\def\SubcubicNormalizedAccuracyMedianFloat{0.000000000000000026916962613914833433808244709598778917961435006955643600701222339921514503657817840576171875}
\def\SubcubicNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicNormalizedAccuracyStdDevFloat{0.205951005673867815204403086681850254535675048828125}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.73561759633376000433457875260501168668270111083984375}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMaxKey{13293}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.6744402969050644625070844995207153260707855224609375}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMeanKey{2773}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.59984506874493315198293430512421764433383941650390625}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMedianKey{2549}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMinFloat{0.5886748106702359706332572386600077152252197265625}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMinKey{11498}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0277599487009831287498418106451936182565987110137939453125}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.166309213880606099333903102888143621385097503662109375}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{1895}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10834467436685824015540902109933085739612579345703125}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{23367}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.069256780745197199511409280603402294218540191650390625}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{14095}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0641773134406526946094118102337233722209930419921875}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0192612986811899582206830672248543123714625835418701171875}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{191741469097210324}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{1895}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{124912904987177120}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{23367}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{79847631860979296}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{14095}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{73991404773622603}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{22206765456199400}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{3284}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{7230.609271523178904317319393157958984375}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{7238}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{10248}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{10248}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{2008.985681842410258468589745461940765380859375}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.4831371307373046875}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{30371}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{1.36984169483184814453125}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{21317}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.4478428364381130677429609932005405426025390625}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{11498}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.172185430463576150117432916886173188686370849609375}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99907410144805919305355246251565404236316680908203125}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{18146}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.988061948722561478319903471856378018856048583984375}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29110}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95318606495857227667301003748434595763683319091796875}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{3284}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94793224334716796875}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{19093}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.009528229840375206094460480699126492254436016082763671875}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.39469309737089641743068568757735192775726318359375}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMaxFloat{7393557}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMaxKey{10248}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6458010.072847682051360607147216796875}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMeanKey{24202}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5896885}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMedianKey{3284}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMinFloat{5896885}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMinKey{3284}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{527408.75618842965923249721527099609375}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMaxFloat{36}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMeanFloat{30.576158940397352381523887743242084980010986328125}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMedianKey{8048}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMinKey{8048}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.8219106516352869817865212098695337772369384765625}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7362903356393937226442858445807360112667083740234375}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{13293}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6752443192679418171309180252137593924999237060546875}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{19093}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.6007763318331817981032827447052113711833953857421875}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2549}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.5909438696948836611255728712421841919422149658203125}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{11498}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0276422937253531335322076500915500218980014324188232421875}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{92.9854123592376851092922152020037174224853515625}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29565}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.6036648987144843658825266174972057342529296875}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{19451}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.923117816448211669921875}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{27300}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{81.9165172576904296875}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinKey{19004}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.5493088914244939058306727019953541457653045654296875}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.7482655048370361328125}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.61012741745702481210855694371275603771209716796875}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMeanKey{8721}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.49540579319000244140625}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMedianKey{28778}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMinFloat{4.49149227142333984375}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMinKey{15043}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0570625438540881269045001999984378926455974578857421875}
\def\SubcubicProofSearchTimeLen{7852}
\def\SubcubicProofSearchTimeMaxFloat{92.9854123592376851092922152020037174224853515625}
\def\SubcubicProofSearchTimeMeanFloat{84.2196891503678983781355782411992549896240234375}
\def\SubcubicProofSearchTimeMedianFloat{81.0932547795772507015499286353588104248046875}
\def\SubcubicProofSearchTimeMinFloat{79.22819805145263671875}
\def\SubcubicProofSearchTimeStdDevFloat{1.497413289789122803341570033808238804340362548828125}
\def\SubcubicProofTimeLen{7852}
\def\SubcubicProofTimeMaxFloat{4.92527079582214444286591970012523233890533447265625}
\def\SubcubicProofTimeMeanFloat{4.59842018712496081178642270970158278942108154296875}
\def\SubcubicProofTimeMedianFloat{4.47186663985252419450944216805510222911834716796875}
\def\SubcubicProofTimeMinFloat{4.446563243865966796875}
\def\SubcubicProofTimeStdDevFloat{0.059249133235251959239686669889124459587037563323974609375}
\def\SubcubicVocabModelSquaredAccuracyLen{7248}
\def\SubcubicVocabModelSquaredAccuracyMaxFloat{0.70495421337041774823006790029467083513736724853515625}
\def\SubcubicVocabModelSquaredAccuracyMeanFloat{0.169780308345267971770198300873744301497936248779296875}
\def\SubcubicVocabModelSquaredAccuracyMedianFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\SubcubicVocabModelSquaredAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicVocabModelSquaredAccuracyStdDevFloat{0.207709389825697865461506808060221374034881591796875}
\def\SubcubicVocabModelSquaredDroppedSequencesFracLen{7248}
\def\SubcubicVocabModelSquaredDroppedSequencesFracMaxFloat{0.46377977035578010767125078928074799478054046630859375}
\def\SubcubicVocabModelSquaredDroppedSequencesFracMeanFloat{0.1463263359118814610493330974350101314485073089599609375}
\def\SubcubicVocabModelSquaredDroppedSequencesFracMedianFloat{0}
\def\SubcubicVocabModelSquaredDroppedSequencesFracMinFloat{0}
\def\SubcubicVocabModelSquaredDroppedSequencesFracStdDevFloat{0.1306021353563418252452521528539364226162433624267578125}
\def\SubcubicVocabModelSquaredDroppedSequencesLen{7248}
\def\SubcubicVocabModelSquaredDroppedSequencesMaxFloat{534701670644804012}
\def\SubcubicVocabModelSquaredDroppedSequencesMeanFloat{168702779363133312}
\def\SubcubicVocabModelSquaredDroppedSequencesMedianFloat{0}
\def\SubcubicVocabModelSquaredDroppedSequencesMinFloat{0}
\def\SubcubicVocabModelSquaredDroppedSequencesStdDevFloat{150574010399900736}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateLen{7248}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateMeanFloat{6468.6666666666669698315672576427459716796875}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateMedianFloat{6338}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateMinFloat{6338}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateStdDevFloat{53.7979760048853705711735528893768787384033203125}
\def\SubcubicVocabModelSquaredErrUpperBoundLen{7248}
\def\SubcubicVocabModelSquaredErrUpperBoundMaxFloat{156.4159393310546875}
\def\SubcubicVocabModelSquaredErrUpperBoundMeanFloat{39.38071070364768644367359229363501071929931640625}
\def\SubcubicVocabModelSquaredErrUpperBoundMedianFloat{3.864933013916016069089209850062616169452667236328125}
\def\SubcubicVocabModelSquaredErrUpperBoundMinFloat{3.745930433273314985598290149937383830547332763671875}
\def\SubcubicVocabModelSquaredErrUpperBoundStdDevFloat{41.02838602361764941406363504938781261444091796875}
\def\SubcubicVocabModelSquaredGapMostBelowValueLen{7248}
\def\SubcubicVocabModelSquaredGapMostBelowValueMaxFloat{23}
\def\SubcubicVocabModelSquaredGapMostBelowValueMeanFloat{5.42411699779249456554452990530990064144134521484375}
\def\SubcubicVocabModelSquaredGapMostBelowValueMedianFloat{1}
\def\SubcubicVocabModelSquaredGapMostBelowValueMinFloat{1}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdLen{7248}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracLen{7248}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracMeanFloat{0.9927807545523770205164737490122206509113311767578125}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracMedianFloat{0.9529183745384217640861379550187848508358001708984375}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracMinFloat{0.941314160823822021484375}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracStdDevFloat{0.010019705689404738435666075702101807110011577606201171875}
\def\SubcubicVocabModelSquaredGapMostBelowValueStdDevFloat{4.87342922490442820304679116816259920597076416015625}
\def\SubcubicVocabModelSquaredInstructionCountBranchLen{7248}
\def\SubcubicVocabModelSquaredInstructionCountBranchMaxFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountBranchMeanFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountBranchMedianFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountBranchMinFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountBranchStdDevFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntLen{7248}
\def\SubcubicVocabModelSquaredInstructionCountIntMaxFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntMeanFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntMedianFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntMinFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntStdDevFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountLen{7248}
\def\SubcubicVocabModelSquaredInstructionCountMaxFloat{8079543}
\def\SubcubicVocabModelSquaredInstructionCountMeanFloat{6305145.208333333022892475128173828125}
\def\SubcubicVocabModelSquaredInstructionCountMedianFloat{5473748}
\def\SubcubicVocabModelSquaredInstructionCountMinFloat{5473748}
\def\SubcubicVocabModelSquaredInstructionCountStdDevFloat{819157.806034749955870211124420166015625}
\def\SubcubicVocabModelSquaredMaxGapLen{7248}
\def\SubcubicVocabModelSquaredMaxGapMaxFloat{47}
\def\SubcubicVocabModelSquaredMaxGapMeanFloat{18.84726821192052881315248669125139713287353515625}
\def\SubcubicVocabModelSquaredMaxGapMedianFloat{1}
\def\SubcubicVocabModelSquaredMaxGapMinFloat{1}
\def\SubcubicVocabModelSquaredMaxGapStdDevFloat{15.8480728676710587166098775924183428287506103515625}
\def\SubcubicVocabModelSquaredNormalizedAccuracyLen{7248}
\def\SubcubicVocabModelSquaredNormalizedAccuracyMaxFloat{0.70586535370262193378465553905698470771312713623046875}
\def\SubcubicVocabModelSquaredNormalizedAccuracyMeanFloat{0.1699799465485488381144563163616112433373928070068359375}
\def\SubcubicVocabModelSquaredNormalizedAccuracyMedianFloat{0.000000000000000026054821497037114438219634609030939328582006345885226095138165192111046053469181060791015625}
\def\SubcubicVocabModelSquaredNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicVocabModelSquaredNormalizedAccuracyStdDevFloat{0.207952184485298230409711095489910803735256195068359375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.70495421337041774823006790029467083513736724853515625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMaxKey{18289}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.62487745964228846862198452072334475815296173095703125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMeanKey{24202}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.5237321854485148531210825240123085677623748779296875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMinFloat{0.521449397118541657647483589244075119495391845703125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMinKey{2306}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0309035344591167028538425398664912790991365909576416015625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.198309672249317003878132936733891256153583526611328125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1355118421907518799773839646150008775293827056884765625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{23633}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08819241261316472513254183240860584191977977752685546875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07640795145471369897993696440607891418039798736572265625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0167626782758810120854686687152934609912335872650146484375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{228635485707773261}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{156234516990607328}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{23633}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{101678929044877776}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{88092370355095476}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19326052259069240}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{742}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6492.2781456953644010354764759540557861328125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{31.4842878800922107984661124646663665771484375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{11.43377780914306640625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{23633}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.044434572687212181563154445029795169830322265625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{6155}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.817322850227355512942040149937383830547332763671875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{15662}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.806694507598876953125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinKey{18289}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.2242014892683481530610833942773751914501190185546875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.887417218543046448786526525509543716907501220703125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1185}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1185}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99766051769256602899105246251565404236316680908203125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{24144}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98323778956141694163051170107792131602764129638671875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{17194}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95128062367439281121761496251565404236316680908203125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{10248}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.941314160823822021484375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{19004}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01126216006376259438914733124192935065366327762603759765625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.50877135938195550135532130298088304698467254638671875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6881493}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMaxKey{9134}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6209911.523178808391094207763671875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMeanKey{742}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6114964}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMinFloat{6114964}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{237574.8963797009200789034366607666015625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMaxFloat{41}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMeanFloat{29.642384105960264406576243345625698566436767578125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMeanKey{1951}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMedianKey{742}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.6982361193426225298708232003264129161834716796875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.70586535370262193378465553905698470771312713623046875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18289}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.62562329264245575277669786373735405504703521728515625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{2773}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.525400740304266644642439132439903914928436279296875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.522058608420906011815532110631465911865234375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2306}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0308397769129801595233697497633329476229846477508544921875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.3213505744933939922702847979962825775146484375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.6141748775709601204653154127299785614013671875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27671}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.276223599910736083984375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{79.694097042083740234375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3390074957860347293348013408831320703029632568359375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.74157428741455078125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.620685501603890799060536664910614490509033203125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMeanKey{19538}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.507993161678314208984375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMinFloat{4.5032379627227783203125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05704269111738767550345841073067276738584041595458984375}
\def\SubcubicVocabModelSquaredProofSearchTimeLen{7248}
\def\SubcubicVocabModelSquaredProofSearchTimeMaxFloat{101.354745388031005859375}
\def\SubcubicVocabModelSquaredProofSearchTimeMeanFloat{84.20196536735983272592420689761638641357421875}
\def\SubcubicVocabModelSquaredProofSearchTimeMedianFloat{81.1719985711574594233752577565610408782958984375}
\def\SubcubicVocabModelSquaredProofSearchTimeMinFloat{78.8330733776092529296875}
\def\SubcubicVocabModelSquaredProofSearchTimeStdDevFloat{1.426264697561210770260231583961285650730133056640625}
\def\SubcubicVocabModelSquaredProofTimeLen{7248}
\def\SubcubicVocabModelSquaredProofTimeMaxFloat{5.38143634796142578125}
\def\SubcubicVocabModelSquaredProofTimeMeanFloat{4.59527143191291287394051323644816875457763671875}
\def\SubcubicVocabModelSquaredProofTimeMedianFloat{4.46693785429000822517764390795491635799407958984375}
\def\SubcubicVocabModelSquaredProofTimeMinFloat{4.4427516460418701171875}
\def\SubcubicVocabModelSquaredProofTimeStdDevFloat{0.05998114231751998370878453670229646377265453338623046875}
\def\SubcubicWithoutVocabSquaredAccuracyLen{4530}
\def\SubcubicWithoutVocabSquaredAccuracyMaxFloat{0.70495421337041774823006790029467083513736724853515625}
\def\SubcubicWithoutVocabSquaredAccuracyMeanFloat{0.195614448055888623390075053976033814251422882080078125}
\def\SubcubicWithoutVocabSquaredAccuracyMedianFloat{0.00000000000000002602085213965210641617886722087860107421875}
\def\SubcubicWithoutVocabSquaredAccuracyMinFloat{0.000000000000000025153490401663705950460815999760012594642833135883709660962637144621112383902072906494140625}
\def\SubcubicWithoutVocabSquaredAccuracyStdDevFloat{0.2317268382155659722787532928123255260288715362548828125}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracLen{4530}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracMaxFloat{0.302663733530732004251007083439617417752742767333984375}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracMeanFloat{0.09874242723707594981963353575338260270655155181884765625}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracMedianFloat{0}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracMinFloat{0}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracStdDevFloat{0.07403403175116836376634665839446824975311756134033203125}
\def\SubcubicWithoutVocabSquaredDroppedSequencesLen{4530}
\def\SubcubicWithoutVocabSquaredDroppedSequencesMaxFloat{348947527052177429}
\def\SubcubicWithoutVocabSquaredDroppedSequencesMeanFloat{113842267778701744}
\def\SubcubicWithoutVocabSquaredDroppedSequencesMedianFloat{0}
\def\SubcubicWithoutVocabSquaredDroppedSequencesMinFloat{0}
\def\SubcubicWithoutVocabSquaredDroppedSequencesStdDevFloat{85355427278668128}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateLen{4530}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateMeanFloat{6457.4666666666662422358058393001556396484375}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateMedianFloat{6338}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateMinFloat{6338}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateStdDevFloat{56.60372975539882389739432255737483501434326171875}
\def\SubcubicWithoutVocabSquaredErrUpperBoundLen{4530}
\def\SubcubicWithoutVocabSquaredErrUpperBoundMaxFloat{33.5944671630859375}
\def\SubcubicWithoutVocabSquaredErrUpperBoundMeanFloat{7.89254473882005669338468578644096851348876953125}
\def\SubcubicWithoutVocabSquaredErrUpperBoundMedianFloat{3.806694507598876953125}
\def\SubcubicWithoutVocabSquaredErrUpperBoundMinFloat{3.745930433273314985598290149937383830547332763671875}
\def\SubcubicWithoutVocabSquaredErrUpperBoundStdDevFloat{3.77648699916363828066323549137450754642486572265625}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueLen{4530}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueMaxFloat{9}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueMeanFloat{3.17086092715231782079854383482597768306732177734375}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueMedianFloat{1}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueMinFloat{1}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdLen{4530}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracLen{4530}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracMeanFloat{0.98907907038071829486369779260712675750255584716796875}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracMedianFloat{0.9518301597237586175737078519887290894985198974609375}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracMinFloat{0.941314160823822021484375}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracStdDevFloat{0.01106941254663927100276854531557546579279005527496337890625}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueStdDevFloat{1.6520609673434847319839491319726221263408660888671875}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchLen{4530}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchMaxFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchMeanFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchMedianFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchMinFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntLen{4530}
\def\SubcubicWithoutVocabSquaredInstructionCountIntMaxFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntMeanFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntMedianFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntMinFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountLen{4530}
\def\SubcubicWithoutVocabSquaredInstructionCountMaxFloat{8079543}
\def\SubcubicWithoutVocabSquaredInstructionCountMeanFloat{6762704.333333333022892475128173828125}
\def\SubcubicWithoutVocabSquaredInstructionCountMedianFloat{6004052}
\def\SubcubicWithoutVocabSquaredInstructionCountMinFloat{6004052}
\def\SubcubicWithoutVocabSquaredInstructionCountStdDevFloat{716580.174071789137087762355804443359375}
\def\SubcubicWithoutVocabSquaredMaxGapLen{4530}
\def\SubcubicWithoutVocabSquaredMaxGapMaxFloat{41}
\def\SubcubicWithoutVocabSquaredMaxGapMeanFloat{15.7333333333333325043668082798831164836883544921875}
\def\SubcubicWithoutVocabSquaredMaxGapMedianFloat{1}
\def\SubcubicWithoutVocabSquaredMaxGapMinFloat{1}
\def\SubcubicWithoutVocabSquaredMaxGapStdDevFloat{13.8512426954759977348885513492859899997711181640625}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyLen{4530}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyMaxFloat{0.70586535370262193378465553905698470771312713623046875}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyMeanFloat{0.195844039139030756668802268904983066022396087646484375}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyMedianFloat{0.000000000000000026054821497037114438219634609030939328582006345885226095138165192111046053469181060791015625}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyMinFloat{0.00000000000000002520137244290273546232755264889815880433404063527824678914157630060799419879913330078125}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyStdDevFloat{0.231996551928451755220095265030977316200733184814453125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.70495421337041774823006790029467083513736724853515625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMaxKey{18289}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.62487745964228846862198452072334475815296173095703125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMeanKey{24202}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.5237321854485148531210825240123085677623748779296875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMinFloat{0.521449397118541657647483589244075119495391845703125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMinKey{2306}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0309035344591167028538425398664912790991365909576416015625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.198309672249317003878132936733891256153583526611328125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12287}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1355118421907518799773839646150008775293827056884765625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{23633}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08819241261316472513254183240860584191977977752685546875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{7238}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07640795145471369897993696440607891418039798736572265625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{4810}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0167626782758810120854686687152934609912335872650146484375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{228635485707773261}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12287}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{156234516990607328}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{23633}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{101678929044877776}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{7238}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{88092370355095476}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinKey{4810}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{19326052259069240}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{742}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6492.2781456953644010354764759540557861328125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{31.4842878800922107984661124646663665771484375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{11.43377780914306640625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{23633}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.044434572687212181563154445029795169830322265625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{6155}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.817322850227355512942040149937383830547332763671875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{15662}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.806694507598876953125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinKey{18289}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.2242014892683481530610833942773751914501190185546875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2549}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.887417218543046448786526525509543716907501220703125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1185}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1185}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99766051769256602899105246251565404236316680908203125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{24144}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98323778956141694163051170107792131602764129638671875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{17194}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95128062367439281121761496251565404236316680908203125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{10248}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.941314160823822021484375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{19004}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01126216006376259438914733124192935065366327762603759765625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.50877135938195550135532130298088304698467254638671875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMaxFloat{6881493}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMaxKey{9134}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMeanFloat{6209911.523178808391094207763671875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMeanKey{742}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMedianFloat{6114964}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMinFloat{6114964}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{237574.8963797009200789034366607666015625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMaxFloat{41}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMeanFloat{29.642384105960264406576243345625698566436767578125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMeanKey{1951}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMedianKey{742}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMinKey{5781}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.6982361193426225298708232003264129161834716796875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.70586535370262193378465553905698470771312713623046875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18289}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.62562329264245575277669786373735405504703521728515625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{2773}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.525400740304266644642439132439903914928436279296875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.522058608420906011815532110631465911865234375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2306}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0308397769129801595233697497633329476229846477508544921875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{90.3213505744933939922702847979962825775146484375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29725}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{84.6141748775709601204653154127299785614013671875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27671}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{81.276223599910736083984375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{3284}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{79.694097042083740234375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinKey{21598}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{1.3390074957860347293348013408831320703029632568359375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMaxFloat{4.74157428741455078125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMaxKey{17197}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMeanFloat{4.620685501603890799060536664910614490509033203125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMeanKey{19538}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMedianFloat{4.507993161678314208984375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMinFloat{4.5032379627227783203125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.05704269111738767550345841073067276738584041595458984375}
\def\SubcubicWithoutVocabSquaredProofSearchTimeLen{4530}
\def\SubcubicWithoutVocabSquaredProofSearchTimeMaxFloat{100.6354253292083598125827847979962825775146484375}
\def\SubcubicWithoutVocabSquaredProofSearchTimeMeanFloat{84.2033788139456902399615501053631305694580078125}
\def\SubcubicWithoutVocabSquaredProofSearchTimeMedianFloat{81.1768663084506982841048738919198513031005859375}
\def\SubcubicWithoutVocabSquaredProofSearchTimeMinFloat{78.8330733776092529296875}
\def\SubcubicWithoutVocabSquaredProofSearchTimeStdDevFloat{1.421929963451891154591066879220306873321533203125}
\def\SubcubicWithoutVocabSquaredProofTimeLen{4530}
\def\SubcubicWithoutVocabSquaredProofTimeMaxFloat{5.38143634796142578125}
\def\SubcubicWithoutVocabSquaredProofTimeMeanFloat{4.59503990945963369796345432405360043048858642578125}
\def\SubcubicWithoutVocabSquaredProofTimeMedianFloat{4.4664830994606017355863514239899814128875732421875}
\def\SubcubicWithoutVocabSquaredProofTimeMinFloat{4.447611331939697265625}
\def\SubcubicWithoutVocabSquaredProofTimeStdDevFloat{0.060364283353939028609058681240639998577535152435302734375}
\def\TrainAccuracyLen{151}
\def\TrainAccuracyMaxFloat{0.9996041666666666269946972533944062888622283935546875}
\def\TrainAccuracyMaxKey{2773}
\def\TrainAccuracyMeanFloat{0.99864064224613680043063368430011905729770660400390625}
\def\TrainAccuracyMeanKey{13468}
\def\TrainAccuracyMedianFloat{0.9909394531249999804600747665972448885440826416015625}
\def\TrainAccuracyMedianKey{5781}
\def\TrainAccuracyMinFloat{0.9861328124999999555910790149937383830547332763671875}
\def\TrainAccuracyMinKey{4810}
\def\TrainAccuracyStdDevFloat{0.001531522878106406602982669795665060519240796566009521484375}
\def\TrainLossLen{151}
\def\TrainLossMaxFloat{0.040539778129440186271725821143263601697981357574462890625}
\def\TrainLossMaxKey{4810}
\def\TrainLossMeanFloat{0.005156686458680955799371847803058699355460703372955322265625}
\def\TrainLossMeanKey{1696}
\def\TrainLossMedianFloat{0.0020721208082201581120174171957160069723613560199737548828125}
\def\TrainLossMedianKey{8048}
\def\TrainLossMinFloat{0.0019288341482921775131564867677980146254412829875946044921875}
\def\TrainLossMinKey{7310}
\def\TrainLossStdDevFloat{0.004980988566630240553523290003568035899661481380462646484375}
\def\UpperWhiskerCrosshatchPercentileFloat{0.91132822467382401665503266485757194459438323974609375}
\def\UpperWhiskerTopEndPercentileFloat{0.97848760463080519667045109599712304770946502685546875}
\def\WEkkPerpFirstSingularLen{151}
\def\WEkkPerpFirstSingularMaxFloat{3.8083894252777099609375}
\def\WEkkPerpFirstSingularMaxKey{742}
\def\WEkkPerpFirstSingularMeanFloat{3.39167200334814200601840639137662947177886962890625}
\def\WEkkPerpFirstSingularMeanKey{1895}
\def\WEkkPerpFirstSingularMedianFloat{3.12218677997589111328125}
\def\WEkkPerpFirstSingularMedianKey{7238}
\def\WEkkPerpFirstSingularMinFloat{3.0717315673828125}
\def\WEkkPerpFirstSingularMinKey{4800}
\def\WEkkPerpFirstSingularStdDevFloat{0.13259159252576735443795996616245247423648834228515625}
\def\WEkkPerpFroNormLen{151}
\def\WEkkPerpFroNormMaxFloat{8.93716144561767578125}
\def\WEkkPerpFroNormMaxKey{26829}
\def\WEkkPerpFroNormMeanFloat{8.5152026549080357398224805365316569805145263671875}
\def\WEkkPerpFroNormMeanKey{18289}
\def\WEkkPerpFroNormMedianFloat{8.1487476825714111328125}
\def\WEkkPerpFroNormMedianKey{16069}
\def\WEkkPerpFroNormMinFloat{8.11903095245361328125}
\def\WEkkPerpFroNormMinKey{7238}
\def\WEkkPerpFroNormStdDevFloat{0.1468510609281961365457647161747445352375507354736328125}
\def\WEqqPerpFirstSingularLen{151}
\def\WEqqPerpFirstSingularMaxFloat{3.823607921600341796875}
\def\WEqqPerpFirstSingularMaxKey{8745}
\def\WEqqPerpFirstSingularMeanFloat{3.42687542075352968851120749604888260364532470703125}
\def\WEqqPerpFirstSingularMeanKey{13468}
\def\WEqqPerpFirstSingularMedianFloat{3.15790903568267822265625}
\def\WEqqPerpFirstSingularMedianKey{1951}
\def\WEqqPerpFirstSingularMinFloat{3.136064052581787109375}
\def\WEqqPerpFirstSingularMinKey{9132}
\def\WEqqPerpFirstSingularStdDevFloat{0.1311080419745109804097182859550230205059051513671875}
\def\WEqqPerpFroNormLen{151}
\def\WEqqPerpFroNormMaxFloat{9.05269622802734375}
\def\WEqqPerpFroNormMaxKey{19451}
\def\WEqqPerpFroNormMeanFloat{8.6761563345296490723512761178426444530487060546875}
\def\WEqqPerpFroNormMeanKey{12287}
\def\WEqqPerpFroNormMedianFloat{8.3731281757354736328125}
\def\WEqqPerpFroNormMedianKey{7238}
\def\WEqqPerpFroNormMinFloat{8.35369396209716796875}
\def\WEqqPerpFroNormMinKey{16069}
\def\WEqqPerpFroNormStdDevFloat{0.1414255003370021857023175471113063395023345947265625}
\def\WKkPerpFirstSingularLen{151}
\def\WKkPerpFirstSingularMaxFloat{1.66061127185821533203125}
\def\WKkPerpFirstSingularMaxKey{7790}
\def\WKkPerpFirstSingularMeanFloat{1.4644347531906027892745214558090083301067352294921875}
\def\WKkPerpFirstSingularMeanKey{32374}
\def\WKkPerpFirstSingularMedianFloat{1.3387131392955780029296875}
\def\WKkPerpFirstSingularMedianKey{17080}
\def\WKkPerpFirstSingularMinFloat{1.33660662174224853515625}
\def\WKkPerpFirstSingularMinKey{2549}
\def\WKkPerpFirstSingularStdDevFloat{0.061627995071164780316319564690275001339614391326904296875}
\def\WKkPerpFroNormLen{151}
\def\WKkPerpFroNormMaxFloat{4.534427642822265625}
\def\WKkPerpFroNormMaxKey{20338}
\def\WKkPerpFroNormMeanFloat{4.27505278113661990602167861652560532093048095703125}
\def\WKkPerpFroNormMeanKey{11598}
\def\WKkPerpFroNormMedianFloat{3.99782884120941162109375}
\def\WKkPerpFroNormMedianKey{2549}
\def\WKkPerpFroNormMinFloat{3.9131908416748046875}
\def\WKkPerpFroNormMinKey{6532}
\def\WKkPerpFroNormStdDevFloat{0.100396761286922930889176086566294543445110321044921875}
\def\WQqPerpFirstSingularLen{151}
\def\WQqPerpFirstSingularMaxFloat{1.72123432159423828125}
\def\WQqPerpFirstSingularMaxKey{7467}
\def\WQqPerpFirstSingularMeanFloat{1.4976005285780951137297734021558426320552825927734375}
\def\WQqPerpFirstSingularMeanKey{23241}
\def\WQqPerpFirstSingularMedianFloat{1.349990308284759521484375}
\def\WQqPerpFirstSingularMedianKey{26374}
\def\WQqPerpFirstSingularMinFloat{1.3414020538330078125}
\def\WQqPerpFirstSingularMinKey{19538}
\def\WQqPerpFirstSingularStdDevFloat{0.061457888202000508781619458886780194006860256195068359375}
\def\WQqPerpFroNormLen{151}
\def\WQqPerpFroNormMaxFloat{4.688735485076904296875}
\def\WQqPerpFroNormMaxKey{2236}
\def\WQqPerpFroNormMeanFloat{4.33065329482223848600597193581052124500274658203125}
\def\WQqPerpFroNormMeanKey{12287}
\def\WQqPerpFroNormMedianFloat{4.05852186679840087890625}
\def\WQqPerpFroNormMedianKey{11498}
\def\WQqPerpFroNormMinFloat{4.040107250213623046875}
\def\WQqPerpFroNormMinKey{26374}
\def\WQqPerpFroNormStdDevFloat{0.08981816615258049474324053562668268568813800811767578125}


==> generated/values-20.tex <==
\def\AllModelsHEADSHASHORT{8830e1d}
\def\AllModelsHEADSHA{8830e1dfd45370596a2540de380db3492fe35914}
\def\AlmostQuadraticAccuracyLen{2718}
\def\AlmostQuadraticAccuracyMaxFloat{0.397668706068207977732953395388904027640819549560546875}
\def\AlmostQuadraticAccuracyMeanFloat{0.1331757127486903613533542056757141835987567901611328125}
\def\AlmostQuadraticAccuracyMedianFloat{0.00000000000000000000000000000000000902779661431516806119989660586684680564735147600963216518721310421824455261230469}
\def\AlmostQuadraticAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\AlmostQuadraticAccuracyStdDevFloat{0.1289398028739690837962683644946082495152950286865234375}
\def\AlmostQuadraticDroppedSequencesFracLen{2718}
\def\AlmostQuadraticDroppedSequencesFracMaxFloat{0.51102902901206170849235377318109385669231414794921875}
\def\AlmostQuadraticDroppedSequencesFracMeanFloat{0.267631010281064452005495013509062118828296661376953125}
\def\AlmostQuadraticDroppedSequencesFracMedianFloat{0}
\def\AlmostQuadraticDroppedSequencesFracMinFloat{0}
\def\AlmostQuadraticDroppedSequencesFracStdDevFloat{0.193659930184946149633873346829204820096492767333984375}
\def\AlmostQuadraticDroppedSequencesLen{2718}
\def\AlmostQuadraticDroppedSequencesMaxFloat{679274092021614382013061870951284366}
\def\AlmostQuadraticDroppedSequencesMeanFloat{355742631405791073334069562835992576}
\def\AlmostQuadraticDroppedSequencesMedianFloat{0}
\def\AlmostQuadraticDroppedSequencesMinFloat{0}
\def\AlmostQuadraticDroppedSequencesStdDevFloat{257418200863581854258183402757816320}
\def\AlmostQuadraticEffectiveDimensionalityEstimateLen{2718}
\def\AlmostQuadraticEffectiveDimensionalityEstimateMaxFloat{6530}
\def\AlmostQuadraticEffectiveDimensionalityEstimateMeanFloat{6487.3333333333330301684327423572540283203125}
\def\AlmostQuadraticEffectiveDimensionalityEstimateMedianFloat{6402}
\def\AlmostQuadraticEffectiveDimensionalityEstimateMinFloat{6402}
\def\AlmostQuadraticEffectiveDimensionalityEstimateStdDevFloat{42.66666666666666429819088079966604709625244140625}
\def\AlmostQuadraticErrUpperBoundLen{2718}
\def\AlmostQuadraticErrUpperBoundMaxFloat{133.0085601806640625}
\def\AlmostQuadraticErrUpperBoundMeanFloat{94.8468834748594389338904875330626964569091796875}
\def\AlmostQuadraticErrUpperBoundMedianFloat{74.71254730224609375}
\def\AlmostQuadraticErrUpperBoundMinFloat{72.31154632568359375}
\def\AlmostQuadraticErrUpperBoundStdDevFloat{9.21741835739664594484565895982086658477783203125}
\def\AlmostQuadraticGapMostBelowValueLen{2718}
\def\AlmostQuadraticGapMostBelowValueMaxFloat{34}
\def\AlmostQuadraticGapMostBelowValueMeanFloat{5.58903605592347307862155503244139254093170166015625}
\def\AlmostQuadraticGapMostBelowValueMedianFloat{1}
\def\AlmostQuadraticGapMostBelowValueMinFloat{1}
\def\AlmostQuadraticGapMostBelowValueNumStdLen{2718}
\def\AlmostQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\AlmostQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\AlmostQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\AlmostQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\AlmostQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\AlmostQuadraticGapMostBelowValueSequenceFracLen{2718}
\def\AlmostQuadraticGapMostBelowValueSequenceFracMaxFloat{1}
\def\AlmostQuadraticGapMostBelowValueSequenceFracMeanFloat{0.99604280024350255740017701100441627204418182373046875}
\def\AlmostQuadraticGapMostBelowValueSequenceFracMedianFloat{0.97226371586322779538846816649311222136020660400390625}
\def\AlmostQuadraticGapMostBelowValueSequenceFracMinFloat{0.96463572978973399774105246251565404236316680908203125}
\def\AlmostQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.0055163893611844816433631422114558517932891845703125}
\def\AlmostQuadraticGapMostBelowValueStdDevFloat{3.697639268087753006142293088487349450588226318359375}
\def\AlmostQuadraticInstructionCountBranchLen{2718}
\def\AlmostQuadraticInstructionCountBranchMaxFloat{0}
\def\AlmostQuadraticInstructionCountBranchMeanFloat{0}
\def\AlmostQuadraticInstructionCountBranchMedianFloat{0}
\def\AlmostQuadraticInstructionCountBranchMinFloat{0}
\def\AlmostQuadraticInstructionCountBranchStdDevFloat{0}
\def\AlmostQuadraticInstructionCountIntLen{2718}
\def\AlmostQuadraticInstructionCountIntMaxFloat{0}
\def\AlmostQuadraticInstructionCountIntMeanFloat{0}
\def\AlmostQuadraticInstructionCountIntMedianFloat{0}
\def\AlmostQuadraticInstructionCountIntMinFloat{0}
\def\AlmostQuadraticInstructionCountIntStdDevFloat{0}
\def\AlmostQuadraticInstructionCountLen{2718}
\def\AlmostQuadraticInstructionCountMaxFloat{17624307}
\def\AlmostQuadraticInstructionCountMeanFloat{17494996.6666666679084300994873046875}
\def\AlmostQuadraticInstructionCountMedianFloat{17365718}
\def\AlmostQuadraticInstructionCountMinFloat{17365718}
\def\AlmostQuadraticInstructionCountStdDevFloat{115433.622899819703889079391956329345703125}
\def\AlmostQuadraticMaxGapLen{2718}
\def\AlmostQuadraticMaxGapMaxFloat{63}
\def\AlmostQuadraticMaxGapMeanFloat{30.428256070640177455288721830584108829498291015625}
\def\AlmostQuadraticMaxGapMedianFloat{1}
\def\AlmostQuadraticMaxGapMinFloat{1}
\def\AlmostQuadraticMaxGapStdDevFloat{22.719062849349146659960752003826200962066650390625}
\def\AlmostQuadraticNormalizedAccuracyLen{2718}
\def\AlmostQuadraticNormalizedAccuracyMaxFloat{0.39786289282033415748429661107365973293781280517578125}
\def\AlmostQuadraticNormalizedAccuracyMeanFloat{0.1337484353910560475053870277406531386077404022216796875}
\def\AlmostQuadraticNormalizedAccuracyMedianFloat{0.00000000000000000000000000000000000918701489667776217044949118979087388873213108951222041500396842134538477567709204720146289220583657453289561090059578418731689453125}
\def\AlmostQuadraticNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\AlmostQuadraticNormalizedAccuracyStdDevFloat{0.129423839396391571199274039827287197113037109375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.397668706068207977732953395388904027640819549560546875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{18146}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.320813463172009871726686469628475606441497802734375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{20751}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.225449495342744554715608273909310810267925262451171875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{6589}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.14620391746150118716940369267831556499004364013671875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03451882648931159369709575912565924227237701416015625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.49450019528885380548643979636835865676403045654296875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.412793657060229357558256424454157240688800811767578125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{11124}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2264651459430972735287213026822428219020366668701171875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1833222082877064007533363110269419848918914794921875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.04494834204990084958186713492978014983236789703369140625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{657303503499052664180563743974875609}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{548696885446894556847883987170885632}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{11124}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{301023812057081660692763048721514496}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{243677011505132896300767516542411365}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{59746594616844563374178661874794496}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6501.6026490066224141628481447696685791015625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{104}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{104}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{31.796555161449202131507263402454555034637451171875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{132.0067138671875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.32800530439970998486387543380260467529296875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{13036}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.435699462890625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{4729}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.464385986328125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.1860173478884359354879052261821925640106201171875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{33}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.5827814569536418076722839032299816608428955078125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99966263771057117804019753748434595763683319091796875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{5928}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99485514456073176337014274395187385380268096923828125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{13654}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97682605683803558349609375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{7098}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.975611507892608642578125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{27714}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004809556475722878178535868443077561096288263797760009765625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.86415993461379247975173711893148720264434814453125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17624307}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17606145.2847682125866413116455078125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{123}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17597590}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{104}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{17597590}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{104}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{8825.115588892740561277605593204498291015625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{59}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{47.5894039735099312338206800632178783416748046875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{2773}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{5358}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{5358}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.7195232897056538234892286709509789943695068359375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.39786289282033415748429661107365973293781280517578125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18146}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.322192355047441925108842042391188442707061767578125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8893}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.232320018548374862543681729221134446561336517333984375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6589}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.171985986117363764957843841330031864345073699951171875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.033851323337207583907826347058289684355258941650390625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.6679251194000244140625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.579345747335054284121724776923656463623046875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22545}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.5120990276336669921875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{51.5117042064666748046875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.0912397709757062358448820305056869983673095703125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.741107463836669921875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{20751}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4383096647578366145125983166508376598358154296875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{8893}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.222578465938568115234375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{8048}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1856682300567644716693394002504646778106689453125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.11823080355049053746796516861650161445140838623046875}
\def\AlmostQuadraticProofSearchTimeLen{2718}
\def\AlmostQuadraticProofSearchTimeMaxFloat{179.0413391590118408203125}
\def\AlmostQuadraticProofSearchTimeMeanFloat{166.994218280334706605572137050330638885498046875}
\def\AlmostQuadraticProofSearchTimeMedianFloat{158.044378738403310080684605054557323455810546875}
\def\AlmostQuadraticProofSearchTimeMinFloat{51.5117042064666748046875}
\def\AlmostQuadraticProofSearchTimeStdDevFloat{6.3021955600439287792369214002974331378936767578125}
\def\AlmostQuadraticProofTimeLen{2718}
\def\AlmostQuadraticProofTimeMaxFloat{9.8223588466644287109375}
\def\AlmostQuadraticProofTimeMeanFloat{9.402661049339680943148778169415891170501708984375}
\def\AlmostQuadraticProofTimeMedianFloat{9.1644240486621857399995860760100185871124267578125}
\def\AlmostQuadraticProofTimeMinFloat{9.11359882354736328125}
\def\AlmostQuadraticProofTimeStdDevFloat{0.12400996058897435780910001312804524786770343780517578125}
\def\AnySubcubicAccuracyLen{15100}
\def\AnySubcubicAccuracyLowerWhiskerBottomEndFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\AnySubcubicAccuracyLowerWhiskerCrosshatchFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\AnySubcubicAccuracyMaxFloat{0.65682941314196041648898471976281143724918365478515625}
\def\AnySubcubicAccuracyMeanFloat{0.285380986446845341664158013372798450291156768798828125}
\def\AnySubcubicAccuracyMedianFloat{0.00000000000000000000000000000000000978011299884143206629988798968908403945129743234376817895281419623643159866333008}
\def\AnySubcubicAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\AnySubcubicAccuracyQuartileOneFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\AnySubcubicAccuracyQuartileThreeFloat{0.00000000000000000000000000000000000978011299884143206629988798968908403945129743234376817895281419623643159866333008}
\def\AnySubcubicAccuracySqrMeanFloat{0.12251917239661909431180930596383404918015003204345703125}
\def\AnySubcubicAccuracyStdDevFloat{0.2026742829548055235822090480724000371992588043212890625}
\def\AnySubcubicAccuracyUpperWhiskerCrosshatchFloat{0.00000000000000000000000000000000000978011299884143206629988798968908403945129743234376817895281419623643159866333008}
\def\AnySubcubicAccuracyUpperWhiskerTopEndFloat{0.00000000000000000000000000000000000978011299884143206629988798968908403945129743234376817895281419623643159866333008}
\def\AnySubcubicDroppedSequencesFracLen{15100}
\def\AnySubcubicDroppedSequencesFracMaxFloat{0.53906418480378193169855194355477578938007354736328125}
\def\AnySubcubicDroppedSequencesFracMeanFloat{0.195794622459914524625901321996934711933135986328125}
\def\AnySubcubicDroppedSequencesFracMedianFloat{0}
\def\AnySubcubicDroppedSequencesFracMinFloat{0}
\def\AnySubcubicDroppedSequencesFracStdDevFloat{0.1465138619459875057859932212522835470736026763916015625}
\def\AnySubcubicDroppedSequencesLen{15100}
\def\AnySubcubicDroppedSequencesMaxFloat{716539205966160580971401308421148540}
\def\AnySubcubicDroppedSequencesMeanFloat{260255693597856974946694159459680256}
\def\AnySubcubicDroppedSequencesMedianFloat{0}
\def\AnySubcubicDroppedSequencesMinFloat{0}
\def\AnySubcubicDroppedSequencesStdDevFloat{194750327069177733286732938170335232}
\def\AnySubcubicEffectiveDimensionalityEstimateLen{15100}
\def\AnySubcubicEffectiveDimensionalityEstimateMaxFloat{10370}
\def\AnySubcubicEffectiveDimensionalityEstimateMeanFloat{6049.600000000000363797880709171295166015625}
\def\AnySubcubicEffectiveDimensionalityEstimateMedianFloat{4290}
\def\AnySubcubicEffectiveDimensionalityEstimateMinFloat{4290}
\def\AnySubcubicEffectiveDimensionalityEstimateStdDevFloat{1530.49032666005450664670206606388092041015625}
\def\AnySubcubicErrUpperBoundLen{15100}
\def\AnySubcubicErrUpperBoundMaxFloat{133.0085601806640625}
\def\AnySubcubicErrUpperBoundMeanFloat{32.2994531018844526215616497211158275604248046875}
\def\AnySubcubicErrUpperBoundMedianFloat{0}
\def\AnySubcubicErrUpperBoundMinFloat{0}
\def\AnySubcubicErrUpperBoundStdDevFloat{41.37278918181758768923828029073774814605712890625}
\def\AnySubcubicGapMostBelowValueLen{15100}
\def\AnySubcubicGapMostBelowValueMaxFloat{40}
\def\AnySubcubicGapMostBelowValueMeanFloat{4.0474172185430461468058638274669647216796875}
\def\AnySubcubicGapMostBelowValueMedianFloat{1}
\def\AnySubcubicGapMostBelowValueMinFloat{1}
\def\AnySubcubicGapMostBelowValueNumStdLen{15100}
\def\AnySubcubicGapMostBelowValueNumStdMaxFloat{1.5}
\def\AnySubcubicGapMostBelowValueNumStdMeanFloat{1.5}
\def\AnySubcubicGapMostBelowValueNumStdMedianFloat{1.5}
\def\AnySubcubicGapMostBelowValueNumStdMinFloat{1.5}
\def\AnySubcubicGapMostBelowValueNumStdStdDevFloat{0}
\def\AnySubcubicGapMostBelowValueSequenceFracLen{15100}
\def\AnySubcubicGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\AnySubcubicGapMostBelowValueSequenceFracMeanFloat{0.99297068597859894367729793884791433811187744140625}
\def\AnySubcubicGapMostBelowValueSequenceFracMedianFloat{0.9482583582401276078854834850062616169452667236328125}
\def\AnySubcubicGapMostBelowValueSequenceFracMinFloat{0.8931427001953125}
\def\AnySubcubicGapMostBelowValueSequenceFracStdDevFloat{0.009872268453546072242144049369017011485993862152099609375}
\def\AnySubcubicGapMostBelowValueStdDevFloat{3.165125038295942605515165269025601446628570556640625}
\def\AnySubcubicInstructionCountBranchLen{15100}
\def\AnySubcubicInstructionCountBranchMaxFloat{0}
\def\AnySubcubicInstructionCountBranchMeanFloat{0}
\def\AnySubcubicInstructionCountBranchMedianFloat{0}
\def\AnySubcubicInstructionCountBranchMinFloat{0}
\def\AnySubcubicInstructionCountBranchStdDevFloat{0}
\def\AnySubcubicInstructionCountIntLen{15100}
\def\AnySubcubicInstructionCountIntMaxFloat{0}
\def\AnySubcubicInstructionCountIntMeanFloat{0}
\def\AnySubcubicInstructionCountIntMedianFloat{0}
\def\AnySubcubicInstructionCountIntMinFloat{0}
\def\AnySubcubicInstructionCountIntStdDevFloat{0}
\def\AnySubcubicInstructionCountLen{15100}
\def\AnySubcubicInstructionCountMaxFloat{20356824}
\def\AnySubcubicInstructionCountMeanFloat{18392610.8000000007450580596923828125}
\def\AnySubcubicInstructionCountMedianFloat{17365718}
\def\AnySubcubicInstructionCountMinFloat{17365718}
\def\AnySubcubicInstructionCountStdDevFloat{802225.011615918134339153766632080078125}
\def\AnySubcubicMaxGapLen{15100}
\def\AnySubcubicMaxGapMaxFloat{63}
\def\AnySubcubicMaxGapMeanFloat{30.06509933774834308906065416522324085235595703125}
\def\AnySubcubicMaxGapMedianFloat{1}
\def\AnySubcubicMaxGapMinFloat{1}
\def\AnySubcubicMaxGapStdDevFloat{20.567577209649659408796651405282318592071533203125}
\def\AnySubcubicNormalizedAccuracyLen{15100}
\def\AnySubcubicNormalizedAccuracyLowerWhiskerBottomEndFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\AnySubcubicNormalizedAccuracyLowerWhiskerCrosshatchFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\AnySubcubicNormalizedAccuracyMaxFloat{0.6572436982471929756144390921690501272678375244140625}
\def\AnySubcubicNormalizedAccuracyMeanFloat{0.28649185540496258095544135358068160712718963623046875}
\def\AnySubcubicNormalizedAccuracyMedianFloat{0.00000000000000000000000000000000000985300171323342070093429178227190602243421973120466404316741577720453947982842516045186103366970709060979061177931725978851318359375}
\def\AnySubcubicNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\AnySubcubicNormalizedAccuracyQuartileOneFloat{0.0000000000000000000000000000000000083917375014352430854313023433258477025093036112278075374873495141465266758000330736439687710596924130612705994280986487865447998046875}
\def\AnySubcubicNormalizedAccuracyQuartileThreeFloat{0.00000000000000000000000000000000000988818944472971676150648252020213578438377551486800723506651384183728498334491473832177682763699966272952224244363605976104736328125}
\def\AnySubcubicNormalizedAccuracySqrMeanFloat{0.123387225387836363399429728815448470413684844970703125}
\def\AnySubcubicNormalizedAccuracyStdDevFloat{0.2032477359639176806016536147581064142286777496337890625}
\def\AnySubcubicNormalizedAccuracyUpperWhiskerCrosshatchFloat{0.000000000000000000000000000000000009921479311965855079314571704399574915083482286627933760793259164241522462752416514191939104182205166893027126207016408443450927734375}
\def\AnySubcubicNormalizedAccuracyUpperWhiskerTopEndFloat{0.0000000000000000000000000000000000105915154051440253389285521283161639956019943026472296838354159206691929272247892578913460045163252853939184205955825746059417724609375}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLowerWhiskerBottomEndFloat{0.2598536867210172740527696078061126172542572021484375}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLowerWhiskerBottomEndKey{15622}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLowerWhiskerCrosshatchFloat{0.282340495289859438887702935971901752054691314697265625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLowerWhiskerCrosshatchKey{15622}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.65682941314196041648898471976281143724918365478515625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMaxKey{27671}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.56121004634953008949338482125313021242618560791015625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMeanKey{7098}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.4200645042537107798352735699154436588287353515625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMinFloat{0.25265074475171689361019389252760447561740875244140625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyQuartileOneFloat{0.336357624502713836722733731221524067223072052001953125}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyQuartileOneKey{15622}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyQuartileThreeFloat{0.476760163244945356364468125320854596793651580810546875}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyQuartileThreeKey{19538}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracySqrMeanFloat{0.316802998860290674354445172866689972579479217529296875}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.042968392297698144999262837018250138498842716217041015625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyUpperWhiskerCrosshatchFloat{0.478485224960457367071597900576307438313961029052734375}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyUpperWhiskerCrosshatchKey{19538}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyUpperWhiskerTopEndFloat{0.479203351472018146406384175861603580415248870849609375}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyUpperWhiskerTopEndKey{19538}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.23052385661848628917169889973592944443225860595703125}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{27300}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.13407621728723950749184723463258706033229827880859375}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12457}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.04783335998494049612350664801851962693035602569580078125}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18289}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.02845918004020230041017924804691574536263942718505859375}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.039519286610340993715073665271120262332260608673095703125}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{306418763913599937668037273980403551}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{27300}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{178217861587140260755829682832670720}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12457}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{63581441224440886256543766388146176}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18289}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{37828738846520300492525058542808020}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{52530142135913202241742431210962944}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{104}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{7383.9735099337749488768167793750762939453125}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{1185}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4400.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{6910}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{8840}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{1820.64069920170322802732698619365692138671875}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{9.1559906005859375}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4157}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0.991665388574663353438154445029795169830322265625}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{3254}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{104}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinKey{104}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.9653311092506668966706229184637777507305145263671875}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{2.867549668874172397181609994731843471527099609375}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999849796295166015625}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{31308}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.992647306019107222851971528143621981143951416015625}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4810}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9595743119716644287109375}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20754}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95257580280303955078125}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{22286}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00910800686383549627789246727616045973263680934906005859375}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.571688525957807502919649778050370514392852783203125}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20348569}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMaxKey{6910}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18476152.19867549836635589599609375}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMeanKey{7467}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17910775}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMedianKey{104}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMinFloat{17910775}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMinKey{104}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{568715.6135063879191875457763671875}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMaxFloat{49}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMaxKey{1185}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMeanFloat{39.35761589403973204071007785387337207794189453125}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMeanKey{7310}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapStdDevFloat{12.4960096257843193967573824920691549777984619140625}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLowerWhiskerBottomEndFloat{0.30326854932331615000151714411913417279720306396484375}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLowerWhiskerBottomEndKey{15622}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLowerWhiskerCrosshatchFloat{0.322201453024718753592736675273044966161251068115234375}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLowerWhiskerCrosshatchKey{15622}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6572436982471929756144390921690501272678375244140625}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27671}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.56354892045871152195246622795821167528629302978515625}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{18668}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.43815901059012152263250072792288847267627716064453125}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{3254}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.297203989016589786853472787697683088481426239013671875}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyQuartileOneFloat{0.36768149980335562698741114218137226998805999755859375}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyQuartileOneKey{15622}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyQuartileThreeFloat{0.48514460744941956260589677185635082423686981201171875}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyQuartileThreeKey{3254}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracySqrMeanFloat{0.319210818795634565514518499185214750468730926513671875}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0402918483747694844421260995659395121037960052490234375}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyUpperWhiskerCrosshatchFloat{0.4851457490107524694877838555839844048023223876953125}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyUpperWhiskerCrosshatchKey{3254}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyUpperWhiskerTopEndFloat{0.48514622423169695419886693343869410455226898193359375}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyUpperWhiskerTopEndKey{3254}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.77167415618896484375}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.857632138081726225209422409534454345703125}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1490}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.964951336383819580078125}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.6911551952362060546875}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8048}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.251991228210260320707902792491950094699859619140625}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.8180291652679443359375}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.44202332780850639437630889005959033966064453125}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMeanKey{17197}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.236496508121490478515625}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMedianKey{9816}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2120714187622088076068394002504646778106689453125}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1194509288843590144590933732615667395293712615966796875}
\def\AnySubcubicProofSearchTimeLen{15100}
\def\AnySubcubicProofSearchTimeMaxFloat{179.535578250885009765625}
\def\AnySubcubicProofSearchTimeMeanFloat{167.053254127739279510933556593954563140869140625}
\def\AnySubcubicProofSearchTimeMedianFloat{158.331018409729011864328640513122081756591796875}
\def\AnySubcubicProofSearchTimeMinFloat{51.5117042064666748046875}
\def\AnySubcubicProofSearchTimeStdDevFloat{5.31773778586767864595685750828124582767486572265625}
\def\AnySubcubicProofTimeLen{15100}
\def\AnySubcubicProofTimeMaxFloat{9.88440799713134765625}
\def\AnySubcubicProofTimeMeanFloat{9.4070758672265810673707164824008941650390625}
\def\AnySubcubicProofTimeMedianFloat{9.1597884130477922326463158242404460906982421875}
\def\AnySubcubicProofTimeMinFloat{9.0863430500030517578125}
\def\AnySubcubicProofTimeStdDevFloat{0.12458653641845711390612194691129843704402446746826171875}
\def\AxisLimitsOVCenteredZmaxFloat{28.4637966156005859375}
\def\AxisLimitsOVCenteredZminFloat{-82.2288665771484375}
\def\AxisLimitsOVZmaxFloat{43.057903289794921875}
\def\AxisLimitsOVZminFloat{-43.057903289794921875}
\def\AxisLimitsQKWithAttnScaleZmaxFloat{144.69254510938191060631652362644672393798828125}
\def\AxisLimitsQKWithAttnScaleZminFloat{-144.69254510938191060631652362644672393798828125}
\def\AxisLimitsQKZmaxFloat{818.504638671875}
\def\AxisLimitsQKZminFloat{-818.504638671875}
\def\BruteForceEffectiveDimensionalityEstimate{85070591730234615865843651857942052864}
\def\BruteForceInstructionCountBranch{0}
\def\BruteForceInstructionCountInt{0}
\def\BruteForceInstructionCount{292810962955378452216344827154123377256431616}
\def\CubicAccuracyLen{151}
\def\CubicAccuracyLowerWhiskerBottomEndFloat{0.66911613739890707375224110364797525107860565185546875}
\def\CubicAccuracyLowerWhiskerBottomEndKey{15622}
\def\CubicAccuracyLowerWhiskerCrosshatchFloat{0.677578984888455249091521181981079280376434326171875}
\def\CubicAccuracyLowerWhiskerCrosshatchKey{15622}
\def\CubicAccuracyMaxFloat{0.9653734496767556461094272890477441251277923583984375}
\def\CubicAccuracyMaxKey{30463}
\def\CubicAccuracyMeanFloat{0.884457346906930563790183441597037017345428466796875}
\def\CubicAccuracyMeanKey{14929}
\def\CubicAccuracyMedianFloat{0.72941103032709564413238467750488780438899993896484375}
\def\CubicAccuracyMedianKey{19538}
\def\CubicAccuracyMinFloat{0.666405330341710122610265898401848971843719482421875}
\def\CubicAccuracyMinKey{15622}
\def\CubicAccuracyQuartileOneFloat{0.69790818033440282786017405669554136693477630615234375}
\def\CubicAccuracyQuartileOneKey{15622}
\def\CubicAccuracyQuartileThreeFloat{0.757018671322049474525783807621337473392486572265625}
\def\CubicAccuracyQuartileThreeKey{19538}
\def\CubicAccuracySqrMeanFloat{0.78387674861219502897569100241526030004024505615234375}
\def\CubicAccuracyStdDevFloat{0.040149098552129593164838894381318823434412479400634765625}
\def\CubicAccuracyUpperWhiskerCrosshatchFloat{0.76980698093993249475630591405206359922885894775390625}
\def\CubicAccuracyUpperWhiskerCrosshatchKey{19538}
\def\CubicAccuracyUpperWhiskerTopEndFloat{0.77513063057638864616905038928962312638759613037109375}
\def\CubicAccuracyUpperWhiskerTopEndKey{19538}
\def\CubicCorrectCountLen{151}
\def\CubicCorrectCountMaxFloat{1283201415697804169451605233208610787}
\def\CubicCorrectCountMaxKey{30463}
\def\CubicCorrectCountMeanFloat{1175645466586344408422351965463248896}
\def\CubicCorrectCountMeanKey{14929}
\def\CubicCorrectCountMedianFloat{969553561945095832798180761246105600}
\def\CubicCorrectCountMedianKey{19538}
\def\CubicCorrectCountMinFloat{885804621630496107045374771652360332}
\def\CubicCorrectCountMinKey{15622}
\def\CubicCorrectCountStdDevFloat{53367305801018268392266210178236416}
\def\CubicEffectiveDimensionalityEstimate{14848}
\def\CubicInstructionCountBranch{0}
\def\CubicInstructionCountInt{0}
\def\CubicInstructionCount{752334304}
\def\CubicNormalizedAccuracyLen{151}
\def\CubicNormalizedAccuracyLowerWhiskerBottomEndFloat{0.7843325480247729242222476386814378201961517333984375}
\def\CubicNormalizedAccuracyLowerWhiskerBottomEndKey{15622}
\def\CubicNormalizedAccuracyLowerWhiskerCrosshatchFloat{0.785616145626899964327094494365155696868896484375}
\def\CubicNormalizedAccuracyLowerWhiskerCrosshatchKey{15622}
\def\CubicNormalizedAccuracyMaxFloat{0.966231051331615464761171097052283585071563720703125}
\def\CubicNormalizedAccuracyMaxKey{30463}
\def\CubicNormalizedAccuracyMeanFloat{0.888482876299318657942194477072916924953460693359375}
\def\CubicNormalizedAccuracyMeanKey{22286}
\def\CubicNormalizedAccuracyMedianFloat{0.793477741776487999203482104348950088024139404296875}
\def\CubicNormalizedAccuracyMedianKey{19538}
\def\CubicNormalizedAccuracyMinFloat{0.78392138789897070072498763693147338926792144775390625}
\def\CubicNormalizedAccuracyMinKey{15622}
\def\CubicNormalizedAccuracyQuartileOneFloat{0.78869956483772940547538610189803875982761383056640625}
\def\CubicNormalizedAccuracyQuartileOneKey{15622}
\def\CubicNormalizedAccuracyQuartileThreeFloat{0.798409331811800626610420295037329196929931640625}
\def\CubicNormalizedAccuracyQuartileThreeKey{19538}
\def\CubicNormalizedAccuracySqrMeanFloat{0.79066763422672903249832643268746323883533477783203125}
\def\CubicNormalizedAccuracyStdDevFloat{0.035578262318707927491789888563289423473179340362548828125}
\def\CubicNormalizedAccuracyUpperWhiskerCrosshatchFloat{0.80178974937273495005030099491705186665058135986328125}
\def\CubicNormalizedAccuracyUpperWhiskerCrosshatchKey{19538}
\def\CubicNormalizedAccuracyUpperWhiskerTopEndFloat{0.8031969845161641696762444553314708173274993896484375}
\def\CubicNormalizedAccuracyUpperWhiskerTopEndKey{19538}
\def\CubicProofTimeLen{151}
\def\CubicProofTimeMaxFloat{286.869518756866455078125}
\def\CubicProofTimeMaxKey{4729}
\def\CubicProofTimeMeanFloat{270.52646698699089711226406507194042205810546875}
\def\CubicProofTimeMeanKey{19093}
\def\CubicProofTimeMedianFloat{220.97906506061553955078125}
\def\CubicProofTimeMedianKey{8893}
\def\CubicProofTimeMinFloat{95.3405177593231201171875}
\def\CubicProofTimeMinKey{123}
\def\CubicProofTimeStdDevFloat{15.6421084031079775655825869762338697910308837890625}
\def\EPVOUAbsLenLen{151}
\def\EPVOUAbsLenMaxFloat{4096}
\def\EPVOUAbsLenMaxKey{50}
\def\EPVOUAbsLenMeanFloat{4096}
\def\EPVOUAbsLenMeanKey{50}
\def\EPVOUAbsLenMedianFloat{4096}
\def\EPVOUAbsLenMedianKey{50}
\def\EPVOUAbsLenMinFloat{4096}
\def\EPVOUAbsLenMinKey{50}
\def\EPVOUAbsLenStdDevFloat{0}
\def\EPVOUAbsMaxLen{151}
\def\EPVOUAbsMaxMaxFloat{43.05789947509765625}
\def\EPVOUAbsMaxMaxKey{10248}
\def\EPVOUAbsMaxMeanFloat{34.080196380615234375}
\def\EPVOUAbsMaxMeanKey{20338}
\def\EPVOUAbsMaxMedianFloat{26.741374492645263671875}
\def\EPVOUAbsMaxMedianKey{11130}
\def\EPVOUAbsMaxMinFloat{26.4571475982666015625}
\def\EPVOUAbsMaxMinKey{1490}
\def\EPVOUAbsMaxStdDevFloat{3.3996829986572265625}
\def\EPVOUAbsMeanLen{151}
\def\EPVOUAbsMeanMaxFloat{6.8591461181640625}
\def\EPVOUAbsMeanMaxKey{20976}
\def\EPVOUAbsMeanMeanFloat{4.08612155914306640625}
\def\EPVOUAbsMeanMeanKey{23367}
\def\EPVOUAbsMeanMedianFloat{2.513208448886871337890625}
\def\EPVOUAbsMeanMedianKey{18668}
\def\EPVOUAbsMeanMinFloat{2.474681377410888671875}
\def\EPVOUAbsMeanMinKey{30371}
\def\EPVOUAbsMeanStdDevFloat{0.921686589717864990234375}
\def\EPVOUAbsMedianLen{151}
\def\EPVOUAbsMedianMaxFloat{0.207202665507793426513671875}
\def\EPVOUAbsMedianMaxKey{20976}
\def\EPVOUAbsMedianMeanFloat{0.042490789488216995639646711424575187265872955322265625}
\def\EPVOUAbsMedianMeanKey{11498}
\def\EPVOUAbsMedianMedianFloat{0.0084453102201223380351979841407228377647697925567626953125}
\def\EPVOUAbsMedianMedianKey{2306}
\def\EPVOUAbsMedianMinFloat{0.00842666774988174403782092980463858111761510372161865234375}
\def\EPVOUAbsMedianMinKey{30371}
\def\EPVOUAbsMedianStdDevFloat{0.034554721712523051024845699430443346500396728515625}
\def\EPVOUAbsMinLen{151}
\def\EPVOUAbsMinMaxFloat{0.0299930572509765625}
\def\EPVOUAbsMinMaxKey{2345}
\def\EPVOUAbsMinMeanFloat{0.00191172468475997447967529296875}
\def\EPVOUAbsMinMeanKey{3254}
\def\EPVOUAbsMinMedianFloat{0.0000099837779998779296875}
\def\EPVOUAbsMinMedianKey{11124}
\def\EPVOUAbsMinMinFloat{0.00000274181365966796875}
\def\EPVOUAbsMinMinKey{18668}
\def\EPVOUAbsMinStdDevFloat{0.00327258347533643245697021484375}
\def\EPVOUAbsStdDevLen{151}
\def\EPVOUAbsStdDevMaxFloat{4.72914981842041015625}
\def\EPVOUAbsStdDevMaxKey{27484}
\def\EPVOUAbsStdDevMeanFloat{3.7594051361083984375}
\def\EPVOUAbsStdDevMeanKey{8721}
\def\EPVOUAbsStdDevMedianFloat{2.90534174442291259765625}
\def\EPVOUAbsStdDevMedianKey{24144}
\def\EPVOUAbsStdDevMinFloat{2.6322252750396728515625}
\def\EPVOUAbsStdDevMinKey{1490}
\def\EPVOUAbsStdDevStdDevFloat{0.3865978717803955078125}
\def\EPVOUCenteredLenLen{151}
\def\EPVOUCenteredLenMaxFloat{4096}
\def\EPVOUCenteredLenMaxKey{50}
\def\EPVOUCenteredLenMeanFloat{4096}
\def\EPVOUCenteredLenMeanKey{50}
\def\EPVOUCenteredLenMedianFloat{4096}
\def\EPVOUCenteredLenMedianKey{50}
\def\EPVOUCenteredLenMinFloat{4096}
\def\EPVOUCenteredLenMinKey{50}
\def\EPVOUCenteredLenStdDevFloat{0}
\def\EPVOUCenteredMaxLen{151}
\def\EPVOUCenteredMaxMaxFloat{28.4637908935546875}
\def\EPVOUCenteredMaxMaxKey{15622}
\def\EPVOUCenteredMaxMeanFloat{10.8519802093505859375}
\def\EPVOUCenteredMaxMeanKey{20539}
\def\EPVOUCenteredMaxMedianFloat{7.424126148223876953125}
\def\EPVOUCenteredMaxMedianKey{14095}
\def\EPVOUCenteredMaxMinFloat{7.173371791839599609375}
\def\EPVOUCenteredMaxMinKey{8048}
\def\EPVOUCenteredMaxStdDevFloat{2.2125437259674072265625}
\def\EPVOUCenteredMeanLen{151}
\def\EPVOUCenteredMeanMaxFloat{-3.720808506011962890625}
\def\EPVOUCenteredMeanMaxKey{1490}
\def\EPVOUCenteredMeanMeanFloat{-7.07141208648681640625}
\def\EPVOUCenteredMeanMeanKey{22286}
\def\EPVOUCenteredMeanMedianFloat{-8.665364742279052734375}
\def\EPVOUCenteredMeanMedianKey{6910}
\def\EPVOUCenteredMeanMinFloat{-8.6850986480712890625}
\def\EPVOUCenteredMeanMinKey{9504}
\def\EPVOUCenteredMeanStdDevFloat{0.88744533061981201171875}
\def\EPVOUCenteredMedianLen{151}
\def\EPVOUCenteredMedianMaxFloat{-36.245299816131591796875}
\def\EPVOUCenteredMedianMaxKey{1490}
\def\EPVOUCenteredMedianMeanFloat{-48.460103367811797170361387543380260467529296875}
\def\EPVOUCenteredMedianMeanKey{28778}
\def\EPVOUCenteredMedianMedianFloat{-59.45346174240112446796047152020037174224853515625}
\def\EPVOUCenteredMedianMedianKey{27484}
\def\EPVOUCenteredMedianMinFloat{-59.54390296936035298358547152020037174224853515625}
\def\EPVOUCenteredMedianMinKey{9504}
\def\EPVOUCenteredMedianStdDevFloat{4.39827466942062272892144392244517803192138671875}
\def\EPVOUCenteredMinLen{151}
\def\EPVOUCenteredMinMaxFloat{-43.65570831298828125}
\def\EPVOUCenteredMinMaxKey{1490}
\def\EPVOUCenteredMinMeanFloat{-60.7017669677734375}
\def\EPVOUCenteredMinMeanKey{4430}
\def\EPVOUCenteredMinMedianFloat{-80.30307769775390625}
\def\EPVOUCenteredMinMedianKey{3175}
\def\EPVOUCenteredMinMinFloat{-82.2288665771484375}
\def\EPVOUCenteredMinMinKey{10248}
\def\EPVOUCenteredMinStdDevFloat{7.140367031097412109375}
\def\EPVOUCenteredOffDiagonalLenLen{151}
\def\EPVOUCenteredOffDiagonalLenMaxFloat{4032}
\def\EPVOUCenteredOffDiagonalLenMaxKey{50}
\def\EPVOUCenteredOffDiagonalLenMeanFloat{4032}
\def\EPVOUCenteredOffDiagonalLenMeanKey{50}
\def\EPVOUCenteredOffDiagonalLenMedianFloat{4032}
\def\EPVOUCenteredOffDiagonalLenMedianKey{50}
\def\EPVOUCenteredOffDiagonalLenMinFloat{4032}
\def\EPVOUCenteredOffDiagonalLenMinKey{50}
\def\EPVOUCenteredOffDiagonalLenStdDevFloat{0}
\def\EPVOUCenteredOffDiagonalMaxLen{151}
\def\EPVOUCenteredOffDiagonalMaxMaxFloat{28.4637908935546875}
\def\EPVOUCenteredOffDiagonalMaxMaxKey{15622}
\def\EPVOUCenteredOffDiagonalMaxMeanFloat{10.8519802093505859375}
\def\EPVOUCenteredOffDiagonalMaxMeanKey{20539}
\def\EPVOUCenteredOffDiagonalMaxMedianFloat{7.424126148223876953125}
\def\EPVOUCenteredOffDiagonalMaxMedianKey{14095}
\def\EPVOUCenteredOffDiagonalMaxMinFloat{7.173371791839599609375}
\def\EPVOUCenteredOffDiagonalMaxMinKey{8048}
\def\EPVOUCenteredOffDiagonalMaxStdDevFloat{2.2125437259674072265625}
\def\EPVOUCenteredOffDiagonalMeanLen{151}
\def\EPVOUCenteredOffDiagonalMeanMaxFloat{-3.7798688411712646484375}
\def\EPVOUCenteredOffDiagonalMeanMaxKey{1490}
\def\EPVOUCenteredOffDiagonalMeanMeanFloat{-7.183658599853515625}
\def\EPVOUCenteredOffDiagonalMeanMeanKey{22286}
\def\EPVOUCenteredOffDiagonalMeanMedianFloat{-8.8029105663299560546875}
\def\EPVOUCenteredOffDiagonalMeanMedianKey{6910}
\def\EPVOUCenteredOffDiagonalMeanMinFloat{-8.82295703887939453125}
\def\EPVOUCenteredOffDiagonalMeanMinKey{9504}
\def\EPVOUCenteredOffDiagonalMeanStdDevFloat{0.901531755924224853515625}
\def\EPVOUCenteredOffDiagonalMedianLen{151}
\def\EPVOUCenteredOffDiagonalMedianMaxFloat{-36.27422437667846821796047152020037174224853515625}
\def\EPVOUCenteredOffDiagonalMedianMaxKey{1490}
\def\EPVOUCenteredOffDiagonalMedianMeanFloat{-48.5438783396790398683151579461991786956787109375}
\def\EPVOUCenteredOffDiagonalMedianMeanKey{26374}
\def\EPVOUCenteredOffDiagonalMedianMedianFloat{-59.46652448654175060482884873636066913604736328125}
\def\EPVOUCenteredOffDiagonalMedianMedianKey{27484}
\def\EPVOUCenteredOffDiagonalMedianMinFloat{-59.55053871154785127828290569595992565155029296875}
\def\EPVOUCenteredOffDiagonalMedianMinKey{9504}
\def\EPVOUCenteredOffDiagonalMedianStdDevFloat{4.41332284087521653503927154815755784511566162109375}
\def\EPVOUCenteredOffDiagonalMinLen{151}
\def\EPVOUCenteredOffDiagonalMinMaxFloat{-43.65570831298828125}
\def\EPVOUCenteredOffDiagonalMinMaxKey{1490}
\def\EPVOUCenteredOffDiagonalMinMeanFloat{-60.7017669677734375}
\def\EPVOUCenteredOffDiagonalMinMeanKey{4430}
\def\EPVOUCenteredOffDiagonalMinMedianFloat{-80.30307769775390625}
\def\EPVOUCenteredOffDiagonalMinMedianKey{3175}
\def\EPVOUCenteredOffDiagonalMinMinFloat{-82.2288665771484375}
\def\EPVOUCenteredOffDiagonalMinMinKey{10248}
\def\EPVOUCenteredOffDiagonalMinStdDevFloat{7.140367031097412109375}
\def\EPVOUCenteredOffDiagonalStdDevLen{151}
\def\EPVOUCenteredOffDiagonalStdDevMaxFloat{15.08925342559814453125}
\def\EPVOUCenteredOffDiagonalStdDevMaxKey{10248}
\def\EPVOUCenteredOffDiagonalStdDevMeanFloat{12.3969707489013671875}
\def\EPVOUCenteredOffDiagonalStdDevMeanKey{1185}
\def\EPVOUCenteredOffDiagonalStdDevMedianFloat{9.0506913661956787109375}
\def\EPVOUCenteredOffDiagonalStdDevMedianKey{1490}
\def\EPVOUCenteredOffDiagonalStdDevMinFloat{9.0365543365478515625}
\def\EPVOUCenteredOffDiagonalStdDevMinKey{15622}
\def\EPVOUCenteredOffDiagonalStdDevStdDevFloat{1.03410661220550537109375}
\def\EPVOUCenteredStdDevLen{151}
\def\EPVOUCenteredStdDevMaxFloat{15.009273529052734375}
\def\EPVOUCenteredStdDevMaxKey{10248}
\def\EPVOUCenteredStdDevMeanFloat{12.3321132659912109375}
\def\EPVOUCenteredStdDevMeanKey{1185}
\def\EPVOUCenteredStdDevMedianFloat{8.9921848773956298828125}
\def\EPVOUCenteredStdDevMedianKey{1490}
\def\EPVOUCenteredStdDevMinFloat{8.97893619537353515625}
\def\EPVOUCenteredStdDevMinKey{15622}
\def\EPVOUCenteredStdDevStdDevFloat{1.0302727222442626953125}
\def\EPVOUDiagonalLenLen{151}
\def\EPVOUDiagonalLenMaxFloat{64}
\def\EPVOUDiagonalLenMaxKey{50}
\def\EPVOUDiagonalLenMeanFloat{64}
\def\EPVOUDiagonalLenMeanKey{50}
\def\EPVOUDiagonalLenMedianFloat{64}
\def\EPVOUDiagonalLenMedianKey{50}
\def\EPVOUDiagonalLenMinFloat{64}
\def\EPVOUDiagonalLenMinKey{50}
\def\EPVOUDiagonalLenStdDevFloat{0}
\def\EPVOUDiagonalMaxLen{151}
\def\EPVOUDiagonalMaxMaxFloat{43.05789947509765625}
\def\EPVOUDiagonalMaxMaxKey{10248}
\def\EPVOUDiagonalMaxMeanFloat{34.0606689453125}
\def\EPVOUDiagonalMaxMeanKey{20338}
\def\EPVOUDiagonalMaxMedianFloat{26.741374492645263671875}
\def\EPVOUDiagonalMaxMedianKey{11130}
\def\EPVOUDiagonalMaxMinFloat{26.4571475982666015625}
\def\EPVOUDiagonalMaxMinKey{1490}
\def\EPVOUDiagonalMaxStdDevFloat{3.395696163177490234375}
\def\EPVOUDiagonalMeanLen{151}
\def\EPVOUDiagonalMeanMaxFloat{10.789218902587890625}
\def\EPVOUDiagonalMeanMaxKey{20976}
\def\EPVOUDiagonalMeanMeanFloat{7.511943340301513671875}
\def\EPVOUDiagonalMeanMeanKey{27584}
\def\EPVOUDiagonalMeanMedianFloat{3.58126986026763916015625}
\def\EPVOUDiagonalMeanMedianKey{15622}
\def\EPVOUDiagonalMeanMinFloat{2.8847277164459228515625}
\def\EPVOUDiagonalMeanMinKey{1490}
\def\EPVOUDiagonalMeanStdDevFloat{1.3667886257171630859375}
\def\EPVOUDiagonalMedianLen{151}
\def\EPVOUDiagonalMedianMaxFloat{2.770182918310165387509869105997495353221893310546875}
\def\EPVOUDiagonalMedianMaxKey{16149}
\def\EPVOUDiagonalMedianMeanFloat{-0.67308657454141707088268731240532360970973968505859375}
\def\EPVOUDiagonalMedianMeanKey{7098}
\def\EPVOUDiagonalMedianMedianFloat{-2.901954807937145108809318116982467472553253173828125}
\def\EPVOUDiagonalMedianMedianKey{15622}
\def\EPVOUDiagonalMedianMinFloat{-3.27623795986175547767516036401502788066864013671875}
\def\EPVOUDiagonalMedianMinKey{16069}
\def\EPVOUDiagonalMedianStdDevFloat{1.163024471878025156712510579382069408893585205078125}
\def\EPVOUDiagonalMinLen{151}
\def\EPVOUDiagonalMinMaxFloat{2.503263950347900390625}
\def\EPVOUDiagonalMinMaxKey{16149}
\def\EPVOUDiagonalMinMeanFloat{-0.818982303142547607421875}
\def\EPVOUDiagonalMinMeanKey{25516}
\def\EPVOUDiagonalMinMedianFloat{-3.06046736240386962890625}
\def\EPVOUDiagonalMinMedianKey{4430}
\def\EPVOUDiagonalMinMinFloat{-3.333894252777099609375}
\def\EPVOUDiagonalMinMinKey{16069}
\def\EPVOUDiagonalMinStdDevFloat{1.19637811183929443359375}
\def\EPVOUDiagonalStdDevLen{151}
\def\EPVOUDiagonalStdDevMaxFloat{12.2696933746337890625}
\def\EPVOUDiagonalStdDevMaxKey{10248}
\def\EPVOUDiagonalStdDevMeanFloat{9.0230007171630859375}
\def\EPVOUDiagonalStdDevMeanKey{19917}
\def\EPVOUDiagonalStdDevMedianFloat{6.7908904552459716796875}
\def\EPVOUDiagonalStdDevMedianKey{1490}
\def\EPVOUDiagonalStdDevMinFloat{6.423083782196044921875}
\def\EPVOUDiagonalStdDevMinKey{15622}
\def\EPVOUDiagonalStdDevStdDevFloat{0.811513245105743408203125}
\def\EPVOUInputsWithCopyingFailureLenLen{151}
\def\EPVOUInputsWithCopyingFailureLenMaxFloat{53}
\def\EPVOUInputsWithCopyingFailureLenMaxKey{19917}
\def\EPVOUInputsWithCopyingFailureLenMeanFloat{45.5695364238410576263049733825027942657470703125}
\def\EPVOUInputsWithCopyingFailureLenMeanKey{123}
\def\EPVOUInputsWithCopyingFailureLenMedianFloat{42}
\def\EPVOUInputsWithCopyingFailureLenMedianKey{104}
\def\EPVOUInputsWithCopyingFailureLenMinFloat{42}
\def\EPVOUInputsWithCopyingFailureLenMinKey{104}
\def\EPVOUInputsWithCopyingFailureLenStdDevFloat{2.024714627181071424644187572994269430637359619140625}
\def\EPVOUInputsWithCopyingFailureMaxLen{151}
\def\EPVOUInputsWithCopyingFailureMaxMaxFloat{61}
\def\EPVOUInputsWithCopyingFailureMaxMaxKey{15622}
\def\EPVOUInputsWithCopyingFailureMaxMeanFloat{46.20529801324503438308965996839106082916259765625}
\def\EPVOUInputsWithCopyingFailureMaxMeanKey{1283}
\def\EPVOUInputsWithCopyingFailureMaxMedianFloat{41}
\def\EPVOUInputsWithCopyingFailureMaxMedianKey{104}
\def\EPVOUInputsWithCopyingFailureMaxMinFloat{41}
\def\EPVOUInputsWithCopyingFailureMaxMinKey{104}
\def\EPVOUInputsWithCopyingFailureMaxStdDevFloat{3.51970400771379932081117658526636660099029541015625}
\def\EPVOUInputsWithCopyingFailureMeanLen{151}
\def\EPVOUInputsWithCopyingFailureMeanMaxFloat{26}
\def\EPVOUInputsWithCopyingFailureMeanMaxKey{19917}
\def\EPVOUInputsWithCopyingFailureMeanMeanFloat{22.334627917051410150861556758172810077667236328125}
\def\EPVOUInputsWithCopyingFailureMeanMeanKey{8745}
\def\EPVOUInputsWithCopyingFailureMeanMedianFloat{20.5}
\def\EPVOUInputsWithCopyingFailureMeanMedianKey{104}
\def\EPVOUInputsWithCopyingFailureMeanMinFloat{20.5}
\def\EPVOUInputsWithCopyingFailureMeanMinKey{104}
\def\EPVOUInputsWithCopyingFailureMeanStdDevFloat{1.0308164299577009526132087557925842702388763427734375}
\def\EPVOUInputsWithCopyingFailureMedianLen{151}
\def\EPVOUInputsWithCopyingFailureMedianMaxFloat{0.2600000000000000088817841970012523233890533447265625}
\def\EPVOUInputsWithCopyingFailureMedianMaxKey{19917}
\def\EPVOUInputsWithCopyingFailureMedianMeanFloat{0.2228476821192053314302228272936190478503704071044921875}
\def\EPVOUInputsWithCopyingFailureMedianMeanKey{123}
\def\EPVOUInputsWithCopyingFailureMedianMedianFloat{0.205000000000000015543122344752191565930843353271484375}
\def\EPVOUInputsWithCopyingFailureMedianMedianKey{104}
\def\EPVOUInputsWithCopyingFailureMedianMinFloat{0.205000000000000015543122344752191565930843353271484375}
\def\EPVOUInputsWithCopyingFailureMedianMinKey{104}
\def\EPVOUInputsWithCopyingFailureMedianStdDevFloat{0.010123573135905360176334255584151833318173885345458984375}
\def\EPVOUInputsWithCopyingFailureMinLen{151}
\def\EPVOUInputsWithCopyingFailureMinMaxFloat{0}
\def\EPVOUInputsWithCopyingFailureMinMaxKey{50}
\def\EPVOUInputsWithCopyingFailureMinMeanFloat{0}
\def\EPVOUInputsWithCopyingFailureMinMeanKey{50}
\def\EPVOUInputsWithCopyingFailureMinMedianFloat{0}
\def\EPVOUInputsWithCopyingFailureMinMedianKey{50}
\def\EPVOUInputsWithCopyingFailureMinMinFloat{0}
\def\EPVOUInputsWithCopyingFailureMinMinKey{50}
\def\EPVOUInputsWithCopyingFailureMinStdDevFloat{0}
\def\EPVOUInputsWithCopyingFailureStdDevLen{151}
\def\EPVOUInputsWithCopyingFailureStdDevMaxFloat{15.297058540778355251177345053292810916900634765625}
\def\EPVOUInputsWithCopyingFailureStdDevMaxKey{19917}
\def\EPVOUInputsWithCopyingFailureStdDevMeanFloat{13.241543890390314430760554387234151363372802734375}
\def\EPVOUInputsWithCopyingFailureStdDevMeanKey{123}
\def\EPVOUInputsWithCopyingFailureStdDevMedianFloat{12.1209185570511390750425562146119773387908935546875}
\def\EPVOUInputsWithCopyingFailureStdDevMedianKey{104}
\def\EPVOUInputsWithCopyingFailureStdDevMinFloat{12.1209185570511390750425562146119773387908935546875}
\def\EPVOUInputsWithCopyingFailureStdDevMinKey{104}
\def\EPVOUInputsWithCopyingFailureStdDevStdDevFloat{0.62928716956718389052838347197393886744976043701171875}
\def\EPVOULenLen{151}
\def\EPVOULenMaxFloat{4096}
\def\EPVOULenMaxKey{50}
\def\EPVOULenMeanFloat{4096}
\def\EPVOULenMeanKey{50}
\def\EPVOULenMedianFloat{4096}
\def\EPVOULenMedianKey{50}
\def\EPVOULenMinFloat{4096}
\def\EPVOULenMinKey{50}
\def\EPVOULenStdDevFloat{0}
\def\EPVOUMaxAboveDiagLenLen{151}
\def\EPVOUMaxAboveDiagLenMaxFloat{64}
\def\EPVOUMaxAboveDiagLenMaxKey{50}
\def\EPVOUMaxAboveDiagLenMeanFloat{64}
\def\EPVOUMaxAboveDiagLenMeanKey{50}
\def\EPVOUMaxAboveDiagLenMedianFloat{64}
\def\EPVOUMaxAboveDiagLenMedianKey{50}
\def\EPVOUMaxAboveDiagLenMinFloat{64}
\def\EPVOUMaxAboveDiagLenMinKey{50}
\def\EPVOUMaxAboveDiagLenStdDevFloat{0}
\def\EPVOUMaxAboveDiagMaxLen{151}
\def\EPVOUMaxAboveDiagMaxMaxFloat{28.4637908935546875}
\def\EPVOUMaxAboveDiagMaxMaxKey{15622}
\def\EPVOUMaxAboveDiagMaxMeanFloat{10.8519802093505859375}
\def\EPVOUMaxAboveDiagMaxMeanKey{20539}
\def\EPVOUMaxAboveDiagMaxMedianFloat{7.424126148223876953125}
\def\EPVOUMaxAboveDiagMaxMedianKey{14095}
\def\EPVOUMaxAboveDiagMaxMinFloat{7.173371791839599609375}
\def\EPVOUMaxAboveDiagMaxMinKey{8048}
\def\EPVOUMaxAboveDiagMaxStdDevFloat{2.2125437259674072265625}
\def\EPVOUMaxAboveDiagMeanLen{151}
\def\EPVOUMaxAboveDiagMeanMaxFloat{4.5374927520751953125}
\def\EPVOUMaxAboveDiagMeanMaxKey{15622}
\def\EPVOUMaxAboveDiagMeanMeanFloat{2.24474239349365234375}
\def\EPVOUMaxAboveDiagMeanMeanKey{3254}
\def\EPVOUMaxAboveDiagMeanMedianFloat{0.69272957742214202880859375}
\def\EPVOUMaxAboveDiagMeanMedianKey{14095}
\def\EPVOUMaxAboveDiagMeanMinFloat{0.572075903415679931640625}
\def\EPVOUMaxAboveDiagMeanMinKey{18146}
\def\EPVOUMaxAboveDiagMeanStdDevFloat{0.751639306545257568359375}
\def\EPVOUMaxAboveDiagMedianLen{151}
\def\EPVOUMaxAboveDiagMedianMaxFloat{-10.601028223037719300236858543939888477325439453125}
\def\EPVOUMaxAboveDiagMedianMaxKey{12457}
\def\EPVOUMaxAboveDiagMedianMeanFloat{-12.2175432442355624829133375897072255611419677734375}
\def\EPVOUMaxAboveDiagMedianMeanKey{20013}
\def\EPVOUMaxAboveDiagMedianMedianFloat{-14.3014197444915769352746792719699442386627197265625}
\def\EPVOUMaxAboveDiagMedianMedianKey{1283}
\def\EPVOUMaxAboveDiagMedianMinFloat{-15.1539766883850095524621792719699442386627197265625}
\def\EPVOUMaxAboveDiagMedianMinKey{13036}
\def\EPVOUMaxAboveDiagMedianStdDevFloat{0.68210705589727094189100853327545337378978729248046875}
\def\EPVOUMaxAboveDiagMinLen{151}
\def\EPVOUMaxAboveDiagMinMaxFloat{-10.7197017669677734375}
\def\EPVOUMaxAboveDiagMinMaxKey{12457}
\def\EPVOUMaxAboveDiagMinMeanFloat{-12.446903228759765625}
\def\EPVOUMaxAboveDiagMinMeanKey{24173}
\def\EPVOUMaxAboveDiagMinMedianFloat{-15.63669586181640625}
\def\EPVOUMaxAboveDiagMinMedianKey{20415}
\def\EPVOUMaxAboveDiagMinMinFloat{-16.245235443115234375}
\def\EPVOUMaxAboveDiagMinMinKey{13036}
\def\EPVOUMaxAboveDiagMinStdDevFloat{0.856358706951141357421875}
\def\EPVOUMaxAboveDiagStdDevLen{151}
\def\EPVOUMaxAboveDiagStdDevMaxFloat{8.21490573883056640625}
\def\EPVOUMaxAboveDiagStdDevMaxKey{16149}
\def\EPVOUMaxAboveDiagStdDevMeanFloat{6.706093311309814453125}
\def\EPVOUMaxAboveDiagStdDevMeanKey{28090}
\def\EPVOUMaxAboveDiagStdDevMedianFloat{4.8679916858673095703125}
\def\EPVOUMaxAboveDiagStdDevMedianKey{19538}
\def\EPVOUMaxAboveDiagStdDevMinFloat{4.589704990386962890625}
\def\EPVOUMaxAboveDiagStdDevMinKey{1490}
\def\EPVOUMaxAboveDiagStdDevStdDevFloat{0.63427507877349853515625}
\def\EPVOUMaxLen{151}
\def\EPVOUMaxMaxFloat{43.05789947509765625}
\def\EPVOUMaxMaxKey{10248}
\def\EPVOUMaxMeanFloat{34.0606689453125}
\def\EPVOUMaxMeanKey{20338}
\def\EPVOUMaxMedianFloat{26.741374492645263671875}
\def\EPVOUMaxMedianKey{11130}
\def\EPVOUMaxMinFloat{26.4571475982666015625}
\def\EPVOUMaxMinKey{1490}
\def\EPVOUMaxRowDiffLenLen{151}
\def\EPVOUMaxRowDiffLenMaxFloat{64}
\def\EPVOUMaxRowDiffLenMaxKey{50}
\def\EPVOUMaxRowDiffLenMeanFloat{64}
\def\EPVOUMaxRowDiffLenMeanKey{50}
\def\EPVOUMaxRowDiffLenMedianFloat{64}
\def\EPVOUMaxRowDiffLenMedianKey{50}
\def\EPVOUMaxRowDiffLenMinFloat{64}
\def\EPVOUMaxRowDiffLenMinKey{50}
\def\EPVOUMaxRowDiffLenStdDevFloat{0}
\def\EPVOUMaxRowDiffMaxLen{151}
\def\EPVOUMaxRowDiffMaxMaxFloat{82.2288665771484375}
\def\EPVOUMaxRowDiffMaxMaxKey{10248}
\def\EPVOUMaxRowDiffMaxMeanFloat{60.756946563720703125}
\def\EPVOUMaxRowDiffMaxMeanKey{1696}
\def\EPVOUMaxRowDiffMaxMedianFloat{44.39314556121826171875}
\def\EPVOUMaxRowDiffMaxMedianKey{11130}
\def\EPVOUMaxRowDiffMaxMinFloat{43.65570831298828125}
\def\EPVOUMaxRowDiffMaxMinKey{1490}
\def\EPVOUMaxRowDiffMaxStdDevFloat{7.0580463409423828125}
\def\EPVOUMaxRowDiffMeanLen{151}
\def\EPVOUMaxRowDiffMeanMaxFloat{34.98807525634765625}
\def\EPVOUMaxRowDiffMeanMaxKey{9504}
\def\EPVOUMaxRowDiffMeanMeanFloat{23.212398529052734375}
\def\EPVOUMaxRowDiffMeanMeanKey{6204}
\def\EPVOUMaxRowDiffMeanMedianFloat{14.6804687976837158203125}
\def\EPVOUMaxRowDiffMeanMedianKey{30371}
\def\EPVOUMaxRowDiffMeanMinFloat{13.45380878448486328125}
\def\EPVOUMaxRowDiffMeanMinKey{1490}
\def\EPVOUMaxRowDiffMeanStdDevFloat{3.8722012042999267578125}
\def\EPVOUMaxRowDiffMedianLen{151}
\def\EPVOUMaxRowDiffMedianMaxFloat{24.81705515861511202047040569595992565155029296875}
\def\EPVOUMaxRowDiffMedianMaxKey{9504}
\def\EPVOUMaxRowDiffMedianMeanFloat{11.4404782983167283560987925739027559757232666015625}
\def\EPVOUMaxRowDiffMedianMeanKey{6204}
\def\EPVOUMaxRowDiffMedianMedianFloat{4.273184958696365498553859652020037174224853515625}
\def\EPVOUMaxRowDiffMedianMedianKey{30371}
\def\EPVOUMaxRowDiffMedianMinFloat{3.811435463428497261162419817992486059665679931640625}
\def\EPVOUMaxRowDiffMedianMinKey{18668}
\def\EPVOUMaxRowDiffMedianStdDevFloat{4.2407541732733680106548490584827959537506103515625}
\def\EPVOUMaxRowDiffMinLen{151}
\def\EPVOUMaxRowDiffMinMaxFloat{24.8167781829833984375}
\def\EPVOUMaxRowDiffMinMaxKey{9504}
\def\EPVOUMaxRowDiffMinMeanFloat{11.10178089141845703125}
\def\EPVOUMaxRowDiffMinMeanKey{13293}
\def\EPVOUMaxRowDiffMinMedianFloat{3.76746237277984619140625}
\def\EPVOUMaxRowDiffMinMedianKey{18668}
\def\EPVOUMaxRowDiffMinMinFloat{3.714051723480224609375}
\def\EPVOUMaxRowDiffMinMinKey{8048}
\def\EPVOUMaxRowDiffMinStdDevFloat{4.27737331390380859375}
\def\EPVOUMaxRowDiffStdDevLen{151}
\def\EPVOUMaxRowDiffStdDevMaxFloat{17.6280956268310546875}
\def\EPVOUMaxRowDiffStdDevMaxKey{10248}
\def\EPVOUMaxRowDiffStdDevMeanFloat{10.623790740966796875}
\def\EPVOUMaxRowDiffStdDevMeanKey{4305}
\def\EPVOUMaxRowDiffStdDevMedianFloat{7.07623565196990966796875}
\def\EPVOUMaxRowDiffStdDevMedianKey{15622}
\def\EPVOUMaxRowDiffStdDevMinFloat{7.0078983306884765625}
\def\EPVOUMaxRowDiffStdDevMinKey{27671}
\def\EPVOUMaxRowDiffStdDevStdDevFloat{1.6677820682525634765625}
\def\EPVOUMaxStdDevFloat{3.395696163177490234375}
\def\EPVOUMeanLen{151}
\def\EPVOUMeanMaxFloat{2.35429668426513671875}
\def\EPVOUMeanMaxKey{16149}
\def\EPVOUMeanMeanFloat{0.4405307471752166748046875}
\def\EPVOUMeanMeanKey{16197}
\def\EPVOUMeanMedianFloat{-0.843249619007110595703125}
\def\EPVOUMeanMedianKey{1490}
\def\EPVOUMeanMinFloat{-0.864755928516387939453125}
\def\EPVOUMeanMinKey{11611}
\def\EPVOUMeanStdDevFloat{0.60309708118438720703125}
\def\EPVOUMedianLen{151}
\def\EPVOUMedianMaxFloat{-12.06594407558441162109375}
\def\EPVOUMedianMaxKey{30371}
\def\EPVOUMedianMeanFloat{-17.69009461418682604971763794310390949249267578125}
\def\EPVOUMedianMeanKey{28090}
\def\EPVOUMedianMedianFloat{-23.029167902469634299222889239899814128875732421875}
\def\EPVOUMedianMedianKey{20976}
\def\EPVOUMedianMinFloat{-23.176358985900879616792735760100185871124267578125}
\def\EPVOUMedianMinKey{6910}
\def\EPVOUMedianStdDevFloat{2.3294404278093967519680518307723104953765869140625}
\def\EPVOUMinLen{151}
\def\EPVOUMinMaxFloat{-17.1985950469970703125}
\def\EPVOUMinMaxKey{6159}
\def\EPVOUMinMeanFloat{-27.5607013702392578125}
\def\EPVOUMinMeanKey{13468}
\def\EPVOUMinMedianFloat{-39.6673679351806640625}
\def\EPVOUMinMedianKey{3175}
\def\EPVOUMinMinFloat{-40.74575042724609375}
\def\EPVOUMinMinKey{23633}
\def\EPVOUMinStdDevFloat{4.26828098297119140625}
\def\EPVOUOffDiagonalAbsLenLen{151}
\def\EPVOUOffDiagonalAbsLenMaxFloat{4032}
\def\EPVOUOffDiagonalAbsLenMaxKey{50}
\def\EPVOUOffDiagonalAbsLenMeanFloat{4032}
\def\EPVOUOffDiagonalAbsLenMeanKey{50}
\def\EPVOUOffDiagonalAbsLenMedianFloat{4032}
\def\EPVOUOffDiagonalAbsLenMedianKey{50}
\def\EPVOUOffDiagonalAbsLenMinFloat{4032}
\def\EPVOUOffDiagonalAbsLenMinKey{50}
\def\EPVOUOffDiagonalAbsLenStdDevFloat{0}
\def\EPVOUOffDiagonalAbsMaxLen{151}
\def\EPVOUOffDiagonalAbsMaxMaxFloat{40.74575042724609375}
\def\EPVOUOffDiagonalAbsMaxMaxKey{23633}
\def\EPVOUOffDiagonalAbsMaxMeanFloat{27.6741619110107421875}
\def\EPVOUOffDiagonalAbsMaxMeanKey{15622}
\def\EPVOUOffDiagonalAbsMaxMedianFloat{19.070469379425048828125}
\def\EPVOUOffDiagonalAbsMaxMedianKey{5615}
\def\EPVOUOffDiagonalAbsMaxMinFloat{18.9504852294921875}
\def\EPVOUOffDiagonalAbsMaxMinKey{6159}
\def\EPVOUOffDiagonalAbsMaxStdDevFloat{4.11807918548583984375}
\def\EPVOUOffDiagonalAbsMeanLen{151}
\def\EPVOUOffDiagonalAbsMeanMaxFloat{6.79676342010498046875}
\def\EPVOUOffDiagonalAbsMeanMaxKey{20976}
\def\EPVOUOffDiagonalAbsMeanMeanFloat{4.02946186065673828125}
\def\EPVOUOffDiagonalAbsMeanMeanKey{23367}
\def\EPVOUOffDiagonalAbsMeanMedianFloat{2.464410960674285888671875}
\def\EPVOUOffDiagonalAbsMeanMedianKey{18668}
\def\EPVOUOffDiagonalAbsMeanMinFloat{2.431762218475341796875}
\def\EPVOUOffDiagonalAbsMeanMinKey{30371}
\def\EPVOUOffDiagonalAbsMeanStdDevFloat{0.918423354625701904296875}
\def\EPVOUOffDiagonalAbsMedianLen{151}
\def\EPVOUOffDiagonalAbsMedianMaxFloat{0.2066276952624321039397869981257827021181583404541015625}
\def\EPVOUOffDiagonalAbsMedianMaxKey{20976}
\def\EPVOUOffDiagonalAbsMedianMeanFloat{0.04221465277362194956634056097755092196166515350341796875}
\def\EPVOUOffDiagonalAbsMedianMeanKey{11498}
\def\EPVOUOffDiagonalAbsMedianMedianFloat{0.00836586244404315983180797644536141888238489627838134765625}
\def\EPVOUOffDiagonalAbsMedianMedianKey{30371}
\def\EPVOUOffDiagonalAbsMedianMinFloat{0.0082989746332168580489341280781445675529539585113525390625}
\def\EPVOUOffDiagonalAbsMedianMinKey{2306}
\def\EPVOUOffDiagonalAbsMedianStdDevFloat{0.03424134182700655504305586873670108616352081298828125}
\def\EPVOUOffDiagonalAbsMinLen{151}
\def\EPVOUOffDiagonalAbsMinMaxFloat{0.0299930572509765625}
\def\EPVOUOffDiagonalAbsMinMaxKey{2345}
\def\EPVOUOffDiagonalAbsMinMeanFloat{0.00193050992675125598907470703125}
\def\EPVOUOffDiagonalAbsMinMeanKey{3254}
\def\EPVOUOffDiagonalAbsMinMedianFloat{0.0000099837779998779296875}
\def\EPVOUOffDiagonalAbsMinMedianKey{11124}
\def\EPVOUOffDiagonalAbsMinMinFloat{0.00000274181365966796875}
\def\EPVOUOffDiagonalAbsMinMinKey{18668}
\def\EPVOUOffDiagonalAbsMinStdDevFloat{0.00327019952237606048583984375}
\def\EPVOUOffDiagonalAbsStdDevLen{151}
\def\EPVOUOffDiagonalAbsStdDevMaxFloat{4.568195819854736328125}
\def\EPVOUOffDiagonalAbsStdDevMaxKey{27484}
\def\EPVOUOffDiagonalAbsStdDevMeanFloat{3.5878849029541015625}
\def\EPVOUOffDiagonalAbsStdDevMeanKey{20754}
\def\EPVOUOffDiagonalAbsStdDevMedianFloat{2.73565208911895751953125}
\def\EPVOUOffDiagonalAbsStdDevMedianKey{24144}
\def\EPVOUOffDiagonalAbsStdDevMinFloat{2.528723239898681640625}
\def\EPVOUOffDiagonalAbsStdDevMinKey{1490}
\def\EPVOUOffDiagonalAbsStdDevStdDevFloat{0.390653192996978759765625}
\def\EPVOUOffDiagonalLenLen{151}
\def\EPVOUOffDiagonalLenMaxFloat{4032}
\def\EPVOUOffDiagonalLenMaxKey{50}
\def\EPVOUOffDiagonalLenMeanFloat{4032}
\def\EPVOUOffDiagonalLenMeanKey{50}
\def\EPVOUOffDiagonalLenMedianFloat{4032}
\def\EPVOUOffDiagonalLenMedianKey{50}
\def\EPVOUOffDiagonalLenMinFloat{4032}
\def\EPVOUOffDiagonalLenMinKey{50}
\def\EPVOUOffDiagonalLenStdDevFloat{0}
\def\EPVOUOffDiagonalMaxLen{151}
\def\EPVOUOffDiagonalMaxMaxFloat{31.6836795806884765625}
\def\EPVOUOffDiagonalMaxMaxKey{10248}
\def\EPVOUOffDiagonalMaxMeanFloat{22.426883697509765625}
\def\EPVOUOffDiagonalMaxMeanKey{28778}
\def\EPVOUOffDiagonalMaxMedianFloat{15.7993414402008056640625}
\def\EPVOUOffDiagonalMaxMedianKey{1490}
\def\EPVOUOffDiagonalMaxMinFloat{14.30925846099853515625}
\def\EPVOUOffDiagonalMaxMinKey{11130}
\def\EPVOUOffDiagonalMaxStdDevFloat{3.1886806488037109375}
\def\EPVOUOffDiagonalMeanLen{151}
\def\EPVOUOffDiagonalMeanMaxFloat{2.221670627593994140625}
\def\EPVOUOffDiagonalMeanMaxKey{16149}
\def\EPVOUOffDiagonalMeanMeanFloat{0.328286111354827880859375}
\def\EPVOUOffDiagonalMeanMeanKey{1696}
\def\EPVOUOffDiagonalMeanMedianFloat{-0.9135603010654449462890625}
\def\EPVOUOffDiagonalMeanMedianKey{1490}
\def\EPVOUOffDiagonalMeanMinFloat{-0.96881711483001708984375}
\def\EPVOUOffDiagonalMeanMinKey{11611}
\def\EPVOUOffDiagonalMeanStdDevFloat{0.59375607967376708984375}
\def\EPVOUOffDiagonalMedianLen{151}
\def\EPVOUOffDiagonalMedianMaxFloat{-12.0931520223617550158223821199499070644378662109375}
\def\EPVOUOffDiagonalMedianMaxKey{30371}
\def\EPVOUOffDiagonalMedianMeanFloat{-17.7478174349488000416386057622730731964111328125}
\def\EPVOUOffDiagonalMedianMeanKey{20415}
\def\EPVOUOffDiagonalMedianMedianFloat{-23.110814783573150776874172152020037174224853515625}
\def\EPVOUOffDiagonalMedianMedianKey{20976}
\def\EPVOUOffDiagonalMedianMinFloat{-23.20035556793212805359871708787977695465087890625}
\def\EPVOUOffDiagonalMedianMinKey{6910}
\def\EPVOUOffDiagonalMedianStdDevFloat{2.3412199217601692424750581267289817333221435546875}
\def\EPVOUOffDiagonalMinLen{151}
\def\EPVOUOffDiagonalMinMaxFloat{-17.1985950469970703125}
\def\EPVOUOffDiagonalMinMaxKey{6159}
\def\EPVOUOffDiagonalMinMeanFloat{-27.5607013702392578125}
\def\EPVOUOffDiagonalMinMeanKey{13468}
\def\EPVOUOffDiagonalMinMedianFloat{-39.6673679351806640625}
\def\EPVOUOffDiagonalMinMedianKey{3175}
\def\EPVOUOffDiagonalMinMinFloat{-40.74575042724609375}
\def\EPVOUOffDiagonalMinMinKey{23633}
\def\EPVOUOffDiagonalMinStdDevFloat{4.26828098297119140625}
\def\EPVOUOffDiagonalStdDevLen{151}
\def\EPVOUOffDiagonalStdDevMaxFloat{7.95101165771484375}
\def\EPVOUOffDiagonalStdDevMaxKey{9504}
\def\EPVOUOffDiagonalStdDevMeanFloat{5.372986316680908203125}
\def\EPVOUOffDiagonalStdDevMeanKey{19488}
\def\EPVOUOffDiagonalStdDevMedianFloat{3.61388289928436279296875}
\def\EPVOUOffDiagonalStdDevMedianKey{30371}
\def\EPVOUOffDiagonalStdDevMinFloat{3.4709565639495849609375}
\def\EPVOUOffDiagonalStdDevMinKey{1490}
\def\EPVOUOffDiagonalStdDevStdDevFloat{0.881070792675018310546875}
\def\EPVOUStdDevLen{151}
\def\EPVOUStdDevMaxFloat{8.04164791107177734375}
\def\EPVOUStdDevMaxKey{9504}
\def\EPVOUStdDevMeanFloat{5.525171756744384765625}
\def\EPVOUStdDevMeanKey{19488}
\def\EPVOUStdDevMedianFloat{3.7877357006072998046875}
\def\EPVOUStdDevMedianKey{30371}
\def\EPVOUStdDevMinFloat{3.581322193145751953125}
\def\EPVOUStdDevMinKey{1490}
\def\EPVOUStdDevStdDevFloat{0.86206734180450439453125}
\def\EQKEErrBoundMaxDiffExactLen{151}
\def\EQKEErrBoundMaxDiffExactMaxFloat{3.039496898651123046875}
\def\EQKEErrBoundMaxDiffExactMaxKey{12457}
\def\EQKEErrBoundMaxDiffExactMeanFloat{1.60029869087484488687778139137662947177886962890625}
\def\EQKEErrBoundMaxDiffExactMeanKey{18289}
\def\EQKEErrBoundMaxDiffExactMedianFloat{0.9556983411312103271484375}
\def\EQKEErrBoundMaxDiffExactMedianKey{24202}
\def\EQKEErrBoundMaxDiffExactMinFloat{0.913126051425933837890625}
\def\EQKEErrBoundMaxDiffExactMinKey{23241}
\def\EQKEErrBoundMaxDiffExactStdDevFloat{0.3881257608771504497013893342227675020694732666015625}
\def\EQKEErrBoundMaxDiffLen{151}
\def\EQKEErrBoundMaxDiffMaxFloat{6.37592983245849609375}
\def\EQKEErrBoundMaxDiffMaxKey{1681}
\def\EQKEErrBoundMaxDiffMeanFloat{4.71346826269137153531119110994040966033935546875}
\def\EQKEErrBoundMaxDiffMeanKey{17096}
\def\EQKEErrBoundMaxDiffMedianFloat{3.6314566135406494140625}
\def\EQKEErrBoundMaxDiffMedianKey{8840}
\def\EQKEErrBoundMaxDiffMinFloat{3.5355336666107177734375}
\def\EQKEErrBoundMaxDiffMinKey{13468}
\def\EQKEErrBoundMaxDiffStdDevFloat{0.542659408063155268564514699392020702362060546875}
\def\EQKEErrBoundMaxDiffSubproductLen{151}
\def\EQKEErrBoundMaxDiffSubproductMaxFloat{6.37592983245849609375}
\def\EQKEErrBoundMaxDiffSubproductMaxKey{1681}
\def\EQKEErrBoundMaxDiffSubproductMeanFloat{4.71346826269137153531119110994040966033935546875}
\def\EQKEErrBoundMaxDiffSubproductMeanKey{17096}
\def\EQKEErrBoundMaxDiffSubproductMedianFloat{3.6314566135406494140625}
\def\EQKEErrBoundMaxDiffSubproductMedianKey{8840}
\def\EQKEErrBoundMaxDiffSubproductMinFloat{3.5355336666107177734375}
\def\EQKEErrBoundMaxDiffSubproductMinKey{13468}
\def\EQKEErrBoundMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMaxFloat{130.0746917724609375}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMaxKey{1490}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMeanFloat{94.1853701357809853789149201475083827972412109375}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMeanKey{26932}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMedianFloat{77.2502727508544921875}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMedianKey{4729}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMinFloat{72.31154632568359375}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMinKey{13468}
\def\EQKEErrBoundMaxDiffSubproductRecursiveStdDevFloat{9.0252993067812550265216486877761781215667724609375}
\def\EQKEErrBoundMaxDiffSubproductStdDevFloat{0.542659408063155268564514699392020702362060546875}
\def\EQKEErrBoundMeanMaxDiffLen{151}
\def\EQKEErrBoundMeanMaxDiffMaxFloat{6.43523406982421875}
\def\EQKEErrBoundMeanMaxDiffMaxKey{1681}
\def\EQKEErrBoundMeanMaxDiffMeanFloat{4.72528035593348594289864195161499083042144775390625}
\def\EQKEErrBoundMeanMaxDiffMeanKey{22286}
\def\EQKEErrBoundMeanMaxDiffMedianFloat{3.649292647838592529296875}
\def\EQKEErrBoundMeanMaxDiffMedianKey{8840}
\def\EQKEErrBoundMeanMaxDiffMinFloat{3.543451786041259765625}
\def\EQKEErrBoundMeanMaxDiffMinKey{13468}
\def\EQKEErrBoundMeanMaxDiffStdDevFloat{0.5437849392883042920487923765904270112514495849609375}
\def\EQKEErrBoundMeanMaxDiffSubproductLen{151}
\def\EQKEErrBoundMeanMaxDiffSubproductMaxFloat{6.43523406982421875}
\def\EQKEErrBoundMeanMaxDiffSubproductMaxKey{1681}
\def\EQKEErrBoundMeanMaxDiffSubproductMeanFloat{4.72528035593348594289864195161499083042144775390625}
\def\EQKEErrBoundMeanMaxDiffSubproductMeanKey{22286}
\def\EQKEErrBoundMeanMaxDiffSubproductMedianFloat{3.649292647838592529296875}
\def\EQKEErrBoundMeanMaxDiffSubproductMedianKey{8840}
\def\EQKEErrBoundMeanMaxDiffSubproductMinFloat{3.543451786041259765625}
\def\EQKEErrBoundMeanMaxDiffSubproductMinKey{13468}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMaxFloat{132.0067138671875}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMaxKey{1490}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMeanFloat{94.214263916015625}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMeanKey{29725}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMedianFloat{77.3510417938232421875}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMedianKey{1895}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMinFloat{72.464385986328125}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMinKey{13468}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveStdDevFloat{9.1318176253022738109166311915032565593719482421875}
\def\EQKEErrBoundMeanMaxDiffSubproductStdDevFloat{0.5437849392883042920487923765904270112514495849609375}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMaxFloat{133.0085601806640625}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMaxKey{1490}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMeanFloat{96.1410164233075050788102089427411556243896484375}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMeanKey{20976}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMedianFloat{78.9849071502685546875}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMedianKey{1895}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMinFloat{74.71254730224609375}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMinKey{13468}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveStdDevFloat{9.355409921102602055498209665529429912567138671875}
\def\EQKEErrBoundSvdLen{151}
\def\EQKEErrBoundSvdMaxFloat{12.87032032012939453125}
\def\EQKEErrBoundSvdMaxKey{27714}
\def\EQKEErrBoundSvdMeanFloat{6.36201049476269897553493137820623815059661865234375}
\def\EQKEErrBoundSvdMeanKey{29195}
\def\EQKEErrBoundSvdMedianFloat{4.5378496646881103515625}
\def\EQKEErrBoundSvdMedianKey{15399}
\def\EQKEErrBoundSvdMinFloat{4.383276462554931640625}
\def\EQKEErrBoundSvdMinKey{20013}
\def\EQKEErrBoundSvdStdDevFloat{1.1900315185613521418162008558283559978008270263671875}
\def\EQKEErrFirstSingularLen{151}
\def\EQKEErrFirstSingularMaxFloat{9.10069179534912109375}
\def\EQKEErrFirstSingularMaxKey{27714}
\def\EQKEErrFirstSingularMeanFloat{4.49862123956743431563154445029795169830322265625}
\def\EQKEErrFirstSingularMeanKey{29195}
\def\EQKEErrFirstSingularMedianFloat{3.20874607563018798828125}
\def\EQKEErrFirstSingularMedianKey{15399}
\def\EQKEErrFirstSingularMinFloat{3.09944820404052734375}
\def\EQKEErrFirstSingularMinKey{20013}
\def\EQKEErrFirstSingularSqrtTwoLen{151}
\def\EQKEErrFirstSingularSqrtTwoMaxFloat{12.8703212738037109375}
\def\EQKEErrFirstSingularSqrtTwoMaxKey{27714}
\def\EQKEErrFirstSingularSqrtTwoMeanFloat{6.36201107265144027991254915832541882991790771484375}
\def\EQKEErrFirstSingularSqrtTwoMeanKey{29195}
\def\EQKEErrFirstSingularSqrtTwoMedianFloat{4.5378520488739013671875}
\def\EQKEErrFirstSingularSqrtTwoMedianKey{15399}
\def\EQKEErrFirstSingularSqrtTwoMinFloat{4.383281707763671875}
\def\EQKEErrFirstSingularSqrtTwoMinKey{20013}
\def\EQKEErrFirstSingularSqrtTwoStdDevFloat{1.1900315196533075567941750705358572304248809814453125}
\def\EQKEErrFirstSingularStdDevFloat{0.84147936205844187096403175019077025353908538818359375}
\def\EQKEErrFroNormLen{151}
\def\EQKEErrFroNormMaxFloat{10.6649570465087890625}
\def\EQKEErrFroNormMaxKey{27714}
\def\EQKEErrFroNormMeanFloat{7.14334223601991791241516693844459950923919677734375}
\def\EQKEErrFroNormMeanKey{14929}
\def\EQKEErrFroNormMedianFloat{5.96014559268951416015625}
\def\EQKEErrFroNormMedianKey{8893}
\def\EQKEErrFroNormMinFloat{5.88724422454833984375}
\def\EQKEErrFroNormMinKey{29052}
\def\EQKEErrFroNormSqrtTwoLen{151}
\def\EQKEErrFroNormSqrtTwoMaxFloat{15.08252620697021484375}
\def\EQKEErrFroNormSqrtTwoMaxKey{27714}
\def\EQKEErrFroNormSqrtTwoMeanFloat{10.1022112637955618907881216728128492832183837890625}
\def\EQKEErrFroNormSqrtTwoMeanKey{14929}
\def\EQKEErrFroNormSqrtTwoMedianFloat{8.4289186000823974609375}
\def\EQKEErrFroNormSqrtTwoMedianKey{8893}
\def\EQKEErrFroNormSqrtTwoMinFloat{8.3258209228515625}
\def\EQKEErrFroNormSqrtTwoMinKey{29052}
\def\EQKEErrFroNormSqrtTwoStdDevFloat{1.038153383584633271397024145699106156826019287109375}
\def\EQKEErrFroNormStdDevFloat{0.7340853009551204788607492446317337453365325927734375}
\def\EQKEErrLen{4096}
\def\EQKEErrMaxAbsLen{151}
\def\EQKEErrMaxAbsMaxFloat{1.8155534267425537109375}
\def\EQKEErrMaxAbsMaxKey{12457}
\def\EQKEErrMaxAbsMeanFloat{0.901712957202204012929769305628724396228790283203125}
\def\EQKEErrMaxAbsMeanKey{12493}
\def\EQKEErrMaxAbsMedianFloat{0.56436114013195037841796875}
\def\EQKEErrMaxAbsMedianKey{32103}
\def\EQKEErrMaxAbsMinFloat{0.561043918132781982421875}
\def\EQKEErrMaxAbsMinKey{1412}
\def\EQKEErrMaxAbsStdDevFloat{0.2232369179676742809714795612308080308139324188232421875}
\def\EQKEErrMaxLen{151}
\def\EQKEErrMaxMaxFloat{1.8155534267425537109375}
\def\EQKEErrMaxMaxKey{12457}
\def\EQKEErrMaxMeanFloat{0.848377883434295654296875}
\def\EQKEErrMaxMeanKey{24566}
\def\EQKEErrMaxMedianFloat{0.51669280230998992919921875}
\def\EQKEErrMaxMedianKey{32103}
\def\EQKEErrMaxMinFloat{0.51148784160614013671875}
\def\EQKEErrMaxMinKey{32374}
\def\EQKEErrMaxRowDiffLen{151}
\def\EQKEErrMaxRowDiffMaxFloat{3.039496898651123046875}
\def\EQKEErrMaxRowDiffMaxKey{12457}
\def\EQKEErrMaxRowDiffMeanFloat{1.60029869087484488687778139137662947177886962890625}
\def\EQKEErrMaxRowDiffMeanKey{18289}
\def\EQKEErrMaxRowDiffMedianFloat{0.9556983411312103271484375}
\def\EQKEErrMaxRowDiffMedianKey{24202}
\def\EQKEErrMaxRowDiffMinFloat{0.913126051425933837890625}
\def\EQKEErrMaxRowDiffMinKey{23241}
\def\EQKEErrMaxRowDiffStdDevFloat{0.3881257608771504497013893342227675020694732666015625}
\def\EQKEErrMaxStdDevFloat{0.2236065566539764404296875}
\def\EQKEErrMeanDimZeroNormLen{151}
\def\EQKEErrMeanDimZeroNormMaxFloat{0.0534259937703609466552734375}
\def\EQKEErrMeanDimZeroNormMaxKey{12457}
\def\EQKEErrMeanDimZeroNormMeanFloat{0.0185644953474649147817654437631063046865165233612060546875}
\def\EQKEErrMeanDimZeroNormMeanKey{17080}
\def\EQKEErrMeanDimZeroNormMedianFloat{0.006496400455944240093231201171875}
\def\EQKEErrMeanDimZeroNormMedianKey{11611}
\def\EQKEErrMeanDimZeroNormMinFloat{0.006293606944382190704345703125}
\def\EQKEErrMeanDimZeroNormMinKey{28778}
\def\EQKEErrMeanDimZeroNormStdDevFloat{0.00809574847955679861855049495034108986146748065948486328125}
\def\EQKEErrMeanLen{151}
\def\EQKEErrMeanMaxFloat{0.00069203344173729419708251953125}
\def\EQKEErrMeanMaxKey{20976}
\def\EQKEErrMeanMeanFloat{0.00000481174492961145006120204925537109375}
\def\EQKEErrMeanMeanKey{7467}
\def\EQKEErrMeanMedianFloat{-0.0004337805221439339220523834228515625}
\def\EQKEErrMeanMedianKey{519}
\def\EQKEErrMeanMinFloat{-0.00055678584612905979156494140625}
\def\EQKEErrMeanMinKey{1681}
\def\EQKEErrMeanStdDevFloat{0.000185640950803644955158233642578125}
\def\EQKEErrMedianLen{151}
\def\EQKEErrMedianMaxFloat{-0.309972257167100917474300558751565404236316680908203125}
\def\EQKEErrMedianMaxKey{4430}
\def\EQKEErrMedianMeanFloat{-0.393768812054829886459828003353322856128215789794921875}
\def\EQKEErrMedianMeanKey{4729}
\def\EQKEErrMedianMedianFloat{-0.61153378151357173919677734375}
\def\EQKEErrMedianMedianKey{8048}
\def\EQKEErrMedianMinFloat{-0.7026398286223412004147803600062616169452667236328125}
\def\EQKEErrMedianMinKey{27714}
\def\EQKEErrMedianStdDevFloat{0.058684328935875183785864095398210338316857814788818359375}
\def\EQKEErrMinLen{151}
\def\EQKEErrMinMaxFloat{-0.53783547878265380859375}
\def\EQKEErrMinMaxKey{23241}
\def\EQKEErrMinMeanFloat{-0.834872424602508544921875}
\def\EQKEErrMinMeanKey{29726}
\def\EQKEErrMinMedianFloat{-1.467702805995941162109375}
\def\EQKEErrMinMedianKey{3284}
\def\EQKEErrMinMinFloat{-1.5506229400634765625}
\def\EQKEErrMinMinKey{23447}
\def\EQKEErrMinStdDevFloat{0.19879297912120819091796875}
\def\EQKEErrProdFirstSingularLen{151}
\def\EQKEErrProdFirstSingularMaxFloat{32.21783885357755394807099946774542331695556640625}
\def\EQKEErrProdFirstSingularMaxKey{23367}
\def\EQKEErrProdFirstSingularMeanFloat{22.170777983306958702769406954757869243621826171875}
\def\EQKEErrProdFirstSingularMeanKey{16069}
\def\EQKEErrProdFirstSingularMedianFloat{16.40603605343367377145114005543291568756103515625}
\def\EQKEErrProdFirstSingularMedianKey{2306}
\def\EQKEErrProdFirstSingularMinFloat{16.241059794367227908651329926215112209320068359375}
\def\EQKEErrProdFirstSingularMinKey{29052}
\def\EQKEErrProdFirstSingularSqrtTwoLen{151}
\def\EQKEErrProdFirstSingularSqrtTwoMaxFloat{45.56290465708023162960671470500528812408447265625}
\def\EQKEErrProdFirstSingularSqrtTwoMaxKey{23367}
\def\EQKEErrProdFirstSingularSqrtTwoMeanFloat{31.35421491235552338139314088039100170135498046875}
\def\EQKEErrProdFirstSingularSqrtTwoMeanKey{16069}
\def\EQKEErrProdFirstSingularSqrtTwoMedianFloat{23.201638691547866955033896374516189098358154296875}
\def\EQKEErrProdFirstSingularSqrtTwoMedianKey{2306}
\def\EQKEErrProdFirstSingularSqrtTwoMinFloat{22.968327028506525522288939100690186023712158203125}
\def\EQKEErrProdFirstSingularSqrtTwoMinKey{29052}
\def\EQKEErrProdFirstSingularSqrtTwoStdDevFloat{3.879954067982376297862856517895124852657318115234375}
\def\EQKEErrProdFirstSingularStdDevFloat{2.74354183216266900302571229985915124416351318359375}
\def\EQKEErrProdFroNormLen{151}
\def\EQKEErrProdFroNormMaxFloat{1287.395390273296698069316335022449493408203125}
\def\EQKEErrProdFroNormMaxKey{29565}
\def\EQKEErrProdFroNormMeanFloat{1140.45086139393015400855801999568939208984375}
\def\EQKEErrProdFroNormMeanKey{21598}
\def\EQKEErrProdFroNormMedianFloat{1006.431758146844686052645556628704071044921875}
\def\EQKEErrProdFroNormMedianKey{29052}
\def\EQKEErrProdFroNormMinFloat{996.3816766187773055207799188792705535888671875}
\def\EQKEErrProdFroNormMinKey{17197}
\def\EQKEErrProdFroNormSqrtTwoLen{151}
\def\EQKEErrProdFroNormSqrtTwoMaxFloat{1820.652021061099958387785591185092926025390625}
\def\EQKEErrProdFroNormSqrtTwoMaxKey{29565}
\def\EQKEErrProdFroNormSqrtTwoMeanFloat{1612.841075403374588859151117503643035888671875}
\def\EQKEErrProdFroNormSqrtTwoMeanKey{21598}
\def\EQKEErrProdFroNormSqrtTwoMedianFloat{1423.30944197426651953719556331634521484375}
\def\EQKEErrProdFroNormSqrtTwoMedianKey{29052}
\def\EQKEErrProdFroNormSqrtTwoMinFloat{1409.096480374318389294785447418689727783203125}
\def\EQKEErrProdFroNormSqrtTwoMinKey{17197}
\def\EQKEErrProdFroNormSqrtTwoStdDevFloat{82.477381176624675163111533038318157196044921875}
\def\EQKEErrProdFroNormStdDevFloat{58.320315524499022785676061175763607025146484375}
\def\EQKEErrSimpleFirstSingularLen{151}
\def\EQKEErrSimpleFirstSingularMaxFloat{18.2210025787353515625}
\def\EQKEErrSimpleFirstSingularMaxKey{20415}
\def\EQKEErrSimpleFirstSingularMeanFloat{7.5459206372696829845381216728128492832183837890625}
\def\EQKEErrSimpleFirstSingularMeanKey{26829}
\def\EQKEErrSimpleFirstSingularMedianFloat{4.6328055858612060546875}
\def\EQKEErrSimpleFirstSingularMedianKey{742}
\def\EQKEErrSimpleFirstSingularMinFloat{4.526645183563232421875}
\def\EQKEErrSimpleFirstSingularMinKey{17197}
\def\EQKEErrSimpleFirstSingularSqrtTwoLen{151}
\def\EQKEErrSimpleFirstSingularSqrtTwoMaxFloat{25.7683887481689453125}
\def\EQKEErrSimpleFirstSingularSqrtTwoMaxKey{20415}
\def\EQKEErrSimpleFirstSingularSqrtTwoMeanFloat{10.671543146600786400313154445029795169830322265625}
\def\EQKEErrSimpleFirstSingularSqrtTwoMeanKey{26829}
\def\EQKEErrSimpleFirstSingularSqrtTwoMedianFloat{6.551776409149169921875}
\def\EQKEErrSimpleFirstSingularSqrtTwoMedianKey{742}
\def\EQKEErrSimpleFirstSingularSqrtTwoMinFloat{6.40164279937744140625}
\def\EQKEErrSimpleFirstSingularSqrtTwoMinKey{17197}
\def\EQKEErrSimpleFirstSingularSqrtTwoStdDevFloat{2.832925966397125794316025348962284624576568603515625}
\def\EQKEErrSimpleFirstSingularStdDevFloat{2.00318120161577883919790110667236149311065673828125}
\def\EQKEErrSimpleFroNormLen{151}
\def\EQKEErrSimpleFroNormMaxFloat{19.863086700439453125}
\def\EQKEErrSimpleFroNormMaxKey{20415}
\def\EQKEErrSimpleFroNormMeanFloat{10.5759189681501570845512105734087526798248291015625}
\def\EQKEErrSimpleFroNormMeanKey{24262}
\def\EQKEErrSimpleFroNormMedianFloat{7.6220600605010986328125}
\def\EQKEErrSimpleFroNormMedianKey{13468}
\def\EQKEErrSimpleFroNormMinFloat{7.573613643646240234375}
\def\EQKEErrSimpleFroNormMinKey{17197}
\def\EQKEErrSimpleFroNormSqrtTwoLen{151}
\def\EQKEErrSimpleFroNormSqrtTwoMaxFloat{28.0906467437744140625}
\def\EQKEErrSimpleFroNormSqrtTwoMaxKey{20415}
\def\EQKEErrSimpleFroNormSqrtTwoMeanFloat{14.9566077743934471300235600210726261138916015625}
\def\EQKEErrSimpleFroNormSqrtTwoMeanKey{24262}
\def\EQKEErrSimpleFroNormSqrtTwoMedianFloat{10.7792203426361083984375}
\def\EQKEErrSimpleFroNormSqrtTwoMedianKey{13468}
\def\EQKEErrSimpleFroNormSqrtTwoMinFloat{10.7107067108154296875}
\def\EQKEErrSimpleFroNormSqrtTwoMinKey{17197}
\def\EQKEErrSimpleFroNormSqrtTwoStdDevFloat{2.422351154718111576613637225818820297718048095703125}
\def\EQKEErrSimpleFroNormStdDevFloat{1.712860958554990542523910335148684680461883544921875}
\def\EQKEErrSimpleLen{4096}
\def\EQKEErrSimpleMaxAbsLen{151}
\def\EQKEErrSimpleMaxAbsMaxFloat{3.6802332401275634765625}
\def\EQKEErrSimpleMaxAbsMaxKey{15622}
\def\EQKEErrSimpleMaxAbsMeanFloat{1.5056603854855163948656127104186452925205230712890625}
\def\EQKEErrSimpleMaxAbsMeanKey{28716}
\def\EQKEErrSimpleMaxAbsMedianFloat{0.8232894241809844970703125}
\def\EQKEErrSimpleMaxAbsMedianKey{3254}
\def\EQKEErrSimpleMaxAbsMinFloat{0.78015422821044921875}
\def\EQKEErrSimpleMaxAbsMinKey{17197}
\def\EQKEErrSimpleMaxAbsStdDevFloat{0.46194301695036588117915243856259621679782867431640625}
\def\EQKEErrSimpleMaxLen{151}
\def\EQKEErrSimpleMaxMaxFloat{3.6802332401275634765625}
\def\EQKEErrSimpleMaxMaxKey{15622}
\def\EQKEErrSimpleMaxMeanFloat{1.151237010955810546875}
\def\EQKEErrSimpleMaxMeanKey{28090}
\def\EQKEErrSimpleMaxMedianFloat{0.653575479984283447265625}
\def\EQKEErrSimpleMaxMedianKey{19093}
\def\EQKEErrSimpleMaxMinFloat{0.6483228206634521484375}
\def\EQKEErrSimpleMaxMinKey{13293}
\def\EQKEErrSimpleMaxRowDiffLen{151}
\def\EQKEErrSimpleMaxRowDiffMaxFloat{4.94961071014404296875}
\def\EQKEErrSimpleMaxRowDiffMaxKey{20415}
\def\EQKEErrSimpleMaxRowDiffMeanFloat{2.2855861131718615553154450026340782642364501953125}
\def\EQKEErrSimpleMaxRowDiffMeanKey{24262}
\def\EQKEErrSimpleMaxRowDiffMedianFloat{1.2941989004611968994140625}
\def\EQKEErrSimpleMaxRowDiffMedianKey{2345}
\def\EQKEErrSimpleMaxRowDiffMinFloat{1.232765674591064453125}
\def\EQKEErrSimpleMaxRowDiffMinKey{3254}
\def\EQKEErrSimpleMaxRowDiffStdDevFloat{0.62018590794563877022227416091482155025005340576171875}
\def\EQKEErrSimpleMaxStdDevFloat{0.413701951503753662109375}
\def\EQKEErrSimpleMeanDimZeroNormLen{151}
\def\EQKEErrSimpleMeanDimZeroNormMaxFloat{0.1296360790729522705078125}
\def\EQKEErrSimpleMeanDimZeroNormMaxKey{27714}
\def\EQKEErrSimpleMeanDimZeroNormMeanFloat{0.037410374052378514431183020860771648585796356201171875}
\def\EQKEErrSimpleMeanDimZeroNormMeanKey{14095}
\def\EQKEErrSimpleMeanDimZeroNormMedianFloat{0.0106709734536707401275634765625}
\def\EQKEErrSimpleMeanDimZeroNormMedianKey{1696}
\def\EQKEErrSimpleMeanDimZeroNormMinFloat{0.009681611321866512298583984375}
\def\EQKEErrSimpleMeanDimZeroNormMinKey{20751}
\def\EQKEErrSimpleMeanDimZeroNormStdDevFloat{0.0226582533594607525573305650823385803960263729095458984375}
\def\EQKEErrSimpleMeanLen{151}
\def\EQKEErrSimpleMeanMaxFloat{0.00831353478133678436279296875}
\def\EQKEErrSimpleMeanMaxKey{30899}
\def\EQKEErrSimpleMeanMeanFloat{0.00026554730720818042755126953125}
\def\EQKEErrSimpleMeanMeanKey{2549}
\def\EQKEErrSimpleMeanMedianFloat{-0.006194973946548998355865478515625}
\def\EQKEErrSimpleMeanMedianKey{27484}
\def\EQKEErrSimpleMeanMinFloat{-0.006569989025592803955078125}
\def\EQKEErrSimpleMeanMinKey{1185}
\def\EQKEErrSimpleMeanStdDevFloat{0.0026572919450700283050537109375}
\def\EQKEErrSimpleMedianLen{151}
\def\EQKEErrSimpleMedianMaxFloat{-0.344818488508462916986019308751565404236316680908203125}
\def\EQKEErrSimpleMedianMaxKey{32103}
\def\EQKEErrSimpleMedianMeanFloat{-0.65288831217596854372686721035279333591461181640625}
\def\EQKEErrSimpleMedianMeanKey{8840}
\def\EQKEErrSimpleMedianMedianFloat{-1.4104827523231506791745459850062616169452667236328125}
\def\EQKEErrSimpleMedianMedianKey{12457}
\def\EQKEErrSimpleMedianMinFloat{-1.626250365376472384326689279987476766109466552734375}
\def\EQKEErrSimpleMedianMinKey{20415}
\def\EQKEErrSimpleMedianStdDevFloat{0.1964603183745192438447446647842298261821269989013671875}
\def\EQKEErrSimpleMinLen{151}
\def\EQKEErrSimpleMinMaxFloat{-0.580299854278564453125}
\def\EQKEErrSimpleMinMaxKey{32103}
\def\EQKEErrSimpleMinMeanFloat{-1.38601005077362060546875}
\def\EQKEErrSimpleMinMeanKey{25516}
\def\EQKEErrSimpleMinMedianFloat{-2.90118896961212158203125}
\def\EQKEErrSimpleMinMedianKey{23447}
\def\EQKEErrSimpleMinMinFloat{-3.654365062713623046875}
\def\EQKEErrSimpleMinMinKey{20415}
\def\EQKEErrSimpleMinStdDevFloat{0.4336081445217132568359375}
\def\EQKEErrSimpleStdDevLen{151}
\def\EQKEErrSimpleStdDevMaxFloat{0.3103322088718414306640625}
\def\EQKEErrSimpleStdDevMaxKey{20415}
\def\EQKEErrSimpleStdDevMeanFloat{0.16522882878780364990234375}
\def\EQKEErrSimpleStdDevMeanKey{24262}
\def\EQKEErrSimpleStdDevMedianFloat{0.11909215338528156280517578125}
\def\EQKEErrSimpleStdDevMedianKey{13468}
\def\EQKEErrSimpleStdDevMinFloat{0.11833114922046661376953125}
\def\EQKEErrSimpleStdDevMinKey{17197}
\def\EQKEErrSimpleStdDevStdDevFloat{0.02675312198698520660400390625}
\def\EQKEErrSimpleWithAttnScaleFirstSingularLen{151}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMaxFloat{3.2210483551025390625}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMaxKey{20415}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMeanFloat{1.3339429426666915556864978498197160661220550537109375}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMeanKey{26829}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMedianFloat{0.8189720213413238525390625}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMedianKey{742}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMinFloat{0.800205409526824951171875}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMinKey{17197}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoLen{151}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMaxFloat{4.5552501678466796875}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMaxKey{20415}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMeanFloat{1.8864801727383342377919461796409450471401214599609375}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMeanKey{26829}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMedianFloat{1.1582013070583343505859375}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMedianKey{742}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMinFloat{1.13166129589080810546875}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMinKey{17197}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoStdDevFloat{0.50079528064844469614769195686676539480686187744140625}
\def\EQKEErrSimpleWithAttnScaleFirstSingularStdDevFloat{0.3541157420274834155549115166650153696537017822265625}
\def\EQKEErrSimpleWithAttnScaleFroNormLen{151}
\def\EQKEErrSimpleWithAttnScaleFroNormMaxFloat{3.511331081390380859375}
\def\EQKEErrSimpleWithAttnScaleFroNormMaxKey{20415}
\def\EQKEErrSimpleWithAttnScaleFroNormMeanFloat{1.869576037324816919493741806945763528347015380859375}
\def\EQKEErrSimpleWithAttnScaleFroNormMeanKey{24262}
\def\EQKEErrSimpleWithAttnScaleFroNormMedianFloat{1.3474025726318359375}
\def\EQKEErrSimpleWithAttnScaleFroNormMedianKey{13468}
\def\EQKEErrSimpleWithAttnScaleFroNormMinFloat{1.33883845806121826171875}
\def\EQKEErrSimpleWithAttnScaleFroNormMinKey{17197}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoLen{151}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMaxFloat{4.965772151947021484375}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMaxKey{20415}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMeanFloat{2.643979744405935861095713335089385509490966796875}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMeanKey{24262}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMedianFloat{1.9055149555206298828125}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMedianKey{13468}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMinFloat{1.893403530120849609375}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMinKey{17197}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoStdDevFloat{0.428215265489182705938020490066264756023883819580078125}
\def\EQKEErrSimpleWithAttnScaleFroNormStdDevFloat{0.302793917786760069521534433079068548977375030517578125}
\def\EQKEErrSimpleWithAttnScaleLen{4096}
\def\EQKEErrSimpleWithAttnScaleMaxAbsLen{151}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMaxFloat{0.6505794525146484375}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMaxKey{15622}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMeanFloat{0.266165670574895596445230694371275603771209716796875}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMeanKey{28716}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMedianFloat{0.145538389682769775390625}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMedianKey{3254}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMinFloat{0.13791309297084808349609375}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMinKey{17197}
\def\EQKEErrSimpleWithAttnScaleMaxAbsStdDevFloat{0.08166075987963196392005471579977893270552158355712890625}
\def\EQKEErrSimpleWithAttnScaleMaxLen{151}
\def\EQKEErrSimpleWithAttnScaleMaxMaxFloat{0.6505794525146484375}
\def\EQKEErrSimpleWithAttnScaleMaxMaxKey{15622}
\def\EQKEErrSimpleWithAttnScaleMaxMeanFloat{0.20351190865039825439453125}
\def\EQKEErrSimpleWithAttnScaleMaxMeanKey{28090}
\def\EQKEErrSimpleWithAttnScaleMaxMedianFloat{0.1155369170010089874267578125}
\def\EQKEErrSimpleWithAttnScaleMaxMedianKey{19093}
\def\EQKEErrSimpleWithAttnScaleMaxMinFloat{0.114608369767665863037109375}
\def\EQKEErrSimpleWithAttnScaleMaxMinKey{13293}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffLen{151}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMaxFloat{0.87497580051422119140625}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMaxKey{20415}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMeanFloat{0.404038366004331239711433454431244172155857086181640625}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMeanKey{24262}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMedianFloat{0.22878421843051910400390625}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMedianKey{2345}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMinFloat{0.2179242670536041259765625}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMinKey{3254}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffStdDevFloat{0.10963441653616108617530500168868456967175006866455078125}
\def\EQKEErrSimpleWithAttnScaleMaxStdDevFloat{0.07313287258148193359375}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormLen{151}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMaxFloat{0.02291664294898509979248046875}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMaxKey{27714}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMeanFloat{0.006613282566976468219988039010104330372996628284454345703125}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMeanKey{14095}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMedianFloat{0.0018863796140067279338836669921875}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMedianKey{1696}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMinFloat{0.001711483695544302463531494140625}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMinKey{20751}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormStdDevFloat{0.004005451359275929469616617240035338909365236759185791015625}
\def\EQKEErrSimpleWithAttnScaleMeanLen{151}
\def\EQKEErrSimpleWithAttnScaleMeanMaxFloat{0.00146963889710605144500732421875}
\def\EQKEErrSimpleWithAttnScaleMeanMaxKey{30899}
\def\EQKEErrSimpleWithAttnScaleMeanMeanFloat{0.000046942601329647004604339599609375}
\def\EQKEErrSimpleWithAttnScaleMeanMeanKey{2549}
\def\EQKEErrSimpleWithAttnScaleMeanMedianFloat{-0.00109512705239467322826385498046875}
\def\EQKEErrSimpleWithAttnScaleMeanMedianKey{27484}
\def\EQKEErrSimpleWithAttnScaleMeanMinFloat{-0.0011614211834967136383056640625}
\def\EQKEErrSimpleWithAttnScaleMeanMinKey{1185}
\def\EQKEErrSimpleWithAttnScaleMeanStdDevFloat{0.0004697472904808819293975830078125}
\def\EQKEErrSimpleWithAttnScaleMedianLen{151}
\def\EQKEErrSimpleWithAttnScaleMedianMaxFloat{-0.06095587490126490315400786812460864894092082977294921875}
\def\EQKEErrSimpleWithAttnScaleMedianMaxKey{32103}
\def\EQKEErrSimpleWithAttnScaleMedianMeanFloat{-0.11541544014020570230183437843152205459773540496826171875}
\def\EQKEErrSimpleWithAttnScaleMedianMeanKey{8840}
\def\EQKEErrSimpleWithAttnScaleMedianMedianFloat{-0.2493404860608279538514153728101518936455249786376953125}
\def\EQKEErrSimpleWithAttnScaleMedianMedianKey{12457}
\def\EQKEErrSimpleWithAttnScaleMedianMinFloat{-0.287483172118663754535106136245303787291049957275390625}
\def\EQKEErrSimpleWithAttnScaleMedianMinKey{20415}
\def\EQKEErrSimpleWithAttnScaleMedianStdDevFloat{0.03472960640951040789392578744809725321829319000244140625}
\def\EQKEErrSimpleWithAttnScaleMinLen{151}
\def\EQKEErrSimpleWithAttnScaleMinMaxFloat{-0.102583490312099456787109375}
\def\EQKEErrSimpleWithAttnScaleMinMaxKey{32103}
\def\EQKEErrSimpleWithAttnScaleMinMeanFloat{-0.24501430988311767578125}
\def\EQKEErrSimpleWithAttnScaleMinMeanKey{25516}
\def\EQKEErrSimpleWithAttnScaleMinMedianFloat{-0.512862600386142730712890625}
\def\EQKEErrSimpleWithAttnScaleMinMedianKey{23447}
\def\EQKEErrSimpleWithAttnScaleMinMinFloat{-0.64600658416748046875}
\def\EQKEErrSimpleWithAttnScaleMinMinKey{20415}
\def\EQKEErrSimpleWithAttnScaleMinStdDevFloat{0.076651819050312042236328125}
\def\EQKEErrSimpleWithAttnScaleStdDevLen{151}
\def\EQKEErrSimpleWithAttnScaleStdDevMaxFloat{0.05485950410366058349609375}
\def\EQKEErrSimpleWithAttnScaleStdDevMaxKey{20415}
\def\EQKEErrSimpleWithAttnScaleStdDevMeanFloat{0.02920860238373279571533203125}
\def\EQKEErrSimpleWithAttnScaleStdDevMeanKey{24262}
\def\EQKEErrSimpleWithAttnScaleStdDevMedianFloat{0.021052717231214046478271484375}
\def\EQKEErrSimpleWithAttnScaleStdDevMedianKey{13468}
\def\EQKEErrSimpleWithAttnScaleStdDevMinFloat{0.020918190479278564453125}
\def\EQKEErrSimpleWithAttnScaleStdDevMinKey{17197}
\def\EQKEErrSimpleWithAttnScaleStdDevStdDevFloat{0.00472932867705821990966796875}
\def\EQKEErrStdDevLen{151}
\def\EQKEErrStdDevMaxFloat{0.1666397750377655029296875}
\def\EQKEErrStdDevMaxKey{27714}
\def\EQKEErrStdDevMeanFloat{0.111614577472209930419921875}
\def\EQKEErrStdDevMeanKey{14929}
\def\EQKEErrStdDevMedianFloat{0.09312727488577365875244140625}
\def\EQKEErrStdDevMedianKey{8893}
\def\EQKEErrStdDevMinFloat{0.09198819100856781005859375}
\def\EQKEErrStdDevMinKey{29052}
\def\EQKEErrStdDevStdDevFloat{0.01147004775702953338623046875}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactLen{151}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMaxFloat{0.537312209606170654296875}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMaxKey{12457}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMeanFloat{0.282895522993921455512378315688692964613437652587890625}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMeanKey{18289}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMedianFloat{0.1689452044665813446044921875}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMedianKey{24202}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMinFloat{0.161419451236724853515625}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMinKey{23241}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactStdDevFloat{0.0686115892298575780205993623894755728542804718017578125}
\def\EQKEErrWithAttnScaleBoundMaxDiffLen{151}
\def\EQKEErrWithAttnScaleBoundMaxDiffMaxFloat{1.12711584568023681640625}
\def\EQKEErrWithAttnScaleBoundMaxDiffMaxKey{1681}
\def\EQKEErrWithAttnScaleBoundMaxDiffMeanFloat{0.83323135715446727811439586730557493865489959716796875}
\def\EQKEErrWithAttnScaleBoundMaxDiffMeanKey{17096}
\def\EQKEErrWithAttnScaleBoundMaxDiffMedianFloat{0.64195692539215087890625}
\def\EQKEErrWithAttnScaleBoundMaxDiffMedianKey{8840}
\def\EQKEErrWithAttnScaleBoundMaxDiffMinFloat{0.625}
\def\EQKEErrWithAttnScaleBoundMaxDiffMinKey{13468}
\def\EQKEErrWithAttnScaleBoundMaxDiffStdDevFloat{0.09592952854352899960677092394689680077135562896728515625}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductLen{151}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMaxFloat{1.12711584568023681640625}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMaxKey{1681}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMeanFloat{0.83323135715446727811439586730557493865489959716796875}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMeanKey{17096}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMedianFloat{0.64195692539215087890625}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMedianKey{8840}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMinFloat{0.625}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMinKey{13468}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMaxFloat{22.994174957275390625}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMaxKey{1490}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMeanFloat{16.64977886503105963811321998946368694305419921875}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMeanKey{26932}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMedianFloat{13.6560475826263427734375}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMedianKey{4729}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMinFloat{12.78299713134765625}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMinKey{13468}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveStdDevFloat{1.5954627095006135295562899045762605965137481689453125}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductStdDevFloat{0.09592952854352899960677092394689680077135562896728515625}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffLen{151}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMaxFloat{1.137599468231201171875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMaxKey{1681}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMeanFloat{0.83531946970137538333034399329335428774356842041015625}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMeanKey{22286}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMedianFloat{0.64510993659496307373046875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMedianKey{8840}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMinFloat{0.626399695873260498046875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMinKey{13468}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffStdDevFloat{0.0961285055630029805495695427453028969466686248779296875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductLen{151}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMaxFloat{1.137599468231201171875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMaxKey{1681}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMeanFloat{0.83531946970137538333034399329335428774356842041015625}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMeanKey{22286}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMedianFloat{0.64510993659496307373046875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMedianKey{8840}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMinFloat{0.626399695873260498046875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMinKey{13468}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMaxFloat{23.335712432861328125}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMaxKey{1490}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMeanFloat{16.654886574145184141571007785387337207794189453125}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMeanKey{29725}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMedianFloat{13.6738617420196533203125}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMedianKey{1895}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMinFloat{12.810016632080078125}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMinKey{13468}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveStdDevFloat{1.61429280020220122793261907645501196384429931640625}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductStdDevFloat{0.0961285055630029805495695427453028969466686248779296875}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMaxFloat{23.5128154754638671875}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMaxKey{1490}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMeanFloat{16.9954915899314613625392667017877101898193359375}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMeanKey{20976}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMedianFloat{13.9626905918121337890625}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMedianKey{1895}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMinFloat{13.20743846893310546875}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMinKey{13468}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveStdDevFloat{1.653818566824245106516855230438522994518280029296875}
\def\EQKEErrWithAttnScaleBoundSvdLen{151}
\def\EQKEErrWithAttnScaleBoundSvdMaxFloat{2.275171756744384765625}
\def\EQKEErrWithAttnScaleBoundSvdMaxKey{27714}
\def\EQKEErrWithAttnScaleBoundSvdMeanFloat{1.1246552672607219580669379865867085754871368408203125}
\def\EQKEErrWithAttnScaleBoundSvdMeanKey{29195}
\def\EQKEErrWithAttnScaleBoundSvdMedianFloat{0.8021863400936126708984375}
\def\EQKEErrWithAttnScaleBoundSvdMedianKey{15399}
\def\EQKEErrWithAttnScaleBoundSvdMinFloat{0.77486169338226318359375}
\def\EQKEErrWithAttnScaleBoundSvdMinKey{20013}
\def\EQKEErrWithAttnScaleBoundSvdStdDevFloat{0.2103699260443962215649804647910059429705142974853515625}
\def\EQKEErrWithAttnScaleFirstSingularLen{151}
\def\EQKEErrWithAttnScaleFirstSingularMaxFloat{1.608789920806884765625}
\def\EQKEErrWithAttnScaleFirstSingularMaxKey{27714}
\def\EQKEErrWithAttnScaleFirstSingularMeanFloat{0.7952514121074549802159481259877793490886688232421875}
\def\EQKEErrWithAttnScaleFirstSingularMeanKey{29195}
\def\EQKEErrWithAttnScaleFirstSingularMedianFloat{0.56723149120807647705078125}
\def\EQKEErrWithAttnScaleFirstSingularMedianKey{15399}
\def\EQKEErrWithAttnScaleFirstSingularMinFloat{0.547910153865814208984375}
\def\EQKEErrWithAttnScaleFirstSingularMinKey{20013}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoLen{151}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMaxFloat{2.2751724720001220703125}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMaxKey{27714}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMeanFloat{1.1246553138391861548228689571260474622249603271484375}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMeanKey{29195}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMedianFloat{0.80218644440174102783203125}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMedianKey{15399}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMinFloat{0.77486193180084228515625}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMinKey{20013}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoStdDevFloat{0.2103698351571407221261011954993591643869876861572265625}
\def\EQKEErrWithAttnScaleFirstSingularStdDevFloat{0.148753939518427802379818558620172552764415740966796875}
\def\EQKEErrWithAttnScaleFroNormLen{151}
\def\EQKEErrWithAttnScaleFroNormMaxFloat{1.88531601428985595703125}
\def\EQKEErrWithAttnScaleFroNormMaxKey{27714}
\def\EQKEErrWithAttnScaleFroNormMeanFloat{1.262776453763443829103607640718109905719757080078125}
\def\EQKEErrWithAttnScaleFroNormMeanKey{14929}
\def\EQKEErrWithAttnScaleFroNormMedianFloat{1.0536148250102996826171875}
\def\EQKEErrWithAttnScaleFroNormMedianKey{8893}
\def\EQKEErrWithAttnScaleFroNormMinFloat{1.0407276153564453125}
\def\EQKEErrWithAttnScaleFroNormMinKey{29052}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoLen{151}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMaxFloat{2.6662395000457763671875}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMaxKey{27714}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMeanFloat{1.7858355605839104640608638874255120754241943359375}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMeanKey{14929}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMedianFloat{1.490036308765411376953125}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMedianKey{8893}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMinFloat{1.4718110561370849609375}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMinKey{29052}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoStdDevFloat{0.183521346563108422866861246802727691829204559326171875}
\def\EQKEErrWithAttnScaleFroNormStdDevFloat{0.1297691823404825972598786165690398775041103363037109375}
\def\EQKEErrWithAttnScaleLen{4096}
\def\EQKEErrWithAttnScaleMaxAbsLen{151}
\def\EQKEErrWithAttnScaleMaxAbsMaxFloat{0.32094752788543701171875}
\def\EQKEErrWithAttnScaleMaxAbsMaxKey{12457}
\def\EQKEErrWithAttnScaleMaxAbsMeanFloat{0.1594018392906283720922289148802519775927066802978515625}
\def\EQKEErrWithAttnScaleMaxAbsMeanKey{12493}
\def\EQKEErrWithAttnScaleMaxAbsMedianFloat{0.0997659005224704742431640625}
\def\EQKEErrWithAttnScaleMaxAbsMedianKey{32103}
\def\EQKEErrWithAttnScaleMaxAbsMinFloat{0.09917949140071868896484375}
\def\EQKEErrWithAttnScaleMaxAbsMinKey{1412}
\def\EQKEErrWithAttnScaleMaxAbsStdDevFloat{0.039463085240546293130936561510679894126951694488525390625}
\def\EQKEErrWithAttnScaleMaxLen{151}
\def\EQKEErrWithAttnScaleMaxMaxFloat{0.32094752788543701171875}
\def\EQKEErrWithAttnScaleMaxMaxKey{12457}
\def\EQKEErrWithAttnScaleMaxMeanFloat{0.14997343719005584716796875}
\def\EQKEErrWithAttnScaleMaxMeanKey{24566}
\def\EQKEErrWithAttnScaleMaxMedianFloat{0.0913392491638660430908203125}
\def\EQKEErrWithAttnScaleMaxMedianKey{32103}
\def\EQKEErrWithAttnScaleMaxMinFloat{0.09041912853717803955078125}
\def\EQKEErrWithAttnScaleMaxMinKey{32374}
\def\EQKEErrWithAttnScaleMaxRowDiffLen{151}
\def\EQKEErrWithAttnScaleMaxRowDiffMaxFloat{0.5373122692108154296875}
\def\EQKEErrWithAttnScaleMaxRowDiffMaxKey{12457}
\def\EQKEErrWithAttnScaleMaxRowDiffMeanFloat{0.282895521316307296810776961137889884412288665771484375}
\def\EQKEErrWithAttnScaleMaxRowDiffMeanKey{18289}
\def\EQKEErrWithAttnScaleMaxRowDiffMedianFloat{0.1689452044665813446044921875}
\def\EQKEErrWithAttnScaleMaxRowDiffMedianKey{24202}
\def\EQKEErrWithAttnScaleMaxRowDiffMinFloat{0.16141940653324127197265625}
\def\EQKEErrWithAttnScaleMaxRowDiffMinKey{23241}
\def\EQKEErrWithAttnScaleMaxRowDiffStdDevFloat{0.06861159296212616942600703850985155440866947174072265625}
\def\EQKEErrWithAttnScaleMaxStdDevFloat{0.0395284257829189300537109375}
\def\EQKEErrWithAttnScaleMeanDimZeroNormLen{151}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMaxFloat{0.00944446958601474761962890625}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMaxKey{12457}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMeanFloat{0.0032817702223886025848786918146515745320357382297515869140625}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMeanKey{17080}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMedianFloat{0.0011484124697744846343994140625}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMedianKey{11611}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMinFloat{0.0011125630699098110198974609375}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMinKey{28778}
\def\EQKEErrWithAttnScaleMeanDimZeroNormStdDevFloat{0.00143113960428447868460100078635832687723450362682342529296875}
\def\EQKEErrWithAttnScaleMeanLen{151}
\def\EQKEErrWithAttnScaleMeanMaxFloat{0.00012233530287630856037139892578125}
\def\EQKEErrWithAttnScaleMeanMaxKey{20976}
\def\EQKEErrWithAttnScaleMeanMeanFloat{0.00000085060395349501050077378749847412109375}
\def\EQKEErrWithAttnScaleMeanMeanKey{7467}
\def\EQKEErrWithAttnScaleMeanMedianFloat{-0.00007668233956792391836643218994140625}
\def\EQKEErrWithAttnScaleMeanMedianKey{519}
\def\EQKEErrWithAttnScaleMeanMinFloat{-0.00009842679719440639019012451171875}
\def\EQKEErrWithAttnScaleMeanMinKey{1681}
\def\EQKEErrWithAttnScaleMeanStdDevFloat{0.00003281699537183158099651336669921875}
\def\EQKEErrWithAttnScaleMedianLen{151}
\def\EQKEErrWithAttnScaleMedianMaxFloat{-0.05479587260633707324064545218789135105907917022705078125}
\def\EQKEErrWithAttnScaleMedianMaxKey{4430}
\def\EQKEErrWithAttnScaleMedianMeanFloat{-0.06960915034291463576732184037609840743243694305419921875}
\def\EQKEErrWithAttnScaleMedianMeanKey{4729}
\def\EQKEErrWithAttnScaleMedianMedianFloat{-0.10810492211021482944488525390625}
\def\EQKEErrWithAttnScaleMedianMedianKey{8048}
\def\EQKEErrWithAttnScaleMedianMinFloat{-0.12421034853905439654386810843789135105907917022705078125}
\def\EQKEErrWithAttnScaleMedianMinKey{27714}
\def\EQKEErrWithAttnScaleMedianStdDevFloat{0.0103740218107524449775436181653276435099542140960693359375}
\def\EQKEErrWithAttnScaleMinLen{151}
\def\EQKEErrWithAttnScaleMinMaxFloat{-0.095076777040958404541015625}
\def\EQKEErrWithAttnScaleMinMaxKey{23241}
\def\EQKEErrWithAttnScaleMinMeanFloat{-0.14758600294589996337890625}
\def\EQKEErrWithAttnScaleMinMeanKey{29726}
\def\EQKEErrWithAttnScaleMinMedianFloat{-0.2594556510448455810546875}
\def\EQKEErrWithAttnScaleMinMedianKey{3284}
\def\EQKEErrWithAttnScaleMinMinFloat{-0.27411401271820068359375}
\def\EQKEErrWithAttnScaleMinMinKey{23447}
\def\EQKEErrWithAttnScaleMinStdDevFloat{0.035141967236995697021484375}
\def\EQKEErrWithAttnScaleStdDevLen{151}
\def\EQKEErrWithAttnScaleStdDevMaxFloat{0.02945802919566631317138671875}
\def\EQKEErrWithAttnScaleStdDevMaxKey{27714}
\def\EQKEErrWithAttnScaleStdDevMeanFloat{0.01973085664212703704833984375}
\def\EQKEErrWithAttnScaleStdDevMeanKey{14929}
\def\EQKEErrWithAttnScaleStdDevMedianFloat{0.016462733037769794464111328125}
\def\EQKEErrWithAttnScaleStdDevMedianKey{8893}
\def\EQKEErrWithAttnScaleStdDevMinFloat{0.0162613689899444580078125}
\def\EQKEErrWithAttnScaleStdDevMinKey{29052}
\def\EQKEErrWithAttnScaleStdDevStdDevFloat{0.002027637325227260589599609375}
\def\EQKEFirstSingularLen{151}
\def\EQKEFirstSingularMaxFloat{8698.4765625}
\def\EQKEFirstSingularMaxKey{15622}
\def\EQKEFirstSingularMeanFloat{6297.2579741825329620041884481906890869140625}
\def\EQKEFirstSingularMeanKey{27484}
\def\EQKEFirstSingularMedianFloat{4934.405517578125}
\def\EQKEFirstSingularMedianKey{9134}
\def\EQKEFirstSingularMinFloat{4814.546875}
\def\EQKEFirstSingularMinKey{30371}
\def\EQKEFirstSingularSqrtTwoLen{151}
\def\EQKEFirstSingularSqrtTwoMaxFloat{12301.5035266720005893148481845855712890625}
\def\EQKEFirstSingularSqrtTwoMaxKey{15622}
\def\EQKEFirstSingularSqrtTwoMeanFloat{8905.66763285106208059005439281463623046875}
\def\EQKEFirstSingularSqrtTwoMeanKey{27484}
\def\EQKEFirstSingularSqrtTwoMedianFloat{6978.303205207615974359214305877685546875}
\def\EQKEFirstSingularSqrtTwoMedianKey{9134}
\def\EQKEFirstSingularSqrtTwoMinFloat{6808.797487306002949480898678302764892578125}
\def\EQKEFirstSingularSqrtTwoMinKey{30371}
\def\EQKEFirstSingularSqrtTwoStdDevFloat{999.3516327597326380782760679721832275390625}
\def\EQKEFirstSingularStdDevFloat{706.6483163142551120472489856183528900146484375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMaxFloat{-4341639585033177088}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMaxKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMeanFloat{-4341639585033174528}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMeanKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMedianFloat{-4341639585033177088}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMedianKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMinFloat{-4341639585033177088}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMinKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenStdDevFloat{2560}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMaxFloat{185.298126220703125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMaxKey{15622}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMeanFloat{17.8674144744873046875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMeanKey{29052}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMedianFloat{7.0456774234771728515625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMedianKey{3254}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMinFloat{6.52538967132568359375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMinKey{21598}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxStdDevFloat{22.763164520263671875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMaxFloat{18.829697981850575416729043354280292987823486328125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMaxKey{19538}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMeanFloat{9.271473361286791003976759384386241436004638671875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMeanKey{22286}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMedianFloat{1.675768274119692424761751681216992437839508056640625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMedianKey{32382}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMinFloat{-5.62679312247577367855910779326222836971282958984375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMinKey{15622}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanStdDevFloat{2.266227991456780888057664924417622387409210205078125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMaxFloat{27.47638702392578125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMaxKey{4647}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMeanFloat{-7.61088966750391993087987430044449865818023681640625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMeanKey{7238}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMedianFloat{-122.5165789065132457835716195404529571533203125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMedianKey{1490}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMinFloat{-173.894211744217074055995908565819263458251953125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMinKey{15622}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianStdDevFloat{20.408891563803049251646370976231992244720458984375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMaxFloat{-3.5273420810699462890625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMaxKey{7790}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMeanFloat{-13.54140377044677734375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMeanKey{30684}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMedianFloat{-175.0927276611328125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMedianKey{1490}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMinFloat{-178.145050048828125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMinKey{15622}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinStdDevFloat{22.5222873687744140625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMaxFloat{nan}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMaxKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMeanFloat{nan}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMeanKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMedianFloat{nan}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMedianKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMinFloat{nan}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMinKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevStdDevFloat{nan}
\def\EQKEHistAttentionDifferenceOverGapLenLen{151}
\def\EQKEHistAttentionDifferenceOverGapLenMaxFloat{258048}
\def\EQKEHistAttentionDifferenceOverGapLenMaxKey{50}
\def\EQKEHistAttentionDifferenceOverGapLenMeanFloat{258048}
\def\EQKEHistAttentionDifferenceOverGapLenMeanKey{50}
\def\EQKEHistAttentionDifferenceOverGapLenMedianFloat{258048}
\def\EQKEHistAttentionDifferenceOverGapLenMedianKey{50}
\def\EQKEHistAttentionDifferenceOverGapLenMinFloat{258048}
\def\EQKEHistAttentionDifferenceOverGapLenMinKey{50}
\def\EQKEHistAttentionDifferenceOverGapLenStdDevFloat{0}
\def\EQKEHistAttentionDifferenceOverGapMaxLen{151}
\def\EQKEHistAttentionDifferenceOverGapMaxMaxFloat{185.298126220703125}
\def\EQKEHistAttentionDifferenceOverGapMaxMaxKey{15622}
\def\EQKEHistAttentionDifferenceOverGapMaxMeanFloat{17.8674144744873046875}
\def\EQKEHistAttentionDifferenceOverGapMaxMeanKey{29052}
\def\EQKEHistAttentionDifferenceOverGapMaxMedianFloat{7.0456774234771728515625}
\def\EQKEHistAttentionDifferenceOverGapMaxMedianKey{3254}
\def\EQKEHistAttentionDifferenceOverGapMaxMinFloat{6.52538967132568359375}
\def\EQKEHistAttentionDifferenceOverGapMaxMinKey{21598}
\def\EQKEHistAttentionDifferenceOverGapMaxStdDevFloat{22.763164520263671875}
\def\EQKEHistAttentionDifferenceOverGapMeanLen{151}
\def\EQKEHistAttentionDifferenceOverGapMeanMaxFloat{0.8408319950103759765625}
\def\EQKEHistAttentionDifferenceOverGapMeanMaxKey{19538}
\def\EQKEHistAttentionDifferenceOverGapMeanMeanFloat{0.69712030887603759765625}
\def\EQKEHistAttentionDifferenceOverGapMeanMeanKey{1185}
\def\EQKEHistAttentionDifferenceOverGapMeanMedianFloat{0.53024305403232574462890625}
\def\EQKEHistAttentionDifferenceOverGapMeanMedianKey{30371}
\def\EQKEHistAttentionDifferenceOverGapMeanMinFloat{0.529929459095001220703125}
\def\EQKEHistAttentionDifferenceOverGapMeanMinKey{29725}
\def\EQKEHistAttentionDifferenceOverGapMeanStdDevFloat{0.05761106312274932861328125}
\def\EQKEHistAttentionDifferenceOverGapMedianLen{151}
\def\EQKEHistAttentionDifferenceOverGapMedianMaxFloat{0.4462631274270647541158041349262930452823638916015625}
\def\EQKEHistAttentionDifferenceOverGapMedianMaxKey{10248}
\def\EQKEHistAttentionDifferenceOverGapMedianMeanFloat{0.28861552496732567618664688779972493648529052734375}
\def\EQKEHistAttentionDifferenceOverGapMedianMeanKey{12287}
\def\EQKEHistAttentionDifferenceOverGapMedianMedianFloat{0.1152928957132665355178602339947246946394443511962890625}
\def\EQKEHistAttentionDifferenceOverGapMedianMedianKey{29725}
\def\EQKEHistAttentionDifferenceOverGapMedianMinFloat{0.1077736516603986782758539675342035479843616485595703125}
\def\EQKEHistAttentionDifferenceOverGapMedianMinKey{6159}
\def\EQKEHistAttentionDifferenceOverGapMedianStdDevFloat{0.06277118309889222202979652820431510917842388153076171875}
\def\EQKEHistAttentionDifferenceOverGapMinLen{151}
\def\EQKEHistAttentionDifferenceOverGapMinMaxFloat{-3.5273420810699462890625}
\def\EQKEHistAttentionDifferenceOverGapMinMaxKey{7790}
\def\EQKEHistAttentionDifferenceOverGapMinMeanFloat{-13.54140377044677734375}
\def\EQKEHistAttentionDifferenceOverGapMinMeanKey{30684}
\def\EQKEHistAttentionDifferenceOverGapMinMedianFloat{-175.0927276611328125}
\def\EQKEHistAttentionDifferenceOverGapMinMedianKey{1490}
\def\EQKEHistAttentionDifferenceOverGapMinMinFloat{-178.145050048828125}
\def\EQKEHistAttentionDifferenceOverGapMinMinKey{15622}
\def\EQKEHistAttentionDifferenceOverGapMinStdDevFloat{22.5222873687744140625}
\def\EQKEHistAttentionDifferenceOverGapStdDevLen{151}
\def\EQKEHistAttentionDifferenceOverGapStdDevMaxFloat{5.9184513092041015625}
\def\EQKEHistAttentionDifferenceOverGapStdDevMaxKey{15622}
\def\EQKEHistAttentionDifferenceOverGapStdDevMeanFloat{1.28688371181488037109375}
\def\EQKEHistAttentionDifferenceOverGapStdDevMeanKey{30463}
\def\EQKEHistAttentionDifferenceOverGapStdDevMedianFloat{1.0431757867336273193359375}
\def\EQKEHistAttentionDifferenceOverGapStdDevMedianKey{26829}
\def\EQKEHistAttentionDifferenceOverGapStdDevMinFloat{1.03886592388153076171875}
\def\EQKEHistAttentionDifferenceOverGapStdDevMinKey{14095}
\def\EQKEHistAttentionDifferenceOverGapStdDevStdDevFloat{0.49725115299224853515625}
\def\EQKEQueryDirectionLen{64}
\def\EQKEQueryDirectionMaxLen{151}
\def\EQKEQueryDirectionMaxMaxFloat{0.23326575756072998046875}
\def\EQKEQueryDirectionMaxMaxKey{1490}
\def\EQKEQueryDirectionMaxMeanFloat{0.1636082828044891357421875}
\def\EQKEQueryDirectionMaxMeanKey{27300}
\def\EQKEQueryDirectionMaxMedianFloat{0.14298801124095916748046875}
\def\EQKEQueryDirectionMaxMedianKey{8840}
\def\EQKEQueryDirectionMaxMinFloat{0.14044634997844696044921875}
\def\EQKEQueryDirectionMaxMinKey{6549}
\def\EQKEQueryDirectionMaxStdDevFloat{0.014722702093422412872314453125}
\def\EQKEQueryDirectionMeanLen{151}
\def\EQKEQueryDirectionMeanMaxFloat{0.12475268542766571044921875}
\def\EQKEQueryDirectionMeanMaxKey{20751}
\def\EQKEQueryDirectionMeanMeanFloat{0.124338112771511077880859375}
\def\EQKEQueryDirectionMeanMeanKey{20415}
\def\EQKEQueryDirectionMeanMedianFloat{0.123358719050884246826171875}
\def\EQKEQueryDirectionMeanMedianKey{30899}
\def\EQKEQueryDirectionMeanMinFloat{0.123075745999813079833984375}
\def\EQKEQueryDirectionMeanMinKey{14929}
\def\EQKEQueryDirectionMeanStdDevFloat{0.00027712641167454421520233154296875}
\def\EQKEQueryDirectionMedianLen{151}
\def\EQKEQueryDirectionMedianMaxFloat{0.11226351790130138785794855493804789148271083831787109375}
\def\EQKEQueryDirectionMedianMaxKey{7467}
\def\EQKEQueryDirectionMedianMeanFloat{0.09470660253088698798951128310363856144249439239501953125}
\def\EQKEQueryDirectionMedianMeanKey{22261}
\def\EQKEQueryDirectionMedianMedianFloat{0.0603038969310000505519298030776553787291049957275390625}
\def\EQKEQueryDirectionMedianMedianKey{2236}
\def\EQKEQueryDirectionMedianMinFloat{0.0567437328584492195471256081873434595763683319091796875}
\def\EQKEQueryDirectionMedianMinKey{519}
\def\EQKEQueryDirectionMedianStdDevFloat{0.011110614493287686299627381458776653744280338287353515625}
\def\EQKEQueryDirectionMinLen{151}
\def\EQKEQueryDirectionMinMaxFloat{0.11173152923583984375}
\def\EQKEQueryDirectionMinMaxKey{7467}
\def\EQKEQueryDirectionMinMeanFloat{0.092159263789653778076171875}
\def\EQKEQueryDirectionMinMeanKey{1951}
\def\EQKEQueryDirectionMinMedianFloat{0.050767769105732440948486328125}
\def\EQKEQueryDirectionMinMedianKey{2236}
\def\EQKEQueryDirectionMinMinFloat{0.0412342064082622528076171875}
\def\EQKEQueryDirectionMinMinKey{519}
\def\EQKEQueryDirectionMinStdDevFloat{0.012797093950212001800537109375}
\def\EQKEQueryDirectionStdDevLen{151}
\def\EQKEQueryDirectionStdDevMaxFloat{0.02184858731925487518310546875}
\def\EQKEQueryDirectionStdDevMaxKey{14929}
\def\EQKEQueryDirectionStdDevMeanFloat{0.01259678415954113006591796875}
\def\EQKEQueryDirectionStdDevMeanKey{1895}
\def\EQKEQueryDirectionStdDevMedianFloat{0.00792146869935095310211181640625}
\def\EQKEQueryDirectionStdDevMedianKey{3175}
\def\EQKEQueryDirectionStdDevMinFloat{0.007859191857278347015380859375}
\def\EQKEQueryDirectionStdDevMinKey{20751}
\def\EQKEQueryDirectionStdDevStdDevFloat{0.0025061839260160923004150390625}
\def\EQKERatioFirstTwoSingularLen{151}
\def\EQKERatioFirstTwoSingularLowerWhiskerBottomEndFloat{339.154339661397671079612337052822113037109375}
\def\EQKERatioFirstTwoSingularLowerWhiskerBottomEndKey{20415}
\def\EQKERatioFirstTwoSingularLowerWhiskerCrosshatchFloat{351.5544866466462963217054493725299835205078125}
\def\EQKERatioFirstTwoSingularLowerWhiskerCrosshatchKey{20415}
\def\EQKERatioFirstTwoSingularMaxFloat{1414.5452880859375}
\def\EQKERatioFirstTwoSingularMaxKey{3254}
\def\EQKERatioFirstTwoSingularMeanFloat{877.7696820189621575991623103618621826171875}
\def\EQKERatioFirstTwoSingularMeanKey{104}
\def\EQKERatioFirstTwoSingularMedianFloat{427.5011444091796875}
\def\EQKERatioFirstTwoSingularMedianKey{12457}
\def\EQKERatioFirstTwoSingularMinFloat{335.182342529296875}
\def\EQKERatioFirstTwoSingularMinKey{20415}
\def\EQKERatioFirstTwoSingularQuartileOneFloat{381.34174346923828125}
\def\EQKERatioFirstTwoSingularQuartileOneKey{20415}
\def\EQKERatioFirstTwoSingularQuartileThreeFloat{466.516033172607421875}
\def\EQKERatioFirstTwoSingularQuartileThreeKey{12457}
\def\EQKERatioFirstTwoSingularSqrMeanFloat{809465.632202302687801420688629150390625}
\def\EQKERatioFirstTwoSingularStdDevFloat{197.44877191472443200837005861103534698486328125}
\def\EQKERatioFirstTwoSingularUpperWhiskerCrosshatchFloat{482.4719524080297787804738618433475494384765625}
\def\EQKERatioFirstTwoSingularUpperWhiskerCrosshatchKey{12457}
\def\EQKERatioFirstTwoSingularUpperWhiskerTopEndFloat{489.114247298841291922144591808319091796875}
\def\EQKERatioFirstTwoSingularUpperWhiskerTopEndKey{12457}
\def\EQKESecondSingularLen{151}
\def\EQKESecondSingularMaxFloat{18.2209987640380859375}
\def\EQKESecondSingularMaxKey{20415}
\def\EQKESecondSingularMeanFloat{7.5459218119943383129566427669487893581390380859375}
\def\EQKESecondSingularMeanKey{26829}
\def\EQKESecondSingularMedianFloat{4.63283360004425048828125}
\def\EQKESecondSingularMedianKey{742}
\def\EQKESecondSingularMinFloat{4.526658535003662109375}
\def\EQKESecondSingularMinKey{17197}
\def\EQKESecondSingularStdDevFloat{2.0031817462219319025962249725125730037689208984375}
\def\EQKESingularLen{32}
\def\EQKESingularMaxLen{151}
\def\EQKESingularMaxMaxFloat{8698.4765625}
\def\EQKESingularMaxMaxKey{15622}
\def\EQKESingularMaxMeanFloat{6297.25830078125}
\def\EQKESingularMaxMeanKey{27484}
\def\EQKESingularMaxMedianFloat{4934.405517578125}
\def\EQKESingularMaxMedianKey{9134}
\def\EQKESingularMaxMinFloat{4814.546875}
\def\EQKESingularMaxMinKey{30371}
\def\EQKESingularMaxStdDevFloat{706.64825439453125}
\def\EQKESingularMeanLen{151}
\def\EQKESingularMeanMaxFloat{273.011260986328125}
\def\EQKESingularMeanMaxKey{15622}
\def\EQKESingularMeanMeanFloat{197.7618865966796875}
\def\EQKESingularMeanMeanKey{11598}
\def\EQKESingularMeanMedianFloat{155.153812408447265625}
\def\EQKESingularMeanMedianKey{9134}
\def\EQKESingularMeanMinFloat{151.3971405029296875}
\def\EQKESingularMeanMinKey{30371}
\def\EQKESingularMeanStdDevFloat{22.0969142913818359375}
\def\EQKESingularMedianLen{151}
\def\EQKESingularMedianMaxFloat{0.00755157905397936708713491071875978377647697925567626953125}
\def\EQKESingularMedianMaxKey{17194}
\def\EQKESingularMedianMeanFloat{0.00136569776834992505192001299718640439095906913280487060546875}
\def\EQKESingularMedianMeanKey{20754}
\def\EQKESingularMedianMedianFloat{0.00035523299105989281955475522778442609705962240695953369140625}
\def\EQKESingularMedianMedianKey{15399}
\def\EQKESingularMedianMinFloat{0.0003545758526888675792564098454562326878658495843410491943359375}
\def\EQKESingularMedianMinKey{1696}
\def\EQKESingularMedianStdDevFloat{0.000923968484171337517581179543668667974998243153095245361328125}
\def\EQKESingularMinLen{151}
\def\EQKESingularMinMaxFloat{0.0072115077637135982513427734375}
\def\EQKESingularMinMaxKey{17194}
\def\EQKESingularMinMeanFloat{0.000798790832050144672393798828125}
\def\EQKESingularMinMeanKey{3254}
\def\EQKESingularMinMedianFloat{0.0003321965996292419731616973876953125}
\def\EQKESingularMinMedianKey{20539}
\def\EQKESingularMinMinFloat{0.000311108189634978771209716796875}
\def\EQKESingularMinMinKey{1696}
\def\EQKESingularMinStdDevFloat{0.00084934197366237640380859375}
\def\EQKESingularStdDevLen{151}
\def\EQKESingularStdDevMaxFloat{1513.2601318359375}
\def\EQKESingularStdDevMaxKey{15622}
\def\EQKESingularStdDevMeanFloat{1095.5030517578125}
\def\EQKESingularStdDevMeanKey{27484}
\def\EQKESingularStdDevMedianFloat{858.3800811767578125}
\def\EQKESingularStdDevMedianKey{9134}
\def\EQKESingularStdDevMinFloat{837.52752685546875}
\def\EQKESingularStdDevMinKey{30371}
\def\EQKESingularStdDevStdDevFloat{122.94905853271484375}
\def\EQKESizeDirectionDiffsLen{63}
\def\EQKESizeDirectionDiffsMaxLen{151}
\def\EQKESizeDirectionDiffsMaxMaxFloat{0.82277286052703857421875}
\def\EQKESizeDirectionDiffsMaxMaxKey{15622}
\def\EQKESizeDirectionDiffsMaxMeanFloat{0.094511829316616058349609375}
\def\EQKESizeDirectionDiffsMaxMeanKey{2549}
\def\EQKESizeDirectionDiffsMaxMedianFloat{0.038037501275539398193359375}
\def\EQKESizeDirectionDiffsMaxMedianKey{3254}
\def\EQKESizeDirectionDiffsMaxMinFloat{0.0357802212238311767578125}
\def\EQKESizeDirectionDiffsMaxMinKey{21598}
\def\EQKESizeDirectionDiffsMaxStdDevFloat{0.08869384229183197021484375}
\def\EQKESizeDirectionDiffsMeanLen{151}
\def\EQKESizeDirectionDiffsMeanMaxFloat{0.0087931118905544281005859375}
\def\EQKESizeDirectionDiffsMeanMaxKey{25516}
\def\EQKESizeDirectionDiffsMeanMeanFloat{0.0075827925466001033782958984375}
\def\EQKESizeDirectionDiffsMeanMeanKey{11598}
\def\EQKESizeDirectionDiffsMeanMedianFloat{0.00638845679350197315216064453125}
\def\EQKESizeDirectionDiffsMeanMedianKey{12552}
\def\EQKESizeDirectionDiffsMeanMinFloat{0.0062267859466373920440673828125}
\def\EQKESizeDirectionDiffsMeanMinKey{8840}
\def\EQKESizeDirectionDiffsMeanStdDevFloat{0.00054384558461606502532958984375}
\def\EQKESizeDirectionDiffsMedianLen{151}
\def\EQKESizeDirectionDiffsMedianMaxFloat{-0.0169443301856517791748046875}
\def\EQKESizeDirectionDiffsMedianMaxKey{7790}
\def\EQKESizeDirectionDiffsMedianMeanFloat{-0.059930393370916899831168933587832725606858730316162109375}
\def\EQKESizeDirectionDiffsMedianMeanKey{4157}
\def\EQKESizeDirectionDiffsMedianMedianFloat{-0.438221751302480699852281986750313080847263336181640625}
\def\EQKESizeDirectionDiffsMedianMedianKey{1490}
\def\EQKESizeDirectionDiffsMedianMinFloat{-0.55471023321151735618883549250313080847263336181640625}
\def\EQKESizeDirectionDiffsMedianMinKey{15622}
\def\EQKESizeDirectionDiffsMedianStdDevFloat{0.0636391336150625430700955575957777909934520721435546875}
\def\EQKESizeDirectionDiffsMinLen{151}
\def\EQKESizeDirectionDiffsMinMaxFloat{-0.017316304147243499755859375}
\def\EQKESizeDirectionDiffsMinMaxKey{7790}
\def\EQKESizeDirectionDiffsMinMeanFloat{-0.070963181555271148681640625}
\def\EQKESizeDirectionDiffsMinMeanKey{4157}
\def\EQKESizeDirectionDiffsMinMedianFloat{-0.61609685420989990234375}
\def\EQKESizeDirectionDiffsMinMedianKey{1490}
\def\EQKESizeDirectionDiffsMinMinFloat{-0.7917325496673583984375}
\def\EQKESizeDirectionDiffsMinMinKey{15622}
\def\EQKESizeDirectionDiffsMinStdDevFloat{0.089533604681491851806640625}
\def\EQKESizeDirectionDiffsStdDevLen{151}
\def\EQKESizeDirectionDiffsStdDevMaxFloat{0.14461763203144073486328125}
\def\EQKESizeDirectionDiffsStdDevMaxKey{15622}
\def\EQKESizeDirectionDiffsStdDevMeanFloat{0.02484705857932567596435546875}
\def\EQKESizeDirectionDiffsStdDevMeanKey{23447}
\def\EQKESizeDirectionDiffsStdDevMedianFloat{0.01441724295727908611297607421875}
\def\EQKESizeDirectionDiffsStdDevMedianKey{16149}
\def\EQKESizeDirectionDiffsStdDevMinFloat{0.014396184124052524566650390625}
\def\EQKESizeDirectionDiffsStdDevMinKey{9504}
\def\EQKESizeDirectionDiffsStdDevStdDevFloat{0.014864421449601650238037109375}
\def\EQKESizeDirectionLen{64}
\def\EQKESizeDirectionMaxLen{151}
\def\EQKESizeDirectionMaxMaxFloat{0.4943087100982666015625}
\def\EQKESizeDirectionMaxMaxKey{18146}
\def\EQKESizeDirectionMaxMeanFloat{0.3855786621570587158203125}
\def\EQKESizeDirectionMaxMeanKey{20294}
\def\EQKESizeDirectionMaxMedianFloat{0.275821678340435028076171875}
\def\EQKESizeDirectionMaxMedianKey{12552}
\def\EQKESizeDirectionMaxMinFloat{0.25489139556884765625}
\def\EQKESizeDirectionMaxMinKey{8840}
\def\EQKESizeDirectionMaxStdDevFloat{0.05119991302490234375}
\def\EQKESizeDirectionMeanLen{151}
\def\EQKESizeDirectionMeanMaxFloat{0.03184597194194793701171875}
\def\EQKESizeDirectionMeanMaxKey{18668}
\def\EQKESizeDirectionMeanMeanFloat{-0.0315770022571086883544921875}
\def\EQKESizeDirectionMeanMeanKey{6159}
\def\EQKESizeDirectionMeanMedianFloat{-0.072078905999660491943359375}
\def\EQKESizeDirectionMeanMedianKey{12552}
\def\EQKESizeDirectionMeanMinFloat{-0.07417185604572296142578125}
\def\EQKESizeDirectionMeanMinKey{8840}
\def\EQKESizeDirectionMeanStdDevFloat{0.02346675284206867218017578125}
\def\EQKESizeDirectionMedianLen{151}
\def\EQKESizeDirectionMedianMaxFloat{-0.0500887261331081357074168636245303787291049957275390625}
\def\EQKESizeDirectionMedianMaxKey{18668}
\def\EQKESizeDirectionMedianMeanFloat{-0.11190460268494405171590955205829231999814510345458984375}
\def\EQKESizeDirectionMedianMeanKey{26829}
\def\EQKESizeDirectionMedianMedianFloat{-0.2481112209707498628130650786260957829654216766357421875}
\def\EQKESizeDirectionMedianMedianKey{1490}
\def\EQKESizeDirectionMedianMinFloat{-0.381689549833536145850843013249686919152736663818359375}
\def\EQKESizeDirectionMedianMinKey{15622}
\def\EQKESizeDirectionMedianStdDevFloat{0.030149929645485691598327804285872844047844409942626953125}
\def\EQKESizeDirectionMinLen{151}
\def\EQKESizeDirectionMinMaxFloat{-0.050147615373134613037109375}
\def\EQKESizeDirectionMinMaxKey{18668}
\def\EQKESizeDirectionMinMeanFloat{-0.1145900189876556396484375}
\def\EQKESizeDirectionMinMeanKey{21317}
\def\EQKESizeDirectionMinMedianFloat{-0.33019332587718963623046875}
\def\EQKESizeDirectionMinMedianKey{1490}
\def\EQKESizeDirectionMinMinFloat{-0.516550481319427490234375}
\def\EQKESizeDirectionMinMinKey{15622}
\def\EQKESizeDirectionMinStdDevFloat{0.04037038981914520263671875}
\def\EQKESizeDirectionStdDevLen{151}
\def\EQKESizeDirectionStdDevMaxFloat{0.124998264014720916748046875}
\def\EQKESizeDirectionStdDevMaxKey{5615}
\def\EQKESizeDirectionStdDevMeanFloat{0.11849088966846466064453125}
\def\EQKESizeDirectionStdDevMeanKey{123}
\def\EQKESizeDirectionStdDevMedianFloat{0.10211475379765033721923828125}
\def\EQKESizeDirectionStdDevMedianKey{12552}
\def\EQKESizeDirectionStdDevMinFloat{0.10061578452587127685546875}
\def\EQKESizeDirectionStdDevMinKey{8840}
\def\EQKESizeDirectionStdDevStdDevFloat{0.00609238632023334503173828125}
\def\EQKEThirdSingularLen{151}
\def\EQKEThirdSingularMaxFloat{7.897576808929443359375}
\def\EQKEThirdSingularMaxKey{27714}
\def\EQKEThirdSingularMeanFloat{4.54634334393684458319739860598929226398468017578125}
\def\EQKEThirdSingularMeanKey{29725}
\def\EQKEThirdSingularMedianFloat{3.085546910762786865234375}
\def\EQKEThirdSingularMedianKey{13468}
\def\EQKEThirdSingularMinFloat{3.061284542083740234375}
\def\EQKEThirdSingularMinKey{18668}
\def\EQKEThirdSingularStdDevFloat{0.715571698165331060437210908276028931140899658203125}
\def\EQKEWithAttnScaleFirstSingularLen{151}
\def\EQKEWithAttnScaleFirstSingularMaxFloat{1537.68798828125}
\def\EQKEWithAttnScaleFirstSingularMaxKey{15622}
\def\EQKEWithAttnScaleFirstSingularMeanFloat{1113.208472245576331260963343083858489990234375}
\def\EQKEWithAttnScaleFirstSingularMeanKey{27484}
\def\EQKEWithAttnScaleFirstSingularMedianFloat{872.28790283203125}
\def\EQKEWithAttnScaleFirstSingularMedianKey{9134}
\def\EQKEWithAttnScaleFirstSingularMinFloat{851.09967041015625}
\def\EQKEWithAttnScaleFirstSingularMinKey{30371}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoLen{151}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMaxFloat{2174.6192077255445838090963661670684814453125}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMaxKey{15622}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMeanFloat{1574.314519198327388949110172688961029052734375}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMeanKey{27484}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMedianFloat{1233.601382479043195417034439742565155029296875}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMedianKey{9134}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMinFloat{1203.6366968253141749300993978977203369140625}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMinKey{30371}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoStdDevFloat{176.662089236493415000950335524976253509521484375}
\def\EQKEWithAttnScaleFirstSingularStdDevFloat{124.9189612777074813720901147462427616119384765625}
\def\EQKEWithAttnScaleRatioFirstTwoSingularLen{151}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMaxFloat{1414.5452880859375}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMaxKey{3254}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMeanFloat{877.76968848626347607932984828948974609375}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMeanKey{104}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMedianFloat{427.5011444091796875}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMedianKey{12457}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMinFloat{335.182342529296875}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMinKey{20415}
\def\EQKEWithAttnScaleRatioFirstTwoSingularStdDevFloat{197.448774399689938263691146858036518096923828125}
\def\EQKEWithAttnScaleSecondSingularLen{151}
\def\EQKEWithAttnScaleSecondSingularMaxFloat{3.2210481166839599609375}
\def\EQKEWithAttnScaleSecondSingularMaxKey{20415}
\def\EQKEWithAttnScaleSecondSingularMeanFloat{1.3339431427961943033011493753292597830295562744140625}
\def\EQKEWithAttnScaleSecondSingularMeanKey{26829}
\def\EQKEWithAttnScaleSecondSingularMedianFloat{0.8189770281314849853515625}
\def\EQKEWithAttnScaleSecondSingularMedianKey{742}
\def\EQKEWithAttnScaleSecondSingularMinFloat{0.80020773410797119140625}
\def\EQKEWithAttnScaleSecondSingularMinKey{17197}
\def\EQKEWithAttnScaleSecondSingularStdDevFloat{0.354115861941504406207315014398773200809955596923828125}
\def\EQKEWithAttnScaleSingularLen{32}
\def\EQKEWithAttnScaleSingularMaxLen{151}
\def\EQKEWithAttnScaleSingularMaxMaxFloat{8698.4765625}
\def\EQKEWithAttnScaleSingularMaxMaxKey{15622}
\def\EQKEWithAttnScaleSingularMaxMeanFloat{6297.25830078125}
\def\EQKEWithAttnScaleSingularMaxMeanKey{27484}
\def\EQKEWithAttnScaleSingularMaxMedianFloat{4934.405517578125}
\def\EQKEWithAttnScaleSingularMaxMedianKey{9134}
\def\EQKEWithAttnScaleSingularMaxMinFloat{4814.546875}
\def\EQKEWithAttnScaleSingularMaxMinKey{30371}
\def\EQKEWithAttnScaleSingularMaxStdDevFloat{706.64825439453125}
\def\EQKEWithAttnScaleSingularMeanLen{151}
\def\EQKEWithAttnScaleSingularMeanMaxFloat{273.011260986328125}
\def\EQKEWithAttnScaleSingularMeanMaxKey{15622}
\def\EQKEWithAttnScaleSingularMeanMeanFloat{197.7618865966796875}
\def\EQKEWithAttnScaleSingularMeanMeanKey{11598}
\def\EQKEWithAttnScaleSingularMeanMedianFloat{155.153812408447265625}
\def\EQKEWithAttnScaleSingularMeanMedianKey{9134}
\def\EQKEWithAttnScaleSingularMeanMinFloat{151.3971405029296875}
\def\EQKEWithAttnScaleSingularMeanMinKey{30371}
\def\EQKEWithAttnScaleSingularMeanStdDevFloat{22.0969142913818359375}
\def\EQKEWithAttnScaleSingularMedianLen{151}
\def\EQKEWithAttnScaleSingularMedianMaxFloat{0.00755157905397936708713491071875978377647697925567626953125}
\def\EQKEWithAttnScaleSingularMedianMaxKey{17194}
\def\EQKEWithAttnScaleSingularMedianMeanFloat{0.00136569776834992505192001299718640439095906913280487060546875}
\def\EQKEWithAttnScaleSingularMedianMeanKey{20754}
\def\EQKEWithAttnScaleSingularMedianMedianFloat{0.00035523299105989281955475522778442609705962240695953369140625}
\def\EQKEWithAttnScaleSingularMedianMedianKey{15399}
\def\EQKEWithAttnScaleSingularMedianMinFloat{0.0003545758526888675792564098454562326878658495843410491943359375}
\def\EQKEWithAttnScaleSingularMedianMinKey{1696}
\def\EQKEWithAttnScaleSingularMedianStdDevFloat{0.000923968484171337517581179543668667974998243153095245361328125}
\def\EQKEWithAttnScaleSingularMinLen{151}
\def\EQKEWithAttnScaleSingularMinMaxFloat{0.0072115077637135982513427734375}
\def\EQKEWithAttnScaleSingularMinMaxKey{17194}
\def\EQKEWithAttnScaleSingularMinMeanFloat{0.000798790832050144672393798828125}
\def\EQKEWithAttnScaleSingularMinMeanKey{3254}
\def\EQKEWithAttnScaleSingularMinMedianFloat{0.0003321965996292419731616973876953125}
\def\EQKEWithAttnScaleSingularMinMedianKey{20539}
\def\EQKEWithAttnScaleSingularMinMinFloat{0.000311108189634978771209716796875}
\def\EQKEWithAttnScaleSingularMinMinKey{1696}
\def\EQKEWithAttnScaleSingularMinStdDevFloat{0.00084934197366237640380859375}
\def\EQKEWithAttnScaleSingularStdDevLen{151}
\def\EQKEWithAttnScaleSingularStdDevMaxFloat{1513.2601318359375}
\def\EQKEWithAttnScaleSingularStdDevMaxKey{15622}
\def\EQKEWithAttnScaleSingularStdDevMeanFloat{1095.5030517578125}
\def\EQKEWithAttnScaleSingularStdDevMeanKey{27484}
\def\EQKEWithAttnScaleSingularStdDevMedianFloat{858.3800811767578125}
\def\EQKEWithAttnScaleSingularStdDevMedianKey{9134}
\def\EQKEWithAttnScaleSingularStdDevMinFloat{837.52752685546875}
\def\EQKEWithAttnScaleSingularStdDevMinKey{30371}
\def\EQKEWithAttnScaleSingularStdDevStdDevFloat{122.94905853271484375}
\def\EQKEWithAttnScaleThirdSingularLen{151}
\def\EQKEWithAttnScaleThirdSingularMaxFloat{1.39610755443572998046875}
\def\EQKEWithAttnScaleThirdSingularMaxKey{27714}
\def\EQKEWithAttnScaleThirdSingularMeanFloat{0.80368756616352410304671138874255120754241943359375}
\def\EQKEWithAttnScaleThirdSingularMeanKey{29725}
\def\EQKEWithAttnScaleThirdSingularMedianFloat{0.54545278847217559814453125}
\def\EQKEWithAttnScaleThirdSingularMedianKey{13468}
\def\EQKEWithAttnScaleThirdSingularMinFloat{0.54116380214691162109375}
\def\EQKEWithAttnScaleThirdSingularMinKey{18668}
\def\EQKEWithAttnScaleThirdSingularStdDevFloat{0.1264964018423887226472146494415937922894954681396484375}
\def\EQKPAbsLen{1280}
\def\EQKPAbsMaxLen{151}
\def\EQKPAbsMaxMaxFloat{20.3558979034423828125}
\def\EQKPAbsMaxMaxKey{3284}
\def\EQKPAbsMaxMeanFloat{6.225250244140625}
\def\EQKPAbsMaxMeanKey{29052}
\def\EQKPAbsMaxMedianFloat{2.013036787509918212890625}
\def\EQKPAbsMaxMedianKey{16069}
\def\EQKPAbsMaxMinFloat{1.73710918426513671875}
\def\EQKPAbsMaxMinKey{26278}
\def\EQKPAbsMaxStdDevFloat{3.2332503795623779296875}
\def\EQKPAbsMeanLen{151}
\def\EQKPAbsMeanMaxFloat{5.19438457489013671875}
\def\EQKPAbsMeanMaxKey{3284}
\def\EQKPAbsMeanMeanFloat{1.6531369686126708984375}
\def\EQKPAbsMeanMeanKey{4800}
\def\EQKPAbsMeanMedianFloat{0.456141136586666107177734375}
\def\EQKPAbsMeanMedianKey{18146}
\def\EQKPAbsMeanMinFloat{0.447037518024444580078125}
\def\EQKPAbsMeanMinKey{26278}
\def\EQKPAbsMeanStdDevFloat{0.7974002361297607421875}
\def\EQKPAbsMedianLen{151}
\def\EQKPAbsMedianMaxFloat{1.23344153821468349718770696199499070644378662109375}
\def\EQKPAbsMedianMaxKey{8299}
\def\EQKPAbsMedianMeanFloat{0.0661791443123616318633395394499530084431171417236328125}
\def\EQKPAbsMedianMeanKey{20976}
\def\EQKPAbsMedianMedianFloat{0.001944120357657084206814968041499014361761510372161865234375}
\def\EQKPAbsMedianMedianKey{12561}
\def\EQKPAbsMedianMinFloat{0.001634901008219458336256924013696334441192448139190673828125}
\def\EQKPAbsMedianMinKey{16284}
\def\EQKPAbsMedianStdDevFloat{0.14347841475829470336833537658094428479671478271484375}
\def\EQKPAbsMinLen{151}
\def\EQKPAbsMinMaxFloat{0.89260399341583251953125}
\def\EQKPAbsMinMaxKey{8299}
\def\EQKPAbsMinMeanFloat{0.02580664865672588348388671875}
\def\EQKPAbsMinMeanKey{1696}
\def\EQKPAbsMinMedianFloat{0.000013152946621630690060555934906005859375}
\def\EQKPAbsMinMedianKey{7467}
\def\EQKPAbsMinMinFloat{0.0000131298029373283497989177703857421875}
\def\EQKPAbsMinMinKey{18668}
\def\EQKPAbsMinStdDevFloat{0.10479195415973663330078125}
\def\EQKPAbsStdDevLen{151}
\def\EQKPAbsStdDevMaxFloat{4.186350345611572265625}
\def\EQKPAbsStdDevMaxKey{3284}
\def\EQKPAbsStdDevMeanFloat{1.23618805408477783203125}
\def\EQKPAbsStdDevMeanKey{29725}
\def\EQKPAbsStdDevMedianFloat{0.43990440666675567626953125}
\def\EQKPAbsStdDevMedianKey{6910}
\def\EQKPAbsStdDevMinFloat{0.338156282901763916015625}
\def\EQKPAbsStdDevMinKey{26278}
\def\EQKPAbsStdDevStdDevFloat{0.585805118083953857421875}
\def\EQKPLen{1280}
\def\EQKPMaxLen{151}
\def\EQKPMaxMaxFloat{20.3558979034423828125}
\def\EQKPMaxMaxKey{3284}
\def\EQKPMaxMeanFloat{5.628391265869140625}
\def\EQKPMaxMeanKey{6155}
\def\EQKPMaxMedianFloat{1.601188123226165771484375}
\def\EQKPMaxMedianKey{8048}
\def\EQKPMaxMinFloat{1.2665655612945556640625}
\def\EQKPMaxMinKey{26278}
\def\EQKPMaxRowDiffLen{64}
\def\EQKPMaxRowDiffMaxLen{151}
\def\EQKPMaxRowDiffMaxMaxFloat{37.13187408447265625}
\def\EQKPMaxRowDiffMaxMaxKey{50}
\def\EQKPMaxRowDiffMaxMeanFloat{10.831920623779296875}
\def\EQKPMaxRowDiffMaxMeanKey{17080}
\def\EQKPMaxRowDiffMaxMedianFloat{3.634555876255035400390625}
\def\EQKPMaxRowDiffMaxMedianKey{16069}
\def\EQKPMaxRowDiffMaxMinFloat{3.0036747455596923828125}
\def\EQKPMaxRowDiffMaxMinKey{26278}
\def\EQKPMaxRowDiffMaxStdDevFloat{5.453211307525634765625}
\def\EQKPMaxRowDiffMeanLen{151}
\def\EQKPMaxRowDiffMeanMaxFloat{28.04830169677734375}
\def\EQKPMaxRowDiffMeanMaxKey{3284}
\def\EQKPMaxRowDiffMeanMeanFloat{8.1563568115234375}
\def\EQKPMaxRowDiffMeanMeanKey{5781}
\def\EQKPMaxRowDiffMeanMedianFloat{2.842803657054901123046875}
\def\EQKPMaxRowDiffMeanMedianKey{6910}
\def\EQKPMaxRowDiffMeanMinFloat{2.0850837230682373046875}
\def\EQKPMaxRowDiffMeanMinKey{26278}
\def\EQKPMaxRowDiffMeanStdDevFloat{3.936489582061767578125}
\def\EQKPMaxRowDiffMedianLen{151}
\def\EQKPMaxRowDiffMedianMaxFloat{21.505544338226318501483547152020037174224853515625}
\def\EQKPMaxRowDiffMedianMaxKey{3284}
\def\EQKPMaxRowDiffMedianMeanFloat{6.20994444932369216161305303103290498256683349609375}
\def\EQKPMaxRowDiffMedianMeanKey{18668}
\def\EQKPMaxRowDiffMedianMedianFloat{1.875412253141403251532892682007513940334320068359375}
\def\EQKPMaxRowDiffMedianMedianKey{27714}
\def\EQKPMaxRowDiffMedianMinFloat{1.7566563045978547119574386670137755572795867919921875}
\def\EQKPMaxRowDiffMedianMinKey{26278}
\def\EQKPMaxRowDiffMedianStdDevFloat{3.0653267662420233818920678459107875823974609375}
\def\EQKPMaxRowDiffMinLen{151}
\def\EQKPMaxRowDiffMinMaxFloat{21.288120269775390625}
\def\EQKPMaxRowDiffMinMaxKey{3284}
\def\EQKPMaxRowDiffMinMeanFloat{6.058154582977294921875}
\def\EQKPMaxRowDiffMinMeanKey{23633}
\def\EQKPMaxRowDiffMinMedianFloat{1.8389036655426025390625}
\def\EQKPMaxRowDiffMinMedianKey{27714}
\def\EQKPMaxRowDiffMinMinFloat{1.74803829193115234375}
\def\EQKPMaxRowDiffMinMinKey{26278}
\def\EQKPMaxRowDiffMinStdDevFloat{3.0445630550384521484375}
\def\EQKPMaxRowDiffStdDevLen{151}
\def\EQKPMaxRowDiffStdDevMaxFloat{3.0663068294525146484375}
\def\EQKPMaxRowDiffStdDevMaxKey{50}
\def\EQKPMaxRowDiffStdDevMeanFloat{0.837051570415496826171875}
\def\EQKPMaxRowDiffStdDevMeanKey{8840}
\def\EQKPMaxRowDiffStdDevMedianFloat{0.2413499914109706878662109375}
\def\EQKPMaxRowDiffStdDevMedianKey{6910}
\def\EQKPMaxRowDiffStdDevMinFloat{0.2209974229335784912109375}
\def\EQKPMaxRowDiffStdDevMinKey{26278}
\def\EQKPMaxRowDiffStdDevStdDevFloat{0.439102470874786376953125}
\def\EQKPMaxStdDevFloat{3.154026031494140625}
\def\EQKPMeanLen{151}
\def\EQKPMeanMaxFloat{0.000002451986119922366924583911895751953125}
\def\EQKPMeanMaxKey{1490}
\def\EQKPMeanMeanFloat{-0.000000015168222233796768705360591411590576171875}
\def\EQKPMeanMeanKey{2773}
\def\EQKPMeanMedianFloat{-0.000001617893531147274188697338104248046875}
\def\EQKPMeanMedianKey{8048}
\def\EQKPMeanMinFloat{-0.000001930817916218074969947338104248046875}
\def\EQKPMeanMinKey{27584}
\def\EQKPMeanStdDevFloat{0.00000070468382773469784297049045562744140625}
\def\EQKPMedianLen{151}
\def\EQKPMedianMaxFloat{-1.440967570543289166806744105997495353221893310546875}
\def\EQKPMedianMaxKey{26278}
\def\EQKPMedianMeanFloat{-4.4469669538460028235249410499818623065948486328125}
\def\EQKPMedianMeanKey{9134}
\def\EQKPMedianMedianFloat{-13.500315945148468443903766456060111522674560546875}
\def\EQKPMedianMedianKey{3284}
\def\EQKPMedianMinFloat{-14.6733789062499990762944435118697583675384521484375}
\def\EQKPMedianMinKey{50}
\def\EQKPMedianStdDevFloat{2.14912816969453235316223072004504501819610595703125}
\def\EQKPMinLen{151}
\def\EQKPMinMaxFloat{-1.73710918426513671875}
\def\EQKPMinMaxKey{26278}
\def\EQKPMinMeanFloat{-5.231881618499755859375}
\def\EQKPMinMeanKey{31308}
\def\EQKPMinMedianFloat{-16.387892246246337890625}
\def\EQKPMinMedianKey{19538}
\def\EQKPMinMinFloat{-19.415576934814453125}
\def\EQKPMinMinKey{50}
\def\EQKPMinStdDevFloat{2.7120263576507568359375}
\def\EQKPStdDevLen{151}
\def\EQKPStdDevMaxFloat{6.67136859893798828125}
\def\EQKPStdDevMaxKey{3284}
\def\EQKPStdDevMeanFloat{2.071108341217041015625}
\def\EQKPStdDevMeanKey{23633}
\def\EQKPStdDevMedianFloat{0.6433396041393280029296875}
\def\EQKPStdDevMedianKey{18146}
\def\EQKPStdDevMinFloat{0.560528457164764404296875}
\def\EQKPStdDevMinKey{26278}
\def\EQKPStdDevStdDevFloat{0.974960267543792724609375}
\def\EQKPWithAttnScaleAbsLen{1280}
\def\EQKPWithAttnScaleAbsMaxLen{151}
\def\EQKPWithAttnScaleAbsMaxMaxFloat{3.5984485149383544921875}
\def\EQKPWithAttnScaleAbsMaxMaxKey{3284}
\def\EQKPWithAttnScaleAbsMaxMeanFloat{1.1004791259765625}
\def\EQKPWithAttnScaleAbsMaxMeanKey{29052}
\def\EQKPWithAttnScaleAbsMaxMedianFloat{0.3558579981327056884765625}
\def\EQKPWithAttnScaleAbsMaxMedianKey{16069}
\def\EQKPWithAttnScaleAbsMaxMinFloat{0.3070804178714752197265625}
\def\EQKPWithAttnScaleAbsMaxMinKey{26278}
\def\EQKPWithAttnScaleAbsMaxStdDevFloat{0.57156336307525634765625}
\def\EQKPWithAttnScaleAbsMeanLen{151}
\def\EQKPWithAttnScaleAbsMeanMaxFloat{0.918246090412139892578125}
\def\EQKPWithAttnScaleAbsMeanMaxKey{3284}
\def\EQKPWithAttnScaleAbsMeanMeanFloat{0.2922360897064208984375}
\def\EQKPWithAttnScaleAbsMeanMeanKey{4800}
\def\EQKPWithAttnScaleAbsMeanMedianFloat{0.080635122954845428466796875}
\def\EQKPWithAttnScaleAbsMeanMedianKey{18146}
\def\EQKPWithAttnScaleAbsMeanMinFloat{0.07902581989765167236328125}
\def\EQKPWithAttnScaleAbsMeanMinKey{26278}
\def\EQKPWithAttnScaleAbsMeanStdDevFloat{0.14096178114414215087890625}
\def\EQKPWithAttnScaleAbsMedianLen{151}
\def\EQKPWithAttnScaleAbsMedianMaxFloat{0.2180437162518501226227130018742172978818416595458984375}
\def\EQKPWithAttnScaleAbsMedianMaxKey{8299}
\def\EQKPWithAttnScaleAbsMedianMeanFloat{0.011698930616938087168055204756456078030169010162353515625}
\def\EQKPWithAttnScaleAbsMedianMeanKey{20976}
\def\EQKPWithAttnScaleAbsMedianMedianFloat{0.0003436751841945806409776842382797212849254719913005828857421875}
\def\EQKPWithAttnScaleAbsMedianMedianKey{12561}
\def\EQKPWithAttnScaleAbsMedianMinFloat{0.0002890124046825804184947250607962132562533952295780181884765625}
\def\EQKPWithAttnScaleAbsMedianMinKey{16284}
\def\EQKPWithAttnScaleAbsMedianStdDevFloat{0.0253636401494782039167663612033720710314810276031494140625}
\def\EQKPWithAttnScaleAbsMinLen{151}
\def\EQKPWithAttnScaleAbsMinMaxFloat{0.1577915847301483154296875}
\def\EQKPWithAttnScaleAbsMinMaxKey{8299}
\def\EQKPWithAttnScaleAbsMinMeanFloat{0.004562013782560825347900390625}
\def\EQKPWithAttnScaleAbsMinMeanKey{1696}
\def\EQKPWithAttnScaleAbsMinMedianFloat{0.00000232513440323600661940872669219970703125}
\def\EQKPWithAttnScaleAbsMinMedianKey{7467}
\def\EQKPWithAttnScaleAbsMinMinFloat{0.000002321043211850337684154510498046875}
\def\EQKPWithAttnScaleAbsMinMinKey{18668}
\def\EQKPWithAttnScaleAbsMinStdDevFloat{0.01852477528154850006103515625}
\def\EQKPWithAttnScaleAbsStdDevLen{151}
\def\EQKPWithAttnScaleAbsStdDevMaxFloat{0.7400491237640380859375}
\def\EQKPWithAttnScaleAbsStdDevMaxKey{3284}
\def\EQKPWithAttnScaleAbsStdDevMeanFloat{0.2185292541980743408203125}
\def\EQKPWithAttnScaleAbsStdDevMeanKey{29725}
\def\EQKPWithAttnScaleAbsStdDevMedianFloat{0.0777648501098155975341796875}
\def\EQKPWithAttnScaleAbsStdDevMedianKey{6910}
\def\EQKPWithAttnScaleAbsStdDevMinFloat{0.059778146445751190185546875}
\def\EQKPWithAttnScaleAbsStdDevMinKey{26278}
\def\EQKPWithAttnScaleAbsStdDevStdDevFloat{0.103556692600250244140625}
\def\EQKPWithAttnScaleLen{1280}
\def\EQKPWithAttnScaleMaxLen{151}
\def\EQKPWithAttnScaleMaxMaxFloat{3.5984485149383544921875}
\def\EQKPWithAttnScaleMaxMaxKey{3284}
\def\EQKPWithAttnScaleMaxMeanFloat{0.994968354701995849609375}
\def\EQKPWithAttnScaleMaxMeanKey{6155}
\def\EQKPWithAttnScaleMaxMedianFloat{0.28305275738239288330078125}
\def\EQKPWithAttnScaleMaxMedianKey{8048}
\def\EQKPWithAttnScaleMaxMinFloat{0.2238992750644683837890625}
\def\EQKPWithAttnScaleMaxMinKey{26278}
\def\EQKPWithAttnScaleMaxRowDiffLen{64}
\def\EQKPWithAttnScaleMaxRowDiffMaxLen{151}
\def\EQKPWithAttnScaleMaxRowDiffMaxMaxFloat{6.5640506744384765625}
\def\EQKPWithAttnScaleMaxRowDiffMaxMaxKey{50}
\def\EQKPWithAttnScaleMaxRowDiffMaxMeanFloat{1.9148309230804443359375}
\def\EQKPWithAttnScaleMaxRowDiffMaxMeanKey{17080}
\def\EQKPWithAttnScaleMaxRowDiffMaxMedianFloat{0.64250482618808746337890625}
\def\EQKPWithAttnScaleMaxRowDiffMaxMedianKey{16069}
\def\EQKPWithAttnScaleMaxRowDiffMaxMinFloat{0.530979692935943603515625}
\def\EQKPWithAttnScaleMaxRowDiffMaxMinKey{26278}
\def\EQKPWithAttnScaleMaxRowDiffMaxStdDevFloat{0.964000642299652099609375}
\def\EQKPWithAttnScaleMaxRowDiffMeanLen{151}
\def\EQKPWithAttnScaleMaxRowDiffMeanMaxFloat{4.958285808563232421875}
\def\EQKPWithAttnScaleMaxRowDiffMeanMaxKey{3284}
\def\EQKPWithAttnScaleMaxRowDiffMeanMeanFloat{1.44185388088226318359375}
\def\EQKPWithAttnScaleMaxRowDiffMeanMeanKey{5781}
\def\EQKPWithAttnScaleMaxRowDiffMeanMedianFloat{0.50254142284393310546875}
\def\EQKPWithAttnScaleMaxRowDiffMeanMedianKey{6910}
\def\EQKPWithAttnScaleMaxRowDiffMeanMinFloat{0.368594229221343994140625}
\def\EQKPWithAttnScaleMaxRowDiffMeanMinKey{26278}
\def\EQKPWithAttnScaleMaxRowDiffMeanStdDevFloat{0.69587957859039306640625}
\def\EQKPWithAttnScaleMaxRowDiffMedianLen{151}
\def\EQKPWithAttnScaleMaxRowDiffMedianMaxFloat{3.801679239273071164717521241982467472553253173828125}
\def\EQKPWithAttnScaleMaxRowDiffMedianMaxKey{3284}
\def\EQKPWithAttnScaleMaxRowDiffMedianMeanFloat{1.097773473460153415004469934501685202121734619140625}
\def\EQKPWithAttnScaleMaxRowDiffMedianMeanKey{18668}
\def\EQKPWithAttnScaleMaxRowDiffMedianMedianFloat{0.3315291845053434105494716277462430298328399658203125}
\def\EQKPWithAttnScaleMaxRowDiffMedianMedianKey{27714}
\def\EQKPWithAttnScaleMaxRowDiffMedianMinFloat{0.310535902678966524437242924250313080847263336181640625}
\def\EQKPWithAttnScaleMaxRowDiffMedianMinKey{26278}
\def\EQKPWithAttnScaleMaxRowDiffMedianStdDevFloat{0.54187834492045261480797080366755835711956024169921875}
\def\EQKPWithAttnScaleMaxRowDiffMinLen{151}
\def\EQKPWithAttnScaleMaxRowDiffMinMaxFloat{3.7632439136505126953125}
\def\EQKPWithAttnScaleMaxRowDiffMinMaxKey{3284}
\def\EQKPWithAttnScaleMaxRowDiffMinMeanFloat{1.070940494537353515625}
\def\EQKPWithAttnScaleMaxRowDiffMinMeanKey{23633}
\def\EQKPWithAttnScaleMaxRowDiffMinMedianFloat{0.325075320899486541748046875}
\def\EQKPWithAttnScaleMaxRowDiffMinMedianKey{27714}
\def\EQKPWithAttnScaleMaxRowDiffMinMinFloat{0.3090124428272247314453125}
\def\EQKPWithAttnScaleMaxRowDiffMinMinKey{26278}
\def\EQKPWithAttnScaleMaxRowDiffMinStdDevFloat{0.538207828998565673828125}
\def\EQKPWithAttnScaleMaxRowDiffStdDevLen{151}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMaxFloat{0.54205167293548583984375}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMaxKey{50}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMeanFloat{0.147971212863922119140625}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMeanKey{8840}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMedianFloat{0.04266505129635334014892578125}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMedianKey{6910}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMinFloat{0.0390671975910663604736328125}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMinKey{26278}
\def\EQKPWithAttnScaleMaxRowDiffStdDevStdDevFloat{0.07762308418750762939453125}
\def\EQKPWithAttnScaleMaxStdDevFloat{0.5575582981109619140625}
\def\EQKPWithAttnScaleMeanLen{151}
\def\EQKPWithAttnScaleMeanMaxFloat{0.000000431574875392470858059823513031005859375}
\def\EQKPWithAttnScaleMeanMaxKey{1490}
\def\EQKPWithAttnScaleMeanMeanFloat{-0.0000000026023059263025061227381229400634765625}
\def\EQKPWithAttnScaleMeanMeanKey{2773}
\def\EQKPWithAttnScaleMeanMedianFloat{-0.000000286543212268952629528939723968505859375}
\def\EQKPWithAttnScaleMeanMedianKey{8048}
\def\EQKPWithAttnScaleMeanMinFloat{-0.00000034198166076748748309910297393798828125}
\def\EQKPWithAttnScaleMeanMinKey{27584}
\def\EQKPWithAttnScaleMeanStdDevFloat{0.0000001245308567376923747360706329345703125}
\def\EQKPWithAttnScaleMedianLen{151}
\def\EQKPWithAttnScaleMedianMaxFloat{-0.254729486703872687325400647750939242541790008544921875}
\def\EQKPWithAttnScaleMedianMaxKey{26278}
\def\EQKPWithAttnScaleMedianMeanFloat{-0.78612013230655353179798794371890835464000701904296875}
\def\EQKPWithAttnScaleMedianMeanKey{9134}
\def\EQKPWithAttnScaleMedianMedianFloat{-2.386541213095188407322666535037569701671600341796875}
\def\EQKPWithAttnScaleMedianMedianKey{3284}
\def\EQKPWithAttnScaleMedianMinFloat{-2.593911529779434399500814834027551114559173583984375}
\def\EQKPWithAttnScaleMedianMinKey{50}
\def\EQKPWithAttnScaleMedianStdDevFloat{0.379915779663264785437348791674594394862651824951171875}
\def\EQKPWithAttnScaleMinLen{151}
\def\EQKPWithAttnScaleMinMaxFloat{-0.3070804178714752197265625}
\def\EQKPWithAttnScaleMinMaxKey{26278}
\def\EQKPWithAttnScaleMinMeanFloat{-0.924874842166900634765625}
\def\EQKPWithAttnScaleMinMeanKey{31308}
\def\EQKPWithAttnScaleMinMedianFloat{-2.89699757099151611328125}
\def\EQKPWithAttnScaleMinMedianKey{19538}
\def\EQKPWithAttnScaleMinMinFloat{-3.4322216510772705078125}
\def\EQKPWithAttnScaleMinMinKey{50}
\def\EQKPWithAttnScaleMinStdDevFloat{0.4794230759143829345703125}
\def\EQKPWithAttnScaleStdDevLen{151}
\def\EQKPWithAttnScaleStdDevMaxFloat{1.1793425083160400390625}
\def\EQKPWithAttnScaleStdDevMaxKey{3284}
\def\EQKPWithAttnScaleStdDevMeanFloat{0.366123676300048828125}
\def\EQKPWithAttnScaleStdDevMeanKey{23633}
\def\EQKPWithAttnScaleStdDevMedianFloat{0.1137274540960788726806640625}
\def\EQKPWithAttnScaleStdDevMedianKey{18146}
\def\EQKPWithAttnScaleStdDevMinFloat{0.099088370800018310546875}
\def\EQKPWithAttnScaleStdDevMinKey{26278}
\def\EQKPWithAttnScaleStdDevStdDevFloat{0.1723502576351165771484375}
\def\EUPUAbsLenLen{151}
\def\EUPUAbsLenMaxFloat{4096}
\def\EUPUAbsLenMaxKey{50}
\def\EUPUAbsLenMeanFloat{4096}
\def\EUPUAbsLenMeanKey{50}
\def\EUPUAbsLenMedianFloat{4096}
\def\EUPUAbsLenMedianKey{50}
\def\EUPUAbsLenMinFloat{4096}
\def\EUPUAbsLenMinKey{50}
\def\EUPUAbsLenStdDevFloat{0}
\def\EUPUAbsMaxLen{151}
\def\EUPUAbsMaxMaxFloat{5.653759479522705078125}
\def\EUPUAbsMaxMaxKey{1490}
\def\EUPUAbsMaxMeanFloat{2.341329097747802734375}
\def\EUPUAbsMaxMeanKey{29195}
\def\EUPUAbsMaxMedianFloat{1.785548746585845947265625}
\def\EUPUAbsMaxMedianKey{11598}
\def\EUPUAbsMaxMinFloat{1.7567684650421142578125}
\def\EUPUAbsMaxMinKey{8299}
\def\EUPUAbsMaxStdDevFloat{0.507970869541168212890625}
\def\EUPUAbsMeanLen{151}
\def\EUPUAbsMeanMaxFloat{1.133113384246826171875}
\def\EUPUAbsMeanMaxKey{11611}
\def\EUPUAbsMeanMeanFloat{0.8306787014007568359375}
\def\EUPUAbsMeanMeanKey{28778}
\def\EUPUAbsMeanMedianFloat{0.62788569927215576171875}
\def\EUPUAbsMeanMedianKey{6589}
\def\EUPUAbsMeanMinFloat{0.6014358997344970703125}
\def\EUPUAbsMeanMinKey{19488}
\def\EUPUAbsMeanStdDevFloat{0.09180362522602081298828125}
\def\EUPUAbsMedianLen{151}
\def\EUPUAbsMedianMaxFloat{0.04006397416815161982572846000039135105907917022705078125}
\def\EUPUAbsMedianMaxKey{6910}
\def\EUPUAbsMedianMeanFloat{0.015722679394291137755512721696504740975797176361083984375}
\def\EUPUAbsMedianMeanKey{5358}
\def\EUPUAbsMedianMedianFloat{0.00636410143342800403709613732416983111761510372161865234375}
\def\EUPUAbsMedianMedianKey{24566}
\def\EUPUAbsMedianMinFloat{0.00595716354437172447566783972661141888238489627838134765625}
\def\EUPUAbsMedianMinKey{30684}
\def\EUPUAbsMedianStdDevFloat{0.006372710152549553898337908464100109995342791080474853515625}
\def\EUPUAbsMinLen{151}
\def\EUPUAbsMinMaxFloat{0.0040351427160203456878662109375}
\def\EUPUAbsMinMaxKey{2345}
\def\EUPUAbsMinMeanFloat{0.00071963411755859851837158203125}
\def\EUPUAbsMinMeanKey{4810}
\def\EUPUAbsMinMedianFloat{0.000006806230658185086213052272796630859375}
\def\EUPUAbsMinMedianKey{16149}
\def\EUPUAbsMinMinFloat{0.00000445844443675014190375804901123046875}
\def\EUPUAbsMinMinKey{16284}
\def\EUPUAbsMinStdDevFloat{0.00063408375717699527740478515625}
\def\EUPUAbsStdDevLen{151}
\def\EUPUAbsStdDevMaxFloat{0.565749466419219970703125}
\def\EUPUAbsStdDevMaxKey{19538}
\def\EUPUAbsStdDevMeanFloat{0.3854966461658477783203125}
\def\EUPUAbsStdDevMeanKey{30684}
\def\EUPUAbsStdDevMedianFloat{0.30876363813877105712890625}
\def\EUPUAbsStdDevMedianKey{32382}
\def\EUPUAbsStdDevMinFloat{0.2909755408763885498046875}
\def\EUPUAbsStdDevMinKey{32103}
\def\EUPUAbsStdDevStdDevFloat{0.040300540626049041748046875}
\def\EUPULenLen{151}
\def\EUPULenMaxFloat{4096}
\def\EUPULenMaxKey{50}
\def\EUPULenMeanFloat{4096}
\def\EUPULenMeanKey{50}
\def\EUPULenMedianFloat{4096}
\def\EUPULenMedianKey{50}
\def\EUPULenMinFloat{4096}
\def\EUPULenMinKey{50}
\def\EUPULenStdDevFloat{0}
\def\EUPUMaxLen{151}
\def\EUPUMaxMaxFloat{5.653759479522705078125}
\def\EUPUMaxMaxKey{1490}
\def\EUPUMaxMeanFloat{2.1531469821929931640625}
\def\EUPUMaxMeanKey{29565}
\def\EUPUMaxMedianFloat{1.5287362039089202880859375}
\def\EUPUMaxMedianKey{4305}
\def\EUPUMaxMinFloat{1.44220125675201416015625}
\def\EUPUMaxMinKey{9504}
\def\EUPUMaxRowDiffLenLen{151}
\def\EUPUMaxRowDiffLenMaxFloat{64}
\def\EUPUMaxRowDiffLenMaxKey{50}
\def\EUPUMaxRowDiffLenMeanFloat{64}
\def\EUPUMaxRowDiffLenMeanKey{50}
\def\EUPUMaxRowDiffLenMedianFloat{64}
\def\EUPUMaxRowDiffLenMedianKey{50}
\def\EUPUMaxRowDiffLenMinFloat{64}
\def\EUPUMaxRowDiffLenMinKey{50}
\def\EUPUMaxRowDiffLenStdDevFloat{0}
\def\EUPUMaxRowDiffMaxLen{151}
\def\EUPUMaxRowDiffMaxMaxFloat{9.20347499847412109375}
\def\EUPUMaxRowDiffMaxMaxKey{19538}
\def\EUPUMaxRowDiffMaxMeanFloat{4.21749591827392578125}
\def\EUPUMaxRowDiffMaxMeanKey{29565}
\def\EUPUMaxRowDiffMaxMedianFloat{3.3031599521636962890625}
\def\EUPUMaxRowDiffMaxMedianKey{11598}
\def\EUPUMaxRowDiffMaxMinFloat{3.287174701690673828125}
\def\EUPUMaxRowDiffMaxMinKey{32103}
\def\EUPUMaxRowDiffMaxStdDevFloat{0.819586813449859619140625}
\def\EUPUMaxRowDiffMeanLen{151}
\def\EUPUMaxRowDiffMeanMaxFloat{3.95758342742919921875}
\def\EUPUMaxRowDiffMeanMaxKey{19538}
\def\EUPUMaxRowDiffMeanMeanFloat{2.913945674896240234375}
\def\EUPUMaxRowDiffMeanMeanKey{16149}
\def\EUPUMaxRowDiffMeanMedianFloat{2.38592636585235595703125}
\def\EUPUMaxRowDiffMeanMedianKey{6589}
\def\EUPUMaxRowDiffMeanMinFloat{2.36717128753662109375}
\def\EUPUMaxRowDiffMeanMinKey{20415}
\def\EUPUMaxRowDiffMeanStdDevFloat{0.275375425815582275390625}
\def\EUPUMaxRowDiffMedianLen{151}
\def\EUPUMaxRowDiffMedianMaxFloat{3.175216199159622387782064834027551114559173583984375}
\def\EUPUMaxRowDiffMedianMaxKey{11611}
\def\EUPUMaxRowDiffMedianMeanFloat{2.29640750957245831642694611218757927417755126953125}
\def\EUPUMaxRowDiffMedianMeanKey{6159}
\def\EUPUMaxRowDiffMedianMedianFloat{1.759941592216491823563728758017532527446746826171875}
\def\EUPUMaxRowDiffMedianMedianKey{20415}
\def\EUPUMaxRowDiffMedianMinFloat{1.744481089115142768974919817992486059665679931640625}
\def\EUPUMaxRowDiffMedianMinKey{24566}
\def\EUPUMaxRowDiffMedianStdDevFloat{0.252796730497298949291717917731148190796375274658203125}
\def\EUPUMaxRowDiffMinLen{151}
\def\EUPUMaxRowDiffMinMaxFloat{3.1242275238037109375}
\def\EUPUMaxRowDiffMinMaxKey{11611}
\def\EUPUMaxRowDiffMinMeanFloat{2.2646000385284423828125}
\def\EUPUMaxRowDiffMinMeanKey{29726}
\def\EUPUMaxRowDiffMinMedianFloat{1.7358996570110321044921875}
\def\EUPUMaxRowDiffMinMedianKey{24566}
\def\EUPUMaxRowDiffMinMinFloat{1.72963392734527587890625}
\def\EUPUMaxRowDiffMinMinKey{19093}
\def\EUPUMaxRowDiffMinStdDevFloat{0.2588231563568115234375}
\def\EUPUMaxRowDiffStdDevLen{151}
\def\EUPUMaxRowDiffStdDevMaxFloat{0.786122739315032958984375}
\def\EUPUMaxRowDiffStdDevMaxKey{19538}
\def\EUPUMaxRowDiffStdDevMeanFloat{0.372166574001312255859375}
\def\EUPUMaxRowDiffStdDevMeanKey{7467}
\def\EUPUMaxRowDiffStdDevMedianFloat{0.2221090383827686309814453125}
\def\EUPUMaxRowDiffStdDevMedianKey{32103}
\def\EUPUMaxRowDiffStdDevMinFloat{0.22020025551319122314453125}
\def\EUPUMaxRowDiffStdDevMinKey{24262}
\def\EUPUMaxRowDiffStdDevStdDevFloat{0.0903910696506500244140625}
\def\EUPUMaxStdDevFloat{0.552904069423675537109375}
\def\EUPUMeanLen{151}
\def\EUPUMeanMaxFloat{-0.361374676227569580078125}
\def\EUPUMeanMaxKey{19488}
\def\EUPUMeanMeanFloat{-0.55691945552825927734375}
\def\EUPUMeanMeanKey{13654}
\def\EUPUMeanMedianFloat{-0.78322581946849822998046875}
\def\EUPUMeanMedianKey{19538}
\def\EUPUMeanMinFloat{-0.80177128314971923828125}
\def\EUPUMeanMinKey{11611}
\def\EUPUMeanStdDevFloat{0.085817821323871612548828125}
\def\EUPUMedianLen{151}
\def\EUPUMedianMaxFloat{-1.3517710268497467041015625}
\def\EUPUMedianMaxKey{32103}
\def\EUPUMedianMeanFloat{-1.7474461421074460876212697257869876921176910400390625}
\def\EUPUMedianMeanKey{22545}
\def\EUPUMedianMedianFloat{-2.414761774241924285888671875}
\def\EUPUMedianMedianKey{19538}
\def\EUPUMedianMinFloat{-2.44518311619758588193462855997495353221893310546875}
\def\EUPUMedianMinKey{1490}
\def\EUPUMedianStdDevFloat{0.1660894113402864302742045765626244246959686279296875}
\def\EUPUMinLen{151}
\def\EUPUMinMaxFloat{-1.65356791019439697265625}
\def\EUPUMinMaxKey{32103}
\def\EUPUMinMeanFloat{-2.2188580036163330078125}
\def\EUPUMinMeanKey{14095}
\def\EUPUMinMedianFloat{-3.64212322235107421875}
\def\EUPUMinMedianKey{1490}
\def\EUPUMinMinFloat{-4.296205997467041015625}
\def\EUPUMinMinKey{19538}
\def\EUPUMinStdDevFloat{0.317187488079071044921875}
\def\EUPUStdDevLen{151}
\def\EUPUStdDevMaxFloat{0.96902668476104736328125}
\def\EUPUStdDevMaxKey{11611}
\def\EUPUStdDevMeanFloat{0.725439369678497314453125}
\def\EUPUStdDevMeanKey{32374}
\def\EUPUStdDevMedianFloat{0.58007918298244476318359375}
\def\EUPUStdDevMedianKey{19488}
\def\EUPUStdDevMinFloat{0.57262384891510009765625}
\def\EUPUStdDevMinKey{24566}
\def\EUPUStdDevStdDevFloat{0.07000477612018585205078125}
\def\EVOUHistMinAboveDiagDupBySeqCountLenLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMaxFloat{1329227995784916168051712239633170432}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMaxKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMeanFloat{1329227995784916168051712239633170432}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMeanKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMedianFloat{1329227995784916168051712239633170432}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMedianKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMinFloat{1329227995784916168051712239633170432}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMinKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountLenStdDevFloat{0}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMaxFloat{31.2299957275390625}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMaxKey{15622}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMeanFloat{9.243762969970703125}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMeanKey{8893}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMedianFloat{5.6327044963836669921875}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMedianKey{5615}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMinFloat{5.50226688385009765625}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMinKey{7310}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxStdDevFloat{2.4151537418365478515625}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMaxFloat{-3.7684218136767437812295611365698277950286865234375}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMaxKey{15622}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMeanFloat{-11.06355992925335840482148341834545135498046875}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMeanKey{20751}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMedianFloat{-12.49699369711698437868108157999813556671142578125}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMedianKey{1283}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMinFloat{-12.6742661394076581160561545402742922306060791015625}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMinKey{17080}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanStdDevFloat{0.85343379370287808516337690889486111700534820556640625}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMaxFloat{-5.09565714185377327538617464597336947917938232421875}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMaxKey{15622}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMeanFloat{-11.550011286459973547380286618135869503021240234375}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMeanKey{17096}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMedianFloat{-13.44212465085052343738425406627357006072998046875}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMedianKey{4430}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMinFloat{-13.4721708697206157268055903841741383075714111328125}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMinKey{1951}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianStdDevFloat{1.0310511558853072688890506469761021435260772705078125}
\def\EVOUHistMinAboveDiagDupBySeqCountMinLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMaxFloat{-11.29123210906982421875}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMaxKey{17197}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMeanFloat{-13.89575672149658203125}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMeanKey{21598}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMedianFloat{-16.5449619293212890625}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMedianKey{26829}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMinFloat{-16.9964542388916015625}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMinKey{4810}
\def\EVOUHistMinAboveDiagDupBySeqCountMinStdDevFloat{0.964361608028411865234375}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMaxFloat{229}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMaxKey{15622}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMeanFloat{-1.78145695364238410007828861125744879245758056640625}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMeanKey{4729}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMedianFloat{-8}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMedianKey{2743}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMinFloat{-8}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMinKey{2743}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMaxFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMaxKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMeanFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMeanKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMedianFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMedianKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMinFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMinKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdStdDevFloat{0}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMaxFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMaxKey{1490}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMeanFloat{0.98274932940737558251242944606929086148738861083984375}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMeanKey{10248}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMedianFloat{0.91719338363786129253441004038904793560504913330078125}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMedianKey{19451}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMinFloat{0.9096479893721791665228693091194145381450653076171875}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMinKey{19488}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracStdDevFloat{0.019569508488055435690977645890598068945109844207763671875}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueStdDevFloat{19.4792788665816516413542558439075946807861328125}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMaxFloat{16.365402987360479158951420686207711696624755859375}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMaxKey{15622}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMeanFloat{12.7152021340820962080897515988908708095550537109375}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMeanKey{19917}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMedianFloat{10.9028829937158899809901413391344249248504638671875}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMedianKey{25516}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMinFloat{10.773840790508682374593263375572860240936279296875}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMinKey{8048}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevStdDevFloat{0.92822100870477008971448640295420773327350616455078125}
\def\EVOUHistMinAboveDiagLenLen{151}
\def\EVOUHistMinAboveDiagLenMaxFloat{64}
\def\EVOUHistMinAboveDiagLenMaxKey{50}
\def\EVOUHistMinAboveDiagLenMeanFloat{64}
\def\EVOUHistMinAboveDiagLenMeanKey{50}
\def\EVOUHistMinAboveDiagLenMedianFloat{64}
\def\EVOUHistMinAboveDiagLenMedianKey{50}
\def\EVOUHistMinAboveDiagLenMinFloat{64}
\def\EVOUHistMinAboveDiagLenMinKey{50}
\def\EVOUHistMinAboveDiagLenStdDevFloat{0}
\def\EVOUHistMinAboveDiagMaxLen{151}
\def\EVOUHistMinAboveDiagMaxMaxFloat{31.2299957275390625}
\def\EVOUHistMinAboveDiagMaxMaxKey{15622}
\def\EVOUHistMinAboveDiagMaxMeanFloat{9.243762969970703125}
\def\EVOUHistMinAboveDiagMaxMeanKey{8893}
\def\EVOUHistMinAboveDiagMaxMedianFloat{5.6327044963836669921875}
\def\EVOUHistMinAboveDiagMaxMedianKey{5615}
\def\EVOUHistMinAboveDiagMaxMinFloat{5.50226688385009765625}
\def\EVOUHistMinAboveDiagMaxMinKey{7310}
\def\EVOUHistMinAboveDiagMaxStdDevFloat{2.4151537418365478515625}
\def\EVOUHistMinAboveDiagMeanLen{151}
\def\EVOUHistMinAboveDiagMeanMaxFloat{3.119003772735595703125}
\def\EVOUHistMinAboveDiagMeanMaxKey{8299}
\def\EVOUHistMinAboveDiagMeanMeanFloat{1.28420984745025634765625}
\def\EVOUHistMinAboveDiagMeanMeanKey{20294}
\def\EVOUHistMinAboveDiagMeanMedianFloat{-0.218912415206432342529296875}
\def\EVOUHistMinAboveDiagMeanMedianKey{27300}
\def\EVOUHistMinAboveDiagMeanMinFloat{-0.2691262066364288330078125}
\def\EVOUHistMinAboveDiagMeanMinKey{18668}
\def\EVOUHistMinAboveDiagMeanStdDevFloat{0.735017597675323486328125}
\def\EVOUHistMinAboveDiagMedianLen{151}
\def\EVOUHistMinAboveDiagMedianMaxFloat{6.8975899219512939453125}
\def\EVOUHistMinAboveDiagMedianMaxKey{9504}
\def\EVOUHistMinAboveDiagMedianMeanFloat{3.786776371349561909340764032094739377498626708984375}
\def\EVOUHistMinAboveDiagMedianMeanKey{11598}
\def\EVOUHistMinAboveDiagMedianMedianFloat{1.39133398234844207763671875}
\def\EVOUHistMinAboveDiagMedianMedianKey{1490}
\def\EVOUHistMinAboveDiagMedianMinFloat{1.328092098236083984375}
\def\EVOUHistMinAboveDiagMedianMinKey{18668}
\def\EVOUHistMinAboveDiagMedianStdDevFloat{1.1619263479609942546488809966831468045711517333984375}
\def\EVOUHistMinAboveDiagMinLen{151}
\def\EVOUHistMinAboveDiagMinMaxFloat{-11.29123210906982421875}
\def\EVOUHistMinAboveDiagMinMaxKey{17197}
\def\EVOUHistMinAboveDiagMinMeanFloat{-13.89575672149658203125}
\def\EVOUHistMinAboveDiagMinMeanKey{21598}
\def\EVOUHistMinAboveDiagMinMedianFloat{-16.5449619293212890625}
\def\EVOUHistMinAboveDiagMinMedianKey{26829}
\def\EVOUHistMinAboveDiagMinMinFloat{-16.9964542388916015625}
\def\EVOUHistMinAboveDiagMinMinKey{4810}
\def\EVOUHistMinAboveDiagMinStdDevFloat{0.964361608028411865234375}
\def\EVOUHistMinAboveDiagMostBelowValueLen{151}
\def\EVOUHistMinAboveDiagMostBelowValueMaxFloat{61}
\def\EVOUHistMinAboveDiagMostBelowValueMaxKey{16149}
\def\EVOUHistMinAboveDiagMostBelowValueMeanFloat{36.98675496688741759498952887952327728271484375}
\def\EVOUHistMinAboveDiagMostBelowValueMeanKey{3175}
\def\EVOUHistMinAboveDiagMostBelowValueMedianFloat{21.25}
\def\EVOUHistMinAboveDiagMostBelowValueMedianKey{19538}
\def\EVOUHistMinAboveDiagMostBelowValueMinFloat{19}
\def\EVOUHistMinAboveDiagMostBelowValueMinKey{1490}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdLen{151}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMaxFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMaxKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMeanFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMeanKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMedianFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMedianKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMinFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMinKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdStdDevFloat{0}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracLen{151}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMaxFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMaxKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMeanFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMeanKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMedianFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMedianKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMinFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMinKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracStdDevFloat{0}
\def\EVOUHistMinAboveDiagMostBelowValueStdDevFloat{7.7775247215462712802036548964679241180419921875}
\def\EVOUHistMinAboveDiagStdDevLen{151}
\def\EVOUHistMinAboveDiagStdDevMaxFloat{7.67364501953125}
\def\EVOUHistMinAboveDiagStdDevMaxKey{16149}
\def\EVOUHistMinAboveDiagStdDevMeanFloat{5.98618984222412109375}
\def\EVOUHistMinAboveDiagStdDevMeanKey{13468}
\def\EVOUHistMinAboveDiagStdDevMedianFloat{4.5033283233642578125}
\def\EVOUHistMinAboveDiagStdDevMedianKey{19538}
\def\EVOUHistMinAboveDiagStdDevMinFloat{4.297507762908935546875}
\def\EVOUHistMinAboveDiagStdDevMinKey{1490}
\def\EVOUHistMinAboveDiagStdDevStdDevFloat{0.601494371891021728515625}
\def\EVOUMaxRowDiffLenLen{151}
\def\EVOUMaxRowDiffLenMaxFloat{64}
\def\EVOUMaxRowDiffLenMaxKey{50}
\def\EVOUMaxRowDiffLenMeanFloat{64}
\def\EVOUMaxRowDiffLenMeanKey{50}
\def\EVOUMaxRowDiffLenMedianFloat{64}
\def\EVOUMaxRowDiffLenMedianKey{50}
\def\EVOUMaxRowDiffLenMinFloat{64}
\def\EVOUMaxRowDiffLenMinKey{50}
\def\EVOUMaxRowDiffLenStdDevFloat{0}
\def\EVOUMaxRowDiffMaxLen{151}
\def\EVOUMaxRowDiffMaxMaxFloat{81.2588653564453125}
\def\EVOUMaxRowDiffMaxMaxKey{10248}
\def\EVOUMaxRowDiffMaxMeanFloat{61.50217437744140625}
\def\EVOUMaxRowDiffMaxMeanKey{24566}
\def\EVOUMaxRowDiffMaxMedianFloat{43.60958194732666015625}
\def\EVOUMaxRowDiffMaxMedianKey{1490}
\def\EVOUMaxRowDiffMaxMinFloat{43.297069549560546875}
\def\EVOUMaxRowDiffMaxMinKey{11130}
\def\EVOUMaxRowDiffMaxStdDevFloat{7.49969005584716796875}
\def\EVOUMaxRowDiffMeanLen{151}
\def\EVOUMaxRowDiffMeanMaxFloat{32.47296142578125}
\def\EVOUMaxRowDiffMeanMaxKey{9504}
\def\EVOUMaxRowDiffMeanMeanFloat{22.42388153076171875}
\def\EVOUMaxRowDiffMeanMeanKey{27584}
\def\EVOUMaxRowDiffMeanMedianFloat{14.016768932342529296875}
\def\EVOUMaxRowDiffMeanMedianKey{30371}
\def\EVOUMaxRowDiffMeanMinFloat{12.33141326904296875}
\def\EVOUMaxRowDiffMeanMinKey{1490}
\def\EVOUMaxRowDiffMeanStdDevFloat{3.482374668121337890625}
\def\EVOUMaxRowDiffMedianLen{151}
\def\EVOUMaxRowDiffMedianMaxFloat{21.954150075912476580697330064140260219573974609375}
\def\EVOUMaxRowDiffMedianMaxKey{9504}
\def\EVOUMaxRowDiffMedianMeanFloat{11.286633502016005792256692075170576572418212890625}
\def\EVOUMaxRowDiffMedianMeanKey{5358}
\def\EVOUMaxRowDiffMedianMedianFloat{4.1380902820825582466568448580801486968994140625}
\def\EVOUMaxRowDiffMedianMedianKey{18668}
\def\EVOUMaxRowDiffMedianMinFloat{3.30193331003189083361348821199499070644378662109375}
\def\EVOUMaxRowDiffMedianMinKey{1490}
\def\EVOUMaxRowDiffMedianStdDevFloat{3.6566456264552567034797903033904731273651123046875}
\def\EVOUMaxRowDiffMinLen{151}
\def\EVOUMaxRowDiffMinMaxFloat{21.8009128570556640625}
\def\EVOUMaxRowDiffMinMaxKey{9504}
\def\EVOUMaxRowDiffMinMeanFloat{10.9655551910400390625}
\def\EVOUMaxRowDiffMinMeanKey{32103}
\def\EVOUMaxRowDiffMinMedianFloat{3.9641535282135009765625}
\def\EVOUMaxRowDiffMinMedianKey{18668}
\def\EVOUMaxRowDiffMinMinFloat{2.70917797088623046875}
\def\EVOUMaxRowDiffMinMinKey{1490}
\def\EVOUMaxRowDiffMinStdDevFloat{3.666030406951904296875}
\def\EVOUMaxRowDiffStdDevLen{151}
\def\EVOUMaxRowDiffStdDevMaxFloat{16.6555614471435546875}
\def\EVOUMaxRowDiffStdDevMaxKey{10248}
\def\EVOUMaxRowDiffStdDevMeanFloat{10.60002803802490234375}
\def\EVOUMaxRowDiffStdDevMeanKey{20976}
\def\EVOUMaxRowDiffStdDevMedianFloat{7.93212282657623291015625}
\def\EVOUMaxRowDiffStdDevMedianKey{15622}
\def\EVOUMaxRowDiffStdDevMinFloat{7.906446933746337890625}
\def\EVOUMaxRowDiffStdDevMinKey{27671}
\def\EVOUMaxRowDiffStdDevStdDevFloat{1.4334104061126708984375}
\def\ImportanceSamplingAccuracyLen{151}
\def\ImportanceSamplingAccuracyMaxFloat{0.9997343995077567768703374895267188549041748046875}
\def\ImportanceSamplingAccuracyMaxKey{16284}
\def\ImportanceSamplingAccuracyMeanFloat{0.9953204378015356734721308384905569255352020263671875}
\def\ImportanceSamplingAccuracyMeanKey{3284}
\def\ImportanceSamplingAccuracyMedianFloat{0.9005807039686288817392778582870960235595703125}
\def\ImportanceSamplingAccuracyMedianKey{1490}
\def\ImportanceSamplingAccuracyMinFloat{0.85009203809042432897769003830035217106342315673828125}
\def\ImportanceSamplingAccuracyMinKey{15622}
\def\ImportanceSamplingAccuracyStdDevFloat{0.01478991148269638566947747904123389162123203277587890625}
\def\ImportanceSamplingBatchSize{4096}
\def\ImportanceSamplingInstructionCountBranch{0}
\def\ImportanceSamplingInstructionCountInt{0}
\def\ImportanceSamplingInstructionCount{0}
\def\ImportanceSamplingLossLen{151}
\def\ImportanceSamplingLossMaxFloat{nan}
\def\ImportanceSamplingLossMaxKey{50}
\def\ImportanceSamplingLossMeanFloat{nan}
\def\ImportanceSamplingLossMeanKey{50}
\def\ImportanceSamplingLossMedianFloat{nan}
\def\ImportanceSamplingLossMedianKey{50}
\def\ImportanceSamplingLossMinFloat{nan}
\def\ImportanceSamplingLossMinKey{50}
\def\ImportanceSamplingLossStdDevFloat{nan}
\def\ImportanceSamplingNSamplesPerKey{5}
\def\ImportanceSamplingNumCorrectLen{151}
\def\ImportanceSamplingNumCorrectMaxFloat{5672263}
\def\ImportanceSamplingNumCorrectMaxKey{16284}
\def\ImportanceSamplingNumCorrectMeanFloat{5031761.688741722144186496734619140625}
\def\ImportanceSamplingNumCorrectMeanKey{29052}
\def\ImportanceSamplingNumCorrectMedianFloat{3944786.75}
\def\ImportanceSamplingNumCorrectMedianKey{1490}
\def\ImportanceSamplingNumCorrectMinFloat{3708620}
\def\ImportanceSamplingNumCorrectMinKey{19917}
\def\ImportanceSamplingNumCorrectStdDevFloat{360077.0059357738937251269817352294921875}
\def\ImportanceSamplingNumIncorrectLen{151}
\def\ImportanceSamplingNumIncorrectMaxFloat{4165688}
\def\ImportanceSamplingNumIncorrectMaxKey{19917}
\def\ImportanceSamplingNumIncorrectMeanFloat{2842546.3112582783214747905731201171875}
\def\ImportanceSamplingNumIncorrectMeanKey{29052}
\def\ImportanceSamplingNumIncorrectMedianFloat{2242029}
\def\ImportanceSamplingNumIncorrectMedianKey{104}
\def\ImportanceSamplingNumIncorrectMinFloat{2202045}
\def\ImportanceSamplingNumIncorrectMinKey{16284}
\def\ImportanceSamplingNumIncorrectStdDevFloat{360077.0059357738937251269817352294921875}
\def\ImportanceSamplingTimeLen{151}
\def\ImportanceSamplingTimeMaxFloat{337.1592676639556884765625}
\def\ImportanceSamplingTimeMaxKey{29726}
\def\ImportanceSamplingTimeMeanFloat{312.21522330606222794813220389187335968017578125}
\def\ImportanceSamplingTimeMeanKey{9504}
\def\ImportanceSamplingTimeMedianFloat{247.79457032680511474609375}
\def\ImportanceSamplingTimeMedianKey{8299}
\def\ImportanceSamplingTimeMinFloat{102.50246906280517578125}
\def\ImportanceSamplingTimeMinKey{123}
\def\ImportanceSamplingTimeStdDevFloat{20.0742313633326574517923290841281414031982421875}
\def\ImportanceSamplingTotalSequences{7874308}
\def\LowerWhiskerBottomEndPercentileFloat{0.02151239536919476169618548055950668640434741973876953125}
\def\LowerWhiskerCrosshatchPercentileFloat{0.08867177532617598334496733514242805540561676025390625}
\def\MedianPercentileFloat{0.5}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffExactLinearFitIntercept{0.309126377704897425946484190717455931007862091064453125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffExactLinearFitRSquared{0.00063255579414767115764561822288669645786285400390625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffExactLinearFitSlope{0.0000281414399991064927684415730713141101659857667982578277587890625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffLinearFitIntercept{0.300723094954763514596862705730018205940723419189453125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffLinearFitRSquared{0.0007318004156868784804146343958564102649688720703125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffLinearFitSlope{0.00002959007391248765809978367447019564906440791673958301544189453125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductLinearFitIntercept{0.30484253605991240565487032654345966875553131103515625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductLinearFitRSquared{0.00062767954826348226760046600247733294963836669921875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductLinearFitSlope{0.000027615156225588291722707057207486514016636647284030914306640625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitIntercept{0.16320473764790033310845274172606877982616424560546875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitRSquared{0.0031938928584016590406235991395078599452972412109375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitSlope{0.0000373145741925850758552614394591984137150575406849384307861328125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffLinearFitIntercept{0.300861875713193060999373074082541279494762420654296875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffLinearFitRSquared{0.0007230858917701699084545907680876553058624267578125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffLinearFitSlope{0.00002941224547214328917496724280500330905852024443447589874267578125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitIntercept{0.304841635127392596160689208772964775562286376953125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitRSquared{0.00062667066486576938899588640197180211544036865234375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitSlope{0.000027588899266285847274894627023655857556150294840335845947265625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitIntercept{0.163154325626059415466073687639436684548854827880859375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitRSquared{0.003208019872293021990117267705500125885009765625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitSlope{0.0000373947407649240118159006396325594323570840060710906982421875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitIntercept{0.1603067972942918417711410938863991759717464447021484375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitRSquared{0.00338206034523624854415402296581305563449859619140625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitSlope{0.0000379368819522619990058757977191561394647578708827495574951171875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMaxDiffExactLinearFitIntercept{0.323270685403282909131661426727077923715114593505859375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMaxDiffExactLinearFitSlope{0}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMaxDiffLinearFitIntercept{0.315296909354759347099417254867148585617542266845703125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMaxDiffLinearFitSlope{0}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMaxDiffSubproductLinearFitIntercept{0.318986057155203617252681169702555052936077117919921875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMaxDiffSubproductLinearFitSlope{0}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMaxDiffSubproductRecursiveLinearFitIntercept{0.188364161160074428114086231289547868072986602783203125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMaxDiffSubproductRecursiveLinearFitSlope{0}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMeanMaxDiffLinearFitIntercept{0.3165383098289737962005574445356614887714385986328125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMeanMaxDiffLinearFitSlope{0}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMeanMaxDiffSubproductLinearFitIntercept{0.319099459414122321732065756805241107940673828125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMeanMaxDiffSubproductLinearFitSlope{0}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMeanMaxDiffSubproductRecursiveLinearFitIntercept{0.1891056711297462999965546259772963821887969970703125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMeanMaxDiffSubproductRecursiveLinearFitSlope{0}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMeanRecursiveMaxDiffSubproductRecursiveLinearFitIntercept{0.1867306096224956579732179307029582560062408447265625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMeanRecursiveMaxDiffSubproductRecursiveLinearFitSlope{0}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestSvdLinearFitIntercept{0.2273994368013643185832961535197682678699493408203125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestSvdLinearFitSlope{0}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioSvdLinearFitIntercept{0.2369556502155456267910693668454769067466259002685546875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioSvdLinearFitRSquared{0.0047377077949448676008614711463451385498046875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioSvdLinearFitSlope{0.00006921609441933493605918215063610432480345480144023895263671875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffExactLinearFitIntercept{0.53698789284777548314053774447529576718807220458984375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffExactLinearFitRSquared{0.0130413532708766322087967637344263494014739990234375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffExactLinearFitSlope{0.00002399235033272601128203314890807718029464012943208217620849609375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffLinearFitIntercept{0.51474301642797304356946597181377001106739044189453125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffLinearFitRSquared{0.02814370405099475558330368585302494466304779052734375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffLinearFitSlope{0.000033945032365638490713492803063644487338024191558361053466796875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductLinearFitIntercept{0.52120955745508734668902661724132485687732696533203125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductLinearFitRSquared{0.0235852086767838198255731185781769454479217529296875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductLinearFitSlope{0.000031328424760419541143623145540431096378597430884838104248046875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitIntercept{0.28526906965212805999954071012325584888458251953125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitRSquared{0.06789922794863023636224852452869527041912078857421875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitSlope{0.0000452211062406076058964830843844850960522308014333248138427734375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffLinearFitIntercept{0.5144700096722065740806328904000110924243927001953125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffLinearFitRSquared{0.0287286917247933093477740840171463787555694580078125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffLinearFitSlope{0.0000341733390213532265376750185481569133116863667964935302734375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitIntercept{0.5212962661428885979830738506279885768890380859375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitRSquared{0.02344416529124682124773926261696033179759979248046875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitSlope{0.000031155038288247527433240391392388346503139473497867584228515625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitIntercept{0.28420311731152825274193673976697027683258056640625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitRSquared{0.07177118787180802872427420879830606281757354736328125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitSlope{0.00004654701474577399209452133188591460566385649144649505615234375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitIntercept{0.281562661088764432104625257125007919967174530029296875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitRSquared{0.0701742543204424418235021221335045993328094482421875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitSlope{0.0000449594118687269436404098377213500725702033378183841705322265625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioSvdLinearFitIntercept{0.41291808809660845991373889773967675864696502685546875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioSvdLinearFitRSquared{0.218703076355180936474198460928164422512054443359375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioSvdLinearFitSlope{0.000097560300680841384869494692377855926679330877959728240966796875}
\def\NumSeeds{151}
\def\PVOUAbsLenLen{151}
\def\PVOUAbsLenMaxFloat{1280}
\def\PVOUAbsLenMaxKey{50}
\def\PVOUAbsLenMeanFloat{1280}
\def\PVOUAbsLenMeanKey{50}
\def\PVOUAbsLenMedianFloat{1280}
\def\PVOUAbsLenMedianKey{50}
\def\PVOUAbsLenMinFloat{1280}
\def\PVOUAbsLenMinKey{50}
\def\PVOUAbsLenStdDevFloat{0}
\def\PVOUAbsMaxLen{151}
\def\PVOUAbsMaxMaxFloat{4.73284244537353515625}
\def\PVOUAbsMaxMaxKey{5928}
\def\PVOUAbsMaxMeanFloat{2.4220111370086669921875}
\def\PVOUAbsMaxMeanKey{11498}
\def\PVOUAbsMaxMedianFloat{0.96512465178966522216796875}
\def\PVOUAbsMaxMedianKey{1490}
\def\PVOUAbsMaxMinFloat{0.948256909847259521484375}
\def\PVOUAbsMaxMinKey{15622}
\def\PVOUAbsMaxStdDevFloat{0.6773588657379150390625}
\def\PVOUAbsMeanLen{151}
\def\PVOUAbsMeanMaxFloat{0.515628159046173095703125}
\def\PVOUAbsMeanMaxKey{19451}
\def\PVOUAbsMeanMeanFloat{0.3589335978031158447265625}
\def\PVOUAbsMeanMeanKey{13468}
\def\PVOUAbsMeanMedianFloat{0.15674111805856227874755859375}
\def\PVOUAbsMeanMedianKey{1490}
\def\PVOUAbsMeanMinFloat{0.101974628865718841552734375}
\def\PVOUAbsMeanMinKey{15622}
\def\PVOUAbsMeanStdDevFloat{0.06434251368045806884765625}
\def\PVOUAbsMedianLen{151}
\def\PVOUAbsMedianMaxFloat{0.008385398387908936379542268468867405317723751068115234375}
\def\PVOUAbsMedianMaxKey{2236}
\def\PVOUAbsMedianMeanFloat{0.0033083693585273751293363009295944721088744699954986572265625}
\def\PVOUAbsMedianMeanKey{23241}
\def\PVOUAbsMedianMedianFloat{0.00084512054920196535805210213965210641617886722087860107421875}
\def\PVOUAbsMedianMedianKey{2345}
\def\PVOUAbsMedianMinFloat{0.00067061603069305439871194973733281585737131536006927490234375}
\def\PVOUAbsMedianMinKey{11130}
\def\PVOUAbsMedianStdDevFloat{0.00147890897366900731478567276866442625760100781917572021484375}
\def\PVOUAbsMinLen{151}
\def\PVOUAbsMinMaxFloat{0.00275290012359619140625}
\def\PVOUAbsMinMaxKey{15399}
\def\PVOUAbsMinMeanFloat{0.0004070333088748157024383544921875}
\def\PVOUAbsMinMeanKey{4157}
\def\PVOUAbsMinMedianFloat{0.00000655651092529296875}
\def\PVOUAbsMinMedianKey{2549}
\def\PVOUAbsMinMinFloat{0.000003337860107421875}
\def\PVOUAbsMinMinKey{6589}
\def\PVOUAbsMinStdDevFloat{0.0005065795849077403545379638671875}
\def\PVOUAbsStdDevLen{151}
\def\PVOUAbsStdDevMaxFloat{0.5604732036590576171875}
\def\PVOUAbsStdDevMaxKey{5928}
\def\PVOUAbsStdDevMeanFloat{0.30739533901214599609375}
\def\PVOUAbsStdDevMeanKey{20751}
\def\PVOUAbsStdDevMedianFloat{0.13578841648995876312255859375}
\def\PVOUAbsStdDevMedianKey{1490}
\def\PVOUAbsStdDevMinFloat{0.102787740528583526611328125}
\def\PVOUAbsStdDevMinKey{15622}
\def\PVOUAbsStdDevStdDevFloat{0.06511379778385162353515625}
\def\PVOULenLen{151}
\def\PVOULenMaxFloat{1280}
\def\PVOULenMaxKey{50}
\def\PVOULenMeanFloat{1280}
\def\PVOULenMeanKey{50}
\def\PVOULenMedianFloat{1280}
\def\PVOULenMedianKey{50}
\def\PVOULenMinFloat{1280}
\def\PVOULenMinKey{50}
\def\PVOULenStdDevFloat{0}
\def\PVOUMaxLen{151}
\def\PVOUMaxMaxFloat{4.73284244537353515625}
\def\PVOUMaxMaxKey{5928}
\def\PVOUMaxMeanFloat{2.1893541812896728515625}
\def\PVOUMaxMeanKey{6204}
\def\PVOUMaxMedianFloat{0.92848460376262664794921875}
\def\PVOUMaxMedianKey{15622}
\def\PVOUMaxMinFloat{0.86916768550872802734375}
\def\PVOUMaxMinKey{1490}
\def\PVOUMaxRowDiffLenLen{151}
\def\PVOUMaxRowDiffLenMaxFloat{20}
\def\PVOUMaxRowDiffLenMaxKey{50}
\def\PVOUMaxRowDiffLenMeanFloat{20}
\def\PVOUMaxRowDiffLenMeanKey{50}
\def\PVOUMaxRowDiffLenMedianFloat{20}
\def\PVOUMaxRowDiffLenMedianKey{50}
\def\PVOUMaxRowDiffLenMinFloat{20}
\def\PVOUMaxRowDiffLenMinKey{50}
\def\PVOUMaxRowDiffLenStdDevFloat{0}
\def\PVOUMaxRowDiffMaxLen{151}
\def\PVOUMaxRowDiffMaxMaxFloat{8.703990936279296875}
\def\PVOUMaxRowDiffMaxMaxKey{5928}
\def\PVOUMaxRowDiffMaxMeanFloat{4.33923053741455078125}
\def\PVOUMaxRowDiffMaxMeanKey{8840}
\def\PVOUMaxRowDiffMaxMedianFloat{1.8593380451202392578125}
\def\PVOUMaxRowDiffMaxMedianKey{15622}
\def\PVOUMaxRowDiffMaxMinFloat{1.7952783107757568359375}
\def\PVOUMaxRowDiffMaxMinKey{1490}
\def\PVOUMaxRowDiffMaxStdDevFloat{1.21213471889495849609375}
\def\PVOUMaxRowDiffMeanLen{151}
\def\PVOUMaxRowDiffMeanMaxFloat{2.5648972988128662109375}
\def\PVOUMaxRowDiffMeanMaxKey{19451}
\def\PVOUMaxRowDiffMeanMeanFloat{1.818210601806640625}
\def\PVOUMaxRowDiffMeanMeanKey{7098}
\def\PVOUMaxRowDiffMeanMedianFloat{0.8647871911525726318359375}
\def\PVOUMaxRowDiffMeanMedianKey{1490}
\def\PVOUMaxRowDiffMeanMinFloat{0.696767628192901611328125}
\def\PVOUMaxRowDiffMeanMinKey{15622}
\def\PVOUMaxRowDiffMeanStdDevFloat{0.241595089435577392578125}
\def\PVOUMaxRowDiffMedianLen{151}
\def\PVOUMaxRowDiffMedianMaxFloat{1.35350463449954983019551946199499070644378662109375}
\def\PVOUMaxRowDiffMedianMaxKey{19451}
\def\PVOUMaxRowDiffMedianMeanFloat{0.834157254791615176969798994832672178745269775390625}
\def\PVOUMaxRowDiffMedianMeanKey{14929}
\def\PVOUMaxRowDiffMedianMedianFloat{0.41112024303525684931770456387312151491641998291015625}
\def\PVOUMaxRowDiffMedianMedianKey{19538}
\def\PVOUMaxRowDiffMedianMinFloat{0.305750499069690706566149174250313080847263336181640625}
\def\PVOUMaxRowDiffMedianMinKey{15622}
\def\PVOUMaxRowDiffMedianStdDevFloat{0.1897112054635170796945686788603779859840869903564453125}
\def\PVOUMaxRowDiffMinLen{151}
\def\PVOUMaxRowDiffMinMaxFloat{1.33855330944061279296875}
\def\PVOUMaxRowDiffMinMaxKey{19451}
\def\PVOUMaxRowDiffMinMeanFloat{0.81849515438079833984375}
\def\PVOUMaxRowDiffMinMeanKey{22401}
\def\PVOUMaxRowDiffMinMedianFloat{0.39614172279834747314453125}
\def\PVOUMaxRowDiffMinMedianKey{7467}
\def\PVOUMaxRowDiffMinMinFloat{0.296641290187835693359375}
\def\PVOUMaxRowDiffMinMinKey{15622}
\def\PVOUMaxRowDiffMinStdDevFloat{0.19503693282604217529296875}
\def\PVOUMaxRowDiffStdDevLen{151}
\def\PVOUMaxRowDiffStdDevMaxFloat{1.6292011737823486328125}
\def\PVOUMaxRowDiffStdDevMaxKey{5928}
\def\PVOUMaxRowDiffStdDevMeanFloat{0.8065874576568603515625}
\def\PVOUMaxRowDiffStdDevMeanKey{15043}
\def\PVOUMaxRowDiffStdDevMedianFloat{0.3489276468753814697265625}
\def\PVOUMaxRowDiffStdDevMedianKey{15622}
\def\PVOUMaxRowDiffStdDevMinFloat{0.3477278053760528564453125}
\def\PVOUMaxRowDiffStdDevMinKey{1490}
\def\PVOUMaxRowDiffStdDevStdDevFloat{0.22180671989917755126953125}
\def\PVOUMaxStdDevFloat{0.665203869342803955078125}
\def\PVOUMeanLen{151}
\def\PVOUMeanMaxFloat{0.0000000298023223876953125}
\def\PVOUMeanMaxKey{11611}
\def\PVOUMeanMeanFloat{-0.00000000110155096155750698017072863876819610595703125}
\def\PVOUMeanMeanKey{15662}
\def\PVOUMeanMedianFloat{-0.000000029429793269031279123737476766109466552734375}
\def\PVOUMeanMedianKey{16284}
\def\PVOUMeanMinFloat{-0.000000032782555337007579510100185871124267578125}
\def\PVOUMeanMinKey{2773}
\def\PVOUMeanStdDevFloat{0.00000001158463192041381262242794036865234375}
\def\PVOUMedianLen{151}
\def\PVOUMedianMaxFloat{-0.427728475928306595132966094752191565930843353271484375}
\def\PVOUMedianMaxKey{15622}
\def\PVOUMedianMeanFloat{-1.3282020173187285561056114602251909673213958740234375}
\def\PVOUMedianMeanKey{4430}
\def\PVOUMedianMedianFloat{-2.411569181680679463397609652020037174224853515625}
\def\PVOUMedianMedianKey{1185}
\def\PVOUMedianMinFloat{-3.04812141776084910560484786401502788066864013671875}
\def\PVOUMedianMinKey{14929}
\def\PVOUMedianStdDevFloat{0.3201449344883771086500701130717061460018157958984375}
\def\PVOUMinLen{151}
\def\PVOUMinMaxFloat{-0.9324343204498291015625}
\def\PVOUMinMaxKey{15622}
\def\PVOUMinMeanFloat{-2.21355915069580078125}
\def\PVOUMinMeanKey{16197}
\def\PVOUMinMedianFloat{-4.1572663784027099609375}
\def\PVOUMinMedianKey{15662}
\def\PVOUMinMinFloat{-4.263576984405517578125}
\def\PVOUMinMinKey{2236}
\def\PVOUMinStdDevFloat{0.639587342739105224609375}
\def\PVOUStdDevLen{151}
\def\PVOUStdDevMaxFloat{0.71957170963287353515625}
\def\PVOUStdDevMaxKey{5928}
\def\PVOUStdDevMeanFloat{0.4732326567173004150390625}
\def\PVOUStdDevMeanKey{31308}
\def\PVOUStdDevMedianFloat{0.207504324615001678466796875}
\def\PVOUStdDevMedianKey{1490}
\def\PVOUStdDevMinFloat{0.14479000866413116455078125}
\def\PVOUStdDevMinKey{15622}
\def\PVOUStdDevStdDevFloat{0.0880671441555023193359375}
\def\ProofFlopEstimateAllSubcubicMean{18392610.8000000007450580596923828125}
\def\ProofFlopEstimateAllSubcubicStdDev{802251.5766774886287748813629150390625}
\def\ProofFlopEstimateAlmostQuadraticMean{17494996.6666666679084300994873046875}
\def\ProofFlopEstimateAlmostQuadraticStdDev{115454.8637911393889226019382476806640625}
\def\ProofFlopEstimateMainlySubcubicMean{18517240.5769230760633945465087890625}
\def\ProofFlopEstimateMainlySubcubicStdDev{759264.18629479617811739444732666015625}
\def\QuartileOnePercentileFloat{0.25}
\def\QuartileThreePercentileFloat{0.75}
\def\RealSubcubicAccuracyLen{15100}
\def\RealSubcubicAccuracyMaxFloat{0.65682941314196041648898471976281143724918365478515625}
\def\RealSubcubicAccuracyMeanFloat{0.285380986446845341664158013372798450291156768798828125}
\def\RealSubcubicAccuracyMedianFloat{0.00000000000000000000000000000000000978011299884143206629988798968908403945129743234376817895281419623643159866333008}
\def\RealSubcubicAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\RealSubcubicAccuracyStdDevFloat{0.2026742829548055235822090480724000371992588043212890625}
\def\RealSubcubicDroppedSequencesFracLen{15100}
\def\RealSubcubicDroppedSequencesFracMaxFloat{0.53906418480378193169855194355477578938007354736328125}
\def\RealSubcubicDroppedSequencesFracMeanFloat{0.195794622459914524625901321996934711933135986328125}
\def\RealSubcubicDroppedSequencesFracMedianFloat{0}
\def\RealSubcubicDroppedSequencesFracMinFloat{0}
\def\RealSubcubicDroppedSequencesFracStdDevFloat{0.1465138619459875057859932212522835470736026763916015625}
\def\RealSubcubicDroppedSequencesLen{15100}
\def\RealSubcubicDroppedSequencesMaxFloat{716539205966160580971401308421148540}
\def\RealSubcubicDroppedSequencesMeanFloat{260255693597856974946694159459680256}
\def\RealSubcubicDroppedSequencesMedianFloat{0}
\def\RealSubcubicDroppedSequencesMinFloat{0}
\def\RealSubcubicDroppedSequencesStdDevFloat{194750327069177733286732938170335232}
\def\RealSubcubicEffectiveDimensionalityEstimateLen{15100}
\def\RealSubcubicEffectiveDimensionalityEstimateMaxFloat{10370}
\def\RealSubcubicEffectiveDimensionalityEstimateMeanFloat{6049.600000000000363797880709171295166015625}
\def\RealSubcubicEffectiveDimensionalityEstimateMedianFloat{4290}
\def\RealSubcubicEffectiveDimensionalityEstimateMinFloat{4290}
\def\RealSubcubicEffectiveDimensionalityEstimateStdDevFloat{1530.49032666005450664670206606388092041015625}
\def\RealSubcubicErrUpperBoundLen{15100}
\def\RealSubcubicErrUpperBoundMaxFloat{133.0085601806640625}
\def\RealSubcubicErrUpperBoundMeanFloat{32.2994531018844526215616497211158275604248046875}
\def\RealSubcubicErrUpperBoundMedianFloat{0}
\def\RealSubcubicErrUpperBoundMinFloat{0}
\def\RealSubcubicErrUpperBoundStdDevFloat{41.37278918181758768923828029073774814605712890625}
\def\RealSubcubicGapMostBelowValueLen{15100}
\def\RealSubcubicGapMostBelowValueMaxFloat{40}
\def\RealSubcubicGapMostBelowValueMeanFloat{4.0474172185430461468058638274669647216796875}
\def\RealSubcubicGapMostBelowValueMedianFloat{1}
\def\RealSubcubicGapMostBelowValueMinFloat{1}
\def\RealSubcubicGapMostBelowValueNumStdLen{15100}
\def\RealSubcubicGapMostBelowValueNumStdMaxFloat{1.5}
\def\RealSubcubicGapMostBelowValueNumStdMeanFloat{1.5}
\def\RealSubcubicGapMostBelowValueNumStdMedianFloat{1.5}
\def\RealSubcubicGapMostBelowValueNumStdMinFloat{1.5}
\def\RealSubcubicGapMostBelowValueNumStdStdDevFloat{0}
\def\RealSubcubicGapMostBelowValueSequenceFracLen{15100}
\def\RealSubcubicGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\RealSubcubicGapMostBelowValueSequenceFracMeanFloat{0.99297068597859894367729793884791433811187744140625}
\def\RealSubcubicGapMostBelowValueSequenceFracMedianFloat{0.9482583582401276078854834850062616169452667236328125}
\def\RealSubcubicGapMostBelowValueSequenceFracMinFloat{0.8931427001953125}
\def\RealSubcubicGapMostBelowValueSequenceFracStdDevFloat{0.009872268453546072242144049369017011485993862152099609375}
\def\RealSubcubicGapMostBelowValueStdDevFloat{3.165125038295942605515165269025601446628570556640625}
\def\RealSubcubicInstructionCountBranchLen{15100}
\def\RealSubcubicInstructionCountBranchMaxFloat{0}
\def\RealSubcubicInstructionCountBranchMeanFloat{0}
\def\RealSubcubicInstructionCountBranchMedianFloat{0}
\def\RealSubcubicInstructionCountBranchMinFloat{0}
\def\RealSubcubicInstructionCountBranchStdDevFloat{0}
\def\RealSubcubicInstructionCountIntLen{15100}
\def\RealSubcubicInstructionCountIntMaxFloat{0}
\def\RealSubcubicInstructionCountIntMeanFloat{0}
\def\RealSubcubicInstructionCountIntMedianFloat{0}
\def\RealSubcubicInstructionCountIntMinFloat{0}
\def\RealSubcubicInstructionCountIntStdDevFloat{0}
\def\RealSubcubicInstructionCountLen{15100}
\def\RealSubcubicInstructionCountMaxFloat{20356824}
\def\RealSubcubicInstructionCountMeanFloat{18392610.8000000007450580596923828125}
\def\RealSubcubicInstructionCountMedianFloat{17365718}
\def\RealSubcubicInstructionCountMinFloat{17365718}
\def\RealSubcubicInstructionCountStdDevFloat{802225.011615918134339153766632080078125}
\def\RealSubcubicMaxGapLen{15100}
\def\RealSubcubicMaxGapMaxFloat{63}
\def\RealSubcubicMaxGapMeanFloat{30.06509933774834308906065416522324085235595703125}
\def\RealSubcubicMaxGapMedianFloat{1}
\def\RealSubcubicMaxGapMinFloat{1}
\def\RealSubcubicMaxGapStdDevFloat{20.567577209649659408796651405282318592071533203125}
\def\RealSubcubicNormalizedAccuracyLen{15100}
\def\RealSubcubicNormalizedAccuracyMaxFloat{0.6572436982471929756144390921690501272678375244140625}
\def\RealSubcubicNormalizedAccuracyMeanFloat{0.28649185540496258095544135358068160712718963623046875}
\def\RealSubcubicNormalizedAccuracyMedianFloat{0.00000000000000000000000000000000000985300171323342070093429178227190602243421973120466404316741577720453947982842516045186103366970709060979061177931725978851318359375}
\def\RealSubcubicNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\RealSubcubicNormalizedAccuracyStdDevFloat{0.2032477359639176806016536147581064142286777496337890625}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.65682941314196041648898471976281143724918365478515625}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMaxKey{27671}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.56121004634953008949338482125313021242618560791015625}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMeanKey{7098}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.4200645042537107798352735699154436588287353515625}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMinFloat{0.25265074475171689361019389252760447561740875244140625}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.042968392297698144999262837018250138498842716217041015625}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.23052385661848628917169889973592944443225860595703125}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{27300}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.13407621728723950749184723463258706033229827880859375}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12457}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.04783335998494049612350664801851962693035602569580078125}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18289}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.02845918004020230041017924804691574536263942718505859375}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.039519286610340993715073665271120262332260608673095703125}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{306418763913599937668037273980403551}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{27300}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{178217861587140260755829682832670720}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12457}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{63581441224440886256543766388146176}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18289}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{37828738846520300492525058542808020}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{52530142135913202241742431210962944}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{104}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{7383.9735099337749488768167793750762939453125}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{1185}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4400.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{6910}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{8840}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{1820.64069920170322802732698619365692138671875}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{9.1559906005859375}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4157}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0.991665388574663353438154445029795169830322265625}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{3254}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{104}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinKey{104}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.9653311092506668966706229184637777507305145263671875}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{2.867549668874172397181609994731843471527099609375}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999849796295166015625}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{31308}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.992647306019107222851971528143621981143951416015625}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4810}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9595743119716644287109375}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20754}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95257580280303955078125}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{22286}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00910800686383549627789246727616045973263680934906005859375}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.571688525957807502919649778050370514392852783203125}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20348569}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMaxKey{6910}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18476152.19867549836635589599609375}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMeanKey{7467}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17910775}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMedianKey{104}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMinFloat{17910775}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMinKey{104}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{568715.6135063879191875457763671875}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMaxFloat{49}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMaxKey{1185}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMeanFloat{39.35761589403973204071007785387337207794189453125}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMeanKey{7310}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapStdDevFloat{12.4960096257843193967573824920691549777984619140625}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6572436982471929756144390921690501272678375244140625}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27671}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.56354892045871152195246622795821167528629302978515625}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{18668}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.43815901059012152263250072792288847267627716064453125}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{3254}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.297203989016589786853472787697683088481426239013671875}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0402918483747694844421260995659395121037960052490234375}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.77167415618896484375}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.857632138081726225209422409534454345703125}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1490}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.964951336383819580078125}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.6911551952362060546875}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8048}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.251991228210260320707902792491950094699859619140625}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.8180291652679443359375}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.44202332780850639437630889005959033966064453125}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMeanKey{17197}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.236496508121490478515625}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMedianKey{9816}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2120714187622088076068394002504646778106689453125}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1194509288843590144590933732615667395293712615966796875}
\def\RealSubcubicProofSearchTimeLen{15100}
\def\RealSubcubicProofSearchTimeMaxFloat{179.535578250885009765625}
\def\RealSubcubicProofSearchTimeMeanFloat{167.053254127739279510933556593954563140869140625}
\def\RealSubcubicProofSearchTimeMedianFloat{158.331018409729011864328640513122081756591796875}
\def\RealSubcubicProofSearchTimeMinFloat{51.5117042064666748046875}
\def\RealSubcubicProofSearchTimeStdDevFloat{5.31773778586767864595685750828124582767486572265625}
\def\RealSubcubicProofTimeLen{15100}
\def\RealSubcubicProofTimeMaxFloat{9.88440799713134765625}
\def\RealSubcubicProofTimeMeanFloat{9.4070758672265810673707164824008941650390625}
\def\RealSubcubicProofTimeMedianFloat{9.1597884130477922326463158242404460906982421875}
\def\RealSubcubicProofTimeMinFloat{9.0863430500030517578125}
\def\RealSubcubicProofTimeStdDevFloat{0.12458653641845711390612194691129843704402446746826171875}
\def\ResampleEQKEErrLen{100}
\def\ResampleEQKEErrMaxLen{151}
\def\ResampleEQKEErrMaxMaxFloat{1.6478106975555419921875}
\def\ResampleEQKEErrMaxMaxKey{1490}
\def\ResampleEQKEErrMaxMeanFloat{1.195182462007004620119232640718109905719757080078125}
\def\ResampleEQKEErrMaxMeanKey{16069}
\def\ResampleEQKEErrMaxMedianFloat{0.98268003761768341064453125}
\def\ResampleEQKEErrMaxMedianKey{13293}
\def\ResampleEQKEErrMaxMinFloat{0.9567348957061767578125}
\def\ResampleEQKEErrMaxMinKey{13468}
\def\ResampleEQKEErrMaxStdDevFloat{0.11593772161485593752416889401501975953578948974609375}
\def\ResampleEQKEErrMeanLen{151}
\def\ResampleEQKEErrMeanMaxFloat{0.9318767488002777099609375}
\def\ResampleEQKEErrMeanMaxKey{29565}
\def\ResampleEQKEErrMeanMeanFloat{0.8287615191462813779565976801677606999874114990234375}
\def\ResampleEQKEErrMeanMeanKey{6159}
\def\ResampleEQKEErrMeanMedianFloat{0.71792771562933921369875633899937383830547332763671875}
\def\ResampleEQKEErrMeanMedianKey{13468}
\def\ResampleEQKEErrMeanMinFloat{0.708258349895477312685443394002504646778106689453125}
\def\ResampleEQKEErrMeanMinKey{17197}
\def\ResampleEQKEErrMeanStdDevFloat{0.044130321758332292925164352936917566694319248199462890625}
\def\ResampleEQKEErrMedianLen{151}
\def\ResampleEQKEErrMedianMaxFloat{0.73794436067342761287335406450438313186168670654296875}
\def\ResampleEQKEErrMedianMaxKey{12561}
\def\ResampleEQKEErrMedianMeanFloat{0.64682587288073356557305260139401070773601531982421875}
\def\ResampleEQKEErrMedianMeanKey{50}
\def\ResampleEQKEErrMedianMedianFloat{0.54889830522239202448275818824185989797115325927734375}
\def\ResampleEQKEErrMedianMedianKey{12552}
\def\ResampleEQKEErrMedianMinFloat{0.54069743484258647736595548849436454474925994873046875}
\def\ResampleEQKEErrMedianMinKey{9132}
\def\ResampleEQKEErrMedianStdDevFloat{0.03897850376809063044358794059007777832448482513427734375}
\def\ResampleEQKEErrMinLen{151}
\def\ResampleEQKEErrMinMaxFloat{0.72500622272491455078125}
\def\ResampleEQKEErrMinMaxKey{23367}
\def\ResampleEQKEErrMinMeanFloat{0.63703837615764691282294052143697626888751983642578125}
\def\ResampleEQKEErrMinMeanKey{3254}
\def\ResampleEQKEErrMinMedianFloat{0.540559232234954833984375}
\def\ResampleEQKEErrMinMedianKey{12552}
\def\ResampleEQKEErrMinMinFloat{0.52851307392120361328125}
\def\ResampleEQKEErrMinMinKey{9132}
\def\ResampleEQKEErrMinStdDevFloat{0.040178866014875559697916429513497860170900821685791015625}
\def\ResampleEQKEErrNumSamples{100}
\def\ResampleEQKEErrSeed{1234}
\def\ResampleEQKEErrStdDevLen{151}
\def\ResampleEQKEErrStdDevMaxFloat{0.13695687723459359919075950529077090322971343994140625}
\def\ResampleEQKEErrStdDevMaxKey{4647}
\def\ResampleEQKEErrStdDevMeanFloat{0.10496552115755260203844301258868654258549213409423828125}
\def\ResampleEQKEErrStdDevMeanKey{26829}
\def\ResampleEQKEErrStdDevMedianFloat{0.07727716561115179072505299018303048796951770782470703125}
\def\ResampleEQKEErrStdDevMedianKey{13468}
\def\ResampleEQKEErrStdDevMinFloat{0.07277411292889024441166156975668855011463165283203125}
\def\ResampleEQKEErrStdDevMinKey{13293}
\def\ResampleEQKEErrStdDevStdDevFloat{0.012809502962128425929133612726218416355550289154052734375}
\def\ResampleNormalEQKEErrLen{100}
\def\ResampleNormalEQKEErrMaxLen{151}
\def\ResampleNormalEQKEErrMaxMaxFloat{1.257103443145751953125}
\def\ResampleNormalEQKEErrMaxMaxKey{29565}
\def\ResampleNormalEQKEErrMaxMeanFloat{1.1180892124870756010324157614377327263355255126953125}
\def\ResampleNormalEQKEErrMaxMeanKey{29195}
\def\ResampleNormalEQKEErrMaxMedianFloat{0.976312458515167236328125}
\def\ResampleNormalEQKEErrMaxMedianKey{17197}
\def\ResampleNormalEQKEErrMaxMinFloat{0.9736526012420654296875}
\def\ResampleNormalEQKEErrMaxMinKey{29052}
\def\ResampleNormalEQKEErrMaxStdDevFloat{0.059265521171248114473684154290822334587574005126953125}
\def\ResampleNormalEQKEErrMeanLen{151}
\def\ResampleNormalEQKEErrMeanMaxFloat{0.8742611545324325827976963410037569701671600341796875}
\def\ResampleNormalEQKEErrMeanMaxKey{29565}
\def\ResampleNormalEQKEErrMeanMeanFloat{0.7743384734131641966570214208331890404224395751953125}
\def\ResampleNormalEQKEErrMeanMeanKey{21598}
\def\ResampleNormalEQKEErrMeanMedianFloat{0.68374649330973624739016258899937383830547332763671875}
\def\ResampleNormalEQKEErrMeanMedianKey{29052}
\def\ResampleNormalEQKEErrMeanMinFloat{0.6764051330089568825343349089962430298328399658203125}
\def\ResampleNormalEQKEErrMeanMinKey{17197}
\def\ResampleNormalEQKEErrMeanStdDevFloat{0.039547250828290948787557823607130558229982852935791015625}
\def\ResampleNormalEQKEErrMedianLen{151}
\def\ResampleNormalEQKEErrMedianMaxFloat{0.7148811656236648826023838410037569701671600341796875}
\def\ResampleNormalEQKEErrMedianMaxKey{29565}
\def\ResampleNormalEQKEErrMedianMeanFloat{0.62665422958451377777322477413690648972988128662109375}
\def\ResampleNormalEQKEErrMedianMeanKey{4430}
\def\ResampleNormalEQKEErrMedianMedianFloat{0.5560520236194133048002186114899814128875732421875}
\def\ResampleNormalEQKEErrMedianMedianKey{18289}
\def\ResampleNormalEQKEErrMedianMinFloat{0.54515074253082274058357370449812151491641998291015625}
\def\ResampleNormalEQKEErrMedianMinKey{17197}
\def\ResampleNormalEQKEErrMedianStdDevFloat{0.03330612356002583818170847962392144836485385894775390625}
\def\ResampleNormalEQKEErrMinLen{151}
\def\ResampleNormalEQKEErrMinMaxFloat{0.714531421661376953125}
\def\ResampleNormalEQKEErrMinMaxKey{29565}
\def\ResampleNormalEQKEErrMinMeanFloat{0.62163962907349035180715191017952747642993927001953125}
\def\ResampleNormalEQKEErrMinMeanKey{742}
\def\ResampleNormalEQKEErrMinMedianFloat{0.542997300624847412109375}
\def\ResampleNormalEQKEErrMinMedianKey{18289}
\def\ResampleNormalEQKEErrMinMinFloat{0.5348818302154541015625}
\def\ResampleNormalEQKEErrMinMinKey{17197}
\def\ResampleNormalEQKEErrMinStdDevFloat{0.034747131478334324083956374806803069077432155609130859375}
\def\ResampleNormalEQKEErrStdDevLen{151}
\def\ResampleNormalEQKEErrStdDevMaxFloat{0.095335937727553388132406553268083371222019195556640625}
\def\ResampleNormalEQKEErrStdDevMaxKey{29565}
\def\ResampleNormalEQKEErrStdDevMeanFloat{0.0848906723346380676087363781334715895354747772216796875}
\def\ResampleNormalEQKEErrStdDevMeanKey{3175}
\def\ResampleNormalEQKEErrStdDevMedianFloat{0.07423341247692248623391009232364012859761714935302734375}
\def\ResampleNormalEQKEErrStdDevMedianKey{17197}
\def\ResampleNormalEQKEErrStdDevMinFloat{0.07402917419454795033839644702311488799750804901123046875}
\def\ResampleNormalEQKEErrStdDevMinKey{29052}
\def\ResampleNormalEQKEErrStdDevStdDevFloat{0.004472937275824167939475284327954796026460826396942138671875}
\def\SubcubicAccuracyLen{7852}
\def\SubcubicAccuracyMaxFloat{0.65682941314196041648898471976281143724918365478515625}
\def\SubcubicAccuracyMeanFloat{0.379361297696823862590775888747884891927242279052734375}
\def\SubcubicAccuracyMedianFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicAccuracyStdDevFloat{0.1699860009085869261280521413937094621360301971435546875}
\def\SubcubicAttentionQuadraticAccuracyLen{1812}
\def\SubcubicAttentionQuadraticAccuracyMaxFloat{0.395645731875382489217685133553459309041500091552734375}
\def\SubcubicAttentionQuadraticAccuracyMeanFloat{0.28621383192044225207695262724882923066616058349609375}
\def\SubcubicAttentionQuadraticAccuracyMedianFloat{0.0686264265696620301415720177828916348516941070556640625}
\def\SubcubicAttentionQuadraticAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicAttentionQuadraticAccuracyStdDevFloat{0.053802209792955156542060279889483354054391384124755859375}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyMaxFloat{0.397668706068207977732953395388904027640819549560546875}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyMeanFloat{0.1331757127486903613533542056757141835987567901611328125}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyMedianFloat{0.00000000000000000000000000000000000902779661431516806119989660586684680564735147600963216518721310421824455261230469}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyStdDevFloat{0.1289398028739690837962683644946082495152950286865234375}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracMaxFloat{0.51102902901206170849235377318109385669231414794921875}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracMeanFloat{0.267631010281064452005495013509062118828296661376953125}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracStdDevFloat{0.193659930184946149633873346829204820096492767333984375}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesMaxFloat{679274092021614382013061870951284366}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesMeanFloat{355742631405791073334069562835992576}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesStdDevFloat{257418200863581854258183402757816320}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateMeanFloat{6487.3333333333330301684327423572540283203125}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateStdDevFloat{42.66666666666666429819088079966604709625244140625}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundMaxFloat{133.0085601806640625}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundMeanFloat{94.8468834748594389338904875330626964569091796875}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundMedianFloat{74.71254730224609375}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundMinFloat{72.31154632568359375}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundStdDevFloat{9.21741835739664594484565895982086658477783203125}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueMaxFloat{34}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueMeanFloat{5.58903605592347307862155503244139254093170166015625}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueMedianFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueMinFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracMeanFloat{0.99604280024350255740017701100441627204418182373046875}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracMedianFloat{0.97226371586322779538846816649311222136020660400390625}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracMinFloat{0.96463572978973399774105246251565404236316680908203125}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.0055163893611844816433631422114558517932891845703125}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueStdDevFloat{3.697639268087753006142293088487349450588226318359375}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountMaxFloat{17624307}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountMeanFloat{17494996.6666666679084300994873046875}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountMedianFloat{17365718}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountMinFloat{17365718}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountStdDevFloat{115433.622899819703889079391956329345703125}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapMaxFloat{63}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapMeanFloat{30.428256070640177455288721830584108829498291015625}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapMedianFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapMinFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapStdDevFloat{22.719062849349146659960752003826200962066650390625}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyMaxFloat{0.39786289282033415748429661107365973293781280517578125}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyMeanFloat{0.1337484353910560475053870277406531386077404022216796875}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyMedianFloat{0.00000000000000000000000000000000000918701489667776217044949118979087388873213108951222041500396842134538477567709204720146289220583657453289561090059578418731689453125}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyStdDevFloat{0.129423839396391571199274039827287197113037109375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.397668706068207977732953395388904027640819549560546875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{18146}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.320813463172009871726686469628475606441497802734375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{20751}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.225449495342744554715608273909310810267925262451171875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{6589}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.14620391746150118716940369267831556499004364013671875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03451882648931159369709575912565924227237701416015625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.49450019528885380548643979636835865676403045654296875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.412793657060229357558256424454157240688800811767578125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{11124}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2264651459430972735287213026822428219020366668701171875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1833222082877064007533363110269419848918914794921875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.04494834204990084958186713492978014983236789703369140625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{657303503499052664180563743974875609}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{548696885446894556847883987170885632}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{11124}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{301023812057081660692763048721514496}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{243677011505132896300767516542411365}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{59746594616844563374178661874794496}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6501.6026490066224141628481447696685791015625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{104}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{104}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{31.796555161449202131507263402454555034637451171875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{132.0067138671875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.32800530439970998486387543380260467529296875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{13036}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.435699462890625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{4729}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.464385986328125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.1860173478884359354879052261821925640106201171875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{33}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.5827814569536418076722839032299816608428955078125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99966263771057117804019753748434595763683319091796875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{5928}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99485514456073176337014274395187385380268096923828125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{13654}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97682605683803558349609375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{7098}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.975611507892608642578125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{27714}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004809556475722878178535868443077561096288263797760009765625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.86415993461379247975173711893148720264434814453125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17624307}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17606145.2847682125866413116455078125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{123}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17597590}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{104}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{17597590}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{104}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{8825.115588892740561277605593204498291015625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{59}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{47.5894039735099312338206800632178783416748046875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{2773}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{5358}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{5358}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.7195232897056538234892286709509789943695068359375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.39786289282033415748429661107365973293781280517578125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18146}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.322192355047441925108842042391188442707061767578125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8893}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.232320018548374862543681729221134446561336517333984375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6589}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.171985986117363764957843841330031864345073699951171875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.033851323337207583907826347058289684355258941650390625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.6679251194000244140625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.579345747335054284121724776923656463623046875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22545}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.5120990276336669921875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{51.5117042064666748046875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.0912397709757062358448820305056869983673095703125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.741107463836669921875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{20751}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4383096647578366145125983166508376598358154296875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{8893}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.222578465938568115234375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{8048}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1856682300567644716693394002504646778106689453125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.11823080355049053746796516861650161445140838623046875}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeMaxFloat{179.0413391590118408203125}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeMeanFloat{166.994218280334706605572137050330638885498046875}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeMedianFloat{158.044378738403310080684605054557323455810546875}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeMinFloat{51.5117042064666748046875}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeStdDevFloat{6.3021955600439287792369214002974331378936767578125}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeMaxFloat{9.8223588466644287109375}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeMeanFloat{9.402661049339680943148778169415891170501708984375}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeMedianFloat{9.1644240486621857399995860760100185871124267578125}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeMinFloat{9.11359882354736328125}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeStdDevFloat{0.12400996058897435780910001312804524786770343780517578125}
\def\SubcubicAttentionQuadraticDroppedSequencesFracLen{1812}
\def\SubcubicAttentionQuadraticDroppedSequencesFracMaxFloat{0.53906418480378193169855194355477578938007354736328125}
\def\SubcubicAttentionQuadraticDroppedSequencesFracMeanFloat{0.43071185785481080898762229480780661106109619140625}
\def\SubcubicAttentionQuadraticDroppedSequencesFracMedianFloat{0.239052186446396586205764833721332252025604248046875}
\def\SubcubicAttentionQuadraticDroppedSequencesFracMinFloat{0.211553882701121409581901389174163341522216796875}
\def\SubcubicAttentionQuadraticDroppedSequencesFracStdDevFloat{0.044301491629269940109026038044248707592487335205078125}
\def\SubcubicAttentionQuadraticDroppedSequencesLen{1812}
\def\SubcubicAttentionQuadraticDroppedSequencesMaxFloat{716539205966160580971401308421148540}
\def\SubcubicAttentionQuadraticDroppedSequencesMeanFloat{572514259577147082530287802808008704}
\def\SubcubicAttentionQuadraticDroppedSequencesMedianFloat{317754858678145764851270458974142464}
\def\SubcubicAttentionQuadraticDroppedSequencesMinFloat{281203343503328808952529059191571680}
\def\SubcubicAttentionQuadraticDroppedSequencesStdDevFloat{58886782928656792788368210324881408}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateLen{1812}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateMeanFloat{4459.6666666666669698315672576427459716796875}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateStdDevFloat{69.8514296362087492298087454400956630706787109375}
\def\SubcubicAttentionQuadraticErrUpperBoundLen{1812}
\def\SubcubicAttentionQuadraticErrUpperBoundMaxFloat{133.0085601806640625}
\def\SubcubicAttentionQuadraticErrUpperBoundMeanFloat{94.8468834748594389338904875330626964569091796875}
\def\SubcubicAttentionQuadraticErrUpperBoundMedianFloat{74.71254730224609375}
\def\SubcubicAttentionQuadraticErrUpperBoundMinFloat{72.31154632568359375}
\def\SubcubicAttentionQuadraticErrUpperBoundStdDevFloat{9.21741835739664594484565895982086658477783203125}
\def\SubcubicAttentionQuadraticGapMostBelowValueLen{1812}
\def\SubcubicAttentionQuadraticGapMostBelowValueMaxFloat{40}
\def\SubcubicAttentionQuadraticGapMostBelowValueMeanFloat{9.400662251655628409707787795923650264739990234375}
\def\SubcubicAttentionQuadraticGapMostBelowValueMedianFloat{5}
\def\SubcubicAttentionQuadraticGapMostBelowValueMinFloat{5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdLen{1812}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracLen{1812}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracMeanFloat{0.99487214481199026661073503419174812734127044677734375}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracMedianFloat{0.9651244974136352627880341970012523233890533447265625}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracMinFloat{0.96287399530410755499332253748434595763683319091796875}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.005637039964510031676836465663882336230017244815826416015625}
\def\SubcubicAttentionQuadraticGapMostBelowValueStdDevFloat{3.8421617700119696792171453125774860382080078125}
\def\SubcubicAttentionQuadraticInstructionCountBranchLen{1812}
\def\SubcubicAttentionQuadraticInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntLen{1812}
\def\SubcubicAttentionQuadraticInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntMinFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountLen{1812}
\def\SubcubicAttentionQuadraticInstructionCountMaxFloat{17888658}
\def\SubcubicAttentionQuadraticInstructionCountMeanFloat{17755902.8333333320915699005126953125}
\def\SubcubicAttentionQuadraticInstructionCountMedianFloat{17623862}
\def\SubcubicAttentionQuadraticInstructionCountMinFloat{17623862}
\def\SubcubicAttentionQuadraticInstructionCountStdDevFloat{115503.357026851052069105207920074462890625}
\def\SubcubicAttentionQuadraticMaxGapLen{1812}
\def\SubcubicAttentionQuadraticMaxGapMaxFloat{59}
\def\SubcubicAttentionQuadraticMaxGapMeanFloat{47.98896247240617896068215486593544483184814453125}
\def\SubcubicAttentionQuadraticMaxGapMedianFloat{7}
\def\SubcubicAttentionQuadraticMaxGapMinFloat{5}
\def\SubcubicAttentionQuadraticMaxGapStdDevFloat{8.6173812768984152654638819512911140918731689453125}
\def\SubcubicAttentionQuadraticNormalizedAccuracyLen{1812}
\def\SubcubicAttentionQuadraticNormalizedAccuracyMaxFloat{0.396284933977182618480838982577552087604999542236328125}
\def\SubcubicAttentionQuadraticNormalizedAccuracyMeanFloat{0.28733007775540475581266264271107502281665802001953125}
\def\SubcubicAttentionQuadraticNormalizedAccuracyMedianFloat{0.068677635770310718754672052455134689807891845703125}
\def\SubcubicAttentionQuadraticNormalizedAccuracyMinFloat{0.000000000000000000000000000000000011181575482347337861056731119226272875001609849420949822953073647966407680182923061018343525128970750159851377247832715511322021484375}
\def\SubcubicAttentionQuadraticNormalizedAccuracyStdDevFloat{0.05361830221153436604186737213240121491253376007080078125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.395645731875382489217685133553459309041500091552734375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{2549}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.32206099986810776680812296035583131015300750732421875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{22261}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.2234384169845317347213864422883489169180393218994140625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{20338}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.14027922166280359927981180589995346963405609130859375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03531570867472944019738179122214205563068389892578125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.51767416503234719993287171746487729251384735107421875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.42446084178531251485111397414584644138813018798828125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{2773}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.303701338076456550663095868003438226878643035888671875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.239032276832243206765582499429001472890377044677734375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.041129682999143608868042321091706980951130390167236328125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{688106992855576642127521065211480032}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{564205234015469079133404676698931200}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{2773}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{403688320928565572207835245661126656}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{317728394261627805337596407425425050}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{54670726100220605413005866639032320}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{104}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4505.205298013244828325696289539337158203125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{1696}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{1696}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{53.12191624156726987848742282949388027191162109375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{132.0067138671875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.454141124194819667536648921668529510498046875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{20294}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.913082122802734375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{74.71254730224609375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.140303078238947165345962275750935077667236328125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{31}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{9134}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.1788079470198677967118783271871507167816162109375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{18289}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99953812360763560906917746251565404236316680908203125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1185}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.995465654805796074100499026826582849025726318359375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6155}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97457800805568683966129128748434595763683319091796875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20754}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97159016132354736328125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20751}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004552097554493796972840957693051677779294550418853759765625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{3.46235400670575810266882399446330964565277099609375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17888658}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{7238}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17863563.735099337995052337646484375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{1696}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17853686}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{17853686}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{8881.119974195416943985037505626678466796875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{55}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{30371}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{49.25827814569536400313154445029795169830322265625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{24.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{20751}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.2837496358333684298713706084527075290679931640625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.396284933977182618480838982577552087604999542236328125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2549}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.323431092135191555758666481779073365032672882080078125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5781}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.2298065820248069712761207483708858489990234375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{20338}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.165016510421524598140052830785862170159816741943359375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.034601856296693385417473365350815583951771259307861328125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.53505229949951171875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.704189933688439850811846554279327392578125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{19004}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{161.123529613018035888671875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4430}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{160.7388155460357666015625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8048}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.107825577041996023552883343654684722423553466796875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7844679355621337890625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{27671}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4404323053675778254500983166508376598358154296875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{21317}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.21865284442901611328125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{9816}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1872019767761248232318394002504646778106689453125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{11124}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12629046188429804420394475528155453503131866455078125}
\def\SubcubicAttentionQuadraticProofSearchTimeLen{1812}
\def\SubcubicAttentionQuadraticProofSearchTimeMaxFloat{177.5690329074859619140625}
\def\SubcubicAttentionQuadraticProofSearchTimeMeanFloat{167.115040506485030391559121198952198028564453125}
\def\SubcubicAttentionQuadraticProofSearchTimeMedianFloat{158.917686175107945700801792554557323455810546875}
\def\SubcubicAttentionQuadraticProofSearchTimeMinFloat{157.49991607666015625}
\def\SubcubicAttentionQuadraticProofSearchTimeStdDevFloat{3.2754195817414739622108754701912403106689453125}
\def\SubcubicAttentionQuadraticProofTimeLen{1812}
\def\SubcubicAttentionQuadraticProofTimeMaxFloat{9.823398113250732421875}
\def\SubcubicAttentionQuadraticProofTimeMeanFloat{9.4124585716403341706381979747675359249114990234375}
\def\SubcubicAttentionQuadraticProofTimeMedianFloat{9.1778050661087018369244105997495353221893310546875}
\def\SubcubicAttentionQuadraticProofTimeMinFloat{9.12524509429931640625}
\def\SubcubicAttentionQuadraticProofTimeStdDevFloat{0.12383048680950255182597885550421779043972492218017578125}
\def\SubcubicAttentionVocabModelSquaredAccuracyLen{3020}
\def\SubcubicAttentionVocabModelSquaredAccuracyMaxFloat{0.641348385379791441351926550851203501224517822265625}
\def\SubcubicAttentionVocabModelSquaredAccuracyMeanFloat{0.48080983686208134120221302509889937937259674072265625}
\def\SubcubicAttentionVocabModelSquaredAccuracyMedianFloat{0.10741857810770978620684701354548451490700244903564453125}
\def\SubcubicAttentionVocabModelSquaredAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicAttentionVocabModelSquaredAccuracyStdDevFloat{0.0830241680284072580686682840678258799016475677490234375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyMaxFloat{0.6064075623937725811885002258350141346454620361328125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyMeanFloat{0.213804944499108862121516949628130532801151275634765625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyMedianFloat{0.00000000000000000000000000000000000902779661431516806119989660586684680564735147600963216518721310421824455261230469}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyStdDevFloat{0.2062285163424837641787945585747365839779376983642578125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracMaxFloat{0.3752746673646409902858067653141915798187255859375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracMeanFloat{0.12126071017211335900665147846666513942182064056396484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracStdDevFloat{0.09315981819434815403013772083795629441738128662109375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesMaxFloat{498825593969952824523070029421222213}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesMeanFloat{161183130749534004192991260446818304}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesStdDevFloat{123830638426161588595420081898389504}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateMeanFloat{6457.4666666666662422358058393001556396484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateMedianFloat{6338}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateMinFloat{6338}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateStdDevFloat{56.60372975539882389739432255737483501434326171875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundMaxFloat{25.76837158203125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundMeanFloat{7.23365771691530756726251638610847294330596923828125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundMedianFloat{3.6845729351043701171875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundMinFloat{3.5355336666107177734375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundStdDevFloat{2.818143393080390968208348567713983356952667236328125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueMaxFloat{9}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueMeanFloat{2.481015452538631205214869623887352645397186279296875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueMedianFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueMinFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracMeanFloat{0.99160490203114270979511957193608395755290985107421875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracMedianFloat{0.94176664024591449919654451150563545525074005126953125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracMinFloat{0.8931427001953125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.01142611030017413875636833608950837515294551849365234375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueStdDevFloat{1.1424835780135025320447539343149401247501373291015625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountMaxFloat{20092473}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountMeanFloat{18715154.3333333320915699005126953125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountMedianFloat{17896022}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountMinFloat{17896022}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountStdDevFloat{723691.281550880405120551586151123046875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapMaxFloat{52}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapMeanFloat{21.915011037527595050278250710107386112213134765625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapMedianFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapMinFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapStdDevFloat{20.27100213181712007326495950110256671905517578125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyMaxFloat{0.6067446714283786235455409041605889797210693359375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyMeanFloat{0.2146696848810800972717771628595073707401752471923828125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyMedianFloat{0.00000000000000000000000000000000000918701489667776217044949118979087388873213108951222041500396842134538477567709204720146289220583657453289561090059578418731689453125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyStdDevFloat{0.206910665536153171029098984945449046790599822998046875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6064075623937725811885002258350141346454620361328125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5259578695325901609436414219089783728122711181640625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{30684}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.3847055762794624467204585016588680446147918701171875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.238996153214439510659161669536842964589595794677734375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.041246108155878986878395409121367265470325946807861328125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.261200279071756080728761162390583194792270660400390625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1667996060247548817390139674898819066584110260009765625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{11498}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.04608553246768244682218806929085985757410526275634765625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0300437945554398004588403381376338074915111064910888671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037539975911930707763719539116209489293396472930908203125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{347194723449011078610315099327629011}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{221714706013998620863807684704468992}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{11498}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{61258179956698243924747025463115776}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{39935052822701027664841858754564702}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49899186943229664998028801826881536}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{123}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6489.7350993377485792734660208225250244140625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6450}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{7310}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{31.7796015184623001914587803184986114501953125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.6324939727783203125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.27478027659536241600335415569134056568145751953125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{27584}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.783549010753631147707665149937383830547332763671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32103}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.6634309291839599609375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{8840}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.738326613671914433467691196710802614688873291015625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.125827814569536400313154445029795169830322265625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99969160556793201788394753748434595763683319091796875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{29022}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99037608089825968082919871449121274054050445556640625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7790}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93811319768428802490234375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.893275201320648193359375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01112124686773548198903682759919320233166217803955078125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.435276204639867103640682444165577180683612823486328125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20092473}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{7310}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18269403.099337749183177947998046875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{123}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18127894}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{18127894}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{313338.1599132127012126147747039794921875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{2306}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{36.68874172185430637682657106779515743255615234375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{29725}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.08395289175145848048487096093595027923583984375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6067446714283786235455409041605889797210693359375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.52814679443530021529795703827403485774993896484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{27584}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.400933579659400962658111211567302234470844268798828125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6204}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.28114150292631900907025510605308227241039276123046875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03874858981339181218661593675278709270060062408447265625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.7373340129852294921875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.602082707234558256459422409534454345703125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{13468}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.731911599636077880859375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{51.602179050445556640625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.0699252308332294347792412736453115940093994140625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7576975822448712705181605997495353221893310546875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.443167899618085669999345554970204830169677734375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{30684}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.20833241939544677734375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{9816}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1634089946746843935443394002504646778106689453125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1283144310823415568112437767922529019415378570556640625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeMaxFloat{179.535578250885009765625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeMeanFloat{167.055883590275101369115873239934444427490234375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeMedianFloat{157.913934996128091370337642729282379150390625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeMinFloat{51.602179050445556640625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeStdDevFloat{6.31639246176139312893837995943613350391387939453125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeMaxFloat{9.8397514820098876953125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeMeanFloat{9.4027398784165878709018215886317193508148193359375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeMedianFloat{9.1531567561626427931287253159098327159881591796875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeMinFloat{9.0864479541778564453125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeStdDevFloat{0.1262909835457892426813231168125639669597148895263671875}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracLen{3020}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracMaxFloat{0.385970026901434615229646851730649359524250030517578125}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracMeanFloat{0.177868555488155333232924704134347848594188690185546875}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracMedianFloat{0.0674845737680082879972331966200727038085460662841796875}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracMinFloat{0.0351667256257661986484919225404155440628528594970703125}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracStdDevFloat{0.049052659747330397410625124621219583787024021148681640625}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesLen{3020}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesMaxFloat{513042165291244041244930547085511911}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesMeanFloat{236427863524679181269763531961532416}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesMedianFloat{89702384736049038711578727637057536}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesMinFloat{46744596221855241737476146234675208}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesStdDevFloat{65202168603863411219879741712498688}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateLen{3020}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateMeanFloat{4429.8000000000001818989403545856475830078125}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateMedianFloat{4290}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateMinFloat{4290}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateStdDevFloat{79.13760168213337919951300136744976043701171875}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundLen{3020}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundMaxFloat{25.76837158203125}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundMeanFloat{7.23365771691530756726251638610847294330596923828125}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundMedianFloat{3.696846004724502865457225198042578995227813720703125}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundMinFloat{3.5355336666107177734375}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundStdDevFloat{2.818143393080390968208348567713983356952667236328125}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueLen{3020}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueMaxFloat{10}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueMeanFloat{3.25927152317880786114301372435875236988067626953125}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueMedianFloat{2}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueMinFloat{2}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdLen{3020}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracLen{3020}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracMeanFloat{0.991870808344803123191013582982122898101806640625}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracMedianFloat{0.94549162685871135369808371251565404236316680908203125}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracMinFloat{0.89577758312225341796875}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracStdDevFloat{0.01021201852157068747095625127485618577338755130767822265625}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueStdDevFloat{0.62825059257422533054437963073723949491977691650390625}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchLen{3020}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntLen{3020}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountLen{3020}
\def\SubcubicAttentionVocabModelSquaredInstructionCountMaxFloat{20356824}
\def\SubcubicAttentionVocabModelSquaredInstructionCountMeanFloat{18976060.5}
\def\SubcubicAttentionVocabModelSquaredInstructionCountMedianFloat{18154166}
\def\SubcubicAttentionVocabModelSquaredInstructionCountMinFloat{18154166}
\def\SubcubicAttentionVocabModelSquaredInstructionCountStdDevFloat{723702.4078870057128369808197021484375}
\def\SubcubicAttentionVocabModelSquaredMaxGapLen{3020}
\def\SubcubicAttentionVocabModelSquaredMaxGapMaxFloat{50}
\def\SubcubicAttentionVocabModelSquaredMaxGapMeanFloat{35.50894039735099028121112496592104434967041015625}
\def\SubcubicAttentionVocabModelSquaredMaxGapMedianFloat{3}
\def\SubcubicAttentionVocabModelSquaredMaxGapMinFloat{3}
\def\SubcubicAttentionVocabModelSquaredMaxGapStdDevFloat{16.16769281407283642693073488771915435791015625}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyLen{3020}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyMaxFloat{0.64175290606356660827458426865632645785808563232421875}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyMeanFloat{0.482609209988254572731847247268888168036937713623046875}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyMedianFloat{0.111319604133652827471223645261488854885101318359375}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyMinFloat{0.000000000000000000000000000000000011181575482347337861056731119226272875001609849420949822953073647966407680182923061018343525128970750159851377247832715511322021484375}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyStdDevFloat{0.0823901853485693724810090543542173691093921661376953125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.641348385379791441351926550851203501224517822265625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMaxKey{27671}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.54685743080981563668530043287319131195545196533203125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMeanKey{8721}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.408998786961925986371824137677322141826152801513671875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMedianKey{3284}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2291356758800124904240647083497606217861175537109375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.043149911616221399424109250730907660908997058868408203125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.254201377561040275931958376531838439404964447021484375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1551303579579767777385512772525544278323650360107421875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{9132}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.07220563313283949458121213638150948099792003631591796875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18668}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.06375108429544999733007415443353238515555858612060546875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{30463}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.038311954230759732997757538441874203272163867950439453125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{337891587621226273234212094562688152}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{206203614793878194434393132784156672}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{9132}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{95977749013545194491520884873887744}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18668}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{84739726007156293810401122551695382}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinKey{30463}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{50925322136756188217032072094547968}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{123}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4492.0397350993380314321257174015045166015625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{104}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{104}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{52.40214858275152920441541937179863452911376953125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{17.708660125732421875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.87777054704577750499083776958286762237548828125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{19538}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.633436143398284912109375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.543451786041260209714209850062616169452667236328125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.037202913893230604713835418806411325931549072265625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.105960264900662348708237914252094924449920654296875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4647}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4647}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999999940395355224609375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{25516}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99497579067748109782343135520932264626026153564453125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4305}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96791388094425201416015625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8299}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.958162844181060791015625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{4647}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.006308926507187491948547286568782510585151612758636474609375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.50365969117434550295087092308676801621913909912109375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20348569}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMaxKey{2306}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18689633.9271523170173168182373046875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMeanKey{1696}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18383990}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMedianKey{519}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMinFloat{18383990}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMinKey{519}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{493671.0644455435685813426971435546875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMaxFloat{49}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMaxKey{1185}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMeanFloat{40.01324503311258240501047112047672271728515625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMeanKey{21317}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapStdDevFloat{12.165517850428638979565221234224736690521240234375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.64175290606356660827458426865632645785808563232421875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27671}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.54911633217501665260584786665276624262332916259765625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20751}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.420666804481374445590091681879130192101001739501953125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{3284}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.26954219733044870732641129507101140916347503662109375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.040627765868241884350542392212446429766714572906494140625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.524883270263671875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.630072641056898419265053234994411468505859375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{19004}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.571762979030609130859375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8048}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.9889867305755615234375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.28130438765850751536845564260147511959075927734375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.88440799713134765625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMaxKey{16284}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4441742739140597251434883219189941883087158203125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMeanKey{15399}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2505727410316449521587855997495353221893310546875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2456076145172119140625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12214101967450698149608712128610932268202304840087890625}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeLen{3020}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeMaxFloat{176.655929088592529296875}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeMeanFloat{167.078262213208034836497972719371318817138671875}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeMedianFloat{158.998518816232689232492703013122081756591796875}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeMinFloat{157.8196036815643310546875}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeStdDevFloat{3.321786266602637649469897951348684728145599365234375}
\def\SubcubicAttentionVocabModelSquaredProofTimeLen{3020}
\def\SubcubicAttentionVocabModelSquaredProofTimeMaxFloat{9.88440799713134765625}
\def\SubcubicAttentionVocabModelSquaredProofTimeMeanFloat{9.41513169806524530258684535510838031768798828125}
\def\SubcubicAttentionVocabModelSquaredProofTimeMedianFloat{9.1593808579444893069876343361102044582366943359375}
\def\SubcubicAttentionVocabModelSquaredProofTimeMinFloat{9.0863430500030517578125}
\def\SubcubicAttentionVocabModelSquaredProofTimeStdDevFloat{0.12311822244441754381494291692433762364089488983154296875}
\def\SubcubicDirectQuadraticAccuracyLen{1812}
\def\SubcubicDirectQuadraticAccuracyMaxFloat{0.62161638823541254250670817782520316541194915771484375}
\def\SubcubicDirectQuadraticAccuracyMeanFloat{0.2220810187626432175012070047159795649349689483642578125}
\def\SubcubicDirectQuadraticAccuracyMedianFloat{0.00000000000000000000000000000000000902779661431516806119989660586684680564735147600963216518721310421824455261230469}
\def\SubcubicDirectQuadraticAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicDirectQuadraticAccuracyStdDevFloat{0.21387178140226426048542407443164847791194915771484375}
\def\SubcubicDirectQuadraticDroppedSequencesFracLen{1812}
\def\SubcubicDirectQuadraticDroppedSequencesFracMaxFloat{0.253903051267039991945040355858509428799152374267578125}
\def\SubcubicDirectQuadraticDroppedSequencesFracMeanFloat{0.10344158288211068030815198426353163085877895355224609375}
\def\SubcubicDirectQuadraticDroppedSequencesFracMedianFloat{0}
\def\SubcubicDirectQuadraticDroppedSequencesFracMinFloat{0}
\def\SubcubicDirectQuadraticDroppedSequencesFracStdDevFloat{0.07914522273174999511535787632965366356074810028076171875}
\def\SubcubicDirectQuadraticDroppedSequencesLen{1812}
\def\SubcubicDirectQuadraticDroppedSequencesMaxFloat{337495043959362320426199472995857804}
\def\SubcubicDirectQuadraticDroppedSequencesMeanFloat{137497447895207536424459434320723968}
\def\SubcubicDirectQuadraticDroppedSequencesMedianFloat{0}
\def\SubcubicDirectQuadraticDroppedSequencesMinFloat{0}
\def\SubcubicDirectQuadraticDroppedSequencesStdDevFloat{105202045787674828881848797965058048}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateLen{1812}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateMeanFloat{8428.666666666666060336865484714508056640625}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateStdDevFloat{1920.237022406927508200169540941715240478515625}
\def\SubcubicDirectQuadraticErrUpperBoundLen{1812}
\def\SubcubicDirectQuadraticErrUpperBoundMaxFloat{4.94955348968505859375}
\def\SubcubicDirectQuadraticErrUpperBoundMeanFloat{1.142796004844817137069412638084031641483306884765625}
\def\SubcubicDirectQuadraticErrUpperBoundMedianFloat{0}
\def\SubcubicDirectQuadraticErrUpperBoundMinFloat{0}
\def\SubcubicDirectQuadraticErrUpperBoundStdDevFloat{1.2240484607244557224703385145403444766998291015625}
\def\SubcubicDirectQuadraticGapMostBelowValueLen{1812}
\def\SubcubicDirectQuadraticGapMostBelowValueMaxFloat{5}
\def\SubcubicDirectQuadraticGapMostBelowValueMeanFloat{2.33002207505518743602124231983907520771026611328125}
\def\SubcubicDirectQuadraticGapMostBelowValueMedianFloat{1}
\def\SubcubicDirectQuadraticGapMostBelowValueMinFloat{1}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdLen{1812}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracLen{1812}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracMeanFloat{0.99251259465354435551631695489049889147281646728515625}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracMedianFloat{0.94706051349639908121247344752191565930843353271484375}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracMinFloat{0.893912732601165771484375}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.0111536160993581275058250668053005938418209552764892578125}
\def\SubcubicDirectQuadraticGapMostBelowValueStdDevFloat{0.9913107025574603436979259640793316066265106201171875}
\def\SubcubicDirectQuadraticInstructionCountBranchLen{1812}
\def\SubcubicDirectQuadraticInstructionCountBranchMaxFloat{0}
\def\SubcubicDirectQuadraticInstructionCountBranchMeanFloat{0}
\def\SubcubicDirectQuadraticInstructionCountBranchMedianFloat{0}
\def\SubcubicDirectQuadraticInstructionCountBranchMinFloat{0}
\def\SubcubicDirectQuadraticInstructionCountBranchStdDevFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntLen{1812}
\def\SubcubicDirectQuadraticInstructionCountIntMaxFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntMeanFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntMedianFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntMinFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntStdDevFloat{0}
\def\SubcubicDirectQuadraticInstructionCountLen{1812}
\def\SubcubicDirectQuadraticInstructionCountMaxFloat{19142136}
\def\SubcubicDirectQuadraticInstructionCountMeanFloat{18410860.8333333320915699005126953125}
\def\SubcubicDirectQuadraticInstructionCountMedianFloat{17678903}
\def\SubcubicDirectQuadraticInstructionCountMinFloat{17678903}
\def\SubcubicDirectQuadraticInstructionCountStdDevFloat{626313.16279622097499668598175048828125}
\def\SubcubicDirectQuadraticMaxGapLen{1812}
\def\SubcubicDirectQuadraticMaxGapMaxFloat{50}
\def\SubcubicDirectQuadraticMaxGapMeanFloat{20.7400662251655631962421466596424579620361328125}
\def\SubcubicDirectQuadraticMaxGapMedianFloat{1}
\def\SubcubicDirectQuadraticMaxGapMinFloat{1}
\def\SubcubicDirectQuadraticMaxGapStdDevFloat{19.7812899535190780397897469811141490936279296875}
\def\SubcubicDirectQuadraticNormalizedAccuracyLen{1812}
\def\SubcubicDirectQuadraticNormalizedAccuracyMaxFloat{0.621961952033637910375318824662826955318450927734375}
\def\SubcubicDirectQuadraticNormalizedAccuracyMeanFloat{0.2229547449309668694095165619728504680097103118896484375}
\def\SubcubicDirectQuadraticNormalizedAccuracyMedianFloat{0.00000000000000000000000000000000000918701489667776217044949118979087388873213108951222041500396842134538477567709204720146289220583657453289561090059578418731689453125}
\def\SubcubicDirectQuadraticNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicDirectQuadraticNormalizedAccuracyStdDevFloat{0.2145527064065662903313835840890533290803432464599609375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.62161638823541254250670817782520316541194915771484375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.53767465222966637217183460961678065359592437744140625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{12141}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.384257413712088158330715259580756537616252899169921875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.23107931630025391189775518796523101627826690673828125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.042702271078237784285303035858305520378053188323974609375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.25143338190381381291871321081998758018016815185546875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.149152929982206028380886664308491162955760955810546875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7238}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0406167729949917510889889626923832111060619354248046875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.00941587681141400033302257810419177985750138759613037109375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.036784711054555108145081021575606428086757659912109375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{334212290301429738629344878731420455}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{198258250185695680801759032388878336}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7238}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{53988951763383900075292072706310144}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{12515847062593605744373671271668502}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{48895267750573507156850585555173376}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{9912.251655629139349912293255329132080078125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{1185}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{1185}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{1244.27492766262957957223989069461822509765625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{2.971518993377685546875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15399}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0.26661406605448945139613670107792131602764129638671875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.744369901476911621784893213771283626556396484375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.006622516556291202505235560238361358642578125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99999922513961803094417746251565404236316680908203125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12561}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9902175084644595504101971528143621981143951416015625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{8745}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93607722222805034295589621251565404236316680908203125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4647}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.89433825016021728515625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0127704671593993068778871702306787483394145965576171875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.481398194579768123890772812956129200756549835205078125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{19142136}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{1185}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18057559.7549668885767459869384765625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17910775}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{17910775}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{398997.81750041223131120204925537109375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{2306}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{35.93377483443708797494764439761638641357421875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{3254}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.5608903855687028539023231132887303829193115234375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.621961952033637910375318824662826955318450927734375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.53989101987162080309445855164085514843463897705078125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{15043}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.404353665278002705196769284157198853790760040283203125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6204}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.27182858554860855893053894760669209063053131103515625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.040135842837279257777627350378679693676531314849853515625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.4286468029022216796875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.447170554407392728535342030227184295654296875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4430}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.8080031871795654296875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{53.86025142669677734375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.91078159166180938655088539235293865203857421875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7203814983367919921875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{20751}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4364197743649516070263416622765362262725830078125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{32382}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2194715738296491025494105997495353221893310546875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{9.20488071441650390625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1183659430054928574094219584367237985134124755859375}
\def\SubcubicDirectQuadraticProofSearchTimeLen{1812}
\def\SubcubicDirectQuadraticProofSearchTimeMaxFloat{178.8347589969635009765625}
\def\SubcubicDirectQuadraticProofSearchTimeMeanFloat{166.958057915138084581485600210726261138916015625}
\def\SubcubicDirectQuadraticProofSearchTimeMedianFloat{158.139666934013376931034144945442676544189453125}
\def\SubcubicDirectQuadraticProofSearchTimeMinFloat{52.930239200592041015625}
\def\SubcubicDirectQuadraticProofSearchTimeStdDevFloat{6.3195306974007650069324881769716739654541015625}
\def\SubcubicDirectQuadraticProofTimeLen{1812}
\def\SubcubicDirectQuadraticProofTimeMaxFloat{9.793557643890380859375}
\def\SubcubicDirectQuadraticProofTimeMeanFloat{9.402364138077953015226739807985723018646240234375}
\def\SubcubicDirectQuadraticProofTimeMedianFloat{9.1670661067962644352746792719699442386627197265625}
\def\SubcubicDirectQuadraticProofTimeMinFloat{9.1124291419982927919818394002504646778106689453125}
\def\SubcubicDirectQuadraticProofTimeStdDevFloat{0.1239236875788114478069701362983323633670806884765625}
\def\SubcubicDroppedSequencesFracLen{7852}
\def\SubcubicDroppedSequencesFracMaxFloat{0.53906418480378193169855194355477578938007354736328125}
\def\SubcubicDroppedSequencesFracMeanFloat{0.213928514534017122361575502509367652237415313720703125}
\def\SubcubicDroppedSequencesFracMedianFloat{0}
\def\SubcubicDroppedSequencesFracMinFloat{0}
\def\SubcubicDroppedSequencesFracStdDevFloat{0.13405986670097380653032814734615385532379150390625}
\def\SubcubicDroppedSequencesLen{7852}
\def\SubcubicDroppedSequencesMaxFloat{716539205966160580971401308421148540}
\def\SubcubicDroppedSequencesMeanFloat{284359770615297079955426507583651840}
\def\SubcubicDroppedSequencesMedianFloat{0}
\def\SubcubicDroppedSequencesMinFloat{0}
\def\SubcubicDroppedSequencesStdDevFloat{178196127930127546144561471976112128}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.57281880589920930457736858443240635097026824951171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{3175}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.42897678039947828576572419478907249867916107177734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{6910}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.09282220202650655338505458757936139591038227081298828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.26376904885858198923642703448422253131866455078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1578502173623005100377980625125928781926631927490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0732318279004200434201266034506261348724365234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.061427238711717797869926727116762776859104633331298828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.03923643553759827151683481361033045686781406402587890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{350609204164386497703745207010680660}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{209818928058703962907029183691489280}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{97341795827741347221155914358718464}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{81650805399378336548174485457430969}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{52154168571385789390043814719127552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{2.986754966887417150900319029460661113262176513671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98950144865654954262623732574866153299808502197265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93056507408618927001953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{27484}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.895777761936187744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0132519272858532093095629278423075447790324687957763671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.445533462027924820336721722924266941845417022705078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17945302}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17945302}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17945302}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{17945302}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{49}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{1185}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{25.172185430463574817849803366698324680328369140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{19.17530199194192164213745854794979095458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.57422045784228725739950505158049054443836212158203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{3175}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.43028967775723925281994297620258294045925140380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000000000000000000134151811522021916719243631753249916095268550227280107599826998463031890391656867414697340383511470207622551242820918560028076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000011181575482347337861056731119226272875001609849420949822953073647966407680182923061018343525128970750159851377247832715511322021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.09283186398392147264946316909117740578949451446533203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{174.827021121978759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.5516115908591245897696353495121002197265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.064307391643524169921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4430}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.5163447856903076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.242916013231606608968604632536880671977996826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7185420989990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{7790}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3828661757589184588823627564124763011932373046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{22286}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.132783412933349609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1016969680786115048931605997495353221893310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1232651291611641941603494387891259975731372833251953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.5702666273277341435488096976769156754016876220703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{3175}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.426016630420692654634962082127458415925502777099609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0934508675566103896859004862562869675457477569580078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.26781697331589982002952865514089353382587432861328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.16397167531394007955469760418054647743701934814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{19488}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0782589620494797133520847864929237402975559234619140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0668364590431758942568052361821173690259456634521484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.039899118545415619696559161866389331407845020294189453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{355989818677875779736993187134293258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{217955741343043464370195803532165120}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{19488}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{104024003277237748575267816021688320}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{88840892499321324055003857538690274}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{53035025377707562848735184048619520}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.94955348968505859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.28559200968963427413882527616806328296661376953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24262}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.294156372547149658203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.23278331756591796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.62018049874634850748833514444413594901561737060546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.02649006622516569819936194107867777347564697265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98925177782576600993280635520932264626026153564453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.92826525866985309942691628748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4647}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.89577758312225341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01309169603448295977898840902753363479860126972198486328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.50095299732655484969967574215843342244625091552734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{19176663}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{19176663}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{19176663}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{19176663}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{25.119205298013245197807918884791433811187744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{9132}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{19.110666607326805888078524731099605560302734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.57166203424879646899370300161535851657390594482421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{3175}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.42730762245444886548995100383763201534748077392578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13293}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000000000000000000134151811522021916719243631753249916095268550227280107599826998463031890391656867414697340383511470207622551242820918560028076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000011181575482347337861056731119226272875001609849420949822953073647966407680182923061018343525128970750159851377247832715511322021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.09347157488867095798124040584298199974000453948974609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.5311839580535888671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.551220993332520947660668753087520599365234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{11498}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{157.96203291416168212890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12141}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.7264058589935302734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.23501330142395904232444081571884453296661376953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7846729755401593564556605997495353221893310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{7790}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.392208290415883453761125565506517887115478515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{32382}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.169945240020751953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1646895408630353330181605997495353221893310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{12561}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12489501212734833990314342599958763457834720611572265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.55401045883382205037293033456080593168735504150390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{3175}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.41648975928402898194491399408434517681598663330078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{15043}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0925042169670395042491151116337277926504611968994140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2788141946330757736660643786308355629444122314453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.181840738423213299501668416269239969551563262939453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.100645977336843051030967899350798688828945159912109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{26374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0873758894602358060499369685203419066965579986572265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.039788075055106404687155219335181755013763904571533203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{370607633128508783525674311724889331}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{241707800286336957482866523366227968}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7238}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{133781450739266064187645532053700608}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{26374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{116142478427153703696251130410681022}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{52887423261638892477006969288261632}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.527103424072265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.008277795172684676572316675446927547454833984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.521240711212158203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0976161956787109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6330534395284164173034469058620743453502655029296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.198675496688741848316794857964850962162017822265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{16069}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{16069}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9901648976944930069521433324553072452545166015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9568832218647003173828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6082}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94544708728790283203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{6155}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00943595559002056820385728741484854253940284252166748046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.4885424673247149573995784521684981882572174072265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18920631}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18920631}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18920631}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{18920631}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{27.576158940397352381523887743242084980010986328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{19.15825936254524464175119646824896335601806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.55536608792300834469557457850896753370761871337890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{3175}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.417742956596187209328263634233735501766204833984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24566}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000000000000000000134151811522021916719243631753249916095268550227280107599826998463031890391656867414697340383511470207622551242820918560028076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000011181575482347337861056731119226272875001609849420949822953073647966407680182923061018343525128970750159851377247832715511322021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.092613130156013190319441719111637212336063385009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.19281673431396484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.61438523065174877046956680715084075927734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.336492061614990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.320393085479736328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.37949336607306083379853589576669037342071533203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.694655895233154296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{16284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3879261111581566723316427669487893581390380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{27671}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1395418047904986025287144002504646778106689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.0863430500030517578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1178852090818638675973062390767154283821582794189453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.5634022941375338433545039151795208454132080078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{3175}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.42055775298939257478281206203973852097988128662109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{24566}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.09326658502954150720132275864671100862324237823486328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.276264047449587379912117057756404392421245574951171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.176327738585551452299426955505623482167720794677734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8721}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0926038696538171446359655192281934432685375213623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.082471578719776894583759485612972639501094818115234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.039940230282205800571571074897292419336736202239990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{367217906098843967480472483088092547}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{234379766561359170651825998974156800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8721}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{123091656061871046678406073973473280}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{109623531290907081457361632325778836}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{53089672249204421187055908043096064}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.37592983245849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.71346825953350911930783695424906909465789794921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.6314566135406494140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.5355336666107177734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.542659408581567692664293645066209137439727783203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.139072847682119249412835415569134056568145751953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{11498}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.989667795351798940117760139401070773601531982421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93305823206901561395198996251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.89577758312225341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.012357398736629714164347859650661121122539043426513671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.460919540167028241040014790996792726218700408935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18162421}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18162421}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18162421}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{18162421}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{26.913907284768210814718258916400372982025146484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{19.026276844431237122989841736853122711181640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.5647809044627880581401768722571432590484619140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{3175}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.4218237389404322357222554273903369903564453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24566}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000000000000000000134151811522021916719243631753249916095268550227280107599826998463031890391656867414697340383511470207622551242820918560028076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000011181575482347337861056731119226272875001609849420949822953073647966407680182923061018343525128970750159851377247832715511322021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0933476504865871081761952154920436441898345947265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.0679476261138916015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.636090305467320149546139873564243316650390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.434976279735565185546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.4052622318267822265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12141}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.3121208135058086696744794608093798160552978515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7154560089111328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3884396474092994822058244608342647552490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{29052}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1677591204643267275287144002504646778106689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{10248}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1557641029357927919818394002504646778106689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1128543534681194782098856421725940890610218048095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.34263410079184908330063308312674053013324737548828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.24244193365554356223157128624734468758106231689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{6082}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.058970471332902112127083427139950799755752086639404296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.5378948233983769089405768681899644434452056884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.434951042491411643542420506491907872259616851806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2437373072276634300425968149284017272293567657470703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.2249975719248054895071931014172150753438472747802734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.045596452537640601299084863740063156001269817352294921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{714984858048905813091643576246896279}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{578149102475419028427066142749622272}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{323982452384239387805656719160246272}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{299073071586081744861000137143436807}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{60608081221510076287020223592136704}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{130.0746917724609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.1853700852552009337159688584506511688232421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.2502727508544921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.31154632568359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.0252993165004991027444702922366559505462646484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{40}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.5033112582781456012526177801191806793212890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9946965748900609138871686809579841792583465576171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.972604274749755859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96372705698013316766292746251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005427673581279894056417223424659823649562895298004150390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{4.20166187900720888848127287928946316242218017578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17632117}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17632117}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17632117}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17632117}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{59}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{46.34437086092714963569960673339664936065673828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{11.324851859397394804318537353537976741790771484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.34387826944988530986080377260805107653141021728515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.2431893988977346932056633477259310893714427947998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000000000000000000134151811522021916719243631753249916095268550227280107599826998463031890391656867414697340383511470207622551242820918560028076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000011181575482347337861056731119226272875001609849420949822953073647966407680182923061018343525128970750159851377247832715511322021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.05906964001933390218113117953180335462093353271484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.7512533664703369140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.603657239320256167047773487865924835205078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{23367}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.0148179531097412109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12141}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.34513759613037109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.2765981123044429779156416771002113819122314453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.728162288665771484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3860428349071778342249672277830541133880615234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.175250232219696044921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.12524509429931640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.11517299119462635903499148071205127052962779998779296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.55455658449539513288328862472553737461566925048828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{3175}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.416426576825638605772184064335306175053119659423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.09269542708270379904877955823394586332142353057861328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.278813768050976185097766801845864392817020416259765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1819525907632621730680710925298626534640789031982421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.10095387276777312290931831739726476371288299560546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{26374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0887052227723645059231927234577597118914127349853515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0397749786418421236167120014215470291674137115478515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{370607066103639535681171930077542519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{241856477548123863892205804890095616}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{134190713965832576626642713344737280}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{26374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{117909465481364617486739433270999784}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{52870015142483650385348071660716032}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.6324939727783203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.049719453647437461540903314016759395599365234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.53863298892974853515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0751361846923828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6428017817939328804044407661422155797481536865234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.1920529801324502017223494476638734340667724609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{16069}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{16069}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{32382}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99010919064086000407343135520932264626026153564453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95670853555202484130859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6082}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94563007354736317022769753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{6155}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00942888824444478197694952115170963224954903125762939453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.484395325772443541278988732301513664424419403076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18928950}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18928950}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18928950}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{18928950}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{27.642384105960264406576243345625698566436767578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{19.0972916393509279942009015940129756927490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.55591354992006269952753427787683904170989990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{3175}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.41767799655285642312918525931308977305889129638671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24566}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000000000000000000134151811522021916719243631753249916095268550227280107599826998463031890391656867414697340383511470207622551242820918560028076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000011181575482347337861056731119226272875001609849420949822953073647966407680182923061018343525128970750159851377247832715511322021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0928092780985796672599263956726645119488239288330078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.454002857208251953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.649570761926923978535342030227184295654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.2675457000732421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.4012415409088134765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.2717242105444679367565186112187802791595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7342886924743634580181605997495353221893310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.38620317377002066905333776958286762237548828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{8893}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.18476331233978271484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{10248}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1810758113861083984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{8299}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.116240271863893462889194552190019749104976654052734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.56349334188583621862989048167946748435497283935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{3175}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.42048146220017679208780236876918934285640716552734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{24566}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0933186557591965948343926129382452927529811859130859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2763926656436159756680126520222984254360198974609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.176415663426775670696855513597256503999233245849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8721}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0942857515890292152693774596627918072044849395751953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.082471578721073302009614280905225314199924468994140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.039953339952531287393444614508553058840334415435791015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{367388869003114065017344072934092996}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{234496638721839382314669657844350976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8721}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{125327260615759879947040881679269888}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{109623531292630246434079335659779476}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{53107097990016569021020805869338624}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.43523406982421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.72528035277562441507370749604888260364532470703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22286}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.649292647838592529296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.543451786041260209714209850062616169452667236328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5437849397142382468217647328856401145458221435546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.139072847682119249412835415569134056568145751953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{11498}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.989658142557207298750654445029795169830322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93305823206901561395198996251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.89577758312225341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01235854640675757877554818975340822362340986728668212890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.460919540167028241040014790996792726218700408935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18187378}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18187378}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18187378}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{18187378}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{26.947019867549670379958115518093109130859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{19.045358225214812364356475882232189178466796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.56487217499926012376221251543029211461544036865234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{3175}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.421747669221591348076572103309445083141326904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24566}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000000000000000000134151811522021916719243631753249916095268550227280107599826998463031890391656867414697340383511470207622551242820918560028076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000011181575482347337861056731119226272875001609849420949822953073647966407680182923061018343525128970750159851377247832715511322021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.09340256429702875617948620856623165309429168701171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.774715900421142578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.63999079710600881298887543380260467529296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.449923992156954000165569595992565155029296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.213154315948486328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{4430}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.272553955232611944126119851716794073581695556640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.736017704010009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3891656240880099204559883219189941883087158203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{26278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.188996374607086181640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{11498}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1582534313201904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.118053602430160164971084668650291860103607177734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.34514949263706917736982404676382429897785186767578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.2425740166637542216676592943258583545684814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.058985545732248380323969882965684519149363040924072265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.53674882231710452362705154882860369980335235595703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.434894298022885428256500972565845586359500885009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2436805781101351875417293513237382285296916961669921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.2254430475796551924805299904619459994137287139892578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.04547656818253480170977098850926267914474010467529296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{713461561328478769595803853621716477}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{578073676139247899469626662384041984}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{323907046453044675085551131628142592}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{299665210297948625585674091529313254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{60448727580446808706065265420402688}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{132.0067138671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.2142638654898263439463335089385509490966796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.3510417938232421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.464385986328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.1318176320167747661571411299519240856170654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{40}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.4834437086092719937369110994040966033935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9947941255885244249412835415569134056568145751953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.972544729709625244140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96377390623092640264957253748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005391928194745960502276549419775619753636419773101806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{4.173162925542527545985649339854717254638671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17644404}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17644404}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17644404}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17644404}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{59}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{46.5231788079470192087683244608342647552490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{11.092527427489965674567429232411086559295654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.3466766943842909398654228425584733486175537109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.243324934168552164948096105945296585559844970703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000000000000000000134151811522021916719243631753249916095268550227280107599826998463031890391656867414697340383511470207622551242820918560028076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000011181575482347337861056731119226272875001609849420949822953073647966407680182923061018343525128970750159851377247832715511322021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.059080586855942140989128574801725335419178009033203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.18827056884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.675938361527897768610273487865924835205078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.5404598712921142578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12141}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.9750258922576904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.31679518225192992986194440163671970367431640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.6703853607177716611431605997495353221893310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{19451}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3824675730522102412578533403575420379638671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{16149}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1814471483230608583880894002504646778106689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.161029815673828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.11804194241666350617681047197038424201309680938720703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.342685349436771702347215295958449132740497589111328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.2396104756059726781369789705422590486705303192138671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{22286}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.057875746822369213140380139748231158591806888580322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.53906418480378193169855194355477578938007354736328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.4391535038195806261995812747045420110225677490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{27714}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2474518101303233852394924952022847719490528106689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.22684361175488121364907101451535709202289581298828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0452393546715994243623271131582441739737987518310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{716539205966160580971401308421148540}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{583735131724024553293425382801801216}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{27714}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{328919873632879295613573110857465856}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{301526879409552373208290159977647873}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{60133416740733083073325642975019008}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{133.0085601806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.14101647383330373486387543380260467529296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{20976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.9849071502685546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{74.71254730224609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.3554099191410902136567528941668570041656494140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{40}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.7880794701986761907619438716210424900054931640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99514820323085151354547406299388967454433441162109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{15043}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.976713240146636962890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97338515520095836297542746251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004489098204116887848302841490522041567601263523101806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{4.32704305612719064555449222098104655742645263671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17658834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17658834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17658834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17658834}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{59}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{46.67549668874172397181609994731843471527099609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{11.14417833875676677735100383870303630828857421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.343061498801153830218169105137349106371402740478515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.2403540189861615716804266185135929845273494720458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000000000000000000134151811522021916719243631753249916095268550227280107599826998463031890391656867414697340383511470207622551242820918560028076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000011181575482347337861056731119226272875001609849420949822953073647966407680182923061018343525128970750159851377247832715511322021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.05797266452312255236023474935791455209255218505859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.803619384765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.6123671863252866387483663856983184814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{157.82850170135498046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12141}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.49991607666015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.31038120399073587662996942526660859584808349609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.760346889495849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{7790}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3891154140826085239268650184385478496551513671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1789225935935956357525355997495353221893310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1693651676177978515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1238014342214257823560075166824390180408954620361328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.526814201378995594637899557710625231266021728515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.377527568517044553875194878855836577713489532470703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0944955784895225026076559515786357223987579345703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.385970026901434615229646851730649359524250030517578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.241199889086781749103494121300172992050647735595703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{2743}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1462214242671726338596016603332827799022197723388671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.12683647491298299936346438698819838464260101318359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.042607979653756421212218441496588638983666896820068359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{513042165291244041244930547085511911}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{320609645154367091317724018412355584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{2743}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{194361610719469815076949445799051264}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{168594593341008251924780636532425432}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{56635719399607121528888460759269376}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{25.76837158203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{10.67154272344728127563939779065549373626708984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26829}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.5517799854278564453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.40165996551513671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.83292431082238493900149478577077388763427734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{10}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.8079470198675497982776505523361265659332275390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98611300946860913629876677077845670282840728759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6155}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93884085118770599365234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.920934379100799560546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0133330284557431517911130214315562625415623188018798828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.91864593549909090430816149819293059408664703369140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20127000}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20127000}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20127000}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{20127000}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{1185}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{33.01324503311258240501047112047672271728515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{2773}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{3.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{18.09210678390872573118031141348183155059814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.5273924602024961938440128506044857203960418701171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3786430946270635811146121341153047978878021240234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{27671}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000000000000000000000000000000134151811522021916719243631753249916095268550227280107599826998463031890391656867414697340383511470207622551242820918560028076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000011181575482347337861056731119226272875001609849420949822953073647966407680182923061018343525128970750159851377247832715511322021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.09488134702224161609596109201447688974440097808837890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{174.632483005523681640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{23696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.64567230079347837090608663856983184814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.10062408447265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.1607201099395751953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.314084433880633895341816241852939128875732421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.755488872528076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.384691863659991639678992214612662792205810546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.169621646404266357421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{9816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1559407711029034970806605997495353221893310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1155678027425110221404480626006261445581912994384765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6450770390078550686752123510814271867275238037109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{27671}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.53997600249350108381207746788277290761470794677734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.245418709802925960605790578483720310032367706298828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.14767899238951109897044489116524346172809600830078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.056641658730845777236506677354554994963109493255615234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2371551214871716883880736759238061495125293731689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1393331066833348452771446090991958044469356536865234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.058652570436791999497483374170769820921123027801513671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.04746804428932920039141407642091508023440837860107421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0369844087900517981548631496480084024369716644287109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{315233226824521445044486147198237039}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{185205466143175117145099486416076800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{77962638649330655693271527136952320}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{63095853374534724303627269721096192}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49160711571290577116808185764642816}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19093}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{2.9403973509933774010960405576042830944061279296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{6549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99023498762522310645550760455080308020114898681640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.90373529493808746337890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.895780980587005615234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0149857190901019725337572907619687612168490886688232421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.55471236003634250000260408342001028358936309814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18175126}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18175126}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18175126}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{18175126}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{49}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{1185}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{32.4105960264900687661793199367821216583251953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{2773}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.92064514417472054219615529291331768035888671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6454839114828712087756912296754308044910430908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27671}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.54192397636344313838208108791150152683258056640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{11598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.264779690733523309642549747877637855708599090576171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.1737211804985785423838251517736352980136871337890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.054116236459894336008336068744029034860432147979736328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.471160411834716796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{168.0048671479256654492928646504878997802734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{17096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.841443121433258056640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12141}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.0753543376922607421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.3439614566779010118580117705278098583221435546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.8180291652679443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.424897659693332485630890005268156528472900390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{20976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.16060531139373779296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1239552497863751767681605997495353221893310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1257233098183270225689511789823882281780242919921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.638620254873305537302030643331818282604217529296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5355513916722161038563854162930510938167572021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{12561}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.2461834182456131003835508863630820997059345245361328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.1622806991445445989885598692126222886145114898681640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.054715183921868082439488034651731140911579132080078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2501971426169780077231052928254939615726470947265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.146229061801731619052446831119596026837825775146484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.062352708040987303572677546981140039861202239990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.04746923139674290303968717807947541587054729461669921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037595663267293653875267267494564293883740901947021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{332569046431878478892634842140087912}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{194371762744224356102686771945406464}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{82880965141083580055018365144530944}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{63097431310943011387288743228063744}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49973208134989325467690883369402368}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.94955348968505859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.28559200968963427413882527616806328296661376953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24262}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.294156372547149658203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.23278331756591796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.62018049874634850748833514444413594901561737060546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{19093}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99165583959478420528199649197631515562534332275390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{17194}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93656888604164112432926003748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.895777761936187744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01200684463607642159244104362869620672427117824554443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.50165289707034765864790415434981696307659149169921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{19406487}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{19406487}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{19406487}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{19406487}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{49}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{1185}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{32.96026490066225278496858663856983184814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.81566629790239630892756395041942596435546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.63897527131925879739782203614595346152782440185546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.53750955060420324560510607625474222004413604736328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{12561}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.266010271436325940186407024157233536243438720703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.1908977991478174318640270712421624921262264251708984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.052097017900023905034867510721596772782504558563232421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.1199843883514404296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{23696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.996418056109092731276177801191806793212890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{160.338760077953338623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4430}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.6806437969207763671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.281530257433641128983481394243426620960235595703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.817537784576416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.431340730742903133432264439761638641357421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{6910}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2170121669769304872943394002504646778106689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{11124}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2097022533416765810443394002504646778106689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{8299}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.117495287484988886195225177289103157818317413330078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.62214612568141836046464732135063968598842620849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5239084384979140196492153336293995380401611328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{20751}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.250366751415271371339343886575079523026943206787109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.19497123662798709897714388716849498450756072998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.051033355757061589497158848871549707837402820587158203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.269369814539180574275434310038690455257892608642578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1657847116767728612440890856305486522614955902099609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{22261}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0792623922012884174481683885460370220243930816650390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.05581492166044769998034524860486271791160106658935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.03813674224085772390679949239711277186870574951171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{358053898704869527189458740782547995}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{220365680033896966995262033742528512}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{22261}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{105357790726836641538190459468251136}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{74190756453609085162873417433354841}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{50692425454581262977961024282427392}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.527103424072265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.008277795172684676572316675446927547454833984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.521240711212158203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0976161956787109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6330534395284164173034469058620743453502655029296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.15231788079470209851251638610847294330596923828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99212500867464681331142628550878725945949554443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93458463251590728759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.89577758312225341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0114217962815393626885285272010150947608053684234619140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.48484782033703643921995762866572476923465728759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{19150455}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{19150455}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{19150455}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{19150455}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{34.20529801324503438308965996839106082916259765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{7790}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.421725990706246278705293661914765834808349609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.62249198396686666878707683281390927731990814208984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.5258887732668837688976282151998020708560943603515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{17096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.271388920281277867818658933174447156488895416259765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2293530910675909695317642444933881051838397979736328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.048302133863325991125492464561830274760723114013671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.5611956119537353515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{6204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.533728241131001368557917885482311248779296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27671}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.775477230548858642578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4430}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.513781070709228515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.2923572485531824582949411706067621707916259765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.769047260284423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{20976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.432395679271774469043521094135940074920654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.191036641597747802734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.14935779571533203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.123344679235785903426148024664144031703472137451171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6331830053245479650314564423752017319202423095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.52796460347147855518556980314315296709537506103515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.250871797309209443316291299197473563253879547119140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.1897712644168524087628924235104932449758052825927734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.052524252801943539792350890138550312258303165435791015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.26612011083549480527921105021960102021694183349609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.159707268887657682920888646549428813159465789794921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.074749994634980776453403450432233512401580810546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.050792627939069100173608006798531278036534786224365234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.038065850830117230196858457702546729706227779388427734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{353734301563924519766741484503511685}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{212287372935823946270293711535472640}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{99359785553588748530659657523396608}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{67514983036097816603729528619809897}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{50598194606764311265043234223554560}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.37592983245849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.71346825953350911930783695424906909465789794921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.6314566135406494140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.5355336666107177734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.542659408581567692664293645066209137439727783203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.08609271523178829710332138347439467906951904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.992154698892934394649500973173417150974273681640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93548361957073211669921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.89577758312225341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.011364699476753663265338190058173495344817638397216796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.444843857582693125163331160365487448871135711669921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18392245}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18392245}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18392245}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{18392245}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{33.89403973509934075991623103618621826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.4010790784880526871347683481872081756591796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.63353499914007915805314041790552437305450439453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.5299400952242987461460188569617457687854766845703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{26278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.2717759713385536901597561154630966484546661376953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2232361390457658079089497960012522526085376739501953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0497834754653748989827732884805300273001194000244140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.4295022487640380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{6204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.563938407708491240555304102599620819091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{28090}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.852134883403778076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.591402530670166015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.23863987073625114732067231670953333377838134765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7609775066375714658306605997495353221893310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4377619304404358757665249868296086788177490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{24144}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2067420482635498046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.15950298309326171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12033347727909869673279530388754210434854030609130859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.383880396983892702156282439318601973354816436767578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.309629448292096653982952147998730652034282684326171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.160512873260654165274985416544950567185878753662109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.1028651591272344012484296627008006907999515533447265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.038712377269653118483372367109041078947484493255615234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.52201725373531016050066000389051623642444610595703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.42931692552162148412975284372805617749691009521484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{23241}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.258530246842955335750957601703703403472900390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.211553882701121409581901389174163341522216796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.044757699505690584640404949823278002440929412841796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{693879947947732152256350605195103585}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{570660076467646923846897942768123904}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{23241}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{343645641860841095187572189053321216}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{281203343503328808952529059191571680}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{59493187209892634135362760171585536}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{130.0746917724609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.1853700852552009337159688584506511688232421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.2502727508544921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.31154632568359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.0252993165004991027444702922366559505462646484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{34}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.23841059602649039561583776958286762237548828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9944568667190754052143120134132914245128631591796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4647}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96577753126621246337890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96351522207260120733707253748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{5358}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0064216562304291492646601824390018009580671787261962890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{3.653372948062662661783406292670406401157379150390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17861941}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17861941}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17861941}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17861941}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{57}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{47.35761589403973204071007785387337207794189453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{9.848080709142625011054406058974564075469970703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.38450059110409429141697046361514367163181304931640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.310806349241272539263292173927766270935535430908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{17096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.173355695520946706533749193113180808722972869873046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.12100473186209588505324319385181297548115253448486328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03764612060571932705688169562563416548073291778564453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.3688895702362060546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{6204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.66418899605605474789626896381378173828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{17194}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.761334836483001708984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.7007153034210205078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.248901269118315671136087985360063612461090087890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7539012432098406435443394002504646778106689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.43368849691176336591524886898696422576904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{5615}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2111055254936200498150355997495353221893310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{10248}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1856987476348876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1223712413373401475258361870146472938358783721923828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.62198529667155988409632527691428549587726593017578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.52395486781640132623039107784279622137546539306640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{26278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.249293941474989233508807728867395780980587005615234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.1971198253255793952920527090100222267210483551025390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.05087638148699735740621008517337031662464141845703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.269228174439247014415599323911010287702083587646484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1658933193653226167985081929145962931215763092041015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{22261}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.07931856862349996595273893262856290675699710845947265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.055814921688027797908038252217011176981031894683837890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.03815362348420898996881334142017294652760028839111328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{357865626718712079158491372644002505}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{220510044414074864714241048137695232}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{22261}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{105432461999943283834986876234629120}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{74190756490269226472181632574083673}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{50714864475847414578771962217103360}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.6324939727783203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.049719453647437461540903314016759395599365234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.53863298892974853515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0751361846923828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6428017817939328804044407661422155797481536865234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.145695364238410451918070975807495415210723876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.991948978000918746289471528143621981143951416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93458463251590728759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.89577758312225341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.011490269729544609622617912236819393001496791839599609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.48002967614357938685998306027613580226898193359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{19158774}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{19158774}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{19158774}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{19158774}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{34.35099337748344083820484229363501071929931640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{7790}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.23959623168531862802410614676773548126220703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.62233106555028638862125944797298870980739593505859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.525937073301772084477079260977916419506072998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13654}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.270311605978762081736732625358854420483112335205078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2318805688009652199443877407247782684862613677978515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.048130580309635372093790550707126385532319545745849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{174.96358966827392578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.676220890702012411566101945936679840087890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{28090}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{160.370454490184783935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{160.0183961391448974609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.268609124590249326303137422655709087848663330078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7368352413177472470806605997495353221893310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{20976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4404968646977902579919827985577285289764404296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{8893}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.228706061840057373046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{10248}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2265923023223876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.121740363337918877650878357599140144884586334228515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.63316274202718669794620609536650590598583221435546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.52783094200860858347112980482052080333232879638671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{29052}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.250848839267382717199694752707728184759616851806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.189679432249545587563233084438252262771129608154296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.05242836732210831574008125244290567934513092041015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.266779904690681080037251149406074546277523040771484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.15978136914216889419293465834925882518291473388671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.07487092567448731805779260639610583893954753875732421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.050792627939711197659899966083685285411775112152099609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.03809809122072528586588902044240967370569705963134765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{354611318027684879993545620110803678}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{212385869068614962013432598172270592}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{99520530476860307543001748933181440}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{67514983036951368785568216942414953}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{50641049436555579927173994446323712}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.43523406982421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.72528035277562441507370749604888260364532470703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22286}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.649292647838592529296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.543451786041260209714209850062616169452667236328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5437849397142382468217647328856401145458221435546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.08609271523178829710332138347439467906951904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9921525886516697756434268740122206509113311767578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93548361957073211669921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.89577758312225341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0113652978464166866390261390051819034852087497711181640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.444843857582693125163331160365487448871135711669921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18417202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18417202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18417202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{18417202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{33.90728476821192316492670215666294097900390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.410847241902313697892168420366942882537841796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.63351472457811464078503149721655063331127166748046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.52980653756046314217797998935566283762454986572265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{26278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.27174896480185173341936888391501270234584808349609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2231281128989580919697033323245705105364322662353515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.049689263314637154012043396278386353515088558197021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.1412742137908935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.699816916952073597713024355471134185791015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{28778}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.673130691051483154296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4430}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.6471717357635498046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.312380415943951827983937619137577712535858154296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7937738895416259765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4378267834518130285914594423957169055938720703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{32382}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2082653045654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{10248}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1835525035858154296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1261873680507164252606600030048866756260395050048828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.384942167363931775359020548421540297567844390869140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.3095486089876422486355522778467275202274322509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.16071847592716725916517361838486976921558380126953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.10495928292075719368003916542875231243669986724853515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0383431311619545078794857317916466854512691497802734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.52239012556723773972322533154510892927646636962890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.42925520547828754924779559587477706372737884521484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{15043}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.258240509881676849612830437763477675616741180419921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.2124997205178371928457892181540955789387226104736328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.04475708851051163339462846124661155045032501220703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{694375579625569936976702535068593634}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{570578036458146694574509411585228800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{15043}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{343260515380496155068656021219049472}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{282460577608779602143538645401481772}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{59492375057995464078178225798250496}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{132.0067138671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.2142638654898263439463335089385509490966796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.3510417938232421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.464385986328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.1318176320167747661571411299519240856170654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{34}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.2052980132450326067328205681405961513519287109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99443238342045159328108638874255120754241943359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{30899}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96571986377239227294921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20751}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.964100301265716552734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{5358}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.006371567035698058080461780861014631227590143680572509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{3.59970175511217060915214460692368447780609130859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17874228}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17874228}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17874228}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17874228}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{57}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{47.37086092715231444572054897435009479522705078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{9.858344966776623863324857666157186031341552734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.385564076871925731637702483567409217357635498046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.31073063952572999024681621449417434632778167724609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{17096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1736340244170280489033331150494632311165332794189453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.12346814017518496775505099094516481272876262664794921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.037276416056866053250207215796763193793594837188720703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{174.8466320037841796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{6204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.88215978256124571998952887952327728271484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15043}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.724610149860382080078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.310707569122314453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{4430}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.2629483401350825033659930340945720672607421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.796686649322509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.43115681528255578314201557077467441558837890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{32382}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.18925559520721435546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1342105865478515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1259886800625731051450628683596733026206493377685546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.3865501647468370105542589953984133899211883544921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.306087255502798860629098953722859732806682586669921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.167833859942753627070288757749949581921100616455078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.1042221578258246961201649583017569966614246368408203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.037564386636518558304498327515830169431865215301513671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.52556053978087369227267799942637793719768524169921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.433513181095357469363449354204931296408176422119140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{22261}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.259082875867303830119681151700206100940704345703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.213776672301960513067342617432586848735809326171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.044423333787116180138010435030082589946687221527099609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{698589782956569280477484740439116781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{576237856853725068404091523874947072}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{22261}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{344380211831288491618594156665896960}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{284157937669503757443536657481115724}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{59048738935932767550345878605660160}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{133.0085601806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.14101647383330373486387543380260467529296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{20976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.9849071502685546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{74.71254730224609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.3554099191410902136567528941668570041656494140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{34}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.4966887417218543987473822198808193206787109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9947422103376577506850253485026769340038299560546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{9504}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96520671248435985223323996251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20751}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96349626779556285516292746251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20754}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005820460909834315917088520819788755034096539020538330078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{3.834099654599034234792043207562528550624847412109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17888658}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17888658}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17888658}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17888658}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{57}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{47.5562913907284752212945022620260715484619140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{9.867758564836261570007991394959390163421630859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.386974462426940057913071768780355341732501983642578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.30726259300705882626658649314776994287967681884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1811668125604246337712055492374929599463939666748046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.12260102807213750508719130039025912992656230926513671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03650850292564299104380864946506335400044918060302734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.4952983856201171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{23696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.92661468872171326438547112047672271728515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.376165807247161865234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.3702747821807861328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{4430}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.32481968180953657565623871050775051116943359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.823398113250732421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.429735815288214695328861125744879245758056640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.22622501850128173828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{10248}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2251939773559552548931605997495353221893310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12239892307348586297788273213882348500192165374755859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.57005075606455613002054860771750099956989288330078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.478902588976757581651355621943366713821887969970703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{22401}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.25669339579231731374164837689022533595561981201171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2040642188657633970816362989353365264832973480224609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04861138921446291061290168045161408372223377227783203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.38480729967982851835728297373862005770206451416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.23025759277562685145568366351653821766376495361328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4305}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.136731469339213707048230617147055454552173614501953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18146}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.126110655522691794683254329356714151799678802490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.042999242593692206526601040650348295457661151885986328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{511496635716823962314489481038291389}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{306064838559405804054811715901063168}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4305}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{181747296950489858879998599217807360}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18146}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{167629813887549641407971355875485543}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{57155797053082870139738257602117632}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{25.76837158203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{10.67154272344728127563939779065549373626708984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26829}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.5517799854278564453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.40165996551513671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{17197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.83292431082238493900149478577077388763427734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.77483443708609289757305305101908743381500244140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.988844837179247093672529445029795169830322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9428064525127410888671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{26278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.93456482887268077508480246251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0126961497248431580409100405404387856833636760711669921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.7648934949923660298054528539068996906280517578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20356824}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20356824}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20356824}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{20356824}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{38.64238410596026795928992214612662792205810546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{19451}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{14.998165172928633381843610550276935100555419921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.5706522114234087172945919519406743347644805908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.480779932040794666381344768524286337196826934814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{27671}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.278366259553259165482330672602984122931957244873046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.24004955901499347437066944621619768440723419189453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.046469768227323800247052787426582654006779193878173828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.8557498455047607421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{6204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.499404962489137460579513572156429290771484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{28090}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.448268473148345947265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.8489902019500732421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{4430}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.27279716919885554915481407078914344310760498046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.8020179271697998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4303631940424832436065116780810058116912841796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.202830016613006591796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1450808048248273252056605997495353221893310546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12339509378872891287581836650133482180535793304443359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.331373565941103509491227896432974375784397125244140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.08759340432841557222420902917292551137506961822509765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{7884}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0784298216470071529737850823948974721133708953857421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2347420161102269087205485220692935399711132049560546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1535399922284701179631127843094873242080211639404296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{18289}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.045006896086901927722667693387847975827753543853759765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.03834429560821560334371582712265080772340297698974609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0373668511321369190003593985238694585859775543212890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{312025659600707336458810012696090770}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{204089656142681041417127854801420288}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{18289}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{59824426282092622277178058954768384}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{50968311201092791040386835520743196}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49669064639163662259000951598743552}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{2.947019867549669047690485967905260622501373291015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99972522258758544921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{32382}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98622999443913139661077593700611032545566558837890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7467}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.935963571071624755859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{31308}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.90176701545715320929019753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01309059684472366029417411681379235233180224895477294921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.411556236775876771449844682138063944876194000244140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17680951}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17680951}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17680951}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{17680951}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{6532}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{22.430463576158938820981347816996276378631591796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{15399}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{17.245216222667494321285630576312541961669921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.3317830693331960123515500526991672813892364501953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.08796412803272031510903872231210698373615741729736328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{7884}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000012270707144190838266104828137736011335449004793147594829440125867917062253394467871636531043459672485340661296504549682140350341796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5781}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000000000000000000000000000000106129771627644823297499798642421075056890645338377140834956904915016825402632616883013874620710070839635363881825469434261322021484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07870130090273501355380147970208781771361827850341796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.458876132965087890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.330088162264274842527811415493488311767578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{16197}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.663352549076080322265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.7175886631011962890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.353077755632096312865542131476104259490966796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.66352367401123046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.372545921249894718130235560238361358642578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{17197}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.15212976932525634765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{11124}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1229970455169677734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1210319840013421022195672094312612898647785186767578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.327239883738155101777778099858551286160945892333984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.08706950608927561952032903036524658091366291046142578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{18289}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07798110377155258177150898291074554435908794403076171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2416161261436949037051391542263445444405078887939453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.157545889160384644522849839631817303597927093505859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{2773}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.04759553100874637510120379602085449732840061187744140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.047236690577168498339499791427442687563598155975341796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0375168354642924917197177592242951504886150360107421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{321162919103299027510851276630350656}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{209414406492810694261089614329544704}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{2773}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{63265312291074814747573642602741760}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{62788331543402024408859410129961763}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49868428012393971742570222687617024}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.94955348968505859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.28559200968963427413882527616806328296661376953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24262}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.294156372547149658203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{2345}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.23278331756591796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.62018049874634850748833514444413594901561737060546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{2.97350993377483430180063805892132222652435302734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99957621097564697265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{32382}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9859336065930246473243414584430865943431854248046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{12457}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93482404947280872686832253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{31308}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.901743471622467041015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0130359001260572128499948263424812466837465763092041015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.397792249474998860225838370752171613276004791259765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18912312}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18912312}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18912312}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{18912312}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{6532}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{22.364238410596026795928992214612662792205810546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{15399}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{17.465759669817476407160938833840191364288330078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.327644278826333457121933179223560728132724761962890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0874397815774131392796419959267950616776943206787109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{18289}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000012270707144190838266104828137736011335449004793147594829440125867917062253394467871636531043459672485340661296504549682140350341796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5781}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000000000000000000000000000000106129771627644823297499798642421075056890645338377140834956904915016825402632616883013874620710070839635363881825469434261322021484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07825117572392430165262311447804677300155162811279296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{174.7248241901397705078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.357228451217252995775197632610797882080078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{19538}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.158313155174226949384319595992565155029296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.9035966396331787109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.331028000385728216059533224324695765972137451171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.76007080078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.389138766471912589395287795923650264739990234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{24173}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.18098485469818115234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{11124}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1699788570404034970806605997495353221893310546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12217152584345856991543399772126576863229274749755859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.305465213810932778581985758137307129800319671630859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.08481360883641830827883723031845875084400177001953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{11498}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07601090508255155253625190425736946053802967071533203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.251284710507925723721456279236008413136005401611328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1697624505502237923781905237774481065571308135986328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{11124}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.064338224940061861101270324070355854928493499755859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{5928}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0512661485375612013815072032230091281235218048095703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037228808624474189759023801116200047545135021209716796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{334014672119842872380079528809217393}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{225653001904409823510588613397053440}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{11124}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{85520169789437516797520190204018688}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{5928}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{68144399872194286912932954308120202}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49485574673370018001284679591788544}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.527103424072265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.008277795172684676572316675446927547454833984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11130}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.521240711212158203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0976161956787109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6330534395284164173034469058620743453502655029296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.03311258278145690070459750131703913211822509765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9993202686309814453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{18668}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98414554027532108460007975736516527831554412841796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9120674431324005126953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.90171241760253917352230246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0139572107614414735177188475745424511842429637908935546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.388872006778892720380014225156628526747226715087890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18656280}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18656280}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18656280}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{18656280}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{6532}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.25827814569536400313154445029795169830322265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{15399}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{3.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{13716}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{17.5798890126607290085303247906267642974853515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.30584270029168625359972111255046911537647247314453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.085174796982768030684241011840640567243099212646484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{11498}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000012270707144190838266104828137736011335449004793147594829440125867917062253394467871636531043459672485340661296504549682140350341796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5781}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000000000000000000000000000000106129771627644823297499798642421075056890645338377140834956904915016825402632616883013874620710070839635363881825469434261322021484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07626815956390912976115004084931570105254650115966796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.717409610748291015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.55345333964618248501210473477840423583984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{913}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.37985670566558837890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8048}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.54995441436767578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.438977887698233981694784233695827424526214599609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.644325733184814453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.373702284516088667487565544433891773223876953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{8893}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.141767799854278564453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1276066303253156064556605997495353221893310546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{11124}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12041224765220504000495793661684729158878326416015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.31382728657551062223518556493218056857585906982421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.085221478588222654426687086015590466558933258056640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{18289}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07638594506956940255459898025947040878236293792724609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2482945352236456126870933758254977874457836151123046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.166215866000802681146097938835737295448780059814453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{17197}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.06067105051144637550830651662181480787694454193115234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.04867126668564909774961080302091431804001331329345703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037503210615365600855142247382900677621364593505859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{330040047419673712111728136442129493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{220938782431901198483398769963433984}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{17197}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{80645658873495316179338499683516416}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{64695210268878588822432824214008961}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49850317481761999113506028659933184}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.37592983245849609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.71346825953350911930783695424906909465789794921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17096}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.6314566135406494140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.5355336666107177734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.542659408581567692664293645066209137439727783203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.019867549668874051604916530777700245380401611328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999550521373748779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{32382}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9849759387654184461524664584430865943431854248046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{30899}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.92668189108371734619140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.90173131227493275030582253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01308432839684640740240961775953110191039741039276123046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.38977321773674600269288248455268330872058868408203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17898070}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17898070}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17898070}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{17898070}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{6532}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.397350993377482808455170015804469585418701171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{11124}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{3.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{13716}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{17.461435073815341212366547551937401294708251953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.314215106702378232927941326124710030853748321533203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.08558416344315757096072871945580118335783481597900390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{18289}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000012270707144190838266104828137736011335449004793147594829440125867917062253394467871636531043459672485340661296504549682140350341796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5781}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000000000000000000000000000000106129771627644823297499798642421075056890645338377140834956904915016825402632616883013874620710070839635363881825469434261322021484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07664406739167091420217303721074131317436695098876953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.2237484455108642578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.55581518040588662188383750617504119873046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{913}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.640973865985870361328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.7437565326690673828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.4242594438264717382480739615857601165771484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7342402935028076171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3744761312244744289046138874255120754241943359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{8840}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1605885028839093564556605997495353221893310546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{8721}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1517693996429443359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1251637275451084885258268286634120158851146697998046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.174251371787928210910223469909396953880786895751953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.050872651634771955120317699083898332901298999786376953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{24144}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04478673807903586767675818691714084707200527191162109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.47666837092500691230867460035369731485843658447265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.37954478773196598240247112698853015899658203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{16069}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.14922545213540361341841844478040002286434173583984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{27714}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1273055417836451985724721680526272393763065338134765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5928}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.057491915565871305748846253891315427608788013458251953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{633600943338707769503595018636416482}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{504501557507572689926697103883501568}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{16069}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{198354648662040476495733199357345792}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{27714}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{169218090157387626247982354191872314}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5928}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{76419863701458732483240765067100160}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{130.0746917724609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.1853700852552009337159688584506511688232421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26932}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.2502727508544921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{4729}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.31154632568359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.0252993165004991027444702922366559505462646484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{7.14569536423841089600728082587011158466339111328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99991154670715320929019753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{11130}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99324853214996544625847718634759075939655303955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{17197}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.972377300262451171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{17194}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.972291469573974609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20751}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0063177846596698568337746593215342727489769458770751953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.71242963211496590503202241961844265460968017578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17367766}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17367766}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17367766}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17367766}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{55}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{29022}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{40.30463576158940242066819337196648120880126953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{8721}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6082}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{19538}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{14.3157364335734502702734971535392105579376220703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.17446670739450043097207299069850705564022064208984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.051108623803731705048658540135875227861106395721435546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24144}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000012270707144190838266104828137736011335449004793147594829440125867917062253394467871636531043459672485340661296504549682140350341796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5781}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000000000000000000000000000000106129771627644823297499798642421075056890645338377140834956904915016825402632616883013874620710070839635363881825469434261322021484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0449784881950211212764401125241420231759548187255859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.9370520114898681640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.485009509206605571307591162621974945068359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27714}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.401825010776519775390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8048}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.923879146575927734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.39765581423783924464032679679803550243377685546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7251527309417724609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3808746416837180959191755391657352447509765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{15399}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.155338943004608154296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{8721}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.15379810333251953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{11124}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1197093219313848655449561420027748681604862213134765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.306538430593440713867181557361618615686893463134765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0848442750168894865847590835983282886445522308349609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{1696}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07598990344699667331962444905002485029399394989013671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.25140907933705192167650466217310167849063873291015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1698600331074686387022865119433845393359661102294921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{11124}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.064338224951368483406355380793684162199497222900390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{5928}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.051266148537573198729067058820874080993235111236572265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037179721913796655308193095379465376026928424835205078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{334179986649320420815925348228756545}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{225782711371399920518661720789483520}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{11124}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{85520169804466669490181720611225600}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{5928}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{68144399872210347525740290171014538}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49420327243316472523420231505281024}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.6324939727783203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.049719453647437461540903314016759395599365234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.53863298892974853515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0751361846923828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6428017817939328804044407661422155797481536865234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.03311258278145690070459750131703913211822509765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9993202686309814453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{18668}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98411895028802731655304114610771648585796356201171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.90811257064342498779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.90171241760253917352230246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01412558841781078218524658751675815437920391559600830078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.388872006778892720380014225156628526747226715087890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18664599}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18664599}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18664599}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{18664599}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{6532}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.158940397350992412839332246221601963043212890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{15399}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{3.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{13716}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{17.566559409095130916966809309087693691253662109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.306917243329387912087469203470391221344470977783203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.08520539138986993332736119555192999541759490966796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{11130}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000012270707144190838266104828137736011335449004793147594829440125867917062253394467871636531043459672485340661296504549682140350341796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5781}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000000000000000000000000000000106129771627644823297499798642421075056890645338377140834956904915016825402632616883013874620710070839635363881825469434261322021484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07624662213053369497206546157030970789492130279541015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.3583126068115234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.465281791244905207349802367389202117919921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{28090}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.64897239208221435546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8048}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.568618297576904296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.40306483203007559268371551297605037689208984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7226428985595703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{19451}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3797045575072441891961716464720666408538818359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{8893}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1492807865142822265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{8048}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.13617229461669921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12373771479018157160023605456444784067571163177490234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.31382728657551062223518556493218056857585906982421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.08531415663097542678716678210548707284033298492431640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{18289}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0764776808355969450747835480797220952808856964111328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.248240712362845006300204886429128237068653106689453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1662780637666566863064332437716075219213962554931640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{17197}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0610483383973795812327267640284844674170017242431640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.04867126668564909774961080302091431804001331329345703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037489483638385869002096484337016590870916843414306640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{329968504566284323750533944586829901}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{221021457443549543452092589097877504}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{17197}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{81147160493948202285167294422188032}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{64695210268878588852231069659398785}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49832071199663044464725997710737408}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.43523406982421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.72528035277562441507370749604888260364532470703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22286}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.649292647838592529296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.543451786041260209714209850062616169452667236328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5437849397142382468217647328856401145458221435546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.019867549668874051604916530777700245380401611328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999550521373748779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{32382}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98494118412598863354645573053858242928981781005859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{30899}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.92470443248748768194644753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.90173131227493275030582253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0131464008399509342528421740325939026661217212677001953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.38977321773674600269288248455268330872058868408203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17923027}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17923027}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17923027}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{17923027}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{6532}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.350993377483444390918521094135940074920654296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{15399}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{3.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{13716}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{17.47171742014011641686010989360511302947998046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.314215106702378232927941326124710030853748321533203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0856771259934590856399694303036085329949855804443359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{18289}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000012270707144190838266104828137736011335449004793147594829440125867917062253394467871636531043459672485340661296504549682140350341796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5781}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000000000000000000000000000000106129771627644823297499798642421075056890645338377140834956904915016825402632616883013874620710070839635363881825469434261322021484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07673562050666025979861473160781315527856349945068359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.312352657318115234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.385257176216072139141033403575420379638671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{12561}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.460457503795623779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.535354137420625875165569595992565155029296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.3320959455966061568688019178807735443115234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7441585063934326171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{20751}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.382408694715689279064463335089385509490966796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{22261}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.164636552333831787109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{11124}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.13593959808349609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12273559404338023337555085845451685599982738494873046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.1746735929475209114780653862908366136252880096435546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0508843388230545701222951038289465941488742828369140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0447487705536858404453681714585400186479091644287109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.476519379935753384369689911181922070682048797607421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.37948308412035525183370054946863092482089996337890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1493067659664481794390411550921271555125713348388671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{27714}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1273057827825583021574828990196692757308483123779296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5928}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.057543981882599293253832684058579616248607635498046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{633402900344672345289420146807219280}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{504419539339578593881139930604765184}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{23447}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{198462733282709438259644151460003840}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{27714}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{169218410499889827076362754466160450}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5928}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{76489071707290959506578290834931712}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{132.0067138671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.2142638654898263439463335089385509490966796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.3510417938232421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.464385986328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.1318176320167747661571411299519240856170654296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{7.139072847682118805323625565506517887115478515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99991154670715320929019753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{11130}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.993471358785566138749345554970204830169677734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9723605811595916748046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{17194}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97222459316253662109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20751}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.006163901308945185682219847222995667834766209125518798828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.6599678250266414192282127260114066302776336669921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17380053}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17380053}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17380053}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17380053}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{53}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{6159}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{40.06622516556291202505235560238361358642578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{2773}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6082}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{19538}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{14.49990585681801036344040767289698123931884765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.17488945032473157681351949577219784259796142578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0511214492458758884563252422594814561307430267333984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{32382}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000012270707144190838266104828137736011335449004793147594829440125867917062253394467871636531043459672485340661296504549682140350341796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5781}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000000000000000000000000000000106129771627644823297499798642421075056890645338377140834956904915016825402632616883013874620710070839635363881825469434261322021484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.044944099961668433629302654708226327784359455108642578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.440039157867431640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.30204209902427692213677801191806793212890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24202}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{157.992972433567047119140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.5823056697845458984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.25942150904722183213380048982799053192138671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.72673702239990234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{12457}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.38418969255409507468357332982122898101806640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{11130}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.15778219699859619140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1355659961700439453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12380969353869876459217636011089780367910861968994140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.1739085519153922010371360329372691921889781951904296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.050019643694983580151092183996297535486519336700439453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{8745}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04416176932026273649345426974832662381231784820556640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.478470320726240405662110788398422300815582275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.3832609764634773430458380971685983240604400634765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{23633}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1496869755729342832406558727598167024552822113037109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{27714}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1273060430661470954216696327421232126653194427490234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5928}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0577967541396907924511339160744682885706424713134765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{635996145461506430424800334058741246}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{509441219607117655741589748644315136}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{23633}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{198968118535917133566387813535973376}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{27714}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{169218756476122920705670238398071054}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5928}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{76825063667974750143088067069607936}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{133.0085601806640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.14101647383330373486387543380260467529296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{20976}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.9849071502685546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{74.71254730224609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.3554099191410902136567528941668570041656494140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{15}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{7.3178807947019866020355038926936686038970947265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{19538}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9937251573366834289657845147303305566310882568359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{24566}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.971786201000213623046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20751}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97057992219924915655582253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{27671}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.006033558251804152679220738519916267250664532184600830078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.7990831400273012974366793059743940830230712890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17394483}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17394483}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17394483}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17394483}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{55}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{29022}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{40.68874172185430637682657106779515743255615234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{8745}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6082}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{19538}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{13.835449923138622096985272946767508983612060546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.17412346387350507992408665813854895532131195068359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.050253018629974353925771168860592297278344631195068359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{15662}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000012270707144190838266104828137736011335449004793147594829440125867917062253394467871636531043459672485340661296504549682140350341796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5781}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000000000000000000000000000000106129771627644823297499798642421075056890645338377140834956904915016825402632616883013874620710070839635363881825469434261322021484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0443557588478022124522937019719392992556095123291015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.191251277923583984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.3725103621451353319571353495121002197265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{23367}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.361196875572176168134319595992565155029296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.503928899764986226728069595992565155029296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.357118005247305969618309973157010972499847412109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7072150707244873046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.378762559385489083751963335089385509490966796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{27584}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1430820226669329287005894002504646778106689453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{11124}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.11359882354736328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.11809008018900145342566787576288334093987941741943359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.285140636702655603240685877608484588563442230224609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.07347044286314739769405690594794577918946743011474609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{8745}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000116609039601570920790498664492446771239611623231791082133668169262818992137908936}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07084178869960401636607372211074107326567173004150390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.3380359174247142828306778028490953147411346435546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20415}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.2206921481145855679084633038655738346278667449951171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{26374}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0940975381552764666981403252066229470074176788330078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.09264827987235839390489644529225188307464122772216796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5928}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.042132915689832295402794670735602267086505889892578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{449326805021768388129524815463623128}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20415}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{293350181723818448554255524334403584}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{26374}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{125077082050432824692589600721338368}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{123150687367654959732181347088750244}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5928}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{56004251078970618201171701929082880}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{25.76837158203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{10.67154272344728127563939779065549373626708984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26829}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.5517799854278564453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{742}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.40165996551513671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{17197}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.83292431082238493900149478577077388763427734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.582781456953642251761493753292597830295562744140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98180567941918273078272250131703913211822509765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94560535252094268798828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.93857264518737804070980246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{3284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01310745150420333966778674295028395135886967182159423828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.7127747839509250837863874039612710475921630859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{19862649}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{19862649}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{19862649}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{19862649}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{51}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{28.582781456953643584029123303480446338653564453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{18146}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{3.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{17.505479791398844469085815944708883762359619140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.2854369672353840314826811663806438446044921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{28716}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0737135711941045157491458894583047367632389068603515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8745}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000012270707144190838266104828137736011335449004793147594829440125867917062253394467871636531043459672485340661296504549682140350341796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5781}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000000000000000000000000000000106129771627644823297499798642421075056890645338377140834956904915016825402632616883013874620710070839635363881825469434261322021484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{29725}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07102646954252063438151054697300423868000507354736328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.91046142578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.578162790134257420504582114517688751220703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{26829}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.208498656749753763506305404007434844970703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.3249394893646240234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.482377188460258121693868815782479941844940185546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.6845717430114763857318394002504646778106689453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{20754}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3822285923736767898617472383193671703338623046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{27714}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.140903174877166748046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1350657939910888671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1220588850298036376340604647339205257594585418701171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.4721245189881038140100599775905720889568328857421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{24202}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.304571477867521422933094754625926725566387176513671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.05956181837274261703374378384978626854717731475830078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.038688731045698199206839262842549942433834075927734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.078266829313634433962221237379708327353000640869140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2486963800703805016478753486808273009955883026123046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1563550269413401527796025902716792188584804534912109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{28778}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.041655292777564023598557696459465660154819488525390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0178683354692423003451384744266761117614805698394775390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.03665918464147195632296671874428284354507923126220703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{330574190839915630717860213915206809}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{207831479092134059453296956672049152}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{28778}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{55369381332555327010352920795283456}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{23751091743793469154267915079323211}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{48728414528092938264707421872062464}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999999940395355224609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{25516}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99006489096887850820394305628724396228790283203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{3284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93692004680633556024105246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{18668}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.894783079624176025390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0117084398287413578298998828586263698525726795196533203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.3817006212182665336740683414973318576812744140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17910775}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17910775}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17910775}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{17910775}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{49}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{32.77483443708609200939463335089385509490966796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{25516}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.38937314618551255307465908117592334747314453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.473355814074218284037698367683333344757556915283203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24202}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.30573277879632809739263166193268261849880218505859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8840}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.06837039025720093032845170455402694642543792724609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.038732223894034280287090865613208734430372714996337890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07804605386186182214292017533807666040956974029541015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.6645886898040771484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.854131496505232234994764439761638641357421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7467}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.676373422145843505859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{17197}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.3374936580657958984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.382290259082959327230355484061874449253082275390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.779011249542236328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{16284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4196498599273486007632527616806328296661376953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{17197}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.188224852085113525390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{11124}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1711761951446515439556605997495353221893310546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1234438042125237944279803059544065035879611968994140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.47147379769011699135461412879521958529949188232421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{24202}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.3027400874933470209526831240509636700153350830078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{4647}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.06908001207977844393415267632008180953562259674072265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.03283241986737429896070494805826456286013126373291015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07799345215813703602325546171414316631853580474853515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.253903051267039991945040355858509428799152374267578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1618902081986625385301437063390039838850498199462890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{14095}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.04354243166483580396164398962355335243046283721923828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.023836905016012800706537433370613143779337406158447265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.036771221263207032325937007044558413326740264892578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{337495043959362320426199472995857804}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{215188996981110998748353582082293760}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{14095}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{57877819173451464143172503452254208}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{31684681480150205204233206518668510}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{48877336742256366084054613057601536}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.94955348968505859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.28559200968963427413882527616806328296661376953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24262}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.294156372547149658203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{2345}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.23278331756591796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.62018049874634850748833514444413594901561737060546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.006622516556291202505235560238361358642578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999999940395355224609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{25516}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.989138631631206965977298750658519566059112548828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{8893}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93388557434082042352230246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{18668}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.89472424983978271484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01207200924136843378509098556605749763548374176025390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.372865914179052959642746145618730224668979644775390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{19142136}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{19142136}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{19142136}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{19142136}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{49}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{33.13245033112583115553206880576908588409423828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{25516}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.23530430624591502919429331086575984954833984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.472703395702886608464865503265173174440860748291015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24202}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.303913525445048626760780052791233174502849578857421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0798235871366552995898047129230690188705921173095703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.032869329205551134354124087622039951384067535400390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07774798909663808987868804933896171860396862030029296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{178.8347589969635009765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.9391949508363950371858663856983184814453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.5526950359344482421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.0142390727996826171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.4319650816160720552261409466154873371124267578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.793557643890380859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{16284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4202199692757719873270616517402231693267822265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{5781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.216085493564605712890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{10248}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1864504814147966982318394002504646778106689453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.11934767395933933153973072194276028312742710113525390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.444906871167569273328723511440330184996128082275390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{3175}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.298239541300535038192975889614899642765522003173828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{29110}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.069801963263366129108788982193800620734691619873046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0204919731341977016947364376164841814897954463958740234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0751137886293118395286683153244666755199432373046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.26171914650467498208996630637557245790958404541015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.178162902498262720740740405744872987270355224609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{2773}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.051661749896105425838843672181610600091516971588134765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.048746528893138900417891790084468084387481212615966796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.03712956698366294550073263280864921398460865020751953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{347884416566947886545471124558604986}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{236819117810989248087423477694332928}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{2773}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{68670244273141865575431379504594944}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{64795250902098603347106332187429052}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49353659906056072059883247091318784}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.527103424072265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.008277795172684676572316675446927547454833984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11130}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.521240711212158203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0976161956787109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6330534395284164173034469058620743453502655029296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.145695364238410451918070975807495415210723876953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99991303682327281610042746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98865372574092535984391361125744879245758056640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19004}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94523152709007274285823996251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{7310}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.894651591777801513671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01096245891101644588661034873666721978224813938140869140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.436684543624756005275600045933970250189304351806640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18886104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18886104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18886104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{18886104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{49}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{34.63576158940397675678468658588826656341552734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{5781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.7881183607681379044151981361210346221923828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.445995530572669995894585781570640392601490020751953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{3175}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.29941642657534039972944128749077208340167999267578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29110}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.08121341981985112645769930850292439572513103485107421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.02051500966849446883077945358309079892933368682861328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0748738691088018659680614064200199209153652191162109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.8602793216705322265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.88196810191828944880398921668529510498046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{20415}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.631670773029327392578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{17197}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.83950519561767578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.475813478337702822074106734362430870532989501953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7305622100830078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{20976}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.419691118972981058732329984195530414581298828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.19608783721923828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{8721}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.169790744781494140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12347715077601366384651981888964655809104442596435546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.45205690185749869414166823844425380229949951171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{3175}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.3002149053765263975179777844459749758243560791015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{27584}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0681510968795022986643772355819237418472766876220703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0240967261681374993187443322995022754184901714324951171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.076063150557599101819761244769324548542499542236328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2604378596686223179546004757867194712162017822265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.17313813217560192203592350779217667877674102783203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{22545}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.049395051091427048806092869881467777304351329803466796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.04497160004438739699939020511010312475264072418212890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037127257893165975521920785240581608377397060394287109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{346181294233836048222719393524244489}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{230140052425719272682480523097931776}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{22545}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{65657284763951134311333726292803584}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{59777509794242024055690251642554405}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49350590598322689436216902534823936}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.37592983245849609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.71346825953350911930783695424906909465789794921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17096}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.6314566135406494140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.5355336666107177734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.542659408581567692664293645066209137439727783203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.125827814569536400313154445029795169830322265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99992692470550537109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98949708488603305145403510323376394808292388916015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19004}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94614583253860484735042746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{7310}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.89465510845184326171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01081521634049953557721313046613431652076542377471923828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.435276204639867103640682444165577180683612823486328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18127894}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18127894}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18127894}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{18127894}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{34.18543046357616077557395328767597675323486328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{5781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.08973346043824648177178460173308849334716796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.45316305694239622514629672878072597086429595947265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{3175}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3013902936704895285657812564750202000141143798828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29565}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0791135290109104827305230855927220545709133148193359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.024123815070469005472642010090567055158317089080810546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07582042825563418964041062508840695954859256744384765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.247266292572021484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.75612680801492615501047112047672271728515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.790357768535614013671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{17197}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.1484248638153076171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.399171512715621457090264811995439231395721435546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7407944202423095703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.420684991293395427192081115208566188812255859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{19917}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1739504337310791015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{8721}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1435012817382794736431605997495353221893310546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1198078386783817672611718307962291873991489410400390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.278524622756606887730157495752791874110698699951171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.179121570973345967114909171868930570781230926513671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{30371}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.06105474627318364932992977855974459089338779449462890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{2773}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.02490164385970609906006956180135603062808513641357421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0397057122394408879006988399851252324879169464111328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.50871451769217512772769396178773604333400726318359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.41735801159428842499465872606378979980945587158203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.23130686032595748624629550249665044248104095458984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.197218488835183392016148218317539431154727935791015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0434017947851752794452551142967422492802143096923828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{676197578778660058842032161826386845}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{554763953276253537017333641346285568}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{307459554362373942079791344966959104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{262148336646120672123635660497950675}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{57690880695766759283350960389226496}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{130.0746917724609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.1853700852552009337159688584506511688232421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26932}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.2502727508544921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{4729}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.31154632568359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.0252993165004991027444702922366559505462646484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{15}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29022}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.0264900662251648100209422409534454345703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999893486499786376953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12561}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99356586569981863998890503353322856128215789794921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{12493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97194145619869243279964621251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{13716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.971351146697998046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.006021602942317345712186504869123382377438247203826904296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.844795865759992548049694960354827344417572021484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17597590}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17597590}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17597590}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17597590}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{63}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{47.0264900662251648100209422409534454345703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{7.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{13716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{9.18027472201979577448582858778536319732666015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.27867945784197567515860782805248163640499114990234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.179901699687508465075325148063711822032928466796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{30371}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.061091752958300250819778653976754867471754550933837890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2773}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0249296376292207945424284076807452947832643985748291015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.039679650916818076655800950902630575001239776611328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.69886302947998046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.798728068143333302941755391657352447509765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{19093}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.37387120723724365234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.969229221343994140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.36509204030076869429422004031948745250701904296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7446186542511004091693394002504646778106689453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.42251925752652397250130889005959033966064453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{30684}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.18196976184844970703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{11124}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1765964031219482421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.124421938217603667009569790025125257670879364013671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.4450087931630017923367859111749567091464996337890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{3175}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.2981416328795798431627872560056857764720916748046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{27714}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0710369430400862034158393498728401027619838714599609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0207083569603109009238384174977909424342215061187744140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07524416164463194889311381530205835588276386260986328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.261711835645901780278421711045666597783565521240234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.17826539268656282910541222008760087192058563232421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{2773}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.05166174973634012068668397432702477090060710906982421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.04874652825407770062593471038780990056693553924560546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037182534153137554444601420300386962480843067169189453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{347874698768793316570299415536474090}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{236955350638570835295451840321159168}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{2773}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{68670244060777349212060650452287488}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{64795250052640525159057765685941360}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49424065350579215705186466449588224}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.6324939727783203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.049719453647437461540903314016759395599365234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.53863298892974853515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0751361846923828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6428017817939328804044407661422155797481536865234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.15231788079470209851251638610847294330596923828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99991303682327281610042746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98868961642120056776406045173644088208675384521484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19004}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94523152709007274285823996251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{7310}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.894651591777801513671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01097184233377733637848638892364760977216064929962158203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.44197546260830689046628094729385338723659515380859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18894423}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18894423}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18894423}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{18894423}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{49}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{34.64900662251655916179515770636498928070068359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{5781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.7976436651425036217233355273492634296417236328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.44609770196487763538328863432980142533779144287109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{3175}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.299320074390391266394573221987229771912097930908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29110}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0813944607017897947542905967566184699535369873046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{20976}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0207316367475828162991735581499597174115478992462158203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07500457273954370951418724189352360554039478302001953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.9772493839263916015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.814602918182771418287302367389202117919921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{8840}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.5290992259979248046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.013798236846923828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.450433580659912013999246482853777706623077392578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7265493869781494140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4218619580300444482645616517402231693267822265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{1283}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1824629306793212890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{11124}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1060764789581298828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1203776244047480847854103558347560465335845947265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.452056903573218094027907909548957832157611846923828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{3175}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.300241922195132515671645023758173920214176177978515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{27584}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0678659184122320235932335208417498506605625152587890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0240967261681124013394938998544603236950933933258056640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07608828748579521406014691820018924772739410400390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.260466437299497588497843025834299623966217041015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1732419352407545687366763331738184206187725067138671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{22545}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.049395032942331322522999670354693080298602581024169921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.04497160004438739699939020511010312475264072418212890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037125948263279050232110733986701234243810176849365234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{346219280420848601658253517624107348}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{230278030365968308725007356935536640}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{22545}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{65657260639665015202219709586997248}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{59777509794242024055690251642554405}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49348849801612890153986091007344640}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.43523406982421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.72528035277562441507370749604888260364532470703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.649292647838592529296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.543451786041260209714209850062616169452667236328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5437849397142382468217647328856401145458221435546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.125827814569536400313154445029795169830322265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99992692470550537109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98948377291887801288083892359281890094280242919921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19004}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94614584743976604119808371251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{7310}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.894655168056488037109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01081734546550935753550515272536358679644763469696044921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.435276204639867103640682444165577180683612823486328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18152851}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18152851}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18152851}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{18152851}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{34.18543046357616077557395328767597675323486328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{5781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.08973346043824648177178460173308849334716796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.4531630586623138778890051980852149426937103271484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{3175}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.301418009020292643196370363511960022151470184326171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{27584}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.07877806125625423649960765715150046162307262420654296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.02412381507044387973781596201661159284412860870361328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0758491454882685711691436836190405301749706268310546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.0394761562347412109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.784995123250581627871724776923656463623046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7467}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.40620052814483642578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.72113895416259765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.45619058412415736114553510560654103755950927734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7648546695709246279193394002504646778106689453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4265765512226433742171138874255120754241943359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{18668}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1989947557449323056744105997495353221893310546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{8745}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1938302516937255859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1222509008466692304040179806179367005825042724609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.2825913141605844725035012743319384753704071044921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.17912670296207455766790417328593321144580841064453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{13654}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.061535072692892524293117872957736835815012454986572265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0238617574878161008145038834982187836430966854095458984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.039969743992649402197780972301188739947974681854248046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.50902839064481042452570136447320692241191864013671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.4171742168876282352840689782169647514820098876953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.23091241633076864392393190428265370428562164306640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.19722304626185849230068924953229725360870361328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.043398363642836168541094821193837560713291168212890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{676614787494422539428075501544181900}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{554519648206684031667298697933225984}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4810}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{306935248361199755987445815246323712}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{262154394505246005225764152017724037}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{57686319925312080904675139528949760}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{132.0067138671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.2142638654898263439463335089385509490966796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29725}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.3510417938232421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.464385986328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.1318176320167747661571411299519240856170654296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{15}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{29022}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.019867549668873607515706680715084075927734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999893486499786376953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12561}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9934271952963822371884816675446927547454833984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97205756604671478271484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{27714}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97135388851165760382144753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00626158260055324593362779950211916002444922924041748046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.8466730373729454139919425870175473392009735107421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17609877}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17609877}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17609877}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17609877}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{63}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{47.13907284768212235803730436600744724273681640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{11130}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{7.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{13716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{9.1868317327620605539095777203328907489776611328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.282748409967122082964152696149540133774280548095703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.179907228938107455196160344712552614510059356689453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.062171406588877299592699188224287354387342929840087890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2773}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0238885822445708273509268337875255383551120758056640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.039947912066005286657599526733974926173686981201171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.0198421478271484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.844655250081956410213024355471134185791015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{12552}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.63183748722076416015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{17197}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.912261962890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.4887312923221287519481847994029521942138671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7195603847503662109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.42445425481985665783213335089385509490966796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{19538}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2037438154220563291119105997495353221893310546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.200155735015869140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{10248}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12068510282831472479880829951071063987910747528076171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.278796425262827274327293025635299272835254669189453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{24202}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.176744552048633207785854892790666781365871429443359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{12561}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0621321269511386498063387762158527038991451263427734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.023972413291513901267837383102232706733047962188720703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03899926952364897447811387110050418414175510406494140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.51102902901206170849235377318109385669231414794921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.421105099511684011215351119972183369100093841552734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8745}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2321236644792637193734918810150702483952045440673828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1989405195766822120884143032526480965316295623779296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.04340042299012626669796333089834661222994327545166015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{679274092021614382013061870951284366}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12493}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{559744687438723146494844084655489024}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8745}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{308545273310022055292417279013158912}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{264437308117323182799050880993423736}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{57689057267383113952086446791720960}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{133.0085601806640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.14101647383330373486387543380260467529296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{20976}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.9849071502685546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{74.71254730224609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.3554099191410902136567528941668570041656494140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{7310}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.1986754966887414042275850079022347927093505859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99978840351104736328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12561}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99355339175028511977671996646677143871784210205078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{11498}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97030900418758403436214621251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96820181608200084344417746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{18289}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.006264783530053754691258038889145609573461115360260009765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.9429610349771102573157577353413216769695281982421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17624307}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17624307}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17624307}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17624307}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{63}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{47.23178807947019919311060220934450626373291015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{7.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{13716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{9.1132998716774462621970087639056146144866943359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.279523522997950524260346583105274476110935211181640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24202}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1775201552145289907169711796086630783975124359130859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.06276753599739294531278943622965016402304172515869140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2773}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.023999362444596904209159760057445964775979518890380859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.038992980727267055607310197729020728729665279388427734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.928661346435546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.84672831541655568798887543380260467529296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27300}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.61326313018798828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{17197}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.0508747100830078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.361770707855291195897962097660638391971588134765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7767784595489501953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{16284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4241799676655144679671138874255120754241943359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{26374}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2173091173171979306744105997495353221893310546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.207682132720947265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{8721}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1175445188383299199852416450085001997649669647216796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.402682654303863907241378683465882204473018646240234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.270652860808612782950177688690018840134143829345703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{23241}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1201181655100109768596894355141557753086090087890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{12457}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.07183956845230819732162075297310366295278072357177734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06211622710491583598813036815045052208006381988525390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.36452386973323147589809423152473755180835723876953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20415}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.2367558606491997064136256767596933059394359588623046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{1951}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.137451946040994477105101623237715102732181549072265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18146}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0972597213599593057864467482431791722774505615234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.040334570201222726126832895943152834661304950714111328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{484535332781265059238307756630093859}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20415}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{314702518141068520243842843659993088}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{1951}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{182704974752807527711069949371875328}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18146}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{129280344493898198923656137480804398}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{53613839909417275175696826839859200}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{25.76837158203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{10.67154272344728127563939779065549373626708984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26829}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.5517799854278564453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{742}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.40165996551513671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{17197}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.83292431082238493900149478577077388763427734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.741721854304635552779245699639432132244110107421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98620329392666850054638416622765362262725830078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{21598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94921083748340606689453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{5928}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94511264562606800421207253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11130}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0120714144375387577579061826327233575284481048583984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.73208019101644927761896042284206487238407135009765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20092473}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20092473}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20092473}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{20092473}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{36.62913907284768555427945102564990520477294921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{29726}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{3.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{15622}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.8747648025710947905508874100632965564727783203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.40312465984834677801273983277496881783008575439453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.271925350332207660386529823881573975086212158203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{30899}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1204619673171003768619158336150576360523700714111328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12457}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.07192032859539831957107480775448493659496307373046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.062195172483820206077442804826205247081816196441650390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.7743294239044189453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.84169802286766071119927801191806793212890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{14095}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.85933589935302734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.6985437870025634765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.4495923550062723705877942848019301891326904296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7304971218109113095806605997495353221893310546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{16284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.41934008314120063687369110994040966033935546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{27584}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2171767354011517880962855997495353221893310546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{11124}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2160532474517822265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.11939665395843246376017532384139485657215118408203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.62270381067795899099337475490756332874298095703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.48613010165508774296228011735365726053714752197265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{12141}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.2400561388844605070769233634564443491399288177490234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.157332829631258608316102254320867359638214111328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.060039334762349995389119072797257103957235813140869140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.27199295133178857941658179697697050869464874267578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1426303485122613068369901156984269618988037109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0459049443661842249131410653717466630041599273681640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0194035467813012986459941799921580241061747074127197265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.03932301215146495609875643140185275115072727203369140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{361540645566377509836848457492673844}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{189588252291057191201576113087184896}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{61018137196481214793428107054284800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{25791737599227993675588937989004610}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{52269248630317647092615124558544896}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{2.953642384105960250195721528143621981143951416015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{913}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{913}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99991881847381602899105246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99270185137426614208067121580825187265872955322265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96431572735309600830078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8299}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94135802984237682000667746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00857857819312275900192066302452076342888176441192626953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.53161939709640992912653700841474346816539764404296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17937047}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17937047}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17937047}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{17937047}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{49}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{34.5695364238410576263049733825027942657470703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{3.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{13716}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.240130954751602843089131056331098079681396484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.623049978986999430929927257238887250423431396484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.48807492245517780649066708065220154821872711181640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.2471153525641084092168142660739249549806118011474609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.1850774064237537264165922579195466823875904083251953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.05879263286149279121861610519772511906921863555908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{173.9022033214569091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.2923156062498719620634801685810089111328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{6159}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.7067306041717529296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.920951366424560546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.058346152653625527051417520851828157901763916015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.6634700298309326171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{20754}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3848964599584103751794827985577285289764404296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{13716}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1298149228096026064349644002504646778106689453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.09371185302734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12293776381100574024429761266219429671764373779296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.62601902872978809622139806378982029855251312255859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.48145094547690414632512556636356748640537261962890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.233590746264712156854415070483810268342494964599609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.126860400374645798660111495337332598865032196044921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.061236072826122082968236526312466594390571117401123046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.277196216846553877832803891578805632889270782470703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1497494686171503552873929265842889435589313507080078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.05494215464364547718556508471010602079331874847412109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0250130784642812985241189238649894832633435726165771484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.040285667460466224876203256144435727037489414215087890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{368456971758105744654572774052511778}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{199051186039831071822663370542153728}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{73030650101077878635240235296882688}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{33248084155487517123035947244736381}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{53548837017333130921031157336244224}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.94955348968505859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.28559200968963427413882527616806328296661376953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24262}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.294156372547149658203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.23278331756591796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.62018049874634850748833514444413594901561737060546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.02649006622516569819936194107867777347564697265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{913}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{913}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13716}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.993392389341695380977625973173417150974273681640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96811603009700786248714621251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24566}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96683228015899658203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.007438966895004344055675193914112242055125534534454345703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.5009529973265547386773732796427793800830841064453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{19168408}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{19168408}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{19168408}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{19168408}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{49}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{34.84105960264900403444698895327746868133544921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{3.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{13716}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.539777080927652974651209660805761814117431640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6263670400071987831580599959124810993671417236328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.48333205206379081797507524242973886430263519287109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{19451}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.23930726518380696088428294387995265424251556396484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.1492313710637902246514130411014775745570659637451171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.060078524901447070971638453329433104954659938812255859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{174.0403287410736083984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.293602318163749487212044186890125274658203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.323090374469757080078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.9418785572052001953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.157730074020864918793449760414659976959228515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.728428363800048828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.398613817644434931253272225148975849151611328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.160625874996185302734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{9816}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1563456058502197265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.11882905037655790148054535393384867347776889801025390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.59778776323339510856413880901527591049671173095703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.469785782126846240824846745454124175012111663818359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.2212827549413714789405815963618806563317775726318359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.1074141636675788047394775048815063200891017913818359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0615406280358803126073752309821429662406444549560546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2898577819123582255400606300099752843379974365234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.16921593600601936291383253774256445467472076416015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{30684}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.06287887216238106924404149822294129990041255950927734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.04157767230364829702526918708826997317373752593994140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.041841438125727471730730400167885818518698215484619140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{385287078514025163083787064444443806}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{224926559472149736710018572492996608}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{30684}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{83580357221617801714731972382687232}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{55266206025580540863347775469591147}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{55616810940619303318435997853679616}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.527103424072265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.008277795172684676572316675446927547454833984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11130}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.521240711212158203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0976161956787109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6330534395284164173034469058620743453502655029296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.139072847682119249412835415569134056568145751953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13716}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99324933858896724547804524263483472168445587158203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96253417432308208123714621251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94471979141235362664730246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.007648573143054689278674818098124887910671532154083251953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.48881171092042208226047250718693248927593231201171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18912376}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18912376}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18912376}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{18912376}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{36.4834437086092719937369110994040966033935546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{14.887149133830963165792127256281673908233642578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.59925051266001172489694681644323281943798065185546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.471579023479888725933761861597304232418537139892578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.226137405252308132386218630927032791078090667724609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.1263559224820702819869211452896706759929656982421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06047141089477721387357433968645636923611164093017578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.58569812774658203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.407119912027525288067408837378025054931640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{30684}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.193850815296173095703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.123701095581026265790569595992565155029296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.250518659980684343935308788786642253398895263671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7828779220581036923931605997495353221893310546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{20976}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.398175929555829810624345554970204830169677734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.133583962917327880859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.110797882080078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.127445219306024981609226642831345088779926300048828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6110330801217533913671786649501882493495941162109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.4738269612419203635766962179332040250301361083984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.22602689876444437278024679471855051815509796142578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.11318946961015689811613782467247801832854747772216796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.061593077953402193547294274367231992073357105255126953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.28265099510117208669868205106467939913272857666015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1632513863080035376729171048282296396791934967041015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.061265538208132873376765559214618406258523464202880859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0351667256257661986484919225404155440628528594970703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.04162249290660514910999978610561811365187168121337890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{375707615724943056252101457619800433}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{216998313031296636114069929368485888}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{81435868563080645373745121642676224}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{46744596221855241737476146234675208}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{55325782825818639960381548264423424}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.37592983245849609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.71346825953350911930783695424906909465789794921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17096}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.6314566135406494140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.5355336666107177734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.542659408581567692664293645066209137439727783203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.125827814569536400313154445029795169830322265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999999940395355224609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13716}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99338740307763717662936642227577976882457733154296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96079768240451823846370871251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29052}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94999307394027721063167746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.007546007668257580756898672547094975016079843044281005859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.50565852102837283155167824588716030120849609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18154166}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18154166}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18154166}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{18154166}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{35.9205298013245055699371732771396636962890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.1677259222694740259385071112774312496185302734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.61137276053559774791068548438488505780696868896484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.475644987501568416998765087555511854588985443115234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29052}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.2311381816051969184666603496225434355437755584716796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.1331496644344725976960575053453794680535793304443359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06046121256467651416954822707339189946651458740234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.454014301300048828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.36857232984328902603010646998882293701171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.200369656085968017578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.1613814830780029296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.171701562965687504203060598229058086872100830078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7154238224029541015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.388837969066290867203861125744879245758056640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.120590686798095703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.113177776336669921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1214884436148562230073366663418710231781005859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.365876613452575216722806317193317227065563201904296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.27698901881101190003420242646825499832630157470703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1267472437132124707392932805305463261902332305908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.10222529026818079345151346615239162929356098175048828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.042194733890469550419144439956653513945639133453369140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.52378258949379574715976559673435986042022705078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.4300187623952453908060533649404533207416534423828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2656643736472419359273544614552520215511322021484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.22061115168241840489571359285037033259868621826171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.04521296195213919677513558781356550753116607666015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{696226481659871498033805212500260631}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{571592977688541980604600586227154944}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{353128522934578419513403897555189760}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{293242518998623167898960486407717834}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{60098334799141651210925934228013056}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{130.0746917724609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.1853700852552009337159688584506511688232421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.2502727508544921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.31154632568359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.0252993165004991027444702922366559505462646484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{35}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{9134}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.403973509933774010960405576042830944061279296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99950522184371959344417746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{16197}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.994357934061265158476317083113826811313629150390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{30899}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9640548527240753173828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.964023649692535400390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{13716}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0068118821218231644099017074722723918966948986053466796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{3.9217154104916485124476821511052548885345458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17623862}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17623862}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17623862}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17623862}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{58}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{48.64900662251655916179515770636498928070068359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.2442703328620527969405884505249559879302978515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.366278218761406371140054716306622140109539031982421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.278174501909150218015298605678253807127475738525390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1313159710699040860770736571794259361922740936279296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.12025202647211134798777010246340068988502025604248046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.042022301900359847193211493276976398192346096038818359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{173.6398675441741943359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.28171000101707477369927801191806793212890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.679586887359619140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.4077732563018798828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.06727047662991925136566351284272968769073486328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.732634067535400390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3940327072775122729808572330512106418609619140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{28090}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.183974564075469970703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1657192707061767578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{8721}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1219880594721303446181792651259456761181354522705078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.59725016132688235614978111698292195796966552734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.469687971750115451641249819658696651458740234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{22286}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.221670746966945497735679282413912005722522735595703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.10848689343180910327202326470796833746135234832763671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06150334120230517565008909741663956083357334136962890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.29008121312270140901290460533346049487590789794921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1693058537445582822922318655400886200368404388427734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0629340734094258336117633234607637859880924224853515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.041798476980794800617058371017265017144381999969482421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.041910405860549303225237594006102881394326686859130859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{385584069533945469722180390074544238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{225046080647533336605069769487417344}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{83653732264591941865495816784838656}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{55559705784043909755064157016225608}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{55708484784550324277771414225813504}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.6324939727783203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.049719453647437461540903314016759395599365234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.53863298892974853515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0751361846923828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6428017817939328804044407661422155797481536865234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.139072847682119249412835415569134056568145751953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13716}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.993244130090372490116124026826582849025726318359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96246944367885600701839621251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94446086883544921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.007673556693411080938116430871787088108249008655548095703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.48881171092042208226047250718693248927593231201171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18920695}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18920695}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18920695}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{18920695}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{36.5033112582781456012526177801191806793212890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{24144}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{14.9200403796239218223718125955201685428619384765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.5987115952751154157596147342701442539691925048828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.471481216990908447161956473792088218033313751220703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.226572762890375478672666531565482728183269500732421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.127617820860321196096975882028345949947834014892578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.060423428979818172290805478041875176131725311279296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{173.7498149871826171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.374351791988146942458115518093109130859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.168059170246124267578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.358112335205078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.122135087277866372090784352621994912624359130859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7514693737030047060443394002504646778106689453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3987593966604077166948627564124763011932373046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.173021018505096435546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{8721}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.159368038177490234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1233681076703857237841788219157024286687374114990234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6111475338155305525589255921659059822559356689453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.473735609584867212173975303812767378985881805419921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.2262777538414598443861081022987491451203823089599609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.11423716442727820108427039258458535186946392059326171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0615696617228202736082920409899088554084300994873046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.282653219334046801325399655979708768427371978759765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1633651586856444681838951282770722173154354095458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.061432179007997245179240053403191268444061279296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.03583139589274229874771293680169037543237209320068359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.04161823211890781915034409621512168087065219879150390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{375710572237549368974290133220531969}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{217149542460804011645708092938649600}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{81657372179500414925801982726766592}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{47628094548685766123146660343095924}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{55320119267527253031360277153579008}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.43523406982421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.72528035277562441507370749604888260364532470703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22286}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.649292647838592529296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.543451786041260209714209850062616169452667236328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5437849397142382468217647328856401145458221435546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.125827814569536400313154445029795169830322265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999999940395355224609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13716}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99337987749781830881801170107792131602764129638671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96068601310253143310546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29052}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94999307394027721063167746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.007552300132325973601454816019895588397048413753509521484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.50565852102837283155167824588716030120849609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18179123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18179123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18179123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{18179123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{35.953642384105961582463351078331470489501953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.1837913528084538228313249419443309307098388671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.61148727785551770796956816411693580448627471923828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.4755527703925890303793266866705380380153656005859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29052}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.231435218363440553535070876023382879793643951416015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.134382113122587298903454211540520191192626953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0604292082571517286115891920417197979986667633056640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{173.78853321075439453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.379171155146423188853077590465545654296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.40055596828460693359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.3773334026336669921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.115617265547614866960657309391535818576812744140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7256786823272705078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.393466436310319522817735560238361358642578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.158598124980926513671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1195471286773681640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12330032031833561279032807078692712821066379547119140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.3615701667363679927547082115779630839824676513671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.276839438642654922517749582766555249691009521484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{7238}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1267828628008805524896018823710619471967220306396484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.1018251201283419948850905711879022419452667236328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0418756389979187126915149974593077786266803741455078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.52340657883643404435503043714561499655246734619140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.429935170143395828379340173341915942728519439697265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.26559039750514645827905724217998795211315155029296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.220493403401791798756903517642058432102203369140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.045238222958576788934603740699458285234868526458740234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{695726677767392826397679198462184985}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{571481864527152322304350718078746624}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{353030191775484947612243541708767232}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{293086004687558677910215494409716910}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{60131912436100220141345972403830784}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{132.0067138671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.2142638654898263439463335089385509490966796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.3510417938232421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.464385986328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.1318176320167747661571411299519240856170654296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{34}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{9134}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.4238410596026493948329516570083796977996826171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99938207864761363641292746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{23367}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99452394207581773510895573053858242928981781005859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96475489437580119744808371251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9635257720947265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.006513361698412945162417475586380533059127628803253173828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{3.89164002285067223141368231154046952724456787109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17636149}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17636149}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17636149}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17636149}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{58}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{48.78807947019867441440510447137057781219482421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.07631931070538744421583032817579805850982666015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.362548821817496758068699591603945009410381317138671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6549}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.27802502976870702156020342954434454441070556640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{15043}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1313340315138205038891783260623924434185028076171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.11978128904379981012340294910245575010776519775390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.041707435445034531096286656293159467168152332305908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{173.6223313808441162109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.272692552465485960055957548320293426513671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{26374}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.641225039958953857421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.4737498760223388671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.02942887931746174245972724747844040393829345703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7486107349395751953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{20754}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3907684727220352982612894265912473201751708984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{6159}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.14559423923492431640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1330697536468505859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.125722950548779743851213197558536194264888763427734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.351165425869312486373274850848247297108173370361328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.27325209993823873499962928690365515649318695068359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.12333521389839548210165531827442464418709278106689453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.095938545513173101308979084933525882661342620849609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04147002771562945111494258298989734612405300140380859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.52624554785913935095464921687380410730838775634765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.43413638277249833041793181109824217855930328369140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.267511555773467912811014457474811933934688568115234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.2223952266047689863004421795267262496054172515869140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.044824843980640509399915316635087947361171245574951171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{699500314871538770258604136220758960}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{577066233970001182299404435502137344}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{355583849130071568041382890126180352}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{295613961331989288776347755373365697}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{59582437525758325442897459665698816}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{133.0085601806640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.14101647383330373486387543380260467529296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{20976}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.9849071502685546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{74.71254730224609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.3554099191410902136567528941668570041656494140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{36}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.72847682119205359185798442922532558441162109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99938213825225841180355246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{23367}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9951740033579188349222022225148975849151611328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7467}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97086398303508758544921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{16149}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96287399530410755499332253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005377856229062046543309971724511342472396790981292724609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{4.0147637718180231303222171845845878124237060546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17650579}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17650579}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17650579}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17650579}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{58}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{48.73509933774834479436321998946368694305419921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{7.23558350782722126126600414863787591457366943359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.353135433665687947790701173289562575519084930419921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.274419421887337977583598558339872397482395172119140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{15399}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.127625656689685340605677765779546461999416351318359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.1128566569435015820577206113739521242678165435791015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0413296917137016828203144314102246426045894622802734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{173.601680755615234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.2951220234498350691865198314189910888671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.4186356067657470703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.8422381877899169921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{2.991170508745589540211540224845521152019500732421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.765802860260009765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{16284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.394590453596304513439463335089385509490966796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1783945560455322265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{8721}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1669747829437255859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12061853625934497447058646457662689499557018280029296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.5388315913303209914175795347546227276325225830078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.430652314452693307789132859397795982658863067626953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{24144}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.2243801052082161628931089580873958766460418701171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2169005352920506946023948557922267355024814605712890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.05955171256192970385967555557726882398128509521484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.38579865454455319895288312181946821510791778564453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.2314799927656893963057171959007973782718181610107421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.12977565758671183449024510991876013576984405517578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.10758716030090749449232845336155151017010211944580078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.044143657666953328710945925195119343698024749755859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{512814372356773666803123781660087988}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{307689686848244030945192469044658176}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{172501437235654557745556140115099648}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{143007865458965772330530277187379493}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{58676985607259799248478056900198400}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{25.76837158203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{10.67154272344728127563939779065549373626708984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26829}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.5517799854278564453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.40165996551513671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.83292431082238493900149478577077388763427734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.78807947019867530258352417149581015110015869140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99973833560943603515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98966761693259741594630440886248834431171417236328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9392581284046173095703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.92620050907134998663394753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01220936576361439894478078116435426636599004268646240234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.78571072582590151256454191752709448337554931640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20118745}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20118745}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20118745}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{20118745}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{2306}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{39.82781456953642162943651783280074596405029296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{13.5782069203158624048910496640019118785858154296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.539423041069625686105837303330190479755401611328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.432491943114589549868043150127050466835498809814453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24144}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.2368594719455353880821490974994958378374576568603515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2170335237663835459276384654003777541220188140869140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.058716433190468618474877615653895190916955471038818359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{174.1119697093963623046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.440690950052641028378275223076343536376953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{28090}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.894414007663726806640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.8196036815643310546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.23132303823582400781333490158431231975555419921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7365868091583234189556605997495353221893310546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3892090320587158203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{19538}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.149247348308563232421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{9.145263195037841796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12159211588429809369760192794274189509451389312744140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.65324082306024877642158799062599427998065948486328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5587881801208192111829475834383629262447357177734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.403029302854967130809171749206143431365489959716796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.25265074475171689361019389252760447561740875244140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.044033037809906916404401044928818009793758392333984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2103768601571602003819094761638552881777286529541015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.125102386206352667041841186801320873200893402099609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.040127874711301948773556347305202507413923740386962890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.02845918004020230041017924804691574536263942718505859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.036073420761969281211900550943028065375983715057373046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{279638812186225580210403332546392172}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{166289594084980623652949489923129344}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{53339094477612218918499665515118592}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{37828738846520300492525058542808020}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{47949800780538391239521137787404288}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{2.874172185430463599686845554970204830169677734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99989861249923717156917746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99346990301119575406119110994040966033935546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9613501727581024169921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20754}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95967924594879161492855246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{22286}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0084093474737528539630915247471421025693416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.62300952722605240641229329412453807890415191650390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18166871}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18166871}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18166871}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{18166871}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{40.65562913907285036430039326660335063934326171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{11.09981585529249059618450701236724853515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6536528447171796596393278377945534884929656982421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.561122483429138174670924854581244289875030517578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.414480170125687108484413556652725674211978912353515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.297203989016589786853472787697683088481426239013671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.04150319611305085254482349910176708362996578216552734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.77167415618896484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.74666317725024100582231767475605010986328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{16149}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{160.078223407268552591631305404007434844970703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.6178452968597412109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.145764149785908347922713801381178200244903564453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7552335262298583984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{7790}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.438937176142307095005890005268156528472900390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.233568251132965087890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2120714187622088076068394002504646778106689453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.115942028149925102642470164937549270689487457275390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.65682941314196041648898471976281143724918365478515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.55416250255749244235659034529817290604114532470703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.39774988027863089623537007355480454862117767333984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.23434523408013940848348966028424911201000213623046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0449129050420496722662022648364654742181301116943359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.219687877138392995135518503957428038120269775390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1322040926656539994166195128855179063975811004638671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.049735034865550899196851020178655744530260562896728515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.031788739839989497981687094352309941314160823822021484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.03642045232033104540381174274443765170872211456298828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{292015276626909003685613348335462987}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{175729381128530635591378225380458496}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{66109200714629143838644591178809344}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{42254482946037378613939609127639049}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{48411084843333724342926775943168000}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.94955348968505859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.28559200968963427413882527616806328296661376953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24262}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.294156372547149658203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.23278331756591796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.62018049874634850748833514444413594901561737060546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{2.947019867549669047690485967905260622501373291015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{913}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{913}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99990135431289683953792746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99390989463060896991208892359281890094280242919921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95170663297176361083984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{22286}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.949099123477935791015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20754}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0086074228885492827523240322307174210436642169952392578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.6066745690383463784911555194412358105182647705078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{19398232}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{19398232}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{19398232}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{19398232}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{40.69536423841059757933180662803351879119873046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{11.0591386665570983183215503231622278690338134765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6572436982471929756144390921690501272678375244140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.55646079989585095493254129905835725367069244384765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.40839308785359562659067478307406418025493621826171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.27567042576537115206036787640186958014965057373046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.04251405654538675804587910533882677555084228515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.4583723545074462890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.8738518061227296129800379276275634765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.964951336383819580078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.6911551952362060546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.218022073402703409072955764713697135448455810546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.848197460174560546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.443224693765703392500654445029795169830322265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.233402729034423828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{10248}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2315745353698712705181605997495353221893310546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1221634774141173995776199490137514658272266387939453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.630989832201026334956850405433215200901031494140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.54075732944748822195180082417209632694721221923828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{28090}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.399917384946232579157054942697868682444095611572265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2244484494726093071204076068170252256095409393310546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0439235812243428946910484000909491442143917083740234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.254209210885715297667530876424279995262622833251953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.153610211404927976541756606820854358375072479248046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.06203810346228215422126339717578957788646221160888671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0466119596942732028477252015363774262368679046630859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037126987230248494065154574172993307001888751983642578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{337901999895684471392304306881330016}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{204182993437869677443331697084989440}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{82462783927466650345924992448856064}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{61957921764026141444368065475695925}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49350230825595379931485845529296896}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.527103424072265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.008277795172684676572316675446927547454833984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11130}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.521240711212158203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0976161956787109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6330534395284164173034469058620743453502655029296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.125827814569536400313154445029795169830322265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99999928474426280633480246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12561}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99499642651602127063625857772422023117542266845703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9670456945896148681640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29052}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.958162844181060791015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.006481754712334995838229900755322887562215328216552734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.53120674516968147127471411295118741691112518310546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{19142200}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{19142200}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{19142200}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{19142200}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{41.27814569536423761064725113101303577423095703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.7943810133891684444051861646585166454315185546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6313406068060458675716972720692865550518035888671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.54298998604682002788734962450689636170864105224609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{30899}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.41002372913582230129492245396249927580356597900390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.264028410355179321555851856828667223453521728515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.041531768373183390596903308278342592529952526092529296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.524883270263671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.658072413198198091777157969772815704345703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.62807905673980712890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.7882397174835205078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.322073951919896739326532042468897998332977294921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.786279201507568359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{16284}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4434430393951611648617472383193671703338623046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{24262}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.237238705158233642578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2121319770813006044818394002504646778106689453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1190666892727703096710456520668230950832366943359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.641348385379791441351926550851203501224517822265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5444912597735236392537672145408578217029571533203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.40191559148199307305304728288319893181324005126953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2102951872027427893119266855137539096176624298095703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.045247652635316104596796549230930395424365997314453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2468951713956774873803823311391170136630535125732421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1468375972595526712805025226771249435842037200927734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{28778}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.057663963362261198841718368157671648077666759490966796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.039416229179302299245879481759402551688253879547119140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037130443949684878435224533177461125887930393218994140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{328179973843249771805715751839229903}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{195180645111187926458132198074613760}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{28778}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{76648554449033318257116211125944320}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{52393155313402926485556264956803845}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49354825593843786668345031485554688}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.37592983245849609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.71346825953350911930783695424906909465789794921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17096}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.6314566135406494140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.5355336666107177734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.542659408581567692664293645066209137439727783203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.08609271523178829710332138347439467906951904296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99999928474426280633480246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12561}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.994747488309215999180423750658519566059112548828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96354834735393524169921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95889359712600719110042746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.006870334840078816916741910603150245151482522487640380859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.56310865349619376729606301523745059967041015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18383990}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18383990}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18383990}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{18383990}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{41.112582781456950442589004524052143096923828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.75281761710498784623268875293433666229248046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.64175290606356660827458426865632645785808563232421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.54672204589683837117064513222430832684040069580078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{16069}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.4115078937570941786106004656176082789897918701171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.24737931633277299159345830048550851643085479736328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.04293709851378997577331375623543863184750080108642578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.6594121456146240234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.6278059672046083505847491323947906494140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{160.004124343395233154296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.9889867305755615234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.303640158474755228468211498693563044071197509765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.88440799713134765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{16284}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4446645335645857954887105734087526798248291015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.245804131031036376953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2417695522308367372943394002504646778106689453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12000490568640127808652806606914964504539966583251953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.395645731875382489217685133553459309041500091552734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.320368655225992726709449698319076560437679290771484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.2234384169845317347213864422883489169180393218994140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.14027922166280359927981180589995346963405609130859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.035369201031999038253861300518110510893166065216064453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.5148122445135745461897158747888170182704925537109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.423127062650797636234045739911380223929882049560546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.304234457916937539589952166352304629981517791748046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.239032276832243206765582499429001472890377044677734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0409235172682686221268255621907883323729038238525390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{684302847980312751871138848543435995}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{562432337449678422465847244036767744}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{404396958745641217392674823729053696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{317728394261627805337596407425425050}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{54396684838970105213342101905866752}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{130.0746917724609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.1853700852552009337159688584506511688232421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.2502727508544921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{4729}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.31154632568359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.0252993165004991027444702922366559505462646484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{32}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.119205298013245197807918884791433811187744140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99953812360763560906917746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9953383096795997975192449302994646131992340087890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9745049774646759033203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20754}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97139424085617076531917746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004726111118083027584635402718049590475857257843017578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{3.43323675272137762704005581326782703399658203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17853686}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17853686}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17853686}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17853686}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{55}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{30371}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{49.25165562913907280062630889005959033966064453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{24.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.29726317193000539873537491075694561004638671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.396284933977182618480838982577552087604999542236328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.321733967707652002143703384717809967696666717529296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.2298065820248069712761207483708858489990234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.165016510421524598140052830785862170159816741943359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03467997667034350417480936812353320419788360595703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.5690329074859619140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.66529454458628833890543319284915924072265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.9453160762786865234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.9602844715118408203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.315806479565974740353340166620910167694091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.816020488739013671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4371994204868538957953205681405961513519287109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2495423555374163271380894002504646778106689453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2468183040618896484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12280432257336591772567402358617982827126979827880859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.63111365901511329301598607344203628599643707275390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5406356746120761780360908232978545129299163818359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{28090}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.400607660984932945069658671854995191097259521484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2255072195518164068772648533922620117664337158203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04383049272260956807922838152080657891929149627685546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.254201377561040275931958376531838439404964447021484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1537484576154500570677186033208272419869899749755859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.062056913982270478502556443345383740961551666259765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.04655510817285850311275652302356320433318614959716796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037099886977102251861548865008444408886134624481201171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{337891587621226273234212094562688152}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{204366754171206765195604142032158720}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{82487787397250365835986226861047808}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{61882353130158697793537547679061994}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49314208410420518099804376413503488}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.6324939727783203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.049719453647437461540903314016759395599365234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.53863298892974853515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0751361846923828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6428017817939328804044407661422155797481536865234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.125827814569536400313154445029795169830322265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99999982118606556280582253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12561}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99498354875488781434711427209549583494663238525390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96703179180622100830078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29052}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.958162844181060791015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.006492404632444124211454461459425147040747106075286865234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.53120674516968147127471411295118741691112518310546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{19150519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{19150519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{19150519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{19150519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{41.27814569536423761064725113101303577423095703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.777188897623734220587721210904419422149658203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.63146450245690266545040003620670177042484283447265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.54286871701997607697620651379111222922801971435546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.41076094353116732182940040729590691626071929931640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6204}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.265273887352688253482568825347698293626308441162109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.041427813052435598362155388940664124675095081329345703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.619036197662353515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{26278}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.682062818514594937369110994040966033935546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{160.079937279224395751953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.354032993316650390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.290075876096982820939729208475910127162933349609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.863525867462158203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{16284}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4426019112795387400183244608342647552490234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{22286}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.22288978099822998046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{9816}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1977503299713117002056605997495353221893310546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.11891023723185493998766304457603837363421916961669921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.64131600951929546017282746106502600014209747314453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5444547653263389630495794335729442536830902099609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{8721}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.40504934042366935731394050890230573713779449462890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{3284}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2133378897269858909258033463629544712603092193603515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04496386152498542398969760824911645613610744476318359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2469492363503749121633745744475163519382476806640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1469885201907770444496037498538498766720294952392578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{28778}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.058084273074022474414590533342561684548854827880859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.041083839409739898729245766162421205081045627593994140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037129138842494351091527704511463525705039501190185546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{328251838494624400153796258984446805}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{195381256096577358492107893169455104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{28778}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{77207241884806703493156641657847808}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{54609789517757925724081991438583431}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49353090808828628301568497370005504}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.43523406982421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.72528035277562441507370749604888260364532470703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22286}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.649292647838592529296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.543451786041260209714209850062616169452667236328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5437849397142382468217647328856401145458221435546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.09271523178807949960855694371275603771209716796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99999982118606556280582253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12561}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99480071841486239492269305628724396228790283203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9630258977413177490234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.958912193775177001953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0068934037178363903597411166401798254810273647308349609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.55613368940972218723572950693778693675994873046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18408947}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18408947}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18408947}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{18408947}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{41.112582781456950442589004524052143096923828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.75281761710498784623268875293433666229248046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6417205097824918436089092210750095546245574951171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.54668711866897512496876743171014823019504547119140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{12561}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.4149606170704249752390069261309690773487091064453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.250958578798373743712346595202689059078693389892578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.042610546456618679511674230298012844286859035491943359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.655929088592529296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.77808175813282787203206680715084075927734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{160.02425301074981689453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.766021728515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.273076733504297397558957527508027851581573486328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.774986743927001953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{20976}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4447326139109026854612238821573555469512939453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.23721611499786376953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2332575321197527529193394002504646778106689453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{8299}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.11789841237834586262778202581102959811687469482421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.394857390795342710898552240905701182782649993896484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.32061827079317206656838834533118642866611480712890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.2228070567974252680354396716211340390145778656005859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.139312079093553198294586081829038448631763458251953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0354360788336620380345465264326776377856731414794921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.5149324209770635984995124090346507728099822998046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.42300904512911807753283710553660057485103607177734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.303791836322608255205324212511186487972736358642578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.2393942698168498861566177993154269643127918243408203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.04096451559806003894781412100201123394072055816650390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{684462589900016792874784059082372473}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{562275465255868283286073768230780928}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{403808613730919778625231954793988096}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{318209565471044753842470307745607553}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{54451180966709269978957789089759232}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{132.0067138671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.2142638654898263439463335089385509490966796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29725}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.3510417938232421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.464385986328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.1318176320167747661571411299519240856170654296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{31}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.139072847682118805323625565506517887115478515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999466598033905029296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99553642051898882936455947856302373111248016357421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97457800805568683966129128748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20754}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97159016132354736328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00452728619040978531862240430427846149541437625885009765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{3.309708246479199811318494539591483771800994873046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17865973}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17865973}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17865973}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17865973}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{55}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{30371}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{49.29801324503311121816295781172811985015869140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{24.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.284261513383182062852938543073832988739013671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.39549531925955572209119281978928484022617340087890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3219832598237009069208625078317709267139434814453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.229132204365924352362782201453228481113910675048828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.163878818823538441318277136815595440566539764404296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03474468342179422297721913537316140718758106231689453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.6403758525848388671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.727942345158140824423753656446933746337890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{23241}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{161.118499577045440673828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{160.718695402145414163896930404007434844970703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.15916685443386580089963899808935821056365966796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7844679355621337890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4412084004736893660947316675446927547454833984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.21865284442901611328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{9816}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1872019767761248232318394002504646778106689453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1206579442170983840210141124771325848996639251708984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.38898691947892538589570676776929758489131927490234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.316606760926428254521169947111047804355621337890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{11130}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.2174437039342986544010472016452695243060588836669921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.1377651284674165921284583191663841716945171356201171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03456005681499400850054115608145366422832012176513671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.51767416503234719993287171746487729251384735107421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.427231714737530243741758795295027084648609161376953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{16197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.304206790562593198945506856034626252949237823486328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.240079670416664392451622234148089773952960968017578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.040799568288011407724003021257885848172008991241455078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{688106992855576642127521065211480032}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{567888355916320305233094478630223872}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{16197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{404360182523677418392675648932937728}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{319120619136645992217892638297421572}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{54231928384363205559614971580514304}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{133.0085601806640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.14101647383330373486387543380260467529296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{20976}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.9849071502685546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{74.71254730224609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.3554099191410902136567528941668570041656494140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{33}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{9.27814569536423761064725113101303577423095703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99946689605712879522769753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9952647638636709093162835415569134056568145751953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97320325672626495361328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20754}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97013860940933238641292746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004955103590718517268809417686270535341463983058929443359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{3.528800971527532137628213604330085217952728271484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17880403}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17880403}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17880403}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17880403}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{55}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{30371}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{49.31788079470198482567866449244320392608642578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{24.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{4.25413061588950025537769761285744607448577880859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.389615363656308832940311503989505581557750701904296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.317956818141799490984311660213279537856578826904296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{23241}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.2236957958949903624290556081177783198654651641845703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.16205907395260477077414407176547683775424957275390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03388592509241246386597623541092616505920886993408203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.661717891693115234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.772798356630943317213677801191806793212890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{20754}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{160.6506345272064208984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{160.3860914707183837890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.136462349056902354504927643574774265289306640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.812288761138916015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{16284}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.439496455603087810004581115208566188812255859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{9132}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.182857215404510498046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1465477943420392392681605997495353221893310546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.11932155352105500156767448061145842075347900390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.5963865013485600830023258822620846331119537353515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.494124508338314505362376394259626977145671844482421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{17096}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.3384524883304533826589022282860241830348968505859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2291356758800124904240647083497606217861175537109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.044700786204173899307523498691807617433369159698486328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.37848898350420900893453790558851324021816253662109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.2204071136493505889131228059341083280742168426513671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1264306788327858310783113893194240517914295196533203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.116122245089761599867728136814548633992671966552734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.042163840198858271168802502870676107704639434814453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{503098152969969894396668949347912775}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{292971305932864458357348081703321600}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{168055197830630297146489508965908480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{154352939106708603495889747887593807}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{56045356802123857732909164075679744}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{25.76837158203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{10.67154272344728127563939779065549373626708984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26829}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.5517799854278564453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.40165996551513671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{17197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.83292431082238493900149478577077388763427734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.71523178807947029866909360862337052822113037109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99977934360504161492855246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30371}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99202047160129669389760920239496044814586639404296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.960518360137939453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95744991302490245477230246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00868196854587769718814005415197243564762175083160400390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.7579816650503043984343776173773221671581268310546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20348569}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20348569}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20348569}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{20348569}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{43.6158940397350960438416223041713237762451171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{4.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{13716}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{9.0560147420728043243798310868442058563232421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.59701574331231033188061019245651550590991973876953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.4961785233205950884638468778575770556926727294921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{27584}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.348706514712058768257207930219010449945926666259765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.26954219733044870732641129507101140916347503662109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.04273043827961263418924175994106917642056941986083984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.5000107288360595703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.69049635312416057786322198808193206787109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{26374}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.55626237392425537109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.9583568572998046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.41202018685953145649136786232702434062957763671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.753912448883056640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{12493}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4434722275133946567393650184385478496551513671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{13716}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2394080758094805361224644002504646778106689453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2147390842437744140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12102260347482189650758499510629917494952678680419921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.528751181102123712918228193302638828754425048828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.406940276552113733288251751218922436237335205078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1172055279658674453724387376496451906859874725341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.056913602943217699026146050300667411647737026214599609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0708504137384647070252441380944219417870044708251953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.23597591141007379089700179974897764623165130615234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.152347384335948021760742676633526571094989776611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0369544658472330256326898734187125228345394134521484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.00903002032406650077811516297288108034990727901458740234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0364388476013942363973541205268702469766139984130859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{313665787777131229002153545629878082}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{202504408343946512443398929216700416}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{49120910573419733117931024273113088}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{12002955817256065141035021725183511}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{48435536365913249923668194141143040}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{2.947019867549669047690485967905260622501373291015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999874174594879150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98905649840437026565354017293429933488368988037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.953875243663787841796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95179170370101917608707253748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00988895534079269576677173603229675791226327419281005859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.34117210257990093769109307686449028551578521728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17680951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17680951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17680951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{17680951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{31.119205298013245197807918884791433811187744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{12457}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.483556788556324335104363854043185710906982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.5293315660558859381268348442972637712955474853515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.40844153519226089610327790069277398288249969482421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{4810}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.119783377024264725552171739764162339270114898681640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.06694993058759103610189100663774297572672367095947265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0703290534957018709238951714723953045904636383056640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.280317783355712890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{165.68353832320661922494764439761638641357421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{133.040353357791872213056194595992565155029296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{57.7237870693206787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.42439495031332086227848776616156101226806640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.724327564239501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{16284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.383882093113779632176374434493482112884521484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{6910}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.131927192211151123046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1124291419982927919818394002504646778106689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1244699304324038691138554213466704823076725006103515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.524161706768248247811925466521643102169036865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.405310971234336514523732830639346502721309661865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{6155}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.11621167003099637515806108467586454935371875762939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0600062734702759004168370893239625729620456695556640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0703327879551425561022170995784108527004718780517578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2393070016442828962244249169089016504585742950439453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1569244857781435242838341537208179943263530731201171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{28778}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.03844845923613270100016592323299846611917018890380859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0148311035531414996124777161412566783837974071502685546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.036631938712217267106741047655305010266602039337158203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{318093566172927729319297224308772036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{208588419720460362021031706401701888}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{28778}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{51106768411462735317636697198428160}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{19713918051220822306723962307836581}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{48692198476156420887759595008688128}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.94955348968505859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.28559200968963427413882527616806328296661376953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24262}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.294156372547149658203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{2345}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.23278331756591796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.62018049874634850748833514444413594901561737060546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{2.96688741721854309929540249868296086788177490234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999874174594879150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98859024126798111797853607640718109905719757080078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9511751234531402587890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95048606395721435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0100941877889709728799427779222241952084004878997802734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.353173288105255223090495064752758480608463287353515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18912312}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18912312}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18912312}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{18912312}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{30.880794701986754802192081115208566188812255859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{12457}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.624774918485453412131391814909875392913818359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.52473705407491999519464798140688799321651458740234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.4068104199069069171201817880501039326190948486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1189246819513952446722981903803884051740169525146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0705879725742038222069396624647197313606739044189453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0697961572605488023146591558543150313198566436767578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.264598369598388671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{165.7705889158690979456878267228603363037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{913}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{133.04763400554656982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{57.7726192474365234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.42779292955162162570559303276240825653076171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7693450450897216796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{20754}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3885908221566918285816427669487893581390380859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{9132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1619110107421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{8721}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.149132251739501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12065834583822833414590292022694484330713748931884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.51500880127585657586308798272511921823024749755859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.39839528272098956307445405400358140468597412109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1170235074458170487776698109883000142872333526611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.069043264829170503116273494015331380069255828857421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06881365404793181317355532655710703693330287933349609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2476155163094294897607738903388963080942630767822265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1705840251339347524162093350241775624454021453857421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{16197}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.043531480442237376060621301121500437147915363311767578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.030759493021117099986749821027842699550092220306396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.036400948762226624511040284914997755549848079681396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{329137476469230200735628677358526876}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{226745061841703917086931141422743552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{16197}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{57863262501785469111978479283339264}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{40886379259819660783710788358405872}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{48385160167883910306657799413694464}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.527103424072265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.008277795172684676572316675446927547454833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.521240711212158203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0976161956787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6330534395284164173034469058620743453502655029296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.079470198675496650508875973173417150974273681640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999874174594879150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98801316804443761743215191017952747642993927001953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95177923142909992559879128748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6155}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95025694370269775390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0095804485128669798765788101491125416941940784454345703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.4072713075899814239022589390515349805355072021484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18656280}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18656280}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18656280}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{18656280}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{31.993377483443708797494764439761638641357421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.553944204480568913595561753027141094207763671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.51557410187469898676937418713350780308246612548828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.399894181797134817824002084307721816003322601318359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{7098}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.12013395582381129755855653229446033947169780731201171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.08121857603120659352402554986838367767632007598876953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0682848955173390448347703340914449654519557952880859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.1136515140533447265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.208248260005433394326246343553066253662109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{27671}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.081105530261993408203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{55.4567220211029052734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.682283453728889099920706939883530139923095703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.76066875457763671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{12493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3872416824694493442393650184385478496551513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{26374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1700794696807861328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1699707508087158203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12149981066409655527937871966059901751577854156494140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.5198227963678989649309869491844438016414642333984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.40054553726219499498739651244250126183032989501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{6082}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.11766185776912464755472598199048661626875400543212890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.06479526030008080084154897804182837717235088348388671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06900836285479393372721546029424644075334072113037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.245303078316888412135909902644925750792026519775390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.166648296422689801143945942385471425950527191162109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{15662}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.042769635979385378643513604401960037648677825927734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0279981302168807004437933727558629470877349376678466796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.036659536825473459931146180679206736385822296142578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{326063719151027922403744149749397657}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{221513581054902529936063924126351360}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{15662}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{56850597513328900462030939874131968}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{37215898513909524954427107496644238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{48728882660927404417606036620312576}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.37592983245849609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.71346825953350911930783695424906909465789794921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17096}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.6314566135406494140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.5355336666107177734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.542659408581567692664293645066209137439727783203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.046357615894039749804278471856378018856048583984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999874174594879150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98830235241264696721685822922154329717159271240234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94957768917083729132144753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94166553020477294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00961560282306807290186867476222687400877475738525390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.404244833431307404314480891116545535624027252197265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17898070}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17898070}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17898070}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{17898070}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{32.21192052980132558559489552862942218780517578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.26706308295009506537098786793649196624755859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.5203933810595600117920866978238336741924285888671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.402042396199506713028171134283184073865413665771484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1205861649330850771111300900884089060127735137939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0762214647317853433161616294455598108470439910888671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0684772692803807536687799029095913283526897430419921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.5442116260528564453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.17802409620475145857199095189571380615234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{30899}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.31705391407012939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{56.713109493255615234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.59589099518223775930891861207783222198486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7260310649871843935443394002504646778106689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{12493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3840396104269476751369438716210424900054931640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.163940966129302978515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1597690582275408388568394002504646778106689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.123352930384128978147373345564119517803192138671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.3647021308474334144733575158170424401760101318359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.25236348450057988213046655801008455455303192138671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0820861456185946469776837375320610590279102325439453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.07979185794317460167501820933466660790145397186279296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.048180870189290132821202661261850153096020221710205078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.48840328573843161397149970071041025221347808837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.391483129908046290079681739371153526008129119873046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2193482933521279931721181810644338838756084442138671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1734601930385548940183326749320258386433124542236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.045092792085739734353477814465804840438067913055419921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{649199320636863096382009965938276772}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{520370336151278448529621283562848256}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{291563892351290952280970517565931520}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{230568144741103040907817474628078599}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{59938601648473743448154222809317376}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{130.0746917724609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.1853700852552009337159688584506511688232421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26932}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.2502727508544921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.31154632568359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.0252993165004991027444702922366559505462646484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{7.51655629139072889444150860072113573551177978515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99970424175262440069644753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{8048}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99453465828042941776487850802368484437465667724609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{11611}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9723308980464935302734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96463572978973399774105246251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{26932}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005829678977306935495905637623081929632462561130523681640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.6908570053065379301671100620296783745288848876953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17367766}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17367766}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17367766}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17367766}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{55}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{45.35099337748344083820484229363501071929931640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{5.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.671617785767960384646357852034270763397216796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.365102446982723538582149558351375162601470947265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.25341898530856032945024480795837007462978363037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{19451}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.09110600401120151625722343169400119222700595855712890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0828933831202112447744667633742210455238819122314453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.04805655741648674761368198460331768728792667388916015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.156330585479736328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.167075007167085232140379957854747772216796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{913}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.981592476367950439453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{58.7807943820953369140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.404487657448196813447793829254806041717529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.695037364959716796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3882138776463381901749016833491623401641845703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1468346714973431943462855997495353221893310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1408903598785400390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.125113890051626597266221097015659324824810028076171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.514563464712366691600209378520958125591278076171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.398404183258415700574772699837922118604183197021484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.116924655134791721788900531464605592191219329833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.06863623188294599997139044944560737349092960357666015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06877873973192129286591267600670107640326023101806640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2478885507610248117860152206048951484262943267822265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1706621472867147215612959598729503341019153594970703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{16197}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.044676984382366724535273760920972563326358795166015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.033347508811551899998715242645630496554076671600341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.036271449084132122153700805711196153424680233001708984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{329500401506104461406311102566742571}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{226848903994269927787094471673380864}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{16197}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{59385898408287336474050491498627072}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{44326442301999039127843679053061681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{48213025570315563164816361597698048}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.6324939727783203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.049719453647437461540903314016759395599365234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.53863298892974853515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0751361846923828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6428017817939328804044407661422155797481536865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.079470198675496650508875973173417150974273681640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999874174594879150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9880189820630660424427560428739525377750396728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95129355788230907098323996251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6155}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.950256884098052978515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00960307170956401466577201375685035600326955318450927734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.4072713075899814239022589390515349805355072021484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18664599}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18664599}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18664599}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{18664599}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{32.019867549668873607515706680715084075927734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.560333281460639653914768132381141185760498046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.51512827648650272305275166218052618205547332763671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.39990251341184279709750626352615654468536376953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{7098}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.12001716107888406315229445908698835410177707672119140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0807397655871765207447054990552715025842189788818359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.068248332784342335965988013413152657449245452880859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.22840785980224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.03408773845393398005398921668529510498046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.508336603641481588056194595992565155029296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{57.59962630271912331636485760100185871124267578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.4803515018606905329079381772316992282867431640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.693142414093017578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{12493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.388567815553273021578206680715084075927734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{26374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.18894612789154052734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{8048}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.177774906158447265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1220481925870832429215084857787587679922580718994140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.51986009038243874424978230308624915778636932373046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.400527122873907626132705672716838307678699493408203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{7098}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.11669116316952267420337108205785625614225864410400390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.05914939797987710246029990912575158290565013885498046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06922624877871101645165907711998443119227886199951171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2453035814799195135638143483447493053972721099853515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1667700857154900961898391642534988932311534881591796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{15662}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.043061975164685802053288199431335669942200183868408203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.029165847387510400456900327981202281080186367034912109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.036606203962028620313429172483665752224624156951904296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{326064387969415208546653845137803827}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{221675466792479712871834422440099840}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{15662}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{57239182942695223527330942143168512}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{38768060868269184543500540126121614}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{48657991125741140425014188653412352}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.43523406982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.72528035277562441507370749604888260364532470703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.649292647838592529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.543451786041260209714209850062616169452667236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5437849397142382468217647328856401145458221435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.046357615894039749804278471856378018856048583984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999874174594879150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9882723515396876212690813190420158207416534423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94958700239658344610660378748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.941702783107757568359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.009632127677607370264123431979896849952638149261474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.404244833431307404314480891116545535624027252197265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17923027}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17923027}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17923027}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{17923027}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{18668}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{32.22516556291390799060536664910614490509033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{16.270955794176092723546389606781303882598876953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.52043071600996082537449183291755616664886474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.40201725236305529964653260321938432753086090087890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1193668622997901274107590552375768311321735382080078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0695799929061156341436600314409588463604450225830078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0687222613408159654913021086031221784651279449462890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.27688312530517578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.10727310022770097930333577096462249755859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{17194}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{133.511666953563690185546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{60.26101207733154296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.2841083620848063873154387692920863628387451171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.8159480094909685732318394002504646778106689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3882865779447239873434227774851024150848388671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.14018142223358154296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.11566638946533203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12352448507783921061164988941527553834021091461181640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.36246308623686840366673322932911105453968048095703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.252383685134612900657913314717006869614124298095703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{12561}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.08203662668389087586628960480084060691297054290771484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.07966457256215879467742269071095506660640239715576171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.048034216567813092790828477518516592681407928466796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.489108589958364980976313063365523703396320343017578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.391413828897979765297776566512766294181346893310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2193227963755117471134070683547179214656352996826171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.174016609551753298479326304004644043743610382080078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.04504638983817109421092794718788354657590389251708984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{650136830751543711160265440273334538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{520278219308561851514342176544784384}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{291530001056164727772777996783452160}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{231307749147763283387854788666314839}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{59876922481938155202569073948884992}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{132.0067138671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.2142638654898263439463335089385509490966796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.3510417938232421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.464385986328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.1318176320167747661571411299519240856170654296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{13}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{7.5099337748344368037578533403575420379638671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999701678752899169921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{8048}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99446460663877578323166517293429933488368988037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{11611}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9724776744842529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.965222656726837158203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{26932}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0059129806612086728556665349287868593819439411163330078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.69482089803286584128727554343640804290771484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17380053}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17380053}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17380053}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17380053}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{55}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{45.23841059602649039561583776958286762237548828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{5.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.6762772297763053330754701164551079273223876953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.362860944679676278301627689870656467974185943603515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.253441172289989136157117854963871650397777557373046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0910021030366269523259603602127754129469394683837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.08286977423697995670526239564424031414091587066650390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.04791810574572873127063843412543064914643764495849609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.4422471523284912109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{165.835775351682258360597188584506511688232421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{133.318266451358795166015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{58.8246948719024658203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.3328796445834338868507984443567693233489990234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7594811916351318359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3903658011101729385927683324553072452545166015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1641350388526934267474644002504646778106689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.11580181121826171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12292303478406918504362010935437865555286407470703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.357827494749345886848601594465435482561588287353515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.249443873677739957894772260260651819407939910888671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0792854064576700434674449979866039939224720001220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.07544192216608079648576534737003385089337825775146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.047150847632245605767220553161678253673017024993896484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.49189994007211279569702355729532428085803985595703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.39522709274599032713837232222431339323520660400390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.219710537314167175804158205210114829242229461669921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.17486635709415609962746884775697253644466400146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.04505046875365847913741390584618784487247467041015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{653847171468774747717255742552443307}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{525346916370651859116461933239205888}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{292045397166937519051552167624179712}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{232437257370474614696298363625895268}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{59882344290596427921705508769103872}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{133.0085601806640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.14101647383330373486387543380260467529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{20976}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.9849071502685546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{74.71254730224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.3554099191410902136567528941668570041656494140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{14}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{7.6953642384105958029749672277830541133880615234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1412}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99964761734008800164730246251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99511723407846408573362850802368484437465667724609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97689336538314808233707253748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.974896013736724853515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00479563926399373223474764671436787466518580913543701171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.76422647809341004432326371897943317890167236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17394483}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17394483}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17394483}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17394483}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{55}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{45.5430463576158928162840311415493488311767578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{5.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{10.4594677155145294733529226505197584629058837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.358220264924463183131564392169821076095104217529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.25048337116403718294321834036963991820812225341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0867111628057966876692574942353530786931514739990234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.08060787172500245845174760006557335145771503448486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.047026796813559514076619194611339480616152286529541015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.3538501262664794921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{165.762933145295704662203206680715084075927734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.996414005756378173828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{58.9913370609283447265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.35435415478244891573922359384596347808837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7350442409515380859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{20754}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.383807922830644798750654445029795169830322265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{28090}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1507360935211181640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.146578311920166015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12447897118690727513712346308238920755684375762939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.489864246228826794027355617799912579357624053955078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.36268510807455367483953523333184421062469482421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{23633}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1369162721789053127618984717628336511552333831787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.1180053654903308046897336680558510124683380126953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.065211365391703413063595462517696432769298553466796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.3653263012773451112735756396432407200336456298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.225439440136174173989758173775044269859790802001953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{14929}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.12364396263516362617362887021954520605504512786865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08970351309256509308998062124373973347246646881103515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.038316348541063638410975045189843513071537017822265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{485601947254401788174884880668789473}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{299660415183080429885082558300946432}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{14929}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{164351016644443590623511460637048832}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{119236420922896353448870195729621069}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{50931163177034296190648788344373248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{25.76837158203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{10.67154272344728127563939779065549373626708984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26829}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.5517799854278564453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.40165996551513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{17197}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.83292431082238493900149478577077388763427734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.6887417218543046004697316675446927547454833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98419884538018942432557878419174812734127044677734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{30899}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94070737063884735107421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.93370443582534801141292746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{3284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.013025449424027883693621987504229764454066753387451171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.8549461116480971956121948096551932394504547119140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{19862649}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{19862649}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{19862649}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{19862649}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{52}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{36.5165562913907280062630889005959033966064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{11498}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{3.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.2939646602275178821628287550993263721466064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.490401946848813496959706981215276755392551422119140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{1283}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.364250924742408888068467831544694490730762481689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{23633}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.137003127219367970557328817449160851538181304931640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.1180658629706853590679571652799495495855808258056640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06483939843321963325539769584793248213827610015869140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.1790688037872314453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.260769433533113215162302367389202117919921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.75512850284576416015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{58.7103278636932373046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.449614285029856119990654406137764453887939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7533125877380353330181605997495353221893310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{7790}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.385003636214907629664594423957169055938720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1500484943389892578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1377911567688006044818394002504646778106689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1263558662745735972077198994156788103282451629638671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.62161638823541254250670817782520316541194915771484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.53736306185184357087081252757343463599681854248046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.384257413712088158330715259580756537616252899169921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.23107931630025391189775518796523101627826690673828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.042786728457581822693267525892224512062966823577880859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2425452943828023955052941573740099556744098663330078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.148431274789244060929860324904439039528369903564453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0406167729949917510889889626923832111060619354248046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.00941587681141400033302257810419177985750138759613037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.036740497311942017788499725838846643455326557159423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{322397995539514968294529734148308702}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{197299005899907068079856722567495680}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{14095}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{53988951763383900075292072706310144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{12515847062593605744373671271668502}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{48836497606093768156412733554688000}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.006622516556291202505235560238361358642578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99999922513961803094417746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12561}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99028087964910549434449649197631515562534332275390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93607722222805034295589621251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.89433825016021728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0127637590445396596761096219552200636826455593109130859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.481398194579768123890772812956129200756549835205078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17910775}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17910775}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17910775}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{17910775}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{35.900662251655631962421466596424579620361328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.5383545826957405466828276985324919223785400390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.621961952033637910375318824662826955318450927734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.53957856899492029345566379561205394566059112548828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{15043}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.404353665278002705196769284157198853790760040283203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6204}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.27182858554860855893053894760669209063053131103515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0402317306822177755964986545222927816212177276611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.497099399566650390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.45553196976516119320876896381378173828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.8080031871795654296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{53.86025142669677734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.90521545315981910562186385504901409149169921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7203814983367919921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{20751}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.434579043988360780303992214612662792205810546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2194715738296491025494105997495353221893310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.20488071441650390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.119386061415710342803464527605683542788028717041015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6167380407885587612071276453207246959209442138671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{27671}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.53324592625645761412300771553418599069118499755859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{15043}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.3807128151550907002587109673186205327510833740234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2216539550831088944971014598195324651896953582763671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.042870466690012841437518176235244027338922023773193359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.25143338190381381291871321081998758018016815185546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1542077960460958296895483954358496703207492828369140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.04249197096556782404785934659230406396090984344482421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.016534955575495398349961106987393577583134174346923828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.036777673254701555294321480005237390287220478057861328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{334212290301429738629344878731420455}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{204977319672761071011681588712833024}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{56481517403512665957955199521783808}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{21978725860008470822839117748407025}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{48885912909979442949965609019899904}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.94955348968505859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.28559200968963427413882527616806328296661376953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24262}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.294156372547149658203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{2345}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.23278331756591796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.62018049874634850748833514444413594901561737060546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.072847682119205448003640412935055792331695556640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9997990131378173828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{12561}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99088640165644770174679933916195295751094818115234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19451}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93174117803573619500667746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.893912732601165771484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01213151734615607046929852685934747569262981414794921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.447203788506864430285503431150573305785655975341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{19142136}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{19142136}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{19142136}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{19142136}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{36.22516556291390799060536664910614490509033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.187208012806191703703007078729569911956787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.61712703887393194346344671430415473878383636474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27671}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.53543835090918745489574348539463244378566741943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{12561}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.401143202941739662747977490653283894062042236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6204}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.260741125844460075455799596966244280338287353515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.040401927425877635913220586871830164454877376556396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.4286468029022216796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.5384518689667174839996732771396636962890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.108272016048431396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{52.930239200592041015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.0083431691450943645804727566428482532501220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7361774444580078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{20751}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4398384473181717879697316675446927547454833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{32382}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2149889469146728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.197172641754150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1185653270722309693407936492803855799138545989990234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6043790041451388983517745145945809781551361083984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.522039272717169655635416347649879753589630126953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.383237107907215823754398797973408363759517669677734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.237139099376977302569002858945168554782867431640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.040805114987667652493019687653941218741238117218017578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.263055763198836611849174005328677594661712646484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1707854977262222018197235229308716952800750732421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.046274577572140575265624562462107860483229160308837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0287144612432513983424353654072547215037047863006591796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037294952025013573815304113168167532421648502349853515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{349661084896461093062074368625926149}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{227012864851755718063381600123486208}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{61509464002010127400484750594408448}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{38168065768410734307806421322147478}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49573494333103391617292359572652032}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.527103424072265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.008277795172684676572316675446927547454833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.521240711212158203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0976161956787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6330534395284164173034469058620743453502655029296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.165562913907284947612197356647811830043792724609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999739944934844970703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{29110}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9900808117247574813291066675446927547454833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7790}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93808048963546764031917746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.893144190311431884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01103006212014590557701776418753070174716413021087646484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.494077018638264531258386114132008515298366546630859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18886104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18886104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18886104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{18886104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{37.072847682119203227557591162621974945068359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.0491905737092448447356218821369111537933349609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.60471498548056168420572475952212698757648468017578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.5242122618267692768512233669753186404705047607421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{27584}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.399869424841895415578818528956617228686809539794921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6204}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2789569702472061152320748078636825084686279296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.038323512301146701874987599012456485070288181304931640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.761911869049072265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.65984878476882613540510646998882293701171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{23447}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{134.07174026966094970703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{58.9938499927520751953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.56445244706153374636414810083806514739990234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.795995235443115234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{20754}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.44536649786083870594666223041713237762451171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{7238}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2259491682052594541119105997495353221893310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{9816}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2042772769927978515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1251748070998326689551305435088579542934894561767578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.60640254548741834295100261442712508141994476318359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5254278898501514305507953395135700702667236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.383939246244386522821656626547337509691715240478515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2359308330741357873083785534618073143064975738525390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04149151248700709559980026597258984111249446868896484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.261200279071756080728761162390583194792270660400390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1658008786350496366335249831536202691495418548583984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.04515734505653300201455380147308460436761379241943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.026331200340249501234968221297094714827835559844970703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037112396905553957093815142798121087253093719482421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{347194723449011078610315099327629011}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{220387169607445291077347860247740416}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{60024407264463296172435549338992640}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{35000168654881060860356216833021297}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49330836957543800164803361384693760}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.37592983245849609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.71346825953350911930783695424906909465789794921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17096}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.6314566135406494140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.5355336666107177734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.542659408581567692664293645066209137439727783203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.112582781456953551213473474490456283092498779296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99969160556793201788394753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99017964609411379672820885389228351414203643798828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93043194711208332403629128748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{18668}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.89327526092529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0116598855418496051561394466489218757487833499908447265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.438888517239228892474756094088661484420299530029296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18127894}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18127894}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18127894}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{18127894}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{36.36423841059602324321531341411173343658447265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.401678520251408599506248719990253448486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.60673965173306765308325338992290198802947998046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.5276098609116484094982979513588361442089080810546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{30684}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.400032112523210192644995686350739561021327972412109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6204}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.277535634381555984528944236444658599793910980224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0389979277319648931499074251405545510351657867431640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.5070712566375732421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.711429952785664454495417885482311248779296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{30371}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.831253528594970703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{53.8872611522674560546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.9266896024844140100640288437716662883758544921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.8091592788696271298931605997495353221893310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4468402767812964526683572330512106418609619140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{30684}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.204099833965301513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1756074428558367372943394002504646778106689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1256430584135459493921871398924849927425384521484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.395537576910560295662122598514542914927005767822265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.31986055049263739658016447720001451671123504638671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{13654}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.225449495342744554715608273909310810267925262451171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.14620391746150118716940369267831556499004364013671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0345693006653144951911826865398325026035308837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.49450019528885380548643979636835865676403045654296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.412486640334750853664758096783771179616451263427734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{20751}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.22692384386542341356829410869977436959743499755859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1833222082877064007533363110269419848918914794921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.044982158895618261362780998524613096378743648529052734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{657303503499052664180563743974875609}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{548288790220214317400854483160793088}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{20751}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{301633526177046014620731710057218048}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{243677011505132896300767516542411365}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{59791544914901304798031385395724288}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{130.0746917724609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.1853700852552009337159688584506511688232421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26932}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.2502727508544921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.31154632568359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.0252993165004991027444702922366559505462646484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{33}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.596026490066225989039594423957169055938720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99960547685623157843082253748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{26932}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9947154727203166846294379865867085754871368408203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{13654}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97336931526660919189453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{27714}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96664273738861083984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20751}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005310291812906232748747736849281864124350249767303466796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.861432994280178387924706839839927852153778076171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17597590}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17597590}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17597590}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17597590}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{59}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{47.5695364238410576263049733825027942657470703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{913}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.6976513034090512377360937534831464290618896484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.3957307230048645596554024450597353279590606689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.32123481446037238651314282833482138812541961669921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20751}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.232320018548374862543681729221134446561336517333984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.171985986117363764957843841330031864345073699951171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.033897341532127471530611018124545807950198650360107421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.7856719493865966796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.62033756995043631832231767475605010986328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.524975717067718505859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{53.6340172290802001953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.9411085503264349227947604958899319171905517578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.8223588466644287109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4367481951681977392354383482597768306732177734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.205481827259063720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.132116794586181640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12365566849841731766890262633751262910664081573486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.60428480249482363628743541994481347501277923583984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5221567399977560253176989135681651532649993896484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{27584}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.3837630812387196055368576708133332431316375732421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.238996153214439510659161669536842964589595794677734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0405867952097184458981615762240835465490818023681640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.263060619700161202327848286586231552064418792724609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1708917623687324083281424691449501551687717437744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0466132916472892511183800934304599650204181671142578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0300437945554398004588403381376338074915111064910888671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037264427558903336079598744845498003996908664703369140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{349667540293983216338661668535732751}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{227154114789542434219214271202459648}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{61959692233264106291619881438674944}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{39935052822701027664841858754564702}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49532920358193257278181459288391680}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.6324939727783203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.049719453647437461540903314016759395599365234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.53863298892974853515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0751361846923828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6428017817939328804044407661422155797481536865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.165562913907284947612197356647811830043792724609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999739944934844970703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{29110}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99007375508744199787969364479067735373973846435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7790}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9380800724029541015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.8931427001953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0110360705950486616411243545599063509143888950347900390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.494077018638264531258386114132008515298366546630859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18894423}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18894423}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18894423}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{18894423}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{37.033112582781456012526177801191806793212890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.0277523483372004164948521065525710582733154296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.60462073146245065569104326641536317765712738037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.5243323069631211641450363458716310560703277587890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{23241}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.3998868140830673656438420948688872158527374267578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6204}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.28114150292631900907025510605308227241039276123046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.038089091576974550001910557739392970688641071319580078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.9955017566680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.569992990683232392257195897400379180908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.221842586994171142578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{51.9414322376251220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.070521676230274721319801756180822849273681640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.8397514820098876953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4438268980443087485809883219189941883087158203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2028756141662615419818394002504646778106689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{11598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1166050434112566591693394002504646778106689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1295320168002212779523318886276683770120143890380859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6064075623937725811885002258350141346454620361328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.525428257311788993177970041870139539241790771484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.38392745879052714297330339832114987075328826904296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2359308330741357873083785534618073143064975738525390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04146905195783938402609436479906435124576091766357421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.26122049795370039237951687027816660702228546142578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1658924366507664449610359724829322658479213714599609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.04515737206331872644060609900407143868505954742431640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.026331152937984901585277697222409187816083431243896484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0371296781430152378344899943840573541820049285888671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{347221598952934882983228583921500905}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{220508871085174403570711557933367296}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{60024443162638966467326398619975680}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{35000105646463890008612209056781345}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49353807662179160018193562157973504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.43523406982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.72528035277562441507370749604888260364532470703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.649292647838592529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.543451786041260209714209850062616169452667236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5437849397142382468217647328856401145458221435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.119205298013245197807918884791433811187744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999739944934844970703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{29110}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99019947075685921245025156167685054242610931396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{8745}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93012526631355274542301003748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{18668}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.893275201320648193359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01169500473271481259807114128079774673096835613250732421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.444646631300517014562245776687632314860820770263671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18152851}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18152851}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18152851}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{18152851}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{36.3907284768211951586636132560670375823974609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.4147832673032016970182667137123644351959228515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6067446714283786235455409041605889797210693359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.5276116136141395518421859378577210009098052978515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{30684}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.40003211026046014975321440942934714257717132568359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6204}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.277535634381555984528944236444658599793910980224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.038990881758337592177809938220889307558536529541015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.7373340129852294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.543892948832734646202879957854747772216796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.731911599636077880859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{51.602179050445556640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.051871232161442293318032170645892620086669921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7528550624847394345806605997495353221893310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.443915703438765518740183324553072452545166015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{9132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.21891677379608154296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1634089946746843935443394002504646778106689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1273303297779194986905082487282925285398960113525390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.39617782237765009067942401088657788932323455810546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.319858403496335430560293389135040342807769775390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{13654}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.22454796667258214437623564663226716220378875732421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.145889295424251608235266530755325220525264739990234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.034414994187750409804227302856816095300018787384033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.49444902328945639080615137572749517858028411865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.41243266263781597213977647697902284562587738037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{20751}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2270274127593203405961475027652340941131114959716796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1855712755525986967786167269878205843269824981689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0449002447722019748521660176265868358314037322998046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{657235484244853393796443913482411146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{548217041554300479234733642572890112}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{20751}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{301771192850306250645897227039408128}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{246666534678031223123065145237693583}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{59682662368806177586752569701564416}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{132.0067138671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.2142638654898263439463335089385509490966796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.3510417938232421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.464385986328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.1318176320167747661571411299519240856170654296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{33}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.5695364238410594026618127827532589435577392578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99966263771057117804019753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{5928}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9945244587809833891611788203590549528598785400390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29052}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96973447501659393310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{16069}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.966607511043548583984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20751}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005643661829085517590842702162490240880288183689117431640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.85524945564679466514235173235647380352020263671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17609877}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17609877}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17609877}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17609877}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{59}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{47.4768211920529807912316755391657352447509765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{6204}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.76162194084250955938841798342764377593994140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.3963712811120638779271985185914672911167144775390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.321234184904015729333792705801897682249546051025390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{19488}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.231402768116355961325325552024878561496734619140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.171615882618975146289841404723119921982288360595703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.033757680868057644840707354205733281560242176055908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.752162933349609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.487675278392060818077879957854747772216796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.5120990276336669921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{51.5117042064666748046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.0596460112051300228586114826612174510955810546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7178266048431396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4390619180060379989072316675446927547454833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.217630684375762939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1856682300567644716693394002504646778106689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12220061406041170248837346434811479412019252777099609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.397668706068207977732953395388904027640819549560546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.316438237061332283683867672152700833976268768310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{27714}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.22455347920994983557108071181573905050754547119140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.1448010256255634065070125870988704264163970947265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.034178143494096833998607820603865548036992549896240234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.499417119825069588667787456870428286492824554443359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{12493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.416155059666427462605753362367977388203144073486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{6532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2272589597188503229840961239460739307105541229248046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1860109352715345887308018291150801815092563629150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.04480887275809648795377171381915104575455188751220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{663839217245752510359243305731390237}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{12493}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{553164955896157604427745429035155456}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{6532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{302078971551252380161673183547621376}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{247250942685059764722007916200828716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{59561208129625891727346479602335744}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{133.0085601806640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.14101647383330373486387543380260467529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{20976}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.9849071502685546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{74.71254730224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.3554099191410902136567528941668570041656494140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{34}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.7880794701986761907619438716210424900054931640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99966144561767578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{5928}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9947367578942254429108515978441573679447174072265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29052}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97642777860164631231754128748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97535288333892822265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{27714}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004784638114200390375529980957480802317149937152862548828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{3.0375340109794120024844232830218970775604248046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17624307}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17624307}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17624307}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17624307}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{59}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{9134}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{47.76821192052980080688939779065549373626708984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{913}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{8.6426048536929211962842600769363343715667724609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.39786289282033415748429661107365973293781280517578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.317801969292294705926593678668723441660404205322265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{32103}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.231360927937333149539966825614101253449916839599609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.1703357038266495593337168656944413669407367706298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.033552426497962396789720429524095379747450351715087890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.6679251194000244140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.559956440072966188381542451679706573486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.94467604160308837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{54.485658168792724609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.85622112550547768705655471421778202056884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.747427463531494140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4376090709736804029716950026340782642364501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{30899}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.225420773029327392578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{8048}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1970374584197998046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1238049010755639944836303811825928278267383575439453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.57036501548934970262649812866584397852420806884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.4770663327731077263393899556831456720829010009765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{30684}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.318196892667536979093512172767077572643756866455078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2137714464151750093368065108734299428761005401611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.042563156905902725657409035875389236025512218475341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.3752746673646409902858067653141915798187255859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.231823636213886852264209892382496036589145660400390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{6155}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1293201457751154415110050877046887762844562530517578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0873038272974560047856584787950851023197174072265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.041071259664019484081354249838113901205360889434814453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{498825593969952824523070029421222213}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{308146467340156374251038984072331264}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{6155}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{171895958183269891211823524045914112}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{116046691382949974996229741699421201}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{54593068167566466873463664373923840}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{25.76837158203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{10.67154272344728127563939779065549373626708984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26829}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.5517799854278564453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.40165996551513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{17197}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.83292431082238493900149478577077388763427734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.84768211920529790148748361389152705669403076171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999911725521087646484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98838589917745023338824239544919691979885101318359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19451}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94379134476184844970703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.93648880720138560906917746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01243747197393938776210919883169481181539595127105712890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.76986576942042983517922039027325809001922607421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20092473}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20092473}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20092473}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{20092473}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{39.4370860927152335762002621777355670928955078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{14.52815314805189927938045002520084381103515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.57096680242045805275807879297644831240177154541015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.47907346645700898957187519044964574277400970458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.327764677814585680959424962566117756068706512451171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.251468590266264946375684985468978993594646453857421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0409057775954025093501087440017727203667163848876953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.7436153888702392578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.79560119426804476461256854236125946044921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{8840}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{133.37755858898162841796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{56.339366912841796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{9.7458512676435891108894793433137238025665283203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.8352782726287841796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.450199643507698255007198895327746868133544921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{13654}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2096004486083966611431605997495353221893310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{9816}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1989953517913818359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1277623873898756645672847298556007444858551025390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000000000000000000165509604595778081121998104440892191436868110393509923028432240244001150131225586}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0000000000000000000000000000000000131829745262019502162726180067030571437762908623750416264785950101904594762699563119376692209294699154042973532341420650482177734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00000000000000000000000000000000000156287964793898766576156863776906754362374651569537278014652247595627007127158329802577461042044359995628610704443417489528656005859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17678903}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17678903}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17678903}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{17678903}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.000000000000000000000000000000000016555357570697848429232115475967500129044760969697819635948426808501338983557062728860521916805781383885687318979762494564056396484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000000000000000000013239192724983814129584763267879810373252011537982660774993484583986563848780952923749415169919763091144204736337997019290924072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29565}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000000000000000000151529983549033140767031914238491166435058217093888721032907685340346286594096172077700507112296701706100066076032817363739013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.9699895381927490234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{6204}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.508692934023628140494110994040966033935546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{17096}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.07797443866729736328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.50109386444091796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.54762500127765623147979567875154316425323486328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.66013240814208984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.374407128782461740001963335089385509490966796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{32103}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.17673766613006591796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{8745}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.176082134246826171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1190694048834064766584361905188416130840778350830078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000000000000000000165509604595778081121998104440892191436868110393509923028432240244001150131225586}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0000000000000000000000000000000000131829745262019502162726180067030571437762908623750416264785950101904594762699563119376692209294699154042973532341420650482177734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00000000000000000000000000000000000156287964793898766576156863776906754362374651569537278014652247595627007127158329802577461042044359995628610704443417489528656005859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.94955348968505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.28559200968963427413882527616806328296661376953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.294156372547149658203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{2345}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.23278331756591796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.62018049874634850748833514444413594901561737060546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18910264}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18910264}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18910264}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{18910264}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.000000000000000000000000000000000016555357570697848429232115475967500129044760969697819635948426808501338983557062728860521916805781383885687318979762494564056396484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000000000000000000013239192724983814129584763267879810373252011537982660774993484583986563848780952923749415169919763091144204736337997019290924072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29565}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000000000000000000151529983549033140767031914238491166435058217093888721032907685340346286594096172077700507112296701706100066076032817363739013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{174.866734981536893656084430404007434844970703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.516277335337463227915577590465545654296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22545}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{157.857379376888246724774944595992565155029296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.09364986419677734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.536522200532744353296266126562841236591339111328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.749812602996826171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{12457}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.376140280275155447498036664910614490509033203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{519}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1647663116455078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1586859226226806640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{10248}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.126271490921403939378109271274297498166561126708984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000000000000000000165509604595778081121998104440892191436868110393509923028432240244001150131225586}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0000000000000000000000000000000000131829745262019502162726180067030571437762908623750416264785950101904594762699563119376692209294699154042973532341420650482177734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00000000000000000000000000000000000156287964793898766576156863776906754362374651569537278014652247595627007127158329802577461042044359995628610704443417489528656005859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.527103424072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.008277795172684676572316675446927547454833984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11130}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.521240711212158203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0976161956787109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6330534395284164173034469058620743453502655029296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18654232}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18654232}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18654232}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{18654232}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.000000000000000000000000000000000016555357570697848429232115475967500129044760969697819635948426808501338983557062728860521916805781383885687318979762494564056396484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000000000000000000013239192724983814129584763267879810373252011537982660774993484583986563848780952923749415169919763091144204736337997019290924072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29565}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000000000000000000151529983549033140767031914238491166435058217093888721032907685340346286594096172077700507112296701706100066076032817363739013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.31329250335693359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.380968843864280870548100210726261138916015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.564140617847442626953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.9311788082122802734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.502412926908857304653110986691899597644805908203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7142920494079607607318394002504646778106689453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{20751}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.368577260844755727475785533897578716278076171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{21598}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.122229278087615966796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1081249713897705078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12265335850307411413862013205289258621633052825927734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000000000000000000165509604595778081121998104440892191436868110393509923028432240244001150131225586}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0000000000000000000000000000000000131829745262019502162726180067030571437762908623750416264785950101904594762699563119376692209294699154042973532341420650482177734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00000000000000000000000000000000000156287964793898766576156863776906754362374651569537278014652247595627007127158329802577461042044359995628610704443417489528656005859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.37592983245849609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.71346825953350911930783695424906909465789794921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17096}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.6314566135406494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.5355336666107177734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.542659408581567692664293645066209137439727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17896022}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17896022}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17896022}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{17896022}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.000000000000000000000000000000000016555357570697848429232115475967500129044760969697819635948426808501338983557062728860521916805781383885687318979762494564056396484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000000000000000000013239192724983814129584763267879810373252011537982660774993484583986563848780952923749415169919763091144204736337997019290924072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29565}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000000000000000000151529983549033140767031914238491166435058217093888721032907685340346286594096172077700507112296701706100066076032817363739013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.433391571044921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.43853392979957561692572198808193206787109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{13468}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{157.824779033660888671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.6369836330413818359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.6276738920769506790975356125272810459136962890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7181446552276593564556605997495353221893310546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{20751}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3705065771443951661012761178426444530487060546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{6589}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.138503015041351318359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{29052}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.0864479541778564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12929778825857629609430432537919841706752777099609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000000000000000000165509604595778081121998104440892191436868110393509923028432240244001150131225586}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0000000000000000000000000000000000131829745262019502162726180067030571437762908623750416264785950101904594762699563119376692209294699154042973532341420650482177734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00000000000000000000000000000000000156287964793898766576156863776906754362374651569537278014652247595627007127158329802577461042044359995628610704443417489528656005859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.00100390701285499989690863653635233276872895658016204833984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.000006648390813609270986301279238173123076194315217435359954833984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00008142582551974903598036858998199249981553293764591217041015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{1334421306651730013590654919443184}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{8837227196369073515971580264448}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{108233486860752608384155889172480}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{130.0746917724609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.1853700852552009337159688584506511688232421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26932}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.2502727508544921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{4729}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.31154632568359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.0252993165004991027444702922366559505462646484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{2}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1.0066225165562914245498404852696694433689117431640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.08110893188023771127603822606033645570278167724609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17365718}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17365718}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17365718}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17365718}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{2}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1.0066225165562914245498404852696694433689117431640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0.08110893188023771127603822606033645570278167724609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.000000000000000000000000000000000016555357570697848429232115475967500129044760969697819635948426808501338983557062728860521916805781383885687318979762494564056396484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000000000000000000013239192724983814129584763267879810373252011537982660774993484583986563848780952923749415169919763091144204736337997019290924072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29565}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000000000000000000151529983549033140767031914238491166435058217093888721032907685340346286594096172077700507112296701706100066076032817363739013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.932476043701171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.448667750453324742920813150703907012939453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{21317}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.332096576690673828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.721299648284912109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.483111407890873589821012501488439738750457763671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.6780529022216796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.374765970849043839052683324553072452545166015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{31308}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.182668030261993408203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{8721}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1563310623168963076068394002504646778106689453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12223700413888947957641306629739119671285152435302734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000000000000000000165509604595778081121998104440892191436868110393509923028432240244001150131225586}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0000000000000000000000000000000000131829745262019502162726180067030571437762908623750416264785950101904594762699563119376692209294699154042973532341420650482177734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00000000000000000000000000000000000156287964793898766576156863776906754362374651569537278014652247595627007127158329802577461042044359995628610704443417489528656005859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.6324939727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.049719453647437461540903314016759395599365234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.53863298892974853515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0751361846923828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6428017817939328804044407661422155797481536865234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18662551}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18662551}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18662551}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{18662551}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.000000000000000000000000000000000016555357570697848429232115475967500129044760969697819635948426808501338983557062728860521916805781383885687318979762494564056396484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000000000000000000013239192724983814129584763267879810373252011537982660774993484583986563848780952923749415169919763091144204736337997019290924072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29565}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000000000000000000151529983549033140767031914238491166435058217093888721032907685340346286594096172077700507112296701706100066076032817363739013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.8187162876129150390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.40159026360669258792768232524394989013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.116588115692138671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.6875133514404296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.484857155220532742845307438983581960201263427734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7288708686828595517681605997495353221893310546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{20976}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.37444283788567389592571998946368694305419921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{21598}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1392610073089599609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{11124}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.13475131988525390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12299823816613460192304074780622613616287708282470703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000000000000000000165509604595778081121998104440892191436868110393509923028432240244001150131225586}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0000000000000000000000000000000000131829745262019502162726180067030571437762908623750416264785950101904594762699563119376692209294699154042973532341420650482177734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00000000000000000000000000000000000156287964793898766576156863776906754362374651569537278014652247595627007127158329802577461042044359995628610704443417489528656005859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.43523406982421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.72528035277562441507370749604888260364532470703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.649292647838592529296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.543451786041260209714209850062616169452667236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5437849397142382468217647328856401145458221435546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17920979}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17920979}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17920979}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{17920979}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.000000000000000000000000000000000016555357570697848429232115475967500129044760969697819635948426808501338983557062728860521916805781383885687318979762494564056396484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000000000000000000013239192724983814129584763267879810373252011537982660774993484583986563848780952923749415169919763091144204736337997019290924072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29565}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000000000000000000151529983549033140767031914238491166435058217093888721032907685340346286594096172077700507112296701706100066076032817363739013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{174.4650313854217529296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.502739165792405628963024355471134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24173}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.433639228343963623046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.1922037601470947265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.405889504694669778217530620167963206768035888671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.702233791351318359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{20754}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3779196139202998239170483429916203022003173828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{1283}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.166779100894927978515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{8721}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1595816612243634580181605997495353221893310546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1265645781733164831894811186430160887539386749267578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000000000000000000165509604595778081121998104440892191436868110393509923028432240244001150131225586}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0000000000000000000000000000000000131829745262019502162726180067030571437762908623750416264785950101904594762699563119376692209294699154042973532341420650482177734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00000000000000000000000000000000000156287964793898766576156863776906754362374651569537278014652247595627007127158329802577461042044359995628610704443417489528656005859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.00100390701285499989690863653635233276872895658016204833984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.000006648390813609270986301279238173123076194315217435359954833984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00008142582551974903598036858998199249981553293764591217041015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{1334421306651730013590654919443184}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{8837227196369073515971580264448}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{108233486860752608384155889172480}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{132.0067138671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.2142638654898263439463335089385509490966796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.3510417938232421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.464385986328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.1318176320167747661571411299519240856170654296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{2}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1.0066225165562914245498404852696694433689117431640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.08110893188023771127603822606033645570278167724609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17378005}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17378005}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17378005}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17378005}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{2}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1.0066225165562914245498404852696694433689117431640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0.08110893188023771127603822606033645570278167724609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.000000000000000000000000000000000016555357570697848429232115475967500129044760969697819635948426808501338983557062728860521916805781383885687318979762494564056396484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000000000000000000013239192724983814129584763267879810373252011537982660774993484583986563848780952923749415169919763091144204736337997019290924072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29565}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000000000000000000151529983549033140767031914238491166435058217093888721032907685340346286594096172077700507112296701706100066076032817363739013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{174.7974846363067626953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29110}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.487562394300056212159688584506511688232421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.263736188411712646484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.6169331073760986328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.523769402991572707861678281915374100208282470703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7074832916259765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3734138832976494626336716464720666408538818359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{26932}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.17316138744354248046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1655292510986328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{8721}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1221669227114921818522219609803869388997554779052734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000000000000000000165509604595778081121998104440892191436868110393509923028432240244001150131225586}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0000000000000000000000000000000000131829745262019502162726180067030571437762908623750416264785950101904594762699563119376692209294699154042973532341420650482177734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00000000000000000000000000000000000156287964793898766576156863776906754362374651569537278014652247595627007127158329802577461042044359995628610704443417489528656005859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.00100390701285499989690863653635233276872895658016204833984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.000006648390813609270986301279238173123076194315217435359954833984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00008142582551974903598036858998199249981553293764591217041015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{1334421306651730013590654919464559}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{8837227196369073515971580264448}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{108233486860752608384155889172480}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{133.0085601806640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.14101647383330373486387543380260467529296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{20976}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.9849071502685546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{74.71254730224609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.3554099191410902136567528941668570041656494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{2}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1.0066225165562914245498404852696694433689117431640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.08110893188023771127603822606033645570278167724609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17392435}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17392435}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17392435}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17392435}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{2}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1.0066225165562914245498404852696694433689117431640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0.08110893188023771127603822606033645570278167724609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.000000000000000000000000000000000016555357570697848429232115475967500129044760969697819635948426808501338983557062728860521916805781383885687318979762494564056396484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000000000000000000013239192724983814129584763267879810373252011537982660774993484583986563848780952923749415169919763091144204736337997019290924072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29565}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000000000000000000151529983549033140767031914238491166435058217093888721032907685340346286594096172077700507112296701706100066076032817363739013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.6295950412750244140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.4473801290752135173534043133258819580078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4430}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.485258877277374267578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.4633846282958984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.494004282961004737018129162606783211231231689453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.675357818603515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.3733358288442847339183572330512106418609619140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{19488}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1654698848724365234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.163347721099853515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{8721}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.11815181418021634962567389948162599466741085052490234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0000000000000000000000000000000000165509604595778081121998104440892191436868110393509923028432240244001150131225586}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0000000000000000000000000000000000131829745262019502162726180067030571437762908623750416264785950101904594762699563119376692209294699154042973532341420650482177734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00000000000000000000000000000000000156287964793898766576156863776906754362374651569537278014652247595627007127158329802577461042044359995628610704443417489528656005859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{25.76837158203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{10.67154272344728127563939779065549373626708984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26829}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.5517799854278564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.40165996551513671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.83292431082238493900149478577077388763427734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{19860601}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{19860601}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{19860601}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{19860601}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.000000000000000000000000000000000016555357570697848429232115475967500129044760969697819635948426808501338983557062728860521916805781383885687318979762494564056396484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000000000000000000000000000000000013239192724983814129584763267879810373252011537982660774993484583986563848780952923749415169919763091144204736337997019290924072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29565}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000000000000000000000000000000151529983549033140767031914238491166435058217093888721032907685340346286594096172077700507112296701706100066076032817363739013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.0191261768341064453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29110}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{166.366188188262327685151831246912479400634765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{158.166524827480287740399944595992565155029296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8048}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{157.776393413543701171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.553579881861107736540361656807363033294677734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.699091434478759765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{20751}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.371668212461155889059227774851024150848388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{20013}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.156078279018402099609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{8721}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1416599750518798828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.11622402290513943190486401135785854421555995941162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.005565179927507399836039692075928542180918157100677490234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000068978598338371066751861793164835034986026585102081298828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{7790}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.000583522354244802167293204586684396417695097625255584716796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.001878177814660000020940966436455710208974778652191162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.00002805891927913244898967586038462940223325858823955059051513671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00020337417263932775477776326855661181980394758284091949462890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{2496526532308334602970352387390310}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{37296701037293740550557137895424}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{270330643891801319636574868078592}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{2}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1.0198675496688742736495214558090083301067352294921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99998508739155644864382566083804704248905181884765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99943704903125762939453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99774819612503040655582253748434595763683319091796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{30684}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00018264140710256399589839215735764810233376920223236083984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.1395450828192415781980884048607549630105495452880859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17908727}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17908727}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17908727}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{17908727}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{3}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{30684}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{1.0264900662251654761547570160473696887493133544921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0.1975686607970370267661763818978215567767620086669921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.005568770902320334566237836071422862005420029163360595703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00006914772897870683312539219489423203413025476038455963134765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{7790}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0005848009502628661281098398916356018162332475185394287109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.7402269840240478515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.7895585038014587553334422409534454345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{8745}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.7859723567962646484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8048}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.3109095096588134765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.56265981857523339471072176820598542690277099609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7409133911132794736431605997495353221893310546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4131840522715588548408049973659217357635498046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{23696}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1782062053680419921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{12561}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1668965816497802734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{11124}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12181341482369843765010131164672202430665493011474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.005543243141816999765281170908792773843742907047271728515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0000685348800689988824075271622859872877597808837890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{7790}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0005798421645859803789935238427233343827538192272186279296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.0019970381219813998323331372120037485728971660137176513671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.00002887818776034635387156730701452289622466196306049823760986328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00021078435988257601695940179897803545827628113329410552978515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{2654518980387447057635981096571221}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{38385695638587428819910868860928}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{280180472229532455892147020759040}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.94955348968505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.28559200968963427413882527616806328296661376953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.294156372547149658203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{2345}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.23278331756591796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.62018049874634850748833514444413594901561737060546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{2}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1.0198675496688742736495214558090083301067352294921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99998490384082916460073420239496044814586639404296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.999430119991302490234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9977204799652099609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{30684}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00018488943522142233509032716032294274555169977247714996337890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.1395450828192415781980884048607549630105495452880859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{19140088}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{19140088}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{19140088}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{19140088}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{3}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{30684}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{1.0264900662251654761547570160473696887493133544921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0.1975686607970370267661763818978215567767620086669921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00554681996175158086026524273393079056404531002044677734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000068702587837800158966639063606862691813148558139801025390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{7790}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.000581106404456247318569828141932021026150323450565338134765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.1306703090667724609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{29110}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.75341206986382758259424008429050445556640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.663987457752227783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8048}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.35162830352783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.471562362662169665128431006451137363910675048828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.743713855743408203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{12493}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.416193272104326439375654445029795169830322265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{7098}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1849925518035906435443394002504646778106689453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{8299}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{9.18466281890869140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12439024832118317220874814665876328945159912109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.005259044314989799913384604934663002495653927326202392578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000065083203595499237981668316788130823624669574201107025146484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{23367}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00056197779122684637410911623334186515421606600284576416015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.001997038121981500012613874872613450861535966396331787109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.00002888030627243840832429899734279388212598860263824462890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0002107943052235636423839826303350264424807392060756683349609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{2654518980387643023697755735526501}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{38388511624170087361673611444224}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{280193691855206959706569474834432}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.527103424072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.008277795172684676572316675446927547454833984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11130}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.521240711212158203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0976161956787109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6330534395284164173034469058620743453502655029296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{2}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1.0198675496688742736495214558090083301067352294921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9999848900251830929875040965271182358264923095703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99942956864833831787109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99771845340728759765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{30684}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000185053775003251480026078557017399361939169466495513916015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.1395450828192415781980884048607549630105495452880859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18884056}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18884056}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18884056}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{18884056}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{3}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{1.03311258278145690070459750131703913211822509765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0.24188056116224732061681379491346888244152069091796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.005262437753462812124738423591452374239452183246612548828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0000652406666614836045457737068176129469065926969051361083984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{23367}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0005632557254678116111235031127080219448544085025787353515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.9412977695465087890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{27671}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.745584926857844720871071331202983856201171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{9132}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.352285206317901611328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.5144655704498291015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.569275277726438044822998563176952302455902099609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.785877227783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4122358426352992211150194634683430194854736328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.170605123043060302734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1695814132690447451068394002504646778106689453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{8048}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.12439691733200676504456083648619824089109897613525390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.005259047063435699602418349485333237680606544017791748046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0000650903331757645537379575184644409091561101377010345458984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{23367}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.000561977587442704686060412910819650278426706790924072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.001997038121981500012613874872613450861535966396331787109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.00002888030627243840832429899734279388212598860263824462890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0002107943052235636423839826303350264424807392060756683349609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{2654518980387643002667516066788409}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{38388511624170087361673611444224}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{280193691855206887648975436906496}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.37592983245849609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.71346825953350911930783695424906909465789794921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{17096}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.6314566135406494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.5355336666107177734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.542659408581567692664293645066209137439727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{2}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1.0198675496688742736495214558090083301067352294921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9999848904199157839656209034728817641735076904296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9994296133518218994140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99771845340728759765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{30684}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00018505380716989861997721911190950550007983110845088958740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.1395450828192415781980884048607549630105495452880859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18125846}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18125846}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18125846}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{18125846}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{3}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{30684}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{1.0264900662251654761547570160473696887493133544921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0.1975686607970370267661763818978215567767620086669921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00526244050368216732815884739693501614965498447418212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000065247801569504680738349755575455901634995825588703155517578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{23367}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.000563255523722213844416140116067026610835455358028411865234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{178.0778472423553466796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{27671}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.740898064430183467266033403575420379638671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{16149}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.40762770175933837890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.9794495105743408203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.582744912069825371503384303650818765163421630859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.8262412548065203310443394002504646778106689453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{20976}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4114919087744706160947316675446927547454833984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{1951}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1754024028778076171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{9504}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1717503070831298828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{8048}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1260207482785682675530125607110676355659961700439453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0022717938083505000677886354054635376087389886379241943359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000015044992108284924639386749556368982894127839244902133941650390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00018426276924744612920568920255703915245248936116695404052734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.0045563391466543999575034007420981652103364467620849609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.00007121646210196422798442694723775048259994946420192718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.000531694636989736547048879256038844687282107770442962646484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{6056413552023808882558446575730637}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{94662915186687714950032098590720}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{706743396695463544228044844564480}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{130.0746917724609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.1853700852552009337159688584506511688232421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26932}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.2502727508544921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{4729}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.31154632568359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.0252993165004991027444702922366559505462646484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{2}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1.0198675496688742736495214558090083301067352294921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9998952383237169616592154852696694433689117431640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99394276738166820184261496251565404236316680908203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99180799722671519891292746251565404236316680908203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0008106583723621091537581140329393747379072010517120361328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.1395450828192415781980884048607549630105495452880859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17595542}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17595542}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17595542}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17595542}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{7}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{30684}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1.09271523178807949960855694371275603771209716796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0.6646314855785100395024755925987847149372100830078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0022732597006400998874975361019323827349580824375152587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000015054700004242555988411174372476608596116420812904834747314453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00018438166620530704810539124327561921745655126869678497314453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{178.583246707916259765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{27671}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.73304611641839301228174008429050445556640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24173}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{160.192811787128448486328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.473267078399658203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.545219776643310893859961652196943759918212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7814679145813006044818394002504646778106689453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{16284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4087078192376143448427683324553072452545166015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{27671}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.180382907390594482421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{9816}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.17906665802001953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{8048}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1223571706207042530945017233534599654376506805419921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.005259044314989799913384604934663002495653927326202392578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000065083203595499237981668316788130823624669574201107025146484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{23367}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00056197779122684637410911623334186515421606600284576416015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.001997038121981500012613874872613450861535966396331787109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.00002888030627243840832429899734279388212598860263824462890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0002107943052235636423839826303350264424807392060756683349609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{2654518980387643023697755735526501}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{38388511624170087361673611444224}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{280193691855206959706569474834432}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.6324939727783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.049719453647437461540903314016759395599365234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{25516}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{5.53863298892974853515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{18668}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.0751361846923828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{3254}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6428017817939328804044407661422155797481536865234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{2}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1.0198675496688742736495214558090083301067352294921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9999848900251830929875040965271182358264923095703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99942956864833831787109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99771845340728759765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{30684}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000185053775003251480026078557017399361939169466495513916015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.1395450828192415781980884048607549630105495452880859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18892375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18892375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18892375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{18892375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{3}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{1.03311258278145690070459750131703913211822509765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0.24188056116224732061681379491346888244152069091796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.005262437753462812124738423591452374239452183246612548828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0000652406666614836045457737068176129469065926969051361083984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{23367}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0005632557254678116111235031127080219448544085025787353515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{179.3189728260040283203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{27671}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.825213550731831446682917885482311248779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7467}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{160.032291591167421529462444595992565155029296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.5608184337615966796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{12287}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.59583980779116263448713652906008064746856689453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7369453907012939453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{20976}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4056561072141136037316755391657352447509765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{8893}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.16223990917205810546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1546463966369646669818394002504646778106689453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{11124}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1257079916788703399799231874567340128123760223388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.005259047063435699602418349485333237680606544017791748046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0000650903331757645537379575184644409091561101377010345458984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{23367}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.000561977587442704686060412910819650278426706790924072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.001997038121981500012613874872613450861535966396331787109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.00002888030627243840832429899734279388212598860263824462890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0002107943052235636423839826303350264424807392060756683349609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{2654518980387643002667516066788409}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{38388511624170087361673611444224}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{280193691855206887648975436906496}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{6.43523406982421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1681}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{4.72528035277562441507370749604888260364532470703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.649292647838592529296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{8840}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.543451786041260209714209850062616169452667236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.5437849397142382468217647328856401145458221435546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{2}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1.0198675496688742736495214558090083301067352294921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9999848904199157839656209034728817641735076904296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9994296133518218994140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99771845340728759765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{30684}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00018505380716989861997721911190950550007983110845088958740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.1395450828192415781980884048607549630105495452880859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{18150803}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18150803}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18150803}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{18150803}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{3}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{30684}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{1.0264900662251654761547570160473696887493133544921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0.1975686607970370267661763818978215567767620086669921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00526244050368216732815884739693501614965498447418212890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000065247801569504680738349755575455901634995825588703155517578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{23367}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.000563255523722213844416140116067026610835455358028411865234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{179.535578250885009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{27671}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.880336477267036343619110994040966033935546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.78183615207672119140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.6993124485015869140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.60743444083324593663064661086536943912506103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7293965816497802734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4098640940836730806040577590465545654296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{16149}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.152956306934356689453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1093616485595703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.11918436792671606438975828723414451815187931060791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0022717938083505000677886354054635376087389886379241943359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000015044992108284924639386749556368982894127839244902133941650390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00018426276924744612920568920255703915245248936116695404052734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.0045563391466543999575034007420981652103364467620849609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.00007121646210196422798442694723775048259994946420192718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.000531694636989736547048879256038844687282107770442962646484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{6056413552023808882558446575730637}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{94662915186687714950032098590720}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{706743396695463544228044844564480}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{132.0067138671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.2142638654898263439463335089385509490966796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{29725}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{77.3510417938232421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{72.464385986328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.1318176320167747661571411299519240856170654296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{2}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1.0198675496688742736495214558090083301067352294921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9998952383237169616592154852696694433689117431640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99394276738166820184261496251565404236316680908203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99180799722671519891292746251565404236316680908203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0008106583723621091537581140329393747379072010517120361328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.1395450828192415781980884048607549630105495452880859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17607829}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17607829}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17607829}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17607829}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{7}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{30684}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1.09271523178807949960855694371275603771209716796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0.6646314855785100395024755925987847149372100830078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0022732597006400998874975361019323827349580824375152587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000015054700004242555988411174372476608596116420812904834747314453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00018438166620530704810539124327561921745655126869678497314453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{179.0413391590118408203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{27671}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.839426380119590476169832982122898101806640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4810}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.5635316371917724609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{12287}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.8720653057098388671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.6553251898304193190369915100745856761932373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.75654125213623046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{20976}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4131050062495358332625983166508376598358154296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{7238}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.2213490009307861328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1944324970245361328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{12561}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.11859405760008683017314723429080913774669170379638671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0022717938083505000677886354054635376087389886379241943359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000015044992108281506014411631200200503144515096209943294525146484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00018426276924744645446634094820836935468832962214946746826171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.0045563391471476998029199734219218953512609004974365234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.0000712164621052311188655059570606908891932107508182525634765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00053169463701729425576802956499022911884821951389312744140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{6056413552679602896583270012595245}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{94662915191030734229089072185344}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{706743396732099786764748545064960}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{133.0085601806640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{1490}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.14101647383330373486387543380260467529296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{20976}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.9849071502685546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{1895}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{74.71254730224609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{13468}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{9.3554099191410902136567528941668570041656494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{2}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1.0198675496688742736495214558090083301067352294921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9998952383237169616592154852696694433689117431640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99394276738166820184261496251565404236316680908203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99180799722671519891292746251565404236316680908203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0008106583723621091537581140329393747379072010517120361328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.1395450828192415781980884048607549630105495452880859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{17622259}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{17622259}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17622259}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{17622259}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{7}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{30684}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1.0993377483443709241583974289824254810810089111328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0.70715329779921665132036423528916202485561370849609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0022732597006400998874975361019323827349580824375152587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000015054700004239120422777110930301347480053664185106754302978515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00018438166620530737336604298892694941969239152967929840087890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{178.953218936920166015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{27671}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.856419879079652446307591162621974945068359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{17096}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.198956429958343505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{8048}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.611385822296142578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.633330385195443934520653783692978322505950927734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.71787548065185546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{7790}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4137832202658753288915249868296086788177490234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{23241}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.188022911548614501953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{12561}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1759130954742431640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{11124}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1215216776916894503290933471362222917377948760986328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00454358776419520014877573288458734168671071529388427734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000057436563648282639858895504136881982049089856445789337158203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{23367}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00049632702677324222646781937129389916663058102130889892578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.0022273197242424999132970331316982992575503885746002197265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.0000347928585312350989000411416451896684520761482417583465576171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.000255366217850433257184616930857146144262515008449554443359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{2960615733027188284143932923177060}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{46247641613103516727644644179968}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{339439925944519945584257831796736}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{25.76837158203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20415}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{10.67154272344728127563939779065549373626708984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{26829}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.5517799854278564453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{6.40165996551513671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.83292431082238493900149478577077388763427734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{2}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1.0198675496688742736495214558090083301067352294921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.999967430995789552383712361915968358516693115234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99762983620166789666683371251565404236316680908203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{30684}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99736344814300537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.000281856110152137553405415903995390181080438196659088134765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.1395450828192415781980884048607549630105495452880859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20090425}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{20090425}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{20090425}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{20090425}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{3}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{1.03311258278145690070459750131703913211822509765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0.24188056116224732061681379491346888244152069091796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.00456382295516236623222905421926043345592916011810302734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{3284}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0000575882172242804112223535373260574488085694611072540283203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{23367}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000008390328334253362262575762310148895442151117219222008762738004108305928123260677973087339788504923632217469275929033756256103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00049768395022339374268727230088416035869158804416656494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{176.5729522705078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.707924545995439302714657969772815704345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{9132}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.631608307361602783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{17197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{158.8928458690643310546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{6549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.487542367056743586317679728381335735321044921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7493402957916259765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{20754}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4158705922941496879730038926936686038970947265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{15399}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.1920194029808026670025355997495353221893310546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{11124}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1898634433746337890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{9504}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.120745680489295015291872914531268179416656494140625}
\def\SubcubicEffectiveDimensionalityEstimateLen{7852}
\def\SubcubicEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicEffectiveDimensionalityEstimateMeanFloat{5662.76923076923048938624560832977294921875}
\def\SubcubicEffectiveDimensionalityEstimateMedianFloat{4290}
\def\SubcubicEffectiveDimensionalityEstimateMinFloat{4290}
\def\SubcubicEffectiveDimensionalityEstimateStdDevFloat{2046.997581970168312182067893445491790771484375}
\def\SubcubicErrUpperBoundLen{7852}
\def\SubcubicErrUpperBoundMaxFloat{133.0085601806640625}
\def\SubcubicErrUpperBoundMeanFloat{25.1094553102599178373566246591508388519287109375}
\def\SubcubicErrUpperBoundMedianFloat{0}
\def\SubcubicErrUpperBoundMinFloat{0}
\def\SubcubicErrUpperBoundStdDevFloat{38.5922816993990380751711199991405010223388671875}
\def\SubcubicGapMostBelowValueLen{7852}
\def\SubcubicGapMostBelowValueMaxFloat{40}
\def\SubcubicGapMostBelowValueMeanFloat{4.4174732552215996150835053413175046443939208984375}
\def\SubcubicGapMostBelowValueMedianFloat{1}
\def\SubcubicGapMostBelowValueMinFloat{1}
\def\SubcubicGapMostBelowValueNumStdLen{7852}
\def\SubcubicGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicGapMostBelowValueSequenceFracLen{7852}
\def\SubcubicGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicGapMostBelowValueSequenceFracMeanFloat{0.9926952140873570584744811640121042728424072265625}
\def\SubcubicGapMostBelowValueSequenceFracMedianFloat{0.947287954986095304121818116982467472553253173828125}
\def\SubcubicGapMostBelowValueSequenceFracMinFloat{0.893912732601165771484375}
\def\SubcubicGapMostBelowValueSequenceFracStdDevFloat{0.00985661597920427061392256717908821883611381053924560546875}
\def\SubcubicGapMostBelowValueStdDevFloat{3.3770434026414957173756192787550389766693115234375}
\def\SubcubicGroupAccuracyLen{1208}
\def\SubcubicGroupAccuracyMaxFloat{0.65682941314196041648898471976281143724918365478515625}
\def\SubcubicGroupAccuracyMeanFloat{0.50138156684952395192311769278603605926036834716796875}
\def\SubcubicGroupAccuracyMedianFloat{0.12713812915624977950557195072178728878498077392578125}
\def\SubcubicGroupAccuracyMinFloat{0.0000000000000000000000000000000000105324293833676960713998793735113212732552433886779041927184152882546186447143555}
\def\SubcubicGroupAccuracyStdDevFloat{0.08303036184035962607996594897485920228064060211181640625}
\def\SubcubicGroupDroppedSequencesFracLen{1208}
\def\SubcubicGroupDroppedSequencesFracMaxFloat{0.277196216846553877832803891578805632889270782470703125}
\def\SubcubicGroupDroppedSequencesFracMeanFloat{0.1446337946453406797520102600174141116440296173095703125}
\def\SubcubicGroupDroppedSequencesFracMedianFloat{0.047708007996685099227907045360552729107439517974853515625}
\def\SubcubicGroupDroppedSequencesFracMinFloat{0.0194035467813012986459941799921580241061747074127197265625}
\def\SubcubicGroupDroppedSequencesFracStdDevFloat{0.04008603278638227240815439245125162415206432342529296875}
\def\SubcubicGroupDroppedSequencesLen{1208}
\def\SubcubicGroupDroppedSequencesMaxFloat{368456971758105744654572774052511778}
\def\SubcubicGroupDroppedSequencesMeanFloat{192251288979193694842508871892729856}
\def\SubcubicGroupDroppedSequencesMedianFloat{63414819852324510727794969599279104}
\def\SubcubicGroupDroppedSequencesMinFloat{25791737599227993675588937989004610}
\def\SubcubicGroupDroppedSequencesStdDevFloat{53283477019611288555548570978091008}
\def\SubcubicGroupEffectiveDimensionalityEstimateLen{1208}
\def\SubcubicGroupEffectiveDimensionalityEstimateMaxFloat{8384}
\def\SubcubicGroupEffectiveDimensionalityEstimateMeanFloat{6401}
\def\SubcubicGroupEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicGroupEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicGroupEffectiveDimensionalityEstimateStdDevFloat{1921.033315692364567439653910696506500244140625}
\def\SubcubicGroupErrUpperBoundLen{1208}
\def\SubcubicGroupErrUpperBoundMaxFloat{4.94955348968505859375}
\def\SubcubicGroupErrUpperBoundMeanFloat{1.142796004844817137069412638084031641483306884765625}
\def\SubcubicGroupErrUpperBoundMedianFloat{0}
\def\SubcubicGroupErrUpperBoundMinFloat{0}
\def\SubcubicGroupErrUpperBoundStdDevFloat{1.2240484607244559445149434395716525614261627197265625}
\def\SubcubicGroupGapMostBelowValueLen{1208}
\def\SubcubicGroupGapMostBelowValueMaxFloat{6}
\def\SubcubicGroupGapMostBelowValueMeanFloat{2.96937086092715230023486583377234637737274169921875}
\def\SubcubicGroupGapMostBelowValueMedianFloat{2}
\def\SubcubicGroupGapMostBelowValueMinFloat{2}
\def\SubcubicGroupGapMostBelowValueNumStdLen{1208}
\def\SubcubicGroupGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicGroupGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicGroupGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicGroupGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicGroupGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicGroupGapMostBelowValueSequenceFracLen{1208}
\def\SubcubicGroupGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicGroupGapMostBelowValueSequenceFracMeanFloat{0.991764761507511138916015625}
\def\SubcubicGroupGapMostBelowValueSequenceFracMedianFloat{0.93917370796203603067198173448559828102588653564453125}
\def\SubcubicGroupGapMostBelowValueSequenceFracMinFloat{0.89577758312225341796875}
\def\SubcubicGroupGapMostBelowValueSequenceFracStdDevFloat{0.01126001454382232445927680686281746602617204189300537109375}
\def\SubcubicGroupGapMostBelowValueStdDevFloat{0.538167975400748677117235274636186659336090087890625}
\def\SubcubicGroupInstructionCountBranchLen{1208}
\def\SubcubicGroupInstructionCountBranchMaxFloat{0}
\def\SubcubicGroupInstructionCountBranchMeanFloat{0}
\def\SubcubicGroupInstructionCountBranchMedianFloat{0}
\def\SubcubicGroupInstructionCountBranchMinFloat{0}
\def\SubcubicGroupInstructionCountBranchStdDevFloat{0}
\def\SubcubicGroupInstructionCountIntLen{1208}
\def\SubcubicGroupInstructionCountIntMaxFloat{0}
\def\SubcubicGroupInstructionCountIntMeanFloat{0}
\def\SubcubicGroupInstructionCountIntMedianFloat{0}
\def\SubcubicGroupInstructionCountIntMinFloat{0}
\def\SubcubicGroupInstructionCountIntStdDevFloat{0}
\def\SubcubicGroupInstructionCountLen{1208}
\def\SubcubicGroupInstructionCountMaxFloat{19406487}
\def\SubcubicGroupInstructionCountMeanFloat{18671767}
\def\SubcubicGroupInstructionCountMedianFloat{17937047}
\def\SubcubicGroupInstructionCountMinFloat{17937047}
\def\SubcubicGroupInstructionCountStdDevFloat{626326.019003282301127910614013671875}
\def\SubcubicGroupMaxGapLen{1208}
\def\SubcubicGroupMaxGapMaxFloat{50}
\def\SubcubicGroupMaxGapMeanFloat{33.302980132450329620041884481906890869140625}
\def\SubcubicGroupMaxGapMedianFloat{3}
\def\SubcubicGroupMaxGapMinFloat{3}
\def\SubcubicGroupMaxGapStdDevFloat{16.95360608633841792425300809554755687713623046875}
\def\SubcubicGroupNormalizedAccuracyLen{1208}
\def\SubcubicGroupNormalizedAccuracyMaxFloat{0.6572436982471929756144390921690501272678375244140625}
\def\SubcubicGroupNormalizedAccuracyMeanFloat{0.50325263562791155980136181824491359293460845947265625}
\def\SubcubicGroupNormalizedAccuracyMedianFloat{0.14701098875105156338349843281321227550506591796875}
\def\SubcubicGroupNormalizedAccuracyMinFloat{0.000000000000000000000000000000000011181575482347337861056731119226272875001609849420949822953073647966407680182923061018343525128970750159851377247832715511322021484375}
\def\SubcubicGroupNormalizedAccuracyStdDevFloat{0.0822806078697621845474685642329859547317028045654296875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.65682941314196041648898471976281143724918365478515625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMaxKey{27671}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.56023581183526671711803146536112762987613677978515625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMeanKey{18668}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.418750827571347017386216293743927963078022003173828125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMedianKey{3254}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMinFloat{0.25265074475171689361019389252760447561740875244140625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.043459079876688989918509520293810055591166019439697265625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2103768601571602003819094761638552881777286529541015625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.128322292726034403731460997732938267290592193603515625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{30371}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.040127874711301948773556347305202507413923740386962890625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.02845918004020230041017924804691574536263942718505859375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.036988353308259287743897658629066427238285541534423828125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{279638812186225580210403332546392172}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{170569583974752072968039860539490304}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{30371}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{53339094477612218918499665515118592}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{37828738846520300492525058542808020}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49165954735321846388803879919681536}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{8384}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{519}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{7383.033112582781541277654469013214111328125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{2743}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{3254}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{3254}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{1683.247442459349485943675972521305084228515625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{3.428576946258544921875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{8048}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0.554284117869193959649010139401070773601531982421875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{519}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{519}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMinKey{519}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.96826607180485113612888881107210181653499603271484375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{2.867549668874172397181609994731843471527099609375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{913}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{913}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99989861249923717156917746251565404236316680908203125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{22261}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99320019475671628139679114610771648585796356201171875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29725}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9595743119716644287109375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20754}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95257580280303955078125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{22286}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0087876393975257517665600204281872720457613468170166015625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.571688525957807502919649778050370514392852783203125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMaxFloat{19406487}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMaxKey{3254}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18485505.993377484381198883056640625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMeanKey{2743}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18166871}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMedianKey{519}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMinFloat{18166871}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMinKey{519}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{539100.60093087726272642612457275390625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMaxFloat{49}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMaxKey{1895}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMeanFloat{39.3774834437086127536531421355903148651123046875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMeanKey{7310}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapStdDevFloat{12.4393850712851818940407611080445349216461181640625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6572436982471929756144390921690501272678375244140625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27671}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.5625726369511718782945308703347109258174896240234375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{11130}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.430216153043765370256323876674287021160125732421875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{3254}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.297203989016589786853472787697683088481426239013671875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.040843438294592006310157472626087837852537631988525390625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.77167415618896484375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.802803170602061300087370909750461578369140625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1185}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.964951336383819580078125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.6911551952362060546875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8048}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.188206915657020079635231013526208698749542236328125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.8180291652679443359375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.4418798345603693888961061020381748676300048828125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMeanKey{17197}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.233568251132965087890625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMedianKey{20338}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2120714187622088076068394002504646778106689453125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.11958670889127175074317932512713014148175716400146484375}
\def\SubcubicGroupProofSearchTimeLen{1208}
\def\SubcubicGroupProofSearchTimeMaxFloat{176.471160411834716796875}
\def\SubcubicGroupProofSearchTimeMeanFloat{167.163818837001628025973332114517688751220703125}
\def\SubcubicGroupProofSearchTimeMedianFloat{158.45990373492242042630095966160297393798828125}
\def\SubcubicGroupProofSearchTimeMinFloat{157.5163447856903076171875}
\def\SubcubicGroupProofSearchTimeStdDevFloat{3.298103233462530425867953454144299030303955078125}
\def\SubcubicGroupProofTimeLen{1208}
\def\SubcubicGroupProofTimeMaxFloat{9.848197460174560546875}
\def\SubcubicGroupProofTimeMeanFloat{9.4121231255152366657057427801191806793212890625}
\def\SubcubicGroupProofTimeMedianFloat{9.1598867154121403899580400320701301097869873046875}
\def\SubcubicGroupProofTimeMinFloat{9.09371185302734375}
\def\SubcubicGroupProofTimeStdDevFloat{0.1236932818705859526975388007485889829695224761962890625}
\def\SubcubicInstructionCountBranchLen{7852}
\def\SubcubicInstructionCountBranchMaxFloat{0}
\def\SubcubicInstructionCountBranchMeanFloat{0}
\def\SubcubicInstructionCountBranchMedianFloat{0}
\def\SubcubicInstructionCountBranchMinFloat{0}
\def\SubcubicInstructionCountBranchStdDevFloat{0}
\def\SubcubicInstructionCountIntLen{7852}
\def\SubcubicInstructionCountIntMaxFloat{0}
\def\SubcubicInstructionCountIntMeanFloat{0}
\def\SubcubicInstructionCountIntMedianFloat{0}
\def\SubcubicInstructionCountIntMinFloat{0}
\def\SubcubicInstructionCountIntStdDevFloat{0}
\def\SubcubicInstructionCountLen{7852}
\def\SubcubicInstructionCountMaxFloat{20356824}
\def\SubcubicInstructionCountMeanFloat{18517240.5769230760633945465087890625}
\def\SubcubicInstructionCountMedianFloat{17623862}
\def\SubcubicInstructionCountMinFloat{17623862}
\def\SubcubicInstructionCountStdDevFloat{759215.836297211819328367710113525390625}
\def\SubcubicMaxGapLen{7852}
\def\SubcubicMaxGapMaxFloat{59}
\def\SubcubicMaxGapMeanFloat{34.6413652572592951628394075669348239898681640625}
\def\SubcubicMaxGapMedianFloat{1}
\def\SubcubicMaxGapMinFloat{1}
\def\SubcubicMaxGapStdDevFloat{18.39744219554213344736126600764691829681396484375}
\def\SubcubicNormalizedAccuracyLen{7852}
\def\SubcubicNormalizedAccuracyMaxFloat{0.6572436982471929756144390921690501272678375244140625}
\def\SubcubicNormalizedAccuracyMeanFloat{0.380800445327400816086793611248140223324298858642578125}
\def\SubcubicNormalizedAccuracyMedianFloat{0.000000000000000000000000000000000010603759289806756996005685292842941274793052395865431894415332660316507490478454630333893606887463167964824606315232813358306884765625}
\def\SubcubicNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicNormalizedAccuracyStdDevFloat{0.1702880802137879678870291400016867555677890777587890625}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.65682941314196041648898471976281143724918365478515625}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMaxKey{27671}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.56121004634953008949338482125313021242618560791015625}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMeanKey{7098}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.4200645042537107798352735699154436588287353515625}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMinFloat{0.25265074475171689361019389252760447561740875244140625}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.042968392297698144999262837018250138498842716217041015625}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.23052385661848628917169889973592944443225860595703125}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{27300}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.13407621728723950749184723463258706033229827880859375}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12457}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.04783335998494049612350664801851962693035602569580078125}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18289}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.02845918004020230041017924804691574536263942718505859375}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.039519286610340993715073665271120262332260608673095703125}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{306418763913599937668037273980403551}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{27300}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{178217861587140260755829682832670720}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12457}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{63581441224440886256543766388146176}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18289}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{37828738846520300492525058542808020}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{52530142135913202241742431210962944}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{104}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{7383.9735099337749488768167793750762939453125}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{1185}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4400.5}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{6910}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{8840}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{1820.64069920170322802732698619365692138671875}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{9.1559906005859375}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4157}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0.991665388574663353438154445029795169830322265625}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{3254}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{104}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinKey{104}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.9653311092506668966706229184637777507305145263671875}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{24438}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{2.867549668874172397181609994731843471527099609375}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999849796295166015625}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{31308}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.992647306019107222851971528143621981143951416015625}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4810}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9595743119716644287109375}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20754}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95257580280303955078125}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{22286}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00910800686383549627789246727616045973263680934906005859375}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.571688525957807502919649778050370514392852783203125}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20348569}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMaxKey{6910}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18476152.19867549836635589599609375}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMeanKey{7467}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMedianFloat{17910775}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMedianKey{104}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMinFloat{17910775}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMinKey{104}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{568715.6135063879191875457763671875}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMaxFloat{49}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMaxKey{1185}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMeanFloat{39.35761589403973204071007785387337207794189453125}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMeanKey{7310}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapStdDevFloat{12.4960096257843193967573824920691549777984619140625}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6572436982471929756144390921690501272678375244140625}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27671}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.56354892045871152195246622795821167528629302978515625}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{18668}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.43815901059012152263250072792288847267627716064453125}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{3254}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.297203989016589786853472787697683088481426239013671875}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0402918483747694844421260995659395121037960052490234375}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{175.77167415618896484375}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.857632138081726225209422409534454345703125}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1490}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{159.964951336383819580078125}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{123}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{159.6911551952362060546875}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinKey{8048}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{3.251991228210260320707902792491950094699859619140625}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.8180291652679443359375}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.44202332780850639437630889005959033966064453125}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMeanKey{17197}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.236496508121490478515625}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMedianKey{9816}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMinFloat{9.2120714187622088076068394002504646778106689453125}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1194509288843590144590933732615667395293712615966796875}
\def\SubcubicProofSearchTimeLen{7852}
\def\SubcubicProofSearchTimeMaxFloat{178.8347589969635009765625}
\def\SubcubicProofSearchTimeMeanFloat{167.072172615762525538229965604841709136962890625}
\def\SubcubicProofSearchTimeMedianFloat{158.550662606954546163251507095992565155029296875}
\def\SubcubicProofSearchTimeMinFloat{52.930239200592041015625}
\def\SubcubicProofSearchTimeStdDevFloat{4.1969070831178356684176833368837833404541015625}
\def\SubcubicProofTimeLen{7852}
\def\SubcubicProofTimeMaxFloat{9.88440799713134765625}
\def\SubcubicProofTimeMeanFloat{9.411105605423966125044898944906890392303466796875}
\def\SubcubicProofTimeMedianFloat{9.16583435893058862120597041212022304534912109375}
\def\SubcubicProofTimeMinFloat{9.0863430500030517578125}
\def\SubcubicProofTimeStdDevFloat{0.123656346995618615647316573813441209495067596435546875}
\def\SubcubicVocabModelSquaredAccuracyLen{7248}
\def\SubcubicVocabModelSquaredAccuracyMaxFloat{0.6064075623937725811885002258350141346454620361328125}
\def\SubcubicVocabModelSquaredAccuracyMeanFloat{0.18356898259270193474179677650681696832180023193359375}
\def\SubcubicVocabModelSquaredAccuracyMedianFloat{0.00000000000000000000000000000000000902779661431516806119989660586684680564735147600963216518721310421824455261230469}
\def\SubcubicVocabModelSquaredAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicVocabModelSquaredAccuracyStdDevFloat{0.1853095164037680542268304861863725818693637847900390625}
\def\SubcubicVocabModelSquaredDroppedSequencesFracLen{7248}
\def\SubcubicVocabModelSquaredDroppedSequencesFracMaxFloat{0.51102902901206170849235377318109385669231414794921875}
\def\SubcubicVocabModelSquaredDroppedSequencesFracMeanFloat{0.1761495727129700206159412800843711011111736297607421875}
\def\SubcubicVocabModelSquaredDroppedSequencesFracMedianFloat{0}
\def\SubcubicVocabModelSquaredDroppedSequencesFracMinFloat{0}
\def\SubcubicVocabModelSquaredDroppedSequencesFracStdDevFloat{0.15655540581590254856081401158007793128490447998046875}
\def\SubcubicVocabModelSquaredDroppedSequencesLen{7248}
\def\SubcubicVocabModelSquaredDroppedSequencesMaxFloat{679274092021614382013061870951284366}
\def\SubcubicVocabModelSquaredDroppedSequencesMeanFloat{234142943495630151478164610336423936}
\def\SubcubicVocabModelSquaredDroppedSequencesMedianFloat{0}
\def\SubcubicVocabModelSquaredDroppedSequencesMinFloat{0}
\def\SubcubicVocabModelSquaredDroppedSequencesStdDevFloat{208097828301969700953589408210092032}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateLen{7248}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateMeanFloat{6468.6666666666669698315672576427459716796875}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateMedianFloat{6338}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateMinFloat{6338}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateStdDevFloat{53.7979760048853705711735528893768787384033203125}
\def\SubcubicVocabModelSquaredErrUpperBoundLen{7248}
\def\SubcubicVocabModelSquaredErrUpperBoundMaxFloat{133.0085601806640625}
\def\SubcubicVocabModelSquaredErrUpperBoundMeanFloat{40.088617376144355830547283403575420379638671875}
\def\SubcubicVocabModelSquaredErrUpperBoundMedianFloat{3.836799144744873046875}
\def\SubcubicVocabModelSquaredErrUpperBoundMinFloat{3.5355336666107177734375}
\def\SubcubicVocabModelSquaredErrUpperBoundStdDevFloat{42.8474577044930100555575336329638957977294921875}
\def\SubcubicVocabModelSquaredGapMostBelowValueLen{7248}
\def\SubcubicVocabModelSquaredGapMostBelowValueMaxFloat{34}
\def\SubcubicVocabModelSquaredGapMostBelowValueMeanFloat{3.646523178807946852231225420837290585041046142578125}
\def\SubcubicVocabModelSquaredGapMostBelowValueMedianFloat{1}
\def\SubcubicVocabModelSquaredGapMostBelowValueMinFloat{1}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdLen{7248}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracLen{7248}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracMeanFloat{0.9932691138607776526470161115867085754871368408203125}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracMedianFloat{0.9503321337699890403172275910037569701671600341796875}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracMinFloat{0.8931427001953125}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracStdDevFloat{0.00988053421651583461959855725353918387554585933685302734375}
\def\SubcubicVocabModelSquaredGapMostBelowValueStdDevFloat{2.86478756267616940789366708486340939998626708984375}
\def\SubcubicVocabModelSquaredInstructionCountBranchLen{7248}
\def\SubcubicVocabModelSquaredInstructionCountBranchMaxFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountBranchMeanFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountBranchMedianFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountBranchMinFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountBranchStdDevFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntLen{7248}
\def\SubcubicVocabModelSquaredInstructionCountIntMaxFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntMeanFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntMedianFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntMinFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntStdDevFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountLen{7248}
\def\SubcubicVocabModelSquaredInstructionCountMaxFloat{20092473}
\def\SubcubicVocabModelSquaredInstructionCountMeanFloat{18257595.2083333320915699005126953125}
\def\SubcubicVocabModelSquaredInstructionCountMedianFloat{17365718}
\def\SubcubicVocabModelSquaredInstructionCountMinFloat{17365718}
\def\SubcubicVocabModelSquaredInstructionCountStdDevFloat{825385.628847307409159839153289794921875}
\def\SubcubicVocabModelSquaredMaxGapLen{7248}
\def\SubcubicVocabModelSquaredMaxGapMaxFloat{63}
\def\SubcubicVocabModelSquaredMaxGapMeanFloat{25.107477924944813452157177380286157131195068359375}
\def\SubcubicVocabModelSquaredMaxGapMedianFloat{1}
\def\SubcubicVocabModelSquaredMaxGapMinFloat{1}
\def\SubcubicVocabModelSquaredMaxGapStdDevFloat{21.6186445914230063181094010360538959503173828125}
\def\SubcubicVocabModelSquaredNormalizedAccuracyLen{7248}
\def\SubcubicVocabModelSquaredNormalizedAccuracyMaxFloat{0.6067446714283786235455409041605889797210693359375}
\def\SubcubicVocabModelSquaredNormalizedAccuracyMeanFloat{0.18432421632232109942606257391162216663360595703125}
\def\SubcubicVocabModelSquaredNormalizedAccuracyMedianFloat{0.00000000000000000000000000000000000918701489667776217044949118979087388873213108951222041500396842134538477567709204720146289220583657453289561090059578418731689453125}
\def\SubcubicVocabModelSquaredNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicVocabModelSquaredNormalizedAccuracyStdDevFloat{0.1859400690868072414385636648148647509515285491943359375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6064075623937725811885002258350141346454620361328125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5259578695325901609436414219089783728122711181640625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMeanKey{30684}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.3847055762794624467204585016588680446147918701171875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMinFloat{0.238996153214439510659161669536842964589595794677734375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.041246108155878986878395409121367265470325946807861328125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.261200279071756080728761162390583194792270660400390625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1667996060247548817390139674898819066584110260009765625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{11498}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.04608553246768244682218806929085985757410526275634765625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0300437945554398004588403381376338074915111064910888671875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037539975911930707763719539116209489293396472930908203125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{347194723449011078610315099327629011}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{221714706013998620863807684704468992}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{11498}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{61258179956698243924747025463115776}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{39935052822701027664841858754564702}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49899186943229664998028801826881536}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{123}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6489.7350993377485792734660208225250244140625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6450}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{7310}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{31.7796015184623001914587803184986114501953125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.6324939727783203125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.27478027659536241600335415569134056568145751953125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{27584}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.783549010753631147707665149937383830547332763671875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32103}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.6634309291839599609375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinKey{8840}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.738326613671914433467691196710802614688873291015625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.125827814569536400313154445029795169830322265625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99969160556793201788394753748434595763683319091796875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{29022}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99037608089825968082919871449121274054050445556640625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7790}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93811319768428802490234375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.893275201320648193359375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01112124686773548198903682759919320233166217803955078125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.435276204639867103640682444165577180683612823486328125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20092473}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMaxKey{7310}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18269403.099337749183177947998046875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMeanKey{123}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18127894}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMinFloat{18127894}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{313338.1599132127012126147747039794921875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMaxKey{2306}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMeanFloat{36.68874172185430637682657106779515743255615234375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMeanKey{29725}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.08395289175145848048487096093595027923583984375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6067446714283786235455409041605889797210693359375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.52814679443530021529795703827403485774993896484375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{27584}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.400933579659400962658111211567302234470844268798828125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6204}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.28114150292631900907025510605308227241039276123046875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03874858981339181218661593675278709270060062408447265625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.7373340129852294921875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.602082707234558256459422409534454345703125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{13468}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.731911599636077880859375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{51.602179050445556640625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.0699252308332294347792412736453115940093994140625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7576975822448712705181605997495353221893310546875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.443167899618085669999345554970204830169677734375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMeanKey{30684}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.20833241939544677734375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMedianKey{9816}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1634089946746843935443394002504646778106689453125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1283144310823415568112437767922529019415378570556640625}
\def\SubcubicVocabModelSquaredProofSearchTimeLen{7248}
\def\SubcubicVocabModelSquaredProofSearchTimeMaxFloat{179.535578250885009765625}
\def\SubcubicVocabModelSquaredProofSearchTimeMeanFloat{167.0327590990474391219322569668292999267578125}
\def\SubcubicVocabModelSquaredProofSearchTimeMedianFloat{157.924977246522900031777680851519107818603515625}
\def\SubcubicVocabModelSquaredProofSearchTimeMinFloat{51.5117042064666748046875}
\def\SubcubicVocabModelSquaredProofSearchTimeStdDevFloat{6.31114297473808338878598078736104071140289306640625}
\def\SubcubicVocabModelSquaredProofTimeLen{7248}
\def\SubcubicVocabModelSquaredProofTimeMaxFloat{9.8397514820098876953125}
\def\SubcubicVocabModelSquaredProofTimeMeanFloat{9.4027103175127475509498253813944756984710693359375}
\def\SubcubicVocabModelSquaredProofTimeMedianFloat{9.1556853044033044142224753159098327159881591796875}
\def\SubcubicVocabModelSquaredProofTimeMinFloat{9.0864479541778564453125}
\def\SubcubicVocabModelSquaredProofTimeStdDevFloat{0.125440466582730392186562085043988190591335296630859375}
\def\SubcubicWithoutVocabSquaredAccuracyLen{4530}
\def\SubcubicWithoutVocabSquaredAccuracyMaxFloat{0.6064075623937725811885002258350141346454620361328125}
\def\SubcubicWithoutVocabSquaredAccuracyMeanFloat{0.213804944499108862121516949628130532801151275634765625}
\def\SubcubicWithoutVocabSquaredAccuracyMedianFloat{0.00000000000000000000000000000000000902779661431516806119989660586684680564735147600963216518721310421824455261230469}
\def\SubcubicWithoutVocabSquaredAccuracyMinFloat{0.0000000000000000000000000000000000082754802297889040560999052220446095718434055196754961514216120122000575065612793}
\def\SubcubicWithoutVocabSquaredAccuracyStdDevFloat{0.2062285163424837641787945585747365839779376983642578125}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracLen{4530}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracMaxFloat{0.3752746673646409902858067653141915798187255859375}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracMeanFloat{0.12126071017211335900665147846666513942182064056396484375}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracMedianFloat{0}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracMinFloat{0}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracStdDevFloat{0.09315981819434815403013772083795629441738128662109375}
\def\SubcubicWithoutVocabSquaredDroppedSequencesLen{4530}
\def\SubcubicWithoutVocabSquaredDroppedSequencesMaxFloat{498825593969952824523070029421222213}
\def\SubcubicWithoutVocabSquaredDroppedSequencesMeanFloat{161183130749534004192991260446818304}
\def\SubcubicWithoutVocabSquaredDroppedSequencesMedianFloat{0}
\def\SubcubicWithoutVocabSquaredDroppedSequencesMinFloat{0}
\def\SubcubicWithoutVocabSquaredDroppedSequencesStdDevFloat{123830638426161588595420081898389504}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateLen{4530}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateMeanFloat{6457.4666666666662422358058393001556396484375}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateMedianFloat{6338}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateMinFloat{6338}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateStdDevFloat{56.60372975539882389739432255737483501434326171875}
\def\SubcubicWithoutVocabSquaredErrUpperBoundLen{4530}
\def\SubcubicWithoutVocabSquaredErrUpperBoundMaxFloat{25.76837158203125}
\def\SubcubicWithoutVocabSquaredErrUpperBoundMeanFloat{7.23365771691530756726251638610847294330596923828125}
\def\SubcubicWithoutVocabSquaredErrUpperBoundMedianFloat{3.6845729351043701171875}
\def\SubcubicWithoutVocabSquaredErrUpperBoundMinFloat{3.5355336666107177734375}
\def\SubcubicWithoutVocabSquaredErrUpperBoundStdDevFloat{2.818143393080390968208348567713983356952667236328125}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueLen{4530}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueMaxFloat{9}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueMeanFloat{2.481015452538631205214869623887352645397186279296875}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueMedianFloat{1}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueMinFloat{1}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdLen{4530}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracLen{4530}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracMeanFloat{0.99160490203114270979511957193608395755290985107421875}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracMedianFloat{0.94176664024591449919654451150563545525074005126953125}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracMinFloat{0.8931427001953125}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracStdDevFloat{0.01142611030017413875636833608950837515294551849365234375}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueStdDevFloat{1.1424835780135025320447539343149401247501373291015625}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchLen{4530}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchMaxFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchMeanFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchMedianFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchMinFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntLen{4530}
\def\SubcubicWithoutVocabSquaredInstructionCountIntMaxFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntMeanFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntMedianFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntMinFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountLen{4530}
\def\SubcubicWithoutVocabSquaredInstructionCountMaxFloat{20092473}
\def\SubcubicWithoutVocabSquaredInstructionCountMeanFloat{18715154.3333333320915699005126953125}
\def\SubcubicWithoutVocabSquaredInstructionCountMedianFloat{17896022}
\def\SubcubicWithoutVocabSquaredInstructionCountMinFloat{17896022}
\def\SubcubicWithoutVocabSquaredInstructionCountStdDevFloat{723691.281550880405120551586151123046875}
\def\SubcubicWithoutVocabSquaredMaxGapLen{4530}
\def\SubcubicWithoutVocabSquaredMaxGapMaxFloat{52}
\def\SubcubicWithoutVocabSquaredMaxGapMeanFloat{21.915011037527595050278250710107386112213134765625}
\def\SubcubicWithoutVocabSquaredMaxGapMedianFloat{1}
\def\SubcubicWithoutVocabSquaredMaxGapMinFloat{1}
\def\SubcubicWithoutVocabSquaredMaxGapStdDevFloat{20.27100213181712007326495950110256671905517578125}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyLen{4530}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyMaxFloat{0.6067446714283786235455409041605889797210693359375}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyMeanFloat{0.2146696848810800972717771628595073707401752471923828125}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyMedianFloat{0.00000000000000000000000000000000000918701489667776217044949118979087388873213108951222041500396842134538477567709204720146289220583657453289561090059578418731689453125}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyMinFloat{0.000000000000000000000000000000000008386100832707718457626787164520215590808324467463673030891527838259783484673866591218132347275437954436938525759615004062652587890625}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyStdDevFloat{0.206910665536153171029098984945449046790599822998046875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.6064075623937725811885002258350141346454620361328125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMaxKey{31308}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5259578695325901609436414219089783728122711181640625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMeanKey{30684}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.3847055762794624467204585016588680446147918701171875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMedianKey{19538}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMinFloat{0.238996153214439510659161669536842964589595794677734375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMinKey{15622}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.041246108155878986878395409121367265470325946807861328125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.261200279071756080728761162390583194792270660400390625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{20294}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1667996060247548817390139674898819066584110260009765625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{11498}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.04608553246768244682218806929085985757410526275634765625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{1490}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0300437945554398004588403381376338074915111064910888671875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{15622}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.037539975911930707763719539116209489293396472930908203125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{347194723449011078610315099327629011}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{20294}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{221714706013998620863807684704468992}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{11498}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{61258179956698243924747025463115776}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{1490}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{39935052822701027664841858754564702}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinKey{15622}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{49899186943229664998028801826881536}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{123}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6489.7350993377485792734660208225250244140625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6450}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{7310}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{31.7796015184623001914587803184986114501953125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{18.6324939727783203125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{15622}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.27478027659536241600335415569134056568145751953125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{27584}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.783549010753631147707665149937383830547332763671875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32103}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.6634309291839599609375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinKey{8840}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.738326613671914433467691196710802614688873291015625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2306}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.125827814569536400313154445029795169830322265625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{2}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1490}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{2}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1490}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99969160556793201788394753748434595763683319091796875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{29022}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99037608089825968082919871449121274054050445556640625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7790}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.93811319768428802490234375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11130}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.893275201320648193359375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1490}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01112124686773548198903682759919320233166217803955078125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.435276204639867103640682444165577180683612823486328125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMaxFloat{20092473}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMaxKey{7310}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMeanFloat{18269403.099337749183177947998046875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMeanKey{123}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMedianFloat{18127894}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMinFloat{18127894}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{313338.1599132127012126147747039794921875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMaxFloat{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMaxKey{2306}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMeanFloat{36.68874172185430637682657106779515743255615234375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMeanKey{29725}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMedianFloat{4}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMedianKey{4647}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMinFloat{4}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMinKey{4647}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapStdDevFloat{15.08395289175145848048487096093595027923583984375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.6067446714283786235455409041605889797210693359375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{31308}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.52814679443530021529795703827403485774993896484375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{27584}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.400933579659400962658111211567302234470844268798828125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6204}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.28114150292631900907025510605308227241039276123046875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15622}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03874858981339181218661593675278709270060062408447265625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{177.7373340129852294921875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{4305}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{167.602082707234558256459422409534454345703125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{13468}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{132.731911599636077880859375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{6549}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{51.602179050445556640625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinKey{123}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{10.0699252308332294347792412736453115940093994140625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMaxFloat{9.7576975822448712705181605997495353221893310546875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMaxKey{20539}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMeanFloat{9.443167899618085669999345554970204830169677734375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMeanKey{30684}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMedianFloat{9.20833241939544677734375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMedianKey{9816}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMinFloat{9.1634089946746843935443394002504646778106689453125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.1283144310823415568112437767922529019415378570556640625}
\def\SubcubicWithoutVocabSquaredProofSearchTimeLen{4530}
\def\SubcubicWithoutVocabSquaredProofSearchTimeMaxFloat{179.535578250885009765625}
\def\SubcubicWithoutVocabSquaredProofSearchTimeMeanFloat{167.055883590275101369115873239934444427490234375}
\def\SubcubicWithoutVocabSquaredProofSearchTimeMedianFloat{157.913934996128091370337642729282379150390625}
\def\SubcubicWithoutVocabSquaredProofSearchTimeMinFloat{51.602179050445556640625}
\def\SubcubicWithoutVocabSquaredProofSearchTimeStdDevFloat{6.31639246176139312893837995943613350391387939453125}
\def\SubcubicWithoutVocabSquaredProofTimeLen{4530}
\def\SubcubicWithoutVocabSquaredProofTimeMaxFloat{9.8397514820098876953125}
\def\SubcubicWithoutVocabSquaredProofTimeMeanFloat{9.4027398784165878709018215886317193508148193359375}
\def\SubcubicWithoutVocabSquaredProofTimeMedianFloat{9.1531567561626427931287253159098327159881591796875}
\def\SubcubicWithoutVocabSquaredProofTimeMinFloat{9.0864479541778564453125}
\def\SubcubicWithoutVocabSquaredProofTimeStdDevFloat{0.1262909835457892426813231168125639669597148895263671875}
\def\TrainAccuracyLen{151}
\def\TrainAccuracyMaxFloat{0.99976302083333334902448541470221243798732757568359375}
\def\TrainAccuracyMaxKey{16284}
\def\TrainAccuracyMeanFloat{0.99534407767660038057755400586756877601146697998046875}
\def\TrainAccuracyMeanKey{50}
\def\TrainAccuracyMedianFloat{0.90603710937500003819167204710538499057292938232421875}
\def\TrainAccuracyMedianKey{1490}
\def\TrainAccuracyMinFloat{0.8591015625000000266453525910037569701671600341796875}
\def\TrainAccuracyMinKey{15622}
\def\TrainAccuracyStdDevFloat{0.01396977803739154859463678093334237928502261638641357421875}
\def\TrainLossLen{151}
\def\TrainLossMaxFloat{0.318804908206065495956949007450020872056484222412109375}
\def\TrainLossMaxKey{15622}
\def\TrainLossMeanFloat{0.01194487167113495416914670244068474858067929744720458984375}
\def\TrainLossMeanKey{8299}
\def\TrainLossMedianFloat{0.0015621644232499723968510263460984788252972066402435302734375}
\def\TrainLossMedianKey{2743}
\def\TrainLossMinFloat{0.001492960045089906408188884512355798506177961826324462890625}
\def\TrainLossMinKey{27714}
\def\TrainLossStdDevFloat{0.031669393632650165437691924807950272224843502044677734375}
\def\UpperWhiskerCrosshatchPercentileFloat{0.91132822467382401665503266485757194459438323974609375}
\def\UpperWhiskerTopEndPercentileFloat{0.97848760463080519667045109599712304770946502685546875}
\def\WEkkPerpFirstSingularLen{151}
\def\WEkkPerpFirstSingularMaxFloat{3.76973247528076171875}
\def\WEkkPerpFirstSingularMaxKey{23367}
\def\WEkkPerpFirstSingularMeanFloat{3.197498119430036922494764439761638641357421875}
\def\WEkkPerpFirstSingularMeanKey{5781}
\def\WEkkPerpFirstSingularMedianFloat{2.9238321781158447265625}
\def\WEkkPerpFirstSingularMedianKey{2306}
\def\WEkkPerpFirstSingularMinFloat{2.88459110260009765625}
\def\WEkkPerpFirstSingularMinKey{29726}
\def\WEkkPerpFirstSingularStdDevFloat{0.17013581242918351943416155336308293044567108154296875}
\def\WEkkPerpFroNormLen{151}
\def\WEkkPerpFroNormMaxFloat{8.31924915313720703125}
\def\WEkkPerpFroNormMaxKey{27300}
\def\WEkkPerpFroNormMeanFloat{7.80512954699282612835986583377234637737274169921875}
\def\WEkkPerpFroNormMeanKey{29195}
\def\WEkkPerpFroNormMedianFloat{7.4531939029693603515625}
\def\WEkkPerpFroNormMedianKey{6549}
\def\WEkkPerpFroNormMinFloat{7.39577960968017578125}
\def\WEkkPerpFroNormMinKey{12552}
\def\WEkkPerpFroNormStdDevFloat{0.1586529750992268505971338754534372128546237945556640625}
\def\WEqqPerpFirstSingularLen{151}
\def\WEqqPerpFirstSingularMaxFloat{3.6455881595611572265625}
\def\WEqqPerpFirstSingularMaxKey{23367}
\def\WEqqPerpFirstSingularMeanFloat{3.1902121502832070376598494476638734340667724609375}
\def\WEqqPerpFirstSingularMeanKey{28716}
\def\WEqqPerpFirstSingularMedianFloat{2.88980567455291748046875}
\def\WEqqPerpFirstSingularMedianKey{29726}
\def\WEqqPerpFirstSingularMinFloat{2.8170874118804931640625}
\def\WEqqPerpFirstSingularMinKey{19538}
\def\WEqqPerpFirstSingularStdDevFloat{0.1556280447538939959439829863185877911746501922607421875}
\def\WEqqPerpFroNormLen{151}
\def\WEqqPerpFroNormMaxFloat{8.36928653717041015625}
\def\WEqqPerpFroNormMaxKey{27300}
\def\WEqqPerpFroNormMeanFloat{7.9532499218618628589183572330512106418609619140625}
\def\WEqqPerpFroNormMeanKey{21598}
\def\WEqqPerpFroNormMedianFloat{7.61717712879180908203125}
\def\WEqqPerpFroNormMedianKey{32374}
\def\WEqqPerpFroNormMinFloat{7.594755649566650390625}
\def\WEqqPerpFroNormMinKey{12552}
\def\WEqqPerpFroNormStdDevFloat{0.1608460146586499772691780663080862723290920257568359375}
\def\WKkPerpFirstSingularLen{151}
\def\WKkPerpFirstSingularMaxFloat{1.62288761138916015625}
\def\WKkPerpFirstSingularMaxKey{12493}
\def\WKkPerpFirstSingularMeanFloat{1.462948450979018044648682916886173188686370849609375}
\def\WKkPerpFirstSingularMeanKey{28090}
\def\WKkPerpFirstSingularMedianFloat{1.345090687274932861328125}
\def\WKkPerpFirstSingularMedianKey{2306}
\def\WKkPerpFirstSingularMinFloat{1.34358632564544677734375}
\def\WKkPerpFirstSingularMinKey{15399}
\def\WKkPerpFirstSingularStdDevFloat{0.058130146167179007343772667582015856169164180755615234375}
\def\WKkPerpFroNormLen{151}
\def\WKkPerpFroNormMaxFloat{4.546871662139892578125}
\def\WKkPerpFroNormMaxKey{29565}
\def\WKkPerpFroNormMeanFloat{4.2662262032363589270289594423957169055938720703125}
\def\WKkPerpFroNormMeanKey{32374}
\def\WKkPerpFroNormMedianFloat{4.0425889492034912109375}
\def\WKkPerpFroNormMedianKey{20751}
\def\WKkPerpFroNormMinFloat{4.029094219207763671875}
\def\WKkPerpFroNormMinKey{16069}
\def\WKkPerpFroNormStdDevFloat{0.10180531292463433634676306382971233688294887542724609375}
\def\WQqPerpFirstSingularLen{151}
\def\WQqPerpFirstSingularMaxFloat{1.66935575008392333984375}
\def\WQqPerpFirstSingularMaxKey{20751}
\def\WQqPerpFirstSingularMeanFloat{1.4816968298905732748238506246707402169704437255859375}
\def\WQqPerpFirstSingularMeanKey{20976}
\def\WQqPerpFirstSingularMedianFloat{1.299220740795135498046875}
\def\WQqPerpFirstSingularMedianKey{4430}
\def\WQqPerpFirstSingularMinFloat{1.28251039981842041015625}
\def\WQqPerpFirstSingularMinKey{20539}
\def\WQqPerpFirstSingularStdDevFloat{0.0750596681775628493671348451243829913437366485595703125}
\def\WQqPerpFroNormLen{151}
\def\WQqPerpFroNormMaxFloat{4.512707233428955078125}
\def\WQqPerpFroNormMaxKey{12457}
\def\WQqPerpFroNormMeanFloat{4.30481002504462395563678001053631305694580078125}
\def\WQqPerpFroNormMeanKey{7790}
\def\WQqPerpFroNormMedianFloat{4.04127037525177001953125}
\def\WQqPerpFroNormMedianKey{1951}
\def\WQqPerpFroNormMinFloat{4.000235080718994140625}
\def\WQqPerpFroNormMinKey{20539}
\def\WQqPerpFroNormStdDevFloat{0.09868336811270243813520863795929471962153911590576171875}


==> generated/values-5.tex <==
\def\AllModelsHEADSHASHORT{ac37d3d}
\def\AllModelsHEADSHA{ac37d3d9accc01c6a5ef109e94152f831a7cab77}
\def\AlmostQuadraticAccuracyLen{2718}
\def\AlmostQuadraticAccuracyMaxFloat{0.4154766835272312164306640625}
\def\AlmostQuadraticAccuracyMeanFloat{0.0724836553318797260914152502664364874362945556640625}
\def\AlmostQuadraticAccuracyMedianFloat{0.00000004470348358154297536744490042422139897126953655970282852649688720703125}
\def\AlmostQuadraticAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\AlmostQuadraticAccuracyStdDevFloat{0.122397661740817620401600152035825885832309722900390625}
\def\AlmostQuadraticDroppedSequencesFracLen{2718}
\def\AlmostQuadraticDroppedSequencesFracMaxFloat{0.378214078024029676239337049992172978818416595458984375}
\def\AlmostQuadraticDroppedSequencesFracMeanFloat{0.1811024858246230440084190149718779139220714569091796875}
\def\AlmostQuadraticDroppedSequencesFracMedianFloat{0}
\def\AlmostQuadraticDroppedSequencesFracMinFloat{0}
\def\AlmostQuadraticDroppedSequencesFracStdDevFloat{0.13462124881513926055731644737534224987030029296875}
\def\AlmostQuadraticDroppedSequencesLen{2718}
\def\AlmostQuadraticDroppedSequencesMaxFloat{406104274}
\def\AlmostQuadraticDroppedSequencesMeanFloat{194457313.4602648913860321044921875}
\def\AlmostQuadraticDroppedSequencesMedianFloat{0}
\def\AlmostQuadraticDroppedSequencesMinFloat{0}
\def\AlmostQuadraticDroppedSequencesStdDevFloat{144548465.25192546844482421875}
\def\AlmostQuadraticEffectiveDimensionalityEstimateLen{2718}
\def\AlmostQuadraticEffectiveDimensionalityEstimateMaxFloat{6530}
\def\AlmostQuadraticEffectiveDimensionalityEstimateMeanFloat{6487.3333333333330301684327423572540283203125}
\def\AlmostQuadraticEffectiveDimensionalityEstimateMedianFloat{6402}
\def\AlmostQuadraticEffectiveDimensionalityEstimateMinFloat{6402}
\def\AlmostQuadraticEffectiveDimensionalityEstimateStdDevFloat{42.66666666666666429819088079966604709625244140625}
\def\AlmostQuadraticErrUpperBoundLen{2718}
\def\AlmostQuadraticErrUpperBoundMaxFloat{144.185821533203125}
\def\AlmostQuadraticErrUpperBoundMeanFloat{95.1135054497792538086287095211446285247802734375}
\def\AlmostQuadraticErrUpperBoundMedianFloat{78.46202850341796875}
\def\AlmostQuadraticErrUpperBoundMinFloat{77.82788848876953125}
\def\AlmostQuadraticErrUpperBoundStdDevFloat{7.5268897599165089928874294855631887912750244140625}
\def\AlmostQuadraticGapMostBelowValueLen{2718}
\def\AlmostQuadraticGapMostBelowValueMaxFloat{73}
\def\AlmostQuadraticGapMostBelowValueMeanFloat{28.147167034584253286766397650353610515594482421875}
\def\AlmostQuadraticGapMostBelowValueMedianFloat{1}
\def\AlmostQuadraticGapMostBelowValueMinFloat{1}
\def\AlmostQuadraticGapMostBelowValueNumStdLen{2718}
\def\AlmostQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\AlmostQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\AlmostQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\AlmostQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\AlmostQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\AlmostQuadraticGapMostBelowValueSequenceFracLen{2718}
\def\AlmostQuadraticGapMostBelowValueSequenceFracMaxFloat{1}
\def\AlmostQuadraticGapMostBelowValueSequenceFracMeanFloat{1}
\def\AlmostQuadraticGapMostBelowValueSequenceFracMedianFloat{1}
\def\AlmostQuadraticGapMostBelowValueSequenceFracMinFloat{1}
\def\AlmostQuadraticGapMostBelowValueSequenceFracStdDevFloat{0}
\def\AlmostQuadraticGapMostBelowValueStdDevFloat{20.017442110895405704695804161019623279571533203125}
\def\AlmostQuadraticInstructionCountBranchLen{2718}
\def\AlmostQuadraticInstructionCountBranchMaxFloat{0}
\def\AlmostQuadraticInstructionCountBranchMeanFloat{0}
\def\AlmostQuadraticInstructionCountBranchMedianFloat{0}
\def\AlmostQuadraticInstructionCountBranchMinFloat{0}
\def\AlmostQuadraticInstructionCountBranchStdDevFloat{0}
\def\AlmostQuadraticInstructionCountIntLen{2718}
\def\AlmostQuadraticInstructionCountIntMaxFloat{0}
\def\AlmostQuadraticInstructionCountIntMeanFloat{0}
\def\AlmostQuadraticInstructionCountIntMedianFloat{0}
\def\AlmostQuadraticInstructionCountIntMinFloat{0}
\def\AlmostQuadraticInstructionCountIntStdDevFloat{0}
\def\AlmostQuadraticInstructionCountLen{2718}
\def\AlmostQuadraticInstructionCountMaxFloat{2411562}
\def\AlmostQuadraticInstructionCountMeanFloat{2372971.6666666665114462375640869140625}
\def\AlmostQuadraticInstructionCountMedianFloat{2334413}
\def\AlmostQuadraticInstructionCountMinFloat{2334413}
\def\AlmostQuadraticInstructionCountStdDevFloat{26559.48824389840956428088247776031494140625}
\def\AlmostQuadraticMaxGapLen{2718}
\def\AlmostQuadraticMaxGapMaxFloat{34}
\def\AlmostQuadraticMaxGapMeanFloat{15.9131714495952909516063300543464720249176025390625}
\def\AlmostQuadraticMaxGapMedianFloat{1}
\def\AlmostQuadraticMaxGapMinFloat{1}
\def\AlmostQuadraticMaxGapStdDevFloat{10.9080292652295991473465619492344558238983154296875}
\def\AlmostQuadraticNormalizedAccuracyLen{2718}
\def\AlmostQuadraticNormalizedAccuracyMaxFloat{0.4157097376548632983173092725337482988834381103515625}
\def\AlmostQuadraticNormalizedAccuracyMeanFloat{0.0725533972296098228493832493768422864377498626708984375}
\def\AlmostQuadraticNormalizedAccuracyMedianFloat{0.00000004477619510034710918767376810860347813303405928309075534343719482421875}
\def\AlmostQuadraticNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\AlmostQuadraticNormalizedAccuracyStdDevFloat{0.1225085209325896540288880487423739396035671234130859375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.4154766835272312164306640625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{27300}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.335266042513069739694486770531511865556240081787109375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{20415}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.248908461770042721550311171085922978818416595458984375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2342543266713618954621978218710864894092082977294921875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.033004201385701419091400765637445147149264812469482421875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.375500188209116403381671034367172978818416595458984375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.312504638960918068590899565606378018856048583984375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{2549}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2444566735066472651372038171757594682276248931884765625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{28090}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.2349676061421631934056364343632594682276248931884765625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.028315214295907935315721459801352466456592082977294921875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{403190257}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{335549301.046357631683349609375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{2549}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{262483354.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{28090}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{252294546}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{30403229.8450390510261058807373046875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6502.0264900662250511231832206249237060546875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{519}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{519}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{31.745667070430105383138652541674673557281494140625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.185821533203125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.69683074951171875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11130}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.7692584991455078125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.29946136474609375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.42973356827689013215376689913682639598846435546875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{69}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{41.27814569536423761064725113101303577423095703125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{29.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{28}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{6.44709384747194480524967730161733925342559814453125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2411562}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{913}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2393577.218543046154081821441650390625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2384845}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{519}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{2384845}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{519}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{8919.140182845294475555419921875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{34}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{24.23841059602649039561583776958286762237548828125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{1283}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{17.75}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{6155}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{20338}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.98718811560862729237442181329242885112762451171875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.4157097376548632983173092725337482988834381103515625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27300}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.33558050608889333776829744238057173788547515869140625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6082}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.2490520827774077294858301456770277582108974456787109375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.23443112806623200849998056582990102469921112060546875}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.032957431535899091301633490047606755979359149932861328125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6513054370880126953125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.74660976675172463501439779065549373626708984375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{8840}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.4892952442169189453125}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4421784877777099609375}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.73073050769386471703370489194639958441257476806640625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.32684421539306640625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{50}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.21747174326157736601317083113826811313629150390625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{2549}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.141332685947418212890625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{21317}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{2.132311344146728515625}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\AlmostQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0303655272331933255569591523226335993967950344085693359375}
\def\AlmostQuadraticProofSearchTimeLen{2718}
\def\AlmostQuadraticProofSearchTimeMaxFloat{52.45428371429443359375}
\def\AlmostQuadraticProofSearchTimeMeanFloat{44.57724635288766279472838505171239376068115234375}
\def\AlmostQuadraticProofSearchTimeMedianFloat{42.4414603543281572228806908242404460906982421875}
\def\AlmostQuadraticProofSearchTimeMinFloat{42.08597469329833984375}
\def\AlmostQuadraticProofSearchTimeStdDevFloat{0.742895826725537222756656774436123669147491455078125}
\def\AlmostQuadraticProofTimeLen{2718}
\def\AlmostQuadraticProofTimeMaxFloat{2.594494342803955078125}
\def\AlmostQuadraticProofTimeMeanFloat{2.209200717755500864569739860598929226398468017578125}
\def\AlmostQuadraticProofTimeMedianFloat{2.131579179763793963076068394002504646778106689453125}
\def\AlmostQuadraticProofTimeMinFloat{2.1170752048492431640625}
\def\AlmostQuadraticProofTimeStdDevFloat{0.03222898597147559607289935001972480677068233489990234375}
\def\AnySubcubicAccuracyLen{15100}
\def\AnySubcubicAccuracyLowerWhiskerBottomEndFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\AnySubcubicAccuracyLowerWhiskerCrosshatchFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\AnySubcubicAccuracyMaxFloat{0.780931304208934307098388671875}
\def\AnySubcubicAccuracyMeanFloat{0.2375207564113230029878565119361155666410923004150390625}
\def\AnySubcubicAccuracyMedianFloat{0.00000004563480615615845388306990042422139897126953655970282852649688720703125}
\def\AnySubcubicAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\AnySubcubicAccuracyQuartileOneFloat{0.00000004470348358154297536744490042422139897126953655970282852649688720703125}
\def\AnySubcubicAccuracyQuartileThreeFloat{0.00000004563480615615845388306990042422139897126953655970282852649688720703125}
\def\AnySubcubicAccuracySqrMeanFloat{0.1174745332955065280078343903369386680424213409423828125}
\def\AnySubcubicAccuracyStdDevFloat{0.2471000274570998855860892717828392051160335540771484375}
\def\AnySubcubicAccuracyUpperWhiskerCrosshatchFloat{0.00000004563480615615845388306990042422139897126953655970282852649688720703125}
\def\AnySubcubicAccuracyUpperWhiskerTopEndFloat{0.00000004563480615615845388306990042422139897126953655970282852649688720703125}
\def\AnySubcubicDroppedSequencesFracLen{15100}
\def\AnySubcubicDroppedSequencesFracMaxFloat{0.402560516260564327239990234375}
\def\AnySubcubicDroppedSequencesFracMeanFloat{0.1339002859487586627462718524839146994054317474365234375}
\def\AnySubcubicDroppedSequencesFracMedianFloat{0}
\def\AnySubcubicDroppedSequencesFracMinFloat{0}
\def\AnySubcubicDroppedSequencesFracStdDevFloat{0.11165436334591223588308395164858666248619556427001953125}
\def\AnySubcubicDroppedSequencesLen{15100}
\def\AnySubcubicDroppedSequencesMaxFloat{432246063}
\def\AnySubcubicDroppedSequencesMeanFloat{143774337.26874172687530517578125}
\def\AnySubcubicDroppedSequencesMedianFloat{0}
\def\AnySubcubicDroppedSequencesMinFloat{0}
\def\AnySubcubicDroppedSequencesStdDevFloat{119887959.75659854710102081298828125}
\def\AnySubcubicEffectiveDimensionalityEstimateLen{15100}
\def\AnySubcubicEffectiveDimensionalityEstimateMaxFloat{10370}
\def\AnySubcubicEffectiveDimensionalityEstimateMeanFloat{6049.600000000000363797880709171295166015625}
\def\AnySubcubicEffectiveDimensionalityEstimateMedianFloat{4290}
\def\AnySubcubicEffectiveDimensionalityEstimateMinFloat{4290}
\def\AnySubcubicEffectiveDimensionalityEstimateStdDevFloat{1530.49032666005450664670206606388092041015625}
\def\AnySubcubicErrUpperBoundLen{15100}
\def\AnySubcubicErrUpperBoundMaxFloat{144.185821533203125}
\def\AnySubcubicErrUpperBoundMeanFloat{33.28911486240411932158167473971843719482421875}
\def\AnySubcubicErrUpperBoundMedianFloat{0}
\def\AnySubcubicErrUpperBoundMinFloat{0}
\def\AnySubcubicErrUpperBoundStdDevFloat{40.9492951108743596932981745339930057525634765625}
\def\AnySubcubicGapMostBelowValueLen{15100}
\def\AnySubcubicGapMostBelowValueMaxFloat{73}
\def\AnySubcubicGapMostBelowValueMeanFloat{12.705761589403973488288102089427411556243896484375}
\def\AnySubcubicGapMostBelowValueMedianFloat{1}
\def\AnySubcubicGapMostBelowValueMinFloat{1}
\def\AnySubcubicGapMostBelowValueNumStdLen{15100}
\def\AnySubcubicGapMostBelowValueNumStdMaxFloat{1.5}
\def\AnySubcubicGapMostBelowValueNumStdMeanFloat{1.5}
\def\AnySubcubicGapMostBelowValueNumStdMedianFloat{1.5}
\def\AnySubcubicGapMostBelowValueNumStdMinFloat{1.5}
\def\AnySubcubicGapMostBelowValueNumStdStdDevFloat{0}
\def\AnySubcubicGapMostBelowValueSequenceFracLen{15100}
\def\AnySubcubicGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\AnySubcubicGapMostBelowValueSequenceFracMeanFloat{0.99453861186835934571348616373143158853054046630859375}
\def\AnySubcubicGapMostBelowValueSequenceFracMedianFloat{0.96024964660406109118184758699499070644378662109375}
\def\AnySubcubicGapMostBelowValueSequenceFracMinFloat{0.9398634433746337890625}
\def\AnySubcubicGapMostBelowValueSequenceFracStdDevFloat{0.00810430416835831134159118249726816429756581783294677734375}
\def\AnySubcubicGapMostBelowValueStdDevFloat{14.769136645981159716711772489361464977264404296875}
\def\AnySubcubicInstructionCountBranchLen{15100}
\def\AnySubcubicInstructionCountBranchMaxFloat{0}
\def\AnySubcubicInstructionCountBranchMeanFloat{0}
\def\AnySubcubicInstructionCountBranchMedianFloat{0}
\def\AnySubcubicInstructionCountBranchMinFloat{0}
\def\AnySubcubicInstructionCountBranchStdDevFloat{0}
\def\AnySubcubicInstructionCountIntLen{15100}
\def\AnySubcubicInstructionCountIntMaxFloat{0}
\def\AnySubcubicInstructionCountIntMeanFloat{0}
\def\AnySubcubicInstructionCountIntMedianFloat{0}
\def\AnySubcubicInstructionCountIntMinFloat{0}
\def\AnySubcubicInstructionCountIntStdDevFloat{0}
\def\AnySubcubicInstructionCountLen{15100}
\def\AnySubcubicInstructionCountMaxFloat{5144079}
\def\AnySubcubicInstructionCountMeanFloat{3270441.799999999813735485076904296875}
\def\AnySubcubicInstructionCountMedianFloat{2334413}
\def\AnySubcubicInstructionCountMinFloat{2334413}
\def\AnySubcubicInstructionCountStdDevFloat{794410.24955004197545349597930908203125}
\def\AnySubcubicMaxGapLen{15100}
\def\AnySubcubicMaxGapMaxFloat{34}
\def\AnySubcubicMaxGapMeanFloat{13.491324503311258098392499960027635097503662109375}
\def\AnySubcubicMaxGapMedianFloat{1}
\def\AnySubcubicMaxGapMinFloat{1}
\def\AnySubcubicMaxGapStdDevFloat{7.92110042989769258525711848051287233829498291015625}
\def\AnySubcubicNormalizedAccuracyLen{15100}
\def\AnySubcubicNormalizedAccuracyLowerWhiskerBottomEndFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\AnySubcubicNormalizedAccuracyLowerWhiskerCrosshatchFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\AnySubcubicNormalizedAccuracyMaxFloat{0.7812433963450775564751893398351967334747314453125}
\def\AnySubcubicNormalizedAccuracyMeanFloat{0.2377466150843743075693481614507618360221385955810546875}
\def\AnySubcubicNormalizedAccuracyMedianFloat{0.000000045658116086492779083511463038280719928252437966875731945037841796875}
\def\AnySubcubicNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\AnySubcubicNormalizedAccuracyQuartileOneFloat{0.00000004477619510034710918767376810860347813303405928309075534343719482421875}
\def\AnySubcubicNormalizedAccuracyQuartileThreeFloat{0.00000004565851532106180983955516570864385794692452691379003226757049560546875}
\def\AnySubcubicNormalizedAccuracySqrMeanFloat{0.11769366750020564260648114895957405678927898406982421875}
\def\AnySubcubicNormalizedAccuracyStdDevFloat{0.2473261298693043286345272235848824493587017059326171875}
\def\AnySubcubicNormalizedAccuracyUpperWhiskerCrosshatchFloat{0.0000000456637246590067298404060601446641243228441453538835048675537109375}
\def\AnySubcubicNormalizedAccuracyUpperWhiskerTopEndFloat{0.00000004566775113709099781243296403178411058121355381445027887821197509765625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLowerWhiskerBottomEndFloat{0.593481302132915278235714140464551746845245361328125}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLowerWhiskerBottomEndKey{1951}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLowerWhiskerCrosshatchFloat{0.59607635751973886417687253924668766558170318603515625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyLowerWhiskerCrosshatchKey{1951}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.780931304208934307098388671875}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMaxKey{29110}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.70537861965794046437139286354067735373973846435546875}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMeanKey{10248}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.6119701839052140712738037109375}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMinFloat{0.59265005774796009063720703125}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyMinKey{1951}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyQuartileOneFloat{0.60231012082658708095550537109375}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyQuartileOneKey{1951}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyQuartileThreeFloat{0.618881361908279359340667724609375}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyQuartileThreeKey{12552}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracySqrMeanFloat{0.498524166845884908472186225480982102453708648681640625}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0310671816446796665578400364893241203390061855316162109375}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyUpperWhiskerCrosshatchFloat{0.619793452226254704129360106890089809894561767578125}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyUpperWhiskerCrosshatchKey{12552}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyUpperWhiskerTopEndFloat{0.62017314660610567411680449367850087583065032958984375}
\def\AnySubcubicOnlyBestAccBoundPerSeedAccuracyUpperWhiskerTopEndKey{12552}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.12679875083267688751220703125}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.08391068376206005374751129011201555840671062469482421875}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{5781}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.06227796920575197348046714296287973411381244659423828125}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{2345}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.058046793565153999294725650770487845875322818756103515625}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01268794889335365938531907659125863574445247650146484375}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{136149122}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{90098410.6357615888118743896484375}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{5781}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{66870460.25}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{2345}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{62327270}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\AnySubcubicOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{13623581.38756833784282207489013671875}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{2236}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{7080.6490066225169357494451105594635009765625}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{1185}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4402}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{104}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{24144}
\def\AnySubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{2075.01463873772081569768488407135009765625}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{9.37257671356201171875}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{17194}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{1.492547126795282341760184863233007490634918212890625}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{27714}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{123}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinKey{123}
\def\AnySubcubicOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.267698926495981925910427889903075993061065673828125}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2236}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.16556291390728450352298750658519566059112548828125}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999912261962890625}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2773}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9853469997841790561921015978441573679447174072265625}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6910}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95145584642887115478515625}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{913}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.943215072154998779296875}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2345}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01196093248701758648966375631061964668333530426025390625}
\def\AnySubcubicOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.87972349340561961650308830940048210322856903076171875}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMaxFloat{4193742}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMaxKey{104}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3312777.3642384107224643230438232421875}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMeanKey{5928}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2696590}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMedianKey{2236}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMinFloat{2696590}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountMinKey{2236}
\def\AnySubcubicOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{556895.864682440995238721370697021484375}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMaxFloat{19}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.132450331125827602818390005268156528472900390625}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMeanKey{1951}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMedianKey{6159}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapMinKey{27300}
\def\AnySubcubicOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.720234448136964022779693550546653568744659423828125}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLowerWhiskerBottomEndFloat{0.5938116223089757728104132183943875133991241455078125}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLowerWhiskerBottomEndKey{1951}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLowerWhiskerCrosshatchFloat{0.59640591642028206731396267059608362615108489990234375}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLowerWhiskerCrosshatchKey{1951}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7812433963450775564751893398351967334747314453125}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29110}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.70604884924443778171365693197003565728664398193359375}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{3284}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.612295080253672185932600768865086138248443603515625}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.59298062177469235134452674174099229276180267333984375}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1951}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyQuartileOneFloat{0.60263785101418221312741252404521219432353973388671875}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyQuartileOneKey{1951}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyQuartileThreeFloat{0.6192087276607127765970517430105246603488922119140625}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyQuartileThreeKey{12552}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracySqrMeanFloat{0.499463505070892488379996621006284840404987335205078125}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0309600961157661565270604597799319890327751636505126953125}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyUpperWhiskerCrosshatchFloat{0.620129256019296359880854652146808803081512451171875}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyUpperWhiskerCrosshatchKey{12552}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyUpperWhiskerTopEndFloat{0.620512463073860320861285799765028059482574462890625}
\def\AnySubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyUpperWhiskerTopEndKey{12552}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7359836101531982421875}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.65898868737631488556871772743761539459228515625}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{12141}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.74832755327224020902576739899814128875732421875}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.6372649669647216796875}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7004619892651062773580861176014877855777740478515625}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2972538471221923828125}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMaxKey{5358}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.2151392137767462742203861125744879245758056640625}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMeanKey{13293}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.1408836841583251953125}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1362316608428955078125}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\AnySubcubicOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.031038837999946923551508604077753261663019657135009765625}
\def\AnySubcubicProofSearchTimeLen{15100}
\def\AnySubcubicProofSearchTimeMaxFloat{52.45428371429443359375}
\def\AnySubcubicProofSearchTimeMeanFloat{44.55526558441831497248131199739873409271240234375}
\def\AnySubcubicProofSearchTimeMedianFloat{42.36292500376701042341665015555918216705322265625}
\def\AnySubcubicProofSearchTimeMinFloat{41.9884622097015380859375}
\def\AnySubcubicProofSearchTimeStdDevFloat{0.74150046099404942623323222505860030651092529296875}
\def\AnySubcubicProofTimeLen{15100}
\def\AnySubcubicProofTimeMaxFloat{2.6413619518280029296875}
\def\AnySubcubicProofTimeMeanFloat{2.208900451928574426574414246715605258941650390625}
\def\AnySubcubicProofTimeMedianFloat{2.131400314569473319892267682007513940334320068359375}
\def\AnySubcubicProofTimeMinFloat{2.1170752048492431640625}
\def\AnySubcubicProofTimeStdDevFloat{0.031684576742139265725928254369136993773281574249267578125}
\def\AxisLimitsOVCenteredZmaxFloat{15.32067108154296875}
\def\AxisLimitsOVCenteredZminFloat{-84.44426727294921875}
\def\AxisLimitsOVZmaxFloat{43.510372161865234375}
\def\AxisLimitsOVZminFloat{-43.510372161865234375}
\def\AxisLimitsQKWithAttnScaleZmaxFloat{75.990376742387752528884448111057281494140625}
\def\AxisLimitsQKWithAttnScaleZminFloat{-75.990376742387752528884448111057281494140625}
\def\AxisLimitsQKZmaxFloat{429.866485595703125}
\def\AxisLimitsQKZminFloat{-429.866485595703125}
\def\BruteForceEffectiveDimensionalityEstimate{68719476736}
\def\BruteForceInstructionCountBranch{0}
\def\BruteForceInstructionCountInt{0}
\def\BruteForceInstructionCount{14272938681565184}
\def\CubicAccuracyLen{151}
\def\CubicAccuracyLowerWhiskerBottomEndFloat{0.89777477724830878624828756073839031159877777099609375}
\def\CubicAccuracyLowerWhiskerBottomEndKey{28090}
\def\CubicAccuracyLowerWhiskerCrosshatchFloat{0.8985991313111265643698288840823806822299957275390625}
\def\CubicAccuracyLowerWhiskerCrosshatchKey{28090}
\def\CubicAccuracyMaxFloat{0.96120722033083438873291015625}
\def\CubicAccuracyMaxKey{18289}
\def\CubicAccuracyMeanFloat{0.9411535216001978287891915897489525377750396728515625}
\def\CubicAccuracyMeanKey{11130}
\def\CubicAccuracyMedianFloat{0.90364801790565263406307394689065404236316680908203125}
\def\CubicAccuracyMedianKey{13036}
\def\CubicAccuracyMinFloat{0.897510721348226070404052734375}
\def\CubicAccuracyMinKey{28090}
\def\CubicAccuracyQuartileOneFloat{0.900579369626939296722412109375}
\def\CubicAccuracyQuartileOneKey{28090}
\def\CubicAccuracyQuartileThreeFloat{0.90664675692096363679439718907815404236316680908203125}
\def\CubicAccuracyQuartileThreeKey{13036}
\def\CubicAccuracySqrMeanFloat{0.88589605481286104460281194405979476869106292724609375}
\def\CubicAccuracyStdDevFloat{0.01122958558482466291661427959525099140591919422149658203125}
\def\CubicAccuracyUpperWhiskerCrosshatchFloat{0.9084916551885411362121658385149203240871429443359375}
\def\CubicAccuracyUpperWhiskerCrosshatchKey{13036}
\def\CubicAccuracyUpperWhiskerTopEndFloat{0.90925966849795880619922172627411782741546630859375}
\def\CubicAccuracyUpperWhiskerTopEndKey{13036}
\def\CubicCorrectCountLen{151}
\def\CubicCorrectCountMaxFloat{1032088394}
\def\CubicCorrectCountMaxKey{18289}
\def\CubicCorrectCountMeanFloat{1010555898.9470198154449462890625}
\def\CubicCorrectCountMeanKey{11130}
\def\CubicCorrectCountMedianFloat{970284671}
\def\CubicCorrectCountMedianKey{13036}
\def\CubicCorrectCountMinFloat{963694799}
\def\CubicCorrectCountMinKey{28090}
\def\CubicCorrectCountStdDevFloat{12057675.7086137495934963226318359375}
\def\CubicEffectiveDimensionalityEstimate{12928}
\def\CubicInstructionCountBranch{0}
\def\CubicInstructionCountInt{0}
\def\CubicInstructionCount{52397344}
\def\CubicNormalizedAccuracyLen{151}
\def\CubicNormalizedAccuracyLowerWhiskerBottomEndFloat{0.91174179285916834292180510601610876619815826416015625}
\def\CubicNormalizedAccuracyLowerWhiskerBottomEndKey{28090}
\def\CubicNormalizedAccuracyLowerWhiskerCrosshatchFloat{0.91201721774668553788245617397478781640529632568359375}
\def\CubicNormalizedAccuracyLowerWhiskerCrosshatchKey{28090}
\def\CubicNormalizedAccuracyMaxFloat{0.96188131821519051722901849643676541745662689208984375}
\def\CubicNormalizedAccuracyMaxKey{18289}
\def\CubicNormalizedAccuracyMeanFloat{0.94204603513713347506808304387959651648998260498046875}
\def\CubicNormalizedAccuracyMeanKey{3175}
\def\CubicNormalizedAccuracyMedianFloat{0.913704100950283315540900730411522090435028076171875}
\def\CubicNormalizedAccuracyMedianKey{2236}
\def\CubicNormalizedAccuracyMinFloat{0.91165356915789852454423680683248676359653472900390625}
\def\CubicNormalizedAccuracyMinKey{28090}
\def\CubicNormalizedAccuracyQuartileOneFloat{0.912678835054090864531417537364177405834197998046875}
\def\CubicNormalizedAccuracyQuartileOneKey{28090}
\def\CubicNormalizedAccuracyQuartileThreeFloat{0.914476862666237622079279390163719654083251953125}
\def\CubicNormalizedAccuracyQuartileThreeKey{2236}
\def\CubicNormalizedAccuracySqrMeanFloat{0.88755882743440139837076685580541379749774932861328125}
\def\CubicNormalizedAccuracyStdDevFloat{0.01039688014782793636092694811168257729150354862213134765625}
\def\CubicNormalizedAccuracyUpperWhiskerCrosshatchFloat{0.91464964736019693791746476563275791704654693603515625}
\def\CubicNormalizedAccuracyUpperWhiskerCrosshatchKey{2236}
\def\CubicNormalizedAccuracyUpperWhiskerTopEndFloat{0.914721575957538224344034460955299437046051025390625}
\def\CubicNormalizedAccuracyUpperWhiskerTopEndKey{2236}
\def\CubicProofTimeLen{151}
\def\CubicProofTimeMaxFloat{54.7442772388458251953125}
\def\CubicProofTimeMaxKey{21317}
\def\CubicProofTimeMeanFloat{52.698758141094486973088351078331470489501953125}
\def\CubicProofTimeMeanKey{2345}
\def\CubicProofTimeMedianFloat{51.113180100917816162109375}
\def\CubicProofTimeMedianKey{28778}
\def\CubicProofTimeMinFloat{51.0632464885711669921875}
\def\CubicProofTimeMinKey{28090}
\def\CubicProofTimeStdDevFloat{0.85548772721279775499425568341393955051898956298828125}
\def\EPVOUAbsLenLen{151}
\def\EPVOUAbsLenMaxFloat{4096}
\def\EPVOUAbsLenMaxKey{50}
\def\EPVOUAbsLenMeanFloat{4096}
\def\EPVOUAbsLenMeanKey{50}
\def\EPVOUAbsLenMedianFloat{4096}
\def\EPVOUAbsLenMedianKey{50}
\def\EPVOUAbsLenMinFloat{4096}
\def\EPVOUAbsLenMinKey{50}
\def\EPVOUAbsLenStdDevFloat{0}
\def\EPVOUAbsMaxLen{151}
\def\EPVOUAbsMaxMaxFloat{43.5103759765625}
\def\EPVOUAbsMaxMaxKey{6532}
\def\EPVOUAbsMaxMeanFloat{35.19858551025390625}
\def\EPVOUAbsMaxMeanKey{26932}
\def\EPVOUAbsMaxMedianFloat{30.3272571563720703125}
\def\EPVOUAbsMaxMedianKey{29110}
\def\EPVOUAbsMaxMinFloat{29.749004364013671875}
\def\EPVOUAbsMaxMinKey{6159}
\def\EPVOUAbsMaxStdDevFloat{2.758265018463134765625}
\def\EPVOUAbsMeanLen{151}
\def\EPVOUAbsMeanMaxFloat{10.1134777069091796875}
\def\EPVOUAbsMeanMaxKey{8721}
\def\EPVOUAbsMeanMeanFloat{8.4475574493408203125}
\def\EPVOUAbsMeanMeanKey{18146}
\def\EPVOUAbsMeanMedianFloat{6.7315742969512939453125}
\def\EPVOUAbsMeanMedianKey{12552}
\def\EPVOUAbsMeanMinFloat{6.63383388519287109375}
\def\EPVOUAbsMeanMinKey{27584}
\def\EPVOUAbsMeanStdDevFloat{0.62955081462860107421875}
\def\EPVOUAbsMedianLen{151}
\def\EPVOUAbsMedianMaxFloat{0.12534775733947756126696049250313080847263336181640625}
\def\EPVOUAbsMedianMaxKey{7467}
\def\EPVOUAbsMedianMeanFloat{0.07809721914718285862289093302024411968886852264404296875}
\def\EPVOUAbsMedianMeanKey{24144}
\def\EPVOUAbsMedianMedianFloat{0.0466487109661102294921875}
\def\EPVOUAbsMedianMedianKey{2549}
\def\EPVOUAbsMedianMinFloat{0.04313963949680328646696381156289135105907917022705078125}
\def\EPVOUAbsMedianMinKey{17096}
\def\EPVOUAbsMedianStdDevFloat{0.0164300988078682590198820179239191929809749126434326171875}
\def\EPVOUAbsMinLen{151}
\def\EPVOUAbsMinMaxFloat{0.0248878002166748046875}
\def\EPVOUAbsMinMaxKey{8893}
\def\EPVOUAbsMinMeanFloat{0.00342048169113695621490478515625}
\def\EPVOUAbsMinMeanKey{16284}
\def\EPVOUAbsMinMedianFloat{0.0000067651271820068359375}
\def\EPVOUAbsMinMedianKey{4305}
\def\EPVOUAbsMinMinFloat{0.00000417232513427734375}
\def\EPVOUAbsMinMinKey{30899}
\def\EPVOUAbsMinStdDevFloat{0.00384899810887873172760009765625}
\def\EPVOUAbsStdDevLen{151}
\def\EPVOUAbsStdDevMaxFloat{6.709218502044677734375}
\def\EPVOUAbsStdDevMaxKey{11611}
\def\EPVOUAbsStdDevMeanFloat{5.731281757354736328125}
\def\EPVOUAbsStdDevMeanKey{29725}
\def\EPVOUAbsStdDevMedianFloat{4.84985256195068359375}
\def\EPVOUAbsStdDevMedianKey{12552}
\def\EPVOUAbsStdDevMinFloat{4.801803112030029296875}
\def\EPVOUAbsStdDevMinKey{27584}
\def\EPVOUAbsStdDevStdDevFloat{0.3681856095790863037109375}
\def\EPVOUCenteredLenLen{151}
\def\EPVOUCenteredLenMaxFloat{4096}
\def\EPVOUCenteredLenMaxKey{50}
\def\EPVOUCenteredLenMeanFloat{4096}
\def\EPVOUCenteredLenMeanKey{50}
\def\EPVOUCenteredLenMedianFloat{4096}
\def\EPVOUCenteredLenMedianKey{50}
\def\EPVOUCenteredLenMinFloat{4096}
\def\EPVOUCenteredLenMinKey{50}
\def\EPVOUCenteredLenStdDevFloat{0}
\def\EPVOUCenteredMaxLen{151}
\def\EPVOUCenteredMaxMaxFloat{15.3206729888916015625}
\def\EPVOUCenteredMaxMaxKey{6549}
\def\EPVOUCenteredMaxMeanFloat{12.2321910858154296875}
\def\EPVOUCenteredMaxMeanKey{16284}
\def\EPVOUCenteredMaxMedianFloat{8.783293247222900390625}
\def\EPVOUCenteredMaxMedianKey{15662}
\def\EPVOUCenteredMaxMinFloat{8.5003681182861328125}
\def\EPVOUCenteredMaxMinKey{27584}
\def\EPVOUCenteredMaxStdDevFloat{1.4382221698760986328125}
\def\EPVOUCenteredMeanLen{151}
\def\EPVOUCenteredMeanMaxFloat{-17.0744686126708984375}
\def\EPVOUCenteredMeanMaxKey{20338}
\def\EPVOUCenteredMeanMeanFloat{-19.7381381988525390625}
\def\EPVOUCenteredMeanMeanKey{29565}
\def\EPVOUCenteredMeanMedianFloat{-21.659896373748779296875}
\def\EPVOUCenteredMeanMedianKey{8721}
\def\EPVOUCenteredMeanMinFloat{-21.748386383056640625}
\def\EPVOUCenteredMeanMinKey{29022}
\def\EPVOUCenteredMeanStdDevFloat{0.80962812900543212890625}
\def\EPVOUCenteredMedianLen{151}
\def\EPVOUCenteredMedianMaxFloat{-48.58237972259521342266452847979962825775146484375}
\def\EPVOUCenteredMedianMaxKey{7884}
\def\EPVOUCenteredMedianMeanFloat{-56.1046193293388313350078533403575420379638671875}
\def\EPVOUCenteredMedianMeanKey{27671}
\def\EPVOUCenteredMedianMedianFloat{-65.311484909057611503158113919198513031005859375}
\def\EPVOUCenteredMedianMedianKey{742}
\def\EPVOUCenteredMedianMinFloat{-65.94977569580078125}
\def\EPVOUCenteredMedianMinKey{6532}
\def\EPVOUCenteredMedianStdDevFloat{3.60210595981024805922743325936608016490936279296875}
\def\EPVOUCenteredMinLen{151}
\def\EPVOUCenteredMinMaxFloat{-55.5420989990234375}
\def\EPVOUCenteredMinMaxKey{20338}
\def\EPVOUCenteredMinMeanFloat{-66.84307861328125}
\def\EPVOUCenteredMinMeanKey{32382}
\def\EPVOUCenteredMinMedianFloat{-79.8543796539306640625}
\def\EPVOUCenteredMinMedianKey{31308}
\def\EPVOUCenteredMinMinFloat{-84.44426727294921875}
\def\EPVOUCenteredMinMinKey{6532}
\def\EPVOUCenteredMinStdDevFloat{5.184821605682373046875}
\def\EPVOUCenteredOffDiagonalLenLen{151}
\def\EPVOUCenteredOffDiagonalLenMaxFloat{4032}
\def\EPVOUCenteredOffDiagonalLenMaxKey{50}
\def\EPVOUCenteredOffDiagonalLenMeanFloat{4032}
\def\EPVOUCenteredOffDiagonalLenMeanKey{50}
\def\EPVOUCenteredOffDiagonalLenMedianFloat{4032}
\def\EPVOUCenteredOffDiagonalLenMedianKey{50}
\def\EPVOUCenteredOffDiagonalLenMinFloat{4032}
\def\EPVOUCenteredOffDiagonalLenMinKey{50}
\def\EPVOUCenteredOffDiagonalLenStdDevFloat{0}
\def\EPVOUCenteredOffDiagonalMaxLen{151}
\def\EPVOUCenteredOffDiagonalMaxMaxFloat{15.3206729888916015625}
\def\EPVOUCenteredOffDiagonalMaxMaxKey{6549}
\def\EPVOUCenteredOffDiagonalMaxMeanFloat{12.2321910858154296875}
\def\EPVOUCenteredOffDiagonalMaxMeanKey{16284}
\def\EPVOUCenteredOffDiagonalMaxMedianFloat{8.783293247222900390625}
\def\EPVOUCenteredOffDiagonalMaxMedianKey{15662}
\def\EPVOUCenteredOffDiagonalMaxMinFloat{8.5003681182861328125}
\def\EPVOUCenteredOffDiagonalMaxMinKey{27584}
\def\EPVOUCenteredOffDiagonalMaxStdDevFloat{1.4382221698760986328125}
\def\EPVOUCenteredOffDiagonalMeanLen{151}
\def\EPVOUCenteredOffDiagonalMeanMaxFloat{-17.3454914093017578125}
\def\EPVOUCenteredOffDiagonalMeanMaxKey{20338}
\def\EPVOUCenteredOffDiagonalMeanMeanFloat{-20.051441192626953125}
\def\EPVOUCenteredOffDiagonalMeanMeanKey{29565}
\def\EPVOUCenteredOffDiagonalMeanMedianFloat{-22.0037059783935546875}
\def\EPVOUCenteredOffDiagonalMeanMedianKey{8721}
\def\EPVOUCenteredOffDiagonalMeanMinFloat{-22.0935993194580078125}
\def\EPVOUCenteredOffDiagonalMeanMinKey{29022}
\def\EPVOUCenteredOffDiagonalMeanStdDevFloat{0.82247936725616455078125}
\def\EPVOUCenteredOffDiagonalMedianLen{151}
\def\EPVOUCenteredOffDiagonalMedianMaxFloat{-48.6115960311889665490525658242404460906982421875}
\def\EPVOUCenteredOffDiagonalMedianMaxKey{7884}
\def\EPVOUCenteredOffDiagonalMedianMeanFloat{-56.1741679602111361191418836824595928192138671875}
\def\EPVOUCenteredOffDiagonalMedianMeanKey{8745}
\def\EPVOUCenteredOffDiagonalMedianMedianFloat{-65.488115768432606955684605054557323455810546875}
\def\EPVOUCenteredOffDiagonalMedianMedianKey{742}
\def\EPVOUCenteredOffDiagonalMedianMinFloat{-66.3572952270507840921709430404007434844970703125}
\def\EPVOUCenteredOffDiagonalMedianMinKey{6532}
\def\EPVOUCenteredOffDiagonalMedianStdDevFloat{3.608700635551362001507413879153318703174591064453125}
\def\EPVOUCenteredOffDiagonalMinLen{151}
\def\EPVOUCenteredOffDiagonalMinMaxFloat{-55.5420989990234375}
\def\EPVOUCenteredOffDiagonalMinMaxKey{20338}
\def\EPVOUCenteredOffDiagonalMinMeanFloat{-66.84307861328125}
\def\EPVOUCenteredOffDiagonalMinMeanKey{32382}
\def\EPVOUCenteredOffDiagonalMinMedianFloat{-79.8543796539306640625}
\def\EPVOUCenteredOffDiagonalMinMedianKey{31308}
\def\EPVOUCenteredOffDiagonalMinMinFloat{-84.44426727294921875}
\def\EPVOUCenteredOffDiagonalMinMinKey{6532}
\def\EPVOUCenteredOffDiagonalMinStdDevFloat{5.184821605682373046875}
\def\EPVOUCenteredOffDiagonalStdDevLen{151}
\def\EPVOUCenteredOffDiagonalStdDevMaxFloat{14.33452701568603515625}
\def\EPVOUCenteredOffDiagonalStdDevMaxKey{1412}
\def\EPVOUCenteredOffDiagonalStdDevMeanFloat{12.61914730072021484375}
\def\EPVOUCenteredOffDiagonalStdDevMeanKey{19004}
\def\EPVOUCenteredOffDiagonalStdDevMedianFloat{11.0625164508819580078125}
\def\EPVOUCenteredOffDiagonalStdDevMedianKey{30899}
\def\EPVOUCenteredOffDiagonalStdDevMinFloat{10.846584320068359375}
\def\EPVOUCenteredOffDiagonalStdDevMinKey{12552}
\def\EPVOUCenteredOffDiagonalStdDevStdDevFloat{0.71573817729949951171875}
\def\EPVOUCenteredStdDevLen{151}
\def\EPVOUCenteredStdDevMaxFloat{14.47194385528564453125}
\def\EPVOUCenteredStdDevMaxKey{1412}
\def\EPVOUCenteredStdDevMeanFloat{12.7649478912353515625}
\def\EPVOUCenteredStdDevMeanKey{24144}
\def\EPVOUCenteredStdDevMedianFloat{11.2176749706268310546875}
\def\EPVOUCenteredStdDevMedianKey{30899}
\def\EPVOUCenteredStdDevMinFloat{10.99025440216064453125}
\def\EPVOUCenteredStdDevMinKey{12552}
\def\EPVOUCenteredStdDevStdDevFloat{0.71383082866668701171875}
\def\EPVOUDiagonalLenLen{151}
\def\EPVOUDiagonalLenMaxFloat{64}
\def\EPVOUDiagonalLenMaxKey{50}
\def\EPVOUDiagonalLenMeanFloat{64}
\def\EPVOUDiagonalLenMeanKey{50}
\def\EPVOUDiagonalLenMedianFloat{64}
\def\EPVOUDiagonalLenMedianKey{50}
\def\EPVOUDiagonalLenMinFloat{64}
\def\EPVOUDiagonalLenMinKey{50}
\def\EPVOUDiagonalLenStdDevFloat{0}
\def\EPVOUDiagonalMaxLen{151}
\def\EPVOUDiagonalMaxMaxFloat{43.5103759765625}
\def\EPVOUDiagonalMaxMaxKey{6532}
\def\EPVOUDiagonalMaxMeanFloat{34.448307037353515625}
\def\EPVOUDiagonalMaxMeanKey{12141}
\def\EPVOUDiagonalMaxMedianFloat{29.68184947967529296875}
\def\EPVOUDiagonalMaxMedianKey{6159}
\def\EPVOUDiagonalMaxMinFloat{29.48038482666015625}
\def\EPVOUDiagonalMaxMinKey{8893}
\def\EPVOUDiagonalMaxStdDevFloat{2.636967182159423828125}
\def\EPVOUDiagonalMeanLen{151}
\def\EPVOUDiagonalMeanMaxFloat{22.6522846221923828125}
\def\EPVOUDiagonalMeanMaxKey{8721}
\def\EPVOUDiagonalMeanMeanFloat{20.5049495697021484375}
\def\EPVOUDiagonalMeanMeanKey{6204}
\def\EPVOUDiagonalMeanMedianFloat{18.102988719940185546875}
\def\EPVOUDiagonalMeanMedianKey{27584}
\def\EPVOUDiagonalMeanMinFloat{17.65077972412109375}
\def\EPVOUDiagonalMeanMinKey{20338}
\def\EPVOUDiagonalMeanStdDevFloat{0.873640120029449462890625}
\def\EPVOUDiagonalMedianLen{151}
\def\EPVOUDiagonalMedianMaxFloat{10.4727361965179444069917735760100185871124267578125}
\def\EPVOUDiagonalMedianMaxKey{27300}
\def\EPVOUDiagonalMedianMeanFloat{7.5525399326330795446438060025684535503387451171875}
\def\EPVOUDiagonalMedianMeanKey{6910}
\def\EPVOUDiagonalMedianMedianFloat{3.823206593394279817488268236047588288784027099609375}
\def\EPVOUDiagonalMedianMedianKey{4800}
\def\EPVOUDiagonalMedianMinFloat{2.566325786113738960381169817992486059665679931640625}
\def\EPVOUDiagonalMedianMinKey{3254}
\def\EPVOUDiagonalMedianStdDevFloat{1.42047412285575092028011567890644073486328125}
\def\EPVOUDiagonalMinLen{151}
\def\EPVOUDiagonalMinMaxFloat{10.400974273681640625}
\def\EPVOUDiagonalMinMaxKey{27300}
\def\EPVOUDiagonalMinMeanFloat{7.251646518707275390625}
\def\EPVOUDiagonalMinMeanKey{12457}
\def\EPVOUDiagonalMinMedianFloat{3.08106195926666259765625}
\def\EPVOUDiagonalMinMedianKey{6155}
\def\EPVOUDiagonalMinMinFloat{1.323558807373046875}
\def\EPVOUDiagonalMinMinKey{3254}
\def\EPVOUDiagonalMinStdDevFloat{1.52545917034149169921875}
\def\EPVOUDiagonalStdDevLen{151}
\def\EPVOUDiagonalStdDevMaxFloat{7.34607601165771484375}
\def\EPVOUDiagonalStdDevMaxKey{15662}
\def\EPVOUDiagonalStdDevMeanFloat{5.591092586517333984375}
\def\EPVOUDiagonalStdDevMeanKey{20294}
\def\EPVOUDiagonalStdDevMedianFloat{4.35108280181884765625}
\def\EPVOUDiagonalStdDevMedianKey{8893}
\def\EPVOUDiagonalStdDevMinFloat{4.315677642822265625}
\def\EPVOUDiagonalStdDevMinKey{7310}
\def\EPVOUDiagonalStdDevStdDevFloat{0.5433480739593505859375}
\def\EPVOUInputsWithCopyingFailureLenLen{151}
\def\EPVOUInputsWithCopyingFailureLenMaxFloat{16}
\def\EPVOUInputsWithCopyingFailureLenMaxKey{20338}
\def\EPVOUInputsWithCopyingFailureLenMeanFloat{12.403973509933774010960405576042830944061279296875}
\def\EPVOUInputsWithCopyingFailureLenMeanKey{123}
\def\EPVOUInputsWithCopyingFailureLenMedianFloat{10}
\def\EPVOUInputsWithCopyingFailureLenMedianKey{12552}
\def\EPVOUInputsWithCopyingFailureLenMinFloat{10}
\def\EPVOUInputsWithCopyingFailureLenMinKey{12552}
\def\EPVOUInputsWithCopyingFailureLenStdDevFloat{1.134520396070339831595674695563502609729766845703125}
\def\EPVOUInputsWithCopyingFailureMaxLen{151}
\def\EPVOUInputsWithCopyingFailureMaxMaxFloat{32}
\def\EPVOUInputsWithCopyingFailureMaxMaxKey{20338}
\def\EPVOUInputsWithCopyingFailureMaxMeanFloat{12.357615894039735593423756654374301433563232421875}
\def\EPVOUInputsWithCopyingFailureMaxMeanKey{742}
\def\EPVOUInputsWithCopyingFailureMaxMedianFloat{9}
\def\EPVOUInputsWithCopyingFailureMaxMedianKey{24144}
\def\EPVOUInputsWithCopyingFailureMaxMinFloat{9}
\def\EPVOUInputsWithCopyingFailureMaxMinKey{24144}
\def\EPVOUInputsWithCopyingFailureMaxStdDevFloat{2.22670240210988890083854130352847278118133544921875}
\def\EPVOUInputsWithCopyingFailureMeanLen{151}
\def\EPVOUInputsWithCopyingFailureMeanMaxFloat{8.5625}
\def\EPVOUInputsWithCopyingFailureMeanMaxKey{20338}
\def\EPVOUInputsWithCopyingFailureMeanMeanFloat{5.8154149106963668458547545014880597591400146484375}
\def\EPVOUInputsWithCopyingFailureMeanMeanKey{17194}
\def\EPVOUInputsWithCopyingFailureMeanMedianFloat{4.5}
\def\EPVOUInputsWithCopyingFailureMeanMedianKey{24144}
\def\EPVOUInputsWithCopyingFailureMeanMinFloat{4.5}
\def\EPVOUInputsWithCopyingFailureMeanMinKey{24144}
\def\EPVOUInputsWithCopyingFailureMeanStdDevFloat{0.61163973845335173340487244786345399916172027587890625}
\def\EPVOUInputsWithCopyingFailureMedianLen{151}
\def\EPVOUInputsWithCopyingFailureMedianMaxFloat{0.07499999999999999722444243843710864894092082977294921875}
\def\EPVOUInputsWithCopyingFailureMedianMaxKey{20338}
\def\EPVOUInputsWithCopyingFailureMedianMeanFloat{0.057019867549668860895462074722672696225345134735107421875}
\def\EPVOUInputsWithCopyingFailureMedianMeanKey{123}
\def\EPVOUInputsWithCopyingFailureMedianMedianFloat{0.04499999999999999833466546306226518936455249786376953125}
\def\EPVOUInputsWithCopyingFailureMedianMedianKey{12552}
\def\EPVOUInputsWithCopyingFailureMedianMinFloat{0.04499999999999999833466546306226518936455249786376953125}
\def\EPVOUInputsWithCopyingFailureMedianMinKey{12552}
\def\EPVOUInputsWithCopyingFailureMedianStdDevFloat{0.0056726019803516984640889830870946752838790416717529296875}
\def\EPVOUInputsWithCopyingFailureMinLen{151}
\def\EPVOUInputsWithCopyingFailureMinMaxFloat{0}
\def\EPVOUInputsWithCopyingFailureMinMaxKey{50}
\def\EPVOUInputsWithCopyingFailureMinMeanFloat{0}
\def\EPVOUInputsWithCopyingFailureMinMeanKey{50}
\def\EPVOUInputsWithCopyingFailureMinMedianFloat{0}
\def\EPVOUInputsWithCopyingFailureMinMedianKey{50}
\def\EPVOUInputsWithCopyingFailureMinMinFloat{0}
\def\EPVOUInputsWithCopyingFailureMinMinKey{50}
\def\EPVOUInputsWithCopyingFailureMinStdDevFloat{0}
\def\EPVOUInputsWithCopyingFailureStdDevLen{151}
\def\EPVOUInputsWithCopyingFailureStdDevMaxFloat{7.356704000433889945043119951151311397552490234375}
\def\EPVOUInputsWithCopyingFailureStdDevMaxKey{20338}
\def\EPVOUInputsWithCopyingFailureStdDevMeanFloat{3.751373162800970106900422251783311367034912109375}
\def\EPVOUInputsWithCopyingFailureStdDevMeanKey{123}
\def\EPVOUInputsWithCopyingFailureStdDevMedianFloat{2.87228132326901430815269122831523418426513671875}
\def\EPVOUInputsWithCopyingFailureStdDevMedianKey{24144}
\def\EPVOUInputsWithCopyingFailureStdDevMinFloat{2.87228132326901430815269122831523418426513671875}
\def\EPVOUInputsWithCopyingFailureStdDevMinKey{24144}
\def\EPVOUInputsWithCopyingFailureStdDevStdDevFloat{0.485230429293137033308624950223020277917385101318359375}
\def\EPVOULenLen{151}
\def\EPVOULenMaxFloat{4096}
\def\EPVOULenMaxKey{50}
\def\EPVOULenMeanFloat{4096}
\def\EPVOULenMeanKey{50}
\def\EPVOULenMedianFloat{4096}
\def\EPVOULenMedianKey{50}
\def\EPVOULenMinFloat{4096}
\def\EPVOULenMinKey{50}
\def\EPVOULenStdDevFloat{0}
\def\EPVOUMaxAboveDiagLenLen{151}
\def\EPVOUMaxAboveDiagLenMaxFloat{64}
\def\EPVOUMaxAboveDiagLenMaxKey{50}
\def\EPVOUMaxAboveDiagLenMeanFloat{64}
\def\EPVOUMaxAboveDiagLenMeanKey{50}
\def\EPVOUMaxAboveDiagLenMedianFloat{64}
\def\EPVOUMaxAboveDiagLenMedianKey{50}
\def\EPVOUMaxAboveDiagLenMinFloat{64}
\def\EPVOUMaxAboveDiagLenMinKey{50}
\def\EPVOUMaxAboveDiagLenStdDevFloat{0}
\def\EPVOUMaxAboveDiagMaxLen{151}
\def\EPVOUMaxAboveDiagMaxMaxFloat{15.3206729888916015625}
\def\EPVOUMaxAboveDiagMaxMaxKey{6549}
\def\EPVOUMaxAboveDiagMaxMeanFloat{12.2321910858154296875}
\def\EPVOUMaxAboveDiagMaxMeanKey{16284}
\def\EPVOUMaxAboveDiagMaxMedianFloat{8.783293247222900390625}
\def\EPVOUMaxAboveDiagMaxMedianKey{15662}
\def\EPVOUMaxAboveDiagMaxMinFloat{8.5003681182861328125}
\def\EPVOUMaxAboveDiagMaxMinKey{27584}
\def\EPVOUMaxAboveDiagMaxStdDevFloat{1.4382221698760986328125}
\def\EPVOUMaxAboveDiagMeanLen{151}
\def\EPVOUMaxAboveDiagMeanMaxFloat{-3.377856731414794921875}
\def\EPVOUMaxAboveDiagMeanMaxKey{20338}
\def\EPVOUMaxAboveDiagMeanMeanFloat{-4.76670742034912109375}
\def\EPVOUMaxAboveDiagMeanMeanKey{5781}
\def\EPVOUMaxAboveDiagMeanMedianFloat{-5.43878328800201416015625}
\def\EPVOUMaxAboveDiagMeanMedianKey{3254}
\def\EPVOUMaxAboveDiagMeanMinFloat{-5.491270542144775390625}
\def\EPVOUMaxAboveDiagMeanMinKey{23367}
\def\EPVOUMaxAboveDiagMeanStdDevFloat{0.347330272197723388671875}
\def\EPVOUMaxAboveDiagMedianLen{151}
\def\EPVOUMaxAboveDiagMedianMaxFloat{-10.8199706840515137429292735760100185871124267578125}
\def\EPVOUMaxAboveDiagMedianMaxKey{17096}
\def\EPVOUMaxAboveDiagMedianMeanFloat{-11.9607116721007997739434358663856983184814453125}
\def\EPVOUMaxAboveDiagMedianMeanKey{18146}
\def\EPVOUMaxAboveDiagMedianMedianFloat{-14.3800064611434930128552878159098327159881591796875}
\def\EPVOUMaxAboveDiagMedianMedianKey{4810}
\def\EPVOUMaxAboveDiagMedianMinFloat{-14.4131346893310539059029906638897955417633056640625}
\def\EPVOUMaxAboveDiagMedianMinKey{21317}
\def\EPVOUMaxAboveDiagMedianStdDevFloat{0.72163298562000210978339964640326797962188720703125}
\def\EPVOUMaxAboveDiagMinLen{151}
\def\EPVOUMaxAboveDiagMinMaxFloat{-10.883441925048828125}
\def\EPVOUMaxAboveDiagMinMaxKey{4800}
\def\EPVOUMaxAboveDiagMinMeanFloat{-12.17718791961669921875}
\def\EPVOUMaxAboveDiagMinMeanKey{18289}
\def\EPVOUMaxAboveDiagMinMedianFloat{-15.44121456146240234375}
\def\EPVOUMaxAboveDiagMinMedianKey{4810}
\def\EPVOUMaxAboveDiagMinMinFloat{-15.953128814697265625}
\def\EPVOUMaxAboveDiagMinMinKey{21317}
\def\EPVOUMaxAboveDiagMinStdDevFloat{0.887768089771270751953125}
\def\EPVOUMaxAboveDiagStdDevLen{151}
\def\EPVOUMaxAboveDiagStdDevMaxFloat{7.156879901885986328125}
\def\EPVOUMaxAboveDiagStdDevMaxKey{24202}
\def\EPVOUMaxAboveDiagStdDevMeanFloat{6.155471324920654296875}
\def\EPVOUMaxAboveDiagStdDevMeanKey{19004}
\def\EPVOUMaxAboveDiagStdDevMedianFloat{5.3048150539398193359375}
\def\EPVOUMaxAboveDiagStdDevMedianKey{12552}
\def\EPVOUMaxAboveDiagStdDevMinFloat{5.300180912017822265625}
\def\EPVOUMaxAboveDiagStdDevMinKey{4430}
\def\EPVOUMaxAboveDiagStdDevStdDevFloat{0.3326545655727386474609375}
\def\EPVOUMaxLen{151}
\def\EPVOUMaxMaxFloat{43.5103759765625}
\def\EPVOUMaxMaxKey{6532}
\def\EPVOUMaxMeanFloat{34.448307037353515625}
\def\EPVOUMaxMeanKey{12141}
\def\EPVOUMaxMedianFloat{29.68184947967529296875}
\def\EPVOUMaxMedianKey{6159}
\def\EPVOUMaxMinFloat{29.48038482666015625}
\def\EPVOUMaxMinKey{8893}
\def\EPVOUMaxRowDiffLenLen{151}
\def\EPVOUMaxRowDiffLenMaxFloat{64}
\def\EPVOUMaxRowDiffLenMaxKey{50}
\def\EPVOUMaxRowDiffLenMeanFloat{64}
\def\EPVOUMaxRowDiffLenMeanKey{50}
\def\EPVOUMaxRowDiffLenMedianFloat{64}
\def\EPVOUMaxRowDiffLenMedianKey{50}
\def\EPVOUMaxRowDiffLenMinFloat{64}
\def\EPVOUMaxRowDiffLenMinKey{50}
\def\EPVOUMaxRowDiffLenStdDevFloat{0}
\def\EPVOUMaxRowDiffMaxLen{151}
\def\EPVOUMaxRowDiffMaxMaxFloat{84.44426727294921875}
\def\EPVOUMaxRowDiffMaxMaxKey{6532}
\def\EPVOUMaxRowDiffMaxMeanFloat{66.84307861328125}
\def\EPVOUMaxRowDiffMaxMeanKey{32382}
\def\EPVOUMaxRowDiffMaxMedianFloat{55.56808567047119140625}
\def\EPVOUMaxRowDiffMaxMedianKey{6159}
\def\EPVOUMaxRowDiffMaxMinFloat{55.5420989990234375}
\def\EPVOUMaxRowDiffMaxMinKey{20338}
\def\EPVOUMaxRowDiffMaxStdDevFloat{5.184821605682373046875}
\def\EPVOUMaxRowDiffMeanLen{151}
\def\EPVOUMaxRowDiffMeanMaxFloat{46.56969451904296875}
\def\EPVOUMaxRowDiffMeanMaxKey{8721}
\def\EPVOUMaxRowDiffMeanMeanFloat{40.45355224609375}
\def\EPVOUMaxRowDiffMeanMeanKey{4800}
\def\EPVOUMaxRowDiffMeanMedianFloat{35.06380462646484375}
\def\EPVOUMaxRowDiffMeanMedianKey{27584}
\def\EPVOUMaxRowDiffMeanMinFloat{34.5764923095703125}
\def\EPVOUMaxRowDiffMeanMinKey{12552}
\def\EPVOUMaxRowDiffMeanStdDevFloat{2.1866447925567626953125}
\def\EPVOUMaxRowDiffMedianLen{151}
\def\EPVOUMaxRowDiffMedianMaxFloat{34.33314563751221015763803734444081783294677734375}
\def\EPVOUMaxRowDiffMedianMaxKey{13716}
\def\EPVOUMaxRowDiffMedianMeanFloat{27.688725977259753818771059741266071796417236328125}
\def\EPVOUMaxRowDiffMedianMeanKey{30371}
\def\EPVOUMaxRowDiffMedianMedianFloat{21.141228859424590069693294935859739780426025390625}
\def\EPVOUMaxRowDiffMedianMedianKey{27584}
\def\EPVOUMaxRowDiffMedianMinFloat{20.678499402999879208664424368180334568023681640625}
\def\EPVOUMaxRowDiffMedianMinKey{3254}
\def\EPVOUMaxRowDiffMedianStdDevFloat{2.28577509058329741975512661156244575977325439453125}
\def\EPVOUMaxRowDiffMinLen{151}
\def\EPVOUMaxRowDiffMinMaxFloat{34.1792144775390625}
\def\EPVOUMaxRowDiffMinMaxKey{13716}
\def\EPVOUMaxRowDiffMinMeanFloat{27.193737030029296875}
\def\EPVOUMaxRowDiffMinMeanKey{20976}
\def\EPVOUMaxRowDiffMinMedianFloat{20.58052158355712890625}
\def\EPVOUMaxRowDiffMinMedianKey{27584}
\def\EPVOUMaxRowDiffMinMinFloat{20.39118194580078125}
\def\EPVOUMaxRowDiffMinMinKey{3254}
\def\EPVOUMaxRowDiffMinStdDevFloat{2.3966529369354248046875}
\def\EPVOUMaxRowDiffStdDevLen{151}
\def\EPVOUMaxRowDiffStdDevMaxFloat{11.77082061767578125}
\def\EPVOUMaxRowDiffStdDevMaxKey{15662}
\def\EPVOUMaxRowDiffStdDevMeanFloat{8.53007030487060546875}
\def\EPVOUMaxRowDiffStdDevMeanKey{20976}
\def\EPVOUMaxRowDiffStdDevMedianFloat{6.364989757537841796875}
\def\EPVOUMaxRowDiffStdDevMedianKey{23241}
\def\EPVOUMaxRowDiffStdDevMinFloat{6.35368442535400390625}
\def\EPVOUMaxRowDiffStdDevMinKey{16149}
\def\EPVOUMaxRowDiffStdDevStdDevFloat{0.971828401088714599609375}
\def\EPVOUMaxStdDevFloat{2.636967182159423828125}
\def\EPVOUMeanLen{151}
\def\EPVOUMeanMaxFloat{1.270294666290283203125}
\def\EPVOUMeanMaxKey{13654}
\def\EPVOUMeanMeanFloat{0.766811192035675048828125}
\def\EPVOUMeanMeanKey{24262}
\def\EPVOUMeanMedianFloat{0.254229962825775146484375}
\def\EPVOUMeanMedianKey{27584}
\def\EPVOUMeanMinFloat{0.25387966632843017578125}
\def\EPVOUMeanMinKey{15662}
\def\EPVOUMeanStdDevFloat{0.21905656158924102783203125}
\def\EPVOUMedianLen{151}
\def\EPVOUMedianMaxFloat{-21.040074777603148703519764239899814128875732421875}
\def\EPVOUMedianMaxKey{20338}
\def\EPVOUMedianMeanFloat{-24.97501691666659695556518272496759891510009765625}
\def\EPVOUMedianMeanKey{4157}
\def\EPVOUMedianMedianFloat{-29.500096487998963112886485760100185871124267578125}
\def\EPVOUMedianMedianKey{21598}
\def\EPVOUMedianMinFloat{-30.571475696563719992582264239899814128875732421875}
\def\EPVOUMedianMinKey{742}
\def\EPVOUMedianStdDevFloat{1.79188791615966369619172837701626121997833251953125}
\def\EPVOUMinLen{151}
\def\EPVOUMinMaxFloat{-26.7918243408203125}
\def\EPVOUMinMaxKey{6159}
\def\EPVOUMinMeanFloat{-33.55941009521484375}
\def\EPVOUMinMeanKey{13654}
\def\EPVOUMinMedianFloat{-41.37764739990234375}
\def\EPVOUMinMedianKey{24202}
\def\EPVOUMinMinFloat{-41.449047088623046875}
\def\EPVOUMinMinKey{31308}
\def\EPVOUMinStdDevFloat{3.0927946567535400390625}
\def\EPVOUOffDiagonalAbsLenLen{151}
\def\EPVOUOffDiagonalAbsLenMaxFloat{4032}
\def\EPVOUOffDiagonalAbsLenMaxKey{50}
\def\EPVOUOffDiagonalAbsLenMeanFloat{4032}
\def\EPVOUOffDiagonalAbsLenMeanKey{50}
\def\EPVOUOffDiagonalAbsLenMedianFloat{4032}
\def\EPVOUOffDiagonalAbsLenMedianKey{50}
\def\EPVOUOffDiagonalAbsLenMinFloat{4032}
\def\EPVOUOffDiagonalAbsLenMinKey{50}
\def\EPVOUOffDiagonalAbsLenStdDevFloat{0}
\def\EPVOUOffDiagonalAbsMaxLen{151}
\def\EPVOUOffDiagonalAbsMaxMaxFloat{41.449047088623046875}
\def\EPVOUOffDiagonalAbsMaxMaxKey{31308}
\def\EPVOUOffDiagonalAbsMaxMeanFloat{33.55941009521484375}
\def\EPVOUOffDiagonalAbsMaxMeanKey{13654}
\def\EPVOUOffDiagonalAbsMaxMedianFloat{27.690407276153564453125}
\def\EPVOUOffDiagonalAbsMaxMedianKey{6155}
\def\EPVOUOffDiagonalAbsMaxMinFloat{26.7918243408203125}
\def\EPVOUOffDiagonalAbsMaxMinKey{6159}
\def\EPVOUOffDiagonalAbsMaxStdDevFloat{3.0927946567535400390625}
\def\EPVOUOffDiagonalAbsMeanLen{151}
\def\EPVOUOffDiagonalAbsMeanMaxFloat{9.91444873809814453125}
\def\EPVOUOffDiagonalAbsMeanMaxKey{8721}
\def\EPVOUOffDiagonalAbsMeanMeanFloat{8.2561702728271484375}
\def\EPVOUOffDiagonalAbsMeanMeanKey{18146}
\def\EPVOUOffDiagonalAbsMeanMedianFloat{6.547023296356201171875}
\def\EPVOUOffDiagonalAbsMeanMedianKey{12552}
\def\EPVOUOffDiagonalAbsMeanMinFloat{6.449390888214111328125}
\def\EPVOUOffDiagonalAbsMeanMinKey{27584}
\def\EPVOUOffDiagonalAbsMeanStdDevFloat{0.627035319805145263671875}
\def\EPVOUOffDiagonalAbsMedianLen{151}
\def\EPVOUOffDiagonalAbsMedianMaxFloat{0.12448752742260695003384540768820443190634250640869140625}
\def\EPVOUOffDiagonalAbsMedianMaxKey{2306}
\def\EPVOUOffDiagonalAbsMedianMeanFloat{0.076805924465078001528439699541195295751094818115234375}
\def\EPVOUOffDiagonalAbsMedianMeanKey{11498}
\def\EPVOUOffDiagonalAbsMedianMedianFloat{0.0460990130901336725433026231257827021181583404541015625}
\def\EPVOUOffDiagonalAbsMedianMedianKey{2549}
\def\EPVOUOffDiagonalAbsMedianMinFloat{0.042559843659400943549631080031758756376802921295166015625}
\def\EPVOUOffDiagonalAbsMedianMinKey{17096}
\def\EPVOUOffDiagonalAbsMedianStdDevFloat{0.0165229799217978222392044784783138311468064785003662109375}
\def\EPVOUOffDiagonalAbsMinLen{151}
\def\EPVOUOffDiagonalAbsMinMaxFloat{0.0248878002166748046875}
\def\EPVOUOffDiagonalAbsMinMaxKey{8893}
\def\EPVOUOffDiagonalAbsMinMeanFloat{0.00342048169113695621490478515625}
\def\EPVOUOffDiagonalAbsMinMeanKey{16284}
\def\EPVOUOffDiagonalAbsMinMedianFloat{0.0000067651271820068359375}
\def\EPVOUOffDiagonalAbsMinMedianKey{4305}
\def\EPVOUOffDiagonalAbsMinMinFloat{0.00000417232513427734375}
\def\EPVOUOffDiagonalAbsMinMinKey{30899}
\def\EPVOUOffDiagonalAbsMinStdDevFloat{0.00384899810887873172760009765625}
\def\EPVOUOffDiagonalAbsStdDevLen{151}
\def\EPVOUOffDiagonalAbsStdDevMaxFloat{6.53835296630859375}
\def\EPVOUOffDiagonalAbsStdDevMaxKey{11611}
\def\EPVOUOffDiagonalAbsStdDevMeanFloat{5.523849964141845703125}
\def\EPVOUOffDiagonalAbsStdDevMeanKey{10248}
\def\EPVOUOffDiagonalAbsStdDevMedianFloat{4.60273826122283935546875}
\def\EPVOUOffDiagonalAbsStdDevMedianKey{12552}
\def\EPVOUOffDiagonalAbsStdDevMinFloat{4.534488201141357421875}
\def\EPVOUOffDiagonalAbsStdDevMinKey{27584}
\def\EPVOUOffDiagonalAbsStdDevStdDevFloat{0.382057607173919677734375}
\def\EPVOUOffDiagonalLenLen{151}
\def\EPVOUOffDiagonalLenMaxFloat{4032}
\def\EPVOUOffDiagonalLenMaxKey{50}
\def\EPVOUOffDiagonalLenMeanFloat{4032}
\def\EPVOUOffDiagonalLenMeanKey{50}
\def\EPVOUOffDiagonalLenMedianFloat{4032}
\def\EPVOUOffDiagonalLenMedianKey{50}
\def\EPVOUOffDiagonalLenMinFloat{4032}
\def\EPVOUOffDiagonalLenMinKey{50}
\def\EPVOUOffDiagonalLenStdDevFloat{0}
\def\EPVOUOffDiagonalMaxLen{151}
\def\EPVOUOffDiagonalMaxMaxFloat{31.9390411376953125}
\def\EPVOUOffDiagonalMaxMaxKey{6532}
\def\EPVOUOffDiagonalMaxMeanFloat{23.8175640106201171875}
\def\EPVOUOffDiagonalMaxMeanKey{50}
\def\EPVOUOffDiagonalMaxMedianFloat{18.88566684722900390625}
\def\EPVOUOffDiagonalMaxMedianKey{30899}
\def\EPVOUOffDiagonalMaxMinFloat{18.794094085693359375}
\def\EPVOUOffDiagonalMaxMinKey{7884}
\def\EPVOUOffDiagonalMaxStdDevFloat{2.3993456363677978515625}
\def\EPVOUOffDiagonalMeanLen{151}
\def\EPVOUOffDiagonalMeanMaxFloat{0.957134425640106201171875}
\def\EPVOUOffDiagonalMeanMaxKey{13654}
\def\EPVOUOffDiagonalMeanMeanFloat{0.4535073935985565185546875}
\def\EPVOUOffDiagonalMeanMeanKey{24262}
\def\EPVOUOffDiagonalMeanMedianFloat{-0.041580063290894031524658203125}
\def\EPVOUOffDiagonalMeanMedianKey{27584}
\def\EPVOUOffDiagonalMeanMinFloat{-0.07224746048450469970703125}
\def\EPVOUOffDiagonalMeanMinKey{15662}
\def\EPVOUOffDiagonalMeanStdDevFloat{0.2172609269618988037109375}
\def\EPVOUOffDiagonalMedianLen{151}
\def\EPVOUOffDiagonalMedianMaxFloat{-21.07560273170471276671378291212022304534912109375}
\def\EPVOUOffDiagonalMedianMaxKey{20338}
\def\EPVOUOffDiagonalMedianMeanFloat{-25.02830975122009959932256606407463550567626953125}
\def\EPVOUOffDiagonalMedianMeanKey{6589}
\def\EPVOUOffDiagonalMedianMedianFloat{-29.6933908605575567207779386080801486968994140625}
\def\EPVOUOffDiagonalMedianMedianKey{21598}
\def\EPVOUOffDiagonalMedianMinFloat{-30.6773069953918451346908113919198513031005859375}
\def\EPVOUOffDiagonalMedianMinKey{742}
\def\EPVOUOffDiagonalMedianStdDevFloat{1.80252330944235961140975632588379085063934326171875}
\def\EPVOUOffDiagonalMinLen{151}
\def\EPVOUOffDiagonalMinMaxFloat{-26.7918243408203125}
\def\EPVOUOffDiagonalMinMaxKey{6159}
\def\EPVOUOffDiagonalMinMeanFloat{-33.55941009521484375}
\def\EPVOUOffDiagonalMinMeanKey{13654}
\def\EPVOUOffDiagonalMinMedianFloat{-41.37764739990234375}
\def\EPVOUOffDiagonalMinMedianKey{24202}
\def\EPVOUOffDiagonalMinMinFloat{-41.449047088623046875}
\def\EPVOUOffDiagonalMinMinKey{31308}
\def\EPVOUOffDiagonalMinStdDevFloat{3.0927946567535400390625}
\def\EPVOUOffDiagonalStdDevLen{151}
\def\EPVOUOffDiagonalStdDevMaxFloat{11.85287189483642578125}
\def\EPVOUOffDiagonalStdDevMaxKey{8721}
\def\EPVOUOffDiagonalStdDevMeanFloat{9.92167949676513671875}
\def\EPVOUOffDiagonalStdDevMeanKey{12561}
\def\EPVOUOffDiagonalStdDevMedianFloat{7.99528789520263671875}
\def\EPVOUOffDiagonalStdDevMedianKey{12552}
\def\EPVOUOffDiagonalStdDevMinFloat{7.8838596343994140625}
\def\EPVOUOffDiagonalStdDevMinKey{27584}
\def\EPVOUOffDiagonalStdDevStdDevFloat{0.72374725341796875}
\def\EPVOUStdDevLen{151}
\def\EPVOUStdDevMaxFloat{12.08998966217041015625}
\def\EPVOUStdDevMaxKey{8721}
\def\EPVOUStdDevMeanFloat{10.17801570892333984375}
\def\EPVOUStdDevMeanKey{12561}
\def\EPVOUStdDevMedianFloat{8.2743537425994873046875}
\def\EPVOUStdDevMedianKey{12552}
\def\EPVOUStdDevMinFloat{8.185375213623046875}
\def\EPVOUStdDevMinKey{27584}
\def\EPVOUStdDevStdDevFloat{0.716039836406707763671875}
\def\EQKEErrBoundMaxDiffExactLen{151}
\def\EQKEErrBoundMaxDiffExactMaxFloat{4.611191272735595703125}
\def\EQKEErrBoundMaxDiffExactMaxKey{4647}
\def\EQKEErrBoundMaxDiffExactMeanFloat{1.833191962431598209803951249341480433940887451171875}
\def\EQKEErrBoundMaxDiffExactMeanKey{6204}
\def\EQKEErrBoundMaxDiffExactMedianFloat{1.14899003505706787109375}
\def\EQKEErrBoundMaxDiffExactMedianKey{27300}
\def\EQKEErrBoundMaxDiffExactMinFloat{1.11769974231719970703125}
\def\EQKEErrBoundMaxDiffExactMinKey{4305}
\def\EQKEErrBoundMaxDiffExactStdDevFloat{0.433994588457784213897383551739039830863475799560546875}
\def\EQKEErrBoundMaxDiffLen{151}
\def\EQKEErrBoundMaxDiffMaxFloat{7.0167236328125}
\def\EQKEErrBoundMaxDiffMaxKey{4647}
\def\EQKEErrBoundMaxDiffMeanFloat{5.06559399105855145961641028407029807567596435546875}
\def\EQKEErrBoundMaxDiffMeanKey{1412}
\def\EQKEErrBoundMaxDiffMedianFloat{3.94751203060150146484375}
\def\EQKEErrBoundMaxDiffMedianKey{6532}
\def\EQKEErrBoundMaxDiffMinFloat{3.858226299285888671875}
\def\EQKEErrBoundMaxDiffMinKey{32374}
\def\EQKEErrBoundMaxDiffStdDevFloat{0.535209767337012198851198263582773506641387939453125}
\def\EQKEErrBoundMaxDiffSubproductLen{151}
\def\EQKEErrBoundMaxDiffSubproductMaxFloat{7.0167236328125}
\def\EQKEErrBoundMaxDiffSubproductMaxKey{4647}
\def\EQKEErrBoundMaxDiffSubproductMeanFloat{5.06559399105855145961641028407029807567596435546875}
\def\EQKEErrBoundMaxDiffSubproductMeanKey{1412}
\def\EQKEErrBoundMaxDiffSubproductMedianFloat{3.94751203060150146484375}
\def\EQKEErrBoundMaxDiffSubproductMedianKey{6532}
\def\EQKEErrBoundMaxDiffSubproductMinFloat{3.858226299285888671875}
\def\EQKEErrBoundMaxDiffSubproductMinKey{32374}
\def\EQKEErrBoundMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMaxFloat{144.185821533203125}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMaxKey{20338}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMeanFloat{94.6145395948397407437369110994040966033935546875}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMeanKey{16149}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMedianFloat{78.5718860626220703125}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMedianKey{32374}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMinFloat{77.82788848876953125}
\def\EQKEErrBoundMaxDiffSubproductRecursiveMinKey{1681}
\def\EQKEErrBoundMaxDiffSubproductRecursiveStdDevFloat{7.51010078068381492499838714138604700565338134765625}
\def\EQKEErrBoundMaxDiffSubproductStdDevFloat{0.535209767337012198851198263582773506641387939453125}
\def\EQKEErrBoundMeanMaxDiffLen{151}
\def\EQKEErrBoundMeanMaxDiffMaxFloat{7.015990734100341796875}
\def\EQKEErrBoundMeanMaxDiffMaxKey{4647}
\def\EQKEErrBoundMeanMaxDiffMeanFloat{5.07849087778306174101317083113826811313629150390625}
\def\EQKEErrBoundMeanMaxDiffMeanKey{5781}
\def\EQKEErrBoundMeanMaxDiffMedianFloat{3.975169837474822998046875}
\def\EQKEErrBoundMeanMaxDiffMedianKey{6532}
\def\EQKEErrBoundMeanMaxDiffMinFloat{3.8679935932159423828125}
\def\EQKEErrBoundMeanMaxDiffMinKey{32374}
\def\EQKEErrBoundMeanMaxDiffStdDevFloat{0.53139427036718023256156584466225467622280120849609375}
\def\EQKEErrBoundMeanMaxDiffSubproductLen{151}
\def\EQKEErrBoundMeanMaxDiffSubproductMaxFloat{7.015990734100341796875}
\def\EQKEErrBoundMeanMaxDiffSubproductMaxKey{4647}
\def\EQKEErrBoundMeanMaxDiffSubproductMeanFloat{5.07849087778306174101317083113826811313629150390625}
\def\EQKEErrBoundMeanMaxDiffSubproductMeanKey{5781}
\def\EQKEErrBoundMeanMaxDiffSubproductMedianFloat{3.975169837474822998046875}
\def\EQKEErrBoundMeanMaxDiffSubproductMedianKey{6532}
\def\EQKEErrBoundMeanMaxDiffSubproductMinFloat{3.8679935932159423828125}
\def\EQKEErrBoundMeanMaxDiffSubproductMinKey{32374}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMaxFloat{144.12237548828125}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMaxKey{20338}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMeanFloat{94.439607481293336377348168753087520599365234375}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMeanKey{16149}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMedianFloat{78.6455821990966796875}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMedianKey{6532}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMinFloat{78.29946136474609375}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveMinKey{1681}
\def\EQKEErrBoundMeanMaxDiffSubproductRecursiveStdDevFloat{7.5064594809721061352547621936537325382232666015625}
\def\EQKEErrBoundMeanMaxDiffSubproductStdDevFloat{0.53139427036718023256156584466225467622280120849609375}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMaxFloat{142.3176116943359375}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMaxKey{20338}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMeanFloat{96.2863692732046700939463335089385509490966796875}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMeanKey{30684}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMedianFloat{79.6405811309814453125}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMedianKey{32374}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMinFloat{78.46202850341796875}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveMinKey{1681}
\def\EQKEErrBoundMeanRecursiveMaxDiffSubproductRecursiveStdDevFloat{7.42529095414309292522148098214529454708099365234375}
\def\EQKEErrBoundSvdLen{151}
\def\EQKEErrBoundSvdMaxFloat{18.5705165863037109375}
\def\EQKEErrBoundSvdMaxKey{4647}
\def\EQKEErrBoundSvdMeanFloat{10.482428222302569764678992214612662792205810546875}
\def\EQKEErrBoundSvdMeanKey{24202}
\def\EQKEErrBoundSvdMedianFloat{6.97518265247344970703125}
\def\EQKEErrBoundSvdMedianKey{913}
\def\EQKEErrBoundSvdMinFloat{6.5847263336181640625}
\def\EQKEErrBoundSvdMinKey{4305}
\def\EQKEErrBoundSvdStdDevFloat{1.8909835564329757762180861391243524849414825439453125}
\def\EQKEErrFirstSingularLen{151}
\def\EQKEErrFirstSingularMaxFloat{13.1313343048095703125}
\def\EQKEErrFirstSingularMaxKey{4647}
\def\EQKEErrFirstSingularMeanFloat{7.412195960417488294069698895327746868133544921875}
\def\EQKEErrFirstSingularMeanKey{24202}
\def\EQKEErrFirstSingularMedianFloat{4.932198047637939453125}
\def\EQKEErrFirstSingularMedianKey{913}
\def\EQKEErrFirstSingularMinFloat{4.656103610992431640625}
\def\EQKEErrFirstSingularMinKey{4305}
\def\EQKEErrFirstSingularSqrtTwoLen{151}
\def\EQKEErrFirstSingularSqrtTwoMaxFloat{18.5705108642578125}
\def\EQKEErrFirstSingularSqrtTwoMaxKey{4647}
\def\EQKEErrFirstSingularSqrtTwoMeanFloat{10.4824278370434083029749672277830541133880615234375}
\def\EQKEErrFirstSingularSqrtTwoMeanKey{24202}
\def\EQKEErrFirstSingularSqrtTwoMedianFloat{6.97518122196197509765625}
\def\EQKEErrFirstSingularSqrtTwoMedianKey{913}
\def\EQKEErrFirstSingularSqrtTwoMinFloat{6.584724903106689453125}
\def\EQKEErrFirstSingularSqrtTwoMinKey{4305}
\def\EQKEErrFirstSingularSqrtTwoStdDevFloat{1.890983479690425017594179735169745981693267822265625}
\def\EQKEErrFirstSingularStdDevFloat{1.3371272511718383935175324950250796973705291748046875}
\def\EQKEErrFroNormLen{151}
\def\EQKEErrFroNormMaxFloat{16.3108386993408203125}
\def\EQKEErrFroNormMaxKey{2306}
\def\EQKEErrFroNormMeanFloat{11.6335738668378620985777160967700183391571044921875}
\def\EQKEErrFroNormMeanKey{19488}
\def\EQKEErrFroNormMedianFloat{9.127948284149169921875}
\def\EQKEErrFroNormMedianKey{9134}
\def\EQKEErrFroNormMinFloat{9.04713153839111328125}
\def\EQKEErrFroNormMinKey{4305}
\def\EQKEErrFroNormSqrtTwoLen{151}
\def\EQKEErrFroNormSqrtTwoMaxFloat{23.06700897216796875}
\def\EQKEErrFroNormSqrtTwoMaxKey{2306}
\def\EQKEErrFroNormSqrtTwoMeanFloat{16.452357664803006542797447764314711093902587890625}
\def\EQKEErrFroNormSqrtTwoMeanKey{19488}
\def\EQKEErrFroNormSqrtTwoMedianFloat{12.90886783599853515625}
\def\EQKEErrFroNormSqrtTwoMedianKey{9134}
\def\EQKEErrFroNormSqrtTwoMinFloat{12.79457569122314453125}
\def\EQKEErrFroNormSqrtTwoMinKey{4305}
\def\EQKEErrFroNormSqrtTwoStdDevFloat{1.828832538874853863575253853923641145229339599609375}
\def\EQKEErrFroNormStdDevFloat{1.2931798794723354806279758122400380671024322509765625}
\def\EQKEErrLen{4096}
\def\EQKEErrMaxAbsLen{151}
\def\EQKEErrMaxAbsMaxFloat{2.68619441986083984375}
\def\EQKEErrMaxAbsMaxKey{4647}
\def\EQKEErrMaxAbsMeanFloat{1.0350526519958547222444167346111498773097991943359375}
\def\EQKEErrMaxAbsMeanKey{12493}
\def\EQKEErrMaxAbsMedianFloat{0.6437278091907501220703125}
\def\EQKEErrMaxAbsMedianKey{4305}
\def\EQKEErrMaxAbsMinFloat{0.6343033313751220703125}
\def\EQKEErrMaxAbsMinKey{913}
\def\EQKEErrMaxAbsStdDevFloat{0.266431363271176613327639870476559735834598541259765625}
\def\EQKEErrMaxLen{151}
\def\EQKEErrMaxMaxFloat{2.68619441986083984375}
\def\EQKEErrMaxMaxKey{4647}
\def\EQKEErrMaxMeanFloat{0.985642910003662109375}
\def\EQKEErrMaxMeanKey{11598}
\def\EQKEErrMaxMedianFloat{0.6266894042491912841796875}
\def\EQKEErrMaxMedianKey{32374}
\def\EQKEErrMaxMinFloat{0.591628551483154296875}
\def\EQKEErrMaxMinKey{913}
\def\EQKEErrMaxRowDiffLen{151}
\def\EQKEErrMaxRowDiffMaxFloat{4.611191272735595703125}
\def\EQKEErrMaxRowDiffMaxKey{4647}
\def\EQKEErrMaxRowDiffMeanFloat{1.833191962431598209803951249341480433940887451171875}
\def\EQKEErrMaxRowDiffMeanKey{6204}
\def\EQKEErrMaxRowDiffMedianFloat{1.14899003505706787109375}
\def\EQKEErrMaxRowDiffMedianKey{27300}
\def\EQKEErrMaxRowDiffMinFloat{1.11769974231719970703125}
\def\EQKEErrMaxRowDiffMinKey{4305}
\def\EQKEErrMaxRowDiffStdDevFloat{0.433994588457784213897383551739039830863475799560546875}
\def\EQKEErrMaxStdDevFloat{0.265725612640380859375}
\def\EQKEErrMeanDimZeroNormLen{151}
\def\EQKEErrMeanDimZeroNormMaxFloat{0.075971461832523345947265625}
\def\EQKEErrMeanDimZeroNormMaxKey{4647}
\def\EQKEErrMeanDimZeroNormMeanFloat{0.029499253054575021171235249539677170105278491973876953125}
\def\EQKEErrMeanDimZeroNormMeanKey{18668}
\def\EQKEErrMeanDimZeroNormMedianFloat{0.01210566074587404727935791015625}
\def\EQKEErrMeanDimZeroNormMedianKey{6159}
\def\EQKEErrMeanDimZeroNormMinFloat{0.01146031916141510009765625}
\def\EQKEErrMeanDimZeroNormMinKey{27300}
\def\EQKEErrMeanDimZeroNormStdDevFloat{0.01100106781816490193748325765454865177161991596221923828125}
\def\EQKEErrMeanLen{151}
\def\EQKEErrMeanMaxFloat{0.000879295985214412212371826171875}
\def\EQKEErrMeanMaxKey{6532}
\def\EQKEErrMeanMeanFloat{0.00003640954309958033263683319091796875}
\def\EQKEErrMeanMeanKey{16069}
\def\EQKEErrMeanMedianFloat{-0.00073912265361286699771881103515625}
\def\EQKEErrMeanMedianKey{17197}
\def\EQKEErrMeanMinFloat{-0.000765967182815074920654296875}
\def\EQKEErrMeanMinKey{8840}
\def\EQKEErrMeanStdDevFloat{0.00025918605388142168521881103515625}
\def\EQKEErrMedianLen{151}
\def\EQKEErrMedianMaxFloat{-0.38664292395114896461194575749686919152736663818359375}
\def\EQKEErrMedianMaxKey{4305}
\def\EQKEErrMedianMeanFloat{-0.56785823806429525095751387198106385767459869384765625}
\def\EQKEErrMedianMeanKey{13036}
\def\EQKEErrMedianMedianFloat{-0.8059551984071731123293602649937383830547332763671875}
\def\EQKEErrMedianMedianKey{2306}
\def\EQKEErrMedianMinFloat{-0.8099833533167839494382178600062616169452667236328125}
\def\EQKEErrMedianMinKey{6910}
\def\EQKEErrMedianStdDevFloat{0.07750836964619589597447202322655357420444488525390625}
\def\EQKEErrMinLen{151}
\def\EQKEErrMinMaxFloat{-0.62433040142059326171875}
\def\EQKEErrMinMaxKey{27300}
\def\EQKEErrMinMeanFloat{-0.957435071468353271484375}
\def\EQKEErrMinMeanKey{24144}
\def\EQKEErrMinMedianFloat{-1.88636100292205810546875}
\def\EQKEErrMinMedianKey{2306}
\def\EQKEErrMinMinFloat{-1.92499697208404541015625}
\def\EQKEErrMinMinKey{4647}
\def\EQKEErrMinStdDevFloat{0.2189793288707733154296875}
\def\EQKEErrProdFirstSingularLen{151}
\def\EQKEErrProdFirstSingularMaxFloat{41.19826851901552089429969782941043376922607421875}
\def\EQKEErrProdFirstSingularMaxKey{6082}
\def\EQKEErrProdFirstSingularMeanFloat{31.151637164015024694663225091062486171722412109375}
\def\EQKEErrProdFirstSingularMeanKey{13036}
\def\EQKEErrProdFirstSingularMedianFloat{24.796069730809801257009894470684230327606201171875}
\def\EQKEErrProdFirstSingularMedianKey{1681}
\def\EQKEErrProdFirstSingularMinFloat{24.5938630089683414325918420217931270599365234375}
\def\EQKEErrProdFirstSingularMinKey{20294}
\def\EQKEErrProdFirstSingularSqrtTwoLen{151}
\def\EQKEErrProdFirstSingularSqrtTwoMaxFloat{58.26315008588027666291964123956859111785888671875}
\def\EQKEErrProdFirstSingularSqrtTwoMaxKey{6082}
\def\EQKEErrProdFirstSingularSqrtTwoMeanFloat{44.055067767475776463470538146793842315673828125}
\def\EQKEErrProdFirstSingularSqrtTwoMeanKey{13036}
\def\EQKEErrProdFirstSingularSqrtTwoMedianFloat{35.06693810686019929789836169220507144927978515625}
\def\EQKEErrProdFirstSingularSqrtTwoMedianKey{1681}
\def\EQKEErrProdFirstSingularSqrtTwoMinFloat{34.78097461842900628425923059694468975067138671875}
\def\EQKEErrProdFirstSingularSqrtTwoMinKey{20294}
\def\EQKEErrProdFirstSingularSqrtTwoStdDevFloat{4.55210180881911607997380997403524816036224365234375}
\def\EQKEErrProdFirstSingularStdDevFloat{3.218822057667546143733261487795971333980560302734375}
\def\EQKEErrProdFroNormLen{151}
\def\EQKEErrProdFroNormMaxFloat{1975.957483143644140000105835497379302978515625}
\def\EQKEErrProdFroNormMaxKey{25516}
\def\EQKEErrProdFroNormMeanFloat{1734.890540940356686405721120536327362060546875}
\def\EQKEErrProdFroNormMeanKey{4810}
\def\EQKEErrProdFroNormMedianFloat{1522.70632183588531916029751300811767578125}
\def\EQKEErrProdFroNormMedianKey{6532}
\def\EQKEErrProdFroNormMinFloat{1507.948378037319571376428939402103424072265625}
\def\EQKEErrProdFroNormMinKey{28090}
\def\EQKEErrProdFroNormSqrtTwoLen{151}
\def\EQKEErrProdFroNormSqrtTwoMaxFloat{2794.42587133434790302999317646026611328125}
\def\EQKEErrProdFroNormSqrtTwoMaxKey{25516}
\def\EQKEErrProdFroNormSqrtTwoMeanFloat{2453.50573223064702688134275376796722412109375}
\def\EQKEErrProdFroNormSqrtTwoMeanKey{4810}
\def\EQKEErrProdFroNormSqrtTwoMedianFloat{2153.4319318515599661623127758502960205078125}
\def\EQKEErrProdFroNormSqrtTwoMedianKey{6532}
\def\EQKEErrProdFroNormSqrtTwoMinFloat{2132.56104757888851963798515498638153076171875}
\def\EQKEErrProdFroNormSqrtTwoMinKey{28090}
\def\EQKEErrProdFroNormSqrtTwoStdDevFloat{126.4513748861005524304346181452274322509765625}
\def\EQKEErrProdFroNormStdDevFloat{89.414624672323981258159619756042957305908203125}
\def\EQKEErrSimpleFirstSingularLen{151}
\def\EQKEErrSimpleFirstSingularMaxFloat{29.37561798095703125}
\def\EQKEErrSimpleFirstSingularMaxKey{123}
\def\EQKEErrSimpleFirstSingularMeanFloat{12.241859186564060024693390005268156528472900390625}
\def\EQKEErrSimpleFirstSingularMeanKey{8048}
\def\EQKEErrSimpleFirstSingularMedianFloat{7.563899993896484375}
\def\EQKEErrSimpleFirstSingularMedianKey{32374}
\def\EQKEErrSimpleFirstSingularMinFloat{7.4513759613037109375}
\def\EQKEErrSimpleFirstSingularMinKey{27671}
\def\EQKEErrSimpleFirstSingularSqrtTwoLen{151}
\def\EQKEErrSimpleFirstSingularSqrtTwoMaxFloat{41.54339599609375}
\def\EQKEErrSimpleFirstSingularSqrtTwoMaxKey{123}
\def\EQKEErrSimpleFirstSingularSqrtTwoMeanFloat{17.312603028404790705963023356162011623382568359375}
\def\EQKEErrSimpleFirstSingularSqrtTwoMeanKey{8048}
\def\EQKEErrSimpleFirstSingularSqrtTwoMedianFloat{10.6969699859619140625}
\def\EQKEErrSimpleFirstSingularSqrtTwoMedianKey{32374}
\def\EQKEErrSimpleFirstSingularSqrtTwoMinFloat{10.53783702850341796875}
\def\EQKEErrSimpleFirstSingularSqrtTwoMinKey{27671}
\def\EQKEErrSimpleFirstSingularSqrtTwoStdDevFloat{4.598987186899702095388420275412499904632568359375}
\def\EQKEErrSimpleFirstSingularStdDevFloat{3.251975118555731736336156245670281350612640380859375}
\def\EQKEErrSimpleFroNormLen{151}
\def\EQKEErrSimpleFroNormMaxFloat{31.7148590087890625}
\def\EQKEErrSimpleFroNormMaxKey{123}
\def\EQKEErrSimpleFroNormMeanFloat{17.228771190769624155336714466102421283721923828125}
\def\EQKEErrSimpleFroNormMeanKey{19917}
\def\EQKEErrSimpleFroNormMedianFloat{12.58577060699462890625}
\def\EQKEErrSimpleFroNormMedianKey{32374}
\def\EQKEErrSimpleFroNormMinFloat{12.5794162750244140625}
\def\EQKEErrSimpleFroNormMinKey{27671}
\def\EQKEErrSimpleFroNormSqrtTwoLen{151}
\def\EQKEErrSimpleFroNormSqrtTwoMaxFloat{44.851581573486328125}
\def\EQKEErrSimpleFroNormSqrtTwoMaxKey{123}
\def\EQKEErrSimpleFroNormSqrtTwoMeanFloat{24.36516135259969217941034003160893917083740234375}
\def\EQKEErrSimpleFroNormSqrtTwoMeanKey{19917}
\def\EQKEErrSimpleFroNormSqrtTwoMedianFloat{17.79896640777587890625}
\def\EQKEErrSimpleFroNormSqrtTwoMedianKey{32374}
\def\EQKEErrSimpleFroNormSqrtTwoMinFloat{17.7899799346923828125}
\def\EQKEErrSimpleFroNormSqrtTwoMinKey{27671}
\def\EQKEErrSimpleFroNormSqrtTwoStdDevFloat{4.024364827723164950157297425903379917144775390625}
\def\EQKEErrSimpleFroNormStdDevFloat{2.845655737927334616443886261549778282642364501953125}
\def\EQKEErrSimpleLen{4096}
\def\EQKEErrSimpleMaxAbsLen{151}
\def\EQKEErrSimpleMaxAbsMaxFloat{3.2045767307281494140625}
\def\EQKEErrSimpleMaxAbsMaxKey{4647}
\def\EQKEErrSimpleMaxAbsMeanFloat{1.54711938535930304539078861125744879245758056640625}
\def\EQKEErrSimpleMaxAbsMeanKey{19488}
\def\EQKEErrSimpleMaxAbsMedianFloat{0.9919011592864990234375}
\def\EQKEErrSimpleMaxAbsMedianKey{27671}
\def\EQKEErrSimpleMaxAbsMinFloat{0.97127246856689453125}
\def\EQKEErrSimpleMaxAbsMinKey{23367}
\def\EQKEErrSimpleMaxAbsStdDevFloat{0.400559609592018972534788190387189388275146484375}
\def\EQKEErrSimpleMaxLen{151}
\def\EQKEErrSimpleMaxMaxFloat{3.2045767307281494140625}
\def\EQKEErrSimpleMaxMaxKey{4647}
\def\EQKEErrSimpleMaxMeanFloat{1.40300524234771728515625}
\def\EQKEErrSimpleMaxMeanKey{4729}
\def\EQKEErrSimpleMaxMedianFloat{0.7941494882106781005859375}
\def\EQKEErrSimpleMaxMedianKey{22286}
\def\EQKEErrSimpleMaxMinFloat{0.7576448917388916015625}
\def\EQKEErrSimpleMaxMinKey{9816}
\def\EQKEErrSimpleMaxRowDiffLen{151}
\def\EQKEErrSimpleMaxRowDiffMaxFloat{5.4248828887939453125}
\def\EQKEErrSimpleMaxRowDiffMaxKey{4647}
\def\EQKEErrSimpleMaxRowDiffMeanFloat{2.4267748831123707731194372172467410564422607421875}
\def\EQKEErrSimpleMaxRowDiffMeanKey{24173}
\def\EQKEErrSimpleMaxRowDiffMedianFloat{1.432242333889007568359375}
\def\EQKEErrSimpleMaxRowDiffMedianKey{23367}
\def\EQKEErrSimpleMaxRowDiffMinFloat{1.4083254337310791015625}
\def\EQKEErrSimpleMaxRowDiffMinKey{6159}
\def\EQKEErrSimpleMaxRowDiffStdDevFloat{0.62293880677555735214667720356374047696590423583984375}
\def\EQKEErrSimpleMaxStdDevFloat{0.4015242755413055419921875}
\def\EQKEErrSimpleMeanDimZeroNormLen{151}
\def\EQKEErrSimpleMeanDimZeroNormMaxFloat{0.272365033626556396484375}
\def\EQKEErrSimpleMeanDimZeroNormMaxKey{12141}
\def\EQKEErrSimpleMeanDimZeroNormMeanFloat{0.060442485433343233480751877095826785080134868621826171875}
\def\EQKEErrSimpleMeanDimZeroNormMeanKey{14929}
\def\EQKEErrSimpleMeanDimZeroNormMedianFloat{0.0141880898736417293548583984375}
\def\EQKEErrSimpleMeanDimZeroNormMedianKey{27300}
\def\EQKEErrSimpleMeanDimZeroNormMinFloat{0.013517717830836772918701171875}
\def\EQKEErrSimpleMeanDimZeroNormMinKey{6159}
\def\EQKEErrSimpleMeanDimZeroNormStdDevFloat{0.03971589832070109016282088987281895242631435394287109375}
\def\EQKEErrSimpleMeanLen{151}
\def\EQKEErrSimpleMeanMaxFloat{0.0099735148251056671142578125}
\def\EQKEErrSimpleMeanMaxKey{11130}
\def\EQKEErrSimpleMeanMeanFloat{-0.001165236695669591426849365234375}
\def\EQKEErrSimpleMeanMeanKey{12552}
\def\EQKEErrSimpleMeanMedianFloat{-0.02088205516338348388671875}
\def\EQKEErrSimpleMeanMedianKey{123}
\def\EQKEErrSimpleMeanMinFloat{-0.0293655693531036376953125}
\def\EQKEErrSimpleMeanMinKey{12141}
\def\EQKEErrSimpleMeanStdDevFloat{0.004684514366090297698974609375}
\def\EQKEErrSimpleMedianLen{151}
\def\EQKEErrSimpleMedianMaxFloat{-0.51253496706485746070569575749686919152736663818359375}
\def\EQKEErrSimpleMedianMaxKey{27671}
\def\EQKEErrSimpleMedianMeanFloat{-0.81413939246870825616753108988632448017597198486328125}
\def\EQKEErrSimpleMedianMeanKey{20754}
\def\EQKEErrSimpleMedianMedianFloat{-1.772340767085552215576171875}
\def\EQKEErrSimpleMedianMedianKey{123}
\def\EQKEErrSimpleMedianMinFloat{-1.7919713139533997026120459850062616169452667236328125}
\def\EQKEErrSimpleMedianMinKey{7467}
\def\EQKEErrSimpleMedianStdDevFloat{0.1876791286172086736794284433926804922521114349365234375}
\def\EQKEErrSimpleMinLen{151}
\def\EQKEErrSimpleMinMaxFloat{-0.78014504909515380859375}
\def\EQKEErrSimpleMinMaxKey{6159}
\def\EQKEErrSimpleMinMeanFloat{-1.3292458057403564453125}
\def\EQKEErrSimpleMinMeanKey{19004}
\def\EQKEErrSimpleMinMedianFloat{-2.597140967845916748046875}
\def\EQKEErrSimpleMinMedianKey{123}
\def\EQKEErrSimpleMinMinFloat{-2.99372577667236328125}
\def\EQKEErrSimpleMinMinKey{7467}
\def\EQKEErrSimpleMinStdDevFloat{0.3571292459964752197265625}
\def\EQKEErrSimpleStdDevLen{151}
\def\EQKEErrSimpleStdDevMaxFloat{0.495215713977813720703125}
\def\EQKEErrSimpleStdDevMaxKey{123}
\def\EQKEErrSimpleStdDevMeanFloat{0.26916372776031494140625}
\def\EQKEErrSimpleStdDevMeanKey{19917}
\def\EQKEErrSimpleStdDevMedianFloat{0.1966501176357269287109375}
\def\EQKEErrSimpleStdDevMedianKey{32374}
\def\EQKEErrSimpleStdDevMinFloat{0.19655172526836395263671875}
\def\EQKEErrSimpleStdDevMinKey{27671}
\def\EQKEErrSimpleStdDevStdDevFloat{0.0444181263446807861328125}
\def\EQKEErrSimpleWithAttnScaleFirstSingularLen{151}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMaxFloat{5.19292545318603515625}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMaxKey{123}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMeanFloat{2.16407544407623486648617472383193671703338623046875}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMeanKey{8048}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMedianFloat{1.3371214568614959716796875}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMedianKey{32374}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMinFloat{1.317229747772216796875}
\def\EQKEErrSimpleWithAttnScaleFirstSingularMinKey{27671}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoLen{151}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMaxFloat{7.34390544891357421875}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMaxKey{123}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMeanFloat{3.060464801377808186089168884791433811187744140625}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMeanKey{8048}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMedianFloat{1.890975296497344970703125}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMedianKey{32374}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMinFloat{1.86284410953521728515625}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoMinKey{27671}
\def\EQKEErrSimpleWithAttnScaleFirstSingularSqrtTwoStdDevFloat{0.81299382495663985448430821634246967732906341552734375}
\def\EQKEErrSimpleWithAttnScaleFirstSingularStdDevFloat{0.57487345160282565803555598904495127499103546142578125}
\def\EQKEErrSimpleWithAttnScaleFroNormLen{151}
\def\EQKEErrSimpleWithAttnScaleFroNormMaxFloat{5.60644817352294921875}
\def\EQKEErrSimpleWithAttnScaleFroNormMaxKey{123}
\def\EQKEErrSimpleWithAttnScaleFroNormMeanFloat{3.0456453001262335789078861125744879245758056640625}
\def\EQKEErrSimpleWithAttnScaleFroNormMeanKey{19917}
\def\EQKEErrSimpleWithAttnScaleFroNormMedianFloat{2.22487103939056396484375}
\def\EQKEErrSimpleWithAttnScaleFroNormMedianKey{32374}
\def\EQKEErrSimpleWithAttnScaleFroNormMinFloat{2.223747730255126953125}
\def\EQKEErrSimpleWithAttnScaleFroNormMinKey{27671}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoLen{151}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMaxFloat{7.928714752197265625}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMaxKey{123}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMeanFloat{4.30719280716599239866582138347439467906951904296875}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMeanKey{19917}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMedianFloat{3.1464426517486572265625}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMedianKey{32374}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMinFloat{3.144854068756103515625}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoMinKey{27671}
\def\EQKEErrSimpleWithAttnScaleFroNormSqrtTwoStdDevFloat{0.71141392636621281209130529532558284699916839599609375}
\def\EQKEErrSimpleWithAttnScaleFroNormStdDevFloat{0.50304561520003598928951760171912610530853271484375}
\def\EQKEErrSimpleWithAttnScaleLen{4096}
\def\EQKEErrSimpleWithAttnScaleMaxAbsLen{151}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMaxFloat{0.566494464874267578125}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMaxKey{4647}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMeanFloat{0.2734946561175466417381585415569134056568145751953125}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMeanKey{19488}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMedianFloat{0.175345011055469512939453125}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMedianKey{27671}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMinFloat{0.17169834673404693603515625}
\def\EQKEErrSimpleWithAttnScaleMaxAbsMinKey{23367}
\def\EQKEErrSimpleWithAttnScaleMaxAbsStdDevFloat{0.0708096033432122073936199058152851648628711700439453125}
\def\EQKEErrSimpleWithAttnScaleMaxLen{151}
\def\EQKEErrSimpleWithAttnScaleMaxMaxFloat{0.566494464874267578125}
\def\EQKEErrSimpleWithAttnScaleMaxMaxKey{4647}
\def\EQKEErrSimpleWithAttnScaleMaxMeanFloat{0.24801863729953765869140625}
\def\EQKEErrSimpleWithAttnScaleMaxMeanKey{4729}
\def\EQKEErrSimpleWithAttnScaleMaxMedianFloat{0.1403871215879917144775390625}
\def\EQKEErrSimpleWithAttnScaleMaxMedianKey{22286}
\def\EQKEErrSimpleWithAttnScaleMaxMinFloat{0.133933961391448974609375}
\def\EQKEErrSimpleWithAttnScaleMaxMinKey{9816}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffLen{151}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMaxFloat{0.958992898464202880859375}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMaxKey{4647}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMeanFloat{0.428997251963773307270599843832314945757389068603515625}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMeanKey{24173}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMedianFloat{0.2531870901584625244140625}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMedianKey{23367}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMinFloat{0.248959124088287353515625}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffMinKey{6159}
\def\EQKEErrSimpleWithAttnScaleMaxRowDiffStdDevFloat{0.11012106514030807480342133430895046330988407135009765625}
\def\EQKEErrSimpleWithAttnScaleMaxStdDevFloat{0.070980139076709747314453125}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormLen{151}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMaxFloat{0.0481477938592433929443359375}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMaxKey{12141}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMeanFloat{0.010684822834041339534305592451346456073224544525146484375}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMeanKey{14929}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMedianFloat{0.0025081238127313554286956787109375}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMedianKey{27300}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMinFloat{0.0023896167986094951629638671875}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormMinKey{6159}
\def\EQKEErrSimpleWithAttnScaleMeanDimZeroNormStdDevFloat{0.00702084516944194957088765107755534700118005275726318359375}
\def\EQKEErrSimpleWithAttnScaleMeanLen{151}
\def\EQKEErrSimpleWithAttnScaleMeanMaxFloat{0.00176308490335941314697265625}
\def\EQKEErrSimpleWithAttnScaleMeanMaxKey{11130}
\def\EQKEErrSimpleWithAttnScaleMeanMeanFloat{-0.000205986769287846982479095458984375}
\def\EQKEErrSimpleWithAttnScaleMeanMeanKey{12552}
\def\EQKEErrSimpleWithAttnScaleMeanMedianFloat{-0.003691461868584156036376953125}
\def\EQKEErrSimpleWithAttnScaleMeanMedianKey{123}
\def\EQKEErrSimpleWithAttnScaleMeanMinFloat{-0.00519114919006824493408203125}
\def\EQKEErrSimpleWithAttnScaleMeanMinKey{12141}
\def\EQKEErrSimpleWithAttnScaleMeanStdDevFloat{0.0008281129994429647922515869140625}
\def\EQKEErrSimpleWithAttnScaleMedianLen{151}
\def\EQKEErrSimpleWithAttnScaleMedianMaxFloat{-0.09060424007475376129150390625}
\def\EQKEErrSimpleWithAttnScaleMedianMaxKey{27671}
\def\EQKEErrSimpleWithAttnScaleMedianMeanFloat{-0.1439208736692536572121525750844739377498626708984375}
\def\EQKEErrSimpleWithAttnScaleMedianMeanKey{20754}
\def\EQKEErrSimpleWithAttnScaleMedianMedianFloat{-0.3133085481822490692138671875}
\def\EQKEErrSimpleWithAttnScaleMedianMedianKey{123}
\def\EQKEErrSimpleWithAttnScaleMedianMinFloat{-0.3167787678539752960205078125}
\def\EQKEErrSimpleWithAttnScaleMedianMinKey{7467}
\def\EQKEErrSimpleWithAttnScaleMedianStdDevFloat{0.033177296362885293212752202407500590197741985321044921875}
\def\EQKEErrSimpleWithAttnScaleMinLen{151}
\def\EQKEErrSimpleWithAttnScaleMinMaxFloat{-0.1379114687442779541015625}
\def\EQKEErrSimpleWithAttnScaleMinMaxKey{6159}
\def\EQKEErrSimpleWithAttnScaleMinMeanFloat{-0.234979689121246337890625}
\def\EQKEErrSimpleWithAttnScaleMinMeanKey{19004}
\def\EQKEErrSimpleWithAttnScaleMinMedianFloat{-0.459114007651805877685546875}
\def\EQKEErrSimpleWithAttnScaleMinMedianKey{123}
\def\EQKEErrSimpleWithAttnScaleMinMinFloat{-0.52922093868255615234375}
\def\EQKEErrSimpleWithAttnScaleMinMinKey{7467}
\def\EQKEErrSimpleWithAttnScaleMinStdDevFloat{0.063132129609584808349609375}
\def\EQKEErrSimpleWithAttnScaleStdDevLen{151}
\def\EQKEErrSimpleWithAttnScaleStdDevMaxFloat{0.08754260838031768798828125}
\def\EQKEErrSimpleWithAttnScaleStdDevMaxKey{123}
\def\EQKEErrSimpleWithAttnScaleStdDevMeanFloat{0.0475818812847137451171875}
\def\EQKEErrSimpleWithAttnScaleStdDevMeanKey{19917}
\def\EQKEErrSimpleWithAttnScaleStdDevMedianFloat{0.034763156436383724212646484375}
\def\EQKEErrSimpleWithAttnScaleStdDevMedianKey{32374}
\def\EQKEErrSimpleWithAttnScaleStdDevMinFloat{0.0347457639873027801513671875}
\def\EQKEErrSimpleWithAttnScaleStdDevMinKey{27671}
\def\EQKEErrSimpleWithAttnScaleStdDevStdDevFloat{0.007852089591324329376220703125}
\def\EQKEErrStdDevLen{151}
\def\EQKEErrStdDevMaxFloat{0.2548564970493316650390625}
\def\EQKEErrStdDevMaxKey{2306}
\def\EQKEErrStdDevMeanFloat{0.1817744076251983642578125}
\def\EQKEErrStdDevMeanKey{19488}
\def\EQKEErrStdDevMedianFloat{0.1426239050924777984619140625}
\def\EQKEErrStdDevMedianKey{9134}
\def\EQKEErrStdDevMinFloat{0.14136140048503875732421875}
\def\EQKEErrStdDevMinKey{4305}
\def\EQKEErrStdDevStdDevFloat{0.02020594291388988494873046875}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactLen{151}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMaxFloat{0.815151214599609375}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMaxKey{4647}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMeanFloat{0.3240656218189277293362238197005353868007659912109375}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMeanKey{6204}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMedianFloat{0.2031146585941314697265625}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMedianKey{27300}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMinFloat{0.19758331775665283203125}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactMinKey{4305}
\def\EQKEErrWithAttnScaleBoundMaxDiffExactStdDevFloat{0.0767201252953545187462935928124352358281612396240234375}
\def\EQKEErrWithAttnScaleBoundMaxDiffLen{151}
\def\EQKEErrWithAttnScaleBoundMaxDiffMaxFloat{1.240393161773681640625}
\def\EQKEErrWithAttnScaleBoundMaxDiffMaxKey{4647}
\def\EQKEErrWithAttnScaleBoundMaxDiffMeanFloat{0.895478988720091795272537638084031641483306884765625}
\def\EQKEErrWithAttnScaleBoundMaxDiffMeanKey{1412}
\def\EQKEErrWithAttnScaleBoundMaxDiffMedianFloat{0.69782815873622894287109375}
\def\EQKEErrWithAttnScaleBoundMaxDiffMedianKey{6532}
\def\EQKEErrWithAttnScaleBoundMaxDiffMinFloat{0.682044565677642822265625}
\def\EQKEErrWithAttnScaleBoundMaxDiffMinKey{32374}
\def\EQKEErrWithAttnScaleBoundMaxDiffStdDevFloat{0.094612611336038543452531257571536116302013397216796875}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductLen{151}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMaxFloat{1.240393161773681640625}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMaxKey{4647}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMeanFloat{0.895478988720091795272537638084031641483306884765625}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMeanKey{1412}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMedianFloat{0.69782815873622894287109375}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMedianKey{6532}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMinFloat{0.682044565677642822265625}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductMinKey{32374}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMaxFloat{25.488689422607421875}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMaxKey{20338}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMeanFloat{16.725645905298900828483965597115457057952880859375}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMeanKey{16149}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMedianFloat{13.889678478240966796875}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMedianKey{32374}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMinFloat{13.75815582275390625}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveMinKey{1681}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductRecursiveStdDevFloat{1.3276105584474116039217506113345734775066375732421875}
\def\EQKEErrWithAttnScaleBoundMaxDiffSubproductStdDevFloat{0.094612611336038543452531257571536116302013397216796875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffLen{151}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMaxFloat{1.2402637004852294921875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMaxKey{4647}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMeanFloat{0.89775885611969907795781864479067735373973846435546875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMeanKey{5781}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMedianFloat{0.70271740853786468505859375}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMedianKey{6532}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMinFloat{0.6837711334228515625}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffMinKey{32374}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffStdDevFloat{0.0939381182988890117702140969413449056446552276611328125}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductLen{151}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMaxFloat{1.2402637004852294921875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMaxKey{4647}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMeanFloat{0.89775885611969907795781864479067735373973846435546875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMeanKey{5781}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMedianFloat{0.70271740853786468505859375}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMedianKey{6532}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMinFloat{0.6837711334228515625}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductMinKey{32374}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMaxFloat{25.47747802734375}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMaxKey{20338}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMeanFloat{16.694721960863528664731347816996276378631591796875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMeanKey{16149}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMedianFloat{13.902704715728759765625}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMedianKey{6532}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMinFloat{13.84151744842529296875}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveMinKey{1681}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductRecursiveStdDevFloat{1.326967051890854509821338069741614162921905517578125}
\def\EQKEErrWithAttnScaleBoundMeanMaxDiffSubproductStdDevFloat{0.0939381182988890117702140969413449056446552276611328125}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveLen{151}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMaxFloat{25.158435821533203125}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMaxKey{20338}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMeanFloat{17.021186512827082282228730036877095699310302734375}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMeanKey{30684}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMedianFloat{14.078598499298095703125}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMedianKey{32374}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMinFloat{13.87025737762451171875}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveMinKey{1681}
\def\EQKEErrWithAttnScaleBoundMeanRecursiveMaxDiffSubproductRecursiveStdDevFloat{1.312618421616210895308540784753859043121337890625}
\def\EQKEErrWithAttnScaleBoundSvdLen{151}
\def\EQKEErrWithAttnScaleBoundSvdMaxFloat{3.2828328609466552734375}
\def\EQKEErrWithAttnScaleBoundSvdMaxKey{4647}
\def\EQKEErrWithAttnScaleBoundSvdMeanFloat{1.85304907141931796132894305628724396228790283203125}
\def\EQKEErrWithAttnScaleBoundSvdMeanKey{24202}
\def\EQKEErrWithAttnScaleBoundSvdMedianFloat{1.23304903507232666015625}
\def\EQKEErrWithAttnScaleBoundSvdMedianKey{913}
\def\EQKEErrWithAttnScaleBoundSvdMinFloat{1.1640250682830810546875}
\def\EQKEErrWithAttnScaleBoundSvdMinKey{4305}
\def\EQKEErrWithAttnScaleBoundSvdStdDevFloat{0.334281923126361457665467469269060529768466949462890625}
\def\EQKEErrWithAttnScaleFirstSingularLen{151}
\def\EQKEErrWithAttnScaleFirstSingularMaxFloat{2.3213138580322265625}
\def\EQKEErrWithAttnScaleFirstSingularMaxKey{4647}
\def\EQKEErrWithAttnScaleFirstSingularMeanFloat{1.31030355344544968687614527880214154720306396484375}
\def\EQKEErrWithAttnScaleFirstSingularMeanKey{24202}
\def\EQKEErrWithAttnScaleFirstSingularMedianFloat{0.8718976676464080810546875}
\def\EQKEErrWithAttnScaleFirstSingularMedianKey{913}
\def\EQKEErrWithAttnScaleFirstSingularMinFloat{0.8230903148651123046875}
\def\EQKEErrWithAttnScaleFirstSingularMinKey{4305}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoLen{151}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMaxFloat{3.282833576202392578125}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMaxKey{4647}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMeanFloat{1.8530490272092503545309227774851024150848388671875}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMeanKey{24202}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMedianFloat{1.2330494821071624755859375}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMedianKey{913}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMinFloat{1.16402542591094970703125}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoMinKey{4305}
\def\EQKEErrWithAttnScaleFirstSingularSqrtTwoStdDevFloat{0.334281831146515162611621008181828074157238006591796875}
\def\EQKEErrWithAttnScaleFirstSingularStdDevFloat{0.236372945977761983460396777445566840469837188720703125}
\def\EQKEErrWithAttnScaleFroNormLen{151}
\def\EQKEErrWithAttnScaleFroNormMaxFloat{2.883376598358154296875}
\def\EQKEErrWithAttnScaleFroNormMaxKey{2306}
\def\EQKEErrWithAttnScaleFroNormMeanFloat{2.056544783099597761832910691737197339534759521484375}
\def\EQKEErrWithAttnScaleFroNormMeanKey{19488}
\def\EQKEErrWithAttnScaleFroNormMedianFloat{1.6136085689067840576171875}
\def\EQKEErrWithAttnScaleFroNormMedianKey{9134}
\def\EQKEErrWithAttnScaleFroNormMinFloat{1.59932196140289306640625}
\def\EQKEErrWithAttnScaleFroNormMinKey{4305}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoLen{151}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMaxFloat{4.07771015167236328125}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMaxKey{2306}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMeanFloat{2.908393480919844176213473474490456283092498779296875}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMeanKey{19488}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMedianFloat{2.28198707103729248046875}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMedianKey{9134}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMinFloat{2.2617828845977783203125}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoMinKey{4305}
\def\EQKEErrWithAttnScaleFroNormSqrtTwoStdDevFloat{0.3232949846339894239832801758893765509128570556640625}
\def\EQKEErrWithAttnScaleFroNormStdDevFloat{0.22860408504391072082029268131009303033351898193359375}
\def\EQKEErrWithAttnScaleLen{4096}
\def\EQKEErrWithAttnScaleMaxAbsLen{151}
\def\EQKEErrWithAttnScaleMaxAbsMaxFloat{0.4748565852642059326171875}
\def\EQKEErrWithAttnScaleMaxAbsMaxKey{4647}
\def\EQKEErrWithAttnScaleMaxAbsMeanFloat{0.1829731909447158411108347308982047252357006072998046875}
\def\EQKEErrWithAttnScaleMaxAbsMeanKey{12493}
\def\EQKEErrWithAttnScaleMaxAbsMedianFloat{0.113796077668666839599609375}
\def\EQKEErrWithAttnScaleMaxAbsMedianKey{4305}
\def\EQKEErrWithAttnScaleMaxAbsMinFloat{0.11213004589080810546875}
\def\EQKEErrWithAttnScaleMaxAbsMinKey{913}
\def\EQKEErrWithAttnScaleMaxAbsStdDevFloat{0.04709885697911044000196767456145607866346836090087890625}
\def\EQKEErrWithAttnScaleMaxLen{151}
\def\EQKEErrWithAttnScaleMaxMaxFloat{0.4748565852642059326171875}
\def\EQKEErrWithAttnScaleMaxMaxKey{4647}
\def\EQKEErrWithAttnScaleMaxMeanFloat{0.17423869669437408447265625}
\def\EQKEErrWithAttnScaleMaxMeanKey{11598}
\def\EQKEErrWithAttnScaleMaxMedianFloat{0.11078408174216747283935546875}
\def\EQKEErrWithAttnScaleMaxMedianKey{32374}
\def\EQKEErrWithAttnScaleMaxMinFloat{0.10458613932132720947265625}
\def\EQKEErrWithAttnScaleMaxMinKey{913}
\def\EQKEErrWithAttnScaleMaxRowDiffLen{151}
\def\EQKEErrWithAttnScaleMaxRowDiffMaxFloat{0.815151214599609375}
\def\EQKEErrWithAttnScaleMaxRowDiffMaxKey{4647}
\def\EQKEErrWithAttnScaleMaxRowDiffMeanFloat{0.32406562349654188803782517425133846700191497802734375}
\def\EQKEErrWithAttnScaleMaxRowDiffMeanKey{6204}
\def\EQKEErrWithAttnScaleMaxRowDiffMedianFloat{0.2031146697700023651123046875}
\def\EQKEErrWithAttnScaleMaxRowDiffMedianKey{27300}
\def\EQKEErrWithAttnScaleMaxRowDiffMinFloat{0.19758327305316925048828125}
\def\EQKEErrWithAttnScaleMaxRowDiffMinKey{4305}
\def\EQKEErrWithAttnScaleMaxRowDiffStdDevFloat{0.07672013202764473016603830046733492054045200347900390625}
\def\EQKEErrWithAttnScaleMaxStdDevFloat{0.0469740964472293853759765625}
\def\EQKEErrWithAttnScaleMeanDimZeroNormLen{151}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMaxFloat{0.013429985381662845611572265625}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMaxKey{4647}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMeanFloat{0.005214780538238042266463434515344488318078219890594482421875}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMeanKey{18668}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMedianFloat{0.00213999883271753787994384765625}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMedianKey{6159}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMinFloat{0.00202591833658516407012939453125}
\def\EQKEErrWithAttnScaleMeanDimZeroNormMinKey{27300}
\def\EQKEErrWithAttnScaleMeanDimZeroNormStdDevFloat{0.00194473253760046719575138585156537374132312834262847900390625}
\def\EQKEErrWithAttnScaleMeanLen{151}
\def\EQKEErrWithAttnScaleMeanMaxFloat{0.000155439091031439602375030517578125}
\def\EQKEErrWithAttnScaleMeanMaxKey{6532}
\def\EQKEErrWithAttnScaleMeanMeanFloat{0.0000064363639467046596109867095947265625}
\def\EQKEErrWithAttnScaleMeanMeanKey{16069}
\def\EQKEErrWithAttnScaleMeanMedianFloat{-0.00013065969687886536121368408203125}
\def\EQKEErrWithAttnScaleMeanMedianKey{17197}
\def\EQKEErrWithAttnScaleMeanMinFloat{-0.0001354051637463271617889404296875}
\def\EQKEErrWithAttnScaleMeanMinKey{8840}
\def\EQKEErrWithAttnScaleMeanStdDevFloat{0.00004581805478665046393871307373046875}
\def\EQKEErrWithAttnScaleMedianLen{151}
\def\EQKEErrWithAttnScaleMedianMaxFloat{-0.06834945958107709051976286218632594682276248931884765625}
\def\EQKEErrWithAttnScaleMedianMaxKey{4305}
\def\EQKEErrWithAttnScaleMedianMeanFloat{-0.1003841042789994641992734614177606999874114990234375}
\def\EQKEErrWithAttnScaleMedianMeanKey{13036}
\def\EQKEErrWithAttnScaleMedianMedianFloat{-0.14247409710660574599927485905936919152736663818359375}
\def\EQKEErrWithAttnScaleMedianMedianKey{2306}
\def\EQKEErrWithAttnScaleMedianMinFloat{-0.14318618364632129669189453125}
\def\EQKEErrWithAttnScaleMedianMinKey{6910}
\def\EQKEErrWithAttnScaleMedianStdDevFloat{0.0137016738688704731163880978783708997070789337158203125}
\def\EQKEErrWithAttnScaleMinLen{151}
\def\EQKEErrWithAttnScaleMinMaxFloat{-0.110367067158222198486328125}
\def\EQKEErrWithAttnScaleMinMaxKey{27300}
\def\EQKEErrWithAttnScaleMinMeanFloat{-0.16925220191478729248046875}
\def\EQKEErrWithAttnScaleMinMeanKey{24144}
\def\EQKEErrWithAttnScaleMinMedianFloat{-0.33346466720104217529296875}
\def\EQKEErrWithAttnScaleMinMedianKey{2306}
\def\EQKEErrWithAttnScaleMinMinFloat{-0.3402945995330810546875}
\def\EQKEErrWithAttnScaleMinMinKey{4647}
\def\EQKEErrWithAttnScaleMinStdDevFloat{0.0387104414403438568115234375}
\def\EQKEErrWithAttnScaleStdDevLen{151}
\def\EQKEErrWithAttnScaleStdDevMaxFloat{0.04505269229412078857421875}
\def\EQKEErrWithAttnScaleStdDevMaxKey{2306}
\def\EQKEErrWithAttnScaleStdDevMeanFloat{0.03213347494602203369140625}
\def\EQKEErrWithAttnScaleStdDevMeanKey{19488}
\def\EQKEErrWithAttnScaleStdDevMedianFloat{0.02521258406341075897216796875}
\def\EQKEErrWithAttnScaleStdDevMedianKey{9134}
\def\EQKEErrWithAttnScaleStdDevMinFloat{0.02498940192162990570068359375}
\def\EQKEErrWithAttnScaleStdDevMinKey{4305}
\def\EQKEErrWithAttnScaleStdDevStdDevFloat{0.003571939654648303985595703125}
\def\EQKEFirstSingularLen{151}
\def\EQKEFirstSingularMaxFloat{9848.4208984375}
\def\EQKEFirstSingularMaxKey{22286}
\def\EQKEFirstSingularMeanFloat{8542.019909587126676342450082302093505859375}
\def\EQKEFirstSingularMeanKey{6082}
\def\EQKEFirstSingularMedianFloat{7468.530517578125}
\def\EQKEFirstSingularMedianKey{11598}
\def\EQKEFirstSingularMinFloat{7395.74609375}
\def\EQKEFirstSingularMinKey{25516}
\def\EQKEFirstSingularSqrtTwoLen{151}
\def\EQKEFirstSingularSqrtTwoMaxFloat{13927.7704025289349374361336231231689453125}
\def\EQKEFirstSingularSqrtTwoMaxKey{22286}
\def\EQKEFirstSingularSqrtTwoMeanFloat{12080.240406199116478092037141323089599609375}
\def\EQKEFirstSingularSqrtTwoMeanKey{6082}
\def\EQKEFirstSingularSqrtTwoMedianFloat{10562.097148956336241099052131175994873046875}
\def\EQKEFirstSingularSqrtTwoMedianKey{11598}
\def\EQKEFirstSingularSqrtTwoMinFloat{10459.164429649090379825793206691741943359375}
\def\EQKEFirstSingularSqrtTwoMinKey{25516}
\def\EQKEFirstSingularSqrtTwoStdDevFloat{636.5179998656152520197792910039424896240234375}
\def\EQKEFirstSingularStdDevFloat{450.0861940522744362169760279357433319091796875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMaxFloat{3630231650304}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMaxKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMeanFloat{3630231650304}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMeanKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMedianFloat{3630231650304}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMedianKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMinFloat{3630231650304}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenMinKey{50}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountLenStdDevFloat{0}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMaxFloat{62.420116424560546875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMaxKey{20338}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMeanFloat{7.518821239471435546875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMeanKey{9134}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMedianFloat{3.91780936717987060546875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMedianKey{12287}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMinFloat{3.893006801605224609375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxMinKey{6910}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMaxStdDevFloat{4.8113384246826171875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMaxFloat{1.6439511710529595145402481648488901555538177490234375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMaxKey{20338}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMeanFloat{1.4389045193925282806191034978837706148624420166015625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMeanKey{9132}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMedianFloat{1.262454190210032134444873008760623633861541748046875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMedianKey{11598}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMinFloat{1.252240274697531408065742652979679405689239501953125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanMinKey{25516}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMeanStdDevFloat{0.06689003796140345625698131470926455222070217132568359375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMaxFloat{1.537063121795654296875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMaxKey{18289}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMeanFloat{1.3487901007939484543385333381593227386474609375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMeanKey{26278}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMedianFloat{1.183238526568619608525523290154524147510528564453125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMedianKey{2236}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMinFloat{1.161244473400942833762883310555480420589447021484375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianMinKey{25516}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMedianStdDevFloat{0.0643541931571993963689948259343509562313556671142578125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMaxFloat{-1.862607479095458984375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMaxKey{16069}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMeanFloat{-4.62305927276611328125}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMeanKey{15399}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMedianFloat{-20.59869289398193359375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMedianKey{913}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMinFloat{-56.62581634521484375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinMinKey{20338}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountMinStdDevFloat{4.485899448394775390625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevLen{151}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMaxFloat{1.06898484583655406510160901234485208988189697265625}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMaxKey{20338}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMeanFloat{0.52154005594053332028892100424855016171932220458984375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMeanKey{2236}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMedianFloat{0.37368574181014080348717243396095000207424163818359375}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMedianKey{29565}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMinFloat{0.3705096222599386646123775790329091250896453857421875}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevMinKey{11598}
\def\EQKEHistAttentionDifferenceOverGapDupBySeqCountStdDevStdDevFloat{0.08091815719843838128344515325807151384651660919189453125}
\def\EQKEHistAttentionDifferenceOverGapLenLen{151}
\def\EQKEHistAttentionDifferenceOverGapLenMaxFloat{258048}
\def\EQKEHistAttentionDifferenceOverGapLenMaxKey{50}
\def\EQKEHistAttentionDifferenceOverGapLenMeanFloat{258048}
\def\EQKEHistAttentionDifferenceOverGapLenMeanKey{50}
\def\EQKEHistAttentionDifferenceOverGapLenMedianFloat{258048}
\def\EQKEHistAttentionDifferenceOverGapLenMedianKey{50}
\def\EQKEHistAttentionDifferenceOverGapLenMinFloat{258048}
\def\EQKEHistAttentionDifferenceOverGapLenMinKey{50}
\def\EQKEHistAttentionDifferenceOverGapLenStdDevFloat{0}
\def\EQKEHistAttentionDifferenceOverGapMaxLen{151}
\def\EQKEHistAttentionDifferenceOverGapMaxMaxFloat{62.420116424560546875}
\def\EQKEHistAttentionDifferenceOverGapMaxMaxKey{20338}
\def\EQKEHistAttentionDifferenceOverGapMaxMeanFloat{7.518821239471435546875}
\def\EQKEHistAttentionDifferenceOverGapMaxMeanKey{9134}
\def\EQKEHistAttentionDifferenceOverGapMaxMedianFloat{3.91780936717987060546875}
\def\EQKEHistAttentionDifferenceOverGapMaxMedianKey{12287}
\def\EQKEHistAttentionDifferenceOverGapMaxMinFloat{3.893006801605224609375}
\def\EQKEHistAttentionDifferenceOverGapMaxMinKey{6910}
\def\EQKEHistAttentionDifferenceOverGapMaxStdDevFloat{4.8113384246826171875}
\def\EQKEHistAttentionDifferenceOverGapMeanLen{151}
\def\EQKEHistAttentionDifferenceOverGapMeanMaxFloat{1.31856119632720947265625}
\def\EQKEHistAttentionDifferenceOverGapMeanMaxKey{29110}
\def\EQKEHistAttentionDifferenceOverGapMeanMeanFloat{1.1863667964935302734375}
\def\EQKEHistAttentionDifferenceOverGapMeanMeanKey{32103}
\def\EQKEHistAttentionDifferenceOverGapMeanMedianFloat{1.0498330295085906982421875}
\def\EQKEHistAttentionDifferenceOverGapMeanMedianKey{2236}
\def\EQKEHistAttentionDifferenceOverGapMeanMinFloat{1.0482518672943115234375}
\def\EQKEHistAttentionDifferenceOverGapMeanMinKey{25516}
\def\EQKEHistAttentionDifferenceOverGapMeanStdDevFloat{0.0517059229314327239990234375}
\def\EQKEHistAttentionDifferenceOverGapMedianLen{151}
\def\EQKEHistAttentionDifferenceOverGapMedianMaxFloat{1.3382390036837745750375461284420453011989593505859375}
\def\EQKEHistAttentionDifferenceOverGapMedianMaxKey{20338}
\def\EQKEHistAttentionDifferenceOverGapMedianMeanFloat{1.176785736316364516795829331385903060436248779296875}
\def\EQKEHistAttentionDifferenceOverGapMedianMeanKey{13716}
\def\EQKEHistAttentionDifferenceOverGapMedianMedianFloat{1.0407579409257146085820977532421238720417022705078125}
\def\EQKEHistAttentionDifferenceOverGapMedianMedianKey{25516}
\def\EQKEHistAttentionDifferenceOverGapMedianMinFloat{1.03922852487054484527106978930532932281494140625}
\def\EQKEHistAttentionDifferenceOverGapMedianMinKey{2236}
\def\EQKEHistAttentionDifferenceOverGapMedianStdDevFloat{0.056282742994565058969325122006921446882188320159912109375}
\def\EQKEHistAttentionDifferenceOverGapMinLen{151}
\def\EQKEHistAttentionDifferenceOverGapMinMaxFloat{-1.862607479095458984375}
\def\EQKEHistAttentionDifferenceOverGapMinMaxKey{16069}
\def\EQKEHistAttentionDifferenceOverGapMinMeanFloat{-4.62305927276611328125}
\def\EQKEHistAttentionDifferenceOverGapMinMeanKey{15399}
\def\EQKEHistAttentionDifferenceOverGapMinMedianFloat{-20.59869289398193359375}
\def\EQKEHistAttentionDifferenceOverGapMinMedianKey{913}
\def\EQKEHistAttentionDifferenceOverGapMinMinFloat{-56.62581634521484375}
\def\EQKEHistAttentionDifferenceOverGapMinMinKey{20338}
\def\EQKEHistAttentionDifferenceOverGapMinStdDevFloat{4.485899448394775390625}
\def\EQKEHistAttentionDifferenceOverGapStdDevLen{151}
\def\EQKEHistAttentionDifferenceOverGapStdDevMaxFloat{1.91934967041015625}
\def\EQKEHistAttentionDifferenceOverGapStdDevMaxKey{20338}
\def\EQKEHistAttentionDifferenceOverGapStdDevMeanFloat{0.516926944255828857421875}
\def\EQKEHistAttentionDifferenceOverGapStdDevMeanKey{32103}
\def\EQKEHistAttentionDifferenceOverGapStdDevMedianFloat{0.39228244125843048095703125}
\def\EQKEHistAttentionDifferenceOverGapStdDevMedianKey{28716}
\def\EQKEHistAttentionDifferenceOverGapStdDevMinFloat{0.3840190470218658447265625}
\def\EQKEHistAttentionDifferenceOverGapStdDevMinKey{11598}
\def\EQKEHistAttentionDifferenceOverGapStdDevStdDevFloat{0.1250131130218505859375}
\def\EQKEQueryDirectionLen{64}
\def\EQKEQueryDirectionMaxLen{151}
\def\EQKEQueryDirectionMaxMaxFloat{0.1869553625583648681640625}
\def\EQKEQueryDirectionMaxMaxKey{24202}
\def\EQKEQueryDirectionMaxMeanFloat{0.15589046478271484375}
\def\EQKEQueryDirectionMaxMeanKey{4430}
\def\EQKEQueryDirectionMaxMedianFloat{0.1432756818830966949462890625}
\def\EQKEQueryDirectionMaxMedianKey{1412}
\def\EQKEQueryDirectionMaxMinFloat{0.142892539501190185546875}
\def\EQKEQueryDirectionMaxMinKey{8299}
\def\EQKEQueryDirectionMaxStdDevFloat{0.007736639119684696197509765625}
\def\EQKEQueryDirectionMeanLen{151}
\def\EQKEQueryDirectionMeanMaxFloat{0.124721832573413848876953125}
\def\EQKEQueryDirectionMeanMaxKey{8299}
\def\EQKEQueryDirectionMeanMeanFloat{0.124324254691600799560546875}
\def\EQKEQueryDirectionMeanMeanKey{1185}
\def\EQKEQueryDirectionMeanMedianFloat{0.12339348159730434417724609375}
\def\EQKEQueryDirectionMeanMedianKey{50}
\def\EQKEQueryDirectionMeanMinFloat{0.123186431825160980224609375}
\def\EQKEQueryDirectionMeanMinKey{22545}
\def\EQKEQueryDirectionMeanStdDevFloat{0.0002715298323892056941986083984375}
\def\EQKEQueryDirectionMedianLen{151}
\def\EQKEQueryDirectionMedianMaxFloat{0.1088720500469207708160723768742172978818416595458984375}
\def\EQKEQueryDirectionMedianMaxKey{4800}
\def\EQKEQueryDirectionMedianMeanFloat{0.09564370101515130839775480353637249208986759185791015625}
\def\EQKEQueryDirectionMedianMeanKey{4157}
\def\EQKEQueryDirectionMedianMedianFloat{0.0674584751157090156681306325481273233890533447265625}
\def\EQKEQueryDirectionMedianMedianKey{123}
\def\EQKEQueryDirectionMedianMinFloat{0.06493842495605349485199297987492172978818416595458984375}
\def\EQKEQueryDirectionMedianMinKey{32103}
\def\EQKEQueryDirectionMedianStdDevFloat{0.007390956268116315348859490796940008294768631458282470703125}
\def\EQKEQueryDirectionMinLen{151}
\def\EQKEQueryDirectionMinMaxFloat{0.108737148344516754150390625}
\def\EQKEQueryDirectionMinMaxKey{4800}
\def\EQKEQueryDirectionMinMeanFloat{0.093764655292034149169921875}
\def\EQKEQueryDirectionMinMeanKey{26278}
\def\EQKEQueryDirectionMinMedianFloat{0.062650219537317752838134765625}
\def\EQKEQueryDirectionMinMedianKey{123}
\def\EQKEQueryDirectionMinMinFloat{0.0590389855206012725830078125}
\def\EQKEQueryDirectionMinMinKey{32103}
\def\EQKEQueryDirectionMinStdDevFloat{0.00845062173902988433837890625}
\def\EQKEQueryDirectionStdDevLen{151}
\def\EQKEQueryDirectionStdDevMaxFloat{0.021215699613094329833984375}
\def\EQKEQueryDirectionStdDevMaxKey{22545}
\def\EQKEQueryDirectionStdDevMeanFloat{0.012751257978379726409912109375}
\def\EQKEQueryDirectionStdDevMeanKey{11498}
\def\EQKEQueryDirectionStdDevMedianFloat{0.008604473434388637542724609375}
\def\EQKEQueryDirectionStdDevMedianKey{1412}
\def\EQKEQueryDirectionStdDevMinFloat{0.008334553800523281097412109375}
\def\EQKEQueryDirectionStdDevMinKey{8299}
\def\EQKEQueryDirectionStdDevStdDevFloat{0.00241120788268744945526123046875}
\def\EQKERatioFirstTwoSingularLen{151}
\def\EQKERatioFirstTwoSingularLowerWhiskerBottomEndFloat{299.64827911022604212121223099529743194580078125}
\def\EQKERatioFirstTwoSingularLowerWhiskerBottomEndKey{123}
\def\EQKERatioFirstTwoSingularLowerWhiskerCrosshatchFloat{302.17365154140901495338766835629940032958984375}
\def\EQKERatioFirstTwoSingularLowerWhiskerCrosshatchKey{123}
\def\EQKERatioFirstTwoSingularMaxFloat{1227.3701171875}
\def\EQKERatioFirstTwoSingularMaxKey{12561}
\def\EQKERatioFirstTwoSingularMeanFloat{736.4365773990454044906073249876499176025390625}
\def\EQKERatioFirstTwoSingularMeanKey{19538}
\def\EQKERatioFirstTwoSingularMedianFloat{317.64069366455078125}
\def\EQKERatioFirstTwoSingularMedianKey{7467}
\def\EQKERatioFirstTwoSingularMinFloat{298.83935546875}
\def\EQKERatioFirstTwoSingularMinKey{123}
\def\EQKERatioFirstTwoSingularQuartileOneFloat{308.240024566650390625}
\def\EQKERatioFirstTwoSingularQuartileOneKey{123}
\def\EQKERatioFirstTwoSingularQuartileThreeFloat{325.952587127685546875}
\def\EQKERatioFirstTwoSingularQuartileThreeKey{7467}
\def\EQKERatioFirstTwoSingularSqrMeanFloat{569224.2810094100423157215118408203125}
\def\EQKERatioFirstTwoSingularStdDevFloat{163.96782757050192458336823619902133941650390625}
\def\EQKERatioFirstTwoSingularUpperWhiskerCrosshatchFloat{329.91115727022867076811962760984897613525390625}
\def\EQKERatioFirstTwoSingularUpperWhiskerCrosshatchKey{7467}
\def\EQKERatioFirstTwoSingularUpperWhiskerTopEndFloat{331.5590717428941616162774153053760528564453125}
\def\EQKERatioFirstTwoSingularUpperWhiskerTopEndKey{7467}
\def\EQKESecondSingularLen{151}
\def\EQKESecondSingularMaxFloat{29.3756313323974609375}
\def\EQKESecondSingularMaxKey{123}
\def\EQKESecondSingularMeanFloat{12.2418563160675244461117472383193671703338623046875}
\def\EQKESecondSingularMeanKey{8048}
\def\EQKESecondSingularMedianFloat{7.56387603282928466796875}
\def\EQKESecondSingularMedianKey{32374}
\def\EQKESecondSingularMinFloat{7.4513759613037109375}
\def\EQKESecondSingularMinKey{27671}
\def\EQKESecondSingularStdDevFloat{3.251972304919191092409391785622574388980865478515625}
\def\EQKESingularLen{32}
\def\EQKESingularMaxLen{151}
\def\EQKESingularMaxMaxFloat{9848.4208984375}
\def\EQKESingularMaxMaxKey{22286}
\def\EQKESingularMaxMeanFloat{8542.01953125}
\def\EQKESingularMaxMeanKey{6082}
\def\EQKESingularMaxMedianFloat{7468.530517578125}
\def\EQKESingularMaxMedianKey{11598}
\def\EQKESingularMaxMinFloat{7395.74609375}
\def\EQKESingularMaxMinKey{25516}
\def\EQKESingularMaxStdDevFloat{450.086212158203125}
\def\EQKESingularMeanLen{151}
\def\EQKESingularMeanMaxFloat{309.27642822265625}
\def\EQKESingularMeanMaxKey{22286}
\def\EQKESingularMeanMeanFloat{268.47491455078125}
\def\EQKESingularMeanMeanKey{6082}
\def\EQKESingularMeanMedianFloat{235.06291961669921875}
\def\EQKESingularMeanMedianKey{11598}
\def\EQKESingularMeanMinFloat{232.81610107421875}
\def\EQKESingularMeanMinKey{25516}
\def\EQKESingularMeanStdDevFloat{14.05150604248046875}
\def\EQKESingularMedianLen{151}
\def\EQKESingularMedianMaxFloat{0.007476751583162695447004608695351635105907917022705078125}
\def\EQKESingularMedianMaxKey{6910}
\def\EQKESingularMedianMeanFloat{0.001757725010468356129089695372158530517481267452239990234375}
\def\EQKESingularMedianMeanKey{11498}
\def\EQKESingularMedianMedianFloat{0.000575148772259126482390978463143937915447168052196502685546875}
\def\EQKESingularMedianMedianKey{24262}
\def\EQKESingularMedianMinFloat{0.000564150660356972362234617701659544763970188796520233154296875}
\def\EQKESingularMedianMinKey{16197}
\def\EQKESingularMedianStdDevFloat{0.00103977103125055410880184236788181806332431733608245849609375}
\def\EQKESingularMinLen{151}
\def\EQKESingularMinMaxFloat{0.0073108687065541744232177734375}
\def\EQKESingularMinMaxKey{6910}
\def\EQKESingularMinMeanFloat{0.001136819017119705677032470703125}
\def\EQKESingularMinMeanKey{12561}
\def\EQKESingularMinMedianFloat{0.000478029876830987632274627685546875}
\def\EQKESingularMinMedianKey{24262}
\def\EQKESingularMinMinFloat{0.00047038073535077273845672607421875}
\def\EQKESingularMinMinKey{25516}
\def\EQKESingularMinStdDevFloat{0.000943380407989025115966796875}
\def\EQKESingularStdDevLen{151}
\def\EQKESingularStdDevMaxFloat{1713.2825927734375}
\def\EQKESingularStdDevMaxKey{22286}
\def\EQKESingularStdDevMeanFloat{1485.9749755859375}
\def\EQKESingularStdDevMeanKey{6082}
\def\EQKESingularStdDevMedianFloat{1299.17242431640625}
\def\EQKESingularStdDevMedianKey{11598}
\def\EQKESingularStdDevMinFloat{1286.5028076171875}
\def\EQKESingularStdDevMinKey{25516}
\def\EQKESingularStdDevStdDevFloat{78.3141632080078125}
\def\EQKESizeDirectionDiffsLen{63}
\def\EQKESizeDirectionDiffsMaxLen{151}
\def\EQKESizeDirectionDiffsMaxMaxFloat{0.2178315818309783935546875}
\def\EQKESizeDirectionDiffsMaxMaxKey{20338}
\def\EQKESizeDirectionDiffsMaxMeanFloat{0.0315846391022205352783203125}
\def\EQKESizeDirectionDiffsMaxMeanKey{11611}
\def\EQKESizeDirectionDiffsMaxMedianFloat{0.0166246034204959869384765625}
\def\EQKESizeDirectionDiffsMaxMedianKey{12287}
\def\EQKESizeDirectionDiffsMaxMinFloat{0.01655907928943634033203125}
\def\EQKESizeDirectionDiffsMaxMinKey{6910}
\def\EQKESizeDirectionDiffsMaxStdDevFloat{0.0168896056711673736572265625}
\def\EQKESizeDirectionDiffsMeanLen{151}
\def\EQKESizeDirectionDiffsMeanMaxFloat{0.0071884761564433574676513671875}
\def\EQKESizeDirectionDiffsMeanMaxKey{27671}
\def\EQKESizeDirectionDiffsMeanMeanFloat{0.006492114625871181488037109375}
\def\EQKESizeDirectionDiffsMeanMeanKey{24202}
\def\EQKESizeDirectionDiffsMeanMedianFloat{0.005811830051243305206298828125}
\def\EQKESizeDirectionDiffsMeanMedianKey{18146}
\def\EQKESizeDirectionDiffsMeanMinFloat{0.0055416435934603214263916015625}
\def\EQKESizeDirectionDiffsMeanMinKey{12561}
\def\EQKESizeDirectionDiffsMeanStdDevFloat{0.0002759453491307795047760009765625}
\def\EQKESizeDirectionDiffsMedianLen{151}
\def\EQKESizeDirectionDiffsMedianMaxFloat{-0.007661091834306716676084025863247006782330572605133056640625}
\def\EQKESizeDirectionDiffsMedianMaxKey{16069}
\def\EQKESizeDirectionDiffsMedianMeanFloat{-0.0171670152522031445319061759846590575762093067169189453125}
\def\EQKESizeDirectionDiffsMedianMeanKey{30899}
\def\EQKESizeDirectionDiffsMedianMedianFloat{-0.05997895590960979073091863256195210851728916168212890625}
\def\EQKESizeDirectionDiffsMedianMedianKey{913}
\def\EQKESizeDirectionDiffsMedianMinFloat{-0.143541645556688302054482164749060757458209991455078125}
\def\EQKESizeDirectionDiffsMedianMinKey{20338}
\def\EQKESizeDirectionDiffsMedianStdDevFloat{0.01148372317050379808056614905353853828273713588714599609375}
\def\EQKESizeDirectionDiffsMinLen{151}
\def\EQKESizeDirectionDiffsMinMaxFloat{-0.0078666210174560546875}
\def\EQKESizeDirectionDiffsMinMaxKey{16069}
\def\EQKESizeDirectionDiffsMinMeanFloat{-0.01937205530703067779541015625}
\def\EQKESizeDirectionDiffsMinMeanKey{12493}
\def\EQKESizeDirectionDiffsMinMedianFloat{-0.0780960880219936370849609375}
\def\EQKESizeDirectionDiffsMinMedianKey{913}
\def\EQKESizeDirectionDiffsMinMinFloat{-0.197634041309356689453125}
\def\EQKESizeDirectionDiffsMinMinKey{20338}
\def\EQKESizeDirectionDiffsMinStdDevFloat{0.01577535830438137054443359375}
\def\EQKESizeDirectionDiffsStdDevLen{151}
\def\EQKESizeDirectionDiffsStdDevMaxFloat{0.038155429065227508544921875}
\def\EQKESizeDirectionDiffsStdDevMaxKey{20338}
\def\EQKESizeDirectionDiffsStdDevMeanFloat{0.00789645500481128692626953125}
\def\EQKESizeDirectionDiffsStdDevMeanKey{12493}
\def\EQKESizeDirectionDiffsStdDevMedianFloat{0.005036249174736440181732177734375}
\def\EQKESizeDirectionDiffsStdDevMedianKey{6910}
\def\EQKESizeDirectionDiffsStdDevMinFloat{0.005021697841584682464599609375}
\def\EQKESizeDirectionDiffsStdDevMinKey{1283}
\def\EQKESizeDirectionDiffsStdDevStdDevFloat{0.00277287210337817668914794921875}
\def\EQKESizeDirectionLen{64}
\def\EQKESizeDirectionMaxLen{151}
\def\EQKESizeDirectionMaxMaxFloat{0.295077264308929443359375}
\def\EQKESizeDirectionMaxMaxKey{7238}
\def\EQKESizeDirectionMaxMeanFloat{0.23006097972393035888671875}
\def\EQKESizeDirectionMaxMeanKey{26932}
\def\EQKESizeDirectionMaxMedianFloat{0.174050830304622650146484375}
\def\EQKESizeDirectionMaxMedianKey{17080}
\def\EQKESizeDirectionMaxMinFloat{0.14864532649517059326171875}
\def\EQKESizeDirectionMaxMinKey{12561}
\def\EQKESizeDirectionMaxStdDevFloat{0.0232656411826610565185546875}
\def\EQKESizeDirectionMeanLen{151}
\def\EQKESizeDirectionMeanMaxFloat{0.001350644044578075408935546875}
\def\EQKESizeDirectionMeanMaxKey{27584}
\def\EQKESizeDirectionMeanMeanFloat{-0.0363770090043544769287109375}
\def\EQKESizeDirectionMeanMeanKey{26278}
\def\EQKESizeDirectionMeanMedianFloat{-0.06571652181446552276611328125}
\def\EQKESizeDirectionMeanMedianKey{20294}
\def\EQKESizeDirectionMeanMinFloat{-0.069434158504009246826171875}
\def\EQKESizeDirectionMeanMinKey{12561}
\def\EQKESizeDirectionMeanStdDevFloat{0.01299597881734371185302734375}
\def\EQKESizeDirectionMedianLen{151}
\def\EQKESizeDirectionMedianMaxFloat{-0.1565812428295612346307308371251565404236316680908203125}
\def\EQKESizeDirectionMedianMaxKey{27584}
\def\EQKESizeDirectionMedianMeanFloat{-0.1892901285214732276518390108321909792721271514892578125}
\def\EQKESizeDirectionMedianMeanKey{12552}
\def\EQKESizeDirectionMedianMedianFloat{-0.2121038905158638965264827902501565404236316680908203125}
\def\EQKESizeDirectionMedianMedianKey{7790}
\def\EQKESizeDirectionMedianMinFloat{-0.2311062625795602676337381353732780553400516510009765625}
\def\EQKESizeDirectionMedianMinKey{20338}
\def\EQKESizeDirectionMedianStdDevFloat{0.00915044308065522844775063759925615158863365650177001953125}
\def\EQKESizeDirectionMinLen{151}
\def\EQKESizeDirectionMinMaxFloat{-0.15679912269115447998046875}
\def\EQKESizeDirectionMinMaxKey{27584}
\def\EQKESizeDirectionMinMeanFloat{-0.19028569757938385009765625}
\def\EQKESizeDirectionMinMeanKey{23633}
\def\EQKESizeDirectionMinMedianFloat{-0.2190941385924816131591796875}
\def\EQKESizeDirectionMinMedianKey{7790}
\def\EQKESizeDirectionMinMinFloat{-0.251815021038055419921875}
\def\EQKESizeDirectionMinMinKey{20338}
\def\EQKESizeDirectionMinStdDevFloat{0.009950297884643077850341796875}
\def\EQKESizeDirectionStdDevLen{151}
\def\EQKESizeDirectionStdDevMaxFloat{0.1249977648258209228515625}
\def\EQKESizeDirectionStdDevMaxKey{21598}
\def\EQKESizeDirectionStdDevMeanFloat{0.118820466101169586181640625}
\def\EQKESizeDirectionStdDevMeanKey{20338}
\def\EQKESizeDirectionStdDevMedianFloat{0.106300890445709228515625}
\def\EQKESizeDirectionStdDevMedianKey{20294}
\def\EQKESizeDirectionStdDevMinFloat{0.103941775858402252197265625}
\def\EQKESizeDirectionStdDevMinKey{12561}
\def\EQKESizeDirectionStdDevStdDevFloat{0.003809547983109951019287109375}
\def\EQKEThirdSingularLen{151}
\def\EQKEThirdSingularMaxFloat{11.53199672698974609375}
\def\EQKEThirdSingularMaxKey{20976}
\def\EQKEThirdSingularMeanFloat{7.62699733822551007023093916359357535839080810546875}
\def\EQKEThirdSingularMeanKey{29726}
\def\EQKEThirdSingularMedianFloat{5.02667140960693359375}
\def\EQKEThirdSingularMedianKey{1951}
\def\EQKEThirdSingularMinFloat{4.93627166748046875}
\def\EQKEThirdSingularMinKey{8721}
\def\EQKEThirdSingularStdDevFloat{1.23931690842624764314905405626632273197174072265625}
\def\EQKEWithAttnScaleFirstSingularLen{151}
\def\EQKEWithAttnScaleFirstSingularMaxFloat{1740.9713134765625}
\def\EQKEWithAttnScaleFirstSingularMaxKey{22286}
\def\EQKEWithAttnScaleFirstSingularMeanFloat{1510.03007699322233747807331383228302001953125}
\def\EQKEWithAttnScaleFirstSingularMeanKey{6082}
\def\EQKEWithAttnScaleFirstSingularMedianFloat{1320.262176513671875}
\def\EQKEWithAttnScaleFirstSingularMedianKey{11598}
\def\EQKEWithAttnScaleFirstSingularMinFloat{1307.3956298828125}
\def\EQKEWithAttnScaleFirstSingularMinKey{25516}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoLen{151}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMaxFloat{2462.10524322105584360542707145214080810546875}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMaxKey{22286}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMeanFloat{2135.50501447510441721533425152301788330078125}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMeanKey{6082}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMedianFloat{1867.13267591385601917863823473453521728515625}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMedianKey{11598}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMinFloat{1848.936631167588757307385094463825225830078125}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoMinKey{25516}
\def\EQKEWithAttnScaleFirstSingularSqrtTwoStdDevFloat{112.5215376794808292970628826878964900970458984375}
\def\EQKEWithAttnScaleFirstSingularStdDevFloat{79.564742322698521093116141855716705322265625}
\def\EQKEWithAttnScaleRatioFirstTwoSingularLen{151}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMaxFloat{1227.3702392578125}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMaxKey{12561}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMeanFloat{736.436576388529601899790577590465545654296875}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMeanKey{19538}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMedianFloat{317.64069366455078125}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMedianKey{7467}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMinFloat{298.83935546875}
\def\EQKEWithAttnScaleRatioFirstTwoSingularMinKey{123}
\def\EQKEWithAttnScaleRatioFirstTwoSingularStdDevFloat{163.967825942548671491749701090157032012939453125}
\def\EQKEWithAttnScaleSecondSingularLen{151}
\def\EQKEWithAttnScaleSecondSingularMaxFloat{5.192926883697509765625}
\def\EQKEWithAttnScaleSecondSingularMaxKey{123}
\def\EQKEWithAttnScaleSecondSingularMeanFloat{2.1640749427656462700042538926936686038970947265625}
\def\EQKEWithAttnScaleSecondSingularMeanKey{8048}
\def\EQKEWithAttnScaleSecondSingularMedianFloat{1.3371170461177825927734375}
\def\EQKEWithAttnScaleSecondSingularMedianKey{32374}
\def\EQKEWithAttnScaleSecondSingularMinFloat{1.31722962856292724609375}
\def\EQKEWithAttnScaleSecondSingularMinKey{27671}
\def\EQKEWithAttnScaleSecondSingularStdDevFloat{0.57487292207279738764924559291102923452854156494140625}
\def\EQKEWithAttnScaleSingularLen{32}
\def\EQKEWithAttnScaleSingularMaxLen{151}
\def\EQKEWithAttnScaleSingularMaxMaxFloat{9848.4208984375}
\def\EQKEWithAttnScaleSingularMaxMaxKey{22286}
\def\EQKEWithAttnScaleSingularMaxMeanFloat{8542.01953125}
\def\EQKEWithAttnScaleSingularMaxMeanKey{6082}
\def\EQKEWithAttnScaleSingularMaxMedianFloat{7468.530517578125}
\def\EQKEWithAttnScaleSingularMaxMedianKey{11598}
\def\EQKEWithAttnScaleSingularMaxMinFloat{7395.74609375}
\def\EQKEWithAttnScaleSingularMaxMinKey{25516}
\def\EQKEWithAttnScaleSingularMaxStdDevFloat{450.086212158203125}
\def\EQKEWithAttnScaleSingularMeanLen{151}
\def\EQKEWithAttnScaleSingularMeanMaxFloat{309.27642822265625}
\def\EQKEWithAttnScaleSingularMeanMaxKey{22286}
\def\EQKEWithAttnScaleSingularMeanMeanFloat{268.47491455078125}
\def\EQKEWithAttnScaleSingularMeanMeanKey{6082}
\def\EQKEWithAttnScaleSingularMeanMedianFloat{235.06291961669921875}
\def\EQKEWithAttnScaleSingularMeanMedianKey{11598}
\def\EQKEWithAttnScaleSingularMeanMinFloat{232.81610107421875}
\def\EQKEWithAttnScaleSingularMeanMinKey{25516}
\def\EQKEWithAttnScaleSingularMeanStdDevFloat{14.05150604248046875}
\def\EQKEWithAttnScaleSingularMedianLen{151}
\def\EQKEWithAttnScaleSingularMedianMaxFloat{0.007476751583162695447004608695351635105907917022705078125}
\def\EQKEWithAttnScaleSingularMedianMaxKey{6910}
\def\EQKEWithAttnScaleSingularMedianMeanFloat{0.001757725010468356129089695372158530517481267452239990234375}
\def\EQKEWithAttnScaleSingularMedianMeanKey{11498}
\def\EQKEWithAttnScaleSingularMedianMedianFloat{0.000575148772259126482390978463143937915447168052196502685546875}
\def\EQKEWithAttnScaleSingularMedianMedianKey{24262}
\def\EQKEWithAttnScaleSingularMedianMinFloat{0.000564150660356972362234617701659544763970188796520233154296875}
\def\EQKEWithAttnScaleSingularMedianMinKey{16197}
\def\EQKEWithAttnScaleSingularMedianStdDevFloat{0.00103977103125055410880184236788181806332431733608245849609375}
\def\EQKEWithAttnScaleSingularMinLen{151}
\def\EQKEWithAttnScaleSingularMinMaxFloat{0.0073108687065541744232177734375}
\def\EQKEWithAttnScaleSingularMinMaxKey{6910}
\def\EQKEWithAttnScaleSingularMinMeanFloat{0.001136819017119705677032470703125}
\def\EQKEWithAttnScaleSingularMinMeanKey{12561}
\def\EQKEWithAttnScaleSingularMinMedianFloat{0.000478029876830987632274627685546875}
\def\EQKEWithAttnScaleSingularMinMedianKey{24262}
\def\EQKEWithAttnScaleSingularMinMinFloat{0.00047038073535077273845672607421875}
\def\EQKEWithAttnScaleSingularMinMinKey{25516}
\def\EQKEWithAttnScaleSingularMinStdDevFloat{0.000943380407989025115966796875}
\def\EQKEWithAttnScaleSingularStdDevLen{151}
\def\EQKEWithAttnScaleSingularStdDevMaxFloat{1713.2825927734375}
\def\EQKEWithAttnScaleSingularStdDevMaxKey{22286}
\def\EQKEWithAttnScaleSingularStdDevMeanFloat{1485.9749755859375}
\def\EQKEWithAttnScaleSingularStdDevMeanKey{6082}
\def\EQKEWithAttnScaleSingularStdDevMedianFloat{1299.17242431640625}
\def\EQKEWithAttnScaleSingularStdDevMedianKey{11598}
\def\EQKEWithAttnScaleSingularStdDevMinFloat{1286.5028076171875}
\def\EQKEWithAttnScaleSingularStdDevMinKey{25516}
\def\EQKEWithAttnScaleSingularStdDevStdDevFloat{78.3141632080078125}
\def\EQKEWithAttnScaleThirdSingularLen{151}
\def\EQKEWithAttnScaleThirdSingularMaxFloat{2.0385882854461669921875}
\def\EQKEWithAttnScaleThirdSingularMaxKey{20976}
\def\EQKEWithAttnScaleThirdSingularMeanFloat{1.348275404497487617305750973173417150974273681640625}
\def\EQKEWithAttnScaleThirdSingularMeanKey{29726}
\def\EQKEWithAttnScaleThirdSingularMedianFloat{0.888598382472991943359375}
\def\EQKEWithAttnScaleThirdSingularMedianKey{1951}
\def\EQKEWithAttnScaleThirdSingularMinFloat{0.872617781162261962890625}
\def\EQKEWithAttnScaleThirdSingularMinKey{8721}
\def\EQKEWithAttnScaleThirdSingularStdDevFloat{0.2190823497691355148386804785332060419023036956787109375}
\def\EQKPAbsLen{320}
\def\EQKPAbsMaxLen{151}
\def\EQKPAbsMaxMaxFloat{7.330049991607666015625}
\def\EQKPAbsMaxMaxKey{28090}
\def\EQKPAbsMaxMeanFloat{2.232570171356201171875}
\def\EQKPAbsMaxMeanKey{9504}
\def\EQKPAbsMaxMedianFloat{0.60901664197444915771484375}
\def\EQKPAbsMaxMedianKey{123}
\def\EQKPAbsMaxMinFloat{0.515166461467742919921875}
\def\EQKPAbsMaxMinKey{6532}
\def\EQKPAbsMaxStdDevFloat{1.26892793178558349609375}
\def\EQKPAbsMeanLen{151}
\def\EQKPAbsMeanMaxFloat{3.5445258617401123046875}
\def\EQKPAbsMeanMaxKey{13036}
\def\EQKPAbsMeanMeanFloat{0.84725010395050048828125}
\def\EQKPAbsMeanMeanKey{2306}
\def\EQKPAbsMeanMedianFloat{0.1898819915950298309326171875}
\def\EQKPAbsMeanMedianKey{123}
\def\EQKPAbsMeanMinFloat{0.13319174945354461669921875}
\def\EQKPAbsMeanMinKey{17197}
\def\EQKPAbsMeanStdDevFloat{0.578513562679290771484375}
\def\EQKPAbsMedianLen{151}
\def\EQKPAbsMedianMaxFloat{1.829904192686080843799345529987476766109466552734375}
\def\EQKPAbsMedianMaxKey{16197}
\def\EQKPAbsMedianMeanFloat{0.0700272271169861404427336992739583365619182586669921875}
\def\EQKPAbsMedianMeanKey{1283}
\def\EQKPAbsMedianMedianFloat{0.000861457731807604466800487585942391888238489627838134765625}
\def\EQKPAbsMedianMedianKey{8893}
\def\EQKPAbsMedianMinFloat{0.0007076496235094965024658986152417128323577344417572021484375}
\def\EQKPAbsMedianMinKey{9504}
\def\EQKPAbsMedianStdDevFloat{0.2088638279648438456082004677227814681828022003173828125}
\def\EQKPAbsMinLen{151}
\def\EQKPAbsMinMaxFloat{1.69769155979156494140625}
\def\EQKPAbsMinMaxKey{16197}
\def\EQKPAbsMinMeanFloat{0.050556741654872894287109375}
\def\EQKPAbsMinMeanKey{4305}
\def\EQKPAbsMinMedianFloat{0.000037619960494339466094970703125}
\def\EQKPAbsMinMedianKey{21598}
\def\EQKPAbsMinMinFloat{0.0000042407773435115814208984375}
\def\EQKPAbsMinMinKey{23447}
\def\EQKPAbsMinStdDevFloat{0.193355143070220947265625}
\def\EQKPAbsStdDevLen{151}
\def\EQKPAbsStdDevMaxFloat{1.875256061553955078125}
\def\EQKPAbsStdDevMaxKey{4800}
\def\EQKPAbsStdDevMeanFloat{0.542787373065948486328125}
\def\EQKPAbsStdDevMeanKey{19004}
\def\EQKPAbsStdDevMedianFloat{0.10666266269981861114501953125}
\def\EQKPAbsStdDevMedianKey{17197}
\def\EQKPAbsStdDevMinFloat{0.10318391025066375732421875}
\def\EQKPAbsStdDevMinKey{6532}
\def\EQKPAbsStdDevStdDevFloat{0.3385366499423980712890625}
\def\EQKPLen{320}
\def\EQKPMaxLen{151}
\def\EQKPMaxMaxFloat{6.806912899017333984375}
\def\EQKPMaxMaxKey{4800}
\def\EQKPMaxMeanFloat{1.93870067596435546875}
\def\EQKPMaxMeanKey{24262}
\def\EQKPMaxMedianFloat{0.4649983346462249755859375}
\def\EQKPMaxMedianKey{8048}
\def\EQKPMaxMinFloat{0.449704468250274658203125}
\def\EQKPMaxMinKey{17197}
\def\EQKPMaxRowDiffLen{64}
\def\EQKPMaxRowDiffMaxLen{151}
\def\EQKPMaxRowDiffMaxMaxFloat{12.8415279388427734375}
\def\EQKPMaxRowDiffMaxMaxKey{13036}
\def\EQKPMaxRowDiffMaxMeanFloat{3.7536633014678955078125}
\def\EQKPMaxRowDiffMaxMeanKey{22286}
\def\EQKPMaxRowDiffMaxMedianFloat{0.98282943665981292724609375}
\def\EQKPMaxRowDiffMaxMedianKey{17197}
\def\EQKPMaxRowDiffMaxMinFloat{0.860009610652923583984375}
\def\EQKPMaxRowDiffMaxMinKey{6532}
\def\EQKPMaxRowDiffMaxStdDevFloat{2.108976840972900390625}
\def\EQKPMaxRowDiffMeanLen{151}
\def\EQKPMaxRowDiffMeanMaxFloat{9.65525054931640625}
\def\EQKPMaxRowDiffMeanMaxKey{13036}
\def\EQKPMaxRowDiffMeanMeanFloat{2.7842528820037841796875}
\def\EQKPMaxRowDiffMeanMeanKey{2236}
\def\EQKPMaxRowDiffMeanMedianFloat{0.5737980902194976806640625}
\def\EQKPMaxRowDiffMeanMedianKey{6532}
\def\EQKPMaxRowDiffMeanMinFloat{0.439956486225128173828125}
\def\EQKPMaxRowDiffMeanMinKey{17197}
\def\EQKPMaxRowDiffMeanStdDevFloat{1.7516193389892578125}
\def\EQKPMaxRowDiffMedianLen{151}
\def\EQKPMaxRowDiffMedianMaxFloat{8.2356859397888175777779906638897955417633056640625}
\def\EQKPMaxRowDiffMedianMaxKey{13036}
\def\EQKPMaxRowDiffMedianMeanFloat{1.8947309110550492050606408156454563140869140625}
\def\EQKPMaxRowDiffMedianMeanKey{20976}
\def\EQKPMaxRowDiffMedianMedianFloat{0.286415448803454653070588165064691565930843353271484375}
\def\EQKPMaxRowDiffMedianMedianKey{123}
\def\EQKPMaxRowDiffMedianMinFloat{0.138732348158955576256090580500313080847263336181640625}
\def\EQKPMaxRowDiffMedianMinKey{17197}
\def\EQKPMaxRowDiffMedianStdDevFloat{1.4429809942105915610000010929070413112640380859375}
\def\EQKPMaxRowDiffMinLen{151}
\def\EQKPMaxRowDiffMinMaxFloat{8.215213775634765625}
\def\EQKPMaxRowDiffMinMaxKey{13036}
\def\EQKPMaxRowDiffMinMeanFloat{1.84808957576751708984375}
\def\EQKPMaxRowDiffMinMeanKey{15662}
\def\EQKPMaxRowDiffMinMedianFloat{0.2759479321539402008056640625}
\def\EQKPMaxRowDiffMinMedianKey{123}
\def\EQKPMaxRowDiffMinMinFloat{0.13849277794361114501953125}
\def\EQKPMaxRowDiffMinMinKey{17197}
\def\EQKPMaxRowDiffMinStdDevFloat{1.4296627044677734375}
\def\EQKPMaxRowDiffStdDevLen{151}
\def\EQKPMaxRowDiffStdDevMaxFloat{1.00380957126617431640625}
\def\EQKPMaxRowDiffStdDevMaxKey{5615}
\def\EQKPMaxRowDiffStdDevMeanFloat{0.4076825082302093505859375}
\def\EQKPMaxRowDiffStdDevMeanKey{11130}
\def\EQKPMaxRowDiffStdDevMedianFloat{0.1323116756975650787353515625}
\def\EQKPMaxRowDiffStdDevMedianKey{30371}
\def\EQKPMaxRowDiffStdDevMinFloat{0.09381572902202606201171875}
\def\EQKPMaxRowDiffStdDevMinKey{6532}
\def\EQKPMaxRowDiffStdDevStdDevFloat{0.1864974498748779296875}
\def\EQKPMaxStdDevFloat{1.17059218883514404296875}
\def\EQKPMeanLen{151}
\def\EQKPMeanMaxFloat{0.00000204704701900482177734375}
\def\EQKPMeanMaxKey{23367}
\def\EQKPMeanMeanFloat{0.00000010967418262453065835870802402496337890625}
\def\EQKPMeanMeanKey{20415}
\def\EQKPMeanMedianFloat{-0.000001553865189407588331960141658782958984375}
\def\EQKPMeanMedianKey{15043}
\def\EQKPMeanMinFloat{-0.0000016869977343958453275263309478759765625}
\def\EQKPMeanMinKey{12561}
\def\EQKPMeanStdDevFloat{0.00000072355129532297723926603794097900390625}
\def\EQKPMedianLen{151}
\def\EQKPMedianMaxFloat{-0.4378727997839451102635166535037569701671600341796875}
\def\EQKPMedianMaxKey{6532}
\def\EQKPMedianMeanFloat{-1.8138961241024220694129098774283193051815032958984375}
\def\EQKPMedianMeanKey{20976}
\def\EQKPMedianMedianFloat{-6.539561558365821980487453402020037174224853515625}
\def\EQKPMedianMedianKey{13036}
\def\EQKPMedianMinFloat{-7.000779237747192240703952847979962825775146484375}
\def\EQKPMedianMinKey{28090}
\def\EQKPMedianStdDevFloat{1.063325423989095686039263455313630402088165283203125}
\def\EQKPMinLen{151}
\def\EQKPMinMaxFloat{-0.46276509761810302734375}
\def\EQKPMinMaxKey{6532}
\def\EQKPMinMeanFloat{-1.9236638545989990234375}
\def\EQKPMinMeanKey{12493}
\def\EQKPMinMedianFloat{-7.01654160022735595703125}
\def\EQKPMinMedianKey{13036}
\def\EQKPMinMinFloat{-7.330049991607666015625}
\def\EQKPMinMinKey{28090}
\def\EQKPMinStdDevFloat{1.096665859222412109375}
\def\EQKPStdDevLen{151}
\def\EQKPStdDevMaxFloat{3.90584087371826171875}
\def\EQKPStdDevMaxKey{13036}
\def\EQKPStdDevMeanFloat{1.0140645503997802734375}
\def\EQKPStdDevMeanKey{20976}
\def\EQKPStdDevMedianFloat{0.2292305529117584228515625}
\def\EQKPStdDevMedianKey{6532}
\def\EQKPStdDevMinFloat{0.17136417329311370849609375}
\def\EQKPStdDevMinKey{17197}
\def\EQKPStdDevStdDevFloat{0.65833818912506103515625}
\def\EQKPWithAttnScaleAbsLen{320}
\def\EQKPWithAttnScaleAbsMaxLen{151}
\def\EQKPWithAttnScaleAbsMaxMaxFloat{1.2957820892333984375}
\def\EQKPWithAttnScaleAbsMaxMaxKey{28090}
\def\EQKPWithAttnScaleAbsMaxMeanFloat{0.3946663439273834228515625}
\def\EQKPWithAttnScaleAbsMaxMeanKey{9504}
\def\EQKPWithAttnScaleAbsMaxMedianFloat{0.10765995271503925323486328125}
\def\EQKPWithAttnScaleAbsMaxMedianKey{123}
\def\EQKPWithAttnScaleAbsMaxMinFloat{0.091069422662258148193359375}
\def\EQKPWithAttnScaleAbsMaxMinKey{6532}
\def\EQKPWithAttnScaleAbsMaxStdDevFloat{0.22431688010692596435546875}
\def\EQKPWithAttnScaleAbsMeanLen{151}
\def\EQKPWithAttnScaleAbsMeanMaxFloat{0.626589596271514892578125}
\def\EQKPWithAttnScaleAbsMeanMaxKey{13036}
\def\EQKPWithAttnScaleAbsMeanMeanFloat{0.14977408945560455322265625}
\def\EQKPWithAttnScaleAbsMeanMeanKey{2306}
\def\EQKPWithAttnScaleAbsMeanMedianFloat{0.0335667133331298828125}
\def\EQKPWithAttnScaleAbsMeanMedianKey{123}
\def\EQKPWithAttnScaleAbsMeanMinFloat{0.023545198142528533935546875}
\def\EQKPWithAttnScaleAbsMeanMinKey{17197}
\def\EQKPWithAttnScaleAbsMeanStdDevFloat{0.10226772725582122802734375}
\def\EQKPWithAttnScaleAbsMedianLen{151}
\def\EQKPWithAttnScaleAbsMedianMaxFloat{0.323484423607587834315069130752817727625370025634765625}
\def\EQKPWithAttnScaleAbsMedianMaxKey{16197}
\def\EQKPWithAttnScaleAbsMedianMeanFloat{0.0123791820263504138976973223407185287214815616607666015625}
\def\EQKPWithAttnScaleAbsMedianMeanKey{1283}
\def\EQKPWithAttnScaleAbsMedianMedianFloat{0.00015228565329380216249351154278457443069783039391040802001953125}
\def\EQKPWithAttnScaleAbsMedianMedianKey{8893}
\def\EQKPWithAttnScaleAbsMedianMinFloat{0.0001250959609751589661323645241708391040447168052196502685546875}
\def\EQKPWithAttnScaleAbsMedianMinKey{9504}
\def\EQKPWithAttnScaleAbsMedianStdDevFloat{0.0369222581634830737673524936326430179178714752197265625}
\def\EQKPWithAttnScaleAbsMinLen{151}
\def\EQKPWithAttnScaleAbsMinMaxFloat{0.300112307071685791015625}
\def\EQKPWithAttnScaleAbsMinMaxKey{16197}
\def\EQKPWithAttnScaleAbsMinMeanFloat{0.00893725454807281494140625}
\def\EQKPWithAttnScaleAbsMinMeanKey{4305}
\def\EQKPWithAttnScaleAbsMinMedianFloat{0.000006650332352364785037934780120849609375}
\def\EQKPWithAttnScaleAbsMinMedianKey{21598}
\def\EQKPWithAttnScaleAbsMinMinFloat{0.00000074967061891584307886660099029541015625}
\def\EQKPWithAttnScaleAbsMinMinKey{23447}
\def\EQKPWithAttnScaleAbsMinStdDevFloat{0.03418068587779998779296875}
\def\EQKPWithAttnScaleAbsStdDevLen{151}
\def\EQKPWithAttnScaleAbsStdDevMaxFloat{0.3315015733242034912109375}
\def\EQKPWithAttnScaleAbsStdDevMaxKey{4800}
\def\EQKPWithAttnScaleAbsStdDevMeanFloat{0.09595215320587158203125}
\def\EQKPWithAttnScaleAbsStdDevMeanKey{19004}
\def\EQKPWithAttnScaleAbsStdDevMedianFloat{0.0188554734922945499420166015625}
\def\EQKPWithAttnScaleAbsStdDevMedianKey{17197}
\def\EQKPWithAttnScaleAbsStdDevMinFloat{0.018240511417388916015625}
\def\EQKPWithAttnScaleAbsStdDevMinKey{6532}
\def\EQKPWithAttnScaleAbsStdDevStdDevFloat{0.059845387935638427734375}
\def\EQKPWithAttnScaleLen{320}
\def\EQKPWithAttnScaleMaxLen{151}
\def\EQKPWithAttnScaleMaxMaxFloat{1.2033035755157470703125}
\def\EQKPWithAttnScaleMaxMaxKey{4800}
\def\EQKPWithAttnScaleMaxMeanFloat{0.342717111110687255859375}
\def\EQKPWithAttnScaleMaxMeanKey{24262}
\def\EQKPWithAttnScaleMaxMedianFloat{0.08220086991786956787109375}
\def\EQKPWithAttnScaleMaxMedianKey{8048}
\def\EQKPWithAttnScaleMaxMinFloat{0.079497270286083221435546875}
\def\EQKPWithAttnScaleMaxMinKey{17197}
\def\EQKPWithAttnScaleMaxRowDiffLen{64}
\def\EQKPWithAttnScaleMaxRowDiffMaxLen{151}
\def\EQKPWithAttnScaleMaxRowDiffMaxMaxFloat{2.270082950592041015625}
\def\EQKPWithAttnScaleMaxRowDiffMaxMaxKey{13036}
\def\EQKPWithAttnScaleMaxRowDiffMaxMeanFloat{0.663560211658477783203125}
\def\EQKPWithAttnScaleMaxRowDiffMaxMeanKey{22286}
\def\EQKPWithAttnScaleMaxRowDiffMaxMedianFloat{0.17374134063720703125}
\def\EQKPWithAttnScaleMaxRowDiffMaxMedianKey{17197}
\def\EQKPWithAttnScaleMaxRowDiffMaxMinFloat{0.1520296633243560791015625}
\def\EQKPWithAttnScaleMaxRowDiffMaxMinKey{6532}
\def\EQKPWithAttnScaleMaxRowDiffMaxStdDevFloat{0.3728179633617401123046875}
\def\EQKPWithAttnScaleMaxRowDiffMeanLen{151}
\def\EQKPWithAttnScaleMaxRowDiffMeanMaxFloat{1.70682322978973388671875}
\def\EQKPWithAttnScaleMaxRowDiffMeanMaxKey{13036}
\def\EQKPWithAttnScaleMaxRowDiffMeanMeanFloat{0.4921910464763641357421875}
\def\EQKPWithAttnScaleMaxRowDiffMeanMeanKey{2236}
\def\EQKPWithAttnScaleMaxRowDiffMeanMedianFloat{0.10143413208425045013427734375}
\def\EQKPWithAttnScaleMaxRowDiffMeanMedianKey{6532}
\def\EQKPWithAttnScaleMaxRowDiffMeanMinFloat{0.0777740478515625}
\def\EQKPWithAttnScaleMaxRowDiffMeanMinKey{17197}
\def\EQKPWithAttnScaleMaxRowDiffMeanStdDevFloat{0.309645473957061767578125}
\def\EQKPWithAttnScaleMaxRowDiffMedianLen{151}
\def\EQKPWithAttnScaleMaxRowDiffMedianMaxFloat{1.4558773565292357776712606209912337362766265869140625}
\def\EQKPWithAttnScaleMaxRowDiffMedianMaxKey{13036}
\def\EQKPWithAttnScaleMaxRowDiffMedianMeanFloat{0.334944275529833135340851413275231607258319854736328125}
\def\EQKPWithAttnScaleMaxRowDiffMedianMeanKey{20976}
\def\EQKPWithAttnScaleMaxRowDiffMedianMedianFloat{0.0506315775564871728420257568359375}
\def\EQKPWithAttnScaleMaxRowDiffMedianMedianKey{123}
\def\EQKPWithAttnScaleMaxRowDiffMedianMinFloat{0.0245246459078043710366756613439065404236316680908203125}
\def\EQKPWithAttnScaleMaxRowDiffMedianMinKey{17197}
\def\EQKPWithAttnScaleMaxRowDiffMedianStdDevFloat{0.255085415875143883823739088256843388080596923828125}
\def\EQKPWithAttnScaleMaxRowDiffMinLen{151}
\def\EQKPWithAttnScaleMaxRowDiffMinMaxFloat{1.4522583484649658203125}
\def\EQKPWithAttnScaleMaxRowDiffMinMaxKey{13036}
\def\EQKPWithAttnScaleMaxRowDiffMinMeanFloat{0.3266991674900054931640625}
\def\EQKPWithAttnScaleMaxRowDiffMinMeanKey{15662}
\def\EQKPWithAttnScaleMaxRowDiffMinMedianFloat{0.048781163990497589111328125}
\def\EQKPWithAttnScaleMaxRowDiffMinMedianKey{123}
\def\EQKPWithAttnScaleMaxRowDiffMinMinFloat{0.02448229491710662841796875}
\def\EQKPWithAttnScaleMaxRowDiffMinMinKey{17197}
\def\EQKPWithAttnScaleMaxRowDiffMinStdDevFloat{0.2527310550212860107421875}
\def\EQKPWithAttnScaleMaxRowDiffStdDevLen{151}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMaxFloat{0.17745013535022735595703125}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMaxKey{5615}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMeanFloat{0.072068773210048675537109375}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMeanKey{11130}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMedianFloat{0.023389621637761592864990234375}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMedianKey{30371}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMinFloat{0.01658443547785282135009765625}
\def\EQKPWithAttnScaleMaxRowDiffStdDevMinKey{6532}
\def\EQKPWithAttnScaleMaxRowDiffStdDevStdDevFloat{0.0329684056341648101806640625}
\def\EQKPWithAttnScaleMaxStdDevFloat{0.2069334089756011962890625}
\def\EQKPWithAttnScaleMeanLen{151}
\def\EQKPWithAttnScaleMeanMaxFloat{0.0000003618770278990268707275390625}
\def\EQKPWithAttnScaleMeanMaxKey{23367}
\def\EQKPWithAttnScaleMeanMeanFloat{0.0000000194277109955010018893517553806304931640625}
\def\EQKPWithAttnScaleMeanMeanKey{20415}
\def\EQKPWithAttnScaleMeanMedianFloat{-0.00000027479254782747375429607927799224853515625}
\def\EQKPWithAttnScaleMeanMedianKey{15043}
\def\EQKPWithAttnScaleMeanMinFloat{-0.00000029841902460248093120753765106201171875}
\def\EQKPWithAttnScaleMeanMinKey{12561}
\def\EQKPWithAttnScaleMeanStdDevFloat{0.000000127967581420307396911084651947021484375}
\def\EQKPWithAttnScaleMedianLen{151}
\def\EQKPWithAttnScaleMedianMaxFloat{-0.07740570720285176731234599856179556809365749359130859375}
\def\EQKPWithAttnScaleMedianMaxKey{6532}
\def\EQKPWithAttnScaleMedianMeanFloat{-0.320654567495136488819440501174540258944034576416015625}
\def\EQKPWithAttnScaleMedianMeanKey{20976}
\def\EQKPWithAttnScaleMedianMedianFloat{-1.1560420833528042283688819225062616169452667236328125}
\def\EQKPWithAttnScaleMedianMedianKey{13036}
\def\EQKPWithAttnScaleMedianMinFloat{-1.237574647665023785947369105997495353221893310546875}
\def\EQKPWithAttnScaleMedianMinKey{28090}
\def\EQKPWithAttnScaleMedianStdDevFloat{0.1879711568738885729690224479782045818865299224853515625}
\def\EQKPWithAttnScaleMinLen{151}
\def\EQKPWithAttnScaleMinMaxFloat{-0.081806086003780364990234375}
\def\EQKPWithAttnScaleMinMaxKey{6532}
\def\EQKPWithAttnScaleMinMeanFloat{-0.3400589525699615478515625}
\def\EQKPWithAttnScaleMinMeanKey{12493}
\def\EQKPWithAttnScaleMinMedianFloat{-1.240361034870147705078125}
\def\EQKPWithAttnScaleMinMedianKey{13036}
\def\EQKPWithAttnScaleMinMinFloat{-1.2957820892333984375}
\def\EQKPWithAttnScaleMinMinKey{28090}
\def\EQKPWithAttnScaleMinStdDevFloat{0.19386495649814605712890625}
\def\EQKPWithAttnScaleStdDevLen{151}
\def\EQKPWithAttnScaleStdDevMaxFloat{0.690461695194244384765625}
\def\EQKPWithAttnScaleStdDevMaxKey{13036}
\def\EQKPWithAttnScaleStdDevMeanFloat{0.17926295101642608642578125}
\def\EQKPWithAttnScaleStdDevMeanKey{20976}
\def\EQKPWithAttnScaleStdDevMedianFloat{0.0405226214788854122161865234375}
\def\EQKPWithAttnScaleStdDevMedianKey{6532}
\def\EQKPWithAttnScaleStdDevMinFloat{0.03029319457709789276123046875}
\def\EQKPWithAttnScaleStdDevMinKey{17197}
\def\EQKPWithAttnScaleStdDevStdDevFloat{0.11637885868549346923828125}
\def\EUPUAbsLenLen{151}
\def\EUPUAbsLenMaxFloat{4096}
\def\EUPUAbsLenMaxKey{50}
\def\EUPUAbsLenMeanFloat{4096}
\def\EUPUAbsLenMeanKey{50}
\def\EUPUAbsLenMedianFloat{4096}
\def\EUPUAbsLenMedianKey{50}
\def\EUPUAbsLenMinFloat{4096}
\def\EUPUAbsLenMinKey{50}
\def\EUPUAbsLenStdDevFloat{0}
\def\EUPUAbsMaxLen{151}
\def\EUPUAbsMaxMaxFloat{3.3545131683349609375}
\def\EUPUAbsMaxMaxKey{20338}
\def\EUPUAbsMaxMeanFloat{2.4737370014190673828125}
\def\EUPUAbsMaxMeanKey{13036}
\def\EUPUAbsMaxMedianFloat{1.9722721278667449951171875}
\def\EUPUAbsMaxMedianKey{29725}
\def\EUPUAbsMaxMinFloat{1.93549072742462158203125}
\def\EUPUAbsMaxMinKey{742}
\def\EUPUAbsMaxStdDevFloat{0.20377455651760101318359375}
\def\EUPUAbsMeanLen{151}
\def\EUPUAbsMeanMaxFloat{0.876845836639404296875}
\def\EUPUAbsMeanMaxKey{32103}
\def\EUPUAbsMeanMeanFloat{0.74820768833160400390625}
\def\EUPUAbsMeanMeanKey{6082}
\def\EUPUAbsMeanMedianFloat{0.5243438780307769775390625}
\def\EUPUAbsMeanMedianKey{22545}
\def\EUPUAbsMeanMinFloat{0.512855708599090576171875}
\def\EUPUAbsMeanMinKey{20976}
\def\EUPUAbsMeanStdDevFloat{0.065898239612579345703125}
\def\EUPUAbsMedianLen{151}
\def\EUPUAbsMedianMaxFloat{0.0122056715656071908260305036719728377647697925567626953125}
\def\EUPUAbsMedianMaxKey{4430}
\def\EUPUAbsMedianMeanFloat{0.006913760279086325795383505266045176540501415729522705078125}
\def\EUPUAbsMedianMeanKey{18146}
\def\EUPUAbsMedianMedianFloat{0.003700923986616544598959865908227584441192448139190673828125}
\def\EUPUAbsMedianMedianKey{4305}
\def\EUPUAbsMedianMinFloat{0.0028793175355531276139731122754028547205962240695953369140625}
\def\EUPUAbsMedianMinKey{1681}
\def\EUPUAbsMedianStdDevFloat{0.00168249555442770187992096442286538149346597492694854736328125}
\def\EUPUAbsMinLen{151}
\def\EUPUAbsMinMaxFloat{0.00239464291371405124664306640625}
\def\EUPUAbsMinMaxKey{20294}
\def\EUPUAbsMinMeanFloat{0.0003328705788590013980865478515625}
\def\EUPUAbsMinMeanKey{20754}
\def\EUPUAbsMinMedianFloat{0.000007992102837306447327136993408203125}
\def\EUPUAbsMinMedianKey{16284}
\def\EUPUAbsMinMinFloat{0.0000022821550373919308185577392578125}
\def\EUPUAbsMinMinKey{7467}
\def\EUPUAbsMinStdDevFloat{0.00035282582393847405910491943359375}
\def\EUPUAbsStdDevLen{151}
\def\EUPUAbsStdDevMaxFloat{0.589696228504180908203125}
\def\EUPUAbsStdDevMaxKey{4647}
\def\EUPUAbsStdDevMeanFloat{0.49544298648834228515625}
\def\EUPUAbsStdDevMeanKey{24202}
\def\EUPUAbsStdDevMedianFloat{0.3781120777130126953125}
\def\EUPUAbsStdDevMedianKey{29725}
\def\EUPUAbsStdDevMinFloat{0.3611139357089996337890625}
\def\EUPUAbsStdDevMinKey{20976}
\def\EUPUAbsStdDevStdDevFloat{0.041514210402965545654296875}
\def\EUPULenLen{151}
\def\EUPULenMaxFloat{4096}
\def\EUPULenMaxKey{50}
\def\EUPULenMeanFloat{4096}
\def\EUPULenMeanKey{50}
\def\EUPULenMedianFloat{4096}
\def\EUPULenMedianKey{50}
\def\EUPULenMinFloat{4096}
\def\EUPULenMinKey{50}
\def\EUPULenStdDevFloat{0}
\def\EUPUMaxLen{151}
\def\EUPUMaxMaxFloat{3.3545131683349609375}
\def\EUPUMaxMaxKey{20338}
\def\EUPUMaxMeanFloat{2.082238674163818359375}
\def\EUPUMaxMeanKey{18289}
\def\EUPUMaxMedianFloat{1.6632813513278961181640625}
\def\EUPUMaxMedianKey{4729}
\def\EUPUMaxMinFloat{1.64611494541168212890625}
\def\EUPUMaxMinKey{11598}
\def\EUPUMaxRowDiffLenLen{151}
\def\EUPUMaxRowDiffLenMaxFloat{64}
\def\EUPUMaxRowDiffLenMaxKey{50}
\def\EUPUMaxRowDiffLenMeanFloat{64}
\def\EUPUMaxRowDiffLenMeanKey{50}
\def\EUPUMaxRowDiffLenMedianFloat{64}
\def\EUPUMaxRowDiffLenMedianKey{50}
\def\EUPUMaxRowDiffLenMinFloat{64}
\def\EUPUMaxRowDiffLenMinKey{50}
\def\EUPUMaxRowDiffLenStdDevFloat{0}
\def\EUPUMaxRowDiffMaxLen{151}
\def\EUPUMaxRowDiffMaxMaxFloat{5.04686069488525390625}
\def\EUPUMaxRowDiffMaxMaxKey{20338}
\def\EUPUMaxRowDiffMaxMeanFloat{4.247914791107177734375}
\def\EUPUMaxRowDiffMaxMeanKey{27300}
\def\EUPUMaxRowDiffMaxMedianFloat{3.555904805660247802734375}
\def\EUPUMaxRowDiffMaxMedianKey{742}
\def\EUPUMaxRowDiffMaxMinFloat{3.502239704132080078125}
\def\EUPUMaxRowDiffMaxMinKey{29725}
\def\EUPUMaxRowDiffMaxStdDevFloat{0.30486166477203369140625}
\def\EUPUMaxRowDiffMeanLen{151}
\def\EUPUMaxRowDiffMeanMaxFloat{3.744059085845947265625}
\def\EUPUMaxRowDiffMeanMaxKey{19451}
\def\EUPUMaxRowDiffMeanMeanFloat{3.218198299407958984375}
\def\EUPUMaxRowDiffMeanMeanKey{7467}
\def\EUPUMaxRowDiffMeanMedianFloat{2.49102056026458740234375}
\def\EUPUMaxRowDiffMeanMedianKey{22545}
\def\EUPUMaxRowDiffMeanMinFloat{2.449840068817138671875}
\def\EUPUMaxRowDiffMeanMinKey{20976}
\def\EUPUMaxRowDiffMeanStdDevFloat{0.211375892162322998046875}
\def\EUPUMaxRowDiffMedianLen{151}
\def\EUPUMaxRowDiffMedianMaxFloat{2.965534255504608029951896241982467472553253173828125}
\def\EUPUMaxRowDiffMedianMaxKey{32382}
\def\EUPUMaxRowDiffMedianMeanFloat{2.497676087377087572605205423315055668354034423828125}
\def\EUPUMaxRowDiffMedianMeanKey{123}
\def\EUPUMaxRowDiffMedianMedianFloat{1.741035361438989514937247804482467472553253173828125}
\def\EUPUMaxRowDiffMedianMedianKey{1681}
\def\EUPUMaxRowDiffMedianMinFloat{1.6061110162734986150923077730112709105014801025390625}
\def\EUPUMaxRowDiffMedianMinKey{22545}
\def\EUPUMaxRowDiffMedianStdDevFloat{0.2350037006188165078501839388991356827318668365478515625}
\def\EUPUMaxRowDiffMinLen{151}
\def\EUPUMaxRowDiffMinMaxFloat{2.936122417449951171875}
\def\EUPUMaxRowDiffMinMaxKey{32382}
\def\EUPUMaxRowDiffMinMeanFloat{2.4643456935882568359375}
\def\EUPUMaxRowDiffMinMeanKey{1412}
\def\EUPUMaxRowDiffMinMedianFloat{1.6929533481597900390625}
\def\EUPUMaxRowDiffMinMedianKey{20976}
\def\EUPUMaxRowDiffMinMinFloat{1.5818347930908203125}
\def\EUPUMaxRowDiffMinMinKey{22545}
\def\EUPUMaxRowDiffMinStdDevFloat{0.23633737862110137939453125}
\def\EUPUMaxRowDiffStdDevLen{151}
\def\EUPUMaxRowDiffStdDevMaxFloat{0.635314881801605224609375}
\def\EUPUMaxRowDiffStdDevMaxKey{22545}
\def\EUPUMaxRowDiffStdDevMeanFloat{0.3836612999439239501953125}
\def\EUPUMaxRowDiffStdDevMeanKey{28090}
\def\EUPUMaxRowDiffStdDevMedianFloat{0.2438377402722835540771484375}
\def\EUPUMaxRowDiffStdDevMedianKey{26374}
\def\EUPUMaxRowDiffStdDevMinFloat{0.236813068389892578125}
\def\EUPUMaxRowDiffStdDevMinKey{8299}
\def\EUPUMaxRowDiffStdDevStdDevFloat{0.075828649103641510009765625}
\def\EUPUMaxStdDevFloat{0.22372888028621673583984375}
\def\EUPUMeanLen{151}
\def\EUPUMeanMaxFloat{-0.174616992473602294921875}
\def\EUPUMeanMaxKey{22545}
\def\EUPUMeanMeanFloat{-0.3560569286346435546875}
\def\EUPUMeanMeanKey{32382}
\def\EUPUMeanMedianFloat{-0.492204360663890838623046875}
\def\EUPUMeanMedianKey{7310}
\def\EUPUMeanMinFloat{-0.496133863925933837890625}
\def\EUPUMeanMinKey{32103}
\def\EUPUMeanStdDevFloat{0.0608513392508029937744140625}
\def\EUPUMedianLen{151}
\def\EUPUMedianMaxFloat{-1.640270495414733797900908029987476766109466552734375}
\def\EUPUMedianMaxKey{20976}
\def\EUPUMedianMeanFloat{-2.02903103396197792562816175632178783416748046875}
\def\EUPUMedianMeanKey{24566}
\def\EUPUMedianMedianFloat{-2.31279916018247622133685581502504646778106689453125}
\def\EUPUMedianMedianKey{32103}
\def\EUPUMedianMinFloat{-2.3694505393505096435546875}
\def\EUPUMedianMinKey{19488}
\def\EUPUMedianStdDevFloat{0.1411028957335200839651179194333963096141815185546875}
\def\EUPUMinLen{151}
\def\EUPUMinMaxFloat{-1.93549072742462158203125}
\def\EUPUMinMaxKey{742}
\def\EUPUMinMeanFloat{-2.4643485546112060546875}
\def\EUPUMinMeanKey{20294}
\def\EUPUMinMedianFloat{-3.004130899906158447265625}
\def\EUPUMinMedianKey{19917}
\def\EUPUMinMinFloat{-3.1007349491119384765625}
\def\EUPUMinMinKey{20338}
\def\EUPUMinStdDevFloat{0.202433884143829345703125}
\def\EUPUStdDevLen{151}
\def\EUPUStdDevMaxFloat{0.933885872364044189453125}
\def\EUPUStdDevMaxKey{19451}
\def\EUPUStdDevMeanFloat{0.82284033298492431640625}
\def\EUPUStdDevMeanKey{18146}
\def\EUPUStdDevMedianFloat{0.62941651046276092529296875}
\def\EUPUStdDevMedianKey{22545}
\def\EUPUStdDevMinFloat{0.593832492828369140625}
\def\EUPUStdDevMinKey{20976}
\def\EUPUStdDevStdDevFloat{0.0616363249719142913818359375}
\def\EVOUHistMinAboveDiagDupBySeqCountLenLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMaxFloat{1073741824}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMaxKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMeanFloat{1073741824}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMeanKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMedianFloat{1073741824}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMedianKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMinFloat{1073741824}
\def\EVOUHistMinAboveDiagDupBySeqCountLenMinKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountLenStdDevFloat{0}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMaxFloat{18.032024383544921875}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMaxKey{742}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMeanFloat{13.03078556060791015625}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMeanKey{3284}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMedianFloat{9.9842927455902099609375}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMedianKey{23241}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMinFloat{9.797515869140625}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxMinKey{27584}
\def\EVOUHistMinAboveDiagDupBySeqCountMaxStdDevFloat{1.63968122005462646484375}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMaxFloat{-7.445113177426065931285847909748554229736328125}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMaxKey{1490}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMeanFloat{-9.0460775926385874612378756864927709102630615234375}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMeanKey{32382}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMedianFloat{-9.8369579125901633886996933142654597759246826171875}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMedianKey{123}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMinFloat{-9.8980826346909847046617869636975228786468505859375}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanMinKey{17080}
\def\EVOUHistMinAboveDiagDupBySeqCountMeanStdDevFloat{0.43029775657320123993798688388778828084468841552734375}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMaxFloat{-6.9356895168367618254023909685201942920684814453125}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMaxKey{1490}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMeanFloat{-9.1925161211539307970497247879393398761749267578125}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMeanKey{8048}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMedianFloat{-10.3003624078271496244951777043752372264862060546875}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMedianKey{20754}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMinFloat{-10.3014516443283934421515368740074336528778076171875}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianMinKey{20294}
\def\EVOUHistMinAboveDiagDupBySeqCountMedianStdDevFloat{0.612852091429516576681635342538356781005859375}
\def\EVOUHistMinAboveDiagDupBySeqCountMinLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMaxFloat{-10.913974761962890625}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMaxKey{12552}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMeanFloat{-13.23870754241943359375}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMeanKey{20754}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMedianFloat{-16.43675518035888671875}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMedianKey{4810}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMinFloat{-17.3886890411376953125}
\def\EVOUHistMinAboveDiagDupBySeqCountMinMinKey{21317}
\def\EVOUHistMinAboveDiagDupBySeqCountMinStdDevFloat{1.0667011737823486328125}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMaxFloat{5}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMaxKey{30463}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMeanFloat{-2.291390728476821347925351801677606999874114990234375}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMeanKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMedianFloat{-5}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMedianKey{913}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMinFloat{-5}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueMinKey{913}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMaxFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMaxKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMeanFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMeanKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMedianFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMedianKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMinFloat{1}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdMinKey{50}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueNumStdStdDevFloat{0}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMaxFloat{0.999969482421875}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMaxKey{1412}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMeanFloat{0.99334280972449195967755031233537010848522186279296875}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMeanKey{7790}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMedianFloat{0.9507879912853240966796875}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMedianKey{6159}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMinFloat{0.94461095333099365234375}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracMinKey{27584}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueSequenceFracStdDevFloat{0.009936352999980420375170098168382537551224231719970703125}
\def\EVOUHistMinAboveDiagDupBySeqCountMostBelowValueStdDevFloat{1.9070778033403643636489732671179808676242828369140625}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevLen{151}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMaxFloat{7.09607978199045863476612794329412281513214111328125}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMaxKey{1412}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMeanFloat{5.7051752944113953702753860852681100368499755859375}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMeanKey{2306}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMedianFloat{4.814672792118923183579681790433824062347412109375}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMedianKey{8048}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMinFloat{4.422168094044128139330496196635067462921142578125}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevMinKey{12552}
\def\EVOUHistMinAboveDiagDupBySeqCountStdDevStdDevFloat{0.381014793494892867187218143953941762447357177734375}
\def\EVOUHistMinAboveDiagLenLen{151}
\def\EVOUHistMinAboveDiagLenMaxFloat{64}
\def\EVOUHistMinAboveDiagLenMaxKey{50}
\def\EVOUHistMinAboveDiagLenMeanFloat{64}
\def\EVOUHistMinAboveDiagLenMeanKey{50}
\def\EVOUHistMinAboveDiagLenMedianFloat{64}
\def\EVOUHistMinAboveDiagLenMedianKey{50}
\def\EVOUHistMinAboveDiagLenMinFloat{64}
\def\EVOUHistMinAboveDiagLenMinKey{50}
\def\EVOUHistMinAboveDiagLenStdDevFloat{0}
\def\EVOUHistMinAboveDiagMaxLen{151}
\def\EVOUHistMinAboveDiagMaxMaxFloat{18.032024383544921875}
\def\EVOUHistMinAboveDiagMaxMaxKey{742}
\def\EVOUHistMinAboveDiagMaxMeanFloat{13.03078556060791015625}
\def\EVOUHistMinAboveDiagMaxMeanKey{3284}
\def\EVOUHistMinAboveDiagMaxMedianFloat{9.9842927455902099609375}
\def\EVOUHistMinAboveDiagMaxMedianKey{23241}
\def\EVOUHistMinAboveDiagMaxMinFloat{9.797515869140625}
\def\EVOUHistMinAboveDiagMaxMinKey{27584}
\def\EVOUHistMinAboveDiagMaxStdDevFloat{1.63968122005462646484375}
\def\EVOUHistMinAboveDiagMeanLen{151}
\def\EVOUHistMinAboveDiagMeanMaxFloat{-2.9787502288818359375}
\def\EVOUHistMinAboveDiagMeanMaxKey{20976}
\def\EVOUHistMinAboveDiagMeanMeanFloat{-3.92082881927490234375}
\def\EVOUHistMinAboveDiagMeanMeanKey{26829}
\def\EVOUHistMinAboveDiagMeanMedianFloat{-4.651565074920654296875}
\def\EVOUHistMinAboveDiagMeanMedianKey{123}
\def\EVOUHistMinAboveDiagMeanMinFloat{-4.755002498626708984375}
\def\EVOUHistMinAboveDiagMeanMinKey{23367}
\def\EVOUHistMinAboveDiagMeanStdDevFloat{0.3901725709438323974609375}
\def\EVOUHistMinAboveDiagMedianLen{151}
\def\EVOUHistMinAboveDiagMedianMaxFloat{-3.668115139007568359375}
\def\EVOUHistMinAboveDiagMedianMaxKey{27484}
\def\EVOUHistMinAboveDiagMedianMeanFloat{-5.4294407888753521973512761178426444530487060546875}
\def\EVOUHistMinAboveDiagMedianMeanKey{4305}
\def\EVOUHistMinAboveDiagMedianMedianFloat{-6.6412785053253173828125}
\def\EVOUHistMinAboveDiagMedianMedianKey{30899}
\def\EVOUHistMinAboveDiagMedianMinFloat{-7.006985187530517578125}
\def\EVOUHistMinAboveDiagMedianMinKey{13654}
\def\EVOUHistMinAboveDiagMedianStdDevFloat{0.55919137272839047891892505504074506461620330810546875}
\def\EVOUHistMinAboveDiagMinLen{151}
\def\EVOUHistMinAboveDiagMinMaxFloat{-10.913974761962890625}
\def\EVOUHistMinAboveDiagMinMaxKey{12552}
\def\EVOUHistMinAboveDiagMinMeanFloat{-13.23870754241943359375}
\def\EVOUHistMinAboveDiagMinMeanKey{20754}
\def\EVOUHistMinAboveDiagMinMedianFloat{-16.43675518035888671875}
\def\EVOUHistMinAboveDiagMinMedianKey{4810}
\def\EVOUHistMinAboveDiagMinMinFloat{-17.3886890411376953125}
\def\EVOUHistMinAboveDiagMinMinKey{21317}
\def\EVOUHistMinAboveDiagMinStdDevFloat{1.0667011737823486328125}
\def\EVOUHistMinAboveDiagMostBelowValueLen{151}
\def\EVOUHistMinAboveDiagMostBelowValueMaxFloat{44}
\def\EVOUHistMinAboveDiagMostBelowValueMaxKey{1696}
\def\EVOUHistMinAboveDiagMostBelowValueMeanFloat{33.29139072847682001565772225148975849151611328125}
\def\EVOUHistMinAboveDiagMostBelowValueMeanKey{519}
\def\EVOUHistMinAboveDiagMostBelowValueMedianFloat{23.5}
\def\EVOUHistMinAboveDiagMostBelowValueMedianKey{2236}
\def\EVOUHistMinAboveDiagMostBelowValueMinFloat{22}
\def\EVOUHistMinAboveDiagMostBelowValueMinKey{4430}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdLen{151}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMaxFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMaxKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMeanFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMeanKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMedianFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMedianKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMinFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdMinKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueNumStdStdDevFloat{0}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracLen{151}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMaxFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMaxKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMeanFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMeanKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMedianFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMedianKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMinFloat{1}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracMinKey{50}
\def\EVOUHistMinAboveDiagMostBelowValueSequenceFracStdDevFloat{0}
\def\EVOUHistMinAboveDiagMostBelowValueStdDevFloat{4.47744813197021596096192297409288585186004638671875}
\def\EVOUHistMinAboveDiagStdDevLen{151}
\def\EVOUHistMinAboveDiagStdDevMaxFloat{6.921452999114990234375}
\def\EVOUHistMinAboveDiagStdDevMaxKey{1696}
\def\EVOUHistMinAboveDiagStdDevMeanFloat{6.1307697296142578125}
\def\EVOUHistMinAboveDiagStdDevMeanKey{23367}
\def\EVOUHistMinAboveDiagStdDevMedianFloat{5.29597938060760498046875}
\def\EVOUHistMinAboveDiagStdDevMedianKey{2236}
\def\EVOUHistMinAboveDiagStdDevMinFloat{5.150132656097412109375}
\def\EVOUHistMinAboveDiagStdDevMinKey{4430}
\def\EVOUHistMinAboveDiagStdDevStdDevFloat{0.3504555523395538330078125}
\def\EVOUMaxRowDiffLenLen{151}
\def\EVOUMaxRowDiffLenMaxFloat{64}
\def\EVOUMaxRowDiffLenMaxKey{50}
\def\EVOUMaxRowDiffLenMeanFloat{64}
\def\EVOUMaxRowDiffLenMeanKey{50}
\def\EVOUMaxRowDiffLenMedianFloat{64}
\def\EVOUMaxRowDiffLenMedianKey{50}
\def\EVOUMaxRowDiffLenMinFloat{64}
\def\EVOUMaxRowDiffLenMinKey{50}
\def\EVOUMaxRowDiffLenStdDevFloat{0}
\def\EVOUMaxRowDiffMaxLen{151}
\def\EVOUMaxRowDiffMaxMaxFloat{83.710205078125}
\def\EVOUMaxRowDiffMaxMaxKey{6532}
\def\EVOUMaxRowDiffMaxMeanFloat{64.777679443359375}
\def\EVOUMaxRowDiffMaxMeanKey{28090}
\def\EVOUMaxRowDiffMaxMedianFloat{54.599857330322265625}
\def\EVOUMaxRowDiffMaxMedianKey{12552}
\def\EVOUMaxRowDiffMaxMinFloat{54.20905303955078125}
\def\EVOUMaxRowDiffMaxMinKey{6159}
\def\EVOUMaxRowDiffMaxStdDevFloat{5.014739990234375}
\def\EVOUMaxRowDiffMeanLen{151}
\def\EVOUMaxRowDiffMeanMaxFloat{46.064239501953125}
\def\EVOUMaxRowDiffMeanMaxKey{1412}
\def\EVOUMaxRowDiffMeanMeanFloat{40.99593353271484375}
\def\EVOUMaxRowDiffMeanMeanKey{24262}
\def\EVOUMaxRowDiffMeanMedianFloat{36.09512424468994140625}
\def\EVOUMaxRowDiffMeanMedianKey{20338}
\def\EVOUMaxRowDiffMeanMinFloat{35.826007843017578125}
\def\EVOUMaxRowDiffMeanMinKey{12552}
\def\EVOUMaxRowDiffMeanStdDevFloat{2.094542980194091796875}
\def\EVOUMaxRowDiffMedianLen{151}
\def\EVOUMaxRowDiffMedianMaxFloat{31.333910045623778017898075631819665431976318359375}
\def\EVOUMaxRowDiffMedianMaxKey{26374}
\def\EVOUMaxRowDiffMedianMeanFloat{25.880793708460220869937984389252960681915283203125}
\def\EVOUMaxRowDiffMedianMeanKey{13654}
\def\EVOUMaxRowDiffMedianMedianFloat{19.985473034381865176101200631819665431976318359375}
\def\EVOUMaxRowDiffMedianMedianKey{26278}
\def\EVOUMaxRowDiffMedianMinFloat{19.8673633480072027168716886080801486968994140625}
\def\EVOUMaxRowDiffMedianMinKey{25516}
\def\EVOUMaxRowDiffMedianStdDevFloat{2.507577341166369766511934358277358114719390869140625}
\def\EVOUMaxRowDiffMinLen{151}
\def\EVOUMaxRowDiffMinMaxFloat{31.3306884765625}
\def\EVOUMaxRowDiffMinMaxKey{26374}
\def\EVOUMaxRowDiffMinMeanFloat{24.9985141754150390625}
\def\EVOUMaxRowDiffMinMeanKey{12457}
\def\EVOUMaxRowDiffMinMedianFloat{17.923167705535888671875}
\def\EVOUMaxRowDiffMinMedianKey{14095}
\def\EVOUMaxRowDiffMinMinFloat{17.6306781768798828125}
\def\EVOUMaxRowDiffMinMinKey{25516}
\def\EVOUMaxRowDiffMinStdDevFloat{2.9584286212921142578125}
\def\EVOUMaxRowDiffStdDevLen{151}
\def\EVOUMaxRowDiffStdDevMaxFloat{9.96619415283203125}
\def\EVOUMaxRowDiffStdDevMaxKey{4430}
\def\EVOUMaxRowDiffStdDevMeanFloat{7.661200046539306640625}
\def\EVOUMaxRowDiffStdDevMeanKey{2743}
\def\EVOUMaxRowDiffStdDevMedianFloat{6.03261387348175048828125}
\def\EVOUMaxRowDiffStdDevMedianKey{29110}
\def\EVOUMaxRowDiffStdDevMinFloat{5.963802337646484375}
\def\EVOUMaxRowDiffStdDevMinKey{20013}
\def\EVOUMaxRowDiffStdDevStdDevFloat{0.814879477024078369140625}
\def\ImportanceSamplingAccuracyLen{151}
\def\ImportanceSamplingAccuracyMaxFloat{0.999790990426329795326410021516494452953338623046875}
\def\ImportanceSamplingAccuracyMaxKey{11598}
\def\ImportanceSamplingAccuracyMeanFloat{0.99904371382544443491724450723268091678619384765625}
\def\ImportanceSamplingAccuracyMeanKey{9132}
\def\ImportanceSamplingAccuracyMedianFloat{0.98527418983453485257228976479382254183292388916015625}
\def\ImportanceSamplingAccuracyMedianKey{13036}
\def\ImportanceSamplingAccuracyMinFloat{0.98448659854122400059139863515156321227550506591796875}
\def\ImportanceSamplingAccuracyMinKey{28090}
\def\ImportanceSamplingAccuracyStdDevFloat{0.00182288756287233601194319732030635350383818149566650390625}
\def\ImportanceSamplingBatchSize{4096}
\def\ImportanceSamplingInstructionCountBranch{0}
\def\ImportanceSamplingInstructionCountInt{0}
\def\ImportanceSamplingInstructionCount{0}
\def\ImportanceSamplingLossLen{151}
\def\ImportanceSamplingLossMaxFloat{0.09694168145628960508997096212624455802142620086669921875}
\def\ImportanceSamplingLossMaxKey{28090}
\def\ImportanceSamplingLossMeanFloat{0.004674988352514779232915742568366113118827342987060546875}
\def\ImportanceSamplingLossMeanKey{4729}
\def\ImportanceSamplingLossMedianFloat{0.0016169221037055999008746898226718258229084312915802001953125}
\def\ImportanceSamplingLossMedianKey{3254}
\def\ImportanceSamplingLossMinFloat{0.00152776866387070004403569978279620045213960111141204833984375}
\def\ImportanceSamplingLossMinKey{23367}
\def\ImportanceSamplingLossStdDevFloat{0.00922773972677012367660243086220361874438822269439697265625}
\def\ImportanceSamplingNSamplesPerKey{30}
\def\ImportanceSamplingNumCorrectLen{151}
\def\ImportanceSamplingNumCorrectMaxFloat{5493692}
\def\ImportanceSamplingNumCorrectMaxKey{32374}
\def\ImportanceSamplingNumCorrectMeanFloat{5473144.072847682051360607147216796875}
\def\ImportanceSamplingNumCorrectMeanKey{22286}
\def\ImportanceSamplingNumCorrectMedianFloat{5411474}
\def\ImportanceSamplingNumCorrectMedianKey{28090}
\def\ImportanceSamplingNumCorrectMinFloat{5384198}
\def\ImportanceSamplingNumCorrectMinKey{20338}
\def\ImportanceSamplingNumCorrectStdDevFloat{13633.202438524580429657362401485443115234375}
\def\ImportanceSamplingNumIncorrectLen{151}
\def\ImportanceSamplingNumIncorrectMaxFloat{133617}
\def\ImportanceSamplingNumIncorrectMaxKey{20338}
\def\ImportanceSamplingNumIncorrectMeanFloat{44670.9271523178831557743251323699951171875}
\def\ImportanceSamplingNumIncorrectMeanKey{22286}
\def\ImportanceSamplingNumIncorrectMedianFloat{25494}
\def\ImportanceSamplingNumIncorrectMedianKey{24262}
\def\ImportanceSamplingNumIncorrectMinFloat{24123}
\def\ImportanceSamplingNumIncorrectMinKey{32374}
\def\ImportanceSamplingNumIncorrectStdDevFloat{13633.20243852457861066795885562896728515625}
\def\ImportanceSamplingTimeLen{151}
\def\ImportanceSamplingTimeMaxFloat{210.2947385311126708984375}
\def\ImportanceSamplingTimeMaxKey{7098}
\def\ImportanceSamplingTimeMeanFloat{198.759514339712268338189460337162017822265625}
\def\ImportanceSamplingTimeMeanKey{20751}
\def\ImportanceSamplingTimeMedianFloat{189.735531151294708251953125}
\def\ImportanceSamplingTimeMedianKey{27300}
\def\ImportanceSamplingTimeMinFloat{189.6438541412353515625}
\def\ImportanceSamplingTimeMinKey{27484}
\def\ImportanceSamplingTimeStdDevFloat{4.71299052693133102565070657874457538127899169921875}
\def\ImportanceSamplingTotalSequences{5517815}
\def\LowerWhiskerBottomEndPercentileFloat{0.02151239536919476169618548055950668640434741973876953125}
\def\LowerWhiskerCrosshatchPercentileFloat{0.08867177532617598334496733514242805540561676025390625}
\def\MedianPercentileFloat{0.5}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffExactLinearFitIntercept{0.28057669584399302920019181328825652599334716796875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffExactLinearFitRSquared{0.00003935813355859796303093389724381268024444580078125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffExactLinearFitSlope{0.000010722005640898462380957399664449525289455777965486049652099609375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffLinearFitIntercept{0.268927735218978225528729808502248488366603851318359375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffLinearFitRSquared{0.00006150568387230936906462375191040337085723876953125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffLinearFitSlope{0.0000129517993662180464528414780556175855963374488055706024169921875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductLinearFitIntercept{0.274159543817290407563547205427312292158603668212890625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductLinearFitRSquared{0.00004345753352108516764928936026990413665771484375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductLinearFitSlope{0.00001101929786809704371239836129259259678292437456548213958740234375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitIntercept{0.1352220490415485532054162831627763807773590087890625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitRSquared{0.00023631123984857449471519430517219007015228271484375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitSlope{0.0000134162701425136933887187484781833290981012396514415740966796875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffLinearFitIntercept{0.26902399941565724450498464648262597620487213134765625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffLinearFitRSquared{0.00005950643902041807820069152512587606906890869140625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffLinearFitSlope{0.000012739161975483342159110901337104593267213203944265842437744140625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitIntercept{0.273829435755729211354747576478985138237476348876953125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitRSquared{0.0000462264724527816639465527259744703769683837890625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitSlope{0.000011362840091242223182596733643823228021574323065578937530517578125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitIntercept{0.13517998017323684667445604645763523876667022705078125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitRSquared{0.000239432259785843370991642586886882781982421875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitSlope{0.0000135122893347359749141069207301057986114756204187870025634765625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitIntercept{0.13181288230463650279489229433238506317138671875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitRSquared{0.0002905133497355105731685398495756089687347412109375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitSlope{0.000014634364060209341317181190589291617243361542932689189910888671875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMaxDiffExactLinearFitIntercept{0.68167945860426026882805672357790172100067138671875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMaxDiffExactLinearFitSlope{-0.00122663929304291639300894534159169779741205275058746337890625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMaxDiffLinearFitIntercept{0.574372210048524234338174210279248654842376708984375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMaxDiffLinearFitSlope{-0.0009325558855067853612774708693677894189022481441497802734375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMaxDiffSubproductLinearFitIntercept{0.604523443841148644395389055716805160045623779296875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMaxDiffSubproductLinearFitSlope{-0.00100839857216946000850743558885369566269218921661376953125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMaxDiffSubproductRecursiveLinearFitIntercept{0.2779791236884026073283848745631985366344451904296875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMaxDiffSubproductRecursiveLinearFitSlope{-0.0004192050895160214624667049942985386223881505429744720458984375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMeanMaxDiffLinearFitIntercept{0.5826909970633333823997190847876481711864471435546875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMeanMaxDiffLinearFitSlope{-0.00095886908413347102068946536945759362424723803997039794921875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMeanMaxDiffSubproductLinearFitIntercept{0.60195453759516570624299447445082478225231170654296875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMeanMaxDiffSubproductLinearFitSlope{-0.00100087736222786278204865961782843442051671445369720458984375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMeanMaxDiffSubproductRecursiveLinearFitIntercept{0.27004180810523958911062436527572572231292724609375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMeanMaxDiffSubproductRecursiveLinearFitSlope{-0.0003928572308201855388214152053905081629636697471141815185546875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMeanRecursiveMaxDiffSubproductRecursiveLinearFitIntercept{0.2274065205686471580204255360513343475759029388427734375}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestMeanRecursiveMaxDiffSubproductRecursiveLinearFitSlope{-0.0002763733547081381920762499504462539334781467914581298828125}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestSvdLinearFitIntercept{0.304985735754721598578242947041871957480907440185546875}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioOnlySmallestSvdLinearFitSlope{-0.0003479354423165919988659988693058267017477191984653472900390625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioSvdLinearFitIntercept{0.1934908796421225540829169631251716054975986480712890625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioSvdLinearFitRSquared{0.0021518917136129633860264220857061445713043212890625}
\def\NormalizedAccuracyBoundAllSecondaryTricksVsEPQKESingularRatioSvdLinearFitSlope{0.0000672528504069615511336277524634397195768542587757110595703125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffExactLinearFitIntercept{0.69271654596089715649753770776442252099514007568359375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffExactLinearFitRSquared{0.00053903596257531827262710066861473023891448974609375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffExactLinearFitSlope{0.0000045145700536691099106719783640162546589635894633829593658447265625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffLinearFitIntercept{0.66574594556542965317902371680247597396373748779296875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffLinearFitRSquared{0.0024186304497051391848572166054509580135345458984375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffLinearFitSlope{0.000009951467219654795560014430566564413993546622805297374725341796875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductLinearFitIntercept{0.68450528139595279153439832953154109418392181396484375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductLinearFitRSquared{0.00079570127962214076688951536198146641254425048828125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductLinearFitSlope{-0.00000568214759963691346911045243484039701797883026301860809326171875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitIntercept{0.329546211530275190426664266851730644702911376953125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitRSquared{0.02906693795916492906172834409517236053943634033203125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMaxDiffSubproductRecursiveLinearFitSlope{0.000033997851974382678323129136632729796474450267851352691650390625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffLinearFitIntercept{0.666098727092784059777841321192681789398193359375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffLinearFitRSquared{0.00207389236956156963742614607326686382293701171875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffLinearFitSlope{0.000009167230049323194028369765629093990355613641440868377685546875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitIntercept{0.68401652574119309324629512047977186739444732666015625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitRSquared{0.00068147607682156330355383033747784793376922607421875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductLinearFitSlope{-0.000005257930534088421872947714807988717211628681980073451995849609375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitIntercept{0.33022781562263980870142177082016132771968841552734375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitRSquared{0.02658378753300449925944803908350877463817596435546875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanMaxDiffSubproductRecursiveLinearFitSlope{0.000033195114115536800028331831935446416537160985171794891357421875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitIntercept{0.324130538922564104264978368519223295152187347412109375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitRSquared{0.02955864979128619562942503762315027415752410888671875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioMeanRecursiveMaxDiffSubproductRecursiveLinearFitSlope{0.0000334858484028736184414352938798487002713955007493495941162109375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestMaxDiffExactLinearFitIntercept{1.07092262270847360383640989311970770359039306640625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestMaxDiffExactLinearFitSlope{-0.0011284987296146346824610162684621172957122325897216796875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestMaxDiffLinearFitIntercept{0.73176303562279521042199803559924475848674774169921875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestMaxDiffLinearFitSlope{-0.00016822313422596422462229615035766983055509626865386962890625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestMaxDiffSubproductLinearFitIntercept{0.7895674723411560957941901506274007260799407958984375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestMaxDiffSubproductLinearFitSlope{-0.0002790864722415566817094456641967781251878477632999420166015625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestMaxDiffSubproductRecursiveLinearFitIntercept{0.31167005315293538902921000044443644583225250244140625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestMaxDiffSubproductRecursiveLinearFitSlope{0.00012423900913624387281307404062857813187292777001857757568359375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestMeanMaxDiffLinearFitIntercept{0.7787958869079585344508132038754411041736602783203125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestMeanMaxDiffLinearFitSlope{-0.0003039252318483127122961118260491275577805936336517333984375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestMeanMaxDiffSubproductLinearFitIntercept{0.79998052528683227802019928276422433555126190185546875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestMeanMaxDiffSubproductLinearFitSlope{-0.0003108604559860256191620997423541439275140874087810516357421875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestMeanMaxDiffSubproductRecursiveLinearFitIntercept{0.191014018491225623375129316627862863242626190185546875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestMeanMaxDiffSubproductRecursiveLinearFitSlope{0.00050112553642357314694077974337460545939393341541290283203125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestMeanRecursiveMaxDiffSubproductRecursiveLinearFitIntercept{0.1858863754807733303930916690660524182021617889404296875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestMeanRecursiveMaxDiffSubproductRecursiveLinearFitSlope{0.00050315425070084226176481134729101540870033204555511474609375}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestSvdLinearFitIntercept{0.235954035293326203071018198897945694625377655029296875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioOnlySmallestSvdLinearFitSlope{0.000727393987062497390620741111177949278498999774456024169921875}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioSvdLinearFitIntercept{0.479888781779188366982680236105807125568389892578125}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioSvdLinearFitRSquared{0.36749972822026766294811750412918627262115478515625}
\def\NormalizedAccuracyBoundVsEPQKESingularRatioSvdLinearFitSlope{0.0001483980438828152938375570801809999466058798134326934814453125}
\def\NumSeeds{151}
\def\PVOUAbsLenLen{151}
\def\PVOUAbsLenMaxFloat{320}
\def\PVOUAbsLenMaxKey{50}
\def\PVOUAbsLenMeanFloat{320}
\def\PVOUAbsLenMeanKey{50}
\def\PVOUAbsLenMedianFloat{320}
\def\PVOUAbsLenMedianKey{50}
\def\PVOUAbsLenMinFloat{320}
\def\PVOUAbsLenMinKey{50}
\def\PVOUAbsLenStdDevFloat{0}
\def\PVOUAbsMaxLen{151}
\def\PVOUAbsMaxMaxFloat{2.042043209075927734375}
\def\PVOUAbsMaxMaxKey{4800}
\def\PVOUAbsMaxMeanFloat{1.061617374420166015625}
\def\PVOUAbsMaxMeanKey{15399}
\def\PVOUAbsMaxMedianFloat{0.62001971900463104248046875}
\def\PVOUAbsMaxMedianKey{20976}
\def\PVOUAbsMaxMinFloat{0.6114838123321533203125}
\def\PVOUAbsMaxMinKey{18289}
\def\PVOUAbsMaxStdDevFloat{0.2581799924373626708984375}
\def\PVOUAbsMeanLen{151}
\def\PVOUAbsMeanMaxFloat{0.416722476482391357421875}
\def\PVOUAbsMeanMaxKey{4430}
\def\PVOUAbsMeanMeanFloat{0.23994076251983642578125}
\def\PVOUAbsMeanMeanKey{2773}
\def\PVOUAbsMeanMedianFloat{0.15492595732212066650390625}
\def\PVOUAbsMeanMedianKey{27300}
\def\PVOUAbsMeanMinFloat{0.15252010524272918701171875}
\def\PVOUAbsMeanMinKey{6910}
\def\PVOUAbsMeanStdDevFloat{0.041588880121707916259765625}
\def\PVOUAbsMedianLen{151}
\def\PVOUAbsMedianMaxFloat{0.01198775008320808466155682481257827021181583404541015625}
\def\PVOUAbsMedianMaxKey{20013}
\def\PVOUAbsMedianMeanFloat{0.002891694517572570947983034983508332516066730022430419921875}
\def\PVOUAbsMedianMeanKey{6549}
\def\PVOUAbsMedianMedianFloat{0.000590581595897674590904535829594124152208678424358367919921875}
\def\PVOUAbsMedianMedianKey{23367}
\def\PVOUAbsMedianMinFloat{0.0004861703515052795431840293449710088680149056017398834228515625}
\def\PVOUAbsMedianMinKey{15622}
\def\PVOUAbsMedianStdDevFloat{0.0020552122975375833845157469426112584187649190425872802734375}
\def\PVOUAbsMinLen{151}
\def\PVOUAbsMinMaxFloat{0.00531101226806640625}
\def\PVOUAbsMinMaxKey{18668}
\def\PVOUAbsMinMeanFloat{0.001049318700097501277923583984375}
\def\PVOUAbsMinMeanKey{26374}
\def\PVOUAbsMinMedianFloat{0.000010669231414794921875}
\def\PVOUAbsMinMedianKey{11498}
\def\PVOUAbsMinMinFloat{0.00000083446502685546875}
\def\PVOUAbsMinMinKey{19538}
\def\PVOUAbsMinStdDevFloat{0.001141055370680987834930419921875}
\def\PVOUAbsStdDevLen{151}
\def\PVOUAbsStdDevMaxFloat{0.3321933746337890625}
\def\PVOUAbsStdDevMaxKey{8299}
\def\PVOUAbsStdDevMeanFloat{0.18971176445484161376953125}
\def\PVOUAbsStdDevMeanKey{12141}
\def\PVOUAbsStdDevMedianFloat{0.124717928469181060791015625}
\def\PVOUAbsStdDevMedianKey{18289}
\def\PVOUAbsStdDevMinFloat{0.12452344596385955810546875}
\def\PVOUAbsStdDevMinKey{6910}
\def\PVOUAbsStdDevStdDevFloat{0.0343817658722400665283203125}
\def\PVOULenLen{151}
\def\PVOULenMaxFloat{320}
\def\PVOULenMaxKey{50}
\def\PVOULenMeanFloat{320}
\def\PVOULenMeanKey{50}
\def\PVOULenMedianFloat{320}
\def\PVOULenMedianKey{50}
\def\PVOULenMinFloat{320}
\def\PVOULenMinKey{50}
\def\PVOULenStdDevFloat{0}
\def\PVOUMaxLen{151}
\def\PVOUMaxMaxFloat{2.042043209075927734375}
\def\PVOUMaxMaxKey{4800}
\def\PVOUMaxMeanFloat{0.9963881969451904296875}
\def\PVOUMaxMeanKey{16069}
\def\PVOUMaxMedianFloat{0.58128784596920013427734375}
\def\PVOUMaxMedianKey{2306}
\def\PVOUMaxMinFloat{0.5455062389373779296875}
\def\PVOUMaxMinKey{6910}
\def\PVOUMaxRowDiffLenLen{151}
\def\PVOUMaxRowDiffLenMaxFloat{5}
\def\PVOUMaxRowDiffLenMaxKey{50}
\def\PVOUMaxRowDiffLenMeanFloat{5}
\def\PVOUMaxRowDiffLenMeanKey{50}
\def\PVOUMaxRowDiffLenMedianFloat{5}
\def\PVOUMaxRowDiffLenMedianKey{50}
\def\PVOUMaxRowDiffLenMinFloat{5}
\def\PVOUMaxRowDiffLenMinKey{50}
\def\PVOUMaxRowDiffLenStdDevFloat{0}
\def\PVOUMaxRowDiffMaxLen{151}
\def\PVOUMaxRowDiffMaxMaxFloat{3.529872417449951171875}
\def\PVOUMaxRowDiffMaxMaxKey{8299}
\def\PVOUMaxRowDiffMaxMeanFloat{1.90646588802337646484375}
\def\PVOUMaxRowDiffMaxMeanKey{1490}
\def\PVOUMaxRowDiffMaxMedianFloat{1.13017880916595458984375}
\def\PVOUMaxRowDiffMaxMedianKey{20976}
\def\PVOUMaxRowDiffMaxMinFloat{1.0260450839996337890625}
\def\PVOUMaxRowDiffMaxMinKey{18289}
\def\PVOUMaxRowDiffMaxStdDevFloat{0.4477876126766204833984375}
\def\PVOUMaxRowDiffMeanLen{151}
\def\PVOUMaxRowDiffMeanMaxFloat{2.048081874847412109375}
\def\PVOUMaxRowDiffMeanMaxKey{5615}
\def\PVOUMaxRowDiffMeanMeanFloat{1.362319469451904296875}
\def\PVOUMaxRowDiffMeanMeanKey{519}
\def\PVOUMaxRowDiffMeanMedianFloat{0.86682318150997161865234375}
\def\PVOUMaxRowDiffMeanMedianKey{18289}
\def\PVOUMaxRowDiffMeanMinFloat{0.849766254425048828125}
\def\PVOUMaxRowDiffMeanMinKey{6910}
\def\PVOUMaxRowDiffMeanStdDevFloat{0.21147523820400238037109375}
\def\PVOUMaxRowDiffMedianLen{151}
\def\PVOUMaxRowDiffMedianMaxFloat{1.53804635524749766517516036401502788066864013671875}
\def\PVOUMaxRowDiffMedianMaxKey{4430}
\def\PVOUMaxRowDiffMedianMeanFloat{0.9380224132616790111427462761639617383480072021484375}
\def\PVOUMaxRowDiffMedianMeanKey{19451}
\def\PVOUMaxRowDiffMedianMedianFloat{0.477318819165229779599712855997495353221893310546875}
\def\PVOUMaxRowDiffMedianMedianKey{3254}
\def\PVOUMaxRowDiffMedianMinFloat{0.45838171720504761186276709850062616169452667236328125}
\def\PVOUMaxRowDiffMedianMinKey{6910}
\def\PVOUMaxRowDiffMedianStdDevFloat{0.180276191464315671542095742552191950380802154541015625}
\def\PVOUMaxRowDiffMinLen{151}
\def\PVOUMaxRowDiffMinMaxFloat{1.53597009181976318359375}
\def\PVOUMaxRowDiffMinMaxKey{4430}
\def\PVOUMaxRowDiffMinMeanFloat{0.933926641941070556640625}
\def\PVOUMaxRowDiffMinMeanKey{19451}
\def\PVOUMaxRowDiffMinMedianFloat{0.46443881094455718994140625}
\def\PVOUMaxRowDiffMinMedianKey{3254}
\def\PVOUMaxRowDiffMinMinFloat{0.452294886112213134765625}
\def\PVOUMaxRowDiffMinMinKey{6910}
\def\PVOUMaxRowDiffMinStdDevFloat{0.181826174259185791015625}
\def\PVOUMaxRowDiffStdDevLen{151}
\def\PVOUMaxRowDiffStdDevMaxFloat{0.884956538677215576171875}
\def\PVOUMaxRowDiffStdDevMaxKey{8299}
\def\PVOUMaxRowDiffStdDevMeanFloat{0.3505952060222625732421875}
\def\PVOUMaxRowDiffStdDevMeanKey{30684}
\def\PVOUMaxRowDiffStdDevMedianFloat{0.08599046058952808380126953125}
\def\PVOUMaxRowDiffStdDevMedianKey{6589}
\def\PVOUMaxRowDiffStdDevMinFloat{0.070503480732440948486328125}
\def\PVOUMaxRowDiffStdDevMinKey{20976}
\def\PVOUMaxRowDiffStdDevStdDevFloat{0.146778404712677001953125}
\def\PVOUMaxStdDevFloat{0.25205194950103759765625}
\def\PVOUMeanLen{151}
\def\PVOUMeanMaxFloat{0.00000003902241729747402132488787174224853515625}
\def\PVOUMeanMaxKey{16284}
\def\PVOUMeanMeanFloat{0.000000000346007833496031480535748414695262908935546875}
\def\PVOUMeanMeanKey{519}
\def\PVOUMeanMedianFloat{-0.00000002942979282494206927367486059665679931640625}
\def\PVOUMeanMedianKey{9504}
\def\PVOUMeanMinFloat{-0.000000037252902984619140625}
\def\PVOUMeanMinKey{29022}
\def\PVOUMeanStdDevFloat{0.00000001250169656685784502769820392131805419921875}
\def\PVOUMedianLen{151}
\def\PVOUMedianMaxFloat{-0.44212230771780014482175147350062616169452667236328125}
\def\PVOUMedianMaxKey{18289}
\def\PVOUMedianMeanFloat{-0.804219153386275475980937699205242097377777099609375}
\def\PVOUMedianMeanKey{1490}
\def\PVOUMedianMedianFloat{-1.329309803098440045943107179482467472553253173828125}
\def\PVOUMedianMedianKey{21317}
\def\PVOUMedianMinFloat{-1.604597377181053108330388567992486059665679931640625}
\def\PVOUMedianMinKey{8299}
\def\PVOUMedianStdDevFloat{0.16929203794091296497725807057577185332775115966796875}
\def\PVOUMinLen{151}
\def\PVOUMinMaxFloat{-0.4832403659820556640625}
\def\PVOUMinMaxKey{18289}
\def\PVOUMinMeanFloat{-0.961053073406219482421875}
\def\PVOUMinMeanKey{7467}
\def\PVOUMinMedianFloat{-1.723498821258544921875}
\def\PVOUMinMedianKey{5615}
\def\PVOUMinMinFloat{-1.7497437000274658203125}
\def\PVOUMinMinKey{8299}
\def\PVOUMinStdDevFloat{0.23411266505718231201171875}
\def\PVOUStdDevLen{151}
\def\PVOUStdDevMaxFloat{0.52219092845916748046875}
\def\PVOUStdDevMaxKey{4430}
\def\PVOUStdDevMeanFloat{0.3060683310031890869140625}
\def\PVOUStdDevMeanKey{6082}
\def\PVOUStdDevMedianFloat{0.2012758441269397735595703125}
\def\PVOUStdDevMedianKey{27300}
\def\PVOUStdDevMinFloat{0.19689710438251495361328125}
\def\PVOUStdDevMinKey{6910}
\def\PVOUStdDevStdDevFloat{0.052877731621265411376953125}
\def\ProofFlopEstimateAllSubcubicMean{3270441.799999999813735485076904296875}
\def\ProofFlopEstimateAllSubcubicStdDev{794436.55583180324174463748931884765625}
\def\ProofFlopEstimateAlmostQuadraticMean{2372971.6666666665114462375640869140625}
\def\ProofFlopEstimateAlmostQuadraticStdDev{26564.375443911048932932317256927490234375}
\def\ProofFlopEstimateMainlySubcubicMean{3394938.65384615398943424224853515625}
\def\ProofFlopEstimateMainlySubcubicStdDev{751134.779896578751504421234130859375}
\def\QuartileOnePercentileFloat{0.25}
\def\QuartileThreePercentileFloat{0.75}
\def\RealSubcubicAccuracyLen{15100}
\def\RealSubcubicAccuracyMaxFloat{0.780931304208934307098388671875}
\def\RealSubcubicAccuracyMeanFloat{0.2375207564113230029878565119361155666410923004150390625}
\def\RealSubcubicAccuracyMedianFloat{0.00000004563480615615845388306990042422139897126953655970282852649688720703125}
\def\RealSubcubicAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\RealSubcubicAccuracyStdDevFloat{0.2471000274570998855860892717828392051160335540771484375}
\def\RealSubcubicDroppedSequencesFracLen{15100}
\def\RealSubcubicDroppedSequencesFracMaxFloat{0.402560516260564327239990234375}
\def\RealSubcubicDroppedSequencesFracMeanFloat{0.1339002859487586627462718524839146994054317474365234375}
\def\RealSubcubicDroppedSequencesFracMedianFloat{0}
\def\RealSubcubicDroppedSequencesFracMinFloat{0}
\def\RealSubcubicDroppedSequencesFracStdDevFloat{0.11165436334591223588308395164858666248619556427001953125}
\def\RealSubcubicDroppedSequencesLen{15100}
\def\RealSubcubicDroppedSequencesMaxFloat{432246063}
\def\RealSubcubicDroppedSequencesMeanFloat{143774337.26874172687530517578125}
\def\RealSubcubicDroppedSequencesMedianFloat{0}
\def\RealSubcubicDroppedSequencesMinFloat{0}
\def\RealSubcubicDroppedSequencesStdDevFloat{119887959.75659854710102081298828125}
\def\RealSubcubicEffectiveDimensionalityEstimateLen{15100}
\def\RealSubcubicEffectiveDimensionalityEstimateMaxFloat{10370}
\def\RealSubcubicEffectiveDimensionalityEstimateMeanFloat{6049.600000000000363797880709171295166015625}
\def\RealSubcubicEffectiveDimensionalityEstimateMedianFloat{4290}
\def\RealSubcubicEffectiveDimensionalityEstimateMinFloat{4290}
\def\RealSubcubicEffectiveDimensionalityEstimateStdDevFloat{1530.49032666005450664670206606388092041015625}
\def\RealSubcubicErrUpperBoundLen{15100}
\def\RealSubcubicErrUpperBoundMaxFloat{144.185821533203125}
\def\RealSubcubicErrUpperBoundMeanFloat{33.28911486240411932158167473971843719482421875}
\def\RealSubcubicErrUpperBoundMedianFloat{0}
\def\RealSubcubicErrUpperBoundMinFloat{0}
\def\RealSubcubicErrUpperBoundStdDevFloat{40.9492951108743596932981745339930057525634765625}
\def\RealSubcubicGapMostBelowValueLen{15100}
\def\RealSubcubicGapMostBelowValueMaxFloat{73}
\def\RealSubcubicGapMostBelowValueMeanFloat{12.705761589403973488288102089427411556243896484375}
\def\RealSubcubicGapMostBelowValueMedianFloat{1}
\def\RealSubcubicGapMostBelowValueMinFloat{1}
\def\RealSubcubicGapMostBelowValueNumStdLen{15100}
\def\RealSubcubicGapMostBelowValueNumStdMaxFloat{1.5}
\def\RealSubcubicGapMostBelowValueNumStdMeanFloat{1.5}
\def\RealSubcubicGapMostBelowValueNumStdMedianFloat{1.5}
\def\RealSubcubicGapMostBelowValueNumStdMinFloat{1.5}
\def\RealSubcubicGapMostBelowValueNumStdStdDevFloat{0}
\def\RealSubcubicGapMostBelowValueSequenceFracLen{15100}
\def\RealSubcubicGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\RealSubcubicGapMostBelowValueSequenceFracMeanFloat{0.99453861186835934571348616373143158853054046630859375}
\def\RealSubcubicGapMostBelowValueSequenceFracMedianFloat{0.96024964660406109118184758699499070644378662109375}
\def\RealSubcubicGapMostBelowValueSequenceFracMinFloat{0.9398634433746337890625}
\def\RealSubcubicGapMostBelowValueSequenceFracStdDevFloat{0.00810430416835831134159118249726816429756581783294677734375}
\def\RealSubcubicGapMostBelowValueStdDevFloat{14.769136645981159716711772489361464977264404296875}
\def\RealSubcubicInstructionCountBranchLen{15100}
\def\RealSubcubicInstructionCountBranchMaxFloat{0}
\def\RealSubcubicInstructionCountBranchMeanFloat{0}
\def\RealSubcubicInstructionCountBranchMedianFloat{0}
\def\RealSubcubicInstructionCountBranchMinFloat{0}
\def\RealSubcubicInstructionCountBranchStdDevFloat{0}
\def\RealSubcubicInstructionCountIntLen{15100}
\def\RealSubcubicInstructionCountIntMaxFloat{0}
\def\RealSubcubicInstructionCountIntMeanFloat{0}
\def\RealSubcubicInstructionCountIntMedianFloat{0}
\def\RealSubcubicInstructionCountIntMinFloat{0}
\def\RealSubcubicInstructionCountIntStdDevFloat{0}
\def\RealSubcubicInstructionCountLen{15100}
\def\RealSubcubicInstructionCountMaxFloat{5144079}
\def\RealSubcubicInstructionCountMeanFloat{3270441.799999999813735485076904296875}
\def\RealSubcubicInstructionCountMedianFloat{2334413}
\def\RealSubcubicInstructionCountMinFloat{2334413}
\def\RealSubcubicInstructionCountStdDevFloat{794410.24955004197545349597930908203125}
\def\RealSubcubicMaxGapLen{15100}
\def\RealSubcubicMaxGapMaxFloat{34}
\def\RealSubcubicMaxGapMeanFloat{13.491324503311258098392499960027635097503662109375}
\def\RealSubcubicMaxGapMedianFloat{1}
\def\RealSubcubicMaxGapMinFloat{1}
\def\RealSubcubicMaxGapStdDevFloat{7.92110042989769258525711848051287233829498291015625}
\def\RealSubcubicNormalizedAccuracyLen{15100}
\def\RealSubcubicNormalizedAccuracyMaxFloat{0.7812433963450775564751893398351967334747314453125}
\def\RealSubcubicNormalizedAccuracyMeanFloat{0.2377466150843743075693481614507618360221385955810546875}
\def\RealSubcubicNormalizedAccuracyMedianFloat{0.000000045658116086492779083511463038280719928252437966875731945037841796875}
\def\RealSubcubicNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\RealSubcubicNormalizedAccuracyStdDevFloat{0.2473261298693043286345272235848824493587017059326171875}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.780931304208934307098388671875}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMaxKey{29110}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.70537861965794046437139286354067735373973846435546875}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMeanKey{10248}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.6119701839052140712738037109375}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMinFloat{0.59265005774796009063720703125}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyMinKey{1951}
\def\RealSubcubicOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0310671816446796665578400364893241203390061855316162109375}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.12679875083267688751220703125}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.08391068376206005374751129011201555840671062469482421875}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{5781}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.06227796920575197348046714296287973411381244659423828125}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{2345}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.058046793565153999294725650770487845875322818756103515625}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01268794889335365938531907659125863574445247650146484375}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{136149122}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{90098410.6357615888118743896484375}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{5781}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{66870460.25}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{2345}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{62327270}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\RealSubcubicOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{13623581.38756833784282207489013671875}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{2236}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{7080.6490066225169357494451105594635009765625}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{1185}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4402}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{104}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{24144}
\def\RealSubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{2075.01463873772081569768488407135009765625}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{9.37257671356201171875}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{17194}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{1.492547126795282341760184863233007490634918212890625}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{27714}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{123}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinKey{123}
\def\RealSubcubicOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.267698926495981925910427889903075993061065673828125}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2236}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.16556291390728450352298750658519566059112548828125}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999912261962890625}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2773}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9853469997841790561921015978441573679447174072265625}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6910}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95145584642887115478515625}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{913}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.943215072154998779296875}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2345}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01196093248701758648966375631061964668333530426025390625}
\def\RealSubcubicOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.87972349340561961650308830940048210322856903076171875}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMaxFloat{4193742}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMaxKey{104}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3312777.3642384107224643230438232421875}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMeanKey{5928}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2696590}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMedianKey{2236}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMinFloat{2696590}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountMinKey{2236}
\def\RealSubcubicOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{556895.864682440995238721370697021484375}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMaxFloat{19}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.132450331125827602818390005268156528472900390625}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMeanKey{1951}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMedianKey{6159}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapMinKey{27300}
\def\RealSubcubicOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.720234448136964022779693550546653568744659423828125}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7812433963450775564751893398351967334747314453125}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29110}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.70604884924443778171365693197003565728664398193359375}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{3284}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.612295080253672185932600768865086138248443603515625}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.59298062177469235134452674174099229276180267333984375}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1951}
\def\RealSubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0309600961157661565270604597799319890327751636505126953125}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7359836101531982421875}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.65898868737631488556871772743761539459228515625}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{12141}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.74832755327224020902576739899814128875732421875}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.6372649669647216796875}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7004619892651062773580861176014877855777740478515625}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2972538471221923828125}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMaxKey{5358}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.2151392137767462742203861125744879245758056640625}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMeanKey{13293}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.1408836841583251953125}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1362316608428955078125}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\RealSubcubicOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.031038837999946923551508604077753261663019657135009765625}
\def\RealSubcubicProofSearchTimeLen{15100}
\def\RealSubcubicProofSearchTimeMaxFloat{52.45428371429443359375}
\def\RealSubcubicProofSearchTimeMeanFloat{44.55526558441831497248131199739873409271240234375}
\def\RealSubcubicProofSearchTimeMedianFloat{42.36292500376701042341665015555918216705322265625}
\def\RealSubcubicProofSearchTimeMinFloat{41.9884622097015380859375}
\def\RealSubcubicProofSearchTimeStdDevFloat{0.74150046099404942623323222505860030651092529296875}
\def\RealSubcubicProofTimeLen{15100}
\def\RealSubcubicProofTimeMaxFloat{2.6413619518280029296875}
\def\RealSubcubicProofTimeMeanFloat{2.208900451928574426574414246715605258941650390625}
\def\RealSubcubicProofTimeMedianFloat{2.131400314569473319892267682007513940334320068359375}
\def\RealSubcubicProofTimeMinFloat{2.1170752048492431640625}
\def\RealSubcubicProofTimeStdDevFloat{0.031684576742139265725928254369136993773281574249267578125}
\def\ResampleEQKEErrLen{100}
\def\ResampleEQKEErrMaxLen{151}
\def\ResampleEQKEErrMaxMaxFloat{2.463964939117431640625}
\def\ResampleEQKEErrMaxMaxKey{12493}
\def\ResampleEQKEErrMaxMeanFloat{1.7132360548373088970919297935324721038341522216796875}
\def\ResampleEQKEErrMaxMeanKey{19093}
\def\ResampleEQKEErrMaxMedianFloat{1.3878984749317169189453125}
\def\ResampleEQKEErrMaxMedianKey{1412}
\def\ResampleEQKEErrMaxMinFloat{1.3223206996917724609375}
\def\ResampleEQKEErrMaxMinKey{28090}
\def\ResampleEQKEErrMaxStdDevFloat{0.1774159992194802859533098171596066094934940338134765625}
\def\ResampleEQKEErrMeanLen{151}
\def\ResampleEQKEErrMeanMaxFloat{1.362024331092834383838408029987476766109466552734375}
\def\ResampleEQKEErrMeanMaxKey{25516}
\def\ResampleEQKEErrMeanMeanFloat{1.20099239805676294423619765439070761203765869140625}
\def\ResampleEQKEErrMeanMeanKey{9816}
\def\ResampleEQKEErrMeanMedianFloat{1.0455022248625756020601329510100185871124267578125}
\def\ResampleEQKEErrMeanMedianKey{6532}
\def\ResampleEQKEErrMeanMinFloat{1.0180645579099654174370925829862244427204132080078125}
\def\ResampleEQKEErrMeanMinKey{28090}
\def\ResampleEQKEErrMeanStdDevFloat{0.06425764060506476693657162968520424328744411468505859375}
\def\ResampleEQKEErrMedianLen{151}
\def\ResampleEQKEErrMedianMaxFloat{1.07929682075977328992166803800500929355621337890625}
\def\ResampleEQKEErrMedianMaxKey{19004}
\def\ResampleEQKEErrMedianMeanFloat{0.9499644003028901995122623702627606689929962158203125}
\def\ResampleEQKEErrMedianMeanKey{23633}
\def\ResampleEQKEErrMedianMedianFloat{0.82419502831995483660421086824499070644378662109375}
\def\ResampleEQKEErrMedianMedianKey{6155}
\def\ResampleEQKEErrMedianMinFloat{0.8131556722521782187840244660037569701671600341796875}
\def\ResampleEQKEErrMedianMinKey{11611}
\def\ResampleEQKEErrMedianStdDevFloat{0.054479643562412645441117575728640076704323291778564453125}
\def\ResampleEQKEErrMinLen{151}
\def\ResampleEQKEErrMinMaxFloat{1.0703563690185546875}
\def\ResampleEQKEErrMinMaxKey{19004}
\def\ResampleEQKEErrMinMeanFloat{0.93773824331776201024268857509014196693897247314453125}
\def\ResampleEQKEErrMinMeanKey{19451}
\def\ResampleEQKEErrMinMedianFloat{0.806213796138763427734375}
\def\ResampleEQKEErrMinMedianKey{28090}
\def\ResampleEQKEErrMinMinFloat{0.78386294841766357421875}
\def\ResampleEQKEErrMinMinKey{11611}
\def\ResampleEQKEErrMinStdDevFloat{0.05692428877047743529526968586651491932570934295654296875}
\def\ResampleEQKEErrNumSamples{100}
\def\ResampleEQKEErrSeed{1234}
\def\ResampleEQKEErrStdDevLen{151}
\def\ResampleEQKEErrStdDevMaxFloat{0.1862994165602061269471079185677808709442615509033203125}
\def\ResampleEQKEErrStdDevMaxKey{26278}
\def\ResampleEQKEErrStdDevMeanFloat{0.1427413590680366717311500224241171963512897491455078125}
\def\ResampleEQKEErrStdDevMeanKey{30371}
\def\ResampleEQKEErrStdDevMedianFloat{0.1104092987022266825203331563898245804011821746826171875}
\def\ResampleEQKEErrStdDevMedianKey{28090}
\def\ResampleEQKEErrStdDevMinFloat{0.10320156368500572885427146729853120632469654083251953125}
\def\ResampleEQKEErrStdDevMinKey{20294}
\def\ResampleEQKEErrStdDevStdDevFloat{0.0156603713199571954739486301377837662585079669952392578125}
\def\ResampleNormalEQKEErrLen{100}
\def\ResampleNormalEQKEErrMaxLen{151}
\def\ResampleNormalEQKEErrMaxMaxFloat{1.956125736236572265625}
\def\ResampleNormalEQKEErrMaxMaxKey{25516}
\def\ResampleNormalEQKEErrMaxMeanFloat{1.7015470874230593789633303458685986697673797607421875}
\def\ResampleNormalEQKEErrMaxMeanKey{4800}
\def\ResampleNormalEQKEErrMaxMedianFloat{1.4930861294269561767578125}
\def\ResampleNormalEQKEErrMaxMedianKey{6532}
\def\ResampleNormalEQKEErrMaxMinFloat{1.47706019878387451171875}
\def\ResampleNormalEQKEErrMaxMinKey{28090}
\def\ResampleNormalEQKEErrMaxStdDevFloat{0.090418091216424356648673210656852461397647857666015625}
\def\ResampleNormalEQKEErrMeanLen{151}
\def\ResampleNormalEQKEErrMeanMaxFloat{1.341671485900878924013568394002504646778106689453125}
\def\ResampleNormalEQKEErrMeanMaxKey{25516}
\def\ResampleNormalEQKEErrMeanMeanFloat{1.177917725037265217480353385326452553272247314453125}
\def\ResampleNormalEQKEErrMeanMeanKey{4810}
\def\ResampleNormalEQKEErrMeanMedianFloat{1.033574126064777498612556883017532527446746826171875}
\def\ResampleNormalEQKEErrMeanMedianKey{6532}
\def\ResampleNormalEQKEErrMeanMinFloat{1.0240682923793793523969952730112709105014801025390625}
\def\ResampleNormalEQKEErrMeanMinKey{28090}
\def\ResampleNormalEQKEErrMeanStdDevFloat{0.060709356498451459704934762839911854825913906097412109375}
\def\ResampleNormalEQKEErrMedianLen{151}
\def\ResampleNormalEQKEErrMedianMaxFloat{1.07425881445407878089781661401502788066864013671875}
\def\ResampleNormalEQKEErrMedianMaxKey{25516}
\def\ResampleNormalEQKEErrMedianMeanFloat{0.95284078530325799771816264183144085109233856201171875}
\def\ResampleNormalEQKEErrMedianMeanKey{11498}
\def\ResampleNormalEQKEErrMedianMedianFloat{0.841983537673950177548931605997495353221893310546875}
\def\ResampleNormalEQKEErrMedianMedianKey{6532}
\def\ResampleNormalEQKEErrMedianMinFloat{0.8343002498149871826171875}
\def\ResampleNormalEQKEErrMedianMinKey{28090}
\def\ResampleNormalEQKEErrMedianStdDevFloat{0.050517496340908039920147842849473818205296993255615234375}
\def\ResampleNormalEQKEErrMinLen{151}
\def\ResampleNormalEQKEErrMinMaxFloat{1.05659854412078857421875}
\def\ResampleNormalEQKEErrMinMaxKey{25516}
\def\ResampleNormalEQKEErrMinMeanFloat{0.94411722240069051448330128550878725945949554443359375}
\def\ResampleNormalEQKEErrMinMeanKey{13293}
\def\ResampleNormalEQKEErrMinMedianFloat{0.835397541522979736328125}
\def\ResampleNormalEQKEErrMinMedianKey{26374}
\def\ResampleNormalEQKEErrMinMinFloat{0.831577003002166748046875}
\def\ResampleNormalEQKEErrMinMinKey{28090}
\def\ResampleNormalEQKEErrMinStdDevFloat{0.052108918485231296713333648540356080047786235809326171875}
\def\ResampleNormalEQKEErrStdDevLen{151}
\def\ResampleNormalEQKEErrStdDevMaxFloat{0.1484659907914729071176651586938533000648021697998046875}
\def\ResampleNormalEQKEErrStdDevMaxKey{25516}
\def\ResampleNormalEQKEErrStdDevMeanFloat{0.1292050273493437206884237866688636131584644317626953125}
\def\ResampleNormalEQKEErrStdDevMeanKey{4810}
\def\ResampleNormalEQKEErrStdDevMedianFloat{0.11324163301427984940072946073996718041598796844482421875}
\def\ResampleNormalEQKEErrStdDevMedianKey{6532}
\def\ResampleNormalEQKEErrStdDevMinFloat{0.112159042703930122986122341899317689239978790283203125}
\def\ResampleNormalEQKEErrStdDevMinKey{28090}
\def\ResampleNormalEQKEErrStdDevStdDevFloat{0.00688510243559518897438209705796907655894756317138671875}
\def\SubcubicAccuracyLen{7852}
\def\SubcubicAccuracyMaxFloat{0.780931304208934307098388671875}
\def\SubcubicAccuracyMeanFloat{0.355811565381892791481988069790531881153583526611328125}
\def\SubcubicAccuracyMedianFloat{0.00000004563480615615845388306990042422139897126953655970282852649688720703125}
\def\SubcubicAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicAccuracyStdDevFloat{0.231914882630729068946351389968185685575008392333984375}
\def\SubcubicAttentionQuadraticAccuracyLen{1812}
\def\SubcubicAttentionQuadraticAccuracyMaxFloat{0.42662229202687740325927734375}
\def\SubcubicAttentionQuadraticAccuracyMeanFloat{0.25160978846025816579867750988341867923736572265625}
\def\SubcubicAttentionQuadraticAccuracyMedianFloat{0.060504367826506470773306745059016975574195384979248046875}
\def\SubcubicAttentionQuadraticAccuracyMinFloat{0.032699271105229799072589003117172978818416595458984375}
\def\SubcubicAttentionQuadraticAccuracyStdDevFloat{0.09406967088664010268050930108074680902063846588134765625}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyMaxFloat{0.4154766835272312164306640625}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyMeanFloat{0.0724836553318797260914152502664364874362945556640625}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyMedianFloat{0.00000004470348358154297536744490042422139897126953655970282852649688720703125}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicAttentionQuadraticDirectQuadraticAccuracyStdDevFloat{0.122397661740817620401600152035825885832309722900390625}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracMaxFloat{0.378214078024029676239337049992172978818416595458984375}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracMeanFloat{0.1811024858246230440084190149718779139220714569091796875}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesFracStdDevFloat{0.13462124881513926055731644737534224987030029296875}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesMaxFloat{406104274}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesMeanFloat{194457313.4602648913860321044921875}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticDroppedSequencesStdDevFloat{144548465.25192546844482421875}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateMeanFloat{6487.3333333333330301684327423572540283203125}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicAttentionQuadraticDirectQuadraticEffectiveDimensionalityEstimateStdDevFloat{42.66666666666666429819088079966604709625244140625}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundMaxFloat{144.185821533203125}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundMeanFloat{95.1135054497792538086287095211446285247802734375}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundMedianFloat{78.46202850341796875}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundMinFloat{77.82788848876953125}
\def\SubcubicAttentionQuadraticDirectQuadraticErrUpperBoundStdDevFloat{7.5268897599165089928874294855631887912750244140625}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueMaxFloat{73}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueMeanFloat{28.147167034584253286766397650353610515594482421875}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueMedianFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueMinFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticGapMostBelowValueStdDevFloat{20.017442110895405704695804161019623279571533203125}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountMaxFloat{2411562}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountMeanFloat{2372971.6666666665114462375640869140625}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountMedianFloat{2334413}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountMinFloat{2334413}
\def\SubcubicAttentionQuadraticDirectQuadraticInstructionCountStdDevFloat{26559.48824389840956428088247776031494140625}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapMaxFloat{34}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapMeanFloat{15.9131714495952909516063300543464720249176025390625}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapMedianFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapMinFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticMaxGapStdDevFloat{10.9080292652295991473465619492344558238983154296875}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyMaxFloat{0.4157097376548632983173092725337482988834381103515625}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyMeanFloat{0.0725533972296098228493832493768422864377498626708984375}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyMedianFloat{0.00000004477619510034710918767376810860347813303405928309075534343719482421875}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicAttentionQuadraticDirectQuadraticNormalizedAccuracyStdDevFloat{0.1225085209325896540288880487423739396035671234130859375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.4154766835272312164306640625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{27300}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.335266042513069739694486770531511865556240081787109375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{20415}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.248908461770042721550311171085922978818416595458984375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2342543266713618954621978218710864894092082977294921875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.033004201385701419091400765637445147149264812469482421875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.375500188209116403381671034367172978818416595458984375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.312504638960918068590899565606378018856048583984375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{2549}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2444566735066472651372038171757594682276248931884765625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{28090}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.2349676061421631934056364343632594682276248931884765625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.028315214295907935315721459801352466456592082977294921875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{403190257}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{335549301.046357631683349609375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{2549}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{262483354.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{28090}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{252294546}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{30403229.8450390510261058807373046875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6502.0264900662250511231832206249237060546875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{519}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{519}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{31.745667070430105383138652541674673557281494140625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.185821533203125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.69683074951171875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11130}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.7692584991455078125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.29946136474609375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.42973356827689013215376689913682639598846435546875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{69}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{41.27814569536423761064725113101303577423095703125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{29.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{28}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{6.44709384747194480524967730161733925342559814453125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2411562}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{913}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2393577.218543046154081821441650390625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2384845}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{519}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{2384845}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{519}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{8919.140182845294475555419921875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{34}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{24.23841059602649039561583776958286762237548828125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{1283}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{17.75}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{6155}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{20338}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.98718811560862729237442181329242885112762451171875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.4157097376548632983173092725337482988834381103515625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27300}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.33558050608889333776829744238057173788547515869140625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6082}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.2490520827774077294858301456770277582108974456787109375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.23443112806623200849998056582990102469921112060546875}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.032957431535899091301633490047606755979359149932861328125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6513054370880126953125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.74660976675172463501439779065549373626708984375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{8840}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.4892952442169189453125}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4421784877777099609375}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.73073050769386471703370489194639958441257476806640625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.32684421539306640625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{50}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.21747174326157736601317083113826811313629150390625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{2549}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.141332685947418212890625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{21317}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{2.132311344146728515625}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicAttentionQuadraticDirectQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0303655272331933255569591523226335993967950344085693359375}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeMaxFloat{52.45428371429443359375}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeMeanFloat{44.57724635288766279472838505171239376068115234375}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeMedianFloat{42.4414603543281572228806908242404460906982421875}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeMinFloat{42.08597469329833984375}
\def\SubcubicAttentionQuadraticDirectQuadraticProofSearchTimeStdDevFloat{0.742895826725537222756656774436123669147491455078125}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeLen{2718}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeMaxFloat{2.594494342803955078125}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeMeanFloat{2.209200717755500864569739860598929226398468017578125}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeMedianFloat{2.131579179763793963076068394002504646778106689453125}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeMinFloat{2.1170752048492431640625}
\def\SubcubicAttentionQuadraticDirectQuadraticProofTimeStdDevFloat{0.03222898597147559607289935001972480677068233489990234375}
\def\SubcubicAttentionQuadraticDroppedSequencesFracLen{1812}
\def\SubcubicAttentionQuadraticDroppedSequencesFracMaxFloat{0.402560516260564327239990234375}
\def\SubcubicAttentionQuadraticDroppedSequencesFracMeanFloat{0.34512680840100806722858806097065098583698272705078125}
\def\SubcubicAttentionQuadraticDroppedSequencesFracMedianFloat{0.30423308528959747132347501974436454474925994873046875}
\def\SubcubicAttentionQuadraticDroppedSequencesFracMinFloat{0.302029694430530015747393690617172978818416595458984375}
\def\SubcubicAttentionQuadraticDroppedSequencesFracStdDevFloat{0.0168734054230428413834186329722797381691634654998779296875}
\def\SubcubicAttentionQuadraticDroppedSequencesLen{1812}
\def\SubcubicAttentionQuadraticDroppedSequencesMaxFloat{432246063}
\def\SubcubicAttentionQuadraticDroppedSequencesMeanFloat{370577088.76379692554473876953125}
\def\SubcubicAttentionQuadraticDroppedSequencesMedianFloat{326667787.920000016689300537109375}
\def\SubcubicAttentionQuadraticDroppedSequencesMinFloat{324301915}
\def\SubcubicAttentionQuadraticDroppedSequencesStdDevFloat{18117681.1160295121371746063232421875}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateLen{1812}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateMeanFloat{4459.6666666666669698315672576427459716796875}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicAttentionQuadraticEffectiveDimensionalityEstimateStdDevFloat{69.8514296362087492298087454400956630706787109375}
\def\SubcubicAttentionQuadraticErrUpperBoundLen{1812}
\def\SubcubicAttentionQuadraticErrUpperBoundMaxFloat{144.185821533203125}
\def\SubcubicAttentionQuadraticErrUpperBoundMeanFloat{95.1135054497792538086287095211446285247802734375}
\def\SubcubicAttentionQuadraticErrUpperBoundMedianFloat{78.46202850341796875}
\def\SubcubicAttentionQuadraticErrUpperBoundMinFloat{77.82788848876953125}
\def\SubcubicAttentionQuadraticErrUpperBoundStdDevFloat{7.5268897599165089928874294855631887912750244140625}
\def\SubcubicAttentionQuadraticGapMostBelowValueLen{1812}
\def\SubcubicAttentionQuadraticGapMostBelowValueMaxFloat{61}
\def\SubcubicAttentionQuadraticGapMostBelowValueMeanFloat{33.729580573951437827417976222932338714599609375}
\def\SubcubicAttentionQuadraticGapMostBelowValueMedianFloat{23}
\def\SubcubicAttentionQuadraticGapMostBelowValueMinFloat{23}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdLen{1812}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracLen{1812}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracMeanFloat{0.99999927356016815593875435297377407550811767578125}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracMinFloat{0.99967092275619517938167746251565404236316680908203125}
\def\SubcubicAttentionQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.00001544432267239767832766282606993257786598405800759792327880859375}
\def\SubcubicAttentionQuadraticGapMostBelowValueStdDevFloat{5.8692286236305211133412740309722721576690673828125}
\def\SubcubicAttentionQuadraticInstructionCountBranchLen{1812}
\def\SubcubicAttentionQuadraticInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntLen{1812}
\def\SubcubicAttentionQuadraticInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntMinFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionQuadraticInstructionCountLen{1812}
\def\SubcubicAttentionQuadraticInstructionCountMaxFloat{2675913}
\def\SubcubicAttentionQuadraticInstructionCountMeanFloat{2633877.8333333334885537624359130859375}
\def\SubcubicAttentionQuadraticInstructionCountMedianFloat{2592557}
\def\SubcubicAttentionQuadraticInstructionCountMinFloat{2592557}
\def\SubcubicAttentionQuadraticInstructionCountStdDevFloat{26860.949433559158933348953723907470703125}
\def\SubcubicAttentionQuadraticMaxGapLen{1812}
\def\SubcubicAttentionQuadraticMaxGapMaxFloat{31}
\def\SubcubicAttentionQuadraticMaxGapMeanFloat{23.54801324503311121816295781172811985015869140625}
\def\SubcubicAttentionQuadraticMaxGapMedianFloat{17}
\def\SubcubicAttentionQuadraticMaxGapMinFloat{17}
\def\SubcubicAttentionQuadraticMaxGapStdDevFloat{2.480478177891220159523300026194192469120025634765625}
\def\SubcubicAttentionQuadraticNormalizedAccuracyLen{1812}
\def\SubcubicAttentionQuadraticNormalizedAccuracyMaxFloat{0.42692148368752214082633145153522491455078125}
\def\SubcubicAttentionQuadraticNormalizedAccuracyMeanFloat{0.251856044718957339245690718598780222237110137939453125}
\def\SubcubicAttentionQuadraticNormalizedAccuracyMedianFloat{0.06053386841573309140596137467582593671977519989013671875}
\def\SubcubicAttentionQuadraticNormalizedAccuracyMinFloat{0.0327286840113341082059150721761398017406463623046875}
\def\SubcubicAttentionQuadraticNormalizedAccuracyStdDevFloat{0.09417041588014303521436687560708378441631793975830078125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.42662229202687740325927734375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{18289}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.35377647794955813242978592825238592922687530517578125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{7884}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.266816673101857249061907850773422978818416595458984375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.258666276000440120697021484375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{25516}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03354685319530149867350843351232470013201236724853515625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.3962266743183135986328125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.34221184121703862590635480955825187265872955322265625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12493}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.303691763430833761017169081242172978818416595458984375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18289}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.302087581716477815430010878117172978818416595458984375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{27300}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0169959471788390971414006713757771649397909641265869140625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{425445152}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{367447166.58278143405914306640625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12493}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{326086548}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18289}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{324364071}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{27300}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18249259.3244143426418304443359375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4511.5231788079472607932984828948974609375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{123}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{4800}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{4800}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{44.32851987900556878230418078601360321044921875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{142.3176116943359375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.737501687561433527662302367389202117919921875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{11130}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.5276889801025390625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{77.82788848876953125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.52193762668032572804577284841798245906829833984375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{56}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{32.72847682119205359185798442922532558441162109375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{742}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{23}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{23}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{6532}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{5.69876688745400628022252931259572505950927734375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2675913}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{16197}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2652438.2582781459204852581024169921875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2640941}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{123}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{2640941}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{123}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{9913.414170176254629041068255901336669921875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{29}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{5781}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.132450331125827602818390005268156528472900390625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{17}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{5928}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{5928}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.340757495236640561842023089411668479442596435546875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.42692148368752214082633145153522491455078125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18289}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3541206840796211618993538650101982057094573974609375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{18146}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.266991979627465958468945927961613051593303680419921875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1490}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.258757218043046799405004776417626999318599700927734375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{25516}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.033627643804422409357091083847990375943481922149658203125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7788383960723876953125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.7109411046994438265755889005959033966064453125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7467}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.60649967193603515625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.3337075710296630859375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7275671222553230510499133742996491491794586181640625}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2816207408905029296875}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{25516}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.216968575850227995971408745390363037586212158203125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{20294}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.15162289142608642578125}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{2.151265621185302734375}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicAttentionQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.030981219550324567979515677507151849567890167236328125}
\def\SubcubicAttentionQuadraticProofSearchTimeLen{1812}
\def\SubcubicAttentionQuadraticProofSearchTimeMaxFloat{46.9079892635345458984375}
\def\SubcubicAttentionQuadraticProofSearchTimeMeanFloat{44.53674874282041429296441492624580860137939453125}
\def\SubcubicAttentionQuadraticProofSearchTimeMedianFloat{42.32317340970039509784328402020037174224853515625}
\def\SubcubicAttentionQuadraticProofSearchTimeMinFloat{41.9884622097015380859375}
\def\SubcubicAttentionQuadraticProofSearchTimeStdDevFloat{0.75911860998109315090687232441268861293792724609375}
\def\SubcubicAttentionQuadraticProofTimeLen{1812}
\def\SubcubicAttentionQuadraticProofTimeMaxFloat{2.3055884838104248046875}
\def\SubcubicAttentionQuadraticProofTimeMeanFloat{2.211001165523697409298620186746120452880859375}
\def\SubcubicAttentionQuadraticProofTimeMedianFloat{2.1340785324573516845703125}
\def\SubcubicAttentionQuadraticProofTimeMinFloat{2.1184813976287841796875}
\def\SubcubicAttentionQuadraticProofTimeStdDevFloat{0.03074438269841588133868270915627363137900829315185546875}
\def\SubcubicAttentionVocabModelSquaredAccuracyLen{3020}
\def\SubcubicAttentionVocabModelSquaredAccuracyMaxFloat{0.74656238220632076263427734375}
\def\SubcubicAttentionVocabModelSquaredAccuracyMeanFloat{0.48427742413948260402634105048491619527339935302734375}
\def\SubcubicAttentionVocabModelSquaredAccuracyMedianFloat{0.1296332139242440117943289124013972468674182891845703125}
\def\SubcubicAttentionVocabModelSquaredAccuracyMinFloat{0.0668736966326831938634001062382594682276248931884765625}
\def\SubcubicAttentionVocabModelSquaredAccuracyStdDevFloat{0.1674624914675899856053575831538182683289051055908203125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyMaxFloat{0.73887385241687297821044921875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyMeanFloat{0.1315056148433346450143943684452096931636333465576171875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyMedianFloat{0.00000004470348358154297536744490042422139897126953655970282852649688720703125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticAccuracyStdDevFloat{0.222434889164279392392842282788478769361972808837890625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracMaxFloat{0.268531928770244121551513671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracMeanFloat{0.07538373267882507444692663511887076310813426971435546875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesFracStdDevFloat{0.0586854999373065677747973722944152541458606719970703125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesMaxFloat{288333963}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesMeanFloat{80942666.62649007141590118408203125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticDroppedSequencesStdDevFloat{63013075.745035469532012939453125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateMeanFloat{6457.4666666666662422358058393001556396484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateMedianFloat{6338}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateMinFloat{6338}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticEffectiveDimensionalityEstimateStdDevFloat{56.60372975539882389739432255737483501434326171875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundMaxFloat{41.54341888427734375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundMeanFloat{9.0247710483753120769279121304862201213836669921875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundMedianFloat{4.010895252227783203125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticErrUpperBoundStdDevFloat{5.03767082298718360533484883490018546581268310546875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueMaxFloat{27}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueMeanFloat{5.51589403973509906364824928459711372852325439453125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueMedianFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueMinFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracMeanFloat{0.99559378463437753215004022422363050282001495361328125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracMedianFloat{0.9716689845919608270463641019887290894985198974609375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracMinFloat{0.943529903888702392578125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.00592686780876558981512314261408391757868230342864990234375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticGapMostBelowValueStdDevFloat{3.731890951335211870087960051023401319980621337890625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountMaxFloat{4879728}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountMeanFloat{3593129.3333333334885537624359130859375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountMedianFloat{2864717}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountMinFloat{2864717}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticInstructionCountStdDevFloat{714919.26545083080418407917022705078125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapMaxFloat{30}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapMeanFloat{8.8136865342163357439630999579094350337982177734375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapMedianFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapMinFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticMaxGapStdDevFloat{5.9526971169174114351108073606155812740325927734375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyMaxFloat{0.73951073329633432162921735653071664273738861083984375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyMeanFloat{0.1316274072079527124312647856640978716313838958740234375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyMedianFloat{0.00000004477619510034710918767376810860347813303405928309075534343719482421875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticNormalizedAccuracyStdDevFloat{0.222624901415622800104898715289891697466373443603515625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.73887385241687297821044921875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.6284136571335476872945946524851024150848388671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{16069}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.476927766110747997085894667179672978818416595458984375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{28090}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.448228550143539905548095703125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.05289101732648844589323999798580189235508441925048828125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1415878655388951024018950874960864894092082977294921875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.11406609109473342389406980146304704248905181884765625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{19488}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.090771424816921297828997694523422978818416595458984375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08902535773813720354485923280662973411381244659423828125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1951}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00999342711442975650815156996031873859465122222900390625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{152028813}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{122477532.70860926806926727294921875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{19488}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{97465075.25}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{95590250}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1951}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{10730360.65785886161029338836669921875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{519}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6496.5165562913907706388272345066070556640625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{31.965597050006547164002768113277852535247802734375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{11.34843730926513671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24202}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.53126487352990192647439471329562366008758544921875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1283}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.94751203060150146484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.3131957128378595189843736079637892544269561767578125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{10}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.4370860927152317998434227774851024150848388671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9919348280161421893552642359281890094280242919921875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19451}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9755818843841552734375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11611}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97523391246795643194644753748434595763683319091796875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{22286}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005465507854250783482952247283037650049664080142974853515625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.75971551786489988078443502672598697245121002197265625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3681678}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{5928}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3036414.85430463589727878570556640625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{519}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2915149}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{2915149}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{264854.7799246955546550452709197998046875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{24173}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{13}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{6159}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{6159}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.012116810835729463491361457272432744503021240234375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.73951073329633432162921735653071664273738861083984375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.62898558894671052765801277928403578698635101318359375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6589}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.47971102572393864438282662376877851784229278564453125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.44856684670357382938021828522323630750179290771484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.052613537072433415320293903505444177426397800445556640625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6924571990966796875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.76375394625379300350687117315828800201416015625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15043}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.6303670406341552734375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.583120822906494140625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.71642306767657737420762487090541981160640716552734375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2991282939910888671875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{4800}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.219771784662410762933859587064944207668304443359375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{12457}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.146164476871490478515625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1422092914581298828125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.02928460812333964768949812196296988986432552337646484375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeMaxFloat{46.852759838104248046875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeMeanFloat{44.57711345954709969419127446599304676055908203125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeMedianFloat{42.3629872667789442175489966757595539093017578125}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeMinFloat{42.007546901702880859375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofSearchTimeStdDevFloat{0.7278673344767969677349128687637858092784881591796875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeLen{4530}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeMaxFloat{2.6413619518280029296875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeMeanFloat{2.208144986340015325509966714889742434024810791015625}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeMedianFloat{2.130373656749725341796875}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeMinFloat{2.1171014308929443359375}
\def\SubcubicAttentionVocabModelSquaredDirectQuadraticProofTimeStdDevFloat{0.0321930554120032075271495841661817394196987152099609375}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracLen{3020}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracMaxFloat{0.277765839360654298584307753117172978818416595458984375}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracMeanFloat{0.11618253188608641812695765338503406383097171783447265625}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracMedianFloat{0.0808456274354829862449633992582676000893115997314453125}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracMinFloat{0.0722891632467508038484282906210864894092082977294921875}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesFracStdDevFloat{0.03188613209208147891704498988474369980394840240478515625}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesLen{3020}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesMaxFloat{298248799}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesMeanFloat{124750043.704304635524749755859375}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesMedianFloat{86807331.4650000035762786865234375}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesMinFloat{77619898}
\def\SubcubicAttentionVocabModelSquaredDroppedSequencesStdDevFloat{34237473.63285650312900543212890625}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateLen{3020}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateMeanFloat{4429.8000000000001818989403545856475830078125}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateMedianFloat{4290}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateMinFloat{4290}
\def\SubcubicAttentionVocabModelSquaredEffectiveDimensionalityEstimateStdDevFloat{79.13760168213337919951300136744976043701171875}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundLen{3020}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundMaxFloat{41.54341888427734375}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundMeanFloat{9.0247710483753120769279121304862201213836669921875}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundMedianFloat{4.01543684720993088177465324406512081623077392578125}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicAttentionVocabModelSquaredErrUpperBoundStdDevFloat{5.03767082298718360533484883490018546581268310546875}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueLen{3020}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueMaxFloat{18}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueMeanFloat{5.42814569536423885409703871118836104869842529296875}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueMedianFloat{4}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueMinFloat{3}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdLen{3020}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracLen{3020}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracMeanFloat{0.98938353259042399745482043726951815187931060791015625}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracMedianFloat{0.956373289823531980147208741982467472553253173828125}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracMinFloat{0.9398634433746337890625}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueSequenceFracStdDevFloat{0.00943658151605220561763953668332760571502149105072021484375}
\def\SubcubicAttentionVocabModelSquaredGapMostBelowValueStdDevFloat{1.742667478045585749413248777273111045360565185546875}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchLen{3020}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntLen{3020}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredInstructionCountLen{3020}
\def\SubcubicAttentionVocabModelSquaredInstructionCountMaxFloat{5144079}
\def\SubcubicAttentionVocabModelSquaredInstructionCountMeanFloat{3854035.5}
\def\SubcubicAttentionVocabModelSquaredInstructionCountMedianFloat{3122861}
\def\SubcubicAttentionVocabModelSquaredInstructionCountMinFloat{3122861}
\def\SubcubicAttentionVocabModelSquaredInstructionCountStdDevFloat{714930.528304289211519062519073486328125}
\def\SubcubicAttentionVocabModelSquaredMaxGapLen{3020}
\def\SubcubicAttentionVocabModelSquaredMaxGapMaxFloat{27}
\def\SubcubicAttentionVocabModelSquaredMaxGapMeanFloat{15.26158940397350960438416223041713237762451171875}
\def\SubcubicAttentionVocabModelSquaredMaxGapMedianFloat{7}
\def\SubcubicAttentionVocabModelSquaredMaxGapMinFloat{6}
\def\SubcubicAttentionVocabModelSquaredMaxGapStdDevFloat{3.0543284003371784507407937780953943729400634765625}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyLen{3020}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyMaxFloat{0.746860739113479166206843729014508426189422607421875}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyMeanFloat{0.48473980995708754182516031505656428635120391845703125}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyMedianFloat{0.1296906710232374193569881981602520681917667388916015625}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyMinFloat{0.06693384934231318139641331299571902491152286529541015625}
\def\SubcubicAttentionVocabModelSquaredNormalizedAccuracyStdDevFloat{0.1676138329742613841677467689805780537426471710205078125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.74656238220632076263427734375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMaxKey{29110}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.68152182372225234008311645084177143871784210205078125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMeanKey{8893}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.5830572047270834445953369140625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMedianKey{1951}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMinFloat{0.576360945589840412139892578125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMinKey{12552}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0326520972394782893477582774721668101847171783447265625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1366814589127897938691802437460864894092082977294921875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.09539359169611270894417742738369270227849483489990234375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{6549}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.07646392728202038024942766014646622352302074432373046875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0722891632467508038484282906210864894092082977294921875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00992546233466068926476477685127974837087094783782958984375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{146760599}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{102428089.1456953585147857666015625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{6549}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{82102516.75}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{77619898}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{10657384.031261868774890899658203125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{123}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4495.0596026490065924008376896381378173828125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{742}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{742}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{47.51175968590705878114022198133170604705810546875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{12.7308502197265625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{6.25922262273876839344666223041713237762451171875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{23696}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.949953854084014892578125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.8679935932159423828125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.9812004423694222765561789856292307376861572265625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2773}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.47682119205297990305325583904050290584564208984375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999912261962890625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2773}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.988440591767923759647374026826582849025726318359375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{27484}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96113267540931690557926003748434595763683319091796875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{3284}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.960617244243621826171875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{28716}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0088009097245529931130558765062232851050794124603271484375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.66943128067852997187259234124212525784969329833984375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3946029}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMaxKey{4647}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3432327.5827814568765461444854736328125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMeanKey{104}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3171245}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMinFloat{3171245}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{353223.79605364613234996795654296875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.7880794701986761907619438716210424900054931640625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMeanKey{742}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMedianKey{7310}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMinKey{27300}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.382633835419216694617716711945831775665283203125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.746860739113479166206843729014508426189422607421875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29110}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6821725206867614854644443767028860747814178466796875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{913}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.58337730952206057200015720809460617601871490478515625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1951}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.5766619895937477036085283543798141181468963623046875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{12552}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03262640758071644331295146912452764809131622314453125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.71249103546142578125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.66405966108208502873821998946368694305419921875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{8840}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.722886621952056884765625}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.647382259368896484375}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.73555103743237737479176985289086587727069854736328125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.275043010711669921875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMaxKey{26374}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.215887184964110634410872080479748547077178955078125}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMeanKey{3175}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.143325030803680419921875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1391570568084716796875}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicAttentionVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0307480955379075028555124760032413178123533725738525390625}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeLen{3020}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeMaxFloat{46.8482859134674072265625}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeMeanFloat{44.52641797436783832608853117562830448150634765625}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeMedianFloat{42.38909483790397558777840458787977695465087890625}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeMinFloat{42.251099109649658203125}
\def\SubcubicAttentionVocabModelSquaredProofSearchTimeStdDevFloat{0.74956114068837920161314514189143665134906768798828125}
\def\SubcubicAttentionVocabModelSquaredProofTimeLen{3020}
\def\SubcubicAttentionVocabModelSquaredProofTimeMaxFloat{2.48164653778076171875}
\def\SubcubicAttentionVocabModelSquaredProofTimeMeanFloat{2.21034630410718602178121727774851024150848388671875}
\def\SubcubicAttentionVocabModelSquaredProofTimeMedianFloat{2.131865792274475257528365546022541821002960205078125}
\def\SubcubicAttentionVocabModelSquaredProofTimeMinFloat{2.1191422939300537109375}
\def\SubcubicAttentionVocabModelSquaredProofTimeStdDevFloat{0.031555088564218680691197960186400450766086578369140625}
\def\SubcubicDirectQuadraticAccuracyLen{1812}
\def\SubcubicDirectQuadraticAccuracyMaxFloat{0.7556504905223846435546875}
\def\SubcubicDirectQuadraticAccuracyMeanFloat{0.1396049355751902698585809048381634056568145751953125}
\def\SubcubicDirectQuadraticAccuracyMedianFloat{0.00000004470348358154297536744490042422139897126953655970282852649688720703125}
\def\SubcubicDirectQuadraticAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicDirectQuadraticAccuracyStdDevFloat{0.235333725517374914293355914196581579744815826416015625}
\def\SubcubicDirectQuadraticDroppedSequencesFracLen{1812}
\def\SubcubicDirectQuadraticDroppedSequencesFracMaxFloat{0.1276281056925654133760161812460864894092082977294921875}
\def\SubcubicDirectQuadraticDroppedSequencesFracMeanFloat{0.06056095187132866375367967748388764448463916778564453125}
\def\SubcubicDirectQuadraticDroppedSequencesFracMedianFloat{0}
\def\SubcubicDirectQuadraticDroppedSequencesFracMinFloat{0}
\def\SubcubicDirectQuadraticDroppedSequencesFracStdDevFloat{0.044774708700993683108126930392245412804186344146728515625}
\def\SubcubicDirectQuadraticDroppedSequencesLen{1812}
\def\SubcubicDirectQuadraticDroppedSequencesMaxFloat{137039635}
\def\SubcubicDirectQuadraticDroppedSequencesMeanFloat{65026826.925496689975261688232421875}
\def\SubcubicDirectQuadraticDroppedSequencesMedianFloat{0}
\def\SubcubicDirectQuadraticDroppedSequencesMinFloat{0}
\def\SubcubicDirectQuadraticDroppedSequencesStdDevFloat{48076477.389673650264739990234375}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateLen{1812}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateMeanFloat{8428.666666666666060336865484714508056640625}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicDirectQuadraticEffectiveDimensionalityEstimateStdDevFloat{1920.237022406927508200169540941715240478515625}
\def\SubcubicDirectQuadraticErrUpperBoundLen{1812}
\def\SubcubicDirectQuadraticErrUpperBoundMaxFloat{5.4248905181884765625}
\def\SubcubicDirectQuadraticErrUpperBoundMeanFloat{1.2133885164134550205261575683834962546825408935546875}
\def\SubcubicDirectQuadraticErrUpperBoundMedianFloat{0}
\def\SubcubicDirectQuadraticErrUpperBoundMinFloat{0}
\def\SubcubicDirectQuadraticErrUpperBoundStdDevFloat{1.2908711057637736185910171116120181977748870849609375}
\def\SubcubicDirectQuadraticGapMostBelowValueLen{1812}
\def\SubcubicDirectQuadraticGapMostBelowValueMaxFloat{9}
\def\SubcubicDirectQuadraticGapMostBelowValueMeanFloat{4.32064017660044186186496517620980739593505859375}
\def\SubcubicDirectQuadraticGapMostBelowValueMedianFloat{1}
\def\SubcubicDirectQuadraticGapMostBelowValueMinFloat{1}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdLen{1812}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicDirectQuadraticGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracLen{1812}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracMeanFloat{0.99243573821406749768669897093786858022212982177734375}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracMedianFloat{0.96433444827795022913363709449185989797115325927734375}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracMinFloat{0.946926116943359375}
\def\SubcubicDirectQuadraticGapMostBelowValueSequenceFracStdDevFloat{0.00786985045308694237953250905093227629549801349639892578125}
\def\SubcubicDirectQuadraticGapMostBelowValueStdDevFloat{2.426935409979765978505383827723562717437744140625}
\def\SubcubicDirectQuadraticInstructionCountBranchLen{1812}
\def\SubcubicDirectQuadraticInstructionCountBranchMaxFloat{0}
\def\SubcubicDirectQuadraticInstructionCountBranchMeanFloat{0}
\def\SubcubicDirectQuadraticInstructionCountBranchMedianFloat{0}
\def\SubcubicDirectQuadraticInstructionCountBranchMinFloat{0}
\def\SubcubicDirectQuadraticInstructionCountBranchStdDevFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntLen{1812}
\def\SubcubicDirectQuadraticInstructionCountIntMaxFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntMeanFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntMedianFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntMinFloat{0}
\def\SubcubicDirectQuadraticInstructionCountIntStdDevFloat{0}
\def\SubcubicDirectQuadraticInstructionCountLen{1812}
\def\SubcubicDirectQuadraticInstructionCountMaxFloat{3929391}
\def\SubcubicDirectQuadraticInstructionCountMeanFloat{3288115.8333333334885537624359130859375}
\def\SubcubicDirectQuadraticInstructionCountMedianFloat{2646158}
\def\SubcubicDirectQuadraticInstructionCountMinFloat{2646158}
\def\SubcubicDirectQuadraticInstructionCountStdDevFloat{616875.807056659949012100696563720703125}
\def\SubcubicDirectQuadraticMaxGapLen{1812}
\def\SubcubicDirectQuadraticMaxGapMaxFloat{26}
\def\SubcubicDirectQuadraticMaxGapMeanFloat{8.0827814569536418076722839032299816608428955078125}
\def\SubcubicDirectQuadraticMaxGapMedianFloat{1}
\def\SubcubicDirectQuadraticMaxGapMinFloat{1}
\def\SubcubicDirectQuadraticMaxGapStdDevFloat{5.33231137325812998284391142078675329685211181640625}
\def\SubcubicDirectQuadraticNormalizedAccuracyLen{1812}
\def\SubcubicDirectQuadraticNormalizedAccuracyMaxFloat{0.7559720149848636605582896663690917193889617919921875}
\def\SubcubicDirectQuadraticNormalizedAccuracyMeanFloat{0.1397320150117158099600800369444186799228191375732421875}
\def\SubcubicDirectQuadraticNormalizedAccuracyMedianFloat{0.00000004477619510034710918767376810860347813303405928309075534343719482421875}
\def\SubcubicDirectQuadraticNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicDirectQuadraticNormalizedAccuracyStdDevFloat{0.2355335635642885894203146790459868498146533966064453125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.7556504905223846435546875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMaxKey{12287}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.6486094781068085790565191928180865943431854248046875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMeanKey{17096}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.4958753963001072406768798828125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinFloat{0.462237928993999902527178846867172978818416595458984375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0552932416205054177993361008702777326107025146484375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1276281056925654133760161812460864894092082977294921875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10003464763354974476072811739868484437465667724609375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{6155}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.07986202277243137359619140625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{27484}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07836645096540449662025906718554324470460414886474609375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1951}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0085299462401241983589006423471801099367439746856689453125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{137039635}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{107411385.01324503123760223388671875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{6155}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{85751194}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{27484}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{84145336}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1951}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9158960.03449290432035923004150390625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{9835.9602649006628780625760555267333984375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{519}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{519}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{1328.72651215985251837992109358310699462890625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{3.96725940704345703125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20751}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0.322178009330042147695394305628724396228790283203125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.826449300470885273028898154734633862972259521484375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{5.66225165562913890227036972646601498126983642578125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98827509098495081030222308982047252357006072998046875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{2236}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.963069438934326171875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{18289}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.960471451282501220703125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{12287}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00795629448668952639345253174951722030527889728546142578125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.7536877743288368236562746460549533367156982421875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3929391}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMaxKey{519}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2868039.14569536410272121429443359375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2696590}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinFloat{2696590}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{426576.9200305151753127574920654296875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMaxKey{24173}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanFloat{12.364238410596026795928992214612662792205810546875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMeanKey{913}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianFloat{7.75}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMedianKey{1696}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapMinKey{6159}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.058986205495547228139230355736799538135528564453125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7559720149848636605582896663690917193889617919921875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12287}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.64919935029943809379204822107567451894283294677734375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{17096}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.496161259854536240698763549517025239765644073486328125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.462586799009633231616334114733035676181316375732421875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.055005449322321077476605211131754913367331027984619140625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.53686046600341796875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.742552586738639774921466596424579620361328125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{6082}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.4549176692962646484375}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20415}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4357960224151611328125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.73009240210249515268259301592479459941387176513671875}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2811653614044189453125}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMaxKey{26374}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.214817225538342260193758193054236471652984619140625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMeanKey{19004}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.14238131046295166015625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMedianKey{21317}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1330397129058837890625}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicDirectQuadraticOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.028874608329009197882353277009315206669270992279052734375}
\def\SubcubicDirectQuadraticProofSearchTimeLen{1812}
\def\SubcubicDirectQuadraticProofSearchTimeMaxFloat{46.628111362457275390625}
\def\SubcubicDirectQuadraticProofSearchTimeMeanFloat{44.5625126075007784720583003945648670196533203125}
\def\SubcubicDirectQuadraticProofSearchTimeMedianFloat{42.37711223244667024800946819595992565155029296875}
\def\SubcubicDirectQuadraticProofSearchTimeMinFloat{42.0871791839599609375}
\def\SubcubicDirectQuadraticProofSearchTimeStdDevFloat{0.73151793598355474568251111122663132846355438232421875}
\def\SubcubicDirectQuadraticProofTimeLen{1812}
\def\SubcubicDirectQuadraticProofTimeMaxFloat{2.4025633335113525390625}
\def\SubcubicDirectQuadraticProofTimeMeanFloat{2.206100981098663371682278011576272547245025634765625}
\def\SubcubicDirectQuadraticProofTimeMedianFloat{2.1298853623867035622652110760100185871124267578125}
\def\SubcubicDirectQuadraticProofTimeMinFloat{2.118173122406005859375}
\def\SubcubicDirectQuadraticProofTimeStdDevFloat{0.031421532737503622689789750666022882796823978424072265625}
\def\SubcubicDroppedSequencesFracLen{7852}
\def\SubcubicDroppedSequencesFracMaxFloat{0.402560516260564327239990234375}
\def\SubcubicDroppedSequencesFracMeanFloat{0.1513206128782288717449233672596164979040622711181640625}
\def\SubcubicDroppedSequencesFracMedianFloat{0}
\def\SubcubicDroppedSequencesFracMinFloat{0}
\def\SubcubicDroppedSequencesFracStdDevFloat{0.11253438820870446945843212915860931389033794403076171875}
\def\SubcubicDroppedSequencesLen{7852}
\def\SubcubicDroppedSequencesMaxFloat{432246063}
\def\SubcubicDroppedSequencesMeanFloat{162479270.8806673586368560791015625}
\def\SubcubicDroppedSequencesMedianFloat{0}
\def\SubcubicDroppedSequencesMinFloat{0}
\def\SubcubicDroppedSequencesStdDevFloat{120832879.25793842971324920654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.519606747664511203765869140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.316182027688089561934248195029795169830322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{9504}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.10859048785641785273003989686912973411381244659423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{32103}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.089983913116156999389971815617172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.08482018947328880120739569292709347791969776153564453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1234241919592022063145719812382594682276248931884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.08851300396444579388077755766062182374298572540283203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.072604254353791419784869276554672978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.06821281462907789749916531718554324470460414886474609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00899922071107442551884947334883690928108990192413330078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{132525717}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{95040114.32450331747531890869140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{77958224.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{73242952}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9662839.660887636244297027587890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2773}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.364238410596026795928992214612662792205810546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99841845035552978515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{11498}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98502926400165680131948420239496044814586639404296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95007731020450592041015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{3284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94847071170806884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{16284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01013873660769488808941485302739238250069320201873779296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.71394291522974395736156338898581452667713165283203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2912557}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2912557}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2912557}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{2912557}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{4430}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{13.403973509933774010960405576042830944061279296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.8741438839742858846193485078401863574981689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.5202887798389654872011078623472712934017181396484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.316483807792376559131497515409137122333049774169921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{9504}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1086488824446163459214176327805034816265106201171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{32103}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.09006485340313973020354154641609056852757930755615234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0848833022154484584387290624363231472671031951904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.5142066478729248046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.404365959546424846848822198808193206787109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.33930504322052001953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.22169661521912331636485760100185871124267578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.75596831132245945195080594203318469226360321044921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.307686328887939453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.200835287965686060118741806945763528347015380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{19093}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.134493350982666015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{20751}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.129741191864013671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.029785244094478767473699321044477983377873897552490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.496975469402968883514404296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.310149921437367692700348698053858242928981781005859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{6204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.103495790623128358642901503117172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{32103}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.08011294342577450489084611717771622352302074432373046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0821409116801595506895949938552803359925746917724609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1285205837339161993870817468632594682276248931884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.09419450606682043536377335612996830604970455169677734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.07781888474710284275825955546679324470460414886474609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{24566}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07166492845863099703240806093162973411381244659423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00899707039623155215013472485452439286746084690093994140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{137997926}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{101140580.7549668848514556884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{83557391.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{24566}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{76949631}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9660530.777906067669391632080078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.4248905181884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.426777032826910041052315136766992509365081787109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.4322891533374786376953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{23367}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.40823304653167724609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.6229550865539874582310631012660451233386993408203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2773}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.5562913907284769976513416622765362262725830078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9998977184295654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30463}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.986013848260538505741124026826582849025726318359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6155}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9555386602878570556640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{913}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95305842161178599969417746251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.008897220820636424221117266597502748481929302215576171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.74260826881960995127229807621915824711322784423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{4145358}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{4145358}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{4145358}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{4145358}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{4430}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{13.609271523178808394050065544433891773223876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{4157}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.86866082196594707198755713761784136295318603515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.497112574992529310247135754252667538821697235107421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.310444008712090158130791905932710506021976470947265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.10355080114316662920348477427978650666773319244384765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{32103}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.080185004802162340720173006047843955457210540771484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.08219668339298784320856583462955313734710216522216796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.4314517974853515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.3964023100619300521429977379739284515380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.217673957347869873046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.2084720134735107421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.75903030692707051940715246018953621387481689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.259760379791260209714209850062616169452667236328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{14095}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.202755868040173314881258193054236471652984619140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{22401}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.1315515041351318359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1302669048309326171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0290032380628030654612370398126586223952472209930419921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.495767078362405300140380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.296996358856065401088386579431244172155857086181640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.09788762149401002143900285545896622352302074432373046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0695653501898050030671782906210864894092082977294921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.076789679652158271405681944088428281247615814208984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.144937380217015687744464003117172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.11195773261889119254419711069203913211822509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.092430671909823958198870741398422978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0902943378314375044713102624882594682276248931884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.009473445757571759273663047906666179187595844268798828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{155625327}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{120213700.033112585544586181640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{99246678.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{96952807}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{10172034.9273001588881015777587890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.27951812744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.801418986541545308455170015804469585418701171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22545}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.205653667449951171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.93181514739990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.594245364275689524902190896682441234588623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{5.24503311258278159812107332982122898101806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999999940395355224609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98896627789301583266734496646677143871784210205078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{26829}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.965402185916900634765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8840}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.964576244354248046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{5928}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00813513244187778587768189453299783053807914257049560546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.79707152260546243471850402784184552729129791259765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3889326}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3889326}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3889326}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3889326}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{22}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.357615894039735593423756654374301433563232421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{4157}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.71919020392778687522650216124020516872406005859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.496401930883097530777803285673144273459911346435546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.2972705087224010167545884542050771415233612060546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.09797234246288803738433870194057817570865154266357421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.06962792403454488854297466104981140233576297760009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07682066817152044535532695590518414974212646484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.768610477447509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.41988161383875421961420215666294097900390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.3587067127227783203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.308929920196533203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.76196009742930481678513388033024966716766357421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.256158351898193803464209850062616169452667236328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20229326336589092960593916359357535839080810546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.13276565074920654296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.131864070892333984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.02870866685420463138012081572014722041785717010498046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.506960985250771045684814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.30517493384514027265907998298644088208675384521484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.10162649932317434353645779765429324470460414886474609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.08499530237168069490838462343162973411381244659423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07975522525543120300195454319691634736955165863037109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.139004149474203586578369140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10475829625440548353854097740622819401323795318603515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.086442478932440280914306640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08110661245882509751137234843554324470460414886474609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00918716273154655295452020169477691524662077426910400390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{149254569}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{112483364.09933774173259735107421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{92816905}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{87087562}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9864640.86875561811029911041259765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.0167236328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.06559399105855145961641028407029807567596435546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1412}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.94751203060150146484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.535209767337012198851198263582773506641387939453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.95364238410596069428493137820623815059661865234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99969661235809315069644753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30463}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98624778346510122428725253485026769340038299560546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94994063675403606072933371251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9398634433746337890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01035463764931248732692470326810507685877382755279541015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.79182702927868209297201929075527004897594451904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3131116}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3131116}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3131116}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{3131116}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{4430}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{13.887417218543046004697316675446927547454833984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{4157}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{23367}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{23367}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.940859230540379343210588558577001094818115234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.507626418686129898816261629690416157245635986328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.305457935493813004246277387210284359753131866455078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.10171458830733837164217447934788651764392852783203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0850717554167629563810493209530250169336795806884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.079789194864500145865093827524106018245220184326171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6595213413238525390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.422637798928263919151504524052143096923828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{6155}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.312935292720794677734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.251099109649658203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7724868512860918468021509397658519446849822998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3077466487884521484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{14929}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.2055945522737818720315772225148975849151611328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{23633}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.129819095134735107421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1191422939300537109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.030820924400883027705067007673278567381203174591064453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.276340342126786708831787109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.1452000536431638233469954002430313266813755035400390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{22401}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.040021192282438201870409244520487845875322818756103515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.034419999457895700256671034367172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04367122848689385106180083084836951456964015960693359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.401241963729262296478594862492172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.34664461257195233745420637205825187265872955322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.30789061659015715122222900390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.304721791297197286407794081242172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0168036946075711020320841981856574420817196369171142578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{430830278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{372206818.58278143405914306640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{330595032.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{327192532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18042829.6978723593056201934814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.185821533203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.6145395948397407437369110994040966033935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.5718860626220703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{77.82788848876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.51010078068381492499838714138604700565338134765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{60}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{34.4701986754966895887264399789273738861083984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{23.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{23}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99999782068050457883856552143697626888751983642578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99991773068904876708984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99967092275619517938167746251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00002669110375110156420396835541541946668075979687273502349853515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{5.99647572767379966052203599247150123119354248046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2600812}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2600812}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2600812}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2600812}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{30}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.980132450331126392484293319284915924072265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{18}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{18}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.482975673335813926456694389344193041324615478515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.276703064522670294511641486678854562342166900634765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.145341154248759096834220372329582460224628448486328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22401}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.040055892114442055718104285233494010753929615020751953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.03445096015450900550636248453884036280214786529541015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.04371087440655008204970499718911014497280120849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.62030029296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.4211262488207268006590311415493488311767578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.2499897480010986328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.206531524658203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.76781586871280149697582828594022430479526519775390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2745163440704345703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{30684}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.205460827871663642696375973173417150974273681640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{4157}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.134675204753875732421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1311380863189697265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0295198978386494066683543024964819778688251972198486328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.4974975474178791046142578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.2966088616159676671912848178180865943431854248046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{16284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0979081555269657732853971765507594682276248931884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0668736966326831938634001062382594682276248931884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07736203627429051599140308326241211034357547760009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.144739002920687198638916015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.11206760979103326525407879898921237327158451080322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09256110712885855240639187968554324470460414886474609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0902680894359945973359771187460864894092082977294921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00943456354417217778196569355486644781194627285003662109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{155412321}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{120331679.74834437668323516845703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{99386732}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{96924623}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{10130285.4685633368790149688720703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.38015460968017578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.8657478844093162706485600210726261138916015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.17229998111724853515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.9324092864990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6180041988517543938286280535976402461528778076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{5.24503311258278159812107332982122898101806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98893718885270176510715600670664571225643157958984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{7790}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.965452253818511962890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8840}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96449130773544322625667746251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{5928}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00813287973752823377393550430269897333346307277679443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.79707152260546243471850402784184552729129791259765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3897645}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3897645}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3897645}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3897645}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{22}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.2847682119205305895093260915018618106842041015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{4157}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.7617409726016202142773181549273431301116943359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.498134615883699172211862560288864187896251678466796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.29688256607704743839093453061650507152080535888671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{16284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.097992866290712132837370518245734274387359619140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.06693384934231318139641331299571902491152286529541015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07739339803216434277022273136026342399418354034423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6693074703216552734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.41106804948768882468357332982122898101806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22545}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.275184810161590576171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.2611141204833984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.76182727897097013425309341982938349246978759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2846319675445556640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{23241}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20229813436798682602102417149581015110015869140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{29052}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.128636777400970458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1195850372314453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0303537684731022029682723228916074731387197971343994140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.4992454946041107177734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.304967537010396971819403688641614280641078948974609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.10125161125324662336755210390037973411381244659423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.08595738653093569492380510155271622352302074432373046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0793237035168515569605318660251214168965816497802734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1390961995348334034883208687460864894092082977294921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.104833150122141949278642414355999790132045745849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.086499414872378055374468885929672978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08111111819744110107421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.009192219469374547646811635104313609190285205841064453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{149353407}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{112563737.82781456410884857177734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{3254}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{92878039.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{87092400}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9870070.49965453706681728363037109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.015990734100341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.07849087778306174101317083113826811313629150390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.975169837474822998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.8679935932159423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.53139427036718023256156584466225467622280120849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.97350993377483430180063805892132222652435302734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99969661235809315069644753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{30463}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98669101584036622565321295041940174996852874755859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94969852268695831298828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9398634433746337890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.010231354398016527518233687032989109866321086883544921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.80517383148481835863918831819319166243076324462890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3156073}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3156073}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3156073}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{3156073}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{4430}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{13.887417218543046004697316675446927547454833984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{4157}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{23367}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{23367}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.940859230540379343210588558577001094818115234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.499900800740533668431453406810760498046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.30525026790884368654843683543731458485126495361328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.1013393884750020124130287513253279030323028564453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.08603470496812255785545886510590207763016223907470703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07935683898242462674943453748710453510284423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.5923202037811279296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.42925044085016139661092893220484256744384765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22401}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.43295371532440185546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.31475162506103515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.76495382616690543731152729378663934767246246337890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3132572174072265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{17096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20657294159693417867629250395111739635467529296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{6155}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.13178348541259765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.12702274322509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.032454740980667577676666013530848431400954723358154296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.279742280952632427215576171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.1455683418432410503040586036149761639535427093505859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{10248}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.03892152151092879985849748436521622352302074432373046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.033719403669238000309515967956031090579926967620849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04344791015314623805476657025792519561946392059326171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.400874502025544587890948378117172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.34656281544154643459165754393325187265872955322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8721}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.3071563723497092723846435546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.303980688564479295532549940617172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.016831650711032340728134926166603690944612026214599609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{430435719}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{372118989.58278143405914306640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8721}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{329806643.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{326396779}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18072847.3353947661817073822021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.12237548828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.439607481293336377348168753087520599365234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.6455821990966796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.29946136474609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.5064594809721061352547621936537325382232666015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{59}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{34.4105960264900687661793199367821216583251953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{23.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{23}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99999782068050457883856552143697626888751983642578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99991773068904876708984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99967092275619517938167746251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00002669110375110156420396835541541946668075979687273502349853515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{5.96709689380997598817657490144483745098114013671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2613099}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2613099}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2613099}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2613099}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{30}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{22261}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.827814569536425182150196633301675319671630859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{19451}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.451547934851329824113008726271800696849822998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.280109468709570652578122462728060781955718994140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1457097056417858971233414422385976649820804595947265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{10248}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0389552704228695867438858613240881823003292083740234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.033749734181830311208205586126496200449764728546142578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.04348875063493308490425448553651222027838230133056640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.38463878631591796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.424733229820304813983966596424579620361328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.154105246067047119140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{41.9884622097015380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.77291994629386839843476764144725166261196136474609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.295291900634765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{30684}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.205023126096914865001963335089385509490966796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{29195}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.129197061061859130859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.123301029205322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.029585923112094424103357681588022387586534023284912109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.291603716090321485321368299992172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.1418804538726115282987194632369210012257099151611328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.03765481011942022060434709374021622352302074432373046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.032699271105229799072589003117172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.044364889726759414168011375068090273998677730560302734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.402560516260564327239990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.349909294482986632512933056204929016530513763427734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{19488}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.310895435046404544632281385929672978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.304346392862498704712237440617172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.016668121367447781555615193838093546219170093536376953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{432246063}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{375712244.092715203762054443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{19488}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{333821431.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{326789451}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17897259.039736755192279815673828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{142.3176116943359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.2863692732046700939463335089385509490966796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{30684}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.6405811309814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.46202850341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.42529095414309292522148098214529454708099365234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{61}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{35.5099337748344368037578533403575420379638671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{24.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{24}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{6.139512189855889090495111304335296154022216796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2627529}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2627529}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2627529}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2627529}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{31}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{27584}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{24.158940397350992412839332246221601963043212890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{18}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{18}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.46590717890811372825510261463932693004608154296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.291986473083870823330698840436525642871856689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.14201982414795255582617983236559666693210601806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0376874614628037729602283434360288083553314208984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0327286840113341082059150721761398017406463623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.044411949817212727220638868175228708423674106597900390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.423552036285400390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.427821983564768970609293319284915924072265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.282036840915679931640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.27365779876708984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.76985008215492845007332789464271627366542816162109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.268847942352294921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{7790}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.2053782197813323051605038926936686038970947265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{29725}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.130111634731292724609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1184813976287841796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0303273536330029118424089773498053546063601970672607421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.439475632272660676758135878117172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.256276335474720451390595599150401540100574493408203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{23696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.07617602939717467436242515077537973411381244659423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0727815646678209027253814156210864894092082977294921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07158876660457948182259002578575746156275272369384765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.277765839360654298584307753117172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.178695667491892695721844575018621981143951416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.141075203428044859688128553898422978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1354111749678849896394439156210864894092082977294921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{23367}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.023310748167516763540429991508062812499701976776123046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{298248799}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{191873011.9536423981189727783203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{151478346.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{145396642}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{23367}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{25029725.2561941035091876983642578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{41.54341888427734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{17.3126035020840873812630889005959033966064453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{10.696970462799072265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{10.537830352783203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27671}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{4.59898901089020117893824135535396635532379150390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{18}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.6887417218543046004697316675446927547454833984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{5928}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5928}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{19917}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99720681700485436227410218634759075939655303955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98666611313819896356136496251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{2773}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.986644923686981201171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{26374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0031821486465828849841963599232030901475809514522552490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.9126121331056633589895454861107282340526580810546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5095695}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5095695}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5095695}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{5095695}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{27}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{17.4900662251655631962421466596424579620361328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{1412}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{9.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{1696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.085680556850544320468543446622788906097412109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.4396512647362584846888466927339322865009307861328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.256520011652247414968286420844378881156444549560546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{23696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0762437971141756987147886093225679360330104827880859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6589}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.072844021825428206806662956296349875628948211669921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{24202}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07164358145153836010532444333875901065766811370849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.5303728580474853515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.40950067153829650123952887952327728271484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.4009685516357421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.33406352996826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7567259326236197569670594020863063633441925048828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2619693279266357421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.203474174272145535979916530777700245380401611328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{23447}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.142811715602874755859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{2.138918399810791015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0275433892509211776522537462597028934396803379058837890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.753120095469057559967041015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.654713135138647484012608401826582849025726318359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.455286094220355097572650038273422978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.4533286578953266143798828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04952300743833436269536463214535615406930446624755859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.10962926130741830477166587343162973411381244659423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{5615}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.08341362230504383024065617746600764803588390350341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{23447}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0688529843464492918858610437382594682276248931884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{20754}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.065018721856176797668780409367172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00842216258769191809807619364391939598135650157928466796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{117713523}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{5615}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{89564694.96026490628719329833984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{23447}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{73930329}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{20754}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{69813321}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9043228.2189328782260417938232421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{8258}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2773}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.1721854304635765942066427669487893581390380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99987208843231201171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2773}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.987022513190642047931078195688314735889434814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95619834959506988525390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12287}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95361793041229236944644753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01022565526152992461395019319070343044586479663848876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.6486010355865057253055283581488765776157379150390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2960941}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2960941}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2960941}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{2960941}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{20976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.25165562913907280062630889005959033966064453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{2743}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{7790}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.107816556516548534006005866103805601596832275390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.75376301272306667211609010337269864976406097412109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.65532989746387004803551690201857127249240875244140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{26278}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.45554599895135916565180878023966215550899505615234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.45358151224778620047572985640726983547210693359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.049431435765213242727877940296821179799735546112060546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.55720806121826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.63062552900503732189463335089385509490966796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{6910}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.56535613536834716796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.46084618568421120698985760100185871124267578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.73978297047708008182809180652839131653308868408203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.275522947311401811276709850062616169452667236328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.214076853745820638863506246707402169704437255859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{23447}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.14254057407379150390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1409122943878173828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0288102014620604078565246908283370430581271648406982421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.76103517971932888031005859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.64805032942592111222523953983909450471401214599609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{24262}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.461929114302620236198748671085922978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.441555338911712114136065565617172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.05058611362548702528041388859492144547402858734130859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.11541429813951249727654868593162973411381244659423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{5615}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.0893270260228818113734661210401100106537342071533203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{3175}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.073645865777507368843401991398422978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0698184575885534008943267281210864894092082977294921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00845880239062728710164318357556112459860742092132568359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{123925159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{5615}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{95914163.8543046414852142333984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{3175}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{79076646.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6204}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{74966998}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9082569.90776770003139972686767578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.4248905181884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.426777032826910041052315136766992509365081787109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24173}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.4322891533374786376953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{23367}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.40823304653167724609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.6229550865539874582310631012660451233386993408203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2773}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.33112582781456989522439471329562366008758544921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.9998238086700439453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2773}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98741537411481339336916107640718109905719757080078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96033975481986988409488503748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9586026668548583984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11611}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.008300055435271187775914114581610192544758319854736328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.64819519487375665267592239615623839199542999267578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{4193742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{4193742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{4193742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{4193742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.364238410596026795928992214612662792205810546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{2743}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{2743}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.163289937379847316378800314851105213165283203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.76168485385615392058156203347607515752315521240234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.64866255548654250251416897299350239336490631103515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24262}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.46219289137181107651741740482975728809833526611328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.4418016264281774407862712905625812709331512451171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.050522292537460600225784901340375654399394989013671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.506034374237060546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.6485902773623450912054977379739284515380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4810}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.5868284702301025390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4924118518829345703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7247434293796970461443152089486829936504364013671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.268134593963623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{32103}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.214147547222920398013457088381983339786529541015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.14547932147979736328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.14163875579833984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0291966581152570854584826776090267230756580829620361328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.715768217109143733978271484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.626590924380680203142901518731378018856048583984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{23696}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.449778104666620437424029432804672978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.437388068996369783203448378117172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.048557364110446470106818850354102323763072490692138671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1366814589127897938691802437460864894092082977294921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1073541085957394891625682475932990200817584991455078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{15662}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08877938939258454842384793437304324470460414886474609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.087078392505645696441973768742172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00898611873298792163122783449580310843884944915771484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{146760599}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{115270596.37748344242572784423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{15662}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{95326143.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{93499712}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9648771.51903901994228363037109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.27951812744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.801418986541545308455170015804469585418701171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22545}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.205653667449951171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.93181514739990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.594245364275689524902190896682441234588623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.96688741721854309929540249868296086788177490234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999761164188385009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{28090}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9880319727177651056848617372452281415462493896484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{16197}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94970695674419414178402121251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.939884841442108154296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0100372173288052167483552779003730393014848232269287109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.722552672687992281197466581943444907665252685546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3937710}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3937710}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3937710}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3937710}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{15}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{8745}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.913771821053523058964174197171814739704132080078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.71637924812454134571026997946319170296192169189453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.62718053425650577281658115680329501628875732421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{16284}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.45001690891474332989474760324810631573200225830078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.43763203212341561521014909885707311332225799560546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.048471138817725099856570381007259129546582698822021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.66625022888184304292735760100185871124267578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.63358291411241651758246007375419139862060546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22545}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.6851856708526611328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.6378672122955322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.717650264437974971798439582926221191883087158203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2824680805206298828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{4305}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.214060672861061451754949302994646131992340087890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{13293}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.135888040065765380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1263964176177978515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0306339611703948244691986246834858320653438568115234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.734355218708515167236328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.634249167473653674420575043768621981143951416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{31308}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.45606109243817627429962158203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.423152363859116975586260878117172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.048326406593793218291477131742794881574809551239013671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1282573323696850897679411218632594682276248931884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{5615}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.09987523552301698359645598657152731902897357940673828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0830043344758450707399077828085864894092082977294921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07867117691785090183298478905271622352302074432373046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0087135196388685130786111443512709229253232479095458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{137715262}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{5615}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{107240217.56291390955448150634765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{89125225.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{84472533}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9356070.47049850039184093475341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.0167236328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.06559399105855145961641028407029807567596435546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1412}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.94751203060150146484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.535209767337012198851198263582773506641387939453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.65562913907284769976513416622765362262725830078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99987816810607921258480246251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98635654496830815762820066083804704248905181884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.960300981998443603515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94997268915176402703792746251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00966914695162584929277738154951293836347758769989013671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.755083062979561514538318078848533332347869873046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3179500}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3179500}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3179500}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{3179500}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.76821192052980080688939779065549373626708984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{2743}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{2743}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.06970608988360549318485936964862048625946044921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.734648697133133854464404066675342619419097900390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.63485007750600341847047047849628143012523651123046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{31308}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.45630305222847045154566103519755415618419647216796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.42338838669837908224025113668176345527172088623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.048286698747862170921774094267675536684691905975341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7349450588226318359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.6421915426949027505543199367821216583251953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{2549}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.5828249454498291015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.5358784198760986328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7396014646590296504058414939208887517452239990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3629238605499267578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{4729}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.217490595697567012933859587064944207668304443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{8721}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.146473705768585205078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1314156055450439453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.03246377478013830197856037784731597639620304107666015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.403285858221352100372314453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.32420634816937299316208509480929933488368988037109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{12493}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.22149550891481339931488037109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.214540841989219188690185546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03470359920569325573591612510426784865558147430419921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.399409448727965299408282362492172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.3450751595001742000334843396558426320552825927734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12493}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.306870394153520409386004530460922978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.304679031483829021453857421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.016625015193371971145008814119137241505086421966552734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{428862630}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{370521631.1788079738616943359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12493}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{329499576.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{327146619}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17850974.137758933007717132568359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.185821533203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.6145395948397407437369110994040966033935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.5718860626220703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{77.82788848876953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.51010078068381492499838714138604700565338134765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{58}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{33.6092715231788048413363867439329624176025390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{6082}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{23.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{23}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{5.75432288976319483708721236325800418853759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2649196}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2649196}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2649196}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2649196}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{31}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.629139072847682001565772225148975849151611328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{19451}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{19451}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.47535105287378964789013480185531079769134521484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.40351207412612011271590972683043219149112701416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.324518344965379734734511885108076967298984527587890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5358}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.221614036313992013305096406838856637477874755859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.214664245406277542915773892673314549028873443603515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03474048215801162076132868605782277882099151611328125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.73500013351439719144764239899814128875732421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.65066537793898504560274886898696422576904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.544130861759185791015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.526856899261474609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.73399851082651934586209563349257223308086395263671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3055884838104248046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{22286}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.215085089601428247618741806945763528347015380859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{22545}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.14007675647735595703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1324388980865478515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0310813719727746039234173025533891632221639156341552734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.718526526354253292083740234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.62694973977813062138153554769814945757389068603515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{5358}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.449957423843443338196124159367172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.440956623293459415435791015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.048607928251806022112990746109062456525862216949462890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.136639510281383991241455078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1074695441045409316505043761935667134821414947509765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{15662}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08882645890116687426019126405662973411381244659423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.087110711261630002777422987492172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0089821598211998789074161919643302098847925662994384765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{146715557}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{115394544.31125827133655548095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{15662}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{95376684}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{93534414}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9644520.66987466998398303985595703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.38015460968017578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.8657478844093162706485600210726261138916015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.17229998111724853515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.9324092864990234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6180041988517543938286280535976402461528778076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.97350993377483430180063805892132222652435302734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999761164188385009765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{28090}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98828828887434194694350253485026769340038299560546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{13468}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94941595196723949090511496251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{19004}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94018870592117320672542746251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.009677635215934309032004279060856788419187068939208984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.71823016351453439209961970846052281558513641357421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3946029}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3946029}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3946029}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3946029}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{15.125827814569536400313154445029795169830322265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{8745}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.847805326150330440526659003808163106441497802734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.719139912059980179748208684031851589679718017578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6275398639085045804364426658139564096927642822265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{32374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.450196353383331082653739940724335610866546630859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.4412025768626939292715860574389807879924774169921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.048523497547516496186670309498367714695632457733154296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.71249103546142578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.63131621973403895253795781172811985015869140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.76794683933258056640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4820387363433837890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7286282794607787938190313070663250982761383056640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.32289791107177734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{17080}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.214058891826907515820721528143621981143951416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.139473021030426025390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1391570568084716796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.030864178667526866173265176485074334777891635894775390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.735402739606797695159912109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.63420747542470101709710661452845670282840728759765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{7790}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.455896027386188451568926893742172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.423530392348766326904296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04830415812352951976382797738551744259893894195556640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1283436957746743878328032906210864894092082977294921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{5615}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.09998383976839823883420166339419665746390819549560546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08315714029595254463966824687304324470460414886474609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.078704641200601999084796034367172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0087298071837691726404528935745474882423877716064453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{137807994}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{5615}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{107356830.4834437072277069091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{13716}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{89289299.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{84508465}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9373559.0886686183512210845947265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.015990734100341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.07849087778306174101317083113826811313629150390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{5781}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.975169837474822998046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.8679935932159423828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.53139427036718023256156584466225467622280120849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.66225165562913890227036972646601498126983642578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99987816810607921258480246251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98644883585291986971554933916195295751094818115234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{23447}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96032708883285511358707253748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20976}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95007693767547596319644753748434595763683319091796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2345}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.009685805647876556678799175870153703726828098297119140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.7536877743288368236562746460549533367156982421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3204457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3204457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3204457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{3204457}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.74834437086092719937369110994040966033935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{2743}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{2743}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.112075483529206820776380482129752635955810546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7356966366636739085294038886786438524723052978515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29110}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.63480811242644408221025287275551818311214447021484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{17096}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.4561379043106186248479616551776416599750518798828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.423766626042002270136066499617299996316432952880859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1951}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.04826038161827465866604569555420312099158763885498046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7795393466949462890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.66707843344732964396825991570949554443359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{43.135441601276397705078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{1185}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.7525475025177001953125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7100517318843169167763562654727138578891754150390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.294235706329345703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{9504}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.21914776903114585593357332982122898101806640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{26829}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.1428306102752685546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.13717937469482421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0305958093772351370775997025930337258614599704742431640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.40814513899385929107666015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.324621213970101407664259340890566818416118621826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{22261}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.221825181273743454735125624210922978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2105841347947715880284391687382594682276248931884765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03464513520642469035504262819813448004424571990966796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.3989619314670562744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.344916512264518526631462691511842422187328338623046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.306485364912077729027117811710922978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.30375556834042072296142578125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.016597840997924918904349311787882470525801181793212890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{428382112}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{370351285.006622493267059326171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{15622}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{329086154.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{326155058}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17821796.067573882639408111572265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.12237548828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.439607481293336377348168753087520599365234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.6455821990966796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.29946136474609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.5064594809721061352547621936537325382232666015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{58}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{33.5496688741721840187892667017877101898193359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1283}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{23}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{23}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{5.7413208228610539407554824720136821269989013671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2661483}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2661483}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2661483}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2661483}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{31}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.69536423841059757933180662803351879119873046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{19451}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{19451}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.502960836050092563453972616116516292095184326171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.4083740806242486254262757938704453408718109130859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.324933426085140586447863597641116939485073089599609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22261}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.22198314963090981510873689330765046179294586181640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2107052623226166598868758228491060435771942138671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03468151150157332274215349343648995272815227508544921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.9079892635345458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.6690889415362022418776177801191806793212890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29565}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.810029685497283935546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{1185}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.486442089080810546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.721893728444265914134803097113035619258880615234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.30289745330810546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.216191024969745182460201249341480433940887451171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.132034480571746826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1266219615936279296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.032121151229600262977381675000287941657006740570068359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.40031538344919681549072265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.317898409792672309581718081972212530672550201416015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{22286}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.20721650333143770694732666015625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2029670886695384979248046875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0360462120086194881540819778820150531828403472900390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.400744490325450897216796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.348278515799501475758148671957314945757389068603515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.30992924072779715061187744140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.303770422935485784332598768742172978818416595458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0165074401756911230687574487774327280931174755096435546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{430296120}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{373961208.814569532871246337890625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{332783988.25}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18289}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{326171008}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{27300}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17724728.9238174594938755035400390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{142.3176116943359375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.2863692732046700939463335089385509490966796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{30684}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.6405811309814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.46202850341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.42529095414309292522148098214529454708099365234375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{59}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{34.6026490066225136388311511836946010589599609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{24}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{24}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{6532}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{5.85371277461275685283226266619749367237091064453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2675913}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2675913}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2675913}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2675913}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{31}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.668874172185429216597185586579144001007080078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{519}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20415}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.567555732816914737526303724735043942928314208984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.40084083461523445368612783568096347153186798095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7098}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3182045507768258563174867958878166973590850830078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22286}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.2073274195385068352504021049753646366298198699951171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2030838348893257150340474481708952225744724273681640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{2236}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03608699134383551443416848769629723392426967620849609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7065861225128173828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.652539382707203685640706680715084075927734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.660353720188140869140625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.3766391277313232421875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.73916731399697199744736053617089055478572845458984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.275061130523681640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{26932}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.214580112735167194415453195688314735889434814453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{11130}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.14894330501556396484375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{21317}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1473972797393798828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.02897911374089824632083178812536061741411685943603515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.656409184448421001434326171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{23367}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.5471605367847527379154826121521182358264923095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.39965101587586104869842529296875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.391731516458094120025634765625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04804710861791716691726605859003029763698577880859375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.274890602566301822662353515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1747929715853653032109349396705511026084423065185546875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{28090}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1374705934431403597795195992148364894092082977294921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{6159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.133535915054380893707275390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{23367}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0232011232475688618237530391752443392761051654815673828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{295161537}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{187682524.1324503421783447265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{28090}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{147607925.75}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{6159}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{143383097}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{23367}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{24912016.3946933932602405548095703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4290}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{41.54341888427734375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{17.3126035020840873812630889005959033966064453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{8048}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{10.696970462799072265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{10.537830352783203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27671}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{4.59898901089020117893824135535396635532379150390625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{18}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{123}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{8.26490066225165520563678001053631305694580078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{5928}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{6}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5928}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99716360205846121811390503353322856128215789794921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{27484}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98064251244068156854183371251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29195}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97915732860565196649105246251565404236316680908203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{13654}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00358299034442967866131990462008616304956376552581787109375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.8331097117460195544680345847154967486858367919921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5144079}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5144079}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5144079}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{5144079}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{23}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{17.675496688741720419102421146817505359649658203125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{742}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{10}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{10}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.233251627732641519941125807235948741436004638671875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.65663089116170414438755642549949698150157928466796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{23367}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.54767961487714134083404360353597439825534820556640625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{9134}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.399882522830667885838096253792173229157924652099609375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.3920271723783432804566473350860178470611572265625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.048023189396180936128200045232006232254207134246826171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7330095767974853515625}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7790}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.6415744759389099272084422409534454345703125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{26374}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.59192180633544921875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4376676082611083984375}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.71984128262006652487769997605937533080577850341796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.48164653778076171875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{7467}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.215125412340985366910217635449953377246856689453125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{19538}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.144901752471923828125}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{2.144378185272216796875}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUGlobalMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.03697916028633130292035957609186880290508270263671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.04820635169744490189369656718554324470460414886474609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.002301594149938073798067339481576709658838808536529541015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{24262}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0072070691415380867816953269766599987633526325225830078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.111094504594802800934161268742172978818416595458984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.07536661156163305952393471898176358081400394439697265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.026641849428415249889656735149401356466114521026611328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.02276856359094379944618680156054324470460414886474609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.016825986196959082097368565200667944736778736114501953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{119286816}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{80924282.966887414455413818359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{28606468}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{24447559}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18066765.1097216717898845672607421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{5.90728476821192050039144305628724396228790283203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99883711338043201788394753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9878318700569355126361870134132914245128631591796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29565}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.960227787494659423828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{2345}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95990699529647838250667746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0079222531612721802662946402051602490246295928955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.74895948464222172891169293507118709385395050048828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2648206}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2648206}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2648206}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{2648206}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{22545}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{11.0463576158940401938934883219189941883087158203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1696}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{1696}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.5455029758204326117976279419963248074054718017578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0482290015440977881677753202893654815852642059326171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0023038772000405966823566306089787758537568151950836181640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24262}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.007212313899378972915921170994124622666276991367340087890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.531283855438232421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.401751942981945830979384481906890869140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.272447884082794189453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.1116964817047119140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.73804990275916770858799509369418956339359283447265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3005874156951904296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{4647}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.199790927748016766685168477124534547328948974609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{3284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.12406885623931884765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{20539}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.121585845947265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.032671750081758578476698318127091624774038791656494140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0473185107111930014500700281132594682276248931884765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.002368341008855003038124920067275525070726871490478515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{24566}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00716964268640666278764594920858144178055226802825927734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.115334573201835099975909315617172978818416595458984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.0785054376052803093433141157220234163105487823486328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{14929}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0292757386341690496733836113207871676422655582427978515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.023667815141379798526966027338858111761510372161865234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.017567920504981300588998038847421412356197834014892578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{123839555}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{84294571.76821191608905792236328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{14929}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{31434585}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{25413123}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18863411.006905622780323028564453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.4248905181884765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.426777032826910041052315136766992509365081787109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24173}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.4322891533374786376953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{23367}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.40823304653167724609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.6229550865539874582310631012660451233386993408203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.14569536423841089600728082587011158466339111328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99798470735549915655582253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98859539410925856284251267425133846700191497802734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{10248}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96078856289386749267578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.954876124858856201171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00743300698395357208048128683230970636941492557525634765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.74936927999023239532760953807155601680278778076171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3881007}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3881007}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3881007}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{3881007}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{22545}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{11.1920529801324502017223494476638734340667724609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1696}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{1696}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.5893487849138125955761324803461320698261260986328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.047340743404058416299307054941891692578792572021484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.002371075801695988506667678308303948142565786838531494140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24566}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.007175830097479512538483081840468003065325319766998291015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.5754642486572265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.38938373919354063446007785387337207794189453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24144}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.346188127994537353515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20013}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.2571561336517333984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.74226712619275347915248630670248530805110931396484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.266102313995361328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{13468}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.202569426290246656918725420837290585041046142578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{23241}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.130356252193450927734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24144}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1256382465362548828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0311998854942860982808472414262723759748041629791259765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.047297030687332097809161268742172978818416595458984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0026522475411954959077787119525737580261193215847015380859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{22401}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004516914486885071462525740042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00784596880127065750276660338613510248251259326934814453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.127750900574028491973876953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.0881170107064065122326468326718895696103572845458984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{27671}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.032103409990668275997283132028314867056906223297119140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0260873129591344989075540894418736570514738559722900390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0197075762632614413794041041683158255182206630706787109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{137171485}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{94614919.80132450163364410400390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{27671}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{34470774}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{28011039}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{21160848.8835334442555904388427734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.27951812744140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.801418986541545308455170015804469585418701171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22545}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.205653667449951171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.93181514739990234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.594245364275689524902190896682441234588623046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{7.04635761589403930571506862179376184940338134765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99202346762284532299958073053858242928981781005859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29110}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95076431334018707275390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{30463}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94432204961776722296207253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00737494418079066328675086339217159547843039035797119140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.8790252604645176770503667285083793103694915771484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3624975}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3624975}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3624975}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3624975}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{16}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{27584}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{11.622516556291390799060536664910614490509033203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{9}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.42234635853338264865897144773043692111968994140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.047319253287767169824373780784299015067517757415771484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0026565090976331542059474255523809915757738053798675537109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22401}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000452601267940656378863114954989865790224712327471934258937835693359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{16284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00785789067237745685046146348895490518771111965179443359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.26540660858154296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.42962689904977224841786664910614490509033203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{11124}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.356202542781829833984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.1722164154052734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7074175543674190436149729066528379917144775390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.267423152923583984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{27484}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.199660342260701728633875973173417150974273681640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{2773}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.139698207378387451171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1376087665557861328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0284487565685103867274552413846322451718151569366455078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0473185107111930014500700281132594682276248931884765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.002622015132809304462091493093112148926593363285064697265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{21598}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004516914486885071462525740042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00781097130843930002874753171226984704844653606414794921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.12418925482779739899452664531054324470460414886474609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.08436410390580721674336217574818874709308147430419921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{27671}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.031485377345234120960437707026358111761510372161865234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0250314557924866017135645535063304123468697071075439453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.018964436035646771439022728600320988334715366363525390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{133347197}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{90585266.80794702470302581787109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{27671}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{33807166.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{26877321}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20362908.1400466859340667724609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.0167236328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.06559399105855145961641028407029807567596435546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.94751203060150146484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.535209767337012198851198263582773506641387939453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.64238410596026529475466304575093090534210205078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99958401918411243780582253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99059501823210560633725663137738592922687530517578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94766505062580108642578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94575321674346923828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00826613809840550002594472545069947955198585987091064453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.86387676074809693904654750440386123955249786376953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2866765}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2866765}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2866765}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{2866765}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{16}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{27714}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{11.4105960264900669898224805365316569805145263671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{8.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{17080}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.41548448719657304906149875023402273654937744140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.047340743404058416299307054941891692578792572021484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0026262537360829175427101578321753549971617758274078369140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{21598}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000452601267940656378863114954989865790224712327471934258937835693359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{16284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00782295618579812064574685592788227950222790241241455078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.352429866790771484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.42487621149479792848069337196648120880126953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{2549}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.31057786941527609769764239899814128875732421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.007546901702880859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7132321280217868153528115726658143103122711181640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2706298828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.203194315070347908402936809579841792583465576171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{29110}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.13749372959136962890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.137235164642333984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{20976}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0295791055701980394598837875719254952855408191680908203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.01552377175539730071174293613012196146883070468902587890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{28090}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0008760005642740064692175483429537052870728075504302978515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{4729}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.002686681382778672265432273746910141198895871639251708984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.337717495858669281005859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.2242821192134492325198635853666928596794605255126953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08868279191665347227502280702537973411381244659423828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0818215496838091971287809656132594682276248931884765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.04956359949264159403536922354760463349521160125732421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{362621400}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{240821091.7748344242572784423828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{95222422.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{87855220}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{53218509.723234452307224273681640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.185821533203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.6145395948397407437369110994040966033935546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.5718860626220703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{77.82788848876953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.51010078068381492499838714138604700565338134765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{61}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{40.980132450331126392484293319284915924072265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{21.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{21}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{7.6664489639960589073552910122089087963104248046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2336461}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2336461}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2336461}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2336461}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{32}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{3175}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{22.139072847682118805323625565506517887115478515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{1185}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.37116666798046171749092536629177629947662353515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.015768393168987628050192739692647592164576053619384765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{28090}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000878301192639353747564079366583200680906884372234344482421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{4729}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0026974751362965096283808019705929837073199450969696044921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.3736917972564697265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.41776622210117153599640005268156528472900390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5358}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.46781218051910400390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.233361721038818359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.6931705805082926108440233292640186846256256103515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3054943084716796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{13468}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.204339306875569892696375973173417150974273681640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{9816}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.140231847763061079348290149937383830547332763671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{21598}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.13930988311767578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.029430069101767049322138092293243971653282642364501953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.047297030687332097809161268742172978818416595458984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0026494467088224739857726941494320271885953843593597412109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{21598}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004516914486885071462525740042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00784007684612165849091791614000612753443419933319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.127843276597559396545733534367172978818416595458984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.088139904299072424631589228738448582589626312255859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{27671}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0321632288396358212434478218710864894092082977294921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.026201457716524600982666015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0197196468938072820564766374218379496596753597259521484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{137270673}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{94639501.609271526336669921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{27671}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{34535004}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{28133601}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{21173809.624392569065093994140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.38015460968017578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.8657478844093162706485600210726261138916015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.17229998111724853515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.9324092864990234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6180041988517543938286280535976402461528778076171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2236}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{7.0596026490066225989039594423957169055938720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99202940716648735364202593700611032545566558837890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{28778}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9505663216114044189453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{30463}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.943529903888702392578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00743479002385217212223178506746990024112164974212646484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.88573528462519135473485221154987812042236328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3633294}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3633294}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3633294}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3633294}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{16}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{27714}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{11.622516556291390799060536664910614490509033203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{9}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.42699481314605947090967674739658832550048828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.047319253287767169824373780784299015067517757415771484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0026537044314146741690041420014267714577727019786834716796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{21598}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000452601267940656378863114954989865790224712327471934258937835693359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{16284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0078520033989117853090444754116106196306645870208740234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.25177669525146484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.397777977368690471848822198808193206787109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{32103}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.303643703460693359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.15496921539306640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.715495324765759388441210830933414399623870849609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.30069637298583984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{30899}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.201888916508251359260839308262802660465240478515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{2345}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.136946260929107666015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{20976}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1302444934844970703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{20539}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.03023837030369806722074343952044728212058544158935546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0473185107111930014500700281132594682276248931884765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0026210557101972718242743898287017145776189863681793212890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{21598}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004516914486885071462525740042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.007815221611724022798828315217178897000849246978759765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.12421219516545529970574790468162973411381244659423828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.0844212006839201445362874665079289115965366363525390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{27671}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0315056000836193283998198921835864894092082977294921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.02503212075680490145135337343162973411381244659423828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.018979464115686302261298834537228685803711414337158203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{133371829}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{90646574.0066225230693817138671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{27671}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{33828880.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{26878035}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{20379044.418119557201862335205078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.015990734100341796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.07849087778306174101317083113826811313629150390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{5781}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.975169837474822998046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.8679935932159423828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.53139427036718023256156584466225467622280120849609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.64900662251655649725989860598929226398468017578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99958401918411243780582253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9906156363076721316218709034728817641735076904296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94766505062580108642578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94575321674346923828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0082906079343064049969047601962301996536552906036376953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.87040125858681960391294296641717664897441864013671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2891722}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2891722}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2891722}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{2891722}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{16}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{27714}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{11.403973509933774010960405576042830944061279296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{8.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{17080}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.4150506412065511074871437813271768391132354736328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.047340743404058416299307054941891692578792572021484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7238}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.002625289171642937978423670841721104807220399379730224609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{21598}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000452601267940656378863114954989865790224712327471934258937835693359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{16284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.007827202927859551462308473901430261321365833282470703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.416004657745361328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.41524648508488581910569337196648120880126953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{30371}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.347027301788330078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.29995059967041015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.723889285158295425759433783241547644138336181640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2770760059356689453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{30899}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.202822664715596179263457088381983339786529541015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.13061130046844482421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{20754}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1304371356964111328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24202}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0310556443409327510851714038153659203089773654937744140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0156398750841616994422533792885587899945676326751708984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{28090}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000885241516921291514419234403021619073115289211273193359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{4729}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0027000066796613771125112890558739309199154376983642578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.337715812958776895325030409367172978818416595458984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.2242033723803446843003683852657559327781200408935546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08873459254391487249780112733787973411381244659423828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08181560039520259508538657655662973411381244659423828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.04957498394583530199053456044566701166331768035888671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{362619593}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{240736538.0066225230693817138671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{95278043.25}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{87848832}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{53230733.6867718994617462158203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.12237548828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.439607481293336377348168753087520599365234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.6455821990966796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.29946136474609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.5064594809721061352547621936537325382232666015625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{60}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{40.913907284768214367431937716901302337646484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1490}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{21.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{21}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{7.64782823984076376433449695468880236148834228515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2348748}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2348748}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2348748}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2348748}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{32}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{3175}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{22.105960264900662792797447764314711093902587890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{1185}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.42014351947185968327858063275925815105438232421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0158863260376893820902122200777739635668694972991943359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{28090}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.000887541487772549827529877664034074769006110727787017822265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{4729}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00271080052452470250667904139163510990329086780548095703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.3943817615509033203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.40728953500457265590739552862942218780517578125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{2345}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.448308408260345458984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.08597469329833984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.73331951903919423418898304589674808084964752197265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.296092987060546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20475947777956537976251638610847294330596923828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{2743}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.135837554931640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{20754}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1331031322479248046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{20976}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.032700694796617801873850339688942767679691314697265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.017322897911071701015917057020487845875322818756103515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{28090}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.000905837438112448711802215939314919523894786834716796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{20976}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00279630262462372998488735476030342397280037403106689453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.340444498695433084289874159367172978818416595458984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.2262855150138601556530915104303858242928981781005859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0895895464345812519990630562460864894092082977294921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08173439837992189926918484843554324470460414886474609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.050168837717936100306648228297490277327597141265869140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{365549497}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{242972221.6357615888118743896484375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{4305}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{96196043}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{87761642}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{53868379.3192166984081268310546875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{142.3176116943359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.2863692732046700939463335089385509490966796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{30684}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.6405811309814453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.46202850341796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.42529095414309292522148098214529454708099365234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{62}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{7790}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{42.01324503311258240501047112047672271728515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{21.75}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{21}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{7.8756786777599696591778410947881639003753662109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2363178}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2363178}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2363178}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2363178}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{32}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{3175}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{22.397350993377482808455170015804469585418701171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{1185}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{1412}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.443160934544667650669680369901470839977264404296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0175958697017715957888750466509009129367768764495849609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{28090}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0009083267528807860251294226117124708252958953380584716796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{20976}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0028088420675911169276106615910748587339185178279876708984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.5463263988494873046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.42088547131873355056086438708007335662841796875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{123}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.320855677127838134765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.2887308597564697265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7466369762210385285783331710263155400753021240234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.30083179473876953125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.204091607340124436831274579162709414958953857421875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{2773}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.124331474304199662839209850062616169452667236328125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24202}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1170752048492431640625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{20976}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.03168856659389794605541368355261511169373989105224609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.05057890154421319783839550154880271293222904205322265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{28090}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.002147813253598091463858477112580658285878598690032958984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{19917}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004516914486885071462525740042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.00751367922752967619393071885269819176755845546722412109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2164433244615792950593657906210864894092082977294921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1272131289410965704345102267325273714959621429443359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{13716}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.04808687511831515049021135155271622352302074432373046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.034658225253224296535936588270487845875322818756103515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.03070176404372411405052645250179921276867389678955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{232404250}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{136594057.1059602797031402587890625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{13716}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{51632889}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{37213986}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{32965768.124325938522815704345703125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{41.54341888427734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{123}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{17.3126035020840873812630889005959033966064453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{8048}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{10.696970462799072265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{10.537830352783203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27671}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{4.59898901089020117893824135535396635532379150390625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{25}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{123}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{11.72847682119205359185798442922532558441162109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{8299}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2306}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99859607732848620909038572790450416505336761474609375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4810}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98053999245166778564453125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{4430}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96610224246978759765625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0035730607584006659170616782006391076720319688320159912109375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.631781746910261343685988322249613702297210693359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{4831344}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{4831344}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{4831344}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{4831344}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{24}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{7467}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.01324503311258240501047112047672271728515625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{10}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{1696}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{10}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{1696}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.263990367397216374456547782756388187408447265625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.051375916766321812201301355571558815427124500274658203125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{28090}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00215442073277194619251861951170212705619633197784423828125}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{19917}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000452601267940656378863114954989865790224712327471934258937835693359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{16284}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.007551163054605107387284856912401664885692298412322998046875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.466024875640869140625}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.44125568471996956532166223041713237762451171875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15043}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.6852262020111083984375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20415}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.383901119232177734375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.704036984358051398658062680624425411224365234375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.6413619518280029296875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{7467}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20494150483845086085921138874255120754241943359375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.131039559841156005859375}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1233196258544921875}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{24144}
\def\SubcubicEUPUMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.04602943641394223461826840093635837547481060028076171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.13738466240465641021728515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.03423211754404546780516938042637775652110576629638671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{27584}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00006040395237505435943603515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{17096}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000049360096454620361328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.028925705781035489227992485439244774170219898223876953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.11829923745244740052040555156054324470460414886474609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.09177856580878522574362676778036984615027904510498046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{30371}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.047323328908532795444852325772444601170718669891357421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.043265732005238498325550011713858111761510372161865234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0140246093328673000766304568287523579783737659454345703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{127022839}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{98546484.65562914311885833740234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{30371}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{50813037.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{46456226}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{15058809.6059603579342365264892578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10306}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.006622516556291202505235560238361358642578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99863708019256602899105246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98862672207371293797706357509014196693897247314453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{13654}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.969218790531158447265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{1895}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96637171506881724969417746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2345}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00626360207568702788416548088434865348972380161285400390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.70473036261843857719355810331762768328189849853515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2696590}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2696590}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2696590}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{2696590}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{27584}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{11.4437086092715230023486583377234637737274169921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{6155}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{6155}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.8862898922158144454641615084256045520305633544921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.1375207004050702230824043681423063389956951141357421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.03426407889583470145478116819504066370427608489990234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{27584}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000060435098786941029622675480847959761376841925084590911865234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{17096}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000049435165283351428827768553157795405894603391061536967754364013671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0289505879364701755596112064949920750223100185394287109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.628111362457275390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.70758927263171500499083776958286762237548828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{32382}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.534511089324951171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.3251478672027587890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7227898068316773727559620965621434152126312255859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.303594112396239790285790149937383830547332763671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{27300}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.2081976821091000573460405576042830944061279296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.14105987548828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24144}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.13433074951171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.031501528802705812404294505313373520039021968841552734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.150259622372686807434405409367172978818416595458984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.03361511588195296995618122082305490039288997650146484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{12457}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00010806368663901518944840673963625476972083561122417449951171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{8840}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000276602804660797119140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.028562239828535958274802197820463334210216999053955078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.123505403287708703796710096867172978818416595458984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.09609529006584782706568148569203913211822509765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29022}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0491512881126254519426055367148364894092082977294921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0465688342228531004796110437382594682276248931884765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01472927406182862435091163177958151209168136119842529296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{132612917}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{103181532.033112585544586181640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29022}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{52775793.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{50002905}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{15815437.59734375588595867156982421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.4248905181884765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.426777032826910041052315136766992509365081787109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24173}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.4322891533374786376953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{23367}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.40823304653167724609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.6229550865539874582310631012660451233386993408203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.2980132450331129945197972119785845279693603515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.998811781406402587890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{25516}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99018170225699220221571295041940174996852874755859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{913}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96954350173473347052066628748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{1951}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95997941493988037109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2345}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0059817441212493271951444739897851832211017608642578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.7260042324394075929916425593546591699123382568359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3929391}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3929391}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3929391}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{3929391}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{27584}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{11.615894039735099596555301104672253131866455078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{8.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{19451}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.86590505764271430422240882762707769870758056640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.15040840913106823251155219622887670993804931640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.033647726481706545509364758572701248340308666229248046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{12457}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00010812175975285085913722704642481176051660440862178802490234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8840}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000027702347338029007980185589206378882209946823422797024250030517578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0285875206398183666356427323762545711360871791839599609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.545078277587890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.71221744619457894032166223041713237762451171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{123}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.9136440753936767578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20415}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.5083472728729248046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.70785621577931168157959973541437648236751556396484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3055384159088134765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{12141}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.210714411261855527612851801677606999874114990234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{18146}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.139162600040435791015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.136139392852783203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.031918883370041901959002217381566879339516162872314453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.131403861567377988617266737492172978818416595458984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.031856660706465957100252950340291135944426059722900390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{30684}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0005419605877250151075574802206347158062271773815155029296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000276602804660797119140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.027495773664860036211710081488490686751902103424072265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1393900932744145115815825874960864894092082977294921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.108585868154140452457312449041637592017650604248046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{28778}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.05640374985523517736840659608787973411381244659423828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.054555445909500101253630788278314867056906223297119140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01665249621640342569950377082932391203939914703369140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{149668973}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{116593188.13245032727718353271484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{28778}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{60563065.25}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{58578464}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17880481.661554105579853057861328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.27951812744140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.801418986541545308455170015804469585418701171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22545}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.205653667449951171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.93181514739990234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.594245364275689524902190896682441234588623046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{10}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{7.125827814569536400313154445029795169830322265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99993425607681285516292746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9927579839498001934572357640718109905719757080078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{2743}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97616931796073924676448996251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96776103973388682977230246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0047193639159830054474742411230181460268795490264892578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.791550040768692841908205082290805876255035400390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3673359}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3673359}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3673359}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3673359}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{3284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{12.1986754966887414042275850079022347927093505859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{9}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{2743}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{2743}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.0263818522810286282265224144794046878814697265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.1315339773915274734772395959225832484662532806396484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0318941922822195689235513782477937638759613037109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{30684}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000542161113749147567826558447023899134364910423755645751953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000027702347338029007980185589206378882209946823422797024250030517578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0275372368722023690146283314561514998786151409149169921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6842620372772216796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.71982017416038246437892667017877101898193359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.95053470134735107421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20415}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.64656352996826171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.69919058330860195393796630014549009501934051513671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.271291255950927734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.210167742722871420113506246707402169704437255859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.144941747188568115234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24202}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1445367336273193359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.03008782563169067059138939157492131926119327545166015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.142116294242441598694171034367172978818416595458984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.03262067492434515825205920691587380133569240570068359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{30684}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00006097345612943172454833984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{4647}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000276602804660797119140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0282236173818713360905707787651408580131828784942626953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.13326989300549030303955078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10358287088128899366967772266434621997177600860595703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{20751}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0534906352404504736863799507773364894092082977294921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.051987076178193002140570655456031090579926967620849609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.016072552667129390291389512412933981977403163909912109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{143097458}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{111221260.71523179113864898681640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{20751}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{57435132.25}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{55820698}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17257772.017139576375484466552734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.0167236328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.06559399105855145961641028407029807567596435546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1412}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.94751203060150146484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.535209767337012198851198263582773506641387939453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{10}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.8013245033112585957724149920977652072906494140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{18289}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99993425607681285516292746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9920047600537735821291107640718109905719757080078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9762557446956634521484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11611}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97041523456573475225894753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005122422913742798178393655916806892491877079010009765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.780727013450948970074705357546918094158172607421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2915149}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2915149}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2915149}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{2915149}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{3284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{11.874172185430463599686845554970204830169677734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{9}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{2743}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{2743}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.9943783102822703057199760223738849163055419921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.1422570174946341803323690555771463550627231597900390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.032656604685820635192161631721319281496107578277587890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{30684}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00006100740959504819351834348228891258258954621851444244384765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{4647}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000027702347338029007980185589206378882209946823422797024250030517578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0282571081486331643350951026150141842663288116455078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6397259235382080078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.73008767500618176882198895327746868133544921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24202}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.7776248455047607421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4678232669830322265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.71623648934183481440385321548092179000377655029296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2723090648651123046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{30899}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.21253284081717982445525194634683430194854736328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{13293}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.141146957874298095703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.137442111968994140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{23696}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0290635808590162976472459632759637315757572650909423828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.066062272526323795318603515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0126730157432472755052454971291808760724961757659912109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004912726581096649169921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000484287738800048828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0132487133007464265299635286510238074697554111480712890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.366168075241148416321124159367172978818416595458984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.279539768676588085138945416474598459899425506591796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{21598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1610117896925657710038848335898364894092082977294921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.15889693982899188995361328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.043261566083853293662730976620878209359943866729736328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{393169977}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{300153541.099337756633758544921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{21598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{172885092.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{170614290}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{46451752.875973172485828399658203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.185821533203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.6145395948397407437369110994040966033935546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.5718860626220703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{77.82788848876953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.51010078068381492499838714138604700565338134765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{71}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{42.96026490066225278496858663856983184814453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{13716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{31.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{31}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{7.09713195939267738054923029267229139804840087890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2384845}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2384845}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2384845}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2384845}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{31}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{3254}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.423841059602647618476112256757915019989013671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{16.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{16}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{1412}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.495384063242891414802215876989066600799560546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.066148985402134263811291248202905990183353424072265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0126913749327942394773405254682074883021414279937744140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24438}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000049189887342117791380402612270994477938756972434930503368377685546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000004845405351841687242085988918637029509994817999540828168392181396484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.01328032854143910111710535915108266635797917842864990234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{52.45428371429443359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.76666587393805230021825991570949554443359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{4729}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.618787229061126708984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.5598800182342529296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.953575744568861072281151791685260832309722900390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2769114971160888671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{26374}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.211318917621839741372014032094739377498626708984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.136954724788665771484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24202}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.133327484130859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24173}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0292700584010079679908589156411835574544966220855712890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.131403884850442409515380859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.031876582214423708483419517278889543376863002777099609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{6589}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0005419605877250151075574802206347158062271773815155029296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000276602804660797119140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.02754126977576894230725912393609178252518177032470703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1393409697338937880406461999882594682276248931884765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.108637229965025172706560852020629681646823883056640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{28778}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0561651755124330243074126656210864894092082977294921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0545557886362074972996794031132594682276248931884765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01668197384227802781975213974874350242316722869873046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{149616227}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{116648337.45695364475250244140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{28778}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{60306898}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{58578832}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17912133.02132789790630340576171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.38015460968017578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.8657478844093162706485600210726261138916015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.17229998111724853515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.9324092864990234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6180041988517543938286280535976402461528778076171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{10}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{7.139072847682118805323625565506517887115478515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99993425607681285516292746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9929082393646240234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{27671}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97625792026519775390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{1185}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96776103973388682977230246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.004724775150580908487929487904466441250406205654144287109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.79767655231330059084626782350824214518070220947265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3681678}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3681678}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3681678}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3681678}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{3284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{12.1986754966887414042275850079022347927093505859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{9}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{2743}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{2743}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.0361626925645310848267399705946445465087890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.1315340006976467301935684872660203836858272552490234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.031913904854181274206581520047620870172977447509765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6589}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000542161113749147567826558447023899134364910423755645751953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000027702347338029007980185589206378882209946823422797024250030517578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.02758192932262286400924011786628398112952709197998046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.852759838104248046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{14095}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.70457476022227893963645328767597675323486328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{28090}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.7289927005767822265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.3387520313262939453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.74094592744219001101413368814974091947078704833984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3377268314361572265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{16069}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.212268804082807349686845554970204830169677734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{23447}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.1434099674224853515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24202}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.141446590423583984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.03157708154942763523198578923256718553602695465087890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.142116294242441598694171034367172978818416595458984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.032545830721393276263597726938314735889434814453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{7884}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00006097345612943172454833984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{4647}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000276602804660797119140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0282323170060215476728782135751316673122346401214599609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1333261914551258087158203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10365128576360786716303863386201555840671062469482421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{20751}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.053540000924840548679473073434564867056906223297119140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.05198737978935240311439969218554324470460414886474609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0160933691972278379578309426278792670927941799163818359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{143157908}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{111294720.6357615888118743896484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{20751}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{57488138.25}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{55821024}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17280123.5961368344724178314208984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.015990734100341796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.07849087778306174101317083113826811313629150390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{5781}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.975169837474822998046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.8679935932159423828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.53139427036718023256156584466225467622280120849609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{10}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.8013245033112585957724149920977652072906494140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{123}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{18289}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99993425607681285516292746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99199419976859692926751677077845670282840728759765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9762557446956634521484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11611}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97041523456573475225894753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005128744990365081794780888202467394876293838024139404296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.780727013450948970074705357546918094158172607421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2940106}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2940106}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2940106}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{2940106}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{3284}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{11.887417218543046004697316675446927547454833984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{9}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{2743}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{2743}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.001797359122118979968263374757952988147735595703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.1422570174946341803323690555771463550627231597900390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.032581636710539839396627570522468886338174343109130859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{7884}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00006100740959504819351834348228891258258954621851444244384765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{4647}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000027702347338029007980185589206378882209946823422797024250030517578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.028265722248386838943989829431302496232092380523681640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.81108188629150390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.705675772483772334453533403575420379638671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{2743}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.518662750720977783203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4378912448883056640625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.74496122065106418208557670368463732302188873291015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.495005369186401811276709850062616169452667236328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{13036}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.216089899176793220902936809579841792583465576171875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.143166363239288330078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.141361236572265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0377937251747292590753346530618728138506412506103515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.0660137580707668980561919624960864894092082977294921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.01272169438912374404837546393309821723960340023040771484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{21317}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004912726581096649169921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0000000484287738800048828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.01320951651498433222775563677942045615054666996002197265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.365639646537601892273272596867172978818416595458984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.279371302420680478473258290250669233500957489013671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{21598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1609049118123948574066162109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.158879451453685704986895643742172978818416595458984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.043213316588009330343478353597674868069589138031005859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{392602581}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{299972651.834437072277069091796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{21598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{172770333.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{170595512}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{46399945.374298594892024993896484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.12237548828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.439607481293336377348168753087520599365234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.6455821990966796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.29946136474609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.5064594809721061352547621936537325382232666015625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{71}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{42.85430463576158643945746007375419139862060546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{6082}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{31.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{12287}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{31}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{7.0414076623543078170541775762103497982025146484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2397132}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2397132}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2397132}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2397132}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{31}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{3254}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.317880794701988378392343292944133281707763671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{16.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{16}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{1412}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.47435421781130582274954576860181987285614013671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0661004072668431030823654737105243839323520660400390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0127399978754209504405725539299965021200478076934814453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{21317}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000049189887342117791380402612270994477938756972434930503368377685546875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00000004845405351841687242085988918637029509994817999540828168392181396484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.01324047627060341049409775138201439403928816318511962890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7779295444488525390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.70886283205044975375130889005959033966064453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24202}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.472418129444122314453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4647643566131591796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.74722742229679095515848530340008437633514404296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3019611835479736328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{1490}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.212857486396436090814177077845670282840728759765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{12457}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.130890309810638427734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.130611896514892578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24144}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.03171528206810776684410058123830822296440601348876953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.06059896666556589817087541405271622352302074432373046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.01250003136398377713567331426247619674541056156158447265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{14095}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004749745130538941091431990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{10248}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004749745130538941091431990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{10248}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0127783038044621301276837499472094350494444370269775390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.36854401789605617523193359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.281947146139002791098704392425133846700191497802734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{21598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1610634594690054377519317085898364894092082977294921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{29726}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.158646604046225492279376112492172978818416595458984375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.04368417104137427287025019495558808557689189910888671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{395721126}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{6910}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{302738442.966887414455413818359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{21598}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{172940572.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{29726}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{170345494}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{46905521.49389319121837615966796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{142.3176116943359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.2863692732046700939463335089385509490966796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{30684}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.6405811309814453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.46202850341796875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.42529095414309292522148098214529454708099365234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{73}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{44.13245033112583115553206880576908588409423828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{7310}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{32}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{18289}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{32}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{7.3011615665620599457952266675420105457305908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2411562}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2411562}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2411562}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2411562}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{31}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{2236}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.79470198675496561691034003160893917083740234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{1895}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{16.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{2549}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{16}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{1412}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.5008378955316903358152558212168514728546142578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0606785084444022293492793096447712741792201995849609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.01251825569683205109650092623496675514616072177886962890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{14095}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0000000475554481159701414001307715091748651303760198061354458332061767578125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{10248}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000475222447969088646788931207427808534049518129904754459857940673828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{15399}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.01281002593215407360516255863558399141766130924224853515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7525675296783447265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{14095}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.72948267286187018498821998946368694305419921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24144}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.620452702045440673828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.506448268890380859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7167713411409246671013306695385836064815521240234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2961215972900390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{31308}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.213832507859792020354916530777700245380401611328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{9816}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.138250768184661865234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.12769985198974609375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24202}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0308771194550855575255976503967758617363870143890380859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.11117270961403839801828752342771622352302074432373046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.026258102661331716998205365598550997674465179443359375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000020582228899002080489268420339377119177015629247762262821197509765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.000000049360096454620361328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.02312497201645456745833229206255055032670497894287109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.243319834582507610321044921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{7467}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1574594884284382934058754699435667134821414947509765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29110}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08334129559807472442667375389646622352302074432373046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0750831505283713063203521187460864894092082977294921875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0277316717613420894716913522870527231134474277496337890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{261262683}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{7467}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{169070838.3112582862377166748046875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29110}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{89487034.75}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{80619919}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{29776655.8195927478373050689697265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6338}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{41.54341888427734375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{123}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{17.3126035020840873812630889005959033966064453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{8048}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{10.696970462799072265625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{10.537830352783203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27671}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{4.59898901089020117893824135535396635532379150390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{27}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{123}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{11.8211920529801322032881216728128492832183837890625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{8}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{8}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5615}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1283}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9991149164193513509957256246707402169704437255859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{16149}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99137520790100108758480246251565404236316680908203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6159}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99043142795562744140625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2773}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.001497430652844370692344799778084052377380430698394775390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.511130435173251296276930588646791875362396240234375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{4879728}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{4879728}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{4879728}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{4879728}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.615894039735099596555301104672253131866455078125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{519}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{11}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{5928}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{5928}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.22228605866138817503951941034756600856781005859375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.11131863413333849266440012115708668716251850128173828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0262892031005494651585419063621884561143815517425537109375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{15043}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.000000205912616437285241318484903250141115904625621624290943145751953125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{28716}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.000000049435165283351428827768553157795405894603391061536967754364013671875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{8299}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0231687535923237840351784910808419226668775081634521484375}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7269332408905029296875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.70866535988864853834456880576908588409423828125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{12141}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.60619318485260009765625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.567219257354736328125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20415}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7376257918704436367107746264082379639148712158203125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3068611621856689453125}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{1895}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20777135653211598054213027353398501873016357421875}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{23367}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.139087736606597900390625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{20976}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1327457427978515625}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicEUPUMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.031515968129765946359466255444203852675855159759521484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.56053528748452663421630859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.405474554334107228914518827878055162727832794189453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.240784759167581741134966932804672978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{32103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2337723206728695990452848718632594682276248931884765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{19093}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0729890875287603491106125375154078938066959381103515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.10646834410727019915032798280662973411381244659423828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.0795847116321916903114441765865194611251354217529296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{9816}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0651389432605355700456328804648364894092082977294921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{23633}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.060517837293446001545316192959944601170718669891357421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.008522748491027735961989009183525922708213329315185546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{114319514}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{85453433.4304635822772979736328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{9816}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{69942407.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{23633}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{64980533}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9151231.51024937070906162261962890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.9337748344370861985908049973659217357635498046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999912261962890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98442706288091397226480694371275603771209716796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4157}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95284430682659138067691628748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{17080}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94308298826217640264957253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{29195}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01271976098415150691067765365005470812320709228515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.5943316595015779579824766187812201678752899169921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2904302}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2904302}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2904302}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{2904302}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.4105960264900669898224805365316569805145263671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.566393927371203087517415042384527623653411865234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.56127104217343271042039987150928936898708343505859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.40587914475008002312961252755485475063323974609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{913}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.240892994135792959387032396989525295794010162353515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{32103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2338819846325828899491483525707735680043697357177734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{19093}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.073144720325669265736934221422416158020496368408203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.36328411102294921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7790}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.36540343271975217476210673339664936065673828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.272457540035247802734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.1888554096221923828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7428585309606117181857598552596755325794219970703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.322057723999022993410790149937383830547332763671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{7467}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.203137977233785793629294857964850962162017822265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.134069919586181640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.127391576766968217526709850062616169452667236328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0309829207832050292081849107717061997391283512115478515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.54539712332189083099365234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.399326233224116811104664748199866153299808502197265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{6549}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.222926429240032974998797499210922978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{19093}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2062617661431430937657438562382594682276248931884765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{32103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07521528079768258212567388909519650042057037353515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.112348807044327203552569471867172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.085557034078812710387040851855999790132045745849609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.07016936666332185268402099609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{23633}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.065527110360562801361083984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0085421950095080391440749423281886265613138675689697265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{120633613}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{91866165.82781456410884857177734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{75343783.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{23633}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{70359199}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9172112.050472863018512725830078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.4248905181884765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.426777032826910041052315136766992509365081787109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24173}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.4322891533374786376953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{23367}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.40823304653167724609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.6229550865539874582310631012660451233386993408203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.16556291390728450352298750658519566059112548828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99984395503997802734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98732211652970469639711836862261407077312469482421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{32374}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9512734115123748779296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.94689720869064319952457253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{20976}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0103574767115324241351093093044255510903894901275634765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.5688429475892029518746539906715042889118194580078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{4137103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{4137103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{4137103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{4137103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{19}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.5496688741721857951461061020381748676300048828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{17096}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.59058085414813188407379129785113036632537841796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.54611300776263804745980223742662928998470306396484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.399723587686238224225832027514115907251834869384765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6549}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.2230296709382719455572186006975243799388408660888671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{19093}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2063531871791343952349251367195392958819866180419921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{32103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.075360226029217936005721867331885732710361480712890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.3248779773712158203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7790}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.36656631697092478816557559184730052947998046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.253577649593353271484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.1480529308319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7309863466726682634799772131373174488544464111328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.271833896636962890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{13293}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20376646439760737195001638610847294330596923828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{6549}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.139335930347442626953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1258227825164794921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0284422157958497956453669530674233101308345794677734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.548801354132592678070068359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.384352352698364374550266120422747917473316192626953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{6549}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.2128063312266021689378447945273364894092082977294921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.20542580075562000274658203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{32103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.071288707263343631392871202479000203311443328857421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1335841389372943999180876062382594682276248931884765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10361016787193859378657379011201555840671062469482421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08586497534997759861763455546679324470460414886474609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.083623224869370404999102674992172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00892890046885170575452495000945418723858892917633056640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{143434877}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{111250570.6357615888118743896484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{92196815.25}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{89789754}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9587333.87573928572237491607666015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.27951812744140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.801418986541545308455170015804469585418701171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.205653667449951171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.93181514739990234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.594245364275689524902190896682441234588623046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.74172185430463599686845554970204830169677734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99996095895767200811832253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98751163877398762114268038203590549528598785400390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95246629416942596435546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95217621326446522100894753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00980039370869302539635015136809670366346836090087890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.74107114313759614443455348009592853486537933349609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3881071}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3881071}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3881071}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3881071}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{15.1721854304635765942066427669487893581390380859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{11598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{11598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.572811458318045918503003122168593108654022216796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.5490028835868321355206944645033217966556549072265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.384729547730272070094059699840727262198925018310546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6549}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.212974317586979378091882608714513480663299560546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2055168512681584680468205306169693358242511749267578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{32103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07140082575507304685213938455490279011428356170654296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.47438764572144265230235760100185871124267578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.3730936981984314115834422409534454345703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.330874979496002197265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.2859363555908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.72529548091774398432818315995973534882068634033203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2767124176025390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{4430}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.204405914079274442229916530777700245380401611328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.126919209957122802734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1238005161285400390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0301826194291080034115548613726787152700126171112060546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.5351390279829502105712890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.3893814573607203843863544534542597830295562744140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.229864005232229773323382460148422978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.220525545999407712738360487492172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{32103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0733502498307961603440929820862947963178157806396484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1260632053017615994416900093710864894092082977294921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.0961826752797262096716934820506139658391475677490234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{9816}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.07923224312253294987495877421679324470460414886474609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0746995788067578991853423531210864894092082977294921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0087112617865365386815579284984778496436774730682373046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{135359336}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{103275361.19205297529697418212890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{9816}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{85074973.25}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{80208062}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9353646.1200172416865825653076171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.0167236328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.06559399105855145961641028407029807567596435546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.94751203060150146484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.535209767337012198851198263582773506641387939453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.4900662251655631962421466596424579620361328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99991858005523681640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.987116581162080120037671804311685264110565185546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{28778}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9638271629810333251953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24262}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9599387645721435546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.008600541689012759782873018821192090399563312530517578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.68925095794742718968706185478367842733860015869140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3122861}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3122861}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3122861}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{3122861}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.887417218543046004697316675446927547454833984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{17096}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{17096}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.445547505317188896611924064927734434604644775390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.5353355403921116195675722337909974157810211181640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.38976761998018838450974499210133217275142669677734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.2300456125376248162073267167215817607939243316650390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2206232891451918032288403992424719035625457763671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{32103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07348817141052475798712606547269388101994991302490234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.5476396083831787109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7790}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.3761088516538535486688488163053989410400390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.336916267871856689453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.274672031402587890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.71794080916011981940982877858914434909820556640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2728521823883056640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.206753356567281887379294857964850962162017822265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{12493}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.131403863430023193359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1216261386871337890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.030010470244400906658643890523308073170483112335205078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.30508704297244548797607421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.1938812367198680386426445920733385719358921051025390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{12561}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0924748620018362721406646187460864894092082977294921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.09176504891365759586374650780271622352302074432373046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.042737278640221094960782721727809985168278217315673828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.3974152170121669769287109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.343330595124241522153596406496944837272167205810546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.304939581081271116058672987492172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.303124837577342987060546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0167674644624115527780094936360910651274025440216064453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{426721340}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{368648419.443708598613739013671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{327426382}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{325477816}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18003927.8757249601185321807861328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.185821533203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.6145395948397407437369110994040966033935546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.5718860626220703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{77.82788848876953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.51010078068381492499838714138604700565338134765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{57}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{33.099337748344368037578533403575420379638671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{23}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{23}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{5.71016865350656388500283355824649333953857421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2592557}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2592557}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2592557}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2592557}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{31}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.26490066225165520563678001053631305694580078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{913}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{19451}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{19451}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.541580013228375012346305084065534174442291259765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.30548749808633990365791532894945703446865081787109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1940774080995183725750763414907851256430149078369140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{12561}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0925551675370929471942105237758369185030460357666015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.09184759132748292198566986144214752130210399627685546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.042823043526113206691530166381198796443641185760498046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.454766750335693359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.37873907278704876944175339303910732269287109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.39905726909637451171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.3097822666168212890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7201261543961809952207886453834362328052520751953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2649166584014892578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{4305}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.206229481476032372455620134132914245128631591796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.13675296306610107421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1329653263092041015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.02879659924750231636547681546289823018014430999755859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.546752418391406536102294921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.3843853736098929996245487927808426320552825927734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.212161867646500412742938124210922978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2049768213182686926732145593632594682276248931884765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{32103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07195156623375846549617307346125016920268535614013671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.133568521589040700714434706242172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1037212989188187606259816675446927547454833984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{11130}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0860449059400706650624357507695094682276248931884765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.083700139075517598907794081242172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0089186217185346083891062107795733027160167694091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{143418108}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{111369896.68874172866344451904296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{11130}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{92390014.25}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{89872340}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9576297.1516253650188446044921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.38015460968017578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.8657478844093162706485600210726261138916015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.17229998111724853515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.9324092864990234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6180041988517543938286280535976402461528778076171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.74172185430463599686845554970204830169677734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99998056888580322265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98749937521700825726611583377234637737274169921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95231644809246052130191628748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.951882421970367431640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0097709725066206128130108510276841116137802600860595703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.74107114313759614443455348009592853486537933349609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3889390}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3889390}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3889390}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3889390}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{15.2119205298013238092380561283789575099945068359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{11598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{11598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.530893283976339613872141853789798915386199951171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.54695319544061160588199754784000106155872344970703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.384762799439542224622101684872177429497241973876953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.212322671260063489118152801893302239477634429931640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2050676728304491602816739259651512838900089263916015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{32103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.072064874150451430079300507713924162089824676513671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.48627614974976296480235760100185871124267578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.36745746088343622659522225148975849151611328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{26374}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.43661797046661376953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4251334667205810546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.73444695040493013227234087025863118469715118408203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.282061100006103515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{30684}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.204472631808148452847717635449953377246856689453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{23241}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.13024032115936279296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1298115253448486328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.030676487874559073276703458077463437803089618682861328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.5349362194538116455078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.389315720721585878383308454431244172155857086181640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.228680420899763647835101210148422978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.218627122230827808380126953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{32103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.07371733315072133418954791750365984626114368438720703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.12605695426464080810546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.09626728820534331820812923297125962562859058380126953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.079298642231151406090106092960922978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0747398752719163061986051843632594682276248931884765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0087234920031514125160487793664287892170250415802001953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{135352624}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{103366213.62913906574249267578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{85146268.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{80251330}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9366778.21511320583522319793701171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.015990734100341796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.07849087778306174101317083113826811313629150390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.975169837474822998046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.8679935932159423828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.53139427036718023256156584466225467622280120849609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.4900662251655631962421466596424579620361328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99991858005523681640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98701317934010990295945475736516527831554412841796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{28778}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96355439722537994384765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{24262}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95978289842605601922542746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.008616223102470420280862839490509941242635250091552734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.68925095794742718968706185478367842733860015869140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3147818}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3147818}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3147818}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{3147818}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.8410596026490058108038283535279333591461181640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{17096}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{17096}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.497926862888816490482213339419104158878326416015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.535132657388134536091683912673033773899078369140625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.38970179130193549621452575593139044940471649169921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.2288611801222619757112397564924322068691253662109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.21872402394161927219329299987293779850006103515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{32103}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.07385445116195045456297663122313679195940494537353515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.449070453643798828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7790}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.3880931841616614974554977379739284515380859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{29726}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.38755095005035400390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.33265399932861328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.74235897730584243792151255547651089727878570556640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.29518222808837890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20727632693107533867760139401070773601531982421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.1367876529693603515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{21317}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1241676807403564453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0304200039569911991066408774031515349633991718292236328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.316071425564587116241455078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.193127064059013531238662153555196709930896759033203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0934785483404993733369536812460864894092082977294921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0916993021965026022801481531132594682276248931884765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04252553097395879444508892675003153271973133087158203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.397499983198940698425616346867172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.343171798395893457023220207702252082526683807373046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.30474520171992480754852294921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.302539958618581295013427734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.016801355112317832574131415412921342067420482635498046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{426812357}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{368477912.754966914653778076171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{6082}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{327217668.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{324849807}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18040317.6839718781411647796630859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.12237548828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.439607481293336377348168753087520599365234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.6455821990966796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.29946136474609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.5064594809721061352547621936537325382232666015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{57}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{33.046357615894038417536648921668529510498046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{23}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{23}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{5.70620406914556355104650720022618770599365234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2604844}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2604844}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2604844}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2604844}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{31}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.23178807947019919311060220934450626373291015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{19451}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{19451}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.474890347719547634142145398072898387908935546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.316486298702069623889343574774102307856082916259765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1933226585926186569253104607923887670040130615234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.09355971450478013651252950921843876130878925323486328125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.09178178547133329645557608955641626380383968353271484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.042613782022367985291566583327949047088623046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.3678734302520751953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7790}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.3897815761187217731276177801191806793212890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.2904574871063232421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.2826626300811767578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7530948493945117672154765386949293315410614013671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2673680782318115234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{26932}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20632234472312660500392667017877101898193359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{18668}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.134566962718963623046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.131385326385498046875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0304005525149485776592594987732809386216104030609130859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.3102470748126506805419921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.1901202313972032709177284459656220860779285430908203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0909992225933819731675811226523364894092082977294921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0860172323882578970799528406132594682276248931884765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04290841503186022809490651752639678306877613067626953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.399610427208244800567626953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.34660556392485142307435808106674812734127044677734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{19488}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.307975045172497574608172499210922978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.302591647021472398559893690617172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0167898307049655394485032644524835632182657718658447265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{429078429}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{372164890.41721856594085693359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{19488}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{330685686.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{324905307}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{18027943.445800907909870147705078125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{142.3176116943359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.2863692732046700939463335089385509490966796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{30684}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.6405811309814453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.46202850341796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.42529095414309292522148098214529454708099365234375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{59}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{34.086092715231785632568062283098697662353515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{24}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{24}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{5.893020225837712899874532013200223445892333984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2619274}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2619274}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2619274}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2619274}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{31}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.649006622516555609081478905864059925079345703125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17.75}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{519}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20415}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.44732229802691048092810888192616403102874755859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.3106543029481658724222370437928475439548492431640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{7098}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1903133130420349983236150137599906884133815765380859375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{29565}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.09107820239468711331909389627980999648571014404296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.08609460465663189288054724102039472199976444244384765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{6589}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.042997131320743557647556798428922775201499462127685546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.4520599842071533203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.38363408410786092872513108886778354644775390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.34187972545623779296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.340331554412841796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.74239297623598188291538235716870985925197601318359375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2798230648040771484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.206052075948147006556609994731843471527099609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.142503798007964643801415149937383830547332763671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.136638164520263671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.029510970372887780632797927182764397002756595611572265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.489576793275773525238037109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.33483307936308992491802882796037010848522186279296875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.1775101630482822379075713570273364894092082977294921875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.1771788299083708884129606531132594682276248931884765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06614247192108312078939746925243525765836238861083984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.273228090256452504913653456242172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.171690644363299060870531320688314735889434814453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{9134}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.13472131476737558841705322265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.12986679375171661376953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{23367}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.023343870578020974038135904038426815532147884368896484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{293376428}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{184351425.642384111881256103515625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{9134}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{144655910.25}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{139443408}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{23367}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{25065290.173664174973964691162109375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{41.54341888427734375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{17.3126035020840873812630889005959033966064453125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{10.696970462799072265625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{10.537830352783203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{4.59898901089020117893824135535396635532379150390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{18}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{123}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{7.993377483443708797494764439761638641357421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9972014190345410700189177077845670282840728759765625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.98137544095516193731754128748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{13654}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.977972209453582763671875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.003695271705708187172378931251159883686341345310211181640625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.766114786837964079069251965847797691822052001953125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5087440}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5087440}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5087440}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{5087440}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{22}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{17.22516556291390799060536664910614490509033203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{10}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{10}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.27910806717462310899691146914847195148468017578125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.489772448215454014874836730086826719343662261962890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.335166978008907545660832738576573319733142852783203125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.177648717537941092103892515297047793865203857421875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.1773308750884212414700158433333854191005229949951171875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{24202}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06626848863440525094770094938212423585355281829833984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6094667911529541015625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.37064427571581148868062882684171199798583984375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{11498}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.43735980987548828125}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.3072755336761474609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7208326030572005382879297030740417540073394775390625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.271193027496337890625}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.202660295347504071372668477124534547328948974609375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{29052}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.120829999446868896484375}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{2.119315624237060546875}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.029729270417771493095759893776630633510649204254150390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.780931304208934307098388671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.69643604546316606462852405456942506134510040283203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{913}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.59544845041818916797637939453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.59265005774796009063720703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.033486974795456425635364894333179108798503875732421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.094699792563915197174395643742172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{16197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.07504798282579273893677651585676358081400394439697265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.06160971289500589975762778749412973411381244659423828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.058046793565153999294725650770487845875322818756103515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.007681540743023108040732349621748653589747846126556396484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{101683128}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{16197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{80582157.966887414455413818359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{66152925.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{62327270}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{8247991.568543945439159870147705078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{8384}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{28090}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.75496688741721840187892667017877101898193359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99939405918121337890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{16069}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.984539260927415060820067083113826811313629150390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{10248}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94983610510826121942073996251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.943215072154998779296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01218043820383983046051756815586486482061445713043212890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.597643134976343137765297797159291803836822509765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2952686}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2952686}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2952686}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{2952686}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{19}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.1920529801324502017223494476638734340667724609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{7310}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{11598}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.47294026082656248632929418818093836307525634765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7812433963450775564751893398351967334747314453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.69709847186921292117034454349777661263942718505859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{1696}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5957883693044145889672336124931462109088897705078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.59298062177469235134452674174099229276180267333984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.033408872319600456390897846858933917246758937835693359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7359836101531982421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.64241324197377736027192440815269947052001953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{2743}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.6176974773406982421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.5589950084686279296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7441261137460630781248482890077866613864898681640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2972538471221923828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.2137705032399157545341950026340782642364501953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{19093}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.135382354259490966796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.13283443450927734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.02990865540815661194340435713456827215850353240966796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.767206414602696895599365234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.69174398193197539352894409603322856128215789794921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.57608345779590308666229248046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{2306}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.572208271361887454986572265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03380716108274890718821126256443676538765430450439453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.10301732178777449344675432030271622352302074432373046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.08113022178214113200311885520932264626026153564453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0670146055053919276200957710898364894092082977294921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{23633}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0629876507446169020543180749882594682276248931884765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.007784575881443232814316246503949514590203762054443359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{110614007}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{87112912.31788079440593719482421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{71956384.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{23633}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{67632475}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{8358624.706007264554500579833984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.4248905181884765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.426777032826910041052315136766992509365081787109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24173}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.4322891533374786376953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{23367}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.40823304653167724609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.6229550865539874582310631012660451233386993408203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.006622516556291202505235560238361358642578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99992173910141002313167746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98738741479962077729481961796409450471401214599609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{17096}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95613335072994232177734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{29052}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95596235990524280889957253748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{29726}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0113424095264565705232229220200679264962673187255859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.5578659520172897234857600778923369944095611572265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{4185487}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{4185487}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{4185487}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{4185487}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{19}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{19451}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.7019867549668870054802027880214154720306396484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.080482311588154775705561405629850924015045166015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.76751302171078139569004861186840571463108062744140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.69240375239563523024344249279238283634185791015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{26374}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5763136651156159917519516966422088444232940673828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2306}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.572527433518100981046927699935622513294219970703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.033765621922273288124660695075363037176430225372314453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.716018199920654296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.6488575445895179427679977379739284515380859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{12141}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.58588135242462158203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.55876994132994894926014239899814128875732421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7254085323161445497675003935000859200954437255859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2884185314178466796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.215440339600013519572030418203212320804595947265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.1405699253082275390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.13704013824462890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0305434822648089042418373395548769622109830379486083984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.739106263034045696258544921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.668276528013709736342207179404795169830322265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{17194}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.56719633541069924831390380859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.554243586957454681396484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.033699906916904824594194423070803168229758739471435546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.12489368859678499912302385155271622352302074432373046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.09938353638701284686884918073701555840671062469482421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0820950712077319344484038765585864894092082977294921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.081290949136018697540606581242172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.008269170735424609397501427565657650120556354522705078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{134103577}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{106712259.6357615888118743896484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{30463}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{88148911.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{87285492}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{8878954.468422241508960723876953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.27951812744140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.801418986541545308455170015804469585418701171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.205653667449951171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.93181514739990234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.594245364275689524902190896682441234588623046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.5761589403973506051670483429916203022003173828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99991589784622203485042746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9880194300847338073623404852696694433689117431640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9613973200321197509765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.9592688083648681640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00922866228671943671091337790812758612446486949920654296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.66548877713023413260629013166180811822414398193359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3929455}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3929455}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3929455}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3929455}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{19}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{15.1854304635761589992171138874255120754241943359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{9.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.9168267565695937815206661980482749640941619873046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7394016401705798546828418693621642887592315673828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.66891426331554482143104678470990620553493499755859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{17194}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.56749750513085484016073678503744304180145263671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.55455272890302598209899542780476622283458709716796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.033674790639359138133546167637177859432995319366455078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6793234348297119140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.67282380331430857722807559184730052947998046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.641533792018890380859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.6239883899688720703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.74074761599776584031218362724757753312587738037109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2718737125396728515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.214155651875679087225989860598929226398468017578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{19451}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.141734063625335693359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1379802227020263671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.031550573311771544504633624228517874144017696380615234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.74656238220632076263427734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.67622139003892611786028510323376394808292388916015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.57643664698116481304168701171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.573907024227082729339599609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.034075746263168608940485881930726463906466960906982421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.116667185910046100616455078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.09178871677460649636248746219280292280018329620361328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.076432369416579548637713514835922978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0722891632467508038484282906210864894092082977294921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00786872531827722231090316284962682402692735195159912109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{125270437}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{98557384.17218543589115142822265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{82068631.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{77619898}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{8448979.47580196522176265716552734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.0167236328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.06559399105855145961641028407029807567596435546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1412}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.94751203060150146484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.535209767337012198851198263582773506641387939453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.28476821192052970133090639137662947177886962890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999916255474090576171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9870352192430307258774746514973230659961700439453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{30899}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9580770432949066162109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95654094219207763671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{16284}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00938331631149649965373260585010939394123852252960205078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.57976340737057718843772136096959002315998077392578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3171245}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3171245}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3171245}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{3171245}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{19}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.6887417218543046004697316675446927547454833984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{7310}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.282050403885764300326854936429299414157867431640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.746860739113479166206843729014508426189422607421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.67686761246545790182693735914654098451137542724609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5767606251201506939452201550011523067951202392578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.5742067865023823269865488327923230826854705810546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0340659998998718849261280183782218955457210540771484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.59687709808349609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.66773735766378905509554897435009479522705078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{30371}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.68202960491180419921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4839541912078857421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.73684007500161563530838293445413000881671905517578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2835080623626708984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.216945501352777458947684863233007490634918212890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{19004}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.14905452728271484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{20539}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.148380756378173828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.030432920312190088474313398592130397446453571319580078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.422637581825256292145098768742172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.349449165436803099726859045404125936329364776611328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{30371}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.266816673101857249061907850773422978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.258666276000440120697021484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0340056360663673895583514195095631293952465057373046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.3962266743183135986328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.341243213153635427392629253517952747642993927001953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{19488}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.30406476999633014202117919921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.302087581716477815430010878117172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.016581152449764248457686477422612369991838932037353515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{425445152}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{366407110.119205296039581298828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{19488}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{326487060.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{324364071}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17803876.875431932508945465087890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4480}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.185821533203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.6145395948397407437369110994040966033935546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.5718860626220703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{77.82788848876953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.51010078068381492499838714138604700565338134765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{56}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{32.4900662251655631962421466596424579620361328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{23}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{23}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{5.5646323425898511771947596571408212184906005859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2640941}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2640941}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2640941}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2640941}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{29}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.01324503311258240501047112047672271728515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.3074505152562050369624557788483798503875732421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.422933978995119141952585550825460813939571380615234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.349789532118438606378418853637413121759891510009765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{30371}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.266991979627465958468945927961613051593303680419921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.258757218043046799405004776417626999318599700927734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03408894801848223743423460518897627480328083038330078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7788383960723876953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.67596116444922671462336438708007335662841796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.634042918682098388671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.3337075710296630859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.733007338980101064151995160500518977642059326171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.287342071533203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.218813779338306257926660691737197339534759521484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.15206992626190185546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.15174198150634765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0307618895150273859162570744274489698000252246856689453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.734028113074600696563720703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.66780817900346411963852233384386636316776275634765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{17194}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.56677820719778537750244140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.549845497123897075653076171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.033527498964771106082505269796456559561192989349365234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1249578436836600026094146187460864894092082977294921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.0994550350140656347353029786972911097109317779541015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0823579616844653805696196968710864894092082977294921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0812791325151920041047759468710864894092082977294921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00827816706867403988290288197049449081532657146453857421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{134172463}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{106789030.7019867599010467529296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{18146}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{88431188}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{87272804}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{8888614.20769480057060718536376953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.38015460968017578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.8657478844093162706485600210726261138916015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.17229998111724853515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.9324092864990234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6180041988517543938286280535976402461528778076171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.5761589403973506051670483429916203022003173828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99991589784622203485042746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{14095}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98810557971726975523552027880214154720306396484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1283}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96124573051929473876953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{2345}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.959544360637664794921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{11611}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0092119215550841293538297804843750782310962677001953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.66548877713023413260629013166180811822414398193359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3937774}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3937774}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3937774}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3937774}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{19}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{1895}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{15.25165562913907280062630889005959033966064453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{9.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{2549}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.891838669200649025725624596816487610340118408203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.73432146077440985099116232959204353392124176025390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.66844573637061788229374315051245503127574920654296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{17194}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.56707911953916667613384561263956129550933837890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.55015218593499837229643389946431852877140045166015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.033508236074929302616975945738886366598308086395263671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7146308422088623046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.66797076787380404994109994731843471527099609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.737996578216552734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.6132180690765380859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7178862135097958674379015064914710819721221923828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.380863666534423828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.216572684168025997308859587064944207668304443359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{12141}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.145803272724151611328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.14550876617431640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.031921337733224676436183386840639286674559116363525390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.746494571678340435028076171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.675964392647640632816319339326582849025726318359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{11124}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.57792116212658584117889404296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.576360945589840412139892578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.034205997787634521978272772457785322330892086029052734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.11680755950510500473793484843554324470460414886474609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.09188411105424161562371665468162973411381244659423828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.07649871543981127952616105858396622352302074432373046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0724283158779144009553618843710864894092082977294921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0078707809906460902971137016947977826930582523345947265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{125421162}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{5615}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{98659813}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{3175}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{82139870.25}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{12457}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{77769312}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{8451186.7372008599340915679931640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.015990734100341796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.07849087778306174101317083113826811313629150390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.975169837474822998046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.8679935932159423828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.53139427036718023256156584466225467622280120849609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{7}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.28476821192052970133090639137662947177886962890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999916255474090576171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2773}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98707485001608230579250857772422023117542266845703125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{16197}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.957870066165924072265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.95635569095611561163394753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{16284}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00925491965838346093697897032370747183449566364288330078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.57976340737057718843772136096959002315998077392578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3196202}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3196202}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3196202}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{3196202}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{19}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.7019867549668870054802027880214154720306396484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{7310}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.254633792048812868102913853363133966922760009765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.74679290148563437501394446371705271303653717041015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29110}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.67661043889366834225285174397868104279041290283203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6159}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.578245961715013745418900725780986249446868896484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.5766619895937477036085283543798141181468963623046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{12552}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.034198476326201703023865974273576284758746623992919921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.69747829437255859375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.67632329542905011976472451351583003997802734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.569633305072784423828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.5672924518585205078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7491511173953326885310843863408081233501434326171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.29370975494384765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{13468}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.21970502272346958960724805365316569805145263671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{22545}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.151972115039825439453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.151729106903076171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.03012781562182111072534240747700096108019351959228515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.42662229202687740325927734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.349848472457749137820570695112110115587711334228515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{5358}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.262384733883663956444109999210922978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.25215045176446437835693359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.034709406216644637932500216948028537444770336151123046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.394959085620939676086749159367172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.3411562445616682648363848784356378018856048583984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{6155}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.303677291609346811096514784367172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.302029694430530015747393690617172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0165502335047310149274135682162523153237998485565185546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{424084089}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{366313728.3046357631683349609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{6155}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{326071009}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{324301915}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17770677.9109957925975322723388671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.12237548828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.439607481293336377348168753087520599365234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.6455821990966796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.29946136474609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.5064594809721061352547621936537325382232666015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{56}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{32.4304635761589423736950266174972057342529296875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{742}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{23}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{23}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99999782068050457883856552143697626888751983642578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99991773068904876708984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99967092275619517938167746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00002669110375110156420396835541541946668075979687273502349853515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{5.53915614317511550979133971850387752056121826171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2653228}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2653228}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2653228}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2653228}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{29}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{5781}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.20529801324503438308965996839106082916259765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{2743}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.241445491489935104567621237947605550289154052734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.42692148368752214082633145153522491455078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3501891597590647275950459516025148332118988037109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.262557352173024061148254304498550482094287872314453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.252239102969724793279482355501386336982250213623046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.034792252575737890596396795217515318654477596282958984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.8473227024078369140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.69211171162839235648789326660335063934326171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{8893}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.49753391742706298828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4154193401336669921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.76396544132289345707675920493784360587596893310546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3000600337982177734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{6155}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.216348142813373112147701249341480433940887451171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.144145548343658447265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.141279697418212890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0315097707754618261422052682974026538431644439697265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.422235920093953609466552734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.343516470161297438057346198547747917473316192626953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{32374}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.26118567143566906452178955078125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.251811563968658391754473768742172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0328257278676844510556520617683418095111846923828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.397403544746339321136474609375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.3446273755911268832363703040755353868007659912109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.306819862918928210060443007023422978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.302087918855249881744384765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01664165514190496519830730903777293860912322998046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{426708807}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{370040826.8675496578216552734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{104}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{329445319.25}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{18289}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{324364433}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{17868841.14644801616668701171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4544}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{142.3176116943359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.2863692732046700939463335089385509490966796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{30684}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.6405811309814453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.46202850341796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.42529095414309292522148098214529454708099365234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{57}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{33.4503311258278159812107332982122898101806640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{4810}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{23.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1681}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{23}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{6532}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99999782068050457883856552143697626888751983642578125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99991773068904876708984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99967092275619517938167746251565404236316680908203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00002669110375110156420396835541541946668075979687273502349853515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{5.74016722386250233256532737868838012218475341796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2667658}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2667658}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2667658}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2667658}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{31}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.25165562913907280062630889005959033966064453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{913}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{5928}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.51147971751215504099263853277079761028289794921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.422472765693030327671664281297125853598117828369140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27300}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3438534591499688986004912294447422027587890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{32374}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.261357418899735183259736004401929676532745361328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1490}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.25190009602754670492430477679590694606304168701171875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{25516}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.032936395559529214882577008438602206297218799591064453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7130401134490966796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.67478214036550099308442440815269947052001953125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.6829869747161865234375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.671779632568359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.746444718030302656330832178355194628238677978515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2998869419097900390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{30684}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.216529760929133008318103748024441301822662353515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.1397821903228759765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1362888813018798828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0305152995259909375069806714009246206842362880706787109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.666021988727152347564697265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{23367}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.58582813868804872736717470615985803306102752685546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.460163631476461831848467909367172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.449777182191610280792559706242172978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.04095636051897409701805230497484444640576839447021484375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.271180302836000919342041015625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1678790079972503068717060159542597830295562744140625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.130809799302369300644244276554672978818416595458984375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1262654569000004889378629968632594682276248931884765625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{23367}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0233271982233698819964029524953730287961661815643310546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{291177633}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{180258712.2582781314849853515625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{2236}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{140455952.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{135576502}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{23367}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{25047388.3691707365214824676513671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4416}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{41.54341888427734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{17.3126035020840873812630889005959033966064453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{8048}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{10.696970462799072265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{10.537830352783203125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27671}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{4.59898901089020117893824135535396635532379150390625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{17}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{7.75496688741721840187892667017877101898193359375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5.75}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999998152256011962890625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99675505169180056430633385389228351414203643798828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{23447}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97184456884860992431640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{8299}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96565926074981678350894753748434595763683319091796875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{12287}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005232033283193947108269394874469071510247886180877685546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{1.651677403107722152952874239417724311351776123046875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{5135824}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{5135824}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{5135824}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{5135824}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{16.841059602649007587160667753778398036956787109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{1185}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{7310}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{7310}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.252570908636236435285127299721352756023406982421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.66624694223114555580167461812379769980907440185546875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{23367}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.58638991880666446743219921700074337422847747802734375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8840}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.46040019927746556049896753393113613128662109375}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1951}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.44994765997517738309596779799903742969036102294921875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.040997131934037180089891450052164145745337009429931640625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.8482859134674072265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.66002463189182236646956880576908588409423828125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{123}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.700883090496063232421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.521884441375732421875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.73636571507234027667010423101601190865039825439453125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.286263227462768998776709850062616169452667236328125}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{4800}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.213862289656077120270083469222299754619598388671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{3254}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.1437418460845947265625}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{20751}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1375713348388671875}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUMaxDiffExactAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.031746843095142966706401210785770672373473644256591796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.3483474738895893096923828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.158077613518431470129854687911574728786945343017578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{6532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0279024161864071772176654206987223005853593349456787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{8721}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.010520822368562200710417897653314867056906223297119140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0656136617750341655241896887673647142946720123291015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1087717832997441014253325874960864894092082977294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.0887661780853638282540174486712203361093997955322265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.05985927465371780609171281639646622352302074432373046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.05716422107070680269647056093162973411381244659423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01052884987511220997447036751282212208025157451629638671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{116792813}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{95311957.966887414455413818359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{64273406.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{61379615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{11305266.4695251546800136566162109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{5.887417218543046004697316675446927547454833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999576032161712646484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98781375261332027282179524263483472168445587158203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96753509342670451776058371251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{13654}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.964610278606414794921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0067955367135954340696013531442076782695949077606201171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.69571104565133234931550987312220968306064605712890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2648206}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2648206}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2648206}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{2648206}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{26}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{11.3311258278145690070459750131703913211822509765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.035193188690741283863872013171203434467315673828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.3486477360315005658009113176376558840274810791015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1582205078255218555494110432846355251967906951904296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0279219835245605174645078250250662676990032196044921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8721}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0105251207910052914373810750703341909684240818023681640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0656524374938336208185063469500164501368999481201171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.3538553714752197265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.4113136790446105806040577590465545654296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.565522015094757080078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.47721958160399680082264239899814128875732421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.66136345031595766830179172757198102772235870361328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2955410480499267578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.200705256683147315044379865867085754871368408203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{3175}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.1225636005401611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1197683811187744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0315677731479653556068143416268867440521717071533203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.352994818240404073517169081242172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.1558811986165133112169911555611179210245609283447265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{23633}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.02735079266130922837074734843554324470460414886474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{8721}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.008518793620169100300199005459944601170718669891357421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0647659625861693732939983192409272305667400360107421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.115009244531392995636309706242172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.092762050989842526060868976855999790132045745849609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{14929}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.06221149093471463331628257265037973411381244659423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.05856804177165030045326687968554324470460414886474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01110376843611468079819903920224533067084848880767822265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{123490236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{99602493.82781456410884857177734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{14929}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{66799079.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{62886956}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{11922580.57386740483343601226806640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.4248905181884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.426777032826910041052315136766992509365081787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.4322891533374786376953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{23367}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.40823304653167724609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.6229550865539874582310631012660451233386993408203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.132450331125827602818390005268156528472900390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99944603443145763055355246251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.989324782857831763749345554970204830169677734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6589}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97045312821865081787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96847128868103038445980246251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005641372364399586426808586026027114712633192539215087890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.67770059896508783037205603250185959041118621826171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3881007}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3881007}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3881007}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{3881007}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{27584}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{11.4635761589403966098643650184385478496551513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.8115700059848423020270047345547936856746673583984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.353299086214633850655530977746821008622646331787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1560216582167485988019706155682797543704509735107421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{23633}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.027370118106608450070371674200941924937069416046142578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8721}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00852227408703777611354013288291753269731998443603515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06480278522326454737623180335504002869129180908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.3684914112091064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.40825440394167600288710673339664936065673828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.50136244297027587890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.418855190277099609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.682648680907103955206594037008471786975860595703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.272531986236572265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20103827849129185523224805365316569805145263671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{10248}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.132597744464874267578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1298820972442626953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.02949836400858292517757064388206345029175281524658203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.34180335514247417449951171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.150774522567328206346104479962377808988094329833984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0294209700077771481308008816313304123468697071075439453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00587948411703100026759472029880271293222904205322265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06206924203675777407251956674372195266187191009521484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.132397164590656701843585096867172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10498217109664775836819217147422023117542266845703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0686460046563296677479826257695094682276248931884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.065201691351830903808917128117172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0129747532312183867786448132619625539518892765045166015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{142160373}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{112723747.880794703960418701171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{73708086.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{70009783}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{13931535.20043831877410411834716796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.27951812744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.801418986541545308455170015804469585418701171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22545}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.205653667449951171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.93181514739990234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.594245364275689524902190896682441234588623046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{7.0596026490066225989039594423957169055938720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9929773322004356028713800697005353868007659912109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{20751}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97893919050693511962890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6204}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97859001159667957647769753748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00472445226903791225259165997840682393871247768402099609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.7740132627118929686815818058676086366176605224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3624975}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3624975}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3624975}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3624975}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{22545}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{11.993377483443708797494764439761638641357421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.6173590145696039588329995240201242268085479736328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.342097976505395473534321126862778328359127044677734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.150913285817929343490817473139031790196895599365234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.02943313809457255569856926058491808362305164337158203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.00588188625876451785801091176608679234050214290618896484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0621033552172665925805716824470437131822109222412109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.3613073825836181640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.478432795859333737098495475947856903076171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.283470213413238525390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.268251895904541015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.73333027343136125697498073350288905203342437744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3204822540283203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.204025170660966370661526525509543716907501220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{1412}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.128169715404510498046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1200492382049560546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.031237091649241953417170947204795083962380886077880859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.3378712572157382965087890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.1523012768551213758083662241915590129792690277099609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{9132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.032723831245675648327075890620108111761510372161865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.002282558940350999827917366502560980734415352344512939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.062753393096146969920567926237708888947963714599609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.125148522667586803436279296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10020465886109312936280701933355885557830333709716796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.06680712499655783176422119140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.06341142114251850647743680156054324470460414886474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01236876521070957336834172934914022334851324558258056640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{134377203}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{107593933.1788079440593719482421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{71733604.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{68087495}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{13280860.51797504164278507232666015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.0167236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.06559399105855145961641028407029807567596435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1412}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.94751203060150146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.535209767337012198851198263582773506641387939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.6754966887417221954592605470679700374603271484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99120289324135180120123322922154329717159271240234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{17197}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97604171931743621826171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.972770631313323974609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{7310}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00542901126718774162949188166749081574380397796630859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.7852081925312386356807792253675870597362518310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2866765}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2866765}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2866765}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{2866765}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{27584}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{11.596026490066225989039594423957169055938720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.703828209895205336721346611739136278629302978515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.338162489261284893160564024583436548709869384765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1524396710800356713466641167542547918856143951416015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{9132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0327373709738682794334607706332462839782238006591796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.002283491510280723398029767423622615751810371875762939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.06278628380270444286903597230775631032884120941162109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.2462227344512939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{27584}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.482427499152180416785995475947856903076171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{9132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.485747635364532470703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.3209221363067626953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.72374744807423707637639154199860058724880218505859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2728617191314697265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20386252340102029023682916886173188686370849609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{22401}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.12127220630645751953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.117793560028076171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0294780814516342193343234612257219851016998291015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.2142596961930393895112700874960864894092082977294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.08947897120224714007097333023921237327158451080322265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.01746563264168797535713650859179324470460414886474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{9134}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.013268347829580300067942033592771622352302074432373046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.040603337932327114578878735073885763995349407196044921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.333862788043916225433349609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{29565}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.267490205749721321470957491328590549528598785400390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{13654}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1775435418821871003114409859335864894092082977294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1702803419902919890294157312382594682276248931884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.034111323134154623859526367368744104169309139251708984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{358482439}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{29565}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{287215421.423841059207916259765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{13654}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{190635926.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{182837125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{36626754.32112057507038116455078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.185821533203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.6145395948397407437369110994040966033935546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.5718860626220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{77.82788848876953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.51010078068381492499838714138604700565338134765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{61}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{40.3774834437086127536531421355903148651123046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{2345}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{28.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{28}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{5.80561696712168551215427214629016816616058349609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2336461}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2336461}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2336461}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2336461}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{32}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.29139072847682001565772225148975849151611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{9132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{9132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.43836824839482080307107025873847305774688720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.2144443798211014551302611153005273081362247467041015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.08956498438049241561653701637624180875718593597412109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.017474195212337895188881020658300258219242095947265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{9134}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.01328242055604550268810282176445980439893901348114013671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0406326193651935507755723619993659667670726776123046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.3659646511077880859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{28090}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.483515553127062958083115518093109130859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{22545}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.416045725345611572265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.2136442661285400390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.72398102161661237463619045229279436171054840087890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.594494342803955078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20556218418853955398617472383193671703338623046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{19004}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.125283777713775634765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.122575283050537109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.043502894046228264557374387777599622495472431182861328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.340988524258136693756426893742172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.1507757209204383663792015113358502276241779327392578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.029045364120975102062427453120108111761510372161865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.005870243534445700184232208584944601170718669891357421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06215116081989312257771729264277382753789424896240234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1323575237765907963716216499960864894092082977294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10503359312894718080588774000716512091457843780517578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.06888154405169182037393937889646622352302074432373046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.065201695077121202270831190617172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01297052502788768359176518885078621678985655307769775390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{142117809}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{112778961.86754967272281646728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{73960994.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{70009787}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{13926995.20168177597224712371826171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.38015460968017578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.8657478844093162706485600210726261138916015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.17229998111724853515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.9324092864990234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6180041988517543938286280535976402461528778076171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{7.0728476821192050039144305628724396228790283203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.993159030841675782852462361915968358516693115234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{20754}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97893925011157989501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{6204}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97859007120132435186832253748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00462102100086353613506151560841317404992878437042236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.7728791767361673503700103537994436919689178466796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3633294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3633294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3633294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3633294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{26}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{12.0397350993377489913882527616806328296661376953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.9458932632802075080036274812300689518451690673828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.34128244326813461650971248673158697783946990966796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1509143234203456918063324110335088334977626800537109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.02905737677563342835629356386561994440853595733642578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.005872641900815830408311146726418883190490305423736572265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0621851333336047584765537976636551320552825927734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.3342201709747314453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.4741111085904350375130889005959033966064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.3371622562408447265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.244799137115478515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7324862972313808118229871979565359652042388916015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.260399341583251953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20207723244925990258025194634683430194854736328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.12896060943603515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1267540454864501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.02987694691659233126035388750096899457275867462158203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.3378920517861843109130859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.1522602565117821826756738801122992299497127532958984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{28090}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.03272367827594280242919921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.002282558940350999827917366502560980734415352344512939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.06271966937506688599679449680479592643678188323974609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.125334869138896409790362440617172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.10028464708551267092762060428867698647081851959228515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0668408733326941451036162789023364894092082977294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.06341142114251850647743680156054324470460414886474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01238183307919042165645695519060609512962400913238525390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{134577291}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{24144}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{107679819.880794703960418701171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{71769841.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{68087495}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{13294892.034913457930088043212890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.015990734100341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.07849087778306174101317083113826811313629150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.975169837474822998046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.8679935932159423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.53139427036718023256156584466225467622280120849609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.6754966887417221954592605470679700374603271484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9911545878214551574814095147303305566310882568359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{17197}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9760403931140899658203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97276532649993896484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{7310}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005444737417629482052749967380123052862472832202911376953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.7852081925312386356807792253675870597362518310546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2891722}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2891722}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2891722}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{2891722}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{20}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{27584}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{11.596026490066225989039594423957169055938720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{4430}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{1.6999369211009323077377075605909340083599090576171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.33818330175585187280518084662617184221744537353515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.152398598810299434891391001656302250921726226806640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.03273721794082896929811710151625447906553745269775390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.002283491510280723398029767423622615751810371875762939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0627525112813241692233390267574577592313289642333984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.497321605682373046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.49220473245279805496465996839106082916259765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.373468339443206787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.270789623260498046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7205958151274216572090836052666418254375457763671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3274505138397216796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.207073696401735229954965689103119075298309326171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{17197}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.121788501739501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1171014308929443359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{20754}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.03549732487196054220301988380015245638787746429443359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.2141888076439499022374235437382594682276248931884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.089269931471308294756994428098550997674465179443359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{3284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0163696999661623980582003667905155452899634838104248046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{9134}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.01316908560693260017704364628343682852573692798614501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.040431195102854679268578053097371594049036502838134765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.334079244174063205718994140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{29565}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.2674644139983894941536846090457402169704437255859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{26829}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.178091760259121600906695448429672978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.170375610701739788055419921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.034099743020087731892875382300189812667667865753173828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{358714857}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{29565}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{287187727.7417218685150146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{26829}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{191224571.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{182939419}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{36614320.268320269882678985595703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.12237548828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.439607481293336377348168753087520599365234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.6455821990966796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.29946136474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.5064594809721061352547621936537325382232666015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{60}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{40.29139072847682001565772225148975849151611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{2345}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{28.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{28}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{5.7250343750649772545102678122930228710174560546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2348748}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2348748}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2348748}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2348748}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{32}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.23178807947019919311060220934450626373291015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{9132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{9132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.342370393766887826103584302472881972789764404296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.2143734301688055843282398882365669123828411102294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.0893556898000740229548455317853949964046478271484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{3284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.01637785433084608388565328596087056212127208709716796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{9134}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.01318305305351476046371583805694172042421996593475341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.040460288155705993740074433162590139545500278472900390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.5424783229827880859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.43391986872186549817342893220484256744384765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.48527681827545166015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.42971897125244140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7021121164840149475594444083981215953826904296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.315169811248779296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{4305}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20676559644029612883286972646601498126983642578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{6204}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.14224326610565185546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1410019397735595703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24202}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.030547621902030919205373038494144566357135772705078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.214458857662975788116455078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.0884538456143823259569813899361179210245609283447265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{23367}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.01797623978927727350640708436912973411381244659423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0128081804141402001706584456997006782330572605133056640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.039878405610341012554886930274733458645641803741455078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.336879915557801723480224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{29565}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.26977273678123359079705778640345670282840728759765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{13654}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.178247974952682797233904921085922978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.169834066182374898712481581242172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.03457646989192357522835408190076122991740703582763671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{361722055}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{29565}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{289666270.45695364475250244140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{13654}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{191392305.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{182357940}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{37126201.849235095083713531494140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{142.3176116943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.2863692732046700939463335089385509490966796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{30684}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.6405811309814453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.46202850341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.42529095414309292522148098214529454708099365234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{62}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{41.4105960264900687661793199367821216583251953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{29}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{29}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{6.1031655266817832483638994744978845119476318359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2363178}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2363178}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2363178}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2363178}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{32}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{23.71523178807947118684751330874860286712646484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{9132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{9132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.42444945726274863062599251861684024333953857421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.21464371296057482840780039623496122658252716064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.08853977555107427066527492343084304593503475189208984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{23367}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.017986209402655932432235630358263733796775341033935546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.01282176507605894445751548715861645177938044071197509765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.039909931998766058625083275046563358046114444732666015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.475329875946044921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.4206958574964545505281421355903148651123046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7310}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.44564831256866455078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.2350151538848876953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.67507466057023624017574547906406223773956298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2726838588714599609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{31308}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.204028131156567926751677077845670282840728759765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{12561}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.130090296268463578854834850062616169452667236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.12646770477294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0308353839059560298763162933255443931557238101959228515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.323529521934688091278076171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.132509588165245661972591051380732096731662750244140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.0216545884031802242375430722631790558807551860809326171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{8721}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.0199887668713926991426177437460864894092082977294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.057224504873779315217152685590917826630175113677978515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.2459435947239398956298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{7467}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.155108530709630987320934991657850332558155059814453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7098}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.09699850529432292589593345155662973411381244659423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.09169922024011610550697781718554324470460414886474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.02462326351494524556695608907830319367349147796630859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{264079924}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{7467}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{166546516.682119190692901611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7098}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{104151352}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{8299}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{98461288}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{26439027.87936995923519134521484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{41.54341888427734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{17.3126035020840873812630889005959033966064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{8048}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{10.696970462799072265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{10.537830352783203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27671}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{4.59898901089020117893824135535396635532379150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{26}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{11.8278145695364234057933572330512106418609619140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{8}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{5928}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{8}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{5928}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{3254}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99933917159276297592640503353322856128215789794921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29110}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99292403459548939093082253748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99256211519241321905582253748434595763683319091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0010835671653123533399176725566803725087083876132965087890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.528674205416491016507052336237393319606781005859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{4831344}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{4831344}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{4831344}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{4831344}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{26}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{19917}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.7880794701986761907619438716210424900054931640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{3175}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{11}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{14929}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{11}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{14929}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.995823298981033389054573490284383296966552734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.32380839195531130325633739630575291812419891357421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.1326336228614018175608890715011511929333209991455078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.0216720774572327114226855115930447936989367008209228515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{8721}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.020009967434731164293015837074563023634254932403564453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.057262733154364919840872971690259873867034912109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.5577757358551025390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.48565923772900276844666223041713237762451171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{23696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.298861920833587646484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.2875878810882568359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.73911969862012105725312949289218522608280181884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2915079593658447265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.202684555622126172380603748024441301822662353515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{2549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.1313154697418212890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{20754}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1271569728851318359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.03098978035989312374010040684879641048610210418701171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.7556504905223846435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.6479131487808775791137350097415037453174591064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{32382}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.4958753963001072406768798828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.462237928993999902527178846867172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.055514729244972534083490955936213140375912189483642578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.12195928022265430101800376405662973411381244659423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.0992770112606863042170601829639053903520107269287109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.07986202277243137359619140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.07836645096540449662025906718554324470460414886474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00799001987947541535139972523893447942100465297698974609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{130952780}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{106597879.15231788158416748046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{85751194}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{84145336}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{8579218.5191841982305049896240234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10370}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{5.615894039735099596555301104672253131866455078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.987856667562825752071375973173417150974273681640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{11124}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96268060803413402215511496251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{20751}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.960471451282501220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00814497095365323588167516533076195628382265567779541015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.72660807869903332179006838487111963331699371337890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2696590}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2696590}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2696590}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{2696590}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{16284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{12.25827814569536400313154445029795169830322265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{913}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{7.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{1696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.05027102510719227979052448063157498836517333984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7559720149848636605582896663690917193889617919921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6485017950485560955797836868441663682460784912109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{32382}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.496161259854536240698763549517025239765644073486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.462586799009633231616334114733035676181316375732421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.05522337262690590886649033564026467502117156982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.53686046600341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.74689306328627935727126896381378173828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.567683160305023193359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4612915515899658203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7234440083661455300756415454088710248470306396484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2811653614044189453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{26374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.213932160510132529651627919520251452922821044921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{29565}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.14238131046295166015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1330397129058837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0287189282476514214093032961727658403106033802032470703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.748260472901165485382080078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.640869906301678060600579556194134056568145751953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.48698424664326012134552001953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.45845983736217021942138671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0549054471134226840245418088670703582465648651123046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1276281056925654133760161812460864894092082977294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1041802770785049403468036643971572630107402801513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{23241}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.08493170607835047458689103905271622352302074432373046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0833008084446190955052458093632594682276248931884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0084223640343097407046091262827758328057825565338134765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{137039635}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{111862720.73509933054447174072265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{23241}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{91194725}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{89443562}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9043444.52059173583984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.4248905181884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.426777032826910041052315136766992509365081787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.4322891533374786376953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{23367}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.40823304653167724609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.6229550865539874582310631012660451233386993408203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{9}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{5.85430463576158910399271917412988841533660888671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{4.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{913}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{4}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98899796703793352303790697988006286323070526123046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{24262}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.96434777975082408563167746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{17080}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.946926116943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.0075902327884350417885883643975830636918544769287109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.7668405205896757781403039189171977341175079345703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3929391}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3929391}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3929391}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{3929391}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{12.642384105960264406576243345625698566436767578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{3284}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{7.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.069491773323777206172735532163642346858978271484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7485788529582968475750703873927704989910125732421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.64145326938879121403402905343682505190372467041015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{15399}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.487265246656892692111995302184368483722209930419921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.45880585589633915422069776468561030924320220947265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.054630589876599751353314360358126577921211719512939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.5115528106689453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{11611}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.75669539053708234632722451351583003997802734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15043}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.4662458896636962890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4357960224151611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7433774155756918133874933118931949138641357421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3069908618927001953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{15622}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.216884848297826504648355694371275603771209716796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{2345}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.136838853359222412109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{21317}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1352980136871337890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0300200958695463204772835297262645326554775238037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.737935961224138736724853515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.6205348873399938458561564402771182358264923095703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.4728746884502470493316650390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{28090}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.433715748600661699097003065617172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0530575863140629599978836949958349578082561492919921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1476541059091686924897857124960864894092082977294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.119041059147689864960995009823818691074848175048828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29726}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.0959824977908283194505401070273364894092082977294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.09569012094289060244012290468162973411381244659423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00971772537486826661068395338816117146052420139312744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{158542389}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{127819363.98013244569301605224609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29726}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{103060422.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{102746485}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{10434328.16914213635027408599853515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.27951812744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.801418986541545308455170015804469585418701171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22545}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.205653667449951171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.93181514739990234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.594245364275689524902190896682441234588623046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.72185430463576150117432916886173188686370849609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999963283538818359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99258709822269464151389684047899208962917327880859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{1895}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97354520857334148065120871251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.966265380382537841796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00537227363851080531864656819607262150384485721588134765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.831171999456277177387164556421339511871337890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3673359}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3673359}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3673359}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3673359}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{22}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{13.3245033112582778045407394529320299625396728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{913}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{8.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.148740248202650082731679503922350704669952392578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.73857203367741786070865828150999732315540313720703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6211002032905967862319585037766955792903900146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{9504}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.475459458829224079767783450733986683189868927001953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{27484}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.434043091751242282594347443591686896979808807373046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.05279352356356505071577345233890810050070285797119140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7296173572540283203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{27584}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.74986408246274294242539326660335063934326171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{32103}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.381806910037994384765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.2837111949920654296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.72757453443383723890036662851343862712383270263671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3431665897369384765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{13468}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.221750652553229787855570975807495415210723876953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.1460258960723876953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1422092914581298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.03258129097315143329893771806382574141025543212890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.73887385241687297821044921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.62750846061189446967176763791940174996852874755859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{16069}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.476904083043336812774981581242172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{28090}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.448228550143539905548095703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.052558096099472477458203201194919529370963573455810546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.141456448473036289215087890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1131235261059162222618823534503462724387645721435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.090685617178678457062090956242172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08841302897781129488397056093162973411381244659423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00940383681966938146656875829876298666931688785552978515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{151887705}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{121465461.25827814638614654541015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{97372940}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{94932767}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{10097292.899350158870220184326171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.0167236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.06559399105855145961641028407029807567596435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1412}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.94751203060150146484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.535209767337012198851198263582773506641387939453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.384105960264900403444698895327746868133544921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99149690163846049273388416622765362262725830078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97429747879505157470703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97148817777633678094417746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{16149}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005899544438415899559602362245414042263291776180267333984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.77083361732193178550431866824510507285594940185546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2915149}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2915149}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2915149}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{2915149}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{12.9536423841059598061065116780810058116912841796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.015056583753727981189740603440441191196441650390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.73951073329633432162921735653071664273738861083984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.62807970765787535238899863543338142335414886474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{16069}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.47886062256679295945360763653297908604145050048828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.44856684670357382938021828522323630750179290771484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.05228043194718350050731459077724139206111431121826171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.657907962799072265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.77331212340601496180170215666294097900390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1696}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.64054930210113525390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.6238498687744140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.69864444484761534237549085446516983211040496826171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3137114048004150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.221688493198116898241778471856378018856048583984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{2306}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.142853438854217529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1394107341766357421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.031332855282961959153542608191855833865702152252197265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.414734554477035999298095703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.333848454329549071406546545404125936329364776611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{9132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.2488825903274118900299072265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.2342543266713618954621978218710864894092082977294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03291243734824673972116926279340987093746662139892578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.375659871846437398712481581242172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.312316584400832653045654296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{22401}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.244346162304282132904376112492172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{28090}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.2349676061421631934056364343632594682276248931884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.028361931554884749207001704007780062966048717498779296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{403361716}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{335347379}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{22401}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{262364694}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{28090}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{252294546}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{30453392.1199051029980182647705078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.185821533203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.6145395948397407437369110994040966033935546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.5718860626220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{77.82788848876953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.51010078068381492499838714138604700565338134765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{68}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{41.24503311258278159812107332982122898101806640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{29.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{28}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{6.53768179686418005047698898124508559703826904296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2384845}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2384845}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2384845}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2384845}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{34}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{24.29139072847682001565772225148975849151611328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{913}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6155}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.97804194521563214692605470190756022930145263671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.415092039732380124750221739304834045469760894775390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.3341616154887543377327574489754624664783477783203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{9132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.24902619782164292505655112108797766268253326416015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.23443112806623200849998056582990102469921112060546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.032866400442517935964747977095612441189587116241455078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6385371685028076171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.76729448110062747900883550755679607391357421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24202}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.46943938732147216796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4421784877777099609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.71110780657676919691567718473379500210285186767578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.30275249481201171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.2186143398284912109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{23367}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.14271199703216552734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.139438629150390180910790149937383830547332763671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.028818454222385596341649005580620723776519298553466796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.737684629857540130615234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.62037772285622472256960691083804704248905181884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{27584}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.47293854248709976673126220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{28090}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.432969102635979596893633924992172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.05308277314946907576853618593304418027400970458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1475925827398895939790435249960864894092082977294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.11911053018681454218619109042265336029231548309326171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29726}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.096056580776348654548968397648422978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.0956638893112539967500396187460864894092082977294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00972116531843588392580723933633635169826447963714599609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{158476329}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{127893957.9403973519802093505859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29726}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{103139968.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{102718319}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{10438021.7804228849709033966064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.38015460968017578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.8657478844093162706485600210726261138916015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.17229998111724853515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.9324092864990234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6180041988517543938286280535976402461528778076171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.71523178807947029866909360862337052822113037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999963283538818359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9925842158841771123434227774851024150848388671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97354713082313548699886496251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.96627306938171397820980246251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{1185}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005367599959626251533706398078038546373136341571807861328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.82492209902092816786733919798280112445354461669921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3681678}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3681678}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3681678}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3681678}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{22}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{18146}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{13.27152317880794640814201557077467441558837890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{8.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{5358}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.134794636818440505265925821731798350811004638671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.73832048567283525830617918472853489220142364501953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.6209428484556418492701368450070731341838836669921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{27584}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.47532880046932890483191158637055195868015289306640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.433295882262078435598340320211718790233135223388671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.05281829692878310666959151831179042346775531768798828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.58330082893370871488514239899814128875732421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.75101918889986762906119110994040966033935546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.46580183506011962890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.27288341522216796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7330192677988567329094848901149816811084747314453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2832050323486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.2182921731708855617171138874255120754241943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{19093}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.143050491809844970703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.142906188964844194089209850062616169452667236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.029478153242387498955690006141594494692981243133544921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.738847848959267139434814453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.62742695182759244953984989479067735373973846435546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{16069}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.476862838957458679001177870304672978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{28090}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.447968841530382577698077284367172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.052554440926168226322356957780357333831489086151123046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1415878655388951024018950874960864894092082977294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.11320334814168163395375898971906281076371669769287109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{7310}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.090771424816921297828997694523422978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08902535773813720354485923280662973411381244659423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0094075542218909867508980227057691081427037715911865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{152028813}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{121551169.5165562927722930908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{7310}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{97465075.25}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{95590250}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{10101284.4295921288430690765380859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.015990734100341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.07849087778306174101317083113826811313629150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.975169837474822998046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.8679935932159423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.53139427036718023256156584466225467622280120849609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.384105960264900403444698895327746868133544921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.991492892337950681991287638084031641483306884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{4729}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.97429747879505157470703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{22286}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97148817777633678094417746251565404236316680908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{16149}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00590009455785865839783088659942222875542938709259033203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.77083361732193178550431866824510507285594940185546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2940106}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2940106}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2940106}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{2940106}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{24173}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{12.9470198675496686036012761178426444530487060546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.99621854274628507397437715553678572177886962890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.739484707424746812165494702639989554882049560546875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.62799823735634152654938588966615498065948486328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{16069}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.478303778438801729944174212505458854138851165771484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.44830694207762256109361942435498349368572235107421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0522780491386653223262470646659494377672672271728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6924571990966796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.75857159001937901621204218827188014984130859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15043}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.577724516391754150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.5615355968475341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.72638021913569905674279425511485897004604339599609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2991282939910888671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{4800}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.218656869913568474572684863233007490634918212890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.143431007862091064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1420414447784423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0302100404004150592529587271428681560792028903961181640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.413109745830297414581622206242172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.33385799713556141288250955767580308020114898681640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{16069}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.248473510844632927696551405460922978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.232514522969722692291583143742172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0327739377939455511778987784055061638355255126953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.375500188209116403381671034367172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.31222315106713616206235428762738592922687530517578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{22401}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.2445781202986835600743376062382594682276248931884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{28090}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.235453393310308400909747206242172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.0283576242577882851880755055162808275781571865081787109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{403190257}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{335247055.72185432910919189453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{22401}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{262613757}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{28090}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{252816156}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{30448767.194864235818386077880859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.12237548828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.439607481293336377348168753087520599365234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.6455821990966796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.29946136474609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.5064594809721061352547621936537325382232666015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{68}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{41.11920529801324164509424008429050445556640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{29.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6532}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{28}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{6.46531976265284225036111820372752845287322998046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2397132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2397132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2397132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2397132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{34}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{24.21192052980132558559489552862942218780517578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{913}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6155}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.980309045540331158719027371262200176715850830078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.413465830562999514530275746437837369740009307861328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.33417096795463019365257650861167348921298980712890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{8893}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.2486168035766085082638454650805215351283550262451171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2326900112630350958564662278149626217782497406005859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.03272556456191665075206032042842707596719264984130859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6513054370880126953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.74331156465391501342310220934450626373291015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{32103}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.49796187877655029296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4768450260162353515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7359962149694856403669973587966524064540863037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.32684421539306640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.21797745590967831930129250395111739635467529296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{6549}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.1441166400909423828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24202}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.132311344146728515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.032141240590030629997730926561416708864271640777587890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.4154766835272312164306640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.329234488555137705390052360598929226398468017578125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{32382}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.244191022124141399185504042179672978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.221716025844216291229571424992172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03275011714765031778373582938002073206007480621337890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.378214078024029676239337049992172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.314948429001976337726631527402787469327449798583984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{16069}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.245768759399652425567950331242172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.235255469568073694031085096867172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.02874384630783359539929477932673762552440166473388671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{406104274}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{338173300.622516572475433349609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{16069}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{263892196}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{252603637}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{30863469.9633489139378070831298828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{142.3176116943359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.2863692732046700939463335089385509490966796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{30684}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.6405811309814453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.46202850341796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.42529095414309292522148098214529454708099365234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{69}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{42.35099337748344083820484229363501071929931640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{30}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{30}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{18289}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{6.64641383710011535157491380232386291027069091796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2411562}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2411562}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2411562}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2411562}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{34}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{25516}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{24.5165562913907280062630889005959033966064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{742}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{17.75}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{6155}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{17}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.985293544166891965829790933639742434024810791015625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.4157097376548632983173092725337482988834381103515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{27300}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.32954403209707028299391140535590238869190216064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{32382}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.244331450578977149579174010796123184263706207275390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.2218833640667000339785630558253615163266658782958984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.032712700471147070080402130543006933294236660003662109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6223361492156982421875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.74642805863690142587074660696089267730712890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{6082}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.63946235179901123046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.560866832733154296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7273867595673391139854402354103513062000274658203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.4121358394622802734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{7098}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.218834040180736710823339308262802660465240478515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{9816}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.139473855495452880859375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1316738128662109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.034236055514669357091595003339534741826355457305908203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.668210080824792385101318359375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{23367}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.542848150319857669643397457548417150974273681640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{22401}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.3978980346582829952239990234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.394104386679828111450518690617172978818416595458984375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.05328199351972374986363689686186262406408786773681640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.268531928770244121551513671875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.1772478241720144287452143316841102205216884613037109375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.1325111244805156907045073921835864894092082977294921875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.1309234229847787978062711999882594682276248931884765625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.022073769922508985896758559874797356314957141876220703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{288333963}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{190318402.0264900624752044677734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{29022}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{142282736.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{5615}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{140577955}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{2773}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{23701529.97915112972259521484375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{41.54341888427734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{17.3126035020840873812630889005959033966064453125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{8048}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{10.696970462799072265625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{10.537830352783203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27671}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{4.59898901089020117893824135535396635532379150390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{24}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{123}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{11.145695364238410007828861125744879245758056640625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{519}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{7}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{6159}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2236}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.99917970903661867954070885389228351414203643798828125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{13654}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.99418310821056365966796875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{12287}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.99345457553863525390625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{5781}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.00121658647182651034023004310569149311049841344356536865234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{2.47476629706278483666892498149536550045013427734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{4879728}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{4879728}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{4879728}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{4879728}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{30}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{26278}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{17.052980132450329620041884481906890869140625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{14929}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{10}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{14929}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.66979451482807572659794459468685090541839599609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.66843577337192938703225308927358128130435943603515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{23367}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.54334952048102180821587126047234050929546356201171875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{22401}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.39813937786019248932234404492191970348358154296875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{1951}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.3944018335030288202602832825505174696445465087890625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.053142881319121156036278108558690291829407215118408203125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.711990833282470703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.75315175782765919620942440815269947052001953125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{9132}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.594264686107635498046875}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.588262081146240234375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20415}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.71659443903751152138426050441921688616275787353515625}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.288826704025268998776709850062616169452667236328125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{12141}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.216415380010541724686845554970204830169677734375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{4157}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.14165604114532470703125}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{21598}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1384370326995849609375}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUMeanQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.03033447281144958929122168456160579808056354522705078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2646158}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2646158}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2646158}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{2646158}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.486072540283203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.44429664896023979281380889005959033966064453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.180627167224884033203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20415}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.0871791839599609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.73959861304431184780838748338283039629459381103515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.269814729690552201901709850062616169452667236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{30899}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.198760267914525723398355694371275603771209716796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{19917}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.126999378204345703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.118173122406005859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.028340896113934248290444628537443350069224834442138671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.4248905181884765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.426777032826910041052315136766992509365081787109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24173}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.4322891533374786376953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{23367}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.40823304653167724609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.6229550865539874582310631012660451233386993408203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3878959}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3878959}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3878959}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{3878959}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.5788686275482177734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{15043}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.44902894828493344903108663856983184814453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{2549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.294956862926483154296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.283283710479736328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20415}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7379337359393272066654390073381364345550537109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.4025633335113525390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{6589}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.201829845542149666215436809579841792583465576171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{12287}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.13258159160614013671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.127448558807373046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.03385236922199467979321951816018554382026195526123046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.27951812744140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.801418986541545308455170015804469585418701171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22545}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.205653667449951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.93181514739990234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.594245364275689524902190896682441234588623046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3622927}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3622927}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3622927}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3622927}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7467181682586669921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{15043}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.427092500080334502854384481906890869140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.30504691600799560546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20415}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.1307837963104248046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.72056982384623202708695544060901738703250885009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.273691892623901811276709850062616169452667236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{6532}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.2023468143892603876565772225148975849151611328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{12457}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.13302838802337646484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.119571208953857421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.03217139280887147678722470800494193099439144134521484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.0167236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.06559399105855145961641028407029807567596435546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1412}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.94751203060150146484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.535209767337012198851198263582773506641387939453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2864717}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2864717}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2864717}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{2864717}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6242630481719970703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{15043}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.42088321028955988367670215666294097900390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1696}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.34640753269195556640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.299345493316650390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20415}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7108956314705541235099417463061399757862091064453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2771766185760498046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{16069}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20186458676066632023093916359357535839080810546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{7790}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.136194407939910888671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1302583217620849609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.029816124918432836132797802974891965277493000030517578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.185821533203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.6145395948397407437369110994040966033935546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.5718860626220703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{77.82788848876953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.51010078068381492499838714138604700565338134765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2334413}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2334413}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2334413}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2334413}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.3412883281707763671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{15043}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.425397525559986888765706680715084075927734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1681}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.334612905979156494140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.2475779056549072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.70173618115506297687744563518208451569080352783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.262837886810302734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.202869067918385770354916530777700245380401611328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{2306}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.13145744800567626953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1271011829376220703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0305690146977181283205471373776163090951740741729736328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.38015460968017578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.8657478844093162706485600210726261138916015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1490}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.17229998111724853515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.9324092864990234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6180041988517543938286280535976402461528778076171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3631246}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3631246}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3631246}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3631246}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.4051401615142822265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.41078235613588987007460673339664936065673828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1490}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.312934458255767822265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.2329647541046142578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.707712353268588056920407325378619134426116943359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2640438079833984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{13468}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20109497158732647648093916359357535839080810546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{2549}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.122722148895263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.12050914764404296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0307331683379143856538195933580936980433762073516845703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.015990734100341796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.07849087778306174101317083113826811313629150390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{5781}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.975169837474822998046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.8679935932159423828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.53139427036718023256156584466225467622280120849609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2889674}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2889674}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2889674}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{2889674}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6160356998443603515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.4441377674506981065860600210726261138916015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1490}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.417535483837127685546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.254027843475341796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20415}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.71539190792449380840167805217788554728031158447265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3938472270965576171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{7310}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.204345155235947206762148198322393000125885009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{22286}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.12510168552398681640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.12239551544189453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.033502258236433428428835412660191650502383708953857421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.12237548828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.439607481293336377348168753087520599365234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.6455821990966796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.29946136474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.5064594809721061352547621936537325382232666015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2346700}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2346700}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2346700}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2346700}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.3869073390960693359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.43543059936422423561452887952327728271484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{24202}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.262150704860687255859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20415}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.0865573883056640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7229427988586782927171725532389245927333831787109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2689735889434814453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{32103}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.203187219354490355982534310896880924701690673828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{7790}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.1300008296966552734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1250140666961669921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24566}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.03042551951989240499596434119666810147464275360107421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{142.3176116943359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.2863692732046700939463335089385509490966796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{30684}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.6405811309814453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.46202850341796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.42529095414309292522148098214529454708099365234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2361130}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2361130}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2361130}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2361130}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.38217449188231711332264239899814128875732421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.4535253047943115234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.364409267902374267578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20415}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.136292934417724609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.72085131446758132778285244057769887149333953857421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2713363170623779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{13468}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20284471290790495601186194107867777347564697265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{2236}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.12559258937835693359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.121596813201904296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{24262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0310401350845224861807469807217785273678600788116455078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{41.54341888427734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{17.3126035020840873812630889005959033966064453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{8048}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{10.696970462799072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{10.537830352783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27671}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{4.59898901089020117893824135535396635532379150390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{4829296}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{4829296}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{4829296}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{4829296}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.46394062042236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.4140365613217369400445022620260715484619140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1185}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.40137779712677001953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.2266175746917724609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20415}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.70284874011298914542322791021433658897876739501953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2611014842987060546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.19947998886866269430129250395111739635467529296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.127018928527831587160790149937383830547332763671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{21317}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{2.119690418243408203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnDropAverageQueryPerOutputLogitReasoningAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.029621436027619567343815987214838969521224498748779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{10370}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2694542}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2694542}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2694542}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{2694542}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.5408723354339599609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.66074510915390050058704218827188014984130859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1681}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.736498296260833740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20415}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.556893825531005859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.6890362065933628432645718930871225893497467041015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2790267467498779296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{15662}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.207783195356659344810168477124534547328948974609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{12493}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.13216578960418701171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1198165416717529296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrExactEqkeMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0305233078452408594649636341955556417815387248992919921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{5.4248905181884765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{2.426777032826910041052315136766992509365081787109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{24173}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{1.4322891533374786376953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{23367}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{1.40823304653167724609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.6229550865539874582310631012660451233386993408203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3927343}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3927343}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3927343}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinFloat{3927343}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.504485607147216796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.66198164579883922442604671232402324676513671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{23696}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.644036233425140380859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.5057799816131591796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20415}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.70179021618498182988332700915634632110595703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.32278728485107421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMaxKey{17080}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.2110054729790089567131872172467410564422607421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMeanKey{12457}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.138189852237701416015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMedianKey{24173}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinFloat{2.133043766021728515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffExactOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0302133685469536499013099017929562251083552837371826171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.27951812744140625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.801418986541545308455170015804469585418701171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{22545}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.205653667449951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.93181514739990234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.594245364275689524902190896682441234588623046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3671311}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3671311}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3671311}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3671311}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.690355777740478515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.65626637667219966942866449244320392608642578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{26374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.622679233551025390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.5457413196563720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.684045674492151700718522988609038293361663818359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.343053817749022993410790149937383830547332763671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{13654}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.208690150684078812304278471856378018856048583984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{12493}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.135901808738708052004540149937383830547332763671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1334760189056396484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.032006427741537092634960259829313145019114017486572265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.0167236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.06559399105855145961641028407029807567596435546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1412}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.94751203060150146484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.535209767337012198851198263582773506641387939453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2913101}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2913101}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2913101}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{2913101}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.547040462493896484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.65158633996319537118324660696089267730712890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{30899}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.633177936077117919921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.574159145355224609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.68349549908705464762448400506400503218173980712890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.270458698272705078125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{14095}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.2116289880891510932769961073063313961029052734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{12457}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.138825893402099609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{21317}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.131032466888427734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.02851425517130525000286667136606411077082157135009765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.185821533203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.6145395948397407437369110994040966033935546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.5718860626220703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{77.82788848876953125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.51010078068381492499838714138604700565338134765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2382797}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2382797}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2382797}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2382797}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.75147438049317116792735760100185871124267578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.66237932325199011529548442922532558441162109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7310}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.929292619228363037109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.6591660976409912109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.67499539310229372812699466521735303103923797607421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2866055965423583984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{13654}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.210690645192632697302315136766992509365081787109375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{2743}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.13649451732635498046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{21317}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1363275051116943359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0285771028598807257103953105570326442830264568328857421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{14.38015460968017578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{7467}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{8.8657478844093162706485600210726261138916015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1490}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{6.17229998111724853515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{12457}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{5.9324092864990234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundMinKey{6159}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.6180041988517543938286280535976402461528778076171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3679630}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3679630}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianFloat{3679630}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinFloat{3679630}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.802142620086669921875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.6585461240730552390232332982122898101806640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{2773}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.58177602291107177734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.4241669178009033203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.68759734292416208045750636301818303763866424560546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2693309783935546875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMaxKey{14929}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.20712959687441401257501638610847294330596923828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMeanKey{27300}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.13397276401519775390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1333444118499755859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0291123868369714024206817981621497892774641513824462890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{7.015990734100341796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{4647}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.07849087778306174101317083113826811313629150390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{5781}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.975169837474822998046875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.8679935932159423828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{0.53139427036718023256156584466225467622280120849609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2938058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2938058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2938058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinFloat{2938058}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.71030521392822265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.684654603730763255953206680715084075927734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{8893}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.670774042606353759765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.59304523468017578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.6657644983118402581823147556860931217670440673828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2774269580841064453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMaxKey{30899}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.212592184938342310118741806945763528347015380859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMeanKey{12457}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.139128625392913818359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinFloat{2.132236957550048828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.029344322331519588631376649345838814042508602142333984375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{144.12237548828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{94.439607481293336377348168753087520599365234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{16149}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{78.6455821990966796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.29946136474609375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.5064594809721061352547621936537325382232666015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2395084}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2395084}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2395084}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2395084}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.65674591064453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.69254225610897179876701557077467441558837890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{12457}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.591224253177642822265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.580876827239990234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.69388082744023638070984816295094788074493408203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.307238101959228515625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{4647}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.210882403203193735663489860598929226398468017578125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{5928}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.134443700313568115234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{24438}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1325709819793701171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0308721494563566657698405748533332371152937412261962890625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6530}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{142.3176116943359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{96.2863692732046700939463335089385509490966796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{30684}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{79.6405811309814453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{78.46202850341796875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundMinKey{1681}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{7.42529095414309292522148098214529454708099365234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxFloat{2409514}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanFloat{2409514}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2409514}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinFloat{2409514}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6921765804290771484375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.6750413518867759421482332982122898101806640625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1681}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.917321383953094482421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.61393833160399680082264239899814128875732421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.6826413421076387155750353485927917063236236572265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.3525607585906982421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMaxKey{16197}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.21215781944477019038686194107867777347564697265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMeanKey{23241}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.143588542938232421875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMedianKey{21598}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinFloat{2.141717433929443359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeMinKey{22261}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrMeanRecursiveMaxDiffSubproductRecursiveOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.031495518889367697668024703716582735069096088409423828125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.00000005029141902923584646119490042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMaxKey{12552}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.00000004777499776802315490149237011720251278035220821038819849491119384765625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMeanKey{742}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.00000004447065293788910573853865042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0000000010867058880102657952281753803679131831216864156886003911495208740234375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6402}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{41.54341888427734375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{123}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{17.3126035020840873812630889005959033966064453125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{8048}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{10.696970462799072265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{32374}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{10.537830352783203125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundMinKey{27671}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{4.59898901089020117893824135535396635532379150390625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxFloat{4877680}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanFloat{4877680}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianFloat{4877680}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinFloat{4877680}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMaxKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMeanKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMedianKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinFloat{1}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapMinKey{50}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedMaxGapStdDevFloat{0}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.0000000503547585037589476267987954882787704491420299746096134185791015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{24144}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.00000004782042352441918734063072454927578736061377639998681843280792236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{5615}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.00000004459868605445639042751689961989469690450960115413181483745574951171875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{11498}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.00000000107125194952379480809302484344523731518705744747421704232692718505859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6405162811279296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.66905683081671440959325991570949554443359375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{7238}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.685733795166015625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20338}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.6433541774749755859375}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20294}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.6934002494159108298532601111219264566898345947265625}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2723586559295654296875}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMaxKey{31308}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.2073120186660464270289594423957169055938720703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMeanKey{12561}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.134781360626220703125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinFloat{2.127907037734985795651709850062616169452667236328125}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicEUPUSvdQueryMaxDiffAttnMeanQueryDiffAttnErrSvdOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0290936957846073436517730925743308034725487232208251953125}
\def\SubcubicEffectiveDimensionalityEstimateLen{7852}
\def\SubcubicEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicEffectiveDimensionalityEstimateMeanFloat{5662.76923076923048938624560832977294921875}
\def\SubcubicEffectiveDimensionalityEstimateMedianFloat{4290}
\def\SubcubicEffectiveDimensionalityEstimateMinFloat{4290}
\def\SubcubicEffectiveDimensionalityEstimateStdDevFloat{2046.997581970168312182067893445491790771484375}
\def\SubcubicErrUpperBoundLen{7852}
\def\SubcubicErrUpperBoundMaxFloat{144.185821533203125}
\def\SubcubicErrUpperBoundMeanFloat{25.887024167175507471938544767908751964569091796875}
\def\SubcubicErrUpperBoundMedianFloat{0}
\def\SubcubicErrUpperBoundMinFloat{0}
\def\SubcubicErrUpperBoundStdDevFloat{38.378400476443317757002660073339939117431640625}
\def\SubcubicGapMostBelowValueLen{7852}
\def\SubcubicGapMostBelowValueMaxFloat{61}
\def\SubcubicGapMostBelowValueMeanFloat{11.5086602139582279136220677173696458339691162109375}
\def\SubcubicGapMostBelowValueMedianFloat{1}
\def\SubcubicGapMostBelowValueMinFloat{1}
\def\SubcubicGapMostBelowValueNumStdLen{7852}
\def\SubcubicGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicGapMostBelowValueSequenceFracLen{7852}
\def\SubcubicGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicGapMostBelowValueSequenceFracMeanFloat{0.9920393778423963748736014167661778628826141357421875}
\def\SubcubicGapMostBelowValueSequenceFracMedianFloat{0.9577003923058509116117420489899814128875732421875}
\def\SubcubicGapMostBelowValueSequenceFracMinFloat{0.9398634433746337890625}
\def\SubcubicGapMostBelowValueSequenceFracStdDevFloat{0.00942486226645522680300803841646484215743839740753173828125}
\def\SubcubicGapMostBelowValueStdDevFloat{12.6073506034814766252338813501410186290740966796875}
\def\SubcubicGroupAccuracyLen{1208}
\def\SubcubicGroupAccuracyMaxFloat{0.780931304208934307098388671875}
\def\SubcubicGroupAccuracyMeanFloat{0.51525952858042389781445535845705308020114898681640625}
\def\SubcubicGroupAccuracyMedianFloat{0.1308169688563793620073028023398364894092082977294921875}
\def\SubcubicGroupAccuracyMinFloat{0.08011294342577450489084611717771622352302074432373046875}
\def\SubcubicGroupAccuracyStdDevFloat{0.1733672379728860291070446919547975994646549224853515625}
\def\SubcubicGroupDroppedSequencesFracLen{1208}
\def\SubcubicGroupDroppedSequencesFracMaxFloat{0.1285205837339161993870817468632594682276248931884765625}
\def\SubcubicGroupDroppedSequencesFracMeanFloat{0.08459601358476627475102560538289253599941730499267578125}
\def\SubcubicGroupDroppedSequencesFracMedianFloat{0.06339302442036565121696867208811454474925994873046875}
\def\SubcubicGroupDroppedSequencesFracMinFloat{0.058046793565153999294725650770487845875322818756103515625}
\def\SubcubicGroupDroppedSequencesFracStdDevFloat{0.01018637047821040024497829534766424330882728099822998046875}
\def\SubcubicGroupDroppedSequencesLen{1208}
\def\SubcubicGroupDroppedSequencesMaxFloat{137997926}
\def\SubcubicGroupDroppedSequencesMeanFloat{90834277.9296357631683349609375}
\def\SubcubicGroupDroppedSequencesMedianFloat{68067741.67000000178813934326171875}
\def\SubcubicGroupDroppedSequencesMinFloat{62327270}
\def\SubcubicGroupDroppedSequencesStdDevFloat{10937532.01721338741481304168701171875}
\def\SubcubicGroupEffectiveDimensionalityEstimateLen{1208}
\def\SubcubicGroupEffectiveDimensionalityEstimateMaxFloat{8384}
\def\SubcubicGroupEffectiveDimensionalityEstimateMeanFloat{6401}
\def\SubcubicGroupEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicGroupEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicGroupEffectiveDimensionalityEstimateStdDevFloat{1921.033315692364567439653910696506500244140625}
\def\SubcubicGroupErrUpperBoundLen{1208}
\def\SubcubicGroupErrUpperBoundMaxFloat{5.4248905181884765625}
\def\SubcubicGroupErrUpperBoundMeanFloat{1.2133885164134550205261575683834962546825408935546875}
\def\SubcubicGroupErrUpperBoundMedianFloat{0}
\def\SubcubicGroupErrUpperBoundMinFloat{0}
\def\SubcubicGroupErrUpperBoundStdDevFloat{1.290871105763773840635622036643326282501220703125}
\def\SubcubicGroupGapMostBelowValueLen{1208}
\def\SubcubicGroupGapMostBelowValueMaxFloat{7}
\def\SubcubicGroupGapMostBelowValueMeanFloat{4.16059602649006610164406083640642464160919189453125}
\def\SubcubicGroupGapMostBelowValueMedianFloat{3}
\def\SubcubicGroupGapMostBelowValueMinFloat{3}
\def\SubcubicGroupGapMostBelowValueNumStdLen{1208}
\def\SubcubicGroupGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicGroupGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicGroupGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicGroupGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicGroupGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicGroupGapMostBelowValueSequenceFracLen{1208}
\def\SubcubicGroupGapMostBelowValueSequenceFracMaxFloat{0.99992173910141002313167746251565404236316680908203125}
\def\SubcubicGroupGapMostBelowValueSequenceFracMeanFloat{0.986144606838163184647783054970204830169677734375}
\def\SubcubicGroupGapMostBelowValueSequenceFracMedianFloat{0.9527435654401779085986845529987476766109466552734375}
\def\SubcubicGroupGapMostBelowValueSequenceFracMinFloat{0.94308298826217640264957253748434595763683319091796875}
\def\SubcubicGroupGapMostBelowValueSequenceFracStdDevFloat{0.010686424133214376952505375584223656915128231048583984375}
\def\SubcubicGroupGapMostBelowValueStdDevFloat{0.68137738547824200363578484029858373105525970458984375}
\def\SubcubicGroupInstructionCountBranchLen{1208}
\def\SubcubicGroupInstructionCountBranchMaxFloat{0}
\def\SubcubicGroupInstructionCountBranchMeanFloat{0}
\def\SubcubicGroupInstructionCountBranchMedianFloat{0}
\def\SubcubicGroupInstructionCountBranchMinFloat{0}
\def\SubcubicGroupInstructionCountBranchStdDevFloat{0}
\def\SubcubicGroupInstructionCountIntLen{1208}
\def\SubcubicGroupInstructionCountIntMaxFloat{0}
\def\SubcubicGroupInstructionCountIntMeanFloat{0}
\def\SubcubicGroupInstructionCountIntMedianFloat{0}
\def\SubcubicGroupInstructionCountIntMinFloat{0}
\def\SubcubicGroupInstructionCountIntStdDevFloat{0}
\def\SubcubicGroupInstructionCountLen{1208}
\def\SubcubicGroupInstructionCountMaxFloat{4193742}
\def\SubcubicGroupInstructionCountMeanFloat{3549022}
\def\SubcubicGroupInstructionCountMedianFloat{2904302}
\def\SubcubicGroupInstructionCountMinFloat{2904302}
\def\SubcubicGroupInstructionCountStdDevFloat{616888.859941967180930078029632568359375}
\def\SubcubicGroupMaxGapLen{1208}
\def\SubcubicGroupMaxGapMaxFloat{21}
\def\SubcubicGroupMaxGapMeanFloat{14.1854304635761589992171138874255120754241943359375}
\def\SubcubicGroupMaxGapMedianFloat{6}
\def\SubcubicGroupMaxGapMinFloat{6}
\def\SubcubicGroupMaxGapStdDevFloat{3.05800214724939412036519570392556488513946533203125}
\def\SubcubicGroupNormalizedAccuracyLen{1208}
\def\SubcubicGroupNormalizedAccuracyMaxFloat{0.7812433963450775564751893398351967334747314453125}
\def\SubcubicGroupNormalizedAccuracyMeanFloat{0.5157531532695056597503935336135327816009521484375}
\def\SubcubicGroupNormalizedAccuracyMedianFloat{0.1309076725628232906739611962620983831584453582763671875}
\def\SubcubicGroupNormalizedAccuracyMinFloat{0.080185004802162340720173006047843955457210540771484375}
\def\SubcubicGroupNormalizedAccuracyStdDevFloat{0.1735210479248866788370975200450629927217960357666015625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.780931304208934307098388671875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMaxKey{29110}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.70144876013725798724607329859281890094280242919921875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMeanKey{16149}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.59544845041818916797637939453125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMedianKey{2236}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMinFloat{0.59265005774796009063720703125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyMinKey{1951}
\def\SubcubicGroupOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.03264304729260390780520850739776506088674068450927734375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.104468864388763904571533203125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{4800}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.07811759208754588679202157663894467987120151519775390625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{12287}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.061983633786439847057625485149401356466114521026611328125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{2743}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.058046793565153999294725650770487845875322818756103515625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00873069279015799108722983845609633135609328746795654296875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{112172589}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{4800}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{83878125.814569532871246337890625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{12287}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{66554420}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{2743}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{62327270}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicGroupOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{9374510.0012878887355327606201171875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{8384}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{123}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6973.642384105960445594973862171173095703125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{4647}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4418}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{104}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4418}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{104}
\def\SubcubicGroupOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{1853.252563512014376101433299481868743896484375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{4.0297718048095703125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{104}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{0.869221426793281626288489860598929226398468017578125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{6159}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{123}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundMinKey{123}
\def\SubcubicGroupOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.21258912908612526138085740967653691768646240234375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{6}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2773}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{3.834437086092715052387802643352188169956207275390625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.99992173910141002313167746251565404236316680908203125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2773}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.98396798593319012571356552143697626888751983642578125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{11598}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.94983610510826121942073996251565404236316680908203125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{1185}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.943215072154998779296875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2345}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01291617579653729641631088043141062371432781219482421875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.63486415688513186950103772687725722789764404296875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMaxFloat{4193742}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMaxKey{104}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3402484.841059602797031402587890625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMeanKey{4647}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2952686}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMedianKey{123}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMinFloat{2952686}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountMinKey{123}
\def\SubcubicGroupOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{593577.773679104633629322052001953125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMaxFloat{19}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.403973509933774010960405576042830944061279296875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMeanKey{1951}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMedianKey{2743}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapMinKey{2743}
\def\SubcubicGroupOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.370287399644644299456786029622890055179595947265625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7812433963450775564751893398351967334747314453125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29110}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.702115802284000611876990660675801336765289306640625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{16149}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.5957883693044145889672336124931462109088897705078125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{2236}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.59298062177469235134452674174099229276180267333984375}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1951}
\def\SubcubicGroupOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.032557212322985841501665760233663604594767093658447265625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7359836101531982421875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.651228836830085811016033403575420379638671875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{1490}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.74832755327224020902576739899814128875732421875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.6372649669647216796875}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.72593005730507853545674379347474314272403717041015625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2972538471221923828125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMaxKey{5358}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.21515968619592928945394305628724396228790283203125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMeanKey{29565}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.136838018894195556640625}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMedianKey{21598}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1362316608428955078125}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicGroupOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.0316540672148004353925188070206786505877971649169921875}
\def\SubcubicGroupProofSearchTimeLen{1208}
\def\SubcubicGroupProofSearchTimeMaxFloat{46.7359836101531982421875}
\def\SubcubicGroupProofSearchTimeMeanFloat{44.512903076528715473614283837378025054931640625}
\def\SubcubicGroupProofSearchTimeMedianFloat{42.30079880118370283526019193232059478759765625}
\def\SubcubicGroupProofSearchTimeMinFloat{42.1480529308319091796875}
\def\SubcubicGroupProofSearchTimeStdDevFloat{0.7518574867828504704192482677171938121318817138671875}
\def\SubcubicGroupProofTimeLen{1208}
\def\SubcubicGroupProofTimeMaxFloat{2.322057723999022993410790149937383830547332763671875}
\def\SubcubicGroupProofTimeMeanFloat{2.2084913551807403564453125}
\def\SubcubicGroupProofTimeMedianFloat{2.1360663604736327414457264239899814128875732421875}
\def\SubcubicGroupProofTimeMinFloat{2.1258227825164794921875}
\def\SubcubicGroupProofTimeStdDevFloat{0.0301848402590701829495412056303393910638988018035888671875}
\def\SubcubicInstructionCountBranchLen{7852}
\def\SubcubicInstructionCountBranchMaxFloat{0}
\def\SubcubicInstructionCountBranchMeanFloat{0}
\def\SubcubicInstructionCountBranchMedianFloat{0}
\def\SubcubicInstructionCountBranchMinFloat{0}
\def\SubcubicInstructionCountBranchStdDevFloat{0}
\def\SubcubicInstructionCountIntLen{7852}
\def\SubcubicInstructionCountIntMaxFloat{0}
\def\SubcubicInstructionCountIntMeanFloat{0}
\def\SubcubicInstructionCountIntMedianFloat{0}
\def\SubcubicInstructionCountIntMinFloat{0}
\def\SubcubicInstructionCountIntStdDevFloat{0}
\def\SubcubicInstructionCountLen{7852}
\def\SubcubicInstructionCountMaxFloat{5144079}
\def\SubcubicInstructionCountMeanFloat{3394938.65384615398943424224853515625}
\def\SubcubicInstructionCountMedianFloat{2592557}
\def\SubcubicInstructionCountMinFloat{2592557}
\def\SubcubicInstructionCountStdDevFloat{751086.947580174193717539310455322265625}
\def\SubcubicMaxGapLen{7852}
\def\SubcubicMaxGapMaxFloat{31}
\def\SubcubicMaxGapMeanFloat{15.3516301579215479478079942055046558380126953125}
\def\SubcubicMaxGapMedianFloat{1}
\def\SubcubicMaxGapMinFloat{1}
\def\SubcubicMaxGapStdDevFloat{6.39661849040693741841323571861721575260162353515625}
\def\SubcubicNormalizedAccuracyLen{7852}
\def\SubcubicNormalizedAccuracyMaxFloat{0.7812433963450775564751893398351967334747314453125}
\def\SubcubicNormalizedAccuracyMeanFloat{0.356151502732036051579456170657067559659481048583984375}
\def\SubcubicNormalizedAccuracyMedianFloat{0.0000000456737632951827134069643153273243552092708341660909354686737060546875}
\def\SubcubicNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicNormalizedAccuracyStdDevFloat{0.232128681605360487338884922792203724384307861328125}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.780931304208934307098388671875}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMaxKey{29110}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.70537861965794046437139286354067735373973846435546875}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMeanKey{10248}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.6119701839052140712738037109375}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMedianKey{12552}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMinFloat{0.59265005774796009063720703125}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyMinKey{1951}
\def\SubcubicOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.0310671816446796665578400364893241203390061855316162109375}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.12679875083267688751220703125}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.08391068376206005374751129011201555840671062469482421875}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{5781}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.06227796920575197348046714296287973411381244659423828125}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{2345}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.058046793565153999294725650770487845875322818756103515625}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{29110}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.01268794889335365938531907659125863574445247650146484375}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{136149122}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{90098410.6357615888118743896484375}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{5781}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{66870460.25}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{2345}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{62327270}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesMinKey{29110}
\def\SubcubicOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{13623581.38756833784282207489013671875}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{10370}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{2236}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{7080.6490066225169357494451105594635009765625}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{1185}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{4402}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{104}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{4354}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{24144}
\def\SubcubicOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{2075.01463873772081569768488407135009765625}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{9.37257671356201171875}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{17194}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{1.492547126795282341760184863233007490634918212890625}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{27714}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{123}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundMinKey{123}
\def\SubcubicOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{2.267698926495981925910427889903075993061065673828125}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{8}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{2236}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{4.16556291390728450352298750658519566059112548828125}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{3}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{3}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{0.999912261962890625}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{2773}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9853469997841790561921015978441573679447174072265625}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{6910}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.95145584642887115478515625}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{913}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.943215072154998779296875}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{2345}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.01196093248701758648966375631061964668333530426025390625}
\def\SubcubicOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.87972349340561961650308830940048210322856903076171875}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMaxFloat{4193742}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMaxKey{104}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3312777.3642384107224643230438232421875}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMeanKey{5928}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2696590}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMedianKey{2236}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMinFloat{2696590}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountMinKey{2236}
\def\SubcubicOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{556895.864682440995238721370697021484375}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMaxFloat{19}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMaxKey{4800}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMeanFloat{14.132450331125827602818390005268156528472900390625}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMeanKey{1951}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMedianFloat{6.75}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMedianKey{6159}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMinFloat{6}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapMinKey{27300}
\def\SubcubicOnlyBestAccBoundPerSeedMaxGapStdDevFloat{2.720234448136964022779693550546653568744659423828125}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.7812433963450775564751893398351967334747314453125}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{29110}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.70604884924443778171365693197003565728664398193359375}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{3284}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.612295080253672185932600768865086138248443603515625}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.59298062177469235134452674174099229276180267333984375}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1951}
\def\SubcubicOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.0309600961157661565270604597799319890327751636505126953125}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.7359836101531982421875}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.65898868737631488556871772743761539459228515625}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{12141}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.74832755327224020902576739899814128875732421875}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.6372649669647216796875}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20013}
\def\SubcubicOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.7004619892651062773580861176014877855777740478515625}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2972538471221923828125}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMaxKey{5358}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.2151392137767462742203861125744879245758056640625}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMeanKey{13293}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.1408836841583251953125}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMedianKey{24262}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1362316608428955078125}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeMinKey{24438}
\def\SubcubicOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.031038837999946923551508604077753261663019657135009765625}
\def\SubcubicProofSearchTimeLen{7852}
\def\SubcubicProofSearchTimeMaxFloat{46.9079892635345458984375}
\def\SubcubicProofSearchTimeMeanFloat{44.53505231352770721287015476264059543609619140625}
\def\SubcubicProofSearchTimeMedianFloat{42.34085793256759444602721487171947956085205078125}
\def\SubcubicProofSearchTimeMinFloat{41.9884622097015380859375}
\def\SubcubicProofSearchTimeStdDevFloat{0.74820566467044147263010245296754874289035797119140625}
\def\SubcubicProofTimeLen{7852}
\def\SubcubicProofTimeMaxFloat{2.48164653778076171875}
\def\SubcubicProofTimeMeanFloat{2.209232359289576397287646614131517708301544189453125}
\def\SubcubicProofTimeMedianFloat{2.131941870450973386397208741982467472553253173828125}
\def\SubcubicProofTimeMinFloat{2.118173122406005859375}
\def\SubcubicProofTimeStdDevFloat{0.0311874749880815781144516307676894939504563808441162109375}
\def\SubcubicVocabModelSquaredAccuracyLen{7248}
\def\SubcubicVocabModelSquaredAccuracyMaxFloat{0.73887385241687297821044921875}
\def\SubcubicVocabModelSquaredAccuracyMeanFloat{0.10937238002653905388772415108178392983973026275634765625}
\def\SubcubicVocabModelSquaredAccuracyMedianFloat{0.00000004470348358154297536744490042422139897126953655970282852649688720703125}
\def\SubcubicVocabModelSquaredAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicVocabModelSquaredAccuracyStdDevFloat{0.193281432383117623974300158806727267801761627197265625}
\def\SubcubicVocabModelSquaredDroppedSequencesFracLen{7248}
\def\SubcubicVocabModelSquaredDroppedSequencesFracMaxFloat{0.378214078024029676239337049992172978818416595458984375}
\def\SubcubicVocabModelSquaredDroppedSequencesFracMeanFloat{0.11502826510849932517555060940139810554683208465576171875}
\def\SubcubicVocabModelSquaredDroppedSequencesFracMedianFloat{0}
\def\SubcubicVocabModelSquaredDroppedSequencesFracMinFloat{0}
\def\SubcubicVocabModelSquaredDroppedSequencesFracStdDevFloat{0.10755488953301210741653193281308631412684917449951171875}
\def\SubcubicVocabModelSquaredDroppedSequencesLen{7248}
\def\SubcubicVocabModelSquaredDroppedSequencesMaxFloat{406104274}
\def\SubcubicVocabModelSquaredDroppedSequencesMeanFloat{123510659.18915562331676483154296875}
\def\SubcubicVocabModelSquaredDroppedSequencesMedianFloat{0}
\def\SubcubicVocabModelSquaredDroppedSequencesMinFloat{0}
\def\SubcubicVocabModelSquaredDroppedSequencesStdDevFloat{115486183.267294943332672119140625}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateLen{7248}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateMeanFloat{6468.6666666666669698315672576427459716796875}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateMedianFloat{6338}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateMinFloat{6338}
\def\SubcubicVocabModelSquaredEffectiveDimensionalityEstimateStdDevFloat{53.7979760048853705711735528893768787384033203125}
\def\SubcubicVocabModelSquaredErrUpperBoundLen{7248}
\def\SubcubicVocabModelSquaredErrUpperBoundMaxFloat{144.185821533203125}
\def\SubcubicVocabModelSquaredErrUpperBoundMeanFloat{41.3080464489017913365387357771396636962890625}
\def\SubcubicVocabModelSquaredErrUpperBoundMedianFloat{4.1212482452392578125}
\def\SubcubicVocabModelSquaredErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicVocabModelSquaredErrUpperBoundStdDevFloat{42.12034017668036511850004899315536022186279296875}
\def\SubcubicVocabModelSquaredGapMostBelowValueLen{7248}
\def\SubcubicVocabModelSquaredGapMostBelowValueMaxFloat{73}
\def\SubcubicVocabModelSquaredGapMostBelowValueMeanFloat{14.002621412803531342206042609177529811859130859375}
\def\SubcubicVocabModelSquaredGapMostBelowValueMedianFloat{1}
\def\SubcubicVocabModelSquaredGapMostBelowValueMinFloat{1}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdLen{7248}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicVocabModelSquaredGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracLen{7248}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracMeanFloat{0.9972461153964859992271385635831393301486968994140625}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracMedianFloat{0.9758636897802352994091279470012523233890533447265625}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracMinFloat{0.943529903888702392578125}
\def\SubcubicVocabModelSquaredGapMostBelowValueSequenceFracStdDevFloat{0.005148318124377773523370205310811797971837222576141357421875}
\def\SubcubicVocabModelSquaredGapMostBelowValueStdDevFloat{16.703503511300734629685393883846700191497802734375}
\def\SubcubicVocabModelSquaredInstructionCountBranchLen{7248}
\def\SubcubicVocabModelSquaredInstructionCountBranchMaxFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountBranchMeanFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountBranchMedianFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountBranchMinFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountBranchStdDevFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntLen{7248}
\def\SubcubicVocabModelSquaredInstructionCountIntMaxFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntMeanFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntMedianFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntMinFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountIntStdDevFloat{0}
\def\SubcubicVocabModelSquaredInstructionCountLen{7248}
\def\SubcubicVocabModelSquaredInstructionCountMaxFloat{4879728}
\def\SubcubicVocabModelSquaredInstructionCountMeanFloat{3135570.2083333334885537624359130859375}
\def\SubcubicVocabModelSquaredInstructionCountMedianFloat{2334413}
\def\SubcubicVocabModelSquaredInstructionCountMinFloat{2334413}
\def\SubcubicVocabModelSquaredInstructionCountStdDevFloat{817705.277852396480739116668701171875}
\def\SubcubicVocabModelSquaredMaxGapLen{7248}
\def\SubcubicVocabModelSquaredMaxGapMaxFloat{34}
\def\SubcubicVocabModelSquaredMaxGapMeanFloat{11.475993377483444390918521094135940074920654296875}
\def\SubcubicVocabModelSquaredMaxGapMedianFloat{1}
\def\SubcubicVocabModelSquaredMaxGapMinFloat{1}
\def\SubcubicVocabModelSquaredMaxGapStdDevFloat{8.8644892587751886736668893718160688877105712890625}
\def\SubcubicVocabModelSquaredNormalizedAccuracyLen{7248}
\def\SubcubicVocabModelSquaredNormalizedAccuracyMaxFloat{0.73951073329633432162921735653071664273738861083984375}
\def\SubcubicVocabModelSquaredNormalizedAccuracyMeanFloat{0.10947465346607411496027140174192027188837528228759765625}
\def\SubcubicVocabModelSquaredNormalizedAccuracyMedianFloat{0.00000004477619510034710918767376810860347813303405928309075534343719482421875}
\def\SubcubicVocabModelSquaredNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicVocabModelSquaredNormalizedAccuracyStdDevFloat{0.19344815414369709305475453220424242317676544189453125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.73887385241687297821044921875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.6284136571335476872945946524851024150848388671875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMeanKey{16069}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.476927766110747997085894667179672978818416595458984375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMedianKey{28090}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMinFloat{0.448228550143539905548095703125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.05289101732648844589323999798580189235508441925048828125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1415878655388951024018950874960864894092082977294921875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.11406609109473342389406980146304704248905181884765625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{19488}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.090771424816921297828997694523422978818416595458984375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08902535773813720354485923280662973411381244659423828125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1951}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00999342711442975650815156996031873859465122222900390625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{152028813}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{122477532.70860926806926727294921875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{19488}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{97465075.25}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{95590250}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1951}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{10730360.65785886161029338836669921875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{519}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6496.5165562913907706388272345066070556640625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{31.965597050006547164002768113277852535247802734375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{11.34843730926513671875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24202}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.53126487352990192647439471329562366008758544921875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1283}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.94751203060150146484375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.3131957128378595189843736079637892544269561767578125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{10}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.4370860927152317998434227774851024150848388671875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9919348280161421893552642359281890094280242919921875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19451}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9755818843841552734375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11611}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97523391246795643194644753748434595763683319091796875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{22286}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005465507854250783482952247283037650049664080142974853515625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.75971551786489988078443502672598697245121002197265625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3681678}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMaxKey{5928}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3036414.85430463589727878570556640625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMeanKey{519}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2915149}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMinFloat{2915149}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{264854.7799246955546550452709197998046875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMaxKey{24173}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMeanFloat{13}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMedianKey{6159}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapMinKey{6159}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.012116810835729463491361457272432744503021240234375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.73951073329633432162921735653071664273738861083984375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.62898558894671052765801277928403578698635101318359375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6589}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.47971102572393864438282662376877851784229278564453125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.44856684670357382938021828522323630750179290771484375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.052613537072433415320293903505444177426397800445556640625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6924571990966796875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.76375394625379300350687117315828800201416015625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15043}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.6303670406341552734375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.583120822906494140625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.71642306767657737420762487090541981160640716552734375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2991282939910888671875}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMaxKey{4800}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.219771784662410762933859587064944207668304443359375}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMeanKey{12457}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.146164476871490478515625}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1422092914581298828125}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicVocabModelSquaredOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.02928460812333964768949812196296988986432552337646484375}
\def\SubcubicVocabModelSquaredProofSearchTimeLen{7248}
\def\SubcubicVocabModelSquaredProofSearchTimeMaxFloat{52.45428371429443359375}
\def\SubcubicVocabModelSquaredProofSearchTimeMeanFloat{44.57716329454981263324953033588826656341552734375}
\def\SubcubicVocabModelSquaredProofSearchTimeMedianFloat{42.38949258208274528669790015555918216705322265625}
\def\SubcubicVocabModelSquaredProofSearchTimeMinFloat{42.007546901702880859375}
\def\SubcubicVocabModelSquaredProofSearchTimeStdDevFloat{0.73353910463281923881595503189601004123687744140625}
\def\SubcubicVocabModelSquaredProofTimeLen{7248}
\def\SubcubicVocabModelSquaredProofTimeMaxFloat{2.6413619518280029296875}
\def\SubcubicVocabModelSquaredProofTimeMeanFloat{2.208540885620822624701986569561995565891265869140625}
\def\SubcubicVocabModelSquaredProofTimeMedianFloat{2.130901585817337018369244105997495353221893310546875}
\def\SubcubicVocabModelSquaredProofTimeMinFloat{2.1170752048492431640625}
\def\SubcubicVocabModelSquaredProofTimeStdDevFloat{0.03221058931196159325072159163028118200600147247314453125}
\def\SubcubicWithoutVocabSquaredAccuracyLen{4530}
\def\SubcubicWithoutVocabSquaredAccuracyMaxFloat{0.73887385241687297821044921875}
\def\SubcubicWithoutVocabSquaredAccuracyMeanFloat{0.1315056148433346450143943684452096931636333465576171875}
\def\SubcubicWithoutVocabSquaredAccuracyMedianFloat{0.00000004470348358154297536744490042422139897126953655970282852649688720703125}
\def\SubcubicWithoutVocabSquaredAccuracyMinFloat{0.00000004377216100692749685181990042422139897126953655970282852649688720703125}
\def\SubcubicWithoutVocabSquaredAccuracyStdDevFloat{0.222434889164279392392842282788478769361972808837890625}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracLen{4530}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracMaxFloat{0.268531928770244121551513671875}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracMeanFloat{0.07538373267882507444692663511887076310813426971435546875}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracMedianFloat{0}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracMinFloat{0}
\def\SubcubicWithoutVocabSquaredDroppedSequencesFracStdDevFloat{0.0586854999373065677747973722944152541458606719970703125}
\def\SubcubicWithoutVocabSquaredDroppedSequencesLen{4530}
\def\SubcubicWithoutVocabSquaredDroppedSequencesMaxFloat{288333963}
\def\SubcubicWithoutVocabSquaredDroppedSequencesMeanFloat{80942666.62649007141590118408203125}
\def\SubcubicWithoutVocabSquaredDroppedSequencesMedianFloat{0}
\def\SubcubicWithoutVocabSquaredDroppedSequencesMinFloat{0}
\def\SubcubicWithoutVocabSquaredDroppedSequencesStdDevFloat{63013075.745035469532012939453125}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateLen{4530}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateMeanFloat{6457.4666666666662422358058393001556396484375}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateMedianFloat{6338}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateMinFloat{6338}
\def\SubcubicWithoutVocabSquaredEffectiveDimensionalityEstimateStdDevFloat{56.60372975539882389739432255737483501434326171875}
\def\SubcubicWithoutVocabSquaredErrUpperBoundLen{4530}
\def\SubcubicWithoutVocabSquaredErrUpperBoundMaxFloat{41.54341888427734375}
\def\SubcubicWithoutVocabSquaredErrUpperBoundMeanFloat{9.0247710483753120769279121304862201213836669921875}
\def\SubcubicWithoutVocabSquaredErrUpperBoundMedianFloat{4.010895252227783203125}
\def\SubcubicWithoutVocabSquaredErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicWithoutVocabSquaredErrUpperBoundStdDevFloat{5.03767082298718360533484883490018546581268310546875}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueLen{4530}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueMaxFloat{27}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueMeanFloat{5.51589403973509906364824928459711372852325439453125}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueMedianFloat{1}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueMinFloat{1}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdLen{4530}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracLen{4530}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracMaxFloat{1.00000011920928955078125}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracMeanFloat{0.99559378463437753215004022422363050282001495361328125}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracMedianFloat{0.9716689845919608270463641019887290894985198974609375}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracMinFloat{0.943529903888702392578125}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueSequenceFracStdDevFloat{0.00592686780876558981512314261408391757868230342864990234375}
\def\SubcubicWithoutVocabSquaredGapMostBelowValueStdDevFloat{3.731890951335211870087960051023401319980621337890625}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchLen{4530}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchMaxFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchMeanFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchMedianFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchMinFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountBranchStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntLen{4530}
\def\SubcubicWithoutVocabSquaredInstructionCountIntMaxFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntMeanFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntMedianFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntMinFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountIntStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredInstructionCountLen{4530}
\def\SubcubicWithoutVocabSquaredInstructionCountMaxFloat{4879728}
\def\SubcubicWithoutVocabSquaredInstructionCountMeanFloat{3593129.3333333334885537624359130859375}
\def\SubcubicWithoutVocabSquaredInstructionCountMedianFloat{2864717}
\def\SubcubicWithoutVocabSquaredInstructionCountMinFloat{2864717}
\def\SubcubicWithoutVocabSquaredInstructionCountStdDevFloat{714919.26545083080418407917022705078125}
\def\SubcubicWithoutVocabSquaredMaxGapLen{4530}
\def\SubcubicWithoutVocabSquaredMaxGapMaxFloat{30}
\def\SubcubicWithoutVocabSquaredMaxGapMeanFloat{8.8136865342163357439630999579094350337982177734375}
\def\SubcubicWithoutVocabSquaredMaxGapMedianFloat{1}
\def\SubcubicWithoutVocabSquaredMaxGapMinFloat{1}
\def\SubcubicWithoutVocabSquaredMaxGapStdDevFloat{5.9526971169174114351108073606155812740325927734375}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyLen{4530}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyMaxFloat{0.73951073329633432162921735653071664273738861083984375}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyMeanFloat{0.1316274072079527124312647856640978716313838958740234375}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyMedianFloat{0.00000004477619510034710918767376810860347813303405928309075534343719482421875}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyMinFloat{0.0000000440661589167842275296013937295469542476666902075521647930145263671875}
\def\SubcubicWithoutVocabSquaredNormalizedAccuracyStdDevFloat{0.222624901415622800104898715289891697466373443603515625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMaxFloat{0.73887385241687297821044921875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMaxKey{6159}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMeanFloat{0.6284136571335476872945946524851024150848388671875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMeanKey{16069}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMedianFloat{0.476927766110747997085894667179672978818416595458984375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMedianKey{28090}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMinFloat{0.448228550143539905548095703125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyMinKey{1490}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedAccuracyStdDevFloat{0.05289101732648844589323999798580189235508441925048828125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxFloat{0.1415878655388951024018950874960864894092082977294921875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMaxKey{11598}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanFloat{0.11406609109473342389406980146304704248905181884765625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMeanKey{19488}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianFloat{0.090771424816921297828997694523422978818416595458984375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMedianKey{30463}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinFloat{0.08902535773813720354485923280662973411381244659423828125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracMinKey{1951}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesFracStdDevFloat{0.00999342711442975650815156996031873859465122222900390625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxFloat{152028813}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMaxKey{11598}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanFloat{122477532.70860926806926727294921875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMeanKey{19488}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianFloat{97465075.25}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMedianKey{30463}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinFloat{95590250}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesMinKey{1951}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedDroppedSequencesStdDevFloat{10730360.65785886161029338836669921875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxFloat{6530}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMaxKey{519}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanFloat{6496.5165562913907706388272345066070556640625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianFloat{6466}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinFloat{6466}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedEffectiveDimensionalityEstimateStdDevFloat{31.965597050006547164002768113277852535247802734375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxFloat{11.34843730926513671875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMaxKey{24202}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanFloat{5.53126487352990192647439471329562366008758544921875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMeanKey{1283}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianFloat{3.94751203060150146484375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMedianKey{6532}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinFloat{3.858226299285888671875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundMinKey{32374}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedErrUpperBoundStdDevFloat{1.3131957128378595189843736079637892544269561767578125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxFloat{10}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMaxKey{13036}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanFloat{6.4370860927152317998434227774851024150848388671875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianFloat{5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMedianKey{104}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinFloat{5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueMinKey{104}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxFloat{1.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMaxKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanFloat{1.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianFloat{1.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinFloat{1.5}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueNumStdStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxFloat{1}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMaxKey{13036}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanFloat{0.9919348280161421893552642359281890094280242919921875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMeanKey{19451}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianFloat{0.9755818843841552734375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMedianKey{11611}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinFloat{0.97523391246795643194644753748434595763683319091796875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracMinKey{22286}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueSequenceFracStdDevFloat{0.005465507854250783482952247283037650049664080142974853515625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedGapMostBelowValueStdDevFloat{0.75971551786489988078443502672598697245121002197265625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMaxKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountBranchStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMaxKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMeanKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountIntStdDevFloat{0}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMaxFloat{3681678}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMaxKey{5928}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMeanFloat{3036414.85430463589727878570556640625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMeanKey{519}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMedianFloat{2915149}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMedianKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMinFloat{2915149}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountMinKey{50}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedInstructionCountStdDevFloat{264854.7799246955546550452709197998046875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMaxFloat{21}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMaxKey{24173}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMeanFloat{13}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMeanKey{2743}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMedianFloat{8}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMedianKey{6159}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMinFloat{8}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapMinKey{6159}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedMaxGapStdDevFloat{3.012116810835729463491361457272432744503021240234375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxFloat{0.73951073329633432162921735653071664273738861083984375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMaxKey{6159}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanFloat{0.62898558894671052765801277928403578698635101318359375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMeanKey{6589}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianFloat{0.47971102572393864438282662376877851784229278564453125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMedianKey{12552}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinFloat{0.44856684670357382938021828522323630750179290771484375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyMinKey{1490}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedNormalizedAccuracyStdDevFloat{0.052613537072433415320293903505444177426397800445556640625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxFloat{46.6924571990966796875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMaxKey{7884}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanFloat{44.76375394625379300350687117315828800201416015625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMeanKey{15043}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianFloat{42.6303670406341552734375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMedianKey{20294}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinFloat{42.583120822906494140625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeMinKey{20338}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofSearchTimeStdDevFloat{0.71642306767657737420762487090541981160640716552734375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeLen{151}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMaxFloat{2.2991282939910888671875}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMaxKey{4800}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMeanFloat{2.219771784662410762933859587064944207668304443359375}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMeanKey{12457}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMedianFloat{2.146164476871490478515625}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMedianKey{22261}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMinFloat{2.1422092914581298828125}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeMinKey{21598}
\def\SubcubicWithoutVocabSquaredOnlyBestAccBoundPerSeedProofTimeStdDevFloat{0.02928460812333964768949812196296988986432552337646484375}
\def\SubcubicWithoutVocabSquaredProofSearchTimeLen{4530}
\def\SubcubicWithoutVocabSquaredProofSearchTimeMaxFloat{46.852759838104248046875}
\def\SubcubicWithoutVocabSquaredProofSearchTimeMeanFloat{44.57711345954709969419127446599304676055908203125}
\def\SubcubicWithoutVocabSquaredProofSearchTimeMedianFloat{42.3629872667789442175489966757595539093017578125}
\def\SubcubicWithoutVocabSquaredProofSearchTimeMinFloat{42.007546901702880859375}
\def\SubcubicWithoutVocabSquaredProofSearchTimeStdDevFloat{0.7278673344767969677349128687637858092784881591796875}
\def\SubcubicWithoutVocabSquaredProofTimeLen{4530}
\def\SubcubicWithoutVocabSquaredProofTimeMaxFloat{2.6413619518280029296875}
\def\SubcubicWithoutVocabSquaredProofTimeMeanFloat{2.208144986340015325509966714889742434024810791015625}
\def\SubcubicWithoutVocabSquaredProofTimeMedianFloat{2.130373656749725341796875}
\def\SubcubicWithoutVocabSquaredProofTimeMinFloat{2.1171014308929443359375}
\def\SubcubicWithoutVocabSquaredProofTimeStdDevFloat{0.0321930554120032075271495841661817394196987152099609375}
\def\TrainAccuracyLen{151}
\def\TrainAccuracyMaxFloat{0.9998333333333333516890206738025881350040435791015625}
\def\TrainAccuracyMaxKey{11598}
\def\TrainAccuracyMeanFloat{0.9988097578642383123082026941119693219661712646484375}
\def\TrainAccuracyMeanKey{27484}
\def\TrainAccuracyMedianFloat{0.9815944010416666198892698957934044301509857177734375}
\def\TrainAccuracyMedianKey{28090}
\def\TrainAccuracyMinFloat{0.97726822916666666873908297930029220879077911376953125}
\def\TrainAccuracyMinKey{13036}
\def\TrainAccuracyStdDevFloat{0.00250043641111774746221829701653405209071934223175048828125}
\def\TrainLossLen{151}
\def\TrainLossMaxFloat{0.1336393639458692550459062431400525383651256561279296875}
\def\TrainLossMaxKey{13036}
\def\TrainLossMeanFloat{0.005911443981539738108665904547933678259141743183135986328125}
\def\TrainLossMeanKey{2345}
\def\TrainLossMedianFloat{0.00155097019068246790192422412957284905132837593555450439453125}
\def\TrainLossMedianKey{14929}
\def\TrainLossMinFloat{0.0015016300991167858512598254350223214714787900447845458984375}
\def\TrainLossMinKey{23367}
\def\TrainLossStdDevFloat{0.01472506209576279583017832663927038083784282207489013671875}
\def\UpperWhiskerCrosshatchPercentileFloat{0.91132822467382401665503266485757194459438323974609375}
\def\UpperWhiskerTopEndPercentileFloat{0.97848760463080519667045109599712304770946502685546875}
\def\WEkkPerpFirstSingularLen{151}
\def\WEkkPerpFirstSingularMaxFloat{4.03815174102783203125}
\def\WEkkPerpFirstSingularMaxKey{8721}
\def\WEkkPerpFirstSingularMeanFloat{3.704933665446098256524010139401070773601531982421875}
\def\WEkkPerpFirstSingularMeanKey{2773}
\def\WEkkPerpFirstSingularMedianFloat{3.398107826709747314453125}
\def\WEkkPerpFirstSingularMedianKey{30371}
\def\WEkkPerpFirstSingularMinFloat{3.377728939056396484375}
\def\WEkkPerpFirstSingularMinKey{3284}
\def\WEkkPerpFirstSingularStdDevFloat{0.128107958562660384504994226517737843096256256103515625}
\def\WEkkPerpFroNormLen{151}
\def\WEkkPerpFroNormMaxFloat{10.03392791748046875}
\def\WEkkPerpFroNormMaxKey{27584}
\def\WEkkPerpFroNormMeanFloat{9.5177879965068488132828861125744879245758056640625}
\def\WEkkPerpFroNormMeanKey{11130}
\def\WEkkPerpFroNormMedianFloat{9.1663553714752197265625}
\def\WEkkPerpFroNormMedianKey{3284}
\def\WEkkPerpFroNormMinFloat{9.1344127655029296875}
\def\WEkkPerpFroNormMinKey{30371}
\def\WEkkPerpFroNormStdDevFloat{0.1736247061329504182136673762215650640428066253662109375}
\def\WEqqPerpFirstSingularLen{151}
\def\WEqqPerpFirstSingularMaxFloat{4.04321193695068359375}
\def\WEqqPerpFirstSingularMaxKey{8721}
\def\WEqqPerpFirstSingularMeanFloat{3.716172756738220783745418884791433811187744140625}
\def\WEqqPerpFirstSingularMeanKey{13293}
\def\WEqqPerpFirstSingularMedianFloat{3.415876686573028564453125}
\def\WEqqPerpFirstSingularMedianKey{30371}
\def\WEqqPerpFirstSingularMinFloat{3.375730991363525390625}
\def\WEqqPerpFirstSingularMinKey{3284}
\def\WEqqPerpFirstSingularStdDevFloat{0.127884325743118865137404327469994314014911651611328125}
\def\WEqqPerpFroNormLen{151}
\def\WEqqPerpFroNormMaxFloat{10.16388607025146484375}
\def\WEqqPerpFroNormMaxKey{28716}
\def\WEqqPerpFroNormMeanFloat{9.616969834889797397181609994731843471527099609375}
\def\WEqqPerpFroNormMeanKey{20976}
\def\WEqqPerpFroNormMedianFloat{9.261005878448486328125}
\def\WEqqPerpFroNormMedianKey{3284}
\def\WEqqPerpFroNormMinFloat{9.25788593292236328125}
\def\WEqqPerpFroNormMinKey{28090}
\def\WEqqPerpFroNormStdDevFloat{0.1705415063144830323249578896138700656592845916748046875}
\def\WKkPerpFirstSingularLen{151}
\def\WKkPerpFirstSingularMaxFloat{1.9113070964813232421875}
\def\WKkPerpFirstSingularMaxKey{6082}
\def\WKkPerpFirstSingularMeanFloat{1.4901907144003356808781290965271182358264923095703125}
\def\WKkPerpFirstSingularMeanKey{29725}
\def\WKkPerpFirstSingularMedianFloat{1.33571898937225341796875}
\def\WKkPerpFirstSingularMedianKey{20294}
\def\WKkPerpFirstSingularMinFloat{1.30693280696868896484375}
\def\WKkPerpFirstSingularMinKey{1681}
\def\WKkPerpFirstSingularStdDevFloat{0.08181575788105514834835929605105775408446788787841796875}
\def\WKkPerpFroNormLen{151}
\def\WKkPerpFroNormMaxFloat{4.63403797149658203125}
\def\WKkPerpFroNormMaxKey{14095}
\def\WKkPerpFroNormMeanFloat{4.3179352299267090842249672277830541133880615234375}
\def\WKkPerpFroNormMeanKey{28716}
\def\WKkPerpFroNormMedianFloat{4.05663394927978515625}
\def\WKkPerpFroNormMedianKey{20294}
\def\WKkPerpFroNormMinFloat{4.056191921234130859375}
\def\WKkPerpFroNormMinKey{6532}
\def\WKkPerpFroNormStdDevFloat{0.10560281405008430100078697932985960505902767181396484375}
\def\WQqPerpFirstSingularLen{151}
\def\WQqPerpFirstSingularMaxFloat{1.67036521434783935546875}
\def\WQqPerpFirstSingularMaxKey{27484}
\def\WQqPerpFirstSingularMeanFloat{1.515867531694323755431241806945763528347015380859375}
\def\WQqPerpFirstSingularMeanKey{8048}
\def\WQqPerpFirstSingularMedianFloat{1.3748886585235595703125}
\def\WQqPerpFirstSingularMedianKey{27300}
\def\WQqPerpFirstSingularMinFloat{1.36820209026336669921875}
\def\WQqPerpFirstSingularMinKey{6155}
\def\WQqPerpFirstSingularStdDevFloat{0.06638575194204558715949104907849687151610851287841796875}
\def\WQqPerpFroNormLen{151}
\def\WQqPerpFroNormMaxFloat{4.62363338470458984375}
\def\WQqPerpFroNormMaxKey{25516}
\def\WQqPerpFroNormMeanFloat{4.387457370758056640625}
\def\WQqPerpFroNormMeanKey{7238}
\def\WQqPerpFroNormMedianFloat{4.17933332920074462890625}
\def\WQqPerpFroNormMedianKey{8745}
\def\WQqPerpFroNormMinFloat{4.171676158905029296875}
\def\WQqPerpFroNormMinKey{13716}
\def\WQqPerpFroNormStdDevFloat{0.09454317097773969058582821389791206456720829010009765625}


==> images/mech_interp_of_model.tex <==
%% Creator: Inkscape 1.1 (c68e22c387, 2021-05-23), www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'mech_interp_of_model_for_tex.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%%
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{337.5bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.66666667)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{mech_interp_of_model_for_tex.pdf}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{mech_interp_of_model_for_tex.pdf}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{mech_interp_of_model_for_tex.pdf}}%
    \put(0,0){\includegraphics[width=\unitlength,page=4]{mech_interp_of_model_for_tex.pdf}}%
    \put(0,0){\includegraphics[width=\unitlength,page=5]{mech_interp_of_model_for_tex.pdf}}%
    \put(0,0){\includegraphics[width=\unitlength,page=6]{mech_interp_of_model_for_tex.pdf}}%
    \put(0,0){\includegraphics[width=\unitlength,page=7]{mech_interp_of_model_for_tex.pdf}}%
    \put(0.29111111,0.02369331){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}{Input}\end{tabular}}}}%
    \put(0.29111111,0.60147022){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}{Logits}\end{tabular}}}}%
    \put(0.53457634,0.606684){\color[rgb]{0,0,0}\makebox(0,0)[ct]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}$(\Logits_0, \Logits_1, \ldots, \Logits_{63})$\end{tabular}}}}%
    \put(0.48304223,0.47608178){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}{Unembed}\end{tabular}}}}%
    % \put(0.49500888,0.14252445){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Embed\end{tabular}}}}%
    \put(0.49827779,0.14497111){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}{Embed}\end{tabular}}}}%
    \put(0.42194444,0.30274889){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}{OV}\end{tabular}}}}%
    \put(0.52107778,0.30274889){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}{QK}\end{tabular}}}}%
    \put(0.43320889,0.02668443){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\Token[0]\end{tabular}}}}%
    \put(0.49987556,0.02668443){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\Token[1]\end{tabular}}}}%
    \put(0.56209778,0.02668443){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\Token[2]\end{tabular}}}}%
    \put(0.63320889,0.02668443){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\Token[3]\end{tabular}}}}%
    \put(0.73833386,0.19822001){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}Direct path \\ “does nothing”\end{tabular}}}}%
    \put(0.02647578,0.25155334){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}OV Circuit performs \\ low-rank copying\end{tabular}}}}%
    \put(0.03548622,0.43821999){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}QK Circuit attends \\ to larger tokens more\end{tabular}}}}%
  \end{picture}%
\endgroup%

